Relaxed virtual memory in Armv8-A (extended version)

Virtual memory is an essential mechanism for enforcing security boundaries, but its relaxed-memory concurrency semantics has not previously been investigated in detail. The concurrent systems code managing virtual memory has been left on an entirely informal basis, and OS and hypervisor verification has had to make major simplifying assumptions. We explore the design space for relaxed virtual memory semantics in the Armv8-A architecture, to support future system-software verification. We identify many design questions, in discussion with Arm; develop a test suite, including use cases from the pKVM production hypervisor under development by Google; delimit the design space with axiomatic-style concurrency models; prove that under simple stable configurations our architectural model collapses to previous "user" models; develop tooling to compute allowed behaviours in the model integrated with the full Armv8-A ISA semantics; and develop a hardware test harness. This lays out some of the main issues in relaxed virtual memory bringing these security-critical systems phenomena into the domain of programming-language semantics and verification with foundational architecture semantics. This document is an extended version of a paper in ESOP 2022, with additional explanation and examples in the main body, and appendices detailing our litmus tests, models, proofs, and test results.

==> pkvm-tests.tex <==

\section{Virtual memory in the pKVM production hypervisor}\label{sec:tests}\label{sec:pkvm}%
%\section{Tests, including real-world pKVM examples}\label{sec:tests}
%
%
%
Protected KVM, or pKVM~\cite{pKVM-lwn,pKVM-linux-talk,pKVM-src}, is currently being developed by Google to provide a common hypervisor for Android, to provide improved compartmentalisation by a small trusted computing base (TCB) between the Linux kernel and other services.
%
pKVM is built as a component of Linux. During boot, the Linux kernel hands over control of EL2 to the pKVM code, which constructs a memory map for itself and a Stage~2 memory map to encapsulate the Linux kernel. The Linux kernel thereafter runs only at EL1 (managing EL1\&0 Stage~1 memory maps for itself and for user processes), as the \emph{principal guest}, also known as the \emph{host} (not to be confused with the host hardware).   Other services can run as other guests, which are protected from the kernel and vice versa.  The kernel remains responsible for scheduling, but context switching %, %other guest control,
and inter-guest communication is done by hypervisor calls to the pKVM code at EL2.
%
This gives us an ideal setting in which to examine the management of virtual memory by production code for Armv8-A relaxed-memory-concurrency, with both one and two stages of translation (for EL2 and EL1\&0 respectively).
%
The pKVM codebase is small, so it is feasible to examine all uses of TLB management, and we benefit from discussions with
%extensive explanations from
the pKVM development team.
We have manually abstracted the main pKVM relaxed-virtual-memory scenarios into \numberOfpKVMTests{} tests.

%We describe the main use-scenarios below, each of which we have manually abstracted into a litmus test.
%
% This is a manual process, so the tests are of course not guaranteed to be correct or complete representations of everything pKVM does, and
%pKVM is under active development, so its usages may change,
%but it is instructive nonetheless, and exercises much of the Armv8-A architecture and our semantics. 

% Google are currently building a new hypervisor
% called \emph{protected KVM} (or \emph{pKVM} for short).
% 
% 
% intended to run above android and provide memory isolation between guests.
% 
% \subsection{pKVM Overview}\label{sec:pkvm:subsec:overview}
% \paragraph{pKVM architecture}
% pKVM is desigend to have a principle guest,
% the \emph{host} guest.
% The host runs android/linux and directly communicates with the hypervisor to manage the other guests and perform scheduling
% but is not allowed to directly access any of the memory of those other guests.
% 
% To do this the hypervisor sets up the initial EL2 state,
% including installing itself in the EL2 vector table.
% Once this is done,
% pKVM switches to the host and only runs when certain events happen in the system:
% a guest accessing memory it was not allowed to,
% or the principal guest performing hypercalls to communicate with the hypervisor.
% 
% KVM controls a set of virtual CPUs (or \emph{vcpu}s).
% Each \cc{vcpu} belongs to a virtual machine (or \emph{VM}).
% The principal guest at EL1 performs scheduling and requests pKVM
% to perform the necessary TLB maintenance
% and to actually do the context switch from one vCPU to another.


%\paragraph{Host interaction with hypervisor}
%The Linux kernel can coordinate with the hypervisor to perform various tasks:
%switching to other guests, performing various cache and TLB maintenance operations,
%creating new mappings, and various other hypervisor-related tasks.
%To do this,
%the host  executes an \asm{HVC} (or ``hypervisor-call'') instruction,
%and the hypervisor then dispatches on register values to perform various actions.
%
%Currently pKVM does not have the final complete list of actions,
%but t

To give a flavour for these we will explore just a few of the most fundamental for
hypervisor control of translation tables:
\cc{__pkvm_init} performs first-time per-CPU initialisation of pKVM,
which includes setting up the \cc{vmemmap},
a large array storing a struct entry for each physical page in memory
with ownership information;
\cc{__kvm_vcpu_run} switches to a different guest;
\cc{__kvm_flush_vm_context} flushes all entries in all TLB caches that relate to Stage~1 translations;
\cc{__kvm_tlb_flush_vmid_ipa} flushes entries in caches that relate to a particular guest for a given address;
\cc{__kvm_tlb_flush_vmid} flushes all entries in caches that relate to a particular guest;
\cc{__kvm_flush_cpu_context} flushes all entries in caches at EL1 for a given guest;
\cc{__pkvm_cpu_set_vector} sets the vector base address for handling exceptions;
\cc{__pkvm_create_mappings} creates entries in the Stage~1 page table that pKVM uses when it executes;
% PS: just skip? 
%\cc{__pkvm_create_private_mapping} also creates entries in the Stage~1 pagetable that pKVM uses when it executes,
%but putting virtual addresses in a private part of the address space (?);
and
\cc{__pkvm_prot_finalize} which enables Stage 2 translations during boot.

%%   See the \TODO{appendix} for a full list of these hypercalls and derived tests,
%%   but to give a flavour we will explore just one (\cc{__kvm_vcpu_run}) in detail in \S\ref{simpletest}.


%%   \paragraph{Guest interaction with hypervisor}
%%   If a guest attempts to access memory that is currently unmapped,
%%   either because the guest does not have permission to access that physical location
%%   or because the hypervisor is currently performing maintenance on that region
%%   (and so permission has been transiently removed during break-before-make),
%%   an exception is taken to EL2 which pKVM has to handle.
%%   %
%%   The pKVM implementation does not yet have support for real guests; 
%%   instead it has a temporary setup where pages are allocated on-demand as
%%   the host tries to read them.
%%   %
%%   This continues until memory runs out,
%%   at which point pKVM revokes all previously allocated pages and starts from the beginning.
%%   %
%%   This is not how the final hypervisor would work
%%   but the underlying operations to add, remove, or update mappings
%%   are a close approximation to what the final code will do
%%   and gives us a simple, clean but `real' implementation to reason about.

In the remainder of this section we describe a selection of litmus tests
extracted from the current pKVM source code~\cite{pKVM-src} as of Dec~2021.

% We do not believe this selection of litmus tests is exhaustive,
% and we are looking for feedback on both potentially missing litmus tests
% in our scope and on the tests given below.

%\subsection{Switching to another guest}\label{simpletest}

\subsection{Switching to another guest}\label{simpletest}
The most basic task that pKVM is in charge of is the actual swapping from one vCPU's context to another
to execute a particular VM on the physical CPU.
Deciding \emph{when} and to \emph{which} vCPU to switch is done by the underlying host Linux guest.
pKVM's role is to safely save the current guest's state,
and load the EL1 state for the target vCPU,
and manage the Stage~2 translation tables for the vCPU's VM.

Aside from the fundamental shape of switching from one VM to another on the same core,
there are a few interesting cases to consider:
\begin{itemize}
  \item Switching from one vCPU in a VM to another vCPU in the same VM.
  \item Switching to a new vCPU, re-using a previous VMID.
  \item Re-using an old VMID with a concurrently executing vCPU on another core.
\end{itemize}

When the host guest Linux kernel wishes to perform the switch from one vCPU to another,
it writes to some general-purpose registers and then performs an \asm{HVC} instruction
(in this case, to call the \cc{\_\_kvm\_vcpu\_run} hypercall).

%%ifnotext Switching between guests (also known as \emph{VM}s) is done by the \cc{__kvm_vcpu_run} hypercall.
%%ifnotext %when requested by the host Linux guest.
%%ifnotext %
%%ifnotext When switching from one VM's vCPU to another,
%%ifnotext pKVM must take care to ensure that any remaining context of the previously running vCPU is cleaned up.
%%ifnotext %
%%ifnotext %The remainder of this section will explore litmus tests created to capture different scenarios
%%ifnotext %of switching vCPUs.  The supplementary materials contains the litmus tests in full,
%%ifnotext %and other pKVM scenarios.
%
\clearpage
\testPara{pKVM.vcpu\_run}
In the simplest case
where pKVM is just switching from one vCPU to another vCPU
in a different VM,
pKVM restores the per-CPU register state
and sets the \asm{VTTBR} with the new VMID.
So long as the two vCPUs are using disjoint VMIDs
%and no other vCPU is using those VMIDs,
there is no requirement for TLB maintenance.

This test, \cc{pKVM.vcpu\_run}, is below, %given below in full.
\begin{figure}[h]
%\centering
%\scalebox{0.9}{\input{tests/tex/vcpurun}}\\[2mm]
%\vspace*{-4mm}
\noindent\hspace*{-20mm}\scalebox{0.9}{\input{tests/tex/vcpurun-hand}}%\\[2mm]
%\vspace*{-4mm}
\end{figure}
%The test is
typeset (lightly hand-edited) from the TOML input format of our Isla tool (\S\ref{isla}).
%
%
Here there is a single physical CPU, initially running a virtual machine VM1, with VMID \texttt{0x0001}, at EL1.
%
The %\texttt{page\_table\_setup}
section on the left defines the initial and all potential states of the page tables, and any other memory state.   
This test sets up separate translation tables for pKVM at EL2 (which has just a single stage) and for two VMs (each with two stages, Stage 2 controlled by pKVM and Stage 1 controlled by the VM). 
%
pKVM's own mapping \texttt{hyp\_map} maps its code. 
%
VM1's own Stage~1 mapping \texttt{vm1\_stage1} maps virtual address \texttt{x} to \texttt{ipa1},
and the initial pKVM-managed Stage 2 mapping \texttt{vm1\_stage2} maps that \texttt{ipa1} to \texttt{pa1}, which implicitly initially holds 0.
%In the combination, \texttt{x} is mapped to \texttt{ipa1} and thence to \texttt{pa1}, which initially (implicitly) holds 0.
%
%In these, \texttt{x} is mapped to \texttt{ipa2} and thence to \texttt{pa2}, which intially holds 1.
%
These page tables are described concisely %and abstractly
by a small declarative language we developed, %but under the hood this
determining the page-table memory (here $\sim$30k)
required for the % detailed
Armv8-A page-table walks. % accesses embodied in our tool. Some tests update this dynamically. 


The %\texttt{[thread.0.reset]} block
top-right block gives the initial Thread~0 register values, including the various page-table base registers.
%
The bottom-right blocks give the code of the test. This starts running at EL2, as one can see from the \texttt{PSTATE.EL} register value. 
%
The key assembly lines are annotated with the pKVM source line numbers they correspond to.
%
To switch to run another virtual machine VM2, with VMID \texttt{0x0002}, on this same physical CPU, pKVM changes  \texttt{VTTBR\_EL2} to the new \texttt{vm2\_stage2} mapping and, as part of the context-switch register-file changes, restores \texttt{TTBR0\_EL1} to the VM2's own Stage~1 mapping \texttt{vm2\_stage1}.
%
The code then executes an \asm{ERET} (``exception-return'') instruction to return to EL1, and then tries to read \texttt{x}.
%
The test includes a final assertion %, not shown in this rendering, that might be allowed by a model or not, here
of the relaxed outcome
that register \texttt{x2=0}, which could occur
if the \texttt{ldr} translation used the old VM1 mapping instead of VM2's mapping.  In this case that should not be allowed.
%
%The %\texttt{[section.thread0\_el2\_handler]} gives
%Thread~0 exception-handler code detects cases in which (e.g.) one might see a mix of VM1 and VM2's Stage~1 and Stage~2 mappings, which should also be forbidden. 
%
%\TODO{The above mostly explains the format - we should actually explain the test, perhaps ideally with an isla-generated diagram.  That might all fit in the same figure, with care}
%$ 
%$ The following is the simplest case,
%$ switching from one vCPU to another,
%$ with different VMIDs,
%$ and no concurrently executing VMs.
%$ Isla reports the final outcome as forbidden.
%$ \TODO{BS: or it used to, it's now broken again...}
%$ We have a collection of isla-compatible tests for the other scenarios described here,
%$ for concurrently-executing vCPUs and switching from vCPUs in the same VM, and for 
%$ VMID changing.
%$ \TODO{BS: add appendix with all test toml?}


%\paragraph{Isla test}
%The test is typeset from the TOML input format of our Isla tool, which is discussed in \S\ref{isla}.
%
%
%Here there is a single physical CPU, initially running a virtual machine VM1, with VMID \texttt{0x0001}, at EL1.
%
%% 
%% Stage 1 controlled by the VM). 
%% 
%% 
%% 
%% 
%% 
%% 
%% 
%% age2} mapping and, as part of the context-switch register-file changes, sets \texttt{TTBR0\_EL1} to the VM2's own Stage~1 mapping \texttt{vm2\_stage1}.
%% 
%% 
%% the main code of the test. This starts running at EL2, as one can see from the \texttt{PSTATE.EL} register value. 
%% 
%% 
%% 
%% 
%% 
%% 1 mapping instead of the current VM2 mapping.  In this case that should not be allowed.
%% 
%%  and Stage~2 mappings, which should also be forbidden. 
% 
% Tests in this format have 3 main sections:
% the \emph{page\_table\_setup} section, which describes the initial and all potential states of the pagetables during the test
% which is described more in \S\TODO{ref to isla section};
% the \emph{thread} sections which contain the code and initial register states;
% and,
% the \emph{final} section which describes the final condition to look for.
% 
% 
% Thread~0 then switches the guest's EL1 register state,
% including its own TTBR,
% to the state for VM2's vCPU.
% It then updates the VTTBR to point to the Stage~2 tables for VM2,
% before performing an exception return which jumps
% into the vCPU's own code (here located after label \asm{L0}).
% 
% The final condition asks whether the vCPU can see the old VM's mappings,
% and isla says forbidden for this test.

%%ifexp \ifexpanded
%%ifexp \clearpage
%%ifexp \testPara{pKVM.vcpu\_run.update\_vmid}
%%ifexp 
%%ifexp Since pKVM's host linux kernel is responsible for all scheduling,
%%ifexp it is responsible for the selection of VMIDs.
%%ifexp Typically each VM is given its own VMID,
%%ifexp and all vCPUs within that VM share that VMID.
%%ifexp %
%%ifexp By giving distinct VMs different VMIDs the host linux kernel
%%ifexp can switch between vCPUs in different VMs without requiring TLB maintenance,
%%ifexp as was seen in the previous test.
%%ifexp %
%%ifexp Eventually the host kernel runs out of VMIDs to allocate,
%%ifexp either from the naive incremental-allocation or because the
%%ifexp number of VMs is larger than the available VMID space
%%ifexp (8 or 16 bits in the worst case).
%%ifexp %
%%ifexp Currently pKVM's host linux kernel will simply revoke all previously allocated VMIDs
%%ifexp and when pKVM goes to switch to a vCPU for a VM without an allocated VMID it will be allocated there and then.
%%ifexp 
%%ifexp 
%%ifexp The \TEST{pKVM.vcpu\_run.update\_vmid} test is the simplest case where
%%ifexp the new vCPU is the only vCPU of that VM that is running and no other physical CPUs are executing.
%%ifexp %
%%ifexp Here we have two VMs and their associated tables in the initial state:
%%ifexp \herd{vm1\_stage2} is the root of the Stage~2 table for the first VM,
%%ifexp and \herd{vm2\_stage2} is the root of the Stage~2 table for the second VM.
%%ifexp Initially the \asm{VTTBR} points to VM1's table,
%%ifexp with VMID 1.
%%ifexp %
%%ifexp When switching to VM2's table,
%%ifexp with the same VMID,
%%ifexp the host linux kernel begins a sequence of calls to the hypervisor:
%%ifexp first it must flush the CPU context,
%%ifexp to make sure any old cached translations for the old VMID are removed.
%%ifexp From there, pKVM can perform the switch to the new vCPU by restoring the EL1 system register
%%ifexp state,
%%ifexp then pointing the \asm{VTTBR} to the new table with the new ASID,
%%ifexp before doing an exception-return to the guest.
%%ifexp If the guest then accesses a location it should be guaranteed to use the
%%ifexp new Stage~2 mapping with its own Stage~1 tables.
%%ifexp %
%%ifexp Figure~\ref{fig:vcpurunupdatevmid_code} contains the code listing and initial conditions for this test;
%%ifexp execution begins at EL2 with \cc{vm1}'s vCPU state, with VMID 1.
%%ifexp The test performs the pKVM \cc{vcpu\_run} sequence to clean up the TLB,
%%ifexp switch to \cc{vm2}'s EL1 state and then switching to \cc{vm2}'s Stage~2 mapping
%%ifexp with VMID 1 (the same as what \cc{vm1} had been using)
%%ifexp before returning to the guest.
%%ifexp The test then asserts that the guest's access uses \cc{vm2}'s own restored Stage~1 translation tables,
%%ifexp and does not see the old Stage~2 entries of \cc{vm1}.
%%ifexp 
%%ifexp Note that this test \emph{begins} with TLB invalidation.
%%ifexp To really capture the full sequence that is microarchitecturally interesting
%%ifexp the test should really begin from execution at EL1 inside the guest
%%ifexp allowing Stage~2 TLB fills.
%%ifexp The test beginning at EL2 from a clean machine state would not give the TLB time to
%%ifexp actually fill with stale entries from \cc{vm1}'s Stage~2 translation tables
%%ifexp in an operational model.
%%ifexp %
%%ifexp Also note that currently Isla does not produce candidates with re-ordering of system register reads,
%%ifexp and so there are no `bad' candidate executions to show from the Isla-generated executions currently.
%%ifexp This is work-in-progress to find the correct semantics for such re-orderings.
%%ifexp 
%%ifexp %\TODO{The above refers to event IDs, but we're not yet giving an execution diagram, or including the IDs in comments in the test code}
%%ifexp %\TODO{Perhaps these tests should start from EL1}?
%%ifexp 
%%ifexp \ifexpanded
%%ifexp \begin{figure}
%%ifexp   \centering
%%ifexp   \scalebox{0.8}{\input{tests/tex/vcpurunupdatevmid}}
%%ifexp \caption{}\label{fig:vcpurunupdatevmid_code}
%%ifexp \end{figure}
%%ifexp \fi
%%ifexp \else
Other tests capture more elaborate scenarios. For example,
currently the host kernel manages VMIDs and assigns each VM its own VMID.
%Currently the VMIDs are managed by the host kernel,
%which assigns each VM its own VMID.
If the host runs out of VMIDs to allocate to new vCPUs,
it currently revokes all previously allocated VMIDs and re-allocates from the beginning, during which
%
%When revoking the old VMIDs
pKVM has to ensure that any old vCPUs' translations using that VMID are expelled from any TLBs (\cc{pKVM.vcpu\_run.update\_vmid}).
%This is captured by the \cc{pKVM.vcpu\_run.update\_vmid} test which stops one guest and switches to another
%re-using the same VMID.
%%\fi ifex
%
%%ifexp \ifexpanded
%%ifexp \clearpage
%%ifexp \testPara{pKVM.vcpu\_run.update\_vmid.concurrent}
%%ifexp 
%%ifexp The concurrent case of the previous \TEST{pKVM.vcpu\_run.update\_vmid} test is critical:
%%ifexp while switching from one vCPU to another on the same core is typically a
%%ifexp %very
%%ifexp thread-local event
%%ifexp care must be taken in the case where another CPU is executing a VM whose current VMID should be revoked, as in Fig.~\ref{fig:vcpurunupdatevmidconcurrent}.
%%ifexp 
%%ifexp In this case pKVM must interrupt the other core so that it is not concurrently executing while the new VMIDs are being
%%ifexp allocated, otherwise it might pollute the address space of the VM that gets allocated that VMID.
%%ifexp 
%%ifexp pKVM does this by sending an IPI to all the other cores to break out of their current vCPUs.
%%ifexp When it does this each CPU will attempt to switch back to the host and in doing so
%%ifexp will be forced to take a lock when acquiring the VMID to use.
%%ifexp %
%%ifexp This lock prevents those CPUs from executing at EL1,
%%ifexp and the architecture prevents the hardware from performing TLB fills while at EL2.
%%ifexp These guarantees ensure that while VMIDs are being re-allocated and TLB maintenance performed
%%ifexp on the original core,
%%ifexp no stale entries can find their way back into the TLB.
%%ifexp 
%%ifexp However,
%%ifexp our understanding of this code leaves a question.
%%ifexp The \cc{tlb.c} file in pKVM uses a \asm{DSB ISHST} to order
%%ifexp from po-previous stores to the translation tables before the TLB maintenance,
%%ifexp but this would not wait for any reads coming back from the IPI message pass.
%%ifexp We assume there must be some other synchronization between the IPI receive on the
%%ifexp core invalidating the VMIDs and the invalidation itself
%%ifexp but we do not know where in pKVM it can be found (if it exists at all).
%%ifexp %
%%ifexp Work needs to be done here to try match the compiled pKVM and all the barriers
%%ifexp with our understanding of the source materials.
%%ifexp 
%%ifexp \ifexpanded
%%ifexp \begin{figure}
%%ifexp \noindent\hspace*{-19mm}
%%ifexp %  \scalebox{0.8}{\input{tests/tex/vcpurunupdatevmidconcurrent}}
%%ifexp   \resizebox*{!}{0.95\textheight}{\input{tests/tex/vcpurunupdatevmidconcurrent}}
%%ifexp \caption{}\label{fig:vcpurunupdatevmidconcurrent}
%%ifexp \end{figure}
%%ifexp \fi
%%ifexp \else
If there is a concurrently executing vCPU using that VMID,
%we get a variation of the test named \cc{pKVM.vcpu\_run.update\_vmid.concurrent}.
%Here care must be taken  to ensure
that vCPU must be paused
until after the new VMID generation (and hence any required TLB maintenance),
%has happened,
before continuing
with the freshly allocated VMID (\cc{pKVM.vcpu\_run.update\_vmid.concurrent}).
%
%Currently pKVM ensures no other vCPUs are running through a combination of an inter-processor interrupt (IPI)
%and an internal lock that prevents the vCPUs from running until the new VMID generation has allocated.
%While we do not model IPIs, this behaviour can be approximated with a message pass and a hypervisor call.
%\fi %ifexp

%Because the EL1 register state is supposed to be per-CPU,
%%ifexp \ifexpanded
%%ifexp \clearpage
%%ifexp \testPara{pKVM.vcpu\_run.same\_vm}
%%ifexp \fi

%In order
For another example, for pKVM to maintain the illusion that each vCPU is on its own core,
the per-core state must be cleaned between running different vCPUs,
including ensuring that translations for one vCPU are not cached and visible
to another, even if they happen to be in the same VM (and using the same VMID) (\cc{pKVM.vcpu\_run.same\_vm}).
%
%To capture this the \cc{pKVM.vcpu\_run.same\_vm} test
%switches from one vCPU to another vCPU on the same core within the same VM.
%
%At EL2 pKVM flushes local caches before dropping back to EL1 in the new guest;
%we assert that translations in the new guest do not see translations from the old guest.

%%ifexp \ifexpanded
%%ifexp \begin{figure}
%%ifexp   \noindent\hspace*{-19mm}
%%ifexp     \resizebox*{!}{0.95\textheight}{\input{tests/tex/vcpurunsamevm}}
%%ifexp   \caption{}\label{fig:vcpurunsamevm}
%%ifexp \end{figure}
%%ifexp \fi

%fig:pkvm_test was here in submitted version

% \begin{tabular}{@{}c@{\hspace*{2mm}}c@{}}
% 
% 
% \begin{lstlisting}[keepspaces=true]
% arch = "AArch64"
% name = "pKVM.vcpu_run"
% symbolic = ["x"]
% 
% page_table_setup = """
% option default_tables = false;
% 
% physical pa1 pa2;
% intermediate ipa1 ipa2;
% 
% s1table hyp_map 0x200000 {
%     identity 0x1000 with code;
%     x |-> invalid;
% }
% 
% s2table vm1_stage2 0x240000  {
%     identity pa_to_ipa(0x1000) with code;
%     ipa1 |-> pa1;
%     ipa2 |-> invalid;
% 
% 
%     s1table vm1_stage1 0x2C0000 {
%         identity pa_to_va(0x1000) with code;
%         x |-> ipa1;
%     }
% }
% 
% s2table vm2_stage2 0x280000  {
%     identity pa_to_ipa(0x1000) with code;
%     ipa1 |-> invalid;
%     ipa2 |-> pa2;
% 
%     s1table vm2_stage1 0x300000 {
%         identity pa_to_va(0x1000) with code;
%         x |-> ipa2;
%     }
% }
% 
% 
% *pa2 = 1;
% """
% \end{lstlisting}
% &
% \begin{lstlisting}[keepspaces=true]
% [thread.0]
% code = """
%     msr ttbr0_el1, x0  // kvm/hyp/sysreg-sr.h:96
%     msr vttbr_el2, x1  // include/asm/kvm_mmu.h:276
%     eret // kvm/hyp/nvhe/host.S
% L0:
%     ldr x2, [x3] // in guest
% """
% 
% [thread.0.reset]
% R0 = "ttbr(asid=0x00, base=vm2_stage1)"
% R1 = "ttbr(vmid=0x0002, base=vm2_stage2)"
% 
% TTBR0_EL2 = "ttbr(asid=0x00, base=hyp_map)"
% VTTBR_EL2 = "ttbr(vmid=0x0001, base=vm1_stage2)"
% TTBR0_EL1 = "ttbr(asid=0x00, base=vm1_stage1)"
% 
% R3 = "x"
% VBAR_EL2 = "extz(0x1000, 64)"
% 
% "PSTATE.EL" = "0b10"
% 
% # return to EL1h at L0
% SPSR_EL2 = "extz(0b00101, 64)"
% ELR_EL2 = "extz(L0:, 64)"
% 
% [section.thread0_el2_handler]
% address = "0x1400" # 0x400 - Lower Exception Level
% code = """
%     mov x2, #0
% """
% 
% [final]
% assertion = "0:X2 = 0"
% \end{lstlisting}
%
%\end{tabular}
%
%}


%%ifexp2 \ifexpanded
%%ifexp2 \clearpage
%%ifexp2 \subsection{Data Aborts}
%%ifexp2 
%%ifexp2 As mentioned earlier,
%%ifexp2 a vCPU accessing a location that it does not have permissions for
%%ifexp2 or which is not mapped,
%%ifexp2 results in an Abort which is handled at EL2.
%%ifexp2 
%%ifexp2 
%%ifexp2 \testPara{pKVM.host\_handle\_trap.stage2\_idmap.l3}
%%ifexp2 %
%%ifexp2 If the vCPU accesses a location which is currently un-mapped,
%%ifexp2 but should be mapped on-demand, then pKVM will make a new mapping
%%ifexp2 for that vCPU, install it into its VM's Stage~2 translation tables,
%%ifexp2 and return to the vCPU to re-try the access.
%%ifexp2 This action typically requires no TLB invalidation, as the previously unmapped entries
%%ifexp2 could not have been stored in any TLB.
%%ifexp2 
%%ifexp2 An added complexity here is that if pKVM wishes
%%ifexp2 to map only a single page then it \emph{must} install this mapping
%%ifexp2 with a Level~3 entry.
%%ifexp2 If the mapping is currently invalid at Level~2 or Level~1 then
%%ifexp2 care must be taken to not create entries out-of-order.
%%ifexp2 pKVM manages this by producing a fresh table of invalid entries first,
%%ifexp2 then installing that new table into the translation tables,
%%ifexp2 and recursing down until it reaches the level it needs to install the valid mapping at.
%%ifexp2 Otherwise, a concurrent translation could see the new table entries before
%%ifexp2 the leaf entries had been installed into the table.
%%ifexp2 
%%ifexp2 \ifexpanded
%%ifexp2 \begin{figure}
%%ifexp2   %  \centering
%%ifexp2   %  \scalebox{0.8}{
%%ifexp2     \noindent\hspace*{-19mm}
%%ifexp2   %  \scalebox{0.8}{\input{tests/tex/vcpurunupdatevmidconcurrent}}
%%ifexp2 %    \resizebox*{!}{0.95\textheight}
%%ifexp2 {\input{tests/tex/hosthandletrapstagetwoidmaplthree}}\
%%ifexp2   \caption{\TEST{pKVM.host\_handle\_trap.stage2\_idmap.l3}: code listing}\label{fig:hosthandletrapstagetwoidmaplthree_code}
%%ifexp2 \end{figure}
%%ifexp2 
%%ifexp2 \begin{figure}
%%ifexp2   \centering
%%ifexp2 %  \includegraphics[trim=10mm 0 0 0, clip,width=140mm,height=120mm]{tests/pKVM/pKVM.host_handle_trap.stage2_idmap.change_block_size_allow_7.pdf}
%%ifexp2 
%%ifexp2   \includegraphics[trim=10mm 0 0 0, clip,width=140mm,height=120mm]{tests/pKVM/pKVM_host_handle_trap_stage2_idmap_l3_allow_4.pdf}
%%ifexp2   \caption{\TEST{pKVM.host\_handle\_trap.stage2\_idmap.l3}: forbidden candidate execution}\label{fig:hosthandletrapstagetwoidmaplthree_exec}
%%ifexp2 \end{figure}
%%ifexp2 \fi
%%ifexp2 
%%ifexp2 \ifexpanded
%%ifexp2 \clearpage
%%ifexp2 \fi
%%ifexp2 \testPara{pKVM.host\_handle\_trap.stage2\_idmap.already\_exists}\label{test:pKVM.host_handle_trap.stage2_idmap.already_exists}
%%ifexp2 If the vCPU tries to access a location that is mapped but that it lacks the necessary permissions for,
%%ifexp2 then there may be an existing entry already mapping that location.
%%ifexp2 Here the process is much more delicate. 
%%ifexp2 Because another vCPU in the same VM may be concurrently accessing the same physical locations
%%ifexp2 mapped by the shared Stage~2 table,
%%ifexp2 pKVM cannot assume its own internal locks are sufficient to prevent race conditions.
%%ifexp2 Therefore this is one case where pKVM is \emph{required} to use the break-before-make sequence as described by
%%ifexp2 \S\ref{subsubsec:questions:tlb:bbm}.
%%ifexp2 
%%ifexp2 In the following code the initial state starts out with \cc{x} mapped at level 3, but without read permissions.
%%ifexp2 The first load will fault and pKVM will naturally map a writeable mapping on-demand,
%%ifexp2 following the break-before-make sequence invalidating the entry by writing zero (event \herd{b})
%%ifexp2 before writing a new valid descriptor (event \herd{m}).
%%ifexp2 After returning to the guest we ask whether loads of \cc{x} are allowed to fault at Stage~2.
%%ifexp2 
%%ifexp2 \ifexpanded
%%ifexp2 \begin{figure}
%%ifexp2   %  \centering
%%ifexp2   %  \scalebox{0.8}{
%%ifexp2     \noindent\hspace*{-19mm}
%%ifexp2     \resizebox*{!}{0.95\textheight}{\input{tests/tex/hosthandletrapstagetwoidmaplthreealreadyexists}}\
%%ifexp2     \caption{\TEST{pKVM.host\_handle\_trap.stage2\_idmap.l3.already\_exists}: code listing}\label{fig:hosthandletrapstagetwoidmaplthreealreadyexists_code}
%%ifexp2   \end{figure}
%%ifexp2 
%%ifexp2   \begin{figure}
%%ifexp2     \centering
%%ifexp2     \includegraphics[trim=10mm 0 0 0, clip,width=140mm,height=120mm]{tests/pKVM/pKVM_host_handle_trap_stage2_idmap_l3_already_exists_allow_5.pdf}
%%ifexp2     \caption{\TEST{pKVM.host\_handle\_trap.stage2\_idmap.l3.already\_exists}: forbidden candidate execution}\label{fig:hosthandletrapstagetwoidmaplthreealreadyexists_exec}
%%ifexp2   \end{figure}
%%ifexp2 \fi
%%ifexp2 
%%ifexp2 \ifexpanded
%%ifexp2 \clearpage
%%ifexp2 \fi
%%ifexp2 \testPara{pKVM.host\_handle\_trap.stage2\_idmap.change\_block\_size}
%%ifexp2 The complexity of the previous scenario is compounded by the fact that pKVM may wish to map a larger region
%%ifexp2 (higher in the table)
%%ifexp2 than is currently mapped, and without \asm{FEAT\_BBM} this adds extra break-before-make requirements.
%%ifexp2 
%%ifexp2 In general pKVM will itself perform a translation table walk. 
%%ifexp2 On the way down it will look for the entry to be replaced,
%%ifexp2 invalidate it, and perform TLB maintenance,
%%ifexp2 ensuring that all entries from old leaf entries below it are cleaned away,
%%ifexp2 but additionally that any old stale Stage~1 translations are invalidated,
%%ifexp2 before it replaces the entry.
%%ifexp2 
%%ifexp2 \ifexpanded
%%ifexp2 
%%ifexp2 Figures~\ref{fig:hosthandletrapstagetwoidmapchangeblocksize_code} and \ref{fig:hosthandletrapstagetwoidmapchangeblocksize_exec} contain the code listing and the interesting candidate execution diagram
%%ifexp2 (as generated by Isla).
%%ifexp2 We consider a scenario where there are two locations,
%%ifexp2 \cc{x} and \cc{y}
%%ifexp2 which are in the same 2~MiB region of memory
%%ifexp2 but are mapped by different Level~3 entries.
%%ifexp2 If the Level~3 table contains all valid entries except for
%%ifexp2 one entry for \cc{x},
%%ifexp2 then on updating the entry for \cc{x} to be valid,
%%ifexp2 if the host kernel maps the whole 2M region,
%%ifexp2 then pKVM will invalidate the 2M entry before
%%ifexp2 writing a new 2M block entry.
%%ifexp2 
%%ifexp2 This in effect `promotes' the set of 4K mappings into a single 2M mapping.
%%ifexp2 pKVM then frees the child table to be re-allocated later.
%%ifexp2 \TODO{BS: is there a concurrent test about re-using that free'd table in another thread?}.
%%ifexp2 
%%ifexp2 %Finally,
%%ifexp2 pKVM may want to \emph{remove} a mapping for an IPA.
%%ifexp2 This is very similar to the previously described break-before-make scenario,
%%ifexp2 but without the final make.
%%ifexp2 pKVM just has to ensure that the old IPA mapping is invalidated,
%%ifexp2 and the necessary TLB maintenance is performed.
%%ifexp2 We do not include this test at present.
%%ifexp2 
%%ifexp2 \ifexpanded
%%ifexp2 \begin{figure}
%%ifexp2 %  \centering
%%ifexp2 %  \scalebox{0.8}{
%%ifexp2   \noindent\hspace*{-19mm}
%%ifexp2 %  \scalebox{0.8}{\input{tests/tex/vcpurunupdatevmidconcurrent}}
%%ifexp2   \resizebox*{!}{0.95\textheight}{\input{tests/tex/hosthandletrapstagetwoidmapchangeblocksize}}\
%%ifexp2   \caption{\TEST{pKVM.host\_handle\_trap.stage2\_idmap.change\_block\_size}: code listing}\label{fig:hosthandletrapstagetwoidmapchangeblocksize_code}
%%ifexp2 \end{figure}
%%ifexp2 
%%ifexp2 \begin{figure}
%%ifexp2   \centering
%%ifexp2 %  \includegraphics[trim=10mm 0 0 0, clip,width=140mm,height=120mm]{tests/pKVM/pKVM.host_handle_trap.stage2_idmap.change_block_size_allow_7.pdf}
%%ifexp2   \includegraphics[trim=10mm 0 0 0, clip,width=140mm,height=120mm]{tests/pKVM/pKVM_host_handle_trap_stage2_idmap_change_block_size_allow_7.pdf}
%%ifexp2   \caption{\TEST{pKVM.host\_handle\_trap.stage2\_idmap.change\_block\_size}: forbidden candidate execution}\label{fig:hosthandletrapstagetwoidmapchangeblocksize_exec}
%%ifexp2 \end{figure}
%%ifexp2 \fi
%%ifexp2 
%%ifexp2 \ifexpanded
%%ifexp2 \clearpage
%%ifexp2 \fi
%%ifexp2 % \testPara{pKVM.host\_handle\_trap.stage2\_idmap.already\_exists.concurrent}
%%ifexp2 
%%ifexp2 % The case where the previous Test~\ref{test:pKVM.host_handle_trap.stage2_idmap.already_exists} \TEST{pKVM.host\_handle\_trap.stage2\_idmap.already\_exists} has a concurrently executing CPU
%%ifexp2 % in the same VM is an interesting one.
%%ifexp2 % Care must be taken to ensure that if that vCPU is accessing memory that is being re-mapped by another core that the break-before-make sequence was correctly
%%ifexp2 % followed as described in \S\ref{subsubsec:questions:tlb:bbm}.
%%ifexp2 
%%ifexp2 % pKVM's own locks prevent two attempts at mapping the same page to happen concurrently,
%%ifexp2 % so the only case we have to consider is that where one CPU updates the mapping while another
%%ifexp2 % concurrently accesses it.
%%ifexp2 
%%ifexp2 % \TODO{BS: diagram and stuff}
%%ifexp2 
%%ifexp2 % \fi
%%ifexp2 
%%ifexp2 % \clearpage
%%ifexp2 
%%ifexp2 
%%ifexp2 
%%ifexp2 % PS moved this to the end - logically it'd be nice at the start, but if we don't handle it, it's terrible to start with something we don't handle. And also nice to start with the one for which we give the concrete test.
%%ifexp2 \subsection{Initialisation}
%%ifexp2 
%%ifexp2 \ifexpanded
%%ifexp2 During execution,
%%ifexp2 and especially at initial start-up of pKVM,
%%ifexp2 it will be required to create its own Stage~1 translation tables.
%%ifexp2 
%%ifexp2 Currently this only happens on a single core,
%%ifexp2 so there are no interesting concurrent cases
%%ifexp2 (\TODO{is that true?}).
%%ifexp2 
%%ifexp2 In future, however, it is expected that pKVM may need to
%%ifexp2 dynamically map some parts of memory, as the hypervisor gains richer features.
%%ifexp2 %Especially, with any requirement for the hypervisor to interact directly with the guests
%%ifexp2 For example, it may need to map some shared page between guests, or between pKVM and a guest, in which to pass messages.
%%ifexp2 
%%ifexp2 \ifexpanded
%%ifexp2 \clearpage
%%ifexp2 \fi
%%ifexp2 \testPara{pKVM.switch\_to\_new\_table}
%%ifexp2 
%%ifexp2 When pKVM first starts it is using translation tables set up by Linux,
%%ifexp2 so one of the first things pKVM does is create its own tables and switch to them.
%%ifexp2 
%%ifexp2 Usually switching from using one translation table to another happens at a higher exception level
%%ifexp2 and then the new one is not used until the return to the lower exception level.
%%ifexp2 The current case
%%ifexp2  is more complicated as pKVM has to change its own translation tables
%%ifexp2 \emph{while it is executing}.
%%ifexp2 If pKVM only had to change the \asm{TTBR} then this would not be a problem,
%%ifexp2 but there are many system registers involved in configuring the translation tables
%%ifexp2 (the \asm{TCR}, \asm{MAIR}, and so on) and these registers cannot all be updated `atomically'.
%%ifexp2 
%%ifexp2 To maintain the atomicity pKVM switches the \asm{TTBR}
%%ifexp2 to a page of memory where the code it is executing is identity-mapped,
%%ifexp2 then it disables translation (disabling the MMU),
%%ifexp2 before updating all of the required system registers (including the new \asm{TTBR}),
%%ifexp2 before re-enabling the MMU.
%%ifexp2 
%%ifexp2 Figure~\ref{fig:switchtonewtable_code} contains the code for a litmus test
%%ifexp2 that tries to capture the core of this process.
%%ifexp2 This \TEST{pKVM.switch\_to\_new\_table} test is an EL2 Stage~1 test
%%ifexp2 with two tables, \cc{hyp\_pgtable} and \cc{new\_hyp\_pgtable} in memory.
%%ifexp2 The code disables the MMU (by writing to the appropriate field of the SCTLR),
%%ifexp2 invalidates all of the old cached TLB entries for EL2,
%%ifexp2 updates all the system registers (only the \asm{TTBR} is included here)
%%ifexp2 and then re-enables the MMU.
%%ifexp2 We check that the final load in the hypervisor after the switch has happened
%%ifexp2 reads using the new state.
%%ifexp2 
%%ifexp2 This test has been cut down for brevity to remove the writes of other system registers,
%%ifexp2 which would be present in a full execution of pKVM;
%%ifexp2 ideally we would have a test that included those too,
%%ifexp2 and a final state which ensured that the load used a translation using
%%ifexp2 all of the new register values.
%%ifexp2 \TODO{Perhaps we should write that test down too?}
%%ifexp2 
%%ifexp2 Note that the model presented in Section~\ref{sec:models}
%%ifexp2 does not currently contain axioms for when the MMU is disabled
%%ifexp2 but the semantics seem clear %to us
%%ifexp2 and we do not see any impediment in extending the model to handle it fully.
%%ifexp2 
%%ifexp2 \begin{figure}[h]
%%ifexp2   \centering
%%ifexp2   \scalebox{0.8}{\input{tests/tex/switchtonewtable}}
%%ifexp2 \caption{pKVM.switch\_to\_new\_table}\label{fig:switchtonewtable_code}
%%ifexp2 \end{figure}
%%ifexp2 
%%ifexp2 \ifexpanded
%%ifexp2 \clearpage
%%ifexp2 \fi
%%ifexp2 \testPara{pKVM.create\_hyp\_mappings.inv.l2}
%%ifexp2 
%%ifexp2 Constructing new translation tables is done incrementally,
%%ifexp2 starting from a single zero'd page of memory as the root table 
%%ifexp2 and then performing a manual translation table walk on insertion to locate an entry to insert into.
%%ifexp2 
%%ifexp2 In the case where there is no Level~3 table to install into,
%%ifexp2 pKVM first creates a Level~2 table and installs that,
%%ifexp2 before writing the new valid Level~3 entry.
%%ifexp2 To avoid break-before-make violations here,
%%ifexp2 pKVM always ensures the table is zeroed before
%%ifexp2 inserting it into the table.
%%ifexp2 
%%ifexp2 The \TEST{pKVM.create\_hyp\_mappings.inv.l2} test,
%%ifexp2 in Figure~\ref{fig:createhypmappingsinvltwo_code},
%%ifexp2 gives the case where pKVM is trying to create a new mapping for itself
%%ifexp2 for a 4K page block.
%%ifexp2 This block mapping \emph{must} be installed as a Level~3 entry,
%%ifexp2 as installing it any higher would end up mapping more than 4K of memory.
%%ifexp2 Initially \herd{x} is translated using an invalid Level~2 entry in \cc{hyp\_pgtable}.
%%ifexp2 The table \cc{hyp\_pgtable\_new} contains the new Level~3 table which starts life zeroed (all invalid);
%%ifexp2 The test then sets the Level~2 entry in \cc{hyp\_pgtable} to point to the new table,
%%ifexp2 and then updates the Level~3 (leaf) entry with a valid descriptor.
%%ifexp2 
%%ifexp2 Interestingly we note that pKVM sets these entries with a store-release;
%%ifexp2 although there seems no relaxed-virtual-memory reason why.
%%ifexp2 Given that pKVM is well locked it is not clear why making these writes store-releases helps.
%%ifexp2 % Presumably this is done just for sanity to ensure that concurrent accesses
%%ifexp2 % (both reading of the translation tables by pKVM itself and by other thread's MMUs)
%%ifexp2 % although in this case this is uncessary as both the initial level~2 entry and level~3 table
%%ifexp2 % are invalid (and the earlier allocation of the table is barriered).
%%ifexp2 % \TODO{the previous isn't sentences}
%%ifexp2 
%%ifexp2 \ifexpanded
%%ifexp2 \begin{figure}[h]\label{fig:createhypmappingsinvltwo_code}
%%ifexp2 %  \centering
%%ifexp2 \hspace*{-13mm}
%%ifexp2 \begin{tabular}{ll}
%%ifexp2   \scalebox{0.8}{\input{tests/tex/createhypmappingsinvltwo}}%
%%ifexp2   &%
%%ifexp2   % TODO: BS: this is really squished and ugly, but at least it fits.
%%ifexp2 %  \includegraphics[trim=10mm 0 0 0, clip,width=50mm,height=40mm]{tests/pKVM/pKVM.create_hyp_mappings.inv.l2_allow_3.pdf}
%%ifexp2   \includegraphics[trim=10mm 0 0 0, clip,width=50mm,height=40mm]{tests/pKVM/pKVM_create_hyp_mappings_inv_l2_allow_3.pdf}
%%ifexp2   \end{tabular}
%%ifexp2 \caption{\TEST{pKVM.create\_hyp\_mappings.inv.l2}: Code listing and (forbidden) candidate execution}\label{fig:createhypmappingsinvltwo_code}
%%ifexp2 \end{figure}
%%ifexp2 \fi
%%ifexp2 
%%ifexp2 \ifexpanded
%%ifexp2 \clearpage
%%ifexp2 \fi
%%ifexp2 \testPara{pKVM.create\_hyp\_mappings.inv.l3}
%%ifexp2 
%%ifexp2 pKVM can set entries at any level of the table
%%ifexp2 assuming they are initially invalid.
%%ifexp2 The following test is a variation on the previous,
%%ifexp2  where the Level~3 table is already created but contains an invalid entry at Level~3.
%%ifexp2 
%%ifexp2 As before we will map a 4K region and so it must go at Level~3.
%%ifexp2 
%%ifexp2 \ifexpanded
%%ifexp2 \begin{figure}[h]
%%ifexp2   \centering
%%ifexp2 \hspace*{-10mm}
%%ifexp2 \begin{tabular}{ll}
%%ifexp2   \scalebox{0.8}{\input{tests/tex/createhypmappingsinvlthree}}%
%%ifexp2   &%
%%ifexp2   % TODO: BS: this is really squished and ugly, but at least it fits.
%%ifexp2 %  \includegraphics[trim=10mm 0 0 0, clip,width=50mm,height=40mm]{tests/pKVM/pKVM.create_hyp_mappings.inv.l3_allow_2.pdf}
%%ifexp2   \includegraphics[trim=10mm 0 0 0, clip,width=50mm,height=40mm]{tests/pKVM/pKVM_create_hyp_mappings_inv_l3_allow_2.pdf}
%%ifexp2   \end{tabular}
%%ifexp2 \caption{\TEST{pKVM.create\_hyp\_mappings.inv.l3}: Code listing and (forbidden) candidate execution}\label{fig:createhypmappingsinvlthree_code}
%%ifexp2 \end{figure}
%%ifexp2 \fi
%%ifexp2 
%%ifexp2 \else
%%ifexp2 During boot, the Linux kernel asks pKVM to initialise itself, during which
%%ifexp2 it creates pagetables for its own future EL2 execution, and switches to them.
%%ifexp2 %
%%ifexp2 This first part of pKVM execution uses pagetables set up by Linux.
%%ifexp2 Creation of the new tables is just C-language data structure
%%ifexp2 manipulation, and the tables are not in use while this is happening.
%%ifexp2 To switch to running with the new tables, 
%%ifexp2 pKVM first jumps to a part of its binary which has been set up (by Linux) as an identity-mapped region, with  virtual and physical addresses coinciding.  Within that, 
%%ifexp2 it disables the MMU (by setting the \asm{M} bit of the \asm{SCTLR} to 0),
%%ifexp2 performs TLB maintenance to remove any old mappings, writes the new page-table base address and configuration values to the appropriate system registers, and 
%%ifexp2 switches the MMU back on.
%%ifexp2 Doing this with the MMU off ensures that the changes to the system registers required to update the translation happen atomically, 
%%ifexp2 and that translations cannot start using a partially-initialised state; the identity maps ensure that execution work correctly over the on/off transitions. 
%%ifexp2 
%%ifexp2 Note that currently our model does not capture the behaviour when the MMU is disabled, but it seems clear what the behaviour should be, 
%%ifexp2 as described in \S\ref{sec:questions:subsec:mmu_off},
%%ifexp2 and we are not aware of any challenges in handling it in the model and tooling. 
%%ifexp2 \fi
%%ifexp2 
%%ifexp2 \fi
%%ifexp2 \fi
%%ifexp2 \ifexpanded
%%ifexp2 \clearpage
%%ifexp2 \fi



%\section{Tests, including real-world pKVM examples}\label{sec:tests}
%
%
%
%%ifnotext Protected KVM, or pKVM~\cite{pKVM-lwn,pKVM-linux-talk,pKVM-src}, is currently being developed by Google to provide a common hypervisor for Android, to provide improved compartmentalisation by a small trusted computing base (TCB) between the Linux kernel and other services.
%%ifnotext %
%%ifnotext pKVM is built as a component of Linux. During boot, the Linux kernel hands over control of EL2 to the pKVM code, which constructs a memory map for itself and a Stage~2 memory map to encapsulate the Linux kernel. The Linux kernel thereafter runs only at EL1 (managing EL1\&0 Stage~1 memory maps for itself and for user processes), as the \emph{principal guest}, also known as the \emph{host} (not to be confused with the host hardware).   Other services can run as other guests, which are protected from the kernel and vice versa.  The kernel remains responsible for scheduling, but context switching %, %other guest control,
%%ifnotext and inter-guest communication is done by hypervisor calls to the pKVM code at EL2.
%%ifnotext %
%%ifnotext This gives us an ideal setting in which to examine the management of virtual memory by production code for Armv8-A relaxed-memory-concurrency, with both one and two stages of translation (for EL2 and EL1\&0 respectively).
%%ifnotext %
%%ifnotext The pKVM codebase is small, so it is feasible to examine all uses of TLB management, and we benefit from discussions with
%%ifnotext %extensive explanations from
%%ifnotext the pKVM development team.
%%ifnotext We have manually abstracted the main pKVM relaxed-virtual-memory scenarios into ten\marginTODO{check number?}
%%ifnotext litmus tests, included in the supplementary material.
%%ifnotext To give a flavour of these, we give one test in detail, which also illustrates the general form of virtual memory litmus tests. 

%We describe the main use-scenarios below, each of which we have manually abstracted into a litmus test.
%
% This is a manual process, so the tests are of course not guaranteed to be correct or complete representations of everything pKVM does, and
%pKVM is under active development, so its usages may change,
%but it is instructive nonetheless, and exercises much of the Armv8-A architecture and our semantics. 

% Google are currently building a new hypervisor
% called \emph{protected KVM} (or \emph{pKVM} for short).
% 
% 
% intended to run above android and provide memory isolation between guests.
% 
% \subsection{pKVM Overview}\label{sec:pkvm:subsec:overview}
% \paragraph{pKVM architecture}
% pKVM is desigend to have a principle guest,
% the \emph{host} guest.
% The host runs Android/Linux and directly communicates with the hypervisor to manage the other guests and perform scheduling
% but is not allowed to directly access any of the memory of those other guests.
% 
% To do this the hypervisor sets up the initial EL2 state,
% including installing itself in the EL2 vector table.
% Once this is done,
% pKVM switches to the host and only runs when certain events happen in the system:
% a guest accessing memory it was not allowed to,
% or the principal guest performing hypercalls to communicate with the hypervisor.
% 
% KVM controls a set of virtual CPUs (or \emph{vcpu}s).
% Each \cc{vcpu} belongs to a virtual machine (or \emph{VM}).
% The principal guest at EL1 performs scheduling and requests pKVM
% to perform the necessary TLB maintenance
% and to actually do the context switch from one vCPU to another.


%\paragraph{Host interaction with hypervisor}
%The Linux kernel can coordinate with the hypervisor to perform various tasks:
%switching to other guests, performing various cache and TLB maintenance operations,
%creating new mappings, and various other hypervisor-related tasks.
%To do this,
%the host  executes an \asm{HVC} (or ``hypervisor-call'') instruction,
%and the hypervisor then dispatches on register values to perform various actions.
%
%Currently pKVM does not have the final complete list of actions,
%but t

%% Here we give our pKVM-derived tests, as manually abstracted from the pKVM source code~\cite{pKVM-src}, in detail.
%% We first recall some of the most fundamental hypervisor calls for
%% management of the translation tables:
%% \cc{__pkvm_init} performs first-time per-CPU initialisation of pKVM,
%% this includes setting up the \cc{vmemmap},
%% a large array storing a struct entry for each physical page in memory
%% with ownership information;
%% \cc{__kvm_vcpu_run} switches to a different guest;
%% \cc{__kvm_flush_vm_context} flushes all entries in all TLB caches that relate to Stage~1 translations;
%% \cc{__kvm_tlb_flush_vmid_ipa} flushes entries in caches that relate to a particular guest for a given address;
%% \cc{__kvm_tlb_flush_vmid} flushes all entries in caches that relate to a particular guest;
%% \cc{__kvm_flush_cpu_context} flushes all entries in caches at EL1 for a given guest;
%% \cc{__pkvm_cpu_set_vector} sets the vector base address for handling exceptions;
%% \cc{__pkvm_create_mappings} creates entries in the Stage~1 page table that pKVM uses when it executes;
%% % PS: just skip? 
%% %\cc{__pkvm_create_private_mapping} also creates entries in the Stage~1 pagetable that pKVM uses when it executes,
%% %but putting virtual addresses in a private part of the address space (?);
%% and
%% \cc{__pkvm_prot_finalize} which enables Stage 2 translations during boot.

%%   See the \TODO{appendix} for a full list of these hypercalls and derived tests,
%%   but to give a flavour we will explore just one (\cc{__kvm_vcpu_run}) in detail in \S\ref{simpletest}.


%%   \paragraph{Guest interaction with hypervisor}
%%   If a guest attempts to access memory that is currently unmapped,
%%   either because the guest does not have permission to access that physical location
%%   or because the hypervisor is currently performing maintenance on that region
%%   (and so permission has been transiently removed during break-before-make),
%%   an exception is taken to EL2 which pKVM has to handle.
%%   %
%%   The pKVM implementation does not yet have support for real guests; 
%%   instead it has a temporary setup where pages are allocated on-demand as
%%   the host tries to read them.
%%   %
%%   This continues until memory runs out,
%%   at which point pKVM revokes all previously allocated pages and starts from the beginning.
%%   %
%%   This is not how the final hypervisor would work
%%   but the underlying operations to add, remove, or update mappings
%%   are a close approximation to what the final code will do
%%   and gives us a simple, clean but `real' implementation to reason about.


%In the remainder of this appendix, we give a selection of litmus tests
%extracted from the current pKVM source code~\cite{pKVM-src}.

% We do not believe this selection of litmus tests is exhaustive,
% and we are looking for feedback on both potentially missing litmus tests
% in our scope and on the tests given below.





The most basic task that pKVM is in charge of is the actual swapping from one vCPU's context to another
to execute a particular VM on the physical CPU.
Deciding \emph{when} and \emph{to which} vCPU to switch is done by the underlying host Linux guest.
pKVM's role is to safely save off the current guest's state,
and load the EL1 state for the target vCPU,
and manage the Stage~2 translation tables for the vCPU's VM.

Aside from the fundamental shape of switching from one VM to another on the same core,
there are a few interesting cases to consider:
\begin{itemize}
  \item Switching from one vCPU in a VM to another vCPU in the same VM.
  \item Switching to a new vCPU, re-using a previous VMID.
  \item Re-using an old VMID with a concurrently executing vCPU on another core.
\end{itemize}

When the host guest Linux kernel wishes to perform the switch from one vCPU to another,
it writes to some general-purpose registers and then performs an \asm{HVC} instruction
(in this case, to call the \cc{\_\_kvm\_vcpu\_run} hypercall).

%%ifnotext Switching between guests (also known as \emph{VM}s) is done by the \cc{__kvm_vcpu_run} hypercall.
%%ifnotext %when requested by the host Linux guest.
%%ifnotext %
%%ifnotext When switching from one VM's vCPU to another,
%%ifnotext pKVM must take care to ensure that any remaining context of the previously running vCPU is cleaned up.
%
%The remainder of this section will explore litmus tests created to capture different scenarios
%of switching vCPUs.  The supplementary materials contains the litmus tests in full,
%and other pKVM scenarios.

%
% In the simplest case,
% where pKVM is just switching from one vCPU to another vCPU
% in a different VM,
% pKVM restores the per-CPU register state
% and sets the \asm{VTTBR} with the new VMID.
% So long as the two vCPUs are using distinct VMIDs,
% %and no other vCPU is using those VMIDs,
% there is no requirement for TLB maintenance.
% 

% We gave this test in full in \S\ref{sec:pkvm}. %}. %Figure~\ref{fig:pkvm_test}.
% This test, \cc{pKVM.vcpu\_run}, is below, %given below in full.
%%%%%     \begin{figure}[h]
%%%%%     %\centering
%%%%%     %\scalebox{0.9}{\input{tests/tex/vcpurun}}\\[2mm]
%%%%%     \vspace*{-4mm}
%%%%%     \noindent\hspace*{-20mm}\scalebox{0.9}{\input{tests/tex/vcpurun-hand}}%\\[2mm]
%%%%%     \ifextended
%%%%%     \begin{minipage}{\textwidth}
%%%%%     \small\setlength{\parindent}{3mm}
%%%%%     \else
%%%%%     \vspace*{-4mm}
%%%%%     \end{figure}
%%%%%     \fi     
%%%%%     %The test is
%%%%%     typeset (lightly hand-edited) from the TOML input format of our Isla tool (\S\ref{isla}).\marginTODO{PS: NB this is a hand-edited version}
%%%%%     %
%%%%%     %
%%%%%     Here there is a single physical CPU, initially running a virtual machine VM1, with VMID \texttt{0x0001}, at EL1.
%%%%%     %
%%%%%     The %\texttt{page\_table\_setup}
%%%%%     section on the left defines the initial and all potential states of the page tables, and any other memory state.   
%%%%%     This test sets up separate translation tables for pKVM at EL2 (which has just a single stage) and for two VMs (each with two stages, Stage 2 controlled by pKVM and Stage 1 controlled by the VM). 
%%%%%     %
%%%%%     pKVM's own mapping \texttt{hyp\_map} maps its code. 
%%%%%     %
%%%%%     VM1's own Stage~1 mapping \texttt{vm1\_stage1} maps virtual address \texttt{x} to \texttt{ipa1},
%%%%%     and the initial pKVM-managed Stage 2 mapping \texttt{vm1\_stage2} maps that \texttt{ipa1} to \texttt{pa1}, which implicitly initially holds 0.
%%%%%     %In the combination, \texttt{x} is mapped to \texttt{ipa1} and thence to \texttt{pa1}, which initially (implicitly) holds 0.
%%%%%     %
%%%%%     %In these, \texttt{x} is mapped to \texttt{ipa2} and thence to \texttt{pa2}, which intially holds 1.
%%%%%     %
%%%%%     These page tables are described concisely %and abstractly
%%%%%     by a small declarative language we developed, %but under the hood this
%%%%%     determining the page-table memory (here $\sim$30k)
%%%%%     required for the % detailed
%%%%%     Armv8-A page-table walks. % accesses embodied in our tool. Some tests update this dynamically. 
%%%%%     
%%%%%     
%%%%%     The %\texttt{[thread.0.reset]} block
%%%%%     top-right block gives the initial Thread~0 register values, including the various page-table base registers.
%%%%%     %
%%%%%     The bottom-right blocks give the code of the test. This starts running at EL2, as one can see from the \texttt{PSTATE.EL} register value. 
%%%%%     %
%%%%%     The key assembly lines are annotated with the pKVM source line numbers they correspond to.
%%%%%     %
%%%%%     To switch to run another virtual machine VM2, with VMID \texttt{0x0002}, on this same physical CPU, pKVM changes  \texttt{VTTBR\_EL2} to the new \texttt{vm2\_stage2} mapping and, as part of the context-switch register-file changes, restores \texttt{TTBR0\_EL1} to the VM2's own Stage~1 mapping \texttt{vm2\_stage1}.
%%%%%     %
%%%%%     The code then executes an \asm{ERET} (``exception-return'') instruction to return to EL1, and then tries to read \texttt{x}.
%%%%%     %
%%%%%     The test includes a final assertion %, not shown in this rendering, that might be allowed by a model or not, here
%%%%%     of the relaxed outcome
%%%%%     that register \texttt{x2=0}, which could occur
%%%%%     if the \texttt{ldr} translation used the old VM1 mapping instead of VM2's mapping.  In this case that should not be allowed.
%%%%%     %
%%%%%     %The %\texttt{[section.thread0\_el2\_handler]} gives
%%%%%     %Thread~0 exception-handler code detects cases in which (e.g.) one might see a mix of VM1 and VM2's Stage~1 and Stage~2 mappings, which should also be forbidden. 
%%%%%     \ifextended
%%%%%     \end{minipage}
%%%%%     \caption{Test pKVM.vcpu\_run, a simple two-stage virtual-memory litmus test from \S\ref{simpletest}.%
%%%%%     %
%%%%%     %
%%%%%     %\TODO{The above mostly explains the format - we should actually explain the test, perhaps ideally with an isla-generated diagram.  That might all fit in the same figure, with care}
%%%%%     %$ 
%%%%%     %$ The following is the simplest case,
%%%%%     %$ switching from one vCPU to another,
%%%%%     %$ with different VMIDs,
%%%%%     %$ and no concurrently executing VMs.
%%%%%     %$ Isla reports the final outcome as forbidden.
%%%%%     %$ \TODO{BS: or it used to, it's now broken again...}
%%%%%     %$ We have a collection of isla-compatible tests for the other scenarios described here,
%%%%%     %$ for concurrently-executing vCPUs and switching from vCPUs in the same VM, and for 
%%%%%     %$ VMID changing.
%%%%%     %$ \TODO{BS: add appendix with all test toml?}
%%%%%     }\label{fig:pkvm_test}
%%%%%     \end{figure}

%\paragraph{Isla test}
%The test is typeset from the TOML input format of our Isla tool, which is discussed in \S\ref{isla}.
%
%
%Here there is a single physical CPU, initially running a virtual machine VM1, with VMID \texttt{0x0001}, at EL1.
%
%% 
%% Stage 1 controlled by the VM). 
%% 
%% 
%% 
%% 
%% 
%% 
%% 
%% age2} mapping and, as part of the context-switch register-file changes, sets \texttt{TTBR0\_EL1} to the VM2's own Stage~1 mapping \texttt{vm2\_stage1}.
%% 
%% 
%% the main code of the test. This starts running at EL2, as one can see from the \texttt{PSTATE.EL} register value. 
%% 
%% 
%% 
%% 
%% 
%% 1 mapping instead of the current VM2 mapping.  In this case that should not be allowed.
%% 
%%  and Stage~2 mappings, which should also be forbidden. 
% 
% Tests in this format have 3 main sections:
% the \emph{page\_table\_setup} section, which describes the initial and all potential states of the pagetables during the test
% which is described more in \S\TODO{ref to isla section};
% the \emph{thread} sections which contain the code and initial register states;
% and,
% the \emph{final} section which describes the final condition to look for.
% 
% 
% Thread~0 then switches the guest's EL1 register state,
% including its own TTBR,
% to the state for VM2's vCPU.
% It then updates the VTTBR to point to the Stage~2 tables for VM2,
% before performing an exception return which jumps
% into the vCPU's own code (here located after label \asm{L0}).
% 
% The final condition asks whether the vCPU can see the old VM's mappings,
% and isla says forbidden for this test.

\clearpage
\testpara{pKVM.vcpu\_run.update\_vmid}

Since pKVM's host Linux kernel is responsible for all scheduling,
it is responsible for the selection of VMIDs.
Typically, each VM is given its own VMID,
and all vCPUs within that VM share that VMID.
%
By giving distinct VMs different VMIDs, the host Linux kernel
can switch between vCPUs in different VMs without requiring TLB maintenance,
as was seen in the previous test.
%
Eventually, the host kernel runs out of VMIDs to allocate,
either from the naive incremental-allocation or because the
number of VMs is larger than the available VMID space
(8 or 16 bits in the worst case).
%
Currently, pKVM's host Linux kernel will simply revoke all previously allocated VMIDs,
and when pKVM goes to switch to a vCPU for a VM without an allocated VMID, it will be allocated there and then.


The \PKVMTEST{pKVM.vcpu\_run.update\_vmid} test in Figure~\ref{fig:vcpurunupdatevmid_code} is the simplest case, where
the new vCPU is the only vCPU of that VM that is running, and no other physical CPUs are executing.
%
Here, we have two VMs and their associated tables in the initial state:
\herd{vm1\_stage2} is the root of the Stage~2 table for the first VM,
and \herd{vm2\_stage2} is the root of the Stage~2 table for the second VM.
Initially, the \asm{VTTBR} points to VM1's table,
with VMID 1.
%
When switching to VM2's table,
with the same VMID,
the host Linux kernel begins a sequence of calls to the hypervisor:
first it must flush the CPU context,
to make sure any old cached translations for the old VMID are removed.
From there, pKVM can perform the switch to the new vCPU by restoring the EL1 system register
state,
then pointing the \asm{VTTBR} to the new table with the new ASID,
before doing an exception-return to the guest.
If the guest then accesses a location, it should be guaranteed to use the
new Stage~2 mapping with its own Stage~1 tables.
%
Figure~\ref{fig:vcpurunupdatevmid_code} contains the code listing and initial conditions for this test;
execution begins at EL2 with \cc{vm1}'s vCPU state, with VMID 1.
The test performs the pKVM \cc{vcpu\_run} sequence to clean up the TLB,
switch to \cc{vm2}'s EL1 state and then switching to \cc{vm2}'s Stage~2 mapping
with VMID 1 (the same as what \cc{vm1} had been using)
before returning to the guest.
The test then asserts that the guest's access uses \cc{vm2}'s own restored Stage~1 translation tables,
and does not see the old Stage~2 entries of \cc{vm1}.

Note that this test \emph{begins} with TLB invalidation.
To really capture the full sequence that is microarchitecturally interesting,
the test should really begin from execution at EL1 inside the guest
allowing Stage~2 TLB fills.
The test beginning at EL2 from a clean machine state would not give the TLB time to
actually fill with stale entries from \cc{vm1}'s Stage~2 translation tables
in an operational model.
%
Also note that, currently, Isla does not produce candidates with re-ordering of system register reads,
and so there are no `bad' candidate executions to show from the Isla-generated executions currently.
This is work-in-progress to find the correct semantics for such re-orderings.

%\TODO{The above refers to event IDs, but we're not yet giving an execution diagram, or including the IDs in comments in the test code}
%\TODO{Perhaps these tests should start from EL1}?

\begin{figure}
  \centering
  \scalebox{0.8}{\input{tests/tex/vcpurunupdatevmid}}
\caption{}\label{fig:vcpurunupdatevmid_code}
\end{figure}

%%ifnotext 
%%ifnotext Other tests capture more elaborate scenarios. For example,
%%ifnotext currently the host kernel manages VMIDs and assigns each VM its own VMID.
%%ifnotext %Currently the VMIDs are managed by the host kernel,
%%ifnotext %which assigns each VM its own VMID.
%%ifnotext If the host runs out of VMIDs to allocate to new vCPUs,
%%ifnotext it currently revokes all previously allocated VMIDs and re-allocates from the beginning, during which
%%ifnotext %
%%ifnotext %When revoking the old VMIDs
%%ifnotext pKVM has to ensure that any old vCPUs' translations using that VMID are expelled from any TLBs (\cc{pKVM.vcpu\_run.update\_vmid}).
%%ifnotext %This is captured by the \cc{pKVM.vcpu\_run.update\_vmid} test which stops one guest and switches to another
%re-using the same VMID.
%

\clearpage
\testpara{pKVM.vcpu\_run.update\_vmid.concurrent}

The concurrent case of the previous \PKVMTEST{pKVM.vcpu\_run.update\_vmid} test is critical:
while switching from one vCPU to another on the same core is typically a
%very
thread-local event,
care must be taken in the case where another CPU is executing a VM whose current VMID should be revoked, as in Fig.~\ref{fig:vcpurunupdatevmidconcurrent}.

In this case, pKVM must interrupt the other core, so that it is not concurrently executing while the new VMIDs are being
allocated; otherwise, it might pollute the address space of the VM that gets allocated that VMID.

pKVM does this by sending an IPI to all the other cores to break out of their current vCPUs.
When it does this, each CPU will attempt to switch back to the host, and, in doing so,
will be forced to take a lock when acquiring the VMID to use.
%
This lock prevents those CPUs from executing at EL1,
and the architecture prevents the hardware from performing TLB fills while at EL2.
These guarantees ensure that while VMIDs are being re-allocated and TLB maintenance performed
on the original core,
no stale entries can find their way back into the TLB.

% suppress for ESOP submission
% \TODO{what should we say about this here?}
% However,
% our understanding of this code raises a question.
% The \cc{tlb.c} file in pKVM uses a \asm{DSB ISHST} to order
% from po-previous stores to the translation tables before the TLB maintenance,
% but this would not wait for any reads coming back from the IPI message pass.
% We assume there must be some other synchronization between the IPI receive on the
% core invalidating the VMIDs and the invalidation itself,
% but we do not know where in pKVM it can be found (if it exists at all).
% %
% Work needs to be done here to try match the compiled pKVM and all the barriers
% with our understanding of the source materials.

\begin{figure}
\noindent\hspace*{-19mm}
%  \scalebox{0.8}{\input{tests/tex/vcpurunupdatevmidconcurrent}}
  \resizebox*{!}{0.95\textheight}{\input{tests/tex/vcpurunupdatevmidconcurrent}}
\caption{}\label{fig:vcpurunupdatevmidconcurrent}
\end{figure}

%%ifnotext If there is a concurrently executing vCPU using that VMID,
%%ifnotext %we get a variation of the test named \cc{pKVM.vcpu\_run.update\_vmid.concurrent}.
%%ifnotext %Here care must be taken  to ensure
%%ifnotext that vCPU must be paused
%%ifnotext until after the new VMID generation (and hence any required TLB maintenance),
%%ifnotext %has happened,
%%ifnotext before continuing
%%ifnotext with the freshly allocated VMID (\cc{pKVM.vcpu\_run.update\_vmid.concurrent}).
%%ifnotext %
%%ifnotext %Currently pKVM ensures no other vCPUs are running through a combination of an inter-processor interrupt (IPI)
%%ifnotext %and an internal lock that prevents the vCPUs from running until the new VMID generation has allocated.
%%ifnotext %While we do not model IPIs, this behaviour can be approximated with a message pass and a hypervisor call.


%Because the EL1 register state is supposed to be per-CPU,
\clearpage
\testpara{pKVM.vcpu\_run.same\_vm}

%In order
For another example, for pKVM to maintain the illusion that each vCPU is on its own core,
the per-core state must be cleaned between running different vCPUs,
including ensuring that translations for one vCPU are not cached and visible
to another, even if they happen to be in the same VM (and using the same VMID) (\cc{pKVM.vcpu\_run.same\_vm} in Figure~\ref{fig:vcpurunsamevm}).
%
%To capture this the \cc{pKVM.vcpu\_run.same\_vm} test
%switches from one vCPU to another vCPU on the same core within the same VM.
%
%At EL2 pKVM flushes local caches before dropping back to EL1 in the new guest;
%we assert that translations in the new guest do not see translations from the old guest.

\begin{figure}
  \noindent\hspace*{-19mm}
    \resizebox*{!}{0.95\textheight}{\input{tests/tex/vcpurunsamevm}}
  \caption{}\label{fig:vcpurunsamevm}
\end{figure}

%fig:pkvm_test was here in submitted version

% \begin{tabular}{@{}c@{\hspace*{2mm}}c@{}}
% 
% 
% \begin{lstlisting}[keepspaces=true]
% arch = "AArch64"
% name = "pKVM.vcpu_run"
% symbolic = ["x"]
% 
% page_table_setup = """
% option default_tables = false;
% 
% physical pa1 pa2;
% intermediate ipa1 ipa2;
% 
% s1table hyp_map 0x200000 {
%     identity 0x1000 with code;
%     x |-> invalid;
% }
% 
% s2table vm1_stage2 0x240000  {
%     identity pa_to_ipa(0x1000) with code;
%     ipa1 |-> pa1;
%     ipa2 |-> invalid;
% 
% 
%     s1table vm1_stage1 0x2C0000 {
%         identity pa_to_va(0x1000) with code;
%         x |-> ipa1;
%     }
% }
% 
% s2table vm2_stage2 0x280000  {
%     identity pa_to_ipa(0x1000) with code;
%     ipa1 |-> invalid;
%     ipa2 |-> pa2;
% 
%     s1table vm2_stage1 0x300000 {
%         identity pa_to_va(0x1000) with code;
%         x |-> ipa2;
%     }
% }
% 
% 
% *pa2 = 1;
% """
% \end{lstlisting}
% &
% \begin{lstlisting}[keepspaces=true]
% [thread.0]
% code = """
%     msr ttbr0_el1, x0  // kvm/hyp/sysreg-sr.h:96
%     msr vttbr_el2, x1  // include/asm/kvm_mmu.h:276
%     eret // kvm/hyp/nvhe/host.S
% L0:
%     ldr x2, [x3] // in guest
% """
% 
% [thread.0.reset]
% R0 = "ttbr(asid=0x00, base=vm2_stage1)"
% R1 = "ttbr(vmid=0x0002, base=vm2_stage2)"
% 
% TTBR0_EL2 = "ttbr(asid=0x00, base=hyp_map)"
% VTTBR_EL2 = "ttbr(vmid=0x0001, base=vm1_stage2)"
% TTBR0_EL1 = "ttbr(asid=0x00, base=vm1_stage1)"
% 
% R3 = "x"
% VBAR_EL2 = "extz(0x1000, 64)"
% 
% "PSTATE.EL" = "0b10"
% 
% # return to EL1h at L0
% SPSR_EL2 = "extz(0b00101, 64)"
% ELR_EL2 = "extz(L0:, 64)"
% 
% [section.thread0_el2_handler]
% address = "0x1400" # 0x400 - Lower Exception Level
% code = """
%     mov x2, #0
% """
% 
% [final]
% assertion = "0:X2 = 0"
% \end{lstlisting}
%
%\end{tabular}
%
%}


\clearpage
\subsection{Data Aborts}

As mentioned earlier,
a vCPU accessing a location that it does not have permissions for
or which is not mapped,
results in an Abort which is handled at EL2.


\testpara{pKVM.host\_handle\_trap.stage2\_idmap.l3}
%
If the vCPU accesses a location which is currently un-mapped,
but should be mapped on-demand, then pKVM will make a new mapping
for that vCPU, install it into its VM's Stage~2 translation tables,
and return to the vCPU to re-try the access
(Figures~\ref{fig:hosthandletrapstagetwoidmaplthree_code} and \ref{fig:hosthandletrapstagetwoidmaplthree_exec}).
This action typically requires no TLB invalidation, as the previously unmapped entries
could not have been stored in any TLB.

An added complexity here is that if pKVM wishes
to map only a single page then it \emph{must} install this mapping
with a Level~3 entry.
If the mapping is currently invalid at Level~2 or Level~1 then
care must be taken to not create entries out-of-order.
pKVM manages this by producing a fresh table of invalid entries first,
then installing that new table into the translation tables,
and recursing down until it reaches the level it needs to install the valid mapping at.
Otherwise, a concurrent translation could see the new table entries before
the leaf entries had been installed into the table.


\begin{figure}
  %  \centering
  %  \scalebox{0.8}{
    \noindent\hspace*{-19mm}
  %  \scalebox{0.8}{\input{tests/tex/vcpurunupdatevmidconcurrent}}
%    \resizebox*{!}{0.95\textheight}
{\input{tests/tex/hosthandletrapstagetwoidmaplthree}}\
  \caption{\PKVMTEST{pKVM.host\_handle\_trap.stage2\_idmap.l3}: code listing}\label{fig:hosthandletrapstagetwoidmaplthree_code}
\end{figure}

\begin{figure}
  \centering
%  \includegraphics[trim=10mm 0 0 0, clip,width=140mm,height=120mm]{tests/pKVM/pKVM.host_handle_trap.stage2_idmap.change_block_size_allow_7.pdf}

  \includegraphics[trim=10mm 0 0 0, clip,width=140mm,height=120mm]{tests/pKVM/pKVM_host_handle_trap_stage2_idmap_l3_allow_4.pdf}
  \caption{\PKVMTEST{pKVM.host\_handle\_trap.stage2\_idmap.l3}: forbidden candidate execution}\label{fig:hosthandletrapstagetwoidmaplthree_exec}
\end{figure}

\clearpage
\testpara{pKVM.host\_handle\_trap.stage2\_idmap.already\_exists}\label{test:pKVM.host_handle_trap.stage2_idmap.already_exists}
If the vCPU tries to access a location that is mapped but that it lacks the necessary permissions for,
then there may be an existing entry already mapping that location.
Here, the process is much more delicate.
Because another vCPU in the same VM may be concurrently accessing the same physical locations
mapped by the shared Stage~2 table,
pKVM cannot assume its own internal locks are sufficient to prevent race conditions.
Therefore, this is one case where pKVM is \emph{required} to use the break-before-make sequence as described by
\S\ref{subsubsec:questions:tlb:bbm}.

In the following code (Figures~\ref{fig:hosthandletrapstagetwoidmaplthreealreadyexists_code} and \ref{fig:hosthandletrapstagetwoidmaplthreealreadyexists_exec}), the initial state starts out with \cc{x} mapped at level 3, but without read permissions.
The first load will fault and pKVM will naturally map a writeable mapping on-demand,
following the break-before-make sequence invalidating the entry by writing zero (event \herd{b})
before writing a new valid descriptor (event \herd{m}).
After returning to the guest, we ask whether loads of \cc{x} are allowed to fault at Stage~2.

\begin{figure}
  %  \centering
  %  \scalebox{0.8}{
    \noindent\hspace*{-19mm}
    \resizebox*{!}{0.95\textheight}{\input{tests/tex/hosthandletrapstagetwoidmaplthreealreadyexists}}\
    \caption{\PKVMTEST{pKVM.host\_handle\_trap.stage2\_idmap.l3.already\_exists}: code listing}\label{fig:hosthandletrapstagetwoidmaplthreealreadyexists_code}
  \end{figure}

  \begin{figure}
    \centering
    \includegraphics[trim=10mm 0 0 0, clip,width=140mm,height=120mm]{tests/pKVM/pKVM_host_handle_trap_stage2_idmap_l3_already_exists_allow_5.pdf}
    \caption{\PKVMTEST{pKVM.host\_handle\_trap.stage2\_idmap.l3.already\_exists}: forbidden candidate execution}\label{fig:hosthandletrapstagetwoidmaplthreealreadyexists_exec}
  \end{figure}

\clearpage

\testpara{pKVM.host\_handle\_trap.stage2\_idmap.change\_block\_size}
The complexity of the previous scenario is compounded by the fact that pKVM may wish to map a larger region
(higher in the table)
than is currently mapped, and, without \asm{FEAT\_BBM}, this adds extra break-before-make requirements.

In general, pKVM will itself perform a translation table walk.
On the way down, it will look for the entry to be replaced,
invalidate it, and perform TLB maintenance,
ensuring that all entries from old leaf entries below it are cleaned away,
but additionally that any old stale Stage~1 translations are invalidated,
before it replaces the entry.


Figures~\ref{fig:hosthandletrapstagetwoidmapchangeblocksize_code} and \ref{fig:hosthandletrapstagetwoidmapchangeblocksize_exec} contain the code listing and the interesting candidate execution diagram
(as generated by Isla).
We consider a scenario where there are two locations,
\cc{x} and \cc{y}
which are in the same 2~MiB region of memory
but are mapped by different Level~3 entries.
If the Level~3 table contains all valid entries except for
one entry for \cc{x},
then on updating the entry for \cc{x} to be valid,
if the host kernel maps the whole 2M region,
then pKVM will invalidate the 2M entry before
writing a new 2M block entry.

This in effect `promotes' the set of 4K mappings into a single 2M mapping.
pKVM then frees the child table to be re-allocated later.
%\TODO{BS: is there a concurrent test about re-using that free'd table in another thread?}.

%Finally,
pKVM may want to \emph{remove} a mapping for an IPA.
This is very similar to the previously described break-before-make scenario,
but without the final make.
pKVM just has to ensure that the old IPA mapping is invalidated,
and the necessary TLB maintenance is performed.
We do not include this test at present.

\begin{figure}
%  \centering
%  \scalebox{0.8}{
  \noindent\hspace*{-19mm}
%  \scalebox{0.8}{\input{tests/tex/vcpurunupdatevmidconcurrent}}
  \resizebox*{!}{0.95\textheight}{\input{tests/tex/hosthandletrapstagetwoidmapchangeblocksize}}\
  \caption{\PKVMTEST{pKVM.host\_handle\_trap.stage2\_idmap.change\_block\_size}: code listing}\label{fig:hosthandletrapstagetwoidmapchangeblocksize_code}
\end{figure}

\begin{figure}
  \centering
%  \includegraphics[trim=10mm 0 0 0, clip,width=140mm,height=120mm]{tests/pKVM/pKVM.host_handle_trap.stage2_idmap.change_block_size_allow_7.pdf}
  \includegraphics[trim=10mm 0 0 0, clip,width=140mm,height=120mm]{tests/pKVM/pKVM_host_handle_trap_stage2_idmap_change_block_size_allow_7.pdf}
  \caption{\PKVMTEST{pKVM.host\_handle\_trap.stage2\_idmap.change\_block\_size}: forbidden candidate execution}\label{fig:hosthandletrapstagetwoidmapchangeblocksize_exec}
\end{figure}

\clearpage

% \testpara{pKVM.host\_handle\_trap.stage2\_idmap.already\_exists.concurrent}

% The case where the previous Test~\ref{test:pKVM.host_handle_trap.stage2_idmap.already_exists} \PKVMTEST{pKVM.host\_handle\_trap.stage2\_idmap.already\_exists} has a concurrently executing CPU
% in the same VM is an interesting one.
% Care must be taken to ensure that if that vCPU is accessing memory that is being re-mapped by another core that the break-before-make sequence was correctly
% followed as described in \S\ref{subsubsec:questions:tlb:bbm}.

% pKVM's own locks prevent two attempts at mapping the same page to happen concurrently,
% so the only case we have to consider is that where one CPU updates the mapping while another
% concurrently accesses it.

% \TODO{BS: diagram and stuff}

% \fi

% \clearpage



% PS moved this to the end - logically it'd be nice at the start, but if we don't handle it, it's terrible to start with something we don't handle. And also nice to start with the one for which we give the concrete test.
\subsection{Initialisation}

During execution,
and especially at initial start-up of pKVM,
it will be required to create its own Stage~1 translation tables.

Currently, this only happens on a single core,
so there are no interesting concurrent cases.
%(\TODO{is that true?}).

In the future, however, it is expected that pKVM may need to
dynamically map some parts of memory, as the hypervisor gains richer features.
%Especially, with any requirement for the hypervisor to interact directly with the guests
For example, it may need to map some shared page between guests, or between pKVM and a guest, in which to pass messages.

\clearpage

\testpara{pKVM.switch\_to\_new\_table}

When pKVM first starts, it is using translation tables set up by Linux,
so one of the first things pKVM does is to create its own tables and switch to them.

Usually, switching from using one translation table to another happens at a higher exception level,
and then the new one is not used until the return to the lower exception level.
The current case
 is more complicated, as pKVM has to change its own translation tables
\emph{while it is executing}.
If pKVM only had to change the \asm{TTBR}, then this would not be a problem,
but there are many system registers involved in configuring the translation tables
(the \asm{TCR}, \asm{MAIR}, and so on), and these registers cannot all be updated `atomically'.

To maintain the atomicity, pKVM switches the \asm{TTBR}
to a page of memory where the code it is executing is identity-mapped,
then it disables translation (disabling the MMU),
before updating all of the required system registers (including the new \asm{TTBR}),
before re-enabling the MMU.

Figure~\ref{fig:switchtonewtable_code} contains the code for a litmus test
that tries to capture the core of this process.
This \PKVMTEST{pKVM.switch\_to\_new\_table} test is an EL2 Stage~1 test
with two tables, \cc{hyp\_pgtable} and \cc{new\_hyp\_pgtable}, in memory.
The code disables the MMU (by writing to the appropriate field of the SCTLR),
invalidates all of the old cached TLB entries for EL2,
updates all the system registers (only the \asm{TTBR} is included here)
and then re-enables the MMU.
We check that the final load in the hypervisor after the switch has happened
reads using the new state.

This test has been cut down for brevity to remove the writes of other system registers,
which would be present in a full execution of pKVM;
ideally, we would have a test that included those too,
and a final state which ensured that the load used a translation using
all of the new register values.
%\TODO{Perhaps we should write that test down too?}

Note that the model presented in Section~\ref{sec:models}
does not currently contain axioms for when the MMU is disabled,
but the semantics seem clear, %to us
and we do not see any impediment in extending the model to handle it fully.

\begin{figure}[h]
  \centering
  \scalebox{0.8}{\input{tests/tex/switchtonewtable}}
\caption{pKVM.switch\_to\_new\_table}\label{fig:switchtonewtable_code}
\end{figure}

\clearpage

\testpara{pKVM.create\_hyp\_mappings.inv.l2}

Constructing new translation tables is done incrementally,
starting from a single zero'd page of memory as the root table,
and then performing a manual translation table walk on insertion to locate an entry to insert into.

In the case where there is no Level~3 table to install into,
pKVM first creates a Level~2 table and installs that,
before writing the new valid Level~3 entry.
To avoid break-before-make violations here,
pKVM always ensures the table is zeroed before
inserting it into the table.

The \PKVMTEST{pKVM.create\_hyp\_mappings.inv.l2} test,
in Figures~\ref{fig:createhypmappingsinvltwo_code} and \ref{fig:createhypmappingsinvltwo_exec},
gives the case where pKVM is trying to create a new mapping for itself
for a 4K page block.
This block mapping \emph{must} be installed as a Level~3 entry,
as installing it any higher would end up mapping more than 4K of memory.
Initially, \herd{x} is translated using an invalid Level~2 entry in \cc{hyp\_pgtable}.
The table \cc{hyp\_pgtable\_new} contains the new Level~3 table which starts life zeroed (all invalid);
The test then sets the Level~2 entry in \cc{hyp\_pgtable} to point to the new table,
and then updates the Level~3 (leaf) entry with a valid descriptor.

Interestingly, we note that pKVM sets these entries with a store-release;
although there seems to be no relaxed-virtual-memory reason why.
Given that pKVM is well locked, it is not clear why making these writes store-releases helps.
% Presumably this is done just for sanity to ensure that concurrent accesses
% (both reading of the translation tables by pKVM itself and by other thread's MMUs)
% although in this case this is unnecessary as both the initial level~2 entry and level~3 table
% are invalid (and the earlier allocation of the table is barriered).
% \TODO{the previous isn't sentences}

\begin{figure}[h]
%  \centering
%\hspace*{-13mm}
%\begin{tabular}{ll}
  \scalebox{0.8}{\input{tests/tex/createhypmappingsinvltwo}}%
%  &%
  % TODO: BS: this is really squished and ugly, but at least it fits.
%  \includegraphics[trim=10mm 0 0 0, clip,width=50mm,height=40mm]{tests/pKVM/pKVM.create_hyp_mappings.inv.l2_allow_3.pdf}
%  \includegraphics[trim=10mm 0 0 0, clip,width=50mm,height=40mm]{tests/pKVM/pKVM_create_hyp_mappings_inv_l2_allow_3.pdf}
%  \end{tabular}
\caption{\PKVMTEST{pKVM.create\_hyp\_mappings.inv.l2}: Code listing }\label{fig:createhypmappingsinvltwo_code}
\end{figure}


\begin{figure}[h]
%  \centering
%\hspace*{-13mm}
%\begin{tabular}{ll}
%  \scalebox{0.8}{\input{tests/tex/createhypmappingsinvltwo}}%
%  &%
  % TODO: BS: this is really squished and ugly, but at least it fits.
%  \includegraphics[trim=10mm 0 0 0, clip,width=50mm,height=40mm]{tests/pKVM/pKVM.create_hyp_mappings.inv.l2_allow_3.pdf}
  \includegraphics[trim=10mm 0 0 0, clip,width=120mm]{tests/pKVM/pKVM_create_hyp_mappings_inv_l2_allow_3.pdf}
%  \end{tabular}
\caption{\PKVMTEST{pKVM.create\_hyp\_mappings.inv.l2}: (forbidden) candidate execution}\label{fig:createhypmappingsinvltwo_exec}
\end{figure}


\clearpage

\testpara{pKVM.create\_hyp\_mappings.inv.l3}

pKVM can set entries at any level of the table,
assuming they are initially invalid.
The following test is a variation on the previous,
 where the Level~3 table is already created, but contains an invalid entry at Level~3.

As before, we will map a 4K region, and so it must go at Level~3.

\begin{figure}[h]
  \centering
%\hspace*{-10mm}
%\begin{tabular}{ll}
  \scalebox{0.8}{\input{tests/tex/createhypmappingsinvlthree}}%
%  &%
  % TODO: BS: this is really squished and ugly, but at least it fits.
%  \includegraphics[trim=10mm 0 0 0, clip,width=50mm,height=40mm]{tests/pKVM/pKVM.create_hyp_mappings.inv.l3_allow_2.pdf}
%  \includegraphics[trim=10mm 0 0 0, clip,width=50mm,height=40mm]{tests/pKVM/pKVM_create_hyp_mappings_inv_l3_allow_2.pdf}
%  \end{tabular}
\caption{\PKVMTEST{pKVM.create\_hyp\_mappings.inv.l3}: Code listing }\label{fig:createhypmappingsinvlthree_code}
\end{figure}
\begin{figure}[h]
  \centering
%\hspace*{-10mm}
%\begin{tabular}{ll}
%  \scalebox{0.8}{\input{tests/tex/createhypmappingsinvlthree}}%
%  &%
  % TODO: BS: this is really squished and ugly, but at least it fits.
%  \includegraphics[trim=10mm 0 0 0, clip,width=50mm,height=40mm]{tests/pKVM/pKVM.create_hyp_mappings.inv.l3_allow_2.pdf}
  \includegraphics[trim=10mm 0 0 0, clip,width=50mm,height=40mm]{tests/pKVM/pKVM_create_hyp_mappings_inv_l3_allow_2.pdf}
%  \end{tabular}
\caption{\PKVMTEST{pKVM.create\_hyp\_mappings.inv.l3}:  (forbidden) candidate execution}\label{fig:createhypmappingsinvlthree_exec}
\end{figure}


%%ifnotext During boot, the Linux kernel asks pKVM to initialise itself, during which
%%ifnotext it creates pagetables for its own future EL2 execution, and switches to them.
%%ifnotext %
%%ifnotext This first part of pKVM execution uses pagetables set up by Linux.
%%ifnotext Creation of the new tables is just C-language data structure
%%ifnotext manipulation, and the tables are not in use while this is happening.
%%ifnotext To switch to running with the new tables, 
%%ifnotext pKVM first jumps to a part of its binary which has been set up (by Linux) as an identity-mapped region, with  virtual and physical addresses coinciding.  Within that, 
%%ifnotext it disables the MMU (by setting the \asm{M} bit of the \asm{SCTLR} to 0),
%%ifnotext performs TLB maintenance to remove any old mappings, writes the new page-table base address and configuration values to the appropriate system registers, and 
%%ifnotext switches the MMU back on.
%%ifnotext Doing this with the MMU off ensures that the changes to the system registers required to update the translation happen atomically, 
%%ifnotext and that translations cannot start using a partially-initialised state; the identity maps ensure that execution work correctly over the on/off transitions. 
%%ifnotext 
%%ifnotext Note that currently our model does not capture the behaviour when the MMU is disabled, but it seems clear what the behaviour should be, 
%%ifnotext as described in \S\ref{sec:questions:subsec:mmu_off},
%%ifnotext and we are not aware of any challenges in handling it in the model and tooling. 

\clearpage



==> tests/tex/hosthandletrapstagetwoidmapchangeblocksizechangepermissions.tex <==
\newlength{\hosthandletrapstagetwoidmapchangeblocksizechangepermissionsH}
\setlength{\hosthandletrapstagetwoidmapchangeblocksizechangepermissionsH}{0cm}
\newsavebox{\hosthandletrapstagetwoidmapchangeblocksizechangepermissionsI}
\begin{lrbox}{\hosthandletrapstagetwoidmapchangeblocksizechangepermissionsI}
\begin{lstlisting}[language=AArch64,showlines=true]
MOV X0,#0
LDR X0,[X1]
MOV X2,#0
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\hosthandletrapstagetwoidmapchangeblocksizechangepermissionsJ}
\settowidth{\hosthandletrapstagetwoidmapchangeblocksizechangepermissionsJ}{\usebox{\hosthandletrapstagetwoidmapchangeblocksizechangepermissionsI}}
\addtolength{\hosthandletrapstagetwoidmapchangeblocksizechangepermissionsH}{\hosthandletrapstagetwoidmapchangeblocksizechangepermissionsJ}
\newsavebox{\hosthandletrapstagetwoidmapchangeblocksizechangepermissionsK}
\begin{lrbox}{\hosthandletrapstagetwoidmapchangeblocksizechangepermissionsK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
// count number of exceptions
add x10,x10,#1
// remember which IPA failed
mrs x9,hpfar_el2
// on second fault just exit test
cmp x10,#2
b.eq 1f
// then pkvm code
0:
// pgtable.c:181
STR X12,[X13]
// tlb.c:116
DSB ISH
// tlb.c:119
MSR VTTBR_EL2,X14
// tlb.c:119
ISB
// tlb.c:121
TLBI vmalls12e1is
// tlb.c:122
DSB ISH
// tlb.c:123
ISB
// tlb.c:125
MSR VTTBR_EL2,X16
// tlb.c:125
ISB
STLR X17,[x18]
DSB ISHST
1:
// return to next instruction
// pKVM doesn't really do this, it just tries the same instr again
// but without this the test can loop forever ...
mrs x20,elr_el2
add x20,x20,#4
msr elr_el2,x20
// return from handle_trap
eret
\end{lstlisting}
\end{lrbox}
\newlength{\hosthandletrapstagetwoidmapchangeblocksizechangepermissionsL}
\settowidth{\hosthandletrapstagetwoidmapchangeblocksizechangepermissionsL}{\usebox{\hosthandletrapstagetwoidmapchangeblocksizechangepermissionsK}}
\addtolength{\hosthandletrapstagetwoidmapchangeblocksizechangepermissionsH}{\hosthandletrapstagetwoidmapchangeblocksizechangepermissionsL}
\newsavebox{\hosthandletrapstagetwoidmapchangeblocksizechangepermissionsM}
\begin{lrbox}{\hosthandletrapstagetwoidmapchangeblocksizechangepermissionsM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
option default_tables = false;
physical pa1 pa2;
intermediate ipa1;

s2table vm_stage2 0x260000  {
    ipa1 |-> pa1 with [AP = 0b00] at level 3;
    ipa1 ?-> invalid at level 2;
    ipa1 ?-> pa2 with default at level 2;

    s1table host_s1 0x2C0000 {
        x |-> ipa1;
    }
};

s1table hyp_map 0x200000  {
    x |-> invalid;
    s2table vm_stage2;
    identity 0x1000 with code;
}

*pa1 = 1;
*pa2 = 2;
\end{lstlisting}
\end{lrbox}
\newlength{\hosthandletrapstagetwoidmapchangeblocksizechangepermissionsN}
\settowidth{\hosthandletrapstagetwoidmapchangeblocksizechangepermissionsN}{\usebox{\hosthandletrapstagetwoidmapchangeblocksizechangepermissionsM}}
\newsavebox{\hosthandletrapstagetwoidmapchangeblocksizechangepermissionsO}
\begin{lrbox}{\hosthandletrapstagetwoidmapchangeblocksizechangepermissionsO}
\begin{minipage}{\hosthandletrapstagetwoidmapchangeblocksizechangepermissionsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|R10=0b0|\\
\lstinline[language=IslaLitmusExp]|R15=ipa1|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x1000|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R1=x|\\
\lstinline[language=IslaLitmusExp]|TTBR0_EL2=ttbr(asid=0x0000,base=hyp_map)|\\
\lstinline[language=IslaLitmusExp]|TTBR0_EL1=ttbr(base=host_s1,asid=0x0000)|\\
\lstinline[language=IslaLitmusExp]|R17=mkdesc2(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|R12=0b0|\\
\lstinline[language=IslaLitmusExp]|VTTBR_EL2=ttbr(vmid=0x0001,base=vm_stage2)|\\
\lstinline[language=IslaLitmusExp]|R13=pte2(ipa1,vm_stage2)|\\
\lstinline[language=IslaLitmusExp]|R14=ttbr(vmid=0x001,base=0b0)|\\
\lstinline[language=IslaLitmusExp]|R18=pte2(x,vm_stage2)|\\
\lstinline[language=IslaLitmusExp]|R16=ttbr(vmid=0x001,base=vm_stage2)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|pKVM.host_handle_trap.stage2_idmap.change_block_size.change_permissions|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\hosthandletrapstagetwoidmapchangeblocksizechangepermissionsN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\hosthandletrapstagetwoidmapchangeblocksizechangepermissionsM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\hosthandletrapstagetwoidmapchangeblocksizechangepermissionsO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\hosthandletrapstagetwoidmapchangeblocksizechangepermissionsI}\\
  \cline{2-2}
  & thread0 el2 handler\\
  \cline{2-2}
  & \usebox{\hosthandletrapstagetwoidmapchangeblocksizechangepermissionsK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R10=2 | 0:R2=1|\\
  \hline
\end{tabular}


==> tests/tex/hosthandletraptwicestagetwoidmaplthhree.tex <==
\newlength{\hosthandletraptwicestagetwoidmaplthhreeH}
\setlength{\hosthandletraptwicestagetwoidmaplthhreeH}{0cm}
\newsavebox{\hosthandletraptwicestagetwoidmaplthhreeI}
\begin{lrbox}{\hosthandletraptwicestagetwoidmaplthhreeI}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\hosthandletraptwicestagetwoidmaplthhreeJ}
\settowidth{\hosthandletraptwicestagetwoidmaplthhreeJ}{\usebox{\hosthandletraptwicestagetwoidmaplthhreeI}}
\addtolength{\hosthandletraptwicestagetwoidmaplthhreeH}{\hosthandletraptwicestagetwoidmaplthhreeJ}
\newsavebox{\hosthandletraptwicestagetwoidmaplthhreeK}
\begin{lrbox}{\hosthandletraptwicestagetwoidmaplthhreeK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
// count number of exceptions
add x10,x10,#1
// remember which IPA failed
mrs x9,hpfar_el2
lsl x9,x9,#8
// pkvm code
stlr x11,[x12]
dsb ishst
// return to next instruction
// pKVM doesn't really do this, it just tries the same instr again
// but without this the test can loop forever ...
mrs x20,elr_el2
add x20,x20,#4
msr elr_el2,x20
// return from handle_trap
eret
\end{lstlisting}
\end{lrbox}
\newlength{\hosthandletraptwicestagetwoidmaplthhreeL}
\settowidth{\hosthandletraptwicestagetwoidmaplthhreeL}{\usebox{\hosthandletraptwicestagetwoidmaplthhreeK}}
\addtolength{\hosthandletraptwicestagetwoidmaplthhreeH}{\hosthandletraptwicestagetwoidmaplthhreeL}
\newsavebox{\hosthandletraptwicestagetwoidmaplthhreeM}
\begin{lrbox}{\hosthandletraptwicestagetwoidmaplthhreeM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
option default_tables = false;
physical pa1;
intermediate ipa1;

s2table vm_stage2 0x260000 {
    ipa1 |-> invalid;
    ipa1 ?-> pa1;

    s1table host_s1 0x2C0000 {
        x |-> ipa1;
    }
}

s1table hyp_map 0x200000 {
    x |-> invalid;
    s1table host_s1;
    s2table vm_stage2;
    identity 0x1000 with code;
}

*pa1 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\hosthandletraptwicestagetwoidmaplthhreeN}
\settowidth{\hosthandletraptwicestagetwoidmaplthhreeN}{\usebox{\hosthandletraptwicestagetwoidmaplthhreeM}}
\newsavebox{\hosthandletraptwicestagetwoidmaplthhreeO}
\begin{lrbox}{\hosthandletraptwicestagetwoidmaplthhreeO}
\begin{minipage}{\hosthandletraptwicestagetwoidmaplthhreeH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|TTBR0_EL1=ttbr(asid=0x0000,base=host_s1)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x1000|\\
\lstinline[language=IslaLitmusExp]|TTBR0_EL2=ttbr(base=hyp_map,asid=0x0000)|\\
\lstinline[language=IslaLitmusExp]|R11=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R1=x|\\
\lstinline[language=IslaLitmusExp]|VTTBR_EL2=ttbr(base=vm_stage2,vmid=0x0000)|\\
\lstinline[language=IslaLitmusExp]|R10=0b0|\\
\lstinline[language=IslaLitmusExp]|R12=pte3(x,vm_stage2)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|pKVM.host_handle_trap_twice.stage2_idmap.l3|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\hosthandletraptwicestagetwoidmaplthhreeN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\hosthandletraptwicestagetwoidmaplthhreeM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\hosthandletraptwicestagetwoidmaplthhreeO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\hosthandletraptwicestagetwoidmaplthhreeI}\\
  \cline{2-2}
  & thread0 el2 handler\\
  \cline{2-2}
  & \usebox{\hosthandletraptwicestagetwoidmaplthhreeK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R10=2 & 0:R9=ipa1|\\
  \hline
\end{tabular}

==> tests/tex/vcpurun.tex <==
\newlength{\pKVMdotvcpurunH}
\setlength{\pKVMdotvcpurunH}{0cm}
\newsavebox{\pKVMdotvcpurunI}
\begin{lrbox}{\pKVMdotvcpurunI}
\begin{lstlisting}[language=AArch64,showlines=true]
// kvm/hyp/sysreg-sr.h:96
msr ttbr0_el1, x0
// include/asm/kvm_mmu.h:276
msr vttbr_el2, x1
// kvm/hyp/nvhe/host.S
eret
L0:
// in guest
ldr x2, [x3]
\end{lstlisting}
\end{lrbox}
\newlength{\pKVMdotvcpurunJ}
\settowidth{\pKVMdotvcpurunJ}{\usebox{\pKVMdotvcpurunI}}
\addtolength{\pKVMdotvcpurunH}{\pKVMdotvcpurunJ}
\newsavebox{\pKVMdotvcpurunK}
\begin{lrbox}{\pKVMdotvcpurunK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
mov x2, #0
\end{lstlisting}
\end{lrbox}
\newlength{\pKVMdotvcpurunL}
\settowidth{\pKVMdotvcpurunL}{\usebox{\pKVMdotvcpurunK}}
\addtolength{\pKVMdotvcpurunH}{\pKVMdotvcpurunL}
\newsavebox{\pKVMdotvcpurunM}
\begin{lrbox}{\pKVMdotvcpurunM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
option default_tables = false;
virtual x;
physical pa1 pa2;
intermediate ipa1 ipa2;
s1table hyp_map 0x200000 {
  identity 0x1000 with code;
  x |-> invalid;
}
s1table vm1_stage1 0x2C0000 {
  x |-> ipa1;
}
s1table vm2_stage1 0x300000 {
  x |-> ipa2;
}
s2table vm1_stage2 0x240000 {
  ipa1 |-> pa1;
  ipa2 |-> invalid;
  s1table vm1_stage1;
}
s2table vm2_stage2 0x280000 {
  ipa1 |-> invalid;
  ipa2 |-> pa2;
  s1table vm2_stage1;
}
*pa2 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\pKVMdotvcpurunN}
\settowidth{\pKVMdotvcpurunN}{\usebox{\pKVMdotvcpurunM}}
\newsavebox{\pKVMdotvcpurunO}
\begin{lrbox}{\pKVMdotvcpurunO}
\begin{tabular}{l}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x1000|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00101|\\
\lstinline[language=IslaLitmusExp]|TTBR0_EL1=ttbr(asid=0x00,base=vm1_stage1)|\\
\lstinline[language=IslaLitmusExp]|R0=ttbr(asid=0x00,base=vm2_stage1)|\\
\lstinline[language=IslaLitmusExp]|VTTBR_EL2=ttbr(vmid=0x0001,base=vm1_stage2)|\\
\lstinline[language=IslaLitmusExp]|R1=ttbr(base=vm2_stage2,vmid=0x0002)|\\
\lstinline[language=IslaLitmusExp]|TTBR0_EL2=ttbr(base=hyp_map,asid=0x00)|\\
\end{tabular}
\end{lrbox}
\newlength{\pKVMdotvcpurunJJ}
\settowidth{\pKVMdotvcpurunJJ}{\usebox{\pKVMdotvcpurunO}}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|pKVM.vcpu_run|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\pKVMdotvcpurunN}%
  %\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}
  \vspace*{-5\baselineskip}%
  Page table setup:\\\usebox{\pKVMdotvcpurunM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\pKVMdotvcpurunO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\pKVMdotvcpurunI}\\
  \cline{2-2}
  & thread0 el2 handler\\
  \cline{2-2}
  & \usebox{\pKVMdotvcpurunK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/Makefile <==
pdfs:
	$(MAKE) -C diagrams/ pdfs
.PHONY: pdfs

ALL_RESULTS = $(wildcard results_strong/*.toml.result)

most_recent_legion_ref = $(shell ls -1 legion-refs/*.tar.gz 2>/dev/null | sort | tail -1)
legion-refs/%/: legion-refs/%.tar.gz
	tar -xvf $(most_recent_legion_ref) -C legion-refs/
	mkdir -p dots/
	cp -r $@/dots/* diagrams/dots/
	cp $@/latex/* ../tests/tex/
	cp $@/results_* .
	$(MAKE) clean_results results_strong/ results_ETS/ pdfs pgtable_table.tex pkvm_table.tex
	python3 rename_diagram_pdfs.py

unpack_legion_refs: $(basename $(basename $(most_recent_legion_ref)))/

clean_results:
	sed 's/\.\..*//' -i results_strong.txt
	sed 's/Execution.*//' -i results_strong.txt
	sed 's/Makefile.*//' -i results_strong.txt
	sed 's/\.\..*//' -i results_ETS.txt
	sed 's/Execution.*//' -i results_ETS.txt
	sed 's/Makefile.*//' -i results_ETS.txt
.PHONY: clean_results

results_strong/:
	python3 make_results_files.py results_strong.txt
.PHONY: results_strong/

results_ETS/:
	python3 make_results_files.py results_ETS.txt
.PHONY: results_ETS/

pkvm_table.tex: results_pkvm.txt
	python3 make_results_table.py $@ results_$*.txt

pgtable_table.tex: results_strong.txt results_ETS.txt
	python3 make_results_table.py $@ $^

ALWAYS:
.PHONY: ALWAYS

clean:
	@rm -f results_ETS.txt
	@rm -rf results_ETS/
	@rm -f results_strong.txt
	@rm -rf results_strong/
	@rm -f results_pkvm.txt
	@rm -rf results_pkvm/
	@rm -f results_allow_all.txt
	@rm -f strong_table.tex pkvm_table.tex table.tex
.PHONY: clean

==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/BBM+dsb-tlbiis-dsb.tex <==
\newlength{\BBMplusdsbtlbiisdsbH}
\setlength{\BBMplusdsbtlbiisdsbH}{0cm}
\newsavebox{\BBMplusdsbtlbiisdsbI}
\begin{lrbox}{\BBMplusdsbtlbiisdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X6
DSB SY
STR X2,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\BBMplusdsbtlbiisdsbJ}
\settowidth{\BBMplusdsbtlbiisdsbJ}{\usebox{\BBMplusdsbtlbiisdsbI}}
\addtolength{\BBMplusdsbtlbiisdsbH}{\BBMplusdsbtlbiisdsbJ}
\newsavebox{\BBMplusdsbtlbiisdsbK}
\begin{lrbox}{\BBMplusdsbtlbiisdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\BBMplusdsbtlbiisdsbL}
\settowidth{\BBMplusdsbtlbiisdsbL}{\usebox{\BBMplusdsbtlbiisdsbK}}
\addtolength{\BBMplusdsbtlbiisdsbH}{\BBMplusdsbtlbiisdsbL}
\newsavebox{\BBMplusdsbtlbiisdsbM}
\begin{lrbox}{\BBMplusdsbtlbiisdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\BBMplusdsbtlbiisdsbN}
\settowidth{\BBMplusdsbtlbiisdsbN}{\usebox{\BBMplusdsbtlbiisdsbM}}
\addtolength{\BBMplusdsbtlbiisdsbH}{\BBMplusdsbtlbiisdsbN}
\newsavebox{\BBMplusdsbtlbiisdsbO}
\begin{lrbox}{\BBMplusdsbtlbiisdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;
    x ?-> pa2;

    identity 0x1000 with code;

    *pa2 = 2;
\end{lstlisting}
\end{lrbox}
\newlength{\BBMplusdsbtlbiisdsbP}
\settowidth{\BBMplusdsbtlbiisdsbP}{\usebox{\BBMplusdsbtlbiisdsbO}}
\newsavebox{\BBMplusdsbtlbiisdsbA}
\begin{lrbox}{\BBMplusdsbtlbiisdsbA}
\begin{minipage}{\BBMplusdsbtlbiisdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R4=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|BBM+dsb-tlbiis-dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\BBMplusdsbtlbiisdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\BBMplusdsbtlbiisdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\BBMplusdsbtlbiisdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\BBMplusdsbtlbiisdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\BBMplusdsbtlbiisdsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\BBMplusdsbtlbiisdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/BBM.Tf+dsb-tlbiis-dsb.tex <==
\newlength{\BBMdotTfplusdsbtlbiisdsbH}
\setlength{\BBMdotTfplusdsbtlbiisdsbH}{0cm}
\newsavebox{\BBMdotTfplusdsbtlbiisdsbI}
\begin{lrbox}{\BBMdotTfplusdsbtlbiisdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X6
DSB SY
STR X2,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\BBMdotTfplusdsbtlbiisdsbJ}
\settowidth{\BBMdotTfplusdsbtlbiisdsbJ}{\usebox{\BBMdotTfplusdsbtlbiisdsbI}}
\addtolength{\BBMdotTfplusdsbtlbiisdsbH}{\BBMdotTfplusdsbtlbiisdsbJ}
\newsavebox{\BBMdotTfplusdsbtlbiisdsbK}
\begin{lrbox}{\BBMdotTfplusdsbtlbiisdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\BBMdotTfplusdsbtlbiisdsbL}
\settowidth{\BBMdotTfplusdsbtlbiisdsbL}{\usebox{\BBMdotTfplusdsbtlbiisdsbK}}
\addtolength{\BBMdotTfplusdsbtlbiisdsbH}{\BBMdotTfplusdsbtlbiisdsbL}
\newsavebox{\BBMdotTfplusdsbtlbiisdsbM}
\begin{lrbox}{\BBMdotTfplusdsbtlbiisdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
\end{lstlisting}
\end{lrbox}
\newlength{\BBMdotTfplusdsbtlbiisdsbN}
\settowidth{\BBMdotTfplusdsbtlbiisdsbN}{\usebox{\BBMdotTfplusdsbtlbiisdsbM}}
\addtolength{\BBMdotTfplusdsbtlbiisdsbH}{\BBMdotTfplusdsbtlbiisdsbN}
\newsavebox{\BBMdotTfplusdsbtlbiisdsbO}
\begin{lrbox}{\BBMdotTfplusdsbtlbiisdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;
    x ?-> pa2;

    identity 0x1000 with code;

    *pa2 = 2;
\end{lstlisting}
\end{lrbox}
\newlength{\BBMdotTfplusdsbtlbiisdsbP}
\settowidth{\BBMdotTfplusdsbtlbiisdsbP}{\usebox{\BBMdotTfplusdsbtlbiisdsbO}}
\newsavebox{\BBMdotTfplusdsbtlbiisdsbA}
\begin{lrbox}{\BBMdotTfplusdsbtlbiisdsbA}
\begin{minipage}{\BBMdotTfplusdsbtlbiisdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R4=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|BBM.Tf+dsb-tlbiis-dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\BBMdotTfplusdsbtlbiisdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\BBMdotTfplusdsbtlbiisdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\BBMdotTfplusdsbtlbiisdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\BBMdotTfplusdsbtlbiisdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\BBMdotTfplusdsbtlbiisdsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\BBMdotTfplusdsbtlbiisdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/Break2.news1.tex <==
\newlength{\BreaktwodotnewsoneH}
\setlength{\BreaktwodotnewsoneH}{0cm}
\newsavebox{\BreaktwodotnewsoneI}
\begin{lrbox}{\BreaktwodotnewsoneI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1IS,X4
DSB SY
TLBI VMALLE1IS
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\BreaktwodotnewsoneJ}
\settowidth{\BreaktwodotnewsoneJ}{\usebox{\BreaktwodotnewsoneI}}
\addtolength{\BreaktwodotnewsoneH}{\BreaktwodotnewsoneJ}
\newsavebox{\BreaktwodotnewsoneK}
\begin{lrbox}{\BreaktwodotnewsoneK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\BreaktwodotnewsoneL}
\settowidth{\BreaktwodotnewsoneL}{\usebox{\BreaktwodotnewsoneK}}
\addtolength{\BreaktwodotnewsoneH}{\BreaktwodotnewsoneL}
\newsavebox{\BreaktwodotnewsoneM}
\begin{lrbox}{\BreaktwodotnewsoneM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#2
\end{lstlisting}
\end{lrbox}
\newlength{\BreaktwodotnewsoneN}
\settowidth{\BreaktwodotnewsoneN}{\usebox{\BreaktwodotnewsoneM}}
\addtolength{\BreaktwodotnewsoneH}{\BreaktwodotnewsoneN}
\newsavebox{\BreaktwodotnewsoneO}
\begin{lrbox}{\BreaktwodotnewsoneO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X0,#3
\end{lstlisting}
\end{lrbox}
\newlength{\BreaktwodotnewsoneP}
\settowidth{\BreaktwodotnewsoneP}{\usebox{\BreaktwodotnewsoneO}}
\addtolength{\BreaktwodotnewsoneH}{\BreaktwodotnewsoneP}
\newsavebox{\BreaktwodotnewsoneA}
\begin{lrbox}{\BreaktwodotnewsoneA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
option default_tables = false;
physical pa1;
intermediate ipa1;

s2table vm_stage2 0x240000  {
    ipa1 |-> pa1 at level 3;
    ipa1 ?-> invalid at level 3;
    identity pa_to_ipa(0x1000) with code;


    s1table vm_stage1 0x280000  {
        x |-> invalid at level 3;
        x ?-> ipa1 at level 3;

        identity pa_to_va(0x1000) with code;
    }
}

s1table hyp_map 0x200000 {
    identity 0x2000 with code;
    s2table vm_stage2;
    s1table vm_stage1;
}

*pa1 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\BreaktwodotnewsoneB}
\settowidth{\BreaktwodotnewsoneB}{\usebox{\BreaktwodotnewsoneA}}
\newsavebox{\BreaktwodotnewsoneC}
\begin{lrbox}{\BreaktwodotnewsoneC}
\begin{minipage}{\BreaktwodotnewsoneH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(ipa1,vm_stage2)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=ipa1)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(x,vm_stage1)|\\
\lstinline[language=IslaLitmusExp]|0:R4=bvlshr(ipa1,0xC)|\\
\lstinline[language=IslaLitmusExp]|0:TTBR0_EL2=ttbr(base=hyp_map,asid=0x0000)|\\
\lstinline[language=IslaLitmusExp]|0:VTTBR_EL2=ttbr(base=vm_stage2,vmid=0x0000)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:TTBR0_EL1=ttbr(asid=0x0000,base=vm_stage1)|\\
\lstinline[language=IslaLitmusExp]|1:TTBR0_EL2=ttbr(base=hyp_map,asid=0x0000)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\lstinline[language=IslaLitmusExp]|1:VTTBR_EL2=ttbr(vmid=0x0000,base=vm_stage2)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|Break2.news1|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\BreaktwodotnewsoneB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\BreaktwodotnewsoneA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\BreaktwodotnewsoneC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\BreaktwodotnewsoneI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\BreaktwodotnewsoneK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\BreaktwodotnewsoneM}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\BreaktwodotnewsoneO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoRR0.alias+po.tex <==
\newlength{\CoRRzerodotaliaspluspoH}
\setlength{\CoRRzerodotaliaspluspoH}{0cm}
\newsavebox{\CoRRzerodotaliaspluspoI}
\begin{lrbox}{\CoRRzerodotaliaspluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRRzerodotaliaspluspoJ}
\settowidth{\CoRRzerodotaliaspluspoJ}{\usebox{\CoRRzerodotaliaspluspoI}}
\addtolength{\CoRRzerodotaliaspluspoH}{\CoRRzerodotaliaspluspoJ}
\newsavebox{\CoRRzerodotaliaspluspoK}
\begin{lrbox}{\CoRRzerodotaliaspluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRRzerodotaliaspluspoL}
\settowidth{\CoRRzerodotaliaspluspoL}{\usebox{\CoRRzerodotaliaspluspoK}}
\addtolength{\CoRRzerodotaliaspluspoH}{\CoRRzerodotaliaspluspoL}
\newsavebox{\CoRRzerodotaliaspluspoM}
\begin{lrbox}{\CoRRzerodotaliaspluspoM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    y |-> pa1;
    *pa1 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRRzerodotaliaspluspoN}
\settowidth{\CoRRzerodotaliaspluspoN}{\usebox{\CoRRzerodotaliaspluspoM}}
\newsavebox{\CoRRzerodotaliaspluspoO}
\begin{lrbox}{\CoRRzerodotaliaspluspoO}
\begin{minipage}{\CoRRzerodotaliaspluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRR0.alias+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRRzerodotaliaspluspoN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRRzerodotaliaspluspoM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRRzerodotaliaspluspoO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRRzerodotaliaspluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRRzerodotaliaspluspoK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoRR2.alias+po.tex <==
\newlength{\CoRRtwodotaliaspluspoH}
\setlength{\CoRRtwodotaliaspluspoH}{0cm}
\newsavebox{\CoRRtwodotaliaspluspoI}
\begin{lrbox}{\CoRRtwodotaliaspluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRRtwodotaliaspluspoJ}
\settowidth{\CoRRtwodotaliaspluspoJ}{\usebox{\CoRRtwodotaliaspluspoI}}
\addtolength{\CoRRtwodotaliaspluspoH}{\CoRRtwodotaliaspluspoJ}
\newsavebox{\CoRRtwodotaliaspluspoK}
\begin{lrbox}{\CoRRtwodotaliaspluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRRtwodotaliaspluspoL}
\settowidth{\CoRRtwodotaliaspluspoL}{\usebox{\CoRRtwodotaliaspluspoK}}
\addtolength{\CoRRtwodotaliaspluspoH}{\CoRRtwodotaliaspluspoL}
\newsavebox{\CoRRtwodotaliaspluspoM}
\begin{lrbox}{\CoRRtwodotaliaspluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRRtwodotaliaspluspoN}
\settowidth{\CoRRtwodotaliaspluspoN}{\usebox{\CoRRtwodotaliaspluspoM}}
\addtolength{\CoRRtwodotaliaspluspoH}{\CoRRtwodotaliaspluspoN}
\newsavebox{\CoRRtwodotaliaspluspoO}
\begin{lrbox}{\CoRRtwodotaliaspluspoO}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRRtwodotaliaspluspoP}
\settowidth{\CoRRtwodotaliaspluspoP}{\usebox{\CoRRtwodotaliaspluspoO}}
\addtolength{\CoRRtwodotaliaspluspoH}{\CoRRtwodotaliaspluspoP}
\newsavebox{\CoRRtwodotaliaspluspoA}
\begin{lrbox}{\CoRRtwodotaliaspluspoA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    u |-> pa1;
    v |-> pa1;
    w |-> pa1;
    x |-> pa1;
    y |-> pa1;
    z |-> pa1;
    *pa1 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRRtwodotaliaspluspoB}
\settowidth{\CoRRtwodotaliaspluspoB}{\usebox{\CoRRtwodotaliaspluspoA}}
\newsavebox{\CoRRtwodotaliaspluspoC}
\begin{lrbox}{\CoRRtwodotaliaspluspoC}
\begin{minipage}{\CoRRtwodotaliaspluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R1=u|\\
\lstinline[language=IslaLitmusExp]|1:R0=0b10|\\
\lstinline[language=IslaLitmusExp]|1:R1=v|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=w|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|3:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|3:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|3:R1=y|\\
\lstinline[language=IslaLitmusExp]|3:R3=z|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRR2.alias+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRRtwodotaliaspluspoB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRRtwodotaliaspluspoA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRRtwodotaliaspluspoC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRRtwodotaliaspluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRRtwodotaliaspluspoK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\CoRRtwodotaliaspluspoM}\\
  \cline{2-2}
  & Thread 3\\
  \cline{2-2}
  & \usebox{\CoRRtwodotaliaspluspoO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|2:R0=1 & 2:R2=2 & 3:R0=2 & 3:R2=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoRT.inv+addr-trfi.tex <==
\newlength{\CoRTdotinvplusaddrtrfiH}
\setlength{\CoRTdotinvplusaddrtrfiH}{0cm}
\newsavebox{\CoRTdotinvplusaddrtrfiI}
\begin{lrbox}{\CoRTdotinvplusaddrtrfiI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRTdotinvplusaddrtrfiJ}
\settowidth{\CoRTdotinvplusaddrtrfiJ}{\usebox{\CoRTdotinvplusaddrtrfiI}}
\addtolength{\CoRTdotinvplusaddrtrfiH}{\CoRTdotinvplusaddrtrfiJ}
\newsavebox{\CoRTdotinvplusaddrtrfiK}
\begin{lrbox}{\CoRTdotinvplusaddrtrfiK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
STR X3,[X4,X2]
LDR X5,[X6]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRTdotinvplusaddrtrfiL}
\settowidth{\CoRTdotinvplusaddrtrfiL}{\usebox{\CoRTdotinvplusaddrtrfiK}}
\addtolength{\CoRTdotinvplusaddrtrfiH}{\CoRTdotinvplusaddrtrfiL}
\newsavebox{\CoRTdotinvplusaddrtrfiM}
\begin{lrbox}{\CoRTdotinvplusaddrtrfiM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X5,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoRTdotinvplusaddrtrfiN}
\settowidth{\CoRTdotinvplusaddrtrfiN}{\usebox{\CoRTdotinvplusaddrtrfiM}}
\addtolength{\CoRTdotinvplusaddrtrfiH}{\CoRTdotinvplusaddrtrfiN}
\newsavebox{\CoRTdotinvplusaddrtrfiO}
\begin{lrbox}{\CoRTdotinvplusaddrtrfiO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    y |-> invalid;
    y ?-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRTdotinvplusaddrtrfiP}
\settowidth{\CoRTdotinvplusaddrtrfiP}{\usebox{\CoRTdotinvplusaddrtrfiO}}
\newsavebox{\CoRTdotinvplusaddrtrfiA}
\begin{lrbox}{\CoRTdotinvplusaddrtrfiA}
\begin{minipage}{\CoRTdotinvplusaddrtrfiH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|1:R4=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R6=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRT.inv+addr-trfi|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRTdotinvplusaddrtrfiP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRTdotinvplusaddrtrfiO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRTdotinvplusaddrtrfiA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRTdotinvplusaddrtrfiI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRTdotinvplusaddrtrfiK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoRTdotinvplusaddrtrfiM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|true|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoRpteT+dsb-isb.tex <==
\newlength{\CoRpteTplusdsbisbH}
\setlength{\CoRpteTplusdsbisbH}{0cm}
\newsavebox{\CoRpteTplusdsbisbI}
\begin{lrbox}{\CoRpteTplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTplusdsbisbJ}
\settowidth{\CoRpteTplusdsbisbJ}{\usebox{\CoRpteTplusdsbisbI}}
\addtolength{\CoRpteTplusdsbisbH}{\CoRpteTplusdsbisbJ}
\newsavebox{\CoRpteTplusdsbisbK}
\begin{lrbox}{\CoRpteTplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTplusdsbisbL}
\settowidth{\CoRpteTplusdsbisbL}{\usebox{\CoRpteTplusdsbisbK}}
\addtolength{\CoRpteTplusdsbisbH}{\CoRpteTplusdsbisbL}
\newsavebox{\CoRpteTplusdsbisbM}
\begin{lrbox}{\CoRpteTplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTplusdsbisbN}
\settowidth{\CoRpteTplusdsbisbN}{\usebox{\CoRpteTplusdsbisbM}}
\addtolength{\CoRpteTplusdsbisbH}{\CoRpteTplusdsbisbN}
\newsavebox{\CoRpteTplusdsbisbO}
\begin{lrbox}{\CoRpteTplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;

    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;

    *pa1 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTplusdsbisbP}
\settowidth{\CoRpteTplusdsbisbP}{\usebox{\CoRpteTplusdsbisbO}}
\newsavebox{\CoRpteTplusdsbisbA}
\begin{lrbox}{\CoRpteTplusdsbisbA}
\begin{minipage}{\CoRpteTplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRpteT+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRpteTplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRpteTplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRpteTplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRpteTplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRpteTplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoRpteTplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=0 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoRpteT+dsb.tex <==
\newlength{\CoRpteTplusdsbH}
\setlength{\CoRpteTplusdsbH}{0cm}
\newsavebox{\CoRpteTplusdsbI}
\begin{lrbox}{\CoRpteTplusdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTplusdsbJ}
\settowidth{\CoRpteTplusdsbJ}{\usebox{\CoRpteTplusdsbI}}
\addtolength{\CoRpteTplusdsbH}{\CoRpteTplusdsbJ}
\newsavebox{\CoRpteTplusdsbK}
\begin{lrbox}{\CoRpteTplusdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTplusdsbL}
\settowidth{\CoRpteTplusdsbL}{\usebox{\CoRpteTplusdsbK}}
\addtolength{\CoRpteTplusdsbH}{\CoRpteTplusdsbL}
\newsavebox{\CoRpteTplusdsbM}
\begin{lrbox}{\CoRpteTplusdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTplusdsbN}
\settowidth{\CoRpteTplusdsbN}{\usebox{\CoRpteTplusdsbM}}
\addtolength{\CoRpteTplusdsbH}{\CoRpteTplusdsbN}
\newsavebox{\CoRpteTplusdsbO}
\begin{lrbox}{\CoRpteTplusdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;

    *x = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTplusdsbP}
\settowidth{\CoRpteTplusdsbP}{\usebox{\CoRpteTplusdsbO}}
\newsavebox{\CoRpteTplusdsbA}
\begin{lrbox}{\CoRpteTplusdsbA}
\begin{minipage}{\CoRpteTplusdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRpteT+dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRpteTplusdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRpteTplusdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRpteTplusdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRpteTplusdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRpteTplusdsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoRpteTplusdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=0 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoRpteT.EL1+dsb-tlbi-dsb-isb.tex <==
\newlength{\CoRpteTdotELoneplusdsbtlbidsbisbH}
\setlength{\CoRpteTdotELoneplusdsbtlbidsbisbH}{0cm}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbisbI}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTdotELoneplusdsbtlbidsbisbJ}
\settowidth{\CoRpteTdotELoneplusdsbtlbidsbisbJ}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbisbI}}
\addtolength{\CoRpteTdotELoneplusdsbtlbidsbisbH}{\CoRpteTdotELoneplusdsbtlbidsbisbJ}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbisbK}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
TLBI VAE1,X4
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTdotELoneplusdsbtlbidsbisbL}
\settowidth{\CoRpteTdotELoneplusdsbtlbidsbisbL}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbisbK}}
\addtolength{\CoRpteTdotELoneplusdsbtlbidsbisbH}{\CoRpteTdotELoneplusdsbtlbidsbisbL}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbisbM}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTdotELoneplusdsbtlbidsbisbN}
\settowidth{\CoRpteTdotELoneplusdsbtlbidsbisbN}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbisbM}}
\addtolength{\CoRpteTdotELoneplusdsbtlbidsbisbH}{\CoRpteTdotELoneplusdsbtlbidsbisbN}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbisbO}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;

    *pa1 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTdotELoneplusdsbtlbidsbisbP}
\settowidth{\CoRpteTdotELoneplusdsbtlbidsbisbP}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbisbO}}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbisbA}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbisbA}
\begin{minipage}{\CoRpteTdotELoneplusdsbtlbidsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRpteT.EL1+dsb-tlbi-dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRpteTdotELoneplusdsbtlbidsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRpteTdotELoneplusdsbtlbidsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRpteTdotELoneplusdsbtlbidsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRpteTdotELoneplusdsbtlbidsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoRpteTdotELoneplusdsbtlbidsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=0 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoRpteT.EL1+dsb-tlbi-dsb.tex <==
\newlength{\CoRpteTdotELoneplusdsbtlbidsbH}
\setlength{\CoRpteTdotELoneplusdsbtlbidsbH}{0cm}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbI}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTdotELoneplusdsbtlbidsbJ}
\settowidth{\CoRpteTdotELoneplusdsbtlbidsbJ}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbI}}
\addtolength{\CoRpteTdotELoneplusdsbtlbidsbH}{\CoRpteTdotELoneplusdsbtlbidsbJ}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbK}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
TLBI VAE1,X4
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTdotELoneplusdsbtlbidsbL}
\settowidth{\CoRpteTdotELoneplusdsbtlbidsbL}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbK}}
\addtolength{\CoRpteTdotELoneplusdsbtlbidsbH}{\CoRpteTdotELoneplusdsbtlbidsbL}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbM}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTdotELoneplusdsbtlbidsbN}
\settowidth{\CoRpteTdotELoneplusdsbtlbidsbN}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbM}}
\addtolength{\CoRpteTdotELoneplusdsbtlbidsbH}{\CoRpteTdotELoneplusdsbtlbidsbN}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbO}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;

    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;

    *pa1 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTdotELoneplusdsbtlbidsbP}
\settowidth{\CoRpteTdotELoneplusdsbtlbidsbP}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbO}}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbA}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbA}
\begin{minipage}{\CoRpteTdotELoneplusdsbtlbidsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRpteT.EL1+dsb-tlbi-dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRpteTdotELoneplusdsbtlbidsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRpteTdotELoneplusdsbtlbidsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRpteTdotELoneplusdsbtlbidsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRpteTdotELoneplusdsbtlbidsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoRpteTdotELoneplusdsbtlbidsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=0 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoRpteTf.inv+dsb-isb.tex <==
\newlength{\CoRpteTfdotinvplusdsbisbH}
\setlength{\CoRpteTfdotinvplusdsbisbH}{0cm}
\newsavebox{\CoRpteTfdotinvplusdsbisbI}
\begin{lrbox}{\CoRpteTfdotinvplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTfdotinvplusdsbisbJ}
\settowidth{\CoRpteTfdotinvplusdsbisbJ}{\usebox{\CoRpteTfdotinvplusdsbisbI}}
\addtolength{\CoRpteTfdotinvplusdsbisbH}{\CoRpteTfdotinvplusdsbisbJ}
\newsavebox{\CoRpteTfdotinvplusdsbisbK}
\begin{lrbox}{\CoRpteTfdotinvplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTfdotinvplusdsbisbL}
\settowidth{\CoRpteTfdotinvplusdsbisbL}{\usebox{\CoRpteTfdotinvplusdsbisbK}}
\addtolength{\CoRpteTfdotinvplusdsbisbH}{\CoRpteTfdotinvplusdsbisbL}
\newsavebox{\CoRpteTfdotinvplusdsbisbM}
\begin{lrbox}{\CoRpteTfdotinvplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTfdotinvplusdsbisbN}
\settowidth{\CoRpteTfdotinvplusdsbisbN}{\usebox{\CoRpteTfdotinvplusdsbisbM}}
\addtolength{\CoRpteTfdotinvplusdsbisbH}{\CoRpteTfdotinvplusdsbisbN}
\newsavebox{\CoRpteTfdotinvplusdsbisbO}
\begin{lrbox}{\CoRpteTfdotinvplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    option default_tables = true;
    physical pa1;
    intermediate ipa1;

    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    identity 0x1000 with code;

    *pa1 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTfdotinvplusdsbisbP}
\settowidth{\CoRpteTfdotinvplusdsbisbP}{\usebox{\CoRpteTfdotinvplusdsbisbO}}
\newsavebox{\CoRpteTfdotinvplusdsbisbA}
\begin{lrbox}{\CoRpteTfdotinvplusdsbisbA}
\begin{minipage}{\CoRpteTfdotinvplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRpteTf.inv+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRpteTfdotinvplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRpteTfdotinvplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRpteTfdotinvplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRpteTfdotinvplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRpteTfdotinvplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoRpteTfdotinvplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=desc3(y,page_table_base) & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoRpteTf.inv+dsb.tex <==
\newlength{\CoRpteTfdotinvplusdsbH}
\setlength{\CoRpteTfdotinvplusdsbH}{0cm}
\newsavebox{\CoRpteTfdotinvplusdsbI}
\begin{lrbox}{\CoRpteTfdotinvplusdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTfdotinvplusdsbJ}
\settowidth{\CoRpteTfdotinvplusdsbJ}{\usebox{\CoRpteTfdotinvplusdsbI}}
\addtolength{\CoRpteTfdotinvplusdsbH}{\CoRpteTfdotinvplusdsbJ}
\newsavebox{\CoRpteTfdotinvplusdsbK}
\begin{lrbox}{\CoRpteTfdotinvplusdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTfdotinvplusdsbL}
\settowidth{\CoRpteTfdotinvplusdsbL}{\usebox{\CoRpteTfdotinvplusdsbK}}
\addtolength{\CoRpteTfdotinvplusdsbH}{\CoRpteTfdotinvplusdsbL}
\newsavebox{\CoRpteTfdotinvplusdsbM}
\begin{lrbox}{\CoRpteTfdotinvplusdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTfdotinvplusdsbN}
\settowidth{\CoRpteTfdotinvplusdsbN}{\usebox{\CoRpteTfdotinvplusdsbM}}
\addtolength{\CoRpteTfdotinvplusdsbH}{\CoRpteTfdotinvplusdsbN}
\newsavebox{\CoRpteTfdotinvplusdsbO}
\begin{lrbox}{\CoRpteTfdotinvplusdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    identity 0x1000 with code;

    *pa1 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTfdotinvplusdsbP}
\settowidth{\CoRpteTfdotinvplusdsbP}{\usebox{\CoRpteTfdotinvplusdsbO}}
\newsavebox{\CoRpteTfdotinvplusdsbA}
\begin{lrbox}{\CoRpteTfdotinvplusdsbA}
\begin{minipage}{\CoRpteTfdotinvplusdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRpteTf.inv+dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRpteTfdotinvplusdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRpteTfdotinvplusdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRpteTfdotinvplusdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRpteTfdotinvplusdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRpteTfdotinvplusdsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoRpteTfdotinvplusdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=desc3(y,page_table_base) & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoTRpte.inv+dsb-isb.tex <==
\newlength{\CoTRptedotinvplusdsbisbH}
\setlength{\CoTRptedotinvplusdsbisbH}{0cm}
\newsavebox{\CoTRptedotinvplusdsbisbI}
\begin{lrbox}{\CoTRptedotinvplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvplusdsbisbJ}
\settowidth{\CoTRptedotinvplusdsbisbJ}{\usebox{\CoTRptedotinvplusdsbisbI}}
\addtolength{\CoTRptedotinvplusdsbisbH}{\CoTRptedotinvplusdsbisbJ}
\newsavebox{\CoTRptedotinvplusdsbisbK}
\begin{lrbox}{\CoTRptedotinvplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvplusdsbisbL}
\settowidth{\CoTRptedotinvplusdsbisbL}{\usebox{\CoTRptedotinvplusdsbisbK}}
\addtolength{\CoTRptedotinvplusdsbisbH}{\CoTRptedotinvplusdsbisbL}
\newsavebox{\CoTRptedotinvplusdsbisbM}
\begin{lrbox}{\CoTRptedotinvplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvplusdsbisbN}
\settowidth{\CoTRptedotinvplusdsbisbN}{\usebox{\CoTRptedotinvplusdsbisbM}}
\addtolength{\CoTRptedotinvplusdsbisbH}{\CoTRptedotinvplusdsbisbN}
\newsavebox{\CoTRptedotinvplusdsbisbO}
\begin{lrbox}{\CoTRptedotinvplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvplusdsbisbP}
\settowidth{\CoTRptedotinvplusdsbisbP}{\usebox{\CoTRptedotinvplusdsbisbO}}
\newsavebox{\CoTRptedotinvplusdsbisbA}
\begin{lrbox}{\CoTRptedotinvplusdsbisbA}
\begin{minipage}{\CoTRptedotinvplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTRpte.inv+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTRptedotinvplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTRptedotinvplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTRptedotinvplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoTRpte.inv+dsb.tex <==
\newlength{\CoTRptedotinvplusdsbH}
\setlength{\CoTRptedotinvplusdsbH}{0cm}
\newsavebox{\CoTRptedotinvplusdsbI}
\begin{lrbox}{\CoTRptedotinvplusdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvplusdsbJ}
\settowidth{\CoTRptedotinvplusdsbJ}{\usebox{\CoTRptedotinvplusdsbI}}
\addtolength{\CoTRptedotinvplusdsbH}{\CoTRptedotinvplusdsbJ}
\newsavebox{\CoTRptedotinvplusdsbK}
\begin{lrbox}{\CoTRptedotinvplusdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvplusdsbL}
\settowidth{\CoTRptedotinvplusdsbL}{\usebox{\CoTRptedotinvplusdsbK}}
\addtolength{\CoTRptedotinvplusdsbH}{\CoTRptedotinvplusdsbL}
\newsavebox{\CoTRptedotinvplusdsbM}
\begin{lrbox}{\CoTRptedotinvplusdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvplusdsbN}
\settowidth{\CoTRptedotinvplusdsbN}{\usebox{\CoTRptedotinvplusdsbM}}
\addtolength{\CoTRptedotinvplusdsbH}{\CoTRptedotinvplusdsbN}
\newsavebox{\CoTRptedotinvplusdsbO}
\begin{lrbox}{\CoTRptedotinvplusdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *y = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvplusdsbP}
\settowidth{\CoTRptedotinvplusdsbP}{\usebox{\CoTRptedotinvplusdsbO}}
\newsavebox{\CoTRptedotinvplusdsbA}
\begin{lrbox}{\CoTRptedotinvplusdsbA}
\begin{minipage}{\CoTRptedotinvplusdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTRpte.inv+dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTRptedotinvplusdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTRptedotinvplusdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTRptedotinvplusdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvplusdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvplusdsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvplusdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoTRpte.inv+po.tex <==
\newlength{\CoTRptedotinvpluspoH}
\setlength{\CoTRptedotinvpluspoH}{0cm}
\newsavebox{\CoTRptedotinvpluspoI}
\begin{lrbox}{\CoTRptedotinvpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvpluspoJ}
\settowidth{\CoTRptedotinvpluspoJ}{\usebox{\CoTRptedotinvpluspoI}}
\addtolength{\CoTRptedotinvpluspoH}{\CoTRptedotinvpluspoJ}
\newsavebox{\CoTRptedotinvpluspoK}
\begin{lrbox}{\CoTRptedotinvpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvpluspoL}
\settowidth{\CoTRptedotinvpluspoL}{\usebox{\CoTRptedotinvpluspoK}}
\addtolength{\CoTRptedotinvpluspoH}{\CoTRptedotinvpluspoL}
\newsavebox{\CoTRptedotinvpluspoM}
\begin{lrbox}{\CoTRptedotinvpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvpluspoN}
\settowidth{\CoTRptedotinvpluspoN}{\usebox{\CoTRptedotinvpluspoM}}
\addtolength{\CoTRptedotinvpluspoH}{\CoTRptedotinvpluspoN}
\newsavebox{\CoTRptedotinvpluspoO}
\begin{lrbox}{\CoTRptedotinvpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *y = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvpluspoP}
\settowidth{\CoTRptedotinvpluspoP}{\usebox{\CoTRptedotinvpluspoO}}
\newsavebox{\CoTRptedotinvpluspoA}
\begin{lrbox}{\CoTRptedotinvpluspoA}
\begin{minipage}{\CoTRptedotinvpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTRpte.inv+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTRptedotinvpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTRptedotinvpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTRptedotinvpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoTT.ro+dmb.tex <==
\newlength{\CoTTdotroplusdmbH}
\setlength{\CoTTdotroplusdmbH}{0cm}
\newsavebox{\CoTTdotroplusdmbI}
\begin{lrbox}{\CoTTdotroplusdmbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotroplusdmbJ}
\settowidth{\CoTTdotroplusdmbJ}{\usebox{\CoTTdotroplusdmbI}}
\addtolength{\CoTTdotroplusdmbH}{\CoTTdotroplusdmbJ}
\newsavebox{\CoTTdotroplusdmbK}
\begin{lrbox}{\CoTTdotroplusdmbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotroplusdmbL}
\settowidth{\CoTTdotroplusdmbL}{\usebox{\CoTTdotroplusdmbK}}
\addtolength{\CoTTdotroplusdmbH}{\CoTTdotroplusdmbL}
\newsavebox{\CoTTdotroplusdmbM}
\begin{lrbox}{\CoTTdotroplusdmbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1 with [AP = 0b11] and default;
    x ?-> pa2 with [AP = 0b11] and default;
    y |-> pa2 with [AP = 0b11] and default;

    *pa2 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotroplusdmbN}
\settowidth{\CoTTdotroplusdmbN}{\usebox{\CoTTdotroplusdmbM}}
\newsavebox{\CoTTdotroplusdmbO}
\begin{lrbox}{\CoTTdotroplusdmbO}
\begin{minipage}{\CoTTdotroplusdmbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTT.ro+dmb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTTdotroplusdmbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTTdotroplusdmbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTTdotroplusdmbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTTdotroplusdmbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTTdotroplusdmbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoTT.ro+dsb-isb.tex <==
\newlength{\CoTTdotroplusdsbisbH}
\setlength{\CoTTdotroplusdsbisbH}{0cm}
\newsavebox{\CoTTdotroplusdsbisbI}
\begin{lrbox}{\CoTTdotroplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotroplusdsbisbJ}
\settowidth{\CoTTdotroplusdsbisbJ}{\usebox{\CoTTdotroplusdsbisbI}}
\addtolength{\CoTTdotroplusdsbisbH}{\CoTTdotroplusdsbisbJ}
\newsavebox{\CoTTdotroplusdsbisbK}
\begin{lrbox}{\CoTTdotroplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotroplusdsbisbL}
\settowidth{\CoTTdotroplusdsbisbL}{\usebox{\CoTTdotroplusdsbisbK}}
\addtolength{\CoTTdotroplusdsbisbH}{\CoTTdotroplusdsbisbL}
\newsavebox{\CoTTdotroplusdsbisbM}
\begin{lrbox}{\CoTTdotroplusdsbisbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1 with [AP = 0b11] and default;
    x ?-> pa2 with [AP = 0b11] and default;
    y |-> pa2 with [AP = 0b11] and default;

    *pa2 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotroplusdsbisbN}
\settowidth{\CoTTdotroplusdsbisbN}{\usebox{\CoTTdotroplusdsbisbM}}
\newsavebox{\CoTTdotroplusdsbisbO}
\begin{lrbox}{\CoTTdotroplusdsbisbO}
\begin{minipage}{\CoTTdotroplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTT.ro+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTTdotroplusdsbisbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTTdotroplusdsbisbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTTdotroplusdsbisbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTTdotroplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTTdotroplusdsbisbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoTT.ro+po.tex <==
\newlength{\CoTTdotropluspoH}
\setlength{\CoTTdotropluspoH}{0cm}
\newsavebox{\CoTTdotropluspoI}
\begin{lrbox}{\CoTTdotropluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotropluspoJ}
\settowidth{\CoTTdotropluspoJ}{\usebox{\CoTTdotropluspoI}}
\addtolength{\CoTTdotropluspoH}{\CoTTdotropluspoJ}
\newsavebox{\CoTTdotropluspoK}
\begin{lrbox}{\CoTTdotropluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotropluspoL}
\settowidth{\CoTTdotropluspoL}{\usebox{\CoTTdotropluspoK}}
\addtolength{\CoTTdotropluspoH}{\CoTTdotropluspoL}
\newsavebox{\CoTTdotropluspoM}
\begin{lrbox}{\CoTTdotropluspoM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1 with [AP = 0b11] and default;
    x ?-> pa2 with [AP = 0b11] and default;
    y |-> pa2 with [AP = 0b11] and default;

    *pa2 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotropluspoN}
\settowidth{\CoTTdotropluspoN}{\usebox{\CoTTdotropluspoM}}
\newsavebox{\CoTTdotropluspoO}
\begin{lrbox}{\CoTTdotropluspoO}
\begin{minipage}{\CoTTdotropluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTT.ro+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTTdotropluspoN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTTdotropluspoM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTTdotropluspoO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTTdotropluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTTdotropluspoK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoTTf.inv+dsb-isb.tex <==
\newlength{\CoTTfdotinvplusdsbisbH}
\setlength{\CoTTfdotinvplusdsbisbH}{0cm}
\newsavebox{\CoTTfdotinvplusdsbisbI}
\begin{lrbox}{\CoTTfdotinvplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTfdotinvplusdsbisbJ}
\settowidth{\CoTTfdotinvplusdsbisbJ}{\usebox{\CoTTfdotinvplusdsbisbI}}
\addtolength{\CoTTfdotinvplusdsbisbH}{\CoTTfdotinvplusdsbisbJ}
\newsavebox{\CoTTfdotinvplusdsbisbK}
\begin{lrbox}{\CoTTfdotinvplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTfdotinvplusdsbisbL}
\settowidth{\CoTTfdotinvplusdsbisbL}{\usebox{\CoTTfdotinvplusdsbisbK}}
\addtolength{\CoTTfdotinvplusdsbisbH}{\CoTTfdotinvplusdsbisbL}
\newsavebox{\CoTTfdotinvplusdsbisbM}
\begin{lrbox}{\CoTTfdotinvplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTfdotinvplusdsbisbN}
\settowidth{\CoTTfdotinvplusdsbisbN}{\usebox{\CoTTfdotinvplusdsbisbM}}
\addtolength{\CoTTfdotinvplusdsbisbH}{\CoTTfdotinvplusdsbisbN}
\newsavebox{\CoTTfdotinvplusdsbisbO}
\begin{lrbox}{\CoTTfdotinvplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTfdotinvplusdsbisbP}
\settowidth{\CoTTfdotinvplusdsbisbP}{\usebox{\CoTTfdotinvplusdsbisbO}}
\newsavebox{\CoTTfdotinvplusdsbisbA}
\begin{lrbox}{\CoTTfdotinvplusdsbisbA}
\begin{minipage}{\CoTTfdotinvplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTTf.inv+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTTfdotinvplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTTfdotinvplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTTfdotinvplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTTfdotinvplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTTfdotinvplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTTfdotinvplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoTTf.inv+po.tex <==
\newlength{\CoTTfdotinvpluspoH}
\setlength{\CoTTfdotinvpluspoH}{0cm}
\newsavebox{\CoTTfdotinvpluspoI}
\begin{lrbox}{\CoTTfdotinvpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTfdotinvpluspoJ}
\settowidth{\CoTTfdotinvpluspoJ}{\usebox{\CoTTfdotinvpluspoI}}
\addtolength{\CoTTfdotinvpluspoH}{\CoTTfdotinvpluspoJ}
\newsavebox{\CoTTfdotinvpluspoK}
\begin{lrbox}{\CoTTfdotinvpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTfdotinvpluspoL}
\settowidth{\CoTTfdotinvpluspoL}{\usebox{\CoTTfdotinvpluspoK}}
\addtolength{\CoTTfdotinvpluspoH}{\CoTTfdotinvpluspoL}
\newsavebox{\CoTTfdotinvpluspoM}
\begin{lrbox}{\CoTTfdotinvpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTfdotinvpluspoN}
\settowidth{\CoTTfdotinvpluspoN}{\usebox{\CoTTfdotinvpluspoM}}
\addtolength{\CoTTfdotinvpluspoH}{\CoTTfdotinvpluspoN}
\newsavebox{\CoTTfdotinvpluspoO}
\begin{lrbox}{\CoTTfdotinvpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTfdotinvpluspoP}
\settowidth{\CoTTfdotinvpluspoP}{\usebox{\CoTTfdotinvpluspoO}}
\newsavebox{\CoTTfdotinvpluspoA}
\begin{lrbox}{\CoTTfdotinvpluspoA}
\begin{minipage}{\CoTTfdotinvpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTTf.inv+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTTfdotinvpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTTfdotinvpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTTfdotinvpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTTfdotinvpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTTfdotinvpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTTfdotinvpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoTW1.inv.tex <==
\newlength{\CoTWonedotinvH}
\setlength{\CoTWonedotinvH}{0cm}
\newsavebox{\CoTWonedotinvI}
\begin{lrbox}{\CoTWonedotinvI}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTWonedotinvJ}
\settowidth{\CoTWonedotinvJ}{\usebox{\CoTWonedotinvI}}
\addtolength{\CoTWonedotinvH}{\CoTWonedotinvJ}
\newsavebox{\CoTWonedotinvK}
\begin{lrbox}{\CoTWonedotinvK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTWonedotinvL}
\settowidth{\CoTWonedotinvL}{\usebox{\CoTWonedotinvK}}
\addtolength{\CoTWonedotinvH}{\CoTWonedotinvL}
\newsavebox{\CoTWonedotinvM}
\begin{lrbox}{\CoTWonedotinvM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTWonedotinvN}
\settowidth{\CoTWonedotinvN}{\usebox{\CoTWonedotinvM}}
\newsavebox{\CoTWonedotinvO}
\begin{lrbox}{\CoTWonedotinvO}
\begin{minipage}{\CoTWonedotinvH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=x|\\
\lstinline[language=IslaLitmusExp]|R2=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTW1.inv|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTWonedotinvN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTWonedotinvM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTWonedotinvO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTWonedotinvI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTWonedotinvK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoTWinv.tex <==
\newlength{\CoTWinvH}
\setlength{\CoTWinvH}{0cm}
\newsavebox{\CoTWinvI}
\begin{lrbox}{\CoTWinvI}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTWinvJ}
\settowidth{\CoTWinvJ}{\usebox{\CoTWinvI}}
\addtolength{\CoTWinvH}{\CoTWinvJ}
\newsavebox{\CoTWinvK}
\begin{lrbox}{\CoTWinvK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTWinvL}
\settowidth{\CoTWinvL}{\usebox{\CoTWinvK}}
\addtolength{\CoTWinvH}{\CoTWinvL}
\newsavebox{\CoTWinvM}
\begin{lrbox}{\CoTWinvM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTWinvN}
\settowidth{\CoTWinvN}{\usebox{\CoTWinvM}}
\newsavebox{\CoTWinvO}
\begin{lrbox}{\CoTWinvO}
\begin{minipage}{\CoTWinvH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=x|\\
\lstinline[language=IslaLitmusExp]|R2=0b0|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTWinv|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTWinvN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTWinvM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTWinvO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTWinvI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTWinvK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoTfRpte+dsb-isb.tex <==
\newlength{\CoTfRpteplusdsbisbH}
\setlength{\CoTfRpteplusdsbisbH}{0cm}
\newsavebox{\CoTfRpteplusdsbisbI}
\begin{lrbox}{\CoTfRpteplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRpteplusdsbisbJ}
\settowidth{\CoTfRpteplusdsbisbJ}{\usebox{\CoTfRpteplusdsbisbI}}
\addtolength{\CoTfRpteplusdsbisbH}{\CoTfRpteplusdsbisbJ}
\newsavebox{\CoTfRpteplusdsbisbK}
\begin{lrbox}{\CoTfRpteplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRpteplusdsbisbL}
\settowidth{\CoTfRpteplusdsbisbL}{\usebox{\CoTfRpteplusdsbisbK}}
\addtolength{\CoTfRpteplusdsbisbH}{\CoTfRpteplusdsbisbL}
\newsavebox{\CoTfRpteplusdsbisbM}
\begin{lrbox}{\CoTfRpteplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRpteplusdsbisbN}
\settowidth{\CoTfRpteplusdsbisbN}{\usebox{\CoTfRpteplusdsbisbM}}
\addtolength{\CoTfRpteplusdsbisbH}{\CoTfRpteplusdsbisbN}
\newsavebox{\CoTfRpteplusdsbisbO}
\begin{lrbox}{\CoTfRpteplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;
    y |-> pa1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRpteplusdsbisbP}
\settowidth{\CoTfRpteplusdsbisbP}{\usebox{\CoTfRpteplusdsbisbO}}
\newsavebox{\CoTfRpteplusdsbisbA}
\begin{lrbox}{\CoTfRpteplusdsbisbA}
\begin{minipage}{\CoTfRpteplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfRpte+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfRpteplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfRpteplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfRpteplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfRpteplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTfRpteplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfRpteplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=desc3(y,page_table_base)|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoTfRpte+dsb.tex <==
\newlength{\CoTfRpteplusdsbH}
\setlength{\CoTfRpteplusdsbH}{0cm}
\newsavebox{\CoTfRpteplusdsbI}
\begin{lrbox}{\CoTfRpteplusdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRpteplusdsbJ}
\settowidth{\CoTfRpteplusdsbJ}{\usebox{\CoTfRpteplusdsbI}}
\addtolength{\CoTfRpteplusdsbH}{\CoTfRpteplusdsbJ}
\newsavebox{\CoTfRpteplusdsbK}
\begin{lrbox}{\CoTfRpteplusdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRpteplusdsbL}
\settowidth{\CoTfRpteplusdsbL}{\usebox{\CoTfRpteplusdsbK}}
\addtolength{\CoTfRpteplusdsbH}{\CoTfRpteplusdsbL}
\newsavebox{\CoTfRpteplusdsbM}
\begin{lrbox}{\CoTfRpteplusdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRpteplusdsbN}
\settowidth{\CoTfRpteplusdsbN}{\usebox{\CoTfRpteplusdsbM}}
\addtolength{\CoTfRpteplusdsbH}{\CoTfRpteplusdsbN}
\newsavebox{\CoTfRpteplusdsbO}
\begin{lrbox}{\CoTfRpteplusdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;
    y |-> pa1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRpteplusdsbP}
\settowidth{\CoTfRpteplusdsbP}{\usebox{\CoTfRpteplusdsbO}}
\newsavebox{\CoTfRpteplusdsbA}
\begin{lrbox}{\CoTfRpteplusdsbA}
\begin{minipage}{\CoTfRpteplusdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfRpte+dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfRpteplusdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfRpteplusdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfRpteplusdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfRpteplusdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTfRpteplusdsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfRpteplusdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=desc3(y,page_table_base)|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoTfRpte+eret.tex <==
\newlength{\CoTfRptepluseretH}
\setlength{\CoTfRptepluseretH}{0cm}
\newsavebox{\CoTfRptepluseretI}
\begin{lrbox}{\CoTfRptepluseretI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRptepluseretJ}
\settowidth{\CoTfRptepluseretJ}{\usebox{\CoTfRptepluseretI}}
\addtolength{\CoTfRptepluseretH}{\CoTfRptepluseretJ}
\newsavebox{\CoTfRptepluseretK}
\begin{lrbox}{\CoTfRptepluseretK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRptepluseretL}
\settowidth{\CoTfRptepluseretL}{\usebox{\CoTfRptepluseretK}}
\addtolength{\CoTfRptepluseretH}{\CoTfRptepluseretL}
\newsavebox{\CoTfRptepluseretM}
\begin{lrbox}{\CoTfRptepluseretM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRptepluseretN}
\settowidth{\CoTfRptepluseretN}{\usebox{\CoTfRptepluseretM}}
\addtolength{\CoTfRptepluseretH}{\CoTfRptepluseretN}
\newsavebox{\CoTfRptepluseretO}
\begin{lrbox}{\CoTfRptepluseretO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;
    y |-> pa1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRptepluseretP}
\settowidth{\CoTfRptepluseretP}{\usebox{\CoTfRptepluseretO}}
\newsavebox{\CoTfRptepluseretA}
\begin{lrbox}{\CoTfRptepluseretA}
\begin{minipage}{\CoTfRptepluseretH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfRpte+eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfRptepluseretP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfRptepluseretO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfRptepluseretA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfRptepluseretI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTfRptepluseretK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfRptepluseretM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=desc3(y,page_table_base)|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoTfRpte+po.tex <==
\newlength{\CoTfRptepluspoH}
\setlength{\CoTfRptepluspoH}{0cm}
\newsavebox{\CoTfRptepluspoI}
\begin{lrbox}{\CoTfRptepluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRptepluspoJ}
\settowidth{\CoTfRptepluspoJ}{\usebox{\CoTfRptepluspoI}}
\addtolength{\CoTfRptepluspoH}{\CoTfRptepluspoJ}
\newsavebox{\CoTfRptepluspoK}
\begin{lrbox}{\CoTfRptepluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRptepluspoL}
\settowidth{\CoTfRptepluspoL}{\usebox{\CoTfRptepluspoK}}
\addtolength{\CoTfRptepluspoH}{\CoTfRptepluspoL}
\newsavebox{\CoTfRptepluspoM}
\begin{lrbox}{\CoTfRptepluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRptepluspoN}
\settowidth{\CoTfRptepluspoN}{\usebox{\CoTfRptepluspoM}}
\addtolength{\CoTfRptepluspoH}{\CoTfRptepluspoN}
\newsavebox{\CoTfRptepluspoO}
\begin{lrbox}{\CoTfRptepluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;
    y |-> pa1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRptepluspoP}
\settowidth{\CoTfRptepluspoP}{\usebox{\CoTfRptepluspoO}}
\newsavebox{\CoTfRptepluspoA}
\begin{lrbox}{\CoTfRptepluspoA}
\begin{minipage}{\CoTfRptepluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfRpte+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfRptepluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfRptepluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfRptepluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfRptepluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTfRptepluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfRptepluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=desc3(y,page_table_base)|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoTfT+dsb-isb.tex <==
\newlength{\CoTfTplusdsbisbH}
\setlength{\CoTfTplusdsbisbH}{0cm}
\newsavebox{\CoTfTplusdsbisbI}
\begin{lrbox}{\CoTfTplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfTplusdsbisbJ}
\settowidth{\CoTfTplusdsbisbJ}{\usebox{\CoTfTplusdsbisbI}}
\addtolength{\CoTfTplusdsbisbH}{\CoTfTplusdsbisbJ}
\newsavebox{\CoTfTplusdsbisbK}
\begin{lrbox}{\CoTfTplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfTplusdsbisbL}
\settowidth{\CoTfTplusdsbisbL}{\usebox{\CoTfTplusdsbisbK}}
\addtolength{\CoTfTplusdsbisbH}{\CoTfTplusdsbisbL}
\newsavebox{\CoTfTplusdsbisbM}
\begin{lrbox}{\CoTfTplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfTplusdsbisbN}
\settowidth{\CoTfTplusdsbisbN}{\usebox{\CoTfTplusdsbisbM}}
\addtolength{\CoTfTplusdsbisbH}{\CoTfTplusdsbisbN}
\newsavebox{\CoTfTplusdsbisbO}
\begin{lrbox}{\CoTfTplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;
    y |-> pa1;
    *pa1 = 0;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfTplusdsbisbP}
\settowidth{\CoTfTplusdsbisbP}{\usebox{\CoTfTplusdsbisbO}}
\newsavebox{\CoTfTplusdsbisbA}
\begin{lrbox}{\CoTfTplusdsbisbA}
\begin{minipage}{\CoTfTplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfT+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfTplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfTplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfTplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfTplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTfTplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfTplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoTfT+po.tex <==
\newlength{\CoTfTpluspoH}
\setlength{\CoTfTpluspoH}{0cm}
\newsavebox{\CoTfTpluspoI}
\begin{lrbox}{\CoTfTpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfTpluspoJ}
\settowidth{\CoTfTpluspoJ}{\usebox{\CoTfTpluspoI}}
\addtolength{\CoTfTpluspoH}{\CoTfTpluspoJ}
\newsavebox{\CoTfTpluspoK}
\begin{lrbox}{\CoTfTpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfTpluspoL}
\settowidth{\CoTfTpluspoL}{\usebox{\CoTfTpluspoK}}
\addtolength{\CoTfTpluspoH}{\CoTfTpluspoL}
\newsavebox{\CoTfTpluspoM}
\begin{lrbox}{\CoTfTpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfTpluspoN}
\settowidth{\CoTfTpluspoN}{\usebox{\CoTfTpluspoM}}
\addtolength{\CoTfTpluspoH}{\CoTfTpluspoN}
\newsavebox{\CoTfTpluspoO}
\begin{lrbox}{\CoTfTpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;
    y |-> pa1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfTpluspoP}
\settowidth{\CoTfTpluspoP}{\usebox{\CoTfTpluspoO}}
\newsavebox{\CoTfTpluspoA}
\begin{lrbox}{\CoTfTpluspoA}
\begin{minipage}{\CoTfTpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfT+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfTpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfTpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfTpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfTpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTfTpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfTpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoTfW.inv+dsb-isb.tex <==
\newlength{\CoTfWdotinvplusdsbisbH}
\setlength{\CoTfWdotinvplusdsbisbH}{0cm}
\newsavebox{\CoTfWdotinvplusdsbisbI}
\begin{lrbox}{\CoTfWdotinvplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvplusdsbisbJ}
\settowidth{\CoTfWdotinvplusdsbisbJ}{\usebox{\CoTfWdotinvplusdsbisbI}}
\addtolength{\CoTfWdotinvplusdsbisbH}{\CoTfWdotinvplusdsbisbJ}
\newsavebox{\CoTfWdotinvplusdsbisbK}
\begin{lrbox}{\CoTfWdotinvplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvplusdsbisbL}
\settowidth{\CoTfWdotinvplusdsbisbL}{\usebox{\CoTfWdotinvplusdsbisbK}}
\addtolength{\CoTfWdotinvplusdsbisbH}{\CoTfWdotinvplusdsbisbL}
\newsavebox{\CoTfWdotinvplusdsbisbM}
\begin{lrbox}{\CoTfWdotinvplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvplusdsbisbN}
\settowidth{\CoTfWdotinvplusdsbisbN}{\usebox{\CoTfWdotinvplusdsbisbM}}
\addtolength{\CoTfWdotinvplusdsbisbH}{\CoTfWdotinvplusdsbisbN}
\newsavebox{\CoTfWdotinvplusdsbisbO}
\begin{lrbox}{\CoTfWdotinvplusdsbisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvplusdsbisbP}
\settowidth{\CoTfWdotinvplusdsbisbP}{\usebox{\CoTfWdotinvplusdsbisbO}}
\addtolength{\CoTfWdotinvplusdsbisbH}{\CoTfWdotinvplusdsbisbP}
\newsavebox{\CoTfWdotinvplusdsbisbA}
\begin{lrbox}{\CoTfWdotinvplusdsbisbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    x ?-> raw(2);
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvplusdsbisbB}
\settowidth{\CoTfWdotinvplusdsbisbB}{\usebox{\CoTfWdotinvplusdsbisbA}}
\newsavebox{\CoTfWdotinvplusdsbisbC}
\begin{lrbox}{\CoTfWdotinvplusdsbisbC}
\begin{minipage}{\CoTfWdotinvplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b10|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:R1=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfW.inv+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfWdotinvplusdsbisbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfWdotinvplusdsbisbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfWdotinvplusdsbisbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfWdotinvplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTfWdotinvplusdsbisbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\CoTfWdotinvplusdsbisbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfWdotinvplusdsbisbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=2 & 2:R2=mkdesc3(oa=pa1)|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoTfW.inv+po.tex <==
\newlength{\CoTfWdotinvpluspoH}
\setlength{\CoTfWdotinvpluspoH}{0cm}
\newsavebox{\CoTfWdotinvpluspoI}
\begin{lrbox}{\CoTfWdotinvpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvpluspoJ}
\settowidth{\CoTfWdotinvpluspoJ}{\usebox{\CoTfWdotinvpluspoI}}
\addtolength{\CoTfWdotinvpluspoH}{\CoTfWdotinvpluspoJ}
\newsavebox{\CoTfWdotinvpluspoK}
\begin{lrbox}{\CoTfWdotinvpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvpluspoL}
\settowidth{\CoTfWdotinvpluspoL}{\usebox{\CoTfWdotinvpluspoK}}
\addtolength{\CoTfWdotinvpluspoH}{\CoTfWdotinvpluspoL}
\newsavebox{\CoTfWdotinvpluspoM}
\begin{lrbox}{\CoTfWdotinvpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvpluspoN}
\settowidth{\CoTfWdotinvpluspoN}{\usebox{\CoTfWdotinvpluspoM}}
\addtolength{\CoTfWdotinvpluspoH}{\CoTfWdotinvpluspoN}
\newsavebox{\CoTfWdotinvpluspoO}
\begin{lrbox}{\CoTfWdotinvpluspoO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvpluspoP}
\settowidth{\CoTfWdotinvpluspoP}{\usebox{\CoTfWdotinvpluspoO}}
\addtolength{\CoTfWdotinvpluspoH}{\CoTfWdotinvpluspoP}
\newsavebox{\CoTfWdotinvpluspoA}
\begin{lrbox}{\CoTfWdotinvpluspoA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    x ?-> raw(2);
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvpluspoB}
\settowidth{\CoTfWdotinvpluspoB}{\usebox{\CoTfWdotinvpluspoA}}
\newsavebox{\CoTfWdotinvpluspoC}
\begin{lrbox}{\CoTfWdotinvpluspoC}
\begin{minipage}{\CoTfWdotinvpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b10|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:R1=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfW.inv+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfWdotinvpluspoB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfWdotinvpluspoA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfWdotinvpluspoC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfWdotinvpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTfWdotinvpluspoK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\CoTfWdotinvpluspoM}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfWdotinvpluspoO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=2 & 2:R2=mkdesc3(oa=pa1)|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoTfW1.inv+si.tex <==
\newlength{\CoTfWonedotinvplussiH}
\setlength{\CoTfWonedotinvplussiH}{0cm}
\newsavebox{\CoTfWonedotinvplussiI}
\begin{lrbox}{\CoTfWonedotinvplussiI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWonedotinvplussiJ}
\settowidth{\CoTfWonedotinvplussiJ}{\usebox{\CoTfWonedotinvplussiI}}
\addtolength{\CoTfWonedotinvplussiH}{\CoTfWonedotinvplussiJ}
\newsavebox{\CoTfWonedotinvplussiK}
\begin{lrbox}{\CoTfWonedotinvplussiK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWonedotinvplussiL}
\settowidth{\CoTfWonedotinvplussiL}{\usebox{\CoTfWonedotinvplussiK}}
\addtolength{\CoTfWonedotinvplussiH}{\CoTfWonedotinvplussiL}
\newsavebox{\CoTfWonedotinvplussiM}
\begin{lrbox}{\CoTfWonedotinvplussiM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWonedotinvplussiN}
\settowidth{\CoTfWonedotinvplussiN}{\usebox{\CoTfWonedotinvplussiM}}
\newsavebox{\CoTfWonedotinvplussiO}
\begin{lrbox}{\CoTfWonedotinvplussiO}
\begin{minipage}{\CoTfWonedotinvplussiH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=0b10|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(0x1000,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfW1.inv+si|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfWonedotinvplussiN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfWonedotinvplussiM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfWonedotinvplussiO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfWonedotinvplussiI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfWonedotinvplussiK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R0=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoWR.alias.tex <==
\newlength{\CoWRdotaliasH}
\setlength{\CoWRdotaliasH}{0cm}
\newsavebox{\CoWRdotaliasI}
\begin{lrbox}{\CoWRdotaliasI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWRdotaliasJ}
\settowidth{\CoWRdotaliasJ}{\usebox{\CoWRdotaliasI}}
\addtolength{\CoWRdotaliasH}{\CoWRdotaliasJ}
\newsavebox{\CoWRdotaliasK}
\begin{lrbox}{\CoWRdotaliasK}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    y |-> pa1;
    *pa1 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWRdotaliasL}
\settowidth{\CoWRdotaliasL}{\usebox{\CoWRdotaliasK}}
\newsavebox{\CoWRdotaliasM}
\begin{lrbox}{\CoWRdotaliasM}
\begin{minipage}{\CoWRdotaliasH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|R0=0x1|\\
\lstinline[language=IslaLitmusExp]|R1=x|\\
\lstinline[language=IslaLitmusExp]|R3=y|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWR.alias|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWRdotaliasL}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWRdotaliasK}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWRdotaliasM}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWRdotaliasI}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoWR.inv.tex <==
\newlength{\CoWRdotinvH}
\setlength{\CoWRdotinvH}{0cm}
\newsavebox{\CoWRdotinvI}
\begin{lrbox}{\CoWRdotinvI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWRdotinvJ}
\settowidth{\CoWRdotinvJ}{\usebox{\CoWRdotinvI}}
\addtolength{\CoWRdotinvH}{\CoWRdotinvJ}
\newsavebox{\CoWRdotinvK}
\begin{lrbox}{\CoWRdotinvK}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWRdotinvL}
\settowidth{\CoWRdotinvL}{\usebox{\CoWRdotinvK}}
\newsavebox{\CoWRdotinvM}
\begin{lrbox}{\CoWRdotinvM}
\begin{minipage}{\CoWRdotinvH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWR.inv|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWRdotinvL}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWRdotinvK}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWRdotinvM}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWRdotinvI}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoWTa1.1.inv+dsb-tlbiasidis-dsb-eret.tex <==
\newlength{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetH}
\setlength{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetH}{0cm}
\newsavebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetI}
\begin{lrbox}{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI ASIDE1IS,X4
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetJ}
\settowidth{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetJ}{\usebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetI}}
\addtolength{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetH}{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetJ}
\newsavebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetK}
\begin{lrbox}{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetL}
\settowidth{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetL}{\usebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetK}}
\addtolength{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetH}{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetL}
\newsavebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetM}
\begin{lrbox}{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;

    y |-> pa1;

    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetN}
\settowidth{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetN}{\usebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetM}}
\newsavebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetO}
\begin{lrbox}{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetO}
\begin{minipage}{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL1=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=asid(0x1)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL1=0b00000|\\
\lstinline[language=IslaLitmusExp]|TTBR0_EL1=ttbr(asid=0x0001,base=page_table_base)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTa1.1.inv+dsb-tlbiasidis-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoWTa2.1.inv+dsb-tlbiasidis-dsb-eret.tex <==
\newlength{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetH}
\setlength{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetH}{0cm}
\newsavebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetI}
\begin{lrbox}{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI ASIDE1IS,X4
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetJ}
\settowidth{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetJ}{\usebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetI}}
\addtolength{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetH}{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetJ}
\newsavebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetK}
\begin{lrbox}{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetL}
\settowidth{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetL}{\usebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetK}}
\addtolength{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetH}{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetL}
\newsavebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetM}
\begin{lrbox}{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;

    y |-> pa1;

    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetN}
\settowidth{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetN}{\usebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetM}}
\newsavebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetO}
\begin{lrbox}{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetO}
\begin{minipage}{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL1=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=asid(0x2)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL1=0b00000|\\
\lstinline[language=IslaLitmusExp]|TTBR0_EL1=ttbr(base=page_table_base,asid=0x0001)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTa2.1.inv+dsb-tlbiasidis-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoWTf.inv+_dmb_-dmb-addr.tex <==
\newlength{\CoWTfdotinvplus[dmb]dmbaddrH}
\setlength{\CoWTfdotinvplus[dmb]dmbaddrH}{0cm}
\newsavebox{\CoWTfdotinvplus[dmb]dmbaddrI}
\begin{lrbox}{\CoWTfdotinvplus[dmb]dmbaddrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X2,[X1]
DSB ST
LDR X3,[X4]
EOR X5,X3,X3
LDR X6,[X7,X5]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplus[dmb]dmbaddrJ}
\settowidth{\CoWTfdotinvplus[dmb]dmbaddrJ}{\usebox{\CoWTfdotinvplus[dmb]dmbaddrI}}
\addtolength{\CoWTfdotinvplus[dmb]dmbaddrH}{\CoWTfdotinvplus[dmb]dmbaddrJ}
\newsavebox{\CoWTfdotinvplus[dmb]dmbaddrK}
\begin{lrbox}{\CoWTfdotinvplus[dmb]dmbaddrK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplus[dmb]dmbaddrL}
\settowidth{\CoWTfdotinvplus[dmb]dmbaddrL}{\usebox{\CoWTfdotinvplus[dmb]dmbaddrK}}
\addtolength{\CoWTfdotinvplus[dmb]dmbaddrH}{\CoWTfdotinvplus[dmb]dmbaddrL}
\newsavebox{\CoWTfdotinvplus[dmb]dmbaddrM}
\begin{lrbox}{\CoWTfdotinvplus[dmb]dmbaddrM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X6,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplus[dmb]dmbaddrN}
\settowidth{\CoWTfdotinvplus[dmb]dmbaddrN}{\usebox{\CoWTfdotinvplus[dmb]dmbaddrM}}
\addtolength{\CoWTfdotinvplus[dmb]dmbaddrH}{\CoWTfdotinvplus[dmb]dmbaddrN}
\newsavebox{\CoWTfdotinvplus[dmb]dmbaddrO}
\begin{lrbox}{\CoWTfdotinvplus[dmb]dmbaddrO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplus[dmb]dmbaddrP}
\settowidth{\CoWTfdotinvplus[dmb]dmbaddrP}{\usebox{\CoWTfdotinvplus[dmb]dmbaddrO}}
\newsavebox{\CoWTfdotinvplus[dmb]dmbaddrA}
\begin{lrbox}{\CoWTfdotinvplus[dmb]dmbaddrA}
\begin{minipage}{\CoWTfdotinvplus[dmb]dmbaddrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R4=y|\\
\lstinline[language=IslaLitmusExp]|0:R7=x|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+[dmb]-dmb-addr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvplus[dmb]dmbaddrP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvplus[dmb]dmbaddrO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvplus[dmb]dmbaddrA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplus[dmb]dmbaddrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplus[dmb]dmbaddrK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplus[dmb]dmbaddrM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R3=2 & 0:R6=0 & 1:R0=desc3(z,page_table_base)|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoWTf.inv+dsb-isb.tex <==
\newlength{\CoWTfdotinvplusdsbisbH}
\setlength{\CoWTfdotinvplusdsbisbH}{0cm}
\newsavebox{\CoWTfdotinvplusdsbisbI}
\begin{lrbox}{\CoWTfdotinvplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusdsbisbJ}
\settowidth{\CoWTfdotinvplusdsbisbJ}{\usebox{\CoWTfdotinvplusdsbisbI}}
\addtolength{\CoWTfdotinvplusdsbisbH}{\CoWTfdotinvplusdsbisbJ}
\newsavebox{\CoWTfdotinvplusdsbisbK}
\begin{lrbox}{\CoWTfdotinvplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusdsbisbL}
\settowidth{\CoWTfdotinvplusdsbisbL}{\usebox{\CoWTfdotinvplusdsbisbK}}
\addtolength{\CoWTfdotinvplusdsbisbH}{\CoWTfdotinvplusdsbisbL}
\newsavebox{\CoWTfdotinvplusdsbisbM}
\begin{lrbox}{\CoWTfdotinvplusdsbisbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusdsbisbN}
\settowidth{\CoWTfdotinvplusdsbisbN}{\usebox{\CoWTfdotinvplusdsbisbM}}
\newsavebox{\CoWTfdotinvplusdsbisbO}
\begin{lrbox}{\CoWTfdotinvplusdsbisbO}
\begin{minipage}{\CoWTfdotinvplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvplusdsbisbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvplusdsbisbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvplusdsbisbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplusdsbisbI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplusdsbisbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoWTf.inv+po-ctrl+po.tex <==
\newlength{\CoWTfdotinvpluspoctrlpluspoH}
\setlength{\CoWTfdotinvpluspoctrlpluspoH}{0cm}
\newsavebox{\CoWTfdotinvpluspoctrlpluspoI}
\begin{lrbox}{\CoWTfdotinvpluspoctrlpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
CBNZ X2,L0
L0:
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlpluspoJ}
\settowidth{\CoWTfdotinvpluspoctrlpluspoJ}{\usebox{\CoWTfdotinvpluspoctrlpluspoI}}
\addtolength{\CoWTfdotinvpluspoctrlpluspoH}{\CoWTfdotinvpluspoctrlpluspoJ}
\newsavebox{\CoWTfdotinvpluspoctrlpluspoK}
\begin{lrbox}{\CoWTfdotinvpluspoctrlpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlpluspoL}
\settowidth{\CoWTfdotinvpluspoctrlpluspoL}{\usebox{\CoWTfdotinvpluspoctrlpluspoK}}
\addtolength{\CoWTfdotinvpluspoctrlpluspoH}{\CoWTfdotinvpluspoctrlpluspoL}
\newsavebox{\CoWTfdotinvpluspoctrlpluspoM}
\begin{lrbox}{\CoWTfdotinvpluspoctrlpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlpluspoN}
\settowidth{\CoWTfdotinvpluspoctrlpluspoN}{\usebox{\CoWTfdotinvpluspoctrlpluspoM}}
\addtolength{\CoWTfdotinvpluspoctrlpluspoH}{\CoWTfdotinvpluspoctrlpluspoN}
\newsavebox{\CoWTfdotinvpluspoctrlpluspoO}
\begin{lrbox}{\CoWTfdotinvpluspoctrlpluspoO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlpluspoP}
\settowidth{\CoWTfdotinvpluspoctrlpluspoP}{\usebox{\CoWTfdotinvpluspoctrlpluspoO}}
\addtolength{\CoWTfdotinvpluspoctrlpluspoH}{\CoWTfdotinvpluspoctrlpluspoP}
\newsavebox{\CoWTfdotinvpluspoctrlpluspoA}
\begin{lrbox}{\CoWTfdotinvpluspoctrlpluspoA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    *pa2 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlpluspoB}
\settowidth{\CoWTfdotinvpluspoctrlpluspoB}{\usebox{\CoWTfdotinvpluspoctrlpluspoA}}
\newsavebox{\CoWTfdotinvpluspoctrlpluspoC}
\begin{lrbox}{\CoWTfdotinvpluspoctrlpluspoC}
\begin{minipage}{\CoWTfdotinvpluspoctrlpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R5=x|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+po-ctrl+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvpluspoctrlpluspoB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvpluspoctrlpluspoA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvpluspoctrlpluspoC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoctrlpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoctrlpluspoK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoctrlpluspoM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoctrlpluspoO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=1 & 0:R4=0 & 1:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoWTf.inv+po-ctrl-isb+po.tex <==
\newlength{\CoWTfdotinvpluspoctrlisbpluspoH}
\setlength{\CoWTfdotinvpluspoctrlisbpluspoH}{0cm}
\newsavebox{\CoWTfdotinvpluspoctrlisbpluspoI}
\begin{lrbox}{\CoWTfdotinvpluspoctrlisbpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
CBNZ X2,L0
L0:
ISB
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlisbpluspoJ}
\settowidth{\CoWTfdotinvpluspoctrlisbpluspoJ}{\usebox{\CoWTfdotinvpluspoctrlisbpluspoI}}
\addtolength{\CoWTfdotinvpluspoctrlisbpluspoH}{\CoWTfdotinvpluspoctrlisbpluspoJ}
\newsavebox{\CoWTfdotinvpluspoctrlisbpluspoK}
\begin{lrbox}{\CoWTfdotinvpluspoctrlisbpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlisbpluspoL}
\settowidth{\CoWTfdotinvpluspoctrlisbpluspoL}{\usebox{\CoWTfdotinvpluspoctrlisbpluspoK}}
\addtolength{\CoWTfdotinvpluspoctrlisbpluspoH}{\CoWTfdotinvpluspoctrlisbpluspoL}
\newsavebox{\CoWTfdotinvpluspoctrlisbpluspoM}
\begin{lrbox}{\CoWTfdotinvpluspoctrlisbpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlisbpluspoN}
\settowidth{\CoWTfdotinvpluspoctrlisbpluspoN}{\usebox{\CoWTfdotinvpluspoctrlisbpluspoM}}
\addtolength{\CoWTfdotinvpluspoctrlisbpluspoH}{\CoWTfdotinvpluspoctrlisbpluspoN}
\newsavebox{\CoWTfdotinvpluspoctrlisbpluspoO}
\begin{lrbox}{\CoWTfdotinvpluspoctrlisbpluspoO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlisbpluspoP}
\settowidth{\CoWTfdotinvpluspoctrlisbpluspoP}{\usebox{\CoWTfdotinvpluspoctrlisbpluspoO}}
\addtolength{\CoWTfdotinvpluspoctrlisbpluspoH}{\CoWTfdotinvpluspoctrlisbpluspoP}
\newsavebox{\CoWTfdotinvpluspoctrlisbpluspoA}
\begin{lrbox}{\CoWTfdotinvpluspoctrlisbpluspoA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    *pa2 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlisbpluspoB}
\settowidth{\CoWTfdotinvpluspoctrlisbpluspoB}{\usebox{\CoWTfdotinvpluspoctrlisbpluspoA}}
\newsavebox{\CoWTfdotinvpluspoctrlisbpluspoC}
\begin{lrbox}{\CoWTfdotinvpluspoctrlisbpluspoC}
\begin{minipage}{\CoWTfdotinvpluspoctrlisbpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R5=x|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+po-ctrl-isb+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvpluspoctrlisbpluspoB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvpluspoctrlisbpluspoA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvpluspoctrlisbpluspoC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoctrlisbpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoctrlisbpluspoK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoctrlisbpluspoM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoctrlisbpluspoO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=1 & 0:R4=0 & 1:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoWTf.inv+po.tex <==
\newlength{\CoWTfdotinvpluspoH}
\setlength{\CoWTfdotinvpluspoH}{0cm}
\newsavebox{\CoWTfdotinvpluspoI}
\begin{lrbox}{\CoWTfdotinvpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoJ}
\settowidth{\CoWTfdotinvpluspoJ}{\usebox{\CoWTfdotinvpluspoI}}
\addtolength{\CoWTfdotinvpluspoH}{\CoWTfdotinvpluspoJ}
\newsavebox{\CoWTfdotinvpluspoK}
\begin{lrbox}{\CoWTfdotinvpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoL}
\settowidth{\CoWTfdotinvpluspoL}{\usebox{\CoWTfdotinvpluspoK}}
\addtolength{\CoWTfdotinvpluspoH}{\CoWTfdotinvpluspoL}
\newsavebox{\CoWTfdotinvpluspoM}
\begin{lrbox}{\CoWTfdotinvpluspoM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoN}
\settowidth{\CoWTfdotinvpluspoN}{\usebox{\CoWTfdotinvpluspoM}}
\newsavebox{\CoWTfdotinvpluspoO}
\begin{lrbox}{\CoWTfdotinvpluspoO}
\begin{minipage}{\CoWTfdotinvpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvpluspoN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvpluspoM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvpluspoO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoWTf.inv+poloc-ctrl-isb.tex <==
\newlength{\CoWTfdotinvpluspolocctrlisbH}
\setlength{\CoWTfdotinvpluspolocctrlisbH}{0cm}
\newsavebox{\CoWTfdotinvpluspolocctrlisbI}
\begin{lrbox}{\CoWTfdotinvpluspolocctrlisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X4,[X1]
CBNZ X4,L0
L0:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspolocctrlisbJ}
\settowidth{\CoWTfdotinvpluspolocctrlisbJ}{\usebox{\CoWTfdotinvpluspolocctrlisbI}}
\addtolength{\CoWTfdotinvpluspolocctrlisbH}{\CoWTfdotinvpluspolocctrlisbJ}
\newsavebox{\CoWTfdotinvpluspolocctrlisbK}
\begin{lrbox}{\CoWTfdotinvpluspolocctrlisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspolocctrlisbL}
\settowidth{\CoWTfdotinvpluspolocctrlisbL}{\usebox{\CoWTfdotinvpluspolocctrlisbK}}
\addtolength{\CoWTfdotinvpluspolocctrlisbH}{\CoWTfdotinvpluspolocctrlisbL}
\newsavebox{\CoWTfdotinvpluspolocctrlisbM}
\begin{lrbox}{\CoWTfdotinvpluspolocctrlisbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *y = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspolocctrlisbN}
\settowidth{\CoWTfdotinvpluspolocctrlisbN}{\usebox{\CoWTfdotinvpluspolocctrlisbM}}
\newsavebox{\CoWTfdotinvpluspolocctrlisbO}
\begin{lrbox}{\CoWTfdotinvpluspolocctrlisbO}
\begin{minipage}{\CoWTfdotinvpluspolocctrlisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+poloc-ctrl-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvpluspolocctrlisbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvpluspolocctrlisbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvpluspolocctrlisbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspolocctrlisbI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspolocctrlisbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoWTf.inv+rfi-addr.tex <==
\newlength{\CoWTfdotinvplusrfiaddrH}
\setlength{\CoWTfdotinvplusrfiaddrH}{0cm}
\newsavebox{\CoWTfdotinvplusrfiaddrI}
\begin{lrbox}{\CoWTfdotinvplusrfiaddrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusrfiaddrJ}
\settowidth{\CoWTfdotinvplusrfiaddrJ}{\usebox{\CoWTfdotinvplusrfiaddrI}}
\addtolength{\CoWTfdotinvplusrfiaddrH}{\CoWTfdotinvplusrfiaddrJ}
\newsavebox{\CoWTfdotinvplusrfiaddrK}
\begin{lrbox}{\CoWTfdotinvplusrfiaddrK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#0
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusrfiaddrL}
\settowidth{\CoWTfdotinvplusrfiaddrL}{\usebox{\CoWTfdotinvplusrfiaddrK}}
\addtolength{\CoWTfdotinvplusrfiaddrH}{\CoWTfdotinvplusrfiaddrL}
\newsavebox{\CoWTfdotinvplusrfiaddrM}
\begin{lrbox}{\CoWTfdotinvplusrfiaddrM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusrfiaddrN}
\settowidth{\CoWTfdotinvplusrfiaddrN}{\usebox{\CoWTfdotinvplusrfiaddrM}}
\newsavebox{\CoWTfdotinvplusrfiaddrO}
\begin{lrbox}{\CoWTfdotinvplusrfiaddrO}
\begin{minipage}{\CoWTfdotinvplusrfiaddrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R5=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+rfi-addr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvplusrfiaddrN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvplusrfiaddrM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvplusrfiaddrO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplusrfiaddrI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplusrfiaddrK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=desc3(y,page_table_base) & 0:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoWTf.inv+rfi-ctrl-isb.tex <==
\newlength{\CoWTfdotinvplusrfictrlisbH}
\setlength{\CoWTfdotinvplusrfictrlisbH}{0cm}
\newsavebox{\CoWTfdotinvplusrfictrlisbI}
\begin{lrbox}{\CoWTfdotinvplusrfictrlisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
CBNZ X2,L0
L0:
ISB
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusrfictrlisbJ}
\settowidth{\CoWTfdotinvplusrfictrlisbJ}{\usebox{\CoWTfdotinvplusrfictrlisbI}}
\addtolength{\CoWTfdotinvplusrfictrlisbH}{\CoWTfdotinvplusrfictrlisbJ}
\newsavebox{\CoWTfdotinvplusrfictrlisbK}
\begin{lrbox}{\CoWTfdotinvplusrfictrlisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusrfictrlisbL}
\settowidth{\CoWTfdotinvplusrfictrlisbL}{\usebox{\CoWTfdotinvplusrfictrlisbK}}
\addtolength{\CoWTfdotinvplusrfictrlisbH}{\CoWTfdotinvplusrfictrlisbL}
\newsavebox{\CoWTfdotinvplusrfictrlisbM}
\begin{lrbox}{\CoWTfdotinvplusrfictrlisbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    *pa2 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusrfictrlisbN}
\settowidth{\CoWTfdotinvplusrfictrlisbN}{\usebox{\CoWTfdotinvplusrfictrlisbM}}
\newsavebox{\CoWTfdotinvplusrfictrlisbO}
\begin{lrbox}{\CoWTfdotinvplusrfictrlisbO}
\begin{minipage}{\CoWTfdotinvplusrfictrlisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R5=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+rfi-ctrl-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvplusrfictrlisbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvplusrfictrlisbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvplusrfictrlisbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplusrfictrlisbI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplusrfictrlisbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=desc3(u,page_table_base) & 0:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoWTf.inv+svc.tex <==
\newlength{\CoWTfdotinvplussvcH}
\setlength{\CoWTfdotinvplussvcH}{0cm}
\newsavebox{\CoWTfdotinvplussvcI}
\begin{lrbox}{\CoWTfdotinvplussvcI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
SVC #0x0
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplussvcJ}
\settowidth{\CoWTfdotinvplussvcJ}{\usebox{\CoWTfdotinvplussvcI}}
\addtolength{\CoWTfdotinvplussvcH}{\CoWTfdotinvplussvcJ}
\newsavebox{\CoWTfdotinvplussvcK}
\begin{lrbox}{\CoWTfdotinvplussvcK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1200:
MOV X2,#0
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplussvcL}
\settowidth{\CoWTfdotinvplussvcL}{\usebox{\CoWTfdotinvplussvcK}}
\addtolength{\CoWTfdotinvplussvcH}{\CoWTfdotinvplussvcL}
\newsavebox{\CoWTfdotinvplussvcM}
\begin{lrbox}{\CoWTfdotinvplussvcM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS X10,ELR_EL1
LDR X2,[X3]
MSR ELR_EL1,X10
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplussvcN}
\settowidth{\CoWTfdotinvplussvcN}{\usebox{\CoWTfdotinvplussvcM}}
\addtolength{\CoWTfdotinvplussvcH}{\CoWTfdotinvplussvcN}
\newsavebox{\CoWTfdotinvplussvcO}
\begin{lrbox}{\CoWTfdotinvplussvcO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *y = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplussvcP}
\settowidth{\CoWTfdotinvplussvcP}{\usebox{\CoWTfdotinvplussvcO}}
\newsavebox{\CoWTfdotinvplussvcA}
\begin{lrbox}{\CoWTfdotinvplussvcA}
\begin{minipage}{\CoWTfdotinvplussvcH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+svc|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvplussvcP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvplussvcO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvplussvcA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplussvcI}\\
  \cline{2-2}
  & thread0 el1 handler same exc\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplussvcK}\\
  \cline{2-2}
  & thread0 el1 handler lower exc\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplussvcM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoWTf.inv.EL1+dsb-eret.tex <==
\newlength{\CoWTfdotinvdotELoneplusdsberetH}
\setlength{\CoWTfdotinvdotELoneplusdsberetH}{0cm}
\newsavebox{\CoWTfdotinvdotELoneplusdsberetI}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELoneplusdsberetJ}
\settowidth{\CoWTfdotinvdotELoneplusdsberetJ}{\usebox{\CoWTfdotinvdotELoneplusdsberetI}}
\addtolength{\CoWTfdotinvdotELoneplusdsberetH}{\CoWTfdotinvdotELoneplusdsberetJ}
\newsavebox{\CoWTfdotinvdotELoneplusdsberetK}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELoneplusdsberetL}
\settowidth{\CoWTfdotinvdotELoneplusdsberetL}{\usebox{\CoWTfdotinvdotELoneplusdsberetK}}
\addtolength{\CoWTfdotinvdotELoneplusdsberetH}{\CoWTfdotinvdotELoneplusdsberetL}
\newsavebox{\CoWTfdotinvdotELoneplusdsberetM}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *y = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELoneplusdsberetN}
\settowidth{\CoWTfdotinvdotELoneplusdsberetN}{\usebox{\CoWTfdotinvdotELoneplusdsberetM}}
\newsavebox{\CoWTfdotinvdotELoneplusdsberetO}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsberetO}
\begin{minipage}{\CoWTfdotinvdotELoneplusdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL1=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL1=0b00000|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv.EL1+dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvdotELoneplusdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvdotELoneplusdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvdotELoneplusdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELoneplusdsberetI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELoneplusdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoWTf.inv.EL1+dsb-svc.tex <==
\newlength{\CoWTfdotinvdotELoneplusdsbsvcH}
\setlength{\CoWTfdotinvdotELoneplusdsbsvcH}{0cm}
\newsavebox{\CoWTfdotinvdotELoneplusdsbsvcI}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsbsvcI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
SVC #0x0
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELoneplusdsbsvcJ}
\settowidth{\CoWTfdotinvdotELoneplusdsbsvcJ}{\usebox{\CoWTfdotinvdotELoneplusdsbsvcI}}
\addtolength{\CoWTfdotinvdotELoneplusdsbsvcH}{\CoWTfdotinvdotELoneplusdsbsvcJ}
\newsavebox{\CoWTfdotinvdotELoneplusdsbsvcK}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsbsvcK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1200:
MOV X2,#0
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELoneplusdsbsvcL}
\settowidth{\CoWTfdotinvdotELoneplusdsbsvcL}{\usebox{\CoWTfdotinvdotELoneplusdsbsvcK}}
\addtolength{\CoWTfdotinvdotELoneplusdsbsvcH}{\CoWTfdotinvdotELoneplusdsbsvcL}
\newsavebox{\CoWTfdotinvdotELoneplusdsbsvcM}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsbsvcM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS X10,ELR_EL1
LDR X2,[X3]
MSR ELR_EL1,X10
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELoneplusdsbsvcN}
\settowidth{\CoWTfdotinvdotELoneplusdsbsvcN}{\usebox{\CoWTfdotinvdotELoneplusdsbsvcM}}
\addtolength{\CoWTfdotinvdotELoneplusdsbsvcH}{\CoWTfdotinvdotELoneplusdsbsvcN}
\newsavebox{\CoWTfdotinvdotELoneplusdsbsvcO}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsbsvcO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *y = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELoneplusdsbsvcP}
\settowidth{\CoWTfdotinvdotELoneplusdsbsvcP}{\usebox{\CoWTfdotinvdotELoneplusdsbsvcO}}
\newsavebox{\CoWTfdotinvdotELoneplusdsbsvcA}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsbsvcA}
\begin{minipage}{\CoWTfdotinvdotELoneplusdsbsvcH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv.EL1+dsb-svc|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvdotELoneplusdsbsvcP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvdotELoneplusdsbsvcO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvdotELoneplusdsbsvcA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELoneplusdsbsvcI}\\
  \cline{2-2}
  & thread0 el1 handler same exc\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELoneplusdsbsvcK}\\
  \cline{2-2}
  & thread0 el1 handler lower exc\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELoneplusdsbsvcM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoWTf.inv.EL1+eret.tex <==
\newlength{\CoWTfdotinvdotELonepluseretH}
\setlength{\CoWTfdotinvdotELonepluseretH}{0cm}
\newsavebox{\CoWTfdotinvdotELonepluseretI}
\begin{lrbox}{\CoWTfdotinvdotELonepluseretI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELonepluseretJ}
\settowidth{\CoWTfdotinvdotELonepluseretJ}{\usebox{\CoWTfdotinvdotELonepluseretI}}
\addtolength{\CoWTfdotinvdotELonepluseretH}{\CoWTfdotinvdotELonepluseretJ}
\newsavebox{\CoWTfdotinvdotELonepluseretK}
\begin{lrbox}{\CoWTfdotinvdotELonepluseretK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELonepluseretL}
\settowidth{\CoWTfdotinvdotELonepluseretL}{\usebox{\CoWTfdotinvdotELonepluseretK}}
\addtolength{\CoWTfdotinvdotELonepluseretH}{\CoWTfdotinvdotELonepluseretL}
\newsavebox{\CoWTfdotinvdotELonepluseretM}
\begin{lrbox}{\CoWTfdotinvdotELonepluseretM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *y = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELonepluseretN}
\settowidth{\CoWTfdotinvdotELonepluseretN}{\usebox{\CoWTfdotinvdotELonepluseretM}}
\newsavebox{\CoWTfdotinvdotELonepluseretO}
\begin{lrbox}{\CoWTfdotinvdotELonepluseretO}
\begin{minipage}{\CoWTfdotinvdotELonepluseretH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL1=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL1=0b00000|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv.EL1+eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvdotELonepluseretN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvdotELonepluseretM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvdotELonepluseretO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELonepluseretI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELonepluseretK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoWTf.inv.EL2+dsb-tlbiipa-dsb-tlbiis-dsb-eret.tex <==
\newlength{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetH}
\setlength{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetH}{0cm}
\newsavebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetI}
\begin{lrbox}{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1,X4
DSB SY
TLBI VMALLE1IS
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetJ}
\settowidth{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetJ}{\usebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetI}}
\addtolength{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetH}{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetJ}
\newsavebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetK}
\begin{lrbox}{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X20,ELR_EL2
ADD X20,X20,#4
MSR ELR_EL2,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetL}
\settowidth{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetL}{\usebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetK}}
\addtolength{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetH}{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetL}
\newsavebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetM}
\begin{lrbox}{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;

    ipa1 |-> invalid;
    ipa1 ?-> pa1;

    *pa1 = 1;

    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetN}
\settowidth{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetN}{\usebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetM}}
\newsavebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetO}
\begin{lrbox}{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetO}
\begin{minipage}{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00100|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv.EL2+dsb-tlbiipa-dsb-tlbiis-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetI}\\
  \cline{2-2}
  & thread0 el2 handler lower exc\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoWTf.inv.EL2+po.tex <==
\newlength{\CoWTfdotinvdotELtwopluspoH}
\setlength{\CoWTfdotinvdotELtwopluspoH}{0cm}
\newsavebox{\CoWTfdotinvdotELtwopluspoI}
\begin{lrbox}{\CoWTfdotinvdotELtwopluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELtwopluspoJ}
\settowidth{\CoWTfdotinvdotELtwopluspoJ}{\usebox{\CoWTfdotinvdotELtwopluspoI}}
\addtolength{\CoWTfdotinvdotELtwopluspoH}{\CoWTfdotinvdotELtwopluspoJ}
\newsavebox{\CoWTfdotinvdotELtwopluspoK}
\begin{lrbox}{\CoWTfdotinvdotELtwopluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X20,ELR_EL2
ADD X20,X20,#4
MSR ELR_EL2,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELtwopluspoL}
\settowidth{\CoWTfdotinvdotELtwopluspoL}{\usebox{\CoWTfdotinvdotELtwopluspoK}}
\addtolength{\CoWTfdotinvdotELtwopluspoH}{\CoWTfdotinvdotELtwopluspoL}
\newsavebox{\CoWTfdotinvdotELtwopluspoM}
\begin{lrbox}{\CoWTfdotinvdotELtwopluspoM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;

    ipa1 |-> invalid;
    ipa1 ?-> pa1;

    *pa1 = 1;

    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELtwopluspoN}
\settowidth{\CoWTfdotinvdotELtwopluspoN}{\usebox{\CoWTfdotinvdotELtwopluspoM}}
\newsavebox{\CoWTfdotinvdotELtwopluspoO}
\begin{lrbox}{\CoWTfdotinvdotELtwopluspoO}
\begin{minipage}{\CoWTfdotinvdotELtwopluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00100|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv.EL2+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvdotELtwopluspoN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvdotELtwopluspoM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvdotELtwopluspoO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELtwopluspoI}\\
  \cline{2-2}
  & thread0 el2 handler lower exc\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELtwopluspoK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoWTv2.2.inv+dsb-tlbivmidis-dsb-eret.tex <==
\newlength{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetH}
\setlength{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetH}{0cm}
\newsavebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetI}
\begin{lrbox}{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VMALLS12E1IS
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetJ}
\settowidth{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetJ}{\usebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetI}}
\addtolength{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetH}{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetJ}
\newsavebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetK}
\begin{lrbox}{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetL}
\settowidth{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetL}{\usebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetK}}
\addtolength{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetH}{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetL}
\newsavebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetM}
\begin{lrbox}{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;
    ipa1 |-> invalid;
    ipa1 ?-> pa1;

    *pa1 = 1;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetN}
\settowidth{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetN}{\usebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetM}}
\newsavebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetO}
\begin{lrbox}{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetO}
\begin{minipage}{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00101|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTv2.2.inv+dsb-tlbivmidis-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetI}\\
  \cline{2-2}
  & thread0 el2 handler\\
  \cline{2-2}
  & \usebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoWW.alias.tex <==
\newlength{\CoWWdotaliasH}
\setlength{\CoWWdotaliasH}{0cm}
\newsavebox{\CoWWdotaliasI}
\begin{lrbox}{\CoWWdotaliasI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWWdotaliasJ}
\settowidth{\CoWWdotaliasJ}{\usebox{\CoWWdotaliasI}}
\addtolength{\CoWWdotaliasH}{\CoWWdotaliasJ}
\newsavebox{\CoWWdotaliasK}
\begin{lrbox}{\CoWWdotaliasK}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    y |-> pa1;
    *pa1 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWWdotaliasL}
\settowidth{\CoWWdotaliasL}{\usebox{\CoWWdotaliasK}}
\newsavebox{\CoWWdotaliasM}
\begin{lrbox}{\CoWWdotaliasM}
\begin{minipage}{\CoWWdotaliasH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=0b01|\\
\lstinline[language=IslaLitmusExp]|R1=x|\\
\lstinline[language=IslaLitmusExp]|R2=0b10|\\
\lstinline[language=IslaLitmusExp]|R3=y|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWW.alias|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWWdotaliasL}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWWdotaliasK}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWWdotaliasM}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWWdotaliasI}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|x=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoWinvRpte+po.tex <==
\newlength{\CoWinvRptepluspoH}
\setlength{\CoWinvRptepluspoH}{0cm}
\newsavebox{\CoWinvRptepluspoI}
\begin{lrbox}{\CoWinvRptepluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvRptepluspoJ}
\settowidth{\CoWinvRptepluspoJ}{\usebox{\CoWinvRptepluspoI}}
\addtolength{\CoWinvRptepluspoH}{\CoWinvRptepluspoJ}
\newsavebox{\CoWinvRptepluspoK}
\begin{lrbox}{\CoWinvRptepluspoK}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;

    *pa1 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvRptepluspoL}
\settowidth{\CoWinvRptepluspoL}{\usebox{\CoWinvRptepluspoK}}
\newsavebox{\CoWinvRptepluspoM}
\begin{lrbox}{\CoWinvRptepluspoM}
\begin{minipage}{\CoWinvRptepluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=0x0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvRpte+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvRptepluspoL}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvRptepluspoK}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvRptepluspoM}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvRptepluspoI}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|~0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoWinvT+dsb-isb.tex <==
\newlength{\CoWinvTplusdsbisbH}
\setlength{\CoWinvTplusdsbisbH}{0cm}
\newsavebox{\CoWinvTplusdsbisbI}
\begin{lrbox}{\CoWinvTplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTplusdsbisbJ}
\settowidth{\CoWinvTplusdsbisbJ}{\usebox{\CoWinvTplusdsbisbI}}
\addtolength{\CoWinvTplusdsbisbH}{\CoWinvTplusdsbisbJ}
\newsavebox{\CoWinvTplusdsbisbK}
\begin{lrbox}{\CoWinvTplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTplusdsbisbL}
\settowidth{\CoWinvTplusdsbisbL}{\usebox{\CoWinvTplusdsbisbK}}
\addtolength{\CoWinvTplusdsbisbH}{\CoWinvTplusdsbisbL}
\newsavebox{\CoWinvTplusdsbisbM}
\begin{lrbox}{\CoWinvTplusdsbisbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTplusdsbisbN}
\settowidth{\CoWinvTplusdsbisbN}{\usebox{\CoWinvTplusdsbisbM}}
\newsavebox{\CoWinvTplusdsbisbO}
\begin{lrbox}{\CoWinvTplusdsbisbO}
\begin{minipage}{\CoWinvTplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvT+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTplusdsbisbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTplusdsbisbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTplusdsbisbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTplusdsbisbI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTplusdsbisbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoWinvT+po.tex <==
\newlength{\CoWinvTpluspoH}
\setlength{\CoWinvTpluspoH}{0cm}
\newsavebox{\CoWinvTpluspoI}
\begin{lrbox}{\CoWinvTpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTpluspoJ}
\settowidth{\CoWinvTpluspoJ}{\usebox{\CoWinvTpluspoI}}
\addtolength{\CoWinvTpluspoH}{\CoWinvTpluspoJ}
\newsavebox{\CoWinvTpluspoK}
\begin{lrbox}{\CoWinvTpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTpluspoL}
\settowidth{\CoWinvTpluspoL}{\usebox{\CoWinvTpluspoK}}
\addtolength{\CoWinvTpluspoH}{\CoWinvTpluspoL}
\newsavebox{\CoWinvTpluspoM}
\begin{lrbox}{\CoWinvTpluspoM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTpluspoN}
\settowidth{\CoWinvTpluspoN}{\usebox{\CoWinvTpluspoM}}
\newsavebox{\CoWinvTpluspoO}
\begin{lrbox}{\CoWinvTpluspoO}
\begin{minipage}{\CoWinvTpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvT+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTpluspoN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTpluspoM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTpluspoO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTpluspoI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTpluspoK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoWinvT.EL1+dsb-tlbi-dsb-isb.tex <==
\newlength{\CoWinvTdotELoneplusdsbtlbidsbisbH}
\setlength{\CoWinvTdotELoneplusdsbtlbidsbisbH}{0cm}
\newsavebox{\CoWinvTdotELoneplusdsbtlbidsbisbI}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbidsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1,X5
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbidsbisbJ}
\settowidth{\CoWinvTdotELoneplusdsbtlbidsbisbJ}{\usebox{\CoWinvTdotELoneplusdsbtlbidsbisbI}}
\addtolength{\CoWinvTdotELoneplusdsbtlbidsbisbH}{\CoWinvTdotELoneplusdsbtlbidsbisbJ}
\newsavebox{\CoWinvTdotELoneplusdsbtlbidsbisbK}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbidsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1000:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbidsbisbL}
\settowidth{\CoWinvTdotELoneplusdsbtlbidsbisbL}{\usebox{\CoWinvTdotELoneplusdsbtlbidsbisbK}}
\addtolength{\CoWinvTdotELoneplusdsbtlbidsbisbH}{\CoWinvTdotELoneplusdsbtlbidsbisbL}
\newsavebox{\CoWinvTdotELoneplusdsbtlbidsbisbM}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbidsbisbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbidsbisbN}
\settowidth{\CoWinvTdotELoneplusdsbtlbidsbisbN}{\usebox{\CoWinvTdotELoneplusdsbtlbidsbisbM}}
\newsavebox{\CoWinvTdotELoneplusdsbtlbidsbisbO}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbidsbisbO}
\begin{minipage}{\CoWinvTdotELoneplusdsbtlbidsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R5=page(x)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvT.EL1+dsb-tlbi-dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTdotELoneplusdsbtlbidsbisbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTdotELoneplusdsbtlbidsbisbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTdotELoneplusdsbtlbidsbisbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTdotELoneplusdsbtlbidsbisbI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTdotELoneplusdsbtlbidsbisbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoWinvT.EL1+dsb-tlbi-dsb.tex <==
\newlength{\CoWinvTdotELoneplusdsbtlbidsbH}
\setlength{\CoWinvTdotELoneplusdsbtlbidsbH}{0cm}
\newsavebox{\CoWinvTdotELoneplusdsbtlbidsbI}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbidsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1,X5
DSB SY
MOV X2,#0
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbidsbJ}
\settowidth{\CoWinvTdotELoneplusdsbtlbidsbJ}{\usebox{\CoWinvTdotELoneplusdsbtlbidsbI}}
\addtolength{\CoWinvTdotELoneplusdsbtlbidsbH}{\CoWinvTdotELoneplusdsbtlbidsbJ}
\newsavebox{\CoWinvTdotELoneplusdsbtlbidsbK}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbidsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1000:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbidsbL}
\settowidth{\CoWinvTdotELoneplusdsbtlbidsbL}{\usebox{\CoWinvTdotELoneplusdsbtlbidsbK}}
\addtolength{\CoWinvTdotELoneplusdsbtlbidsbH}{\CoWinvTdotELoneplusdsbtlbidsbL}
\newsavebox{\CoWinvTdotELoneplusdsbtlbidsbM}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbidsbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbidsbN}
\settowidth{\CoWinvTdotELoneplusdsbtlbidsbN}{\usebox{\CoWinvTdotELoneplusdsbtlbidsbM}}
\newsavebox{\CoWinvTdotELoneplusdsbtlbidsbO}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbidsbO}
\begin{minipage}{\CoWinvTdotELoneplusdsbtlbidsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R5=page(x)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvT.EL1+dsb-tlbi-dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTdotELoneplusdsbtlbidsbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTdotELoneplusdsbtlbidsbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTdotELoneplusdsbtlbidsbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTdotELoneplusdsbtlbidsbI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTdotELoneplusdsbtlbidsbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoWinvT.EL1+dsb-tlbiis-dsb-isb.tex <==
\newlength{\CoWinvTdotELoneplusdsbtlbiisdsbisbH}
\setlength{\CoWinvTdotELoneplusdsbtlbiisdsbisbH}{0cm}
\newsavebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbI}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbiisdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X5
DSB SY
ISB
MOV X2,#0
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbiisdsbisbJ}
\settowidth{\CoWinvTdotELoneplusdsbtlbiisdsbisbJ}{\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbI}}
\addtolength{\CoWinvTdotELoneplusdsbtlbiisdsbisbH}{\CoWinvTdotELoneplusdsbtlbiisdsbisbJ}
\newsavebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbK}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbiisdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1000:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbiisdsbisbL}
\settowidth{\CoWinvTdotELoneplusdsbtlbiisdsbisbL}{\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbK}}
\addtolength{\CoWinvTdotELoneplusdsbtlbiisdsbisbH}{\CoWinvTdotELoneplusdsbtlbiisdsbisbL}
\newsavebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbM}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbiisdsbisbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbiisdsbisbN}
\settowidth{\CoWinvTdotELoneplusdsbtlbiisdsbisbN}{\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbM}}
\newsavebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbO}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbiisdsbisbO}
\begin{minipage}{\CoWinvTdotELoneplusdsbtlbiisdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R5=page(x)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvT.EL1+dsb-tlbiis-dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTdotELoneplusdsbtlbiisdsbisbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoWinvT.EL1+dsb-tlbiis-dsb.tex <==
\newlength{\CoWinvTdotELoneplusdsbtlbiisdsbH}
\setlength{\CoWinvTdotELoneplusdsbtlbiisdsbH}{0cm}
\newsavebox{\CoWinvTdotELoneplusdsbtlbiisdsbI}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbiisdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X5
DSB SY
MOV X2,#0
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbiisdsbJ}
\settowidth{\CoWinvTdotELoneplusdsbtlbiisdsbJ}{\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbI}}
\addtolength{\CoWinvTdotELoneplusdsbtlbiisdsbH}{\CoWinvTdotELoneplusdsbtlbiisdsbJ}
\newsavebox{\CoWinvTdotELoneplusdsbtlbiisdsbK}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbiisdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1000:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbiisdsbL}
\settowidth{\CoWinvTdotELoneplusdsbtlbiisdsbL}{\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbK}}
\addtolength{\CoWinvTdotELoneplusdsbtlbiisdsbH}{\CoWinvTdotELoneplusdsbtlbiisdsbL}
\newsavebox{\CoWinvTdotELoneplusdsbtlbiisdsbM}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbiisdsbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbiisdsbN}
\settowidth{\CoWinvTdotELoneplusdsbtlbiisdsbN}{\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbM}}
\newsavebox{\CoWinvTdotELoneplusdsbtlbiisdsbO}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbiisdsbO}
\begin{minipage}{\CoWinvTdotELoneplusdsbtlbiisdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R5=page(x)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvT.EL1+dsb-tlbiis-dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTdotELoneplusdsbtlbiisdsbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTdotELoneplusdsbtlbiisdsbI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTdotELoneplusdsbtlbiisdsbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoWinvT2+dsb-tlbiipa-dsb-eret.tex <==
\newlength{\CoWinvTtwoplusdsbtlbiipadsberetH}
\setlength{\CoWinvTtwoplusdsbtlbiipadsberetH}{0cm}
\newsavebox{\CoWinvTtwoplusdsbtlbiipadsberetI}
\begin{lrbox}{\CoWinvTtwoplusdsbtlbiipadsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1,X4
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTtwoplusdsbtlbiipadsberetJ}
\settowidth{\CoWinvTtwoplusdsbtlbiipadsberetJ}{\usebox{\CoWinvTtwoplusdsbtlbiipadsberetI}}
\addtolength{\CoWinvTtwoplusdsbtlbiipadsberetH}{\CoWinvTtwoplusdsbtlbiipadsberetJ}
\newsavebox{\CoWinvTtwoplusdsbtlbiipadsberetK}
\begin{lrbox}{\CoWinvTtwoplusdsbtlbiipadsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X20,ELR_EL2
ADD X20,X20,#4
MSR ELR_EL2,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTtwoplusdsbtlbiipadsberetL}
\settowidth{\CoWinvTtwoplusdsbtlbiipadsberetL}{\usebox{\CoWinvTtwoplusdsbtlbiipadsberetK}}
\addtolength{\CoWinvTtwoplusdsbtlbiipadsberetH}{\CoWinvTtwoplusdsbtlbiipadsberetL}
\newsavebox{\CoWinvTtwoplusdsbtlbiipadsberetM}
\begin{lrbox}{\CoWinvTtwoplusdsbtlbiipadsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;

    ipa1 |-> invalid;
    ipa1 ?-> pa1;

    *pa1 = 1;

    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTtwoplusdsbtlbiipadsberetN}
\settowidth{\CoWinvTtwoplusdsbtlbiipadsberetN}{\usebox{\CoWinvTtwoplusdsbtlbiipadsberetM}}
\newsavebox{\CoWinvTtwoplusdsbtlbiipadsberetO}
\begin{lrbox}{\CoWinvTtwoplusdsbtlbiipadsberetO}
\begin{minipage}{\CoWinvTtwoplusdsbtlbiipadsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=page(ipa1)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00100|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvT2+dsb-tlbiipa-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTtwoplusdsbtlbiipadsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTtwoplusdsbtlbiipadsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTtwoplusdsbtlbiipadsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTtwoplusdsbtlbiipadsberetI}\\
  \cline{2-2}
  & thread0 el2 handler lower exc\\
  \cline{2-2}
  & \usebox{\CoWinvTtwoplusdsbtlbiipadsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoWinvT2+dsb-tlbiipa-dsb-tlbivmall-dsb-eret.tex <==
\newlength{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetH}
\setlength{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetH}{0cm}
\newsavebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetI}
\begin{lrbox}{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1,X4
DSB SY
TLBI VMALLE1
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetJ}
\settowidth{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetJ}{\usebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetI}}
\addtolength{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetH}{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetJ}
\newsavebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetK}
\begin{lrbox}{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#1
MRS X20,ELR_EL2
ADD X20,X20,#4
MSR ELR_EL2,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetL}
\settowidth{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetL}{\usebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetK}}
\addtolength{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetH}{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetL}
\newsavebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetM}
\begin{lrbox}{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;

    ipa1 |-> pa1;
    ipa1 ?-> invalid;

    *pa1 = 0;

    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetN}
\settowidth{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetN}{\usebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetM}}
\newsavebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetO}
\begin{lrbox}{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetO}
\begin{minipage}{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=page(ipa1)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00100|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvT2+dsb-tlbiipa-dsb-tlbivmall-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetI}\\
  \cline{2-2}
  & thread0 el2 handler lower exc\\
  \cline{2-2}
  & \usebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoWinvTa1.1+dsb-tlbiasidis-dsb-eret.tex <==
\newlength{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetH}
\setlength{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetH}{0cm}
\newsavebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetI}
\begin{lrbox}{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI ASIDE1IS,X4
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetJ}
\settowidth{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetJ}{\usebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetI}}
\addtolength{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetH}{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetJ}
\newsavebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetK}
\begin{lrbox}{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetL}
\settowidth{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetL}{\usebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetK}}
\addtolength{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetH}{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetL}
\newsavebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetM}
\begin{lrbox}{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetN}
\settowidth{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetN}{\usebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetM}}
\newsavebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetO}
\begin{lrbox}{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetO}
\begin{minipage}{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL1=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=asid(0x1)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL1=0b00000|\\
\lstinline[language=IslaLitmusExp]|TTBR0_EL1=ttbr(base=page_table_base,asid=0x0001)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvTa1.1+dsb-tlbiasidis-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoWinvTa2.1+dsb-tlbiasidis-dsb-eret.tex <==
\newlength{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetH}
\setlength{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetH}{0cm}
\newsavebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetI}
\begin{lrbox}{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI ASIDE1IS,X4
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetJ}
\settowidth{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetJ}{\usebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetI}}
\addtolength{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetH}{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetJ}
\newsavebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetK}
\begin{lrbox}{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetL}
\settowidth{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetL}{\usebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetK}}
\addtolength{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetH}{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetL}
\newsavebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetM}
\begin{lrbox}{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetN}
\settowidth{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetN}{\usebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetM}}
\newsavebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetO}
\begin{lrbox}{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetO}
\begin{minipage}{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL1=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=asid(0x2)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL1=0b00000|\\
\lstinline[language=IslaLitmusExp]|TTBR0_EL1=ttbr(base=page_table_base,asid=0x0001)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvTa2.1+dsb-tlbiasidis-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoWinvTv1.2+dsb-tlbivmidis-dsb-eret.tex <==
\newlength{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetH}
\setlength{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetH}{0cm}
\newsavebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetI}
\begin{lrbox}{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VMALLS12E1IS
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetJ}
\settowidth{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetJ}{\usebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetI}}
\addtolength{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetH}{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetJ}
\newsavebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetK}
\begin{lrbox}{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#1
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetL}
\settowidth{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetL}{\usebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetK}}
\addtolength{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetH}{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetL}
\newsavebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetM}
\begin{lrbox}{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;
    ipa1 |-> pa1;
    ipa1 ?-> invalid;

    *pa1 = 0;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetN}
\settowidth{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetN}{\usebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetM}}
\newsavebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetO}
\begin{lrbox}{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetO}
\begin{minipage}{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00101|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvTv1.2+dsb-tlbivmidis-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetI}\\
  \cline{2-2}
  & thread0 el2 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/CoWinvTv2.2+dsb-tlbivmidis-msrvttbr-dsb-eret.tex <==
\newlength{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetH}
\setlength{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetH}{0cm}
\newsavebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetI}
\begin{lrbox}{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VMALLS12E1IS
DSB SY
MSR VTTBR_EL2,X4
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetJ}
\settowidth{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetJ}{\usebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetI}}
\addtolength{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetH}{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetJ}
\newsavebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetK}
\begin{lrbox}{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#1
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetL}
\settowidth{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetL}{\usebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetK}}
\addtolength{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetH}{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetL}
\newsavebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetM}
\begin{lrbox}{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;
    ipa1 |-> pa1;
    ipa1 ?-> invalid;

    *pa1 = 0;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetN}
\settowidth{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetN}{\usebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetM}}
\newsavebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetO}
\begin{lrbox}{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetO}
\begin{minipage}{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=ttbr(vmid=0x0001,base=s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00101|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvTv2.2+dsb-tlbivmidis-msrvttbr-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetI}\\
  \cline{2-2}
  & thread0 el2 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/ETS.tex <==
\newlength{\ETSH}
\setlength{\ETSH}{0cm}
\newsavebox{\ETSI}
\begin{lrbox}{\ETSI}
\begin{lstlisting}[language=AArch64,showlines=true]
MOV X0,#1
STR X0,[X3]
DMB SY
STR X0,[X2]
\end{lstlisting}
\end{lrbox}
\newlength{\ETSJ}
\settowidth{\ETSJ}{\usebox{\ETSI}}
\addtolength{\ETSH}{\ETSJ}
\newsavebox{\ETSK}
\begin{lrbox}{\ETSK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X2]
STR X0,[X1]
MOV X4,#2
STR X4,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\ETSL}
\settowidth{\ETSL}{\usebox{\ETSK}}
\addtolength{\ETSH}{\ETSL}
\newsavebox{\ETSM}
\begin{lrbox}{\ETSM}
\begin{lstlisting}[language=AArch64,showlines=true]
MOV X0,#0
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\ETSN}
\settowidth{\ETSN}{\usebox{\ETSM}}
\addtolength{\ETSH}{\ETSN}
\newsavebox{\ETSO}
\begin{lrbox}{\ETSO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
LDR X7,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\ETSP}
\settowidth{\ETSP}{\usebox{\ETSO}}
\addtolength{\ETSH}{\ETSP}
\newsavebox{\ETSA}
\begin{lrbox}{\ETSA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> pa1;
    x ?-> invalid;
    y |-> pa2;
    z |-> pa3;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\ETSB}
\settowidth{\ETSB}{\usebox{\ETSA}}
\newsavebox{\ETSC}
\begin{lrbox}{\ETSC}
\begin{minipage}{\ETSH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R2=y|\\
\lstinline[language=IslaLitmusExp]|0:R3=z|\\
\lstinline[language=IslaLitmusExp]|1:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=z|\\
\lstinline[language=IslaLitmusExp]|1:R6=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R7=0b1|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:R1=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|ETS|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\ETSB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\ETSA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\ETSC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\ETSI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\ETSK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\ETSM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\ETSO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & x=1 & 1:R7=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/IRIW.TTf.TTf.inv+addrs.tex <==
\newlength{\IRIWdotTTfdotTTfdotinvplusaddrsH}
\setlength{\IRIWdotTTfdotTTfdotinvplusaddrsH}{0cm}
\newsavebox{\IRIWdotTTfdotTTfdotinvplusaddrsI}
\begin{lrbox}{\IRIWdotTTfdotTTfdotinvplusaddrsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\IRIWdotTTfdotTTfdotinvplusaddrsJ}
\settowidth{\IRIWdotTTfdotTTfdotinvplusaddrsJ}{\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsI}}
\addtolength{\IRIWdotTTfdotTTfdotinvplusaddrsH}{\IRIWdotTTfdotTTfdotinvplusaddrsJ}
\newsavebox{\IRIWdotTTfdotTTfdotinvplusaddrsK}
\begin{lrbox}{\IRIWdotTTfdotTTfdotinvplusaddrsK}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\IRIWdotTTfdotTTfdotinvplusaddrsL}
\settowidth{\IRIWdotTTfdotTTfdotinvplusaddrsL}{\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsK}}
\addtolength{\IRIWdotTTfdotTTfdotinvplusaddrsH}{\IRIWdotTTfdotTTfdotinvplusaddrsL}
\newsavebox{\IRIWdotTTfdotTTfdotinvplusaddrsM}
\begin{lrbox}{\IRIWdotTTfdotTTfdotinvplusaddrsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\IRIWdotTTfdotTTfdotinvplusaddrsN}
\settowidth{\IRIWdotTTfdotTTfdotinvplusaddrsN}{\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsM}}
\addtolength{\IRIWdotTTfdotTTfdotinvplusaddrsH}{\IRIWdotTTfdotTTfdotinvplusaddrsN}
\newsavebox{\IRIWdotTTfdotTTfdotinvplusaddrsO}
\begin{lrbox}{\IRIWdotTTfdotTTfdotinvplusaddrsO}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\IRIWdotTTfdotTTfdotinvplusaddrsP}
\settowidth{\IRIWdotTTfdotTTfdotinvplusaddrsP}{\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsO}}
\addtolength{\IRIWdotTTfdotTTfdotinvplusaddrsH}{\IRIWdotTTfdotTTfdotinvplusaddrsP}
\newsavebox{\IRIWdotTTfdotTTfdotinvplusaddrsA}
\begin{lrbox}{\IRIWdotTTfdotTTfdotinvplusaddrsA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\IRIWdotTTfdotTTfdotinvplusaddrsB}
\settowidth{\IRIWdotTTfdotTTfdotinvplusaddrsB}{\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsA}}
\addtolength{\IRIWdotTTfdotTTfdotinvplusaddrsH}{\IRIWdotTTfdotTTfdotinvplusaddrsB}
\newsavebox{\IRIWdotTTfdotTTfdotinvplusaddrsC}
\begin{lrbox}{\IRIWdotTTfdotTTfdotinvplusaddrsC}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\IRIWdotTTfdotTTfdotinvplusaddrsD}
\settowidth{\IRIWdotTTfdotTTfdotinvplusaddrsD}{\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsC}}
\addtolength{\IRIWdotTTfdotTTfdotinvplusaddrsH}{\IRIWdotTTfdotTTfdotinvplusaddrsD}
\newsavebox{\IRIWdotTTfdotTTfdotinvplusaddrsE}
\begin{lrbox}{\IRIWdotTTfdotTTfdotinvplusaddrsE}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> invalid;
    y ?-> pa2;
    v |-> pa2;
    *pa2 = 1;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\IRIWdotTTfdotTTfdotinvplusaddrsF}
\settowidth{\IRIWdotTTfdotTTfdotinvplusaddrsF}{\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsE}}
\newsavebox{\IRIWdotTTfdotTTfdotinvplusaddrsHG}
\begin{lrbox}{\IRIWdotTTfdotTTfdotinvplusaddrsHG}
\begin{minipage}{\IRIWdotTTfdotTTfdotinvplusaddrsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R0=desc3(v,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=x|\\
\lstinline[language=IslaLitmusExp]|2:R3=y|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|3:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|3:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|3:R1=y|\\
\lstinline[language=IslaLitmusExp]|3:R3=x|\\
\lstinline[language=IslaLitmusExp]|3:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|IRIW.TTf.TTf.inv+addrs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\IRIWdotTTfdotTTfdotinvplusaddrsF}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsE}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsHG}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\IRIWdotTTfdotTTfdotinvplusaddrsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\IRIWdotTTfdotTTfdotinvplusaddrsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\IRIWdotTTfdotTTfdotinvplusaddrsM}\\
  \cline{2-2}
  & Thread 3\\
  \cline{2-2}
  & \usebox{\IRIWdotTTfdotTTfdotinvplusaddrsO}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\IRIWdotTTfdotTTfdotinvplusaddrsA}\\
  \cline{2-2}
  & thread3 el1 handler\\
  \cline{2-2}
  & \usebox{\IRIWdotTTfdotTTfdotinvplusaddrsC}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|2:R0=1 & 2:R2=0 & 3:R0=1 & 3:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/ISA2.RRTf.inv+dsb+addr+addr.tex <==
\newlength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrH}
\setlength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrH}{0cm}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrI}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrJ}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrJ}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrI}}
\addtolength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrH}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrJ}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrK}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
STR X3,[X4,X2]
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrL}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrL}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrK}}
\addtolength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrH}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrL}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrM}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
LDR X3,[X4,X2]
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrN}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrN}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrM}}
\addtolength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrH}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrN}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrO}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X3,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrP}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrP}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrO}}
\addtolength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrH}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrP}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrA}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    *pa2 = 0;

    z |-> pa3;
    *pa3 = 0;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrB}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrB}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrA}}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrC}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrC}
\begin{minipage}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R4=z|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=z|\\
\lstinline[language=IslaLitmusExp]|2:R4=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|ISA2.RRTf.inv+dsb+addr+addr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrM}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R3=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/ISA2.RRTf.inv+dsb+data+addr.tex <==
\newlength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrH}
\setlength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrH}{0cm}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrI}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrJ}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrJ}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrI}}
\addtolength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrH}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrJ}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrK}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
ORR X3,X3,X2
STR X3,[X4]
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrL}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrL}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrK}}
\addtolength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrH}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrL}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrM}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
LDR X3,[X4,X2]
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrN}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrN}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrM}}
\addtolength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrH}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrN}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrO}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X3,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrP}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrP}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrO}}
\addtolength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrH}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrP}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrA}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    *pa2 = 0;

    z |-> pa3;
    *pa3 = 0;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrB}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrB}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrA}}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrC}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrC}
\begin{minipage}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R4=z|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=z|\\
\lstinline[language=IslaLitmusExp]|2:R4=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|ISA2.RRTf.inv+dsb+data+addr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrM}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R3=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/LB+addr-trfis.tex <==
\newlength{\LBplusaddrtrfisH}
\setlength{\LBplusaddrtrfisH}{0cm}
\newsavebox{\LBplusaddrtrfisI}
\begin{lrbox}{\LBplusaddrtrfisI}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
STR X3,[X4,X2]
STR X5,[X6]
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusaddrtrfisJ}
\settowidth{\LBplusaddrtrfisJ}{\usebox{\LBplusaddrtrfisI}}
\addtolength{\LBplusaddrtrfisH}{\LBplusaddrtrfisJ}
\newsavebox{\LBplusaddrtrfisK}
\begin{lrbox}{\LBplusaddrtrfisK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
STR X3,[X4,X2]
STR X5,[X6]
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusaddrtrfisL}
\settowidth{\LBplusaddrtrfisL}{\usebox{\LBplusaddrtrfisK}}
\addtolength{\LBplusaddrtrfisH}{\LBplusaddrtrfisL}
\newsavebox{\LBplusaddrtrfisM}
\begin{lrbox}{\LBplusaddrtrfisM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X7,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusaddrtrfisN}
\settowidth{\LBplusaddrtrfisN}{\usebox{\LBplusaddrtrfisM}}
\addtolength{\LBplusaddrtrfisH}{\LBplusaddrtrfisN}
\newsavebox{\LBplusaddrtrfisO}
\begin{lrbox}{\LBplusaddrtrfisO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X7,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusaddrtrfisP}
\settowidth{\LBplusaddrtrfisP}{\usebox{\LBplusaddrtrfisO}}
\addtolength{\LBplusaddrtrfisH}{\LBplusaddrtrfisP}
\newsavebox{\LBplusaddrtrfisA}
\begin{lrbox}{\LBplusaddrtrfisA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3 pa4;
    x |-> pa1;
    y |-> pa2;
    u |-> invalid;
    u ?-> pa2;
    v |-> invalid;
    v ?-> pa1;
    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusaddrtrfisB}
\settowidth{\LBplusaddrtrfisB}{\usebox{\LBplusaddrtrfisA}}
\newsavebox{\LBplusaddrtrfisC}
\begin{lrbox}{\LBplusaddrtrfisC}
\begin{minipage}{\LBplusaddrtrfisH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R3=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R4=pte3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R5=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R6=u|\\
\lstinline[language=IslaLitmusExp]|0:R7=0b1|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|0:__isla_monomorphize_writes=true|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=desc3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R4=pte3(v,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R5=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R6=v|\\
\lstinline[language=IslaLitmusExp]|1:R7=0b1|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\lstinline[language=IslaLitmusExp]|1:__isla_monomorphize_writes=true|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|LB+addr-trfis|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\LBplusaddrtrfisB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\LBplusaddrtrfisA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\LBplusaddrtrfisC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\LBplusaddrtrfisI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\LBplusaddrtrfisK}\\
  \cline{2-2}
  & thread1 el0 handler\\
  \cline{2-2}
  & \usebox{\LBplusaddrtrfisM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\LBplusaddrtrfisO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R0=1 & 0:R7=1 & 1:R0=1 & 1:R7=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/LB+data-trfis.tex <==
\newlength{\LBplusdatatrfisH}
\setlength{\LBplusdatatrfisH}{0cm}
\newsavebox{\LBplusdatatrfisI}
\begin{lrbox}{\LBplusdatatrfisI}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
ORR X3,X3,X2
STR X3,[X4]
STR X5,[X6]
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusdatatrfisJ}
\settowidth{\LBplusdatatrfisJ}{\usebox{\LBplusdatatrfisI}}
\addtolength{\LBplusdatatrfisH}{\LBplusdatatrfisJ}
\newsavebox{\LBplusdatatrfisK}
\begin{lrbox}{\LBplusdatatrfisK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
ORR X3,X3,X2
STR X3,[X4]
STR X5,[X6]
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusdatatrfisL}
\settowidth{\LBplusdatatrfisL}{\usebox{\LBplusdatatrfisK}}
\addtolength{\LBplusdatatrfisH}{\LBplusdatatrfisL}
\newsavebox{\LBplusdatatrfisM}
\begin{lrbox}{\LBplusdatatrfisM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X7,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusdatatrfisN}
\settowidth{\LBplusdatatrfisN}{\usebox{\LBplusdatatrfisM}}
\addtolength{\LBplusdatatrfisH}{\LBplusdatatrfisN}
\newsavebox{\LBplusdatatrfisO}
\begin{lrbox}{\LBplusdatatrfisO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X7,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusdatatrfisP}
\settowidth{\LBplusdatatrfisP}{\usebox{\LBplusdatatrfisO}}
\addtolength{\LBplusdatatrfisH}{\LBplusdatatrfisP}
\newsavebox{\LBplusdatatrfisA}
\begin{lrbox}{\LBplusdatatrfisA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3 pa4;
    x |-> pa1;
    y |-> pa2;
    u |-> invalid;
    u ?-> pa2;
    v |-> invalid;
    v ?-> pa1;
    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusdatatrfisB}
\settowidth{\LBplusdatatrfisB}{\usebox{\LBplusdatatrfisA}}
\newsavebox{\LBplusdatatrfisC}
\begin{lrbox}{\LBplusdatatrfisC}
\begin{minipage}{\LBplusdatatrfisH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R3=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R4=pte3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R5=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R6=u|\\
\lstinline[language=IslaLitmusExp]|0:R7=0b1|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=desc3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R4=pte3(v,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R5=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R6=v|\\
\lstinline[language=IslaLitmusExp]|1:R7=0b1|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|LB+data-trfis|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\LBplusdatatrfisB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\LBplusdatatrfisA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\LBplusdatatrfisC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\LBplusdatatrfisI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\LBplusdatatrfisK}\\
  \cline{2-2}
  & thread1 el0 handler\\
  \cline{2-2}
  & \usebox{\LBplusdatatrfisM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\LBplusdatatrfisO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R0=1 & 0:R7=1 & 1:R0=1 & 1:R7=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/LB.TT.inv+pos.tex <==
\newlength{\LBdotTTdotinvplusposH}
\setlength{\LBdotTTdotinvplusposH}{0cm}
\newsavebox{\LBdotTTdotinvplusposI}
\begin{lrbox}{\LBdotTTdotinvplusposI}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\LBdotTTdotinvplusposJ}
\settowidth{\LBdotTTdotinvplusposJ}{\usebox{\LBdotTTdotinvplusposI}}
\addtolength{\LBdotTTdotinvplusposH}{\LBdotTTdotinvplusposJ}
\newsavebox{\LBdotTTdotinvplusposK}
\begin{lrbox}{\LBdotTTdotinvplusposK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\LBdotTTdotinvplusposL}
\settowidth{\LBdotTTdotinvplusposL}{\usebox{\LBdotTTdotinvplusposK}}
\addtolength{\LBdotTTdotinvplusposH}{\LBdotTTdotinvplusposL}
\newsavebox{\LBdotTTdotinvplusposM}
\begin{lrbox}{\LBdotTTdotinvplusposM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\LBdotTTdotinvplusposN}
\settowidth{\LBdotTTdotinvplusposN}{\usebox{\LBdotTTdotinvplusposM}}
\addtolength{\LBdotTTdotinvplusposH}{\LBdotTTdotinvplusposN}
\newsavebox{\LBdotTTdotinvplusposO}
\begin{lrbox}{\LBdotTTdotinvplusposO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\LBdotTTdotinvplusposP}
\settowidth{\LBdotTTdotinvplusposP}{\usebox{\LBdotTTdotinvplusposO}}
\addtolength{\LBdotTTdotinvplusposH}{\LBdotTTdotinvplusposP}
\newsavebox{\LBdotTTdotinvplusposA}
\begin{lrbox}{\LBdotTTdotinvplusposA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    y |-> invalid;

    x ?-> pa1;
    y ?-> pa1;

    *pa1 = 1;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\LBdotTTdotinvplusposB}
\settowidth{\LBdotTTdotinvplusposB}{\usebox{\LBdotTTdotinvplusposA}}
\newsavebox{\LBdotTTdotinvplusposC}
\begin{lrbox}{\LBdotTTdotinvplusposC}
\begin{minipage}{\LBdotTTdotinvplusposH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|LB.TT.inv+pos|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\LBdotTTdotinvplusposB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\LBdotTTdotinvplusposA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\LBdotTTdotinvplusposC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\LBdotTTdotinvplusposI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\LBdotTTdotinvplusposK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\LBdotTTdotinvplusposM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\LBdotTTdotinvplusposO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R0=1 & 1:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.BBM1+dsb-tlbiis-dsb-dsb+ctrl-isb.tex <==
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbH}
\setlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbH}{0cm}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbI}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X6
DSB SY
STR X2,[X1]
DSB SY
STR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbJ}
\settowidth{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbJ}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbI}}
\addtolength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbH}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbJ}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbK}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBNZ X0,L0
L0:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbL}
\settowidth{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbL}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbK}}
\addtolength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbH}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbL}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbM}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbN}
\settowidth{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbN}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbM}}
\addtolength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbH}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbN}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbO}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> pa1;
    x ?-> invalid;
    x ?-> pa2;

    y |-> pa3;
    identity 0x1000 with code;

    *pa2 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbP}
\settowidth{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbP}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbO}}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbA}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbA}
\begin{minipage}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R4=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R5=y|\\
\lstinline[language=IslaLitmusExp]|0:R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.BBM1+dsb-tlbiis-dsb-dsb+ctrl-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.BBM1+dsb-tlbiis-dsb-dsb+dsb-isb.tex <==
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbH}
\setlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbI}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X6
DSB SY
STR X2,[X1]
DSB SY
STR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbJ}
\settowidth{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbJ}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbI}}
\addtolength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbH}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbJ}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbK}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbL}
\settowidth{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbL}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbK}}
\addtolength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbH}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbL}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbM}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbN}
\settowidth{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbN}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbM}}
\addtolength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbH}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbN}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbO}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> pa1;
    x ?-> invalid;
    x ?-> pa2;

    y |-> pa3;
    identity 0x1000 with code;

    *pa2 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbP}
\settowidth{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbP}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbO}}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbA}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbA}
\begin{minipage}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R4=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R5=y|\\
\lstinline[language=IslaLitmusExp]|0:R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.BBM1+dsb-tlbiis-dsb-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.RT.EL1+dsb+dsb-tlbi-dsb+dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbH}
\setlength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbJ}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbJ}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbI}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
TLBI VAE1,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbL}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbL}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbK}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbL}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbN}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbN}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbM}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbN}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbP}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbP}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbO}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbP}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbB}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbB}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbA}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbB}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbC}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> pa1;
    x ?-> invalid;

    y |-> pa2;

    a |-> pa3;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbD}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbD}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbC}}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbE}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbE}
\begin{minipage}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R3=a|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:R1=a|\\
\lstinline[language=IslaLitmusExp]|1:R2=0x2|\\
\lstinline[language=IslaLitmusExp]|1:R3=a|\\
\lstinline[language=IslaLitmusExp]|1:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|2:R1=a|\\
\lstinline[language=IslaLitmusExp]|2:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|2:R3=y|\\
\lstinline[language=IslaLitmusExp]|3:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|3:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|3:R1=y|\\
\lstinline[language=IslaLitmusExp]|3:R3=x|\\
\lstinline[language=IslaLitmusExp]|3:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL1+dsb+dsb-tlbi-dsb+dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbM}\\
  \cline{2-2}
  & Thread 3\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbO}\\
  \cline{2-2}
  & thread3 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=2 & 3:R0=1 & 3:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.RT.EL1+dsb+dsb-tlbiis-dsb+dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbH}
\setlength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbJ}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbJ}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbI}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbL}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbL}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbK}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbL}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbN}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbN}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbM}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbN}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbP}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbP}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbO}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbP}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbB}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbB}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbA}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbB}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbC}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> pa1;
    x ?-> invalid;

    y |-> pa2;

    a |-> pa3;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbD}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbD}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbC}}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbE}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbE}
\begin{minipage}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R3=a|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:R1=a|\\
\lstinline[language=IslaLitmusExp]|1:R2=0x2|\\
\lstinline[language=IslaLitmusExp]|1:R3=a|\\
\lstinline[language=IslaLitmusExp]|1:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|2:R1=a|\\
\lstinline[language=IslaLitmusExp]|2:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|2:R3=y|\\
\lstinline[language=IslaLitmusExp]|3:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|3:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|3:R1=y|\\
\lstinline[language=IslaLitmusExp]|3:R3=x|\\
\lstinline[language=IslaLitmusExp]|3:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL1+dsb+dsb-tlbiis-dsb+dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbM}\\
  \cline{2-2}
  & Thread 3\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbO}\\
  \cline{2-2}
  & thread3 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=2 & 3:R0=1 & 3:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.RT.EL1+dsb-shootdown-dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbH}
\setlength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X4,[X5]
LDR X6,[X5]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbJ}
\settowidth{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbJ}{\usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbI}}
\addtolength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbH}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X4,[X5]
SVC #0
STR X7,[X5]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbL}
\settowidth{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbL}{\usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbK}}
\addtolength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbH}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbL}
\newsavebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS X9,ESR_EL1
LSR X9,X9,#26
SUB X9,X9,#0b010101
CBNZ X9,1f
0:
DSB SY
TLBI VAE1,X6
DSB SY
ISB
ERET
1:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbN}
\settowidth{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbN}{\usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbM}}
\addtolength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbH}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbN}
\newsavebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> pa1;
    x ?-> invalid;

    y |-> pa2;
    *pa2 = 0;

    f |-> pa3;
    *pa3 = 0;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbP}
\settowidth{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbP}{\usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbO}}
\newsavebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbA}
\begin{minipage}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R5=f|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=f|\\
\lstinline[language=IslaLitmusExp]|1:R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:R7=0b10|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL1+dsb-shootdown-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R4=1 & 0:R6=2 & 1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.RT.EL1+dsb-tlbi-dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbH}
\setlength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbJ}
\settowidth{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbJ}{\usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbI}}
\addtolength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbH}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbL}
\settowidth{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbL}{\usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbK}}
\addtolength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbH}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbL}
\newsavebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbN}
\settowidth{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbN}{\usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbM}}
\addtolength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbH}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbN}
\newsavebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbP}
\settowidth{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbP}{\usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbO}}
\newsavebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbA}
\begin{minipage}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL1+dsb-tlbi-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.RT.EL1+dsb-tlbiis-dsb+dmb.tex <==
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbH}
\setlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbH}{0cm}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbI}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbJ}
\settowidth{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbJ}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbI}}
\addtolength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbJ}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbK}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbL}
\settowidth{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbL}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbK}}
\addtolength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbL}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbM}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbN}
\settowidth{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbN}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbM}}
\addtolength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbN}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbO}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbP}
\settowidth{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbP}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbO}}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbA}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbA}
\begin{minipage}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL1+dsb-tlbiis-dsb+dmb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.RT.EL1+dsb-tlbiis-dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbH}
\setlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbJ}
\settowidth{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbJ}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbI}}
\addtolength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbL}
\settowidth{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbL}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbK}}
\addtolength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbL}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbN}
\settowidth{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbN}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbM}}
\addtolength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbN}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbP}
\settowidth{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbP}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbO}}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbA}
\begin{minipage}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL1+dsb-tlbiis-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.RT.EL2+dsb-tlbiipa-dsb-tlbiis-dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbH}
\setlength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1,X4
DSB SY
TLBI VMALLE1IS
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbJ}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbJ}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbI}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbL}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbL}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbK}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbL}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#1
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbN}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbN}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbM}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbN}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
physical pa1 pa2;
intermediate ipa1 ipa2;

x |-> ipa1;
ipa1 |-> pa1;
ipa1 ?-> invalid;

y |-> ipa2;
ipa2 |-> pa2;

identity 0x2000 with code;

*pa1 = 0;
*pa2 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbP}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbP}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbO}}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbA}
\begin{minipage}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=bvlshr(ipa1,0xC)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL2+dsb-tlbiipa-dsb-tlbiis-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.RT.EL2+dsb-tlbiipais-dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbH}
\setlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbJ}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbJ}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbI}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbL}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbL}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbK}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbL}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#1
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbN}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbN}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbM}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbN}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
physical pa1 pa2;
intermediate ipa1 ipa2;

x |-> ipa1;
ipa1 |-> pa1;
ipa1 ?-> invalid;

y |-> ipa2;
ipa2 |-> pa2;

identity 0x2000 with code;

*pa1 = 1;
*pa2 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbP}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbP}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbO}}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbA}
\begin{minipage}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(ipa1)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL2+dsb-tlbiipais-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|true|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.RT.EL2+dsb-tlbiipais-dsb-tlbiis-dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbH}
\setlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1IS,X4
DSB SY
TLBI VMALLE1IS
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbJ}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbJ}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbI}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
isb
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbL}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbL}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbK}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbL}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#1
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbN}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbN}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbM}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbN}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
physical pa1 pa2;
intermediate ipa1 ipa2;

x |-> ipa1;
ipa1 |-> pa1;
ipa1 ?-> invalid;

y |-> ipa2;
ipa2 |-> pa2;

identity 0x2000 with code;

*pa1 = 0;
*pa2 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbP}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbP}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbO}}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbA}
\begin{minipage}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(ipa1)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL2+dsb-tlbiipais-dsb-tlbiis-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.RT.EL2+dsb-tlbiis-dsb-tlbiipais-dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbH}
\setlength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VMALLE1IS
DSB SY
TLBI IPAS2E1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbJ}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbJ}{\usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbI}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
isb
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbL}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbL}{\usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbK}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbL}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#1
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbN}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbN}{\usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbM}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbN}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
physical pa1 pa2;
intermediate ipa1 ipa2;

x |-> ipa1;
ipa1 |-> pa1;
ipa1 ?-> invalid;

y |-> ipa2;
ipa2 |-> pa2;

identity 0x2000 with code;

*pa1 = 0;
*pa2 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbP}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbP}{\usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbO}}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbA}
\begin{minipage}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(ipa1)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL2+dsb-tlbiis-dsb-tlbiipais-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.RT.inv+dmb+addr-po-isb.tex <==
\newlength{\MPdotRTdotinvplusdmbplusaddrpoisbH}
\setlength{\MPdotRTdotinvplusdmbplusaddrpoisbH}{0cm}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpoisbI}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpoisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpoisbJ}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpoisbJ}{\usebox{\MPdotRTdotinvplusdmbplusaddrpoisbI}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpoisbH}{\MPdotRTdotinvplusdmbplusaddrpoisbJ}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpoisbK}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpoisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
EOR X6,X2,X2
LDR X7,[X8,X6]
ISB
LDR X4,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpoisbL}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpoisbL}{\usebox{\MPdotRTdotinvplusdmbplusaddrpoisbK}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpoisbH}{\MPdotRTdotinvplusdmbplusaddrpoisbL}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpoisbM}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpoisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpoisbN}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpoisbN}{\usebox{\MPdotRTdotinvplusdmbplusaddrpoisbM}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpoisbH}{\MPdotRTdotinvplusdmbplusaddrpoisbN}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpoisbO}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpoisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X4,#0
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpoisbP}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpoisbP}{\usebox{\MPdotRTdotinvplusdmbplusaddrpoisbO}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpoisbH}{\MPdotRTdotinvplusdmbplusaddrpoisbP}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpoisbA}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpoisbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;

    x |-> invalid;
    x ?-> pa1;

    y |-> pa2;

    z |-> pa3;

    *pa1 = 1;
    *pa2 = 0;
    *pa3 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpoisbB}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpoisbB}{\usebox{\MPdotRTdotinvplusdmbplusaddrpoisbA}}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpoisbC}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpoisbC}
\begin{minipage}{\MPdotRTdotinvplusdmbplusaddrpoisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R8=z|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.inv+dmb+addr-po-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotinvplusdmbplusaddrpoisbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotinvplusdmbplusaddrpoisbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotinvplusdmbplusaddrpoisbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpoisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpoisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpoisbM}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpoisbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R2=1 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.RT.inv+dmb+addr-po-msr-isb.tex <==
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrisbH}
\setlength{\MPdotRTdotinvplusdmbplusaddrpomsrisbH}{0cm}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbI}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrisbJ}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrisbJ}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbI}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpomsrisbH}{\MPdotRTdotinvplusdmbplusaddrpomsrisbJ}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbK}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
EOR X6,X2,X2
LDR X7,[X8,X6]
MSR ELR_EL1,X5
ISB
LDR X4,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrisbL}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrisbL}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbK}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpomsrisbH}{\MPdotRTdotinvplusdmbplusaddrpomsrisbL}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbM}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrisbN}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrisbN}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbM}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpomsrisbH}{\MPdotRTdotinvplusdmbplusaddrpomsrisbN}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbO}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X4,#0
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrisbP}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrisbP}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbO}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpomsrisbH}{\MPdotRTdotinvplusdmbplusaddrpomsrisbP}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbA}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrisbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;

    x |-> invalid;
    x ?-> pa1;

    y |-> pa2;

    z |-> pa3;

    *pa1 = 1;
    *pa2 = 0;
    *pa3 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrisbB}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrisbB}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbA}}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbC}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrisbC}
\begin{minipage}{\MPdotRTdotinvplusdmbplusaddrpomsrisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:R8=z|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.inv+dmb+addr-po-msr-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotinvplusdmbplusaddrpomsrisbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbM}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R2=1 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.RT.inv+dmb+addr-po-msr.tex <==
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrH}
\setlength{\MPdotRTdotinvplusdmbplusaddrpomsrH}{0cm}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrI}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrJ}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrJ}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrI}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpomsrH}{\MPdotRTdotinvplusdmbplusaddrpomsrJ}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrK}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
EOR X6,X2,X2
LDR X7,[X8,X6]
MSR ELR_EL1,X5
LDR X4,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrL}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrL}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrK}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpomsrH}{\MPdotRTdotinvplusdmbplusaddrpomsrL}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrM}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrN}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrN}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrM}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpomsrH}{\MPdotRTdotinvplusdmbplusaddrpomsrN}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrO}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X4,#0
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrP}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrP}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrO}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpomsrH}{\MPdotRTdotinvplusdmbplusaddrpomsrP}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrA}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;

    x |-> invalid;
    x ?-> pa1;

    y |-> pa2;

    z |-> pa3;

    *pa1 = 1;
    *pa2 = 0;
    *pa3 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrB}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrB}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrA}}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrC}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrC}
\begin{minipage}{\MPdotRTdotinvplusdmbplusaddrpomsrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:R8=z|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.inv+dmb+addr-po-msr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotinvplusdmbplusaddrpomsrB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpomsrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpomsrK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpomsrM}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpomsrO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R2=1 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.RT.inv+dmb+ctrl-trfi.tex <==
\newlength{\MPdotRTdotinvplusdmbplusctrltrfiH}
\setlength{\MPdotRTdotinvplusdmbplusctrltrfiH}{0cm}
\newsavebox{\MPdotRTdotinvplusdmbplusctrltrfiI}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusctrltrfiI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusctrltrfiJ}
\settowidth{\MPdotRTdotinvplusdmbplusctrltrfiJ}{\usebox{\MPdotRTdotinvplusdmbplusctrltrfiI}}
\addtolength{\MPdotRTdotinvplusdmbplusctrltrfiH}{\MPdotRTdotinvplusdmbplusctrltrfiJ}
\newsavebox{\MPdotRTdotinvplusdmbplusctrltrfiK}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusctrltrfiK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBZ X0,LC00
LC00:
STR X2,[X3]
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusctrltrfiL}
\settowidth{\MPdotRTdotinvplusdmbplusctrltrfiL}{\usebox{\MPdotRTdotinvplusdmbplusctrltrfiK}}
\addtolength{\MPdotRTdotinvplusdmbplusctrltrfiH}{\MPdotRTdotinvplusdmbplusctrltrfiL}
\newsavebox{\MPdotRTdotinvplusdmbplusctrltrfiM}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusctrltrfiM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#2
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusctrltrfiN}
\settowidth{\MPdotRTdotinvplusdmbplusctrltrfiN}{\usebox{\MPdotRTdotinvplusdmbplusctrltrfiM}}
\addtolength{\MPdotRTdotinvplusdmbplusctrltrfiH}{\MPdotRTdotinvplusdmbplusctrltrfiN}
\newsavebox{\MPdotRTdotinvplusdmbplusctrltrfiO}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusctrltrfiO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    w |-> invalid;
    w ?-> pa1;
    x |-> pa1;
    *pa1 = 0;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusctrltrfiP}
\settowidth{\MPdotRTdotinvplusdmbplusctrltrfiP}{\usebox{\MPdotRTdotinvplusdmbplusctrltrfiO}}
\newsavebox{\MPdotRTdotinvplusdmbplusctrltrfiA}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusctrltrfiA}
\begin{minipage}{\MPdotRTdotinvplusdmbplusctrltrfiH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(w,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R5=w|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.inv+dmb+ctrl-trfi|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotinvplusdmbplusctrltrfiP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotinvplusdmbplusctrltrfiO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotinvplusdmbplusctrltrfiA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusctrltrfiI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusctrltrfiK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusctrltrfiM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.RT.inv+trfi-data+addr.toml.tex <==
\newlength{\MPdotRTdotinvplustrfidataplusaddrdottomlH}
\setlength{\MPdotRTdotinvplustrfidataplusaddrdottomlH}{0cm}
\newsavebox{\MPdotRTdotinvplustrfidataplusaddrdottomlI}
\begin{lrbox}{\MPdotRTdotinvplustrfidataplusaddrdottomlI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
STR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplustrfidataplusaddrdottomlJ}
\settowidth{\MPdotRTdotinvplustrfidataplusaddrdottomlJ}{\usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlI}}
\addtolength{\MPdotRTdotinvplustrfidataplusaddrdottomlH}{\MPdotRTdotinvplustrfidataplusaddrdottomlJ}
\newsavebox{\MPdotRTdotinvplustrfidataplusaddrdottomlK}
\begin{lrbox}{\MPdotRTdotinvplustrfidataplusaddrdottomlK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
LDR X3,[X4,X2]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplustrfidataplusaddrdottomlL}
\settowidth{\MPdotRTdotinvplustrfidataplusaddrdottomlL}{\usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlK}}
\addtolength{\MPdotRTdotinvplustrfidataplusaddrdottomlH}{\MPdotRTdotinvplustrfidataplusaddrdottomlL}
\newsavebox{\MPdotRTdotinvplustrfidataplusaddrdottomlM}
\begin{lrbox}{\MPdotRTdotinvplustrfidataplusaddrdottomlM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplustrfidataplusaddrdottomlN}
\settowidth{\MPdotRTdotinvplustrfidataplusaddrdottomlN}{\usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlM}}
\addtolength{\MPdotRTdotinvplustrfidataplusaddrdottomlH}{\MPdotRTdotinvplustrfidataplusaddrdottomlN}
\newsavebox{\MPdotRTdotinvplustrfidataplusaddrdottomlO}
\begin{lrbox}{\MPdotRTdotinvplustrfidataplusaddrdottomlO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X3,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplustrfidataplusaddrdottomlP}
\settowidth{\MPdotRTdotinvplustrfidataplusaddrdottomlP}{\usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlO}}
\addtolength{\MPdotRTdotinvplustrfidataplusaddrdottomlH}{\MPdotRTdotinvplustrfidataplusaddrdottomlP}
\newsavebox{\MPdotRTdotinvplustrfidataplusaddrdottomlA}
\begin{lrbox}{\MPdotRTdotinvplustrfidataplusaddrdottomlA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    w |-> invalid;
    w ?-> pa1;
    x |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplustrfidataplusaddrdottomlB}
\settowidth{\MPdotRTdotinvplustrfidataplusaddrdottomlB}{\usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlA}}
\newsavebox{\MPdotRTdotinvplustrfidataplusaddrdottomlC}
\begin{lrbox}{\MPdotRTdotinvplustrfidataplusaddrdottomlC}
\begin{minipage}{\MPdotRTdotinvplustrfidataplusaddrdottomlH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(w,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R3=w|\\
\lstinline[language=IslaLitmusExp]|0:R4=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R5=y|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(w,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R4=w|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.inv+trfi-data+addr.toml|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotinvplustrfidataplusaddrdottomlB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=1 & 1:R0=1 & 1:R3=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.RTT.EL1+dsb-tlbiis-tlbiis-dsb+dsb-isb.tex <==
\newlength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbH}
\setlength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
STR X2,[X3]
DSB SY
TLBI VAE1IS,X4
TLBI VAE1IS,X5
DSB SY
STR X6,[X7]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbJ}
\settowidth{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbJ}{\usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbI}}
\addtolength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbH}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbJ}
\newsavebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X4,[X3]
MOV X2,X4
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbL}
\settowidth{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbL}{\usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbK}}
\addtolength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbH}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbL}
\newsavebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbN}
\settowidth{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbN}{\usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbM}}
\addtolength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbH}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbN}
\newsavebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> pa1;
    x ?-> invalid;

    y |-> pa2;

    z |-> pa3;
    z ?-> invalid;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbP}
\settowidth{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbP}{\usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbO}}
\newsavebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbA}
\begin{minipage}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|0:R5=page(z)|\\
\lstinline[language=IslaLitmusExp]|0:R6=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R7=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=z|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTT.EL1+dsb-tlbiis-tlbiis-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.RTf.inv+dmb+addr.tex <==
\newlength{\MPdotRTfdotinvplusdmbplusaddrH}
\setlength{\MPdotRTfdotinvplusdmbplusaddrH}{0cm}
\newsavebox{\MPdotRTfdotinvplusdmbplusaddrI}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusaddrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB ST
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusaddrJ}
\settowidth{\MPdotRTfdotinvplusdmbplusaddrJ}{\usebox{\MPdotRTfdotinvplusdmbplusaddrI}}
\addtolength{\MPdotRTfdotinvplusdmbplusaddrH}{\MPdotRTfdotinvplusdmbplusaddrJ}
\newsavebox{\MPdotRTfdotinvplusdmbplusaddrK}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusaddrK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusaddrL}
\settowidth{\MPdotRTfdotinvplusdmbplusaddrL}{\usebox{\MPdotRTfdotinvplusdmbplusaddrK}}
\addtolength{\MPdotRTfdotinvplusdmbplusaddrH}{\MPdotRTfdotinvplusdmbplusaddrL}
\newsavebox{\MPdotRTfdotinvplusdmbplusaddrM}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusaddrM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusaddrN}
\settowidth{\MPdotRTfdotinvplusdmbplusaddrN}{\usebox{\MPdotRTfdotinvplusdmbplusaddrM}}
\addtolength{\MPdotRTfdotinvplusdmbplusaddrH}{\MPdotRTfdotinvplusdmbplusaddrN}
\newsavebox{\MPdotRTfdotinvplusdmbplusaddrO}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusaddrO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusaddrP}
\settowidth{\MPdotRTfdotinvplusdmbplusaddrP}{\usebox{\MPdotRTfdotinvplusdmbplusaddrO}}
\newsavebox{\MPdotRTfdotinvplusdmbplusaddrA}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusaddrA}
\begin{minipage}{\MPdotRTfdotinvplusdmbplusaddrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv+dmb+addr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvplusdmbplusaddrP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvplusdmbplusaddrO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvplusdmbplusaddrA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusaddrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusaddrK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusaddrM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.RTf.inv+dmb+ctrl-isb.tex <==
\newlength{\MPdotRTfdotinvplusdmbplusctrlisbH}
\setlength{\MPdotRTfdotinvplusdmbplusctrlisbH}{0cm}
\newsavebox{\MPdotRTfdotinvplusdmbplusctrlisbI}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusctrlisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusctrlisbJ}
\settowidth{\MPdotRTfdotinvplusdmbplusctrlisbJ}{\usebox{\MPdotRTfdotinvplusdmbplusctrlisbI}}
\addtolength{\MPdotRTfdotinvplusdmbplusctrlisbH}{\MPdotRTfdotinvplusdmbplusctrlisbJ}
\newsavebox{\MPdotRTfdotinvplusdmbplusctrlisbK}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusctrlisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBNZ X0,L0
L0:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusctrlisbL}
\settowidth{\MPdotRTfdotinvplusdmbplusctrlisbL}{\usebox{\MPdotRTfdotinvplusdmbplusctrlisbK}}
\addtolength{\MPdotRTfdotinvplusdmbplusctrlisbH}{\MPdotRTfdotinvplusdmbplusctrlisbL}
\newsavebox{\MPdotRTfdotinvplusdmbplusctrlisbM}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusctrlisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusctrlisbN}
\settowidth{\MPdotRTfdotinvplusdmbplusctrlisbN}{\usebox{\MPdotRTfdotinvplusdmbplusctrlisbM}}
\addtolength{\MPdotRTfdotinvplusdmbplusctrlisbH}{\MPdotRTfdotinvplusdmbplusctrlisbN}
\newsavebox{\MPdotRTfdotinvplusdmbplusctrlisbO}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusctrlisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusctrlisbP}
\settowidth{\MPdotRTfdotinvplusdmbplusctrlisbP}{\usebox{\MPdotRTfdotinvplusdmbplusctrlisbO}}
\newsavebox{\MPdotRTfdotinvplusdmbplusctrlisbA}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusctrlisbA}
\begin{minipage}{\MPdotRTfdotinvplusdmbplusctrlisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv+dmb+ctrl-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvplusdmbplusctrlisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvplusdmbplusctrlisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvplusdmbplusctrlisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusctrlisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusctrlisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusctrlisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.RTf.inv+dmb+data.tex <==
\newlength{\MPdotRTfdotinvplusdmbplusdataH}
\setlength{\MPdotRTfdotinvplusdmbplusdataH}{0cm}
\newsavebox{\MPdotRTfdotinvplusdmbplusdataI}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdataI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB ST
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusdataJ}
\settowidth{\MPdotRTfdotinvplusdmbplusdataJ}{\usebox{\MPdotRTfdotinvplusdmbplusdataI}}
\addtolength{\MPdotRTfdotinvplusdmbplusdataH}{\MPdotRTfdotinvplusdmbplusdataJ}
\newsavebox{\MPdotRTfdotinvplusdmbplusdataK}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdataK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
ORR X6,X4,X5
STR X6,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusdataL}
\settowidth{\MPdotRTfdotinvplusdmbplusdataL}{\usebox{\MPdotRTfdotinvplusdmbplusdataK}}
\addtolength{\MPdotRTfdotinvplusdmbplusdataH}{\MPdotRTfdotinvplusdmbplusdataL}
\newsavebox{\MPdotRTfdotinvplusdmbplusdataM}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdataM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusdataN}
\settowidth{\MPdotRTfdotinvplusdmbplusdataN}{\usebox{\MPdotRTfdotinvplusdmbplusdataM}}
\addtolength{\MPdotRTfdotinvplusdmbplusdataH}{\MPdotRTfdotinvplusdmbplusdataN}
\newsavebox{\MPdotRTfdotinvplusdmbplusdataO}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdataO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusdataP}
\settowidth{\MPdotRTfdotinvplusdmbplusdataP}{\usebox{\MPdotRTfdotinvplusdmbplusdataO}}
\newsavebox{\MPdotRTfdotinvplusdmbplusdataA}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdataA}
\begin{minipage}{\MPdotRTfdotinvplusdmbplusdataH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=0b1|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv+dmb+data|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvplusdmbplusdataP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvplusdmbplusdataO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvplusdmbplusdataA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusdataI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusdataK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusdataM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.RTf.inv+dmb+dsb-isb.tex <==
\newlength{\MPdotRTfdotinvplusdmbplusdsbisbH}
\setlength{\MPdotRTfdotinvplusdmbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTfdotinvplusdmbplusdsbisbI}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusdsbisbJ}
\settowidth{\MPdotRTfdotinvplusdmbplusdsbisbJ}{\usebox{\MPdotRTfdotinvplusdmbplusdsbisbI}}
\addtolength{\MPdotRTfdotinvplusdmbplusdsbisbH}{\MPdotRTfdotinvplusdmbplusdsbisbJ}
\newsavebox{\MPdotRTfdotinvplusdmbplusdsbisbK}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusdsbisbL}
\settowidth{\MPdotRTfdotinvplusdmbplusdsbisbL}{\usebox{\MPdotRTfdotinvplusdmbplusdsbisbK}}
\addtolength{\MPdotRTfdotinvplusdmbplusdsbisbH}{\MPdotRTfdotinvplusdmbplusdsbisbL}
\newsavebox{\MPdotRTfdotinvplusdmbplusdsbisbM}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusdsbisbN}
\settowidth{\MPdotRTfdotinvplusdmbplusdsbisbN}{\usebox{\MPdotRTfdotinvplusdmbplusdsbisbM}}
\addtolength{\MPdotRTfdotinvplusdmbplusdsbisbH}{\MPdotRTfdotinvplusdmbplusdsbisbN}
\newsavebox{\MPdotRTfdotinvplusdmbplusdsbisbO}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusdsbisbP}
\settowidth{\MPdotRTfdotinvplusdmbplusdsbisbP}{\usebox{\MPdotRTfdotinvplusdmbplusdsbisbO}}
\newsavebox{\MPdotRTfdotinvplusdmbplusdsbisbA}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdsbisbA}
\begin{minipage}{\MPdotRTfdotinvplusdmbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv+dmb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvplusdmbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvplusdmbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvplusdmbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.RTf.inv+dmb+po.tex <==
\newlength{\MPdotRTfdotinvplusdmbpluspoH}
\setlength{\MPdotRTfdotinvplusdmbpluspoH}{0cm}
\newsavebox{\MPdotRTfdotinvplusdmbpluspoI}
\begin{lrbox}{\MPdotRTfdotinvplusdmbpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB ST
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbpluspoJ}
\settowidth{\MPdotRTfdotinvplusdmbpluspoJ}{\usebox{\MPdotRTfdotinvplusdmbpluspoI}}
\addtolength{\MPdotRTfdotinvplusdmbpluspoH}{\MPdotRTfdotinvplusdmbpluspoJ}
\newsavebox{\MPdotRTfdotinvplusdmbpluspoK}
\begin{lrbox}{\MPdotRTfdotinvplusdmbpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbpluspoL}
\settowidth{\MPdotRTfdotinvplusdmbpluspoL}{\usebox{\MPdotRTfdotinvplusdmbpluspoK}}
\addtolength{\MPdotRTfdotinvplusdmbpluspoH}{\MPdotRTfdotinvplusdmbpluspoL}
\newsavebox{\MPdotRTfdotinvplusdmbpluspoM}
\begin{lrbox}{\MPdotRTfdotinvplusdmbpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbpluspoN}
\settowidth{\MPdotRTfdotinvplusdmbpluspoN}{\usebox{\MPdotRTfdotinvplusdmbpluspoM}}
\addtolength{\MPdotRTfdotinvplusdmbpluspoH}{\MPdotRTfdotinvplusdmbpluspoN}
\newsavebox{\MPdotRTfdotinvplusdmbpluspoO}
\begin{lrbox}{\MPdotRTfdotinvplusdmbpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbpluspoP}
\settowidth{\MPdotRTfdotinvplusdmbpluspoP}{\usebox{\MPdotRTfdotinvplusdmbpluspoO}}
\newsavebox{\MPdotRTfdotinvplusdmbpluspoA}
\begin{lrbox}{\MPdotRTfdotinvplusdmbpluspoA}
\begin{minipage}{\MPdotRTfdotinvplusdmbpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv+dmb+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvplusdmbpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvplusdmbpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvplusdmbpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.RTf.inv+dmbs.tex <==
\newlength{\MPdotRTfdotinvplusdmbsH}
\setlength{\MPdotRTfdotinvplusdmbsH}{0cm}
\newsavebox{\MPdotRTfdotinvplusdmbsI}
\begin{lrbox}{\MPdotRTfdotinvplusdmbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB ST
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbsJ}
\settowidth{\MPdotRTfdotinvplusdmbsJ}{\usebox{\MPdotRTfdotinvplusdmbsI}}
\addtolength{\MPdotRTfdotinvplusdmbsH}{\MPdotRTfdotinvplusdmbsJ}
\newsavebox{\MPdotRTfdotinvplusdmbsK}
\begin{lrbox}{\MPdotRTfdotinvplusdmbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbsL}
\settowidth{\MPdotRTfdotinvplusdmbsL}{\usebox{\MPdotRTfdotinvplusdmbsK}}
\addtolength{\MPdotRTfdotinvplusdmbsH}{\MPdotRTfdotinvplusdmbsL}
\newsavebox{\MPdotRTfdotinvplusdmbsM}
\begin{lrbox}{\MPdotRTfdotinvplusdmbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbsN}
\settowidth{\MPdotRTfdotinvplusdmbsN}{\usebox{\MPdotRTfdotinvplusdmbsM}}
\addtolength{\MPdotRTfdotinvplusdmbsH}{\MPdotRTfdotinvplusdmbsN}
\newsavebox{\MPdotRTfdotinvplusdmbsO}
\begin{lrbox}{\MPdotRTfdotinvplusdmbsO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbsP}
\settowidth{\MPdotRTfdotinvplusdmbsP}{\usebox{\MPdotRTfdotinvplusdmbsO}}
\newsavebox{\MPdotRTfdotinvplusdmbsA}
\begin{lrbox}{\MPdotRTfdotinvplusdmbsA}
\begin{minipage}{\MPdotRTfdotinvplusdmbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv+dmbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvplusdmbsP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvplusdmbsO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvplusdmbsA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbsK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbsM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.RTf.inv.EL1+dsb-tlbiis-dsb+addr.tex <==
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrH}
\setlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrH}{0cm}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrI}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrJ}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrJ}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrI}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrJ}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrK}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrL}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrL}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrK}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrL}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrM}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrN}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrN}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrM}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrN}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrO}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrP}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrP}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrO}}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrA}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrA}
\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv.EL1+dsb-tlbiis-dsb+addr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.RTf.inv.EL1+dsb-tlbiis-dsb+ctrl-isb.tex <==
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbH}
\setlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbH}{0cm}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbI}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbJ}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbJ}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbI}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbJ}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbK}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBNZ X0,L0
L0:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbL}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbL}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbK}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbL}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbM}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbN}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbN}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbM}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbN}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbO}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbP}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbP}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbO}}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbA}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbA}
\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv.EL1+dsb-tlbiis-dsb+ctrl-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.RTf.inv.EL1+dsb-tlbiis-dsb+ctrl.tex <==
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}
\setlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}{0cm}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlI}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlJ}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlJ}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlI}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlJ}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlK}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBNZ X0,L0
L0:
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlL}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlL}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlK}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlL}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlM}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlN}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlN}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlM}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlN}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlO}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlP}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlP}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlO}}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlA}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlA}
\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv.EL1+dsb-tlbiis-dsb+ctrl|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.RTf.inv.EL1+dsb-tlbiis-dsb+data.tex <==
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}
\setlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}{0cm}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataI}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataJ}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataJ}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataI}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataJ}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataK}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
STR X4,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataL}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataL}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataK}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataL}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataM}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataN}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataN}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataM}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataN}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataO}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataP}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataP}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataO}}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataA}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataA}
\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv.EL1+dsb-tlbiis-dsb+data|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.RTf.inv.EL1+dsb-tlbiis-dsb+dmb.tex <==
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}
\setlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{0cm}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}
\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv.EL1+dsb-tlbiis-dsb+dmb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.RTf.inv.EL1+dsb-tlbiis-dsb+dsb-isb.tex <==
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}
\setlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbJ}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbJ}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbI}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbJ}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbL}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbL}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbK}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbL}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbN}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbN}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbM}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbN}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbP}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbP}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbO}}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbA}
\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv.EL1+dsb-tlbiis-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.RTf.inv.EL1+dsb-tlbiis-dsb+po.tex <==
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}
\setlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}{0cm}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoI}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoJ}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoJ}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoI}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoJ}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoK}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoL}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoL}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoK}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoL}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoM}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoN}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoN}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoM}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoN}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoO}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoP}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoP}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoO}}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoA}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoA}
\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv.EL1+dsb-tlbiis-dsb+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.RTf.inv.EL1+dsb-tlbiis-dsb+poap.tex <==
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}
\setlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}{0cm}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapI}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapJ}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapJ}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapI}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapJ}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapK}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDAR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapL}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapL}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapK}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapL}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapM}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapN}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapN}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapM}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapN}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapO}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapP}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapP}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapO}}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapA}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapA}
\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv.EL1+dsb-tlbiis-dsb+poap|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.TR.inv+dmb+isb.tex <==
\newlength{\MPdotTRdotinvplusdmbplusisbH}
\setlength{\MPdotTRdotinvplusdmbplusisbH}{0cm}
\newsavebox{\MPdotTRdotinvplusdmbplusisbI}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusisbJ}
\settowidth{\MPdotTRdotinvplusdmbplusisbJ}{\usebox{\MPdotTRdotinvplusdmbplusisbI}}
\addtolength{\MPdotTRdotinvplusdmbplusisbH}{\MPdotTRdotinvplusdmbplusisbJ}
\newsavebox{\MPdotTRdotinvplusdmbplusisbK}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
ISB
LDR X4,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusisbL}
\settowidth{\MPdotTRdotinvplusdmbplusisbL}{\usebox{\MPdotTRdotinvplusdmbplusisbK}}
\addtolength{\MPdotTRdotinvplusdmbplusisbH}{\MPdotTRdotinvplusdmbplusisbL}
\newsavebox{\MPdotTRdotinvplusdmbplusisbM}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusisbN}
\settowidth{\MPdotTRdotinvplusdmbplusisbN}{\usebox{\MPdotTRdotinvplusdmbplusisbM}}
\addtolength{\MPdotTRdotinvplusdmbplusisbH}{\MPdotTRdotinvplusdmbplusisbN}
\newsavebox{\MPdotTRdotinvplusdmbplusisbO}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusisbP}
\settowidth{\MPdotTRdotinvplusdmbplusisbP}{\usebox{\MPdotTRdotinvplusdmbplusisbO}}
\addtolength{\MPdotTRdotinvplusdmbplusisbH}{\MPdotTRdotinvplusdmbplusisbP}
\newsavebox{\MPdotTRdotinvplusdmbplusisbA}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusisbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 0;
    *pa2 = 1;
    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusisbB}
\settowidth{\MPdotTRdotinvplusdmbplusisbB}{\usebox{\MPdotTRdotinvplusdmbplusisbA}}
\newsavebox{\MPdotTRdotinvplusdmbplusisbC}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusisbC}
\begin{minipage}{\MPdotTRdotinvplusdmbplusisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TR.inv+dmb+isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTRdotinvplusdmbplusisbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTRdotinvplusdmbplusisbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTRdotinvplusdmbplusisbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusisbM}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusisbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R2=1 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.TR.inv+dmb+msr-isb.tex <==
\newlength{\MPdotTRdotinvplusdmbplusmsrisbH}
\setlength{\MPdotTRdotinvplusdmbplusmsrisbH}{0cm}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrisbI}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrisbJ}
\settowidth{\MPdotTRdotinvplusdmbplusmsrisbJ}{\usebox{\MPdotTRdotinvplusdmbplusmsrisbI}}
\addtolength{\MPdotTRdotinvplusdmbplusmsrisbH}{\MPdotTRdotinvplusdmbplusmsrisbJ}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrisbK}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MSR ELR_EL1,X5
ISB
LDR X4,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrisbL}
\settowidth{\MPdotTRdotinvplusdmbplusmsrisbL}{\usebox{\MPdotTRdotinvplusdmbplusmsrisbK}}
\addtolength{\MPdotTRdotinvplusdmbplusmsrisbH}{\MPdotTRdotinvplusdmbplusmsrisbL}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrisbM}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrisbN}
\settowidth{\MPdotTRdotinvplusdmbplusmsrisbN}{\usebox{\MPdotTRdotinvplusdmbplusmsrisbM}}
\addtolength{\MPdotTRdotinvplusdmbplusmsrisbH}{\MPdotTRdotinvplusdmbplusmsrisbN}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrisbO}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrisbP}
\settowidth{\MPdotTRdotinvplusdmbplusmsrisbP}{\usebox{\MPdotTRdotinvplusdmbplusmsrisbO}}
\addtolength{\MPdotTRdotinvplusdmbplusmsrisbH}{\MPdotTRdotinvplusdmbplusmsrisbP}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrisbA}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrisbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 0;
    *pa2 = 1;
    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrisbB}
\settowidth{\MPdotTRdotinvplusdmbplusmsrisbB}{\usebox{\MPdotTRdotinvplusdmbplusmsrisbA}}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrisbC}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrisbC}
\begin{minipage}{\MPdotTRdotinvplusdmbplusmsrisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TR.inv+dmb+msr-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTRdotinvplusdmbplusmsrisbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTRdotinvplusdmbplusmsrisbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTRdotinvplusdmbplusmsrisbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusmsrisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusmsrisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusmsrisbM}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusmsrisbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R2=1 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.TR.inv+dmb+msr.tex <==
\newlength{\MPdotTRdotinvplusdmbplusmsrH}
\setlength{\MPdotTRdotinvplusdmbplusmsrH}{0cm}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrI}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrJ}
\settowidth{\MPdotTRdotinvplusdmbplusmsrJ}{\usebox{\MPdotTRdotinvplusdmbplusmsrI}}
\addtolength{\MPdotTRdotinvplusdmbplusmsrH}{\MPdotTRdotinvplusdmbplusmsrJ}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrK}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MSR ELR_EL1,X5
LDR X4,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrL}
\settowidth{\MPdotTRdotinvplusdmbplusmsrL}{\usebox{\MPdotTRdotinvplusdmbplusmsrK}}
\addtolength{\MPdotTRdotinvplusdmbplusmsrH}{\MPdotTRdotinvplusdmbplusmsrL}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrM}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrN}
\settowidth{\MPdotTRdotinvplusdmbplusmsrN}{\usebox{\MPdotTRdotinvplusdmbplusmsrM}}
\addtolength{\MPdotTRdotinvplusdmbplusmsrH}{\MPdotTRdotinvplusdmbplusmsrN}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrO}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrP}
\settowidth{\MPdotTRdotinvplusdmbplusmsrP}{\usebox{\MPdotTRdotinvplusdmbplusmsrO}}
\addtolength{\MPdotTRdotinvplusdmbplusmsrH}{\MPdotTRdotinvplusdmbplusmsrP}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrA}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 0;
    *pa2 = 1;
    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrB}
\settowidth{\MPdotTRdotinvplusdmbplusmsrB}{\usebox{\MPdotTRdotinvplusdmbplusmsrA}}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrC}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrC}
\begin{minipage}{\MPdotTRdotinvplusdmbplusmsrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TR.inv+dmb+msr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTRdotinvplusdmbplusmsrB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTRdotinvplusdmbplusmsrA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTRdotinvplusdmbplusmsrC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusmsrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusmsrK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusmsrM}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusmsrO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R2=1 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.TTf.inv+dmb+addr.tex <==
\newlength{\MPdotTTfdotinvplusdmbplusaddrH}
\setlength{\MPdotTTfdotinvplusdmbplusaddrH}{0cm}
\newsavebox{\MPdotTTfdotinvplusdmbplusaddrI}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusaddrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbplusaddrJ}
\settowidth{\MPdotTTfdotinvplusdmbplusaddrJ}{\usebox{\MPdotTTfdotinvplusdmbplusaddrI}}
\addtolength{\MPdotTTfdotinvplusdmbplusaddrH}{\MPdotTTfdotinvplusdmbplusaddrJ}
\newsavebox{\MPdotTTfdotinvplusdmbplusaddrK}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusaddrK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
EOR X4,X0,X0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbplusaddrL}
\settowidth{\MPdotTTfdotinvplusdmbplusaddrL}{\usebox{\MPdotTTfdotinvplusdmbplusaddrK}}
\addtolength{\MPdotTTfdotinvplusdmbplusaddrH}{\MPdotTTfdotinvplusdmbplusaddrL}
\newsavebox{\MPdotTTfdotinvplusdmbplusaddrM}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusaddrM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbplusaddrN}
\settowidth{\MPdotTTfdotinvplusdmbplusaddrN}{\usebox{\MPdotTTfdotinvplusdmbplusaddrM}}
\addtolength{\MPdotTTfdotinvplusdmbplusaddrH}{\MPdotTTfdotinvplusdmbplusaddrN}
\newsavebox{\MPdotTTfdotinvplusdmbplusaddrO}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusaddrO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbplusaddrP}
\settowidth{\MPdotTTfdotinvplusdmbplusaddrP}{\usebox{\MPdotTTfdotinvplusdmbplusaddrO}}
\newsavebox{\MPdotTTfdotinvplusdmbplusaddrA}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusaddrA}
\begin{minipage}{\MPdotTTfdotinvplusdmbplusaddrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv+dmb+addr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvplusdmbplusaddrP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvplusdmbplusaddrO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvplusdmbplusaddrA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbplusaddrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbplusaddrK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbplusaddrM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.TTf.inv+dmb+dsb-isb.tex <==
\newlength{\MPdotTTfdotinvplusdmbplusdsbisbH}
\setlength{\MPdotTTfdotinvplusdmbplusdsbisbH}{0cm}
\newsavebox{\MPdotTTfdotinvplusdmbplusdsbisbI}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbplusdsbisbJ}
\settowidth{\MPdotTTfdotinvplusdmbplusdsbisbJ}{\usebox{\MPdotTTfdotinvplusdmbplusdsbisbI}}
\addtolength{\MPdotTTfdotinvplusdmbplusdsbisbH}{\MPdotTTfdotinvplusdmbplusdsbisbJ}
\newsavebox{\MPdotTTfdotinvplusdmbplusdsbisbK}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbplusdsbisbL}
\settowidth{\MPdotTTfdotinvplusdmbplusdsbisbL}{\usebox{\MPdotTTfdotinvplusdmbplusdsbisbK}}
\addtolength{\MPdotTTfdotinvplusdmbplusdsbisbH}{\MPdotTTfdotinvplusdmbplusdsbisbL}
\newsavebox{\MPdotTTfdotinvplusdmbplusdsbisbM}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbplusdsbisbN}
\settowidth{\MPdotTTfdotinvplusdmbplusdsbisbN}{\usebox{\MPdotTTfdotinvplusdmbplusdsbisbM}}
\addtolength{\MPdotTTfdotinvplusdmbplusdsbisbH}{\MPdotTTfdotinvplusdmbplusdsbisbN}
\newsavebox{\MPdotTTfdotinvplusdmbplusdsbisbO}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbplusdsbisbP}
\settowidth{\MPdotTTfdotinvplusdmbplusdsbisbP}{\usebox{\MPdotTTfdotinvplusdmbplusdsbisbO}}
\newsavebox{\MPdotTTfdotinvplusdmbplusdsbisbA}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusdsbisbA}
\begin{minipage}{\MPdotTTfdotinvplusdmbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv+dmb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvplusdmbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvplusdmbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvplusdmbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.TTf.inv+dmb+po.tex <==
\newlength{\MPdotTTfdotinvplusdmbpluspoH}
\setlength{\MPdotTTfdotinvplusdmbpluspoH}{0cm}
\newsavebox{\MPdotTTfdotinvplusdmbpluspoI}
\begin{lrbox}{\MPdotTTfdotinvplusdmbpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbpluspoJ}
\settowidth{\MPdotTTfdotinvplusdmbpluspoJ}{\usebox{\MPdotTTfdotinvplusdmbpluspoI}}
\addtolength{\MPdotTTfdotinvplusdmbpluspoH}{\MPdotTTfdotinvplusdmbpluspoJ}
\newsavebox{\MPdotTTfdotinvplusdmbpluspoK}
\begin{lrbox}{\MPdotTTfdotinvplusdmbpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbpluspoL}
\settowidth{\MPdotTTfdotinvplusdmbpluspoL}{\usebox{\MPdotTTfdotinvplusdmbpluspoK}}
\addtolength{\MPdotTTfdotinvplusdmbpluspoH}{\MPdotTTfdotinvplusdmbpluspoL}
\newsavebox{\MPdotTTfdotinvplusdmbpluspoM}
\begin{lrbox}{\MPdotTTfdotinvplusdmbpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbpluspoN}
\settowidth{\MPdotTTfdotinvplusdmbpluspoN}{\usebox{\MPdotTTfdotinvplusdmbpluspoM}}
\addtolength{\MPdotTTfdotinvplusdmbpluspoH}{\MPdotTTfdotinvplusdmbpluspoN}
\newsavebox{\MPdotTTfdotinvplusdmbpluspoO}
\begin{lrbox}{\MPdotTTfdotinvplusdmbpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbpluspoP}
\settowidth{\MPdotTTfdotinvplusdmbpluspoP}{\usebox{\MPdotTTfdotinvplusdmbpluspoO}}
\newsavebox{\MPdotTTfdotinvplusdmbpluspoA}
\begin{lrbox}{\MPdotTTfdotinvplusdmbpluspoA}
\begin{minipage}{\MPdotTTfdotinvplusdmbpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv+dmb+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvplusdmbpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvplusdmbpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvplusdmbpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.TTf.inv+dsb+ctrl-isb.tex <==
\newlength{\MPdotTTfdotinvplusdsbplusctrlisbH}
\setlength{\MPdotTTfdotinvplusdsbplusctrlisbH}{0cm}
\newsavebox{\MPdotTTfdotinvplusdsbplusctrlisbI}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusctrlisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbplusctrlisbJ}
\settowidth{\MPdotTTfdotinvplusdsbplusctrlisbJ}{\usebox{\MPdotTTfdotinvplusdsbplusctrlisbI}}
\addtolength{\MPdotTTfdotinvplusdsbplusctrlisbH}{\MPdotTTfdotinvplusdsbplusctrlisbJ}
\newsavebox{\MPdotTTfdotinvplusdsbplusctrlisbK}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusctrlisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
CBNZ X0,L0
L0:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbplusctrlisbL}
\settowidth{\MPdotTTfdotinvplusdsbplusctrlisbL}{\usebox{\MPdotTTfdotinvplusdsbplusctrlisbK}}
\addtolength{\MPdotTTfdotinvplusdsbplusctrlisbH}{\MPdotTTfdotinvplusdsbplusctrlisbL}
\newsavebox{\MPdotTTfdotinvplusdsbplusctrlisbM}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusctrlisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbplusctrlisbN}
\settowidth{\MPdotTTfdotinvplusdsbplusctrlisbN}{\usebox{\MPdotTTfdotinvplusdsbplusctrlisbM}}
\addtolength{\MPdotTTfdotinvplusdsbplusctrlisbH}{\MPdotTTfdotinvplusdsbplusctrlisbN}
\newsavebox{\MPdotTTfdotinvplusdsbplusctrlisbO}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusctrlisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbplusctrlisbP}
\settowidth{\MPdotTTfdotinvplusdsbplusctrlisbP}{\usebox{\MPdotTTfdotinvplusdsbplusctrlisbO}}
\newsavebox{\MPdotTTfdotinvplusdsbplusctrlisbA}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusctrlisbA}
\begin{minipage}{\MPdotTTfdotinvplusdsbplusctrlisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv+dsb+ctrl-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvplusdsbplusctrlisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvplusdsbplusctrlisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvplusdsbplusctrlisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbplusctrlisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbplusctrlisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbplusctrlisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.TTf.inv+dsb+dsb-isb.tex <==
\newlength{\MPdotTTfdotinvplusdsbplusdsbisbH}
\setlength{\MPdotTTfdotinvplusdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotTTfdotinvplusdsbplusdsbisbI}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbplusdsbisbJ}
\settowidth{\MPdotTTfdotinvplusdsbplusdsbisbJ}{\usebox{\MPdotTTfdotinvplusdsbplusdsbisbI}}
\addtolength{\MPdotTTfdotinvplusdsbplusdsbisbH}{\MPdotTTfdotinvplusdsbplusdsbisbJ}
\newsavebox{\MPdotTTfdotinvplusdsbplusdsbisbK}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbplusdsbisbL}
\settowidth{\MPdotTTfdotinvplusdsbplusdsbisbL}{\usebox{\MPdotTTfdotinvplusdsbplusdsbisbK}}
\addtolength{\MPdotTTfdotinvplusdsbplusdsbisbH}{\MPdotTTfdotinvplusdsbplusdsbisbL}
\newsavebox{\MPdotTTfdotinvplusdsbplusdsbisbM}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbplusdsbisbN}
\settowidth{\MPdotTTfdotinvplusdsbplusdsbisbN}{\usebox{\MPdotTTfdotinvplusdsbplusdsbisbM}}
\addtolength{\MPdotTTfdotinvplusdsbplusdsbisbH}{\MPdotTTfdotinvplusdsbplusdsbisbN}
\newsavebox{\MPdotTTfdotinvplusdsbplusdsbisbO}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbplusdsbisbP}
\settowidth{\MPdotTTfdotinvplusdsbplusdsbisbP}{\usebox{\MPdotTTfdotinvplusdsbplusdsbisbO}}
\newsavebox{\MPdotTTfdotinvplusdsbplusdsbisbA}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusdsbisbA}
\begin{minipage}{\MPdotTTfdotinvplusdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv+dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvplusdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvplusdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvplusdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.TTf.inv+dsb+po.tex <==
\newlength{\MPdotTTfdotinvplusdsbpluspoH}
\setlength{\MPdotTTfdotinvplusdsbpluspoH}{0cm}
\newsavebox{\MPdotTTfdotinvplusdsbpluspoI}
\begin{lrbox}{\MPdotTTfdotinvplusdsbpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbpluspoJ}
\settowidth{\MPdotTTfdotinvplusdsbpluspoJ}{\usebox{\MPdotTTfdotinvplusdsbpluspoI}}
\addtolength{\MPdotTTfdotinvplusdsbpluspoH}{\MPdotTTfdotinvplusdsbpluspoJ}
\newsavebox{\MPdotTTfdotinvplusdsbpluspoK}
\begin{lrbox}{\MPdotTTfdotinvplusdsbpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbpluspoL}
\settowidth{\MPdotTTfdotinvplusdsbpluspoL}{\usebox{\MPdotTTfdotinvplusdsbpluspoK}}
\addtolength{\MPdotTTfdotinvplusdsbpluspoH}{\MPdotTTfdotinvplusdsbpluspoL}
\newsavebox{\MPdotTTfdotinvplusdsbpluspoM}
\begin{lrbox}{\MPdotTTfdotinvplusdsbpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbpluspoN}
\settowidth{\MPdotTTfdotinvplusdsbpluspoN}{\usebox{\MPdotTTfdotinvplusdsbpluspoM}}
\addtolength{\MPdotTTfdotinvplusdsbpluspoH}{\MPdotTTfdotinvplusdsbpluspoN}
\newsavebox{\MPdotTTfdotinvplusdsbpluspoO}
\begin{lrbox}{\MPdotTTfdotinvplusdsbpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbpluspoP}
\settowidth{\MPdotTTfdotinvplusdsbpluspoP}{\usebox{\MPdotTTfdotinvplusdsbpluspoO}}
\newsavebox{\MPdotTTfdotinvplusdsbpluspoA}
\begin{lrbox}{\MPdotTTfdotinvplusdsbpluspoA}
\begin{minipage}{\MPdotTTfdotinvplusdsbpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv+dsb+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvplusdsbpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvplusdsbpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvplusdsbpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.TTf.inv+dsbs.tex <==
\newlength{\MPdotTTfdotinvplusdsbsH}
\setlength{\MPdotTTfdotinvplusdsbsH}{0cm}
\newsavebox{\MPdotTTfdotinvplusdsbsI}
\begin{lrbox}{\MPdotTTfdotinvplusdsbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbsJ}
\settowidth{\MPdotTTfdotinvplusdsbsJ}{\usebox{\MPdotTTfdotinvplusdsbsI}}
\addtolength{\MPdotTTfdotinvplusdsbsH}{\MPdotTTfdotinvplusdsbsJ}
\newsavebox{\MPdotTTfdotinvplusdsbsK}
\begin{lrbox}{\MPdotTTfdotinvplusdsbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbsL}
\settowidth{\MPdotTTfdotinvplusdsbsL}{\usebox{\MPdotTTfdotinvplusdsbsK}}
\addtolength{\MPdotTTfdotinvplusdsbsH}{\MPdotTTfdotinvplusdsbsL}
\newsavebox{\MPdotTTfdotinvplusdsbsM}
\begin{lrbox}{\MPdotTTfdotinvplusdsbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbsN}
\settowidth{\MPdotTTfdotinvplusdsbsN}{\usebox{\MPdotTTfdotinvplusdsbsM}}
\addtolength{\MPdotTTfdotinvplusdsbsH}{\MPdotTTfdotinvplusdsbsN}
\newsavebox{\MPdotTTfdotinvplusdsbsO}
\begin{lrbox}{\MPdotTTfdotinvplusdsbsO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbsP}
\settowidth{\MPdotTTfdotinvplusdsbsP}{\usebox{\MPdotTTfdotinvplusdsbsO}}
\newsavebox{\MPdotTTfdotinvplusdsbsA}
\begin{lrbox}{\MPdotTTfdotinvplusdsbsA}
\begin{minipage}{\MPdotTTfdotinvplusdsbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv+dsbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvplusdsbsP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvplusdsbsO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvplusdsbsA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbsK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbsM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.TTf.inv.EL1+dsb-tlbiis-dsb+dmb.tex <==
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}
\setlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{0cm}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}
\begin{minipage}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv.EL1+dsb-tlbiis-dsb+dmb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.TTf.inv.EL1+dsb-tlbiis-dsb+dsb-isb.tex <==
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}
\setlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbI}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbJ}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbJ}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbI}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbJ}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbK}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbL}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbL}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbK}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbL}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbM}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbN}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbN}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbM}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbN}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbO}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbP}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbP}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbO}}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbA}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbA}
\begin{minipage}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv.EL1+dsb-tlbiis-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.TTf.inv.EL1+dsb-tlbiis-dsb+po.tex <==
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}
\setlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}{0cm}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoI}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoJ}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoJ}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoI}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoJ}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoK}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoL}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoL}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoK}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoL}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoM}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoN}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoN}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoM}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoN}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoO}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoP}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoP}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoO}}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoA}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoA}
\begin{minipage}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv.EL1+dsb-tlbiis-dsb+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.TfR+dmb+eret.tex <==
\newlength{\MPdotTfRplusdmbpluseretH}
\setlength{\MPdotTfRplusdmbpluseretH}{0cm}
\newsavebox{\MPdotTfRplusdmbpluseretI}
\begin{lrbox}{\MPdotTfRplusdmbpluseretI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTfRplusdmbpluseretJ}
\settowidth{\MPdotTfRplusdmbpluseretJ}{\usebox{\MPdotTfRplusdmbpluseretI}}
\addtolength{\MPdotTfRplusdmbpluseretH}{\MPdotTfRplusdmbpluseretJ}
\newsavebox{\MPdotTfRplusdmbpluseretK}
\begin{lrbox}{\MPdotTfRplusdmbpluseretK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
LDR X4,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTfRplusdmbpluseretL}
\settowidth{\MPdotTfRplusdmbpluseretL}{\usebox{\MPdotTfRplusdmbpluseretK}}
\addtolength{\MPdotTfRplusdmbpluseretH}{\MPdotTfRplusdmbpluseretL}
\newsavebox{\MPdotTfRplusdmbpluseretM}
\begin{lrbox}{\MPdotTfRplusdmbpluseretM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTfRplusdmbpluseretN}
\settowidth{\MPdotTfRplusdmbpluseretN}{\usebox{\MPdotTfRplusdmbpluseretM}}
\addtolength{\MPdotTfRplusdmbpluseretH}{\MPdotTfRplusdmbpluseretN}
\newsavebox{\MPdotTfRplusdmbpluseretO}
\begin{lrbox}{\MPdotTfRplusdmbpluseretO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;

    y |-> pa2;
    y ?-> invalid;

    *pa1 = 0;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTfRplusdmbpluseretP}
\settowidth{\MPdotTfRplusdmbpluseretP}{\usebox{\MPdotTfRplusdmbpluseretO}}
\newsavebox{\MPdotTfRplusdmbpluseretA}
\begin{lrbox}{\MPdotTfRplusdmbpluseretA}
\begin{minipage}{\MPdotTfRplusdmbpluseretH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TfR+dmb+eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTfRplusdmbpluseretP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTfRplusdmbpluseretO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTfRplusdmbpluseretA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTfRplusdmbpluseretI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTfRplusdmbpluseretK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTfRplusdmbpluseretM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R2=0 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/MP.alias3+rfi-data+dmb.tex <==
\newlength{\MPdotaliasthreeplusrfidataplusdmbH}
\setlength{\MPdotaliasthreeplusrfidataplusdmbH}{0cm}
\newsavebox{\MPdotaliasthreeplusrfidataplusdmbI}
\begin{lrbox}{\MPdotaliasthreeplusrfidataplusdmbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
STR X2,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotaliasthreeplusrfidataplusdmbJ}
\settowidth{\MPdotaliasthreeplusrfidataplusdmbJ}{\usebox{\MPdotaliasthreeplusrfidataplusdmbI}}
\addtolength{\MPdotaliasthreeplusrfidataplusdmbH}{\MPdotaliasthreeplusrfidataplusdmbJ}
\newsavebox{\MPdotaliasthreeplusrfidataplusdmbK}
\begin{lrbox}{\MPdotaliasthreeplusrfidataplusdmbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotaliasthreeplusrfidataplusdmbL}
\settowidth{\MPdotaliasthreeplusrfidataplusdmbL}{\usebox{\MPdotaliasthreeplusrfidataplusdmbK}}
\addtolength{\MPdotaliasthreeplusrfidataplusdmbH}{\MPdotaliasthreeplusrfidataplusdmbL}
\newsavebox{\MPdotaliasthreeplusrfidataplusdmbM}
\begin{lrbox}{\MPdotaliasthreeplusrfidataplusdmbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    y |-> pa2;
    z |-> pa1;
    *pa1 = 0;
    *pa2 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotaliasthreeplusrfidataplusdmbN}
\settowidth{\MPdotaliasthreeplusrfidataplusdmbN}{\usebox{\MPdotaliasthreeplusrfidataplusdmbM}}
\newsavebox{\MPdotaliasthreeplusrfidataplusdmbO}
\begin{lrbox}{\MPdotaliasthreeplusrfidataplusdmbO}
\begin{minipage}{\MPdotaliasthreeplusrfidataplusdmbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R3=z|\\
\lstinline[language=IslaLitmusExp]|0:R5=y|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.alias3+rfi-data+dmb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotaliasthreeplusrfidataplusdmbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotaliasthreeplusrfidataplusdmbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotaliasthreeplusrfidataplusdmbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotaliasthreeplusrfidataplusdmbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotaliasthreeplusrfidataplusdmbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/PPOAA.alias.tex <==
\newlength{\PPOAAdotaliasH}
\setlength{\PPOAAdotaliasH}{0cm}
\newsavebox{\PPOAAdotaliasI}
\begin{lrbox}{\PPOAAdotaliasI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\PPOAAdotaliasJ}
\settowidth{\PPOAAdotaliasJ}{\usebox{\PPOAAdotaliasI}}
\addtolength{\PPOAAdotaliasH}{\PPOAAdotaliasJ}
\newsavebox{\PPOAAdotaliasK}
\begin{lrbox}{\PPOAAdotaliasK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X9,X0,X0
STR X2,[X3,X9]
LDR X4,[X5]
EOR X8,X4,X4
LDR X6,[X7,X8]
\end{lstlisting}
\end{lrbox}
\newlength{\PPOAAdotaliasL}
\settowidth{\PPOAAdotaliasL}{\usebox{\PPOAAdotaliasK}}
\addtolength{\PPOAAdotaliasH}{\PPOAAdotaliasL}
\newsavebox{\PPOAAdotaliasM}
\begin{lrbox}{\PPOAAdotaliasM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    w |-> pa1;
    x |-> pa1;
    y |-> pa2;
    z |-> pa3;
\end{lstlisting}
\end{lrbox}
\newlength{\PPOAAdotaliasN}
\settowidth{\PPOAAdotaliasN}{\usebox{\PPOAAdotaliasM}}
\newsavebox{\PPOAAdotaliasO}
\begin{lrbox}{\PPOAAdotaliasO}
\begin{minipage}{\PPOAAdotaliasH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R1=z|\\
\lstinline[language=IslaLitmusExp]|0:R2=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0x1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=w|\\
\lstinline[language=IslaLitmusExp]|1:R7=z|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|PPOAA.alias|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\PPOAAdotaliasN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\PPOAAdotaliasM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\PPOAAdotaliasO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\PPOAAdotaliasI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\PPOAAdotaliasK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R4=1 & 1:R6=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/PPOCA.alias.tex <==
\newlength{\PPOCAdotaliasH}
\setlength{\PPOCAdotaliasH}{0cm}
\newsavebox{\PPOCAdotaliasI}
\begin{lrbox}{\PPOCAdotaliasI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\PPOCAdotaliasJ}
\settowidth{\PPOCAdotaliasJ}{\usebox{\PPOCAdotaliasI}}
\addtolength{\PPOCAdotaliasH}{\PPOCAdotaliasJ}
\newsavebox{\PPOCAdotaliasK}
\begin{lrbox}{\PPOCAdotaliasK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBNZ X0,L0
L0:
STR X2,[X3]
LDR X4,[X5]
EOR X8,X4,X4
LDR X6,[X7,X8]
\end{lstlisting}
\end{lrbox}
\newlength{\PPOCAdotaliasL}
\settowidth{\PPOCAdotaliasL}{\usebox{\PPOCAdotaliasK}}
\addtolength{\PPOCAdotaliasH}{\PPOCAdotaliasL}
\newsavebox{\PPOCAdotaliasM}
\begin{lrbox}{\PPOCAdotaliasM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    w |-> pa1;
    x |-> pa1;
    y |-> pa2;
    z |-> pa3;
    *pa1 = 0;
    *pa2 = 0;
    *pa3 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\PPOCAdotaliasN}
\settowidth{\PPOCAdotaliasN}{\usebox{\PPOCAdotaliasM}}
\newsavebox{\PPOCAdotaliasO}
\begin{lrbox}{\PPOCAdotaliasO}
\begin{minipage}{\PPOCAdotaliasH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R1=z|\\
\lstinline[language=IslaLitmusExp]|0:R2=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0x1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=w|\\
\lstinline[language=IslaLitmusExp]|1:R7=z|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|PPOCA.alias|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\PPOCAdotaliasN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\PPOCAdotaliasM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\PPOCAdotaliasO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\PPOCAdotaliasI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\PPOCAdotaliasK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R4=1 & 1:R6=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/PPODA.RT.inv.tex <==
\newlength{\PPODAdotRTdotinvH}
\setlength{\PPODAdotRTdotinvH}{0cm}
\newsavebox{\PPODAdotRTdotinvI}
\begin{lrbox}{\PPODAdotRTdotinvI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\PPODAdotRTdotinvJ}
\settowidth{\PPODAdotRTdotinvJ}{\usebox{\PPODAdotRTdotinvI}}
\addtolength{\PPODAdotRTdotinvH}{\PPODAdotRTdotinvJ}
\newsavebox{\PPODAdotRTdotinvK}
\begin{lrbox}{\PPODAdotRTdotinvK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
ORR X2,X2,X3
STR X2,[X4]
LDR X6,[X5]
EOR X8,X6,X6
LDR X9,[X7,X8]
\end{lstlisting}
\end{lrbox}
\newlength{\PPODAdotRTdotinvL}
\settowidth{\PPODAdotRTdotinvL}{\usebox{\PPODAdotRTdotinvK}}
\addtolength{\PPODAdotRTdotinvH}{\PPODAdotRTdotinvL}
\newsavebox{\PPODAdotRTdotinvM}
\begin{lrbox}{\PPODAdotRTdotinvM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X6,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\PPODAdotRTdotinvN}
\settowidth{\PPODAdotRTdotinvN}{\usebox{\PPODAdotRTdotinvM}}
\addtolength{\PPODAdotRTdotinvH}{\PPODAdotRTdotinvN}
\newsavebox{\PPODAdotRTdotinvO}
\begin{lrbox}{\PPODAdotRTdotinvO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    w |-> pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa2;
    z |-> pa3;
    *pa1 = 1;
    *pa2 = 0;
    *pa3 = 0;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\PPODAdotRTdotinvP}
\settowidth{\PPODAdotRTdotinvP}{\usebox{\PPODAdotRTdotinvO}}
\newsavebox{\PPODAdotRTdotinvA}
\begin{lrbox}{\PPODAdotRTdotinvA}
\begin{minipage}{\PPODAdotRTdotinvH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R1=z|\\
\lstinline[language=IslaLitmusExp]|0:R2=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=desc3(w,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R4=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R5=x|\\
\lstinline[language=IslaLitmusExp]|1:R7=z|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|PPODA.RT.inv|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\PPODAdotRTdotinvP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\PPODAdotRTdotinvO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\PPODAdotRTdotinvA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\PPODAdotRTdotinvI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\PPODAdotRTdotinvK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\PPODAdotRTdotinvM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R6=1 & 1:R9=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/R.RTf.inv.EL1+dsb-tlbiis-dsb+popl.tex <==
\newlength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}
\setlength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}{0cm}
\newsavebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplI}
\begin{lrbox}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplJ}
\settowidth{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplJ}{\usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplI}}
\addtolength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplJ}
\newsavebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplK}
\begin{lrbox}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplK}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
STLR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplL}
\settowidth{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplL}{\usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplK}}
\addtolength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplL}
\newsavebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplM}
\begin{lrbox}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplN}
\settowidth{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplN}{\usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplM}}
\addtolength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplN}
\newsavebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplO}
\begin{lrbox}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplP}
\settowidth{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplP}{\usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplO}}
\newsavebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplA}
\begin{lrbox}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplA}
\begin{minipage}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R0=0x2|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|R.RTf.inv.EL1+dsb-tlbiis-dsb+popl|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|y=2 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/R.inv.tex <==
\newlength{\RdotinvH}
\setlength{\RdotinvH}{0cm}
\newsavebox{\RdotinvI}
\begin{lrbox}{\RdotinvI}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\RdotinvJ}
\settowidth{\RdotinvJ}{\usebox{\RdotinvI}}
\addtolength{\RdotinvH}{\RdotinvJ}
\newsavebox{\RdotinvK}
\begin{lrbox}{\RdotinvK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\RdotinvL}
\settowidth{\RdotinvL}{\usebox{\RdotinvK}}
\addtolength{\RdotinvH}{\RdotinvL}
\newsavebox{\RdotinvM}
\begin{lrbox}{\RdotinvM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    identity 0x1000 with code;
    *pa1 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\RdotinvN}
\settowidth{\RdotinvN}{\usebox{\RdotinvM}}
\newsavebox{\RdotinvO}
\begin{lrbox}{\RdotinvO}
\begin{minipage}{\RdotinvH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|R.inv|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\RdotinvN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\RdotinvM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\RdotinvO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\RdotinvI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\RdotinvK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R0=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/RBS+dsb-tlbiis-dsb.tex <==
\newlength{\RBSplusdsbtlbiisdsbH}
\setlength{\RBSplusdsbtlbiisdsbH}{0cm}
\newsavebox{\RBSplusdsbtlbiisdsbI}
\begin{lrbox}{\RBSplusdsbtlbiisdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X5
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\RBSplusdsbtlbiisdsbJ}
\settowidth{\RBSplusdsbtlbiisdsbJ}{\usebox{\RBSplusdsbtlbiisdsbI}}
\addtolength{\RBSplusdsbtlbiisdsbH}{\RBSplusdsbtlbiisdsbJ}
\newsavebox{\RBSplusdsbtlbiisdsbK}
\begin{lrbox}{\RBSplusdsbtlbiisdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\RBSplusdsbtlbiisdsbL}
\settowidth{\RBSplusdsbtlbiisdsbL}{\usebox{\RBSplusdsbtlbiisdsbK}}
\addtolength{\RBSplusdsbtlbiisdsbH}{\RBSplusdsbtlbiisdsbL}
\newsavebox{\RBSplusdsbtlbiisdsbM}
\begin{lrbox}{\RBSplusdsbtlbiisdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\RBSplusdsbtlbiisdsbN}
\settowidth{\RBSplusdsbtlbiisdsbN}{\usebox{\RBSplusdsbtlbiisdsbM}}
\addtolength{\RBSplusdsbtlbiisdsbH}{\RBSplusdsbtlbiisdsbN}
\newsavebox{\RBSplusdsbtlbiisdsbO}
\begin{lrbox}{\RBSplusdsbtlbiisdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;
    y |-> pa1;
    *pa1 = 0;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\RBSplusdsbtlbiisdsbP}
\settowidth{\RBSplusdsbtlbiisdsbP}{\usebox{\RBSplusdsbtlbiisdsbO}}
\newsavebox{\RBSplusdsbtlbiisdsbA}
\begin{lrbox}{\RBSplusdsbtlbiisdsbA}
\begin{minipage}{\RBSplusdsbtlbiisdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0x2|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R5=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|RBS+dsb-tlbiis-dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\RBSplusdsbtlbiisdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\RBSplusdsbtlbiisdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\RBSplusdsbtlbiisdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\RBSplusdsbtlbiisdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\RBSplusdsbtlbiisdsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\RBSplusdsbtlbiisdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=2|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/RDW.alias.tex <==
\newlength{\RDWdotaliasH}
\setlength{\RDWdotaliasH}{0cm}
\newsavebox{\RDWdotaliasI}
\begin{lrbox}{\RDWdotaliasI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\RDWdotaliasJ}
\settowidth{\RDWdotaliasJ}{\usebox{\RDWdotaliasI}}
\addtolength{\RDWdotaliasH}{\RDWdotaliasJ}
\newsavebox{\RDWdotaliasK}
\begin{lrbox}{\RDWdotaliasK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
LDR X3,[X4,X2]
LDR X5,[X6]
EOR X7,X5,X5
LDR X8,[X9,X7]
\end{lstlisting}
\end{lrbox}
\newlength{\RDWdotaliasL}
\settowidth{\RDWdotaliasL}{\usebox{\RDWdotaliasK}}
\addtolength{\RDWdotaliasH}{\RDWdotaliasL}
\newsavebox{\RDWdotaliasM}
\begin{lrbox}{\RDWdotaliasM}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\RDWdotaliasN}
\settowidth{\RDWdotaliasN}{\usebox{\RDWdotaliasM}}
\addtolength{\RDWdotaliasH}{\RDWdotaliasN}
\newsavebox{\RDWdotaliasO}
\begin{lrbox}{\RDWdotaliasO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    w |-> pa1;
    x |-> pa1;
    y |-> pa2;
    z |-> pa3;
    *pa1 = 0;
    *pa2 = 0;
    *pa3 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\RDWdotaliasP}
\settowidth{\RDWdotaliasP}{\usebox{\RDWdotaliasO}}
\newsavebox{\RDWdotaliasA}
\begin{lrbox}{\RDWdotaliasA}
\begin{minipage}{\RDWdotaliasH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=z|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R4=w|\\
\lstinline[language=IslaLitmusExp]|1:R6=x|\\
\lstinline[language=IslaLitmusExp]|1:R9=z|\\
\lstinline[language=IslaLitmusExp]|2:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|2:R1=x|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|RDW.alias|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\RDWdotaliasP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\RDWdotaliasO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\RDWdotaliasA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\RDWdotaliasI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\RDWdotaliasK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\RDWdotaliasM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R3=0 & 1:R5=1 & 1:R8=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/ROT.inv+dmbst.tex <==
\newlength{\ROTdotinvplusdmbstH}
\setlength{\ROTdotinvplusdmbstH}{0cm}
\newsavebox{\ROTdotinvplusdmbstI}
\begin{lrbox}{\ROTdotinvplusdmbstI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB ST
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvplusdmbstJ}
\settowidth{\ROTdotinvplusdmbstJ}{\usebox{\ROTdotinvplusdmbstI}}
\addtolength{\ROTdotinvplusdmbstH}{\ROTdotinvplusdmbstJ}
\newsavebox{\ROTdotinvplusdmbstK}
\begin{lrbox}{\ROTdotinvplusdmbstK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvplusdmbstL}
\settowidth{\ROTdotinvplusdmbstL}{\usebox{\ROTdotinvplusdmbstK}}
\addtolength{\ROTdotinvplusdmbstH}{\ROTdotinvplusdmbstL}
\newsavebox{\ROTdotinvplusdmbstM}
\begin{lrbox}{\ROTdotinvplusdmbstM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS x14,esr_el1
AND X14,X14,#0b111
CMP x14,#0b111
MOV X17,#1
MOV X18,#2
// if ESR_EL1.ISS.DFSC == Translation Level 3 then x2 = 1 else x2 = 2
CSEL x0,x17,x18,eq
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvplusdmbstN}
\settowidth{\ROTdotinvplusdmbstN}{\usebox{\ROTdotinvplusdmbstM}}
\addtolength{\ROTdotinvplusdmbstH}{\ROTdotinvplusdmbstN}
\newsavebox{\ROTdotinvplusdmbstO}
\begin{lrbox}{\ROTdotinvplusdmbstO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
physical pa1;
intermediate ipa1;

assert pa1 == ipa1;
ipa1 |-> pa1;

s1table new_table 0x280000 {
  x |-> invalid;
  x ?-> ipa1;
};

identity 0x283000 with default;

x |-> invalid at level 2;
x ?-> table(0x283000) at level 2;

identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvplusdmbstP}
\settowidth{\ROTdotinvplusdmbstP}{\usebox{\ROTdotinvplusdmbstO}}
\newsavebox{\ROTdotinvplusdmbstA}
\begin{lrbox}{\ROTdotinvplusdmbstA}
\begin{minipage}{\ROTdotinvplusdmbstH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=ipa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,new_table)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc2(table=0x283000)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte2(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|ROT.inv+dmbst|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\ROTdotinvplusdmbstP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\ROTdotinvplusdmbstO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\ROTdotinvplusdmbstA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\ROTdotinvplusdmbstI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\ROTdotinvplusdmbstK}\\
  \cline{2-2}
  & thread 1 el1 handler\\
  \cline{2-2}
  & \usebox{\ROTdotinvplusdmbstM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/ROT.inv+dsb.tex <==
\newlength{\ROTdotinvplusdsbH}
\setlength{\ROTdotinvplusdsbH}{0cm}
\newsavebox{\ROTdotinvplusdsbI}
\begin{lrbox}{\ROTdotinvplusdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvplusdsbJ}
\settowidth{\ROTdotinvplusdsbJ}{\usebox{\ROTdotinvplusdsbI}}
\addtolength{\ROTdotinvplusdsbH}{\ROTdotinvplusdsbJ}
\newsavebox{\ROTdotinvplusdsbK}
\begin{lrbox}{\ROTdotinvplusdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvplusdsbL}
\settowidth{\ROTdotinvplusdsbL}{\usebox{\ROTdotinvplusdsbK}}
\addtolength{\ROTdotinvplusdsbH}{\ROTdotinvplusdsbL}
\newsavebox{\ROTdotinvplusdsbM}
\begin{lrbox}{\ROTdotinvplusdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS X14,ESR_EL1
AND X14,X14,#0b111
CMP X14,#0b111
MOV X17,#1
MOV X18,#2
// if ESR_EL1.ISS.DFSC == Translation Level 3 then x2 = 1 else x2 = 2
CSEL X0,X17,X18,eq
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvplusdsbN}
\settowidth{\ROTdotinvplusdsbN}{\usebox{\ROTdotinvplusdsbM}}
\addtolength{\ROTdotinvplusdsbH}{\ROTdotinvplusdsbN}
\newsavebox{\ROTdotinvplusdsbO}
\begin{lrbox}{\ROTdotinvplusdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
physical pa1;
intermediate ipa1;

assert pa1 == ipa1;
ipa1 |-> pa1;

s1table new_table 0x280000 {
  x |-> invalid;
  x ?-> ipa1;
};

identity 0x283000 with default;

x |-> invalid at level 2;
x ?-> table(0x283000) at level 2;

identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvplusdsbP}
\settowidth{\ROTdotinvplusdsbP}{\usebox{\ROTdotinvplusdsbO}}
\newsavebox{\ROTdotinvplusdsbA}
\begin{lrbox}{\ROTdotinvplusdsbA}
\begin{minipage}{\ROTdotinvplusdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=ipa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,new_table)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc2(table=0x283000)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte2(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|ROT.inv+dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\ROTdotinvplusdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\ROTdotinvplusdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\ROTdotinvplusdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\ROTdotinvplusdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\ROTdotinvplusdsbK}\\
  \cline{2-2}
  & thread 1 el1 handler\\
  \cline{2-2}
  & \usebox{\ROTdotinvplusdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/ROT.inv+po.tex <==
\newlength{\ROTdotinvpluspoH}
\setlength{\ROTdotinvpluspoH}{0cm}
\newsavebox{\ROTdotinvpluspoI}
\begin{lrbox}{\ROTdotinvpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvpluspoJ}
\settowidth{\ROTdotinvpluspoJ}{\usebox{\ROTdotinvpluspoI}}
\addtolength{\ROTdotinvpluspoH}{\ROTdotinvpluspoJ}
\newsavebox{\ROTdotinvpluspoK}
\begin{lrbox}{\ROTdotinvpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvpluspoL}
\settowidth{\ROTdotinvpluspoL}{\usebox{\ROTdotinvpluspoK}}
\addtolength{\ROTdotinvpluspoH}{\ROTdotinvpluspoL}
\newsavebox{\ROTdotinvpluspoM}
\begin{lrbox}{\ROTdotinvpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS X14,ESR_EL1
AND X14,X14,#0b111
CMP X14,#0b111
MOV X17,#1
MOV X18,#2
// if ESR_EL1.ISS.DFSC == Translation Level 3 then x2 = 1 else x2 = 2
CSEL X0,X17,X18,eq
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvpluspoN}
\settowidth{\ROTdotinvpluspoN}{\usebox{\ROTdotinvpluspoM}}
\addtolength{\ROTdotinvpluspoH}{\ROTdotinvpluspoN}
\newsavebox{\ROTdotinvpluspoO}
\begin{lrbox}{\ROTdotinvpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
physical pa1;
intermediate ipa1;

assert pa1 == ipa1;
ipa1 |-> pa1;

s1table new_table 0x280000 {
  x |-> invalid;
  x ?-> ipa1;
};

identity 0x283000 with default;

x |-> invalid at level 2;
x ?-> table(0x283000) at level 2;

identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvpluspoP}
\settowidth{\ROTdotinvpluspoP}{\usebox{\ROTdotinvpluspoO}}
\newsavebox{\ROTdotinvpluspoA}
\begin{lrbox}{\ROTdotinvpluspoA}
\begin{minipage}{\ROTdotinvpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=ipa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,new_table)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc2(table=0x283000)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte2(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|ROT.inv+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\ROTdotinvpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\ROTdotinvpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\ROTdotinvpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\ROTdotinvpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\ROTdotinvpluspoK}\\
  \cline{2-2}
  & thread 1 el1 handler\\
  \cline{2-2}
  & \usebox{\ROTdotinvpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/RSW.alias.tex <==
\newlength{\RSWdotaliasH}
\setlength{\RSWdotaliasH}{0cm}
\newsavebox{\RSWdotaliasI}
\begin{lrbox}{\RSWdotaliasI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\RSWdotaliasJ}
\settowidth{\RSWdotaliasJ}{\usebox{\RSWdotaliasI}}
\addtolength{\RSWdotaliasH}{\RSWdotaliasJ}
\newsavebox{\RSWdotaliasK}
\begin{lrbox}{\RSWdotaliasK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
LDR X3,[X4,X2]
LDR X5,[X6]
EOR X7,X5,X5
LDR X8,[X9,X7]
\end{lstlisting}
\end{lrbox}
\newlength{\RSWdotaliasL}
\settowidth{\RSWdotaliasL}{\usebox{\RSWdotaliasK}}
\addtolength{\RSWdotaliasH}{\RSWdotaliasL}
\newsavebox{\RSWdotaliasM}
\begin{lrbox}{\RSWdotaliasM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    w |-> pa1;
    x |-> pa1;
    y |-> pa2;
    z |-> pa3;
    *pa1 = 0;
    *pa2 = 0;
    *pa3 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\RSWdotaliasN}
\settowidth{\RSWdotaliasN}{\usebox{\RSWdotaliasM}}
\newsavebox{\RSWdotaliasO}
\begin{lrbox}{\RSWdotaliasO}
\begin{minipage}{\RSWdotaliasH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=z|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R4=w|\\
\lstinline[language=IslaLitmusExp]|1:R6=x|\\
\lstinline[language=IslaLitmusExp]|1:R9=z|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|RSW.alias|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\RSWdotaliasN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\RSWdotaliasM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\RSWdotaliasO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\RSWdotaliasI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\RSWdotaliasK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R8=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/RWC.RTR.EL1+dsb-isb+dsb-tlbi-dsb.tex <==
\newlength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbH}
\setlength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbH}{0cm}
\newsavebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbI}
\begin{lrbox}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbJ}
\settowidth{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbJ}{\usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbI}}
\addtolength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbH}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbJ}
\newsavebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbK}
\begin{lrbox}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X3,[X4,X2]
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbL}
\settowidth{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbL}{\usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbK}}
\addtolength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbH}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbL}
\newsavebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbM}
\begin{lrbox}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X2
DSB SY
LDR X3,[X4]
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbN}
\settowidth{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbN}{\usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbM}}
\addtolength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbH}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbN}
\newsavebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbO}
\begin{lrbox}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X3,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbP}
\settowidth{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbP}{\usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbO}}
\addtolength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbH}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbP}
\newsavebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbA}
\begin{lrbox}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;

    y |-> pa2;
    y ?-> invalid;
    z |-> pa2;
    *pa1 = 1;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbB}
\settowidth{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbB}{\usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbA}}
\newsavebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbC}
\begin{lrbox}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbC}
\begin{minipage}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R4=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|2:R1=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R2=page(x)|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|RWC.RTR.EL1+dsb-isb+dsb-tlbi-dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R1=1 & 1:R3=0 & 2:R3=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/RWC.RTfR.inv+addr+dmb.tex <==
\newlength{\RWCdotRTfRdotinvplusaddrplusdmbH}
\setlength{\RWCdotRTfRdotinvplusaddrplusdmbH}{0cm}
\newsavebox{\RWCdotRTfRdotinvplusaddrplusdmbI}
\begin{lrbox}{\RWCdotRTfRdotinvplusaddrplusdmbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTfRdotinvplusaddrplusdmbJ}
\settowidth{\RWCdotRTfRdotinvplusaddrplusdmbJ}{\usebox{\RWCdotRTfRdotinvplusaddrplusdmbI}}
\addtolength{\RWCdotRTfRdotinvplusaddrplusdmbH}{\RWCdotRTfRdotinvplusaddrplusdmbJ}
\newsavebox{\RWCdotRTfRdotinvplusaddrplusdmbK}
\begin{lrbox}{\RWCdotRTfRdotinvplusaddrplusdmbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
LDR X3,[X4,X2]
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTfRdotinvplusaddrplusdmbL}
\settowidth{\RWCdotRTfRdotinvplusaddrplusdmbL}{\usebox{\RWCdotRTfRdotinvplusaddrplusdmbK}}
\addtolength{\RWCdotRTfRdotinvplusaddrplusdmbH}{\RWCdotRTfRdotinvplusaddrplusdmbL}
\newsavebox{\RWCdotRTfRdotinvplusaddrplusdmbM}
\begin{lrbox}{\RWCdotRTfRdotinvplusaddrplusdmbM}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTfRdotinvplusaddrplusdmbN}
\settowidth{\RWCdotRTfRdotinvplusaddrplusdmbN}{\usebox{\RWCdotRTfRdotinvplusaddrplusdmbM}}
\addtolength{\RWCdotRTfRdotinvplusaddrplusdmbH}{\RWCdotRTfRdotinvplusaddrplusdmbN}
\newsavebox{\RWCdotRTfRdotinvplusaddrplusdmbO}
\begin{lrbox}{\RWCdotRTfRdotinvplusaddrplusdmbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X3,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTfRdotinvplusaddrplusdmbP}
\settowidth{\RWCdotRTfRdotinvplusaddrplusdmbP}{\usebox{\RWCdotRTfRdotinvplusaddrplusdmbO}}
\addtolength{\RWCdotRTfRdotinvplusaddrplusdmbH}{\RWCdotRTfRdotinvplusaddrplusdmbP}
\newsavebox{\RWCdotRTfRdotinvplusaddrplusdmbA}
\begin{lrbox}{\RWCdotRTfRdotinvplusaddrplusdmbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;

    y |-> invalid;
    y ?-> pa2;
    z |-> pa2;
    *pa1 = 1;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTfRdotinvplusaddrplusdmbB}
\settowidth{\RWCdotRTfRdotinvplusaddrplusdmbB}{\usebox{\RWCdotRTfRdotinvplusaddrplusdmbA}}
\newsavebox{\RWCdotRTfRdotinvplusaddrplusdmbC}
\begin{lrbox}{\RWCdotRTfRdotinvplusaddrplusdmbC}
\begin{minipage}{\RWCdotRTfRdotinvplusaddrplusdmbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R4=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|2:R1=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|RWC.RTfR.inv+addr+dmb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\RWCdotRTfRdotinvplusaddrplusdmbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\RWCdotRTfRdotinvplusaddrplusdmbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\RWCdotRTfRdotinvplusaddrplusdmbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\RWCdotRTfRdotinvplusaddrplusdmbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\RWCdotRTfRdotinvplusaddrplusdmbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\RWCdotRTfRdotinvplusaddrplusdmbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\RWCdotRTfRdotinvplusaddrplusdmbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R1=1 & 1:R3=0 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/S.RT.ro+dsb-tlbiis-dsb+dsb-isb.tex <==
\newlength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbH}
\setlength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbH}{0cm}
\newsavebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbI}
\begin{lrbox}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbJ}
\settowidth{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbJ}{\usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbI}}
\addtolength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbH}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbJ}
\newsavebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbK}
\begin{lrbox}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbL}
\settowidth{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbL}{\usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbK}}
\addtolength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbH}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbL}
\newsavebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbM}
\begin{lrbox}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbN}
\settowidth{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbN}{\usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbM}}
\addtolength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbH}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbN}
\newsavebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbO}
\begin{lrbox}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1 with [AP = 0b11] and default;
    x ?-> pa1;
    z |-> pa1;
    y |-> pa2;

    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbP}
\settowidth{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbP}{\usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbO}}
\newsavebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbA}
\begin{lrbox}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbA}
\begin{minipage}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|S.RT.ro+dsb-tlbiis-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/S.RTf.inv.EL1+dsb-tlbiis-dsb+ctrl.tex <==
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}
\setlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}{0cm}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlI}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlJ}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlJ}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlI}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlJ}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlK}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBNZ X0,L0
L0:
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlL}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlL}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlK}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlL}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlM}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlN}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlN}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlM}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlN}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlO}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlP}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlP}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlO}}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlA}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlA}
\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|S.RTf.inv.EL1+dsb-tlbiis-dsb+ctrl|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/S.RTf.inv.EL1+dsb-tlbiis-dsb+data.tex <==
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}
\setlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}{0cm}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataI}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataJ}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataJ}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataI}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataJ}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataK}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
ORR X2,X2,X4
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataL}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataL}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataK}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataL}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataM}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataN}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataN}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataM}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataN}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataO}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataP}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataP}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataO}}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataA}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataA}
\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|S.RTf.inv.EL1+dsb-tlbiis-dsb+data|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/S.RTf.inv.EL1+dsb-tlbiis-dsb+dmb.tex <==
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}
\setlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{0cm}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}
\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|S.RTf.inv.EL1+dsb-tlbiis-dsb+dmb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/S.RTf.inv.EL1+dsb-tlbiis-dsb+poap.tex <==
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}
\setlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}{0cm}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapI}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapJ}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapJ}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapI}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapJ}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapK}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDAR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapL}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapL}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapK}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapL}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapM}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapN}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapN}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapM}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapN}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapO}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapP}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapP}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapO}}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapA}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapA}
\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|S.RTf.inv.EL1+dsb-tlbiis-dsb+poap|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/S.RTf.inv.EL1+dsb-tlbiis-dsb+popl.tex <==
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}
\setlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}{0cm}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplI}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplJ}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplJ}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplI}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplJ}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplK}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STLR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplL}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplL}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplK}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplL}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplM}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplN}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplN}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplM}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplN}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplO}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplP}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplP}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplO}}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplA}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplA}
\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|S.RTf.inv.EL1+dsb-tlbiis-dsb+popl|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/S.T+dmb+po.tex <==
\newlength{\SdotTplusdmbpluspoH}
\setlength{\SdotTplusdmbpluspoH}{0cm}
\newsavebox{\SdotTplusdmbpluspoI}
\begin{lrbox}{\SdotTplusdmbpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotTplusdmbpluspoJ}
\settowidth{\SdotTplusdmbpluspoJ}{\usebox{\SdotTplusdmbpluspoI}}
\addtolength{\SdotTplusdmbpluspoH}{\SdotTplusdmbpluspoJ}
\newsavebox{\SdotTplusdmbpluspoK}
\begin{lrbox}{\SdotTplusdmbpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotTplusdmbpluspoL}
\settowidth{\SdotTplusdmbpluspoL}{\usebox{\SdotTplusdmbpluspoK}}
\addtolength{\SdotTplusdmbpluspoH}{\SdotTplusdmbpluspoL}
\newsavebox{\SdotTplusdmbpluspoM}
\begin{lrbox}{\SdotTplusdmbpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SdotTplusdmbpluspoN}
\settowidth{\SdotTplusdmbpluspoN}{\usebox{\SdotTplusdmbpluspoM}}
\addtolength{\SdotTplusdmbpluspoH}{\SdotTplusdmbpluspoN}
\newsavebox{\SdotTplusdmbpluspoO}
\begin{lrbox}{\SdotTplusdmbpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 0;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SdotTplusdmbpluspoP}
\settowidth{\SdotTplusdmbpluspoP}{\usebox{\SdotTplusdmbpluspoO}}
\newsavebox{\SdotTplusdmbpluspoA}
\begin{lrbox}{\SdotTplusdmbpluspoA}
\begin{minipage}{\SdotTplusdmbpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0x2|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|S.T+dmb+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SdotTplusdmbpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SdotTplusdmbpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SdotTplusdmbpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SdotTplusdmbpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SdotTplusdmbpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SdotTplusdmbpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & x=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/SB.TfTf.inv+dmb-ctrl-isbs.tex <==
\newlength{\SBdotTfTfdotinvplusdmbctrlisbsH}
\setlength{\SBdotTfTfdotinvplusdmbctrlisbsH}{0cm}
\newsavebox{\SBdotTfTfdotinvplusdmbctrlisbsI}
\begin{lrbox}{\SBdotTfTfdotinvplusdmbctrlisbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
LDR X7,[X8]
CBNZ X7,L0
L0:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdmbctrlisbsJ}
\settowidth{\SBdotTfTfdotinvplusdmbctrlisbsJ}{\usebox{\SBdotTfTfdotinvplusdmbctrlisbsI}}
\addtolength{\SBdotTfTfdotinvplusdmbctrlisbsH}{\SBdotTfTfdotinvplusdmbctrlisbsJ}
\newsavebox{\SBdotTfTfdotinvplusdmbctrlisbsK}
\begin{lrbox}{\SBdotTfTfdotinvplusdmbctrlisbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
LDR X7,[X8]
CBNZ X7,L1
L1:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdmbctrlisbsL}
\settowidth{\SBdotTfTfdotinvplusdmbctrlisbsL}{\usebox{\SBdotTfTfdotinvplusdmbctrlisbsK}}
\addtolength{\SBdotTfTfdotinvplusdmbctrlisbsH}{\SBdotTfTfdotinvplusdmbctrlisbsL}
\newsavebox{\SBdotTfTfdotinvplusdmbctrlisbsM}
\begin{lrbox}{\SBdotTfTfdotinvplusdmbctrlisbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdmbctrlisbsN}
\settowidth{\SBdotTfTfdotinvplusdmbctrlisbsN}{\usebox{\SBdotTfTfdotinvplusdmbctrlisbsM}}
\addtolength{\SBdotTfTfdotinvplusdmbctrlisbsH}{\SBdotTfTfdotinvplusdmbctrlisbsN}
\newsavebox{\SBdotTfTfdotinvplusdmbctrlisbsO}
\begin{lrbox}{\SBdotTfTfdotinvplusdmbctrlisbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdmbctrlisbsP}
\settowidth{\SBdotTfTfdotinvplusdmbctrlisbsP}{\usebox{\SBdotTfTfdotinvplusdmbctrlisbsO}}
\addtolength{\SBdotTfTfdotinvplusdmbctrlisbsH}{\SBdotTfTfdotinvplusdmbctrlisbsP}
\newsavebox{\SBdotTfTfdotinvplusdmbctrlisbsA}
\begin{lrbox}{\SBdotTfTfdotinvplusdmbctrlisbsA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> invalid;
    y ?-> pa2;
    v |-> pa2;
    *pa2 = 1;

    z |-> pa3;
    *pa3 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdmbctrlisbsB}
\settowidth{\SBdotTfTfdotinvplusdmbctrlisbsB}{\usebox{\SBdotTfTfdotinvplusdmbctrlisbsA}}
\newsavebox{\SBdotTfTfdotinvplusdmbctrlisbsC}
\begin{lrbox}{\SBdotTfTfdotinvplusdmbctrlisbsC}
\begin{minipage}{\SBdotTfTfdotinvplusdmbctrlisbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R8=z|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R0=desc3(v,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R8=z|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|SB.TfTf.inv+dmb-ctrl-isbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SBdotTfTfdotinvplusdmbctrlisbsB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SBdotTfTfdotinvplusdmbctrlisbsA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SBdotTfTfdotinvplusdmbctrlisbsC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvplusdmbctrlisbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvplusdmbctrlisbsK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvplusdmbctrlisbsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvplusdmbctrlisbsO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/SB.TfTf.inv+dsb-isbs.tex <==
\newlength{\SBdotTfTfdotinvplusdsbisbsH}
\setlength{\SBdotTfTfdotinvplusdsbisbsH}{0cm}
\newsavebox{\SBdotTfTfdotinvplusdsbisbsI}
\begin{lrbox}{\SBdotTfTfdotinvplusdsbisbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdsbisbsJ}
\settowidth{\SBdotTfTfdotinvplusdsbisbsJ}{\usebox{\SBdotTfTfdotinvplusdsbisbsI}}
\addtolength{\SBdotTfTfdotinvplusdsbisbsH}{\SBdotTfTfdotinvplusdsbisbsJ}
\newsavebox{\SBdotTfTfdotinvplusdsbisbsK}
\begin{lrbox}{\SBdotTfTfdotinvplusdsbisbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdsbisbsL}
\settowidth{\SBdotTfTfdotinvplusdsbisbsL}{\usebox{\SBdotTfTfdotinvplusdsbisbsK}}
\addtolength{\SBdotTfTfdotinvplusdsbisbsH}{\SBdotTfTfdotinvplusdsbisbsL}
\newsavebox{\SBdotTfTfdotinvplusdsbisbsM}
\begin{lrbox}{\SBdotTfTfdotinvplusdsbisbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdsbisbsN}
\settowidth{\SBdotTfTfdotinvplusdsbisbsN}{\usebox{\SBdotTfTfdotinvplusdsbisbsM}}
\addtolength{\SBdotTfTfdotinvplusdsbisbsH}{\SBdotTfTfdotinvplusdsbisbsN}
\newsavebox{\SBdotTfTfdotinvplusdsbisbsO}
\begin{lrbox}{\SBdotTfTfdotinvplusdsbisbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdsbisbsP}
\settowidth{\SBdotTfTfdotinvplusdsbisbsP}{\usebox{\SBdotTfTfdotinvplusdsbisbsO}}
\addtolength{\SBdotTfTfdotinvplusdsbisbsH}{\SBdotTfTfdotinvplusdsbisbsP}
\newsavebox{\SBdotTfTfdotinvplusdsbisbsA}
\begin{lrbox}{\SBdotTfTfdotinvplusdsbisbsA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> invalid;
    y ?-> pa2;
    v |-> pa2;
    *pa2 = 1;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdsbisbsB}
\settowidth{\SBdotTfTfdotinvplusdsbisbsB}{\usebox{\SBdotTfTfdotinvplusdsbisbsA}}
\newsavebox{\SBdotTfTfdotinvplusdsbisbsC}
\begin{lrbox}{\SBdotTfTfdotinvplusdsbisbsC}
\begin{minipage}{\SBdotTfTfdotinvplusdsbisbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R0=desc3(v,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|SB.TfTf.inv+dsb-isbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SBdotTfTfdotinvplusdsbisbsB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SBdotTfTfdotinvplusdsbisbsA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SBdotTfTfdotinvplusdsbisbsC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvplusdsbisbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvplusdsbisbsK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvplusdsbisbsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvplusdsbisbsO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/SB.TfTf.invv+rfi-ctrl-isbs.tex <==
\newlength{\SBdotTfTfdotinvvplusrfictrlisbsH}
\setlength{\SBdotTfTfdotinvvplusrfictrlisbsH}{0cm}
\newsavebox{\SBdotTfTfdotinvvplusrfictrlisbsI}
\begin{lrbox}{\SBdotTfTfdotinvvplusrfictrlisbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X7,[X1]
CBNZ X7,L0
L0:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvvplusrfictrlisbsJ}
\settowidth{\SBdotTfTfdotinvvplusrfictrlisbsJ}{\usebox{\SBdotTfTfdotinvvplusrfictrlisbsI}}
\addtolength{\SBdotTfTfdotinvvplusrfictrlisbsH}{\SBdotTfTfdotinvvplusrfictrlisbsJ}
\newsavebox{\SBdotTfTfdotinvvplusrfictrlisbsK}
\begin{lrbox}{\SBdotTfTfdotinvvplusrfictrlisbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X7,[X1]
CBNZ X7,L1
L1:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvvplusrfictrlisbsL}
\settowidth{\SBdotTfTfdotinvvplusrfictrlisbsL}{\usebox{\SBdotTfTfdotinvvplusrfictrlisbsK}}
\addtolength{\SBdotTfTfdotinvvplusrfictrlisbsH}{\SBdotTfTfdotinvvplusrfictrlisbsL}
\newsavebox{\SBdotTfTfdotinvvplusrfictrlisbsM}
\begin{lrbox}{\SBdotTfTfdotinvvplusrfictrlisbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvvplusrfictrlisbsN}
\settowidth{\SBdotTfTfdotinvvplusrfictrlisbsN}{\usebox{\SBdotTfTfdotinvvplusrfictrlisbsM}}
\addtolength{\SBdotTfTfdotinvvplusrfictrlisbsH}{\SBdotTfTfdotinvvplusrfictrlisbsN}
\newsavebox{\SBdotTfTfdotinvvplusrfictrlisbsO}
\begin{lrbox}{\SBdotTfTfdotinvvplusrfictrlisbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvvplusrfictrlisbsP}
\settowidth{\SBdotTfTfdotinvvplusrfictrlisbsP}{\usebox{\SBdotTfTfdotinvvplusrfictrlisbsO}}
\addtolength{\SBdotTfTfdotinvvplusrfictrlisbsH}{\SBdotTfTfdotinvvplusrfictrlisbsP}
\newsavebox{\SBdotTfTfdotinvvplusrfictrlisbsA}
\begin{lrbox}{\SBdotTfTfdotinvvplusrfictrlisbsA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> invalid;
    y ?-> pa2;
    v |-> pa2;
    *pa2 = 1;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvvplusrfictrlisbsB}
\settowidth{\SBdotTfTfdotinvvplusrfictrlisbsB}{\usebox{\SBdotTfTfdotinvvplusrfictrlisbsA}}
\newsavebox{\SBdotTfTfdotinvvplusrfictrlisbsC}
\begin{lrbox}{\SBdotTfTfdotinvvplusrfictrlisbsC}
\begin{minipage}{\SBdotTfTfdotinvvplusrfictrlisbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R0=desc3(v,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|SB.TfTf.invv+rfi-ctrl-isbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SBdotTfTfdotinvvplusrfictrlisbsB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SBdotTfTfdotinvvplusrfictrlisbsA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SBdotTfTfdotinvvplusrfictrlisbsC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvvplusrfictrlisbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvvplusrfictrlisbsK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvvplusrfictrlisbsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvvplusrfictrlisbsO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0 & 0:R7=desc3(u,page_table_base) & 1:R2=0 & 1:R7=desc3(v,page_table_base)|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/SwitchTable.EL2+msrttbr-eret.tex <==
\newlength{\SwitchTabledotELtwoplusmsrttbreretH}
\setlength{\SwitchTabledotELtwoplusmsrttbreretH}{0cm}
\newsavebox{\SwitchTabledotELtwoplusmsrttbreretI}
\begin{lrbox}{\SwitchTabledotELtwoplusmsrttbreretI}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
HVC #0
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SwitchTabledotELtwoplusmsrttbreretJ}
\settowidth{\SwitchTabledotELtwoplusmsrttbreretJ}{\usebox{\SwitchTabledotELtwoplusmsrttbreretI}}
\addtolength{\SwitchTabledotELtwoplusmsrttbreretH}{\SwitchTabledotELtwoplusmsrttbreretJ}
\newsavebox{\SwitchTabledotELtwoplusmsrttbreretK}
\begin{lrbox}{\SwitchTabledotELtwoplusmsrttbreretK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MSR TTBR0_EL1,X4
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SwitchTabledotELtwoplusmsrttbreretL}
\settowidth{\SwitchTabledotELtwoplusmsrttbreretL}{\usebox{\SwitchTabledotELtwoplusmsrttbreretK}}
\addtolength{\SwitchTabledotELtwoplusmsrttbreretH}{\SwitchTabledotELtwoplusmsrttbreretL}
\newsavebox{\SwitchTabledotELtwoplusmsrttbreretM}
\begin{lrbox}{\SwitchTabledotELtwoplusmsrttbreretM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
option default_tables = false;
physical pa1 pa2;

s1table initial_table 0x200000 {
    x |-> pa1 at level 3;
}

s1table new_table 0x280000  {
    x |-> pa2 at level 3;
}

s1table el2_table 0x300000 {
    identity 0x2000 with code;
}

*pa1 = 0;
*pa2 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\SwitchTabledotELtwoplusmsrttbreretN}
\settowidth{\SwitchTabledotELtwoplusmsrttbreretN}{\usebox{\SwitchTabledotELtwoplusmsrttbreretM}}
\newsavebox{\SwitchTabledotELtwoplusmsrttbreretO}
\begin{lrbox}{\SwitchTabledotELtwoplusmsrttbreretO}
\begin{minipage}{\SwitchTabledotELtwoplusmsrttbreretH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|R1=x|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=ttbr(asid=0x0000,base=new_table)|\\
\lstinline[language=IslaLitmusExp]|TTBR0_EL1=ttbr(asid=0x0000,base=initial_table)|\\
\lstinline[language=IslaLitmusExp]|TTBR0_EL2=ttbr(asid=0x0000,base=el2_table)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|SwitchTable.EL2+msrttbr-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SwitchTabledotELtwoplusmsrttbreretN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SwitchTabledotELtwoplusmsrttbreretM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SwitchTabledotELtwoplusmsrttbreretO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SwitchTabledotELtwoplusmsrttbreretI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\SwitchTabledotELtwoplusmsrttbreretK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/SwitchTable.same-asid+eret.toml.tex <==
\newlength{\SwitchTabledotsameasidpluseretdottomlH}
\setlength{\SwitchTabledotsameasidpluseretdottomlH}{0cm}
\newsavebox{\SwitchTabledotsameasidpluseretdottomlI}
\begin{lrbox}{\SwitchTabledotsameasidpluseretdottomlI}
\begin{lstlisting}[language=AArch64,showlines=true]
MSR TTBR0_EL1,X0
ERET
L0:
LDR X1,[X2]
\end{lstlisting}
\end{lrbox}
\newlength{\SwitchTabledotsameasidpluseretdottomlJ}
\settowidth{\SwitchTabledotsameasidpluseretdottomlJ}{\usebox{\SwitchTabledotsameasidpluseretdottomlI}}
\addtolength{\SwitchTabledotsameasidpluseretdottomlH}{\SwitchTabledotsameasidpluseretdottomlJ}
\newsavebox{\SwitchTabledotsameasidpluseretdottomlK}
\begin{lrbox}{\SwitchTabledotsameasidpluseretdottomlK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X1,#1
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SwitchTabledotsameasidpluseretdottomlL}
\settowidth{\SwitchTabledotsameasidpluseretdottomlL}{\usebox{\SwitchTabledotsameasidpluseretdottomlK}}
\addtolength{\SwitchTabledotsameasidpluseretdottomlH}{\SwitchTabledotsameasidpluseretdottomlL}
\newsavebox{\SwitchTabledotsameasidpluseretdottomlM}
\begin{lrbox}{\SwitchTabledotsameasidpluseretdottomlM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    intermediate ipa1;
    physical pa1;

    *pa1 = 0;

    s1table table0 0x2C0000 {
        identity 0x1000 with code;
        x |-> pa1;
    };
    s1table table1 0x300000 {
        identity 0x1000 with code;
        x |-> invalid;
    };

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SwitchTabledotsameasidpluseretdottomlN}
\settowidth{\SwitchTabledotsameasidpluseretdottomlN}{\usebox{\SwitchTabledotsameasidpluseretdottomlM}}
\newsavebox{\SwitchTabledotsameasidpluseretdottomlO}
\begin{lrbox}{\SwitchTabledotsameasidpluseretdottomlO}
\begin{minipage}{\SwitchTabledotsameasidpluseretdottomlH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL1=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b1|\\
\lstinline[language=IslaLitmusExp]|R0=ttbr(asid=0x01,base=table1)|\\
\lstinline[language=IslaLitmusExp]|R2=x|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL1=0b00000|\\
\lstinline[language=IslaLitmusExp]|TTBR0_EL1=ttbr(asid=0x00,base=table0)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|SwitchTable.same-asid+eret.toml|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SwitchTabledotsameasidpluseretdottomlN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SwitchTabledotsameasidpluseretdottomlM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SwitchTabledotsameasidpluseretdottomlO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SwitchTabledotsameasidpluseretdottomlI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\SwitchTabledotsameasidpluseretdottomlK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R1=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/W+T.tex <==
\newlength{\WplusTH}
\setlength{\WplusTH}{0cm}
\newsavebox{\WplusTI}
\begin{lrbox}{\WplusTI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WplusTJ}
\settowidth{\WplusTJ}{\usebox{\WplusTI}}
\addtolength{\WplusTH}{\WplusTJ}
\newsavebox{\WplusTK}
\begin{lrbox}{\WplusTK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WplusTL}
\settowidth{\WplusTL}{\usebox{\WplusTK}}
\addtolength{\WplusTH}{\WplusTL}
\newsavebox{\WplusTM}
\begin{lrbox}{\WplusTM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1000:
MOV X0,#0
\end{lstlisting}
\end{lrbox}
\newlength{\WplusTN}
\settowidth{\WplusTN}{\usebox{\WplusTM}}
\addtolength{\WplusTH}{\WplusTN}
\newsavebox{\WplusTO}
\begin{lrbox}{\WplusTO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid at level 2;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WplusTP}
\settowidth{\WplusTP}{\usebox{\WplusTO}}
\newsavebox{\WplusTA}
\begin{lrbox}{\WplusTA}
\begin{minipage}{\WplusTH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte2(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|W+T|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WplusTP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WplusTO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WplusTA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WplusTI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WplusTK}\\
  \cline{2-2}
  & handler\\
  \cline{2-2}
  & \usebox{\WplusTM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|true|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/W.tex <==
\newlength{\WH}
\setlength{\WH}{0cm}
\newsavebox{\WI}
\begin{lrbox}{\WI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WJ}
\settowidth{\WJ}{\usebox{\WI}}
\addtolength{\WH}{\WJ}
\newsavebox{\WK}
\begin{lrbox}{\WK}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
\end{lstlisting}
\end{lrbox}
\newlength{\WL}
\settowidth{\WL}{\usebox{\WK}}
\newsavebox{\WM}
\begin{lrbox}{\WM}
\begin{minipage}{\WH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=x|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|W|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WL}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WK}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WM}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WI}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|true|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/WBM+dsb-tlbiis-dsb.tex <==
\newlength{\WBMplusdsbtlbiisdsbH}
\setlength{\WBMplusdsbtlbiisdsbH}{0cm}
\newsavebox{\WBMplusdsbtlbiisdsbI}
\begin{lrbox}{\WBMplusdsbtlbiisdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X5
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WBMplusdsbtlbiisdsbJ}
\settowidth{\WBMplusdsbtlbiisdsbJ}{\usebox{\WBMplusdsbtlbiisdsbI}}
\addtolength{\WBMplusdsbtlbiisdsbH}{\WBMplusdsbtlbiisdsbJ}
\newsavebox{\WBMplusdsbtlbiisdsbK}
\begin{lrbox}{\WBMplusdsbtlbiisdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WBMplusdsbtlbiisdsbL}
\settowidth{\WBMplusdsbtlbiisdsbL}{\usebox{\WBMplusdsbtlbiisdsbK}}
\addtolength{\WBMplusdsbtlbiisdsbH}{\WBMplusdsbtlbiisdsbL}
\newsavebox{\WBMplusdsbtlbiisdsbM}
\begin{lrbox}{\WBMplusdsbtlbiisdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WBMplusdsbtlbiisdsbN}
\settowidth{\WBMplusdsbtlbiisdsbN}{\usebox{\WBMplusdsbtlbiisdsbM}}
\addtolength{\WBMplusdsbtlbiisdsbH}{\WBMplusdsbtlbiisdsbN}
\newsavebox{\WBMplusdsbtlbiisdsbO}
\begin{lrbox}{\WBMplusdsbtlbiisdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    y |-> pa1;
    *pa1 = 0;
    x ?-> invalid;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WBMplusdsbtlbiisdsbP}
\settowidth{\WBMplusdsbtlbiisdsbP}{\usebox{\WBMplusdsbtlbiisdsbO}}
\newsavebox{\WBMplusdsbtlbiisdsbA}
\begin{lrbox}{\WBMplusdsbtlbiisdsbA}
\begin{minipage}{\WBMplusdsbtlbiisdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0x2|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R5=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:R0=0x1|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WBM+dsb-tlbiis-dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WBMplusdsbtlbiisdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WBMplusdsbtlbiisdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WBMplusdsbtlbiisdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WBMplusdsbtlbiisdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WBMplusdsbtlbiisdsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WBMplusdsbtlbiisdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|x=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/WDS+dsb-tlbiipa-dsb-eret-po.tex <==
\newlength{\WDSplusdsbtlbiipadsberetpoH}
\setlength{\WDSplusdsbtlbiipadsberetpoH}{0cm}
\newsavebox{\WDSplusdsbtlbiipadsberetpoI}
\begin{lrbox}{\WDSplusdsbtlbiipadsberetpoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1,X6
DSB SY
ERET
L0:
STR X2,[X3]
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\WDSplusdsbtlbiipadsberetpoJ}
\settowidth{\WDSplusdsbtlbiipadsberetpoJ}{\usebox{\WDSplusdsbtlbiipadsberetpoI}}
\addtolength{\WDSplusdsbtlbiipadsberetpoH}{\WDSplusdsbtlbiipadsberetpoJ}
\newsavebox{\WDSplusdsbtlbiipadsberetpoK}
\begin{lrbox}{\WDSplusdsbtlbiipadsberetpoK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1200:
MOV X4,#1
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WDSplusdsbtlbiipadsberetpoL}
\settowidth{\WDSplusdsbtlbiipadsberetpoL}{\usebox{\WDSplusdsbtlbiipadsberetpoK}}
\addtolength{\WDSplusdsbtlbiipadsberetpoH}{\WDSplusdsbtlbiipadsberetpoL}
\newsavebox{\WDSplusdsbtlbiipadsberetpoM}
\begin{lrbox}{\WDSplusdsbtlbiipadsberetpoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X4,#2
MRS X20,ELR_EL2
ADD X20,X20,#4
MSR ELR_EL2,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WDSplusdsbtlbiipadsberetpoN}
\settowidth{\WDSplusdsbtlbiipadsberetpoN}{\usebox{\WDSplusdsbtlbiipadsberetpoM}}
\addtolength{\WDSplusdsbtlbiipadsberetpoH}{\WDSplusdsbtlbiipadsberetpoN}
\newsavebox{\WDSplusdsbtlbiipadsberetpoO}
\begin{lrbox}{\WDSplusdsbtlbiipadsberetpoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;
    x ?-> invalid;

    ipa1 |-> pa1;
    ipa1 ?-> invalid;

    *pa1 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WDSplusdsbtlbiipadsberetpoP}
\settowidth{\WDSplusdsbtlbiipadsberetpoP}{\usebox{\WDSplusdsbtlbiipadsberetpoO}}
\newsavebox{\WDSplusdsbtlbiipadsberetpoA}
\begin{lrbox}{\WDSplusdsbtlbiipadsberetpoA}
\begin{minipage}{\WDSplusdsbtlbiipadsberetpoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R2=0b0|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R5=x|\\
\lstinline[language=IslaLitmusExp]|R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00100|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WDS+dsb-tlbiipa-dsb-eret-po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WDSplusdsbtlbiipadsberetpoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WDSplusdsbtlbiipadsberetpoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WDSplusdsbtlbiipadsberetpoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WDSplusdsbtlbiipadsberetpoI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\WDSplusdsbtlbiipadsberetpoK}\\
  \cline{2-2}
  & thread0 el2 handler lower exc\\
  \cline{2-2}
  & \usebox{\WDSplusdsbtlbiipadsberetpoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/WDS+po-dsb-tlbiipa-dsb-eret.tex <==
\newlength{\WDSpluspodsbtlbiipadsberetH}
\setlength{\WDSpluspodsbtlbiipadsberetH}{0cm}
\newsavebox{\WDSpluspodsbtlbiipadsberetI}
\begin{lrbox}{\WDSpluspodsbtlbiipadsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
STR X2,[X3]
DSB SY
TLBI IPAS2E1,X6
DSB SY
ERET
L0:
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsberetJ}
\settowidth{\WDSpluspodsbtlbiipadsberetJ}{\usebox{\WDSpluspodsbtlbiipadsberetI}}
\addtolength{\WDSpluspodsbtlbiipadsberetH}{\WDSpluspodsbtlbiipadsberetJ}
\newsavebox{\WDSpluspodsbtlbiipadsberetK}
\begin{lrbox}{\WDSpluspodsbtlbiipadsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1200:
MOV X4,#1
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsberetL}
\settowidth{\WDSpluspodsbtlbiipadsberetL}{\usebox{\WDSpluspodsbtlbiipadsberetK}}
\addtolength{\WDSpluspodsbtlbiipadsberetH}{\WDSpluspodsbtlbiipadsberetL}
\newsavebox{\WDSpluspodsbtlbiipadsberetM}
\begin{lrbox}{\WDSpluspodsbtlbiipadsberetM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X4,#2
MRS X20,ELR_EL2
ADD X20,X20,#4
MSR ELR_EL2,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsberetN}
\settowidth{\WDSpluspodsbtlbiipadsberetN}{\usebox{\WDSpluspodsbtlbiipadsberetM}}
\addtolength{\WDSpluspodsbtlbiipadsberetH}{\WDSpluspodsbtlbiipadsberetN}
\newsavebox{\WDSpluspodsbtlbiipadsberetO}
\begin{lrbox}{\WDSpluspodsbtlbiipadsberetO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;
    x ?-> invalid;

    ipa1 |-> pa1;
    ipa1 ?-> invalid;

    *pa1 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsberetP}
\settowidth{\WDSpluspodsbtlbiipadsberetP}{\usebox{\WDSpluspodsbtlbiipadsberetO}}
\newsavebox{\WDSpluspodsbtlbiipadsberetA}
\begin{lrbox}{\WDSpluspodsbtlbiipadsberetA}
\begin{minipage}{\WDSpluspodsbtlbiipadsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R2=0b0|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R5=x|\\
\lstinline[language=IslaLitmusExp]|R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00100|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WDS+po-dsb-tlbiipa-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WDSpluspodsbtlbiipadsberetP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WDSpluspodsbtlbiipadsberetO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WDSpluspodsbtlbiipadsberetA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsberetI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsberetK}\\
  \cline{2-2}
  & thread0 el2 handler lower exc\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsberetM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/WDS+po-dsb-tlbiipa-dsb-po-eret.tex <==
\newlength{\WDSpluspodsbtlbiipadsbpoeretH}
\setlength{\WDSpluspodsbtlbiipadsbpoeretH}{0cm}
\newsavebox{\WDSpluspodsbtlbiipadsbpoeretI}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbpoeretI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1,X6
DSB SY
STR X2,[X3]
ERET
L0:
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsbpoeretJ}
\settowidth{\WDSpluspodsbtlbiipadsbpoeretJ}{\usebox{\WDSpluspodsbtlbiipadsbpoeretI}}
\addtolength{\WDSpluspodsbtlbiipadsbpoeretH}{\WDSpluspodsbtlbiipadsbpoeretJ}
\newsavebox{\WDSpluspodsbtlbiipadsbpoeretK}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbpoeretK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1200:
MOV X4,#1
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsbpoeretL}
\settowidth{\WDSpluspodsbtlbiipadsbpoeretL}{\usebox{\WDSpluspodsbtlbiipadsbpoeretK}}
\addtolength{\WDSpluspodsbtlbiipadsbpoeretH}{\WDSpluspodsbtlbiipadsbpoeretL}
\newsavebox{\WDSpluspodsbtlbiipadsbpoeretM}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbpoeretM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X4,#2
MRS X20,ELR_EL2
ADD X20,X20,#4
MSR ELR_EL2,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsbpoeretN}
\settowidth{\WDSpluspodsbtlbiipadsbpoeretN}{\usebox{\WDSpluspodsbtlbiipadsbpoeretM}}
\addtolength{\WDSpluspodsbtlbiipadsbpoeretH}{\WDSpluspodsbtlbiipadsbpoeretN}
\newsavebox{\WDSpluspodsbtlbiipadsbpoeretO}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbpoeretO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;
    x ?-> invalid;

    ipa1 |-> pa1;
    ipa1 ?-> invalid;

    *pa1 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsbpoeretP}
\settowidth{\WDSpluspodsbtlbiipadsbpoeretP}{\usebox{\WDSpluspodsbtlbiipadsbpoeretO}}
\newsavebox{\WDSpluspodsbtlbiipadsbpoeretA}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbpoeretA}
\begin{minipage}{\WDSpluspodsbtlbiipadsbpoeretH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R2=0b0|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R5=x|\\
\lstinline[language=IslaLitmusExp]|R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00100|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WDS+po-dsb-tlbiipa-dsb-po-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WDSpluspodsbtlbiipadsbpoeretP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WDSpluspodsbtlbiipadsbpoeretO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WDSpluspodsbtlbiipadsbpoeretA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsbpoeretI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsbpoeretK}\\
  \cline{2-2}
  & thread0 el2 handler lower exc\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsbpoeretM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/WDS+po-dsb-tlbiipa-dsb-tlbiis-dsb-eret.tex <==
\newlength{\WDSpluspodsbtlbiipadsbtlbiisdsberetH}
\setlength{\WDSpluspodsbtlbiipadsbtlbiisdsberetH}{0cm}
\newsavebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetI}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbtlbiisdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
STR X2,[X3]
DSB SY
TLBI IPAS2E1,X6
DSB SY
TLBI VMALLE1IS
DSB SY
ERET
L0:
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsbtlbiisdsberetJ}
\settowidth{\WDSpluspodsbtlbiipadsbtlbiisdsberetJ}{\usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetI}}
\addtolength{\WDSpluspodsbtlbiipadsbtlbiisdsberetH}{\WDSpluspodsbtlbiipadsbtlbiisdsberetJ}
\newsavebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetK}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbtlbiisdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1200:
MOV X4,#1
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsbtlbiisdsberetL}
\settowidth{\WDSpluspodsbtlbiipadsbtlbiisdsberetL}{\usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetK}}
\addtolength{\WDSpluspodsbtlbiipadsbtlbiisdsberetH}{\WDSpluspodsbtlbiipadsbtlbiisdsberetL}
\newsavebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetM}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbtlbiisdsberetM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X4,#2
MRS X20,ELR_EL2
ADD X20,X20,#4
MSR ELR_EL2,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsbtlbiisdsberetN}
\settowidth{\WDSpluspodsbtlbiipadsbtlbiisdsberetN}{\usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetM}}
\addtolength{\WDSpluspodsbtlbiipadsbtlbiisdsberetH}{\WDSpluspodsbtlbiipadsbtlbiisdsberetN}
\newsavebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetO}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbtlbiisdsberetO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;
    x ?-> invalid;

    ipa1 |-> pa1;
    ipa1 ?-> invalid;

    *pa1 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsbtlbiisdsberetP}
\settowidth{\WDSpluspodsbtlbiipadsbtlbiisdsberetP}{\usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetO}}
\newsavebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetA}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbtlbiisdsberetA}
\begin{minipage}{\WDSpluspodsbtlbiipadsbtlbiisdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R2=0b0|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R5=x|\\
\lstinline[language=IslaLitmusExp]|R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00100|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WDS+po-dsb-tlbiipa-dsb-tlbiis-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WDSpluspodsbtlbiipadsbtlbiisdsberetP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetK}\\
  \cline{2-2}
  & thread0 el2 handler lower exc\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/WRC.RRTf.inv+addrs.tex <==
\newlength{\WRCdotRRTfdotinvplusaddrsH}
\setlength{\WRCdotRRTfdotinvplusaddrsH}{0cm}
\newsavebox{\WRCdotRRTfdotinvplusaddrsI}
\begin{lrbox}{\WRCdotRRTfdotinvplusaddrsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusaddrsJ}
\settowidth{\WRCdotRRTfdotinvplusaddrsJ}{\usebox{\WRCdotRRTfdotinvplusaddrsI}}
\addtolength{\WRCdotRRTfdotinvplusaddrsH}{\WRCdotRRTfdotinvplusaddrsJ}
\newsavebox{\WRCdotRRTfdotinvplusaddrsK}
\begin{lrbox}{\WRCdotRRTfdotinvplusaddrsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
STR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusaddrsL}
\settowidth{\WRCdotRRTfdotinvplusaddrsL}{\usebox{\WRCdotRRTfdotinvplusaddrsK}}
\addtolength{\WRCdotRRTfdotinvplusaddrsH}{\WRCdotRRTfdotinvplusaddrsL}
\newsavebox{\WRCdotRRTfdotinvplusaddrsM}
\begin{lrbox}{\WRCdotRRTfdotinvplusaddrsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusaddrsN}
\settowidth{\WRCdotRRTfdotinvplusaddrsN}{\usebox{\WRCdotRRTfdotinvplusaddrsM}}
\addtolength{\WRCdotRRTfdotinvplusaddrsH}{\WRCdotRRTfdotinvplusaddrsN}
\newsavebox{\WRCdotRRTfdotinvplusaddrsO}
\begin{lrbox}{\WRCdotRRTfdotinvplusaddrsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusaddrsP}
\settowidth{\WRCdotRRTfdotinvplusaddrsP}{\usebox{\WRCdotRRTfdotinvplusaddrsO}}
\addtolength{\WRCdotRRTfdotinvplusaddrsH}{\WRCdotRRTfdotinvplusaddrsP}
\newsavebox{\WRCdotRRTfdotinvplusaddrsA}
\begin{lrbox}{\WRCdotRRTfdotinvplusaddrsA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusaddrsB}
\settowidth{\WRCdotRRTfdotinvplusaddrsB}{\usebox{\WRCdotRRTfdotinvplusaddrsA}}
\newsavebox{\WRCdotRRTfdotinvplusaddrsC}
\begin{lrbox}{\WRCdotRRTfdotinvplusaddrsC}
\begin{minipage}{\WRCdotRRTfdotinvplusaddrsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.RRTf.inv+addrs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotRRTfdotinvplusaddrsB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotRRTfdotinvplusaddrsA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotRRTfdotinvplusaddrsC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusaddrsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusaddrsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusaddrsM}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusaddrsO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=desc3(z,page_table_base) & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/WRC.RRTf.inv+dmbs.tex <==
\newlength{\WRCdotRRTfdotinvplusdmbsH}
\setlength{\WRCdotRRTfdotinvplusdmbsH}{0cm}
\newsavebox{\WRCdotRRTfdotinvplusdmbsI}
\begin{lrbox}{\WRCdotRRTfdotinvplusdmbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdmbsJ}
\settowidth{\WRCdotRRTfdotinvplusdmbsJ}{\usebox{\WRCdotRRTfdotinvplusdmbsI}}
\addtolength{\WRCdotRRTfdotinvplusdmbsH}{\WRCdotRRTfdotinvplusdmbsJ}
\newsavebox{\WRCdotRRTfdotinvplusdmbsK}
\begin{lrbox}{\WRCdotRRTfdotinvplusdmbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdmbsL}
\settowidth{\WRCdotRRTfdotinvplusdmbsL}{\usebox{\WRCdotRRTfdotinvplusdmbsK}}
\addtolength{\WRCdotRRTfdotinvplusdmbsH}{\WRCdotRRTfdotinvplusdmbsL}
\newsavebox{\WRCdotRRTfdotinvplusdmbsM}
\begin{lrbox}{\WRCdotRRTfdotinvplusdmbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdmbsN}
\settowidth{\WRCdotRRTfdotinvplusdmbsN}{\usebox{\WRCdotRRTfdotinvplusdmbsM}}
\addtolength{\WRCdotRRTfdotinvplusdmbsH}{\WRCdotRRTfdotinvplusdmbsN}
\newsavebox{\WRCdotRRTfdotinvplusdmbsO}
\begin{lrbox}{\WRCdotRRTfdotinvplusdmbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdmbsP}
\settowidth{\WRCdotRRTfdotinvplusdmbsP}{\usebox{\WRCdotRRTfdotinvplusdmbsO}}
\addtolength{\WRCdotRRTfdotinvplusdmbsH}{\WRCdotRRTfdotinvplusdmbsP}
\newsavebox{\WRCdotRRTfdotinvplusdmbsA}
\begin{lrbox}{\WRCdotRRTfdotinvplusdmbsA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdmbsB}
\settowidth{\WRCdotRRTfdotinvplusdmbsB}{\usebox{\WRCdotRRTfdotinvplusdmbsA}}
\newsavebox{\WRCdotRRTfdotinvplusdmbsC}
\begin{lrbox}{\WRCdotRRTfdotinvplusdmbsC}
\begin{minipage}{\WRCdotRRTfdotinvplusdmbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.RRTf.inv+dmbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotRRTfdotinvplusdmbsB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotRRTfdotinvplusdmbsA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotRRTfdotinvplusdmbsC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdmbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdmbsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdmbsM}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdmbsO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=desc3(z,page_table_base) & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/WRC.RRTf.inv+dsb+ctrl-isb.tex <==
\newlength{\WRCdotRRTfdotinvplusdsbplusctrlisbH}
\setlength{\WRCdotRRTfdotinvplusdsbplusctrlisbH}{0cm}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusctrlisbI}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusctrlisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusctrlisbJ}
\settowidth{\WRCdotRRTfdotinvplusdsbplusctrlisbJ}{\usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbI}}
\addtolength{\WRCdotRRTfdotinvplusdsbplusctrlisbH}{\WRCdotRRTfdotinvplusdsbplusctrlisbJ}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusctrlisbK}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusctrlisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusctrlisbL}
\settowidth{\WRCdotRRTfdotinvplusdsbplusctrlisbL}{\usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbK}}
\addtolength{\WRCdotRRTfdotinvplusdsbplusctrlisbH}{\WRCdotRRTfdotinvplusdsbplusctrlisbL}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusctrlisbM}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusctrlisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBNZ X0,L0
L0:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusctrlisbN}
\settowidth{\WRCdotRRTfdotinvplusdsbplusctrlisbN}{\usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbM}}
\addtolength{\WRCdotRRTfdotinvplusdsbplusctrlisbH}{\WRCdotRRTfdotinvplusdsbplusctrlisbN}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusctrlisbO}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusctrlisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusctrlisbP}
\settowidth{\WRCdotRRTfdotinvplusdsbplusctrlisbP}{\usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbO}}
\addtolength{\WRCdotRRTfdotinvplusdsbplusctrlisbH}{\WRCdotRRTfdotinvplusdsbplusctrlisbP}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusctrlisbA}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusctrlisbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusctrlisbB}
\settowidth{\WRCdotRRTfdotinvplusdsbplusctrlisbB}{\usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbA}}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusctrlisbC}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusctrlisbC}
\begin{minipage}{\WRCdotRRTfdotinvplusdsbplusctrlisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.RRTf.inv+dsb+ctrl-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotRRTfdotinvplusdsbplusctrlisbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbM}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=desc3(z,page_table_base) & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/WRC.RRTf.inv+dsb+dsb-isb.tex <==
\newlength{\WRCdotRRTfdotinvplusdsbplusdsbisbH}
\setlength{\WRCdotRRTfdotinvplusdsbplusdsbisbH}{0cm}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusdsbisbI}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusdsbisbJ}
\settowidth{\WRCdotRRTfdotinvplusdsbplusdsbisbJ}{\usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbI}}
\addtolength{\WRCdotRRTfdotinvplusdsbplusdsbisbH}{\WRCdotRRTfdotinvplusdsbplusdsbisbJ}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusdsbisbK}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusdsbisbL}
\settowidth{\WRCdotRRTfdotinvplusdsbplusdsbisbL}{\usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbK}}
\addtolength{\WRCdotRRTfdotinvplusdsbplusdsbisbH}{\WRCdotRRTfdotinvplusdsbplusdsbisbL}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusdsbisbM}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusdsbisbN}
\settowidth{\WRCdotRRTfdotinvplusdsbplusdsbisbN}{\usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbM}}
\addtolength{\WRCdotRRTfdotinvplusdsbplusdsbisbH}{\WRCdotRRTfdotinvplusdsbplusdsbisbN}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusdsbisbO}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusdsbisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusdsbisbP}
\settowidth{\WRCdotRRTfdotinvplusdsbplusdsbisbP}{\usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbO}}
\addtolength{\WRCdotRRTfdotinvplusdsbplusdsbisbH}{\WRCdotRRTfdotinvplusdsbplusdsbisbP}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusdsbisbA}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusdsbisbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusdsbisbB}
\settowidth{\WRCdotRRTfdotinvplusdsbplusdsbisbB}{\usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbA}}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusdsbisbC}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusdsbisbC}
\begin{minipage}{\WRCdotRRTfdotinvplusdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.RRTf.inv+dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotRRTfdotinvplusdsbplusdsbisbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbM}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=desc3(z,page_table_base) & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/WRC.RRTf.inv+dsbs.tex <==
\newlength{\WRCdotRRTfdotinvplusdsbsH}
\setlength{\WRCdotRRTfdotinvplusdsbsH}{0cm}
\newsavebox{\WRCdotRRTfdotinvplusdsbsI}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbsJ}
\settowidth{\WRCdotRRTfdotinvplusdsbsJ}{\usebox{\WRCdotRRTfdotinvplusdsbsI}}
\addtolength{\WRCdotRRTfdotinvplusdsbsH}{\WRCdotRRTfdotinvplusdsbsJ}
\newsavebox{\WRCdotRRTfdotinvplusdsbsK}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbsL}
\settowidth{\WRCdotRRTfdotinvplusdsbsL}{\usebox{\WRCdotRRTfdotinvplusdsbsK}}
\addtolength{\WRCdotRRTfdotinvplusdsbsH}{\WRCdotRRTfdotinvplusdsbsL}
\newsavebox{\WRCdotRRTfdotinvplusdsbsM}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbsN}
\settowidth{\WRCdotRRTfdotinvplusdsbsN}{\usebox{\WRCdotRRTfdotinvplusdsbsM}}
\addtolength{\WRCdotRRTfdotinvplusdsbsH}{\WRCdotRRTfdotinvplusdsbsN}
\newsavebox{\WRCdotRRTfdotinvplusdsbsO}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbsP}
\settowidth{\WRCdotRRTfdotinvplusdsbsP}{\usebox{\WRCdotRRTfdotinvplusdsbsO}}
\addtolength{\WRCdotRRTfdotinvplusdsbsH}{\WRCdotRRTfdotinvplusdsbsP}
\newsavebox{\WRCdotRRTfdotinvplusdsbsA}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbsA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbsB}
\settowidth{\WRCdotRRTfdotinvplusdsbsB}{\usebox{\WRCdotRRTfdotinvplusdsbsA}}
\newsavebox{\WRCdotRRTfdotinvplusdsbsC}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbsC}
\begin{minipage}{\WRCdotRRTfdotinvplusdsbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.RRTf.inv+dsbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotRRTfdotinvplusdsbsB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotRRTfdotinvplusdsbsA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotRRTfdotinvplusdsbsC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbsM}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbsO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=desc3(z,page_table_base) & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/WRC.RRTf.inv+pos.tex <==
\newlength{\WRCdotRRTfdotinvplusposH}
\setlength{\WRCdotRRTfdotinvplusposH}{0cm}
\newsavebox{\WRCdotRRTfdotinvplusposI}
\begin{lrbox}{\WRCdotRRTfdotinvplusposI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusposJ}
\settowidth{\WRCdotRRTfdotinvplusposJ}{\usebox{\WRCdotRRTfdotinvplusposI}}
\addtolength{\WRCdotRRTfdotinvplusposH}{\WRCdotRRTfdotinvplusposJ}
\newsavebox{\WRCdotRRTfdotinvplusposK}
\begin{lrbox}{\WRCdotRRTfdotinvplusposK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusposL}
\settowidth{\WRCdotRRTfdotinvplusposL}{\usebox{\WRCdotRRTfdotinvplusposK}}
\addtolength{\WRCdotRRTfdotinvplusposH}{\WRCdotRRTfdotinvplusposL}
\newsavebox{\WRCdotRRTfdotinvplusposM}
\begin{lrbox}{\WRCdotRRTfdotinvplusposM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusposN}
\settowidth{\WRCdotRRTfdotinvplusposN}{\usebox{\WRCdotRRTfdotinvplusposM}}
\addtolength{\WRCdotRRTfdotinvplusposH}{\WRCdotRRTfdotinvplusposN}
\newsavebox{\WRCdotRRTfdotinvplusposO}
\begin{lrbox}{\WRCdotRRTfdotinvplusposO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusposP}
\settowidth{\WRCdotRRTfdotinvplusposP}{\usebox{\WRCdotRRTfdotinvplusposO}}
\addtolength{\WRCdotRRTfdotinvplusposH}{\WRCdotRRTfdotinvplusposP}
\newsavebox{\WRCdotRRTfdotinvplusposA}
\begin{lrbox}{\WRCdotRRTfdotinvplusposA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusposB}
\settowidth{\WRCdotRRTfdotinvplusposB}{\usebox{\WRCdotRRTfdotinvplusposA}}
\newsavebox{\WRCdotRRTfdotinvplusposC}
\begin{lrbox}{\WRCdotRRTfdotinvplusposC}
\begin{minipage}{\WRCdotRRTfdotinvplusposH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.RRTf.inv+pos|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotRRTfdotinvplusposB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotRRTfdotinvplusposA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotRRTfdotinvplusposC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusposI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusposK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusposM}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusposO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=desc3(z,page_table_base) & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/WRC.TRTf.inv+addrs.tex <==
\newlength{\WRCdotTRTfdotinvplusaddrsH}
\setlength{\WRCdotTRTfdotinvplusaddrsH}{0cm}
\newsavebox{\WRCdotTRTfdotinvplusaddrsI}
\begin{lrbox}{\WRCdotTRTfdotinvplusaddrsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusaddrsJ}
\settowidth{\WRCdotTRTfdotinvplusaddrsJ}{\usebox{\WRCdotTRTfdotinvplusaddrsI}}
\addtolength{\WRCdotTRTfdotinvplusaddrsH}{\WRCdotTRTfdotinvplusaddrsJ}
\newsavebox{\WRCdotTRTfdotinvplusaddrsK}
\begin{lrbox}{\WRCdotTRTfdotinvplusaddrsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
STR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusaddrsL}
\settowidth{\WRCdotTRTfdotinvplusaddrsL}{\usebox{\WRCdotTRTfdotinvplusaddrsK}}
\addtolength{\WRCdotTRTfdotinvplusaddrsH}{\WRCdotTRTfdotinvplusaddrsL}
\newsavebox{\WRCdotTRTfdotinvplusaddrsM}
\begin{lrbox}{\WRCdotTRTfdotinvplusaddrsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusaddrsN}
\settowidth{\WRCdotTRTfdotinvplusaddrsN}{\usebox{\WRCdotTRTfdotinvplusaddrsM}}
\addtolength{\WRCdotTRTfdotinvplusaddrsH}{\WRCdotTRTfdotinvplusaddrsN}
\newsavebox{\WRCdotTRTfdotinvplusaddrsO}
\begin{lrbox}{\WRCdotTRTfdotinvplusaddrsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusaddrsP}
\settowidth{\WRCdotTRTfdotinvplusaddrsP}{\usebox{\WRCdotTRTfdotinvplusaddrsO}}
\addtolength{\WRCdotTRTfdotinvplusaddrsH}{\WRCdotTRTfdotinvplusaddrsP}
\newsavebox{\WRCdotTRTfdotinvplusaddrsA}
\begin{lrbox}{\WRCdotTRTfdotinvplusaddrsA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusaddrsB}
\settowidth{\WRCdotTRTfdotinvplusaddrsB}{\usebox{\WRCdotTRTfdotinvplusaddrsA}}
\addtolength{\WRCdotTRTfdotinvplusaddrsH}{\WRCdotTRTfdotinvplusaddrsB}
\newsavebox{\WRCdotTRTfdotinvplusaddrsC}
\begin{lrbox}{\WRCdotTRTfdotinvplusaddrsC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusaddrsD}
\settowidth{\WRCdotTRTfdotinvplusaddrsD}{\usebox{\WRCdotTRTfdotinvplusaddrsC}}
\newsavebox{\WRCdotTRTfdotinvplusaddrsE}
\begin{lrbox}{\WRCdotTRTfdotinvplusaddrsE}
\begin{minipage}{\WRCdotTRTfdotinvplusaddrsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TRTf.inv+addrs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTRTfdotinvplusaddrsD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTRTfdotinvplusaddrsC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTRTfdotinvplusaddrsE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusaddrsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusaddrsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusaddrsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusaddrsO}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusaddrsA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/WRC.TRTf.inv+dmbs.tex <==
\newlength{\WRCdotTRTfdotinvplusdmbsH}
\setlength{\WRCdotTRTfdotinvplusdmbsH}{0cm}
\newsavebox{\WRCdotTRTfdotinvplusdmbsI}
\begin{lrbox}{\WRCdotTRTfdotinvplusdmbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdmbsJ}
\settowidth{\WRCdotTRTfdotinvplusdmbsJ}{\usebox{\WRCdotTRTfdotinvplusdmbsI}}
\addtolength{\WRCdotTRTfdotinvplusdmbsH}{\WRCdotTRTfdotinvplusdmbsJ}
\newsavebox{\WRCdotTRTfdotinvplusdmbsK}
\begin{lrbox}{\WRCdotTRTfdotinvplusdmbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdmbsL}
\settowidth{\WRCdotTRTfdotinvplusdmbsL}{\usebox{\WRCdotTRTfdotinvplusdmbsK}}
\addtolength{\WRCdotTRTfdotinvplusdmbsH}{\WRCdotTRTfdotinvplusdmbsL}
\newsavebox{\WRCdotTRTfdotinvplusdmbsM}
\begin{lrbox}{\WRCdotTRTfdotinvplusdmbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdmbsN}
\settowidth{\WRCdotTRTfdotinvplusdmbsN}{\usebox{\WRCdotTRTfdotinvplusdmbsM}}
\addtolength{\WRCdotTRTfdotinvplusdmbsH}{\WRCdotTRTfdotinvplusdmbsN}
\newsavebox{\WRCdotTRTfdotinvplusdmbsO}
\begin{lrbox}{\WRCdotTRTfdotinvplusdmbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdmbsP}
\settowidth{\WRCdotTRTfdotinvplusdmbsP}{\usebox{\WRCdotTRTfdotinvplusdmbsO}}
\addtolength{\WRCdotTRTfdotinvplusdmbsH}{\WRCdotTRTfdotinvplusdmbsP}
\newsavebox{\WRCdotTRTfdotinvplusdmbsA}
\begin{lrbox}{\WRCdotTRTfdotinvplusdmbsA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdmbsB}
\settowidth{\WRCdotTRTfdotinvplusdmbsB}{\usebox{\WRCdotTRTfdotinvplusdmbsA}}
\addtolength{\WRCdotTRTfdotinvplusdmbsH}{\WRCdotTRTfdotinvplusdmbsB}
\newsavebox{\WRCdotTRTfdotinvplusdmbsC}
\begin{lrbox}{\WRCdotTRTfdotinvplusdmbsC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdmbsD}
\settowidth{\WRCdotTRTfdotinvplusdmbsD}{\usebox{\WRCdotTRTfdotinvplusdmbsC}}
\newsavebox{\WRCdotTRTfdotinvplusdmbsE}
\begin{lrbox}{\WRCdotTRTfdotinvplusdmbsE}
\begin{minipage}{\WRCdotTRTfdotinvplusdmbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TRTf.inv+dmbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTRTfdotinvplusdmbsD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTRTfdotinvplusdmbsC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTRTfdotinvplusdmbsE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdmbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdmbsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdmbsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdmbsO}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdmbsA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/WRC.TRTf.inv+dsb+dsb-isb.tex <==
\newlength{\WRCdotTRTfdotinvplusdsbplusdsbisbH}
\setlength{\WRCdotTRTfdotinvplusdsbplusdsbisbH}{0cm}
\newsavebox{\WRCdotTRTfdotinvplusdsbplusdsbisbI}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbplusdsbisbJ}
\settowidth{\WRCdotTRTfdotinvplusdsbplusdsbisbJ}{\usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbI}}
\addtolength{\WRCdotTRTfdotinvplusdsbplusdsbisbH}{\WRCdotTRTfdotinvplusdsbplusdsbisbJ}
\newsavebox{\WRCdotTRTfdotinvplusdsbplusdsbisbK}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbplusdsbisbL}
\settowidth{\WRCdotTRTfdotinvplusdsbplusdsbisbL}{\usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbK}}
\addtolength{\WRCdotTRTfdotinvplusdsbplusdsbisbH}{\WRCdotTRTfdotinvplusdsbplusdsbisbL}
\newsavebox{\WRCdotTRTfdotinvplusdsbplusdsbisbM}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbplusdsbisbN}
\settowidth{\WRCdotTRTfdotinvplusdsbplusdsbisbN}{\usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbM}}
\addtolength{\WRCdotTRTfdotinvplusdsbplusdsbisbH}{\WRCdotTRTfdotinvplusdsbplusdsbisbN}
\newsavebox{\WRCdotTRTfdotinvplusdsbplusdsbisbO}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbplusdsbisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbplusdsbisbP}
\settowidth{\WRCdotTRTfdotinvplusdsbplusdsbisbP}{\usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbO}}
\addtolength{\WRCdotTRTfdotinvplusdsbplusdsbisbH}{\WRCdotTRTfdotinvplusdsbplusdsbisbP}
\newsavebox{\WRCdotTRTfdotinvplusdsbplusdsbisbA}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbplusdsbisbA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbplusdsbisbB}
\settowidth{\WRCdotTRTfdotinvplusdsbplusdsbisbB}{\usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbA}}
\addtolength{\WRCdotTRTfdotinvplusdsbplusdsbisbH}{\WRCdotTRTfdotinvplusdsbplusdsbisbB}
\newsavebox{\WRCdotTRTfdotinvplusdsbplusdsbisbC}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbplusdsbisbC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbplusdsbisbD}
\settowidth{\WRCdotTRTfdotinvplusdsbplusdsbisbD}{\usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbC}}
\newsavebox{\WRCdotTRTfdotinvplusdsbplusdsbisbE}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbplusdsbisbE}
\begin{minipage}{\WRCdotTRTfdotinvplusdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TRTf.inv+dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTRTfdotinvplusdsbplusdsbisbD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbO}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/WRC.TRTf.inv+dsbs.tex <==
\newlength{\WRCdotTRTfdotinvplusdsbsH}
\setlength{\WRCdotTRTfdotinvplusdsbsH}{0cm}
\newsavebox{\WRCdotTRTfdotinvplusdsbsI}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbsJ}
\settowidth{\WRCdotTRTfdotinvplusdsbsJ}{\usebox{\WRCdotTRTfdotinvplusdsbsI}}
\addtolength{\WRCdotTRTfdotinvplusdsbsH}{\WRCdotTRTfdotinvplusdsbsJ}
\newsavebox{\WRCdotTRTfdotinvplusdsbsK}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbsL}
\settowidth{\WRCdotTRTfdotinvplusdsbsL}{\usebox{\WRCdotTRTfdotinvplusdsbsK}}
\addtolength{\WRCdotTRTfdotinvplusdsbsH}{\WRCdotTRTfdotinvplusdsbsL}
\newsavebox{\WRCdotTRTfdotinvplusdsbsM}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbsN}
\settowidth{\WRCdotTRTfdotinvplusdsbsN}{\usebox{\WRCdotTRTfdotinvplusdsbsM}}
\addtolength{\WRCdotTRTfdotinvplusdsbsH}{\WRCdotTRTfdotinvplusdsbsN}
\newsavebox{\WRCdotTRTfdotinvplusdsbsO}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbsP}
\settowidth{\WRCdotTRTfdotinvplusdsbsP}{\usebox{\WRCdotTRTfdotinvplusdsbsO}}
\addtolength{\WRCdotTRTfdotinvplusdsbsH}{\WRCdotTRTfdotinvplusdsbsP}
\newsavebox{\WRCdotTRTfdotinvplusdsbsA}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbsA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbsB}
\settowidth{\WRCdotTRTfdotinvplusdsbsB}{\usebox{\WRCdotTRTfdotinvplusdsbsA}}
\addtolength{\WRCdotTRTfdotinvplusdsbsH}{\WRCdotTRTfdotinvplusdsbsB}
\newsavebox{\WRCdotTRTfdotinvplusdsbsC}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbsC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbsD}
\settowidth{\WRCdotTRTfdotinvplusdsbsD}{\usebox{\WRCdotTRTfdotinvplusdsbsC}}
\newsavebox{\WRCdotTRTfdotinvplusdsbsE}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbsE}
\begin{minipage}{\WRCdotTRTfdotinvplusdsbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TRTf.inv+dsbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTRTfdotinvplusdsbsD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTRTfdotinvplusdsbsC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTRTfdotinvplusdsbsE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbsO}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbsA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/WRC.TRTf.inv+pos.tex <==
\newlength{\WRCdotTRTfdotinvplusposH}
\setlength{\WRCdotTRTfdotinvplusposH}{0cm}
\newsavebox{\WRCdotTRTfdotinvplusposI}
\begin{lrbox}{\WRCdotTRTfdotinvplusposI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusposJ}
\settowidth{\WRCdotTRTfdotinvplusposJ}{\usebox{\WRCdotTRTfdotinvplusposI}}
\addtolength{\WRCdotTRTfdotinvplusposH}{\WRCdotTRTfdotinvplusposJ}
\newsavebox{\WRCdotTRTfdotinvplusposK}
\begin{lrbox}{\WRCdotTRTfdotinvplusposK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusposL}
\settowidth{\WRCdotTRTfdotinvplusposL}{\usebox{\WRCdotTRTfdotinvplusposK}}
\addtolength{\WRCdotTRTfdotinvplusposH}{\WRCdotTRTfdotinvplusposL}
\newsavebox{\WRCdotTRTfdotinvplusposM}
\begin{lrbox}{\WRCdotTRTfdotinvplusposM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusposN}
\settowidth{\WRCdotTRTfdotinvplusposN}{\usebox{\WRCdotTRTfdotinvplusposM}}
\addtolength{\WRCdotTRTfdotinvplusposH}{\WRCdotTRTfdotinvplusposN}
\newsavebox{\WRCdotTRTfdotinvplusposO}
\begin{lrbox}{\WRCdotTRTfdotinvplusposO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusposP}
\settowidth{\WRCdotTRTfdotinvplusposP}{\usebox{\WRCdotTRTfdotinvplusposO}}
\addtolength{\WRCdotTRTfdotinvplusposH}{\WRCdotTRTfdotinvplusposP}
\newsavebox{\WRCdotTRTfdotinvplusposA}
\begin{lrbox}{\WRCdotTRTfdotinvplusposA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusposB}
\settowidth{\WRCdotTRTfdotinvplusposB}{\usebox{\WRCdotTRTfdotinvplusposA}}
\addtolength{\WRCdotTRTfdotinvplusposH}{\WRCdotTRTfdotinvplusposB}
\newsavebox{\WRCdotTRTfdotinvplusposC}
\begin{lrbox}{\WRCdotTRTfdotinvplusposC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusposD}
\settowidth{\WRCdotTRTfdotinvplusposD}{\usebox{\WRCdotTRTfdotinvplusposC}}
\newsavebox{\WRCdotTRTfdotinvplusposE}
\begin{lrbox}{\WRCdotTRTfdotinvplusposE}
\begin{minipage}{\WRCdotTRTfdotinvplusposH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TRTf.inv+pos|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTRTfdotinvplusposD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTRTfdotinvplusposC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTRTfdotinvplusposE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusposI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusposK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusposM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusposO}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusposA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/WRC.TTTf.inv+addrs.tex <==
\newlength{\WRCdotTTTfdotinvplusaddrsH}
\setlength{\WRCdotTTTfdotinvplusaddrsH}{0cm}
\newsavebox{\WRCdotTTTfdotinvplusaddrsI}
\begin{lrbox}{\WRCdotTTTfdotinvplusaddrsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusaddrsJ}
\settowidth{\WRCdotTTTfdotinvplusaddrsJ}{\usebox{\WRCdotTTTfdotinvplusaddrsI}}
\addtolength{\WRCdotTTTfdotinvplusaddrsH}{\WRCdotTTTfdotinvplusaddrsJ}
\newsavebox{\WRCdotTTTfdotinvplusaddrsK}
\begin{lrbox}{\WRCdotTTTfdotinvplusaddrsK}
\begin{lstlisting}[language=AArch64,showlines=true]
MOV X0,#0
LDR X0,[X1]
EOR X4,X0,X0
STR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusaddrsL}
\settowidth{\WRCdotTTTfdotinvplusaddrsL}{\usebox{\WRCdotTTTfdotinvplusaddrsK}}
\addtolength{\WRCdotTTTfdotinvplusaddrsH}{\WRCdotTTTfdotinvplusaddrsL}
\newsavebox{\WRCdotTTTfdotinvplusaddrsM}
\begin{lrbox}{\WRCdotTTTfdotinvplusaddrsM}
\begin{lstlisting}[language=AArch64,showlines=true]
MOV X0,#0
LDR X0,[X1]
EOR X4,X0,X0
MOV X2,#0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusaddrsN}
\settowidth{\WRCdotTTTfdotinvplusaddrsN}{\usebox{\WRCdotTTTfdotinvplusaddrsM}}
\addtolength{\WRCdotTTTfdotinvplusaddrsH}{\WRCdotTTTfdotinvplusaddrsN}
\newsavebox{\WRCdotTTTfdotinvplusaddrsO}
\begin{lrbox}{\WRCdotTTTfdotinvplusaddrsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusaddrsP}
\settowidth{\WRCdotTTTfdotinvplusaddrsP}{\usebox{\WRCdotTTTfdotinvplusaddrsO}}
\addtolength{\WRCdotTTTfdotinvplusaddrsH}{\WRCdotTTTfdotinvplusaddrsP}
\newsavebox{\WRCdotTTTfdotinvplusaddrsA}
\begin{lrbox}{\WRCdotTTTfdotinvplusaddrsA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusaddrsB}
\settowidth{\WRCdotTTTfdotinvplusaddrsB}{\usebox{\WRCdotTTTfdotinvplusaddrsA}}
\addtolength{\WRCdotTTTfdotinvplusaddrsH}{\WRCdotTTTfdotinvplusaddrsB}
\newsavebox{\WRCdotTTTfdotinvplusaddrsC}
\begin{lrbox}{\WRCdotTTTfdotinvplusaddrsC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusaddrsD}
\settowidth{\WRCdotTTTfdotinvplusaddrsD}{\usebox{\WRCdotTTTfdotinvplusaddrsC}}
\newsavebox{\WRCdotTTTfdotinvplusaddrsE}
\begin{lrbox}{\WRCdotTTTfdotinvplusaddrsE}
\begin{minipage}{\WRCdotTTTfdotinvplusaddrsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:__isla_monomorphize_writes=true|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TTTf.inv+addrs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTTTfdotinvplusaddrsD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTTTfdotinvplusaddrsC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTTTfdotinvplusaddrsE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusaddrsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusaddrsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusaddrsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusaddrsO}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusaddrsA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/WRC.TTTf.inv+data+addr.tex <==
\newlength{\WRCdotTTTfdotinvplusdataplusaddrH}
\setlength{\WRCdotTTTfdotinvplusdataplusaddrH}{0cm}
\newsavebox{\WRCdotTTTfdotinvplusdataplusaddrI}
\begin{lrbox}{\WRCdotTTTfdotinvplusdataplusaddrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusdataplusaddrJ}
\settowidth{\WRCdotTTTfdotinvplusdataplusaddrJ}{\usebox{\WRCdotTTTfdotinvplusdataplusaddrI}}
\addtolength{\WRCdotTTTfdotinvplusdataplusaddrH}{\WRCdotTTTfdotinvplusdataplusaddrJ}
\newsavebox{\WRCdotTTTfdotinvplusdataplusaddrK}
\begin{lrbox}{\WRCdotTTTfdotinvplusdataplusaddrK}
\begin{lstlisting}[language=AArch64,showlines=true]
MOV X0,#0
LDR X0,[X1]
EOR X4,X0,X0
ORR X2,X2,X4
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusdataplusaddrL}
\settowidth{\WRCdotTTTfdotinvplusdataplusaddrL}{\usebox{\WRCdotTTTfdotinvplusdataplusaddrK}}
\addtolength{\WRCdotTTTfdotinvplusdataplusaddrH}{\WRCdotTTTfdotinvplusdataplusaddrL}
\newsavebox{\WRCdotTTTfdotinvplusdataplusaddrM}
\begin{lrbox}{\WRCdotTTTfdotinvplusdataplusaddrM}
\begin{lstlisting}[language=AArch64,showlines=true]
MOV X0,#0
LDR X0,[X1]
EOR X4,X0,X0
MOV X2,#0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusdataplusaddrN}
\settowidth{\WRCdotTTTfdotinvplusdataplusaddrN}{\usebox{\WRCdotTTTfdotinvplusdataplusaddrM}}
\addtolength{\WRCdotTTTfdotinvplusdataplusaddrH}{\WRCdotTTTfdotinvplusdataplusaddrN}
\newsavebox{\WRCdotTTTfdotinvplusdataplusaddrO}
\begin{lrbox}{\WRCdotTTTfdotinvplusdataplusaddrO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusdataplusaddrP}
\settowidth{\WRCdotTTTfdotinvplusdataplusaddrP}{\usebox{\WRCdotTTTfdotinvplusdataplusaddrO}}
\addtolength{\WRCdotTTTfdotinvplusdataplusaddrH}{\WRCdotTTTfdotinvplusdataplusaddrP}
\newsavebox{\WRCdotTTTfdotinvplusdataplusaddrA}
\begin{lrbox}{\WRCdotTTTfdotinvplusdataplusaddrA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusdataplusaddrB}
\settowidth{\WRCdotTTTfdotinvplusdataplusaddrB}{\usebox{\WRCdotTTTfdotinvplusdataplusaddrA}}
\addtolength{\WRCdotTTTfdotinvplusdataplusaddrH}{\WRCdotTTTfdotinvplusdataplusaddrB}
\newsavebox{\WRCdotTTTfdotinvplusdataplusaddrC}
\begin{lrbox}{\WRCdotTTTfdotinvplusdataplusaddrC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusdataplusaddrD}
\settowidth{\WRCdotTTTfdotinvplusdataplusaddrD}{\usebox{\WRCdotTTTfdotinvplusdataplusaddrC}}
\newsavebox{\WRCdotTTTfdotinvplusdataplusaddrE}
\begin{lrbox}{\WRCdotTTTfdotinvplusdataplusaddrE}
\begin{minipage}{\WRCdotTTTfdotinvplusdataplusaddrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:__isla_monomorphize_writes=true|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TTTf.inv+data+addr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTTTfdotinvplusdataplusaddrD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTTTfdotinvplusdataplusaddrC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTTTfdotinvplusdataplusaddrE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusdataplusaddrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusdataplusaddrK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusdataplusaddrM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusdataplusaddrO}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusdataplusaddrA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/WRC.TfRR+ctrl-isb+dsb.tex <==
\newlength{\WRCdotTfRRplusctrlisbplusdsbH}
\setlength{\WRCdotTfRRplusctrlisbplusdsbH}{0cm}
\newsavebox{\WRCdotTfRRplusctrlisbplusdsbI}
\begin{lrbox}{\WRCdotTfRRplusctrlisbplusdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusctrlisbplusdsbJ}
\settowidth{\WRCdotTfRRplusctrlisbplusdsbJ}{\usebox{\WRCdotTfRRplusctrlisbplusdsbI}}
\addtolength{\WRCdotTfRRplusctrlisbplusdsbH}{\WRCdotTfRRplusctrlisbplusdsbJ}
\newsavebox{\WRCdotTfRRplusctrlisbplusdsbK}
\begin{lrbox}{\WRCdotTfRRplusctrlisbplusdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBNZ X0,L0
L0:
ISB
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusctrlisbplusdsbL}
\settowidth{\WRCdotTfRRplusctrlisbplusdsbL}{\usebox{\WRCdotTfRRplusctrlisbplusdsbK}}
\addtolength{\WRCdotTfRRplusctrlisbplusdsbH}{\WRCdotTfRRplusctrlisbplusdsbL}
\newsavebox{\WRCdotTfRRplusctrlisbplusdsbM}
\begin{lrbox}{\WRCdotTfRRplusctrlisbplusdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusctrlisbplusdsbN}
\settowidth{\WRCdotTfRRplusctrlisbplusdsbN}{\usebox{\WRCdotTfRRplusctrlisbplusdsbM}}
\addtolength{\WRCdotTfRRplusctrlisbplusdsbH}{\WRCdotTfRRplusctrlisbplusdsbN}
\newsavebox{\WRCdotTfRRplusctrlisbplusdsbO}
\begin{lrbox}{\WRCdotTfRRplusctrlisbplusdsbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusctrlisbplusdsbP}
\settowidth{\WRCdotTfRRplusctrlisbplusdsbP}{\usebox{\WRCdotTfRRplusctrlisbplusdsbO}}
\addtolength{\WRCdotTfRRplusctrlisbplusdsbH}{\WRCdotTfRRplusctrlisbplusdsbP}
\newsavebox{\WRCdotTfRRplusctrlisbplusdsbA}
\begin{lrbox}{\WRCdotTfRRplusctrlisbplusdsbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    *pa1 = 0;

    y |-> pa2;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusctrlisbplusdsbB}
\settowidth{\WRCdotTfRRplusctrlisbplusdsbB}{\usebox{\WRCdotTfRRplusctrlisbplusdsbA}}
\newsavebox{\WRCdotTfRRplusctrlisbplusdsbC}
\begin{lrbox}{\WRCdotTfRRplusctrlisbplusdsbC}
\begin{minipage}{\WRCdotTfRRplusctrlisbplusdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TfRR+ctrl-isb+dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTfRRplusctrlisbplusdsbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTfRRplusctrlisbplusdsbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTfRRplusctrlisbplusdsbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusctrlisbplusdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusctrlisbplusdsbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusctrlisbplusdsbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusctrlisbplusdsbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & ~2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/WRC.TfRR+dmbs.tex <==
\newlength{\WRCdotTfRRplusdmbsH}
\setlength{\WRCdotTfRRplusdmbsH}{0cm}
\newsavebox{\WRCdotTfRRplusdmbsI}
\begin{lrbox}{\WRCdotTfRRplusdmbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdmbsJ}
\settowidth{\WRCdotTfRRplusdmbsJ}{\usebox{\WRCdotTfRRplusdmbsI}}
\addtolength{\WRCdotTfRRplusdmbsH}{\WRCdotTfRRplusdmbsJ}
\newsavebox{\WRCdotTfRRplusdmbsK}
\begin{lrbox}{\WRCdotTfRRplusdmbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdmbsL}
\settowidth{\WRCdotTfRRplusdmbsL}{\usebox{\WRCdotTfRRplusdmbsK}}
\addtolength{\WRCdotTfRRplusdmbsH}{\WRCdotTfRRplusdmbsL}
\newsavebox{\WRCdotTfRRplusdmbsM}
\begin{lrbox}{\WRCdotTfRRplusdmbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdmbsN}
\settowidth{\WRCdotTfRRplusdmbsN}{\usebox{\WRCdotTfRRplusdmbsM}}
\addtolength{\WRCdotTfRRplusdmbsH}{\WRCdotTfRRplusdmbsN}
\newsavebox{\WRCdotTfRRplusdmbsO}
\begin{lrbox}{\WRCdotTfRRplusdmbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdmbsP}
\settowidth{\WRCdotTfRRplusdmbsP}{\usebox{\WRCdotTfRRplusdmbsO}}
\addtolength{\WRCdotTfRRplusdmbsH}{\WRCdotTfRRplusdmbsP}
\newsavebox{\WRCdotTfRRplusdmbsA}
\begin{lrbox}{\WRCdotTfRRplusdmbsA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    *pa1 = 0;

    y |-> pa2;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdmbsB}
\settowidth{\WRCdotTfRRplusdmbsB}{\usebox{\WRCdotTfRRplusdmbsA}}
\newsavebox{\WRCdotTfRRplusdmbsC}
\begin{lrbox}{\WRCdotTfRRplusdmbsC}
\begin{minipage}{\WRCdotTfRRplusdmbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TfRR+dmbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTfRRplusdmbsB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTfRRplusdmbsA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTfRRplusdmbsC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdmbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdmbsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdmbsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdmbsO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & ~2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/WRC.TfRR+dsb-isb+dsb.tex <==
\newlength{\WRCdotTfRRplusdsbisbplusdsbH}
\setlength{\WRCdotTfRRplusdsbisbplusdsbH}{0cm}
\newsavebox{\WRCdotTfRRplusdsbisbplusdsbI}
\begin{lrbox}{\WRCdotTfRRplusdsbisbplusdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbisbplusdsbJ}
\settowidth{\WRCdotTfRRplusdsbisbplusdsbJ}{\usebox{\WRCdotTfRRplusdsbisbplusdsbI}}
\addtolength{\WRCdotTfRRplusdsbisbplusdsbH}{\WRCdotTfRRplusdsbisbplusdsbJ}
\newsavebox{\WRCdotTfRRplusdsbisbplusdsbK}
\begin{lrbox}{\WRCdotTfRRplusdsbisbplusdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbisbplusdsbL}
\settowidth{\WRCdotTfRRplusdsbisbplusdsbL}{\usebox{\WRCdotTfRRplusdsbisbplusdsbK}}
\addtolength{\WRCdotTfRRplusdsbisbplusdsbH}{\WRCdotTfRRplusdsbisbplusdsbL}
\newsavebox{\WRCdotTfRRplusdsbisbplusdsbM}
\begin{lrbox}{\WRCdotTfRRplusdsbisbplusdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbisbplusdsbN}
\settowidth{\WRCdotTfRRplusdsbisbplusdsbN}{\usebox{\WRCdotTfRRplusdsbisbplusdsbM}}
\addtolength{\WRCdotTfRRplusdsbisbplusdsbH}{\WRCdotTfRRplusdsbisbplusdsbN}
\newsavebox{\WRCdotTfRRplusdsbisbplusdsbO}
\begin{lrbox}{\WRCdotTfRRplusdsbisbplusdsbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbisbplusdsbP}
\settowidth{\WRCdotTfRRplusdsbisbplusdsbP}{\usebox{\WRCdotTfRRplusdsbisbplusdsbO}}
\addtolength{\WRCdotTfRRplusdsbisbplusdsbH}{\WRCdotTfRRplusdsbisbplusdsbP}
\newsavebox{\WRCdotTfRRplusdsbisbplusdsbA}
\begin{lrbox}{\WRCdotTfRRplusdsbisbplusdsbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    *pa1 = 0;

    y |-> pa2;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbisbplusdsbB}
\settowidth{\WRCdotTfRRplusdsbisbplusdsbB}{\usebox{\WRCdotTfRRplusdsbisbplusdsbA}}
\newsavebox{\WRCdotTfRRplusdsbisbplusdsbC}
\begin{lrbox}{\WRCdotTfRRplusdsbisbplusdsbC}
\begin{minipage}{\WRCdotTfRRplusdsbisbplusdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TfRR+dsb-isb+dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTfRRplusdsbisbplusdsbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTfRRplusdsbisbplusdsbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTfRRplusdsbisbplusdsbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdsbisbplusdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdsbisbplusdsbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdsbisbplusdsbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdsbisbplusdsbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & ~2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/WRC.TfRR+dsbs.tex <==
\newlength{\WRCdotTfRRplusdsbsH}
\setlength{\WRCdotTfRRplusdsbsH}{0cm}
\newsavebox{\WRCdotTfRRplusdsbsI}
\begin{lrbox}{\WRCdotTfRRplusdsbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbsJ}
\settowidth{\WRCdotTfRRplusdsbsJ}{\usebox{\WRCdotTfRRplusdsbsI}}
\addtolength{\WRCdotTfRRplusdsbsH}{\WRCdotTfRRplusdsbsJ}
\newsavebox{\WRCdotTfRRplusdsbsK}
\begin{lrbox}{\WRCdotTfRRplusdsbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbsL}
\settowidth{\WRCdotTfRRplusdsbsL}{\usebox{\WRCdotTfRRplusdsbsK}}
\addtolength{\WRCdotTfRRplusdsbsH}{\WRCdotTfRRplusdsbsL}
\newsavebox{\WRCdotTfRRplusdsbsM}
\begin{lrbox}{\WRCdotTfRRplusdsbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbsN}
\settowidth{\WRCdotTfRRplusdsbsN}{\usebox{\WRCdotTfRRplusdsbsM}}
\addtolength{\WRCdotTfRRplusdsbsH}{\WRCdotTfRRplusdsbsN}
\newsavebox{\WRCdotTfRRplusdsbsO}
\begin{lrbox}{\WRCdotTfRRplusdsbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbsP}
\settowidth{\WRCdotTfRRplusdsbsP}{\usebox{\WRCdotTfRRplusdsbsO}}
\addtolength{\WRCdotTfRRplusdsbsH}{\WRCdotTfRRplusdsbsP}
\newsavebox{\WRCdotTfRRplusdsbsA}
\begin{lrbox}{\WRCdotTfRRplusdsbsA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    *pa1 = 0;

    y |-> pa2;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbsB}
\settowidth{\WRCdotTfRRplusdsbsB}{\usebox{\WRCdotTfRRplusdsbsA}}
\newsavebox{\WRCdotTfRRplusdsbsC}
\begin{lrbox}{\WRCdotTfRRplusdsbsC}
\begin{minipage}{\WRCdotTfRRplusdsbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TfRR+dsbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTfRRplusdsbsB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTfRRplusdsbsA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTfRRplusdsbsC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdsbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdsbsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdsbsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdsbsO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & ~2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/WRC.TfRR+po+dsb.tex <==
\newlength{\WRCdotTfRRpluspoplusdsbH}
\setlength{\WRCdotTfRRpluspoplusdsbH}{0cm}
\newsavebox{\WRCdotTfRRpluspoplusdsbI}
\begin{lrbox}{\WRCdotTfRRpluspoplusdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRpluspoplusdsbJ}
\settowidth{\WRCdotTfRRpluspoplusdsbJ}{\usebox{\WRCdotTfRRpluspoplusdsbI}}
\addtolength{\WRCdotTfRRpluspoplusdsbH}{\WRCdotTfRRpluspoplusdsbJ}
\newsavebox{\WRCdotTfRRpluspoplusdsbK}
\begin{lrbox}{\WRCdotTfRRpluspoplusdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRpluspoplusdsbL}
\settowidth{\WRCdotTfRRpluspoplusdsbL}{\usebox{\WRCdotTfRRpluspoplusdsbK}}
\addtolength{\WRCdotTfRRpluspoplusdsbH}{\WRCdotTfRRpluspoplusdsbL}
\newsavebox{\WRCdotTfRRpluspoplusdsbM}
\begin{lrbox}{\WRCdotTfRRpluspoplusdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRpluspoplusdsbN}
\settowidth{\WRCdotTfRRpluspoplusdsbN}{\usebox{\WRCdotTfRRpluspoplusdsbM}}
\addtolength{\WRCdotTfRRpluspoplusdsbH}{\WRCdotTfRRpluspoplusdsbN}
\newsavebox{\WRCdotTfRRpluspoplusdsbO}
\begin{lrbox}{\WRCdotTfRRpluspoplusdsbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRpluspoplusdsbP}
\settowidth{\WRCdotTfRRpluspoplusdsbP}{\usebox{\WRCdotTfRRpluspoplusdsbO}}
\addtolength{\WRCdotTfRRpluspoplusdsbH}{\WRCdotTfRRpluspoplusdsbP}
\newsavebox{\WRCdotTfRRpluspoplusdsbA}
\begin{lrbox}{\WRCdotTfRRpluspoplusdsbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    *pa1 = 0;

    y |-> pa2;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRpluspoplusdsbB}
\settowidth{\WRCdotTfRRpluspoplusdsbB}{\usebox{\WRCdotTfRRpluspoplusdsbA}}
\newsavebox{\WRCdotTfRRpluspoplusdsbC}
\begin{lrbox}{\WRCdotTfRRpluspoplusdsbC}
\begin{minipage}{\WRCdotTfRRpluspoplusdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TfRR+po+dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTfRRpluspoplusdsbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTfRRpluspoplusdsbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTfRRpluspoplusdsbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRpluspoplusdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRpluspoplusdsbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRpluspoplusdsbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRpluspoplusdsbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & ~2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/WRC.TfRR+pos.tex <==
\newlength{\WRCdotTfRRplusposH}
\setlength{\WRCdotTfRRplusposH}{0cm}
\newsavebox{\WRCdotTfRRplusposI}
\begin{lrbox}{\WRCdotTfRRplusposI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusposJ}
\settowidth{\WRCdotTfRRplusposJ}{\usebox{\WRCdotTfRRplusposI}}
\addtolength{\WRCdotTfRRplusposH}{\WRCdotTfRRplusposJ}
\newsavebox{\WRCdotTfRRplusposK}
\begin{lrbox}{\WRCdotTfRRplusposK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusposL}
\settowidth{\WRCdotTfRRplusposL}{\usebox{\WRCdotTfRRplusposK}}
\addtolength{\WRCdotTfRRplusposH}{\WRCdotTfRRplusposL}
\newsavebox{\WRCdotTfRRplusposM}
\begin{lrbox}{\WRCdotTfRRplusposM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusposN}
\settowidth{\WRCdotTfRRplusposN}{\usebox{\WRCdotTfRRplusposM}}
\addtolength{\WRCdotTfRRplusposH}{\WRCdotTfRRplusposN}
\newsavebox{\WRCdotTfRRplusposO}
\begin{lrbox}{\WRCdotTfRRplusposO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusposP}
\settowidth{\WRCdotTfRRplusposP}{\usebox{\WRCdotTfRRplusposO}}
\addtolength{\WRCdotTfRRplusposH}{\WRCdotTfRRplusposP}
\newsavebox{\WRCdotTfRRplusposA}
\begin{lrbox}{\WRCdotTfRRplusposA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    *pa1 = 0;

    y |-> pa2;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusposB}
\settowidth{\WRCdotTfRRplusposB}{\usebox{\WRCdotTfRRplusposA}}
\newsavebox{\WRCdotTfRRplusposC}
\begin{lrbox}{\WRCdotTfRRplusposC}
\begin{minipage}{\WRCdotTfRRplusposH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TfRR+pos|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTfRRplusposB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTfRRplusposA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTfRRplusposC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusposI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusposK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusposM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusposO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & ~2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/WRC.TfRT+dsb-tlbiis-dsb+dsb-isb.tex <==
\newlength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbH}
\setlength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbH}{0cm}
\newsavebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbI}
\begin{lrbox}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbJ}
\settowidth{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbJ}{\usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbI}}
\addtolength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbH}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbJ}
\newsavebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbK}
\begin{lrbox}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
// the TLBI is in the handler
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbL}
\settowidth{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbL}{\usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbK}}
\addtolength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbH}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbL}
\newsavebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbM}
\begin{lrbox}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbN}
\settowidth{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbN}{\usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbM}}
\addtolength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbH}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbN}
\newsavebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbO}
\begin{lrbox}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
DSB SY
TLBI VAE1IS,X4
DSB SY
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbP}
\settowidth{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbP}{\usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbO}}
\addtolength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbH}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbP}
\newsavebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbA}
\begin{lrbox}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbB}
\settowidth{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbB}{\usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbA}}
\addtolength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbH}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbB}
\newsavebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbC}
\begin{lrbox}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;

    x |-> pa1;
    x ?-> invalid;
    *pa1 = 1;

    y |-> pa2;
    *pa2 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbD}
\settowidth{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbD}{\usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbC}}
\newsavebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbE}
\begin{lrbox}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbE}
\begin{minipage}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TfRT+dsb-tlbiis-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbO}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=0 & 2:R0=1 & 2:R2=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-23/latex/WRC.TfRT+po+dsb-isb.tex <==
\newlength{\WRCdotTfRTpluspoplusdsbisbH}
\setlength{\WRCdotTfRTpluspoplusdsbisbH}{0cm}
\newsavebox{\WRCdotTfRTpluspoplusdsbisbI}
\begin{lrbox}{\WRCdotTfRTpluspoplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTpluspoplusdsbisbJ}
\settowidth{\WRCdotTfRTpluspoplusdsbisbJ}{\usebox{\WRCdotTfRTpluspoplusdsbisbI}}
\addtolength{\WRCdotTfRTpluspoplusdsbisbH}{\WRCdotTfRTpluspoplusdsbisbJ}
\newsavebox{\WRCdotTfRTpluspoplusdsbisbK}
\begin{lrbox}{\WRCdotTfRTpluspoplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTpluspoplusdsbisbL}
\settowidth{\WRCdotTfRTpluspoplusdsbisbL}{\usebox{\WRCdotTfRTpluspoplusdsbisbK}}
\addtolength{\WRCdotTfRTpluspoplusdsbisbH}{\WRCdotTfRTpluspoplusdsbisbL}
\newsavebox{\WRCdotTfRTpluspoplusdsbisbM}
\begin{lrbox}{\WRCdotTfRTpluspoplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTpluspoplusdsbisbN}
\settowidth{\WRCdotTfRTpluspoplusdsbisbN}{\usebox{\WRCdotTfRTpluspoplusdsbisbM}}
\addtolength{\WRCdotTfRTpluspoplusdsbisbH}{\WRCdotTfRTpluspoplusdsbisbN}
\newsavebox{\WRCdotTfRTpluspoplusdsbisbO}
\begin{lrbox}{\WRCdotTfRTpluspoplusdsbisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTpluspoplusdsbisbP}
\settowidth{\WRCdotTfRTpluspoplusdsbisbP}{\usebox{\WRCdotTfRTpluspoplusdsbisbO}}
\addtolength{\WRCdotTfRTpluspoplusdsbisbH}{\WRCdotTfRTpluspoplusdsbisbP}
\newsavebox{\WRCdotTfRTpluspoplusdsbisbA}
\begin{lrbox}{\WRCdotTfRTpluspoplusdsbisbA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTpluspoplusdsbisbB}
\settowidth{\WRCdotTfRTpluspoplusdsbisbB}{\usebox{\WRCdotTfRTpluspoplusdsbisbA}}
\addtolength{\WRCdotTfRTpluspoplusdsbisbH}{\WRCdotTfRTpluspoplusdsbisbB}
\newsavebox{\WRCdotTfRTpluspoplusdsbisbC}
\begin{lrbox}{\WRCdotTfRTpluspoplusdsbisbC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;

    x |-> pa1;
    x ?-> invalid;
    *pa1 = 1;

    y |-> pa2;
    *pa2 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTpluspoplusdsbisbD}
\settowidth{\WRCdotTfRTpluspoplusdsbisbD}{\usebox{\WRCdotTfRTpluspoplusdsbisbC}}
\newsavebox{\WRCdotTfRTpluspoplusdsbisbE}
\begin{lrbox}{\WRCdotTfRTpluspoplusdsbisbE}
\begin{minipage}{\WRCdotTfRTpluspoplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TfRT+po+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTfRTpluspoplusdsbisbD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTfRTpluspoplusdsbisbC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTfRTpluspoplusdsbisbE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTpluspoplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTpluspoplusdsbisbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTpluspoplusdsbisbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTpluspoplusdsbisbO}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTpluspoplusdsbisbA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=0 & 2:R0=1 & 2:R2=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/BBM+dsb-tlbiis-dsb.tex <==
\newlength{\BBMplusdsbtlbiisdsbH}
\setlength{\BBMplusdsbtlbiisdsbH}{0cm}
\newsavebox{\BBMplusdsbtlbiisdsbI}
\begin{lrbox}{\BBMplusdsbtlbiisdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X6
DSB SY
STR X2,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\BBMplusdsbtlbiisdsbJ}
\settowidth{\BBMplusdsbtlbiisdsbJ}{\usebox{\BBMplusdsbtlbiisdsbI}}
\addtolength{\BBMplusdsbtlbiisdsbH}{\BBMplusdsbtlbiisdsbJ}
\newsavebox{\BBMplusdsbtlbiisdsbK}
\begin{lrbox}{\BBMplusdsbtlbiisdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\BBMplusdsbtlbiisdsbL}
\settowidth{\BBMplusdsbtlbiisdsbL}{\usebox{\BBMplusdsbtlbiisdsbK}}
\addtolength{\BBMplusdsbtlbiisdsbH}{\BBMplusdsbtlbiisdsbL}
\newsavebox{\BBMplusdsbtlbiisdsbM}
\begin{lrbox}{\BBMplusdsbtlbiisdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\BBMplusdsbtlbiisdsbN}
\settowidth{\BBMplusdsbtlbiisdsbN}{\usebox{\BBMplusdsbtlbiisdsbM}}
\addtolength{\BBMplusdsbtlbiisdsbH}{\BBMplusdsbtlbiisdsbN}
\newsavebox{\BBMplusdsbtlbiisdsbO}
\begin{lrbox}{\BBMplusdsbtlbiisdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;
    x ?-> pa2;

    identity 0x1000 with code;

    *pa2 = 2;
\end{lstlisting}
\end{lrbox}
\newlength{\BBMplusdsbtlbiisdsbP}
\settowidth{\BBMplusdsbtlbiisdsbP}{\usebox{\BBMplusdsbtlbiisdsbO}}
\newsavebox{\BBMplusdsbtlbiisdsbA}
\begin{lrbox}{\BBMplusdsbtlbiisdsbA}
\begin{minipage}{\BBMplusdsbtlbiisdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R4=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|BBM+dsb-tlbiis-dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\BBMplusdsbtlbiisdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\BBMplusdsbtlbiisdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\BBMplusdsbtlbiisdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\BBMplusdsbtlbiisdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\BBMplusdsbtlbiisdsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\BBMplusdsbtlbiisdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/BBM.Tf+dsb-tlbiis-dsb.tex <==
\newlength{\BBMdotTfplusdsbtlbiisdsbH}
\setlength{\BBMdotTfplusdsbtlbiisdsbH}{0cm}
\newsavebox{\BBMdotTfplusdsbtlbiisdsbI}
\begin{lrbox}{\BBMdotTfplusdsbtlbiisdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X6
DSB SY
STR X2,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\BBMdotTfplusdsbtlbiisdsbJ}
\settowidth{\BBMdotTfplusdsbtlbiisdsbJ}{\usebox{\BBMdotTfplusdsbtlbiisdsbI}}
\addtolength{\BBMdotTfplusdsbtlbiisdsbH}{\BBMdotTfplusdsbtlbiisdsbJ}
\newsavebox{\BBMdotTfplusdsbtlbiisdsbK}
\begin{lrbox}{\BBMdotTfplusdsbtlbiisdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\BBMdotTfplusdsbtlbiisdsbL}
\settowidth{\BBMdotTfplusdsbtlbiisdsbL}{\usebox{\BBMdotTfplusdsbtlbiisdsbK}}
\addtolength{\BBMdotTfplusdsbtlbiisdsbH}{\BBMdotTfplusdsbtlbiisdsbL}
\newsavebox{\BBMdotTfplusdsbtlbiisdsbM}
\begin{lrbox}{\BBMdotTfplusdsbtlbiisdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
\end{lstlisting}
\end{lrbox}
\newlength{\BBMdotTfplusdsbtlbiisdsbN}
\settowidth{\BBMdotTfplusdsbtlbiisdsbN}{\usebox{\BBMdotTfplusdsbtlbiisdsbM}}
\addtolength{\BBMdotTfplusdsbtlbiisdsbH}{\BBMdotTfplusdsbtlbiisdsbN}
\newsavebox{\BBMdotTfplusdsbtlbiisdsbO}
\begin{lrbox}{\BBMdotTfplusdsbtlbiisdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;
    x ?-> pa2;

    identity 0x1000 with code;

    *pa2 = 2;
\end{lstlisting}
\end{lrbox}
\newlength{\BBMdotTfplusdsbtlbiisdsbP}
\settowidth{\BBMdotTfplusdsbtlbiisdsbP}{\usebox{\BBMdotTfplusdsbtlbiisdsbO}}
\newsavebox{\BBMdotTfplusdsbtlbiisdsbA}
\begin{lrbox}{\BBMdotTfplusdsbtlbiisdsbA}
\begin{minipage}{\BBMdotTfplusdsbtlbiisdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R4=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|BBM.Tf+dsb-tlbiis-dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\BBMdotTfplusdsbtlbiisdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\BBMdotTfplusdsbtlbiisdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\BBMdotTfplusdsbtlbiisdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\BBMdotTfplusdsbtlbiisdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\BBMdotTfplusdsbtlbiisdsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\BBMdotTfplusdsbtlbiisdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/Break2.news1.tex <==
\newlength{\BreaktwodotnewsoneH}
\setlength{\BreaktwodotnewsoneH}{0cm}
\newsavebox{\BreaktwodotnewsoneI}
\begin{lrbox}{\BreaktwodotnewsoneI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1IS,X4
DSB SY
TLBI VMALLE1IS
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\BreaktwodotnewsoneJ}
\settowidth{\BreaktwodotnewsoneJ}{\usebox{\BreaktwodotnewsoneI}}
\addtolength{\BreaktwodotnewsoneH}{\BreaktwodotnewsoneJ}
\newsavebox{\BreaktwodotnewsoneK}
\begin{lrbox}{\BreaktwodotnewsoneK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\BreaktwodotnewsoneL}
\settowidth{\BreaktwodotnewsoneL}{\usebox{\BreaktwodotnewsoneK}}
\addtolength{\BreaktwodotnewsoneH}{\BreaktwodotnewsoneL}
\newsavebox{\BreaktwodotnewsoneM}
\begin{lrbox}{\BreaktwodotnewsoneM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#2
\end{lstlisting}
\end{lrbox}
\newlength{\BreaktwodotnewsoneN}
\settowidth{\BreaktwodotnewsoneN}{\usebox{\BreaktwodotnewsoneM}}
\addtolength{\BreaktwodotnewsoneH}{\BreaktwodotnewsoneN}
\newsavebox{\BreaktwodotnewsoneO}
\begin{lrbox}{\BreaktwodotnewsoneO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X0,#3
\end{lstlisting}
\end{lrbox}
\newlength{\BreaktwodotnewsoneP}
\settowidth{\BreaktwodotnewsoneP}{\usebox{\BreaktwodotnewsoneO}}
\addtolength{\BreaktwodotnewsoneH}{\BreaktwodotnewsoneP}
\newsavebox{\BreaktwodotnewsoneA}
\begin{lrbox}{\BreaktwodotnewsoneA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
option default_tables = false;
physical pa1;
intermediate ipa1;

s2table vm_stage2 0x240000  {
    ipa1 |-> pa1 at level 3;
    ipa1 ?-> invalid at level 3;
    identity pa_to_ipa(0x1000) with code;


    s1table vm_stage1 0x280000  {
        x |-> invalid at level 3;
        x ?-> ipa1 at level 3;

        identity pa_to_va(0x1000) with code;
    }
}

s1table hyp_map 0x200000 {
    identity 0x2000 with code;
    s2table vm_stage2;
    s1table vm_stage1;
}

*pa1 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\BreaktwodotnewsoneB}
\settowidth{\BreaktwodotnewsoneB}{\usebox{\BreaktwodotnewsoneA}}
\newsavebox{\BreaktwodotnewsoneC}
\begin{lrbox}{\BreaktwodotnewsoneC}
\begin{minipage}{\BreaktwodotnewsoneH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(ipa1,vm_stage2)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=ipa1)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(x,vm_stage1)|\\
\lstinline[language=IslaLitmusExp]|0:R4=bvlshr(ipa1,0xC)|\\
\lstinline[language=IslaLitmusExp]|0:TTBR0_EL2=ttbr(asid=0x0000,base=hyp_map)|\\
\lstinline[language=IslaLitmusExp]|0:VTTBR_EL2=ttbr(base=vm_stage2,vmid=0x0000)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:TTBR0_EL1=ttbr(base=vm_stage1,asid=0x0000)|\\
\lstinline[language=IslaLitmusExp]|1:TTBR0_EL2=ttbr(base=hyp_map,asid=0x0000)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\lstinline[language=IslaLitmusExp]|1:VTTBR_EL2=ttbr(vmid=0x0000,base=vm_stage2)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|Break2.news1|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\BreaktwodotnewsoneB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\BreaktwodotnewsoneA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\BreaktwodotnewsoneC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\BreaktwodotnewsoneI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\BreaktwodotnewsoneK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\BreaktwodotnewsoneM}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\BreaktwodotnewsoneO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoRR0.alias+po.tex <==
\newlength{\CoRRzerodotaliaspluspoH}
\setlength{\CoRRzerodotaliaspluspoH}{0cm}
\newsavebox{\CoRRzerodotaliaspluspoI}
\begin{lrbox}{\CoRRzerodotaliaspluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRRzerodotaliaspluspoJ}
\settowidth{\CoRRzerodotaliaspluspoJ}{\usebox{\CoRRzerodotaliaspluspoI}}
\addtolength{\CoRRzerodotaliaspluspoH}{\CoRRzerodotaliaspluspoJ}
\newsavebox{\CoRRzerodotaliaspluspoK}
\begin{lrbox}{\CoRRzerodotaliaspluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRRzerodotaliaspluspoL}
\settowidth{\CoRRzerodotaliaspluspoL}{\usebox{\CoRRzerodotaliaspluspoK}}
\addtolength{\CoRRzerodotaliaspluspoH}{\CoRRzerodotaliaspluspoL}
\newsavebox{\CoRRzerodotaliaspluspoM}
\begin{lrbox}{\CoRRzerodotaliaspluspoM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    y |-> pa1;
    *pa1 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRRzerodotaliaspluspoN}
\settowidth{\CoRRzerodotaliaspluspoN}{\usebox{\CoRRzerodotaliaspluspoM}}
\newsavebox{\CoRRzerodotaliaspluspoO}
\begin{lrbox}{\CoRRzerodotaliaspluspoO}
\begin{minipage}{\CoRRzerodotaliaspluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRR0.alias+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRRzerodotaliaspluspoN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRRzerodotaliaspluspoM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRRzerodotaliaspluspoO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRRzerodotaliaspluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRRzerodotaliaspluspoK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoRR2.alias+po.tex <==
\newlength{\CoRRtwodotaliaspluspoH}
\setlength{\CoRRtwodotaliaspluspoH}{0cm}
\newsavebox{\CoRRtwodotaliaspluspoI}
\begin{lrbox}{\CoRRtwodotaliaspluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRRtwodotaliaspluspoJ}
\settowidth{\CoRRtwodotaliaspluspoJ}{\usebox{\CoRRtwodotaliaspluspoI}}
\addtolength{\CoRRtwodotaliaspluspoH}{\CoRRtwodotaliaspluspoJ}
\newsavebox{\CoRRtwodotaliaspluspoK}
\begin{lrbox}{\CoRRtwodotaliaspluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRRtwodotaliaspluspoL}
\settowidth{\CoRRtwodotaliaspluspoL}{\usebox{\CoRRtwodotaliaspluspoK}}
\addtolength{\CoRRtwodotaliaspluspoH}{\CoRRtwodotaliaspluspoL}
\newsavebox{\CoRRtwodotaliaspluspoM}
\begin{lrbox}{\CoRRtwodotaliaspluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRRtwodotaliaspluspoN}
\settowidth{\CoRRtwodotaliaspluspoN}{\usebox{\CoRRtwodotaliaspluspoM}}
\addtolength{\CoRRtwodotaliaspluspoH}{\CoRRtwodotaliaspluspoN}
\newsavebox{\CoRRtwodotaliaspluspoO}
\begin{lrbox}{\CoRRtwodotaliaspluspoO}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRRtwodotaliaspluspoP}
\settowidth{\CoRRtwodotaliaspluspoP}{\usebox{\CoRRtwodotaliaspluspoO}}
\addtolength{\CoRRtwodotaliaspluspoH}{\CoRRtwodotaliaspluspoP}
\newsavebox{\CoRRtwodotaliaspluspoA}
\begin{lrbox}{\CoRRtwodotaliaspluspoA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    u |-> pa1;
    v |-> pa1;
    w |-> pa1;
    x |-> pa1;
    y |-> pa1;
    z |-> pa1;
    *pa1 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRRtwodotaliaspluspoB}
\settowidth{\CoRRtwodotaliaspluspoB}{\usebox{\CoRRtwodotaliaspluspoA}}
\newsavebox{\CoRRtwodotaliaspluspoC}
\begin{lrbox}{\CoRRtwodotaliaspluspoC}
\begin{minipage}{\CoRRtwodotaliaspluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R1=u|\\
\lstinline[language=IslaLitmusExp]|1:R0=0b10|\\
\lstinline[language=IslaLitmusExp]|1:R1=v|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=w|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|3:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|3:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|3:R1=y|\\
\lstinline[language=IslaLitmusExp]|3:R3=z|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRR2.alias+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRRtwodotaliaspluspoB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRRtwodotaliaspluspoA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRRtwodotaliaspluspoC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRRtwodotaliaspluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRRtwodotaliaspluspoK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\CoRRtwodotaliaspluspoM}\\
  \cline{2-2}
  & Thread 3\\
  \cline{2-2}
  & \usebox{\CoRRtwodotaliaspluspoO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|2:R0=1 & 2:R2=2 & 3:R0=2 & 3:R2=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoRT.inv+addr-trfi.tex <==
\newlength{\CoRTdotinvplusaddrtrfiH}
\setlength{\CoRTdotinvplusaddrtrfiH}{0cm}
\newsavebox{\CoRTdotinvplusaddrtrfiI}
\begin{lrbox}{\CoRTdotinvplusaddrtrfiI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRTdotinvplusaddrtrfiJ}
\settowidth{\CoRTdotinvplusaddrtrfiJ}{\usebox{\CoRTdotinvplusaddrtrfiI}}
\addtolength{\CoRTdotinvplusaddrtrfiH}{\CoRTdotinvplusaddrtrfiJ}
\newsavebox{\CoRTdotinvplusaddrtrfiK}
\begin{lrbox}{\CoRTdotinvplusaddrtrfiK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
STR X3,[X4,X2]
LDR X5,[X6]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRTdotinvplusaddrtrfiL}
\settowidth{\CoRTdotinvplusaddrtrfiL}{\usebox{\CoRTdotinvplusaddrtrfiK}}
\addtolength{\CoRTdotinvplusaddrtrfiH}{\CoRTdotinvplusaddrtrfiL}
\newsavebox{\CoRTdotinvplusaddrtrfiM}
\begin{lrbox}{\CoRTdotinvplusaddrtrfiM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X5,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoRTdotinvplusaddrtrfiN}
\settowidth{\CoRTdotinvplusaddrtrfiN}{\usebox{\CoRTdotinvplusaddrtrfiM}}
\addtolength{\CoRTdotinvplusaddrtrfiH}{\CoRTdotinvplusaddrtrfiN}
\newsavebox{\CoRTdotinvplusaddrtrfiO}
\begin{lrbox}{\CoRTdotinvplusaddrtrfiO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    y |-> invalid;
    y ?-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRTdotinvplusaddrtrfiP}
\settowidth{\CoRTdotinvplusaddrtrfiP}{\usebox{\CoRTdotinvplusaddrtrfiO}}
\newsavebox{\CoRTdotinvplusaddrtrfiA}
\begin{lrbox}{\CoRTdotinvplusaddrtrfiA}
\begin{minipage}{\CoRTdotinvplusaddrtrfiH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|1:R4=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R6=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRT.inv+addr-trfi|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRTdotinvplusaddrtrfiP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRTdotinvplusaddrtrfiO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRTdotinvplusaddrtrfiA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRTdotinvplusaddrtrfiI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRTdotinvplusaddrtrfiK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoRTdotinvplusaddrtrfiM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|true|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoRpteT+dsb-isb.tex <==
\newlength{\CoRpteTplusdsbisbH}
\setlength{\CoRpteTplusdsbisbH}{0cm}
\newsavebox{\CoRpteTplusdsbisbI}
\begin{lrbox}{\CoRpteTplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTplusdsbisbJ}
\settowidth{\CoRpteTplusdsbisbJ}{\usebox{\CoRpteTplusdsbisbI}}
\addtolength{\CoRpteTplusdsbisbH}{\CoRpteTplusdsbisbJ}
\newsavebox{\CoRpteTplusdsbisbK}
\begin{lrbox}{\CoRpteTplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTplusdsbisbL}
\settowidth{\CoRpteTplusdsbisbL}{\usebox{\CoRpteTplusdsbisbK}}
\addtolength{\CoRpteTplusdsbisbH}{\CoRpteTplusdsbisbL}
\newsavebox{\CoRpteTplusdsbisbM}
\begin{lrbox}{\CoRpteTplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTplusdsbisbN}
\settowidth{\CoRpteTplusdsbisbN}{\usebox{\CoRpteTplusdsbisbM}}
\addtolength{\CoRpteTplusdsbisbH}{\CoRpteTplusdsbisbN}
\newsavebox{\CoRpteTplusdsbisbO}
\begin{lrbox}{\CoRpteTplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;

    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;

    *pa1 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTplusdsbisbP}
\settowidth{\CoRpteTplusdsbisbP}{\usebox{\CoRpteTplusdsbisbO}}
\newsavebox{\CoRpteTplusdsbisbA}
\begin{lrbox}{\CoRpteTplusdsbisbA}
\begin{minipage}{\CoRpteTplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRpteT+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRpteTplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRpteTplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRpteTplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRpteTplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRpteTplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoRpteTplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=0 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoRpteT+dsb.tex <==
\newlength{\CoRpteTplusdsbH}
\setlength{\CoRpteTplusdsbH}{0cm}
\newsavebox{\CoRpteTplusdsbI}
\begin{lrbox}{\CoRpteTplusdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTplusdsbJ}
\settowidth{\CoRpteTplusdsbJ}{\usebox{\CoRpteTplusdsbI}}
\addtolength{\CoRpteTplusdsbH}{\CoRpteTplusdsbJ}
\newsavebox{\CoRpteTplusdsbK}
\begin{lrbox}{\CoRpteTplusdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTplusdsbL}
\settowidth{\CoRpteTplusdsbL}{\usebox{\CoRpteTplusdsbK}}
\addtolength{\CoRpteTplusdsbH}{\CoRpteTplusdsbL}
\newsavebox{\CoRpteTplusdsbM}
\begin{lrbox}{\CoRpteTplusdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTplusdsbN}
\settowidth{\CoRpteTplusdsbN}{\usebox{\CoRpteTplusdsbM}}
\addtolength{\CoRpteTplusdsbH}{\CoRpteTplusdsbN}
\newsavebox{\CoRpteTplusdsbO}
\begin{lrbox}{\CoRpteTplusdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;

    *x = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTplusdsbP}
\settowidth{\CoRpteTplusdsbP}{\usebox{\CoRpteTplusdsbO}}
\newsavebox{\CoRpteTplusdsbA}
\begin{lrbox}{\CoRpteTplusdsbA}
\begin{minipage}{\CoRpteTplusdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRpteT+dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRpteTplusdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRpteTplusdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRpteTplusdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRpteTplusdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRpteTplusdsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoRpteTplusdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=0 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoRpteT.EL1+dsb-tlbi-dsb-isb.tex <==
\newlength{\CoRpteTdotELoneplusdsbtlbidsbisbH}
\setlength{\CoRpteTdotELoneplusdsbtlbidsbisbH}{0cm}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbisbI}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTdotELoneplusdsbtlbidsbisbJ}
\settowidth{\CoRpteTdotELoneplusdsbtlbidsbisbJ}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbisbI}}
\addtolength{\CoRpteTdotELoneplusdsbtlbidsbisbH}{\CoRpteTdotELoneplusdsbtlbidsbisbJ}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbisbK}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
TLBI VAE1,X4
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTdotELoneplusdsbtlbidsbisbL}
\settowidth{\CoRpteTdotELoneplusdsbtlbidsbisbL}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbisbK}}
\addtolength{\CoRpteTdotELoneplusdsbtlbidsbisbH}{\CoRpteTdotELoneplusdsbtlbidsbisbL}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbisbM}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTdotELoneplusdsbtlbidsbisbN}
\settowidth{\CoRpteTdotELoneplusdsbtlbidsbisbN}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbisbM}}
\addtolength{\CoRpteTdotELoneplusdsbtlbidsbisbH}{\CoRpteTdotELoneplusdsbtlbidsbisbN}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbisbO}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;

    *pa1 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTdotELoneplusdsbtlbidsbisbP}
\settowidth{\CoRpteTdotELoneplusdsbtlbidsbisbP}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbisbO}}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbisbA}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbisbA}
\begin{minipage}{\CoRpteTdotELoneplusdsbtlbidsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRpteT.EL1+dsb-tlbi-dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRpteTdotELoneplusdsbtlbidsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRpteTdotELoneplusdsbtlbidsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRpteTdotELoneplusdsbtlbidsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRpteTdotELoneplusdsbtlbidsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoRpteTdotELoneplusdsbtlbidsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=0 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoRpteT.EL1+dsb-tlbi-dsb.tex <==
\newlength{\CoRpteTdotELoneplusdsbtlbidsbH}
\setlength{\CoRpteTdotELoneplusdsbtlbidsbH}{0cm}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbI}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTdotELoneplusdsbtlbidsbJ}
\settowidth{\CoRpteTdotELoneplusdsbtlbidsbJ}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbI}}
\addtolength{\CoRpteTdotELoneplusdsbtlbidsbH}{\CoRpteTdotELoneplusdsbtlbidsbJ}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbK}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
TLBI VAE1,X4
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTdotELoneplusdsbtlbidsbL}
\settowidth{\CoRpteTdotELoneplusdsbtlbidsbL}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbK}}
\addtolength{\CoRpteTdotELoneplusdsbtlbidsbH}{\CoRpteTdotELoneplusdsbtlbidsbL}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbM}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTdotELoneplusdsbtlbidsbN}
\settowidth{\CoRpteTdotELoneplusdsbtlbidsbN}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbM}}
\addtolength{\CoRpteTdotELoneplusdsbtlbidsbH}{\CoRpteTdotELoneplusdsbtlbidsbN}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbO}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;

    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;

    *pa1 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTdotELoneplusdsbtlbidsbP}
\settowidth{\CoRpteTdotELoneplusdsbtlbidsbP}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbO}}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbA}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbA}
\begin{minipage}{\CoRpteTdotELoneplusdsbtlbidsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRpteT.EL1+dsb-tlbi-dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRpteTdotELoneplusdsbtlbidsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRpteTdotELoneplusdsbtlbidsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRpteTdotELoneplusdsbtlbidsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRpteTdotELoneplusdsbtlbidsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoRpteTdotELoneplusdsbtlbidsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=0 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoRpteTf.inv+dsb-isb.tex <==
\newlength{\CoRpteTfdotinvplusdsbisbH}
\setlength{\CoRpteTfdotinvplusdsbisbH}{0cm}
\newsavebox{\CoRpteTfdotinvplusdsbisbI}
\begin{lrbox}{\CoRpteTfdotinvplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTfdotinvplusdsbisbJ}
\settowidth{\CoRpteTfdotinvplusdsbisbJ}{\usebox{\CoRpteTfdotinvplusdsbisbI}}
\addtolength{\CoRpteTfdotinvplusdsbisbH}{\CoRpteTfdotinvplusdsbisbJ}
\newsavebox{\CoRpteTfdotinvplusdsbisbK}
\begin{lrbox}{\CoRpteTfdotinvplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTfdotinvplusdsbisbL}
\settowidth{\CoRpteTfdotinvplusdsbisbL}{\usebox{\CoRpteTfdotinvplusdsbisbK}}
\addtolength{\CoRpteTfdotinvplusdsbisbH}{\CoRpteTfdotinvplusdsbisbL}
\newsavebox{\CoRpteTfdotinvplusdsbisbM}
\begin{lrbox}{\CoRpteTfdotinvplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTfdotinvplusdsbisbN}
\settowidth{\CoRpteTfdotinvplusdsbisbN}{\usebox{\CoRpteTfdotinvplusdsbisbM}}
\addtolength{\CoRpteTfdotinvplusdsbisbH}{\CoRpteTfdotinvplusdsbisbN}
\newsavebox{\CoRpteTfdotinvplusdsbisbO}
\begin{lrbox}{\CoRpteTfdotinvplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    option default_tables = true;
    physical pa1;
    intermediate ipa1;

    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    identity 0x1000 with code;

    *pa1 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTfdotinvplusdsbisbP}
\settowidth{\CoRpteTfdotinvplusdsbisbP}{\usebox{\CoRpteTfdotinvplusdsbisbO}}
\newsavebox{\CoRpteTfdotinvplusdsbisbA}
\begin{lrbox}{\CoRpteTfdotinvplusdsbisbA}
\begin{minipage}{\CoRpteTfdotinvplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRpteTf.inv+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRpteTfdotinvplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRpteTfdotinvplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRpteTfdotinvplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRpteTfdotinvplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRpteTfdotinvplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoRpteTfdotinvplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=desc3(y,page_table_base) & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoRpteTf.inv+dsb.tex <==
\newlength{\CoRpteTfdotinvplusdsbH}
\setlength{\CoRpteTfdotinvplusdsbH}{0cm}
\newsavebox{\CoRpteTfdotinvplusdsbI}
\begin{lrbox}{\CoRpteTfdotinvplusdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTfdotinvplusdsbJ}
\settowidth{\CoRpteTfdotinvplusdsbJ}{\usebox{\CoRpteTfdotinvplusdsbI}}
\addtolength{\CoRpteTfdotinvplusdsbH}{\CoRpteTfdotinvplusdsbJ}
\newsavebox{\CoRpteTfdotinvplusdsbK}
\begin{lrbox}{\CoRpteTfdotinvplusdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTfdotinvplusdsbL}
\settowidth{\CoRpteTfdotinvplusdsbL}{\usebox{\CoRpteTfdotinvplusdsbK}}
\addtolength{\CoRpteTfdotinvplusdsbH}{\CoRpteTfdotinvplusdsbL}
\newsavebox{\CoRpteTfdotinvplusdsbM}
\begin{lrbox}{\CoRpteTfdotinvplusdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTfdotinvplusdsbN}
\settowidth{\CoRpteTfdotinvplusdsbN}{\usebox{\CoRpteTfdotinvplusdsbM}}
\addtolength{\CoRpteTfdotinvplusdsbH}{\CoRpteTfdotinvplusdsbN}
\newsavebox{\CoRpteTfdotinvplusdsbO}
\begin{lrbox}{\CoRpteTfdotinvplusdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    identity 0x1000 with code;

    *pa1 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTfdotinvplusdsbP}
\settowidth{\CoRpteTfdotinvplusdsbP}{\usebox{\CoRpteTfdotinvplusdsbO}}
\newsavebox{\CoRpteTfdotinvplusdsbA}
\begin{lrbox}{\CoRpteTfdotinvplusdsbA}
\begin{minipage}{\CoRpteTfdotinvplusdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRpteTf.inv+dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRpteTfdotinvplusdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRpteTfdotinvplusdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRpteTfdotinvplusdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRpteTfdotinvplusdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRpteTfdotinvplusdsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoRpteTfdotinvplusdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=desc3(y,page_table_base) & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoTRpte.inv+dsb-isb.tex <==
\newlength{\CoTRptedotinvplusdsbisbH}
\setlength{\CoTRptedotinvplusdsbisbH}{0cm}
\newsavebox{\CoTRptedotinvplusdsbisbI}
\begin{lrbox}{\CoTRptedotinvplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvplusdsbisbJ}
\settowidth{\CoTRptedotinvplusdsbisbJ}{\usebox{\CoTRptedotinvplusdsbisbI}}
\addtolength{\CoTRptedotinvplusdsbisbH}{\CoTRptedotinvplusdsbisbJ}
\newsavebox{\CoTRptedotinvplusdsbisbK}
\begin{lrbox}{\CoTRptedotinvplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvplusdsbisbL}
\settowidth{\CoTRptedotinvplusdsbisbL}{\usebox{\CoTRptedotinvplusdsbisbK}}
\addtolength{\CoTRptedotinvplusdsbisbH}{\CoTRptedotinvplusdsbisbL}
\newsavebox{\CoTRptedotinvplusdsbisbM}
\begin{lrbox}{\CoTRptedotinvplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvplusdsbisbN}
\settowidth{\CoTRptedotinvplusdsbisbN}{\usebox{\CoTRptedotinvplusdsbisbM}}
\addtolength{\CoTRptedotinvplusdsbisbH}{\CoTRptedotinvplusdsbisbN}
\newsavebox{\CoTRptedotinvplusdsbisbO}
\begin{lrbox}{\CoTRptedotinvplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvplusdsbisbP}
\settowidth{\CoTRptedotinvplusdsbisbP}{\usebox{\CoTRptedotinvplusdsbisbO}}
\newsavebox{\CoTRptedotinvplusdsbisbA}
\begin{lrbox}{\CoTRptedotinvplusdsbisbA}
\begin{minipage}{\CoTRptedotinvplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTRpte.inv+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTRptedotinvplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTRptedotinvplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTRptedotinvplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoTRpte.inv+dsb.tex <==
\newlength{\CoTRptedotinvplusdsbH}
\setlength{\CoTRptedotinvplusdsbH}{0cm}
\newsavebox{\CoTRptedotinvplusdsbI}
\begin{lrbox}{\CoTRptedotinvplusdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvplusdsbJ}
\settowidth{\CoTRptedotinvplusdsbJ}{\usebox{\CoTRptedotinvplusdsbI}}
\addtolength{\CoTRptedotinvplusdsbH}{\CoTRptedotinvplusdsbJ}
\newsavebox{\CoTRptedotinvplusdsbK}
\begin{lrbox}{\CoTRptedotinvplusdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvplusdsbL}
\settowidth{\CoTRptedotinvplusdsbL}{\usebox{\CoTRptedotinvplusdsbK}}
\addtolength{\CoTRptedotinvplusdsbH}{\CoTRptedotinvplusdsbL}
\newsavebox{\CoTRptedotinvplusdsbM}
\begin{lrbox}{\CoTRptedotinvplusdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvplusdsbN}
\settowidth{\CoTRptedotinvplusdsbN}{\usebox{\CoTRptedotinvplusdsbM}}
\addtolength{\CoTRptedotinvplusdsbH}{\CoTRptedotinvplusdsbN}
\newsavebox{\CoTRptedotinvplusdsbO}
\begin{lrbox}{\CoTRptedotinvplusdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *y = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvplusdsbP}
\settowidth{\CoTRptedotinvplusdsbP}{\usebox{\CoTRptedotinvplusdsbO}}
\newsavebox{\CoTRptedotinvplusdsbA}
\begin{lrbox}{\CoTRptedotinvplusdsbA}
\begin{minipage}{\CoTRptedotinvplusdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTRpte.inv+dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTRptedotinvplusdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTRptedotinvplusdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTRptedotinvplusdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvplusdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvplusdsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvplusdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoTRpte.inv+po.tex <==
\newlength{\CoTRptedotinvpluspoH}
\setlength{\CoTRptedotinvpluspoH}{0cm}
\newsavebox{\CoTRptedotinvpluspoI}
\begin{lrbox}{\CoTRptedotinvpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvpluspoJ}
\settowidth{\CoTRptedotinvpluspoJ}{\usebox{\CoTRptedotinvpluspoI}}
\addtolength{\CoTRptedotinvpluspoH}{\CoTRptedotinvpluspoJ}
\newsavebox{\CoTRptedotinvpluspoK}
\begin{lrbox}{\CoTRptedotinvpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvpluspoL}
\settowidth{\CoTRptedotinvpluspoL}{\usebox{\CoTRptedotinvpluspoK}}
\addtolength{\CoTRptedotinvpluspoH}{\CoTRptedotinvpluspoL}
\newsavebox{\CoTRptedotinvpluspoM}
\begin{lrbox}{\CoTRptedotinvpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvpluspoN}
\settowidth{\CoTRptedotinvpluspoN}{\usebox{\CoTRptedotinvpluspoM}}
\addtolength{\CoTRptedotinvpluspoH}{\CoTRptedotinvpluspoN}
\newsavebox{\CoTRptedotinvpluspoO}
\begin{lrbox}{\CoTRptedotinvpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *y = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvpluspoP}
\settowidth{\CoTRptedotinvpluspoP}{\usebox{\CoTRptedotinvpluspoO}}
\newsavebox{\CoTRptedotinvpluspoA}
\begin{lrbox}{\CoTRptedotinvpluspoA}
\begin{minipage}{\CoTRptedotinvpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTRpte.inv+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTRptedotinvpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTRptedotinvpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTRptedotinvpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoTT.ro+dmb.tex <==
\newlength{\CoTTdotroplusdmbH}
\setlength{\CoTTdotroplusdmbH}{0cm}
\newsavebox{\CoTTdotroplusdmbI}
\begin{lrbox}{\CoTTdotroplusdmbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotroplusdmbJ}
\settowidth{\CoTTdotroplusdmbJ}{\usebox{\CoTTdotroplusdmbI}}
\addtolength{\CoTTdotroplusdmbH}{\CoTTdotroplusdmbJ}
\newsavebox{\CoTTdotroplusdmbK}
\begin{lrbox}{\CoTTdotroplusdmbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotroplusdmbL}
\settowidth{\CoTTdotroplusdmbL}{\usebox{\CoTTdotroplusdmbK}}
\addtolength{\CoTTdotroplusdmbH}{\CoTTdotroplusdmbL}
\newsavebox{\CoTTdotroplusdmbM}
\begin{lrbox}{\CoTTdotroplusdmbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1 with [AP = 0b11] and default;
    x ?-> pa2 with [AP = 0b11] and default;
    y |-> pa2 with [AP = 0b11] and default;

    *pa2 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotroplusdmbN}
\settowidth{\CoTTdotroplusdmbN}{\usebox{\CoTTdotroplusdmbM}}
\newsavebox{\CoTTdotroplusdmbO}
\begin{lrbox}{\CoTTdotroplusdmbO}
\begin{minipage}{\CoTTdotroplusdmbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTT.ro+dmb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTTdotroplusdmbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTTdotroplusdmbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTTdotroplusdmbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTTdotroplusdmbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTTdotroplusdmbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoTT.ro+dsb-isb.tex <==
\newlength{\CoTTdotroplusdsbisbH}
\setlength{\CoTTdotroplusdsbisbH}{0cm}
\newsavebox{\CoTTdotroplusdsbisbI}
\begin{lrbox}{\CoTTdotroplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotroplusdsbisbJ}
\settowidth{\CoTTdotroplusdsbisbJ}{\usebox{\CoTTdotroplusdsbisbI}}
\addtolength{\CoTTdotroplusdsbisbH}{\CoTTdotroplusdsbisbJ}
\newsavebox{\CoTTdotroplusdsbisbK}
\begin{lrbox}{\CoTTdotroplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotroplusdsbisbL}
\settowidth{\CoTTdotroplusdsbisbL}{\usebox{\CoTTdotroplusdsbisbK}}
\addtolength{\CoTTdotroplusdsbisbH}{\CoTTdotroplusdsbisbL}
\newsavebox{\CoTTdotroplusdsbisbM}
\begin{lrbox}{\CoTTdotroplusdsbisbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1 with [AP = 0b11] and default;
    x ?-> pa2 with [AP = 0b11] and default;
    y |-> pa2 with [AP = 0b11] and default;

    *pa2 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotroplusdsbisbN}
\settowidth{\CoTTdotroplusdsbisbN}{\usebox{\CoTTdotroplusdsbisbM}}
\newsavebox{\CoTTdotroplusdsbisbO}
\begin{lrbox}{\CoTTdotroplusdsbisbO}
\begin{minipage}{\CoTTdotroplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTT.ro+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTTdotroplusdsbisbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTTdotroplusdsbisbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTTdotroplusdsbisbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTTdotroplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTTdotroplusdsbisbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoTT.ro+po.tex <==
\newlength{\CoTTdotropluspoH}
\setlength{\CoTTdotropluspoH}{0cm}
\newsavebox{\CoTTdotropluspoI}
\begin{lrbox}{\CoTTdotropluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotropluspoJ}
\settowidth{\CoTTdotropluspoJ}{\usebox{\CoTTdotropluspoI}}
\addtolength{\CoTTdotropluspoH}{\CoTTdotropluspoJ}
\newsavebox{\CoTTdotropluspoK}
\begin{lrbox}{\CoTTdotropluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotropluspoL}
\settowidth{\CoTTdotropluspoL}{\usebox{\CoTTdotropluspoK}}
\addtolength{\CoTTdotropluspoH}{\CoTTdotropluspoL}
\newsavebox{\CoTTdotropluspoM}
\begin{lrbox}{\CoTTdotropluspoM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1 with [AP = 0b11] and default;
    x ?-> pa2 with [AP = 0b11] and default;
    y |-> pa2 with [AP = 0b11] and default;

    *pa2 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotropluspoN}
\settowidth{\CoTTdotropluspoN}{\usebox{\CoTTdotropluspoM}}
\newsavebox{\CoTTdotropluspoO}
\begin{lrbox}{\CoTTdotropluspoO}
\begin{minipage}{\CoTTdotropluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTT.ro+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTTdotropluspoN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTTdotropluspoM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTTdotropluspoO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTTdotropluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTTdotropluspoK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoTTf.inv+dsb-isb.tex <==
\newlength{\CoTTfdotinvplusdsbisbH}
\setlength{\CoTTfdotinvplusdsbisbH}{0cm}
\newsavebox{\CoTTfdotinvplusdsbisbI}
\begin{lrbox}{\CoTTfdotinvplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTfdotinvplusdsbisbJ}
\settowidth{\CoTTfdotinvplusdsbisbJ}{\usebox{\CoTTfdotinvplusdsbisbI}}
\addtolength{\CoTTfdotinvplusdsbisbH}{\CoTTfdotinvplusdsbisbJ}
\newsavebox{\CoTTfdotinvplusdsbisbK}
\begin{lrbox}{\CoTTfdotinvplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTfdotinvplusdsbisbL}
\settowidth{\CoTTfdotinvplusdsbisbL}{\usebox{\CoTTfdotinvplusdsbisbK}}
\addtolength{\CoTTfdotinvplusdsbisbH}{\CoTTfdotinvplusdsbisbL}
\newsavebox{\CoTTfdotinvplusdsbisbM}
\begin{lrbox}{\CoTTfdotinvplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTfdotinvplusdsbisbN}
\settowidth{\CoTTfdotinvplusdsbisbN}{\usebox{\CoTTfdotinvplusdsbisbM}}
\addtolength{\CoTTfdotinvplusdsbisbH}{\CoTTfdotinvplusdsbisbN}
\newsavebox{\CoTTfdotinvplusdsbisbO}
\begin{lrbox}{\CoTTfdotinvplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTfdotinvplusdsbisbP}
\settowidth{\CoTTfdotinvplusdsbisbP}{\usebox{\CoTTfdotinvplusdsbisbO}}
\newsavebox{\CoTTfdotinvplusdsbisbA}
\begin{lrbox}{\CoTTfdotinvplusdsbisbA}
\begin{minipage}{\CoTTfdotinvplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTTf.inv+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTTfdotinvplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTTfdotinvplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTTfdotinvplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTTfdotinvplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTTfdotinvplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTTfdotinvplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoTTf.inv+po.tex <==
\newlength{\CoTTfdotinvpluspoH}
\setlength{\CoTTfdotinvpluspoH}{0cm}
\newsavebox{\CoTTfdotinvpluspoI}
\begin{lrbox}{\CoTTfdotinvpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTfdotinvpluspoJ}
\settowidth{\CoTTfdotinvpluspoJ}{\usebox{\CoTTfdotinvpluspoI}}
\addtolength{\CoTTfdotinvpluspoH}{\CoTTfdotinvpluspoJ}
\newsavebox{\CoTTfdotinvpluspoK}
\begin{lrbox}{\CoTTfdotinvpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTfdotinvpluspoL}
\settowidth{\CoTTfdotinvpluspoL}{\usebox{\CoTTfdotinvpluspoK}}
\addtolength{\CoTTfdotinvpluspoH}{\CoTTfdotinvpluspoL}
\newsavebox{\CoTTfdotinvpluspoM}
\begin{lrbox}{\CoTTfdotinvpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTfdotinvpluspoN}
\settowidth{\CoTTfdotinvpluspoN}{\usebox{\CoTTfdotinvpluspoM}}
\addtolength{\CoTTfdotinvpluspoH}{\CoTTfdotinvpluspoN}
\newsavebox{\CoTTfdotinvpluspoO}
\begin{lrbox}{\CoTTfdotinvpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTfdotinvpluspoP}
\settowidth{\CoTTfdotinvpluspoP}{\usebox{\CoTTfdotinvpluspoO}}
\newsavebox{\CoTTfdotinvpluspoA}
\begin{lrbox}{\CoTTfdotinvpluspoA}
\begin{minipage}{\CoTTfdotinvpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTTf.inv+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTTfdotinvpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTTfdotinvpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTTfdotinvpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTTfdotinvpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTTfdotinvpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTTfdotinvpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoTW1.inv.tex <==
\newlength{\CoTWonedotinvH}
\setlength{\CoTWonedotinvH}{0cm}
\newsavebox{\CoTWonedotinvI}
\begin{lrbox}{\CoTWonedotinvI}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTWonedotinvJ}
\settowidth{\CoTWonedotinvJ}{\usebox{\CoTWonedotinvI}}
\addtolength{\CoTWonedotinvH}{\CoTWonedotinvJ}
\newsavebox{\CoTWonedotinvK}
\begin{lrbox}{\CoTWonedotinvK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTWonedotinvL}
\settowidth{\CoTWonedotinvL}{\usebox{\CoTWonedotinvK}}
\addtolength{\CoTWonedotinvH}{\CoTWonedotinvL}
\newsavebox{\CoTWonedotinvM}
\begin{lrbox}{\CoTWonedotinvM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTWonedotinvN}
\settowidth{\CoTWonedotinvN}{\usebox{\CoTWonedotinvM}}
\newsavebox{\CoTWonedotinvO}
\begin{lrbox}{\CoTWonedotinvO}
\begin{minipage}{\CoTWonedotinvH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=x|\\
\lstinline[language=IslaLitmusExp]|R2=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTW1.inv|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTWonedotinvN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTWonedotinvM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTWonedotinvO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTWonedotinvI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTWonedotinvK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoTWinv.tex <==
\newlength{\CoTWinvH}
\setlength{\CoTWinvH}{0cm}
\newsavebox{\CoTWinvI}
\begin{lrbox}{\CoTWinvI}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTWinvJ}
\settowidth{\CoTWinvJ}{\usebox{\CoTWinvI}}
\addtolength{\CoTWinvH}{\CoTWinvJ}
\newsavebox{\CoTWinvK}
\begin{lrbox}{\CoTWinvK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTWinvL}
\settowidth{\CoTWinvL}{\usebox{\CoTWinvK}}
\addtolength{\CoTWinvH}{\CoTWinvL}
\newsavebox{\CoTWinvM}
\begin{lrbox}{\CoTWinvM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTWinvN}
\settowidth{\CoTWinvN}{\usebox{\CoTWinvM}}
\newsavebox{\CoTWinvO}
\begin{lrbox}{\CoTWinvO}
\begin{minipage}{\CoTWinvH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=x|\\
\lstinline[language=IslaLitmusExp]|R2=0b0|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTWinv|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTWinvN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTWinvM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTWinvO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTWinvI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTWinvK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoTfRpte+dsb-isb.tex <==
\newlength{\CoTfRpteplusdsbisbH}
\setlength{\CoTfRpteplusdsbisbH}{0cm}
\newsavebox{\CoTfRpteplusdsbisbI}
\begin{lrbox}{\CoTfRpteplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRpteplusdsbisbJ}
\settowidth{\CoTfRpteplusdsbisbJ}{\usebox{\CoTfRpteplusdsbisbI}}
\addtolength{\CoTfRpteplusdsbisbH}{\CoTfRpteplusdsbisbJ}
\newsavebox{\CoTfRpteplusdsbisbK}
\begin{lrbox}{\CoTfRpteplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRpteplusdsbisbL}
\settowidth{\CoTfRpteplusdsbisbL}{\usebox{\CoTfRpteplusdsbisbK}}
\addtolength{\CoTfRpteplusdsbisbH}{\CoTfRpteplusdsbisbL}
\newsavebox{\CoTfRpteplusdsbisbM}
\begin{lrbox}{\CoTfRpteplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRpteplusdsbisbN}
\settowidth{\CoTfRpteplusdsbisbN}{\usebox{\CoTfRpteplusdsbisbM}}
\addtolength{\CoTfRpteplusdsbisbH}{\CoTfRpteplusdsbisbN}
\newsavebox{\CoTfRpteplusdsbisbO}
\begin{lrbox}{\CoTfRpteplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;
    y |-> pa1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRpteplusdsbisbP}
\settowidth{\CoTfRpteplusdsbisbP}{\usebox{\CoTfRpteplusdsbisbO}}
\newsavebox{\CoTfRpteplusdsbisbA}
\begin{lrbox}{\CoTfRpteplusdsbisbA}
\begin{minipage}{\CoTfRpteplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfRpte+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfRpteplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfRpteplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfRpteplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfRpteplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTfRpteplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfRpteplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=desc3(y,page_table_base)|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoTfRpte+dsb.tex <==
\newlength{\CoTfRpteplusdsbH}
\setlength{\CoTfRpteplusdsbH}{0cm}
\newsavebox{\CoTfRpteplusdsbI}
\begin{lrbox}{\CoTfRpteplusdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRpteplusdsbJ}
\settowidth{\CoTfRpteplusdsbJ}{\usebox{\CoTfRpteplusdsbI}}
\addtolength{\CoTfRpteplusdsbH}{\CoTfRpteplusdsbJ}
\newsavebox{\CoTfRpteplusdsbK}
\begin{lrbox}{\CoTfRpteplusdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRpteplusdsbL}
\settowidth{\CoTfRpteplusdsbL}{\usebox{\CoTfRpteplusdsbK}}
\addtolength{\CoTfRpteplusdsbH}{\CoTfRpteplusdsbL}
\newsavebox{\CoTfRpteplusdsbM}
\begin{lrbox}{\CoTfRpteplusdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRpteplusdsbN}
\settowidth{\CoTfRpteplusdsbN}{\usebox{\CoTfRpteplusdsbM}}
\addtolength{\CoTfRpteplusdsbH}{\CoTfRpteplusdsbN}
\newsavebox{\CoTfRpteplusdsbO}
\begin{lrbox}{\CoTfRpteplusdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;
    y |-> pa1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRpteplusdsbP}
\settowidth{\CoTfRpteplusdsbP}{\usebox{\CoTfRpteplusdsbO}}
\newsavebox{\CoTfRpteplusdsbA}
\begin{lrbox}{\CoTfRpteplusdsbA}
\begin{minipage}{\CoTfRpteplusdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfRpte+dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfRpteplusdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfRpteplusdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfRpteplusdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfRpteplusdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTfRpteplusdsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfRpteplusdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=desc3(y,page_table_base)|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoTfRpte+eret.tex <==
\newlength{\CoTfRptepluseretH}
\setlength{\CoTfRptepluseretH}{0cm}
\newsavebox{\CoTfRptepluseretI}
\begin{lrbox}{\CoTfRptepluseretI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRptepluseretJ}
\settowidth{\CoTfRptepluseretJ}{\usebox{\CoTfRptepluseretI}}
\addtolength{\CoTfRptepluseretH}{\CoTfRptepluseretJ}
\newsavebox{\CoTfRptepluseretK}
\begin{lrbox}{\CoTfRptepluseretK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRptepluseretL}
\settowidth{\CoTfRptepluseretL}{\usebox{\CoTfRptepluseretK}}
\addtolength{\CoTfRptepluseretH}{\CoTfRptepluseretL}
\newsavebox{\CoTfRptepluseretM}
\begin{lrbox}{\CoTfRptepluseretM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRptepluseretN}
\settowidth{\CoTfRptepluseretN}{\usebox{\CoTfRptepluseretM}}
\addtolength{\CoTfRptepluseretH}{\CoTfRptepluseretN}
\newsavebox{\CoTfRptepluseretO}
\begin{lrbox}{\CoTfRptepluseretO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;
    y |-> pa1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRptepluseretP}
\settowidth{\CoTfRptepluseretP}{\usebox{\CoTfRptepluseretO}}
\newsavebox{\CoTfRptepluseretA}
\begin{lrbox}{\CoTfRptepluseretA}
\begin{minipage}{\CoTfRptepluseretH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfRpte+eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfRptepluseretP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfRptepluseretO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfRptepluseretA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfRptepluseretI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTfRptepluseretK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfRptepluseretM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=desc3(y,page_table_base)|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoTfRpte+po.tex <==
\newlength{\CoTfRptepluspoH}
\setlength{\CoTfRptepluspoH}{0cm}
\newsavebox{\CoTfRptepluspoI}
\begin{lrbox}{\CoTfRptepluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRptepluspoJ}
\settowidth{\CoTfRptepluspoJ}{\usebox{\CoTfRptepluspoI}}
\addtolength{\CoTfRptepluspoH}{\CoTfRptepluspoJ}
\newsavebox{\CoTfRptepluspoK}
\begin{lrbox}{\CoTfRptepluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRptepluspoL}
\settowidth{\CoTfRptepluspoL}{\usebox{\CoTfRptepluspoK}}
\addtolength{\CoTfRptepluspoH}{\CoTfRptepluspoL}
\newsavebox{\CoTfRptepluspoM}
\begin{lrbox}{\CoTfRptepluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRptepluspoN}
\settowidth{\CoTfRptepluspoN}{\usebox{\CoTfRptepluspoM}}
\addtolength{\CoTfRptepluspoH}{\CoTfRptepluspoN}
\newsavebox{\CoTfRptepluspoO}
\begin{lrbox}{\CoTfRptepluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;
    y |-> pa1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRptepluspoP}
\settowidth{\CoTfRptepluspoP}{\usebox{\CoTfRptepluspoO}}
\newsavebox{\CoTfRptepluspoA}
\begin{lrbox}{\CoTfRptepluspoA}
\begin{minipage}{\CoTfRptepluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfRpte+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfRptepluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfRptepluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfRptepluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfRptepluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTfRptepluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfRptepluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=desc3(y,page_table_base)|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoTfT+dsb-isb.tex <==
\newlength{\CoTfTplusdsbisbH}
\setlength{\CoTfTplusdsbisbH}{0cm}
\newsavebox{\CoTfTplusdsbisbI}
\begin{lrbox}{\CoTfTplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfTplusdsbisbJ}
\settowidth{\CoTfTplusdsbisbJ}{\usebox{\CoTfTplusdsbisbI}}
\addtolength{\CoTfTplusdsbisbH}{\CoTfTplusdsbisbJ}
\newsavebox{\CoTfTplusdsbisbK}
\begin{lrbox}{\CoTfTplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfTplusdsbisbL}
\settowidth{\CoTfTplusdsbisbL}{\usebox{\CoTfTplusdsbisbK}}
\addtolength{\CoTfTplusdsbisbH}{\CoTfTplusdsbisbL}
\newsavebox{\CoTfTplusdsbisbM}
\begin{lrbox}{\CoTfTplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfTplusdsbisbN}
\settowidth{\CoTfTplusdsbisbN}{\usebox{\CoTfTplusdsbisbM}}
\addtolength{\CoTfTplusdsbisbH}{\CoTfTplusdsbisbN}
\newsavebox{\CoTfTplusdsbisbO}
\begin{lrbox}{\CoTfTplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;
    y |-> pa1;
    *pa1 = 0;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfTplusdsbisbP}
\settowidth{\CoTfTplusdsbisbP}{\usebox{\CoTfTplusdsbisbO}}
\newsavebox{\CoTfTplusdsbisbA}
\begin{lrbox}{\CoTfTplusdsbisbA}
\begin{minipage}{\CoTfTplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfT+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfTplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfTplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfTplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfTplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTfTplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfTplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoTfT+po.tex <==
\newlength{\CoTfTpluspoH}
\setlength{\CoTfTpluspoH}{0cm}
\newsavebox{\CoTfTpluspoI}
\begin{lrbox}{\CoTfTpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfTpluspoJ}
\settowidth{\CoTfTpluspoJ}{\usebox{\CoTfTpluspoI}}
\addtolength{\CoTfTpluspoH}{\CoTfTpluspoJ}
\newsavebox{\CoTfTpluspoK}
\begin{lrbox}{\CoTfTpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfTpluspoL}
\settowidth{\CoTfTpluspoL}{\usebox{\CoTfTpluspoK}}
\addtolength{\CoTfTpluspoH}{\CoTfTpluspoL}
\newsavebox{\CoTfTpluspoM}
\begin{lrbox}{\CoTfTpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfTpluspoN}
\settowidth{\CoTfTpluspoN}{\usebox{\CoTfTpluspoM}}
\addtolength{\CoTfTpluspoH}{\CoTfTpluspoN}
\newsavebox{\CoTfTpluspoO}
\begin{lrbox}{\CoTfTpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;
    y |-> pa1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfTpluspoP}
\settowidth{\CoTfTpluspoP}{\usebox{\CoTfTpluspoO}}
\newsavebox{\CoTfTpluspoA}
\begin{lrbox}{\CoTfTpluspoA}
\begin{minipage}{\CoTfTpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfT+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfTpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfTpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfTpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfTpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTfTpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfTpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoTfW.inv+dsb-isb.tex <==
\newlength{\CoTfWdotinvplusdsbisbH}
\setlength{\CoTfWdotinvplusdsbisbH}{0cm}
\newsavebox{\CoTfWdotinvplusdsbisbI}
\begin{lrbox}{\CoTfWdotinvplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvplusdsbisbJ}
\settowidth{\CoTfWdotinvplusdsbisbJ}{\usebox{\CoTfWdotinvplusdsbisbI}}
\addtolength{\CoTfWdotinvplusdsbisbH}{\CoTfWdotinvplusdsbisbJ}
\newsavebox{\CoTfWdotinvplusdsbisbK}
\begin{lrbox}{\CoTfWdotinvplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvplusdsbisbL}
\settowidth{\CoTfWdotinvplusdsbisbL}{\usebox{\CoTfWdotinvplusdsbisbK}}
\addtolength{\CoTfWdotinvplusdsbisbH}{\CoTfWdotinvplusdsbisbL}
\newsavebox{\CoTfWdotinvplusdsbisbM}
\begin{lrbox}{\CoTfWdotinvplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvplusdsbisbN}
\settowidth{\CoTfWdotinvplusdsbisbN}{\usebox{\CoTfWdotinvplusdsbisbM}}
\addtolength{\CoTfWdotinvplusdsbisbH}{\CoTfWdotinvplusdsbisbN}
\newsavebox{\CoTfWdotinvplusdsbisbO}
\begin{lrbox}{\CoTfWdotinvplusdsbisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvplusdsbisbP}
\settowidth{\CoTfWdotinvplusdsbisbP}{\usebox{\CoTfWdotinvplusdsbisbO}}
\addtolength{\CoTfWdotinvplusdsbisbH}{\CoTfWdotinvplusdsbisbP}
\newsavebox{\CoTfWdotinvplusdsbisbA}
\begin{lrbox}{\CoTfWdotinvplusdsbisbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    x ?-> raw(2);
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvplusdsbisbB}
\settowidth{\CoTfWdotinvplusdsbisbB}{\usebox{\CoTfWdotinvplusdsbisbA}}
\newsavebox{\CoTfWdotinvplusdsbisbC}
\begin{lrbox}{\CoTfWdotinvplusdsbisbC}
\begin{minipage}{\CoTfWdotinvplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b10|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:R1=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfW.inv+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfWdotinvplusdsbisbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfWdotinvplusdsbisbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfWdotinvplusdsbisbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfWdotinvplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTfWdotinvplusdsbisbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\CoTfWdotinvplusdsbisbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfWdotinvplusdsbisbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=2 & 2:R2=mkdesc3(oa=pa1)|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoTfW.inv+po.tex <==
\newlength{\CoTfWdotinvpluspoH}
\setlength{\CoTfWdotinvpluspoH}{0cm}
\newsavebox{\CoTfWdotinvpluspoI}
\begin{lrbox}{\CoTfWdotinvpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvpluspoJ}
\settowidth{\CoTfWdotinvpluspoJ}{\usebox{\CoTfWdotinvpluspoI}}
\addtolength{\CoTfWdotinvpluspoH}{\CoTfWdotinvpluspoJ}
\newsavebox{\CoTfWdotinvpluspoK}
\begin{lrbox}{\CoTfWdotinvpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvpluspoL}
\settowidth{\CoTfWdotinvpluspoL}{\usebox{\CoTfWdotinvpluspoK}}
\addtolength{\CoTfWdotinvpluspoH}{\CoTfWdotinvpluspoL}
\newsavebox{\CoTfWdotinvpluspoM}
\begin{lrbox}{\CoTfWdotinvpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvpluspoN}
\settowidth{\CoTfWdotinvpluspoN}{\usebox{\CoTfWdotinvpluspoM}}
\addtolength{\CoTfWdotinvpluspoH}{\CoTfWdotinvpluspoN}
\newsavebox{\CoTfWdotinvpluspoO}
\begin{lrbox}{\CoTfWdotinvpluspoO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvpluspoP}
\settowidth{\CoTfWdotinvpluspoP}{\usebox{\CoTfWdotinvpluspoO}}
\addtolength{\CoTfWdotinvpluspoH}{\CoTfWdotinvpluspoP}
\newsavebox{\CoTfWdotinvpluspoA}
\begin{lrbox}{\CoTfWdotinvpluspoA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    x ?-> raw(2);
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvpluspoB}
\settowidth{\CoTfWdotinvpluspoB}{\usebox{\CoTfWdotinvpluspoA}}
\newsavebox{\CoTfWdotinvpluspoC}
\begin{lrbox}{\CoTfWdotinvpluspoC}
\begin{minipage}{\CoTfWdotinvpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b10|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:R1=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfW.inv+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfWdotinvpluspoB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfWdotinvpluspoA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfWdotinvpluspoC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfWdotinvpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTfWdotinvpluspoK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\CoTfWdotinvpluspoM}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfWdotinvpluspoO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=2 & 2:R2=mkdesc3(oa=pa1)|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoTfW1.inv+si.tex <==
\newlength{\CoTfWonedotinvplussiH}
\setlength{\CoTfWonedotinvplussiH}{0cm}
\newsavebox{\CoTfWonedotinvplussiI}
\begin{lrbox}{\CoTfWonedotinvplussiI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWonedotinvplussiJ}
\settowidth{\CoTfWonedotinvplussiJ}{\usebox{\CoTfWonedotinvplussiI}}
\addtolength{\CoTfWonedotinvplussiH}{\CoTfWonedotinvplussiJ}
\newsavebox{\CoTfWonedotinvplussiK}
\begin{lrbox}{\CoTfWonedotinvplussiK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWonedotinvplussiL}
\settowidth{\CoTfWonedotinvplussiL}{\usebox{\CoTfWonedotinvplussiK}}
\addtolength{\CoTfWonedotinvplussiH}{\CoTfWonedotinvplussiL}
\newsavebox{\CoTfWonedotinvplussiM}
\begin{lrbox}{\CoTfWonedotinvplussiM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWonedotinvplussiN}
\settowidth{\CoTfWonedotinvplussiN}{\usebox{\CoTfWonedotinvplussiM}}
\newsavebox{\CoTfWonedotinvplussiO}
\begin{lrbox}{\CoTfWonedotinvplussiO}
\begin{minipage}{\CoTfWonedotinvplussiH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=0b10|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(0x1000,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfW1.inv+si|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfWonedotinvplussiN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfWonedotinvplussiM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfWonedotinvplussiO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfWonedotinvplussiI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfWonedotinvplussiK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R0=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoWR.alias.tex <==
\newlength{\CoWRdotaliasH}
\setlength{\CoWRdotaliasH}{0cm}
\newsavebox{\CoWRdotaliasI}
\begin{lrbox}{\CoWRdotaliasI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWRdotaliasJ}
\settowidth{\CoWRdotaliasJ}{\usebox{\CoWRdotaliasI}}
\addtolength{\CoWRdotaliasH}{\CoWRdotaliasJ}
\newsavebox{\CoWRdotaliasK}
\begin{lrbox}{\CoWRdotaliasK}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    y |-> pa1;
    *pa1 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWRdotaliasL}
\settowidth{\CoWRdotaliasL}{\usebox{\CoWRdotaliasK}}
\newsavebox{\CoWRdotaliasM}
\begin{lrbox}{\CoWRdotaliasM}
\begin{minipage}{\CoWRdotaliasH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|R0=0x1|\\
\lstinline[language=IslaLitmusExp]|R1=x|\\
\lstinline[language=IslaLitmusExp]|R3=y|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWR.alias|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWRdotaliasL}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWRdotaliasK}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWRdotaliasM}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWRdotaliasI}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoWR.inv.tex <==
\newlength{\CoWRdotinvH}
\setlength{\CoWRdotinvH}{0cm}
\newsavebox{\CoWRdotinvI}
\begin{lrbox}{\CoWRdotinvI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWRdotinvJ}
\settowidth{\CoWRdotinvJ}{\usebox{\CoWRdotinvI}}
\addtolength{\CoWRdotinvH}{\CoWRdotinvJ}
\newsavebox{\CoWRdotinvK}
\begin{lrbox}{\CoWRdotinvK}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWRdotinvL}
\settowidth{\CoWRdotinvL}{\usebox{\CoWRdotinvK}}
\newsavebox{\CoWRdotinvM}
\begin{lrbox}{\CoWRdotinvM}
\begin{minipage}{\CoWRdotinvH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWR.inv|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWRdotinvL}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWRdotinvK}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWRdotinvM}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWRdotinvI}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoWTa1.1.inv+dsb-tlbiasidis-dsb-eret.tex <==
\newlength{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetH}
\setlength{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetH}{0cm}
\newsavebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetI}
\begin{lrbox}{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI ASIDE1IS,X4
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetJ}
\settowidth{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetJ}{\usebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetI}}
\addtolength{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetH}{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetJ}
\newsavebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetK}
\begin{lrbox}{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetL}
\settowidth{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetL}{\usebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetK}}
\addtolength{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetH}{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetL}
\newsavebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetM}
\begin{lrbox}{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;

    y |-> pa1;

    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetN}
\settowidth{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetN}{\usebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetM}}
\newsavebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetO}
\begin{lrbox}{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetO}
\begin{minipage}{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL1=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=asid(0x1)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL1=0b00000|\\
\lstinline[language=IslaLitmusExp]|TTBR0_EL1=ttbr(asid=0x0001,base=page_table_base)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTa1.1.inv+dsb-tlbiasidis-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoWTa2.1.inv+dsb-tlbiasidis-dsb-eret.tex <==
\newlength{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetH}
\setlength{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetH}{0cm}
\newsavebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetI}
\begin{lrbox}{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI ASIDE1IS,X4
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetJ}
\settowidth{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetJ}{\usebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetI}}
\addtolength{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetH}{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetJ}
\newsavebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetK}
\begin{lrbox}{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetL}
\settowidth{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetL}{\usebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetK}}
\addtolength{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetH}{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetL}
\newsavebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetM}
\begin{lrbox}{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;

    y |-> pa1;

    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetN}
\settowidth{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetN}{\usebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetM}}
\newsavebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetO}
\begin{lrbox}{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetO}
\begin{minipage}{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL1=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=asid(0x2)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL1=0b00000|\\
\lstinline[language=IslaLitmusExp]|TTBR0_EL1=ttbr(asid=0x0001,base=page_table_base)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTa2.1.inv+dsb-tlbiasidis-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoWTf.inv+_dmb_-dmb-addr.tex <==
\newlength{\CoWTfdotinvplus[dmb]dmbaddrH}
\setlength{\CoWTfdotinvplus[dmb]dmbaddrH}{0cm}
\newsavebox{\CoWTfdotinvplus[dmb]dmbaddrI}
\begin{lrbox}{\CoWTfdotinvplus[dmb]dmbaddrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X2,[X1]
DSB ST
LDR X3,[X4]
EOR X5,X3,X3
LDR X6,[X7,X5]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplus[dmb]dmbaddrJ}
\settowidth{\CoWTfdotinvplus[dmb]dmbaddrJ}{\usebox{\CoWTfdotinvplus[dmb]dmbaddrI}}
\addtolength{\CoWTfdotinvplus[dmb]dmbaddrH}{\CoWTfdotinvplus[dmb]dmbaddrJ}
\newsavebox{\CoWTfdotinvplus[dmb]dmbaddrK}
\begin{lrbox}{\CoWTfdotinvplus[dmb]dmbaddrK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplus[dmb]dmbaddrL}
\settowidth{\CoWTfdotinvplus[dmb]dmbaddrL}{\usebox{\CoWTfdotinvplus[dmb]dmbaddrK}}
\addtolength{\CoWTfdotinvplus[dmb]dmbaddrH}{\CoWTfdotinvplus[dmb]dmbaddrL}
\newsavebox{\CoWTfdotinvplus[dmb]dmbaddrM}
\begin{lrbox}{\CoWTfdotinvplus[dmb]dmbaddrM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X6,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplus[dmb]dmbaddrN}
\settowidth{\CoWTfdotinvplus[dmb]dmbaddrN}{\usebox{\CoWTfdotinvplus[dmb]dmbaddrM}}
\addtolength{\CoWTfdotinvplus[dmb]dmbaddrH}{\CoWTfdotinvplus[dmb]dmbaddrN}
\newsavebox{\CoWTfdotinvplus[dmb]dmbaddrO}
\begin{lrbox}{\CoWTfdotinvplus[dmb]dmbaddrO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplus[dmb]dmbaddrP}
\settowidth{\CoWTfdotinvplus[dmb]dmbaddrP}{\usebox{\CoWTfdotinvplus[dmb]dmbaddrO}}
\newsavebox{\CoWTfdotinvplus[dmb]dmbaddrA}
\begin{lrbox}{\CoWTfdotinvplus[dmb]dmbaddrA}
\begin{minipage}{\CoWTfdotinvplus[dmb]dmbaddrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R4=y|\\
\lstinline[language=IslaLitmusExp]|0:R7=x|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+[dmb]-dmb-addr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvplus[dmb]dmbaddrP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvplus[dmb]dmbaddrO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvplus[dmb]dmbaddrA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplus[dmb]dmbaddrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplus[dmb]dmbaddrK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplus[dmb]dmbaddrM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R3=2 & 0:R6=0 & 1:R0=desc3(z,page_table_base)|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoWTf.inv+dsb-isb.tex <==
\newlength{\CoWTfdotinvplusdsbisbH}
\setlength{\CoWTfdotinvplusdsbisbH}{0cm}
\newsavebox{\CoWTfdotinvplusdsbisbI}
\begin{lrbox}{\CoWTfdotinvplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusdsbisbJ}
\settowidth{\CoWTfdotinvplusdsbisbJ}{\usebox{\CoWTfdotinvplusdsbisbI}}
\addtolength{\CoWTfdotinvplusdsbisbH}{\CoWTfdotinvplusdsbisbJ}
\newsavebox{\CoWTfdotinvplusdsbisbK}
\begin{lrbox}{\CoWTfdotinvplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusdsbisbL}
\settowidth{\CoWTfdotinvplusdsbisbL}{\usebox{\CoWTfdotinvplusdsbisbK}}
\addtolength{\CoWTfdotinvplusdsbisbH}{\CoWTfdotinvplusdsbisbL}
\newsavebox{\CoWTfdotinvplusdsbisbM}
\begin{lrbox}{\CoWTfdotinvplusdsbisbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusdsbisbN}
\settowidth{\CoWTfdotinvplusdsbisbN}{\usebox{\CoWTfdotinvplusdsbisbM}}
\newsavebox{\CoWTfdotinvplusdsbisbO}
\begin{lrbox}{\CoWTfdotinvplusdsbisbO}
\begin{minipage}{\CoWTfdotinvplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvplusdsbisbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvplusdsbisbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvplusdsbisbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplusdsbisbI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplusdsbisbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoWTf.inv+po-ctrl+po.tex <==
\newlength{\CoWTfdotinvpluspoctrlpluspoH}
\setlength{\CoWTfdotinvpluspoctrlpluspoH}{0cm}
\newsavebox{\CoWTfdotinvpluspoctrlpluspoI}
\begin{lrbox}{\CoWTfdotinvpluspoctrlpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
CBNZ X2,L0
L0:
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlpluspoJ}
\settowidth{\CoWTfdotinvpluspoctrlpluspoJ}{\usebox{\CoWTfdotinvpluspoctrlpluspoI}}
\addtolength{\CoWTfdotinvpluspoctrlpluspoH}{\CoWTfdotinvpluspoctrlpluspoJ}
\newsavebox{\CoWTfdotinvpluspoctrlpluspoK}
\begin{lrbox}{\CoWTfdotinvpluspoctrlpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlpluspoL}
\settowidth{\CoWTfdotinvpluspoctrlpluspoL}{\usebox{\CoWTfdotinvpluspoctrlpluspoK}}
\addtolength{\CoWTfdotinvpluspoctrlpluspoH}{\CoWTfdotinvpluspoctrlpluspoL}
\newsavebox{\CoWTfdotinvpluspoctrlpluspoM}
\begin{lrbox}{\CoWTfdotinvpluspoctrlpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlpluspoN}
\settowidth{\CoWTfdotinvpluspoctrlpluspoN}{\usebox{\CoWTfdotinvpluspoctrlpluspoM}}
\addtolength{\CoWTfdotinvpluspoctrlpluspoH}{\CoWTfdotinvpluspoctrlpluspoN}
\newsavebox{\CoWTfdotinvpluspoctrlpluspoO}
\begin{lrbox}{\CoWTfdotinvpluspoctrlpluspoO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlpluspoP}
\settowidth{\CoWTfdotinvpluspoctrlpluspoP}{\usebox{\CoWTfdotinvpluspoctrlpluspoO}}
\addtolength{\CoWTfdotinvpluspoctrlpluspoH}{\CoWTfdotinvpluspoctrlpluspoP}
\newsavebox{\CoWTfdotinvpluspoctrlpluspoA}
\begin{lrbox}{\CoWTfdotinvpluspoctrlpluspoA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    *pa2 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlpluspoB}
\settowidth{\CoWTfdotinvpluspoctrlpluspoB}{\usebox{\CoWTfdotinvpluspoctrlpluspoA}}
\newsavebox{\CoWTfdotinvpluspoctrlpluspoC}
\begin{lrbox}{\CoWTfdotinvpluspoctrlpluspoC}
\begin{minipage}{\CoWTfdotinvpluspoctrlpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R5=x|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+po-ctrl+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvpluspoctrlpluspoB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvpluspoctrlpluspoA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvpluspoctrlpluspoC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoctrlpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoctrlpluspoK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoctrlpluspoM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoctrlpluspoO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=1 & 0:R4=0 & 1:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoWTf.inv+po-ctrl-isb+po.tex <==
\newlength{\CoWTfdotinvpluspoctrlisbpluspoH}
\setlength{\CoWTfdotinvpluspoctrlisbpluspoH}{0cm}
\newsavebox{\CoWTfdotinvpluspoctrlisbpluspoI}
\begin{lrbox}{\CoWTfdotinvpluspoctrlisbpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
CBNZ X2,L0
L0:
ISB
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlisbpluspoJ}
\settowidth{\CoWTfdotinvpluspoctrlisbpluspoJ}{\usebox{\CoWTfdotinvpluspoctrlisbpluspoI}}
\addtolength{\CoWTfdotinvpluspoctrlisbpluspoH}{\CoWTfdotinvpluspoctrlisbpluspoJ}
\newsavebox{\CoWTfdotinvpluspoctrlisbpluspoK}
\begin{lrbox}{\CoWTfdotinvpluspoctrlisbpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlisbpluspoL}
\settowidth{\CoWTfdotinvpluspoctrlisbpluspoL}{\usebox{\CoWTfdotinvpluspoctrlisbpluspoK}}
\addtolength{\CoWTfdotinvpluspoctrlisbpluspoH}{\CoWTfdotinvpluspoctrlisbpluspoL}
\newsavebox{\CoWTfdotinvpluspoctrlisbpluspoM}
\begin{lrbox}{\CoWTfdotinvpluspoctrlisbpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlisbpluspoN}
\settowidth{\CoWTfdotinvpluspoctrlisbpluspoN}{\usebox{\CoWTfdotinvpluspoctrlisbpluspoM}}
\addtolength{\CoWTfdotinvpluspoctrlisbpluspoH}{\CoWTfdotinvpluspoctrlisbpluspoN}
\newsavebox{\CoWTfdotinvpluspoctrlisbpluspoO}
\begin{lrbox}{\CoWTfdotinvpluspoctrlisbpluspoO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlisbpluspoP}
\settowidth{\CoWTfdotinvpluspoctrlisbpluspoP}{\usebox{\CoWTfdotinvpluspoctrlisbpluspoO}}
\addtolength{\CoWTfdotinvpluspoctrlisbpluspoH}{\CoWTfdotinvpluspoctrlisbpluspoP}
\newsavebox{\CoWTfdotinvpluspoctrlisbpluspoA}
\begin{lrbox}{\CoWTfdotinvpluspoctrlisbpluspoA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    *pa2 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlisbpluspoB}
\settowidth{\CoWTfdotinvpluspoctrlisbpluspoB}{\usebox{\CoWTfdotinvpluspoctrlisbpluspoA}}
\newsavebox{\CoWTfdotinvpluspoctrlisbpluspoC}
\begin{lrbox}{\CoWTfdotinvpluspoctrlisbpluspoC}
\begin{minipage}{\CoWTfdotinvpluspoctrlisbpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R5=x|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+po-ctrl-isb+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvpluspoctrlisbpluspoB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvpluspoctrlisbpluspoA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvpluspoctrlisbpluspoC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoctrlisbpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoctrlisbpluspoK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoctrlisbpluspoM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoctrlisbpluspoO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=1 & 0:R4=0 & 1:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoWTf.inv+po.tex <==
\newlength{\CoWTfdotinvpluspoH}
\setlength{\CoWTfdotinvpluspoH}{0cm}
\newsavebox{\CoWTfdotinvpluspoI}
\begin{lrbox}{\CoWTfdotinvpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoJ}
\settowidth{\CoWTfdotinvpluspoJ}{\usebox{\CoWTfdotinvpluspoI}}
\addtolength{\CoWTfdotinvpluspoH}{\CoWTfdotinvpluspoJ}
\newsavebox{\CoWTfdotinvpluspoK}
\begin{lrbox}{\CoWTfdotinvpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoL}
\settowidth{\CoWTfdotinvpluspoL}{\usebox{\CoWTfdotinvpluspoK}}
\addtolength{\CoWTfdotinvpluspoH}{\CoWTfdotinvpluspoL}
\newsavebox{\CoWTfdotinvpluspoM}
\begin{lrbox}{\CoWTfdotinvpluspoM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoN}
\settowidth{\CoWTfdotinvpluspoN}{\usebox{\CoWTfdotinvpluspoM}}
\newsavebox{\CoWTfdotinvpluspoO}
\begin{lrbox}{\CoWTfdotinvpluspoO}
\begin{minipage}{\CoWTfdotinvpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvpluspoN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvpluspoM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvpluspoO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoWTf.inv+poloc-ctrl-isb.tex <==
\newlength{\CoWTfdotinvpluspolocctrlisbH}
\setlength{\CoWTfdotinvpluspolocctrlisbH}{0cm}
\newsavebox{\CoWTfdotinvpluspolocctrlisbI}
\begin{lrbox}{\CoWTfdotinvpluspolocctrlisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X4,[X1]
CBNZ X4,L0
L0:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspolocctrlisbJ}
\settowidth{\CoWTfdotinvpluspolocctrlisbJ}{\usebox{\CoWTfdotinvpluspolocctrlisbI}}
\addtolength{\CoWTfdotinvpluspolocctrlisbH}{\CoWTfdotinvpluspolocctrlisbJ}
\newsavebox{\CoWTfdotinvpluspolocctrlisbK}
\begin{lrbox}{\CoWTfdotinvpluspolocctrlisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspolocctrlisbL}
\settowidth{\CoWTfdotinvpluspolocctrlisbL}{\usebox{\CoWTfdotinvpluspolocctrlisbK}}
\addtolength{\CoWTfdotinvpluspolocctrlisbH}{\CoWTfdotinvpluspolocctrlisbL}
\newsavebox{\CoWTfdotinvpluspolocctrlisbM}
\begin{lrbox}{\CoWTfdotinvpluspolocctrlisbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *y = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspolocctrlisbN}
\settowidth{\CoWTfdotinvpluspolocctrlisbN}{\usebox{\CoWTfdotinvpluspolocctrlisbM}}
\newsavebox{\CoWTfdotinvpluspolocctrlisbO}
\begin{lrbox}{\CoWTfdotinvpluspolocctrlisbO}
\begin{minipage}{\CoWTfdotinvpluspolocctrlisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+poloc-ctrl-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvpluspolocctrlisbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvpluspolocctrlisbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvpluspolocctrlisbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspolocctrlisbI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspolocctrlisbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoWTf.inv+rfi-addr.tex <==
\newlength{\CoWTfdotinvplusrfiaddrH}
\setlength{\CoWTfdotinvplusrfiaddrH}{0cm}
\newsavebox{\CoWTfdotinvplusrfiaddrI}
\begin{lrbox}{\CoWTfdotinvplusrfiaddrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusrfiaddrJ}
\settowidth{\CoWTfdotinvplusrfiaddrJ}{\usebox{\CoWTfdotinvplusrfiaddrI}}
\addtolength{\CoWTfdotinvplusrfiaddrH}{\CoWTfdotinvplusrfiaddrJ}
\newsavebox{\CoWTfdotinvplusrfiaddrK}
\begin{lrbox}{\CoWTfdotinvplusrfiaddrK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#0
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusrfiaddrL}
\settowidth{\CoWTfdotinvplusrfiaddrL}{\usebox{\CoWTfdotinvplusrfiaddrK}}
\addtolength{\CoWTfdotinvplusrfiaddrH}{\CoWTfdotinvplusrfiaddrL}
\newsavebox{\CoWTfdotinvplusrfiaddrM}
\begin{lrbox}{\CoWTfdotinvplusrfiaddrM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusrfiaddrN}
\settowidth{\CoWTfdotinvplusrfiaddrN}{\usebox{\CoWTfdotinvplusrfiaddrM}}
\newsavebox{\CoWTfdotinvplusrfiaddrO}
\begin{lrbox}{\CoWTfdotinvplusrfiaddrO}
\begin{minipage}{\CoWTfdotinvplusrfiaddrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R5=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+rfi-addr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvplusrfiaddrN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvplusrfiaddrM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvplusrfiaddrO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplusrfiaddrI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplusrfiaddrK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=desc3(y,page_table_base) & 0:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoWTf.inv+rfi-ctrl-isb.tex <==
\newlength{\CoWTfdotinvplusrfictrlisbH}
\setlength{\CoWTfdotinvplusrfictrlisbH}{0cm}
\newsavebox{\CoWTfdotinvplusrfictrlisbI}
\begin{lrbox}{\CoWTfdotinvplusrfictrlisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
CBNZ X2,L0
L0:
ISB
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusrfictrlisbJ}
\settowidth{\CoWTfdotinvplusrfictrlisbJ}{\usebox{\CoWTfdotinvplusrfictrlisbI}}
\addtolength{\CoWTfdotinvplusrfictrlisbH}{\CoWTfdotinvplusrfictrlisbJ}
\newsavebox{\CoWTfdotinvplusrfictrlisbK}
\begin{lrbox}{\CoWTfdotinvplusrfictrlisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusrfictrlisbL}
\settowidth{\CoWTfdotinvplusrfictrlisbL}{\usebox{\CoWTfdotinvplusrfictrlisbK}}
\addtolength{\CoWTfdotinvplusrfictrlisbH}{\CoWTfdotinvplusrfictrlisbL}
\newsavebox{\CoWTfdotinvplusrfictrlisbM}
\begin{lrbox}{\CoWTfdotinvplusrfictrlisbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    *pa2 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusrfictrlisbN}
\settowidth{\CoWTfdotinvplusrfictrlisbN}{\usebox{\CoWTfdotinvplusrfictrlisbM}}
\newsavebox{\CoWTfdotinvplusrfictrlisbO}
\begin{lrbox}{\CoWTfdotinvplusrfictrlisbO}
\begin{minipage}{\CoWTfdotinvplusrfictrlisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R5=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+rfi-ctrl-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvplusrfictrlisbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvplusrfictrlisbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvplusrfictrlisbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplusrfictrlisbI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplusrfictrlisbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=desc3(u,page_table_base) & 0:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoWTf.inv+svc.tex <==
\newlength{\CoWTfdotinvplussvcH}
\setlength{\CoWTfdotinvplussvcH}{0cm}
\newsavebox{\CoWTfdotinvplussvcI}
\begin{lrbox}{\CoWTfdotinvplussvcI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
SVC #0x0
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplussvcJ}
\settowidth{\CoWTfdotinvplussvcJ}{\usebox{\CoWTfdotinvplussvcI}}
\addtolength{\CoWTfdotinvplussvcH}{\CoWTfdotinvplussvcJ}
\newsavebox{\CoWTfdotinvplussvcK}
\begin{lrbox}{\CoWTfdotinvplussvcK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1200:
MOV X2,#0
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplussvcL}
\settowidth{\CoWTfdotinvplussvcL}{\usebox{\CoWTfdotinvplussvcK}}
\addtolength{\CoWTfdotinvplussvcH}{\CoWTfdotinvplussvcL}
\newsavebox{\CoWTfdotinvplussvcM}
\begin{lrbox}{\CoWTfdotinvplussvcM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS X10,ELR_EL1
LDR X2,[X3]
MSR ELR_EL1,X10
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplussvcN}
\settowidth{\CoWTfdotinvplussvcN}{\usebox{\CoWTfdotinvplussvcM}}
\addtolength{\CoWTfdotinvplussvcH}{\CoWTfdotinvplussvcN}
\newsavebox{\CoWTfdotinvplussvcO}
\begin{lrbox}{\CoWTfdotinvplussvcO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *y = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplussvcP}
\settowidth{\CoWTfdotinvplussvcP}{\usebox{\CoWTfdotinvplussvcO}}
\newsavebox{\CoWTfdotinvplussvcA}
\begin{lrbox}{\CoWTfdotinvplussvcA}
\begin{minipage}{\CoWTfdotinvplussvcH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+svc|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvplussvcP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvplussvcO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvplussvcA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplussvcI}\\
  \cline{2-2}
  & thread0 el1 handler same exc\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplussvcK}\\
  \cline{2-2}
  & thread0 el1 handler lower exc\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplussvcM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoWTf.inv.EL1+dsb-eret.tex <==
\newlength{\CoWTfdotinvdotELoneplusdsberetH}
\setlength{\CoWTfdotinvdotELoneplusdsberetH}{0cm}
\newsavebox{\CoWTfdotinvdotELoneplusdsberetI}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELoneplusdsberetJ}
\settowidth{\CoWTfdotinvdotELoneplusdsberetJ}{\usebox{\CoWTfdotinvdotELoneplusdsberetI}}
\addtolength{\CoWTfdotinvdotELoneplusdsberetH}{\CoWTfdotinvdotELoneplusdsberetJ}
\newsavebox{\CoWTfdotinvdotELoneplusdsberetK}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELoneplusdsberetL}
\settowidth{\CoWTfdotinvdotELoneplusdsberetL}{\usebox{\CoWTfdotinvdotELoneplusdsberetK}}
\addtolength{\CoWTfdotinvdotELoneplusdsberetH}{\CoWTfdotinvdotELoneplusdsberetL}
\newsavebox{\CoWTfdotinvdotELoneplusdsberetM}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *y = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELoneplusdsberetN}
\settowidth{\CoWTfdotinvdotELoneplusdsberetN}{\usebox{\CoWTfdotinvdotELoneplusdsberetM}}
\newsavebox{\CoWTfdotinvdotELoneplusdsberetO}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsberetO}
\begin{minipage}{\CoWTfdotinvdotELoneplusdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL1=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL1=0b00000|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv.EL1+dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvdotELoneplusdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvdotELoneplusdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvdotELoneplusdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELoneplusdsberetI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELoneplusdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoWTf.inv.EL1+dsb-svc.tex <==
\newlength{\CoWTfdotinvdotELoneplusdsbsvcH}
\setlength{\CoWTfdotinvdotELoneplusdsbsvcH}{0cm}
\newsavebox{\CoWTfdotinvdotELoneplusdsbsvcI}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsbsvcI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
SVC #0x0
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELoneplusdsbsvcJ}
\settowidth{\CoWTfdotinvdotELoneplusdsbsvcJ}{\usebox{\CoWTfdotinvdotELoneplusdsbsvcI}}
\addtolength{\CoWTfdotinvdotELoneplusdsbsvcH}{\CoWTfdotinvdotELoneplusdsbsvcJ}
\newsavebox{\CoWTfdotinvdotELoneplusdsbsvcK}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsbsvcK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1200:
MOV X2,#0
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELoneplusdsbsvcL}
\settowidth{\CoWTfdotinvdotELoneplusdsbsvcL}{\usebox{\CoWTfdotinvdotELoneplusdsbsvcK}}
\addtolength{\CoWTfdotinvdotELoneplusdsbsvcH}{\CoWTfdotinvdotELoneplusdsbsvcL}
\newsavebox{\CoWTfdotinvdotELoneplusdsbsvcM}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsbsvcM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS X10,ELR_EL1
LDR X2,[X3]
MSR ELR_EL1,X10
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELoneplusdsbsvcN}
\settowidth{\CoWTfdotinvdotELoneplusdsbsvcN}{\usebox{\CoWTfdotinvdotELoneplusdsbsvcM}}
\addtolength{\CoWTfdotinvdotELoneplusdsbsvcH}{\CoWTfdotinvdotELoneplusdsbsvcN}
\newsavebox{\CoWTfdotinvdotELoneplusdsbsvcO}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsbsvcO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *y = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELoneplusdsbsvcP}
\settowidth{\CoWTfdotinvdotELoneplusdsbsvcP}{\usebox{\CoWTfdotinvdotELoneplusdsbsvcO}}
\newsavebox{\CoWTfdotinvdotELoneplusdsbsvcA}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsbsvcA}
\begin{minipage}{\CoWTfdotinvdotELoneplusdsbsvcH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv.EL1+dsb-svc|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvdotELoneplusdsbsvcP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvdotELoneplusdsbsvcO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvdotELoneplusdsbsvcA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELoneplusdsbsvcI}\\
  \cline{2-2}
  & thread0 el1 handler same exc\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELoneplusdsbsvcK}\\
  \cline{2-2}
  & thread0 el1 handler lower exc\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELoneplusdsbsvcM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoWTf.inv.EL1+eret.tex <==
\newlength{\CoWTfdotinvdotELonepluseretH}
\setlength{\CoWTfdotinvdotELonepluseretH}{0cm}
\newsavebox{\CoWTfdotinvdotELonepluseretI}
\begin{lrbox}{\CoWTfdotinvdotELonepluseretI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELonepluseretJ}
\settowidth{\CoWTfdotinvdotELonepluseretJ}{\usebox{\CoWTfdotinvdotELonepluseretI}}
\addtolength{\CoWTfdotinvdotELonepluseretH}{\CoWTfdotinvdotELonepluseretJ}
\newsavebox{\CoWTfdotinvdotELonepluseretK}
\begin{lrbox}{\CoWTfdotinvdotELonepluseretK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELonepluseretL}
\settowidth{\CoWTfdotinvdotELonepluseretL}{\usebox{\CoWTfdotinvdotELonepluseretK}}
\addtolength{\CoWTfdotinvdotELonepluseretH}{\CoWTfdotinvdotELonepluseretL}
\newsavebox{\CoWTfdotinvdotELonepluseretM}
\begin{lrbox}{\CoWTfdotinvdotELonepluseretM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *y = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELonepluseretN}
\settowidth{\CoWTfdotinvdotELonepluseretN}{\usebox{\CoWTfdotinvdotELonepluseretM}}
\newsavebox{\CoWTfdotinvdotELonepluseretO}
\begin{lrbox}{\CoWTfdotinvdotELonepluseretO}
\begin{minipage}{\CoWTfdotinvdotELonepluseretH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL1=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL1=0b00000|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv.EL1+eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvdotELonepluseretN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvdotELonepluseretM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvdotELonepluseretO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELonepluseretI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELonepluseretK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoWTf.inv.EL2+dsb-tlbiipa-dsb-tlbiis-dsb-eret.tex <==
\newlength{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetH}
\setlength{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetH}{0cm}
\newsavebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetI}
\begin{lrbox}{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1,X4
DSB SY
TLBI VMALLE1IS
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetJ}
\settowidth{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetJ}{\usebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetI}}
\addtolength{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetH}{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetJ}
\newsavebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetK}
\begin{lrbox}{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X20,ELR_EL2
ADD X20,X20,#4
MSR ELR_EL2,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetL}
\settowidth{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetL}{\usebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetK}}
\addtolength{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetH}{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetL}
\newsavebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetM}
\begin{lrbox}{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;

    ipa1 |-> invalid;
    ipa1 ?-> pa1;

    *pa1 = 1;

    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetN}
\settowidth{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetN}{\usebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetM}}
\newsavebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetO}
\begin{lrbox}{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetO}
\begin{minipage}{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00100|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv.EL2+dsb-tlbiipa-dsb-tlbiis-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetI}\\
  \cline{2-2}
  & thread0 el2 handler lower exc\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoWTf.inv.EL2+po.tex <==
\newlength{\CoWTfdotinvdotELtwopluspoH}
\setlength{\CoWTfdotinvdotELtwopluspoH}{0cm}
\newsavebox{\CoWTfdotinvdotELtwopluspoI}
\begin{lrbox}{\CoWTfdotinvdotELtwopluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELtwopluspoJ}
\settowidth{\CoWTfdotinvdotELtwopluspoJ}{\usebox{\CoWTfdotinvdotELtwopluspoI}}
\addtolength{\CoWTfdotinvdotELtwopluspoH}{\CoWTfdotinvdotELtwopluspoJ}
\newsavebox{\CoWTfdotinvdotELtwopluspoK}
\begin{lrbox}{\CoWTfdotinvdotELtwopluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X20,ELR_EL2
ADD X20,X20,#4
MSR ELR_EL2,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELtwopluspoL}
\settowidth{\CoWTfdotinvdotELtwopluspoL}{\usebox{\CoWTfdotinvdotELtwopluspoK}}
\addtolength{\CoWTfdotinvdotELtwopluspoH}{\CoWTfdotinvdotELtwopluspoL}
\newsavebox{\CoWTfdotinvdotELtwopluspoM}
\begin{lrbox}{\CoWTfdotinvdotELtwopluspoM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;

    ipa1 |-> invalid;
    ipa1 ?-> pa1;

    *pa1 = 1;

    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELtwopluspoN}
\settowidth{\CoWTfdotinvdotELtwopluspoN}{\usebox{\CoWTfdotinvdotELtwopluspoM}}
\newsavebox{\CoWTfdotinvdotELtwopluspoO}
\begin{lrbox}{\CoWTfdotinvdotELtwopluspoO}
\begin{minipage}{\CoWTfdotinvdotELtwopluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00100|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv.EL2+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvdotELtwopluspoN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvdotELtwopluspoM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvdotELtwopluspoO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELtwopluspoI}\\
  \cline{2-2}
  & thread0 el2 handler lower exc\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELtwopluspoK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoWTv2.2.inv+dsb-tlbivmidis-dsb-eret.tex <==
\newlength{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetH}
\setlength{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetH}{0cm}
\newsavebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetI}
\begin{lrbox}{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VMALLS12E1IS
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetJ}
\settowidth{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetJ}{\usebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetI}}
\addtolength{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetH}{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetJ}
\newsavebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetK}
\begin{lrbox}{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetL}
\settowidth{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetL}{\usebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetK}}
\addtolength{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetH}{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetL}
\newsavebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetM}
\begin{lrbox}{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;
    ipa1 |-> invalid;
    ipa1 ?-> pa1;

    *pa1 = 1;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetN}
\settowidth{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetN}{\usebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetM}}
\newsavebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetO}
\begin{lrbox}{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetO}
\begin{minipage}{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00101|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTv2.2.inv+dsb-tlbivmidis-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetI}\\
  \cline{2-2}
  & thread0 el2 handler\\
  \cline{2-2}
  & \usebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoWW.alias.tex <==
\newlength{\CoWWdotaliasH}
\setlength{\CoWWdotaliasH}{0cm}
\newsavebox{\CoWWdotaliasI}
\begin{lrbox}{\CoWWdotaliasI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWWdotaliasJ}
\settowidth{\CoWWdotaliasJ}{\usebox{\CoWWdotaliasI}}
\addtolength{\CoWWdotaliasH}{\CoWWdotaliasJ}
\newsavebox{\CoWWdotaliasK}
\begin{lrbox}{\CoWWdotaliasK}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    y |-> pa1;
    *pa1 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWWdotaliasL}
\settowidth{\CoWWdotaliasL}{\usebox{\CoWWdotaliasK}}
\newsavebox{\CoWWdotaliasM}
\begin{lrbox}{\CoWWdotaliasM}
\begin{minipage}{\CoWWdotaliasH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=0b01|\\
\lstinline[language=IslaLitmusExp]|R1=x|\\
\lstinline[language=IslaLitmusExp]|R2=0b10|\\
\lstinline[language=IslaLitmusExp]|R3=y|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWW.alias|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWWdotaliasL}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWWdotaliasK}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWWdotaliasM}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWWdotaliasI}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|x=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoWinvRpte+po.tex <==
\newlength{\CoWinvRptepluspoH}
\setlength{\CoWinvRptepluspoH}{0cm}
\newsavebox{\CoWinvRptepluspoI}
\begin{lrbox}{\CoWinvRptepluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvRptepluspoJ}
\settowidth{\CoWinvRptepluspoJ}{\usebox{\CoWinvRptepluspoI}}
\addtolength{\CoWinvRptepluspoH}{\CoWinvRptepluspoJ}
\newsavebox{\CoWinvRptepluspoK}
\begin{lrbox}{\CoWinvRptepluspoK}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;

    *pa1 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvRptepluspoL}
\settowidth{\CoWinvRptepluspoL}{\usebox{\CoWinvRptepluspoK}}
\newsavebox{\CoWinvRptepluspoM}
\begin{lrbox}{\CoWinvRptepluspoM}
\begin{minipage}{\CoWinvRptepluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=0x0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvRpte+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvRptepluspoL}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvRptepluspoK}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvRptepluspoM}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvRptepluspoI}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|~0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoWinvT+dsb-isb.tex <==
\newlength{\CoWinvTplusdsbisbH}
\setlength{\CoWinvTplusdsbisbH}{0cm}
\newsavebox{\CoWinvTplusdsbisbI}
\begin{lrbox}{\CoWinvTplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTplusdsbisbJ}
\settowidth{\CoWinvTplusdsbisbJ}{\usebox{\CoWinvTplusdsbisbI}}
\addtolength{\CoWinvTplusdsbisbH}{\CoWinvTplusdsbisbJ}
\newsavebox{\CoWinvTplusdsbisbK}
\begin{lrbox}{\CoWinvTplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTplusdsbisbL}
\settowidth{\CoWinvTplusdsbisbL}{\usebox{\CoWinvTplusdsbisbK}}
\addtolength{\CoWinvTplusdsbisbH}{\CoWinvTplusdsbisbL}
\newsavebox{\CoWinvTplusdsbisbM}
\begin{lrbox}{\CoWinvTplusdsbisbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTplusdsbisbN}
\settowidth{\CoWinvTplusdsbisbN}{\usebox{\CoWinvTplusdsbisbM}}
\newsavebox{\CoWinvTplusdsbisbO}
\begin{lrbox}{\CoWinvTplusdsbisbO}
\begin{minipage}{\CoWinvTplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvT+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTplusdsbisbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTplusdsbisbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTplusdsbisbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTplusdsbisbI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTplusdsbisbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoWinvT+po.tex <==
\newlength{\CoWinvTpluspoH}
\setlength{\CoWinvTpluspoH}{0cm}
\newsavebox{\CoWinvTpluspoI}
\begin{lrbox}{\CoWinvTpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTpluspoJ}
\settowidth{\CoWinvTpluspoJ}{\usebox{\CoWinvTpluspoI}}
\addtolength{\CoWinvTpluspoH}{\CoWinvTpluspoJ}
\newsavebox{\CoWinvTpluspoK}
\begin{lrbox}{\CoWinvTpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTpluspoL}
\settowidth{\CoWinvTpluspoL}{\usebox{\CoWinvTpluspoK}}
\addtolength{\CoWinvTpluspoH}{\CoWinvTpluspoL}
\newsavebox{\CoWinvTpluspoM}
\begin{lrbox}{\CoWinvTpluspoM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTpluspoN}
\settowidth{\CoWinvTpluspoN}{\usebox{\CoWinvTpluspoM}}
\newsavebox{\CoWinvTpluspoO}
\begin{lrbox}{\CoWinvTpluspoO}
\begin{minipage}{\CoWinvTpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvT+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTpluspoN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTpluspoM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTpluspoO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTpluspoI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTpluspoK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoWinvT.EL1+dsb-tlbi-dsb-isb.tex <==
\newlength{\CoWinvTdotELoneplusdsbtlbidsbisbH}
\setlength{\CoWinvTdotELoneplusdsbtlbidsbisbH}{0cm}
\newsavebox{\CoWinvTdotELoneplusdsbtlbidsbisbI}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbidsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1,X5
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbidsbisbJ}
\settowidth{\CoWinvTdotELoneplusdsbtlbidsbisbJ}{\usebox{\CoWinvTdotELoneplusdsbtlbidsbisbI}}
\addtolength{\CoWinvTdotELoneplusdsbtlbidsbisbH}{\CoWinvTdotELoneplusdsbtlbidsbisbJ}
\newsavebox{\CoWinvTdotELoneplusdsbtlbidsbisbK}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbidsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1000:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbidsbisbL}
\settowidth{\CoWinvTdotELoneplusdsbtlbidsbisbL}{\usebox{\CoWinvTdotELoneplusdsbtlbidsbisbK}}
\addtolength{\CoWinvTdotELoneplusdsbtlbidsbisbH}{\CoWinvTdotELoneplusdsbtlbidsbisbL}
\newsavebox{\CoWinvTdotELoneplusdsbtlbidsbisbM}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbidsbisbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbidsbisbN}
\settowidth{\CoWinvTdotELoneplusdsbtlbidsbisbN}{\usebox{\CoWinvTdotELoneplusdsbtlbidsbisbM}}
\newsavebox{\CoWinvTdotELoneplusdsbtlbidsbisbO}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbidsbisbO}
\begin{minipage}{\CoWinvTdotELoneplusdsbtlbidsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R5=page(x)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvT.EL1+dsb-tlbi-dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTdotELoneplusdsbtlbidsbisbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTdotELoneplusdsbtlbidsbisbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTdotELoneplusdsbtlbidsbisbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTdotELoneplusdsbtlbidsbisbI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTdotELoneplusdsbtlbidsbisbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoWinvT.EL1+dsb-tlbi-dsb.tex <==
\newlength{\CoWinvTdotELoneplusdsbtlbidsbH}
\setlength{\CoWinvTdotELoneplusdsbtlbidsbH}{0cm}
\newsavebox{\CoWinvTdotELoneplusdsbtlbidsbI}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbidsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1,X5
DSB SY
MOV X2,#0
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbidsbJ}
\settowidth{\CoWinvTdotELoneplusdsbtlbidsbJ}{\usebox{\CoWinvTdotELoneplusdsbtlbidsbI}}
\addtolength{\CoWinvTdotELoneplusdsbtlbidsbH}{\CoWinvTdotELoneplusdsbtlbidsbJ}
\newsavebox{\CoWinvTdotELoneplusdsbtlbidsbK}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbidsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1000:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbidsbL}
\settowidth{\CoWinvTdotELoneplusdsbtlbidsbL}{\usebox{\CoWinvTdotELoneplusdsbtlbidsbK}}
\addtolength{\CoWinvTdotELoneplusdsbtlbidsbH}{\CoWinvTdotELoneplusdsbtlbidsbL}
\newsavebox{\CoWinvTdotELoneplusdsbtlbidsbM}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbidsbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbidsbN}
\settowidth{\CoWinvTdotELoneplusdsbtlbidsbN}{\usebox{\CoWinvTdotELoneplusdsbtlbidsbM}}
\newsavebox{\CoWinvTdotELoneplusdsbtlbidsbO}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbidsbO}
\begin{minipage}{\CoWinvTdotELoneplusdsbtlbidsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R5=page(x)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvT.EL1+dsb-tlbi-dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTdotELoneplusdsbtlbidsbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTdotELoneplusdsbtlbidsbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTdotELoneplusdsbtlbidsbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTdotELoneplusdsbtlbidsbI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTdotELoneplusdsbtlbidsbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoWinvT.EL1+dsb-tlbiis-dsb-isb.tex <==
\newlength{\CoWinvTdotELoneplusdsbtlbiisdsbisbH}
\setlength{\CoWinvTdotELoneplusdsbtlbiisdsbisbH}{0cm}
\newsavebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbI}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbiisdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X5
DSB SY
ISB
MOV X2,#0
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbiisdsbisbJ}
\settowidth{\CoWinvTdotELoneplusdsbtlbiisdsbisbJ}{\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbI}}
\addtolength{\CoWinvTdotELoneplusdsbtlbiisdsbisbH}{\CoWinvTdotELoneplusdsbtlbiisdsbisbJ}
\newsavebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbK}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbiisdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1000:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbiisdsbisbL}
\settowidth{\CoWinvTdotELoneplusdsbtlbiisdsbisbL}{\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbK}}
\addtolength{\CoWinvTdotELoneplusdsbtlbiisdsbisbH}{\CoWinvTdotELoneplusdsbtlbiisdsbisbL}
\newsavebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbM}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbiisdsbisbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbiisdsbisbN}
\settowidth{\CoWinvTdotELoneplusdsbtlbiisdsbisbN}{\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbM}}
\newsavebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbO}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbiisdsbisbO}
\begin{minipage}{\CoWinvTdotELoneplusdsbtlbiisdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R5=page(x)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvT.EL1+dsb-tlbiis-dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTdotELoneplusdsbtlbiisdsbisbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoWinvT.EL1+dsb-tlbiis-dsb.tex <==
\newlength{\CoWinvTdotELoneplusdsbtlbiisdsbH}
\setlength{\CoWinvTdotELoneplusdsbtlbiisdsbH}{0cm}
\newsavebox{\CoWinvTdotELoneplusdsbtlbiisdsbI}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbiisdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X5
DSB SY
MOV X2,#0
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbiisdsbJ}
\settowidth{\CoWinvTdotELoneplusdsbtlbiisdsbJ}{\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbI}}
\addtolength{\CoWinvTdotELoneplusdsbtlbiisdsbH}{\CoWinvTdotELoneplusdsbtlbiisdsbJ}
\newsavebox{\CoWinvTdotELoneplusdsbtlbiisdsbK}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbiisdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1000:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbiisdsbL}
\settowidth{\CoWinvTdotELoneplusdsbtlbiisdsbL}{\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbK}}
\addtolength{\CoWinvTdotELoneplusdsbtlbiisdsbH}{\CoWinvTdotELoneplusdsbtlbiisdsbL}
\newsavebox{\CoWinvTdotELoneplusdsbtlbiisdsbM}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbiisdsbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbiisdsbN}
\settowidth{\CoWinvTdotELoneplusdsbtlbiisdsbN}{\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbM}}
\newsavebox{\CoWinvTdotELoneplusdsbtlbiisdsbO}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbiisdsbO}
\begin{minipage}{\CoWinvTdotELoneplusdsbtlbiisdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R5=page(x)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvT.EL1+dsb-tlbiis-dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTdotELoneplusdsbtlbiisdsbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTdotELoneplusdsbtlbiisdsbI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTdotELoneplusdsbtlbiisdsbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoWinvT2+dsb-tlbiipa-dsb-eret.tex <==
\newlength{\CoWinvTtwoplusdsbtlbiipadsberetH}
\setlength{\CoWinvTtwoplusdsbtlbiipadsberetH}{0cm}
\newsavebox{\CoWinvTtwoplusdsbtlbiipadsberetI}
\begin{lrbox}{\CoWinvTtwoplusdsbtlbiipadsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1,X4
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTtwoplusdsbtlbiipadsberetJ}
\settowidth{\CoWinvTtwoplusdsbtlbiipadsberetJ}{\usebox{\CoWinvTtwoplusdsbtlbiipadsberetI}}
\addtolength{\CoWinvTtwoplusdsbtlbiipadsberetH}{\CoWinvTtwoplusdsbtlbiipadsberetJ}
\newsavebox{\CoWinvTtwoplusdsbtlbiipadsberetK}
\begin{lrbox}{\CoWinvTtwoplusdsbtlbiipadsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X20,ELR_EL2
ADD X20,X20,#4
MSR ELR_EL2,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTtwoplusdsbtlbiipadsberetL}
\settowidth{\CoWinvTtwoplusdsbtlbiipadsberetL}{\usebox{\CoWinvTtwoplusdsbtlbiipadsberetK}}
\addtolength{\CoWinvTtwoplusdsbtlbiipadsberetH}{\CoWinvTtwoplusdsbtlbiipadsberetL}
\newsavebox{\CoWinvTtwoplusdsbtlbiipadsberetM}
\begin{lrbox}{\CoWinvTtwoplusdsbtlbiipadsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;

    ipa1 |-> invalid;
    ipa1 ?-> pa1;

    *pa1 = 1;

    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTtwoplusdsbtlbiipadsberetN}
\settowidth{\CoWinvTtwoplusdsbtlbiipadsberetN}{\usebox{\CoWinvTtwoplusdsbtlbiipadsberetM}}
\newsavebox{\CoWinvTtwoplusdsbtlbiipadsberetO}
\begin{lrbox}{\CoWinvTtwoplusdsbtlbiipadsberetO}
\begin{minipage}{\CoWinvTtwoplusdsbtlbiipadsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=page(ipa1)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00100|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvT2+dsb-tlbiipa-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTtwoplusdsbtlbiipadsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTtwoplusdsbtlbiipadsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTtwoplusdsbtlbiipadsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTtwoplusdsbtlbiipadsberetI}\\
  \cline{2-2}
  & thread0 el2 handler lower exc\\
  \cline{2-2}
  & \usebox{\CoWinvTtwoplusdsbtlbiipadsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoWinvT2+dsb-tlbiipa-dsb-tlbivmall-dsb-eret.tex <==
\newlength{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetH}
\setlength{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetH}{0cm}
\newsavebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetI}
\begin{lrbox}{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1,X4
DSB SY
TLBI VMALLE1
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetJ}
\settowidth{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetJ}{\usebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetI}}
\addtolength{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetH}{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetJ}
\newsavebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetK}
\begin{lrbox}{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#1
MRS X20,ELR_EL2
ADD X20,X20,#4
MSR ELR_EL2,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetL}
\settowidth{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetL}{\usebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetK}}
\addtolength{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetH}{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetL}
\newsavebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetM}
\begin{lrbox}{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;

    ipa1 |-> pa1;
    ipa1 ?-> invalid;

    *pa1 = 0;

    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetN}
\settowidth{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetN}{\usebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetM}}
\newsavebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetO}
\begin{lrbox}{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetO}
\begin{minipage}{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=page(ipa1)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00100|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvT2+dsb-tlbiipa-dsb-tlbivmall-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetI}\\
  \cline{2-2}
  & thread0 el2 handler lower exc\\
  \cline{2-2}
  & \usebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoWinvTa1.1+dsb-tlbiasidis-dsb-eret.tex <==
\newlength{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetH}
\setlength{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetH}{0cm}
\newsavebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetI}
\begin{lrbox}{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI ASIDE1IS,X4
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetJ}
\settowidth{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetJ}{\usebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetI}}
\addtolength{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetH}{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetJ}
\newsavebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetK}
\begin{lrbox}{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetL}
\settowidth{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetL}{\usebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetK}}
\addtolength{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetH}{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetL}
\newsavebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetM}
\begin{lrbox}{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetN}
\settowidth{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetN}{\usebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetM}}
\newsavebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetO}
\begin{lrbox}{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetO}
\begin{minipage}{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL1=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=asid(0x1)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL1=0b00000|\\
\lstinline[language=IslaLitmusExp]|TTBR0_EL1=ttbr(asid=0x0001,base=page_table_base)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvTa1.1+dsb-tlbiasidis-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoWinvTa2.1+dsb-tlbiasidis-dsb-eret.tex <==
\newlength{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetH}
\setlength{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetH}{0cm}
\newsavebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetI}
\begin{lrbox}{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI ASIDE1IS,X4
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetJ}
\settowidth{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetJ}{\usebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetI}}
\addtolength{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetH}{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetJ}
\newsavebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetK}
\begin{lrbox}{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetL}
\settowidth{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetL}{\usebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetK}}
\addtolength{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetH}{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetL}
\newsavebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetM}
\begin{lrbox}{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetN}
\settowidth{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetN}{\usebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetM}}
\newsavebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetO}
\begin{lrbox}{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetO}
\begin{minipage}{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL1=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=asid(0x2)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL1=0b00000|\\
\lstinline[language=IslaLitmusExp]|TTBR0_EL1=ttbr(base=page_table_base,asid=0x0001)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvTa2.1+dsb-tlbiasidis-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoWinvTv1.2+dsb-tlbivmidis-dsb-eret.tex <==
\newlength{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetH}
\setlength{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetH}{0cm}
\newsavebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetI}
\begin{lrbox}{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VMALLS12E1IS
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetJ}
\settowidth{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetJ}{\usebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetI}}
\addtolength{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetH}{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetJ}
\newsavebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetK}
\begin{lrbox}{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#1
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetL}
\settowidth{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetL}{\usebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetK}}
\addtolength{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetH}{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetL}
\newsavebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetM}
\begin{lrbox}{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;
    ipa1 |-> pa1;
    ipa1 ?-> invalid;

    *pa1 = 0;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetN}
\settowidth{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetN}{\usebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetM}}
\newsavebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetO}
\begin{lrbox}{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetO}
\begin{minipage}{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00101|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvTv1.2+dsb-tlbivmidis-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetI}\\
  \cline{2-2}
  & thread0 el2 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/CoWinvTv2.2+dsb-tlbivmidis-msrvttbr-dsb-eret.tex <==
\newlength{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetH}
\setlength{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetH}{0cm}
\newsavebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetI}
\begin{lrbox}{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VMALLS12E1IS
DSB SY
MSR VTTBR_EL2,X4
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetJ}
\settowidth{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetJ}{\usebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetI}}
\addtolength{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetH}{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetJ}
\newsavebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetK}
\begin{lrbox}{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#1
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetL}
\settowidth{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetL}{\usebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetK}}
\addtolength{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetH}{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetL}
\newsavebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetM}
\begin{lrbox}{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;
    ipa1 |-> pa1;
    ipa1 ?-> invalid;

    *pa1 = 0;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetN}
\settowidth{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetN}{\usebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetM}}
\newsavebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetO}
\begin{lrbox}{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetO}
\begin{minipage}{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=ttbr(base=s2_page_table_base,vmid=0x0001)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00101|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvTv2.2+dsb-tlbivmidis-msrvttbr-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetI}\\
  \cline{2-2}
  & thread0 el2 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/ETS.tex <==
\newlength{\ETSH}
\setlength{\ETSH}{0cm}
\newsavebox{\ETSI}
\begin{lrbox}{\ETSI}
\begin{lstlisting}[language=AArch64,showlines=true]
MOV X0,#1
STR X0,[X3]
DMB SY
STR X0,[X2]
\end{lstlisting}
\end{lrbox}
\newlength{\ETSJ}
\settowidth{\ETSJ}{\usebox{\ETSI}}
\addtolength{\ETSH}{\ETSJ}
\newsavebox{\ETSK}
\begin{lrbox}{\ETSK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X2]
STR X0,[X1]
MOV X4,#2
STR X4,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\ETSL}
\settowidth{\ETSL}{\usebox{\ETSK}}
\addtolength{\ETSH}{\ETSL}
\newsavebox{\ETSM}
\begin{lrbox}{\ETSM}
\begin{lstlisting}[language=AArch64,showlines=true]
MOV X0,#0
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\ETSN}
\settowidth{\ETSN}{\usebox{\ETSM}}
\addtolength{\ETSH}{\ETSN}
\newsavebox{\ETSO}
\begin{lrbox}{\ETSO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
LDR X7,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\ETSP}
\settowidth{\ETSP}{\usebox{\ETSO}}
\addtolength{\ETSH}{\ETSP}
\newsavebox{\ETSA}
\begin{lrbox}{\ETSA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> pa1;
    x ?-> invalid;
    y |-> pa2;
    z |-> pa3;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\ETSB}
\settowidth{\ETSB}{\usebox{\ETSA}}
\newsavebox{\ETSC}
\begin{lrbox}{\ETSC}
\begin{minipage}{\ETSH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R2=y|\\
\lstinline[language=IslaLitmusExp]|0:R3=z|\\
\lstinline[language=IslaLitmusExp]|1:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=z|\\
\lstinline[language=IslaLitmusExp]|1:R6=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R7=0b1|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:R1=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|ETS|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\ETSB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\ETSA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\ETSC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\ETSI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\ETSK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\ETSM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\ETSO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & x=1 & 1:R7=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/IRIW.TTf.TTf.inv+addrs.tex <==
\newlength{\IRIWdotTTfdotTTfdotinvplusaddrsH}
\setlength{\IRIWdotTTfdotTTfdotinvplusaddrsH}{0cm}
\newsavebox{\IRIWdotTTfdotTTfdotinvplusaddrsI}
\begin{lrbox}{\IRIWdotTTfdotTTfdotinvplusaddrsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\IRIWdotTTfdotTTfdotinvplusaddrsJ}
\settowidth{\IRIWdotTTfdotTTfdotinvplusaddrsJ}{\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsI}}
\addtolength{\IRIWdotTTfdotTTfdotinvplusaddrsH}{\IRIWdotTTfdotTTfdotinvplusaddrsJ}
\newsavebox{\IRIWdotTTfdotTTfdotinvplusaddrsK}
\begin{lrbox}{\IRIWdotTTfdotTTfdotinvplusaddrsK}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\IRIWdotTTfdotTTfdotinvplusaddrsL}
\settowidth{\IRIWdotTTfdotTTfdotinvplusaddrsL}{\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsK}}
\addtolength{\IRIWdotTTfdotTTfdotinvplusaddrsH}{\IRIWdotTTfdotTTfdotinvplusaddrsL}
\newsavebox{\IRIWdotTTfdotTTfdotinvplusaddrsM}
\begin{lrbox}{\IRIWdotTTfdotTTfdotinvplusaddrsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\IRIWdotTTfdotTTfdotinvplusaddrsN}
\settowidth{\IRIWdotTTfdotTTfdotinvplusaddrsN}{\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsM}}
\addtolength{\IRIWdotTTfdotTTfdotinvplusaddrsH}{\IRIWdotTTfdotTTfdotinvplusaddrsN}
\newsavebox{\IRIWdotTTfdotTTfdotinvplusaddrsO}
\begin{lrbox}{\IRIWdotTTfdotTTfdotinvplusaddrsO}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\IRIWdotTTfdotTTfdotinvplusaddrsP}
\settowidth{\IRIWdotTTfdotTTfdotinvplusaddrsP}{\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsO}}
\addtolength{\IRIWdotTTfdotTTfdotinvplusaddrsH}{\IRIWdotTTfdotTTfdotinvplusaddrsP}
\newsavebox{\IRIWdotTTfdotTTfdotinvplusaddrsA}
\begin{lrbox}{\IRIWdotTTfdotTTfdotinvplusaddrsA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\IRIWdotTTfdotTTfdotinvplusaddrsB}
\settowidth{\IRIWdotTTfdotTTfdotinvplusaddrsB}{\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsA}}
\addtolength{\IRIWdotTTfdotTTfdotinvplusaddrsH}{\IRIWdotTTfdotTTfdotinvplusaddrsB}
\newsavebox{\IRIWdotTTfdotTTfdotinvplusaddrsC}
\begin{lrbox}{\IRIWdotTTfdotTTfdotinvplusaddrsC}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\IRIWdotTTfdotTTfdotinvplusaddrsD}
\settowidth{\IRIWdotTTfdotTTfdotinvplusaddrsD}{\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsC}}
\addtolength{\IRIWdotTTfdotTTfdotinvplusaddrsH}{\IRIWdotTTfdotTTfdotinvplusaddrsD}
\newsavebox{\IRIWdotTTfdotTTfdotinvplusaddrsE}
\begin{lrbox}{\IRIWdotTTfdotTTfdotinvplusaddrsE}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> invalid;
    y ?-> pa2;
    v |-> pa2;
    *pa2 = 1;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\IRIWdotTTfdotTTfdotinvplusaddrsF}
\settowidth{\IRIWdotTTfdotTTfdotinvplusaddrsF}{\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsE}}
\newsavebox{\IRIWdotTTfdotTTfdotinvplusaddrsHG}
\begin{lrbox}{\IRIWdotTTfdotTTfdotinvplusaddrsHG}
\begin{minipage}{\IRIWdotTTfdotTTfdotinvplusaddrsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R0=desc3(v,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=x|\\
\lstinline[language=IslaLitmusExp]|2:R3=y|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|3:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|3:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|3:R1=y|\\
\lstinline[language=IslaLitmusExp]|3:R3=x|\\
\lstinline[language=IslaLitmusExp]|3:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|IRIW.TTf.TTf.inv+addrs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\IRIWdotTTfdotTTfdotinvplusaddrsF}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsE}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsHG}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\IRIWdotTTfdotTTfdotinvplusaddrsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\IRIWdotTTfdotTTfdotinvplusaddrsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\IRIWdotTTfdotTTfdotinvplusaddrsM}\\
  \cline{2-2}
  & Thread 3\\
  \cline{2-2}
  & \usebox{\IRIWdotTTfdotTTfdotinvplusaddrsO}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\IRIWdotTTfdotTTfdotinvplusaddrsA}\\
  \cline{2-2}
  & thread3 el1 handler\\
  \cline{2-2}
  & \usebox{\IRIWdotTTfdotTTfdotinvplusaddrsC}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|2:R0=1 & 2:R2=0 & 3:R0=1 & 3:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/ISA2.RRTf.inv+dsb+addr+addr.tex <==
\newlength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrH}
\setlength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrH}{0cm}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrI}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrJ}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrJ}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrI}}
\addtolength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrH}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrJ}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrK}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
STR X3,[X4,X2]
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrL}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrL}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrK}}
\addtolength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrH}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrL}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrM}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
LDR X3,[X4,X2]
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrN}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrN}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrM}}
\addtolength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrH}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrN}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrO}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X3,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrP}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrP}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrO}}
\addtolength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrH}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrP}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrA}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    *pa2 = 0;

    z |-> pa3;
    *pa3 = 0;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrB}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrB}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrA}}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrC}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrC}
\begin{minipage}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R4=z|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=z|\\
\lstinline[language=IslaLitmusExp]|2:R4=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|ISA2.RRTf.inv+dsb+addr+addr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrM}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R3=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/ISA2.RRTf.inv+dsb+data+addr.tex <==
\newlength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrH}
\setlength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrH}{0cm}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrI}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrJ}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrJ}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrI}}
\addtolength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrH}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrJ}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrK}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
ORR X3,X3,X2
STR X3,[X4]
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrL}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrL}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrK}}
\addtolength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrH}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrL}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrM}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
LDR X3,[X4,X2]
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrN}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrN}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrM}}
\addtolength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrH}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrN}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrO}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X3,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrP}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrP}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrO}}
\addtolength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrH}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrP}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrA}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    *pa2 = 0;

    z |-> pa3;
    *pa3 = 0;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrB}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrB}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrA}}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrC}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrC}
\begin{minipage}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R4=z|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=z|\\
\lstinline[language=IslaLitmusExp]|2:R4=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|ISA2.RRTf.inv+dsb+data+addr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrM}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R3=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/LB+addr-trfis.tex <==
\newlength{\LBplusaddrtrfisH}
\setlength{\LBplusaddrtrfisH}{0cm}
\newsavebox{\LBplusaddrtrfisI}
\begin{lrbox}{\LBplusaddrtrfisI}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
STR X3,[X4,X2]
STR X5,[X6]
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusaddrtrfisJ}
\settowidth{\LBplusaddrtrfisJ}{\usebox{\LBplusaddrtrfisI}}
\addtolength{\LBplusaddrtrfisH}{\LBplusaddrtrfisJ}
\newsavebox{\LBplusaddrtrfisK}
\begin{lrbox}{\LBplusaddrtrfisK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
STR X3,[X4,X2]
STR X5,[X6]
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusaddrtrfisL}
\settowidth{\LBplusaddrtrfisL}{\usebox{\LBplusaddrtrfisK}}
\addtolength{\LBplusaddrtrfisH}{\LBplusaddrtrfisL}
\newsavebox{\LBplusaddrtrfisM}
\begin{lrbox}{\LBplusaddrtrfisM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X7,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusaddrtrfisN}
\settowidth{\LBplusaddrtrfisN}{\usebox{\LBplusaddrtrfisM}}
\addtolength{\LBplusaddrtrfisH}{\LBplusaddrtrfisN}
\newsavebox{\LBplusaddrtrfisO}
\begin{lrbox}{\LBplusaddrtrfisO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X7,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusaddrtrfisP}
\settowidth{\LBplusaddrtrfisP}{\usebox{\LBplusaddrtrfisO}}
\addtolength{\LBplusaddrtrfisH}{\LBplusaddrtrfisP}
\newsavebox{\LBplusaddrtrfisA}
\begin{lrbox}{\LBplusaddrtrfisA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3 pa4;
    x |-> pa1;
    y |-> pa2;
    u |-> invalid;
    u ?-> pa2;
    v |-> invalid;
    v ?-> pa1;
    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusaddrtrfisB}
\settowidth{\LBplusaddrtrfisB}{\usebox{\LBplusaddrtrfisA}}
\newsavebox{\LBplusaddrtrfisC}
\begin{lrbox}{\LBplusaddrtrfisC}
\begin{minipage}{\LBplusaddrtrfisH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R3=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R4=pte3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R5=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R6=u|\\
\lstinline[language=IslaLitmusExp]|0:R7=0b1|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|0:__isla_monomorphize_writes=true|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=desc3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R4=pte3(v,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R5=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R6=v|\\
\lstinline[language=IslaLitmusExp]|1:R7=0b1|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\lstinline[language=IslaLitmusExp]|1:__isla_monomorphize_writes=true|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|LB+addr-trfis|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\LBplusaddrtrfisB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\LBplusaddrtrfisA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\LBplusaddrtrfisC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\LBplusaddrtrfisI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\LBplusaddrtrfisK}\\
  \cline{2-2}
  & thread1 el0 handler\\
  \cline{2-2}
  & \usebox{\LBplusaddrtrfisM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\LBplusaddrtrfisO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R0=1 & 0:R7=1 & 1:R0=1 & 1:R7=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/LB+data-trfis.tex <==
\newlength{\LBplusdatatrfisH}
\setlength{\LBplusdatatrfisH}{0cm}
\newsavebox{\LBplusdatatrfisI}
\begin{lrbox}{\LBplusdatatrfisI}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
ORR X3,X3,X2
STR X3,[X4]
STR X5,[X6]
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusdatatrfisJ}
\settowidth{\LBplusdatatrfisJ}{\usebox{\LBplusdatatrfisI}}
\addtolength{\LBplusdatatrfisH}{\LBplusdatatrfisJ}
\newsavebox{\LBplusdatatrfisK}
\begin{lrbox}{\LBplusdatatrfisK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
ORR X3,X3,X2
STR X3,[X4]
STR X5,[X6]
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusdatatrfisL}
\settowidth{\LBplusdatatrfisL}{\usebox{\LBplusdatatrfisK}}
\addtolength{\LBplusdatatrfisH}{\LBplusdatatrfisL}
\newsavebox{\LBplusdatatrfisM}
\begin{lrbox}{\LBplusdatatrfisM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X7,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusdatatrfisN}
\settowidth{\LBplusdatatrfisN}{\usebox{\LBplusdatatrfisM}}
\addtolength{\LBplusdatatrfisH}{\LBplusdatatrfisN}
\newsavebox{\LBplusdatatrfisO}
\begin{lrbox}{\LBplusdatatrfisO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X7,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusdatatrfisP}
\settowidth{\LBplusdatatrfisP}{\usebox{\LBplusdatatrfisO}}
\addtolength{\LBplusdatatrfisH}{\LBplusdatatrfisP}
\newsavebox{\LBplusdatatrfisA}
\begin{lrbox}{\LBplusdatatrfisA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3 pa4;
    x |-> pa1;
    y |-> pa2;
    u |-> invalid;
    u ?-> pa2;
    v |-> invalid;
    v ?-> pa1;
    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusdatatrfisB}
\settowidth{\LBplusdatatrfisB}{\usebox{\LBplusdatatrfisA}}
\newsavebox{\LBplusdatatrfisC}
\begin{lrbox}{\LBplusdatatrfisC}
\begin{minipage}{\LBplusdatatrfisH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R3=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R4=pte3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R5=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R6=u|\\
\lstinline[language=IslaLitmusExp]|0:R7=0b1|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=desc3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R4=pte3(v,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R5=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R6=v|\\
\lstinline[language=IslaLitmusExp]|1:R7=0b1|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|LB+data-trfis|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\LBplusdatatrfisB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\LBplusdatatrfisA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\LBplusdatatrfisC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\LBplusdatatrfisI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\LBplusdatatrfisK}\\
  \cline{2-2}
  & thread1 el0 handler\\
  \cline{2-2}
  & \usebox{\LBplusdatatrfisM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\LBplusdatatrfisO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R0=1 & 0:R7=1 & 1:R0=1 & 1:R7=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/LB.TT.inv+pos.tex <==
\newlength{\LBdotTTdotinvplusposH}
\setlength{\LBdotTTdotinvplusposH}{0cm}
\newsavebox{\LBdotTTdotinvplusposI}
\begin{lrbox}{\LBdotTTdotinvplusposI}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\LBdotTTdotinvplusposJ}
\settowidth{\LBdotTTdotinvplusposJ}{\usebox{\LBdotTTdotinvplusposI}}
\addtolength{\LBdotTTdotinvplusposH}{\LBdotTTdotinvplusposJ}
\newsavebox{\LBdotTTdotinvplusposK}
\begin{lrbox}{\LBdotTTdotinvplusposK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\LBdotTTdotinvplusposL}
\settowidth{\LBdotTTdotinvplusposL}{\usebox{\LBdotTTdotinvplusposK}}
\addtolength{\LBdotTTdotinvplusposH}{\LBdotTTdotinvplusposL}
\newsavebox{\LBdotTTdotinvplusposM}
\begin{lrbox}{\LBdotTTdotinvplusposM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\LBdotTTdotinvplusposN}
\settowidth{\LBdotTTdotinvplusposN}{\usebox{\LBdotTTdotinvplusposM}}
\addtolength{\LBdotTTdotinvplusposH}{\LBdotTTdotinvplusposN}
\newsavebox{\LBdotTTdotinvplusposO}
\begin{lrbox}{\LBdotTTdotinvplusposO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\LBdotTTdotinvplusposP}
\settowidth{\LBdotTTdotinvplusposP}{\usebox{\LBdotTTdotinvplusposO}}
\addtolength{\LBdotTTdotinvplusposH}{\LBdotTTdotinvplusposP}
\newsavebox{\LBdotTTdotinvplusposA}
\begin{lrbox}{\LBdotTTdotinvplusposA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    y |-> invalid;

    x ?-> pa1;
    y ?-> pa1;

    *pa1 = 1;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\LBdotTTdotinvplusposB}
\settowidth{\LBdotTTdotinvplusposB}{\usebox{\LBdotTTdotinvplusposA}}
\newsavebox{\LBdotTTdotinvplusposC}
\begin{lrbox}{\LBdotTTdotinvplusposC}
\begin{minipage}{\LBdotTTdotinvplusposH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|LB.TT.inv+pos|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\LBdotTTdotinvplusposB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\LBdotTTdotinvplusposA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\LBdotTTdotinvplusposC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\LBdotTTdotinvplusposI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\LBdotTTdotinvplusposK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\LBdotTTdotinvplusposM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\LBdotTTdotinvplusposO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R0=1 & 1:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.BBM1+dsb-tlbiis-dsb-dsb+ctrl-isb.tex <==
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbH}
\setlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbH}{0cm}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbI}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X6
DSB SY
STR X2,[X1]
DSB SY
STR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbJ}
\settowidth{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbJ}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbI}}
\addtolength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbH}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbJ}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbK}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBNZ X0,L0
L0:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbL}
\settowidth{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbL}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbK}}
\addtolength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbH}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbL}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbM}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbN}
\settowidth{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbN}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbM}}
\addtolength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbH}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbN}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbO}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> pa1;
    x ?-> invalid;
    x ?-> pa2;

    y |-> pa3;
    identity 0x1000 with code;

    *pa2 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbP}
\settowidth{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbP}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbO}}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbA}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbA}
\begin{minipage}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R4=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R5=y|\\
\lstinline[language=IslaLitmusExp]|0:R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.BBM1+dsb-tlbiis-dsb-dsb+ctrl-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.BBM1+dsb-tlbiis-dsb-dsb+dsb-isb.tex <==
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbH}
\setlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbI}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X6
DSB SY
STR X2,[X1]
DSB SY
STR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbJ}
\settowidth{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbJ}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbI}}
\addtolength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbH}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbJ}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbK}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbL}
\settowidth{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbL}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbK}}
\addtolength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbH}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbL}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbM}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbN}
\settowidth{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbN}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbM}}
\addtolength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbH}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbN}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbO}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> pa1;
    x ?-> invalid;
    x ?-> pa2;

    y |-> pa3;
    identity 0x1000 with code;

    *pa2 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbP}
\settowidth{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbP}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbO}}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbA}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbA}
\begin{minipage}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R4=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R5=y|\\
\lstinline[language=IslaLitmusExp]|0:R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.BBM1+dsb-tlbiis-dsb-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.RT.EL1+dsb+dsb-tlbi-dsb+dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbH}
\setlength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbJ}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbJ}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbI}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
TLBI VAE1,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbL}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbL}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbK}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbL}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbN}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbN}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbM}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbN}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbP}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbP}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbO}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbP}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbB}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbB}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbA}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbB}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbC}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> pa1;
    x ?-> invalid;

    y |-> pa2;

    a |-> pa3;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbD}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbD}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbC}}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbE}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbE}
\begin{minipage}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R3=a|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:R1=a|\\
\lstinline[language=IslaLitmusExp]|1:R2=0x2|\\
\lstinline[language=IslaLitmusExp]|1:R3=a|\\
\lstinline[language=IslaLitmusExp]|1:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|2:R1=a|\\
\lstinline[language=IslaLitmusExp]|2:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|2:R3=y|\\
\lstinline[language=IslaLitmusExp]|3:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|3:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|3:R1=y|\\
\lstinline[language=IslaLitmusExp]|3:R3=x|\\
\lstinline[language=IslaLitmusExp]|3:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL1+dsb+dsb-tlbi-dsb+dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbM}\\
  \cline{2-2}
  & Thread 3\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbO}\\
  \cline{2-2}
  & thread3 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=2 & 3:R0=1 & 3:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.RT.EL1+dsb+dsb-tlbiis-dsb+dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbH}
\setlength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbJ}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbJ}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbI}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbL}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbL}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbK}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbL}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbN}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbN}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbM}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbN}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbP}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbP}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbO}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbP}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbB}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbB}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbA}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbB}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbC}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> pa1;
    x ?-> invalid;

    y |-> pa2;

    a |-> pa3;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbD}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbD}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbC}}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbE}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbE}
\begin{minipage}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R3=a|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:R1=a|\\
\lstinline[language=IslaLitmusExp]|1:R2=0x2|\\
\lstinline[language=IslaLitmusExp]|1:R3=a|\\
\lstinline[language=IslaLitmusExp]|1:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|2:R1=a|\\
\lstinline[language=IslaLitmusExp]|2:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|2:R3=y|\\
\lstinline[language=IslaLitmusExp]|3:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|3:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|3:R1=y|\\
\lstinline[language=IslaLitmusExp]|3:R3=x|\\
\lstinline[language=IslaLitmusExp]|3:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL1+dsb+dsb-tlbiis-dsb+dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbM}\\
  \cline{2-2}
  & Thread 3\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbO}\\
  \cline{2-2}
  & thread3 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=2 & 3:R0=1 & 3:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.RT.EL1+dsb-shootdown-dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbH}
\setlength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X4,[X5]
LDR X6,[X5]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbJ}
\settowidth{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbJ}{\usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbI}}
\addtolength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbH}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X4,[X5]
SVC #0
STR X7,[X5]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbL}
\settowidth{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbL}{\usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbK}}
\addtolength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbH}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbL}
\newsavebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS X9,ESR_EL1
LSR X9,X9,#26
SUB X9,X9,#0b010101
CBNZ X9,1f
0:
DSB SY
TLBI VAE1,X6
DSB SY
ISB
ERET
1:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbN}
\settowidth{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbN}{\usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbM}}
\addtolength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbH}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbN}
\newsavebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> pa1;
    x ?-> invalid;

    y |-> pa2;
    *pa2 = 0;

    f |-> pa3;
    *pa3 = 0;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbP}
\settowidth{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbP}{\usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbO}}
\newsavebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbA}
\begin{minipage}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R5=f|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=f|\\
\lstinline[language=IslaLitmusExp]|1:R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:R7=0b10|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL1+dsb-shootdown-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R4=1 & 0:R6=2 & 1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.RT.EL1+dsb-tlbi-dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbH}
\setlength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbJ}
\settowidth{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbJ}{\usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbI}}
\addtolength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbH}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbL}
\settowidth{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbL}{\usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbK}}
\addtolength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbH}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbL}
\newsavebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbN}
\settowidth{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbN}{\usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbM}}
\addtolength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbH}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbN}
\newsavebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbP}
\settowidth{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbP}{\usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbO}}
\newsavebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbA}
\begin{minipage}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL1+dsb-tlbi-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.RT.EL1+dsb-tlbiis-dsb+dmb.tex <==
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbH}
\setlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbH}{0cm}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbI}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbJ}
\settowidth{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbJ}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbI}}
\addtolength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbJ}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbK}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbL}
\settowidth{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbL}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbK}}
\addtolength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbL}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbM}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbN}
\settowidth{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbN}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbM}}
\addtolength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbN}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbO}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbP}
\settowidth{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbP}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbO}}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbA}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbA}
\begin{minipage}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL1+dsb-tlbiis-dsb+dmb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.RT.EL1+dsb-tlbiis-dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbH}
\setlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbJ}
\settowidth{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbJ}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbI}}
\addtolength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbL}
\settowidth{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbL}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbK}}
\addtolength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbL}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbN}
\settowidth{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbN}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbM}}
\addtolength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbN}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbP}
\settowidth{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbP}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbO}}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbA}
\begin{minipage}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL1+dsb-tlbiis-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.RT.EL2+dsb-tlbiipa-dsb-tlbiis-dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbH}
\setlength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1,X4
DSB SY
TLBI VMALLE1IS
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbJ}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbJ}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbI}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbL}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbL}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbK}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbL}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#1
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbN}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbN}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbM}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbN}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
physical pa1 pa2;
intermediate ipa1 ipa2;

x |-> ipa1;
ipa1 |-> pa1;
ipa1 ?-> invalid;

y |-> ipa2;
ipa2 |-> pa2;

identity 0x2000 with code;

*pa1 = 0;
*pa2 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbP}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbP}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbO}}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbA}
\begin{minipage}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=bvlshr(ipa1,0xC)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL2+dsb-tlbiipa-dsb-tlbiis-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.RT.EL2+dsb-tlbiipais-dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbH}
\setlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbJ}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbJ}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbI}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbL}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbL}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbK}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbL}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#1
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbN}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbN}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbM}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbN}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
physical pa1 pa2;
intermediate ipa1 ipa2;

x |-> ipa1;
ipa1 |-> pa1;
ipa1 ?-> invalid;

y |-> ipa2;
ipa2 |-> pa2;

identity 0x2000 with code;

*pa1 = 1;
*pa2 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbP}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbP}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbO}}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbA}
\begin{minipage}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(ipa1)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL2+dsb-tlbiipais-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|true|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.RT.EL2+dsb-tlbiipais-dsb-tlbiis-dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbH}
\setlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1IS,X4
DSB SY
TLBI VMALLE1IS
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbJ}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbJ}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbI}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
isb
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbL}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbL}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbK}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbL}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#1
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbN}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbN}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbM}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbN}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
physical pa1 pa2;
intermediate ipa1 ipa2;

x |-> ipa1;
ipa1 |-> pa1;
ipa1 ?-> invalid;

y |-> ipa2;
ipa2 |-> pa2;

identity 0x2000 with code;

*pa1 = 0;
*pa2 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbP}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbP}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbO}}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbA}
\begin{minipage}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(ipa1)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL2+dsb-tlbiipais-dsb-tlbiis-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.RT.EL2+dsb-tlbiis-dsb-tlbiipais-dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbH}
\setlength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VMALLE1IS
DSB SY
TLBI IPAS2E1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbJ}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbJ}{\usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbI}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
isb
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbL}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbL}{\usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbK}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbL}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#1
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbN}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbN}{\usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbM}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbN}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
physical pa1 pa2;
intermediate ipa1 ipa2;

x |-> ipa1;
ipa1 |-> pa1;
ipa1 ?-> invalid;

y |-> ipa2;
ipa2 |-> pa2;

identity 0x2000 with code;

*pa1 = 0;
*pa2 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbP}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbP}{\usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbO}}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbA}
\begin{minipage}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(ipa1)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL2+dsb-tlbiis-dsb-tlbiipais-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.RT.inv+dmb+addr-po-isb.tex <==
\newlength{\MPdotRTdotinvplusdmbplusaddrpoisbH}
\setlength{\MPdotRTdotinvplusdmbplusaddrpoisbH}{0cm}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpoisbI}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpoisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpoisbJ}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpoisbJ}{\usebox{\MPdotRTdotinvplusdmbplusaddrpoisbI}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpoisbH}{\MPdotRTdotinvplusdmbplusaddrpoisbJ}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpoisbK}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpoisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
EOR X6,X2,X2
LDR X7,[X8,X6]
ISB
LDR X4,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpoisbL}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpoisbL}{\usebox{\MPdotRTdotinvplusdmbplusaddrpoisbK}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpoisbH}{\MPdotRTdotinvplusdmbplusaddrpoisbL}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpoisbM}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpoisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpoisbN}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpoisbN}{\usebox{\MPdotRTdotinvplusdmbplusaddrpoisbM}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpoisbH}{\MPdotRTdotinvplusdmbplusaddrpoisbN}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpoisbO}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpoisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X4,#0
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpoisbP}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpoisbP}{\usebox{\MPdotRTdotinvplusdmbplusaddrpoisbO}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpoisbH}{\MPdotRTdotinvplusdmbplusaddrpoisbP}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpoisbA}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpoisbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;

    x |-> invalid;
    x ?-> pa1;

    y |-> pa2;

    z |-> pa3;

    *pa1 = 1;
    *pa2 = 0;
    *pa3 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpoisbB}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpoisbB}{\usebox{\MPdotRTdotinvplusdmbplusaddrpoisbA}}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpoisbC}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpoisbC}
\begin{minipage}{\MPdotRTdotinvplusdmbplusaddrpoisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R8=z|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.inv+dmb+addr-po-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotinvplusdmbplusaddrpoisbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotinvplusdmbplusaddrpoisbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotinvplusdmbplusaddrpoisbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpoisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpoisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpoisbM}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpoisbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R2=1 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.RT.inv+dmb+addr-po-msr-isb.tex <==
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrisbH}
\setlength{\MPdotRTdotinvplusdmbplusaddrpomsrisbH}{0cm}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbI}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrisbJ}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrisbJ}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbI}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpomsrisbH}{\MPdotRTdotinvplusdmbplusaddrpomsrisbJ}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbK}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
EOR X6,X2,X2
LDR X7,[X8,X6]
MSR ELR_EL1,X5
ISB
LDR X4,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrisbL}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrisbL}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbK}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpomsrisbH}{\MPdotRTdotinvplusdmbplusaddrpomsrisbL}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbM}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrisbN}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrisbN}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbM}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpomsrisbH}{\MPdotRTdotinvplusdmbplusaddrpomsrisbN}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbO}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X4,#0
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrisbP}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrisbP}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbO}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpomsrisbH}{\MPdotRTdotinvplusdmbplusaddrpomsrisbP}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbA}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrisbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;

    x |-> invalid;
    x ?-> pa1;

    y |-> pa2;

    z |-> pa3;

    *pa1 = 1;
    *pa2 = 0;
    *pa3 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrisbB}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrisbB}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbA}}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbC}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrisbC}
\begin{minipage}{\MPdotRTdotinvplusdmbplusaddrpomsrisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:R8=z|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.inv+dmb+addr-po-msr-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotinvplusdmbplusaddrpomsrisbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbM}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R2=1 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.RT.inv+dmb+addr-po-msr.tex <==
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrH}
\setlength{\MPdotRTdotinvplusdmbplusaddrpomsrH}{0cm}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrI}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrJ}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrJ}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrI}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpomsrH}{\MPdotRTdotinvplusdmbplusaddrpomsrJ}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrK}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
EOR X6,X2,X2
LDR X7,[X8,X6]
MSR ELR_EL1,X5
LDR X4,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrL}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrL}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrK}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpomsrH}{\MPdotRTdotinvplusdmbplusaddrpomsrL}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrM}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrN}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrN}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrM}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpomsrH}{\MPdotRTdotinvplusdmbplusaddrpomsrN}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrO}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X4,#0
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrP}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrP}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrO}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpomsrH}{\MPdotRTdotinvplusdmbplusaddrpomsrP}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrA}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;

    x |-> invalid;
    x ?-> pa1;

    y |-> pa2;

    z |-> pa3;

    *pa1 = 1;
    *pa2 = 0;
    *pa3 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrB}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrB}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrA}}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrC}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrC}
\begin{minipage}{\MPdotRTdotinvplusdmbplusaddrpomsrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:R8=z|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.inv+dmb+addr-po-msr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotinvplusdmbplusaddrpomsrB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpomsrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpomsrK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpomsrM}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpomsrO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R2=1 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.RT.inv+dmb+ctrl-trfi.tex <==
\newlength{\MPdotRTdotinvplusdmbplusctrltrfiH}
\setlength{\MPdotRTdotinvplusdmbplusctrltrfiH}{0cm}
\newsavebox{\MPdotRTdotinvplusdmbplusctrltrfiI}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusctrltrfiI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusctrltrfiJ}
\settowidth{\MPdotRTdotinvplusdmbplusctrltrfiJ}{\usebox{\MPdotRTdotinvplusdmbplusctrltrfiI}}
\addtolength{\MPdotRTdotinvplusdmbplusctrltrfiH}{\MPdotRTdotinvplusdmbplusctrltrfiJ}
\newsavebox{\MPdotRTdotinvplusdmbplusctrltrfiK}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusctrltrfiK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBZ X0,LC00
LC00:
STR X2,[X3]
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusctrltrfiL}
\settowidth{\MPdotRTdotinvplusdmbplusctrltrfiL}{\usebox{\MPdotRTdotinvplusdmbplusctrltrfiK}}
\addtolength{\MPdotRTdotinvplusdmbplusctrltrfiH}{\MPdotRTdotinvplusdmbplusctrltrfiL}
\newsavebox{\MPdotRTdotinvplusdmbplusctrltrfiM}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusctrltrfiM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#2
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusctrltrfiN}
\settowidth{\MPdotRTdotinvplusdmbplusctrltrfiN}{\usebox{\MPdotRTdotinvplusdmbplusctrltrfiM}}
\addtolength{\MPdotRTdotinvplusdmbplusctrltrfiH}{\MPdotRTdotinvplusdmbplusctrltrfiN}
\newsavebox{\MPdotRTdotinvplusdmbplusctrltrfiO}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusctrltrfiO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    w |-> invalid;
    w ?-> pa1;
    x |-> pa1;
    *pa1 = 0;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusctrltrfiP}
\settowidth{\MPdotRTdotinvplusdmbplusctrltrfiP}{\usebox{\MPdotRTdotinvplusdmbplusctrltrfiO}}
\newsavebox{\MPdotRTdotinvplusdmbplusctrltrfiA}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusctrltrfiA}
\begin{minipage}{\MPdotRTdotinvplusdmbplusctrltrfiH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(w,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R5=w|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.inv+dmb+ctrl-trfi|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotinvplusdmbplusctrltrfiP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotinvplusdmbplusctrltrfiO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotinvplusdmbplusctrltrfiA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusctrltrfiI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusctrltrfiK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusctrltrfiM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.RT.inv+trfi-data+addr.toml.tex <==
\newlength{\MPdotRTdotinvplustrfidataplusaddrdottomlH}
\setlength{\MPdotRTdotinvplustrfidataplusaddrdottomlH}{0cm}
\newsavebox{\MPdotRTdotinvplustrfidataplusaddrdottomlI}
\begin{lrbox}{\MPdotRTdotinvplustrfidataplusaddrdottomlI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
STR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplustrfidataplusaddrdottomlJ}
\settowidth{\MPdotRTdotinvplustrfidataplusaddrdottomlJ}{\usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlI}}
\addtolength{\MPdotRTdotinvplustrfidataplusaddrdottomlH}{\MPdotRTdotinvplustrfidataplusaddrdottomlJ}
\newsavebox{\MPdotRTdotinvplustrfidataplusaddrdottomlK}
\begin{lrbox}{\MPdotRTdotinvplustrfidataplusaddrdottomlK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
LDR X3,[X4,X2]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplustrfidataplusaddrdottomlL}
\settowidth{\MPdotRTdotinvplustrfidataplusaddrdottomlL}{\usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlK}}
\addtolength{\MPdotRTdotinvplustrfidataplusaddrdottomlH}{\MPdotRTdotinvplustrfidataplusaddrdottomlL}
\newsavebox{\MPdotRTdotinvplustrfidataplusaddrdottomlM}
\begin{lrbox}{\MPdotRTdotinvplustrfidataplusaddrdottomlM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplustrfidataplusaddrdottomlN}
\settowidth{\MPdotRTdotinvplustrfidataplusaddrdottomlN}{\usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlM}}
\addtolength{\MPdotRTdotinvplustrfidataplusaddrdottomlH}{\MPdotRTdotinvplustrfidataplusaddrdottomlN}
\newsavebox{\MPdotRTdotinvplustrfidataplusaddrdottomlO}
\begin{lrbox}{\MPdotRTdotinvplustrfidataplusaddrdottomlO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X3,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplustrfidataplusaddrdottomlP}
\settowidth{\MPdotRTdotinvplustrfidataplusaddrdottomlP}{\usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlO}}
\addtolength{\MPdotRTdotinvplustrfidataplusaddrdottomlH}{\MPdotRTdotinvplustrfidataplusaddrdottomlP}
\newsavebox{\MPdotRTdotinvplustrfidataplusaddrdottomlA}
\begin{lrbox}{\MPdotRTdotinvplustrfidataplusaddrdottomlA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    w |-> invalid;
    w ?-> pa1;
    x |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplustrfidataplusaddrdottomlB}
\settowidth{\MPdotRTdotinvplustrfidataplusaddrdottomlB}{\usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlA}}
\newsavebox{\MPdotRTdotinvplustrfidataplusaddrdottomlC}
\begin{lrbox}{\MPdotRTdotinvplustrfidataplusaddrdottomlC}
\begin{minipage}{\MPdotRTdotinvplustrfidataplusaddrdottomlH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(w,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R3=w|\\
\lstinline[language=IslaLitmusExp]|0:R4=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R5=y|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(w,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R4=w|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.inv+trfi-data+addr.toml|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotinvplustrfidataplusaddrdottomlB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=1 & 1:R0=1 & 1:R3=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.RTT.EL1+dsb-tlbiis-tlbiis-dsb+dsb-isb.tex <==
\newlength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbH}
\setlength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
STR X2,[X3]
DSB SY
TLBI VAE1IS,X4
TLBI VAE1IS,X5
DSB SY
STR X6,[X7]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbJ}
\settowidth{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbJ}{\usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbI}}
\addtolength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbH}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbJ}
\newsavebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X4,[X3]
MOV X2,X4
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbL}
\settowidth{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbL}{\usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbK}}
\addtolength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbH}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbL}
\newsavebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbN}
\settowidth{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbN}{\usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbM}}
\addtolength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbH}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbN}
\newsavebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> pa1;
    x ?-> invalid;

    y |-> pa2;

    z |-> pa3;
    z ?-> invalid;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbP}
\settowidth{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbP}{\usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbO}}
\newsavebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbA}
\begin{minipage}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|0:R5=page(z)|\\
\lstinline[language=IslaLitmusExp]|0:R6=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R7=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=z|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTT.EL1+dsb-tlbiis-tlbiis-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.RTf.inv+dmb+addr.tex <==
\newlength{\MPdotRTfdotinvplusdmbplusaddrH}
\setlength{\MPdotRTfdotinvplusdmbplusaddrH}{0cm}
\newsavebox{\MPdotRTfdotinvplusdmbplusaddrI}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusaddrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB ST
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusaddrJ}
\settowidth{\MPdotRTfdotinvplusdmbplusaddrJ}{\usebox{\MPdotRTfdotinvplusdmbplusaddrI}}
\addtolength{\MPdotRTfdotinvplusdmbplusaddrH}{\MPdotRTfdotinvplusdmbplusaddrJ}
\newsavebox{\MPdotRTfdotinvplusdmbplusaddrK}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusaddrK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusaddrL}
\settowidth{\MPdotRTfdotinvplusdmbplusaddrL}{\usebox{\MPdotRTfdotinvplusdmbplusaddrK}}
\addtolength{\MPdotRTfdotinvplusdmbplusaddrH}{\MPdotRTfdotinvplusdmbplusaddrL}
\newsavebox{\MPdotRTfdotinvplusdmbplusaddrM}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusaddrM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusaddrN}
\settowidth{\MPdotRTfdotinvplusdmbplusaddrN}{\usebox{\MPdotRTfdotinvplusdmbplusaddrM}}
\addtolength{\MPdotRTfdotinvplusdmbplusaddrH}{\MPdotRTfdotinvplusdmbplusaddrN}
\newsavebox{\MPdotRTfdotinvplusdmbplusaddrO}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusaddrO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusaddrP}
\settowidth{\MPdotRTfdotinvplusdmbplusaddrP}{\usebox{\MPdotRTfdotinvplusdmbplusaddrO}}
\newsavebox{\MPdotRTfdotinvplusdmbplusaddrA}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusaddrA}
\begin{minipage}{\MPdotRTfdotinvplusdmbplusaddrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv+dmb+addr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvplusdmbplusaddrP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvplusdmbplusaddrO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvplusdmbplusaddrA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusaddrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusaddrK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusaddrM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.RTf.inv+dmb+ctrl-isb.tex <==
\newlength{\MPdotRTfdotinvplusdmbplusctrlisbH}
\setlength{\MPdotRTfdotinvplusdmbplusctrlisbH}{0cm}
\newsavebox{\MPdotRTfdotinvplusdmbplusctrlisbI}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusctrlisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusctrlisbJ}
\settowidth{\MPdotRTfdotinvplusdmbplusctrlisbJ}{\usebox{\MPdotRTfdotinvplusdmbplusctrlisbI}}
\addtolength{\MPdotRTfdotinvplusdmbplusctrlisbH}{\MPdotRTfdotinvplusdmbplusctrlisbJ}
\newsavebox{\MPdotRTfdotinvplusdmbplusctrlisbK}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusctrlisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBNZ X0,L0
L0:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusctrlisbL}
\settowidth{\MPdotRTfdotinvplusdmbplusctrlisbL}{\usebox{\MPdotRTfdotinvplusdmbplusctrlisbK}}
\addtolength{\MPdotRTfdotinvplusdmbplusctrlisbH}{\MPdotRTfdotinvplusdmbplusctrlisbL}
\newsavebox{\MPdotRTfdotinvplusdmbplusctrlisbM}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusctrlisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusctrlisbN}
\settowidth{\MPdotRTfdotinvplusdmbplusctrlisbN}{\usebox{\MPdotRTfdotinvplusdmbplusctrlisbM}}
\addtolength{\MPdotRTfdotinvplusdmbplusctrlisbH}{\MPdotRTfdotinvplusdmbplusctrlisbN}
\newsavebox{\MPdotRTfdotinvplusdmbplusctrlisbO}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusctrlisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusctrlisbP}
\settowidth{\MPdotRTfdotinvplusdmbplusctrlisbP}{\usebox{\MPdotRTfdotinvplusdmbplusctrlisbO}}
\newsavebox{\MPdotRTfdotinvplusdmbplusctrlisbA}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusctrlisbA}
\begin{minipage}{\MPdotRTfdotinvplusdmbplusctrlisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv+dmb+ctrl-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvplusdmbplusctrlisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvplusdmbplusctrlisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvplusdmbplusctrlisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusctrlisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusctrlisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusctrlisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.RTf.inv+dmb+data.tex <==
\newlength{\MPdotRTfdotinvplusdmbplusdataH}
\setlength{\MPdotRTfdotinvplusdmbplusdataH}{0cm}
\newsavebox{\MPdotRTfdotinvplusdmbplusdataI}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdataI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB ST
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusdataJ}
\settowidth{\MPdotRTfdotinvplusdmbplusdataJ}{\usebox{\MPdotRTfdotinvplusdmbplusdataI}}
\addtolength{\MPdotRTfdotinvplusdmbplusdataH}{\MPdotRTfdotinvplusdmbplusdataJ}
\newsavebox{\MPdotRTfdotinvplusdmbplusdataK}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdataK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
ORR X6,X4,X5
STR X6,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusdataL}
\settowidth{\MPdotRTfdotinvplusdmbplusdataL}{\usebox{\MPdotRTfdotinvplusdmbplusdataK}}
\addtolength{\MPdotRTfdotinvplusdmbplusdataH}{\MPdotRTfdotinvplusdmbplusdataL}
\newsavebox{\MPdotRTfdotinvplusdmbplusdataM}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdataM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusdataN}
\settowidth{\MPdotRTfdotinvplusdmbplusdataN}{\usebox{\MPdotRTfdotinvplusdmbplusdataM}}
\addtolength{\MPdotRTfdotinvplusdmbplusdataH}{\MPdotRTfdotinvplusdmbplusdataN}
\newsavebox{\MPdotRTfdotinvplusdmbplusdataO}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdataO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusdataP}
\settowidth{\MPdotRTfdotinvplusdmbplusdataP}{\usebox{\MPdotRTfdotinvplusdmbplusdataO}}
\newsavebox{\MPdotRTfdotinvplusdmbplusdataA}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdataA}
\begin{minipage}{\MPdotRTfdotinvplusdmbplusdataH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=0b1|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv+dmb+data|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvplusdmbplusdataP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvplusdmbplusdataO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvplusdmbplusdataA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusdataI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusdataK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusdataM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.RTf.inv+dmb+dsb-isb.tex <==
\newlength{\MPdotRTfdotinvplusdmbplusdsbisbH}
\setlength{\MPdotRTfdotinvplusdmbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTfdotinvplusdmbplusdsbisbI}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusdsbisbJ}
\settowidth{\MPdotRTfdotinvplusdmbplusdsbisbJ}{\usebox{\MPdotRTfdotinvplusdmbplusdsbisbI}}
\addtolength{\MPdotRTfdotinvplusdmbplusdsbisbH}{\MPdotRTfdotinvplusdmbplusdsbisbJ}
\newsavebox{\MPdotRTfdotinvplusdmbplusdsbisbK}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusdsbisbL}
\settowidth{\MPdotRTfdotinvplusdmbplusdsbisbL}{\usebox{\MPdotRTfdotinvplusdmbplusdsbisbK}}
\addtolength{\MPdotRTfdotinvplusdmbplusdsbisbH}{\MPdotRTfdotinvplusdmbplusdsbisbL}
\newsavebox{\MPdotRTfdotinvplusdmbplusdsbisbM}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusdsbisbN}
\settowidth{\MPdotRTfdotinvplusdmbplusdsbisbN}{\usebox{\MPdotRTfdotinvplusdmbplusdsbisbM}}
\addtolength{\MPdotRTfdotinvplusdmbplusdsbisbH}{\MPdotRTfdotinvplusdmbplusdsbisbN}
\newsavebox{\MPdotRTfdotinvplusdmbplusdsbisbO}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusdsbisbP}
\settowidth{\MPdotRTfdotinvplusdmbplusdsbisbP}{\usebox{\MPdotRTfdotinvplusdmbplusdsbisbO}}
\newsavebox{\MPdotRTfdotinvplusdmbplusdsbisbA}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdsbisbA}
\begin{minipage}{\MPdotRTfdotinvplusdmbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv+dmb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvplusdmbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvplusdmbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvplusdmbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.RTf.inv+dmb+po.tex <==
\newlength{\MPdotRTfdotinvplusdmbpluspoH}
\setlength{\MPdotRTfdotinvplusdmbpluspoH}{0cm}
\newsavebox{\MPdotRTfdotinvplusdmbpluspoI}
\begin{lrbox}{\MPdotRTfdotinvplusdmbpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB ST
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbpluspoJ}
\settowidth{\MPdotRTfdotinvplusdmbpluspoJ}{\usebox{\MPdotRTfdotinvplusdmbpluspoI}}
\addtolength{\MPdotRTfdotinvplusdmbpluspoH}{\MPdotRTfdotinvplusdmbpluspoJ}
\newsavebox{\MPdotRTfdotinvplusdmbpluspoK}
\begin{lrbox}{\MPdotRTfdotinvplusdmbpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbpluspoL}
\settowidth{\MPdotRTfdotinvplusdmbpluspoL}{\usebox{\MPdotRTfdotinvplusdmbpluspoK}}
\addtolength{\MPdotRTfdotinvplusdmbpluspoH}{\MPdotRTfdotinvplusdmbpluspoL}
\newsavebox{\MPdotRTfdotinvplusdmbpluspoM}
\begin{lrbox}{\MPdotRTfdotinvplusdmbpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbpluspoN}
\settowidth{\MPdotRTfdotinvplusdmbpluspoN}{\usebox{\MPdotRTfdotinvplusdmbpluspoM}}
\addtolength{\MPdotRTfdotinvplusdmbpluspoH}{\MPdotRTfdotinvplusdmbpluspoN}
\newsavebox{\MPdotRTfdotinvplusdmbpluspoO}
\begin{lrbox}{\MPdotRTfdotinvplusdmbpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbpluspoP}
\settowidth{\MPdotRTfdotinvplusdmbpluspoP}{\usebox{\MPdotRTfdotinvplusdmbpluspoO}}
\newsavebox{\MPdotRTfdotinvplusdmbpluspoA}
\begin{lrbox}{\MPdotRTfdotinvplusdmbpluspoA}
\begin{minipage}{\MPdotRTfdotinvplusdmbpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv+dmb+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvplusdmbpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvplusdmbpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvplusdmbpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.RTf.inv+dmbs.tex <==
\newlength{\MPdotRTfdotinvplusdmbsH}
\setlength{\MPdotRTfdotinvplusdmbsH}{0cm}
\newsavebox{\MPdotRTfdotinvplusdmbsI}
\begin{lrbox}{\MPdotRTfdotinvplusdmbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB ST
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbsJ}
\settowidth{\MPdotRTfdotinvplusdmbsJ}{\usebox{\MPdotRTfdotinvplusdmbsI}}
\addtolength{\MPdotRTfdotinvplusdmbsH}{\MPdotRTfdotinvplusdmbsJ}
\newsavebox{\MPdotRTfdotinvplusdmbsK}
\begin{lrbox}{\MPdotRTfdotinvplusdmbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbsL}
\settowidth{\MPdotRTfdotinvplusdmbsL}{\usebox{\MPdotRTfdotinvplusdmbsK}}
\addtolength{\MPdotRTfdotinvplusdmbsH}{\MPdotRTfdotinvplusdmbsL}
\newsavebox{\MPdotRTfdotinvplusdmbsM}
\begin{lrbox}{\MPdotRTfdotinvplusdmbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbsN}
\settowidth{\MPdotRTfdotinvplusdmbsN}{\usebox{\MPdotRTfdotinvplusdmbsM}}
\addtolength{\MPdotRTfdotinvplusdmbsH}{\MPdotRTfdotinvplusdmbsN}
\newsavebox{\MPdotRTfdotinvplusdmbsO}
\begin{lrbox}{\MPdotRTfdotinvplusdmbsO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbsP}
\settowidth{\MPdotRTfdotinvplusdmbsP}{\usebox{\MPdotRTfdotinvplusdmbsO}}
\newsavebox{\MPdotRTfdotinvplusdmbsA}
\begin{lrbox}{\MPdotRTfdotinvplusdmbsA}
\begin{minipage}{\MPdotRTfdotinvplusdmbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv+dmbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvplusdmbsP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvplusdmbsO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvplusdmbsA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbsK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbsM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.RTf.inv.EL1+dsb-tlbiis-dsb+addr.tex <==
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrH}
\setlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrH}{0cm}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrI}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrJ}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrJ}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrI}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrJ}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrK}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrL}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrL}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrK}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrL}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrM}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrN}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrN}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrM}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrN}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrO}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrP}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrP}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrO}}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrA}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrA}
\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv.EL1+dsb-tlbiis-dsb+addr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.RTf.inv.EL1+dsb-tlbiis-dsb+ctrl-isb.tex <==
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbH}
\setlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbH}{0cm}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbI}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbJ}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbJ}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbI}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbJ}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbK}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBNZ X0,L0
L0:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbL}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbL}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbK}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbL}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbM}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbN}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbN}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbM}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbN}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbO}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbP}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbP}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbO}}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbA}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbA}
\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv.EL1+dsb-tlbiis-dsb+ctrl-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.RTf.inv.EL1+dsb-tlbiis-dsb+ctrl.tex <==
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}
\setlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}{0cm}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlI}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlJ}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlJ}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlI}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlJ}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlK}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBNZ X0,L0
L0:
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlL}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlL}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlK}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlL}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlM}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlN}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlN}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlM}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlN}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlO}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlP}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlP}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlO}}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlA}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlA}
\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv.EL1+dsb-tlbiis-dsb+ctrl|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.RTf.inv.EL1+dsb-tlbiis-dsb+data.tex <==
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}
\setlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}{0cm}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataI}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataJ}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataJ}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataI}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataJ}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataK}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
STR X4,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataL}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataL}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataK}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataL}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataM}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataN}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataN}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataM}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataN}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataO}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataP}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataP}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataO}}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataA}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataA}
\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv.EL1+dsb-tlbiis-dsb+data|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.RTf.inv.EL1+dsb-tlbiis-dsb+dmb.tex <==
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}
\setlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{0cm}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}
\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv.EL1+dsb-tlbiis-dsb+dmb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.RTf.inv.EL1+dsb-tlbiis-dsb+dsb-isb.tex <==
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}
\setlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbJ}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbJ}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbI}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbJ}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbL}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbL}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbK}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbL}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbN}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbN}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbM}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbN}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbP}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbP}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbO}}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbA}
\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv.EL1+dsb-tlbiis-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.RTf.inv.EL1+dsb-tlbiis-dsb+po.tex <==
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}
\setlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}{0cm}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoI}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoJ}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoJ}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoI}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoJ}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoK}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoL}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoL}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoK}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoL}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoM}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoN}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoN}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoM}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoN}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoO}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoP}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoP}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoO}}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoA}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoA}
\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv.EL1+dsb-tlbiis-dsb+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.RTf.inv.EL1+dsb-tlbiis-dsb+poap.tex <==
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}
\setlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}{0cm}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapI}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapJ}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapJ}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapI}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapJ}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapK}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDAR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapL}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapL}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapK}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapL}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapM}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapN}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapN}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapM}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapN}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapO}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapP}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapP}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapO}}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapA}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapA}
\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv.EL1+dsb-tlbiis-dsb+poap|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.TR.inv+dmb+isb.tex <==
\newlength{\MPdotTRdotinvplusdmbplusisbH}
\setlength{\MPdotTRdotinvplusdmbplusisbH}{0cm}
\newsavebox{\MPdotTRdotinvplusdmbplusisbI}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusisbJ}
\settowidth{\MPdotTRdotinvplusdmbplusisbJ}{\usebox{\MPdotTRdotinvplusdmbplusisbI}}
\addtolength{\MPdotTRdotinvplusdmbplusisbH}{\MPdotTRdotinvplusdmbplusisbJ}
\newsavebox{\MPdotTRdotinvplusdmbplusisbK}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
ISB
LDR X4,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusisbL}
\settowidth{\MPdotTRdotinvplusdmbplusisbL}{\usebox{\MPdotTRdotinvplusdmbplusisbK}}
\addtolength{\MPdotTRdotinvplusdmbplusisbH}{\MPdotTRdotinvplusdmbplusisbL}
\newsavebox{\MPdotTRdotinvplusdmbplusisbM}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusisbN}
\settowidth{\MPdotTRdotinvplusdmbplusisbN}{\usebox{\MPdotTRdotinvplusdmbplusisbM}}
\addtolength{\MPdotTRdotinvplusdmbplusisbH}{\MPdotTRdotinvplusdmbplusisbN}
\newsavebox{\MPdotTRdotinvplusdmbplusisbO}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusisbP}
\settowidth{\MPdotTRdotinvplusdmbplusisbP}{\usebox{\MPdotTRdotinvplusdmbplusisbO}}
\addtolength{\MPdotTRdotinvplusdmbplusisbH}{\MPdotTRdotinvplusdmbplusisbP}
\newsavebox{\MPdotTRdotinvplusdmbplusisbA}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusisbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 0;
    *pa2 = 1;
    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusisbB}
\settowidth{\MPdotTRdotinvplusdmbplusisbB}{\usebox{\MPdotTRdotinvplusdmbplusisbA}}
\newsavebox{\MPdotTRdotinvplusdmbplusisbC}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusisbC}
\begin{minipage}{\MPdotTRdotinvplusdmbplusisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TR.inv+dmb+isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTRdotinvplusdmbplusisbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTRdotinvplusdmbplusisbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTRdotinvplusdmbplusisbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusisbM}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusisbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R2=1 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.TR.inv+dmb+msr-isb.tex <==
\newlength{\MPdotTRdotinvplusdmbplusmsrisbH}
\setlength{\MPdotTRdotinvplusdmbplusmsrisbH}{0cm}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrisbI}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrisbJ}
\settowidth{\MPdotTRdotinvplusdmbplusmsrisbJ}{\usebox{\MPdotTRdotinvplusdmbplusmsrisbI}}
\addtolength{\MPdotTRdotinvplusdmbplusmsrisbH}{\MPdotTRdotinvplusdmbplusmsrisbJ}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrisbK}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MSR ELR_EL1,X5
ISB
LDR X4,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrisbL}
\settowidth{\MPdotTRdotinvplusdmbplusmsrisbL}{\usebox{\MPdotTRdotinvplusdmbplusmsrisbK}}
\addtolength{\MPdotTRdotinvplusdmbplusmsrisbH}{\MPdotTRdotinvplusdmbplusmsrisbL}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrisbM}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrisbN}
\settowidth{\MPdotTRdotinvplusdmbplusmsrisbN}{\usebox{\MPdotTRdotinvplusdmbplusmsrisbM}}
\addtolength{\MPdotTRdotinvplusdmbplusmsrisbH}{\MPdotTRdotinvplusdmbplusmsrisbN}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrisbO}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrisbP}
\settowidth{\MPdotTRdotinvplusdmbplusmsrisbP}{\usebox{\MPdotTRdotinvplusdmbplusmsrisbO}}
\addtolength{\MPdotTRdotinvplusdmbplusmsrisbH}{\MPdotTRdotinvplusdmbplusmsrisbP}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrisbA}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrisbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 0;
    *pa2 = 1;
    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrisbB}
\settowidth{\MPdotTRdotinvplusdmbplusmsrisbB}{\usebox{\MPdotTRdotinvplusdmbplusmsrisbA}}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrisbC}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrisbC}
\begin{minipage}{\MPdotTRdotinvplusdmbplusmsrisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TR.inv+dmb+msr-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTRdotinvplusdmbplusmsrisbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTRdotinvplusdmbplusmsrisbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTRdotinvplusdmbplusmsrisbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusmsrisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusmsrisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusmsrisbM}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusmsrisbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R2=1 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.TR.inv+dmb+msr.tex <==
\newlength{\MPdotTRdotinvplusdmbplusmsrH}
\setlength{\MPdotTRdotinvplusdmbplusmsrH}{0cm}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrI}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrJ}
\settowidth{\MPdotTRdotinvplusdmbplusmsrJ}{\usebox{\MPdotTRdotinvplusdmbplusmsrI}}
\addtolength{\MPdotTRdotinvplusdmbplusmsrH}{\MPdotTRdotinvplusdmbplusmsrJ}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrK}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MSR ELR_EL1,X5
LDR X4,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrL}
\settowidth{\MPdotTRdotinvplusdmbplusmsrL}{\usebox{\MPdotTRdotinvplusdmbplusmsrK}}
\addtolength{\MPdotTRdotinvplusdmbplusmsrH}{\MPdotTRdotinvplusdmbplusmsrL}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrM}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrN}
\settowidth{\MPdotTRdotinvplusdmbplusmsrN}{\usebox{\MPdotTRdotinvplusdmbplusmsrM}}
\addtolength{\MPdotTRdotinvplusdmbplusmsrH}{\MPdotTRdotinvplusdmbplusmsrN}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrO}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrP}
\settowidth{\MPdotTRdotinvplusdmbplusmsrP}{\usebox{\MPdotTRdotinvplusdmbplusmsrO}}
\addtolength{\MPdotTRdotinvplusdmbplusmsrH}{\MPdotTRdotinvplusdmbplusmsrP}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrA}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 0;
    *pa2 = 1;
    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrB}
\settowidth{\MPdotTRdotinvplusdmbplusmsrB}{\usebox{\MPdotTRdotinvplusdmbplusmsrA}}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrC}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrC}
\begin{minipage}{\MPdotTRdotinvplusdmbplusmsrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TR.inv+dmb+msr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTRdotinvplusdmbplusmsrB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTRdotinvplusdmbplusmsrA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTRdotinvplusdmbplusmsrC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusmsrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusmsrK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusmsrM}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusmsrO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R2=1 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.TTf.inv+dmb+addr.tex <==
\newlength{\MPdotTTfdotinvplusdmbplusaddrH}
\setlength{\MPdotTTfdotinvplusdmbplusaddrH}{0cm}
\newsavebox{\MPdotTTfdotinvplusdmbplusaddrI}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusaddrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbplusaddrJ}
\settowidth{\MPdotTTfdotinvplusdmbplusaddrJ}{\usebox{\MPdotTTfdotinvplusdmbplusaddrI}}
\addtolength{\MPdotTTfdotinvplusdmbplusaddrH}{\MPdotTTfdotinvplusdmbplusaddrJ}
\newsavebox{\MPdotTTfdotinvplusdmbplusaddrK}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusaddrK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
EOR X4,X0,X0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbplusaddrL}
\settowidth{\MPdotTTfdotinvplusdmbplusaddrL}{\usebox{\MPdotTTfdotinvplusdmbplusaddrK}}
\addtolength{\MPdotTTfdotinvplusdmbplusaddrH}{\MPdotTTfdotinvplusdmbplusaddrL}
\newsavebox{\MPdotTTfdotinvplusdmbplusaddrM}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusaddrM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbplusaddrN}
\settowidth{\MPdotTTfdotinvplusdmbplusaddrN}{\usebox{\MPdotTTfdotinvplusdmbplusaddrM}}
\addtolength{\MPdotTTfdotinvplusdmbplusaddrH}{\MPdotTTfdotinvplusdmbplusaddrN}
\newsavebox{\MPdotTTfdotinvplusdmbplusaddrO}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusaddrO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbplusaddrP}
\settowidth{\MPdotTTfdotinvplusdmbplusaddrP}{\usebox{\MPdotTTfdotinvplusdmbplusaddrO}}
\newsavebox{\MPdotTTfdotinvplusdmbplusaddrA}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusaddrA}
\begin{minipage}{\MPdotTTfdotinvplusdmbplusaddrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv+dmb+addr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvplusdmbplusaddrP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvplusdmbplusaddrO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvplusdmbplusaddrA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbplusaddrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbplusaddrK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbplusaddrM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.TTf.inv+dmb+dsb-isb.tex <==
\newlength{\MPdotTTfdotinvplusdmbplusdsbisbH}
\setlength{\MPdotTTfdotinvplusdmbplusdsbisbH}{0cm}
\newsavebox{\MPdotTTfdotinvplusdmbplusdsbisbI}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbplusdsbisbJ}
\settowidth{\MPdotTTfdotinvplusdmbplusdsbisbJ}{\usebox{\MPdotTTfdotinvplusdmbplusdsbisbI}}
\addtolength{\MPdotTTfdotinvplusdmbplusdsbisbH}{\MPdotTTfdotinvplusdmbplusdsbisbJ}
\newsavebox{\MPdotTTfdotinvplusdmbplusdsbisbK}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbplusdsbisbL}
\settowidth{\MPdotTTfdotinvplusdmbplusdsbisbL}{\usebox{\MPdotTTfdotinvplusdmbplusdsbisbK}}
\addtolength{\MPdotTTfdotinvplusdmbplusdsbisbH}{\MPdotTTfdotinvplusdmbplusdsbisbL}
\newsavebox{\MPdotTTfdotinvplusdmbplusdsbisbM}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbplusdsbisbN}
\settowidth{\MPdotTTfdotinvplusdmbplusdsbisbN}{\usebox{\MPdotTTfdotinvplusdmbplusdsbisbM}}
\addtolength{\MPdotTTfdotinvplusdmbplusdsbisbH}{\MPdotTTfdotinvplusdmbplusdsbisbN}
\newsavebox{\MPdotTTfdotinvplusdmbplusdsbisbO}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbplusdsbisbP}
\settowidth{\MPdotTTfdotinvplusdmbplusdsbisbP}{\usebox{\MPdotTTfdotinvplusdmbplusdsbisbO}}
\newsavebox{\MPdotTTfdotinvplusdmbplusdsbisbA}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusdsbisbA}
\begin{minipage}{\MPdotTTfdotinvplusdmbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv+dmb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvplusdmbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvplusdmbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvplusdmbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.TTf.inv+dmb+po.tex <==
\newlength{\MPdotTTfdotinvplusdmbpluspoH}
\setlength{\MPdotTTfdotinvplusdmbpluspoH}{0cm}
\newsavebox{\MPdotTTfdotinvplusdmbpluspoI}
\begin{lrbox}{\MPdotTTfdotinvplusdmbpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbpluspoJ}
\settowidth{\MPdotTTfdotinvplusdmbpluspoJ}{\usebox{\MPdotTTfdotinvplusdmbpluspoI}}
\addtolength{\MPdotTTfdotinvplusdmbpluspoH}{\MPdotTTfdotinvplusdmbpluspoJ}
\newsavebox{\MPdotTTfdotinvplusdmbpluspoK}
\begin{lrbox}{\MPdotTTfdotinvplusdmbpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbpluspoL}
\settowidth{\MPdotTTfdotinvplusdmbpluspoL}{\usebox{\MPdotTTfdotinvplusdmbpluspoK}}
\addtolength{\MPdotTTfdotinvplusdmbpluspoH}{\MPdotTTfdotinvplusdmbpluspoL}
\newsavebox{\MPdotTTfdotinvplusdmbpluspoM}
\begin{lrbox}{\MPdotTTfdotinvplusdmbpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbpluspoN}
\settowidth{\MPdotTTfdotinvplusdmbpluspoN}{\usebox{\MPdotTTfdotinvplusdmbpluspoM}}
\addtolength{\MPdotTTfdotinvplusdmbpluspoH}{\MPdotTTfdotinvplusdmbpluspoN}
\newsavebox{\MPdotTTfdotinvplusdmbpluspoO}
\begin{lrbox}{\MPdotTTfdotinvplusdmbpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbpluspoP}
\settowidth{\MPdotTTfdotinvplusdmbpluspoP}{\usebox{\MPdotTTfdotinvplusdmbpluspoO}}
\newsavebox{\MPdotTTfdotinvplusdmbpluspoA}
\begin{lrbox}{\MPdotTTfdotinvplusdmbpluspoA}
\begin{minipage}{\MPdotTTfdotinvplusdmbpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv+dmb+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvplusdmbpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvplusdmbpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvplusdmbpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.TTf.inv+dsb+ctrl-isb.tex <==
\newlength{\MPdotTTfdotinvplusdsbplusctrlisbH}
\setlength{\MPdotTTfdotinvplusdsbplusctrlisbH}{0cm}
\newsavebox{\MPdotTTfdotinvplusdsbplusctrlisbI}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusctrlisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbplusctrlisbJ}
\settowidth{\MPdotTTfdotinvplusdsbplusctrlisbJ}{\usebox{\MPdotTTfdotinvplusdsbplusctrlisbI}}
\addtolength{\MPdotTTfdotinvplusdsbplusctrlisbH}{\MPdotTTfdotinvplusdsbplusctrlisbJ}
\newsavebox{\MPdotTTfdotinvplusdsbplusctrlisbK}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusctrlisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
CBNZ X0,L0
L0:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbplusctrlisbL}
\settowidth{\MPdotTTfdotinvplusdsbplusctrlisbL}{\usebox{\MPdotTTfdotinvplusdsbplusctrlisbK}}
\addtolength{\MPdotTTfdotinvplusdsbplusctrlisbH}{\MPdotTTfdotinvplusdsbplusctrlisbL}
\newsavebox{\MPdotTTfdotinvplusdsbplusctrlisbM}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusctrlisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbplusctrlisbN}
\settowidth{\MPdotTTfdotinvplusdsbplusctrlisbN}{\usebox{\MPdotTTfdotinvplusdsbplusctrlisbM}}
\addtolength{\MPdotTTfdotinvplusdsbplusctrlisbH}{\MPdotTTfdotinvplusdsbplusctrlisbN}
\newsavebox{\MPdotTTfdotinvplusdsbplusctrlisbO}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusctrlisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbplusctrlisbP}
\settowidth{\MPdotTTfdotinvplusdsbplusctrlisbP}{\usebox{\MPdotTTfdotinvplusdsbplusctrlisbO}}
\newsavebox{\MPdotTTfdotinvplusdsbplusctrlisbA}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusctrlisbA}
\begin{minipage}{\MPdotTTfdotinvplusdsbplusctrlisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv+dsb+ctrl-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvplusdsbplusctrlisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvplusdsbplusctrlisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvplusdsbplusctrlisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbplusctrlisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbplusctrlisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbplusctrlisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.TTf.inv+dsb+dsb-isb.tex <==
\newlength{\MPdotTTfdotinvplusdsbplusdsbisbH}
\setlength{\MPdotTTfdotinvplusdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotTTfdotinvplusdsbplusdsbisbI}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbplusdsbisbJ}
\settowidth{\MPdotTTfdotinvplusdsbplusdsbisbJ}{\usebox{\MPdotTTfdotinvplusdsbplusdsbisbI}}
\addtolength{\MPdotTTfdotinvplusdsbplusdsbisbH}{\MPdotTTfdotinvplusdsbplusdsbisbJ}
\newsavebox{\MPdotTTfdotinvplusdsbplusdsbisbK}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbplusdsbisbL}
\settowidth{\MPdotTTfdotinvplusdsbplusdsbisbL}{\usebox{\MPdotTTfdotinvplusdsbplusdsbisbK}}
\addtolength{\MPdotTTfdotinvplusdsbplusdsbisbH}{\MPdotTTfdotinvplusdsbplusdsbisbL}
\newsavebox{\MPdotTTfdotinvplusdsbplusdsbisbM}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbplusdsbisbN}
\settowidth{\MPdotTTfdotinvplusdsbplusdsbisbN}{\usebox{\MPdotTTfdotinvplusdsbplusdsbisbM}}
\addtolength{\MPdotTTfdotinvplusdsbplusdsbisbH}{\MPdotTTfdotinvplusdsbplusdsbisbN}
\newsavebox{\MPdotTTfdotinvplusdsbplusdsbisbO}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbplusdsbisbP}
\settowidth{\MPdotTTfdotinvplusdsbplusdsbisbP}{\usebox{\MPdotTTfdotinvplusdsbplusdsbisbO}}
\newsavebox{\MPdotTTfdotinvplusdsbplusdsbisbA}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusdsbisbA}
\begin{minipage}{\MPdotTTfdotinvplusdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv+dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvplusdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvplusdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvplusdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.TTf.inv+dsb+po.tex <==
\newlength{\MPdotTTfdotinvplusdsbpluspoH}
\setlength{\MPdotTTfdotinvplusdsbpluspoH}{0cm}
\newsavebox{\MPdotTTfdotinvplusdsbpluspoI}
\begin{lrbox}{\MPdotTTfdotinvplusdsbpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbpluspoJ}
\settowidth{\MPdotTTfdotinvplusdsbpluspoJ}{\usebox{\MPdotTTfdotinvplusdsbpluspoI}}
\addtolength{\MPdotTTfdotinvplusdsbpluspoH}{\MPdotTTfdotinvplusdsbpluspoJ}
\newsavebox{\MPdotTTfdotinvplusdsbpluspoK}
\begin{lrbox}{\MPdotTTfdotinvplusdsbpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbpluspoL}
\settowidth{\MPdotTTfdotinvplusdsbpluspoL}{\usebox{\MPdotTTfdotinvplusdsbpluspoK}}
\addtolength{\MPdotTTfdotinvplusdsbpluspoH}{\MPdotTTfdotinvplusdsbpluspoL}
\newsavebox{\MPdotTTfdotinvplusdsbpluspoM}
\begin{lrbox}{\MPdotTTfdotinvplusdsbpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbpluspoN}
\settowidth{\MPdotTTfdotinvplusdsbpluspoN}{\usebox{\MPdotTTfdotinvplusdsbpluspoM}}
\addtolength{\MPdotTTfdotinvplusdsbpluspoH}{\MPdotTTfdotinvplusdsbpluspoN}
\newsavebox{\MPdotTTfdotinvplusdsbpluspoO}
\begin{lrbox}{\MPdotTTfdotinvplusdsbpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbpluspoP}
\settowidth{\MPdotTTfdotinvplusdsbpluspoP}{\usebox{\MPdotTTfdotinvplusdsbpluspoO}}
\newsavebox{\MPdotTTfdotinvplusdsbpluspoA}
\begin{lrbox}{\MPdotTTfdotinvplusdsbpluspoA}
\begin{minipage}{\MPdotTTfdotinvplusdsbpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv+dsb+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvplusdsbpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvplusdsbpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvplusdsbpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.TTf.inv+dsbs.tex <==
\newlength{\MPdotTTfdotinvplusdsbsH}
\setlength{\MPdotTTfdotinvplusdsbsH}{0cm}
\newsavebox{\MPdotTTfdotinvplusdsbsI}
\begin{lrbox}{\MPdotTTfdotinvplusdsbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbsJ}
\settowidth{\MPdotTTfdotinvplusdsbsJ}{\usebox{\MPdotTTfdotinvplusdsbsI}}
\addtolength{\MPdotTTfdotinvplusdsbsH}{\MPdotTTfdotinvplusdsbsJ}
\newsavebox{\MPdotTTfdotinvplusdsbsK}
\begin{lrbox}{\MPdotTTfdotinvplusdsbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbsL}
\settowidth{\MPdotTTfdotinvplusdsbsL}{\usebox{\MPdotTTfdotinvplusdsbsK}}
\addtolength{\MPdotTTfdotinvplusdsbsH}{\MPdotTTfdotinvplusdsbsL}
\newsavebox{\MPdotTTfdotinvplusdsbsM}
\begin{lrbox}{\MPdotTTfdotinvplusdsbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbsN}
\settowidth{\MPdotTTfdotinvplusdsbsN}{\usebox{\MPdotTTfdotinvplusdsbsM}}
\addtolength{\MPdotTTfdotinvplusdsbsH}{\MPdotTTfdotinvplusdsbsN}
\newsavebox{\MPdotTTfdotinvplusdsbsO}
\begin{lrbox}{\MPdotTTfdotinvplusdsbsO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbsP}
\settowidth{\MPdotTTfdotinvplusdsbsP}{\usebox{\MPdotTTfdotinvplusdsbsO}}
\newsavebox{\MPdotTTfdotinvplusdsbsA}
\begin{lrbox}{\MPdotTTfdotinvplusdsbsA}
\begin{minipage}{\MPdotTTfdotinvplusdsbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv+dsbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvplusdsbsP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvplusdsbsO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvplusdsbsA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbsK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbsM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.TTf.inv.EL1+dsb-tlbiis-dsb+dmb.tex <==
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}
\setlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{0cm}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}
\begin{minipage}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv.EL1+dsb-tlbiis-dsb+dmb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.TTf.inv.EL1+dsb-tlbiis-dsb+dsb-isb.tex <==
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}
\setlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbI}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbJ}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbJ}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbI}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbJ}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbK}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbL}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbL}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbK}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbL}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbM}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbN}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbN}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbM}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbN}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbO}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbP}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbP}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbO}}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbA}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbA}
\begin{minipage}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv.EL1+dsb-tlbiis-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.TTf.inv.EL1+dsb-tlbiis-dsb+po.tex <==
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}
\setlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}{0cm}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoI}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoJ}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoJ}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoI}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoJ}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoK}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoL}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoL}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoK}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoL}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoM}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoN}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoN}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoM}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoN}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoO}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoP}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoP}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoO}}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoA}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoA}
\begin{minipage}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv.EL1+dsb-tlbiis-dsb+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.TfR+dmb+eret.tex <==
\newlength{\MPdotTfRplusdmbpluseretH}
\setlength{\MPdotTfRplusdmbpluseretH}{0cm}
\newsavebox{\MPdotTfRplusdmbpluseretI}
\begin{lrbox}{\MPdotTfRplusdmbpluseretI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTfRplusdmbpluseretJ}
\settowidth{\MPdotTfRplusdmbpluseretJ}{\usebox{\MPdotTfRplusdmbpluseretI}}
\addtolength{\MPdotTfRplusdmbpluseretH}{\MPdotTfRplusdmbpluseretJ}
\newsavebox{\MPdotTfRplusdmbpluseretK}
\begin{lrbox}{\MPdotTfRplusdmbpluseretK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
LDR X4,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTfRplusdmbpluseretL}
\settowidth{\MPdotTfRplusdmbpluseretL}{\usebox{\MPdotTfRplusdmbpluseretK}}
\addtolength{\MPdotTfRplusdmbpluseretH}{\MPdotTfRplusdmbpluseretL}
\newsavebox{\MPdotTfRplusdmbpluseretM}
\begin{lrbox}{\MPdotTfRplusdmbpluseretM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTfRplusdmbpluseretN}
\settowidth{\MPdotTfRplusdmbpluseretN}{\usebox{\MPdotTfRplusdmbpluseretM}}
\addtolength{\MPdotTfRplusdmbpluseretH}{\MPdotTfRplusdmbpluseretN}
\newsavebox{\MPdotTfRplusdmbpluseretO}
\begin{lrbox}{\MPdotTfRplusdmbpluseretO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;

    y |-> pa2;
    y ?-> invalid;

    *pa1 = 0;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTfRplusdmbpluseretP}
\settowidth{\MPdotTfRplusdmbpluseretP}{\usebox{\MPdotTfRplusdmbpluseretO}}
\newsavebox{\MPdotTfRplusdmbpluseretA}
\begin{lrbox}{\MPdotTfRplusdmbpluseretA}
\begin{minipage}{\MPdotTfRplusdmbpluseretH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TfR+dmb+eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTfRplusdmbpluseretP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTfRplusdmbpluseretO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTfRplusdmbpluseretA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTfRplusdmbpluseretI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTfRplusdmbpluseretK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTfRplusdmbpluseretM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R2=0 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/MP.alias3+rfi-data+dmb.tex <==
\newlength{\MPdotaliasthreeplusrfidataplusdmbH}
\setlength{\MPdotaliasthreeplusrfidataplusdmbH}{0cm}
\newsavebox{\MPdotaliasthreeplusrfidataplusdmbI}
\begin{lrbox}{\MPdotaliasthreeplusrfidataplusdmbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
STR X2,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotaliasthreeplusrfidataplusdmbJ}
\settowidth{\MPdotaliasthreeplusrfidataplusdmbJ}{\usebox{\MPdotaliasthreeplusrfidataplusdmbI}}
\addtolength{\MPdotaliasthreeplusrfidataplusdmbH}{\MPdotaliasthreeplusrfidataplusdmbJ}
\newsavebox{\MPdotaliasthreeplusrfidataplusdmbK}
\begin{lrbox}{\MPdotaliasthreeplusrfidataplusdmbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotaliasthreeplusrfidataplusdmbL}
\settowidth{\MPdotaliasthreeplusrfidataplusdmbL}{\usebox{\MPdotaliasthreeplusrfidataplusdmbK}}
\addtolength{\MPdotaliasthreeplusrfidataplusdmbH}{\MPdotaliasthreeplusrfidataplusdmbL}
\newsavebox{\MPdotaliasthreeplusrfidataplusdmbM}
\begin{lrbox}{\MPdotaliasthreeplusrfidataplusdmbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    y |-> pa2;
    z |-> pa1;
    *pa1 = 0;
    *pa2 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotaliasthreeplusrfidataplusdmbN}
\settowidth{\MPdotaliasthreeplusrfidataplusdmbN}{\usebox{\MPdotaliasthreeplusrfidataplusdmbM}}
\newsavebox{\MPdotaliasthreeplusrfidataplusdmbO}
\begin{lrbox}{\MPdotaliasthreeplusrfidataplusdmbO}
\begin{minipage}{\MPdotaliasthreeplusrfidataplusdmbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R3=z|\\
\lstinline[language=IslaLitmusExp]|0:R5=y|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.alias3+rfi-data+dmb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotaliasthreeplusrfidataplusdmbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotaliasthreeplusrfidataplusdmbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotaliasthreeplusrfidataplusdmbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotaliasthreeplusrfidataplusdmbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotaliasthreeplusrfidataplusdmbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/PPOAA.alias.tex <==
\newlength{\PPOAAdotaliasH}
\setlength{\PPOAAdotaliasH}{0cm}
\newsavebox{\PPOAAdotaliasI}
\begin{lrbox}{\PPOAAdotaliasI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\PPOAAdotaliasJ}
\settowidth{\PPOAAdotaliasJ}{\usebox{\PPOAAdotaliasI}}
\addtolength{\PPOAAdotaliasH}{\PPOAAdotaliasJ}
\newsavebox{\PPOAAdotaliasK}
\begin{lrbox}{\PPOAAdotaliasK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X9,X0,X0
STR X2,[X3,X9]
LDR X4,[X5]
EOR X8,X4,X4
LDR X6,[X7,X8]
\end{lstlisting}
\end{lrbox}
\newlength{\PPOAAdotaliasL}
\settowidth{\PPOAAdotaliasL}{\usebox{\PPOAAdotaliasK}}
\addtolength{\PPOAAdotaliasH}{\PPOAAdotaliasL}
\newsavebox{\PPOAAdotaliasM}
\begin{lrbox}{\PPOAAdotaliasM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    w |-> pa1;
    x |-> pa1;
    y |-> pa2;
    z |-> pa3;
\end{lstlisting}
\end{lrbox}
\newlength{\PPOAAdotaliasN}
\settowidth{\PPOAAdotaliasN}{\usebox{\PPOAAdotaliasM}}
\newsavebox{\PPOAAdotaliasO}
\begin{lrbox}{\PPOAAdotaliasO}
\begin{minipage}{\PPOAAdotaliasH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R1=z|\\
\lstinline[language=IslaLitmusExp]|0:R2=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0x1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=w|\\
\lstinline[language=IslaLitmusExp]|1:R7=z|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|PPOAA.alias|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\PPOAAdotaliasN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\PPOAAdotaliasM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\PPOAAdotaliasO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\PPOAAdotaliasI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\PPOAAdotaliasK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R4=1 & 1:R6=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/PPOCA.alias.tex <==
\newlength{\PPOCAdotaliasH}
\setlength{\PPOCAdotaliasH}{0cm}
\newsavebox{\PPOCAdotaliasI}
\begin{lrbox}{\PPOCAdotaliasI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\PPOCAdotaliasJ}
\settowidth{\PPOCAdotaliasJ}{\usebox{\PPOCAdotaliasI}}
\addtolength{\PPOCAdotaliasH}{\PPOCAdotaliasJ}
\newsavebox{\PPOCAdotaliasK}
\begin{lrbox}{\PPOCAdotaliasK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBNZ X0,L0
L0:
STR X2,[X3]
LDR X4,[X5]
EOR X8,X4,X4
LDR X6,[X7,X8]
\end{lstlisting}
\end{lrbox}
\newlength{\PPOCAdotaliasL}
\settowidth{\PPOCAdotaliasL}{\usebox{\PPOCAdotaliasK}}
\addtolength{\PPOCAdotaliasH}{\PPOCAdotaliasL}
\newsavebox{\PPOCAdotaliasM}
\begin{lrbox}{\PPOCAdotaliasM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    w |-> pa1;
    x |-> pa1;
    y |-> pa2;
    z |-> pa3;
    *pa1 = 0;
    *pa2 = 0;
    *pa3 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\PPOCAdotaliasN}
\settowidth{\PPOCAdotaliasN}{\usebox{\PPOCAdotaliasM}}
\newsavebox{\PPOCAdotaliasO}
\begin{lrbox}{\PPOCAdotaliasO}
\begin{minipage}{\PPOCAdotaliasH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R1=z|\\
\lstinline[language=IslaLitmusExp]|0:R2=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0x1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=w|\\
\lstinline[language=IslaLitmusExp]|1:R7=z|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|PPOCA.alias|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\PPOCAdotaliasN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\PPOCAdotaliasM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\PPOCAdotaliasO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\PPOCAdotaliasI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\PPOCAdotaliasK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R4=1 & 1:R6=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/PPODA.RT.inv.tex <==
\newlength{\PPODAdotRTdotinvH}
\setlength{\PPODAdotRTdotinvH}{0cm}
\newsavebox{\PPODAdotRTdotinvI}
\begin{lrbox}{\PPODAdotRTdotinvI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\PPODAdotRTdotinvJ}
\settowidth{\PPODAdotRTdotinvJ}{\usebox{\PPODAdotRTdotinvI}}
\addtolength{\PPODAdotRTdotinvH}{\PPODAdotRTdotinvJ}
\newsavebox{\PPODAdotRTdotinvK}
\begin{lrbox}{\PPODAdotRTdotinvK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
ORR X2,X2,X3
STR X2,[X4]
LDR X6,[X5]
EOR X8,X6,X6
LDR X9,[X7,X8]
\end{lstlisting}
\end{lrbox}
\newlength{\PPODAdotRTdotinvL}
\settowidth{\PPODAdotRTdotinvL}{\usebox{\PPODAdotRTdotinvK}}
\addtolength{\PPODAdotRTdotinvH}{\PPODAdotRTdotinvL}
\newsavebox{\PPODAdotRTdotinvM}
\begin{lrbox}{\PPODAdotRTdotinvM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X6,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\PPODAdotRTdotinvN}
\settowidth{\PPODAdotRTdotinvN}{\usebox{\PPODAdotRTdotinvM}}
\addtolength{\PPODAdotRTdotinvH}{\PPODAdotRTdotinvN}
\newsavebox{\PPODAdotRTdotinvO}
\begin{lrbox}{\PPODAdotRTdotinvO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    w |-> pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa2;
    z |-> pa3;
    *pa1 = 1;
    *pa2 = 0;
    *pa3 = 0;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\PPODAdotRTdotinvP}
\settowidth{\PPODAdotRTdotinvP}{\usebox{\PPODAdotRTdotinvO}}
\newsavebox{\PPODAdotRTdotinvA}
\begin{lrbox}{\PPODAdotRTdotinvA}
\begin{minipage}{\PPODAdotRTdotinvH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R1=z|\\
\lstinline[language=IslaLitmusExp]|0:R2=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=desc3(w,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R4=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R5=x|\\
\lstinline[language=IslaLitmusExp]|1:R7=z|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|PPODA.RT.inv|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\PPODAdotRTdotinvP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\PPODAdotRTdotinvO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\PPODAdotRTdotinvA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\PPODAdotRTdotinvI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\PPODAdotRTdotinvK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\PPODAdotRTdotinvM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R6=1 & 1:R9=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/R.RTf.inv.EL1+dsb-tlbiis-dsb+popl.tex <==
\newlength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}
\setlength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}{0cm}
\newsavebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplI}
\begin{lrbox}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplJ}
\settowidth{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplJ}{\usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplI}}
\addtolength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplJ}
\newsavebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplK}
\begin{lrbox}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplK}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
STLR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplL}
\settowidth{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplL}{\usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplK}}
\addtolength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplL}
\newsavebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplM}
\begin{lrbox}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplN}
\settowidth{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplN}{\usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplM}}
\addtolength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplN}
\newsavebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplO}
\begin{lrbox}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplP}
\settowidth{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplP}{\usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplO}}
\newsavebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplA}
\begin{lrbox}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplA}
\begin{minipage}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R0=0x2|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|R.RTf.inv.EL1+dsb-tlbiis-dsb+popl|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|y=2 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/R.inv.tex <==
\newlength{\RdotinvH}
\setlength{\RdotinvH}{0cm}
\newsavebox{\RdotinvI}
\begin{lrbox}{\RdotinvI}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\RdotinvJ}
\settowidth{\RdotinvJ}{\usebox{\RdotinvI}}
\addtolength{\RdotinvH}{\RdotinvJ}
\newsavebox{\RdotinvK}
\begin{lrbox}{\RdotinvK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\RdotinvL}
\settowidth{\RdotinvL}{\usebox{\RdotinvK}}
\addtolength{\RdotinvH}{\RdotinvL}
\newsavebox{\RdotinvM}
\begin{lrbox}{\RdotinvM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    identity 0x1000 with code;
    *pa1 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\RdotinvN}
\settowidth{\RdotinvN}{\usebox{\RdotinvM}}
\newsavebox{\RdotinvO}
\begin{lrbox}{\RdotinvO}
\begin{minipage}{\RdotinvH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|R.inv|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\RdotinvN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\RdotinvM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\RdotinvO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\RdotinvI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\RdotinvK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R0=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/RBS+dsb-tlbiis-dsb.tex <==
\newlength{\RBSplusdsbtlbiisdsbH}
\setlength{\RBSplusdsbtlbiisdsbH}{0cm}
\newsavebox{\RBSplusdsbtlbiisdsbI}
\begin{lrbox}{\RBSplusdsbtlbiisdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X5
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\RBSplusdsbtlbiisdsbJ}
\settowidth{\RBSplusdsbtlbiisdsbJ}{\usebox{\RBSplusdsbtlbiisdsbI}}
\addtolength{\RBSplusdsbtlbiisdsbH}{\RBSplusdsbtlbiisdsbJ}
\newsavebox{\RBSplusdsbtlbiisdsbK}
\begin{lrbox}{\RBSplusdsbtlbiisdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\RBSplusdsbtlbiisdsbL}
\settowidth{\RBSplusdsbtlbiisdsbL}{\usebox{\RBSplusdsbtlbiisdsbK}}
\addtolength{\RBSplusdsbtlbiisdsbH}{\RBSplusdsbtlbiisdsbL}
\newsavebox{\RBSplusdsbtlbiisdsbM}
\begin{lrbox}{\RBSplusdsbtlbiisdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\RBSplusdsbtlbiisdsbN}
\settowidth{\RBSplusdsbtlbiisdsbN}{\usebox{\RBSplusdsbtlbiisdsbM}}
\addtolength{\RBSplusdsbtlbiisdsbH}{\RBSplusdsbtlbiisdsbN}
\newsavebox{\RBSplusdsbtlbiisdsbO}
\begin{lrbox}{\RBSplusdsbtlbiisdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;
    y |-> pa1;
    *pa1 = 0;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\RBSplusdsbtlbiisdsbP}
\settowidth{\RBSplusdsbtlbiisdsbP}{\usebox{\RBSplusdsbtlbiisdsbO}}
\newsavebox{\RBSplusdsbtlbiisdsbA}
\begin{lrbox}{\RBSplusdsbtlbiisdsbA}
\begin{minipage}{\RBSplusdsbtlbiisdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0x2|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R5=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|RBS+dsb-tlbiis-dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\RBSplusdsbtlbiisdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\RBSplusdsbtlbiisdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\RBSplusdsbtlbiisdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\RBSplusdsbtlbiisdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\RBSplusdsbtlbiisdsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\RBSplusdsbtlbiisdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=2|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/RDW.alias.tex <==
\newlength{\RDWdotaliasH}
\setlength{\RDWdotaliasH}{0cm}
\newsavebox{\RDWdotaliasI}
\begin{lrbox}{\RDWdotaliasI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\RDWdotaliasJ}
\settowidth{\RDWdotaliasJ}{\usebox{\RDWdotaliasI}}
\addtolength{\RDWdotaliasH}{\RDWdotaliasJ}
\newsavebox{\RDWdotaliasK}
\begin{lrbox}{\RDWdotaliasK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
LDR X3,[X4,X2]
LDR X5,[X6]
EOR X7,X5,X5
LDR X8,[X9,X7]
\end{lstlisting}
\end{lrbox}
\newlength{\RDWdotaliasL}
\settowidth{\RDWdotaliasL}{\usebox{\RDWdotaliasK}}
\addtolength{\RDWdotaliasH}{\RDWdotaliasL}
\newsavebox{\RDWdotaliasM}
\begin{lrbox}{\RDWdotaliasM}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\RDWdotaliasN}
\settowidth{\RDWdotaliasN}{\usebox{\RDWdotaliasM}}
\addtolength{\RDWdotaliasH}{\RDWdotaliasN}
\newsavebox{\RDWdotaliasO}
\begin{lrbox}{\RDWdotaliasO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    w |-> pa1;
    x |-> pa1;
    y |-> pa2;
    z |-> pa3;
    *pa1 = 0;
    *pa2 = 0;
    *pa3 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\RDWdotaliasP}
\settowidth{\RDWdotaliasP}{\usebox{\RDWdotaliasO}}
\newsavebox{\RDWdotaliasA}
\begin{lrbox}{\RDWdotaliasA}
\begin{minipage}{\RDWdotaliasH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=z|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R4=w|\\
\lstinline[language=IslaLitmusExp]|1:R6=x|\\
\lstinline[language=IslaLitmusExp]|1:R9=z|\\
\lstinline[language=IslaLitmusExp]|2:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|2:R1=x|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|RDW.alias|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\RDWdotaliasP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\RDWdotaliasO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\RDWdotaliasA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\RDWdotaliasI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\RDWdotaliasK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\RDWdotaliasM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R3=0 & 1:R5=1 & 1:R8=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/ROT.inv+dmbst.tex <==
\newlength{\ROTdotinvplusdmbstH}
\setlength{\ROTdotinvplusdmbstH}{0cm}
\newsavebox{\ROTdotinvplusdmbstI}
\begin{lrbox}{\ROTdotinvplusdmbstI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB ST
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvplusdmbstJ}
\settowidth{\ROTdotinvplusdmbstJ}{\usebox{\ROTdotinvplusdmbstI}}
\addtolength{\ROTdotinvplusdmbstH}{\ROTdotinvplusdmbstJ}
\newsavebox{\ROTdotinvplusdmbstK}
\begin{lrbox}{\ROTdotinvplusdmbstK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvplusdmbstL}
\settowidth{\ROTdotinvplusdmbstL}{\usebox{\ROTdotinvplusdmbstK}}
\addtolength{\ROTdotinvplusdmbstH}{\ROTdotinvplusdmbstL}
\newsavebox{\ROTdotinvplusdmbstM}
\begin{lrbox}{\ROTdotinvplusdmbstM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS x14,esr_el1
AND X14,X14,#0b111
CMP x14,#0b111
MOV X17,#1
MOV X18,#2
// if ESR_EL1.ISS.DFSC == Translation Level 3 then x2 = 1 else x2 = 2
CSEL x0,x17,x18,eq
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvplusdmbstN}
\settowidth{\ROTdotinvplusdmbstN}{\usebox{\ROTdotinvplusdmbstM}}
\addtolength{\ROTdotinvplusdmbstH}{\ROTdotinvplusdmbstN}
\newsavebox{\ROTdotinvplusdmbstO}
\begin{lrbox}{\ROTdotinvplusdmbstO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
physical pa1;
intermediate ipa1;

assert pa1 == ipa1;
ipa1 |-> pa1;

s1table new_table 0x280000 {
  x |-> invalid;
  x ?-> ipa1;
};

identity 0x283000 with default;

x |-> invalid at level 2;
x ?-> table(0x283000) at level 2;

identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvplusdmbstP}
\settowidth{\ROTdotinvplusdmbstP}{\usebox{\ROTdotinvplusdmbstO}}
\newsavebox{\ROTdotinvplusdmbstA}
\begin{lrbox}{\ROTdotinvplusdmbstA}
\begin{minipage}{\ROTdotinvplusdmbstH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=ipa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,new_table)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc2(table=0x283000)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte2(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|ROT.inv+dmbst|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\ROTdotinvplusdmbstP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\ROTdotinvplusdmbstO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\ROTdotinvplusdmbstA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\ROTdotinvplusdmbstI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\ROTdotinvplusdmbstK}\\
  \cline{2-2}
  & thread 1 el1 handler\\
  \cline{2-2}
  & \usebox{\ROTdotinvplusdmbstM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/ROT.inv+dsb.tex <==
\newlength{\ROTdotinvplusdsbH}
\setlength{\ROTdotinvplusdsbH}{0cm}
\newsavebox{\ROTdotinvplusdsbI}
\begin{lrbox}{\ROTdotinvplusdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvplusdsbJ}
\settowidth{\ROTdotinvplusdsbJ}{\usebox{\ROTdotinvplusdsbI}}
\addtolength{\ROTdotinvplusdsbH}{\ROTdotinvplusdsbJ}
\newsavebox{\ROTdotinvplusdsbK}
\begin{lrbox}{\ROTdotinvplusdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvplusdsbL}
\settowidth{\ROTdotinvplusdsbL}{\usebox{\ROTdotinvplusdsbK}}
\addtolength{\ROTdotinvplusdsbH}{\ROTdotinvplusdsbL}
\newsavebox{\ROTdotinvplusdsbM}
\begin{lrbox}{\ROTdotinvplusdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS X14,ESR_EL1
AND X14,X14,#0b111
CMP X14,#0b111
MOV X17,#1
MOV X18,#2
// if ESR_EL1.ISS.DFSC == Translation Level 3 then x2 = 1 else x2 = 2
CSEL X0,X17,X18,eq
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvplusdsbN}
\settowidth{\ROTdotinvplusdsbN}{\usebox{\ROTdotinvplusdsbM}}
\addtolength{\ROTdotinvplusdsbH}{\ROTdotinvplusdsbN}
\newsavebox{\ROTdotinvplusdsbO}
\begin{lrbox}{\ROTdotinvplusdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
physical pa1;
intermediate ipa1;

assert pa1 == ipa1;
ipa1 |-> pa1;

s1table new_table 0x280000 {
  x |-> invalid;
  x ?-> ipa1;
};

identity 0x283000 with default;

x |-> invalid at level 2;
x ?-> table(0x283000) at level 2;

identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvplusdsbP}
\settowidth{\ROTdotinvplusdsbP}{\usebox{\ROTdotinvplusdsbO}}
\newsavebox{\ROTdotinvplusdsbA}
\begin{lrbox}{\ROTdotinvplusdsbA}
\begin{minipage}{\ROTdotinvplusdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=ipa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,new_table)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc2(table=0x283000)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte2(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|ROT.inv+dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\ROTdotinvplusdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\ROTdotinvplusdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\ROTdotinvplusdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\ROTdotinvplusdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\ROTdotinvplusdsbK}\\
  \cline{2-2}
  & thread 1 el1 handler\\
  \cline{2-2}
  & \usebox{\ROTdotinvplusdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/ROT.inv+po.tex <==
\newlength{\ROTdotinvpluspoH}
\setlength{\ROTdotinvpluspoH}{0cm}
\newsavebox{\ROTdotinvpluspoI}
\begin{lrbox}{\ROTdotinvpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvpluspoJ}
\settowidth{\ROTdotinvpluspoJ}{\usebox{\ROTdotinvpluspoI}}
\addtolength{\ROTdotinvpluspoH}{\ROTdotinvpluspoJ}
\newsavebox{\ROTdotinvpluspoK}
\begin{lrbox}{\ROTdotinvpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvpluspoL}
\settowidth{\ROTdotinvpluspoL}{\usebox{\ROTdotinvpluspoK}}
\addtolength{\ROTdotinvpluspoH}{\ROTdotinvpluspoL}
\newsavebox{\ROTdotinvpluspoM}
\begin{lrbox}{\ROTdotinvpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS X14,ESR_EL1
AND X14,X14,#0b111
CMP X14,#0b111
MOV X17,#1
MOV X18,#2
// if ESR_EL1.ISS.DFSC == Translation Level 3 then x2 = 1 else x2 = 2
CSEL X0,X17,X18,eq
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvpluspoN}
\settowidth{\ROTdotinvpluspoN}{\usebox{\ROTdotinvpluspoM}}
\addtolength{\ROTdotinvpluspoH}{\ROTdotinvpluspoN}
\newsavebox{\ROTdotinvpluspoO}
\begin{lrbox}{\ROTdotinvpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
physical pa1;
intermediate ipa1;

assert pa1 == ipa1;
ipa1 |-> pa1;

s1table new_table 0x280000 {
  x |-> invalid;
  x ?-> ipa1;
};

identity 0x283000 with default;

x |-> invalid at level 2;
x ?-> table(0x283000) at level 2;

identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvpluspoP}
\settowidth{\ROTdotinvpluspoP}{\usebox{\ROTdotinvpluspoO}}
\newsavebox{\ROTdotinvpluspoA}
\begin{lrbox}{\ROTdotinvpluspoA}
\begin{minipage}{\ROTdotinvpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=ipa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,new_table)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc2(table=0x283000)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte2(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|ROT.inv+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\ROTdotinvpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\ROTdotinvpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\ROTdotinvpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\ROTdotinvpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\ROTdotinvpluspoK}\\
  \cline{2-2}
  & thread 1 el1 handler\\
  \cline{2-2}
  & \usebox{\ROTdotinvpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/RSW.alias.tex <==
\newlength{\RSWdotaliasH}
\setlength{\RSWdotaliasH}{0cm}
\newsavebox{\RSWdotaliasI}
\begin{lrbox}{\RSWdotaliasI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\RSWdotaliasJ}
\settowidth{\RSWdotaliasJ}{\usebox{\RSWdotaliasI}}
\addtolength{\RSWdotaliasH}{\RSWdotaliasJ}
\newsavebox{\RSWdotaliasK}
\begin{lrbox}{\RSWdotaliasK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
LDR X3,[X4,X2]
LDR X5,[X6]
EOR X7,X5,X5
LDR X8,[X9,X7]
\end{lstlisting}
\end{lrbox}
\newlength{\RSWdotaliasL}
\settowidth{\RSWdotaliasL}{\usebox{\RSWdotaliasK}}
\addtolength{\RSWdotaliasH}{\RSWdotaliasL}
\newsavebox{\RSWdotaliasM}
\begin{lrbox}{\RSWdotaliasM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    w |-> pa1;
    x |-> pa1;
    y |-> pa2;
    z |-> pa3;
    *pa1 = 0;
    *pa2 = 0;
    *pa3 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\RSWdotaliasN}
\settowidth{\RSWdotaliasN}{\usebox{\RSWdotaliasM}}
\newsavebox{\RSWdotaliasO}
\begin{lrbox}{\RSWdotaliasO}
\begin{minipage}{\RSWdotaliasH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=z|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R4=w|\\
\lstinline[language=IslaLitmusExp]|1:R6=x|\\
\lstinline[language=IslaLitmusExp]|1:R9=z|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|RSW.alias|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\RSWdotaliasN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\RSWdotaliasM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\RSWdotaliasO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\RSWdotaliasI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\RSWdotaliasK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R8=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/RWC.RTR.EL1+dsb-isb+dsb-tlbi-dsb.tex <==
\newlength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbH}
\setlength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbH}{0cm}
\newsavebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbI}
\begin{lrbox}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbJ}
\settowidth{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbJ}{\usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbI}}
\addtolength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbH}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbJ}
\newsavebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbK}
\begin{lrbox}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X3,[X4,X2]
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbL}
\settowidth{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbL}{\usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbK}}
\addtolength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbH}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbL}
\newsavebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbM}
\begin{lrbox}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X2
DSB SY
LDR X3,[X4]
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbN}
\settowidth{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbN}{\usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbM}}
\addtolength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbH}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbN}
\newsavebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbO}
\begin{lrbox}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X3,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbP}
\settowidth{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbP}{\usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbO}}
\addtolength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbH}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbP}
\newsavebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbA}
\begin{lrbox}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;

    y |-> pa2;
    y ?-> invalid;
    z |-> pa2;
    *pa1 = 1;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbB}
\settowidth{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbB}{\usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbA}}
\newsavebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbC}
\begin{lrbox}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbC}
\begin{minipage}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R4=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|2:R1=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R2=page(x)|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|RWC.RTR.EL1+dsb-isb+dsb-tlbi-dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R1=1 & 1:R3=0 & 2:R3=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/RWC.RTfR.inv+addr+dmb.tex <==
\newlength{\RWCdotRTfRdotinvplusaddrplusdmbH}
\setlength{\RWCdotRTfRdotinvplusaddrplusdmbH}{0cm}
\newsavebox{\RWCdotRTfRdotinvplusaddrplusdmbI}
\begin{lrbox}{\RWCdotRTfRdotinvplusaddrplusdmbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTfRdotinvplusaddrplusdmbJ}
\settowidth{\RWCdotRTfRdotinvplusaddrplusdmbJ}{\usebox{\RWCdotRTfRdotinvplusaddrplusdmbI}}
\addtolength{\RWCdotRTfRdotinvplusaddrplusdmbH}{\RWCdotRTfRdotinvplusaddrplusdmbJ}
\newsavebox{\RWCdotRTfRdotinvplusaddrplusdmbK}
\begin{lrbox}{\RWCdotRTfRdotinvplusaddrplusdmbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
LDR X3,[X4,X2]
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTfRdotinvplusaddrplusdmbL}
\settowidth{\RWCdotRTfRdotinvplusaddrplusdmbL}{\usebox{\RWCdotRTfRdotinvplusaddrplusdmbK}}
\addtolength{\RWCdotRTfRdotinvplusaddrplusdmbH}{\RWCdotRTfRdotinvplusaddrplusdmbL}
\newsavebox{\RWCdotRTfRdotinvplusaddrplusdmbM}
\begin{lrbox}{\RWCdotRTfRdotinvplusaddrplusdmbM}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTfRdotinvplusaddrplusdmbN}
\settowidth{\RWCdotRTfRdotinvplusaddrplusdmbN}{\usebox{\RWCdotRTfRdotinvplusaddrplusdmbM}}
\addtolength{\RWCdotRTfRdotinvplusaddrplusdmbH}{\RWCdotRTfRdotinvplusaddrplusdmbN}
\newsavebox{\RWCdotRTfRdotinvplusaddrplusdmbO}
\begin{lrbox}{\RWCdotRTfRdotinvplusaddrplusdmbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X3,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTfRdotinvplusaddrplusdmbP}
\settowidth{\RWCdotRTfRdotinvplusaddrplusdmbP}{\usebox{\RWCdotRTfRdotinvplusaddrplusdmbO}}
\addtolength{\RWCdotRTfRdotinvplusaddrplusdmbH}{\RWCdotRTfRdotinvplusaddrplusdmbP}
\newsavebox{\RWCdotRTfRdotinvplusaddrplusdmbA}
\begin{lrbox}{\RWCdotRTfRdotinvplusaddrplusdmbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;

    y |-> invalid;
    y ?-> pa2;
    z |-> pa2;
    *pa1 = 1;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTfRdotinvplusaddrplusdmbB}
\settowidth{\RWCdotRTfRdotinvplusaddrplusdmbB}{\usebox{\RWCdotRTfRdotinvplusaddrplusdmbA}}
\newsavebox{\RWCdotRTfRdotinvplusaddrplusdmbC}
\begin{lrbox}{\RWCdotRTfRdotinvplusaddrplusdmbC}
\begin{minipage}{\RWCdotRTfRdotinvplusaddrplusdmbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R4=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|2:R1=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|RWC.RTfR.inv+addr+dmb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\RWCdotRTfRdotinvplusaddrplusdmbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\RWCdotRTfRdotinvplusaddrplusdmbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\RWCdotRTfRdotinvplusaddrplusdmbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\RWCdotRTfRdotinvplusaddrplusdmbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\RWCdotRTfRdotinvplusaddrplusdmbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\RWCdotRTfRdotinvplusaddrplusdmbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\RWCdotRTfRdotinvplusaddrplusdmbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R1=1 & 1:R3=0 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/S.RT.ro+dsb-tlbiis-dsb+dsb-isb.tex <==
\newlength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbH}
\setlength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbH}{0cm}
\newsavebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbI}
\begin{lrbox}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbJ}
\settowidth{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbJ}{\usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbI}}
\addtolength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbH}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbJ}
\newsavebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbK}
\begin{lrbox}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbL}
\settowidth{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbL}{\usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbK}}
\addtolength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbH}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbL}
\newsavebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbM}
\begin{lrbox}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbN}
\settowidth{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbN}{\usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbM}}
\addtolength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbH}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbN}
\newsavebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbO}
\begin{lrbox}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1 with [AP = 0b11] and default;
    x ?-> pa1;
    z |-> pa1;
    y |-> pa2;

    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbP}
\settowidth{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbP}{\usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbO}}
\newsavebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbA}
\begin{lrbox}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbA}
\begin{minipage}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|S.RT.ro+dsb-tlbiis-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/S.RTf.inv.EL1+dsb-tlbiis-dsb+ctrl.tex <==
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}
\setlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}{0cm}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlI}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlJ}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlJ}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlI}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlJ}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlK}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBNZ X0,L0
L0:
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlL}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlL}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlK}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlL}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlM}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlN}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlN}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlM}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlN}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlO}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlP}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlP}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlO}}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlA}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlA}
\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|S.RTf.inv.EL1+dsb-tlbiis-dsb+ctrl|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/S.RTf.inv.EL1+dsb-tlbiis-dsb+data.tex <==
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}
\setlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}{0cm}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataI}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataJ}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataJ}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataI}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataJ}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataK}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
ORR X2,X2,X4
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataL}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataL}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataK}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataL}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataM}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataN}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataN}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataM}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataN}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataO}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataP}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataP}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataO}}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataA}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataA}
\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|S.RTf.inv.EL1+dsb-tlbiis-dsb+data|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/S.RTf.inv.EL1+dsb-tlbiis-dsb+dmb.tex <==
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}
\setlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{0cm}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}
\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|S.RTf.inv.EL1+dsb-tlbiis-dsb+dmb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/S.RTf.inv.EL1+dsb-tlbiis-dsb+poap.tex <==
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}
\setlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}{0cm}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapI}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapJ}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapJ}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapI}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapJ}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapK}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDAR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapL}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapL}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapK}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapL}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapM}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapN}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapN}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapM}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapN}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapO}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapP}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapP}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapO}}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapA}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapA}
\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|S.RTf.inv.EL1+dsb-tlbiis-dsb+poap|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/S.RTf.inv.EL1+dsb-tlbiis-dsb+popl.tex <==
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}
\setlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}{0cm}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplI}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplJ}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplJ}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplI}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplJ}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplK}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STLR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplL}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplL}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplK}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplL}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplM}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplN}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplN}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplM}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplN}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplO}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplP}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplP}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplO}}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplA}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplA}
\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|S.RTf.inv.EL1+dsb-tlbiis-dsb+popl|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/S.T+dmb+po.tex <==
\newlength{\SdotTplusdmbpluspoH}
\setlength{\SdotTplusdmbpluspoH}{0cm}
\newsavebox{\SdotTplusdmbpluspoI}
\begin{lrbox}{\SdotTplusdmbpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotTplusdmbpluspoJ}
\settowidth{\SdotTplusdmbpluspoJ}{\usebox{\SdotTplusdmbpluspoI}}
\addtolength{\SdotTplusdmbpluspoH}{\SdotTplusdmbpluspoJ}
\newsavebox{\SdotTplusdmbpluspoK}
\begin{lrbox}{\SdotTplusdmbpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotTplusdmbpluspoL}
\settowidth{\SdotTplusdmbpluspoL}{\usebox{\SdotTplusdmbpluspoK}}
\addtolength{\SdotTplusdmbpluspoH}{\SdotTplusdmbpluspoL}
\newsavebox{\SdotTplusdmbpluspoM}
\begin{lrbox}{\SdotTplusdmbpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SdotTplusdmbpluspoN}
\settowidth{\SdotTplusdmbpluspoN}{\usebox{\SdotTplusdmbpluspoM}}
\addtolength{\SdotTplusdmbpluspoH}{\SdotTplusdmbpluspoN}
\newsavebox{\SdotTplusdmbpluspoO}
\begin{lrbox}{\SdotTplusdmbpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 0;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SdotTplusdmbpluspoP}
\settowidth{\SdotTplusdmbpluspoP}{\usebox{\SdotTplusdmbpluspoO}}
\newsavebox{\SdotTplusdmbpluspoA}
\begin{lrbox}{\SdotTplusdmbpluspoA}
\begin{minipage}{\SdotTplusdmbpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0x2|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|S.T+dmb+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SdotTplusdmbpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SdotTplusdmbpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SdotTplusdmbpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SdotTplusdmbpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SdotTplusdmbpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SdotTplusdmbpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & x=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/SB.TfTf.inv+dmb-ctrl-isbs.tex <==
\newlength{\SBdotTfTfdotinvplusdmbctrlisbsH}
\setlength{\SBdotTfTfdotinvplusdmbctrlisbsH}{0cm}
\newsavebox{\SBdotTfTfdotinvplusdmbctrlisbsI}
\begin{lrbox}{\SBdotTfTfdotinvplusdmbctrlisbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
LDR X7,[X8]
CBNZ X7,L0
L0:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdmbctrlisbsJ}
\settowidth{\SBdotTfTfdotinvplusdmbctrlisbsJ}{\usebox{\SBdotTfTfdotinvplusdmbctrlisbsI}}
\addtolength{\SBdotTfTfdotinvplusdmbctrlisbsH}{\SBdotTfTfdotinvplusdmbctrlisbsJ}
\newsavebox{\SBdotTfTfdotinvplusdmbctrlisbsK}
\begin{lrbox}{\SBdotTfTfdotinvplusdmbctrlisbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
LDR X7,[X8]
CBNZ X7,L1
L1:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdmbctrlisbsL}
\settowidth{\SBdotTfTfdotinvplusdmbctrlisbsL}{\usebox{\SBdotTfTfdotinvplusdmbctrlisbsK}}
\addtolength{\SBdotTfTfdotinvplusdmbctrlisbsH}{\SBdotTfTfdotinvplusdmbctrlisbsL}
\newsavebox{\SBdotTfTfdotinvplusdmbctrlisbsM}
\begin{lrbox}{\SBdotTfTfdotinvplusdmbctrlisbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdmbctrlisbsN}
\settowidth{\SBdotTfTfdotinvplusdmbctrlisbsN}{\usebox{\SBdotTfTfdotinvplusdmbctrlisbsM}}
\addtolength{\SBdotTfTfdotinvplusdmbctrlisbsH}{\SBdotTfTfdotinvplusdmbctrlisbsN}
\newsavebox{\SBdotTfTfdotinvplusdmbctrlisbsO}
\begin{lrbox}{\SBdotTfTfdotinvplusdmbctrlisbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdmbctrlisbsP}
\settowidth{\SBdotTfTfdotinvplusdmbctrlisbsP}{\usebox{\SBdotTfTfdotinvplusdmbctrlisbsO}}
\addtolength{\SBdotTfTfdotinvplusdmbctrlisbsH}{\SBdotTfTfdotinvplusdmbctrlisbsP}
\newsavebox{\SBdotTfTfdotinvplusdmbctrlisbsA}
\begin{lrbox}{\SBdotTfTfdotinvplusdmbctrlisbsA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> invalid;
    y ?-> pa2;
    v |-> pa2;
    *pa2 = 1;

    z |-> pa3;
    *pa3 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdmbctrlisbsB}
\settowidth{\SBdotTfTfdotinvplusdmbctrlisbsB}{\usebox{\SBdotTfTfdotinvplusdmbctrlisbsA}}
\newsavebox{\SBdotTfTfdotinvplusdmbctrlisbsC}
\begin{lrbox}{\SBdotTfTfdotinvplusdmbctrlisbsC}
\begin{minipage}{\SBdotTfTfdotinvplusdmbctrlisbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R8=z|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R0=desc3(v,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R8=z|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|SB.TfTf.inv+dmb-ctrl-isbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SBdotTfTfdotinvplusdmbctrlisbsB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SBdotTfTfdotinvplusdmbctrlisbsA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SBdotTfTfdotinvplusdmbctrlisbsC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvplusdmbctrlisbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvplusdmbctrlisbsK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvplusdmbctrlisbsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvplusdmbctrlisbsO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/SB.TfTf.inv+dsb-isbs.tex <==
\newlength{\SBdotTfTfdotinvplusdsbisbsH}
\setlength{\SBdotTfTfdotinvplusdsbisbsH}{0cm}
\newsavebox{\SBdotTfTfdotinvplusdsbisbsI}
\begin{lrbox}{\SBdotTfTfdotinvplusdsbisbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdsbisbsJ}
\settowidth{\SBdotTfTfdotinvplusdsbisbsJ}{\usebox{\SBdotTfTfdotinvplusdsbisbsI}}
\addtolength{\SBdotTfTfdotinvplusdsbisbsH}{\SBdotTfTfdotinvplusdsbisbsJ}
\newsavebox{\SBdotTfTfdotinvplusdsbisbsK}
\begin{lrbox}{\SBdotTfTfdotinvplusdsbisbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdsbisbsL}
\settowidth{\SBdotTfTfdotinvplusdsbisbsL}{\usebox{\SBdotTfTfdotinvplusdsbisbsK}}
\addtolength{\SBdotTfTfdotinvplusdsbisbsH}{\SBdotTfTfdotinvplusdsbisbsL}
\newsavebox{\SBdotTfTfdotinvplusdsbisbsM}
\begin{lrbox}{\SBdotTfTfdotinvplusdsbisbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdsbisbsN}
\settowidth{\SBdotTfTfdotinvplusdsbisbsN}{\usebox{\SBdotTfTfdotinvplusdsbisbsM}}
\addtolength{\SBdotTfTfdotinvplusdsbisbsH}{\SBdotTfTfdotinvplusdsbisbsN}
\newsavebox{\SBdotTfTfdotinvplusdsbisbsO}
\begin{lrbox}{\SBdotTfTfdotinvplusdsbisbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdsbisbsP}
\settowidth{\SBdotTfTfdotinvplusdsbisbsP}{\usebox{\SBdotTfTfdotinvplusdsbisbsO}}
\addtolength{\SBdotTfTfdotinvplusdsbisbsH}{\SBdotTfTfdotinvplusdsbisbsP}
\newsavebox{\SBdotTfTfdotinvplusdsbisbsA}
\begin{lrbox}{\SBdotTfTfdotinvplusdsbisbsA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> invalid;
    y ?-> pa2;
    v |-> pa2;
    *pa2 = 1;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdsbisbsB}
\settowidth{\SBdotTfTfdotinvplusdsbisbsB}{\usebox{\SBdotTfTfdotinvplusdsbisbsA}}
\newsavebox{\SBdotTfTfdotinvplusdsbisbsC}
\begin{lrbox}{\SBdotTfTfdotinvplusdsbisbsC}
\begin{minipage}{\SBdotTfTfdotinvplusdsbisbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R0=desc3(v,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|SB.TfTf.inv+dsb-isbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SBdotTfTfdotinvplusdsbisbsB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SBdotTfTfdotinvplusdsbisbsA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SBdotTfTfdotinvplusdsbisbsC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvplusdsbisbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvplusdsbisbsK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvplusdsbisbsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvplusdsbisbsO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/SB.TfTf.invv+rfi-ctrl-isbs.tex <==
\newlength{\SBdotTfTfdotinvvplusrfictrlisbsH}
\setlength{\SBdotTfTfdotinvvplusrfictrlisbsH}{0cm}
\newsavebox{\SBdotTfTfdotinvvplusrfictrlisbsI}
\begin{lrbox}{\SBdotTfTfdotinvvplusrfictrlisbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X7,[X1]
CBNZ X7,L0
L0:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvvplusrfictrlisbsJ}
\settowidth{\SBdotTfTfdotinvvplusrfictrlisbsJ}{\usebox{\SBdotTfTfdotinvvplusrfictrlisbsI}}
\addtolength{\SBdotTfTfdotinvvplusrfictrlisbsH}{\SBdotTfTfdotinvvplusrfictrlisbsJ}
\newsavebox{\SBdotTfTfdotinvvplusrfictrlisbsK}
\begin{lrbox}{\SBdotTfTfdotinvvplusrfictrlisbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X7,[X1]
CBNZ X7,L1
L1:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvvplusrfictrlisbsL}
\settowidth{\SBdotTfTfdotinvvplusrfictrlisbsL}{\usebox{\SBdotTfTfdotinvvplusrfictrlisbsK}}
\addtolength{\SBdotTfTfdotinvvplusrfictrlisbsH}{\SBdotTfTfdotinvvplusrfictrlisbsL}
\newsavebox{\SBdotTfTfdotinvvplusrfictrlisbsM}
\begin{lrbox}{\SBdotTfTfdotinvvplusrfictrlisbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvvplusrfictrlisbsN}
\settowidth{\SBdotTfTfdotinvvplusrfictrlisbsN}{\usebox{\SBdotTfTfdotinvvplusrfictrlisbsM}}
\addtolength{\SBdotTfTfdotinvvplusrfictrlisbsH}{\SBdotTfTfdotinvvplusrfictrlisbsN}
\newsavebox{\SBdotTfTfdotinvvplusrfictrlisbsO}
\begin{lrbox}{\SBdotTfTfdotinvvplusrfictrlisbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvvplusrfictrlisbsP}
\settowidth{\SBdotTfTfdotinvvplusrfictrlisbsP}{\usebox{\SBdotTfTfdotinvvplusrfictrlisbsO}}
\addtolength{\SBdotTfTfdotinvvplusrfictrlisbsH}{\SBdotTfTfdotinvvplusrfictrlisbsP}
\newsavebox{\SBdotTfTfdotinvvplusrfictrlisbsA}
\begin{lrbox}{\SBdotTfTfdotinvvplusrfictrlisbsA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> invalid;
    y ?-> pa2;
    v |-> pa2;
    *pa2 = 1;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvvplusrfictrlisbsB}
\settowidth{\SBdotTfTfdotinvvplusrfictrlisbsB}{\usebox{\SBdotTfTfdotinvvplusrfictrlisbsA}}
\newsavebox{\SBdotTfTfdotinvvplusrfictrlisbsC}
\begin{lrbox}{\SBdotTfTfdotinvvplusrfictrlisbsC}
\begin{minipage}{\SBdotTfTfdotinvvplusrfictrlisbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R0=desc3(v,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|SB.TfTf.invv+rfi-ctrl-isbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SBdotTfTfdotinvvplusrfictrlisbsB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SBdotTfTfdotinvvplusrfictrlisbsA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SBdotTfTfdotinvvplusrfictrlisbsC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvvplusrfictrlisbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvvplusrfictrlisbsK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvvplusrfictrlisbsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvvplusrfictrlisbsO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0 & 0:R7=desc3(u,page_table_base) & 1:R2=0 & 1:R7=desc3(v,page_table_base)|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/SwitchTable.EL2+msrttbr-eret.tex <==
\newlength{\SwitchTabledotELtwoplusmsrttbreretH}
\setlength{\SwitchTabledotELtwoplusmsrttbreretH}{0cm}
\newsavebox{\SwitchTabledotELtwoplusmsrttbreretI}
\begin{lrbox}{\SwitchTabledotELtwoplusmsrttbreretI}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
HVC #0
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SwitchTabledotELtwoplusmsrttbreretJ}
\settowidth{\SwitchTabledotELtwoplusmsrttbreretJ}{\usebox{\SwitchTabledotELtwoplusmsrttbreretI}}
\addtolength{\SwitchTabledotELtwoplusmsrttbreretH}{\SwitchTabledotELtwoplusmsrttbreretJ}
\newsavebox{\SwitchTabledotELtwoplusmsrttbreretK}
\begin{lrbox}{\SwitchTabledotELtwoplusmsrttbreretK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MSR TTBR0_EL1,X4
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SwitchTabledotELtwoplusmsrttbreretL}
\settowidth{\SwitchTabledotELtwoplusmsrttbreretL}{\usebox{\SwitchTabledotELtwoplusmsrttbreretK}}
\addtolength{\SwitchTabledotELtwoplusmsrttbreretH}{\SwitchTabledotELtwoplusmsrttbreretL}
\newsavebox{\SwitchTabledotELtwoplusmsrttbreretM}
\begin{lrbox}{\SwitchTabledotELtwoplusmsrttbreretM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
option default_tables = false;
physical pa1 pa2;

s1table initial_table 0x200000 {
    x |-> pa1 at level 3;
}

s1table new_table 0x280000  {
    x |-> pa2 at level 3;
}

s1table el2_table 0x300000 {
    identity 0x2000 with code;
}

*pa1 = 0;
*pa2 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\SwitchTabledotELtwoplusmsrttbreretN}
\settowidth{\SwitchTabledotELtwoplusmsrttbreretN}{\usebox{\SwitchTabledotELtwoplusmsrttbreretM}}
\newsavebox{\SwitchTabledotELtwoplusmsrttbreretO}
\begin{lrbox}{\SwitchTabledotELtwoplusmsrttbreretO}
\begin{minipage}{\SwitchTabledotELtwoplusmsrttbreretH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|R1=x|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=ttbr(asid=0x0000,base=new_table)|\\
\lstinline[language=IslaLitmusExp]|TTBR0_EL1=ttbr(base=initial_table,asid=0x0000)|\\
\lstinline[language=IslaLitmusExp]|TTBR0_EL2=ttbr(base=el2_table,asid=0x0000)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|SwitchTable.EL2+msrttbr-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SwitchTabledotELtwoplusmsrttbreretN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SwitchTabledotELtwoplusmsrttbreretM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SwitchTabledotELtwoplusmsrttbreretO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SwitchTabledotELtwoplusmsrttbreretI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\SwitchTabledotELtwoplusmsrttbreretK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/SwitchTable.same-asid+eret.toml.tex <==
\newlength{\SwitchTabledotsameasidpluseretdottomlH}
\setlength{\SwitchTabledotsameasidpluseretdottomlH}{0cm}
\newsavebox{\SwitchTabledotsameasidpluseretdottomlI}
\begin{lrbox}{\SwitchTabledotsameasidpluseretdottomlI}
\begin{lstlisting}[language=AArch64,showlines=true]
MSR TTBR0_EL1,X0
ERET
L0:
LDR X1,[X2]
\end{lstlisting}
\end{lrbox}
\newlength{\SwitchTabledotsameasidpluseretdottomlJ}
\settowidth{\SwitchTabledotsameasidpluseretdottomlJ}{\usebox{\SwitchTabledotsameasidpluseretdottomlI}}
\addtolength{\SwitchTabledotsameasidpluseretdottomlH}{\SwitchTabledotsameasidpluseretdottomlJ}
\newsavebox{\SwitchTabledotsameasidpluseretdottomlK}
\begin{lrbox}{\SwitchTabledotsameasidpluseretdottomlK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X1,#1
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SwitchTabledotsameasidpluseretdottomlL}
\settowidth{\SwitchTabledotsameasidpluseretdottomlL}{\usebox{\SwitchTabledotsameasidpluseretdottomlK}}
\addtolength{\SwitchTabledotsameasidpluseretdottomlH}{\SwitchTabledotsameasidpluseretdottomlL}
\newsavebox{\SwitchTabledotsameasidpluseretdottomlM}
\begin{lrbox}{\SwitchTabledotsameasidpluseretdottomlM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    intermediate ipa1;
    physical pa1;

    *pa1 = 0;

    s1table table0 0x2C0000 {
        identity 0x1000 with code;
        x |-> pa1;
    };
    s1table table1 0x300000 {
        identity 0x1000 with code;
        x |-> invalid;
    };

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SwitchTabledotsameasidpluseretdottomlN}
\settowidth{\SwitchTabledotsameasidpluseretdottomlN}{\usebox{\SwitchTabledotsameasidpluseretdottomlM}}
\newsavebox{\SwitchTabledotsameasidpluseretdottomlO}
\begin{lrbox}{\SwitchTabledotsameasidpluseretdottomlO}
\begin{minipage}{\SwitchTabledotsameasidpluseretdottomlH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL1=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b1|\\
\lstinline[language=IslaLitmusExp]|R0=ttbr(asid=0x01,base=table1)|\\
\lstinline[language=IslaLitmusExp]|R2=x|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL1=0b00000|\\
\lstinline[language=IslaLitmusExp]|TTBR0_EL1=ttbr(base=table0,asid=0x00)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|SwitchTable.same-asid+eret.toml|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SwitchTabledotsameasidpluseretdottomlN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SwitchTabledotsameasidpluseretdottomlM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SwitchTabledotsameasidpluseretdottomlO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SwitchTabledotsameasidpluseretdottomlI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\SwitchTabledotsameasidpluseretdottomlK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R1=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/W+T.tex <==
\newlength{\WplusTH}
\setlength{\WplusTH}{0cm}
\newsavebox{\WplusTI}
\begin{lrbox}{\WplusTI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WplusTJ}
\settowidth{\WplusTJ}{\usebox{\WplusTI}}
\addtolength{\WplusTH}{\WplusTJ}
\newsavebox{\WplusTK}
\begin{lrbox}{\WplusTK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WplusTL}
\settowidth{\WplusTL}{\usebox{\WplusTK}}
\addtolength{\WplusTH}{\WplusTL}
\newsavebox{\WplusTM}
\begin{lrbox}{\WplusTM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1000:
MOV X0,#0
\end{lstlisting}
\end{lrbox}
\newlength{\WplusTN}
\settowidth{\WplusTN}{\usebox{\WplusTM}}
\addtolength{\WplusTH}{\WplusTN}
\newsavebox{\WplusTO}
\begin{lrbox}{\WplusTO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid at level 2;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WplusTP}
\settowidth{\WplusTP}{\usebox{\WplusTO}}
\newsavebox{\WplusTA}
\begin{lrbox}{\WplusTA}
\begin{minipage}{\WplusTH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte2(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|W+T|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WplusTP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WplusTO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WplusTA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WplusTI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WplusTK}\\
  \cline{2-2}
  & handler\\
  \cline{2-2}
  & \usebox{\WplusTM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|true|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/W.tex <==
\newlength{\WH}
\setlength{\WH}{0cm}
\newsavebox{\WI}
\begin{lrbox}{\WI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WJ}
\settowidth{\WJ}{\usebox{\WI}}
\addtolength{\WH}{\WJ}
\newsavebox{\WK}
\begin{lrbox}{\WK}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
\end{lstlisting}
\end{lrbox}
\newlength{\WL}
\settowidth{\WL}{\usebox{\WK}}
\newsavebox{\WM}
\begin{lrbox}{\WM}
\begin{minipage}{\WH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=x|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|W|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WL}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WK}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WM}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WI}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|true|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/WBM+dsb-tlbiis-dsb.tex <==
\newlength{\WBMplusdsbtlbiisdsbH}
\setlength{\WBMplusdsbtlbiisdsbH}{0cm}
\newsavebox{\WBMplusdsbtlbiisdsbI}
\begin{lrbox}{\WBMplusdsbtlbiisdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X5
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WBMplusdsbtlbiisdsbJ}
\settowidth{\WBMplusdsbtlbiisdsbJ}{\usebox{\WBMplusdsbtlbiisdsbI}}
\addtolength{\WBMplusdsbtlbiisdsbH}{\WBMplusdsbtlbiisdsbJ}
\newsavebox{\WBMplusdsbtlbiisdsbK}
\begin{lrbox}{\WBMplusdsbtlbiisdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WBMplusdsbtlbiisdsbL}
\settowidth{\WBMplusdsbtlbiisdsbL}{\usebox{\WBMplusdsbtlbiisdsbK}}
\addtolength{\WBMplusdsbtlbiisdsbH}{\WBMplusdsbtlbiisdsbL}
\newsavebox{\WBMplusdsbtlbiisdsbM}
\begin{lrbox}{\WBMplusdsbtlbiisdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WBMplusdsbtlbiisdsbN}
\settowidth{\WBMplusdsbtlbiisdsbN}{\usebox{\WBMplusdsbtlbiisdsbM}}
\addtolength{\WBMplusdsbtlbiisdsbH}{\WBMplusdsbtlbiisdsbN}
\newsavebox{\WBMplusdsbtlbiisdsbO}
\begin{lrbox}{\WBMplusdsbtlbiisdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    y |-> pa1;
    *pa1 = 0;
    x ?-> invalid;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WBMplusdsbtlbiisdsbP}
\settowidth{\WBMplusdsbtlbiisdsbP}{\usebox{\WBMplusdsbtlbiisdsbO}}
\newsavebox{\WBMplusdsbtlbiisdsbA}
\begin{lrbox}{\WBMplusdsbtlbiisdsbA}
\begin{minipage}{\WBMplusdsbtlbiisdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0x2|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R5=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:R0=0x1|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WBM+dsb-tlbiis-dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WBMplusdsbtlbiisdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WBMplusdsbtlbiisdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WBMplusdsbtlbiisdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WBMplusdsbtlbiisdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WBMplusdsbtlbiisdsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WBMplusdsbtlbiisdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|x=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/WDS+dsb-tlbiipa-dsb-eret-po.tex <==
\newlength{\WDSplusdsbtlbiipadsberetpoH}
\setlength{\WDSplusdsbtlbiipadsberetpoH}{0cm}
\newsavebox{\WDSplusdsbtlbiipadsberetpoI}
\begin{lrbox}{\WDSplusdsbtlbiipadsberetpoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1,X6
DSB SY
ERET
L0:
STR X2,[X3]
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\WDSplusdsbtlbiipadsberetpoJ}
\settowidth{\WDSplusdsbtlbiipadsberetpoJ}{\usebox{\WDSplusdsbtlbiipadsberetpoI}}
\addtolength{\WDSplusdsbtlbiipadsberetpoH}{\WDSplusdsbtlbiipadsberetpoJ}
\newsavebox{\WDSplusdsbtlbiipadsberetpoK}
\begin{lrbox}{\WDSplusdsbtlbiipadsberetpoK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1200:
MOV X4,#1
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WDSplusdsbtlbiipadsberetpoL}
\settowidth{\WDSplusdsbtlbiipadsberetpoL}{\usebox{\WDSplusdsbtlbiipadsberetpoK}}
\addtolength{\WDSplusdsbtlbiipadsberetpoH}{\WDSplusdsbtlbiipadsberetpoL}
\newsavebox{\WDSplusdsbtlbiipadsberetpoM}
\begin{lrbox}{\WDSplusdsbtlbiipadsberetpoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X4,#2
MRS X20,ELR_EL2
ADD X20,X20,#4
MSR ELR_EL2,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WDSplusdsbtlbiipadsberetpoN}
\settowidth{\WDSplusdsbtlbiipadsberetpoN}{\usebox{\WDSplusdsbtlbiipadsberetpoM}}
\addtolength{\WDSplusdsbtlbiipadsberetpoH}{\WDSplusdsbtlbiipadsberetpoN}
\newsavebox{\WDSplusdsbtlbiipadsberetpoO}
\begin{lrbox}{\WDSplusdsbtlbiipadsberetpoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;
    x ?-> invalid;

    ipa1 |-> pa1;
    ipa1 ?-> invalid;

    *pa1 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WDSplusdsbtlbiipadsberetpoP}
\settowidth{\WDSplusdsbtlbiipadsberetpoP}{\usebox{\WDSplusdsbtlbiipadsberetpoO}}
\newsavebox{\WDSplusdsbtlbiipadsberetpoA}
\begin{lrbox}{\WDSplusdsbtlbiipadsberetpoA}
\begin{minipage}{\WDSplusdsbtlbiipadsberetpoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R2=0b0|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R5=x|\\
\lstinline[language=IslaLitmusExp]|R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00100|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WDS+dsb-tlbiipa-dsb-eret-po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WDSplusdsbtlbiipadsberetpoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WDSplusdsbtlbiipadsberetpoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WDSplusdsbtlbiipadsberetpoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WDSplusdsbtlbiipadsberetpoI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\WDSplusdsbtlbiipadsberetpoK}\\
  \cline{2-2}
  & thread0 el2 handler lower exc\\
  \cline{2-2}
  & \usebox{\WDSplusdsbtlbiipadsberetpoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/WDS+po-dsb-tlbiipa-dsb-eret.tex <==
\newlength{\WDSpluspodsbtlbiipadsberetH}
\setlength{\WDSpluspodsbtlbiipadsberetH}{0cm}
\newsavebox{\WDSpluspodsbtlbiipadsberetI}
\begin{lrbox}{\WDSpluspodsbtlbiipadsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
STR X2,[X3]
DSB SY
TLBI IPAS2E1,X6
DSB SY
ERET
L0:
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsberetJ}
\settowidth{\WDSpluspodsbtlbiipadsberetJ}{\usebox{\WDSpluspodsbtlbiipadsberetI}}
\addtolength{\WDSpluspodsbtlbiipadsberetH}{\WDSpluspodsbtlbiipadsberetJ}
\newsavebox{\WDSpluspodsbtlbiipadsberetK}
\begin{lrbox}{\WDSpluspodsbtlbiipadsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1200:
MOV X4,#1
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsberetL}
\settowidth{\WDSpluspodsbtlbiipadsberetL}{\usebox{\WDSpluspodsbtlbiipadsberetK}}
\addtolength{\WDSpluspodsbtlbiipadsberetH}{\WDSpluspodsbtlbiipadsberetL}
\newsavebox{\WDSpluspodsbtlbiipadsberetM}
\begin{lrbox}{\WDSpluspodsbtlbiipadsberetM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X4,#2
MRS X20,ELR_EL2
ADD X20,X20,#4
MSR ELR_EL2,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsberetN}
\settowidth{\WDSpluspodsbtlbiipadsberetN}{\usebox{\WDSpluspodsbtlbiipadsberetM}}
\addtolength{\WDSpluspodsbtlbiipadsberetH}{\WDSpluspodsbtlbiipadsberetN}
\newsavebox{\WDSpluspodsbtlbiipadsberetO}
\begin{lrbox}{\WDSpluspodsbtlbiipadsberetO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;
    x ?-> invalid;

    ipa1 |-> pa1;
    ipa1 ?-> invalid;

    *pa1 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsberetP}
\settowidth{\WDSpluspodsbtlbiipadsberetP}{\usebox{\WDSpluspodsbtlbiipadsberetO}}
\newsavebox{\WDSpluspodsbtlbiipadsberetA}
\begin{lrbox}{\WDSpluspodsbtlbiipadsberetA}
\begin{minipage}{\WDSpluspodsbtlbiipadsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R2=0b0|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R5=x|\\
\lstinline[language=IslaLitmusExp]|R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00100|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WDS+po-dsb-tlbiipa-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WDSpluspodsbtlbiipadsberetP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WDSpluspodsbtlbiipadsberetO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WDSpluspodsbtlbiipadsberetA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsberetI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsberetK}\\
  \cline{2-2}
  & thread0 el2 handler lower exc\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsberetM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/WDS+po-dsb-tlbiipa-dsb-po-eret.tex <==
\newlength{\WDSpluspodsbtlbiipadsbpoeretH}
\setlength{\WDSpluspodsbtlbiipadsbpoeretH}{0cm}
\newsavebox{\WDSpluspodsbtlbiipadsbpoeretI}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbpoeretI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1,X6
DSB SY
STR X2,[X3]
ERET
L0:
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsbpoeretJ}
\settowidth{\WDSpluspodsbtlbiipadsbpoeretJ}{\usebox{\WDSpluspodsbtlbiipadsbpoeretI}}
\addtolength{\WDSpluspodsbtlbiipadsbpoeretH}{\WDSpluspodsbtlbiipadsbpoeretJ}
\newsavebox{\WDSpluspodsbtlbiipadsbpoeretK}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbpoeretK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1200:
MOV X4,#1
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsbpoeretL}
\settowidth{\WDSpluspodsbtlbiipadsbpoeretL}{\usebox{\WDSpluspodsbtlbiipadsbpoeretK}}
\addtolength{\WDSpluspodsbtlbiipadsbpoeretH}{\WDSpluspodsbtlbiipadsbpoeretL}
\newsavebox{\WDSpluspodsbtlbiipadsbpoeretM}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbpoeretM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X4,#2
MRS X20,ELR_EL2
ADD X20,X20,#4
MSR ELR_EL2,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsbpoeretN}
\settowidth{\WDSpluspodsbtlbiipadsbpoeretN}{\usebox{\WDSpluspodsbtlbiipadsbpoeretM}}
\addtolength{\WDSpluspodsbtlbiipadsbpoeretH}{\WDSpluspodsbtlbiipadsbpoeretN}
\newsavebox{\WDSpluspodsbtlbiipadsbpoeretO}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbpoeretO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;
    x ?-> invalid;

    ipa1 |-> pa1;
    ipa1 ?-> invalid;

    *pa1 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsbpoeretP}
\settowidth{\WDSpluspodsbtlbiipadsbpoeretP}{\usebox{\WDSpluspodsbtlbiipadsbpoeretO}}
\newsavebox{\WDSpluspodsbtlbiipadsbpoeretA}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbpoeretA}
\begin{minipage}{\WDSpluspodsbtlbiipadsbpoeretH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R2=0b0|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R5=x|\\
\lstinline[language=IslaLitmusExp]|R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00100|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WDS+po-dsb-tlbiipa-dsb-po-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WDSpluspodsbtlbiipadsbpoeretP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WDSpluspodsbtlbiipadsbpoeretO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WDSpluspodsbtlbiipadsbpoeretA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsbpoeretI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsbpoeretK}\\
  \cline{2-2}
  & thread0 el2 handler lower exc\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsbpoeretM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/WDS+po-dsb-tlbiipa-dsb-tlbiis-dsb-eret.tex <==
\newlength{\WDSpluspodsbtlbiipadsbtlbiisdsberetH}
\setlength{\WDSpluspodsbtlbiipadsbtlbiisdsberetH}{0cm}
\newsavebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetI}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbtlbiisdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
STR X2,[X3]
DSB SY
TLBI IPAS2E1,X6
DSB SY
TLBI VMALLE1IS
DSB SY
ERET
L0:
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsbtlbiisdsberetJ}
\settowidth{\WDSpluspodsbtlbiipadsbtlbiisdsberetJ}{\usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetI}}
\addtolength{\WDSpluspodsbtlbiipadsbtlbiisdsberetH}{\WDSpluspodsbtlbiipadsbtlbiisdsberetJ}
\newsavebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetK}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbtlbiisdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1200:
MOV X4,#1
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsbtlbiisdsberetL}
\settowidth{\WDSpluspodsbtlbiipadsbtlbiisdsberetL}{\usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetK}}
\addtolength{\WDSpluspodsbtlbiipadsbtlbiisdsberetH}{\WDSpluspodsbtlbiipadsbtlbiisdsberetL}
\newsavebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetM}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbtlbiisdsberetM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X4,#2
MRS X20,ELR_EL2
ADD X20,X20,#4
MSR ELR_EL2,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsbtlbiisdsberetN}
\settowidth{\WDSpluspodsbtlbiipadsbtlbiisdsberetN}{\usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetM}}
\addtolength{\WDSpluspodsbtlbiipadsbtlbiisdsberetH}{\WDSpluspodsbtlbiipadsbtlbiisdsberetN}
\newsavebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetO}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbtlbiisdsberetO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;
    x ?-> invalid;

    ipa1 |-> pa1;
    ipa1 ?-> invalid;

    *pa1 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsbtlbiisdsberetP}
\settowidth{\WDSpluspodsbtlbiipadsbtlbiisdsberetP}{\usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetO}}
\newsavebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetA}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbtlbiisdsberetA}
\begin{minipage}{\WDSpluspodsbtlbiipadsbtlbiisdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R2=0b0|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R5=x|\\
\lstinline[language=IslaLitmusExp]|R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00100|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WDS+po-dsb-tlbiipa-dsb-tlbiis-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WDSpluspodsbtlbiipadsbtlbiisdsberetP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetK}\\
  \cline{2-2}
  & thread0 el2 handler lower exc\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/WRC.RRTf.inv+addrs.tex <==
\newlength{\WRCdotRRTfdotinvplusaddrsH}
\setlength{\WRCdotRRTfdotinvplusaddrsH}{0cm}
\newsavebox{\WRCdotRRTfdotinvplusaddrsI}
\begin{lrbox}{\WRCdotRRTfdotinvplusaddrsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusaddrsJ}
\settowidth{\WRCdotRRTfdotinvplusaddrsJ}{\usebox{\WRCdotRRTfdotinvplusaddrsI}}
\addtolength{\WRCdotRRTfdotinvplusaddrsH}{\WRCdotRRTfdotinvplusaddrsJ}
\newsavebox{\WRCdotRRTfdotinvplusaddrsK}
\begin{lrbox}{\WRCdotRRTfdotinvplusaddrsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
STR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusaddrsL}
\settowidth{\WRCdotRRTfdotinvplusaddrsL}{\usebox{\WRCdotRRTfdotinvplusaddrsK}}
\addtolength{\WRCdotRRTfdotinvplusaddrsH}{\WRCdotRRTfdotinvplusaddrsL}
\newsavebox{\WRCdotRRTfdotinvplusaddrsM}
\begin{lrbox}{\WRCdotRRTfdotinvplusaddrsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusaddrsN}
\settowidth{\WRCdotRRTfdotinvplusaddrsN}{\usebox{\WRCdotRRTfdotinvplusaddrsM}}
\addtolength{\WRCdotRRTfdotinvplusaddrsH}{\WRCdotRRTfdotinvplusaddrsN}
\newsavebox{\WRCdotRRTfdotinvplusaddrsO}
\begin{lrbox}{\WRCdotRRTfdotinvplusaddrsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusaddrsP}
\settowidth{\WRCdotRRTfdotinvplusaddrsP}{\usebox{\WRCdotRRTfdotinvplusaddrsO}}
\addtolength{\WRCdotRRTfdotinvplusaddrsH}{\WRCdotRRTfdotinvplusaddrsP}
\newsavebox{\WRCdotRRTfdotinvplusaddrsA}
\begin{lrbox}{\WRCdotRRTfdotinvplusaddrsA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusaddrsB}
\settowidth{\WRCdotRRTfdotinvplusaddrsB}{\usebox{\WRCdotRRTfdotinvplusaddrsA}}
\newsavebox{\WRCdotRRTfdotinvplusaddrsC}
\begin{lrbox}{\WRCdotRRTfdotinvplusaddrsC}
\begin{minipage}{\WRCdotRRTfdotinvplusaddrsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.RRTf.inv+addrs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotRRTfdotinvplusaddrsB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotRRTfdotinvplusaddrsA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotRRTfdotinvplusaddrsC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusaddrsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusaddrsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusaddrsM}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusaddrsO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=desc3(z,page_table_base) & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/WRC.RRTf.inv+dmbs.tex <==
\newlength{\WRCdotRRTfdotinvplusdmbsH}
\setlength{\WRCdotRRTfdotinvplusdmbsH}{0cm}
\newsavebox{\WRCdotRRTfdotinvplusdmbsI}
\begin{lrbox}{\WRCdotRRTfdotinvplusdmbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdmbsJ}
\settowidth{\WRCdotRRTfdotinvplusdmbsJ}{\usebox{\WRCdotRRTfdotinvplusdmbsI}}
\addtolength{\WRCdotRRTfdotinvplusdmbsH}{\WRCdotRRTfdotinvplusdmbsJ}
\newsavebox{\WRCdotRRTfdotinvplusdmbsK}
\begin{lrbox}{\WRCdotRRTfdotinvplusdmbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdmbsL}
\settowidth{\WRCdotRRTfdotinvplusdmbsL}{\usebox{\WRCdotRRTfdotinvplusdmbsK}}
\addtolength{\WRCdotRRTfdotinvplusdmbsH}{\WRCdotRRTfdotinvplusdmbsL}
\newsavebox{\WRCdotRRTfdotinvplusdmbsM}
\begin{lrbox}{\WRCdotRRTfdotinvplusdmbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdmbsN}
\settowidth{\WRCdotRRTfdotinvplusdmbsN}{\usebox{\WRCdotRRTfdotinvplusdmbsM}}
\addtolength{\WRCdotRRTfdotinvplusdmbsH}{\WRCdotRRTfdotinvplusdmbsN}
\newsavebox{\WRCdotRRTfdotinvplusdmbsO}
\begin{lrbox}{\WRCdotRRTfdotinvplusdmbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdmbsP}
\settowidth{\WRCdotRRTfdotinvplusdmbsP}{\usebox{\WRCdotRRTfdotinvplusdmbsO}}
\addtolength{\WRCdotRRTfdotinvplusdmbsH}{\WRCdotRRTfdotinvplusdmbsP}
\newsavebox{\WRCdotRRTfdotinvplusdmbsA}
\begin{lrbox}{\WRCdotRRTfdotinvplusdmbsA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdmbsB}
\settowidth{\WRCdotRRTfdotinvplusdmbsB}{\usebox{\WRCdotRRTfdotinvplusdmbsA}}
\newsavebox{\WRCdotRRTfdotinvplusdmbsC}
\begin{lrbox}{\WRCdotRRTfdotinvplusdmbsC}
\begin{minipage}{\WRCdotRRTfdotinvplusdmbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.RRTf.inv+dmbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotRRTfdotinvplusdmbsB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotRRTfdotinvplusdmbsA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotRRTfdotinvplusdmbsC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdmbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdmbsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdmbsM}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdmbsO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=desc3(z,page_table_base) & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/WRC.RRTf.inv+dsb+ctrl-isb.tex <==
\newlength{\WRCdotRRTfdotinvplusdsbplusctrlisbH}
\setlength{\WRCdotRRTfdotinvplusdsbplusctrlisbH}{0cm}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusctrlisbI}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusctrlisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusctrlisbJ}
\settowidth{\WRCdotRRTfdotinvplusdsbplusctrlisbJ}{\usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbI}}
\addtolength{\WRCdotRRTfdotinvplusdsbplusctrlisbH}{\WRCdotRRTfdotinvplusdsbplusctrlisbJ}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusctrlisbK}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusctrlisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusctrlisbL}
\settowidth{\WRCdotRRTfdotinvplusdsbplusctrlisbL}{\usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbK}}
\addtolength{\WRCdotRRTfdotinvplusdsbplusctrlisbH}{\WRCdotRRTfdotinvplusdsbplusctrlisbL}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusctrlisbM}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusctrlisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBNZ X0,L0
L0:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusctrlisbN}
\settowidth{\WRCdotRRTfdotinvplusdsbplusctrlisbN}{\usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbM}}
\addtolength{\WRCdotRRTfdotinvplusdsbplusctrlisbH}{\WRCdotRRTfdotinvplusdsbplusctrlisbN}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusctrlisbO}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusctrlisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusctrlisbP}
\settowidth{\WRCdotRRTfdotinvplusdsbplusctrlisbP}{\usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbO}}
\addtolength{\WRCdotRRTfdotinvplusdsbplusctrlisbH}{\WRCdotRRTfdotinvplusdsbplusctrlisbP}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusctrlisbA}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusctrlisbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusctrlisbB}
\settowidth{\WRCdotRRTfdotinvplusdsbplusctrlisbB}{\usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbA}}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusctrlisbC}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusctrlisbC}
\begin{minipage}{\WRCdotRRTfdotinvplusdsbplusctrlisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.RRTf.inv+dsb+ctrl-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotRRTfdotinvplusdsbplusctrlisbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbM}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=desc3(z,page_table_base) & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/WRC.RRTf.inv+dsb+dsb-isb.tex <==
\newlength{\WRCdotRRTfdotinvplusdsbplusdsbisbH}
\setlength{\WRCdotRRTfdotinvplusdsbplusdsbisbH}{0cm}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusdsbisbI}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusdsbisbJ}
\settowidth{\WRCdotRRTfdotinvplusdsbplusdsbisbJ}{\usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbI}}
\addtolength{\WRCdotRRTfdotinvplusdsbplusdsbisbH}{\WRCdotRRTfdotinvplusdsbplusdsbisbJ}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusdsbisbK}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusdsbisbL}
\settowidth{\WRCdotRRTfdotinvplusdsbplusdsbisbL}{\usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbK}}
\addtolength{\WRCdotRRTfdotinvplusdsbplusdsbisbH}{\WRCdotRRTfdotinvplusdsbplusdsbisbL}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusdsbisbM}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusdsbisbN}
\settowidth{\WRCdotRRTfdotinvplusdsbplusdsbisbN}{\usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbM}}
\addtolength{\WRCdotRRTfdotinvplusdsbplusdsbisbH}{\WRCdotRRTfdotinvplusdsbplusdsbisbN}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusdsbisbO}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusdsbisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusdsbisbP}
\settowidth{\WRCdotRRTfdotinvplusdsbplusdsbisbP}{\usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbO}}
\addtolength{\WRCdotRRTfdotinvplusdsbplusdsbisbH}{\WRCdotRRTfdotinvplusdsbplusdsbisbP}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusdsbisbA}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusdsbisbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusdsbisbB}
\settowidth{\WRCdotRRTfdotinvplusdsbplusdsbisbB}{\usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbA}}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusdsbisbC}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusdsbisbC}
\begin{minipage}{\WRCdotRRTfdotinvplusdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.RRTf.inv+dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotRRTfdotinvplusdsbplusdsbisbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbM}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=desc3(z,page_table_base) & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/WRC.RRTf.inv+dsbs.tex <==
\newlength{\WRCdotRRTfdotinvplusdsbsH}
\setlength{\WRCdotRRTfdotinvplusdsbsH}{0cm}
\newsavebox{\WRCdotRRTfdotinvplusdsbsI}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbsJ}
\settowidth{\WRCdotRRTfdotinvplusdsbsJ}{\usebox{\WRCdotRRTfdotinvplusdsbsI}}
\addtolength{\WRCdotRRTfdotinvplusdsbsH}{\WRCdotRRTfdotinvplusdsbsJ}
\newsavebox{\WRCdotRRTfdotinvplusdsbsK}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbsL}
\settowidth{\WRCdotRRTfdotinvplusdsbsL}{\usebox{\WRCdotRRTfdotinvplusdsbsK}}
\addtolength{\WRCdotRRTfdotinvplusdsbsH}{\WRCdotRRTfdotinvplusdsbsL}
\newsavebox{\WRCdotRRTfdotinvplusdsbsM}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbsN}
\settowidth{\WRCdotRRTfdotinvplusdsbsN}{\usebox{\WRCdotRRTfdotinvplusdsbsM}}
\addtolength{\WRCdotRRTfdotinvplusdsbsH}{\WRCdotRRTfdotinvplusdsbsN}
\newsavebox{\WRCdotRRTfdotinvplusdsbsO}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbsP}
\settowidth{\WRCdotRRTfdotinvplusdsbsP}{\usebox{\WRCdotRRTfdotinvplusdsbsO}}
\addtolength{\WRCdotRRTfdotinvplusdsbsH}{\WRCdotRRTfdotinvplusdsbsP}
\newsavebox{\WRCdotRRTfdotinvplusdsbsA}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbsA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbsB}
\settowidth{\WRCdotRRTfdotinvplusdsbsB}{\usebox{\WRCdotRRTfdotinvplusdsbsA}}
\newsavebox{\WRCdotRRTfdotinvplusdsbsC}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbsC}
\begin{minipage}{\WRCdotRRTfdotinvplusdsbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.RRTf.inv+dsbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotRRTfdotinvplusdsbsB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotRRTfdotinvplusdsbsA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotRRTfdotinvplusdsbsC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbsM}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbsO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=desc3(z,page_table_base) & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/WRC.RRTf.inv+pos.tex <==
\newlength{\WRCdotRRTfdotinvplusposH}
\setlength{\WRCdotRRTfdotinvplusposH}{0cm}
\newsavebox{\WRCdotRRTfdotinvplusposI}
\begin{lrbox}{\WRCdotRRTfdotinvplusposI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusposJ}
\settowidth{\WRCdotRRTfdotinvplusposJ}{\usebox{\WRCdotRRTfdotinvplusposI}}
\addtolength{\WRCdotRRTfdotinvplusposH}{\WRCdotRRTfdotinvplusposJ}
\newsavebox{\WRCdotRRTfdotinvplusposK}
\begin{lrbox}{\WRCdotRRTfdotinvplusposK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusposL}
\settowidth{\WRCdotRRTfdotinvplusposL}{\usebox{\WRCdotRRTfdotinvplusposK}}
\addtolength{\WRCdotRRTfdotinvplusposH}{\WRCdotRRTfdotinvplusposL}
\newsavebox{\WRCdotRRTfdotinvplusposM}
\begin{lrbox}{\WRCdotRRTfdotinvplusposM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusposN}
\settowidth{\WRCdotRRTfdotinvplusposN}{\usebox{\WRCdotRRTfdotinvplusposM}}
\addtolength{\WRCdotRRTfdotinvplusposH}{\WRCdotRRTfdotinvplusposN}
\newsavebox{\WRCdotRRTfdotinvplusposO}
\begin{lrbox}{\WRCdotRRTfdotinvplusposO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusposP}
\settowidth{\WRCdotRRTfdotinvplusposP}{\usebox{\WRCdotRRTfdotinvplusposO}}
\addtolength{\WRCdotRRTfdotinvplusposH}{\WRCdotRRTfdotinvplusposP}
\newsavebox{\WRCdotRRTfdotinvplusposA}
\begin{lrbox}{\WRCdotRRTfdotinvplusposA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusposB}
\settowidth{\WRCdotRRTfdotinvplusposB}{\usebox{\WRCdotRRTfdotinvplusposA}}
\newsavebox{\WRCdotRRTfdotinvplusposC}
\begin{lrbox}{\WRCdotRRTfdotinvplusposC}
\begin{minipage}{\WRCdotRRTfdotinvplusposH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.RRTf.inv+pos|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotRRTfdotinvplusposB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotRRTfdotinvplusposA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotRRTfdotinvplusposC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusposI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusposK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusposM}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusposO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=desc3(z,page_table_base) & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/WRC.TRTf.inv+addrs.tex <==
\newlength{\WRCdotTRTfdotinvplusaddrsH}
\setlength{\WRCdotTRTfdotinvplusaddrsH}{0cm}
\newsavebox{\WRCdotTRTfdotinvplusaddrsI}
\begin{lrbox}{\WRCdotTRTfdotinvplusaddrsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusaddrsJ}
\settowidth{\WRCdotTRTfdotinvplusaddrsJ}{\usebox{\WRCdotTRTfdotinvplusaddrsI}}
\addtolength{\WRCdotTRTfdotinvplusaddrsH}{\WRCdotTRTfdotinvplusaddrsJ}
\newsavebox{\WRCdotTRTfdotinvplusaddrsK}
\begin{lrbox}{\WRCdotTRTfdotinvplusaddrsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
STR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusaddrsL}
\settowidth{\WRCdotTRTfdotinvplusaddrsL}{\usebox{\WRCdotTRTfdotinvplusaddrsK}}
\addtolength{\WRCdotTRTfdotinvplusaddrsH}{\WRCdotTRTfdotinvplusaddrsL}
\newsavebox{\WRCdotTRTfdotinvplusaddrsM}
\begin{lrbox}{\WRCdotTRTfdotinvplusaddrsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusaddrsN}
\settowidth{\WRCdotTRTfdotinvplusaddrsN}{\usebox{\WRCdotTRTfdotinvplusaddrsM}}
\addtolength{\WRCdotTRTfdotinvplusaddrsH}{\WRCdotTRTfdotinvplusaddrsN}
\newsavebox{\WRCdotTRTfdotinvplusaddrsO}
\begin{lrbox}{\WRCdotTRTfdotinvplusaddrsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusaddrsP}
\settowidth{\WRCdotTRTfdotinvplusaddrsP}{\usebox{\WRCdotTRTfdotinvplusaddrsO}}
\addtolength{\WRCdotTRTfdotinvplusaddrsH}{\WRCdotTRTfdotinvplusaddrsP}
\newsavebox{\WRCdotTRTfdotinvplusaddrsA}
\begin{lrbox}{\WRCdotTRTfdotinvplusaddrsA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusaddrsB}
\settowidth{\WRCdotTRTfdotinvplusaddrsB}{\usebox{\WRCdotTRTfdotinvplusaddrsA}}
\addtolength{\WRCdotTRTfdotinvplusaddrsH}{\WRCdotTRTfdotinvplusaddrsB}
\newsavebox{\WRCdotTRTfdotinvplusaddrsC}
\begin{lrbox}{\WRCdotTRTfdotinvplusaddrsC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusaddrsD}
\settowidth{\WRCdotTRTfdotinvplusaddrsD}{\usebox{\WRCdotTRTfdotinvplusaddrsC}}
\newsavebox{\WRCdotTRTfdotinvplusaddrsE}
\begin{lrbox}{\WRCdotTRTfdotinvplusaddrsE}
\begin{minipage}{\WRCdotTRTfdotinvplusaddrsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TRTf.inv+addrs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTRTfdotinvplusaddrsD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTRTfdotinvplusaddrsC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTRTfdotinvplusaddrsE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusaddrsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusaddrsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusaddrsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusaddrsO}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusaddrsA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/WRC.TRTf.inv+dmbs.tex <==
\newlength{\WRCdotTRTfdotinvplusdmbsH}
\setlength{\WRCdotTRTfdotinvplusdmbsH}{0cm}
\newsavebox{\WRCdotTRTfdotinvplusdmbsI}
\begin{lrbox}{\WRCdotTRTfdotinvplusdmbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdmbsJ}
\settowidth{\WRCdotTRTfdotinvplusdmbsJ}{\usebox{\WRCdotTRTfdotinvplusdmbsI}}
\addtolength{\WRCdotTRTfdotinvplusdmbsH}{\WRCdotTRTfdotinvplusdmbsJ}
\newsavebox{\WRCdotTRTfdotinvplusdmbsK}
\begin{lrbox}{\WRCdotTRTfdotinvplusdmbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdmbsL}
\settowidth{\WRCdotTRTfdotinvplusdmbsL}{\usebox{\WRCdotTRTfdotinvplusdmbsK}}
\addtolength{\WRCdotTRTfdotinvplusdmbsH}{\WRCdotTRTfdotinvplusdmbsL}
\newsavebox{\WRCdotTRTfdotinvplusdmbsM}
\begin{lrbox}{\WRCdotTRTfdotinvplusdmbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdmbsN}
\settowidth{\WRCdotTRTfdotinvplusdmbsN}{\usebox{\WRCdotTRTfdotinvplusdmbsM}}
\addtolength{\WRCdotTRTfdotinvplusdmbsH}{\WRCdotTRTfdotinvplusdmbsN}
\newsavebox{\WRCdotTRTfdotinvplusdmbsO}
\begin{lrbox}{\WRCdotTRTfdotinvplusdmbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdmbsP}
\settowidth{\WRCdotTRTfdotinvplusdmbsP}{\usebox{\WRCdotTRTfdotinvplusdmbsO}}
\addtolength{\WRCdotTRTfdotinvplusdmbsH}{\WRCdotTRTfdotinvplusdmbsP}
\newsavebox{\WRCdotTRTfdotinvplusdmbsA}
\begin{lrbox}{\WRCdotTRTfdotinvplusdmbsA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdmbsB}
\settowidth{\WRCdotTRTfdotinvplusdmbsB}{\usebox{\WRCdotTRTfdotinvplusdmbsA}}
\addtolength{\WRCdotTRTfdotinvplusdmbsH}{\WRCdotTRTfdotinvplusdmbsB}
\newsavebox{\WRCdotTRTfdotinvplusdmbsC}
\begin{lrbox}{\WRCdotTRTfdotinvplusdmbsC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdmbsD}
\settowidth{\WRCdotTRTfdotinvplusdmbsD}{\usebox{\WRCdotTRTfdotinvplusdmbsC}}
\newsavebox{\WRCdotTRTfdotinvplusdmbsE}
\begin{lrbox}{\WRCdotTRTfdotinvplusdmbsE}
\begin{minipage}{\WRCdotTRTfdotinvplusdmbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TRTf.inv+dmbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTRTfdotinvplusdmbsD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTRTfdotinvplusdmbsC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTRTfdotinvplusdmbsE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdmbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdmbsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdmbsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdmbsO}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdmbsA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/WRC.TRTf.inv+dsb+dsb-isb.tex <==
\newlength{\WRCdotTRTfdotinvplusdsbplusdsbisbH}
\setlength{\WRCdotTRTfdotinvplusdsbplusdsbisbH}{0cm}
\newsavebox{\WRCdotTRTfdotinvplusdsbplusdsbisbI}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbplusdsbisbJ}
\settowidth{\WRCdotTRTfdotinvplusdsbplusdsbisbJ}{\usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbI}}
\addtolength{\WRCdotTRTfdotinvplusdsbplusdsbisbH}{\WRCdotTRTfdotinvplusdsbplusdsbisbJ}
\newsavebox{\WRCdotTRTfdotinvplusdsbplusdsbisbK}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbplusdsbisbL}
\settowidth{\WRCdotTRTfdotinvplusdsbplusdsbisbL}{\usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbK}}
\addtolength{\WRCdotTRTfdotinvplusdsbplusdsbisbH}{\WRCdotTRTfdotinvplusdsbplusdsbisbL}
\newsavebox{\WRCdotTRTfdotinvplusdsbplusdsbisbM}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbplusdsbisbN}
\settowidth{\WRCdotTRTfdotinvplusdsbplusdsbisbN}{\usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbM}}
\addtolength{\WRCdotTRTfdotinvplusdsbplusdsbisbH}{\WRCdotTRTfdotinvplusdsbplusdsbisbN}
\newsavebox{\WRCdotTRTfdotinvplusdsbplusdsbisbO}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbplusdsbisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbplusdsbisbP}
\settowidth{\WRCdotTRTfdotinvplusdsbplusdsbisbP}{\usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbO}}
\addtolength{\WRCdotTRTfdotinvplusdsbplusdsbisbH}{\WRCdotTRTfdotinvplusdsbplusdsbisbP}
\newsavebox{\WRCdotTRTfdotinvplusdsbplusdsbisbA}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbplusdsbisbA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbplusdsbisbB}
\settowidth{\WRCdotTRTfdotinvplusdsbplusdsbisbB}{\usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbA}}
\addtolength{\WRCdotTRTfdotinvplusdsbplusdsbisbH}{\WRCdotTRTfdotinvplusdsbplusdsbisbB}
\newsavebox{\WRCdotTRTfdotinvplusdsbplusdsbisbC}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbplusdsbisbC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbplusdsbisbD}
\settowidth{\WRCdotTRTfdotinvplusdsbplusdsbisbD}{\usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbC}}
\newsavebox{\WRCdotTRTfdotinvplusdsbplusdsbisbE}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbplusdsbisbE}
\begin{minipage}{\WRCdotTRTfdotinvplusdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TRTf.inv+dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTRTfdotinvplusdsbplusdsbisbD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbO}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/WRC.TRTf.inv+dsbs.tex <==
\newlength{\WRCdotTRTfdotinvplusdsbsH}
\setlength{\WRCdotTRTfdotinvplusdsbsH}{0cm}
\newsavebox{\WRCdotTRTfdotinvplusdsbsI}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbsJ}
\settowidth{\WRCdotTRTfdotinvplusdsbsJ}{\usebox{\WRCdotTRTfdotinvplusdsbsI}}
\addtolength{\WRCdotTRTfdotinvplusdsbsH}{\WRCdotTRTfdotinvplusdsbsJ}
\newsavebox{\WRCdotTRTfdotinvplusdsbsK}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbsL}
\settowidth{\WRCdotTRTfdotinvplusdsbsL}{\usebox{\WRCdotTRTfdotinvplusdsbsK}}
\addtolength{\WRCdotTRTfdotinvplusdsbsH}{\WRCdotTRTfdotinvplusdsbsL}
\newsavebox{\WRCdotTRTfdotinvplusdsbsM}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbsN}
\settowidth{\WRCdotTRTfdotinvplusdsbsN}{\usebox{\WRCdotTRTfdotinvplusdsbsM}}
\addtolength{\WRCdotTRTfdotinvplusdsbsH}{\WRCdotTRTfdotinvplusdsbsN}
\newsavebox{\WRCdotTRTfdotinvplusdsbsO}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbsP}
\settowidth{\WRCdotTRTfdotinvplusdsbsP}{\usebox{\WRCdotTRTfdotinvplusdsbsO}}
\addtolength{\WRCdotTRTfdotinvplusdsbsH}{\WRCdotTRTfdotinvplusdsbsP}
\newsavebox{\WRCdotTRTfdotinvplusdsbsA}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbsA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbsB}
\settowidth{\WRCdotTRTfdotinvplusdsbsB}{\usebox{\WRCdotTRTfdotinvplusdsbsA}}
\addtolength{\WRCdotTRTfdotinvplusdsbsH}{\WRCdotTRTfdotinvplusdsbsB}
\newsavebox{\WRCdotTRTfdotinvplusdsbsC}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbsC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbsD}
\settowidth{\WRCdotTRTfdotinvplusdsbsD}{\usebox{\WRCdotTRTfdotinvplusdsbsC}}
\newsavebox{\WRCdotTRTfdotinvplusdsbsE}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbsE}
\begin{minipage}{\WRCdotTRTfdotinvplusdsbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TRTf.inv+dsbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTRTfdotinvplusdsbsD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTRTfdotinvplusdsbsC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTRTfdotinvplusdsbsE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbsO}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbsA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/WRC.TRTf.inv+pos.tex <==
\newlength{\WRCdotTRTfdotinvplusposH}
\setlength{\WRCdotTRTfdotinvplusposH}{0cm}
\newsavebox{\WRCdotTRTfdotinvplusposI}
\begin{lrbox}{\WRCdotTRTfdotinvplusposI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusposJ}
\settowidth{\WRCdotTRTfdotinvplusposJ}{\usebox{\WRCdotTRTfdotinvplusposI}}
\addtolength{\WRCdotTRTfdotinvplusposH}{\WRCdotTRTfdotinvplusposJ}
\newsavebox{\WRCdotTRTfdotinvplusposK}
\begin{lrbox}{\WRCdotTRTfdotinvplusposK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusposL}
\settowidth{\WRCdotTRTfdotinvplusposL}{\usebox{\WRCdotTRTfdotinvplusposK}}
\addtolength{\WRCdotTRTfdotinvplusposH}{\WRCdotTRTfdotinvplusposL}
\newsavebox{\WRCdotTRTfdotinvplusposM}
\begin{lrbox}{\WRCdotTRTfdotinvplusposM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusposN}
\settowidth{\WRCdotTRTfdotinvplusposN}{\usebox{\WRCdotTRTfdotinvplusposM}}
\addtolength{\WRCdotTRTfdotinvplusposH}{\WRCdotTRTfdotinvplusposN}
\newsavebox{\WRCdotTRTfdotinvplusposO}
\begin{lrbox}{\WRCdotTRTfdotinvplusposO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusposP}
\settowidth{\WRCdotTRTfdotinvplusposP}{\usebox{\WRCdotTRTfdotinvplusposO}}
\addtolength{\WRCdotTRTfdotinvplusposH}{\WRCdotTRTfdotinvplusposP}
\newsavebox{\WRCdotTRTfdotinvplusposA}
\begin{lrbox}{\WRCdotTRTfdotinvplusposA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusposB}
\settowidth{\WRCdotTRTfdotinvplusposB}{\usebox{\WRCdotTRTfdotinvplusposA}}
\addtolength{\WRCdotTRTfdotinvplusposH}{\WRCdotTRTfdotinvplusposB}
\newsavebox{\WRCdotTRTfdotinvplusposC}
\begin{lrbox}{\WRCdotTRTfdotinvplusposC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusposD}
\settowidth{\WRCdotTRTfdotinvplusposD}{\usebox{\WRCdotTRTfdotinvplusposC}}
\newsavebox{\WRCdotTRTfdotinvplusposE}
\begin{lrbox}{\WRCdotTRTfdotinvplusposE}
\begin{minipage}{\WRCdotTRTfdotinvplusposH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TRTf.inv+pos|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTRTfdotinvplusposD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTRTfdotinvplusposC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTRTfdotinvplusposE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusposI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusposK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusposM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusposO}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusposA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/WRC.TTTf.inv+addrs.tex <==
\newlength{\WRCdotTTTfdotinvplusaddrsH}
\setlength{\WRCdotTTTfdotinvplusaddrsH}{0cm}
\newsavebox{\WRCdotTTTfdotinvplusaddrsI}
\begin{lrbox}{\WRCdotTTTfdotinvplusaddrsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusaddrsJ}
\settowidth{\WRCdotTTTfdotinvplusaddrsJ}{\usebox{\WRCdotTTTfdotinvplusaddrsI}}
\addtolength{\WRCdotTTTfdotinvplusaddrsH}{\WRCdotTTTfdotinvplusaddrsJ}
\newsavebox{\WRCdotTTTfdotinvplusaddrsK}
\begin{lrbox}{\WRCdotTTTfdotinvplusaddrsK}
\begin{lstlisting}[language=AArch64,showlines=true]
MOV X0,#0
LDR X0,[X1]
EOR X4,X0,X0
STR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusaddrsL}
\settowidth{\WRCdotTTTfdotinvplusaddrsL}{\usebox{\WRCdotTTTfdotinvplusaddrsK}}
\addtolength{\WRCdotTTTfdotinvplusaddrsH}{\WRCdotTTTfdotinvplusaddrsL}
\newsavebox{\WRCdotTTTfdotinvplusaddrsM}
\begin{lrbox}{\WRCdotTTTfdotinvplusaddrsM}
\begin{lstlisting}[language=AArch64,showlines=true]
MOV X0,#0
LDR X0,[X1]
EOR X4,X0,X0
MOV X2,#0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusaddrsN}
\settowidth{\WRCdotTTTfdotinvplusaddrsN}{\usebox{\WRCdotTTTfdotinvplusaddrsM}}
\addtolength{\WRCdotTTTfdotinvplusaddrsH}{\WRCdotTTTfdotinvplusaddrsN}
\newsavebox{\WRCdotTTTfdotinvplusaddrsO}
\begin{lrbox}{\WRCdotTTTfdotinvplusaddrsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusaddrsP}
\settowidth{\WRCdotTTTfdotinvplusaddrsP}{\usebox{\WRCdotTTTfdotinvplusaddrsO}}
\addtolength{\WRCdotTTTfdotinvplusaddrsH}{\WRCdotTTTfdotinvplusaddrsP}
\newsavebox{\WRCdotTTTfdotinvplusaddrsA}
\begin{lrbox}{\WRCdotTTTfdotinvplusaddrsA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusaddrsB}
\settowidth{\WRCdotTTTfdotinvplusaddrsB}{\usebox{\WRCdotTTTfdotinvplusaddrsA}}
\addtolength{\WRCdotTTTfdotinvplusaddrsH}{\WRCdotTTTfdotinvplusaddrsB}
\newsavebox{\WRCdotTTTfdotinvplusaddrsC}
\begin{lrbox}{\WRCdotTTTfdotinvplusaddrsC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusaddrsD}
\settowidth{\WRCdotTTTfdotinvplusaddrsD}{\usebox{\WRCdotTTTfdotinvplusaddrsC}}
\newsavebox{\WRCdotTTTfdotinvplusaddrsE}
\begin{lrbox}{\WRCdotTTTfdotinvplusaddrsE}
\begin{minipage}{\WRCdotTTTfdotinvplusaddrsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:__isla_monomorphize_writes=true|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TTTf.inv+addrs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTTTfdotinvplusaddrsD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTTTfdotinvplusaddrsC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTTTfdotinvplusaddrsE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusaddrsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusaddrsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusaddrsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusaddrsO}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusaddrsA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/WRC.TTTf.inv+data+addr.tex <==
\newlength{\WRCdotTTTfdotinvplusdataplusaddrH}
\setlength{\WRCdotTTTfdotinvplusdataplusaddrH}{0cm}
\newsavebox{\WRCdotTTTfdotinvplusdataplusaddrI}
\begin{lrbox}{\WRCdotTTTfdotinvplusdataplusaddrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusdataplusaddrJ}
\settowidth{\WRCdotTTTfdotinvplusdataplusaddrJ}{\usebox{\WRCdotTTTfdotinvplusdataplusaddrI}}
\addtolength{\WRCdotTTTfdotinvplusdataplusaddrH}{\WRCdotTTTfdotinvplusdataplusaddrJ}
\newsavebox{\WRCdotTTTfdotinvplusdataplusaddrK}
\begin{lrbox}{\WRCdotTTTfdotinvplusdataplusaddrK}
\begin{lstlisting}[language=AArch64,showlines=true]
MOV X0,#0
LDR X0,[X1]
EOR X4,X0,X0
ORR X2,X2,X4
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusdataplusaddrL}
\settowidth{\WRCdotTTTfdotinvplusdataplusaddrL}{\usebox{\WRCdotTTTfdotinvplusdataplusaddrK}}
\addtolength{\WRCdotTTTfdotinvplusdataplusaddrH}{\WRCdotTTTfdotinvplusdataplusaddrL}
\newsavebox{\WRCdotTTTfdotinvplusdataplusaddrM}
\begin{lrbox}{\WRCdotTTTfdotinvplusdataplusaddrM}
\begin{lstlisting}[language=AArch64,showlines=true]
MOV X0,#0
LDR X0,[X1]
EOR X4,X0,X0
MOV X2,#0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusdataplusaddrN}
\settowidth{\WRCdotTTTfdotinvplusdataplusaddrN}{\usebox{\WRCdotTTTfdotinvplusdataplusaddrM}}
\addtolength{\WRCdotTTTfdotinvplusdataplusaddrH}{\WRCdotTTTfdotinvplusdataplusaddrN}
\newsavebox{\WRCdotTTTfdotinvplusdataplusaddrO}
\begin{lrbox}{\WRCdotTTTfdotinvplusdataplusaddrO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusdataplusaddrP}
\settowidth{\WRCdotTTTfdotinvplusdataplusaddrP}{\usebox{\WRCdotTTTfdotinvplusdataplusaddrO}}
\addtolength{\WRCdotTTTfdotinvplusdataplusaddrH}{\WRCdotTTTfdotinvplusdataplusaddrP}
\newsavebox{\WRCdotTTTfdotinvplusdataplusaddrA}
\begin{lrbox}{\WRCdotTTTfdotinvplusdataplusaddrA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusdataplusaddrB}
\settowidth{\WRCdotTTTfdotinvplusdataplusaddrB}{\usebox{\WRCdotTTTfdotinvplusdataplusaddrA}}
\addtolength{\WRCdotTTTfdotinvplusdataplusaddrH}{\WRCdotTTTfdotinvplusdataplusaddrB}
\newsavebox{\WRCdotTTTfdotinvplusdataplusaddrC}
\begin{lrbox}{\WRCdotTTTfdotinvplusdataplusaddrC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusdataplusaddrD}
\settowidth{\WRCdotTTTfdotinvplusdataplusaddrD}{\usebox{\WRCdotTTTfdotinvplusdataplusaddrC}}
\newsavebox{\WRCdotTTTfdotinvplusdataplusaddrE}
\begin{lrbox}{\WRCdotTTTfdotinvplusdataplusaddrE}
\begin{minipage}{\WRCdotTTTfdotinvplusdataplusaddrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:__isla_monomorphize_writes=true|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TTTf.inv+data+addr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTTTfdotinvplusdataplusaddrD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTTTfdotinvplusdataplusaddrC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTTTfdotinvplusdataplusaddrE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusdataplusaddrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusdataplusaddrK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusdataplusaddrM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusdataplusaddrO}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusdataplusaddrA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/WRC.TfRR+ctrl-isb+dsb.tex <==
\newlength{\WRCdotTfRRplusctrlisbplusdsbH}
\setlength{\WRCdotTfRRplusctrlisbplusdsbH}{0cm}
\newsavebox{\WRCdotTfRRplusctrlisbplusdsbI}
\begin{lrbox}{\WRCdotTfRRplusctrlisbplusdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusctrlisbplusdsbJ}
\settowidth{\WRCdotTfRRplusctrlisbplusdsbJ}{\usebox{\WRCdotTfRRplusctrlisbplusdsbI}}
\addtolength{\WRCdotTfRRplusctrlisbplusdsbH}{\WRCdotTfRRplusctrlisbplusdsbJ}
\newsavebox{\WRCdotTfRRplusctrlisbplusdsbK}
\begin{lrbox}{\WRCdotTfRRplusctrlisbplusdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBNZ X0,L0
L0:
ISB
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusctrlisbplusdsbL}
\settowidth{\WRCdotTfRRplusctrlisbplusdsbL}{\usebox{\WRCdotTfRRplusctrlisbplusdsbK}}
\addtolength{\WRCdotTfRRplusctrlisbplusdsbH}{\WRCdotTfRRplusctrlisbplusdsbL}
\newsavebox{\WRCdotTfRRplusctrlisbplusdsbM}
\begin{lrbox}{\WRCdotTfRRplusctrlisbplusdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusctrlisbplusdsbN}
\settowidth{\WRCdotTfRRplusctrlisbplusdsbN}{\usebox{\WRCdotTfRRplusctrlisbplusdsbM}}
\addtolength{\WRCdotTfRRplusctrlisbplusdsbH}{\WRCdotTfRRplusctrlisbplusdsbN}
\newsavebox{\WRCdotTfRRplusctrlisbplusdsbO}
\begin{lrbox}{\WRCdotTfRRplusctrlisbplusdsbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusctrlisbplusdsbP}
\settowidth{\WRCdotTfRRplusctrlisbplusdsbP}{\usebox{\WRCdotTfRRplusctrlisbplusdsbO}}
\addtolength{\WRCdotTfRRplusctrlisbplusdsbH}{\WRCdotTfRRplusctrlisbplusdsbP}
\newsavebox{\WRCdotTfRRplusctrlisbplusdsbA}
\begin{lrbox}{\WRCdotTfRRplusctrlisbplusdsbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    *pa1 = 0;

    y |-> pa2;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusctrlisbplusdsbB}
\settowidth{\WRCdotTfRRplusctrlisbplusdsbB}{\usebox{\WRCdotTfRRplusctrlisbplusdsbA}}
\newsavebox{\WRCdotTfRRplusctrlisbplusdsbC}
\begin{lrbox}{\WRCdotTfRRplusctrlisbplusdsbC}
\begin{minipage}{\WRCdotTfRRplusctrlisbplusdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TfRR+ctrl-isb+dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTfRRplusctrlisbplusdsbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTfRRplusctrlisbplusdsbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTfRRplusctrlisbplusdsbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusctrlisbplusdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusctrlisbplusdsbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusctrlisbplusdsbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusctrlisbplusdsbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & ~2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/WRC.TfRR+dmbs.tex <==
\newlength{\WRCdotTfRRplusdmbsH}
\setlength{\WRCdotTfRRplusdmbsH}{0cm}
\newsavebox{\WRCdotTfRRplusdmbsI}
\begin{lrbox}{\WRCdotTfRRplusdmbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdmbsJ}
\settowidth{\WRCdotTfRRplusdmbsJ}{\usebox{\WRCdotTfRRplusdmbsI}}
\addtolength{\WRCdotTfRRplusdmbsH}{\WRCdotTfRRplusdmbsJ}
\newsavebox{\WRCdotTfRRplusdmbsK}
\begin{lrbox}{\WRCdotTfRRplusdmbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdmbsL}
\settowidth{\WRCdotTfRRplusdmbsL}{\usebox{\WRCdotTfRRplusdmbsK}}
\addtolength{\WRCdotTfRRplusdmbsH}{\WRCdotTfRRplusdmbsL}
\newsavebox{\WRCdotTfRRplusdmbsM}
\begin{lrbox}{\WRCdotTfRRplusdmbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdmbsN}
\settowidth{\WRCdotTfRRplusdmbsN}{\usebox{\WRCdotTfRRplusdmbsM}}
\addtolength{\WRCdotTfRRplusdmbsH}{\WRCdotTfRRplusdmbsN}
\newsavebox{\WRCdotTfRRplusdmbsO}
\begin{lrbox}{\WRCdotTfRRplusdmbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdmbsP}
\settowidth{\WRCdotTfRRplusdmbsP}{\usebox{\WRCdotTfRRplusdmbsO}}
\addtolength{\WRCdotTfRRplusdmbsH}{\WRCdotTfRRplusdmbsP}
\newsavebox{\WRCdotTfRRplusdmbsA}
\begin{lrbox}{\WRCdotTfRRplusdmbsA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    *pa1 = 0;

    y |-> pa2;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdmbsB}
\settowidth{\WRCdotTfRRplusdmbsB}{\usebox{\WRCdotTfRRplusdmbsA}}
\newsavebox{\WRCdotTfRRplusdmbsC}
\begin{lrbox}{\WRCdotTfRRplusdmbsC}
\begin{minipage}{\WRCdotTfRRplusdmbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TfRR+dmbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTfRRplusdmbsB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTfRRplusdmbsA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTfRRplusdmbsC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdmbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdmbsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdmbsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdmbsO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & ~2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/WRC.TfRR+dsb-isb+dsb.tex <==
\newlength{\WRCdotTfRRplusdsbisbplusdsbH}
\setlength{\WRCdotTfRRplusdsbisbplusdsbH}{0cm}
\newsavebox{\WRCdotTfRRplusdsbisbplusdsbI}
\begin{lrbox}{\WRCdotTfRRplusdsbisbplusdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbisbplusdsbJ}
\settowidth{\WRCdotTfRRplusdsbisbplusdsbJ}{\usebox{\WRCdotTfRRplusdsbisbplusdsbI}}
\addtolength{\WRCdotTfRRplusdsbisbplusdsbH}{\WRCdotTfRRplusdsbisbplusdsbJ}
\newsavebox{\WRCdotTfRRplusdsbisbplusdsbK}
\begin{lrbox}{\WRCdotTfRRplusdsbisbplusdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbisbplusdsbL}
\settowidth{\WRCdotTfRRplusdsbisbplusdsbL}{\usebox{\WRCdotTfRRplusdsbisbplusdsbK}}
\addtolength{\WRCdotTfRRplusdsbisbplusdsbH}{\WRCdotTfRRplusdsbisbplusdsbL}
\newsavebox{\WRCdotTfRRplusdsbisbplusdsbM}
\begin{lrbox}{\WRCdotTfRRplusdsbisbplusdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbisbplusdsbN}
\settowidth{\WRCdotTfRRplusdsbisbplusdsbN}{\usebox{\WRCdotTfRRplusdsbisbplusdsbM}}
\addtolength{\WRCdotTfRRplusdsbisbplusdsbH}{\WRCdotTfRRplusdsbisbplusdsbN}
\newsavebox{\WRCdotTfRRplusdsbisbplusdsbO}
\begin{lrbox}{\WRCdotTfRRplusdsbisbplusdsbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbisbplusdsbP}
\settowidth{\WRCdotTfRRplusdsbisbplusdsbP}{\usebox{\WRCdotTfRRplusdsbisbplusdsbO}}
\addtolength{\WRCdotTfRRplusdsbisbplusdsbH}{\WRCdotTfRRplusdsbisbplusdsbP}
\newsavebox{\WRCdotTfRRplusdsbisbplusdsbA}
\begin{lrbox}{\WRCdotTfRRplusdsbisbplusdsbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    *pa1 = 0;

    y |-> pa2;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbisbplusdsbB}
\settowidth{\WRCdotTfRRplusdsbisbplusdsbB}{\usebox{\WRCdotTfRRplusdsbisbplusdsbA}}
\newsavebox{\WRCdotTfRRplusdsbisbplusdsbC}
\begin{lrbox}{\WRCdotTfRRplusdsbisbplusdsbC}
\begin{minipage}{\WRCdotTfRRplusdsbisbplusdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TfRR+dsb-isb+dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTfRRplusdsbisbplusdsbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTfRRplusdsbisbplusdsbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTfRRplusdsbisbplusdsbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdsbisbplusdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdsbisbplusdsbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdsbisbplusdsbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdsbisbplusdsbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & ~2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/WRC.TfRR+dsbs.tex <==
\newlength{\WRCdotTfRRplusdsbsH}
\setlength{\WRCdotTfRRplusdsbsH}{0cm}
\newsavebox{\WRCdotTfRRplusdsbsI}
\begin{lrbox}{\WRCdotTfRRplusdsbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbsJ}
\settowidth{\WRCdotTfRRplusdsbsJ}{\usebox{\WRCdotTfRRplusdsbsI}}
\addtolength{\WRCdotTfRRplusdsbsH}{\WRCdotTfRRplusdsbsJ}
\newsavebox{\WRCdotTfRRplusdsbsK}
\begin{lrbox}{\WRCdotTfRRplusdsbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbsL}
\settowidth{\WRCdotTfRRplusdsbsL}{\usebox{\WRCdotTfRRplusdsbsK}}
\addtolength{\WRCdotTfRRplusdsbsH}{\WRCdotTfRRplusdsbsL}
\newsavebox{\WRCdotTfRRplusdsbsM}
\begin{lrbox}{\WRCdotTfRRplusdsbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbsN}
\settowidth{\WRCdotTfRRplusdsbsN}{\usebox{\WRCdotTfRRplusdsbsM}}
\addtolength{\WRCdotTfRRplusdsbsH}{\WRCdotTfRRplusdsbsN}
\newsavebox{\WRCdotTfRRplusdsbsO}
\begin{lrbox}{\WRCdotTfRRplusdsbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbsP}
\settowidth{\WRCdotTfRRplusdsbsP}{\usebox{\WRCdotTfRRplusdsbsO}}
\addtolength{\WRCdotTfRRplusdsbsH}{\WRCdotTfRRplusdsbsP}
\newsavebox{\WRCdotTfRRplusdsbsA}
\begin{lrbox}{\WRCdotTfRRplusdsbsA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    *pa1 = 0;

    y |-> pa2;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbsB}
\settowidth{\WRCdotTfRRplusdsbsB}{\usebox{\WRCdotTfRRplusdsbsA}}
\newsavebox{\WRCdotTfRRplusdsbsC}
\begin{lrbox}{\WRCdotTfRRplusdsbsC}
\begin{minipage}{\WRCdotTfRRplusdsbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TfRR+dsbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTfRRplusdsbsB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTfRRplusdsbsA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTfRRplusdsbsC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdsbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdsbsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdsbsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdsbsO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & ~2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/WRC.TfRR+po+dsb.tex <==
\newlength{\WRCdotTfRRpluspoplusdsbH}
\setlength{\WRCdotTfRRpluspoplusdsbH}{0cm}
\newsavebox{\WRCdotTfRRpluspoplusdsbI}
\begin{lrbox}{\WRCdotTfRRpluspoplusdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRpluspoplusdsbJ}
\settowidth{\WRCdotTfRRpluspoplusdsbJ}{\usebox{\WRCdotTfRRpluspoplusdsbI}}
\addtolength{\WRCdotTfRRpluspoplusdsbH}{\WRCdotTfRRpluspoplusdsbJ}
\newsavebox{\WRCdotTfRRpluspoplusdsbK}
\begin{lrbox}{\WRCdotTfRRpluspoplusdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRpluspoplusdsbL}
\settowidth{\WRCdotTfRRpluspoplusdsbL}{\usebox{\WRCdotTfRRpluspoplusdsbK}}
\addtolength{\WRCdotTfRRpluspoplusdsbH}{\WRCdotTfRRpluspoplusdsbL}
\newsavebox{\WRCdotTfRRpluspoplusdsbM}
\begin{lrbox}{\WRCdotTfRRpluspoplusdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRpluspoplusdsbN}
\settowidth{\WRCdotTfRRpluspoplusdsbN}{\usebox{\WRCdotTfRRpluspoplusdsbM}}
\addtolength{\WRCdotTfRRpluspoplusdsbH}{\WRCdotTfRRpluspoplusdsbN}
\newsavebox{\WRCdotTfRRpluspoplusdsbO}
\begin{lrbox}{\WRCdotTfRRpluspoplusdsbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRpluspoplusdsbP}
\settowidth{\WRCdotTfRRpluspoplusdsbP}{\usebox{\WRCdotTfRRpluspoplusdsbO}}
\addtolength{\WRCdotTfRRpluspoplusdsbH}{\WRCdotTfRRpluspoplusdsbP}
\newsavebox{\WRCdotTfRRpluspoplusdsbA}
\begin{lrbox}{\WRCdotTfRRpluspoplusdsbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    *pa1 = 0;

    y |-> pa2;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRpluspoplusdsbB}
\settowidth{\WRCdotTfRRpluspoplusdsbB}{\usebox{\WRCdotTfRRpluspoplusdsbA}}
\newsavebox{\WRCdotTfRRpluspoplusdsbC}
\begin{lrbox}{\WRCdotTfRRpluspoplusdsbC}
\begin{minipage}{\WRCdotTfRRpluspoplusdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TfRR+po+dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTfRRpluspoplusdsbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTfRRpluspoplusdsbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTfRRpluspoplusdsbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRpluspoplusdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRpluspoplusdsbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRpluspoplusdsbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRpluspoplusdsbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & ~2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/WRC.TfRR+pos.tex <==
\newlength{\WRCdotTfRRplusposH}
\setlength{\WRCdotTfRRplusposH}{0cm}
\newsavebox{\WRCdotTfRRplusposI}
\begin{lrbox}{\WRCdotTfRRplusposI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusposJ}
\settowidth{\WRCdotTfRRplusposJ}{\usebox{\WRCdotTfRRplusposI}}
\addtolength{\WRCdotTfRRplusposH}{\WRCdotTfRRplusposJ}
\newsavebox{\WRCdotTfRRplusposK}
\begin{lrbox}{\WRCdotTfRRplusposK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusposL}
\settowidth{\WRCdotTfRRplusposL}{\usebox{\WRCdotTfRRplusposK}}
\addtolength{\WRCdotTfRRplusposH}{\WRCdotTfRRplusposL}
\newsavebox{\WRCdotTfRRplusposM}
\begin{lrbox}{\WRCdotTfRRplusposM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusposN}
\settowidth{\WRCdotTfRRplusposN}{\usebox{\WRCdotTfRRplusposM}}
\addtolength{\WRCdotTfRRplusposH}{\WRCdotTfRRplusposN}
\newsavebox{\WRCdotTfRRplusposO}
\begin{lrbox}{\WRCdotTfRRplusposO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusposP}
\settowidth{\WRCdotTfRRplusposP}{\usebox{\WRCdotTfRRplusposO}}
\addtolength{\WRCdotTfRRplusposH}{\WRCdotTfRRplusposP}
\newsavebox{\WRCdotTfRRplusposA}
\begin{lrbox}{\WRCdotTfRRplusposA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    *pa1 = 0;

    y |-> pa2;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusposB}
\settowidth{\WRCdotTfRRplusposB}{\usebox{\WRCdotTfRRplusposA}}
\newsavebox{\WRCdotTfRRplusposC}
\begin{lrbox}{\WRCdotTfRRplusposC}
\begin{minipage}{\WRCdotTfRRplusposH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TfRR+pos|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTfRRplusposB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTfRRplusposA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTfRRplusposC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusposI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusposK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusposM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusposO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & ~2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/WRC.TfRT+dsb-tlbiis-dsb+dsb-isb.tex <==
\newlength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbH}
\setlength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbH}{0cm}
\newsavebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbI}
\begin{lrbox}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbJ}
\settowidth{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbJ}{\usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbI}}
\addtolength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbH}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbJ}
\newsavebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbK}
\begin{lrbox}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
// the TLBI is in the handler
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbL}
\settowidth{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbL}{\usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbK}}
\addtolength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbH}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbL}
\newsavebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbM}
\begin{lrbox}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbN}
\settowidth{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbN}{\usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbM}}
\addtolength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbH}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbN}
\newsavebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbO}
\begin{lrbox}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
DSB SY
TLBI VAE1IS,X4
DSB SY
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbP}
\settowidth{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbP}{\usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbO}}
\addtolength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbH}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbP}
\newsavebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbA}
\begin{lrbox}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbB}
\settowidth{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbB}{\usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbA}}
\addtolength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbH}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbB}
\newsavebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbC}
\begin{lrbox}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;

    x |-> pa1;
    x ?-> invalid;
    *pa1 = 1;

    y |-> pa2;
    *pa2 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbD}
\settowidth{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbD}{\usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbC}}
\newsavebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbE}
\begin{lrbox}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbE}
\begin{minipage}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TfRT+dsb-tlbiis-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbO}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=0 & 2:R0=1 & 2:R2=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-24/latex/WRC.TfRT+po+dsb-isb.tex <==
\newlength{\WRCdotTfRTpluspoplusdsbisbH}
\setlength{\WRCdotTfRTpluspoplusdsbisbH}{0cm}
\newsavebox{\WRCdotTfRTpluspoplusdsbisbI}
\begin{lrbox}{\WRCdotTfRTpluspoplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTpluspoplusdsbisbJ}
\settowidth{\WRCdotTfRTpluspoplusdsbisbJ}{\usebox{\WRCdotTfRTpluspoplusdsbisbI}}
\addtolength{\WRCdotTfRTpluspoplusdsbisbH}{\WRCdotTfRTpluspoplusdsbisbJ}
\newsavebox{\WRCdotTfRTpluspoplusdsbisbK}
\begin{lrbox}{\WRCdotTfRTpluspoplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTpluspoplusdsbisbL}
\settowidth{\WRCdotTfRTpluspoplusdsbisbL}{\usebox{\WRCdotTfRTpluspoplusdsbisbK}}
\addtolength{\WRCdotTfRTpluspoplusdsbisbH}{\WRCdotTfRTpluspoplusdsbisbL}
\newsavebox{\WRCdotTfRTpluspoplusdsbisbM}
\begin{lrbox}{\WRCdotTfRTpluspoplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTpluspoplusdsbisbN}
\settowidth{\WRCdotTfRTpluspoplusdsbisbN}{\usebox{\WRCdotTfRTpluspoplusdsbisbM}}
\addtolength{\WRCdotTfRTpluspoplusdsbisbH}{\WRCdotTfRTpluspoplusdsbisbN}
\newsavebox{\WRCdotTfRTpluspoplusdsbisbO}
\begin{lrbox}{\WRCdotTfRTpluspoplusdsbisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTpluspoplusdsbisbP}
\settowidth{\WRCdotTfRTpluspoplusdsbisbP}{\usebox{\WRCdotTfRTpluspoplusdsbisbO}}
\addtolength{\WRCdotTfRTpluspoplusdsbisbH}{\WRCdotTfRTpluspoplusdsbisbP}
\newsavebox{\WRCdotTfRTpluspoplusdsbisbA}
\begin{lrbox}{\WRCdotTfRTpluspoplusdsbisbA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTpluspoplusdsbisbB}
\settowidth{\WRCdotTfRTpluspoplusdsbisbB}{\usebox{\WRCdotTfRTpluspoplusdsbisbA}}
\addtolength{\WRCdotTfRTpluspoplusdsbisbH}{\WRCdotTfRTpluspoplusdsbisbB}
\newsavebox{\WRCdotTfRTpluspoplusdsbisbC}
\begin{lrbox}{\WRCdotTfRTpluspoplusdsbisbC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;

    x |-> pa1;
    x ?-> invalid;
    *pa1 = 1;

    y |-> pa2;
    *pa2 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTpluspoplusdsbisbD}
\settowidth{\WRCdotTfRTpluspoplusdsbisbD}{\usebox{\WRCdotTfRTpluspoplusdsbisbC}}
\newsavebox{\WRCdotTfRTpluspoplusdsbisbE}
\begin{lrbox}{\WRCdotTfRTpluspoplusdsbisbE}
\begin{minipage}{\WRCdotTfRTpluspoplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TfRT+po+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTfRTpluspoplusdsbisbD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTfRTpluspoplusdsbisbC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTfRTpluspoplusdsbisbE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTpluspoplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTpluspoplusdsbisbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTpluspoplusdsbisbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTpluspoplusdsbisbO}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTpluspoplusdsbisbA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=0 & 2:R0=1 & 2:R2=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/BBM+dsb-tlbiis-dsb.tex <==
\newlength{\BBMplusdsbtlbiisdsbH}
\setlength{\BBMplusdsbtlbiisdsbH}{0cm}
\newsavebox{\BBMplusdsbtlbiisdsbI}
\begin{lrbox}{\BBMplusdsbtlbiisdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X6
DSB SY
STR X2,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\BBMplusdsbtlbiisdsbJ}
\settowidth{\BBMplusdsbtlbiisdsbJ}{\usebox{\BBMplusdsbtlbiisdsbI}}
\addtolength{\BBMplusdsbtlbiisdsbH}{\BBMplusdsbtlbiisdsbJ}
\newsavebox{\BBMplusdsbtlbiisdsbK}
\begin{lrbox}{\BBMplusdsbtlbiisdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\BBMplusdsbtlbiisdsbL}
\settowidth{\BBMplusdsbtlbiisdsbL}{\usebox{\BBMplusdsbtlbiisdsbK}}
\addtolength{\BBMplusdsbtlbiisdsbH}{\BBMplusdsbtlbiisdsbL}
\newsavebox{\BBMplusdsbtlbiisdsbM}
\begin{lrbox}{\BBMplusdsbtlbiisdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\BBMplusdsbtlbiisdsbN}
\settowidth{\BBMplusdsbtlbiisdsbN}{\usebox{\BBMplusdsbtlbiisdsbM}}
\addtolength{\BBMplusdsbtlbiisdsbH}{\BBMplusdsbtlbiisdsbN}
\newsavebox{\BBMplusdsbtlbiisdsbO}
\begin{lrbox}{\BBMplusdsbtlbiisdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;
    x ?-> pa2;

    identity 0x1000 with code;

    *pa2 = 2;
\end{lstlisting}
\end{lrbox}
\newlength{\BBMplusdsbtlbiisdsbP}
\settowidth{\BBMplusdsbtlbiisdsbP}{\usebox{\BBMplusdsbtlbiisdsbO}}
\newsavebox{\BBMplusdsbtlbiisdsbA}
\begin{lrbox}{\BBMplusdsbtlbiisdsbA}
\begin{minipage}{\BBMplusdsbtlbiisdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R4=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|BBM+dsb-tlbiis-dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\BBMplusdsbtlbiisdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\BBMplusdsbtlbiisdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\BBMplusdsbtlbiisdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\BBMplusdsbtlbiisdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\BBMplusdsbtlbiisdsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\BBMplusdsbtlbiisdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/BBM.Tf+dsb-tlbiis-dsb.tex <==
\newlength{\BBMdotTfplusdsbtlbiisdsbH}
\setlength{\BBMdotTfplusdsbtlbiisdsbH}{0cm}
\newsavebox{\BBMdotTfplusdsbtlbiisdsbI}
\begin{lrbox}{\BBMdotTfplusdsbtlbiisdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X6
DSB SY
STR X2,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\BBMdotTfplusdsbtlbiisdsbJ}
\settowidth{\BBMdotTfplusdsbtlbiisdsbJ}{\usebox{\BBMdotTfplusdsbtlbiisdsbI}}
\addtolength{\BBMdotTfplusdsbtlbiisdsbH}{\BBMdotTfplusdsbtlbiisdsbJ}
\newsavebox{\BBMdotTfplusdsbtlbiisdsbK}
\begin{lrbox}{\BBMdotTfplusdsbtlbiisdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\BBMdotTfplusdsbtlbiisdsbL}
\settowidth{\BBMdotTfplusdsbtlbiisdsbL}{\usebox{\BBMdotTfplusdsbtlbiisdsbK}}
\addtolength{\BBMdotTfplusdsbtlbiisdsbH}{\BBMdotTfplusdsbtlbiisdsbL}
\newsavebox{\BBMdotTfplusdsbtlbiisdsbM}
\begin{lrbox}{\BBMdotTfplusdsbtlbiisdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
\end{lstlisting}
\end{lrbox}
\newlength{\BBMdotTfplusdsbtlbiisdsbN}
\settowidth{\BBMdotTfplusdsbtlbiisdsbN}{\usebox{\BBMdotTfplusdsbtlbiisdsbM}}
\addtolength{\BBMdotTfplusdsbtlbiisdsbH}{\BBMdotTfplusdsbtlbiisdsbN}
\newsavebox{\BBMdotTfplusdsbtlbiisdsbO}
\begin{lrbox}{\BBMdotTfplusdsbtlbiisdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;
    x ?-> pa2;

    identity 0x1000 with code;

    *pa2 = 2;
\end{lstlisting}
\end{lrbox}
\newlength{\BBMdotTfplusdsbtlbiisdsbP}
\settowidth{\BBMdotTfplusdsbtlbiisdsbP}{\usebox{\BBMdotTfplusdsbtlbiisdsbO}}
\newsavebox{\BBMdotTfplusdsbtlbiisdsbA}
\begin{lrbox}{\BBMdotTfplusdsbtlbiisdsbA}
\begin{minipage}{\BBMdotTfplusdsbtlbiisdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R4=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|BBM.Tf+dsb-tlbiis-dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\BBMdotTfplusdsbtlbiisdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\BBMdotTfplusdsbtlbiisdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\BBMdotTfplusdsbtlbiisdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\BBMdotTfplusdsbtlbiisdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\BBMdotTfplusdsbtlbiisdsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\BBMdotTfplusdsbtlbiisdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/Break2.news1.tex <==
\newlength{\BreaktwodotnewsoneH}
\setlength{\BreaktwodotnewsoneH}{0cm}
\newsavebox{\BreaktwodotnewsoneI}
\begin{lrbox}{\BreaktwodotnewsoneI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1IS,X4
DSB SY
TLBI VMALLE1IS
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\BreaktwodotnewsoneJ}
\settowidth{\BreaktwodotnewsoneJ}{\usebox{\BreaktwodotnewsoneI}}
\addtolength{\BreaktwodotnewsoneH}{\BreaktwodotnewsoneJ}
\newsavebox{\BreaktwodotnewsoneK}
\begin{lrbox}{\BreaktwodotnewsoneK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\BreaktwodotnewsoneL}
\settowidth{\BreaktwodotnewsoneL}{\usebox{\BreaktwodotnewsoneK}}
\addtolength{\BreaktwodotnewsoneH}{\BreaktwodotnewsoneL}
\newsavebox{\BreaktwodotnewsoneM}
\begin{lrbox}{\BreaktwodotnewsoneM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#2
\end{lstlisting}
\end{lrbox}
\newlength{\BreaktwodotnewsoneN}
\settowidth{\BreaktwodotnewsoneN}{\usebox{\BreaktwodotnewsoneM}}
\addtolength{\BreaktwodotnewsoneH}{\BreaktwodotnewsoneN}
\newsavebox{\BreaktwodotnewsoneO}
\begin{lrbox}{\BreaktwodotnewsoneO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X0,#3
\end{lstlisting}
\end{lrbox}
\newlength{\BreaktwodotnewsoneP}
\settowidth{\BreaktwodotnewsoneP}{\usebox{\BreaktwodotnewsoneO}}
\addtolength{\BreaktwodotnewsoneH}{\BreaktwodotnewsoneP}
\newsavebox{\BreaktwodotnewsoneA}
\begin{lrbox}{\BreaktwodotnewsoneA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
option default_tables = false;
physical pa1;
intermediate ipa1;

s2table vm_stage2 0x240000  {
    ipa1 |-> pa1 at level 3;
    ipa1 ?-> invalid at level 3;
    identity pa_to_ipa(0x1000) with code;


    s1table vm_stage1 0x280000  {
        x |-> invalid at level 3;
        x ?-> ipa1 at level 3;

        identity pa_to_va(0x1000) with code;
    }
}

s1table hyp_map 0x200000 {
    identity 0x2000 with code;
    s2table vm_stage2;
    s1table vm_stage1;
}

*pa1 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\BreaktwodotnewsoneB}
\settowidth{\BreaktwodotnewsoneB}{\usebox{\BreaktwodotnewsoneA}}
\newsavebox{\BreaktwodotnewsoneC}
\begin{lrbox}{\BreaktwodotnewsoneC}
\begin{minipage}{\BreaktwodotnewsoneH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(ipa1,vm_stage2)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=ipa1)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(x,vm_stage1)|\\
\lstinline[language=IslaLitmusExp]|0:R4=bvlshr(ipa1,0xC)|\\
\lstinline[language=IslaLitmusExp]|0:TTBR0_EL2=ttbr(asid=0x0000,base=hyp_map)|\\
\lstinline[language=IslaLitmusExp]|0:VTTBR_EL2=ttbr(base=vm_stage2,vmid=0x0000)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:TTBR0_EL1=ttbr(base=vm_stage1,asid=0x0000)|\\
\lstinline[language=IslaLitmusExp]|1:TTBR0_EL2=ttbr(base=hyp_map,asid=0x0000)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\lstinline[language=IslaLitmusExp]|1:VTTBR_EL2=ttbr(vmid=0x0000,base=vm_stage2)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|Break2.news1|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\BreaktwodotnewsoneB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\BreaktwodotnewsoneA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\BreaktwodotnewsoneC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\BreaktwodotnewsoneI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\BreaktwodotnewsoneK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\BreaktwodotnewsoneM}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\BreaktwodotnewsoneO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoRR0.alias+po.tex <==
\newlength{\CoRRzerodotaliaspluspoH}
\setlength{\CoRRzerodotaliaspluspoH}{0cm}
\newsavebox{\CoRRzerodotaliaspluspoI}
\begin{lrbox}{\CoRRzerodotaliaspluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRRzerodotaliaspluspoJ}
\settowidth{\CoRRzerodotaliaspluspoJ}{\usebox{\CoRRzerodotaliaspluspoI}}
\addtolength{\CoRRzerodotaliaspluspoH}{\CoRRzerodotaliaspluspoJ}
\newsavebox{\CoRRzerodotaliaspluspoK}
\begin{lrbox}{\CoRRzerodotaliaspluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRRzerodotaliaspluspoL}
\settowidth{\CoRRzerodotaliaspluspoL}{\usebox{\CoRRzerodotaliaspluspoK}}
\addtolength{\CoRRzerodotaliaspluspoH}{\CoRRzerodotaliaspluspoL}
\newsavebox{\CoRRzerodotaliaspluspoM}
\begin{lrbox}{\CoRRzerodotaliaspluspoM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    y |-> pa1;
    *pa1 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRRzerodotaliaspluspoN}
\settowidth{\CoRRzerodotaliaspluspoN}{\usebox{\CoRRzerodotaliaspluspoM}}
\newsavebox{\CoRRzerodotaliaspluspoO}
\begin{lrbox}{\CoRRzerodotaliaspluspoO}
\begin{minipage}{\CoRRzerodotaliaspluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRR0.alias+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRRzerodotaliaspluspoN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRRzerodotaliaspluspoM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRRzerodotaliaspluspoO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRRzerodotaliaspluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRRzerodotaliaspluspoK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoRR2.alias+po.tex <==
\newlength{\CoRRtwodotaliaspluspoH}
\setlength{\CoRRtwodotaliaspluspoH}{0cm}
\newsavebox{\CoRRtwodotaliaspluspoI}
\begin{lrbox}{\CoRRtwodotaliaspluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRRtwodotaliaspluspoJ}
\settowidth{\CoRRtwodotaliaspluspoJ}{\usebox{\CoRRtwodotaliaspluspoI}}
\addtolength{\CoRRtwodotaliaspluspoH}{\CoRRtwodotaliaspluspoJ}
\newsavebox{\CoRRtwodotaliaspluspoK}
\begin{lrbox}{\CoRRtwodotaliaspluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRRtwodotaliaspluspoL}
\settowidth{\CoRRtwodotaliaspluspoL}{\usebox{\CoRRtwodotaliaspluspoK}}
\addtolength{\CoRRtwodotaliaspluspoH}{\CoRRtwodotaliaspluspoL}
\newsavebox{\CoRRtwodotaliaspluspoM}
\begin{lrbox}{\CoRRtwodotaliaspluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRRtwodotaliaspluspoN}
\settowidth{\CoRRtwodotaliaspluspoN}{\usebox{\CoRRtwodotaliaspluspoM}}
\addtolength{\CoRRtwodotaliaspluspoH}{\CoRRtwodotaliaspluspoN}
\newsavebox{\CoRRtwodotaliaspluspoO}
\begin{lrbox}{\CoRRtwodotaliaspluspoO}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRRtwodotaliaspluspoP}
\settowidth{\CoRRtwodotaliaspluspoP}{\usebox{\CoRRtwodotaliaspluspoO}}
\addtolength{\CoRRtwodotaliaspluspoH}{\CoRRtwodotaliaspluspoP}
\newsavebox{\CoRRtwodotaliaspluspoA}
\begin{lrbox}{\CoRRtwodotaliaspluspoA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    u |-> pa1;
    v |-> pa1;
    w |-> pa1;
    x |-> pa1;
    y |-> pa1;
    z |-> pa1;
    *pa1 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRRtwodotaliaspluspoB}
\settowidth{\CoRRtwodotaliaspluspoB}{\usebox{\CoRRtwodotaliaspluspoA}}
\newsavebox{\CoRRtwodotaliaspluspoC}
\begin{lrbox}{\CoRRtwodotaliaspluspoC}
\begin{minipage}{\CoRRtwodotaliaspluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R1=u|\\
\lstinline[language=IslaLitmusExp]|1:R0=0b10|\\
\lstinline[language=IslaLitmusExp]|1:R1=v|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=w|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|3:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|3:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|3:R1=y|\\
\lstinline[language=IslaLitmusExp]|3:R3=z|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRR2.alias+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRRtwodotaliaspluspoB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRRtwodotaliaspluspoA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRRtwodotaliaspluspoC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRRtwodotaliaspluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRRtwodotaliaspluspoK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\CoRRtwodotaliaspluspoM}\\
  \cline{2-2}
  & Thread 3\\
  \cline{2-2}
  & \usebox{\CoRRtwodotaliaspluspoO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|2:R0=1 & 2:R2=2 & 3:R0=2 & 3:R2=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoRT.inv+addr-trfi.tex <==
\newlength{\CoRTdotinvplusaddrtrfiH}
\setlength{\CoRTdotinvplusaddrtrfiH}{0cm}
\newsavebox{\CoRTdotinvplusaddrtrfiI}
\begin{lrbox}{\CoRTdotinvplusaddrtrfiI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRTdotinvplusaddrtrfiJ}
\settowidth{\CoRTdotinvplusaddrtrfiJ}{\usebox{\CoRTdotinvplusaddrtrfiI}}
\addtolength{\CoRTdotinvplusaddrtrfiH}{\CoRTdotinvplusaddrtrfiJ}
\newsavebox{\CoRTdotinvplusaddrtrfiK}
\begin{lrbox}{\CoRTdotinvplusaddrtrfiK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
STR X3,[X4,X2]
LDR X5,[X6]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRTdotinvplusaddrtrfiL}
\settowidth{\CoRTdotinvplusaddrtrfiL}{\usebox{\CoRTdotinvplusaddrtrfiK}}
\addtolength{\CoRTdotinvplusaddrtrfiH}{\CoRTdotinvplusaddrtrfiL}
\newsavebox{\CoRTdotinvplusaddrtrfiM}
\begin{lrbox}{\CoRTdotinvplusaddrtrfiM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X5,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoRTdotinvplusaddrtrfiN}
\settowidth{\CoRTdotinvplusaddrtrfiN}{\usebox{\CoRTdotinvplusaddrtrfiM}}
\addtolength{\CoRTdotinvplusaddrtrfiH}{\CoRTdotinvplusaddrtrfiN}
\newsavebox{\CoRTdotinvplusaddrtrfiO}
\begin{lrbox}{\CoRTdotinvplusaddrtrfiO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    y |-> invalid;
    y ?-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRTdotinvplusaddrtrfiP}
\settowidth{\CoRTdotinvplusaddrtrfiP}{\usebox{\CoRTdotinvplusaddrtrfiO}}
\newsavebox{\CoRTdotinvplusaddrtrfiA}
\begin{lrbox}{\CoRTdotinvplusaddrtrfiA}
\begin{minipage}{\CoRTdotinvplusaddrtrfiH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|1:R4=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R6=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRT.inv+addr-trfi|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRTdotinvplusaddrtrfiP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRTdotinvplusaddrtrfiO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRTdotinvplusaddrtrfiA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRTdotinvplusaddrtrfiI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRTdotinvplusaddrtrfiK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoRTdotinvplusaddrtrfiM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|true|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoRpteT+dsb-isb.tex <==
\newlength{\CoRpteTplusdsbisbH}
\setlength{\CoRpteTplusdsbisbH}{0cm}
\newsavebox{\CoRpteTplusdsbisbI}
\begin{lrbox}{\CoRpteTplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTplusdsbisbJ}
\settowidth{\CoRpteTplusdsbisbJ}{\usebox{\CoRpteTplusdsbisbI}}
\addtolength{\CoRpteTplusdsbisbH}{\CoRpteTplusdsbisbJ}
\newsavebox{\CoRpteTplusdsbisbK}
\begin{lrbox}{\CoRpteTplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTplusdsbisbL}
\settowidth{\CoRpteTplusdsbisbL}{\usebox{\CoRpteTplusdsbisbK}}
\addtolength{\CoRpteTplusdsbisbH}{\CoRpteTplusdsbisbL}
\newsavebox{\CoRpteTplusdsbisbM}
\begin{lrbox}{\CoRpteTplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTplusdsbisbN}
\settowidth{\CoRpteTplusdsbisbN}{\usebox{\CoRpteTplusdsbisbM}}
\addtolength{\CoRpteTplusdsbisbH}{\CoRpteTplusdsbisbN}
\newsavebox{\CoRpteTplusdsbisbO}
\begin{lrbox}{\CoRpteTplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;

    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;

    *pa1 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTplusdsbisbP}
\settowidth{\CoRpteTplusdsbisbP}{\usebox{\CoRpteTplusdsbisbO}}
\newsavebox{\CoRpteTplusdsbisbA}
\begin{lrbox}{\CoRpteTplusdsbisbA}
\begin{minipage}{\CoRpteTplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRpteT+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRpteTplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRpteTplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRpteTplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRpteTplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRpteTplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoRpteTplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=0 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoRpteT+dsb.tex <==
\newlength{\CoRpteTplusdsbH}
\setlength{\CoRpteTplusdsbH}{0cm}
\newsavebox{\CoRpteTplusdsbI}
\begin{lrbox}{\CoRpteTplusdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTplusdsbJ}
\settowidth{\CoRpteTplusdsbJ}{\usebox{\CoRpteTplusdsbI}}
\addtolength{\CoRpteTplusdsbH}{\CoRpteTplusdsbJ}
\newsavebox{\CoRpteTplusdsbK}
\begin{lrbox}{\CoRpteTplusdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTplusdsbL}
\settowidth{\CoRpteTplusdsbL}{\usebox{\CoRpteTplusdsbK}}
\addtolength{\CoRpteTplusdsbH}{\CoRpteTplusdsbL}
\newsavebox{\CoRpteTplusdsbM}
\begin{lrbox}{\CoRpteTplusdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTplusdsbN}
\settowidth{\CoRpteTplusdsbN}{\usebox{\CoRpteTplusdsbM}}
\addtolength{\CoRpteTplusdsbH}{\CoRpteTplusdsbN}
\newsavebox{\CoRpteTplusdsbO}
\begin{lrbox}{\CoRpteTplusdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;

    *x = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTplusdsbP}
\settowidth{\CoRpteTplusdsbP}{\usebox{\CoRpteTplusdsbO}}
\newsavebox{\CoRpteTplusdsbA}
\begin{lrbox}{\CoRpteTplusdsbA}
\begin{minipage}{\CoRpteTplusdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRpteT+dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRpteTplusdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRpteTplusdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRpteTplusdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRpteTplusdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRpteTplusdsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoRpteTplusdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=0 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoRpteT.EL1+dsb-tlbi-dsb-isb.tex <==
\newlength{\CoRpteTdotELoneplusdsbtlbidsbisbH}
\setlength{\CoRpteTdotELoneplusdsbtlbidsbisbH}{0cm}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbisbI}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTdotELoneplusdsbtlbidsbisbJ}
\settowidth{\CoRpteTdotELoneplusdsbtlbidsbisbJ}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbisbI}}
\addtolength{\CoRpteTdotELoneplusdsbtlbidsbisbH}{\CoRpteTdotELoneplusdsbtlbidsbisbJ}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbisbK}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
TLBI VAE1,X4
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTdotELoneplusdsbtlbidsbisbL}
\settowidth{\CoRpteTdotELoneplusdsbtlbidsbisbL}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbisbK}}
\addtolength{\CoRpteTdotELoneplusdsbtlbidsbisbH}{\CoRpteTdotELoneplusdsbtlbidsbisbL}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbisbM}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTdotELoneplusdsbtlbidsbisbN}
\settowidth{\CoRpteTdotELoneplusdsbtlbidsbisbN}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbisbM}}
\addtolength{\CoRpteTdotELoneplusdsbtlbidsbisbH}{\CoRpteTdotELoneplusdsbtlbidsbisbN}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbisbO}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;

    *pa1 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTdotELoneplusdsbtlbidsbisbP}
\settowidth{\CoRpteTdotELoneplusdsbtlbidsbisbP}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbisbO}}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbisbA}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbisbA}
\begin{minipage}{\CoRpteTdotELoneplusdsbtlbidsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRpteT.EL1+dsb-tlbi-dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRpteTdotELoneplusdsbtlbidsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRpteTdotELoneplusdsbtlbidsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRpteTdotELoneplusdsbtlbidsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRpteTdotELoneplusdsbtlbidsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoRpteTdotELoneplusdsbtlbidsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=0 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoRpteT.EL1+dsb-tlbi-dsb.tex <==
\newlength{\CoRpteTdotELoneplusdsbtlbidsbH}
\setlength{\CoRpteTdotELoneplusdsbtlbidsbH}{0cm}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbI}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTdotELoneplusdsbtlbidsbJ}
\settowidth{\CoRpteTdotELoneplusdsbtlbidsbJ}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbI}}
\addtolength{\CoRpteTdotELoneplusdsbtlbidsbH}{\CoRpteTdotELoneplusdsbtlbidsbJ}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbK}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
TLBI VAE1,X4
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTdotELoneplusdsbtlbidsbL}
\settowidth{\CoRpteTdotELoneplusdsbtlbidsbL}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbK}}
\addtolength{\CoRpteTdotELoneplusdsbtlbidsbH}{\CoRpteTdotELoneplusdsbtlbidsbL}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbM}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTdotELoneplusdsbtlbidsbN}
\settowidth{\CoRpteTdotELoneplusdsbtlbidsbN}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbM}}
\addtolength{\CoRpteTdotELoneplusdsbtlbidsbH}{\CoRpteTdotELoneplusdsbtlbidsbN}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbO}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;

    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;

    *pa1 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTdotELoneplusdsbtlbidsbP}
\settowidth{\CoRpteTdotELoneplusdsbtlbidsbP}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbO}}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbA}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbA}
\begin{minipage}{\CoRpteTdotELoneplusdsbtlbidsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRpteT.EL1+dsb-tlbi-dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRpteTdotELoneplusdsbtlbidsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRpteTdotELoneplusdsbtlbidsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRpteTdotELoneplusdsbtlbidsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRpteTdotELoneplusdsbtlbidsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoRpteTdotELoneplusdsbtlbidsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=0 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoRpteTf.inv+dsb-isb.tex <==
\newlength{\CoRpteTfdotinvplusdsbisbH}
\setlength{\CoRpteTfdotinvplusdsbisbH}{0cm}
\newsavebox{\CoRpteTfdotinvplusdsbisbI}
\begin{lrbox}{\CoRpteTfdotinvplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTfdotinvplusdsbisbJ}
\settowidth{\CoRpteTfdotinvplusdsbisbJ}{\usebox{\CoRpteTfdotinvplusdsbisbI}}
\addtolength{\CoRpteTfdotinvplusdsbisbH}{\CoRpteTfdotinvplusdsbisbJ}
\newsavebox{\CoRpteTfdotinvplusdsbisbK}
\begin{lrbox}{\CoRpteTfdotinvplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTfdotinvplusdsbisbL}
\settowidth{\CoRpteTfdotinvplusdsbisbL}{\usebox{\CoRpteTfdotinvplusdsbisbK}}
\addtolength{\CoRpteTfdotinvplusdsbisbH}{\CoRpteTfdotinvplusdsbisbL}
\newsavebox{\CoRpteTfdotinvplusdsbisbM}
\begin{lrbox}{\CoRpteTfdotinvplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTfdotinvplusdsbisbN}
\settowidth{\CoRpteTfdotinvplusdsbisbN}{\usebox{\CoRpteTfdotinvplusdsbisbM}}
\addtolength{\CoRpteTfdotinvplusdsbisbH}{\CoRpteTfdotinvplusdsbisbN}
\newsavebox{\CoRpteTfdotinvplusdsbisbO}
\begin{lrbox}{\CoRpteTfdotinvplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    option default_tables = true;
    physical pa1;
    intermediate ipa1;

    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    identity 0x1000 with code;

    *pa1 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTfdotinvplusdsbisbP}
\settowidth{\CoRpteTfdotinvplusdsbisbP}{\usebox{\CoRpteTfdotinvplusdsbisbO}}
\newsavebox{\CoRpteTfdotinvplusdsbisbA}
\begin{lrbox}{\CoRpteTfdotinvplusdsbisbA}
\begin{minipage}{\CoRpteTfdotinvplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRpteTf.inv+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRpteTfdotinvplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRpteTfdotinvplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRpteTfdotinvplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRpteTfdotinvplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRpteTfdotinvplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoRpteTfdotinvplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=desc3(y,page_table_base) & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoRpteTf.inv+dsb.tex <==
\newlength{\CoRpteTfdotinvplusdsbH}
\setlength{\CoRpteTfdotinvplusdsbH}{0cm}
\newsavebox{\CoRpteTfdotinvplusdsbI}
\begin{lrbox}{\CoRpteTfdotinvplusdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTfdotinvplusdsbJ}
\settowidth{\CoRpteTfdotinvplusdsbJ}{\usebox{\CoRpteTfdotinvplusdsbI}}
\addtolength{\CoRpteTfdotinvplusdsbH}{\CoRpteTfdotinvplusdsbJ}
\newsavebox{\CoRpteTfdotinvplusdsbK}
\begin{lrbox}{\CoRpteTfdotinvplusdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTfdotinvplusdsbL}
\settowidth{\CoRpteTfdotinvplusdsbL}{\usebox{\CoRpteTfdotinvplusdsbK}}
\addtolength{\CoRpteTfdotinvplusdsbH}{\CoRpteTfdotinvplusdsbL}
\newsavebox{\CoRpteTfdotinvplusdsbM}
\begin{lrbox}{\CoRpteTfdotinvplusdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTfdotinvplusdsbN}
\settowidth{\CoRpteTfdotinvplusdsbN}{\usebox{\CoRpteTfdotinvplusdsbM}}
\addtolength{\CoRpteTfdotinvplusdsbH}{\CoRpteTfdotinvplusdsbN}
\newsavebox{\CoRpteTfdotinvplusdsbO}
\begin{lrbox}{\CoRpteTfdotinvplusdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    identity 0x1000 with code;

    *pa1 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTfdotinvplusdsbP}
\settowidth{\CoRpteTfdotinvplusdsbP}{\usebox{\CoRpteTfdotinvplusdsbO}}
\newsavebox{\CoRpteTfdotinvplusdsbA}
\begin{lrbox}{\CoRpteTfdotinvplusdsbA}
\begin{minipage}{\CoRpteTfdotinvplusdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRpteTf.inv+dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRpteTfdotinvplusdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRpteTfdotinvplusdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRpteTfdotinvplusdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRpteTfdotinvplusdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRpteTfdotinvplusdsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoRpteTfdotinvplusdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=desc3(y,page_table_base) & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoTRpte.inv+dsb-isb.tex <==
\newlength{\CoTRptedotinvplusdsbisbH}
\setlength{\CoTRptedotinvplusdsbisbH}{0cm}
\newsavebox{\CoTRptedotinvplusdsbisbI}
\begin{lrbox}{\CoTRptedotinvplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvplusdsbisbJ}
\settowidth{\CoTRptedotinvplusdsbisbJ}{\usebox{\CoTRptedotinvplusdsbisbI}}
\addtolength{\CoTRptedotinvplusdsbisbH}{\CoTRptedotinvplusdsbisbJ}
\newsavebox{\CoTRptedotinvplusdsbisbK}
\begin{lrbox}{\CoTRptedotinvplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvplusdsbisbL}
\settowidth{\CoTRptedotinvplusdsbisbL}{\usebox{\CoTRptedotinvplusdsbisbK}}
\addtolength{\CoTRptedotinvplusdsbisbH}{\CoTRptedotinvplusdsbisbL}
\newsavebox{\CoTRptedotinvplusdsbisbM}
\begin{lrbox}{\CoTRptedotinvplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvplusdsbisbN}
\settowidth{\CoTRptedotinvplusdsbisbN}{\usebox{\CoTRptedotinvplusdsbisbM}}
\addtolength{\CoTRptedotinvplusdsbisbH}{\CoTRptedotinvplusdsbisbN}
\newsavebox{\CoTRptedotinvplusdsbisbO}
\begin{lrbox}{\CoTRptedotinvplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvplusdsbisbP}
\settowidth{\CoTRptedotinvplusdsbisbP}{\usebox{\CoTRptedotinvplusdsbisbO}}
\newsavebox{\CoTRptedotinvplusdsbisbA}
\begin{lrbox}{\CoTRptedotinvplusdsbisbA}
\begin{minipage}{\CoTRptedotinvplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTRpte.inv+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTRptedotinvplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTRptedotinvplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTRptedotinvplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoTRpte.inv+dsb.tex <==
\newlength{\CoTRptedotinvplusdsbH}
\setlength{\CoTRptedotinvplusdsbH}{0cm}
\newsavebox{\CoTRptedotinvplusdsbI}
\begin{lrbox}{\CoTRptedotinvplusdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvplusdsbJ}
\settowidth{\CoTRptedotinvplusdsbJ}{\usebox{\CoTRptedotinvplusdsbI}}
\addtolength{\CoTRptedotinvplusdsbH}{\CoTRptedotinvplusdsbJ}
\newsavebox{\CoTRptedotinvplusdsbK}
\begin{lrbox}{\CoTRptedotinvplusdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvplusdsbL}
\settowidth{\CoTRptedotinvplusdsbL}{\usebox{\CoTRptedotinvplusdsbK}}
\addtolength{\CoTRptedotinvplusdsbH}{\CoTRptedotinvplusdsbL}
\newsavebox{\CoTRptedotinvplusdsbM}
\begin{lrbox}{\CoTRptedotinvplusdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvplusdsbN}
\settowidth{\CoTRptedotinvplusdsbN}{\usebox{\CoTRptedotinvplusdsbM}}
\addtolength{\CoTRptedotinvplusdsbH}{\CoTRptedotinvplusdsbN}
\newsavebox{\CoTRptedotinvplusdsbO}
\begin{lrbox}{\CoTRptedotinvplusdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *y = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvplusdsbP}
\settowidth{\CoTRptedotinvplusdsbP}{\usebox{\CoTRptedotinvplusdsbO}}
\newsavebox{\CoTRptedotinvplusdsbA}
\begin{lrbox}{\CoTRptedotinvplusdsbA}
\begin{minipage}{\CoTRptedotinvplusdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTRpte.inv+dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTRptedotinvplusdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTRptedotinvplusdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTRptedotinvplusdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvplusdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvplusdsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvplusdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoTRpte.inv+po.tex <==
\newlength{\CoTRptedotinvpluspoH}
\setlength{\CoTRptedotinvpluspoH}{0cm}
\newsavebox{\CoTRptedotinvpluspoI}
\begin{lrbox}{\CoTRptedotinvpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvpluspoJ}
\settowidth{\CoTRptedotinvpluspoJ}{\usebox{\CoTRptedotinvpluspoI}}
\addtolength{\CoTRptedotinvpluspoH}{\CoTRptedotinvpluspoJ}
\newsavebox{\CoTRptedotinvpluspoK}
\begin{lrbox}{\CoTRptedotinvpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvpluspoL}
\settowidth{\CoTRptedotinvpluspoL}{\usebox{\CoTRptedotinvpluspoK}}
\addtolength{\CoTRptedotinvpluspoH}{\CoTRptedotinvpluspoL}
\newsavebox{\CoTRptedotinvpluspoM}
\begin{lrbox}{\CoTRptedotinvpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvpluspoN}
\settowidth{\CoTRptedotinvpluspoN}{\usebox{\CoTRptedotinvpluspoM}}
\addtolength{\CoTRptedotinvpluspoH}{\CoTRptedotinvpluspoN}
\newsavebox{\CoTRptedotinvpluspoO}
\begin{lrbox}{\CoTRptedotinvpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *y = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvpluspoP}
\settowidth{\CoTRptedotinvpluspoP}{\usebox{\CoTRptedotinvpluspoO}}
\newsavebox{\CoTRptedotinvpluspoA}
\begin{lrbox}{\CoTRptedotinvpluspoA}
\begin{minipage}{\CoTRptedotinvpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTRpte.inv+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTRptedotinvpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTRptedotinvpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTRptedotinvpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoTT.ro+dmb.tex <==
\newlength{\CoTTdotroplusdmbH}
\setlength{\CoTTdotroplusdmbH}{0cm}
\newsavebox{\CoTTdotroplusdmbI}
\begin{lrbox}{\CoTTdotroplusdmbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotroplusdmbJ}
\settowidth{\CoTTdotroplusdmbJ}{\usebox{\CoTTdotroplusdmbI}}
\addtolength{\CoTTdotroplusdmbH}{\CoTTdotroplusdmbJ}
\newsavebox{\CoTTdotroplusdmbK}
\begin{lrbox}{\CoTTdotroplusdmbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotroplusdmbL}
\settowidth{\CoTTdotroplusdmbL}{\usebox{\CoTTdotroplusdmbK}}
\addtolength{\CoTTdotroplusdmbH}{\CoTTdotroplusdmbL}
\newsavebox{\CoTTdotroplusdmbM}
\begin{lrbox}{\CoTTdotroplusdmbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1 with [AP = 0b11] and default;
    x ?-> pa2 with [AP = 0b11] and default;
    y |-> pa2 with [AP = 0b11] and default;

    *pa2 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotroplusdmbN}
\settowidth{\CoTTdotroplusdmbN}{\usebox{\CoTTdotroplusdmbM}}
\newsavebox{\CoTTdotroplusdmbO}
\begin{lrbox}{\CoTTdotroplusdmbO}
\begin{minipage}{\CoTTdotroplusdmbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTT.ro+dmb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTTdotroplusdmbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTTdotroplusdmbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTTdotroplusdmbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTTdotroplusdmbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTTdotroplusdmbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoTT.ro+dsb-isb.tex <==
\newlength{\CoTTdotroplusdsbisbH}
\setlength{\CoTTdotroplusdsbisbH}{0cm}
\newsavebox{\CoTTdotroplusdsbisbI}
\begin{lrbox}{\CoTTdotroplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotroplusdsbisbJ}
\settowidth{\CoTTdotroplusdsbisbJ}{\usebox{\CoTTdotroplusdsbisbI}}
\addtolength{\CoTTdotroplusdsbisbH}{\CoTTdotroplusdsbisbJ}
\newsavebox{\CoTTdotroplusdsbisbK}
\begin{lrbox}{\CoTTdotroplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotroplusdsbisbL}
\settowidth{\CoTTdotroplusdsbisbL}{\usebox{\CoTTdotroplusdsbisbK}}
\addtolength{\CoTTdotroplusdsbisbH}{\CoTTdotroplusdsbisbL}
\newsavebox{\CoTTdotroplusdsbisbM}
\begin{lrbox}{\CoTTdotroplusdsbisbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1 with [AP = 0b11] and default;
    x ?-> pa2 with [AP = 0b11] and default;
    y |-> pa2 with [AP = 0b11] and default;

    *pa2 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotroplusdsbisbN}
\settowidth{\CoTTdotroplusdsbisbN}{\usebox{\CoTTdotroplusdsbisbM}}
\newsavebox{\CoTTdotroplusdsbisbO}
\begin{lrbox}{\CoTTdotroplusdsbisbO}
\begin{minipage}{\CoTTdotroplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTT.ro+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTTdotroplusdsbisbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTTdotroplusdsbisbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTTdotroplusdsbisbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTTdotroplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTTdotroplusdsbisbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoTT.ro+po.tex <==
\newlength{\CoTTdotropluspoH}
\setlength{\CoTTdotropluspoH}{0cm}
\newsavebox{\CoTTdotropluspoI}
\begin{lrbox}{\CoTTdotropluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotropluspoJ}
\settowidth{\CoTTdotropluspoJ}{\usebox{\CoTTdotropluspoI}}
\addtolength{\CoTTdotropluspoH}{\CoTTdotropluspoJ}
\newsavebox{\CoTTdotropluspoK}
\begin{lrbox}{\CoTTdotropluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotropluspoL}
\settowidth{\CoTTdotropluspoL}{\usebox{\CoTTdotropluspoK}}
\addtolength{\CoTTdotropluspoH}{\CoTTdotropluspoL}
\newsavebox{\CoTTdotropluspoM}
\begin{lrbox}{\CoTTdotropluspoM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1 with [AP = 0b11] and default;
    x ?-> pa2 with [AP = 0b11] and default;
    y |-> pa2 with [AP = 0b11] and default;

    *pa2 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotropluspoN}
\settowidth{\CoTTdotropluspoN}{\usebox{\CoTTdotropluspoM}}
\newsavebox{\CoTTdotropluspoO}
\begin{lrbox}{\CoTTdotropluspoO}
\begin{minipage}{\CoTTdotropluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTT.ro+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTTdotropluspoN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTTdotropluspoM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTTdotropluspoO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTTdotropluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTTdotropluspoK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoTTf.inv+dsb-isb.tex <==
\newlength{\CoTTfdotinvplusdsbisbH}
\setlength{\CoTTfdotinvplusdsbisbH}{0cm}
\newsavebox{\CoTTfdotinvplusdsbisbI}
\begin{lrbox}{\CoTTfdotinvplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTfdotinvplusdsbisbJ}
\settowidth{\CoTTfdotinvplusdsbisbJ}{\usebox{\CoTTfdotinvplusdsbisbI}}
\addtolength{\CoTTfdotinvplusdsbisbH}{\CoTTfdotinvplusdsbisbJ}
\newsavebox{\CoTTfdotinvplusdsbisbK}
\begin{lrbox}{\CoTTfdotinvplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTfdotinvplusdsbisbL}
\settowidth{\CoTTfdotinvplusdsbisbL}{\usebox{\CoTTfdotinvplusdsbisbK}}
\addtolength{\CoTTfdotinvplusdsbisbH}{\CoTTfdotinvplusdsbisbL}
\newsavebox{\CoTTfdotinvplusdsbisbM}
\begin{lrbox}{\CoTTfdotinvplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTfdotinvplusdsbisbN}
\settowidth{\CoTTfdotinvplusdsbisbN}{\usebox{\CoTTfdotinvplusdsbisbM}}
\addtolength{\CoTTfdotinvplusdsbisbH}{\CoTTfdotinvplusdsbisbN}
\newsavebox{\CoTTfdotinvplusdsbisbO}
\begin{lrbox}{\CoTTfdotinvplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTfdotinvplusdsbisbP}
\settowidth{\CoTTfdotinvplusdsbisbP}{\usebox{\CoTTfdotinvplusdsbisbO}}
\newsavebox{\CoTTfdotinvplusdsbisbA}
\begin{lrbox}{\CoTTfdotinvplusdsbisbA}
\begin{minipage}{\CoTTfdotinvplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTTf.inv+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTTfdotinvplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTTfdotinvplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTTfdotinvplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTTfdotinvplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTTfdotinvplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTTfdotinvplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoTTf.inv+po.tex <==
\newlength{\CoTTfdotinvpluspoH}
\setlength{\CoTTfdotinvpluspoH}{0cm}
\newsavebox{\CoTTfdotinvpluspoI}
\begin{lrbox}{\CoTTfdotinvpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTfdotinvpluspoJ}
\settowidth{\CoTTfdotinvpluspoJ}{\usebox{\CoTTfdotinvpluspoI}}
\addtolength{\CoTTfdotinvpluspoH}{\CoTTfdotinvpluspoJ}
\newsavebox{\CoTTfdotinvpluspoK}
\begin{lrbox}{\CoTTfdotinvpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTfdotinvpluspoL}
\settowidth{\CoTTfdotinvpluspoL}{\usebox{\CoTTfdotinvpluspoK}}
\addtolength{\CoTTfdotinvpluspoH}{\CoTTfdotinvpluspoL}
\newsavebox{\CoTTfdotinvpluspoM}
\begin{lrbox}{\CoTTfdotinvpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTfdotinvpluspoN}
\settowidth{\CoTTfdotinvpluspoN}{\usebox{\CoTTfdotinvpluspoM}}
\addtolength{\CoTTfdotinvpluspoH}{\CoTTfdotinvpluspoN}
\newsavebox{\CoTTfdotinvpluspoO}
\begin{lrbox}{\CoTTfdotinvpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTfdotinvpluspoP}
\settowidth{\CoTTfdotinvpluspoP}{\usebox{\CoTTfdotinvpluspoO}}
\newsavebox{\CoTTfdotinvpluspoA}
\begin{lrbox}{\CoTTfdotinvpluspoA}
\begin{minipage}{\CoTTfdotinvpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTTf.inv+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTTfdotinvpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTTfdotinvpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTTfdotinvpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTTfdotinvpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTTfdotinvpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTTfdotinvpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoTW1.inv.tex <==
\newlength{\CoTWonedotinvH}
\setlength{\CoTWonedotinvH}{0cm}
\newsavebox{\CoTWonedotinvI}
\begin{lrbox}{\CoTWonedotinvI}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTWonedotinvJ}
\settowidth{\CoTWonedotinvJ}{\usebox{\CoTWonedotinvI}}
\addtolength{\CoTWonedotinvH}{\CoTWonedotinvJ}
\newsavebox{\CoTWonedotinvK}
\begin{lrbox}{\CoTWonedotinvK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTWonedotinvL}
\settowidth{\CoTWonedotinvL}{\usebox{\CoTWonedotinvK}}
\addtolength{\CoTWonedotinvH}{\CoTWonedotinvL}
\newsavebox{\CoTWonedotinvM}
\begin{lrbox}{\CoTWonedotinvM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTWonedotinvN}
\settowidth{\CoTWonedotinvN}{\usebox{\CoTWonedotinvM}}
\newsavebox{\CoTWonedotinvO}
\begin{lrbox}{\CoTWonedotinvO}
\begin{minipage}{\CoTWonedotinvH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=x|\\
\lstinline[language=IslaLitmusExp]|R2=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTW1.inv|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTWonedotinvN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTWonedotinvM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTWonedotinvO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTWonedotinvI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTWonedotinvK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoTWinv.tex <==
\newlength{\CoTWinvH}
\setlength{\CoTWinvH}{0cm}
\newsavebox{\CoTWinvI}
\begin{lrbox}{\CoTWinvI}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTWinvJ}
\settowidth{\CoTWinvJ}{\usebox{\CoTWinvI}}
\addtolength{\CoTWinvH}{\CoTWinvJ}
\newsavebox{\CoTWinvK}
\begin{lrbox}{\CoTWinvK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTWinvL}
\settowidth{\CoTWinvL}{\usebox{\CoTWinvK}}
\addtolength{\CoTWinvH}{\CoTWinvL}
\newsavebox{\CoTWinvM}
\begin{lrbox}{\CoTWinvM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTWinvN}
\settowidth{\CoTWinvN}{\usebox{\CoTWinvM}}
\newsavebox{\CoTWinvO}
\begin{lrbox}{\CoTWinvO}
\begin{minipage}{\CoTWinvH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=x|\\
\lstinline[language=IslaLitmusExp]|R2=0b0|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTWinv|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTWinvN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTWinvM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTWinvO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTWinvI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTWinvK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoTfRpte+dsb-isb.tex <==
\newlength{\CoTfRpteplusdsbisbH}
\setlength{\CoTfRpteplusdsbisbH}{0cm}
\newsavebox{\CoTfRpteplusdsbisbI}
\begin{lrbox}{\CoTfRpteplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRpteplusdsbisbJ}
\settowidth{\CoTfRpteplusdsbisbJ}{\usebox{\CoTfRpteplusdsbisbI}}
\addtolength{\CoTfRpteplusdsbisbH}{\CoTfRpteplusdsbisbJ}
\newsavebox{\CoTfRpteplusdsbisbK}
\begin{lrbox}{\CoTfRpteplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRpteplusdsbisbL}
\settowidth{\CoTfRpteplusdsbisbL}{\usebox{\CoTfRpteplusdsbisbK}}
\addtolength{\CoTfRpteplusdsbisbH}{\CoTfRpteplusdsbisbL}
\newsavebox{\CoTfRpteplusdsbisbM}
\begin{lrbox}{\CoTfRpteplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRpteplusdsbisbN}
\settowidth{\CoTfRpteplusdsbisbN}{\usebox{\CoTfRpteplusdsbisbM}}
\addtolength{\CoTfRpteplusdsbisbH}{\CoTfRpteplusdsbisbN}
\newsavebox{\CoTfRpteplusdsbisbO}
\begin{lrbox}{\CoTfRpteplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;
    y |-> pa1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRpteplusdsbisbP}
\settowidth{\CoTfRpteplusdsbisbP}{\usebox{\CoTfRpteplusdsbisbO}}
\newsavebox{\CoTfRpteplusdsbisbA}
\begin{lrbox}{\CoTfRpteplusdsbisbA}
\begin{minipage}{\CoTfRpteplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfRpte+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfRpteplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfRpteplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfRpteplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfRpteplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTfRpteplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfRpteplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=desc3(y,page_table_base)|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoTfRpte+dsb.tex <==
\newlength{\CoTfRpteplusdsbH}
\setlength{\CoTfRpteplusdsbH}{0cm}
\newsavebox{\CoTfRpteplusdsbI}
\begin{lrbox}{\CoTfRpteplusdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRpteplusdsbJ}
\settowidth{\CoTfRpteplusdsbJ}{\usebox{\CoTfRpteplusdsbI}}
\addtolength{\CoTfRpteplusdsbH}{\CoTfRpteplusdsbJ}
\newsavebox{\CoTfRpteplusdsbK}
\begin{lrbox}{\CoTfRpteplusdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRpteplusdsbL}
\settowidth{\CoTfRpteplusdsbL}{\usebox{\CoTfRpteplusdsbK}}
\addtolength{\CoTfRpteplusdsbH}{\CoTfRpteplusdsbL}
\newsavebox{\CoTfRpteplusdsbM}
\begin{lrbox}{\CoTfRpteplusdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRpteplusdsbN}
\settowidth{\CoTfRpteplusdsbN}{\usebox{\CoTfRpteplusdsbM}}
\addtolength{\CoTfRpteplusdsbH}{\CoTfRpteplusdsbN}
\newsavebox{\CoTfRpteplusdsbO}
\begin{lrbox}{\CoTfRpteplusdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;
    y |-> pa1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRpteplusdsbP}
\settowidth{\CoTfRpteplusdsbP}{\usebox{\CoTfRpteplusdsbO}}
\newsavebox{\CoTfRpteplusdsbA}
\begin{lrbox}{\CoTfRpteplusdsbA}
\begin{minipage}{\CoTfRpteplusdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfRpte+dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfRpteplusdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfRpteplusdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfRpteplusdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfRpteplusdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTfRpteplusdsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfRpteplusdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=desc3(y,page_table_base)|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoTfRpte+eret.tex <==
\newlength{\CoTfRptepluseretH}
\setlength{\CoTfRptepluseretH}{0cm}
\newsavebox{\CoTfRptepluseretI}
\begin{lrbox}{\CoTfRptepluseretI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRptepluseretJ}
\settowidth{\CoTfRptepluseretJ}{\usebox{\CoTfRptepluseretI}}
\addtolength{\CoTfRptepluseretH}{\CoTfRptepluseretJ}
\newsavebox{\CoTfRptepluseretK}
\begin{lrbox}{\CoTfRptepluseretK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRptepluseretL}
\settowidth{\CoTfRptepluseretL}{\usebox{\CoTfRptepluseretK}}
\addtolength{\CoTfRptepluseretH}{\CoTfRptepluseretL}
\newsavebox{\CoTfRptepluseretM}
\begin{lrbox}{\CoTfRptepluseretM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRptepluseretN}
\settowidth{\CoTfRptepluseretN}{\usebox{\CoTfRptepluseretM}}
\addtolength{\CoTfRptepluseretH}{\CoTfRptepluseretN}
\newsavebox{\CoTfRptepluseretO}
\begin{lrbox}{\CoTfRptepluseretO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;
    y |-> pa1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRptepluseretP}
\settowidth{\CoTfRptepluseretP}{\usebox{\CoTfRptepluseretO}}
\newsavebox{\CoTfRptepluseretA}
\begin{lrbox}{\CoTfRptepluseretA}
\begin{minipage}{\CoTfRptepluseretH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfRpte+eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfRptepluseretP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfRptepluseretO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfRptepluseretA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfRptepluseretI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTfRptepluseretK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfRptepluseretM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=desc3(y,page_table_base)|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoTfRpte+po.tex <==
\newlength{\CoTfRptepluspoH}
\setlength{\CoTfRptepluspoH}{0cm}
\newsavebox{\CoTfRptepluspoI}
\begin{lrbox}{\CoTfRptepluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRptepluspoJ}
\settowidth{\CoTfRptepluspoJ}{\usebox{\CoTfRptepluspoI}}
\addtolength{\CoTfRptepluspoH}{\CoTfRptepluspoJ}
\newsavebox{\CoTfRptepluspoK}
\begin{lrbox}{\CoTfRptepluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRptepluspoL}
\settowidth{\CoTfRptepluspoL}{\usebox{\CoTfRptepluspoK}}
\addtolength{\CoTfRptepluspoH}{\CoTfRptepluspoL}
\newsavebox{\CoTfRptepluspoM}
\begin{lrbox}{\CoTfRptepluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRptepluspoN}
\settowidth{\CoTfRptepluspoN}{\usebox{\CoTfRptepluspoM}}
\addtolength{\CoTfRptepluspoH}{\CoTfRptepluspoN}
\newsavebox{\CoTfRptepluspoO}
\begin{lrbox}{\CoTfRptepluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;
    y |-> pa1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRptepluspoP}
\settowidth{\CoTfRptepluspoP}{\usebox{\CoTfRptepluspoO}}
\newsavebox{\CoTfRptepluspoA}
\begin{lrbox}{\CoTfRptepluspoA}
\begin{minipage}{\CoTfRptepluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfRpte+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfRptepluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfRptepluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfRptepluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfRptepluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTfRptepluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfRptepluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=desc3(y,page_table_base)|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoTfT+dsb-isb.tex <==
\newlength{\CoTfTplusdsbisbH}
\setlength{\CoTfTplusdsbisbH}{0cm}
\newsavebox{\CoTfTplusdsbisbI}
\begin{lrbox}{\CoTfTplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfTplusdsbisbJ}
\settowidth{\CoTfTplusdsbisbJ}{\usebox{\CoTfTplusdsbisbI}}
\addtolength{\CoTfTplusdsbisbH}{\CoTfTplusdsbisbJ}
\newsavebox{\CoTfTplusdsbisbK}
\begin{lrbox}{\CoTfTplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfTplusdsbisbL}
\settowidth{\CoTfTplusdsbisbL}{\usebox{\CoTfTplusdsbisbK}}
\addtolength{\CoTfTplusdsbisbH}{\CoTfTplusdsbisbL}
\newsavebox{\CoTfTplusdsbisbM}
\begin{lrbox}{\CoTfTplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfTplusdsbisbN}
\settowidth{\CoTfTplusdsbisbN}{\usebox{\CoTfTplusdsbisbM}}
\addtolength{\CoTfTplusdsbisbH}{\CoTfTplusdsbisbN}
\newsavebox{\CoTfTplusdsbisbO}
\begin{lrbox}{\CoTfTplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;
    y |-> pa1;
    *pa1 = 0;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfTplusdsbisbP}
\settowidth{\CoTfTplusdsbisbP}{\usebox{\CoTfTplusdsbisbO}}
\newsavebox{\CoTfTplusdsbisbA}
\begin{lrbox}{\CoTfTplusdsbisbA}
\begin{minipage}{\CoTfTplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfT+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfTplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfTplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfTplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfTplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTfTplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfTplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoTfT+po.tex <==
\newlength{\CoTfTpluspoH}
\setlength{\CoTfTpluspoH}{0cm}
\newsavebox{\CoTfTpluspoI}
\begin{lrbox}{\CoTfTpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfTpluspoJ}
\settowidth{\CoTfTpluspoJ}{\usebox{\CoTfTpluspoI}}
\addtolength{\CoTfTpluspoH}{\CoTfTpluspoJ}
\newsavebox{\CoTfTpluspoK}
\begin{lrbox}{\CoTfTpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfTpluspoL}
\settowidth{\CoTfTpluspoL}{\usebox{\CoTfTpluspoK}}
\addtolength{\CoTfTpluspoH}{\CoTfTpluspoL}
\newsavebox{\CoTfTpluspoM}
\begin{lrbox}{\CoTfTpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfTpluspoN}
\settowidth{\CoTfTpluspoN}{\usebox{\CoTfTpluspoM}}
\addtolength{\CoTfTpluspoH}{\CoTfTpluspoN}
\newsavebox{\CoTfTpluspoO}
\begin{lrbox}{\CoTfTpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;
    y |-> pa1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfTpluspoP}
\settowidth{\CoTfTpluspoP}{\usebox{\CoTfTpluspoO}}
\newsavebox{\CoTfTpluspoA}
\begin{lrbox}{\CoTfTpluspoA}
\begin{minipage}{\CoTfTpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfT+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfTpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfTpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfTpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfTpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTfTpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfTpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoTfW.inv+dsb-isb.tex <==
\newlength{\CoTfWdotinvplusdsbisbH}
\setlength{\CoTfWdotinvplusdsbisbH}{0cm}
\newsavebox{\CoTfWdotinvplusdsbisbI}
\begin{lrbox}{\CoTfWdotinvplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvplusdsbisbJ}
\settowidth{\CoTfWdotinvplusdsbisbJ}{\usebox{\CoTfWdotinvplusdsbisbI}}
\addtolength{\CoTfWdotinvplusdsbisbH}{\CoTfWdotinvplusdsbisbJ}
\newsavebox{\CoTfWdotinvplusdsbisbK}
\begin{lrbox}{\CoTfWdotinvplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvplusdsbisbL}
\settowidth{\CoTfWdotinvplusdsbisbL}{\usebox{\CoTfWdotinvplusdsbisbK}}
\addtolength{\CoTfWdotinvplusdsbisbH}{\CoTfWdotinvplusdsbisbL}
\newsavebox{\CoTfWdotinvplusdsbisbM}
\begin{lrbox}{\CoTfWdotinvplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvplusdsbisbN}
\settowidth{\CoTfWdotinvplusdsbisbN}{\usebox{\CoTfWdotinvplusdsbisbM}}
\addtolength{\CoTfWdotinvplusdsbisbH}{\CoTfWdotinvplusdsbisbN}
\newsavebox{\CoTfWdotinvplusdsbisbO}
\begin{lrbox}{\CoTfWdotinvplusdsbisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvplusdsbisbP}
\settowidth{\CoTfWdotinvplusdsbisbP}{\usebox{\CoTfWdotinvplusdsbisbO}}
\addtolength{\CoTfWdotinvplusdsbisbH}{\CoTfWdotinvplusdsbisbP}
\newsavebox{\CoTfWdotinvplusdsbisbA}
\begin{lrbox}{\CoTfWdotinvplusdsbisbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    x ?-> raw(2);
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvplusdsbisbB}
\settowidth{\CoTfWdotinvplusdsbisbB}{\usebox{\CoTfWdotinvplusdsbisbA}}
\newsavebox{\CoTfWdotinvplusdsbisbC}
\begin{lrbox}{\CoTfWdotinvplusdsbisbC}
\begin{minipage}{\CoTfWdotinvplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b10|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:R1=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfW.inv+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfWdotinvplusdsbisbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfWdotinvplusdsbisbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfWdotinvplusdsbisbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfWdotinvplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTfWdotinvplusdsbisbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\CoTfWdotinvplusdsbisbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfWdotinvplusdsbisbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=2 & 2:R2=mkdesc3(oa=pa1)|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoTfW.inv+po.tex <==
\newlength{\CoTfWdotinvpluspoH}
\setlength{\CoTfWdotinvpluspoH}{0cm}
\newsavebox{\CoTfWdotinvpluspoI}
\begin{lrbox}{\CoTfWdotinvpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvpluspoJ}
\settowidth{\CoTfWdotinvpluspoJ}{\usebox{\CoTfWdotinvpluspoI}}
\addtolength{\CoTfWdotinvpluspoH}{\CoTfWdotinvpluspoJ}
\newsavebox{\CoTfWdotinvpluspoK}
\begin{lrbox}{\CoTfWdotinvpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvpluspoL}
\settowidth{\CoTfWdotinvpluspoL}{\usebox{\CoTfWdotinvpluspoK}}
\addtolength{\CoTfWdotinvpluspoH}{\CoTfWdotinvpluspoL}
\newsavebox{\CoTfWdotinvpluspoM}
\begin{lrbox}{\CoTfWdotinvpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvpluspoN}
\settowidth{\CoTfWdotinvpluspoN}{\usebox{\CoTfWdotinvpluspoM}}
\addtolength{\CoTfWdotinvpluspoH}{\CoTfWdotinvpluspoN}
\newsavebox{\CoTfWdotinvpluspoO}
\begin{lrbox}{\CoTfWdotinvpluspoO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvpluspoP}
\settowidth{\CoTfWdotinvpluspoP}{\usebox{\CoTfWdotinvpluspoO}}
\addtolength{\CoTfWdotinvpluspoH}{\CoTfWdotinvpluspoP}
\newsavebox{\CoTfWdotinvpluspoA}
\begin{lrbox}{\CoTfWdotinvpluspoA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    x ?-> raw(2);
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvpluspoB}
\settowidth{\CoTfWdotinvpluspoB}{\usebox{\CoTfWdotinvpluspoA}}
\newsavebox{\CoTfWdotinvpluspoC}
\begin{lrbox}{\CoTfWdotinvpluspoC}
\begin{minipage}{\CoTfWdotinvpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b10|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:R1=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfW.inv+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfWdotinvpluspoB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfWdotinvpluspoA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfWdotinvpluspoC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfWdotinvpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTfWdotinvpluspoK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\CoTfWdotinvpluspoM}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfWdotinvpluspoO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=2 & 2:R2=mkdesc3(oa=pa1)|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoTfW1.inv+si.tex <==
\newlength{\CoTfWonedotinvplussiH}
\setlength{\CoTfWonedotinvplussiH}{0cm}
\newsavebox{\CoTfWonedotinvplussiI}
\begin{lrbox}{\CoTfWonedotinvplussiI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWonedotinvplussiJ}
\settowidth{\CoTfWonedotinvplussiJ}{\usebox{\CoTfWonedotinvplussiI}}
\addtolength{\CoTfWonedotinvplussiH}{\CoTfWonedotinvplussiJ}
\newsavebox{\CoTfWonedotinvplussiK}
\begin{lrbox}{\CoTfWonedotinvplussiK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWonedotinvplussiL}
\settowidth{\CoTfWonedotinvplussiL}{\usebox{\CoTfWonedotinvplussiK}}
\addtolength{\CoTfWonedotinvplussiH}{\CoTfWonedotinvplussiL}
\newsavebox{\CoTfWonedotinvplussiM}
\begin{lrbox}{\CoTfWonedotinvplussiM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWonedotinvplussiN}
\settowidth{\CoTfWonedotinvplussiN}{\usebox{\CoTfWonedotinvplussiM}}
\newsavebox{\CoTfWonedotinvplussiO}
\begin{lrbox}{\CoTfWonedotinvplussiO}
\begin{minipage}{\CoTfWonedotinvplussiH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=0b10|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(0x1000,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfW1.inv+si|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfWonedotinvplussiN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfWonedotinvplussiM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfWonedotinvplussiO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfWonedotinvplussiI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfWonedotinvplussiK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R0=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoWR.alias.tex <==
\newlength{\CoWRdotaliasH}
\setlength{\CoWRdotaliasH}{0cm}
\newsavebox{\CoWRdotaliasI}
\begin{lrbox}{\CoWRdotaliasI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWRdotaliasJ}
\settowidth{\CoWRdotaliasJ}{\usebox{\CoWRdotaliasI}}
\addtolength{\CoWRdotaliasH}{\CoWRdotaliasJ}
\newsavebox{\CoWRdotaliasK}
\begin{lrbox}{\CoWRdotaliasK}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    y |-> pa1;
    *pa1 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWRdotaliasL}
\settowidth{\CoWRdotaliasL}{\usebox{\CoWRdotaliasK}}
\newsavebox{\CoWRdotaliasM}
\begin{lrbox}{\CoWRdotaliasM}
\begin{minipage}{\CoWRdotaliasH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|R0=0x1|\\
\lstinline[language=IslaLitmusExp]|R1=x|\\
\lstinline[language=IslaLitmusExp]|R3=y|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWR.alias|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWRdotaliasL}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWRdotaliasK}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWRdotaliasM}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWRdotaliasI}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoWR.inv.tex <==
\newlength{\CoWRdotinvH}
\setlength{\CoWRdotinvH}{0cm}
\newsavebox{\CoWRdotinvI}
\begin{lrbox}{\CoWRdotinvI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWRdotinvJ}
\settowidth{\CoWRdotinvJ}{\usebox{\CoWRdotinvI}}
\addtolength{\CoWRdotinvH}{\CoWRdotinvJ}
\newsavebox{\CoWRdotinvK}
\begin{lrbox}{\CoWRdotinvK}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWRdotinvL}
\settowidth{\CoWRdotinvL}{\usebox{\CoWRdotinvK}}
\newsavebox{\CoWRdotinvM}
\begin{lrbox}{\CoWRdotinvM}
\begin{minipage}{\CoWRdotinvH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWR.inv|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWRdotinvL}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWRdotinvK}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWRdotinvM}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWRdotinvI}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoWTa1.1.inv+dsb-tlbiasidis-dsb-eret.tex <==
\newlength{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetH}
\setlength{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetH}{0cm}
\newsavebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetI}
\begin{lrbox}{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI ASIDE1IS,X4
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetJ}
\settowidth{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetJ}{\usebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetI}}
\addtolength{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetH}{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetJ}
\newsavebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetK}
\begin{lrbox}{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetL}
\settowidth{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetL}{\usebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetK}}
\addtolength{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetH}{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetL}
\newsavebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetM}
\begin{lrbox}{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;

    y |-> pa1;

    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetN}
\settowidth{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetN}{\usebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetM}}
\newsavebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetO}
\begin{lrbox}{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetO}
\begin{minipage}{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL1=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=asid(0x1)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL1=0b00000|\\
\lstinline[language=IslaLitmusExp]|TTBR0_EL1=ttbr(asid=0x0001,base=page_table_base)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTa1.1.inv+dsb-tlbiasidis-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoWTa2.1.inv+dsb-tlbiasidis-dsb-eret.tex <==
\newlength{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetH}
\setlength{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetH}{0cm}
\newsavebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetI}
\begin{lrbox}{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI ASIDE1IS,X4
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetJ}
\settowidth{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetJ}{\usebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetI}}
\addtolength{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetH}{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetJ}
\newsavebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetK}
\begin{lrbox}{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetL}
\settowidth{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetL}{\usebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetK}}
\addtolength{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetH}{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetL}
\newsavebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetM}
\begin{lrbox}{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;

    y |-> pa1;

    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetN}
\settowidth{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetN}{\usebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetM}}
\newsavebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetO}
\begin{lrbox}{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetO}
\begin{minipage}{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL1=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=asid(0x2)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL1=0b00000|\\
\lstinline[language=IslaLitmusExp]|TTBR0_EL1=ttbr(asid=0x0001,base=page_table_base)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTa2.1.inv+dsb-tlbiasidis-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoWTf.inv+_dmb_-dmb-addr.tex <==
\newlength{\CoWTfdotinvplus[dmb]dmbaddrH}
\setlength{\CoWTfdotinvplus[dmb]dmbaddrH}{0cm}
\newsavebox{\CoWTfdotinvplus[dmb]dmbaddrI}
\begin{lrbox}{\CoWTfdotinvplus[dmb]dmbaddrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X2,[X1]
DSB ST
LDR X3,[X4]
EOR X5,X3,X3
LDR X6,[X7,X5]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplus[dmb]dmbaddrJ}
\settowidth{\CoWTfdotinvplus[dmb]dmbaddrJ}{\usebox{\CoWTfdotinvplus[dmb]dmbaddrI}}
\addtolength{\CoWTfdotinvplus[dmb]dmbaddrH}{\CoWTfdotinvplus[dmb]dmbaddrJ}
\newsavebox{\CoWTfdotinvplus[dmb]dmbaddrK}
\begin{lrbox}{\CoWTfdotinvplus[dmb]dmbaddrK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplus[dmb]dmbaddrL}
\settowidth{\CoWTfdotinvplus[dmb]dmbaddrL}{\usebox{\CoWTfdotinvplus[dmb]dmbaddrK}}
\addtolength{\CoWTfdotinvplus[dmb]dmbaddrH}{\CoWTfdotinvplus[dmb]dmbaddrL}
\newsavebox{\CoWTfdotinvplus[dmb]dmbaddrM}
\begin{lrbox}{\CoWTfdotinvplus[dmb]dmbaddrM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X6,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplus[dmb]dmbaddrN}
\settowidth{\CoWTfdotinvplus[dmb]dmbaddrN}{\usebox{\CoWTfdotinvplus[dmb]dmbaddrM}}
\addtolength{\CoWTfdotinvplus[dmb]dmbaddrH}{\CoWTfdotinvplus[dmb]dmbaddrN}
\newsavebox{\CoWTfdotinvplus[dmb]dmbaddrO}
\begin{lrbox}{\CoWTfdotinvplus[dmb]dmbaddrO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplus[dmb]dmbaddrP}
\settowidth{\CoWTfdotinvplus[dmb]dmbaddrP}{\usebox{\CoWTfdotinvplus[dmb]dmbaddrO}}
\newsavebox{\CoWTfdotinvplus[dmb]dmbaddrA}
\begin{lrbox}{\CoWTfdotinvplus[dmb]dmbaddrA}
\begin{minipage}{\CoWTfdotinvplus[dmb]dmbaddrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R4=y|\\
\lstinline[language=IslaLitmusExp]|0:R7=x|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+[dmb]-dmb-addr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvplus[dmb]dmbaddrP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvplus[dmb]dmbaddrO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvplus[dmb]dmbaddrA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplus[dmb]dmbaddrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplus[dmb]dmbaddrK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplus[dmb]dmbaddrM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R3=2 & 0:R6=0 & 1:R0=desc3(z,page_table_base)|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoWTf.inv+dsb-isb.tex <==
\newlength{\CoWTfdotinvplusdsbisbH}
\setlength{\CoWTfdotinvplusdsbisbH}{0cm}
\newsavebox{\CoWTfdotinvplusdsbisbI}
\begin{lrbox}{\CoWTfdotinvplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusdsbisbJ}
\settowidth{\CoWTfdotinvplusdsbisbJ}{\usebox{\CoWTfdotinvplusdsbisbI}}
\addtolength{\CoWTfdotinvplusdsbisbH}{\CoWTfdotinvplusdsbisbJ}
\newsavebox{\CoWTfdotinvplusdsbisbK}
\begin{lrbox}{\CoWTfdotinvplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusdsbisbL}
\settowidth{\CoWTfdotinvplusdsbisbL}{\usebox{\CoWTfdotinvplusdsbisbK}}
\addtolength{\CoWTfdotinvplusdsbisbH}{\CoWTfdotinvplusdsbisbL}
\newsavebox{\CoWTfdotinvplusdsbisbM}
\begin{lrbox}{\CoWTfdotinvplusdsbisbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusdsbisbN}
\settowidth{\CoWTfdotinvplusdsbisbN}{\usebox{\CoWTfdotinvplusdsbisbM}}
\newsavebox{\CoWTfdotinvplusdsbisbO}
\begin{lrbox}{\CoWTfdotinvplusdsbisbO}
\begin{minipage}{\CoWTfdotinvplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvplusdsbisbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvplusdsbisbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvplusdsbisbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplusdsbisbI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplusdsbisbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoWTf.inv+po-ctrl+po.tex <==
\newlength{\CoWTfdotinvpluspoctrlpluspoH}
\setlength{\CoWTfdotinvpluspoctrlpluspoH}{0cm}
\newsavebox{\CoWTfdotinvpluspoctrlpluspoI}
\begin{lrbox}{\CoWTfdotinvpluspoctrlpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
CBNZ X2,L0
L0:
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlpluspoJ}
\settowidth{\CoWTfdotinvpluspoctrlpluspoJ}{\usebox{\CoWTfdotinvpluspoctrlpluspoI}}
\addtolength{\CoWTfdotinvpluspoctrlpluspoH}{\CoWTfdotinvpluspoctrlpluspoJ}
\newsavebox{\CoWTfdotinvpluspoctrlpluspoK}
\begin{lrbox}{\CoWTfdotinvpluspoctrlpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlpluspoL}
\settowidth{\CoWTfdotinvpluspoctrlpluspoL}{\usebox{\CoWTfdotinvpluspoctrlpluspoK}}
\addtolength{\CoWTfdotinvpluspoctrlpluspoH}{\CoWTfdotinvpluspoctrlpluspoL}
\newsavebox{\CoWTfdotinvpluspoctrlpluspoM}
\begin{lrbox}{\CoWTfdotinvpluspoctrlpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlpluspoN}
\settowidth{\CoWTfdotinvpluspoctrlpluspoN}{\usebox{\CoWTfdotinvpluspoctrlpluspoM}}
\addtolength{\CoWTfdotinvpluspoctrlpluspoH}{\CoWTfdotinvpluspoctrlpluspoN}
\newsavebox{\CoWTfdotinvpluspoctrlpluspoO}
\begin{lrbox}{\CoWTfdotinvpluspoctrlpluspoO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlpluspoP}
\settowidth{\CoWTfdotinvpluspoctrlpluspoP}{\usebox{\CoWTfdotinvpluspoctrlpluspoO}}
\addtolength{\CoWTfdotinvpluspoctrlpluspoH}{\CoWTfdotinvpluspoctrlpluspoP}
\newsavebox{\CoWTfdotinvpluspoctrlpluspoA}
\begin{lrbox}{\CoWTfdotinvpluspoctrlpluspoA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    *pa2 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlpluspoB}
\settowidth{\CoWTfdotinvpluspoctrlpluspoB}{\usebox{\CoWTfdotinvpluspoctrlpluspoA}}
\newsavebox{\CoWTfdotinvpluspoctrlpluspoC}
\begin{lrbox}{\CoWTfdotinvpluspoctrlpluspoC}
\begin{minipage}{\CoWTfdotinvpluspoctrlpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R5=x|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+po-ctrl+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvpluspoctrlpluspoB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvpluspoctrlpluspoA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvpluspoctrlpluspoC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoctrlpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoctrlpluspoK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoctrlpluspoM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoctrlpluspoO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=1 & 0:R4=0 & 1:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoWTf.inv+po-ctrl-isb+po.tex <==
\newlength{\CoWTfdotinvpluspoctrlisbpluspoH}
\setlength{\CoWTfdotinvpluspoctrlisbpluspoH}{0cm}
\newsavebox{\CoWTfdotinvpluspoctrlisbpluspoI}
\begin{lrbox}{\CoWTfdotinvpluspoctrlisbpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
CBNZ X2,L0
L0:
ISB
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlisbpluspoJ}
\settowidth{\CoWTfdotinvpluspoctrlisbpluspoJ}{\usebox{\CoWTfdotinvpluspoctrlisbpluspoI}}
\addtolength{\CoWTfdotinvpluspoctrlisbpluspoH}{\CoWTfdotinvpluspoctrlisbpluspoJ}
\newsavebox{\CoWTfdotinvpluspoctrlisbpluspoK}
\begin{lrbox}{\CoWTfdotinvpluspoctrlisbpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlisbpluspoL}
\settowidth{\CoWTfdotinvpluspoctrlisbpluspoL}{\usebox{\CoWTfdotinvpluspoctrlisbpluspoK}}
\addtolength{\CoWTfdotinvpluspoctrlisbpluspoH}{\CoWTfdotinvpluspoctrlisbpluspoL}
\newsavebox{\CoWTfdotinvpluspoctrlisbpluspoM}
\begin{lrbox}{\CoWTfdotinvpluspoctrlisbpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlisbpluspoN}
\settowidth{\CoWTfdotinvpluspoctrlisbpluspoN}{\usebox{\CoWTfdotinvpluspoctrlisbpluspoM}}
\addtolength{\CoWTfdotinvpluspoctrlisbpluspoH}{\CoWTfdotinvpluspoctrlisbpluspoN}
\newsavebox{\CoWTfdotinvpluspoctrlisbpluspoO}
\begin{lrbox}{\CoWTfdotinvpluspoctrlisbpluspoO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlisbpluspoP}
\settowidth{\CoWTfdotinvpluspoctrlisbpluspoP}{\usebox{\CoWTfdotinvpluspoctrlisbpluspoO}}
\addtolength{\CoWTfdotinvpluspoctrlisbpluspoH}{\CoWTfdotinvpluspoctrlisbpluspoP}
\newsavebox{\CoWTfdotinvpluspoctrlisbpluspoA}
\begin{lrbox}{\CoWTfdotinvpluspoctrlisbpluspoA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    *pa2 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlisbpluspoB}
\settowidth{\CoWTfdotinvpluspoctrlisbpluspoB}{\usebox{\CoWTfdotinvpluspoctrlisbpluspoA}}
\newsavebox{\CoWTfdotinvpluspoctrlisbpluspoC}
\begin{lrbox}{\CoWTfdotinvpluspoctrlisbpluspoC}
\begin{minipage}{\CoWTfdotinvpluspoctrlisbpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R5=x|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+po-ctrl-isb+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvpluspoctrlisbpluspoB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvpluspoctrlisbpluspoA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvpluspoctrlisbpluspoC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoctrlisbpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoctrlisbpluspoK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoctrlisbpluspoM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoctrlisbpluspoO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=1 & 0:R4=0 & 1:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoWTf.inv+po.tex <==
\newlength{\CoWTfdotinvpluspoH}
\setlength{\CoWTfdotinvpluspoH}{0cm}
\newsavebox{\CoWTfdotinvpluspoI}
\begin{lrbox}{\CoWTfdotinvpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoJ}
\settowidth{\CoWTfdotinvpluspoJ}{\usebox{\CoWTfdotinvpluspoI}}
\addtolength{\CoWTfdotinvpluspoH}{\CoWTfdotinvpluspoJ}
\newsavebox{\CoWTfdotinvpluspoK}
\begin{lrbox}{\CoWTfdotinvpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoL}
\settowidth{\CoWTfdotinvpluspoL}{\usebox{\CoWTfdotinvpluspoK}}
\addtolength{\CoWTfdotinvpluspoH}{\CoWTfdotinvpluspoL}
\newsavebox{\CoWTfdotinvpluspoM}
\begin{lrbox}{\CoWTfdotinvpluspoM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoN}
\settowidth{\CoWTfdotinvpluspoN}{\usebox{\CoWTfdotinvpluspoM}}
\newsavebox{\CoWTfdotinvpluspoO}
\begin{lrbox}{\CoWTfdotinvpluspoO}
\begin{minipage}{\CoWTfdotinvpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvpluspoN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvpluspoM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvpluspoO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoWTf.inv+poloc-ctrl-isb.tex <==
\newlength{\CoWTfdotinvpluspolocctrlisbH}
\setlength{\CoWTfdotinvpluspolocctrlisbH}{0cm}
\newsavebox{\CoWTfdotinvpluspolocctrlisbI}
\begin{lrbox}{\CoWTfdotinvpluspolocctrlisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X4,[X1]
CBNZ X4,L0
L0:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspolocctrlisbJ}
\settowidth{\CoWTfdotinvpluspolocctrlisbJ}{\usebox{\CoWTfdotinvpluspolocctrlisbI}}
\addtolength{\CoWTfdotinvpluspolocctrlisbH}{\CoWTfdotinvpluspolocctrlisbJ}
\newsavebox{\CoWTfdotinvpluspolocctrlisbK}
\begin{lrbox}{\CoWTfdotinvpluspolocctrlisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspolocctrlisbL}
\settowidth{\CoWTfdotinvpluspolocctrlisbL}{\usebox{\CoWTfdotinvpluspolocctrlisbK}}
\addtolength{\CoWTfdotinvpluspolocctrlisbH}{\CoWTfdotinvpluspolocctrlisbL}
\newsavebox{\CoWTfdotinvpluspolocctrlisbM}
\begin{lrbox}{\CoWTfdotinvpluspolocctrlisbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *y = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspolocctrlisbN}
\settowidth{\CoWTfdotinvpluspolocctrlisbN}{\usebox{\CoWTfdotinvpluspolocctrlisbM}}
\newsavebox{\CoWTfdotinvpluspolocctrlisbO}
\begin{lrbox}{\CoWTfdotinvpluspolocctrlisbO}
\begin{minipage}{\CoWTfdotinvpluspolocctrlisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+poloc-ctrl-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvpluspolocctrlisbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvpluspolocctrlisbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvpluspolocctrlisbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspolocctrlisbI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspolocctrlisbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoWTf.inv+rfi-addr.tex <==
\newlength{\CoWTfdotinvplusrfiaddrH}
\setlength{\CoWTfdotinvplusrfiaddrH}{0cm}
\newsavebox{\CoWTfdotinvplusrfiaddrI}
\begin{lrbox}{\CoWTfdotinvplusrfiaddrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusrfiaddrJ}
\settowidth{\CoWTfdotinvplusrfiaddrJ}{\usebox{\CoWTfdotinvplusrfiaddrI}}
\addtolength{\CoWTfdotinvplusrfiaddrH}{\CoWTfdotinvplusrfiaddrJ}
\newsavebox{\CoWTfdotinvplusrfiaddrK}
\begin{lrbox}{\CoWTfdotinvplusrfiaddrK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#0
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusrfiaddrL}
\settowidth{\CoWTfdotinvplusrfiaddrL}{\usebox{\CoWTfdotinvplusrfiaddrK}}
\addtolength{\CoWTfdotinvplusrfiaddrH}{\CoWTfdotinvplusrfiaddrL}
\newsavebox{\CoWTfdotinvplusrfiaddrM}
\begin{lrbox}{\CoWTfdotinvplusrfiaddrM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusrfiaddrN}
\settowidth{\CoWTfdotinvplusrfiaddrN}{\usebox{\CoWTfdotinvplusrfiaddrM}}
\newsavebox{\CoWTfdotinvplusrfiaddrO}
\begin{lrbox}{\CoWTfdotinvplusrfiaddrO}
\begin{minipage}{\CoWTfdotinvplusrfiaddrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R5=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+rfi-addr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvplusrfiaddrN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvplusrfiaddrM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvplusrfiaddrO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplusrfiaddrI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplusrfiaddrK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=desc3(y,page_table_base) & 0:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoWTf.inv+rfi-ctrl-isb.tex <==
\newlength{\CoWTfdotinvplusrfictrlisbH}
\setlength{\CoWTfdotinvplusrfictrlisbH}{0cm}
\newsavebox{\CoWTfdotinvplusrfictrlisbI}
\begin{lrbox}{\CoWTfdotinvplusrfictrlisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
CBNZ X2,L0
L0:
ISB
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusrfictrlisbJ}
\settowidth{\CoWTfdotinvplusrfictrlisbJ}{\usebox{\CoWTfdotinvplusrfictrlisbI}}
\addtolength{\CoWTfdotinvplusrfictrlisbH}{\CoWTfdotinvplusrfictrlisbJ}
\newsavebox{\CoWTfdotinvplusrfictrlisbK}
\begin{lrbox}{\CoWTfdotinvplusrfictrlisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusrfictrlisbL}
\settowidth{\CoWTfdotinvplusrfictrlisbL}{\usebox{\CoWTfdotinvplusrfictrlisbK}}
\addtolength{\CoWTfdotinvplusrfictrlisbH}{\CoWTfdotinvplusrfictrlisbL}
\newsavebox{\CoWTfdotinvplusrfictrlisbM}
\begin{lrbox}{\CoWTfdotinvplusrfictrlisbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    *pa2 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusrfictrlisbN}
\settowidth{\CoWTfdotinvplusrfictrlisbN}{\usebox{\CoWTfdotinvplusrfictrlisbM}}
\newsavebox{\CoWTfdotinvplusrfictrlisbO}
\begin{lrbox}{\CoWTfdotinvplusrfictrlisbO}
\begin{minipage}{\CoWTfdotinvplusrfictrlisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R5=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+rfi-ctrl-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvplusrfictrlisbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvplusrfictrlisbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvplusrfictrlisbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplusrfictrlisbI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplusrfictrlisbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=desc3(u,page_table_base) & 0:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoWTf.inv+svc.tex <==
\newlength{\CoWTfdotinvplussvcH}
\setlength{\CoWTfdotinvplussvcH}{0cm}
\newsavebox{\CoWTfdotinvplussvcI}
\begin{lrbox}{\CoWTfdotinvplussvcI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
SVC #0x0
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplussvcJ}
\settowidth{\CoWTfdotinvplussvcJ}{\usebox{\CoWTfdotinvplussvcI}}
\addtolength{\CoWTfdotinvplussvcH}{\CoWTfdotinvplussvcJ}
\newsavebox{\CoWTfdotinvplussvcK}
\begin{lrbox}{\CoWTfdotinvplussvcK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1200:
MOV X2,#0
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplussvcL}
\settowidth{\CoWTfdotinvplussvcL}{\usebox{\CoWTfdotinvplussvcK}}
\addtolength{\CoWTfdotinvplussvcH}{\CoWTfdotinvplussvcL}
\newsavebox{\CoWTfdotinvplussvcM}
\begin{lrbox}{\CoWTfdotinvplussvcM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS X10,ELR_EL1
LDR X2,[X3]
MSR ELR_EL1,X10
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplussvcN}
\settowidth{\CoWTfdotinvplussvcN}{\usebox{\CoWTfdotinvplussvcM}}
\addtolength{\CoWTfdotinvplussvcH}{\CoWTfdotinvplussvcN}
\newsavebox{\CoWTfdotinvplussvcO}
\begin{lrbox}{\CoWTfdotinvplussvcO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *y = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplussvcP}
\settowidth{\CoWTfdotinvplussvcP}{\usebox{\CoWTfdotinvplussvcO}}
\newsavebox{\CoWTfdotinvplussvcA}
\begin{lrbox}{\CoWTfdotinvplussvcA}
\begin{minipage}{\CoWTfdotinvplussvcH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+svc|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvplussvcP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvplussvcO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvplussvcA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplussvcI}\\
  \cline{2-2}
  & thread0 el1 handler same exc\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplussvcK}\\
  \cline{2-2}
  & thread0 el1 handler lower exc\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplussvcM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoWTf.inv.EL1+dsb-eret.tex <==
\newlength{\CoWTfdotinvdotELoneplusdsberetH}
\setlength{\CoWTfdotinvdotELoneplusdsberetH}{0cm}
\newsavebox{\CoWTfdotinvdotELoneplusdsberetI}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELoneplusdsberetJ}
\settowidth{\CoWTfdotinvdotELoneplusdsberetJ}{\usebox{\CoWTfdotinvdotELoneplusdsberetI}}
\addtolength{\CoWTfdotinvdotELoneplusdsberetH}{\CoWTfdotinvdotELoneplusdsberetJ}
\newsavebox{\CoWTfdotinvdotELoneplusdsberetK}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELoneplusdsberetL}
\settowidth{\CoWTfdotinvdotELoneplusdsberetL}{\usebox{\CoWTfdotinvdotELoneplusdsberetK}}
\addtolength{\CoWTfdotinvdotELoneplusdsberetH}{\CoWTfdotinvdotELoneplusdsberetL}
\newsavebox{\CoWTfdotinvdotELoneplusdsberetM}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *y = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELoneplusdsberetN}
\settowidth{\CoWTfdotinvdotELoneplusdsberetN}{\usebox{\CoWTfdotinvdotELoneplusdsberetM}}
\newsavebox{\CoWTfdotinvdotELoneplusdsberetO}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsberetO}
\begin{minipage}{\CoWTfdotinvdotELoneplusdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL1=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL1=0b00000|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv.EL1+dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvdotELoneplusdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvdotELoneplusdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvdotELoneplusdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELoneplusdsberetI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELoneplusdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoWTf.inv.EL1+dsb-svc.tex <==
\newlength{\CoWTfdotinvdotELoneplusdsbsvcH}
\setlength{\CoWTfdotinvdotELoneplusdsbsvcH}{0cm}
\newsavebox{\CoWTfdotinvdotELoneplusdsbsvcI}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsbsvcI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
SVC #0x0
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELoneplusdsbsvcJ}
\settowidth{\CoWTfdotinvdotELoneplusdsbsvcJ}{\usebox{\CoWTfdotinvdotELoneplusdsbsvcI}}
\addtolength{\CoWTfdotinvdotELoneplusdsbsvcH}{\CoWTfdotinvdotELoneplusdsbsvcJ}
\newsavebox{\CoWTfdotinvdotELoneplusdsbsvcK}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsbsvcK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1200:
MOV X2,#0
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELoneplusdsbsvcL}
\settowidth{\CoWTfdotinvdotELoneplusdsbsvcL}{\usebox{\CoWTfdotinvdotELoneplusdsbsvcK}}
\addtolength{\CoWTfdotinvdotELoneplusdsbsvcH}{\CoWTfdotinvdotELoneplusdsbsvcL}
\newsavebox{\CoWTfdotinvdotELoneplusdsbsvcM}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsbsvcM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS X10,ELR_EL1
LDR X2,[X3]
MSR ELR_EL1,X10
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELoneplusdsbsvcN}
\settowidth{\CoWTfdotinvdotELoneplusdsbsvcN}{\usebox{\CoWTfdotinvdotELoneplusdsbsvcM}}
\addtolength{\CoWTfdotinvdotELoneplusdsbsvcH}{\CoWTfdotinvdotELoneplusdsbsvcN}
\newsavebox{\CoWTfdotinvdotELoneplusdsbsvcO}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsbsvcO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *y = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELoneplusdsbsvcP}
\settowidth{\CoWTfdotinvdotELoneplusdsbsvcP}{\usebox{\CoWTfdotinvdotELoneplusdsbsvcO}}
\newsavebox{\CoWTfdotinvdotELoneplusdsbsvcA}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsbsvcA}
\begin{minipage}{\CoWTfdotinvdotELoneplusdsbsvcH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv.EL1+dsb-svc|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvdotELoneplusdsbsvcP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvdotELoneplusdsbsvcO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvdotELoneplusdsbsvcA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELoneplusdsbsvcI}\\
  \cline{2-2}
  & thread0 el1 handler same exc\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELoneplusdsbsvcK}\\
  \cline{2-2}
  & thread0 el1 handler lower exc\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELoneplusdsbsvcM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoWTf.inv.EL1+eret.tex <==
\newlength{\CoWTfdotinvdotELonepluseretH}
\setlength{\CoWTfdotinvdotELonepluseretH}{0cm}
\newsavebox{\CoWTfdotinvdotELonepluseretI}
\begin{lrbox}{\CoWTfdotinvdotELonepluseretI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELonepluseretJ}
\settowidth{\CoWTfdotinvdotELonepluseretJ}{\usebox{\CoWTfdotinvdotELonepluseretI}}
\addtolength{\CoWTfdotinvdotELonepluseretH}{\CoWTfdotinvdotELonepluseretJ}
\newsavebox{\CoWTfdotinvdotELonepluseretK}
\begin{lrbox}{\CoWTfdotinvdotELonepluseretK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELonepluseretL}
\settowidth{\CoWTfdotinvdotELonepluseretL}{\usebox{\CoWTfdotinvdotELonepluseretK}}
\addtolength{\CoWTfdotinvdotELonepluseretH}{\CoWTfdotinvdotELonepluseretL}
\newsavebox{\CoWTfdotinvdotELonepluseretM}
\begin{lrbox}{\CoWTfdotinvdotELonepluseretM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *y = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELonepluseretN}
\settowidth{\CoWTfdotinvdotELonepluseretN}{\usebox{\CoWTfdotinvdotELonepluseretM}}
\newsavebox{\CoWTfdotinvdotELonepluseretO}
\begin{lrbox}{\CoWTfdotinvdotELonepluseretO}
\begin{minipage}{\CoWTfdotinvdotELonepluseretH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL1=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL1=0b00000|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv.EL1+eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvdotELonepluseretN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvdotELonepluseretM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvdotELonepluseretO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELonepluseretI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELonepluseretK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoWTf.inv.EL2+dsb-tlbiipa-dsb-tlbiis-dsb-eret.tex <==
\newlength{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetH}
\setlength{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetH}{0cm}
\newsavebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetI}
\begin{lrbox}{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1,X4
DSB SY
TLBI VMALLE1IS
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetJ}
\settowidth{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetJ}{\usebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetI}}
\addtolength{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetH}{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetJ}
\newsavebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetK}
\begin{lrbox}{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X20,ELR_EL2
ADD X20,X20,#4
MSR ELR_EL2,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetL}
\settowidth{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetL}{\usebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetK}}
\addtolength{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetH}{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetL}
\newsavebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetM}
\begin{lrbox}{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;

    ipa1 |-> invalid;
    ipa1 ?-> pa1;

    *pa1 = 1;

    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetN}
\settowidth{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetN}{\usebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetM}}
\newsavebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetO}
\begin{lrbox}{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetO}
\begin{minipage}{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00100|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv.EL2+dsb-tlbiipa-dsb-tlbiis-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetI}\\
  \cline{2-2}
  & thread0 el2 handler lower exc\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoWTf.inv.EL2+po.tex <==
\newlength{\CoWTfdotinvdotELtwopluspoH}
\setlength{\CoWTfdotinvdotELtwopluspoH}{0cm}
\newsavebox{\CoWTfdotinvdotELtwopluspoI}
\begin{lrbox}{\CoWTfdotinvdotELtwopluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELtwopluspoJ}
\settowidth{\CoWTfdotinvdotELtwopluspoJ}{\usebox{\CoWTfdotinvdotELtwopluspoI}}
\addtolength{\CoWTfdotinvdotELtwopluspoH}{\CoWTfdotinvdotELtwopluspoJ}
\newsavebox{\CoWTfdotinvdotELtwopluspoK}
\begin{lrbox}{\CoWTfdotinvdotELtwopluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X20,ELR_EL2
ADD X20,X20,#4
MSR ELR_EL2,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELtwopluspoL}
\settowidth{\CoWTfdotinvdotELtwopluspoL}{\usebox{\CoWTfdotinvdotELtwopluspoK}}
\addtolength{\CoWTfdotinvdotELtwopluspoH}{\CoWTfdotinvdotELtwopluspoL}
\newsavebox{\CoWTfdotinvdotELtwopluspoM}
\begin{lrbox}{\CoWTfdotinvdotELtwopluspoM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;

    ipa1 |-> invalid;
    ipa1 ?-> pa1;

    *pa1 = 1;

    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELtwopluspoN}
\settowidth{\CoWTfdotinvdotELtwopluspoN}{\usebox{\CoWTfdotinvdotELtwopluspoM}}
\newsavebox{\CoWTfdotinvdotELtwopluspoO}
\begin{lrbox}{\CoWTfdotinvdotELtwopluspoO}
\begin{minipage}{\CoWTfdotinvdotELtwopluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00100|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv.EL2+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvdotELtwopluspoN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvdotELtwopluspoM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvdotELtwopluspoO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELtwopluspoI}\\
  \cline{2-2}
  & thread0 el2 handler lower exc\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELtwopluspoK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoWTv2.2.inv+dsb-tlbivmidis-dsb-eret.tex <==
\newlength{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetH}
\setlength{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetH}{0cm}
\newsavebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetI}
\begin{lrbox}{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VMALLS12E1IS
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetJ}
\settowidth{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetJ}{\usebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetI}}
\addtolength{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetH}{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetJ}
\newsavebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetK}
\begin{lrbox}{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetL}
\settowidth{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetL}{\usebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetK}}
\addtolength{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetH}{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetL}
\newsavebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetM}
\begin{lrbox}{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;
    ipa1 |-> invalid;
    ipa1 ?-> pa1;

    *pa1 = 1;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetN}
\settowidth{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetN}{\usebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetM}}
\newsavebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetO}
\begin{lrbox}{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetO}
\begin{minipage}{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00101|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTv2.2.inv+dsb-tlbivmidis-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetI}\\
  \cline{2-2}
  & thread0 el2 handler\\
  \cline{2-2}
  & \usebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoWW.alias.tex <==
\newlength{\CoWWdotaliasH}
\setlength{\CoWWdotaliasH}{0cm}
\newsavebox{\CoWWdotaliasI}
\begin{lrbox}{\CoWWdotaliasI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWWdotaliasJ}
\settowidth{\CoWWdotaliasJ}{\usebox{\CoWWdotaliasI}}
\addtolength{\CoWWdotaliasH}{\CoWWdotaliasJ}
\newsavebox{\CoWWdotaliasK}
\begin{lrbox}{\CoWWdotaliasK}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    y |-> pa1;
    *pa1 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWWdotaliasL}
\settowidth{\CoWWdotaliasL}{\usebox{\CoWWdotaliasK}}
\newsavebox{\CoWWdotaliasM}
\begin{lrbox}{\CoWWdotaliasM}
\begin{minipage}{\CoWWdotaliasH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=0b01|\\
\lstinline[language=IslaLitmusExp]|R1=x|\\
\lstinline[language=IslaLitmusExp]|R2=0b10|\\
\lstinline[language=IslaLitmusExp]|R3=y|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWW.alias|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWWdotaliasL}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWWdotaliasK}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWWdotaliasM}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWWdotaliasI}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|x=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoWinvRpte+po.tex <==
\newlength{\CoWinvRptepluspoH}
\setlength{\CoWinvRptepluspoH}{0cm}
\newsavebox{\CoWinvRptepluspoI}
\begin{lrbox}{\CoWinvRptepluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvRptepluspoJ}
\settowidth{\CoWinvRptepluspoJ}{\usebox{\CoWinvRptepluspoI}}
\addtolength{\CoWinvRptepluspoH}{\CoWinvRptepluspoJ}
\newsavebox{\CoWinvRptepluspoK}
\begin{lrbox}{\CoWinvRptepluspoK}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;

    *pa1 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvRptepluspoL}
\settowidth{\CoWinvRptepluspoL}{\usebox{\CoWinvRptepluspoK}}
\newsavebox{\CoWinvRptepluspoM}
\begin{lrbox}{\CoWinvRptepluspoM}
\begin{minipage}{\CoWinvRptepluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=0x0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvRpte+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvRptepluspoL}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvRptepluspoK}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvRptepluspoM}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvRptepluspoI}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|~0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoWinvT+dsb-isb.tex <==
\newlength{\CoWinvTplusdsbisbH}
\setlength{\CoWinvTplusdsbisbH}{0cm}
\newsavebox{\CoWinvTplusdsbisbI}
\begin{lrbox}{\CoWinvTplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTplusdsbisbJ}
\settowidth{\CoWinvTplusdsbisbJ}{\usebox{\CoWinvTplusdsbisbI}}
\addtolength{\CoWinvTplusdsbisbH}{\CoWinvTplusdsbisbJ}
\newsavebox{\CoWinvTplusdsbisbK}
\begin{lrbox}{\CoWinvTplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTplusdsbisbL}
\settowidth{\CoWinvTplusdsbisbL}{\usebox{\CoWinvTplusdsbisbK}}
\addtolength{\CoWinvTplusdsbisbH}{\CoWinvTplusdsbisbL}
\newsavebox{\CoWinvTplusdsbisbM}
\begin{lrbox}{\CoWinvTplusdsbisbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTplusdsbisbN}
\settowidth{\CoWinvTplusdsbisbN}{\usebox{\CoWinvTplusdsbisbM}}
\newsavebox{\CoWinvTplusdsbisbO}
\begin{lrbox}{\CoWinvTplusdsbisbO}
\begin{minipage}{\CoWinvTplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvT+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTplusdsbisbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTplusdsbisbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTplusdsbisbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTplusdsbisbI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTplusdsbisbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoWinvT+po.tex <==
\newlength{\CoWinvTpluspoH}
\setlength{\CoWinvTpluspoH}{0cm}
\newsavebox{\CoWinvTpluspoI}
\begin{lrbox}{\CoWinvTpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTpluspoJ}
\settowidth{\CoWinvTpluspoJ}{\usebox{\CoWinvTpluspoI}}
\addtolength{\CoWinvTpluspoH}{\CoWinvTpluspoJ}
\newsavebox{\CoWinvTpluspoK}
\begin{lrbox}{\CoWinvTpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTpluspoL}
\settowidth{\CoWinvTpluspoL}{\usebox{\CoWinvTpluspoK}}
\addtolength{\CoWinvTpluspoH}{\CoWinvTpluspoL}
\newsavebox{\CoWinvTpluspoM}
\begin{lrbox}{\CoWinvTpluspoM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTpluspoN}
\settowidth{\CoWinvTpluspoN}{\usebox{\CoWinvTpluspoM}}
\newsavebox{\CoWinvTpluspoO}
\begin{lrbox}{\CoWinvTpluspoO}
\begin{minipage}{\CoWinvTpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvT+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTpluspoN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTpluspoM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTpluspoO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTpluspoI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTpluspoK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoWinvT.EL1+dsb-tlbi-dsb-isb.tex <==
\newlength{\CoWinvTdotELoneplusdsbtlbidsbisbH}
\setlength{\CoWinvTdotELoneplusdsbtlbidsbisbH}{0cm}
\newsavebox{\CoWinvTdotELoneplusdsbtlbidsbisbI}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbidsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1,X5
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbidsbisbJ}
\settowidth{\CoWinvTdotELoneplusdsbtlbidsbisbJ}{\usebox{\CoWinvTdotELoneplusdsbtlbidsbisbI}}
\addtolength{\CoWinvTdotELoneplusdsbtlbidsbisbH}{\CoWinvTdotELoneplusdsbtlbidsbisbJ}
\newsavebox{\CoWinvTdotELoneplusdsbtlbidsbisbK}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbidsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1000:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbidsbisbL}
\settowidth{\CoWinvTdotELoneplusdsbtlbidsbisbL}{\usebox{\CoWinvTdotELoneplusdsbtlbidsbisbK}}
\addtolength{\CoWinvTdotELoneplusdsbtlbidsbisbH}{\CoWinvTdotELoneplusdsbtlbidsbisbL}
\newsavebox{\CoWinvTdotELoneplusdsbtlbidsbisbM}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbidsbisbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbidsbisbN}
\settowidth{\CoWinvTdotELoneplusdsbtlbidsbisbN}{\usebox{\CoWinvTdotELoneplusdsbtlbidsbisbM}}
\newsavebox{\CoWinvTdotELoneplusdsbtlbidsbisbO}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbidsbisbO}
\begin{minipage}{\CoWinvTdotELoneplusdsbtlbidsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R5=page(x)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvT.EL1+dsb-tlbi-dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTdotELoneplusdsbtlbidsbisbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTdotELoneplusdsbtlbidsbisbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTdotELoneplusdsbtlbidsbisbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTdotELoneplusdsbtlbidsbisbI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTdotELoneplusdsbtlbidsbisbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoWinvT.EL1+dsb-tlbi-dsb.tex <==
\newlength{\CoWinvTdotELoneplusdsbtlbidsbH}
\setlength{\CoWinvTdotELoneplusdsbtlbidsbH}{0cm}
\newsavebox{\CoWinvTdotELoneplusdsbtlbidsbI}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbidsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1,X5
DSB SY
MOV X2,#0
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbidsbJ}
\settowidth{\CoWinvTdotELoneplusdsbtlbidsbJ}{\usebox{\CoWinvTdotELoneplusdsbtlbidsbI}}
\addtolength{\CoWinvTdotELoneplusdsbtlbidsbH}{\CoWinvTdotELoneplusdsbtlbidsbJ}
\newsavebox{\CoWinvTdotELoneplusdsbtlbidsbK}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbidsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1000:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbidsbL}
\settowidth{\CoWinvTdotELoneplusdsbtlbidsbL}{\usebox{\CoWinvTdotELoneplusdsbtlbidsbK}}
\addtolength{\CoWinvTdotELoneplusdsbtlbidsbH}{\CoWinvTdotELoneplusdsbtlbidsbL}
\newsavebox{\CoWinvTdotELoneplusdsbtlbidsbM}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbidsbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbidsbN}
\settowidth{\CoWinvTdotELoneplusdsbtlbidsbN}{\usebox{\CoWinvTdotELoneplusdsbtlbidsbM}}
\newsavebox{\CoWinvTdotELoneplusdsbtlbidsbO}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbidsbO}
\begin{minipage}{\CoWinvTdotELoneplusdsbtlbidsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R5=page(x)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvT.EL1+dsb-tlbi-dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTdotELoneplusdsbtlbidsbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTdotELoneplusdsbtlbidsbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTdotELoneplusdsbtlbidsbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTdotELoneplusdsbtlbidsbI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTdotELoneplusdsbtlbidsbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoWinvT.EL1+dsb-tlbiis-dsb-isb.tex <==
\newlength{\CoWinvTdotELoneplusdsbtlbiisdsbisbH}
\setlength{\CoWinvTdotELoneplusdsbtlbiisdsbisbH}{0cm}
\newsavebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbI}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbiisdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X5
DSB SY
ISB
MOV X2,#0
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbiisdsbisbJ}
\settowidth{\CoWinvTdotELoneplusdsbtlbiisdsbisbJ}{\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbI}}
\addtolength{\CoWinvTdotELoneplusdsbtlbiisdsbisbH}{\CoWinvTdotELoneplusdsbtlbiisdsbisbJ}
\newsavebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbK}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbiisdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1000:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbiisdsbisbL}
\settowidth{\CoWinvTdotELoneplusdsbtlbiisdsbisbL}{\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbK}}
\addtolength{\CoWinvTdotELoneplusdsbtlbiisdsbisbH}{\CoWinvTdotELoneplusdsbtlbiisdsbisbL}
\newsavebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbM}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbiisdsbisbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbiisdsbisbN}
\settowidth{\CoWinvTdotELoneplusdsbtlbiisdsbisbN}{\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbM}}
\newsavebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbO}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbiisdsbisbO}
\begin{minipage}{\CoWinvTdotELoneplusdsbtlbiisdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R5=page(x)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvT.EL1+dsb-tlbiis-dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTdotELoneplusdsbtlbiisdsbisbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoWinvT.EL1+dsb-tlbiis-dsb.tex <==
\newlength{\CoWinvTdotELoneplusdsbtlbiisdsbH}
\setlength{\CoWinvTdotELoneplusdsbtlbiisdsbH}{0cm}
\newsavebox{\CoWinvTdotELoneplusdsbtlbiisdsbI}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbiisdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X5
DSB SY
MOV X2,#0
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbiisdsbJ}
\settowidth{\CoWinvTdotELoneplusdsbtlbiisdsbJ}{\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbI}}
\addtolength{\CoWinvTdotELoneplusdsbtlbiisdsbH}{\CoWinvTdotELoneplusdsbtlbiisdsbJ}
\newsavebox{\CoWinvTdotELoneplusdsbtlbiisdsbK}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbiisdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1000:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbiisdsbL}
\settowidth{\CoWinvTdotELoneplusdsbtlbiisdsbL}{\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbK}}
\addtolength{\CoWinvTdotELoneplusdsbtlbiisdsbH}{\CoWinvTdotELoneplusdsbtlbiisdsbL}
\newsavebox{\CoWinvTdotELoneplusdsbtlbiisdsbM}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbiisdsbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbiisdsbN}
\settowidth{\CoWinvTdotELoneplusdsbtlbiisdsbN}{\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbM}}
\newsavebox{\CoWinvTdotELoneplusdsbtlbiisdsbO}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbiisdsbO}
\begin{minipage}{\CoWinvTdotELoneplusdsbtlbiisdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R5=page(x)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvT.EL1+dsb-tlbiis-dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTdotELoneplusdsbtlbiisdsbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTdotELoneplusdsbtlbiisdsbI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTdotELoneplusdsbtlbiisdsbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoWinvT2+dsb-tlbiipa-dsb-eret.tex <==
\newlength{\CoWinvTtwoplusdsbtlbiipadsberetH}
\setlength{\CoWinvTtwoplusdsbtlbiipadsberetH}{0cm}
\newsavebox{\CoWinvTtwoplusdsbtlbiipadsberetI}
\begin{lrbox}{\CoWinvTtwoplusdsbtlbiipadsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1,X4
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTtwoplusdsbtlbiipadsberetJ}
\settowidth{\CoWinvTtwoplusdsbtlbiipadsberetJ}{\usebox{\CoWinvTtwoplusdsbtlbiipadsberetI}}
\addtolength{\CoWinvTtwoplusdsbtlbiipadsberetH}{\CoWinvTtwoplusdsbtlbiipadsberetJ}
\newsavebox{\CoWinvTtwoplusdsbtlbiipadsberetK}
\begin{lrbox}{\CoWinvTtwoplusdsbtlbiipadsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X20,ELR_EL2
ADD X20,X20,#4
MSR ELR_EL2,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTtwoplusdsbtlbiipadsberetL}
\settowidth{\CoWinvTtwoplusdsbtlbiipadsberetL}{\usebox{\CoWinvTtwoplusdsbtlbiipadsberetK}}
\addtolength{\CoWinvTtwoplusdsbtlbiipadsberetH}{\CoWinvTtwoplusdsbtlbiipadsberetL}
\newsavebox{\CoWinvTtwoplusdsbtlbiipadsberetM}
\begin{lrbox}{\CoWinvTtwoplusdsbtlbiipadsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;

    ipa1 |-> invalid;
    ipa1 ?-> pa1;

    *pa1 = 1;

    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTtwoplusdsbtlbiipadsberetN}
\settowidth{\CoWinvTtwoplusdsbtlbiipadsberetN}{\usebox{\CoWinvTtwoplusdsbtlbiipadsberetM}}
\newsavebox{\CoWinvTtwoplusdsbtlbiipadsberetO}
\begin{lrbox}{\CoWinvTtwoplusdsbtlbiipadsberetO}
\begin{minipage}{\CoWinvTtwoplusdsbtlbiipadsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=page(ipa1)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00100|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvT2+dsb-tlbiipa-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTtwoplusdsbtlbiipadsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTtwoplusdsbtlbiipadsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTtwoplusdsbtlbiipadsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTtwoplusdsbtlbiipadsberetI}\\
  \cline{2-2}
  & thread0 el2 handler lower exc\\
  \cline{2-2}
  & \usebox{\CoWinvTtwoplusdsbtlbiipadsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoWinvT2+dsb-tlbiipa-dsb-tlbivmall-dsb-eret.tex <==
\newlength{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetH}
\setlength{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetH}{0cm}
\newsavebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetI}
\begin{lrbox}{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1,X4
DSB SY
TLBI VMALLE1
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetJ}
\settowidth{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetJ}{\usebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetI}}
\addtolength{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetH}{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetJ}
\newsavebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetK}
\begin{lrbox}{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#1
MRS X20,ELR_EL2
ADD X20,X20,#4
MSR ELR_EL2,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetL}
\settowidth{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetL}{\usebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetK}}
\addtolength{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetH}{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetL}
\newsavebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetM}
\begin{lrbox}{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;

    ipa1 |-> pa1;
    ipa1 ?-> invalid;

    *pa1 = 0;

    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetN}
\settowidth{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetN}{\usebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetM}}
\newsavebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetO}
\begin{lrbox}{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetO}
\begin{minipage}{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=page(ipa1)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00100|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvT2+dsb-tlbiipa-dsb-tlbivmall-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetI}\\
  \cline{2-2}
  & thread0 el2 handler lower exc\\
  \cline{2-2}
  & \usebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoWinvTa1.1+dsb-tlbiasidis-dsb-eret.tex <==
\newlength{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetH}
\setlength{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetH}{0cm}
\newsavebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetI}
\begin{lrbox}{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI ASIDE1IS,X4
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetJ}
\settowidth{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetJ}{\usebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetI}}
\addtolength{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetH}{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetJ}
\newsavebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetK}
\begin{lrbox}{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetL}
\settowidth{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetL}{\usebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetK}}
\addtolength{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetH}{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetL}
\newsavebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetM}
\begin{lrbox}{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetN}
\settowidth{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetN}{\usebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetM}}
\newsavebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetO}
\begin{lrbox}{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetO}
\begin{minipage}{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL1=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=asid(0x1)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL1=0b00000|\\
\lstinline[language=IslaLitmusExp]|TTBR0_EL1=ttbr(asid=0x0001,base=page_table_base)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvTa1.1+dsb-tlbiasidis-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoWinvTa2.1+dsb-tlbiasidis-dsb-eret.tex <==
\newlength{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetH}
\setlength{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetH}{0cm}
\newsavebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetI}
\begin{lrbox}{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI ASIDE1IS,X4
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetJ}
\settowidth{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetJ}{\usebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetI}}
\addtolength{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetH}{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetJ}
\newsavebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetK}
\begin{lrbox}{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetL}
\settowidth{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetL}{\usebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetK}}
\addtolength{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetH}{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetL}
\newsavebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetM}
\begin{lrbox}{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetN}
\settowidth{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetN}{\usebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetM}}
\newsavebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetO}
\begin{lrbox}{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetO}
\begin{minipage}{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL1=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=asid(0x2)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL1=0b00000|\\
\lstinline[language=IslaLitmusExp]|TTBR0_EL1=ttbr(base=page_table_base,asid=0x0001)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvTa2.1+dsb-tlbiasidis-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoWinvTv1.2+dsb-tlbivmidis-dsb-eret.tex <==
\newlength{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetH}
\setlength{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetH}{0cm}
\newsavebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetI}
\begin{lrbox}{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VMALLS12E1IS
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetJ}
\settowidth{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetJ}{\usebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetI}}
\addtolength{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetH}{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetJ}
\newsavebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetK}
\begin{lrbox}{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#1
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetL}
\settowidth{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetL}{\usebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetK}}
\addtolength{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetH}{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetL}
\newsavebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetM}
\begin{lrbox}{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;
    ipa1 |-> pa1;
    ipa1 ?-> invalid;

    *pa1 = 0;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetN}
\settowidth{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetN}{\usebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetM}}
\newsavebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetO}
\begin{lrbox}{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetO}
\begin{minipage}{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00101|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvTv1.2+dsb-tlbivmidis-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetI}\\
  \cline{2-2}
  & thread0 el2 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/CoWinvTv2.2+dsb-tlbivmidis-msrvttbr-dsb-eret.tex <==
\newlength{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetH}
\setlength{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetH}{0cm}
\newsavebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetI}
\begin{lrbox}{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VMALLS12E1IS
DSB SY
MSR VTTBR_EL2,X4
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetJ}
\settowidth{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetJ}{\usebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetI}}
\addtolength{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetH}{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetJ}
\newsavebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetK}
\begin{lrbox}{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#1
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetL}
\settowidth{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetL}{\usebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetK}}
\addtolength{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetH}{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetL}
\newsavebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetM}
\begin{lrbox}{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;
    ipa1 |-> pa1;
    ipa1 ?-> invalid;

    *pa1 = 0;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetN}
\settowidth{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetN}{\usebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetM}}
\newsavebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetO}
\begin{lrbox}{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetO}
\begin{minipage}{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=ttbr(base=s2_page_table_base,vmid=0x0001)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00101|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvTv2.2+dsb-tlbivmidis-msrvttbr-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetI}\\
  \cline{2-2}
  & thread0 el2 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/ETS.tex <==
\newlength{\ETSH}
\setlength{\ETSH}{0cm}
\newsavebox{\ETSI}
\begin{lrbox}{\ETSI}
\begin{lstlisting}[language=AArch64,showlines=true]
MOV X0,#1
STR X0,[X3]
DMB SY
STR X0,[X2]
\end{lstlisting}
\end{lrbox}
\newlength{\ETSJ}
\settowidth{\ETSJ}{\usebox{\ETSI}}
\addtolength{\ETSH}{\ETSJ}
\newsavebox{\ETSK}
\begin{lrbox}{\ETSK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X2]
STR X0,[X1]
MOV X4,#2
STR X4,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\ETSL}
\settowidth{\ETSL}{\usebox{\ETSK}}
\addtolength{\ETSH}{\ETSL}
\newsavebox{\ETSM}
\begin{lrbox}{\ETSM}
\begin{lstlisting}[language=AArch64,showlines=true]
MOV X0,#0
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\ETSN}
\settowidth{\ETSN}{\usebox{\ETSM}}
\addtolength{\ETSH}{\ETSN}
\newsavebox{\ETSO}
\begin{lrbox}{\ETSO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
LDR X7,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\ETSP}
\settowidth{\ETSP}{\usebox{\ETSO}}
\addtolength{\ETSH}{\ETSP}
\newsavebox{\ETSA}
\begin{lrbox}{\ETSA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> pa1;
    x ?-> invalid;
    y |-> pa2;
    z |-> pa3;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\ETSB}
\settowidth{\ETSB}{\usebox{\ETSA}}
\newsavebox{\ETSC}
\begin{lrbox}{\ETSC}
\begin{minipage}{\ETSH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R2=y|\\
\lstinline[language=IslaLitmusExp]|0:R3=z|\\
\lstinline[language=IslaLitmusExp]|1:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=z|\\
\lstinline[language=IslaLitmusExp]|1:R6=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R7=0b1|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:R1=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|ETS|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\ETSB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\ETSA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\ETSC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\ETSI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\ETSK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\ETSM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\ETSO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & x=1 & 1:R7=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/IRIW.TTf.TTf.inv+addrs.tex <==
\newlength{\IRIWdotTTfdotTTfdotinvplusaddrsH}
\setlength{\IRIWdotTTfdotTTfdotinvplusaddrsH}{0cm}
\newsavebox{\IRIWdotTTfdotTTfdotinvplusaddrsI}
\begin{lrbox}{\IRIWdotTTfdotTTfdotinvplusaddrsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\IRIWdotTTfdotTTfdotinvplusaddrsJ}
\settowidth{\IRIWdotTTfdotTTfdotinvplusaddrsJ}{\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsI}}
\addtolength{\IRIWdotTTfdotTTfdotinvplusaddrsH}{\IRIWdotTTfdotTTfdotinvplusaddrsJ}
\newsavebox{\IRIWdotTTfdotTTfdotinvplusaddrsK}
\begin{lrbox}{\IRIWdotTTfdotTTfdotinvplusaddrsK}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\IRIWdotTTfdotTTfdotinvplusaddrsL}
\settowidth{\IRIWdotTTfdotTTfdotinvplusaddrsL}{\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsK}}
\addtolength{\IRIWdotTTfdotTTfdotinvplusaddrsH}{\IRIWdotTTfdotTTfdotinvplusaddrsL}
\newsavebox{\IRIWdotTTfdotTTfdotinvplusaddrsM}
\begin{lrbox}{\IRIWdotTTfdotTTfdotinvplusaddrsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\IRIWdotTTfdotTTfdotinvplusaddrsN}
\settowidth{\IRIWdotTTfdotTTfdotinvplusaddrsN}{\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsM}}
\addtolength{\IRIWdotTTfdotTTfdotinvplusaddrsH}{\IRIWdotTTfdotTTfdotinvplusaddrsN}
\newsavebox{\IRIWdotTTfdotTTfdotinvplusaddrsO}
\begin{lrbox}{\IRIWdotTTfdotTTfdotinvplusaddrsO}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\IRIWdotTTfdotTTfdotinvplusaddrsP}
\settowidth{\IRIWdotTTfdotTTfdotinvplusaddrsP}{\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsO}}
\addtolength{\IRIWdotTTfdotTTfdotinvplusaddrsH}{\IRIWdotTTfdotTTfdotinvplusaddrsP}
\newsavebox{\IRIWdotTTfdotTTfdotinvplusaddrsA}
\begin{lrbox}{\IRIWdotTTfdotTTfdotinvplusaddrsA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\IRIWdotTTfdotTTfdotinvplusaddrsB}
\settowidth{\IRIWdotTTfdotTTfdotinvplusaddrsB}{\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsA}}
\addtolength{\IRIWdotTTfdotTTfdotinvplusaddrsH}{\IRIWdotTTfdotTTfdotinvplusaddrsB}
\newsavebox{\IRIWdotTTfdotTTfdotinvplusaddrsC}
\begin{lrbox}{\IRIWdotTTfdotTTfdotinvplusaddrsC}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\IRIWdotTTfdotTTfdotinvplusaddrsD}
\settowidth{\IRIWdotTTfdotTTfdotinvplusaddrsD}{\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsC}}
\addtolength{\IRIWdotTTfdotTTfdotinvplusaddrsH}{\IRIWdotTTfdotTTfdotinvplusaddrsD}
\newsavebox{\IRIWdotTTfdotTTfdotinvplusaddrsE}
\begin{lrbox}{\IRIWdotTTfdotTTfdotinvplusaddrsE}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> invalid;
    y ?-> pa2;
    v |-> pa2;
    *pa2 = 1;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\IRIWdotTTfdotTTfdotinvplusaddrsF}
\settowidth{\IRIWdotTTfdotTTfdotinvplusaddrsF}{\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsE}}
\newsavebox{\IRIWdotTTfdotTTfdotinvplusaddrsHG}
\begin{lrbox}{\IRIWdotTTfdotTTfdotinvplusaddrsHG}
\begin{minipage}{\IRIWdotTTfdotTTfdotinvplusaddrsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R0=desc3(v,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=x|\\
\lstinline[language=IslaLitmusExp]|2:R3=y|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|3:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|3:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|3:R1=y|\\
\lstinline[language=IslaLitmusExp]|3:R3=x|\\
\lstinline[language=IslaLitmusExp]|3:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|IRIW.TTf.TTf.inv+addrs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\IRIWdotTTfdotTTfdotinvplusaddrsF}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsE}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsHG}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\IRIWdotTTfdotTTfdotinvplusaddrsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\IRIWdotTTfdotTTfdotinvplusaddrsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\IRIWdotTTfdotTTfdotinvplusaddrsM}\\
  \cline{2-2}
  & Thread 3\\
  \cline{2-2}
  & \usebox{\IRIWdotTTfdotTTfdotinvplusaddrsO}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\IRIWdotTTfdotTTfdotinvplusaddrsA}\\
  \cline{2-2}
  & thread3 el1 handler\\
  \cline{2-2}
  & \usebox{\IRIWdotTTfdotTTfdotinvplusaddrsC}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|2:R0=1 & 2:R2=0 & 3:R0=1 & 3:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/ISA2.RRTf.inv+dsb+addr+addr.tex <==
\newlength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrH}
\setlength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrH}{0cm}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrI}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrJ}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrJ}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrI}}
\addtolength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrH}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrJ}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrK}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
STR X3,[X4,X2]
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrL}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrL}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrK}}
\addtolength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrH}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrL}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrM}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
LDR X3,[X4,X2]
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrN}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrN}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrM}}
\addtolength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrH}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrN}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrO}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X3,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrP}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrP}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrO}}
\addtolength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrH}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrP}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrA}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    *pa2 = 0;

    z |-> pa3;
    *pa3 = 0;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrB}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrB}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrA}}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrC}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrC}
\begin{minipage}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R4=z|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=z|\\
\lstinline[language=IslaLitmusExp]|2:R4=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|ISA2.RRTf.inv+dsb+addr+addr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrM}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R3=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/ISA2.RRTf.inv+dsb+data+addr.tex <==
\newlength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrH}
\setlength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrH}{0cm}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrI}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrJ}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrJ}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrI}}
\addtolength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrH}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrJ}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrK}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
ORR X3,X3,X2
STR X3,[X4]
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrL}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrL}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrK}}
\addtolength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrH}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrL}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrM}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
LDR X3,[X4,X2]
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrN}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrN}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrM}}
\addtolength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrH}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrN}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrO}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X3,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrP}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrP}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrO}}
\addtolength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrH}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrP}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrA}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    *pa2 = 0;

    z |-> pa3;
    *pa3 = 0;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrB}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrB}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrA}}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrC}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrC}
\begin{minipage}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R4=z|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=z|\\
\lstinline[language=IslaLitmusExp]|2:R4=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|ISA2.RRTf.inv+dsb+data+addr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrM}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R3=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/LB+addr-trfis.tex <==
\newlength{\LBplusaddrtrfisH}
\setlength{\LBplusaddrtrfisH}{0cm}
\newsavebox{\LBplusaddrtrfisI}
\begin{lrbox}{\LBplusaddrtrfisI}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
STR X3,[X4,X2]
STR X5,[X6]
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusaddrtrfisJ}
\settowidth{\LBplusaddrtrfisJ}{\usebox{\LBplusaddrtrfisI}}
\addtolength{\LBplusaddrtrfisH}{\LBplusaddrtrfisJ}
\newsavebox{\LBplusaddrtrfisK}
\begin{lrbox}{\LBplusaddrtrfisK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
STR X3,[X4,X2]
STR X5,[X6]
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusaddrtrfisL}
\settowidth{\LBplusaddrtrfisL}{\usebox{\LBplusaddrtrfisK}}
\addtolength{\LBplusaddrtrfisH}{\LBplusaddrtrfisL}
\newsavebox{\LBplusaddrtrfisM}
\begin{lrbox}{\LBplusaddrtrfisM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X7,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusaddrtrfisN}
\settowidth{\LBplusaddrtrfisN}{\usebox{\LBplusaddrtrfisM}}
\addtolength{\LBplusaddrtrfisH}{\LBplusaddrtrfisN}
\newsavebox{\LBplusaddrtrfisO}
\begin{lrbox}{\LBplusaddrtrfisO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X7,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusaddrtrfisP}
\settowidth{\LBplusaddrtrfisP}{\usebox{\LBplusaddrtrfisO}}
\addtolength{\LBplusaddrtrfisH}{\LBplusaddrtrfisP}
\newsavebox{\LBplusaddrtrfisA}
\begin{lrbox}{\LBplusaddrtrfisA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3 pa4;
    x |-> pa1;
    y |-> pa2;
    u |-> invalid;
    u ?-> pa2;
    v |-> invalid;
    v ?-> pa1;
    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusaddrtrfisB}
\settowidth{\LBplusaddrtrfisB}{\usebox{\LBplusaddrtrfisA}}
\newsavebox{\LBplusaddrtrfisC}
\begin{lrbox}{\LBplusaddrtrfisC}
\begin{minipage}{\LBplusaddrtrfisH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R3=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R4=pte3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R5=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R6=u|\\
\lstinline[language=IslaLitmusExp]|0:R7=0b1|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|0:__isla_monomorphize_writes=true|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=desc3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R4=pte3(v,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R5=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R6=v|\\
\lstinline[language=IslaLitmusExp]|1:R7=0b1|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\lstinline[language=IslaLitmusExp]|1:__isla_monomorphize_writes=true|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|LB+addr-trfis|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\LBplusaddrtrfisB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\LBplusaddrtrfisA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\LBplusaddrtrfisC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\LBplusaddrtrfisI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\LBplusaddrtrfisK}\\
  \cline{2-2}
  & thread1 el0 handler\\
  \cline{2-2}
  & \usebox{\LBplusaddrtrfisM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\LBplusaddrtrfisO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R0=1 & 0:R7=1 & 1:R0=1 & 1:R7=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/LB+data-trfis.tex <==
\newlength{\LBplusdatatrfisH}
\setlength{\LBplusdatatrfisH}{0cm}
\newsavebox{\LBplusdatatrfisI}
\begin{lrbox}{\LBplusdatatrfisI}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
ORR X3,X3,X2
STR X3,[X4]
STR X5,[X6]
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusdatatrfisJ}
\settowidth{\LBplusdatatrfisJ}{\usebox{\LBplusdatatrfisI}}
\addtolength{\LBplusdatatrfisH}{\LBplusdatatrfisJ}
\newsavebox{\LBplusdatatrfisK}
\begin{lrbox}{\LBplusdatatrfisK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
ORR X3,X3,X2
STR X3,[X4]
STR X5,[X6]
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusdatatrfisL}
\settowidth{\LBplusdatatrfisL}{\usebox{\LBplusdatatrfisK}}
\addtolength{\LBplusdatatrfisH}{\LBplusdatatrfisL}
\newsavebox{\LBplusdatatrfisM}
\begin{lrbox}{\LBplusdatatrfisM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X7,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusdatatrfisN}
\settowidth{\LBplusdatatrfisN}{\usebox{\LBplusdatatrfisM}}
\addtolength{\LBplusdatatrfisH}{\LBplusdatatrfisN}
\newsavebox{\LBplusdatatrfisO}
\begin{lrbox}{\LBplusdatatrfisO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X7,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusdatatrfisP}
\settowidth{\LBplusdatatrfisP}{\usebox{\LBplusdatatrfisO}}
\addtolength{\LBplusdatatrfisH}{\LBplusdatatrfisP}
\newsavebox{\LBplusdatatrfisA}
\begin{lrbox}{\LBplusdatatrfisA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3 pa4;
    x |-> pa1;
    y |-> pa2;
    u |-> invalid;
    u ?-> pa2;
    v |-> invalid;
    v ?-> pa1;
    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusdatatrfisB}
\settowidth{\LBplusdatatrfisB}{\usebox{\LBplusdatatrfisA}}
\newsavebox{\LBplusdatatrfisC}
\begin{lrbox}{\LBplusdatatrfisC}
\begin{minipage}{\LBplusdatatrfisH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R3=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R4=pte3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R5=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R6=u|\\
\lstinline[language=IslaLitmusExp]|0:R7=0b1|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=desc3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R4=pte3(v,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R5=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R6=v|\\
\lstinline[language=IslaLitmusExp]|1:R7=0b1|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|LB+data-trfis|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\LBplusdatatrfisB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\LBplusdatatrfisA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\LBplusdatatrfisC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\LBplusdatatrfisI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\LBplusdatatrfisK}\\
  \cline{2-2}
  & thread1 el0 handler\\
  \cline{2-2}
  & \usebox{\LBplusdatatrfisM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\LBplusdatatrfisO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R0=1 & 0:R7=1 & 1:R0=1 & 1:R7=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/LB.TT.inv+pos.tex <==
\newlength{\LBdotTTdotinvplusposH}
\setlength{\LBdotTTdotinvplusposH}{0cm}
\newsavebox{\LBdotTTdotinvplusposI}
\begin{lrbox}{\LBdotTTdotinvplusposI}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\LBdotTTdotinvplusposJ}
\settowidth{\LBdotTTdotinvplusposJ}{\usebox{\LBdotTTdotinvplusposI}}
\addtolength{\LBdotTTdotinvplusposH}{\LBdotTTdotinvplusposJ}
\newsavebox{\LBdotTTdotinvplusposK}
\begin{lrbox}{\LBdotTTdotinvplusposK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\LBdotTTdotinvplusposL}
\settowidth{\LBdotTTdotinvplusposL}{\usebox{\LBdotTTdotinvplusposK}}
\addtolength{\LBdotTTdotinvplusposH}{\LBdotTTdotinvplusposL}
\newsavebox{\LBdotTTdotinvplusposM}
\begin{lrbox}{\LBdotTTdotinvplusposM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\LBdotTTdotinvplusposN}
\settowidth{\LBdotTTdotinvplusposN}{\usebox{\LBdotTTdotinvplusposM}}
\addtolength{\LBdotTTdotinvplusposH}{\LBdotTTdotinvplusposN}
\newsavebox{\LBdotTTdotinvplusposO}
\begin{lrbox}{\LBdotTTdotinvplusposO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\LBdotTTdotinvplusposP}
\settowidth{\LBdotTTdotinvplusposP}{\usebox{\LBdotTTdotinvplusposO}}
\addtolength{\LBdotTTdotinvplusposH}{\LBdotTTdotinvplusposP}
\newsavebox{\LBdotTTdotinvplusposA}
\begin{lrbox}{\LBdotTTdotinvplusposA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    y |-> invalid;

    x ?-> pa1;
    y ?-> pa1;

    *pa1 = 1;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\LBdotTTdotinvplusposB}
\settowidth{\LBdotTTdotinvplusposB}{\usebox{\LBdotTTdotinvplusposA}}
\newsavebox{\LBdotTTdotinvplusposC}
\begin{lrbox}{\LBdotTTdotinvplusposC}
\begin{minipage}{\LBdotTTdotinvplusposH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|LB.TT.inv+pos|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\LBdotTTdotinvplusposB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\LBdotTTdotinvplusposA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\LBdotTTdotinvplusposC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\LBdotTTdotinvplusposI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\LBdotTTdotinvplusposK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\LBdotTTdotinvplusposM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\LBdotTTdotinvplusposO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R0=1 & 1:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.BBM1+dsb-tlbiis-dsb-dsb+ctrl-isb.tex <==
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbH}
\setlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbH}{0cm}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbI}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X6
DSB SY
STR X2,[X1]
DSB SY
STR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbJ}
\settowidth{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbJ}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbI}}
\addtolength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbH}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbJ}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbK}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBNZ X0,L0
L0:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbL}
\settowidth{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbL}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbK}}
\addtolength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbH}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbL}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbM}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbN}
\settowidth{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbN}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbM}}
\addtolength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbH}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbN}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbO}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> pa1;
    x ?-> invalid;
    x ?-> pa2;

    y |-> pa3;
    identity 0x1000 with code;

    *pa2 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbP}
\settowidth{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbP}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbO}}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbA}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbA}
\begin{minipage}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R4=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R5=y|\\
\lstinline[language=IslaLitmusExp]|0:R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.BBM1+dsb-tlbiis-dsb-dsb+ctrl-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.BBM1+dsb-tlbiis-dsb-dsb+dsb-isb.tex <==
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbH}
\setlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbI}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X6
DSB SY
STR X2,[X1]
DSB SY
STR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbJ}
\settowidth{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbJ}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbI}}
\addtolength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbH}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbJ}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbK}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbL}
\settowidth{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbL}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbK}}
\addtolength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbH}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbL}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbM}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbN}
\settowidth{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbN}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbM}}
\addtolength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbH}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbN}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbO}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> pa1;
    x ?-> invalid;
    x ?-> pa2;

    y |-> pa3;
    identity 0x1000 with code;

    *pa2 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbP}
\settowidth{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbP}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbO}}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbA}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbA}
\begin{minipage}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R4=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R5=y|\\
\lstinline[language=IslaLitmusExp]|0:R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.BBM1+dsb-tlbiis-dsb-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.RT.EL1+dsb+dsb-tlbi-dsb+dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbH}
\setlength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbJ}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbJ}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbI}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
TLBI VAE1,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbL}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbL}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbK}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbL}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbN}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbN}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbM}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbN}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbP}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbP}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbO}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbP}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbB}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbB}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbA}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbB}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbC}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> pa1;
    x ?-> invalid;

    y |-> pa2;

    a |-> pa3;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbD}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbD}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbC}}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbE}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbE}
\begin{minipage}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R3=a|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:R1=a|\\
\lstinline[language=IslaLitmusExp]|1:R2=0x2|\\
\lstinline[language=IslaLitmusExp]|1:R3=a|\\
\lstinline[language=IslaLitmusExp]|1:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|2:R1=a|\\
\lstinline[language=IslaLitmusExp]|2:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|2:R3=y|\\
\lstinline[language=IslaLitmusExp]|3:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|3:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|3:R1=y|\\
\lstinline[language=IslaLitmusExp]|3:R3=x|\\
\lstinline[language=IslaLitmusExp]|3:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL1+dsb+dsb-tlbi-dsb+dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbM}\\
  \cline{2-2}
  & Thread 3\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbO}\\
  \cline{2-2}
  & thread3 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=2 & 3:R0=1 & 3:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.RT.EL1+dsb+dsb-tlbiis-dsb+dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbH}
\setlength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbJ}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbJ}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbI}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbL}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbL}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbK}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbL}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbN}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbN}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbM}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbN}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbP}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbP}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbO}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbP}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbB}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbB}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbA}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbB}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbC}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> pa1;
    x ?-> invalid;

    y |-> pa2;

    a |-> pa3;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbD}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbD}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbC}}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbE}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbE}
\begin{minipage}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R3=a|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:R1=a|\\
\lstinline[language=IslaLitmusExp]|1:R2=0x2|\\
\lstinline[language=IslaLitmusExp]|1:R3=a|\\
\lstinline[language=IslaLitmusExp]|1:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|2:R1=a|\\
\lstinline[language=IslaLitmusExp]|2:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|2:R3=y|\\
\lstinline[language=IslaLitmusExp]|3:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|3:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|3:R1=y|\\
\lstinline[language=IslaLitmusExp]|3:R3=x|\\
\lstinline[language=IslaLitmusExp]|3:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL1+dsb+dsb-tlbiis-dsb+dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbM}\\
  \cline{2-2}
  & Thread 3\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbO}\\
  \cline{2-2}
  & thread3 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=2 & 3:R0=1 & 3:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.RT.EL1+dsb-shootdown-dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbH}
\setlength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X4,[X5]
LDR X6,[X5]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbJ}
\settowidth{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbJ}{\usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbI}}
\addtolength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbH}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X4,[X5]
SVC #0
STR X7,[X5]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbL}
\settowidth{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbL}{\usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbK}}
\addtolength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbH}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbL}
\newsavebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS X9,ESR_EL1
LSR X9,X9,#26
SUB X9,X9,#0b010101
CBNZ X9,1f
0:
DSB SY
TLBI VAE1,X6
DSB SY
ISB
ERET
1:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbN}
\settowidth{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbN}{\usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbM}}
\addtolength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbH}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbN}
\newsavebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> pa1;
    x ?-> invalid;

    y |-> pa2;
    *pa2 = 0;

    f |-> pa3;
    *pa3 = 0;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbP}
\settowidth{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbP}{\usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbO}}
\newsavebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbA}
\begin{minipage}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R5=f|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=f|\\
\lstinline[language=IslaLitmusExp]|1:R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:R7=0b10|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL1+dsb-shootdown-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R4=1 & 0:R6=2 & 1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.RT.EL1+dsb-tlbi-dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbH}
\setlength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbJ}
\settowidth{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbJ}{\usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbI}}
\addtolength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbH}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbL}
\settowidth{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbL}{\usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbK}}
\addtolength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbH}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbL}
\newsavebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbN}
\settowidth{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbN}{\usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbM}}
\addtolength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbH}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbN}
\newsavebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbP}
\settowidth{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbP}{\usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbO}}
\newsavebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbA}
\begin{minipage}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL1+dsb-tlbi-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.RT.EL1+dsb-tlbiis-dsb+dmb.tex <==
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbH}
\setlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbH}{0cm}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbI}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbJ}
\settowidth{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbJ}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbI}}
\addtolength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbJ}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbK}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbL}
\settowidth{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbL}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbK}}
\addtolength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbL}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbM}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbN}
\settowidth{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbN}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbM}}
\addtolength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbN}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbO}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbP}
\settowidth{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbP}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbO}}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbA}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbA}
\begin{minipage}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL1+dsb-tlbiis-dsb+dmb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.RT.EL1+dsb-tlbiis-dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbH}
\setlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbJ}
\settowidth{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbJ}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbI}}
\addtolength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbL}
\settowidth{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbL}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbK}}
\addtolength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbL}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbN}
\settowidth{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbN}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbM}}
\addtolength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbN}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbP}
\settowidth{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbP}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbO}}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbA}
\begin{minipage}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL1+dsb-tlbiis-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.RT.EL2+dsb-tlbiipa-dsb-tlbiis-dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbH}
\setlength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1,X4
DSB SY
TLBI VMALLE1IS
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbJ}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbJ}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbI}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbL}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbL}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbK}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbL}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#1
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbN}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbN}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbM}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbN}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
physical pa1 pa2;
intermediate ipa1 ipa2;

x |-> ipa1;
ipa1 |-> pa1;
ipa1 ?-> invalid;

y |-> ipa2;
ipa2 |-> pa2;

identity 0x2000 with code;

*pa1 = 0;
*pa2 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbP}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbP}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbO}}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbA}
\begin{minipage}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=bvlshr(ipa1,0xC)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL2+dsb-tlbiipa-dsb-tlbiis-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.RT.EL2+dsb-tlbiipais-dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbH}
\setlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbJ}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbJ}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbI}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbL}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbL}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbK}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbL}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#1
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbN}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbN}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbM}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbN}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
physical pa1 pa2;
intermediate ipa1 ipa2;

x |-> ipa1;
ipa1 |-> pa1;
ipa1 ?-> invalid;

y |-> ipa2;
ipa2 |-> pa2;

identity 0x2000 with code;

*pa1 = 1;
*pa2 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbP}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbP}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbO}}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbA}
\begin{minipage}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(ipa1)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL2+dsb-tlbiipais-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|true|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.RT.EL2+dsb-tlbiipais-dsb-tlbiis-dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbH}
\setlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1IS,X4
DSB SY
TLBI VMALLE1IS
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbJ}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbJ}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbI}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
isb
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbL}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbL}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbK}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbL}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#1
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbN}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbN}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbM}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbN}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
physical pa1 pa2;
intermediate ipa1 ipa2;

x |-> ipa1;
ipa1 |-> pa1;
ipa1 ?-> invalid;

y |-> ipa2;
ipa2 |-> pa2;

identity 0x2000 with code;

*pa1 = 0;
*pa2 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbP}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbP}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbO}}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbA}
\begin{minipage}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(ipa1)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL2+dsb-tlbiipais-dsb-tlbiis-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.RT.EL2+dsb-tlbiis-dsb-tlbiipais-dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbH}
\setlength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VMALLE1IS
DSB SY
TLBI IPAS2E1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbJ}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbJ}{\usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbI}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
isb
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbL}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbL}{\usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbK}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbL}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#1
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbN}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbN}{\usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbM}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbN}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
physical pa1 pa2;
intermediate ipa1 ipa2;

x |-> ipa1;
ipa1 |-> pa1;
ipa1 ?-> invalid;

y |-> ipa2;
ipa2 |-> pa2;

identity 0x2000 with code;

*pa1 = 0;
*pa2 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbP}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbP}{\usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbO}}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbA}
\begin{minipage}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(ipa1)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL2+dsb-tlbiis-dsb-tlbiipais-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.RT.inv+dmb+addr-po-isb.tex <==
\newlength{\MPdotRTdotinvplusdmbplusaddrpoisbH}
\setlength{\MPdotRTdotinvplusdmbplusaddrpoisbH}{0cm}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpoisbI}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpoisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpoisbJ}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpoisbJ}{\usebox{\MPdotRTdotinvplusdmbplusaddrpoisbI}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpoisbH}{\MPdotRTdotinvplusdmbplusaddrpoisbJ}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpoisbK}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpoisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
EOR X6,X2,X2
LDR X7,[X8,X6]
ISB
LDR X4,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpoisbL}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpoisbL}{\usebox{\MPdotRTdotinvplusdmbplusaddrpoisbK}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpoisbH}{\MPdotRTdotinvplusdmbplusaddrpoisbL}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpoisbM}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpoisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpoisbN}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpoisbN}{\usebox{\MPdotRTdotinvplusdmbplusaddrpoisbM}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpoisbH}{\MPdotRTdotinvplusdmbplusaddrpoisbN}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpoisbO}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpoisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X4,#0
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpoisbP}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpoisbP}{\usebox{\MPdotRTdotinvplusdmbplusaddrpoisbO}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpoisbH}{\MPdotRTdotinvplusdmbplusaddrpoisbP}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpoisbA}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpoisbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;

    x |-> invalid;
    x ?-> pa1;

    y |-> pa2;

    z |-> pa3;

    *pa1 = 1;
    *pa2 = 0;
    *pa3 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpoisbB}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpoisbB}{\usebox{\MPdotRTdotinvplusdmbplusaddrpoisbA}}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpoisbC}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpoisbC}
\begin{minipage}{\MPdotRTdotinvplusdmbplusaddrpoisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R8=z|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.inv+dmb+addr-po-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotinvplusdmbplusaddrpoisbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotinvplusdmbplusaddrpoisbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotinvplusdmbplusaddrpoisbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpoisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpoisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpoisbM}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpoisbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R2=1 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.RT.inv+dmb+addr-po-msr-isb.tex <==
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrisbH}
\setlength{\MPdotRTdotinvplusdmbplusaddrpomsrisbH}{0cm}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbI}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrisbJ}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrisbJ}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbI}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpomsrisbH}{\MPdotRTdotinvplusdmbplusaddrpomsrisbJ}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbK}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
EOR X6,X2,X2
LDR X7,[X8,X6]
MSR ELR_EL1,X5
ISB
LDR X4,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrisbL}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrisbL}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbK}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpomsrisbH}{\MPdotRTdotinvplusdmbplusaddrpomsrisbL}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbM}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrisbN}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrisbN}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbM}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpomsrisbH}{\MPdotRTdotinvplusdmbplusaddrpomsrisbN}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbO}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X4,#0
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrisbP}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrisbP}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbO}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpomsrisbH}{\MPdotRTdotinvplusdmbplusaddrpomsrisbP}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbA}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrisbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;

    x |-> invalid;
    x ?-> pa1;

    y |-> pa2;

    z |-> pa3;

    *pa1 = 1;
    *pa2 = 0;
    *pa3 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrisbB}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrisbB}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbA}}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbC}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrisbC}
\begin{minipage}{\MPdotRTdotinvplusdmbplusaddrpomsrisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:R8=z|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.inv+dmb+addr-po-msr-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotinvplusdmbplusaddrpomsrisbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbM}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R2=1 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.RT.inv+dmb+addr-po-msr.tex <==
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrH}
\setlength{\MPdotRTdotinvplusdmbplusaddrpomsrH}{0cm}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrI}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrJ}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrJ}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrI}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpomsrH}{\MPdotRTdotinvplusdmbplusaddrpomsrJ}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrK}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
EOR X6,X2,X2
LDR X7,[X8,X6]
MSR ELR_EL1,X5
LDR X4,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrL}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrL}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrK}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpomsrH}{\MPdotRTdotinvplusdmbplusaddrpomsrL}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrM}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrN}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrN}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrM}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpomsrH}{\MPdotRTdotinvplusdmbplusaddrpomsrN}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrO}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X4,#0
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrP}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrP}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrO}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpomsrH}{\MPdotRTdotinvplusdmbplusaddrpomsrP}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrA}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;

    x |-> invalid;
    x ?-> pa1;

    y |-> pa2;

    z |-> pa3;

    *pa1 = 1;
    *pa2 = 0;
    *pa3 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrB}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrB}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrA}}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrC}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrC}
\begin{minipage}{\MPdotRTdotinvplusdmbplusaddrpomsrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:R8=z|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.inv+dmb+addr-po-msr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotinvplusdmbplusaddrpomsrB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpomsrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpomsrK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpomsrM}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpomsrO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R2=1 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.RT.inv+dmb+ctrl-trfi.tex <==
\newlength{\MPdotRTdotinvplusdmbplusctrltrfiH}
\setlength{\MPdotRTdotinvplusdmbplusctrltrfiH}{0cm}
\newsavebox{\MPdotRTdotinvplusdmbplusctrltrfiI}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusctrltrfiI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusctrltrfiJ}
\settowidth{\MPdotRTdotinvplusdmbplusctrltrfiJ}{\usebox{\MPdotRTdotinvplusdmbplusctrltrfiI}}
\addtolength{\MPdotRTdotinvplusdmbplusctrltrfiH}{\MPdotRTdotinvplusdmbplusctrltrfiJ}
\newsavebox{\MPdotRTdotinvplusdmbplusctrltrfiK}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusctrltrfiK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBZ X0,LC00
LC00:
STR X2,[X3]
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusctrltrfiL}
\settowidth{\MPdotRTdotinvplusdmbplusctrltrfiL}{\usebox{\MPdotRTdotinvplusdmbplusctrltrfiK}}
\addtolength{\MPdotRTdotinvplusdmbplusctrltrfiH}{\MPdotRTdotinvplusdmbplusctrltrfiL}
\newsavebox{\MPdotRTdotinvplusdmbplusctrltrfiM}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusctrltrfiM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#2
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusctrltrfiN}
\settowidth{\MPdotRTdotinvplusdmbplusctrltrfiN}{\usebox{\MPdotRTdotinvplusdmbplusctrltrfiM}}
\addtolength{\MPdotRTdotinvplusdmbplusctrltrfiH}{\MPdotRTdotinvplusdmbplusctrltrfiN}
\newsavebox{\MPdotRTdotinvplusdmbplusctrltrfiO}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusctrltrfiO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    w |-> invalid;
    w ?-> pa1;
    x |-> pa1;
    *pa1 = 0;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusctrltrfiP}
\settowidth{\MPdotRTdotinvplusdmbplusctrltrfiP}{\usebox{\MPdotRTdotinvplusdmbplusctrltrfiO}}
\newsavebox{\MPdotRTdotinvplusdmbplusctrltrfiA}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusctrltrfiA}
\begin{minipage}{\MPdotRTdotinvplusdmbplusctrltrfiH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(w,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R5=w|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.inv+dmb+ctrl-trfi|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotinvplusdmbplusctrltrfiP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotinvplusdmbplusctrltrfiO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotinvplusdmbplusctrltrfiA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusctrltrfiI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusctrltrfiK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusctrltrfiM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.RT.inv+trfi-data+addr.toml.tex <==
\newlength{\MPdotRTdotinvplustrfidataplusaddrdottomlH}
\setlength{\MPdotRTdotinvplustrfidataplusaddrdottomlH}{0cm}
\newsavebox{\MPdotRTdotinvplustrfidataplusaddrdottomlI}
\begin{lrbox}{\MPdotRTdotinvplustrfidataplusaddrdottomlI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
STR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplustrfidataplusaddrdottomlJ}
\settowidth{\MPdotRTdotinvplustrfidataplusaddrdottomlJ}{\usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlI}}
\addtolength{\MPdotRTdotinvplustrfidataplusaddrdottomlH}{\MPdotRTdotinvplustrfidataplusaddrdottomlJ}
\newsavebox{\MPdotRTdotinvplustrfidataplusaddrdottomlK}
\begin{lrbox}{\MPdotRTdotinvplustrfidataplusaddrdottomlK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
LDR X3,[X4,X2]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplustrfidataplusaddrdottomlL}
\settowidth{\MPdotRTdotinvplustrfidataplusaddrdottomlL}{\usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlK}}
\addtolength{\MPdotRTdotinvplustrfidataplusaddrdottomlH}{\MPdotRTdotinvplustrfidataplusaddrdottomlL}
\newsavebox{\MPdotRTdotinvplustrfidataplusaddrdottomlM}
\begin{lrbox}{\MPdotRTdotinvplustrfidataplusaddrdottomlM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplustrfidataplusaddrdottomlN}
\settowidth{\MPdotRTdotinvplustrfidataplusaddrdottomlN}{\usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlM}}
\addtolength{\MPdotRTdotinvplustrfidataplusaddrdottomlH}{\MPdotRTdotinvplustrfidataplusaddrdottomlN}
\newsavebox{\MPdotRTdotinvplustrfidataplusaddrdottomlO}
\begin{lrbox}{\MPdotRTdotinvplustrfidataplusaddrdottomlO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X3,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplustrfidataplusaddrdottomlP}
\settowidth{\MPdotRTdotinvplustrfidataplusaddrdottomlP}{\usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlO}}
\addtolength{\MPdotRTdotinvplustrfidataplusaddrdottomlH}{\MPdotRTdotinvplustrfidataplusaddrdottomlP}
\newsavebox{\MPdotRTdotinvplustrfidataplusaddrdottomlA}
\begin{lrbox}{\MPdotRTdotinvplustrfidataplusaddrdottomlA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    w |-> invalid;
    w ?-> pa1;
    x |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplustrfidataplusaddrdottomlB}
\settowidth{\MPdotRTdotinvplustrfidataplusaddrdottomlB}{\usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlA}}
\newsavebox{\MPdotRTdotinvplustrfidataplusaddrdottomlC}
\begin{lrbox}{\MPdotRTdotinvplustrfidataplusaddrdottomlC}
\begin{minipage}{\MPdotRTdotinvplustrfidataplusaddrdottomlH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(w,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R3=w|\\
\lstinline[language=IslaLitmusExp]|0:R4=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R5=y|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(w,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R4=w|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.inv+trfi-data+addr.toml|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotinvplustrfidataplusaddrdottomlB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=1 & 1:R0=1 & 1:R3=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.RTT.EL1+dsb-tlbiis-tlbiis-dsb+dsb-isb.tex <==
\newlength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbH}
\setlength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
STR X2,[X3]
DSB SY
TLBI VAE1IS,X4
TLBI VAE1IS,X5
DSB SY
STR X6,[X7]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbJ}
\settowidth{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbJ}{\usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbI}}
\addtolength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbH}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbJ}
\newsavebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X4,[X3]
MOV X2,X4
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbL}
\settowidth{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbL}{\usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbK}}
\addtolength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbH}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbL}
\newsavebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbN}
\settowidth{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbN}{\usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbM}}
\addtolength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbH}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbN}
\newsavebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> pa1;
    x ?-> invalid;

    y |-> pa2;

    z |-> pa3;
    z ?-> invalid;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbP}
\settowidth{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbP}{\usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbO}}
\newsavebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbA}
\begin{minipage}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|0:R5=page(z)|\\
\lstinline[language=IslaLitmusExp]|0:R6=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R7=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=z|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTT.EL1+dsb-tlbiis-tlbiis-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.RTf.inv+dmb+addr.tex <==
\newlength{\MPdotRTfdotinvplusdmbplusaddrH}
\setlength{\MPdotRTfdotinvplusdmbplusaddrH}{0cm}
\newsavebox{\MPdotRTfdotinvplusdmbplusaddrI}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusaddrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB ST
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusaddrJ}
\settowidth{\MPdotRTfdotinvplusdmbplusaddrJ}{\usebox{\MPdotRTfdotinvplusdmbplusaddrI}}
\addtolength{\MPdotRTfdotinvplusdmbplusaddrH}{\MPdotRTfdotinvplusdmbplusaddrJ}
\newsavebox{\MPdotRTfdotinvplusdmbplusaddrK}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusaddrK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusaddrL}
\settowidth{\MPdotRTfdotinvplusdmbplusaddrL}{\usebox{\MPdotRTfdotinvplusdmbplusaddrK}}
\addtolength{\MPdotRTfdotinvplusdmbplusaddrH}{\MPdotRTfdotinvplusdmbplusaddrL}
\newsavebox{\MPdotRTfdotinvplusdmbplusaddrM}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusaddrM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusaddrN}
\settowidth{\MPdotRTfdotinvplusdmbplusaddrN}{\usebox{\MPdotRTfdotinvplusdmbplusaddrM}}
\addtolength{\MPdotRTfdotinvplusdmbplusaddrH}{\MPdotRTfdotinvplusdmbplusaddrN}
\newsavebox{\MPdotRTfdotinvplusdmbplusaddrO}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusaddrO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusaddrP}
\settowidth{\MPdotRTfdotinvplusdmbplusaddrP}{\usebox{\MPdotRTfdotinvplusdmbplusaddrO}}
\newsavebox{\MPdotRTfdotinvplusdmbplusaddrA}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusaddrA}
\begin{minipage}{\MPdotRTfdotinvplusdmbplusaddrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv+dmb+addr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvplusdmbplusaddrP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvplusdmbplusaddrO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvplusdmbplusaddrA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusaddrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusaddrK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusaddrM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.RTf.inv+dmb+ctrl-isb.tex <==
\newlength{\MPdotRTfdotinvplusdmbplusctrlisbH}
\setlength{\MPdotRTfdotinvplusdmbplusctrlisbH}{0cm}
\newsavebox{\MPdotRTfdotinvplusdmbplusctrlisbI}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusctrlisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusctrlisbJ}
\settowidth{\MPdotRTfdotinvplusdmbplusctrlisbJ}{\usebox{\MPdotRTfdotinvplusdmbplusctrlisbI}}
\addtolength{\MPdotRTfdotinvplusdmbplusctrlisbH}{\MPdotRTfdotinvplusdmbplusctrlisbJ}
\newsavebox{\MPdotRTfdotinvplusdmbplusctrlisbK}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusctrlisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBNZ X0,L0
L0:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusctrlisbL}
\settowidth{\MPdotRTfdotinvplusdmbplusctrlisbL}{\usebox{\MPdotRTfdotinvplusdmbplusctrlisbK}}
\addtolength{\MPdotRTfdotinvplusdmbplusctrlisbH}{\MPdotRTfdotinvplusdmbplusctrlisbL}
\newsavebox{\MPdotRTfdotinvplusdmbplusctrlisbM}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusctrlisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusctrlisbN}
\settowidth{\MPdotRTfdotinvplusdmbplusctrlisbN}{\usebox{\MPdotRTfdotinvplusdmbplusctrlisbM}}
\addtolength{\MPdotRTfdotinvplusdmbplusctrlisbH}{\MPdotRTfdotinvplusdmbplusctrlisbN}
\newsavebox{\MPdotRTfdotinvplusdmbplusctrlisbO}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusctrlisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusctrlisbP}
\settowidth{\MPdotRTfdotinvplusdmbplusctrlisbP}{\usebox{\MPdotRTfdotinvplusdmbplusctrlisbO}}
\newsavebox{\MPdotRTfdotinvplusdmbplusctrlisbA}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusctrlisbA}
\begin{minipage}{\MPdotRTfdotinvplusdmbplusctrlisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv+dmb+ctrl-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvplusdmbplusctrlisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvplusdmbplusctrlisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvplusdmbplusctrlisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusctrlisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusctrlisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusctrlisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.RTf.inv+dmb+data.tex <==
\newlength{\MPdotRTfdotinvplusdmbplusdataH}
\setlength{\MPdotRTfdotinvplusdmbplusdataH}{0cm}
\newsavebox{\MPdotRTfdotinvplusdmbplusdataI}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdataI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB ST
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusdataJ}
\settowidth{\MPdotRTfdotinvplusdmbplusdataJ}{\usebox{\MPdotRTfdotinvplusdmbplusdataI}}
\addtolength{\MPdotRTfdotinvplusdmbplusdataH}{\MPdotRTfdotinvplusdmbplusdataJ}
\newsavebox{\MPdotRTfdotinvplusdmbplusdataK}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdataK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
ORR X6,X4,X5
STR X6,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusdataL}
\settowidth{\MPdotRTfdotinvplusdmbplusdataL}{\usebox{\MPdotRTfdotinvplusdmbplusdataK}}
\addtolength{\MPdotRTfdotinvplusdmbplusdataH}{\MPdotRTfdotinvplusdmbplusdataL}
\newsavebox{\MPdotRTfdotinvplusdmbplusdataM}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdataM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusdataN}
\settowidth{\MPdotRTfdotinvplusdmbplusdataN}{\usebox{\MPdotRTfdotinvplusdmbplusdataM}}
\addtolength{\MPdotRTfdotinvplusdmbplusdataH}{\MPdotRTfdotinvplusdmbplusdataN}
\newsavebox{\MPdotRTfdotinvplusdmbplusdataO}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdataO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusdataP}
\settowidth{\MPdotRTfdotinvplusdmbplusdataP}{\usebox{\MPdotRTfdotinvplusdmbplusdataO}}
\newsavebox{\MPdotRTfdotinvplusdmbplusdataA}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdataA}
\begin{minipage}{\MPdotRTfdotinvplusdmbplusdataH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=0b1|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv+dmb+data|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvplusdmbplusdataP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvplusdmbplusdataO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvplusdmbplusdataA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusdataI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusdataK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusdataM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.RTf.inv+dmb+dsb-isb.tex <==
\newlength{\MPdotRTfdotinvplusdmbplusdsbisbH}
\setlength{\MPdotRTfdotinvplusdmbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTfdotinvplusdmbplusdsbisbI}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusdsbisbJ}
\settowidth{\MPdotRTfdotinvplusdmbplusdsbisbJ}{\usebox{\MPdotRTfdotinvplusdmbplusdsbisbI}}
\addtolength{\MPdotRTfdotinvplusdmbplusdsbisbH}{\MPdotRTfdotinvplusdmbplusdsbisbJ}
\newsavebox{\MPdotRTfdotinvplusdmbplusdsbisbK}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusdsbisbL}
\settowidth{\MPdotRTfdotinvplusdmbplusdsbisbL}{\usebox{\MPdotRTfdotinvplusdmbplusdsbisbK}}
\addtolength{\MPdotRTfdotinvplusdmbplusdsbisbH}{\MPdotRTfdotinvplusdmbplusdsbisbL}
\newsavebox{\MPdotRTfdotinvplusdmbplusdsbisbM}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusdsbisbN}
\settowidth{\MPdotRTfdotinvplusdmbplusdsbisbN}{\usebox{\MPdotRTfdotinvplusdmbplusdsbisbM}}
\addtolength{\MPdotRTfdotinvplusdmbplusdsbisbH}{\MPdotRTfdotinvplusdmbplusdsbisbN}
\newsavebox{\MPdotRTfdotinvplusdmbplusdsbisbO}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusdsbisbP}
\settowidth{\MPdotRTfdotinvplusdmbplusdsbisbP}{\usebox{\MPdotRTfdotinvplusdmbplusdsbisbO}}
\newsavebox{\MPdotRTfdotinvplusdmbplusdsbisbA}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdsbisbA}
\begin{minipage}{\MPdotRTfdotinvplusdmbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv+dmb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvplusdmbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvplusdmbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvplusdmbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.RTf.inv+dmb+po.tex <==
\newlength{\MPdotRTfdotinvplusdmbpluspoH}
\setlength{\MPdotRTfdotinvplusdmbpluspoH}{0cm}
\newsavebox{\MPdotRTfdotinvplusdmbpluspoI}
\begin{lrbox}{\MPdotRTfdotinvplusdmbpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB ST
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbpluspoJ}
\settowidth{\MPdotRTfdotinvplusdmbpluspoJ}{\usebox{\MPdotRTfdotinvplusdmbpluspoI}}
\addtolength{\MPdotRTfdotinvplusdmbpluspoH}{\MPdotRTfdotinvplusdmbpluspoJ}
\newsavebox{\MPdotRTfdotinvplusdmbpluspoK}
\begin{lrbox}{\MPdotRTfdotinvplusdmbpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbpluspoL}
\settowidth{\MPdotRTfdotinvplusdmbpluspoL}{\usebox{\MPdotRTfdotinvplusdmbpluspoK}}
\addtolength{\MPdotRTfdotinvplusdmbpluspoH}{\MPdotRTfdotinvplusdmbpluspoL}
\newsavebox{\MPdotRTfdotinvplusdmbpluspoM}
\begin{lrbox}{\MPdotRTfdotinvplusdmbpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbpluspoN}
\settowidth{\MPdotRTfdotinvplusdmbpluspoN}{\usebox{\MPdotRTfdotinvplusdmbpluspoM}}
\addtolength{\MPdotRTfdotinvplusdmbpluspoH}{\MPdotRTfdotinvplusdmbpluspoN}
\newsavebox{\MPdotRTfdotinvplusdmbpluspoO}
\begin{lrbox}{\MPdotRTfdotinvplusdmbpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbpluspoP}
\settowidth{\MPdotRTfdotinvplusdmbpluspoP}{\usebox{\MPdotRTfdotinvplusdmbpluspoO}}
\newsavebox{\MPdotRTfdotinvplusdmbpluspoA}
\begin{lrbox}{\MPdotRTfdotinvplusdmbpluspoA}
\begin{minipage}{\MPdotRTfdotinvplusdmbpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv+dmb+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvplusdmbpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvplusdmbpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvplusdmbpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.RTf.inv+dmbs.tex <==
\newlength{\MPdotRTfdotinvplusdmbsH}
\setlength{\MPdotRTfdotinvplusdmbsH}{0cm}
\newsavebox{\MPdotRTfdotinvplusdmbsI}
\begin{lrbox}{\MPdotRTfdotinvplusdmbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB ST
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbsJ}
\settowidth{\MPdotRTfdotinvplusdmbsJ}{\usebox{\MPdotRTfdotinvplusdmbsI}}
\addtolength{\MPdotRTfdotinvplusdmbsH}{\MPdotRTfdotinvplusdmbsJ}
\newsavebox{\MPdotRTfdotinvplusdmbsK}
\begin{lrbox}{\MPdotRTfdotinvplusdmbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbsL}
\settowidth{\MPdotRTfdotinvplusdmbsL}{\usebox{\MPdotRTfdotinvplusdmbsK}}
\addtolength{\MPdotRTfdotinvplusdmbsH}{\MPdotRTfdotinvplusdmbsL}
\newsavebox{\MPdotRTfdotinvplusdmbsM}
\begin{lrbox}{\MPdotRTfdotinvplusdmbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbsN}
\settowidth{\MPdotRTfdotinvplusdmbsN}{\usebox{\MPdotRTfdotinvplusdmbsM}}
\addtolength{\MPdotRTfdotinvplusdmbsH}{\MPdotRTfdotinvplusdmbsN}
\newsavebox{\MPdotRTfdotinvplusdmbsO}
\begin{lrbox}{\MPdotRTfdotinvplusdmbsO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbsP}
\settowidth{\MPdotRTfdotinvplusdmbsP}{\usebox{\MPdotRTfdotinvplusdmbsO}}
\newsavebox{\MPdotRTfdotinvplusdmbsA}
\begin{lrbox}{\MPdotRTfdotinvplusdmbsA}
\begin{minipage}{\MPdotRTfdotinvplusdmbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv+dmbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvplusdmbsP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvplusdmbsO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvplusdmbsA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbsK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbsM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.RTf.inv.EL1+dsb-tlbiis-dsb+addr.tex <==
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrH}
\setlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrH}{0cm}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrI}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrJ}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrJ}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrI}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrJ}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrK}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrL}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrL}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrK}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrL}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrM}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrN}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrN}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrM}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrN}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrO}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrP}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrP}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrO}}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrA}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrA}
\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv.EL1+dsb-tlbiis-dsb+addr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.RTf.inv.EL1+dsb-tlbiis-dsb+ctrl-isb.tex <==
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbH}
\setlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbH}{0cm}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbI}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbJ}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbJ}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbI}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbJ}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbK}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBNZ X0,L0
L0:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbL}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbL}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbK}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbL}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbM}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbN}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbN}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbM}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbN}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbO}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbP}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbP}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbO}}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbA}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbA}
\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv.EL1+dsb-tlbiis-dsb+ctrl-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.RTf.inv.EL1+dsb-tlbiis-dsb+ctrl.tex <==
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}
\setlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}{0cm}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlI}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlJ}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlJ}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlI}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlJ}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlK}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBNZ X0,L0
L0:
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlL}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlL}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlK}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlL}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlM}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlN}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlN}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlM}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlN}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlO}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlP}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlP}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlO}}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlA}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlA}
\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv.EL1+dsb-tlbiis-dsb+ctrl|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.RTf.inv.EL1+dsb-tlbiis-dsb+data.tex <==
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}
\setlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}{0cm}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataI}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataJ}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataJ}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataI}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataJ}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataK}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
STR X4,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataL}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataL}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataK}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataL}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataM}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataN}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataN}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataM}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataN}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataO}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataP}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataP}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataO}}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataA}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataA}
\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv.EL1+dsb-tlbiis-dsb+data|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.RTf.inv.EL1+dsb-tlbiis-dsb+dmb.tex <==
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}
\setlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{0cm}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}
\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv.EL1+dsb-tlbiis-dsb+dmb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.RTf.inv.EL1+dsb-tlbiis-dsb+dsb-isb.tex <==
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}
\setlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbJ}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbJ}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbI}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbJ}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbL}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbL}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbK}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbL}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbN}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbN}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbM}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbN}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbP}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbP}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbO}}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbA}
\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv.EL1+dsb-tlbiis-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.RTf.inv.EL1+dsb-tlbiis-dsb+po.tex <==
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}
\setlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}{0cm}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoI}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoJ}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoJ}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoI}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoJ}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoK}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoL}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoL}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoK}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoL}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoM}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoN}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoN}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoM}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoN}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoO}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoP}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoP}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoO}}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoA}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoA}
\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv.EL1+dsb-tlbiis-dsb+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.RTf.inv.EL1+dsb-tlbiis-dsb+poap.tex <==
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}
\setlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}{0cm}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapI}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapJ}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapJ}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapI}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapJ}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapK}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDAR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapL}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapL}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapK}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapL}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapM}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapN}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapN}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapM}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapN}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapO}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapP}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapP}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapO}}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapA}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapA}
\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv.EL1+dsb-tlbiis-dsb+poap|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.TR.inv+dmb+isb.tex <==
\newlength{\MPdotTRdotinvplusdmbplusisbH}
\setlength{\MPdotTRdotinvplusdmbplusisbH}{0cm}
\newsavebox{\MPdotTRdotinvplusdmbplusisbI}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusisbJ}
\settowidth{\MPdotTRdotinvplusdmbplusisbJ}{\usebox{\MPdotTRdotinvplusdmbplusisbI}}
\addtolength{\MPdotTRdotinvplusdmbplusisbH}{\MPdotTRdotinvplusdmbplusisbJ}
\newsavebox{\MPdotTRdotinvplusdmbplusisbK}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
ISB
LDR X4,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusisbL}
\settowidth{\MPdotTRdotinvplusdmbplusisbL}{\usebox{\MPdotTRdotinvplusdmbplusisbK}}
\addtolength{\MPdotTRdotinvplusdmbplusisbH}{\MPdotTRdotinvplusdmbplusisbL}
\newsavebox{\MPdotTRdotinvplusdmbplusisbM}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusisbN}
\settowidth{\MPdotTRdotinvplusdmbplusisbN}{\usebox{\MPdotTRdotinvplusdmbplusisbM}}
\addtolength{\MPdotTRdotinvplusdmbplusisbH}{\MPdotTRdotinvplusdmbplusisbN}
\newsavebox{\MPdotTRdotinvplusdmbplusisbO}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusisbP}
\settowidth{\MPdotTRdotinvplusdmbplusisbP}{\usebox{\MPdotTRdotinvplusdmbplusisbO}}
\addtolength{\MPdotTRdotinvplusdmbplusisbH}{\MPdotTRdotinvplusdmbplusisbP}
\newsavebox{\MPdotTRdotinvplusdmbplusisbA}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusisbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 0;
    *pa2 = 1;
    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusisbB}
\settowidth{\MPdotTRdotinvplusdmbplusisbB}{\usebox{\MPdotTRdotinvplusdmbplusisbA}}
\newsavebox{\MPdotTRdotinvplusdmbplusisbC}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusisbC}
\begin{minipage}{\MPdotTRdotinvplusdmbplusisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TR.inv+dmb+isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTRdotinvplusdmbplusisbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTRdotinvplusdmbplusisbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTRdotinvplusdmbplusisbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusisbM}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusisbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R2=1 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.TR.inv+dmb+msr-isb.tex <==
\newlength{\MPdotTRdotinvplusdmbplusmsrisbH}
\setlength{\MPdotTRdotinvplusdmbplusmsrisbH}{0cm}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrisbI}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrisbJ}
\settowidth{\MPdotTRdotinvplusdmbplusmsrisbJ}{\usebox{\MPdotTRdotinvplusdmbplusmsrisbI}}
\addtolength{\MPdotTRdotinvplusdmbplusmsrisbH}{\MPdotTRdotinvplusdmbplusmsrisbJ}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrisbK}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MSR ELR_EL1,X5
ISB
LDR X4,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrisbL}
\settowidth{\MPdotTRdotinvplusdmbplusmsrisbL}{\usebox{\MPdotTRdotinvplusdmbplusmsrisbK}}
\addtolength{\MPdotTRdotinvplusdmbplusmsrisbH}{\MPdotTRdotinvplusdmbplusmsrisbL}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrisbM}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrisbN}
\settowidth{\MPdotTRdotinvplusdmbplusmsrisbN}{\usebox{\MPdotTRdotinvplusdmbplusmsrisbM}}
\addtolength{\MPdotTRdotinvplusdmbplusmsrisbH}{\MPdotTRdotinvplusdmbplusmsrisbN}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrisbO}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrisbP}
\settowidth{\MPdotTRdotinvplusdmbplusmsrisbP}{\usebox{\MPdotTRdotinvplusdmbplusmsrisbO}}
\addtolength{\MPdotTRdotinvplusdmbplusmsrisbH}{\MPdotTRdotinvplusdmbplusmsrisbP}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrisbA}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrisbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 0;
    *pa2 = 1;
    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrisbB}
\settowidth{\MPdotTRdotinvplusdmbplusmsrisbB}{\usebox{\MPdotTRdotinvplusdmbplusmsrisbA}}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrisbC}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrisbC}
\begin{minipage}{\MPdotTRdotinvplusdmbplusmsrisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TR.inv+dmb+msr-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTRdotinvplusdmbplusmsrisbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTRdotinvplusdmbplusmsrisbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTRdotinvplusdmbplusmsrisbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusmsrisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusmsrisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusmsrisbM}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusmsrisbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R2=1 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.TR.inv+dmb+msr.tex <==
\newlength{\MPdotTRdotinvplusdmbplusmsrH}
\setlength{\MPdotTRdotinvplusdmbplusmsrH}{0cm}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrI}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrJ}
\settowidth{\MPdotTRdotinvplusdmbplusmsrJ}{\usebox{\MPdotTRdotinvplusdmbplusmsrI}}
\addtolength{\MPdotTRdotinvplusdmbplusmsrH}{\MPdotTRdotinvplusdmbplusmsrJ}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrK}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MSR ELR_EL1,X5
LDR X4,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrL}
\settowidth{\MPdotTRdotinvplusdmbplusmsrL}{\usebox{\MPdotTRdotinvplusdmbplusmsrK}}
\addtolength{\MPdotTRdotinvplusdmbplusmsrH}{\MPdotTRdotinvplusdmbplusmsrL}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrM}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrN}
\settowidth{\MPdotTRdotinvplusdmbplusmsrN}{\usebox{\MPdotTRdotinvplusdmbplusmsrM}}
\addtolength{\MPdotTRdotinvplusdmbplusmsrH}{\MPdotTRdotinvplusdmbplusmsrN}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrO}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrP}
\settowidth{\MPdotTRdotinvplusdmbplusmsrP}{\usebox{\MPdotTRdotinvplusdmbplusmsrO}}
\addtolength{\MPdotTRdotinvplusdmbplusmsrH}{\MPdotTRdotinvplusdmbplusmsrP}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrA}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 0;
    *pa2 = 1;
    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrB}
\settowidth{\MPdotTRdotinvplusdmbplusmsrB}{\usebox{\MPdotTRdotinvplusdmbplusmsrA}}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrC}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrC}
\begin{minipage}{\MPdotTRdotinvplusdmbplusmsrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TR.inv+dmb+msr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTRdotinvplusdmbplusmsrB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTRdotinvplusdmbplusmsrA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTRdotinvplusdmbplusmsrC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusmsrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusmsrK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusmsrM}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusmsrO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R2=1 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.TTf.inv+dmb+addr.tex <==
\newlength{\MPdotTTfdotinvplusdmbplusaddrH}
\setlength{\MPdotTTfdotinvplusdmbplusaddrH}{0cm}
\newsavebox{\MPdotTTfdotinvplusdmbplusaddrI}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusaddrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbplusaddrJ}
\settowidth{\MPdotTTfdotinvplusdmbplusaddrJ}{\usebox{\MPdotTTfdotinvplusdmbplusaddrI}}
\addtolength{\MPdotTTfdotinvplusdmbplusaddrH}{\MPdotTTfdotinvplusdmbplusaddrJ}
\newsavebox{\MPdotTTfdotinvplusdmbplusaddrK}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusaddrK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
EOR X4,X0,X0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbplusaddrL}
\settowidth{\MPdotTTfdotinvplusdmbplusaddrL}{\usebox{\MPdotTTfdotinvplusdmbplusaddrK}}
\addtolength{\MPdotTTfdotinvplusdmbplusaddrH}{\MPdotTTfdotinvplusdmbplusaddrL}
\newsavebox{\MPdotTTfdotinvplusdmbplusaddrM}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusaddrM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbplusaddrN}
\settowidth{\MPdotTTfdotinvplusdmbplusaddrN}{\usebox{\MPdotTTfdotinvplusdmbplusaddrM}}
\addtolength{\MPdotTTfdotinvplusdmbplusaddrH}{\MPdotTTfdotinvplusdmbplusaddrN}
\newsavebox{\MPdotTTfdotinvplusdmbplusaddrO}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusaddrO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbplusaddrP}
\settowidth{\MPdotTTfdotinvplusdmbplusaddrP}{\usebox{\MPdotTTfdotinvplusdmbplusaddrO}}
\newsavebox{\MPdotTTfdotinvplusdmbplusaddrA}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusaddrA}
\begin{minipage}{\MPdotTTfdotinvplusdmbplusaddrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv+dmb+addr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvplusdmbplusaddrP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvplusdmbplusaddrO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvplusdmbplusaddrA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbplusaddrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbplusaddrK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbplusaddrM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.TTf.inv+dmb+dsb-isb.tex <==
\newlength{\MPdotTTfdotinvplusdmbplusdsbisbH}
\setlength{\MPdotTTfdotinvplusdmbplusdsbisbH}{0cm}
\newsavebox{\MPdotTTfdotinvplusdmbplusdsbisbI}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbplusdsbisbJ}
\settowidth{\MPdotTTfdotinvplusdmbplusdsbisbJ}{\usebox{\MPdotTTfdotinvplusdmbplusdsbisbI}}
\addtolength{\MPdotTTfdotinvplusdmbplusdsbisbH}{\MPdotTTfdotinvplusdmbplusdsbisbJ}
\newsavebox{\MPdotTTfdotinvplusdmbplusdsbisbK}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbplusdsbisbL}
\settowidth{\MPdotTTfdotinvplusdmbplusdsbisbL}{\usebox{\MPdotTTfdotinvplusdmbplusdsbisbK}}
\addtolength{\MPdotTTfdotinvplusdmbplusdsbisbH}{\MPdotTTfdotinvplusdmbplusdsbisbL}
\newsavebox{\MPdotTTfdotinvplusdmbplusdsbisbM}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbplusdsbisbN}
\settowidth{\MPdotTTfdotinvplusdmbplusdsbisbN}{\usebox{\MPdotTTfdotinvplusdmbplusdsbisbM}}
\addtolength{\MPdotTTfdotinvplusdmbplusdsbisbH}{\MPdotTTfdotinvplusdmbplusdsbisbN}
\newsavebox{\MPdotTTfdotinvplusdmbplusdsbisbO}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbplusdsbisbP}
\settowidth{\MPdotTTfdotinvplusdmbplusdsbisbP}{\usebox{\MPdotTTfdotinvplusdmbplusdsbisbO}}
\newsavebox{\MPdotTTfdotinvplusdmbplusdsbisbA}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusdsbisbA}
\begin{minipage}{\MPdotTTfdotinvplusdmbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv+dmb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvplusdmbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvplusdmbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvplusdmbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.TTf.inv+dmb+po.tex <==
\newlength{\MPdotTTfdotinvplusdmbpluspoH}
\setlength{\MPdotTTfdotinvplusdmbpluspoH}{0cm}
\newsavebox{\MPdotTTfdotinvplusdmbpluspoI}
\begin{lrbox}{\MPdotTTfdotinvplusdmbpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbpluspoJ}
\settowidth{\MPdotTTfdotinvplusdmbpluspoJ}{\usebox{\MPdotTTfdotinvplusdmbpluspoI}}
\addtolength{\MPdotTTfdotinvplusdmbpluspoH}{\MPdotTTfdotinvplusdmbpluspoJ}
\newsavebox{\MPdotTTfdotinvplusdmbpluspoK}
\begin{lrbox}{\MPdotTTfdotinvplusdmbpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbpluspoL}
\settowidth{\MPdotTTfdotinvplusdmbpluspoL}{\usebox{\MPdotTTfdotinvplusdmbpluspoK}}
\addtolength{\MPdotTTfdotinvplusdmbpluspoH}{\MPdotTTfdotinvplusdmbpluspoL}
\newsavebox{\MPdotTTfdotinvplusdmbpluspoM}
\begin{lrbox}{\MPdotTTfdotinvplusdmbpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbpluspoN}
\settowidth{\MPdotTTfdotinvplusdmbpluspoN}{\usebox{\MPdotTTfdotinvplusdmbpluspoM}}
\addtolength{\MPdotTTfdotinvplusdmbpluspoH}{\MPdotTTfdotinvplusdmbpluspoN}
\newsavebox{\MPdotTTfdotinvplusdmbpluspoO}
\begin{lrbox}{\MPdotTTfdotinvplusdmbpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbpluspoP}
\settowidth{\MPdotTTfdotinvplusdmbpluspoP}{\usebox{\MPdotTTfdotinvplusdmbpluspoO}}
\newsavebox{\MPdotTTfdotinvplusdmbpluspoA}
\begin{lrbox}{\MPdotTTfdotinvplusdmbpluspoA}
\begin{minipage}{\MPdotTTfdotinvplusdmbpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv+dmb+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvplusdmbpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvplusdmbpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvplusdmbpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.TTf.inv+dsb+ctrl-isb.tex <==
\newlength{\MPdotTTfdotinvplusdsbplusctrlisbH}
\setlength{\MPdotTTfdotinvplusdsbplusctrlisbH}{0cm}
\newsavebox{\MPdotTTfdotinvplusdsbplusctrlisbI}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusctrlisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbplusctrlisbJ}
\settowidth{\MPdotTTfdotinvplusdsbplusctrlisbJ}{\usebox{\MPdotTTfdotinvplusdsbplusctrlisbI}}
\addtolength{\MPdotTTfdotinvplusdsbplusctrlisbH}{\MPdotTTfdotinvplusdsbplusctrlisbJ}
\newsavebox{\MPdotTTfdotinvplusdsbplusctrlisbK}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusctrlisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
CBNZ X0,L0
L0:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbplusctrlisbL}
\settowidth{\MPdotTTfdotinvplusdsbplusctrlisbL}{\usebox{\MPdotTTfdotinvplusdsbplusctrlisbK}}
\addtolength{\MPdotTTfdotinvplusdsbplusctrlisbH}{\MPdotTTfdotinvplusdsbplusctrlisbL}
\newsavebox{\MPdotTTfdotinvplusdsbplusctrlisbM}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusctrlisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbplusctrlisbN}
\settowidth{\MPdotTTfdotinvplusdsbplusctrlisbN}{\usebox{\MPdotTTfdotinvplusdsbplusctrlisbM}}
\addtolength{\MPdotTTfdotinvplusdsbplusctrlisbH}{\MPdotTTfdotinvplusdsbplusctrlisbN}
\newsavebox{\MPdotTTfdotinvplusdsbplusctrlisbO}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusctrlisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbplusctrlisbP}
\settowidth{\MPdotTTfdotinvplusdsbplusctrlisbP}{\usebox{\MPdotTTfdotinvplusdsbplusctrlisbO}}
\newsavebox{\MPdotTTfdotinvplusdsbplusctrlisbA}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusctrlisbA}
\begin{minipage}{\MPdotTTfdotinvplusdsbplusctrlisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv+dsb+ctrl-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvplusdsbplusctrlisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvplusdsbplusctrlisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvplusdsbplusctrlisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbplusctrlisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbplusctrlisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbplusctrlisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.TTf.inv+dsb+dsb-isb.tex <==
\newlength{\MPdotTTfdotinvplusdsbplusdsbisbH}
\setlength{\MPdotTTfdotinvplusdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotTTfdotinvplusdsbplusdsbisbI}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbplusdsbisbJ}
\settowidth{\MPdotTTfdotinvplusdsbplusdsbisbJ}{\usebox{\MPdotTTfdotinvplusdsbplusdsbisbI}}
\addtolength{\MPdotTTfdotinvplusdsbplusdsbisbH}{\MPdotTTfdotinvplusdsbplusdsbisbJ}
\newsavebox{\MPdotTTfdotinvplusdsbplusdsbisbK}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbplusdsbisbL}
\settowidth{\MPdotTTfdotinvplusdsbplusdsbisbL}{\usebox{\MPdotTTfdotinvplusdsbplusdsbisbK}}
\addtolength{\MPdotTTfdotinvplusdsbplusdsbisbH}{\MPdotTTfdotinvplusdsbplusdsbisbL}
\newsavebox{\MPdotTTfdotinvplusdsbplusdsbisbM}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbplusdsbisbN}
\settowidth{\MPdotTTfdotinvplusdsbplusdsbisbN}{\usebox{\MPdotTTfdotinvplusdsbplusdsbisbM}}
\addtolength{\MPdotTTfdotinvplusdsbplusdsbisbH}{\MPdotTTfdotinvplusdsbplusdsbisbN}
\newsavebox{\MPdotTTfdotinvplusdsbplusdsbisbO}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbplusdsbisbP}
\settowidth{\MPdotTTfdotinvplusdsbplusdsbisbP}{\usebox{\MPdotTTfdotinvplusdsbplusdsbisbO}}
\newsavebox{\MPdotTTfdotinvplusdsbplusdsbisbA}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusdsbisbA}
\begin{minipage}{\MPdotTTfdotinvplusdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv+dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvplusdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvplusdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvplusdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.TTf.inv+dsb+po.tex <==
\newlength{\MPdotTTfdotinvplusdsbpluspoH}
\setlength{\MPdotTTfdotinvplusdsbpluspoH}{0cm}
\newsavebox{\MPdotTTfdotinvplusdsbpluspoI}
\begin{lrbox}{\MPdotTTfdotinvplusdsbpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbpluspoJ}
\settowidth{\MPdotTTfdotinvplusdsbpluspoJ}{\usebox{\MPdotTTfdotinvplusdsbpluspoI}}
\addtolength{\MPdotTTfdotinvplusdsbpluspoH}{\MPdotTTfdotinvplusdsbpluspoJ}
\newsavebox{\MPdotTTfdotinvplusdsbpluspoK}
\begin{lrbox}{\MPdotTTfdotinvplusdsbpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbpluspoL}
\settowidth{\MPdotTTfdotinvplusdsbpluspoL}{\usebox{\MPdotTTfdotinvplusdsbpluspoK}}
\addtolength{\MPdotTTfdotinvplusdsbpluspoH}{\MPdotTTfdotinvplusdsbpluspoL}
\newsavebox{\MPdotTTfdotinvplusdsbpluspoM}
\begin{lrbox}{\MPdotTTfdotinvplusdsbpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbpluspoN}
\settowidth{\MPdotTTfdotinvplusdsbpluspoN}{\usebox{\MPdotTTfdotinvplusdsbpluspoM}}
\addtolength{\MPdotTTfdotinvplusdsbpluspoH}{\MPdotTTfdotinvplusdsbpluspoN}
\newsavebox{\MPdotTTfdotinvplusdsbpluspoO}
\begin{lrbox}{\MPdotTTfdotinvplusdsbpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbpluspoP}
\settowidth{\MPdotTTfdotinvplusdsbpluspoP}{\usebox{\MPdotTTfdotinvplusdsbpluspoO}}
\newsavebox{\MPdotTTfdotinvplusdsbpluspoA}
\begin{lrbox}{\MPdotTTfdotinvplusdsbpluspoA}
\begin{minipage}{\MPdotTTfdotinvplusdsbpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv+dsb+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvplusdsbpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvplusdsbpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvplusdsbpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.TTf.inv+dsbs.tex <==
\newlength{\MPdotTTfdotinvplusdsbsH}
\setlength{\MPdotTTfdotinvplusdsbsH}{0cm}
\newsavebox{\MPdotTTfdotinvplusdsbsI}
\begin{lrbox}{\MPdotTTfdotinvplusdsbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbsJ}
\settowidth{\MPdotTTfdotinvplusdsbsJ}{\usebox{\MPdotTTfdotinvplusdsbsI}}
\addtolength{\MPdotTTfdotinvplusdsbsH}{\MPdotTTfdotinvplusdsbsJ}
\newsavebox{\MPdotTTfdotinvplusdsbsK}
\begin{lrbox}{\MPdotTTfdotinvplusdsbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbsL}
\settowidth{\MPdotTTfdotinvplusdsbsL}{\usebox{\MPdotTTfdotinvplusdsbsK}}
\addtolength{\MPdotTTfdotinvplusdsbsH}{\MPdotTTfdotinvplusdsbsL}
\newsavebox{\MPdotTTfdotinvplusdsbsM}
\begin{lrbox}{\MPdotTTfdotinvplusdsbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbsN}
\settowidth{\MPdotTTfdotinvplusdsbsN}{\usebox{\MPdotTTfdotinvplusdsbsM}}
\addtolength{\MPdotTTfdotinvplusdsbsH}{\MPdotTTfdotinvplusdsbsN}
\newsavebox{\MPdotTTfdotinvplusdsbsO}
\begin{lrbox}{\MPdotTTfdotinvplusdsbsO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbsP}
\settowidth{\MPdotTTfdotinvplusdsbsP}{\usebox{\MPdotTTfdotinvplusdsbsO}}
\newsavebox{\MPdotTTfdotinvplusdsbsA}
\begin{lrbox}{\MPdotTTfdotinvplusdsbsA}
\begin{minipage}{\MPdotTTfdotinvplusdsbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv+dsbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvplusdsbsP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvplusdsbsO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvplusdsbsA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbsK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbsM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.TTf.inv.EL1+dsb-tlbiis-dsb+dmb.tex <==
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}
\setlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{0cm}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}
\begin{minipage}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv.EL1+dsb-tlbiis-dsb+dmb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.TTf.inv.EL1+dsb-tlbiis-dsb+dsb-isb.tex <==
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}
\setlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbI}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbJ}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbJ}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbI}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbJ}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbK}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbL}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbL}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbK}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbL}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbM}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbN}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbN}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbM}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbN}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbO}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbP}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbP}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbO}}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbA}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbA}
\begin{minipage}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv.EL1+dsb-tlbiis-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.TTf.inv.EL1+dsb-tlbiis-dsb+po.tex <==
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}
\setlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}{0cm}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoI}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoJ}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoJ}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoI}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoJ}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoK}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoL}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoL}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoK}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoL}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoM}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoN}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoN}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoM}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoN}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoO}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoP}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoP}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoO}}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoA}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoA}
\begin{minipage}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv.EL1+dsb-tlbiis-dsb+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.TfR+dmb+eret.tex <==
\newlength{\MPdotTfRplusdmbpluseretH}
\setlength{\MPdotTfRplusdmbpluseretH}{0cm}
\newsavebox{\MPdotTfRplusdmbpluseretI}
\begin{lrbox}{\MPdotTfRplusdmbpluseretI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTfRplusdmbpluseretJ}
\settowidth{\MPdotTfRplusdmbpluseretJ}{\usebox{\MPdotTfRplusdmbpluseretI}}
\addtolength{\MPdotTfRplusdmbpluseretH}{\MPdotTfRplusdmbpluseretJ}
\newsavebox{\MPdotTfRplusdmbpluseretK}
\begin{lrbox}{\MPdotTfRplusdmbpluseretK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
LDR X4,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTfRplusdmbpluseretL}
\settowidth{\MPdotTfRplusdmbpluseretL}{\usebox{\MPdotTfRplusdmbpluseretK}}
\addtolength{\MPdotTfRplusdmbpluseretH}{\MPdotTfRplusdmbpluseretL}
\newsavebox{\MPdotTfRplusdmbpluseretM}
\begin{lrbox}{\MPdotTfRplusdmbpluseretM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTfRplusdmbpluseretN}
\settowidth{\MPdotTfRplusdmbpluseretN}{\usebox{\MPdotTfRplusdmbpluseretM}}
\addtolength{\MPdotTfRplusdmbpluseretH}{\MPdotTfRplusdmbpluseretN}
\newsavebox{\MPdotTfRplusdmbpluseretO}
\begin{lrbox}{\MPdotTfRplusdmbpluseretO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;

    y |-> pa2;
    y ?-> invalid;

    *pa1 = 0;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTfRplusdmbpluseretP}
\settowidth{\MPdotTfRplusdmbpluseretP}{\usebox{\MPdotTfRplusdmbpluseretO}}
\newsavebox{\MPdotTfRplusdmbpluseretA}
\begin{lrbox}{\MPdotTfRplusdmbpluseretA}
\begin{minipage}{\MPdotTfRplusdmbpluseretH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TfR+dmb+eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTfRplusdmbpluseretP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTfRplusdmbpluseretO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTfRplusdmbpluseretA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTfRplusdmbpluseretI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTfRplusdmbpluseretK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTfRplusdmbpluseretM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R2=0 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/MP.alias3+rfi-data+dmb.tex <==
\newlength{\MPdotaliasthreeplusrfidataplusdmbH}
\setlength{\MPdotaliasthreeplusrfidataplusdmbH}{0cm}
\newsavebox{\MPdotaliasthreeplusrfidataplusdmbI}
\begin{lrbox}{\MPdotaliasthreeplusrfidataplusdmbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
STR X2,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotaliasthreeplusrfidataplusdmbJ}
\settowidth{\MPdotaliasthreeplusrfidataplusdmbJ}{\usebox{\MPdotaliasthreeplusrfidataplusdmbI}}
\addtolength{\MPdotaliasthreeplusrfidataplusdmbH}{\MPdotaliasthreeplusrfidataplusdmbJ}
\newsavebox{\MPdotaliasthreeplusrfidataplusdmbK}
\begin{lrbox}{\MPdotaliasthreeplusrfidataplusdmbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotaliasthreeplusrfidataplusdmbL}
\settowidth{\MPdotaliasthreeplusrfidataplusdmbL}{\usebox{\MPdotaliasthreeplusrfidataplusdmbK}}
\addtolength{\MPdotaliasthreeplusrfidataplusdmbH}{\MPdotaliasthreeplusrfidataplusdmbL}
\newsavebox{\MPdotaliasthreeplusrfidataplusdmbM}
\begin{lrbox}{\MPdotaliasthreeplusrfidataplusdmbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    y |-> pa2;
    z |-> pa1;
    *pa1 = 0;
    *pa2 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotaliasthreeplusrfidataplusdmbN}
\settowidth{\MPdotaliasthreeplusrfidataplusdmbN}{\usebox{\MPdotaliasthreeplusrfidataplusdmbM}}
\newsavebox{\MPdotaliasthreeplusrfidataplusdmbO}
\begin{lrbox}{\MPdotaliasthreeplusrfidataplusdmbO}
\begin{minipage}{\MPdotaliasthreeplusrfidataplusdmbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R3=z|\\
\lstinline[language=IslaLitmusExp]|0:R5=y|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.alias3+rfi-data+dmb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotaliasthreeplusrfidataplusdmbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotaliasthreeplusrfidataplusdmbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotaliasthreeplusrfidataplusdmbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotaliasthreeplusrfidataplusdmbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotaliasthreeplusrfidataplusdmbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/PPOAA.alias.tex <==
\newlength{\PPOAAdotaliasH}
\setlength{\PPOAAdotaliasH}{0cm}
\newsavebox{\PPOAAdotaliasI}
\begin{lrbox}{\PPOAAdotaliasI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\PPOAAdotaliasJ}
\settowidth{\PPOAAdotaliasJ}{\usebox{\PPOAAdotaliasI}}
\addtolength{\PPOAAdotaliasH}{\PPOAAdotaliasJ}
\newsavebox{\PPOAAdotaliasK}
\begin{lrbox}{\PPOAAdotaliasK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X9,X0,X0
STR X2,[X3,X9]
LDR X4,[X5]
EOR X8,X4,X4
LDR X6,[X7,X8]
\end{lstlisting}
\end{lrbox}
\newlength{\PPOAAdotaliasL}
\settowidth{\PPOAAdotaliasL}{\usebox{\PPOAAdotaliasK}}
\addtolength{\PPOAAdotaliasH}{\PPOAAdotaliasL}
\newsavebox{\PPOAAdotaliasM}
\begin{lrbox}{\PPOAAdotaliasM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    w |-> pa1;
    x |-> pa1;
    y |-> pa2;
    z |-> pa3;
\end{lstlisting}
\end{lrbox}
\newlength{\PPOAAdotaliasN}
\settowidth{\PPOAAdotaliasN}{\usebox{\PPOAAdotaliasM}}
\newsavebox{\PPOAAdotaliasO}
\begin{lrbox}{\PPOAAdotaliasO}
\begin{minipage}{\PPOAAdotaliasH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R1=z|\\
\lstinline[language=IslaLitmusExp]|0:R2=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0x1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=w|\\
\lstinline[language=IslaLitmusExp]|1:R7=z|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|PPOAA.alias|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\PPOAAdotaliasN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\PPOAAdotaliasM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\PPOAAdotaliasO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\PPOAAdotaliasI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\PPOAAdotaliasK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R4=1 & 1:R6=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/PPOCA.alias.tex <==
\newlength{\PPOCAdotaliasH}
\setlength{\PPOCAdotaliasH}{0cm}
\newsavebox{\PPOCAdotaliasI}
\begin{lrbox}{\PPOCAdotaliasI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\PPOCAdotaliasJ}
\settowidth{\PPOCAdotaliasJ}{\usebox{\PPOCAdotaliasI}}
\addtolength{\PPOCAdotaliasH}{\PPOCAdotaliasJ}
\newsavebox{\PPOCAdotaliasK}
\begin{lrbox}{\PPOCAdotaliasK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBNZ X0,L0
L0:
STR X2,[X3]
LDR X4,[X5]
EOR X8,X4,X4
LDR X6,[X7,X8]
\end{lstlisting}
\end{lrbox}
\newlength{\PPOCAdotaliasL}
\settowidth{\PPOCAdotaliasL}{\usebox{\PPOCAdotaliasK}}
\addtolength{\PPOCAdotaliasH}{\PPOCAdotaliasL}
\newsavebox{\PPOCAdotaliasM}
\begin{lrbox}{\PPOCAdotaliasM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    w |-> pa1;
    x |-> pa1;
    y |-> pa2;
    z |-> pa3;
    *pa1 = 0;
    *pa2 = 0;
    *pa3 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\PPOCAdotaliasN}
\settowidth{\PPOCAdotaliasN}{\usebox{\PPOCAdotaliasM}}
\newsavebox{\PPOCAdotaliasO}
\begin{lrbox}{\PPOCAdotaliasO}
\begin{minipage}{\PPOCAdotaliasH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R1=z|\\
\lstinline[language=IslaLitmusExp]|0:R2=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0x1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=w|\\
\lstinline[language=IslaLitmusExp]|1:R7=z|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|PPOCA.alias|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\PPOCAdotaliasN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\PPOCAdotaliasM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\PPOCAdotaliasO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\PPOCAdotaliasI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\PPOCAdotaliasK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R4=1 & 1:R6=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/PPODA.RT.inv.tex <==
\newlength{\PPODAdotRTdotinvH}
\setlength{\PPODAdotRTdotinvH}{0cm}
\newsavebox{\PPODAdotRTdotinvI}
\begin{lrbox}{\PPODAdotRTdotinvI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\PPODAdotRTdotinvJ}
\settowidth{\PPODAdotRTdotinvJ}{\usebox{\PPODAdotRTdotinvI}}
\addtolength{\PPODAdotRTdotinvH}{\PPODAdotRTdotinvJ}
\newsavebox{\PPODAdotRTdotinvK}
\begin{lrbox}{\PPODAdotRTdotinvK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
ORR X2,X2,X3
STR X2,[X4]
LDR X6,[X5]
EOR X8,X6,X6
LDR X9,[X7,X8]
\end{lstlisting}
\end{lrbox}
\newlength{\PPODAdotRTdotinvL}
\settowidth{\PPODAdotRTdotinvL}{\usebox{\PPODAdotRTdotinvK}}
\addtolength{\PPODAdotRTdotinvH}{\PPODAdotRTdotinvL}
\newsavebox{\PPODAdotRTdotinvM}
\begin{lrbox}{\PPODAdotRTdotinvM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X6,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\PPODAdotRTdotinvN}
\settowidth{\PPODAdotRTdotinvN}{\usebox{\PPODAdotRTdotinvM}}
\addtolength{\PPODAdotRTdotinvH}{\PPODAdotRTdotinvN}
\newsavebox{\PPODAdotRTdotinvO}
\begin{lrbox}{\PPODAdotRTdotinvO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    w |-> pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa2;
    z |-> pa3;
    *pa1 = 1;
    *pa2 = 0;
    *pa3 = 0;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\PPODAdotRTdotinvP}
\settowidth{\PPODAdotRTdotinvP}{\usebox{\PPODAdotRTdotinvO}}
\newsavebox{\PPODAdotRTdotinvA}
\begin{lrbox}{\PPODAdotRTdotinvA}
\begin{minipage}{\PPODAdotRTdotinvH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R1=z|\\
\lstinline[language=IslaLitmusExp]|0:R2=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=desc3(w,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R4=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R5=x|\\
\lstinline[language=IslaLitmusExp]|1:R7=z|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|PPODA.RT.inv|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\PPODAdotRTdotinvP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\PPODAdotRTdotinvO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\PPODAdotRTdotinvA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\PPODAdotRTdotinvI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\PPODAdotRTdotinvK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\PPODAdotRTdotinvM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R6=1 & 1:R9=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/R.RTf.inv.EL1+dsb-tlbiis-dsb+popl.tex <==
\newlength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}
\setlength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}{0cm}
\newsavebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplI}
\begin{lrbox}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplJ}
\settowidth{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplJ}{\usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplI}}
\addtolength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplJ}
\newsavebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplK}
\begin{lrbox}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplK}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
STLR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplL}
\settowidth{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplL}{\usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplK}}
\addtolength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplL}
\newsavebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplM}
\begin{lrbox}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplN}
\settowidth{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplN}{\usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplM}}
\addtolength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplN}
\newsavebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplO}
\begin{lrbox}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplP}
\settowidth{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplP}{\usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplO}}
\newsavebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplA}
\begin{lrbox}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplA}
\begin{minipage}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R0=0x2|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|R.RTf.inv.EL1+dsb-tlbiis-dsb+popl|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|y=2 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/R.inv.tex <==
\newlength{\RdotinvH}
\setlength{\RdotinvH}{0cm}
\newsavebox{\RdotinvI}
\begin{lrbox}{\RdotinvI}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\RdotinvJ}
\settowidth{\RdotinvJ}{\usebox{\RdotinvI}}
\addtolength{\RdotinvH}{\RdotinvJ}
\newsavebox{\RdotinvK}
\begin{lrbox}{\RdotinvK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\RdotinvL}
\settowidth{\RdotinvL}{\usebox{\RdotinvK}}
\addtolength{\RdotinvH}{\RdotinvL}
\newsavebox{\RdotinvM}
\begin{lrbox}{\RdotinvM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    identity 0x1000 with code;
    *pa1 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\RdotinvN}
\settowidth{\RdotinvN}{\usebox{\RdotinvM}}
\newsavebox{\RdotinvO}
\begin{lrbox}{\RdotinvO}
\begin{minipage}{\RdotinvH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|R.inv|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\RdotinvN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\RdotinvM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\RdotinvO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\RdotinvI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\RdotinvK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R0=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/RBS+dsb-tlbiis-dsb.tex <==
\newlength{\RBSplusdsbtlbiisdsbH}
\setlength{\RBSplusdsbtlbiisdsbH}{0cm}
\newsavebox{\RBSplusdsbtlbiisdsbI}
\begin{lrbox}{\RBSplusdsbtlbiisdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X5
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\RBSplusdsbtlbiisdsbJ}
\settowidth{\RBSplusdsbtlbiisdsbJ}{\usebox{\RBSplusdsbtlbiisdsbI}}
\addtolength{\RBSplusdsbtlbiisdsbH}{\RBSplusdsbtlbiisdsbJ}
\newsavebox{\RBSplusdsbtlbiisdsbK}
\begin{lrbox}{\RBSplusdsbtlbiisdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\RBSplusdsbtlbiisdsbL}
\settowidth{\RBSplusdsbtlbiisdsbL}{\usebox{\RBSplusdsbtlbiisdsbK}}
\addtolength{\RBSplusdsbtlbiisdsbH}{\RBSplusdsbtlbiisdsbL}
\newsavebox{\RBSplusdsbtlbiisdsbM}
\begin{lrbox}{\RBSplusdsbtlbiisdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\RBSplusdsbtlbiisdsbN}
\settowidth{\RBSplusdsbtlbiisdsbN}{\usebox{\RBSplusdsbtlbiisdsbM}}
\addtolength{\RBSplusdsbtlbiisdsbH}{\RBSplusdsbtlbiisdsbN}
\newsavebox{\RBSplusdsbtlbiisdsbO}
\begin{lrbox}{\RBSplusdsbtlbiisdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;
    y |-> pa1;
    *pa1 = 0;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\RBSplusdsbtlbiisdsbP}
\settowidth{\RBSplusdsbtlbiisdsbP}{\usebox{\RBSplusdsbtlbiisdsbO}}
\newsavebox{\RBSplusdsbtlbiisdsbA}
\begin{lrbox}{\RBSplusdsbtlbiisdsbA}
\begin{minipage}{\RBSplusdsbtlbiisdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0x2|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R5=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|RBS+dsb-tlbiis-dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\RBSplusdsbtlbiisdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\RBSplusdsbtlbiisdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\RBSplusdsbtlbiisdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\RBSplusdsbtlbiisdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\RBSplusdsbtlbiisdsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\RBSplusdsbtlbiisdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=2|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/RDW.alias.tex <==
\newlength{\RDWdotaliasH}
\setlength{\RDWdotaliasH}{0cm}
\newsavebox{\RDWdotaliasI}
\begin{lrbox}{\RDWdotaliasI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\RDWdotaliasJ}
\settowidth{\RDWdotaliasJ}{\usebox{\RDWdotaliasI}}
\addtolength{\RDWdotaliasH}{\RDWdotaliasJ}
\newsavebox{\RDWdotaliasK}
\begin{lrbox}{\RDWdotaliasK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
LDR X3,[X4,X2]
LDR X5,[X6]
EOR X7,X5,X5
LDR X8,[X9,X7]
\end{lstlisting}
\end{lrbox}
\newlength{\RDWdotaliasL}
\settowidth{\RDWdotaliasL}{\usebox{\RDWdotaliasK}}
\addtolength{\RDWdotaliasH}{\RDWdotaliasL}
\newsavebox{\RDWdotaliasM}
\begin{lrbox}{\RDWdotaliasM}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\RDWdotaliasN}
\settowidth{\RDWdotaliasN}{\usebox{\RDWdotaliasM}}
\addtolength{\RDWdotaliasH}{\RDWdotaliasN}
\newsavebox{\RDWdotaliasO}
\begin{lrbox}{\RDWdotaliasO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    w |-> pa1;
    x |-> pa1;
    y |-> pa2;
    z |-> pa3;
    *pa1 = 0;
    *pa2 = 0;
    *pa3 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\RDWdotaliasP}
\settowidth{\RDWdotaliasP}{\usebox{\RDWdotaliasO}}
\newsavebox{\RDWdotaliasA}
\begin{lrbox}{\RDWdotaliasA}
\begin{minipage}{\RDWdotaliasH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=z|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R4=w|\\
\lstinline[language=IslaLitmusExp]|1:R6=x|\\
\lstinline[language=IslaLitmusExp]|1:R9=z|\\
\lstinline[language=IslaLitmusExp]|2:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|2:R1=x|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|RDW.alias|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\RDWdotaliasP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\RDWdotaliasO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\RDWdotaliasA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\RDWdotaliasI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\RDWdotaliasK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\RDWdotaliasM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R3=0 & 1:R5=1 & 1:R8=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/ROT.inv+dmbst.tex <==
\newlength{\ROTdotinvplusdmbstH}
\setlength{\ROTdotinvplusdmbstH}{0cm}
\newsavebox{\ROTdotinvplusdmbstI}
\begin{lrbox}{\ROTdotinvplusdmbstI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB ST
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvplusdmbstJ}
\settowidth{\ROTdotinvplusdmbstJ}{\usebox{\ROTdotinvplusdmbstI}}
\addtolength{\ROTdotinvplusdmbstH}{\ROTdotinvplusdmbstJ}
\newsavebox{\ROTdotinvplusdmbstK}
\begin{lrbox}{\ROTdotinvplusdmbstK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvplusdmbstL}
\settowidth{\ROTdotinvplusdmbstL}{\usebox{\ROTdotinvplusdmbstK}}
\addtolength{\ROTdotinvplusdmbstH}{\ROTdotinvplusdmbstL}
\newsavebox{\ROTdotinvplusdmbstM}
\begin{lrbox}{\ROTdotinvplusdmbstM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS x14,esr_el1
AND X14,X14,#0b111
CMP x14,#0b111
MOV X17,#1
MOV X18,#2
// if ESR_EL1.ISS.DFSC == Translation Level 3 then x2 = 1 else x2 = 2
CSEL x0,x17,x18,eq
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvplusdmbstN}
\settowidth{\ROTdotinvplusdmbstN}{\usebox{\ROTdotinvplusdmbstM}}
\addtolength{\ROTdotinvplusdmbstH}{\ROTdotinvplusdmbstN}
\newsavebox{\ROTdotinvplusdmbstO}
\begin{lrbox}{\ROTdotinvplusdmbstO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
physical pa1;
intermediate ipa1;

assert pa1 == ipa1;
ipa1 |-> pa1;

s1table new_table 0x280000 {
  x |-> invalid;
  x ?-> ipa1;
};

identity 0x283000 with default;

x |-> invalid at level 2;
x ?-> table(0x283000) at level 2;

identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvplusdmbstP}
\settowidth{\ROTdotinvplusdmbstP}{\usebox{\ROTdotinvplusdmbstO}}
\newsavebox{\ROTdotinvplusdmbstA}
\begin{lrbox}{\ROTdotinvplusdmbstA}
\begin{minipage}{\ROTdotinvplusdmbstH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=ipa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,new_table)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc2(table=0x283000)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte2(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|ROT.inv+dmbst|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\ROTdotinvplusdmbstP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\ROTdotinvplusdmbstO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\ROTdotinvplusdmbstA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\ROTdotinvplusdmbstI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\ROTdotinvplusdmbstK}\\
  \cline{2-2}
  & thread 1 el1 handler\\
  \cline{2-2}
  & \usebox{\ROTdotinvplusdmbstM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/ROT.inv+dsb.tex <==
\newlength{\ROTdotinvplusdsbH}
\setlength{\ROTdotinvplusdsbH}{0cm}
\newsavebox{\ROTdotinvplusdsbI}
\begin{lrbox}{\ROTdotinvplusdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvplusdsbJ}
\settowidth{\ROTdotinvplusdsbJ}{\usebox{\ROTdotinvplusdsbI}}
\addtolength{\ROTdotinvplusdsbH}{\ROTdotinvplusdsbJ}
\newsavebox{\ROTdotinvplusdsbK}
\begin{lrbox}{\ROTdotinvplusdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvplusdsbL}
\settowidth{\ROTdotinvplusdsbL}{\usebox{\ROTdotinvplusdsbK}}
\addtolength{\ROTdotinvplusdsbH}{\ROTdotinvplusdsbL}
\newsavebox{\ROTdotinvplusdsbM}
\begin{lrbox}{\ROTdotinvplusdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS X14,ESR_EL1
AND X14,X14,#0b111
CMP X14,#0b111
MOV X17,#1
MOV X18,#2
// if ESR_EL1.ISS.DFSC == Translation Level 3 then x2 = 1 else x2 = 2
CSEL X0,X17,X18,eq
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvplusdsbN}
\settowidth{\ROTdotinvplusdsbN}{\usebox{\ROTdotinvplusdsbM}}
\addtolength{\ROTdotinvplusdsbH}{\ROTdotinvplusdsbN}
\newsavebox{\ROTdotinvplusdsbO}
\begin{lrbox}{\ROTdotinvplusdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
physical pa1;
intermediate ipa1;

assert pa1 == ipa1;
ipa1 |-> pa1;

s1table new_table 0x280000 {
  x |-> invalid;
  x ?-> ipa1;
};

identity 0x283000 with default;

x |-> invalid at level 2;
x ?-> table(0x283000) at level 2;

identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvplusdsbP}
\settowidth{\ROTdotinvplusdsbP}{\usebox{\ROTdotinvplusdsbO}}
\newsavebox{\ROTdotinvplusdsbA}
\begin{lrbox}{\ROTdotinvplusdsbA}
\begin{minipage}{\ROTdotinvplusdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=ipa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,new_table)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc2(table=0x283000)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte2(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|ROT.inv+dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\ROTdotinvplusdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\ROTdotinvplusdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\ROTdotinvplusdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\ROTdotinvplusdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\ROTdotinvplusdsbK}\\
  \cline{2-2}
  & thread 1 el1 handler\\
  \cline{2-2}
  & \usebox{\ROTdotinvplusdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/ROT.inv+po.tex <==
\newlength{\ROTdotinvpluspoH}
\setlength{\ROTdotinvpluspoH}{0cm}
\newsavebox{\ROTdotinvpluspoI}
\begin{lrbox}{\ROTdotinvpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvpluspoJ}
\settowidth{\ROTdotinvpluspoJ}{\usebox{\ROTdotinvpluspoI}}
\addtolength{\ROTdotinvpluspoH}{\ROTdotinvpluspoJ}
\newsavebox{\ROTdotinvpluspoK}
\begin{lrbox}{\ROTdotinvpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvpluspoL}
\settowidth{\ROTdotinvpluspoL}{\usebox{\ROTdotinvpluspoK}}
\addtolength{\ROTdotinvpluspoH}{\ROTdotinvpluspoL}
\newsavebox{\ROTdotinvpluspoM}
\begin{lrbox}{\ROTdotinvpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS X14,ESR_EL1
AND X14,X14,#0b111
CMP X14,#0b111
MOV X17,#1
MOV X18,#2
// if ESR_EL1.ISS.DFSC == Translation Level 3 then x2 = 1 else x2 = 2
CSEL X0,X17,X18,eq
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvpluspoN}
\settowidth{\ROTdotinvpluspoN}{\usebox{\ROTdotinvpluspoM}}
\addtolength{\ROTdotinvpluspoH}{\ROTdotinvpluspoN}
\newsavebox{\ROTdotinvpluspoO}
\begin{lrbox}{\ROTdotinvpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
physical pa1;
intermediate ipa1;

assert pa1 == ipa1;
ipa1 |-> pa1;

s1table new_table 0x280000 {
  x |-> invalid;
  x ?-> ipa1;
};

identity 0x283000 with default;

x |-> invalid at level 2;
x ?-> table(0x283000) at level 2;

identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvpluspoP}
\settowidth{\ROTdotinvpluspoP}{\usebox{\ROTdotinvpluspoO}}
\newsavebox{\ROTdotinvpluspoA}
\begin{lrbox}{\ROTdotinvpluspoA}
\begin{minipage}{\ROTdotinvpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=ipa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,new_table)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc2(table=0x283000)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte2(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|ROT.inv+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\ROTdotinvpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\ROTdotinvpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\ROTdotinvpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\ROTdotinvpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\ROTdotinvpluspoK}\\
  \cline{2-2}
  & thread 1 el1 handler\\
  \cline{2-2}
  & \usebox{\ROTdotinvpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/RSW.alias.tex <==
\newlength{\RSWdotaliasH}
\setlength{\RSWdotaliasH}{0cm}
\newsavebox{\RSWdotaliasI}
\begin{lrbox}{\RSWdotaliasI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\RSWdotaliasJ}
\settowidth{\RSWdotaliasJ}{\usebox{\RSWdotaliasI}}
\addtolength{\RSWdotaliasH}{\RSWdotaliasJ}
\newsavebox{\RSWdotaliasK}
\begin{lrbox}{\RSWdotaliasK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
LDR X3,[X4,X2]
LDR X5,[X6]
EOR X7,X5,X5
LDR X8,[X9,X7]
\end{lstlisting}
\end{lrbox}
\newlength{\RSWdotaliasL}
\settowidth{\RSWdotaliasL}{\usebox{\RSWdotaliasK}}
\addtolength{\RSWdotaliasH}{\RSWdotaliasL}
\newsavebox{\RSWdotaliasM}
\begin{lrbox}{\RSWdotaliasM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    w |-> pa1;
    x |-> pa1;
    y |-> pa2;
    z |-> pa3;
    *pa1 = 0;
    *pa2 = 0;
    *pa3 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\RSWdotaliasN}
\settowidth{\RSWdotaliasN}{\usebox{\RSWdotaliasM}}
\newsavebox{\RSWdotaliasO}
\begin{lrbox}{\RSWdotaliasO}
\begin{minipage}{\RSWdotaliasH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=z|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R4=w|\\
\lstinline[language=IslaLitmusExp]|1:R6=x|\\
\lstinline[language=IslaLitmusExp]|1:R9=z|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|RSW.alias|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\RSWdotaliasN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\RSWdotaliasM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\RSWdotaliasO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\RSWdotaliasI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\RSWdotaliasK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R8=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/RWC.RTR.EL1+dsb-isb+dsb-tlbi-dsb.tex <==
\newlength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbH}
\setlength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbH}{0cm}
\newsavebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbI}
\begin{lrbox}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbJ}
\settowidth{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbJ}{\usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbI}}
\addtolength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbH}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbJ}
\newsavebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbK}
\begin{lrbox}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X3,[X4,X2]
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbL}
\settowidth{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbL}{\usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbK}}
\addtolength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbH}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbL}
\newsavebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbM}
\begin{lrbox}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X2
DSB SY
LDR X3,[X4]
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbN}
\settowidth{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbN}{\usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbM}}
\addtolength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbH}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbN}
\newsavebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbO}
\begin{lrbox}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X3,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbP}
\settowidth{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbP}{\usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbO}}
\addtolength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbH}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbP}
\newsavebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbA}
\begin{lrbox}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;

    y |-> pa2;
    y ?-> invalid;
    z |-> pa2;
    *pa1 = 1;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbB}
\settowidth{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbB}{\usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbA}}
\newsavebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbC}
\begin{lrbox}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbC}
\begin{minipage}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R4=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|2:R1=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R2=page(x)|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|RWC.RTR.EL1+dsb-isb+dsb-tlbi-dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R1=1 & 1:R3=0 & 2:R3=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/RWC.RTfR.inv+addr+dmb.tex <==
\newlength{\RWCdotRTfRdotinvplusaddrplusdmbH}
\setlength{\RWCdotRTfRdotinvplusaddrplusdmbH}{0cm}
\newsavebox{\RWCdotRTfRdotinvplusaddrplusdmbI}
\begin{lrbox}{\RWCdotRTfRdotinvplusaddrplusdmbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTfRdotinvplusaddrplusdmbJ}
\settowidth{\RWCdotRTfRdotinvplusaddrplusdmbJ}{\usebox{\RWCdotRTfRdotinvplusaddrplusdmbI}}
\addtolength{\RWCdotRTfRdotinvplusaddrplusdmbH}{\RWCdotRTfRdotinvplusaddrplusdmbJ}
\newsavebox{\RWCdotRTfRdotinvplusaddrplusdmbK}
\begin{lrbox}{\RWCdotRTfRdotinvplusaddrplusdmbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
LDR X3,[X4,X2]
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTfRdotinvplusaddrplusdmbL}
\settowidth{\RWCdotRTfRdotinvplusaddrplusdmbL}{\usebox{\RWCdotRTfRdotinvplusaddrplusdmbK}}
\addtolength{\RWCdotRTfRdotinvplusaddrplusdmbH}{\RWCdotRTfRdotinvplusaddrplusdmbL}
\newsavebox{\RWCdotRTfRdotinvplusaddrplusdmbM}
\begin{lrbox}{\RWCdotRTfRdotinvplusaddrplusdmbM}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTfRdotinvplusaddrplusdmbN}
\settowidth{\RWCdotRTfRdotinvplusaddrplusdmbN}{\usebox{\RWCdotRTfRdotinvplusaddrplusdmbM}}
\addtolength{\RWCdotRTfRdotinvplusaddrplusdmbH}{\RWCdotRTfRdotinvplusaddrplusdmbN}
\newsavebox{\RWCdotRTfRdotinvplusaddrplusdmbO}
\begin{lrbox}{\RWCdotRTfRdotinvplusaddrplusdmbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X3,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTfRdotinvplusaddrplusdmbP}
\settowidth{\RWCdotRTfRdotinvplusaddrplusdmbP}{\usebox{\RWCdotRTfRdotinvplusaddrplusdmbO}}
\addtolength{\RWCdotRTfRdotinvplusaddrplusdmbH}{\RWCdotRTfRdotinvplusaddrplusdmbP}
\newsavebox{\RWCdotRTfRdotinvplusaddrplusdmbA}
\begin{lrbox}{\RWCdotRTfRdotinvplusaddrplusdmbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;

    y |-> invalid;
    y ?-> pa2;
    z |-> pa2;
    *pa1 = 1;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTfRdotinvplusaddrplusdmbB}
\settowidth{\RWCdotRTfRdotinvplusaddrplusdmbB}{\usebox{\RWCdotRTfRdotinvplusaddrplusdmbA}}
\newsavebox{\RWCdotRTfRdotinvplusaddrplusdmbC}
\begin{lrbox}{\RWCdotRTfRdotinvplusaddrplusdmbC}
\begin{minipage}{\RWCdotRTfRdotinvplusaddrplusdmbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R4=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|2:R1=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|RWC.RTfR.inv+addr+dmb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\RWCdotRTfRdotinvplusaddrplusdmbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\RWCdotRTfRdotinvplusaddrplusdmbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\RWCdotRTfRdotinvplusaddrplusdmbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\RWCdotRTfRdotinvplusaddrplusdmbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\RWCdotRTfRdotinvplusaddrplusdmbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\RWCdotRTfRdotinvplusaddrplusdmbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\RWCdotRTfRdotinvplusaddrplusdmbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R1=1 & 1:R3=0 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/S.RT.ro+dsb-tlbiis-dsb+dsb-isb.tex <==
\newlength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbH}
\setlength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbH}{0cm}
\newsavebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbI}
\begin{lrbox}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbJ}
\settowidth{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbJ}{\usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbI}}
\addtolength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbH}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbJ}
\newsavebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbK}
\begin{lrbox}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbL}
\settowidth{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbL}{\usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbK}}
\addtolength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbH}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbL}
\newsavebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbM}
\begin{lrbox}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbN}
\settowidth{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbN}{\usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbM}}
\addtolength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbH}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbN}
\newsavebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbO}
\begin{lrbox}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1 with [AP = 0b11] and default;
    x ?-> pa1;
    z |-> pa1;
    y |-> pa2;

    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbP}
\settowidth{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbP}{\usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbO}}
\newsavebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbA}
\begin{lrbox}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbA}
\begin{minipage}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|S.RT.ro+dsb-tlbiis-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/S.RTf.inv.EL1+dsb-tlbiis-dsb+ctrl.tex <==
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}
\setlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}{0cm}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlI}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlJ}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlJ}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlI}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlJ}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlK}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBNZ X0,L0
L0:
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlL}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlL}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlK}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlL}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlM}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlN}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlN}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlM}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlN}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlO}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlP}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlP}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlO}}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlA}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlA}
\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|S.RTf.inv.EL1+dsb-tlbiis-dsb+ctrl|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/S.RTf.inv.EL1+dsb-tlbiis-dsb+data.tex <==
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}
\setlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}{0cm}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataI}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataJ}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataJ}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataI}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataJ}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataK}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
ORR X2,X2,X4
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataL}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataL}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataK}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataL}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataM}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataN}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataN}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataM}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataN}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataO}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataP}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataP}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataO}}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataA}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataA}
\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|S.RTf.inv.EL1+dsb-tlbiis-dsb+data|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/S.RTf.inv.EL1+dsb-tlbiis-dsb+dmb.tex <==
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}
\setlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{0cm}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}
\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|S.RTf.inv.EL1+dsb-tlbiis-dsb+dmb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/S.RTf.inv.EL1+dsb-tlbiis-dsb+poap.tex <==
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}
\setlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}{0cm}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapI}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapJ}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapJ}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapI}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapJ}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapK}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDAR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapL}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapL}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapK}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapL}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapM}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapN}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapN}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapM}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapN}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapO}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapP}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapP}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapO}}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapA}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapA}
\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|S.RTf.inv.EL1+dsb-tlbiis-dsb+poap|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/S.RTf.inv.EL1+dsb-tlbiis-dsb+popl.tex <==
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}
\setlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}{0cm}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplI}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplJ}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplJ}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplI}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplJ}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplK}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STLR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplL}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplL}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplK}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplL}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplM}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplN}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplN}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplM}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplN}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplO}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplP}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplP}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplO}}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplA}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplA}
\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|S.RTf.inv.EL1+dsb-tlbiis-dsb+popl|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/S.T+dmb+po.tex <==
\newlength{\SdotTplusdmbpluspoH}
\setlength{\SdotTplusdmbpluspoH}{0cm}
\newsavebox{\SdotTplusdmbpluspoI}
\begin{lrbox}{\SdotTplusdmbpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotTplusdmbpluspoJ}
\settowidth{\SdotTplusdmbpluspoJ}{\usebox{\SdotTplusdmbpluspoI}}
\addtolength{\SdotTplusdmbpluspoH}{\SdotTplusdmbpluspoJ}
\newsavebox{\SdotTplusdmbpluspoK}
\begin{lrbox}{\SdotTplusdmbpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotTplusdmbpluspoL}
\settowidth{\SdotTplusdmbpluspoL}{\usebox{\SdotTplusdmbpluspoK}}
\addtolength{\SdotTplusdmbpluspoH}{\SdotTplusdmbpluspoL}
\newsavebox{\SdotTplusdmbpluspoM}
\begin{lrbox}{\SdotTplusdmbpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SdotTplusdmbpluspoN}
\settowidth{\SdotTplusdmbpluspoN}{\usebox{\SdotTplusdmbpluspoM}}
\addtolength{\SdotTplusdmbpluspoH}{\SdotTplusdmbpluspoN}
\newsavebox{\SdotTplusdmbpluspoO}
\begin{lrbox}{\SdotTplusdmbpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 0;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SdotTplusdmbpluspoP}
\settowidth{\SdotTplusdmbpluspoP}{\usebox{\SdotTplusdmbpluspoO}}
\newsavebox{\SdotTplusdmbpluspoA}
\begin{lrbox}{\SdotTplusdmbpluspoA}
\begin{minipage}{\SdotTplusdmbpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0x2|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|S.T+dmb+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SdotTplusdmbpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SdotTplusdmbpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SdotTplusdmbpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SdotTplusdmbpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SdotTplusdmbpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SdotTplusdmbpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & x=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/SB.TfTf.inv+dmb-ctrl-isbs.tex <==
\newlength{\SBdotTfTfdotinvplusdmbctrlisbsH}
\setlength{\SBdotTfTfdotinvplusdmbctrlisbsH}{0cm}
\newsavebox{\SBdotTfTfdotinvplusdmbctrlisbsI}
\begin{lrbox}{\SBdotTfTfdotinvplusdmbctrlisbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
LDR X7,[X8]
CBNZ X7,L0
L0:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdmbctrlisbsJ}
\settowidth{\SBdotTfTfdotinvplusdmbctrlisbsJ}{\usebox{\SBdotTfTfdotinvplusdmbctrlisbsI}}
\addtolength{\SBdotTfTfdotinvplusdmbctrlisbsH}{\SBdotTfTfdotinvplusdmbctrlisbsJ}
\newsavebox{\SBdotTfTfdotinvplusdmbctrlisbsK}
\begin{lrbox}{\SBdotTfTfdotinvplusdmbctrlisbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
LDR X7,[X8]
CBNZ X7,L1
L1:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdmbctrlisbsL}
\settowidth{\SBdotTfTfdotinvplusdmbctrlisbsL}{\usebox{\SBdotTfTfdotinvplusdmbctrlisbsK}}
\addtolength{\SBdotTfTfdotinvplusdmbctrlisbsH}{\SBdotTfTfdotinvplusdmbctrlisbsL}
\newsavebox{\SBdotTfTfdotinvplusdmbctrlisbsM}
\begin{lrbox}{\SBdotTfTfdotinvplusdmbctrlisbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdmbctrlisbsN}
\settowidth{\SBdotTfTfdotinvplusdmbctrlisbsN}{\usebox{\SBdotTfTfdotinvplusdmbctrlisbsM}}
\addtolength{\SBdotTfTfdotinvplusdmbctrlisbsH}{\SBdotTfTfdotinvplusdmbctrlisbsN}
\newsavebox{\SBdotTfTfdotinvplusdmbctrlisbsO}
\begin{lrbox}{\SBdotTfTfdotinvplusdmbctrlisbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdmbctrlisbsP}
\settowidth{\SBdotTfTfdotinvplusdmbctrlisbsP}{\usebox{\SBdotTfTfdotinvplusdmbctrlisbsO}}
\addtolength{\SBdotTfTfdotinvplusdmbctrlisbsH}{\SBdotTfTfdotinvplusdmbctrlisbsP}
\newsavebox{\SBdotTfTfdotinvplusdmbctrlisbsA}
\begin{lrbox}{\SBdotTfTfdotinvplusdmbctrlisbsA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> invalid;
    y ?-> pa2;
    v |-> pa2;
    *pa2 = 1;

    z |-> pa3;
    *pa3 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdmbctrlisbsB}
\settowidth{\SBdotTfTfdotinvplusdmbctrlisbsB}{\usebox{\SBdotTfTfdotinvplusdmbctrlisbsA}}
\newsavebox{\SBdotTfTfdotinvplusdmbctrlisbsC}
\begin{lrbox}{\SBdotTfTfdotinvplusdmbctrlisbsC}
\begin{minipage}{\SBdotTfTfdotinvplusdmbctrlisbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R8=z|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R0=desc3(v,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R8=z|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|SB.TfTf.inv+dmb-ctrl-isbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SBdotTfTfdotinvplusdmbctrlisbsB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SBdotTfTfdotinvplusdmbctrlisbsA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SBdotTfTfdotinvplusdmbctrlisbsC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvplusdmbctrlisbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvplusdmbctrlisbsK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvplusdmbctrlisbsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvplusdmbctrlisbsO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/SB.TfTf.inv+dsb-isbs.tex <==
\newlength{\SBdotTfTfdotinvplusdsbisbsH}
\setlength{\SBdotTfTfdotinvplusdsbisbsH}{0cm}
\newsavebox{\SBdotTfTfdotinvplusdsbisbsI}
\begin{lrbox}{\SBdotTfTfdotinvplusdsbisbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdsbisbsJ}
\settowidth{\SBdotTfTfdotinvplusdsbisbsJ}{\usebox{\SBdotTfTfdotinvplusdsbisbsI}}
\addtolength{\SBdotTfTfdotinvplusdsbisbsH}{\SBdotTfTfdotinvplusdsbisbsJ}
\newsavebox{\SBdotTfTfdotinvplusdsbisbsK}
\begin{lrbox}{\SBdotTfTfdotinvplusdsbisbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdsbisbsL}
\settowidth{\SBdotTfTfdotinvplusdsbisbsL}{\usebox{\SBdotTfTfdotinvplusdsbisbsK}}
\addtolength{\SBdotTfTfdotinvplusdsbisbsH}{\SBdotTfTfdotinvplusdsbisbsL}
\newsavebox{\SBdotTfTfdotinvplusdsbisbsM}
\begin{lrbox}{\SBdotTfTfdotinvplusdsbisbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdsbisbsN}
\settowidth{\SBdotTfTfdotinvplusdsbisbsN}{\usebox{\SBdotTfTfdotinvplusdsbisbsM}}
\addtolength{\SBdotTfTfdotinvplusdsbisbsH}{\SBdotTfTfdotinvplusdsbisbsN}
\newsavebox{\SBdotTfTfdotinvplusdsbisbsO}
\begin{lrbox}{\SBdotTfTfdotinvplusdsbisbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdsbisbsP}
\settowidth{\SBdotTfTfdotinvplusdsbisbsP}{\usebox{\SBdotTfTfdotinvplusdsbisbsO}}
\addtolength{\SBdotTfTfdotinvplusdsbisbsH}{\SBdotTfTfdotinvplusdsbisbsP}
\newsavebox{\SBdotTfTfdotinvplusdsbisbsA}
\begin{lrbox}{\SBdotTfTfdotinvplusdsbisbsA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> invalid;
    y ?-> pa2;
    v |-> pa2;
    *pa2 = 1;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdsbisbsB}
\settowidth{\SBdotTfTfdotinvplusdsbisbsB}{\usebox{\SBdotTfTfdotinvplusdsbisbsA}}
\newsavebox{\SBdotTfTfdotinvplusdsbisbsC}
\begin{lrbox}{\SBdotTfTfdotinvplusdsbisbsC}
\begin{minipage}{\SBdotTfTfdotinvplusdsbisbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R0=desc3(v,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|SB.TfTf.inv+dsb-isbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SBdotTfTfdotinvplusdsbisbsB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SBdotTfTfdotinvplusdsbisbsA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SBdotTfTfdotinvplusdsbisbsC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvplusdsbisbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvplusdsbisbsK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvplusdsbisbsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvplusdsbisbsO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/SB.TfTf.invv+rfi-ctrl-isbs.tex <==
\newlength{\SBdotTfTfdotinvvplusrfictrlisbsH}
\setlength{\SBdotTfTfdotinvvplusrfictrlisbsH}{0cm}
\newsavebox{\SBdotTfTfdotinvvplusrfictrlisbsI}
\begin{lrbox}{\SBdotTfTfdotinvvplusrfictrlisbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X7,[X1]
CBNZ X7,L0
L0:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvvplusrfictrlisbsJ}
\settowidth{\SBdotTfTfdotinvvplusrfictrlisbsJ}{\usebox{\SBdotTfTfdotinvvplusrfictrlisbsI}}
\addtolength{\SBdotTfTfdotinvvplusrfictrlisbsH}{\SBdotTfTfdotinvvplusrfictrlisbsJ}
\newsavebox{\SBdotTfTfdotinvvplusrfictrlisbsK}
\begin{lrbox}{\SBdotTfTfdotinvvplusrfictrlisbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X7,[X1]
CBNZ X7,L1
L1:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvvplusrfictrlisbsL}
\settowidth{\SBdotTfTfdotinvvplusrfictrlisbsL}{\usebox{\SBdotTfTfdotinvvplusrfictrlisbsK}}
\addtolength{\SBdotTfTfdotinvvplusrfictrlisbsH}{\SBdotTfTfdotinvvplusrfictrlisbsL}
\newsavebox{\SBdotTfTfdotinvvplusrfictrlisbsM}
\begin{lrbox}{\SBdotTfTfdotinvvplusrfictrlisbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvvplusrfictrlisbsN}
\settowidth{\SBdotTfTfdotinvvplusrfictrlisbsN}{\usebox{\SBdotTfTfdotinvvplusrfictrlisbsM}}
\addtolength{\SBdotTfTfdotinvvplusrfictrlisbsH}{\SBdotTfTfdotinvvplusrfictrlisbsN}
\newsavebox{\SBdotTfTfdotinvvplusrfictrlisbsO}
\begin{lrbox}{\SBdotTfTfdotinvvplusrfictrlisbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvvplusrfictrlisbsP}
\settowidth{\SBdotTfTfdotinvvplusrfictrlisbsP}{\usebox{\SBdotTfTfdotinvvplusrfictrlisbsO}}
\addtolength{\SBdotTfTfdotinvvplusrfictrlisbsH}{\SBdotTfTfdotinvvplusrfictrlisbsP}
\newsavebox{\SBdotTfTfdotinvvplusrfictrlisbsA}
\begin{lrbox}{\SBdotTfTfdotinvvplusrfictrlisbsA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> invalid;
    y ?-> pa2;
    v |-> pa2;
    *pa2 = 1;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvvplusrfictrlisbsB}
\settowidth{\SBdotTfTfdotinvvplusrfictrlisbsB}{\usebox{\SBdotTfTfdotinvvplusrfictrlisbsA}}
\newsavebox{\SBdotTfTfdotinvvplusrfictrlisbsC}
\begin{lrbox}{\SBdotTfTfdotinvvplusrfictrlisbsC}
\begin{minipage}{\SBdotTfTfdotinvvplusrfictrlisbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R0=desc3(v,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|SB.TfTf.invv+rfi-ctrl-isbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SBdotTfTfdotinvvplusrfictrlisbsB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SBdotTfTfdotinvvplusrfictrlisbsA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SBdotTfTfdotinvvplusrfictrlisbsC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvvplusrfictrlisbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvvplusrfictrlisbsK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvvplusrfictrlisbsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvvplusrfictrlisbsO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0 & 0:R7=desc3(u,page_table_base) & 1:R2=0 & 1:R7=desc3(v,page_table_base)|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/SwitchTable.EL2+msrttbr-eret.tex <==
\newlength{\SwitchTabledotELtwoplusmsrttbreretH}
\setlength{\SwitchTabledotELtwoplusmsrttbreretH}{0cm}
\newsavebox{\SwitchTabledotELtwoplusmsrttbreretI}
\begin{lrbox}{\SwitchTabledotELtwoplusmsrttbreretI}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
HVC #0
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SwitchTabledotELtwoplusmsrttbreretJ}
\settowidth{\SwitchTabledotELtwoplusmsrttbreretJ}{\usebox{\SwitchTabledotELtwoplusmsrttbreretI}}
\addtolength{\SwitchTabledotELtwoplusmsrttbreretH}{\SwitchTabledotELtwoplusmsrttbreretJ}
\newsavebox{\SwitchTabledotELtwoplusmsrttbreretK}
\begin{lrbox}{\SwitchTabledotELtwoplusmsrttbreretK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MSR TTBR0_EL1,X4
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SwitchTabledotELtwoplusmsrttbreretL}
\settowidth{\SwitchTabledotELtwoplusmsrttbreretL}{\usebox{\SwitchTabledotELtwoplusmsrttbreretK}}
\addtolength{\SwitchTabledotELtwoplusmsrttbreretH}{\SwitchTabledotELtwoplusmsrttbreretL}
\newsavebox{\SwitchTabledotELtwoplusmsrttbreretM}
\begin{lrbox}{\SwitchTabledotELtwoplusmsrttbreretM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
option default_tables = false;
physical pa1 pa2;

s1table initial_table 0x200000 {
    x |-> pa1 at level 3;
}

s1table new_table 0x280000  {
    x |-> pa2 at level 3;
}

s1table el2_table 0x300000 {
    identity 0x2000 with code;
}

*pa1 = 0;
*pa2 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\SwitchTabledotELtwoplusmsrttbreretN}
\settowidth{\SwitchTabledotELtwoplusmsrttbreretN}{\usebox{\SwitchTabledotELtwoplusmsrttbreretM}}
\newsavebox{\SwitchTabledotELtwoplusmsrttbreretO}
\begin{lrbox}{\SwitchTabledotELtwoplusmsrttbreretO}
\begin{minipage}{\SwitchTabledotELtwoplusmsrttbreretH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|R1=x|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=ttbr(asid=0x0000,base=new_table)|\\
\lstinline[language=IslaLitmusExp]|TTBR0_EL1=ttbr(base=initial_table,asid=0x0000)|\\
\lstinline[language=IslaLitmusExp]|TTBR0_EL2=ttbr(base=el2_table,asid=0x0000)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|SwitchTable.EL2+msrttbr-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SwitchTabledotELtwoplusmsrttbreretN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SwitchTabledotELtwoplusmsrttbreretM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SwitchTabledotELtwoplusmsrttbreretO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SwitchTabledotELtwoplusmsrttbreretI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\SwitchTabledotELtwoplusmsrttbreretK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/SwitchTable.same-asid+eret.toml.tex <==
\newlength{\SwitchTabledotsameasidpluseretdottomlH}
\setlength{\SwitchTabledotsameasidpluseretdottomlH}{0cm}
\newsavebox{\SwitchTabledotsameasidpluseretdottomlI}
\begin{lrbox}{\SwitchTabledotsameasidpluseretdottomlI}
\begin{lstlisting}[language=AArch64,showlines=true]
MSR TTBR0_EL1,X0
ERET
L0:
LDR X1,[X2]
\end{lstlisting}
\end{lrbox}
\newlength{\SwitchTabledotsameasidpluseretdottomlJ}
\settowidth{\SwitchTabledotsameasidpluseretdottomlJ}{\usebox{\SwitchTabledotsameasidpluseretdottomlI}}
\addtolength{\SwitchTabledotsameasidpluseretdottomlH}{\SwitchTabledotsameasidpluseretdottomlJ}
\newsavebox{\SwitchTabledotsameasidpluseretdottomlK}
\begin{lrbox}{\SwitchTabledotsameasidpluseretdottomlK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X1,#1
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SwitchTabledotsameasidpluseretdottomlL}
\settowidth{\SwitchTabledotsameasidpluseretdottomlL}{\usebox{\SwitchTabledotsameasidpluseretdottomlK}}
\addtolength{\SwitchTabledotsameasidpluseretdottomlH}{\SwitchTabledotsameasidpluseretdottomlL}
\newsavebox{\SwitchTabledotsameasidpluseretdottomlM}
\begin{lrbox}{\SwitchTabledotsameasidpluseretdottomlM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    intermediate ipa1;
    physical pa1;

    *pa1 = 0;

    s1table table0 0x2C0000 {
        identity 0x1000 with code;
        x |-> pa1;
    };
    s1table table1 0x300000 {
        identity 0x1000 with code;
        x |-> invalid;
    };

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SwitchTabledotsameasidpluseretdottomlN}
\settowidth{\SwitchTabledotsameasidpluseretdottomlN}{\usebox{\SwitchTabledotsameasidpluseretdottomlM}}
\newsavebox{\SwitchTabledotsameasidpluseretdottomlO}
\begin{lrbox}{\SwitchTabledotsameasidpluseretdottomlO}
\begin{minipage}{\SwitchTabledotsameasidpluseretdottomlH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL1=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b1|\\
\lstinline[language=IslaLitmusExp]|R0=ttbr(asid=0x01,base=table1)|\\
\lstinline[language=IslaLitmusExp]|R2=x|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL1=0b00000|\\
\lstinline[language=IslaLitmusExp]|TTBR0_EL1=ttbr(base=table0,asid=0x00)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|SwitchTable.same-asid+eret.toml|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SwitchTabledotsameasidpluseretdottomlN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SwitchTabledotsameasidpluseretdottomlM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SwitchTabledotsameasidpluseretdottomlO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SwitchTabledotsameasidpluseretdottomlI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\SwitchTabledotsameasidpluseretdottomlK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R1=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/W+T.tex <==
\newlength{\WplusTH}
\setlength{\WplusTH}{0cm}
\newsavebox{\WplusTI}
\begin{lrbox}{\WplusTI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WplusTJ}
\settowidth{\WplusTJ}{\usebox{\WplusTI}}
\addtolength{\WplusTH}{\WplusTJ}
\newsavebox{\WplusTK}
\begin{lrbox}{\WplusTK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WplusTL}
\settowidth{\WplusTL}{\usebox{\WplusTK}}
\addtolength{\WplusTH}{\WplusTL}
\newsavebox{\WplusTM}
\begin{lrbox}{\WplusTM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1000:
MOV X0,#0
\end{lstlisting}
\end{lrbox}
\newlength{\WplusTN}
\settowidth{\WplusTN}{\usebox{\WplusTM}}
\addtolength{\WplusTH}{\WplusTN}
\newsavebox{\WplusTO}
\begin{lrbox}{\WplusTO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid at level 2;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WplusTP}
\settowidth{\WplusTP}{\usebox{\WplusTO}}
\newsavebox{\WplusTA}
\begin{lrbox}{\WplusTA}
\begin{minipage}{\WplusTH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte2(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|W+T|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WplusTP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WplusTO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WplusTA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WplusTI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WplusTK}\\
  \cline{2-2}
  & handler\\
  \cline{2-2}
  & \usebox{\WplusTM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|true|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/W.tex <==
\newlength{\WH}
\setlength{\WH}{0cm}
\newsavebox{\WI}
\begin{lrbox}{\WI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WJ}
\settowidth{\WJ}{\usebox{\WI}}
\addtolength{\WH}{\WJ}
\newsavebox{\WK}
\begin{lrbox}{\WK}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
\end{lstlisting}
\end{lrbox}
\newlength{\WL}
\settowidth{\WL}{\usebox{\WK}}
\newsavebox{\WM}
\begin{lrbox}{\WM}
\begin{minipage}{\WH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=x|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|W|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WL}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WK}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WM}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WI}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|true|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/WBM+dsb-tlbiis-dsb.tex <==
\newlength{\WBMplusdsbtlbiisdsbH}
\setlength{\WBMplusdsbtlbiisdsbH}{0cm}
\newsavebox{\WBMplusdsbtlbiisdsbI}
\begin{lrbox}{\WBMplusdsbtlbiisdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X5
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WBMplusdsbtlbiisdsbJ}
\settowidth{\WBMplusdsbtlbiisdsbJ}{\usebox{\WBMplusdsbtlbiisdsbI}}
\addtolength{\WBMplusdsbtlbiisdsbH}{\WBMplusdsbtlbiisdsbJ}
\newsavebox{\WBMplusdsbtlbiisdsbK}
\begin{lrbox}{\WBMplusdsbtlbiisdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WBMplusdsbtlbiisdsbL}
\settowidth{\WBMplusdsbtlbiisdsbL}{\usebox{\WBMplusdsbtlbiisdsbK}}
\addtolength{\WBMplusdsbtlbiisdsbH}{\WBMplusdsbtlbiisdsbL}
\newsavebox{\WBMplusdsbtlbiisdsbM}
\begin{lrbox}{\WBMplusdsbtlbiisdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WBMplusdsbtlbiisdsbN}
\settowidth{\WBMplusdsbtlbiisdsbN}{\usebox{\WBMplusdsbtlbiisdsbM}}
\addtolength{\WBMplusdsbtlbiisdsbH}{\WBMplusdsbtlbiisdsbN}
\newsavebox{\WBMplusdsbtlbiisdsbO}
\begin{lrbox}{\WBMplusdsbtlbiisdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    y |-> pa1;
    *pa1 = 0;
    x ?-> invalid;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WBMplusdsbtlbiisdsbP}
\settowidth{\WBMplusdsbtlbiisdsbP}{\usebox{\WBMplusdsbtlbiisdsbO}}
\newsavebox{\WBMplusdsbtlbiisdsbA}
\begin{lrbox}{\WBMplusdsbtlbiisdsbA}
\begin{minipage}{\WBMplusdsbtlbiisdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0x2|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R5=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:R0=0x1|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WBM+dsb-tlbiis-dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WBMplusdsbtlbiisdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WBMplusdsbtlbiisdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WBMplusdsbtlbiisdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WBMplusdsbtlbiisdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WBMplusdsbtlbiisdsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WBMplusdsbtlbiisdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|x=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/WDS+dsb-tlbiipa-dsb-eret-po.tex <==
\newlength{\WDSplusdsbtlbiipadsberetpoH}
\setlength{\WDSplusdsbtlbiipadsberetpoH}{0cm}
\newsavebox{\WDSplusdsbtlbiipadsberetpoI}
\begin{lrbox}{\WDSplusdsbtlbiipadsberetpoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1,X6
DSB SY
ERET
L0:
STR X2,[X3]
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\WDSplusdsbtlbiipadsberetpoJ}
\settowidth{\WDSplusdsbtlbiipadsberetpoJ}{\usebox{\WDSplusdsbtlbiipadsberetpoI}}
\addtolength{\WDSplusdsbtlbiipadsberetpoH}{\WDSplusdsbtlbiipadsberetpoJ}
\newsavebox{\WDSplusdsbtlbiipadsberetpoK}
\begin{lrbox}{\WDSplusdsbtlbiipadsberetpoK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1200:
MOV X4,#1
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WDSplusdsbtlbiipadsberetpoL}
\settowidth{\WDSplusdsbtlbiipadsberetpoL}{\usebox{\WDSplusdsbtlbiipadsberetpoK}}
\addtolength{\WDSplusdsbtlbiipadsberetpoH}{\WDSplusdsbtlbiipadsberetpoL}
\newsavebox{\WDSplusdsbtlbiipadsberetpoM}
\begin{lrbox}{\WDSplusdsbtlbiipadsberetpoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X4,#2
MRS X20,ELR_EL2
ADD X20,X20,#4
MSR ELR_EL2,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WDSplusdsbtlbiipadsberetpoN}
\settowidth{\WDSplusdsbtlbiipadsberetpoN}{\usebox{\WDSplusdsbtlbiipadsberetpoM}}
\addtolength{\WDSplusdsbtlbiipadsberetpoH}{\WDSplusdsbtlbiipadsberetpoN}
\newsavebox{\WDSplusdsbtlbiipadsberetpoO}
\begin{lrbox}{\WDSplusdsbtlbiipadsberetpoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;
    x ?-> invalid;

    ipa1 |-> pa1;
    ipa1 ?-> invalid;

    *pa1 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WDSplusdsbtlbiipadsberetpoP}
\settowidth{\WDSplusdsbtlbiipadsberetpoP}{\usebox{\WDSplusdsbtlbiipadsberetpoO}}
\newsavebox{\WDSplusdsbtlbiipadsberetpoA}
\begin{lrbox}{\WDSplusdsbtlbiipadsberetpoA}
\begin{minipage}{\WDSplusdsbtlbiipadsberetpoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R2=0b0|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R5=x|\\
\lstinline[language=IslaLitmusExp]|R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00100|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WDS+dsb-tlbiipa-dsb-eret-po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WDSplusdsbtlbiipadsberetpoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WDSplusdsbtlbiipadsberetpoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WDSplusdsbtlbiipadsberetpoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WDSplusdsbtlbiipadsberetpoI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\WDSplusdsbtlbiipadsberetpoK}\\
  \cline{2-2}
  & thread0 el2 handler lower exc\\
  \cline{2-2}
  & \usebox{\WDSplusdsbtlbiipadsberetpoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/WDS+po-dsb-tlbiipa-dsb-eret.tex <==
\newlength{\WDSpluspodsbtlbiipadsberetH}
\setlength{\WDSpluspodsbtlbiipadsberetH}{0cm}
\newsavebox{\WDSpluspodsbtlbiipadsberetI}
\begin{lrbox}{\WDSpluspodsbtlbiipadsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
STR X2,[X3]
DSB SY
TLBI IPAS2E1,X6
DSB SY
ERET
L0:
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsberetJ}
\settowidth{\WDSpluspodsbtlbiipadsberetJ}{\usebox{\WDSpluspodsbtlbiipadsberetI}}
\addtolength{\WDSpluspodsbtlbiipadsberetH}{\WDSpluspodsbtlbiipadsberetJ}
\newsavebox{\WDSpluspodsbtlbiipadsberetK}
\begin{lrbox}{\WDSpluspodsbtlbiipadsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1200:
MOV X4,#1
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsberetL}
\settowidth{\WDSpluspodsbtlbiipadsberetL}{\usebox{\WDSpluspodsbtlbiipadsberetK}}
\addtolength{\WDSpluspodsbtlbiipadsberetH}{\WDSpluspodsbtlbiipadsberetL}
\newsavebox{\WDSpluspodsbtlbiipadsberetM}
\begin{lrbox}{\WDSpluspodsbtlbiipadsberetM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X4,#2
MRS X20,ELR_EL2
ADD X20,X20,#4
MSR ELR_EL2,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsberetN}
\settowidth{\WDSpluspodsbtlbiipadsberetN}{\usebox{\WDSpluspodsbtlbiipadsberetM}}
\addtolength{\WDSpluspodsbtlbiipadsberetH}{\WDSpluspodsbtlbiipadsberetN}
\newsavebox{\WDSpluspodsbtlbiipadsberetO}
\begin{lrbox}{\WDSpluspodsbtlbiipadsberetO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;
    x ?-> invalid;

    ipa1 |-> pa1;
    ipa1 ?-> invalid;

    *pa1 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsberetP}
\settowidth{\WDSpluspodsbtlbiipadsberetP}{\usebox{\WDSpluspodsbtlbiipadsberetO}}
\newsavebox{\WDSpluspodsbtlbiipadsberetA}
\begin{lrbox}{\WDSpluspodsbtlbiipadsberetA}
\begin{minipage}{\WDSpluspodsbtlbiipadsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R2=0b0|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R5=x|\\
\lstinline[language=IslaLitmusExp]|R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00100|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WDS+po-dsb-tlbiipa-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WDSpluspodsbtlbiipadsberetP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WDSpluspodsbtlbiipadsberetO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WDSpluspodsbtlbiipadsberetA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsberetI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsberetK}\\
  \cline{2-2}
  & thread0 el2 handler lower exc\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsberetM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/WDS+po-dsb-tlbiipa-dsb-po-eret.tex <==
\newlength{\WDSpluspodsbtlbiipadsbpoeretH}
\setlength{\WDSpluspodsbtlbiipadsbpoeretH}{0cm}
\newsavebox{\WDSpluspodsbtlbiipadsbpoeretI}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbpoeretI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1,X6
DSB SY
STR X2,[X3]
ERET
L0:
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsbpoeretJ}
\settowidth{\WDSpluspodsbtlbiipadsbpoeretJ}{\usebox{\WDSpluspodsbtlbiipadsbpoeretI}}
\addtolength{\WDSpluspodsbtlbiipadsbpoeretH}{\WDSpluspodsbtlbiipadsbpoeretJ}
\newsavebox{\WDSpluspodsbtlbiipadsbpoeretK}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbpoeretK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1200:
MOV X4,#1
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsbpoeretL}
\settowidth{\WDSpluspodsbtlbiipadsbpoeretL}{\usebox{\WDSpluspodsbtlbiipadsbpoeretK}}
\addtolength{\WDSpluspodsbtlbiipadsbpoeretH}{\WDSpluspodsbtlbiipadsbpoeretL}
\newsavebox{\WDSpluspodsbtlbiipadsbpoeretM}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbpoeretM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X4,#2
MRS X20,ELR_EL2
ADD X20,X20,#4
MSR ELR_EL2,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsbpoeretN}
\settowidth{\WDSpluspodsbtlbiipadsbpoeretN}{\usebox{\WDSpluspodsbtlbiipadsbpoeretM}}
\addtolength{\WDSpluspodsbtlbiipadsbpoeretH}{\WDSpluspodsbtlbiipadsbpoeretN}
\newsavebox{\WDSpluspodsbtlbiipadsbpoeretO}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbpoeretO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;
    x ?-> invalid;

    ipa1 |-> pa1;
    ipa1 ?-> invalid;

    *pa1 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsbpoeretP}
\settowidth{\WDSpluspodsbtlbiipadsbpoeretP}{\usebox{\WDSpluspodsbtlbiipadsbpoeretO}}
\newsavebox{\WDSpluspodsbtlbiipadsbpoeretA}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbpoeretA}
\begin{minipage}{\WDSpluspodsbtlbiipadsbpoeretH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R2=0b0|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R5=x|\\
\lstinline[language=IslaLitmusExp]|R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00100|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WDS+po-dsb-tlbiipa-dsb-po-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WDSpluspodsbtlbiipadsbpoeretP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WDSpluspodsbtlbiipadsbpoeretO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WDSpluspodsbtlbiipadsbpoeretA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsbpoeretI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsbpoeretK}\\
  \cline{2-2}
  & thread0 el2 handler lower exc\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsbpoeretM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/WDS+po-dsb-tlbiipa-dsb-tlbiis-dsb-eret.tex <==
\newlength{\WDSpluspodsbtlbiipadsbtlbiisdsberetH}
\setlength{\WDSpluspodsbtlbiipadsbtlbiisdsberetH}{0cm}
\newsavebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetI}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbtlbiisdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
STR X2,[X3]
DSB SY
TLBI IPAS2E1,X6
DSB SY
TLBI VMALLE1IS
DSB SY
ERET
L0:
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsbtlbiisdsberetJ}
\settowidth{\WDSpluspodsbtlbiipadsbtlbiisdsberetJ}{\usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetI}}
\addtolength{\WDSpluspodsbtlbiipadsbtlbiisdsberetH}{\WDSpluspodsbtlbiipadsbtlbiisdsberetJ}
\newsavebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetK}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbtlbiisdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1200:
MOV X4,#1
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsbtlbiisdsberetL}
\settowidth{\WDSpluspodsbtlbiipadsbtlbiisdsberetL}{\usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetK}}
\addtolength{\WDSpluspodsbtlbiipadsbtlbiisdsberetH}{\WDSpluspodsbtlbiipadsbtlbiisdsberetL}
\newsavebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetM}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbtlbiisdsberetM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X4,#2
MRS X20,ELR_EL2
ADD X20,X20,#4
MSR ELR_EL2,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsbtlbiisdsberetN}
\settowidth{\WDSpluspodsbtlbiipadsbtlbiisdsberetN}{\usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetM}}
\addtolength{\WDSpluspodsbtlbiipadsbtlbiisdsberetH}{\WDSpluspodsbtlbiipadsbtlbiisdsberetN}
\newsavebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetO}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbtlbiisdsberetO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;
    x ?-> invalid;

    ipa1 |-> pa1;
    ipa1 ?-> invalid;

    *pa1 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsbtlbiisdsberetP}
\settowidth{\WDSpluspodsbtlbiipadsbtlbiisdsberetP}{\usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetO}}
\newsavebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetA}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbtlbiisdsberetA}
\begin{minipage}{\WDSpluspodsbtlbiipadsbtlbiisdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R2=0b0|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R5=x|\\
\lstinline[language=IslaLitmusExp]|R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00100|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WDS+po-dsb-tlbiipa-dsb-tlbiis-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WDSpluspodsbtlbiipadsbtlbiisdsberetP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetK}\\
  \cline{2-2}
  & thread0 el2 handler lower exc\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/WRC.RRTf.inv+addrs.tex <==
\newlength{\WRCdotRRTfdotinvplusaddrsH}
\setlength{\WRCdotRRTfdotinvplusaddrsH}{0cm}
\newsavebox{\WRCdotRRTfdotinvplusaddrsI}
\begin{lrbox}{\WRCdotRRTfdotinvplusaddrsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusaddrsJ}
\settowidth{\WRCdotRRTfdotinvplusaddrsJ}{\usebox{\WRCdotRRTfdotinvplusaddrsI}}
\addtolength{\WRCdotRRTfdotinvplusaddrsH}{\WRCdotRRTfdotinvplusaddrsJ}
\newsavebox{\WRCdotRRTfdotinvplusaddrsK}
\begin{lrbox}{\WRCdotRRTfdotinvplusaddrsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
STR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusaddrsL}
\settowidth{\WRCdotRRTfdotinvplusaddrsL}{\usebox{\WRCdotRRTfdotinvplusaddrsK}}
\addtolength{\WRCdotRRTfdotinvplusaddrsH}{\WRCdotRRTfdotinvplusaddrsL}
\newsavebox{\WRCdotRRTfdotinvplusaddrsM}
\begin{lrbox}{\WRCdotRRTfdotinvplusaddrsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusaddrsN}
\settowidth{\WRCdotRRTfdotinvplusaddrsN}{\usebox{\WRCdotRRTfdotinvplusaddrsM}}
\addtolength{\WRCdotRRTfdotinvplusaddrsH}{\WRCdotRRTfdotinvplusaddrsN}
\newsavebox{\WRCdotRRTfdotinvplusaddrsO}
\begin{lrbox}{\WRCdotRRTfdotinvplusaddrsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusaddrsP}
\settowidth{\WRCdotRRTfdotinvplusaddrsP}{\usebox{\WRCdotRRTfdotinvplusaddrsO}}
\addtolength{\WRCdotRRTfdotinvplusaddrsH}{\WRCdotRRTfdotinvplusaddrsP}
\newsavebox{\WRCdotRRTfdotinvplusaddrsA}
\begin{lrbox}{\WRCdotRRTfdotinvplusaddrsA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusaddrsB}
\settowidth{\WRCdotRRTfdotinvplusaddrsB}{\usebox{\WRCdotRRTfdotinvplusaddrsA}}
\newsavebox{\WRCdotRRTfdotinvplusaddrsC}
\begin{lrbox}{\WRCdotRRTfdotinvplusaddrsC}
\begin{minipage}{\WRCdotRRTfdotinvplusaddrsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.RRTf.inv+addrs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotRRTfdotinvplusaddrsB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotRRTfdotinvplusaddrsA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotRRTfdotinvplusaddrsC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusaddrsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusaddrsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusaddrsM}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusaddrsO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=desc3(z,page_table_base) & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/WRC.RRTf.inv+dmbs.tex <==
\newlength{\WRCdotRRTfdotinvplusdmbsH}
\setlength{\WRCdotRRTfdotinvplusdmbsH}{0cm}
\newsavebox{\WRCdotRRTfdotinvplusdmbsI}
\begin{lrbox}{\WRCdotRRTfdotinvplusdmbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdmbsJ}
\settowidth{\WRCdotRRTfdotinvplusdmbsJ}{\usebox{\WRCdotRRTfdotinvplusdmbsI}}
\addtolength{\WRCdotRRTfdotinvplusdmbsH}{\WRCdotRRTfdotinvplusdmbsJ}
\newsavebox{\WRCdotRRTfdotinvplusdmbsK}
\begin{lrbox}{\WRCdotRRTfdotinvplusdmbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdmbsL}
\settowidth{\WRCdotRRTfdotinvplusdmbsL}{\usebox{\WRCdotRRTfdotinvplusdmbsK}}
\addtolength{\WRCdotRRTfdotinvplusdmbsH}{\WRCdotRRTfdotinvplusdmbsL}
\newsavebox{\WRCdotRRTfdotinvplusdmbsM}
\begin{lrbox}{\WRCdotRRTfdotinvplusdmbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdmbsN}
\settowidth{\WRCdotRRTfdotinvplusdmbsN}{\usebox{\WRCdotRRTfdotinvplusdmbsM}}
\addtolength{\WRCdotRRTfdotinvplusdmbsH}{\WRCdotRRTfdotinvplusdmbsN}
\newsavebox{\WRCdotRRTfdotinvplusdmbsO}
\begin{lrbox}{\WRCdotRRTfdotinvplusdmbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdmbsP}
\settowidth{\WRCdotRRTfdotinvplusdmbsP}{\usebox{\WRCdotRRTfdotinvplusdmbsO}}
\addtolength{\WRCdotRRTfdotinvplusdmbsH}{\WRCdotRRTfdotinvplusdmbsP}
\newsavebox{\WRCdotRRTfdotinvplusdmbsA}
\begin{lrbox}{\WRCdotRRTfdotinvplusdmbsA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdmbsB}
\settowidth{\WRCdotRRTfdotinvplusdmbsB}{\usebox{\WRCdotRRTfdotinvplusdmbsA}}
\newsavebox{\WRCdotRRTfdotinvplusdmbsC}
\begin{lrbox}{\WRCdotRRTfdotinvplusdmbsC}
\begin{minipage}{\WRCdotRRTfdotinvplusdmbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.RRTf.inv+dmbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotRRTfdotinvplusdmbsB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotRRTfdotinvplusdmbsA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotRRTfdotinvplusdmbsC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdmbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdmbsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdmbsM}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdmbsO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=desc3(z,page_table_base) & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/WRC.RRTf.inv+dsb+ctrl-isb.tex <==
\newlength{\WRCdotRRTfdotinvplusdsbplusctrlisbH}
\setlength{\WRCdotRRTfdotinvplusdsbplusctrlisbH}{0cm}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusctrlisbI}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusctrlisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusctrlisbJ}
\settowidth{\WRCdotRRTfdotinvplusdsbplusctrlisbJ}{\usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbI}}
\addtolength{\WRCdotRRTfdotinvplusdsbplusctrlisbH}{\WRCdotRRTfdotinvplusdsbplusctrlisbJ}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusctrlisbK}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusctrlisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusctrlisbL}
\settowidth{\WRCdotRRTfdotinvplusdsbplusctrlisbL}{\usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbK}}
\addtolength{\WRCdotRRTfdotinvplusdsbplusctrlisbH}{\WRCdotRRTfdotinvplusdsbplusctrlisbL}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusctrlisbM}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusctrlisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBNZ X0,L0
L0:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusctrlisbN}
\settowidth{\WRCdotRRTfdotinvplusdsbplusctrlisbN}{\usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbM}}
\addtolength{\WRCdotRRTfdotinvplusdsbplusctrlisbH}{\WRCdotRRTfdotinvplusdsbplusctrlisbN}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusctrlisbO}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusctrlisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusctrlisbP}
\settowidth{\WRCdotRRTfdotinvplusdsbplusctrlisbP}{\usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbO}}
\addtolength{\WRCdotRRTfdotinvplusdsbplusctrlisbH}{\WRCdotRRTfdotinvplusdsbplusctrlisbP}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusctrlisbA}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusctrlisbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusctrlisbB}
\settowidth{\WRCdotRRTfdotinvplusdsbplusctrlisbB}{\usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbA}}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusctrlisbC}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusctrlisbC}
\begin{minipage}{\WRCdotRRTfdotinvplusdsbplusctrlisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.RRTf.inv+dsb+ctrl-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotRRTfdotinvplusdsbplusctrlisbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbM}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=desc3(z,page_table_base) & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/WRC.RRTf.inv+dsb+dsb-isb.tex <==
\newlength{\WRCdotRRTfdotinvplusdsbplusdsbisbH}
\setlength{\WRCdotRRTfdotinvplusdsbplusdsbisbH}{0cm}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusdsbisbI}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusdsbisbJ}
\settowidth{\WRCdotRRTfdotinvplusdsbplusdsbisbJ}{\usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbI}}
\addtolength{\WRCdotRRTfdotinvplusdsbplusdsbisbH}{\WRCdotRRTfdotinvplusdsbplusdsbisbJ}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusdsbisbK}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusdsbisbL}
\settowidth{\WRCdotRRTfdotinvplusdsbplusdsbisbL}{\usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbK}}
\addtolength{\WRCdotRRTfdotinvplusdsbplusdsbisbH}{\WRCdotRRTfdotinvplusdsbplusdsbisbL}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusdsbisbM}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusdsbisbN}
\settowidth{\WRCdotRRTfdotinvplusdsbplusdsbisbN}{\usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbM}}
\addtolength{\WRCdotRRTfdotinvplusdsbplusdsbisbH}{\WRCdotRRTfdotinvplusdsbplusdsbisbN}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusdsbisbO}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusdsbisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusdsbisbP}
\settowidth{\WRCdotRRTfdotinvplusdsbplusdsbisbP}{\usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbO}}
\addtolength{\WRCdotRRTfdotinvplusdsbplusdsbisbH}{\WRCdotRRTfdotinvplusdsbplusdsbisbP}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusdsbisbA}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusdsbisbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusdsbisbB}
\settowidth{\WRCdotRRTfdotinvplusdsbplusdsbisbB}{\usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbA}}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusdsbisbC}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusdsbisbC}
\begin{minipage}{\WRCdotRRTfdotinvplusdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.RRTf.inv+dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotRRTfdotinvplusdsbplusdsbisbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbM}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=desc3(z,page_table_base) & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/WRC.RRTf.inv+dsbs.tex <==
\newlength{\WRCdotRRTfdotinvplusdsbsH}
\setlength{\WRCdotRRTfdotinvplusdsbsH}{0cm}
\newsavebox{\WRCdotRRTfdotinvplusdsbsI}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbsJ}
\settowidth{\WRCdotRRTfdotinvplusdsbsJ}{\usebox{\WRCdotRRTfdotinvplusdsbsI}}
\addtolength{\WRCdotRRTfdotinvplusdsbsH}{\WRCdotRRTfdotinvplusdsbsJ}
\newsavebox{\WRCdotRRTfdotinvplusdsbsK}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbsL}
\settowidth{\WRCdotRRTfdotinvplusdsbsL}{\usebox{\WRCdotRRTfdotinvplusdsbsK}}
\addtolength{\WRCdotRRTfdotinvplusdsbsH}{\WRCdotRRTfdotinvplusdsbsL}
\newsavebox{\WRCdotRRTfdotinvplusdsbsM}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbsN}
\settowidth{\WRCdotRRTfdotinvplusdsbsN}{\usebox{\WRCdotRRTfdotinvplusdsbsM}}
\addtolength{\WRCdotRRTfdotinvplusdsbsH}{\WRCdotRRTfdotinvplusdsbsN}
\newsavebox{\WRCdotRRTfdotinvplusdsbsO}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbsP}
\settowidth{\WRCdotRRTfdotinvplusdsbsP}{\usebox{\WRCdotRRTfdotinvplusdsbsO}}
\addtolength{\WRCdotRRTfdotinvplusdsbsH}{\WRCdotRRTfdotinvplusdsbsP}
\newsavebox{\WRCdotRRTfdotinvplusdsbsA}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbsA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbsB}
\settowidth{\WRCdotRRTfdotinvplusdsbsB}{\usebox{\WRCdotRRTfdotinvplusdsbsA}}
\newsavebox{\WRCdotRRTfdotinvplusdsbsC}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbsC}
\begin{minipage}{\WRCdotRRTfdotinvplusdsbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.RRTf.inv+dsbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotRRTfdotinvplusdsbsB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotRRTfdotinvplusdsbsA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotRRTfdotinvplusdsbsC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbsM}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbsO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=desc3(z,page_table_base) & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/WRC.RRTf.inv+pos.tex <==
\newlength{\WRCdotRRTfdotinvplusposH}
\setlength{\WRCdotRRTfdotinvplusposH}{0cm}
\newsavebox{\WRCdotRRTfdotinvplusposI}
\begin{lrbox}{\WRCdotRRTfdotinvplusposI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusposJ}
\settowidth{\WRCdotRRTfdotinvplusposJ}{\usebox{\WRCdotRRTfdotinvplusposI}}
\addtolength{\WRCdotRRTfdotinvplusposH}{\WRCdotRRTfdotinvplusposJ}
\newsavebox{\WRCdotRRTfdotinvplusposK}
\begin{lrbox}{\WRCdotRRTfdotinvplusposK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusposL}
\settowidth{\WRCdotRRTfdotinvplusposL}{\usebox{\WRCdotRRTfdotinvplusposK}}
\addtolength{\WRCdotRRTfdotinvplusposH}{\WRCdotRRTfdotinvplusposL}
\newsavebox{\WRCdotRRTfdotinvplusposM}
\begin{lrbox}{\WRCdotRRTfdotinvplusposM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusposN}
\settowidth{\WRCdotRRTfdotinvplusposN}{\usebox{\WRCdotRRTfdotinvplusposM}}
\addtolength{\WRCdotRRTfdotinvplusposH}{\WRCdotRRTfdotinvplusposN}
\newsavebox{\WRCdotRRTfdotinvplusposO}
\begin{lrbox}{\WRCdotRRTfdotinvplusposO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusposP}
\settowidth{\WRCdotRRTfdotinvplusposP}{\usebox{\WRCdotRRTfdotinvplusposO}}
\addtolength{\WRCdotRRTfdotinvplusposH}{\WRCdotRRTfdotinvplusposP}
\newsavebox{\WRCdotRRTfdotinvplusposA}
\begin{lrbox}{\WRCdotRRTfdotinvplusposA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusposB}
\settowidth{\WRCdotRRTfdotinvplusposB}{\usebox{\WRCdotRRTfdotinvplusposA}}
\newsavebox{\WRCdotRRTfdotinvplusposC}
\begin{lrbox}{\WRCdotRRTfdotinvplusposC}
\begin{minipage}{\WRCdotRRTfdotinvplusposH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.RRTf.inv+pos|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotRRTfdotinvplusposB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotRRTfdotinvplusposA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotRRTfdotinvplusposC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusposI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusposK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusposM}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusposO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=desc3(z,page_table_base) & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/WRC.TRTf.inv+addrs.tex <==
\newlength{\WRCdotTRTfdotinvplusaddrsH}
\setlength{\WRCdotTRTfdotinvplusaddrsH}{0cm}
\newsavebox{\WRCdotTRTfdotinvplusaddrsI}
\begin{lrbox}{\WRCdotTRTfdotinvplusaddrsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusaddrsJ}
\settowidth{\WRCdotTRTfdotinvplusaddrsJ}{\usebox{\WRCdotTRTfdotinvplusaddrsI}}
\addtolength{\WRCdotTRTfdotinvplusaddrsH}{\WRCdotTRTfdotinvplusaddrsJ}
\newsavebox{\WRCdotTRTfdotinvplusaddrsK}
\begin{lrbox}{\WRCdotTRTfdotinvplusaddrsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
STR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusaddrsL}
\settowidth{\WRCdotTRTfdotinvplusaddrsL}{\usebox{\WRCdotTRTfdotinvplusaddrsK}}
\addtolength{\WRCdotTRTfdotinvplusaddrsH}{\WRCdotTRTfdotinvplusaddrsL}
\newsavebox{\WRCdotTRTfdotinvplusaddrsM}
\begin{lrbox}{\WRCdotTRTfdotinvplusaddrsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusaddrsN}
\settowidth{\WRCdotTRTfdotinvplusaddrsN}{\usebox{\WRCdotTRTfdotinvplusaddrsM}}
\addtolength{\WRCdotTRTfdotinvplusaddrsH}{\WRCdotTRTfdotinvplusaddrsN}
\newsavebox{\WRCdotTRTfdotinvplusaddrsO}
\begin{lrbox}{\WRCdotTRTfdotinvplusaddrsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusaddrsP}
\settowidth{\WRCdotTRTfdotinvplusaddrsP}{\usebox{\WRCdotTRTfdotinvplusaddrsO}}
\addtolength{\WRCdotTRTfdotinvplusaddrsH}{\WRCdotTRTfdotinvplusaddrsP}
\newsavebox{\WRCdotTRTfdotinvplusaddrsA}
\begin{lrbox}{\WRCdotTRTfdotinvplusaddrsA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusaddrsB}
\settowidth{\WRCdotTRTfdotinvplusaddrsB}{\usebox{\WRCdotTRTfdotinvplusaddrsA}}
\addtolength{\WRCdotTRTfdotinvplusaddrsH}{\WRCdotTRTfdotinvplusaddrsB}
\newsavebox{\WRCdotTRTfdotinvplusaddrsC}
\begin{lrbox}{\WRCdotTRTfdotinvplusaddrsC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusaddrsD}
\settowidth{\WRCdotTRTfdotinvplusaddrsD}{\usebox{\WRCdotTRTfdotinvplusaddrsC}}
\newsavebox{\WRCdotTRTfdotinvplusaddrsE}
\begin{lrbox}{\WRCdotTRTfdotinvplusaddrsE}
\begin{minipage}{\WRCdotTRTfdotinvplusaddrsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TRTf.inv+addrs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTRTfdotinvplusaddrsD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTRTfdotinvplusaddrsC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTRTfdotinvplusaddrsE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusaddrsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusaddrsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusaddrsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusaddrsO}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusaddrsA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/WRC.TRTf.inv+dmbs.tex <==
\newlength{\WRCdotTRTfdotinvplusdmbsH}
\setlength{\WRCdotTRTfdotinvplusdmbsH}{0cm}
\newsavebox{\WRCdotTRTfdotinvplusdmbsI}
\begin{lrbox}{\WRCdotTRTfdotinvplusdmbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdmbsJ}
\settowidth{\WRCdotTRTfdotinvplusdmbsJ}{\usebox{\WRCdotTRTfdotinvplusdmbsI}}
\addtolength{\WRCdotTRTfdotinvplusdmbsH}{\WRCdotTRTfdotinvplusdmbsJ}
\newsavebox{\WRCdotTRTfdotinvplusdmbsK}
\begin{lrbox}{\WRCdotTRTfdotinvplusdmbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdmbsL}
\settowidth{\WRCdotTRTfdotinvplusdmbsL}{\usebox{\WRCdotTRTfdotinvplusdmbsK}}
\addtolength{\WRCdotTRTfdotinvplusdmbsH}{\WRCdotTRTfdotinvplusdmbsL}
\newsavebox{\WRCdotTRTfdotinvplusdmbsM}
\begin{lrbox}{\WRCdotTRTfdotinvplusdmbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdmbsN}
\settowidth{\WRCdotTRTfdotinvplusdmbsN}{\usebox{\WRCdotTRTfdotinvplusdmbsM}}
\addtolength{\WRCdotTRTfdotinvplusdmbsH}{\WRCdotTRTfdotinvplusdmbsN}
\newsavebox{\WRCdotTRTfdotinvplusdmbsO}
\begin{lrbox}{\WRCdotTRTfdotinvplusdmbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdmbsP}
\settowidth{\WRCdotTRTfdotinvplusdmbsP}{\usebox{\WRCdotTRTfdotinvplusdmbsO}}
\addtolength{\WRCdotTRTfdotinvplusdmbsH}{\WRCdotTRTfdotinvplusdmbsP}
\newsavebox{\WRCdotTRTfdotinvplusdmbsA}
\begin{lrbox}{\WRCdotTRTfdotinvplusdmbsA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdmbsB}
\settowidth{\WRCdotTRTfdotinvplusdmbsB}{\usebox{\WRCdotTRTfdotinvplusdmbsA}}
\addtolength{\WRCdotTRTfdotinvplusdmbsH}{\WRCdotTRTfdotinvplusdmbsB}
\newsavebox{\WRCdotTRTfdotinvplusdmbsC}
\begin{lrbox}{\WRCdotTRTfdotinvplusdmbsC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdmbsD}
\settowidth{\WRCdotTRTfdotinvplusdmbsD}{\usebox{\WRCdotTRTfdotinvplusdmbsC}}
\newsavebox{\WRCdotTRTfdotinvplusdmbsE}
\begin{lrbox}{\WRCdotTRTfdotinvplusdmbsE}
\begin{minipage}{\WRCdotTRTfdotinvplusdmbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TRTf.inv+dmbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTRTfdotinvplusdmbsD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTRTfdotinvplusdmbsC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTRTfdotinvplusdmbsE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdmbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdmbsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdmbsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdmbsO}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdmbsA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/WRC.TRTf.inv+dsb+dsb-isb.tex <==
\newlength{\WRCdotTRTfdotinvplusdsbplusdsbisbH}
\setlength{\WRCdotTRTfdotinvplusdsbplusdsbisbH}{0cm}
\newsavebox{\WRCdotTRTfdotinvplusdsbplusdsbisbI}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbplusdsbisbJ}
\settowidth{\WRCdotTRTfdotinvplusdsbplusdsbisbJ}{\usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbI}}
\addtolength{\WRCdotTRTfdotinvplusdsbplusdsbisbH}{\WRCdotTRTfdotinvplusdsbplusdsbisbJ}
\newsavebox{\WRCdotTRTfdotinvplusdsbplusdsbisbK}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbplusdsbisbL}
\settowidth{\WRCdotTRTfdotinvplusdsbplusdsbisbL}{\usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbK}}
\addtolength{\WRCdotTRTfdotinvplusdsbplusdsbisbH}{\WRCdotTRTfdotinvplusdsbplusdsbisbL}
\newsavebox{\WRCdotTRTfdotinvplusdsbplusdsbisbM}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbplusdsbisbN}
\settowidth{\WRCdotTRTfdotinvplusdsbplusdsbisbN}{\usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbM}}
\addtolength{\WRCdotTRTfdotinvplusdsbplusdsbisbH}{\WRCdotTRTfdotinvplusdsbplusdsbisbN}
\newsavebox{\WRCdotTRTfdotinvplusdsbplusdsbisbO}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbplusdsbisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbplusdsbisbP}
\settowidth{\WRCdotTRTfdotinvplusdsbplusdsbisbP}{\usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbO}}
\addtolength{\WRCdotTRTfdotinvplusdsbplusdsbisbH}{\WRCdotTRTfdotinvplusdsbplusdsbisbP}
\newsavebox{\WRCdotTRTfdotinvplusdsbplusdsbisbA}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbplusdsbisbA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbplusdsbisbB}
\settowidth{\WRCdotTRTfdotinvplusdsbplusdsbisbB}{\usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbA}}
\addtolength{\WRCdotTRTfdotinvplusdsbplusdsbisbH}{\WRCdotTRTfdotinvplusdsbplusdsbisbB}
\newsavebox{\WRCdotTRTfdotinvplusdsbplusdsbisbC}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbplusdsbisbC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbplusdsbisbD}
\settowidth{\WRCdotTRTfdotinvplusdsbplusdsbisbD}{\usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbC}}
\newsavebox{\WRCdotTRTfdotinvplusdsbplusdsbisbE}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbplusdsbisbE}
\begin{minipage}{\WRCdotTRTfdotinvplusdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TRTf.inv+dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTRTfdotinvplusdsbplusdsbisbD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbO}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/WRC.TRTf.inv+dsbs.tex <==
\newlength{\WRCdotTRTfdotinvplusdsbsH}
\setlength{\WRCdotTRTfdotinvplusdsbsH}{0cm}
\newsavebox{\WRCdotTRTfdotinvplusdsbsI}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbsJ}
\settowidth{\WRCdotTRTfdotinvplusdsbsJ}{\usebox{\WRCdotTRTfdotinvplusdsbsI}}
\addtolength{\WRCdotTRTfdotinvplusdsbsH}{\WRCdotTRTfdotinvplusdsbsJ}
\newsavebox{\WRCdotTRTfdotinvplusdsbsK}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbsL}
\settowidth{\WRCdotTRTfdotinvplusdsbsL}{\usebox{\WRCdotTRTfdotinvplusdsbsK}}
\addtolength{\WRCdotTRTfdotinvplusdsbsH}{\WRCdotTRTfdotinvplusdsbsL}
\newsavebox{\WRCdotTRTfdotinvplusdsbsM}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbsN}
\settowidth{\WRCdotTRTfdotinvplusdsbsN}{\usebox{\WRCdotTRTfdotinvplusdsbsM}}
\addtolength{\WRCdotTRTfdotinvplusdsbsH}{\WRCdotTRTfdotinvplusdsbsN}
\newsavebox{\WRCdotTRTfdotinvplusdsbsO}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbsP}
\settowidth{\WRCdotTRTfdotinvplusdsbsP}{\usebox{\WRCdotTRTfdotinvplusdsbsO}}
\addtolength{\WRCdotTRTfdotinvplusdsbsH}{\WRCdotTRTfdotinvplusdsbsP}
\newsavebox{\WRCdotTRTfdotinvplusdsbsA}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbsA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbsB}
\settowidth{\WRCdotTRTfdotinvplusdsbsB}{\usebox{\WRCdotTRTfdotinvplusdsbsA}}
\addtolength{\WRCdotTRTfdotinvplusdsbsH}{\WRCdotTRTfdotinvplusdsbsB}
\newsavebox{\WRCdotTRTfdotinvplusdsbsC}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbsC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbsD}
\settowidth{\WRCdotTRTfdotinvplusdsbsD}{\usebox{\WRCdotTRTfdotinvplusdsbsC}}
\newsavebox{\WRCdotTRTfdotinvplusdsbsE}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbsE}
\begin{minipage}{\WRCdotTRTfdotinvplusdsbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TRTf.inv+dsbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTRTfdotinvplusdsbsD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTRTfdotinvplusdsbsC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTRTfdotinvplusdsbsE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbsO}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbsA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/WRC.TRTf.inv+pos.tex <==
\newlength{\WRCdotTRTfdotinvplusposH}
\setlength{\WRCdotTRTfdotinvplusposH}{0cm}
\newsavebox{\WRCdotTRTfdotinvplusposI}
\begin{lrbox}{\WRCdotTRTfdotinvplusposI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusposJ}
\settowidth{\WRCdotTRTfdotinvplusposJ}{\usebox{\WRCdotTRTfdotinvplusposI}}
\addtolength{\WRCdotTRTfdotinvplusposH}{\WRCdotTRTfdotinvplusposJ}
\newsavebox{\WRCdotTRTfdotinvplusposK}
\begin{lrbox}{\WRCdotTRTfdotinvplusposK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusposL}
\settowidth{\WRCdotTRTfdotinvplusposL}{\usebox{\WRCdotTRTfdotinvplusposK}}
\addtolength{\WRCdotTRTfdotinvplusposH}{\WRCdotTRTfdotinvplusposL}
\newsavebox{\WRCdotTRTfdotinvplusposM}
\begin{lrbox}{\WRCdotTRTfdotinvplusposM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusposN}
\settowidth{\WRCdotTRTfdotinvplusposN}{\usebox{\WRCdotTRTfdotinvplusposM}}
\addtolength{\WRCdotTRTfdotinvplusposH}{\WRCdotTRTfdotinvplusposN}
\newsavebox{\WRCdotTRTfdotinvplusposO}
\begin{lrbox}{\WRCdotTRTfdotinvplusposO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusposP}
\settowidth{\WRCdotTRTfdotinvplusposP}{\usebox{\WRCdotTRTfdotinvplusposO}}
\addtolength{\WRCdotTRTfdotinvplusposH}{\WRCdotTRTfdotinvplusposP}
\newsavebox{\WRCdotTRTfdotinvplusposA}
\begin{lrbox}{\WRCdotTRTfdotinvplusposA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusposB}
\settowidth{\WRCdotTRTfdotinvplusposB}{\usebox{\WRCdotTRTfdotinvplusposA}}
\addtolength{\WRCdotTRTfdotinvplusposH}{\WRCdotTRTfdotinvplusposB}
\newsavebox{\WRCdotTRTfdotinvplusposC}
\begin{lrbox}{\WRCdotTRTfdotinvplusposC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusposD}
\settowidth{\WRCdotTRTfdotinvplusposD}{\usebox{\WRCdotTRTfdotinvplusposC}}
\newsavebox{\WRCdotTRTfdotinvplusposE}
\begin{lrbox}{\WRCdotTRTfdotinvplusposE}
\begin{minipage}{\WRCdotTRTfdotinvplusposH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TRTf.inv+pos|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTRTfdotinvplusposD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTRTfdotinvplusposC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTRTfdotinvplusposE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusposI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusposK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusposM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusposO}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusposA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/WRC.TTTf.inv+addrs.tex <==
\newlength{\WRCdotTTTfdotinvplusaddrsH}
\setlength{\WRCdotTTTfdotinvplusaddrsH}{0cm}
\newsavebox{\WRCdotTTTfdotinvplusaddrsI}
\begin{lrbox}{\WRCdotTTTfdotinvplusaddrsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusaddrsJ}
\settowidth{\WRCdotTTTfdotinvplusaddrsJ}{\usebox{\WRCdotTTTfdotinvplusaddrsI}}
\addtolength{\WRCdotTTTfdotinvplusaddrsH}{\WRCdotTTTfdotinvplusaddrsJ}
\newsavebox{\WRCdotTTTfdotinvplusaddrsK}
\begin{lrbox}{\WRCdotTTTfdotinvplusaddrsK}
\begin{lstlisting}[language=AArch64,showlines=true]
MOV X0,#0
LDR X0,[X1]
EOR X4,X0,X0
STR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusaddrsL}
\settowidth{\WRCdotTTTfdotinvplusaddrsL}{\usebox{\WRCdotTTTfdotinvplusaddrsK}}
\addtolength{\WRCdotTTTfdotinvplusaddrsH}{\WRCdotTTTfdotinvplusaddrsL}
\newsavebox{\WRCdotTTTfdotinvplusaddrsM}
\begin{lrbox}{\WRCdotTTTfdotinvplusaddrsM}
\begin{lstlisting}[language=AArch64,showlines=true]
MOV X0,#0
LDR X0,[X1]
EOR X4,X0,X0
MOV X2,#0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusaddrsN}
\settowidth{\WRCdotTTTfdotinvplusaddrsN}{\usebox{\WRCdotTTTfdotinvplusaddrsM}}
\addtolength{\WRCdotTTTfdotinvplusaddrsH}{\WRCdotTTTfdotinvplusaddrsN}
\newsavebox{\WRCdotTTTfdotinvplusaddrsO}
\begin{lrbox}{\WRCdotTTTfdotinvplusaddrsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusaddrsP}
\settowidth{\WRCdotTTTfdotinvplusaddrsP}{\usebox{\WRCdotTTTfdotinvplusaddrsO}}
\addtolength{\WRCdotTTTfdotinvplusaddrsH}{\WRCdotTTTfdotinvplusaddrsP}
\newsavebox{\WRCdotTTTfdotinvplusaddrsA}
\begin{lrbox}{\WRCdotTTTfdotinvplusaddrsA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusaddrsB}
\settowidth{\WRCdotTTTfdotinvplusaddrsB}{\usebox{\WRCdotTTTfdotinvplusaddrsA}}
\addtolength{\WRCdotTTTfdotinvplusaddrsH}{\WRCdotTTTfdotinvplusaddrsB}
\newsavebox{\WRCdotTTTfdotinvplusaddrsC}
\begin{lrbox}{\WRCdotTTTfdotinvplusaddrsC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusaddrsD}
\settowidth{\WRCdotTTTfdotinvplusaddrsD}{\usebox{\WRCdotTTTfdotinvplusaddrsC}}
\newsavebox{\WRCdotTTTfdotinvplusaddrsE}
\begin{lrbox}{\WRCdotTTTfdotinvplusaddrsE}
\begin{minipage}{\WRCdotTTTfdotinvplusaddrsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:__isla_monomorphize_writes=true|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TTTf.inv+addrs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTTTfdotinvplusaddrsD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTTTfdotinvplusaddrsC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTTTfdotinvplusaddrsE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusaddrsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusaddrsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusaddrsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusaddrsO}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusaddrsA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/WRC.TTTf.inv+data+addr.tex <==
\newlength{\WRCdotTTTfdotinvplusdataplusaddrH}
\setlength{\WRCdotTTTfdotinvplusdataplusaddrH}{0cm}
\newsavebox{\WRCdotTTTfdotinvplusdataplusaddrI}
\begin{lrbox}{\WRCdotTTTfdotinvplusdataplusaddrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusdataplusaddrJ}
\settowidth{\WRCdotTTTfdotinvplusdataplusaddrJ}{\usebox{\WRCdotTTTfdotinvplusdataplusaddrI}}
\addtolength{\WRCdotTTTfdotinvplusdataplusaddrH}{\WRCdotTTTfdotinvplusdataplusaddrJ}
\newsavebox{\WRCdotTTTfdotinvplusdataplusaddrK}
\begin{lrbox}{\WRCdotTTTfdotinvplusdataplusaddrK}
\begin{lstlisting}[language=AArch64,showlines=true]
MOV X0,#0
LDR X0,[X1]
EOR X4,X0,X0
ORR X2,X2,X4
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusdataplusaddrL}
\settowidth{\WRCdotTTTfdotinvplusdataplusaddrL}{\usebox{\WRCdotTTTfdotinvplusdataplusaddrK}}
\addtolength{\WRCdotTTTfdotinvplusdataplusaddrH}{\WRCdotTTTfdotinvplusdataplusaddrL}
\newsavebox{\WRCdotTTTfdotinvplusdataplusaddrM}
\begin{lrbox}{\WRCdotTTTfdotinvplusdataplusaddrM}
\begin{lstlisting}[language=AArch64,showlines=true]
MOV X0,#0
LDR X0,[X1]
EOR X4,X0,X0
MOV X2,#0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusdataplusaddrN}
\settowidth{\WRCdotTTTfdotinvplusdataplusaddrN}{\usebox{\WRCdotTTTfdotinvplusdataplusaddrM}}
\addtolength{\WRCdotTTTfdotinvplusdataplusaddrH}{\WRCdotTTTfdotinvplusdataplusaddrN}
\newsavebox{\WRCdotTTTfdotinvplusdataplusaddrO}
\begin{lrbox}{\WRCdotTTTfdotinvplusdataplusaddrO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusdataplusaddrP}
\settowidth{\WRCdotTTTfdotinvplusdataplusaddrP}{\usebox{\WRCdotTTTfdotinvplusdataplusaddrO}}
\addtolength{\WRCdotTTTfdotinvplusdataplusaddrH}{\WRCdotTTTfdotinvplusdataplusaddrP}
\newsavebox{\WRCdotTTTfdotinvplusdataplusaddrA}
\begin{lrbox}{\WRCdotTTTfdotinvplusdataplusaddrA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusdataplusaddrB}
\settowidth{\WRCdotTTTfdotinvplusdataplusaddrB}{\usebox{\WRCdotTTTfdotinvplusdataplusaddrA}}
\addtolength{\WRCdotTTTfdotinvplusdataplusaddrH}{\WRCdotTTTfdotinvplusdataplusaddrB}
\newsavebox{\WRCdotTTTfdotinvplusdataplusaddrC}
\begin{lrbox}{\WRCdotTTTfdotinvplusdataplusaddrC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusdataplusaddrD}
\settowidth{\WRCdotTTTfdotinvplusdataplusaddrD}{\usebox{\WRCdotTTTfdotinvplusdataplusaddrC}}
\newsavebox{\WRCdotTTTfdotinvplusdataplusaddrE}
\begin{lrbox}{\WRCdotTTTfdotinvplusdataplusaddrE}
\begin{minipage}{\WRCdotTTTfdotinvplusdataplusaddrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:__isla_monomorphize_writes=true|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TTTf.inv+data+addr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTTTfdotinvplusdataplusaddrD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTTTfdotinvplusdataplusaddrC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTTTfdotinvplusdataplusaddrE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusdataplusaddrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusdataplusaddrK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusdataplusaddrM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusdataplusaddrO}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusdataplusaddrA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/WRC.TfRR+ctrl-isb+dsb.tex <==
\newlength{\WRCdotTfRRplusctrlisbplusdsbH}
\setlength{\WRCdotTfRRplusctrlisbplusdsbH}{0cm}
\newsavebox{\WRCdotTfRRplusctrlisbplusdsbI}
\begin{lrbox}{\WRCdotTfRRplusctrlisbplusdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusctrlisbplusdsbJ}
\settowidth{\WRCdotTfRRplusctrlisbplusdsbJ}{\usebox{\WRCdotTfRRplusctrlisbplusdsbI}}
\addtolength{\WRCdotTfRRplusctrlisbplusdsbH}{\WRCdotTfRRplusctrlisbplusdsbJ}
\newsavebox{\WRCdotTfRRplusctrlisbplusdsbK}
\begin{lrbox}{\WRCdotTfRRplusctrlisbplusdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBNZ X0,L0
L0:
ISB
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusctrlisbplusdsbL}
\settowidth{\WRCdotTfRRplusctrlisbplusdsbL}{\usebox{\WRCdotTfRRplusctrlisbplusdsbK}}
\addtolength{\WRCdotTfRRplusctrlisbplusdsbH}{\WRCdotTfRRplusctrlisbplusdsbL}
\newsavebox{\WRCdotTfRRplusctrlisbplusdsbM}
\begin{lrbox}{\WRCdotTfRRplusctrlisbplusdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusctrlisbplusdsbN}
\settowidth{\WRCdotTfRRplusctrlisbplusdsbN}{\usebox{\WRCdotTfRRplusctrlisbplusdsbM}}
\addtolength{\WRCdotTfRRplusctrlisbplusdsbH}{\WRCdotTfRRplusctrlisbplusdsbN}
\newsavebox{\WRCdotTfRRplusctrlisbplusdsbO}
\begin{lrbox}{\WRCdotTfRRplusctrlisbplusdsbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusctrlisbplusdsbP}
\settowidth{\WRCdotTfRRplusctrlisbplusdsbP}{\usebox{\WRCdotTfRRplusctrlisbplusdsbO}}
\addtolength{\WRCdotTfRRplusctrlisbplusdsbH}{\WRCdotTfRRplusctrlisbplusdsbP}
\newsavebox{\WRCdotTfRRplusctrlisbplusdsbA}
\begin{lrbox}{\WRCdotTfRRplusctrlisbplusdsbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    *pa1 = 0;

    y |-> pa2;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusctrlisbplusdsbB}
\settowidth{\WRCdotTfRRplusctrlisbplusdsbB}{\usebox{\WRCdotTfRRplusctrlisbplusdsbA}}
\newsavebox{\WRCdotTfRRplusctrlisbplusdsbC}
\begin{lrbox}{\WRCdotTfRRplusctrlisbplusdsbC}
\begin{minipage}{\WRCdotTfRRplusctrlisbplusdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TfRR+ctrl-isb+dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTfRRplusctrlisbplusdsbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTfRRplusctrlisbplusdsbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTfRRplusctrlisbplusdsbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusctrlisbplusdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusctrlisbplusdsbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusctrlisbplusdsbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusctrlisbplusdsbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & ~2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/WRC.TfRR+dmbs.tex <==
\newlength{\WRCdotTfRRplusdmbsH}
\setlength{\WRCdotTfRRplusdmbsH}{0cm}
\newsavebox{\WRCdotTfRRplusdmbsI}
\begin{lrbox}{\WRCdotTfRRplusdmbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdmbsJ}
\settowidth{\WRCdotTfRRplusdmbsJ}{\usebox{\WRCdotTfRRplusdmbsI}}
\addtolength{\WRCdotTfRRplusdmbsH}{\WRCdotTfRRplusdmbsJ}
\newsavebox{\WRCdotTfRRplusdmbsK}
\begin{lrbox}{\WRCdotTfRRplusdmbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdmbsL}
\settowidth{\WRCdotTfRRplusdmbsL}{\usebox{\WRCdotTfRRplusdmbsK}}
\addtolength{\WRCdotTfRRplusdmbsH}{\WRCdotTfRRplusdmbsL}
\newsavebox{\WRCdotTfRRplusdmbsM}
\begin{lrbox}{\WRCdotTfRRplusdmbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdmbsN}
\settowidth{\WRCdotTfRRplusdmbsN}{\usebox{\WRCdotTfRRplusdmbsM}}
\addtolength{\WRCdotTfRRplusdmbsH}{\WRCdotTfRRplusdmbsN}
\newsavebox{\WRCdotTfRRplusdmbsO}
\begin{lrbox}{\WRCdotTfRRplusdmbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdmbsP}
\settowidth{\WRCdotTfRRplusdmbsP}{\usebox{\WRCdotTfRRplusdmbsO}}
\addtolength{\WRCdotTfRRplusdmbsH}{\WRCdotTfRRplusdmbsP}
\newsavebox{\WRCdotTfRRplusdmbsA}
\begin{lrbox}{\WRCdotTfRRplusdmbsA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    *pa1 = 0;

    y |-> pa2;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdmbsB}
\settowidth{\WRCdotTfRRplusdmbsB}{\usebox{\WRCdotTfRRplusdmbsA}}
\newsavebox{\WRCdotTfRRplusdmbsC}
\begin{lrbox}{\WRCdotTfRRplusdmbsC}
\begin{minipage}{\WRCdotTfRRplusdmbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TfRR+dmbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTfRRplusdmbsB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTfRRplusdmbsA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTfRRplusdmbsC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdmbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdmbsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdmbsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdmbsO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & ~2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/WRC.TfRR+dsb-isb+dsb.tex <==
\newlength{\WRCdotTfRRplusdsbisbplusdsbH}
\setlength{\WRCdotTfRRplusdsbisbplusdsbH}{0cm}
\newsavebox{\WRCdotTfRRplusdsbisbplusdsbI}
\begin{lrbox}{\WRCdotTfRRplusdsbisbplusdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbisbplusdsbJ}
\settowidth{\WRCdotTfRRplusdsbisbplusdsbJ}{\usebox{\WRCdotTfRRplusdsbisbplusdsbI}}
\addtolength{\WRCdotTfRRplusdsbisbplusdsbH}{\WRCdotTfRRplusdsbisbplusdsbJ}
\newsavebox{\WRCdotTfRRplusdsbisbplusdsbK}
\begin{lrbox}{\WRCdotTfRRplusdsbisbplusdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbisbplusdsbL}
\settowidth{\WRCdotTfRRplusdsbisbplusdsbL}{\usebox{\WRCdotTfRRplusdsbisbplusdsbK}}
\addtolength{\WRCdotTfRRplusdsbisbplusdsbH}{\WRCdotTfRRplusdsbisbplusdsbL}
\newsavebox{\WRCdotTfRRplusdsbisbplusdsbM}
\begin{lrbox}{\WRCdotTfRRplusdsbisbplusdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbisbplusdsbN}
\settowidth{\WRCdotTfRRplusdsbisbplusdsbN}{\usebox{\WRCdotTfRRplusdsbisbplusdsbM}}
\addtolength{\WRCdotTfRRplusdsbisbplusdsbH}{\WRCdotTfRRplusdsbisbplusdsbN}
\newsavebox{\WRCdotTfRRplusdsbisbplusdsbO}
\begin{lrbox}{\WRCdotTfRRplusdsbisbplusdsbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbisbplusdsbP}
\settowidth{\WRCdotTfRRplusdsbisbplusdsbP}{\usebox{\WRCdotTfRRplusdsbisbplusdsbO}}
\addtolength{\WRCdotTfRRplusdsbisbplusdsbH}{\WRCdotTfRRplusdsbisbplusdsbP}
\newsavebox{\WRCdotTfRRplusdsbisbplusdsbA}
\begin{lrbox}{\WRCdotTfRRplusdsbisbplusdsbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    *pa1 = 0;

    y |-> pa2;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbisbplusdsbB}
\settowidth{\WRCdotTfRRplusdsbisbplusdsbB}{\usebox{\WRCdotTfRRplusdsbisbplusdsbA}}
\newsavebox{\WRCdotTfRRplusdsbisbplusdsbC}
\begin{lrbox}{\WRCdotTfRRplusdsbisbplusdsbC}
\begin{minipage}{\WRCdotTfRRplusdsbisbplusdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TfRR+dsb-isb+dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTfRRplusdsbisbplusdsbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTfRRplusdsbisbplusdsbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTfRRplusdsbisbplusdsbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdsbisbplusdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdsbisbplusdsbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdsbisbplusdsbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdsbisbplusdsbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & ~2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/WRC.TfRR+dsbs.tex <==
\newlength{\WRCdotTfRRplusdsbsH}
\setlength{\WRCdotTfRRplusdsbsH}{0cm}
\newsavebox{\WRCdotTfRRplusdsbsI}
\begin{lrbox}{\WRCdotTfRRplusdsbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbsJ}
\settowidth{\WRCdotTfRRplusdsbsJ}{\usebox{\WRCdotTfRRplusdsbsI}}
\addtolength{\WRCdotTfRRplusdsbsH}{\WRCdotTfRRplusdsbsJ}
\newsavebox{\WRCdotTfRRplusdsbsK}
\begin{lrbox}{\WRCdotTfRRplusdsbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbsL}
\settowidth{\WRCdotTfRRplusdsbsL}{\usebox{\WRCdotTfRRplusdsbsK}}
\addtolength{\WRCdotTfRRplusdsbsH}{\WRCdotTfRRplusdsbsL}
\newsavebox{\WRCdotTfRRplusdsbsM}
\begin{lrbox}{\WRCdotTfRRplusdsbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbsN}
\settowidth{\WRCdotTfRRplusdsbsN}{\usebox{\WRCdotTfRRplusdsbsM}}
\addtolength{\WRCdotTfRRplusdsbsH}{\WRCdotTfRRplusdsbsN}
\newsavebox{\WRCdotTfRRplusdsbsO}
\begin{lrbox}{\WRCdotTfRRplusdsbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbsP}
\settowidth{\WRCdotTfRRplusdsbsP}{\usebox{\WRCdotTfRRplusdsbsO}}
\addtolength{\WRCdotTfRRplusdsbsH}{\WRCdotTfRRplusdsbsP}
\newsavebox{\WRCdotTfRRplusdsbsA}
\begin{lrbox}{\WRCdotTfRRplusdsbsA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    *pa1 = 0;

    y |-> pa2;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbsB}
\settowidth{\WRCdotTfRRplusdsbsB}{\usebox{\WRCdotTfRRplusdsbsA}}
\newsavebox{\WRCdotTfRRplusdsbsC}
\begin{lrbox}{\WRCdotTfRRplusdsbsC}
\begin{minipage}{\WRCdotTfRRplusdsbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TfRR+dsbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTfRRplusdsbsB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTfRRplusdsbsA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTfRRplusdsbsC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdsbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdsbsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdsbsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdsbsO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & ~2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/WRC.TfRR+po+dsb.tex <==
\newlength{\WRCdotTfRRpluspoplusdsbH}
\setlength{\WRCdotTfRRpluspoplusdsbH}{0cm}
\newsavebox{\WRCdotTfRRpluspoplusdsbI}
\begin{lrbox}{\WRCdotTfRRpluspoplusdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRpluspoplusdsbJ}
\settowidth{\WRCdotTfRRpluspoplusdsbJ}{\usebox{\WRCdotTfRRpluspoplusdsbI}}
\addtolength{\WRCdotTfRRpluspoplusdsbH}{\WRCdotTfRRpluspoplusdsbJ}
\newsavebox{\WRCdotTfRRpluspoplusdsbK}
\begin{lrbox}{\WRCdotTfRRpluspoplusdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRpluspoplusdsbL}
\settowidth{\WRCdotTfRRpluspoplusdsbL}{\usebox{\WRCdotTfRRpluspoplusdsbK}}
\addtolength{\WRCdotTfRRpluspoplusdsbH}{\WRCdotTfRRpluspoplusdsbL}
\newsavebox{\WRCdotTfRRpluspoplusdsbM}
\begin{lrbox}{\WRCdotTfRRpluspoplusdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRpluspoplusdsbN}
\settowidth{\WRCdotTfRRpluspoplusdsbN}{\usebox{\WRCdotTfRRpluspoplusdsbM}}
\addtolength{\WRCdotTfRRpluspoplusdsbH}{\WRCdotTfRRpluspoplusdsbN}
\newsavebox{\WRCdotTfRRpluspoplusdsbO}
\begin{lrbox}{\WRCdotTfRRpluspoplusdsbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRpluspoplusdsbP}
\settowidth{\WRCdotTfRRpluspoplusdsbP}{\usebox{\WRCdotTfRRpluspoplusdsbO}}
\addtolength{\WRCdotTfRRpluspoplusdsbH}{\WRCdotTfRRpluspoplusdsbP}
\newsavebox{\WRCdotTfRRpluspoplusdsbA}
\begin{lrbox}{\WRCdotTfRRpluspoplusdsbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    *pa1 = 0;

    y |-> pa2;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRpluspoplusdsbB}
\settowidth{\WRCdotTfRRpluspoplusdsbB}{\usebox{\WRCdotTfRRpluspoplusdsbA}}
\newsavebox{\WRCdotTfRRpluspoplusdsbC}
\begin{lrbox}{\WRCdotTfRRpluspoplusdsbC}
\begin{minipage}{\WRCdotTfRRpluspoplusdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TfRR+po+dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTfRRpluspoplusdsbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTfRRpluspoplusdsbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTfRRpluspoplusdsbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRpluspoplusdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRpluspoplusdsbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRpluspoplusdsbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRpluspoplusdsbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & ~2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/WRC.TfRR+pos.tex <==
\newlength{\WRCdotTfRRplusposH}
\setlength{\WRCdotTfRRplusposH}{0cm}
\newsavebox{\WRCdotTfRRplusposI}
\begin{lrbox}{\WRCdotTfRRplusposI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusposJ}
\settowidth{\WRCdotTfRRplusposJ}{\usebox{\WRCdotTfRRplusposI}}
\addtolength{\WRCdotTfRRplusposH}{\WRCdotTfRRplusposJ}
\newsavebox{\WRCdotTfRRplusposK}
\begin{lrbox}{\WRCdotTfRRplusposK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusposL}
\settowidth{\WRCdotTfRRplusposL}{\usebox{\WRCdotTfRRplusposK}}
\addtolength{\WRCdotTfRRplusposH}{\WRCdotTfRRplusposL}
\newsavebox{\WRCdotTfRRplusposM}
\begin{lrbox}{\WRCdotTfRRplusposM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusposN}
\settowidth{\WRCdotTfRRplusposN}{\usebox{\WRCdotTfRRplusposM}}
\addtolength{\WRCdotTfRRplusposH}{\WRCdotTfRRplusposN}
\newsavebox{\WRCdotTfRRplusposO}
\begin{lrbox}{\WRCdotTfRRplusposO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusposP}
\settowidth{\WRCdotTfRRplusposP}{\usebox{\WRCdotTfRRplusposO}}
\addtolength{\WRCdotTfRRplusposH}{\WRCdotTfRRplusposP}
\newsavebox{\WRCdotTfRRplusposA}
\begin{lrbox}{\WRCdotTfRRplusposA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    *pa1 = 0;

    y |-> pa2;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusposB}
\settowidth{\WRCdotTfRRplusposB}{\usebox{\WRCdotTfRRplusposA}}
\newsavebox{\WRCdotTfRRplusposC}
\begin{lrbox}{\WRCdotTfRRplusposC}
\begin{minipage}{\WRCdotTfRRplusposH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TfRR+pos|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTfRRplusposB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTfRRplusposA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTfRRplusposC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusposI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusposK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusposM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusposO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & ~2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/WRC.TfRT+dsb-tlbiis-dsb+dsb-isb.tex <==
\newlength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbH}
\setlength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbH}{0cm}
\newsavebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbI}
\begin{lrbox}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbJ}
\settowidth{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbJ}{\usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbI}}
\addtolength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbH}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbJ}
\newsavebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbK}
\begin{lrbox}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
// the TLBI is in the handler
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbL}
\settowidth{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbL}{\usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbK}}
\addtolength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbH}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbL}
\newsavebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbM}
\begin{lrbox}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbN}
\settowidth{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbN}{\usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbM}}
\addtolength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbH}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbN}
\newsavebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbO}
\begin{lrbox}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
DSB SY
TLBI VAE1IS,X4
DSB SY
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbP}
\settowidth{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbP}{\usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbO}}
\addtolength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbH}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbP}
\newsavebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbA}
\begin{lrbox}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbB}
\settowidth{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbB}{\usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbA}}
\addtolength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbH}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbB}
\newsavebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbC}
\begin{lrbox}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;

    x |-> pa1;
    x ?-> invalid;
    *pa1 = 1;

    y |-> pa2;
    *pa2 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbD}
\settowidth{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbD}{\usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbC}}
\newsavebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbE}
\begin{lrbox}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbE}
\begin{minipage}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TfRT+dsb-tlbiis-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbO}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=0 & 2:R0=1 & 2:R2=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2021-11-30/latex/WRC.TfRT+po+dsb-isb.tex <==
\newlength{\WRCdotTfRTpluspoplusdsbisbH}
\setlength{\WRCdotTfRTpluspoplusdsbisbH}{0cm}
\newsavebox{\WRCdotTfRTpluspoplusdsbisbI}
\begin{lrbox}{\WRCdotTfRTpluspoplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTpluspoplusdsbisbJ}
\settowidth{\WRCdotTfRTpluspoplusdsbisbJ}{\usebox{\WRCdotTfRTpluspoplusdsbisbI}}
\addtolength{\WRCdotTfRTpluspoplusdsbisbH}{\WRCdotTfRTpluspoplusdsbisbJ}
\newsavebox{\WRCdotTfRTpluspoplusdsbisbK}
\begin{lrbox}{\WRCdotTfRTpluspoplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTpluspoplusdsbisbL}
\settowidth{\WRCdotTfRTpluspoplusdsbisbL}{\usebox{\WRCdotTfRTpluspoplusdsbisbK}}
\addtolength{\WRCdotTfRTpluspoplusdsbisbH}{\WRCdotTfRTpluspoplusdsbisbL}
\newsavebox{\WRCdotTfRTpluspoplusdsbisbM}
\begin{lrbox}{\WRCdotTfRTpluspoplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTpluspoplusdsbisbN}
\settowidth{\WRCdotTfRTpluspoplusdsbisbN}{\usebox{\WRCdotTfRTpluspoplusdsbisbM}}
\addtolength{\WRCdotTfRTpluspoplusdsbisbH}{\WRCdotTfRTpluspoplusdsbisbN}
\newsavebox{\WRCdotTfRTpluspoplusdsbisbO}
\begin{lrbox}{\WRCdotTfRTpluspoplusdsbisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTpluspoplusdsbisbP}
\settowidth{\WRCdotTfRTpluspoplusdsbisbP}{\usebox{\WRCdotTfRTpluspoplusdsbisbO}}
\addtolength{\WRCdotTfRTpluspoplusdsbisbH}{\WRCdotTfRTpluspoplusdsbisbP}
\newsavebox{\WRCdotTfRTpluspoplusdsbisbA}
\begin{lrbox}{\WRCdotTfRTpluspoplusdsbisbA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTpluspoplusdsbisbB}
\settowidth{\WRCdotTfRTpluspoplusdsbisbB}{\usebox{\WRCdotTfRTpluspoplusdsbisbA}}
\addtolength{\WRCdotTfRTpluspoplusdsbisbH}{\WRCdotTfRTpluspoplusdsbisbB}
\newsavebox{\WRCdotTfRTpluspoplusdsbisbC}
\begin{lrbox}{\WRCdotTfRTpluspoplusdsbisbC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;

    x |-> pa1;
    x ?-> invalid;
    *pa1 = 1;

    y |-> pa2;
    *pa2 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTpluspoplusdsbisbD}
\settowidth{\WRCdotTfRTpluspoplusdsbisbD}{\usebox{\WRCdotTfRTpluspoplusdsbisbC}}
\newsavebox{\WRCdotTfRTpluspoplusdsbisbE}
\begin{lrbox}{\WRCdotTfRTpluspoplusdsbisbE}
\begin{minipage}{\WRCdotTfRTpluspoplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TfRT+po+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTfRTpluspoplusdsbisbD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTfRTpluspoplusdsbisbC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTfRTpluspoplusdsbisbE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTpluspoplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTpluspoplusdsbisbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTpluspoplusdsbisbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTpluspoplusdsbisbO}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTpluspoplusdsbisbA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=0 & 2:R0=1 & 2:R2=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/BBM+dsb-tlbiis-dsb.tex <==
\newlength{\BBMplusdsbtlbiisdsbH}
\setlength{\BBMplusdsbtlbiisdsbH}{0cm}
\newsavebox{\BBMplusdsbtlbiisdsbI}
\begin{lrbox}{\BBMplusdsbtlbiisdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X6
DSB SY
STR X2,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\BBMplusdsbtlbiisdsbJ}
\settowidth{\BBMplusdsbtlbiisdsbJ}{\usebox{\BBMplusdsbtlbiisdsbI}}
\addtolength{\BBMplusdsbtlbiisdsbH}{\BBMplusdsbtlbiisdsbJ}
\newsavebox{\BBMplusdsbtlbiisdsbK}
\begin{lrbox}{\BBMplusdsbtlbiisdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\BBMplusdsbtlbiisdsbL}
\settowidth{\BBMplusdsbtlbiisdsbL}{\usebox{\BBMplusdsbtlbiisdsbK}}
\addtolength{\BBMplusdsbtlbiisdsbH}{\BBMplusdsbtlbiisdsbL}
\newsavebox{\BBMplusdsbtlbiisdsbM}
\begin{lrbox}{\BBMplusdsbtlbiisdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\BBMplusdsbtlbiisdsbN}
\settowidth{\BBMplusdsbtlbiisdsbN}{\usebox{\BBMplusdsbtlbiisdsbM}}
\addtolength{\BBMplusdsbtlbiisdsbH}{\BBMplusdsbtlbiisdsbN}
\newsavebox{\BBMplusdsbtlbiisdsbO}
\begin{lrbox}{\BBMplusdsbtlbiisdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;
    x ?-> pa2;

    identity 0x1000 with code;

    *pa2 = 2;
\end{lstlisting}
\end{lrbox}
\newlength{\BBMplusdsbtlbiisdsbP}
\settowidth{\BBMplusdsbtlbiisdsbP}{\usebox{\BBMplusdsbtlbiisdsbO}}
\newsavebox{\BBMplusdsbtlbiisdsbA}
\begin{lrbox}{\BBMplusdsbtlbiisdsbA}
\begin{minipage}{\BBMplusdsbtlbiisdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R4=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|BBM+dsb-tlbiis-dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\BBMplusdsbtlbiisdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\BBMplusdsbtlbiisdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\BBMplusdsbtlbiisdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\BBMplusdsbtlbiisdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\BBMplusdsbtlbiisdsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\BBMplusdsbtlbiisdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/BBM.Tf+dsb-tlbiis-dsb.tex <==
\newlength{\BBMdotTfplusdsbtlbiisdsbH}
\setlength{\BBMdotTfplusdsbtlbiisdsbH}{0cm}
\newsavebox{\BBMdotTfplusdsbtlbiisdsbI}
\begin{lrbox}{\BBMdotTfplusdsbtlbiisdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X6
DSB SY
STR X2,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\BBMdotTfplusdsbtlbiisdsbJ}
\settowidth{\BBMdotTfplusdsbtlbiisdsbJ}{\usebox{\BBMdotTfplusdsbtlbiisdsbI}}
\addtolength{\BBMdotTfplusdsbtlbiisdsbH}{\BBMdotTfplusdsbtlbiisdsbJ}
\newsavebox{\BBMdotTfplusdsbtlbiisdsbK}
\begin{lrbox}{\BBMdotTfplusdsbtlbiisdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\BBMdotTfplusdsbtlbiisdsbL}
\settowidth{\BBMdotTfplusdsbtlbiisdsbL}{\usebox{\BBMdotTfplusdsbtlbiisdsbK}}
\addtolength{\BBMdotTfplusdsbtlbiisdsbH}{\BBMdotTfplusdsbtlbiisdsbL}
\newsavebox{\BBMdotTfplusdsbtlbiisdsbM}
\begin{lrbox}{\BBMdotTfplusdsbtlbiisdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
\end{lstlisting}
\end{lrbox}
\newlength{\BBMdotTfplusdsbtlbiisdsbN}
\settowidth{\BBMdotTfplusdsbtlbiisdsbN}{\usebox{\BBMdotTfplusdsbtlbiisdsbM}}
\addtolength{\BBMdotTfplusdsbtlbiisdsbH}{\BBMdotTfplusdsbtlbiisdsbN}
\newsavebox{\BBMdotTfplusdsbtlbiisdsbO}
\begin{lrbox}{\BBMdotTfplusdsbtlbiisdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;
    x ?-> pa2;

    identity 0x1000 with code;

    *pa2 = 2;
\end{lstlisting}
\end{lrbox}
\newlength{\BBMdotTfplusdsbtlbiisdsbP}
\settowidth{\BBMdotTfplusdsbtlbiisdsbP}{\usebox{\BBMdotTfplusdsbtlbiisdsbO}}
\newsavebox{\BBMdotTfplusdsbtlbiisdsbA}
\begin{lrbox}{\BBMdotTfplusdsbtlbiisdsbA}
\begin{minipage}{\BBMdotTfplusdsbtlbiisdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R4=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|BBM.Tf+dsb-tlbiis-dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\BBMdotTfplusdsbtlbiisdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\BBMdotTfplusdsbtlbiisdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\BBMdotTfplusdsbtlbiisdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\BBMdotTfplusdsbtlbiisdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\BBMdotTfplusdsbtlbiisdsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\BBMdotTfplusdsbtlbiisdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/Break2.news1.tex <==
\newlength{\BreaktwodotnewsoneH}
\setlength{\BreaktwodotnewsoneH}{0cm}
\newsavebox{\BreaktwodotnewsoneI}
\begin{lrbox}{\BreaktwodotnewsoneI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1IS,X4
DSB SY
TLBI VMALLE1IS
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\BreaktwodotnewsoneJ}
\settowidth{\BreaktwodotnewsoneJ}{\usebox{\BreaktwodotnewsoneI}}
\addtolength{\BreaktwodotnewsoneH}{\BreaktwodotnewsoneJ}
\newsavebox{\BreaktwodotnewsoneK}
\begin{lrbox}{\BreaktwodotnewsoneK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\BreaktwodotnewsoneL}
\settowidth{\BreaktwodotnewsoneL}{\usebox{\BreaktwodotnewsoneK}}
\addtolength{\BreaktwodotnewsoneH}{\BreaktwodotnewsoneL}
\newsavebox{\BreaktwodotnewsoneM}
\begin{lrbox}{\BreaktwodotnewsoneM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#2
\end{lstlisting}
\end{lrbox}
\newlength{\BreaktwodotnewsoneN}
\settowidth{\BreaktwodotnewsoneN}{\usebox{\BreaktwodotnewsoneM}}
\addtolength{\BreaktwodotnewsoneH}{\BreaktwodotnewsoneN}
\newsavebox{\BreaktwodotnewsoneO}
\begin{lrbox}{\BreaktwodotnewsoneO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X0,#3
\end{lstlisting}
\end{lrbox}
\newlength{\BreaktwodotnewsoneP}
\settowidth{\BreaktwodotnewsoneP}{\usebox{\BreaktwodotnewsoneO}}
\addtolength{\BreaktwodotnewsoneH}{\BreaktwodotnewsoneP}
\newsavebox{\BreaktwodotnewsoneA}
\begin{lrbox}{\BreaktwodotnewsoneA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
option default_tables = false;
physical pa1;
intermediate ipa1;

s2table vm_stage2 0x240000  {
    ipa1 |-> pa1 at level 3;
    ipa1 ?-> invalid at level 3;
    identity pa_to_ipa(0x1000) with code;


    s1table vm_stage1 0x280000  {
        x |-> invalid at level 3;
        x ?-> ipa1 at level 3;

        identity pa_to_va(0x1000) with code;
    }
}

s1table hyp_map 0x200000 {
    identity 0x2000 with code;
    s2table vm_stage2;
    s1table vm_stage1;
}

*pa1 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\BreaktwodotnewsoneB}
\settowidth{\BreaktwodotnewsoneB}{\usebox{\BreaktwodotnewsoneA}}
\newsavebox{\BreaktwodotnewsoneC}
\begin{lrbox}{\BreaktwodotnewsoneC}
\begin{minipage}{\BreaktwodotnewsoneH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(ipa1,vm_stage2)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=ipa1)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(x,vm_stage1)|\\
\lstinline[language=IslaLitmusExp]|0:R4=bvlshr(ipa1,0xC)|\\
\lstinline[language=IslaLitmusExp]|0:TTBR0_EL2=ttbr(asid=0x0000,base=hyp_map)|\\
\lstinline[language=IslaLitmusExp]|0:VTTBR_EL2=ttbr(base=vm_stage2,vmid=0x0000)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:TTBR0_EL1=ttbr(base=vm_stage1,asid=0x0000)|\\
\lstinline[language=IslaLitmusExp]|1:TTBR0_EL2=ttbr(base=hyp_map,asid=0x0000)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\lstinline[language=IslaLitmusExp]|1:VTTBR_EL2=ttbr(vmid=0x0000,base=vm_stage2)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|Break2.news1|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\BreaktwodotnewsoneB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\BreaktwodotnewsoneA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\BreaktwodotnewsoneC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\BreaktwodotnewsoneI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\BreaktwodotnewsoneK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\BreaktwodotnewsoneM}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\BreaktwodotnewsoneO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoRR0.alias+po.tex <==
\newlength{\CoRRzerodotaliaspluspoH}
\setlength{\CoRRzerodotaliaspluspoH}{0cm}
\newsavebox{\CoRRzerodotaliaspluspoI}
\begin{lrbox}{\CoRRzerodotaliaspluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRRzerodotaliaspluspoJ}
\settowidth{\CoRRzerodotaliaspluspoJ}{\usebox{\CoRRzerodotaliaspluspoI}}
\addtolength{\CoRRzerodotaliaspluspoH}{\CoRRzerodotaliaspluspoJ}
\newsavebox{\CoRRzerodotaliaspluspoK}
\begin{lrbox}{\CoRRzerodotaliaspluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRRzerodotaliaspluspoL}
\settowidth{\CoRRzerodotaliaspluspoL}{\usebox{\CoRRzerodotaliaspluspoK}}
\addtolength{\CoRRzerodotaliaspluspoH}{\CoRRzerodotaliaspluspoL}
\newsavebox{\CoRRzerodotaliaspluspoM}
\begin{lrbox}{\CoRRzerodotaliaspluspoM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    y |-> pa1;
    *pa1 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRRzerodotaliaspluspoN}
\settowidth{\CoRRzerodotaliaspluspoN}{\usebox{\CoRRzerodotaliaspluspoM}}
\newsavebox{\CoRRzerodotaliaspluspoO}
\begin{lrbox}{\CoRRzerodotaliaspluspoO}
\begin{minipage}{\CoRRzerodotaliaspluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRR0.alias+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRRzerodotaliaspluspoN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRRzerodotaliaspluspoM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRRzerodotaliaspluspoO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRRzerodotaliaspluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRRzerodotaliaspluspoK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoRR2.alias+po.tex <==
\newlength{\CoRRtwodotaliaspluspoH}
\setlength{\CoRRtwodotaliaspluspoH}{0cm}
\newsavebox{\CoRRtwodotaliaspluspoI}
\begin{lrbox}{\CoRRtwodotaliaspluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRRtwodotaliaspluspoJ}
\settowidth{\CoRRtwodotaliaspluspoJ}{\usebox{\CoRRtwodotaliaspluspoI}}
\addtolength{\CoRRtwodotaliaspluspoH}{\CoRRtwodotaliaspluspoJ}
\newsavebox{\CoRRtwodotaliaspluspoK}
\begin{lrbox}{\CoRRtwodotaliaspluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRRtwodotaliaspluspoL}
\settowidth{\CoRRtwodotaliaspluspoL}{\usebox{\CoRRtwodotaliaspluspoK}}
\addtolength{\CoRRtwodotaliaspluspoH}{\CoRRtwodotaliaspluspoL}
\newsavebox{\CoRRtwodotaliaspluspoM}
\begin{lrbox}{\CoRRtwodotaliaspluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRRtwodotaliaspluspoN}
\settowidth{\CoRRtwodotaliaspluspoN}{\usebox{\CoRRtwodotaliaspluspoM}}
\addtolength{\CoRRtwodotaliaspluspoH}{\CoRRtwodotaliaspluspoN}
\newsavebox{\CoRRtwodotaliaspluspoO}
\begin{lrbox}{\CoRRtwodotaliaspluspoO}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRRtwodotaliaspluspoP}
\settowidth{\CoRRtwodotaliaspluspoP}{\usebox{\CoRRtwodotaliaspluspoO}}
\addtolength{\CoRRtwodotaliaspluspoH}{\CoRRtwodotaliaspluspoP}
\newsavebox{\CoRRtwodotaliaspluspoA}
\begin{lrbox}{\CoRRtwodotaliaspluspoA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    u |-> pa1;
    v |-> pa1;
    w |-> pa1;
    x |-> pa1;
    y |-> pa1;
    z |-> pa1;
    *pa1 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRRtwodotaliaspluspoB}
\settowidth{\CoRRtwodotaliaspluspoB}{\usebox{\CoRRtwodotaliaspluspoA}}
\newsavebox{\CoRRtwodotaliaspluspoC}
\begin{lrbox}{\CoRRtwodotaliaspluspoC}
\begin{minipage}{\CoRRtwodotaliaspluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R1=u|\\
\lstinline[language=IslaLitmusExp]|1:R0=0b10|\\
\lstinline[language=IslaLitmusExp]|1:R1=v|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=w|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|3:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|3:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|3:R1=y|\\
\lstinline[language=IslaLitmusExp]|3:R3=z|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRR2.alias+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRRtwodotaliaspluspoB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRRtwodotaliaspluspoA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRRtwodotaliaspluspoC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRRtwodotaliaspluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRRtwodotaliaspluspoK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\CoRRtwodotaliaspluspoM}\\
  \cline{2-2}
  & Thread 3\\
  \cline{2-2}
  & \usebox{\CoRRtwodotaliaspluspoO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|2:R0=1 & 2:R2=2 & 3:R0=2 & 3:R2=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoRT.inv+addr-trfi.tex <==
\newlength{\CoRTdotinvplusaddrtrfiH}
\setlength{\CoRTdotinvplusaddrtrfiH}{0cm}
\newsavebox{\CoRTdotinvplusaddrtrfiI}
\begin{lrbox}{\CoRTdotinvplusaddrtrfiI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRTdotinvplusaddrtrfiJ}
\settowidth{\CoRTdotinvplusaddrtrfiJ}{\usebox{\CoRTdotinvplusaddrtrfiI}}
\addtolength{\CoRTdotinvplusaddrtrfiH}{\CoRTdotinvplusaddrtrfiJ}
\newsavebox{\CoRTdotinvplusaddrtrfiK}
\begin{lrbox}{\CoRTdotinvplusaddrtrfiK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
STR X3,[X4,X2]
LDR X5,[X6]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRTdotinvplusaddrtrfiL}
\settowidth{\CoRTdotinvplusaddrtrfiL}{\usebox{\CoRTdotinvplusaddrtrfiK}}
\addtolength{\CoRTdotinvplusaddrtrfiH}{\CoRTdotinvplusaddrtrfiL}
\newsavebox{\CoRTdotinvplusaddrtrfiM}
\begin{lrbox}{\CoRTdotinvplusaddrtrfiM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X5,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoRTdotinvplusaddrtrfiN}
\settowidth{\CoRTdotinvplusaddrtrfiN}{\usebox{\CoRTdotinvplusaddrtrfiM}}
\addtolength{\CoRTdotinvplusaddrtrfiH}{\CoRTdotinvplusaddrtrfiN}
\newsavebox{\CoRTdotinvplusaddrtrfiO}
\begin{lrbox}{\CoRTdotinvplusaddrtrfiO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    y |-> invalid;
    y ?-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRTdotinvplusaddrtrfiP}
\settowidth{\CoRTdotinvplusaddrtrfiP}{\usebox{\CoRTdotinvplusaddrtrfiO}}
\newsavebox{\CoRTdotinvplusaddrtrfiA}
\begin{lrbox}{\CoRTdotinvplusaddrtrfiA}
\begin{minipage}{\CoRTdotinvplusaddrtrfiH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|1:R4=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R6=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRT.inv+addr-trfi|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRTdotinvplusaddrtrfiP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRTdotinvplusaddrtrfiO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRTdotinvplusaddrtrfiA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRTdotinvplusaddrtrfiI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRTdotinvplusaddrtrfiK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoRTdotinvplusaddrtrfiM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|true|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoRpteT+dsb-isb.tex <==
\newlength{\CoRpteTplusdsbisbH}
\setlength{\CoRpteTplusdsbisbH}{0cm}
\newsavebox{\CoRpteTplusdsbisbI}
\begin{lrbox}{\CoRpteTplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTplusdsbisbJ}
\settowidth{\CoRpteTplusdsbisbJ}{\usebox{\CoRpteTplusdsbisbI}}
\addtolength{\CoRpteTplusdsbisbH}{\CoRpteTplusdsbisbJ}
\newsavebox{\CoRpteTplusdsbisbK}
\begin{lrbox}{\CoRpteTplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTplusdsbisbL}
\settowidth{\CoRpteTplusdsbisbL}{\usebox{\CoRpteTplusdsbisbK}}
\addtolength{\CoRpteTplusdsbisbH}{\CoRpteTplusdsbisbL}
\newsavebox{\CoRpteTplusdsbisbM}
\begin{lrbox}{\CoRpteTplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTplusdsbisbN}
\settowidth{\CoRpteTplusdsbisbN}{\usebox{\CoRpteTplusdsbisbM}}
\addtolength{\CoRpteTplusdsbisbH}{\CoRpteTplusdsbisbN}
\newsavebox{\CoRpteTplusdsbisbO}
\begin{lrbox}{\CoRpteTplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;

    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;

    *pa1 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTplusdsbisbP}
\settowidth{\CoRpteTplusdsbisbP}{\usebox{\CoRpteTplusdsbisbO}}
\newsavebox{\CoRpteTplusdsbisbA}
\begin{lrbox}{\CoRpteTplusdsbisbA}
\begin{minipage}{\CoRpteTplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRpteT+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRpteTplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRpteTplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRpteTplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRpteTplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRpteTplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoRpteTplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=0 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoRpteT+dsb.tex <==
\newlength{\CoRpteTplusdsbH}
\setlength{\CoRpteTplusdsbH}{0cm}
\newsavebox{\CoRpteTplusdsbI}
\begin{lrbox}{\CoRpteTplusdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTplusdsbJ}
\settowidth{\CoRpteTplusdsbJ}{\usebox{\CoRpteTplusdsbI}}
\addtolength{\CoRpteTplusdsbH}{\CoRpteTplusdsbJ}
\newsavebox{\CoRpteTplusdsbK}
\begin{lrbox}{\CoRpteTplusdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTplusdsbL}
\settowidth{\CoRpteTplusdsbL}{\usebox{\CoRpteTplusdsbK}}
\addtolength{\CoRpteTplusdsbH}{\CoRpteTplusdsbL}
\newsavebox{\CoRpteTplusdsbM}
\begin{lrbox}{\CoRpteTplusdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTplusdsbN}
\settowidth{\CoRpteTplusdsbN}{\usebox{\CoRpteTplusdsbM}}
\addtolength{\CoRpteTplusdsbH}{\CoRpteTplusdsbN}
\newsavebox{\CoRpteTplusdsbO}
\begin{lrbox}{\CoRpteTplusdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;

    *x = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTplusdsbP}
\settowidth{\CoRpteTplusdsbP}{\usebox{\CoRpteTplusdsbO}}
\newsavebox{\CoRpteTplusdsbA}
\begin{lrbox}{\CoRpteTplusdsbA}
\begin{minipage}{\CoRpteTplusdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRpteT+dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRpteTplusdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRpteTplusdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRpteTplusdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRpteTplusdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRpteTplusdsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoRpteTplusdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=0 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoRpteT.EL1+dsb-tlbi-dsb-isb.tex <==
\newlength{\CoRpteTdotELoneplusdsbtlbidsbisbH}
\setlength{\CoRpteTdotELoneplusdsbtlbidsbisbH}{0cm}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbisbI}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTdotELoneplusdsbtlbidsbisbJ}
\settowidth{\CoRpteTdotELoneplusdsbtlbidsbisbJ}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbisbI}}
\addtolength{\CoRpteTdotELoneplusdsbtlbidsbisbH}{\CoRpteTdotELoneplusdsbtlbidsbisbJ}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbisbK}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
TLBI VAE1,X4
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTdotELoneplusdsbtlbidsbisbL}
\settowidth{\CoRpteTdotELoneplusdsbtlbidsbisbL}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbisbK}}
\addtolength{\CoRpteTdotELoneplusdsbtlbidsbisbH}{\CoRpteTdotELoneplusdsbtlbidsbisbL}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbisbM}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTdotELoneplusdsbtlbidsbisbN}
\settowidth{\CoRpteTdotELoneplusdsbtlbidsbisbN}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbisbM}}
\addtolength{\CoRpteTdotELoneplusdsbtlbidsbisbH}{\CoRpteTdotELoneplusdsbtlbidsbisbN}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbisbO}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;

    *pa1 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTdotELoneplusdsbtlbidsbisbP}
\settowidth{\CoRpteTdotELoneplusdsbtlbidsbisbP}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbisbO}}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbisbA}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbisbA}
\begin{minipage}{\CoRpteTdotELoneplusdsbtlbidsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRpteT.EL1+dsb-tlbi-dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRpteTdotELoneplusdsbtlbidsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRpteTdotELoneplusdsbtlbidsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRpteTdotELoneplusdsbtlbidsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRpteTdotELoneplusdsbtlbidsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoRpteTdotELoneplusdsbtlbidsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=0 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoRpteT.EL1+dsb-tlbi-dsb.tex <==
\newlength{\CoRpteTdotELoneplusdsbtlbidsbH}
\setlength{\CoRpteTdotELoneplusdsbtlbidsbH}{0cm}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbI}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTdotELoneplusdsbtlbidsbJ}
\settowidth{\CoRpteTdotELoneplusdsbtlbidsbJ}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbI}}
\addtolength{\CoRpteTdotELoneplusdsbtlbidsbH}{\CoRpteTdotELoneplusdsbtlbidsbJ}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbK}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
TLBI VAE1,X4
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTdotELoneplusdsbtlbidsbL}
\settowidth{\CoRpteTdotELoneplusdsbtlbidsbL}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbK}}
\addtolength{\CoRpteTdotELoneplusdsbtlbidsbH}{\CoRpteTdotELoneplusdsbtlbidsbL}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbM}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTdotELoneplusdsbtlbidsbN}
\settowidth{\CoRpteTdotELoneplusdsbtlbidsbN}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbM}}
\addtolength{\CoRpteTdotELoneplusdsbtlbidsbH}{\CoRpteTdotELoneplusdsbtlbidsbN}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbO}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;

    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;

    *pa1 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTdotELoneplusdsbtlbidsbP}
\settowidth{\CoRpteTdotELoneplusdsbtlbidsbP}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbO}}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbA}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbA}
\begin{minipage}{\CoRpteTdotELoneplusdsbtlbidsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRpteT.EL1+dsb-tlbi-dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRpteTdotELoneplusdsbtlbidsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRpteTdotELoneplusdsbtlbidsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRpteTdotELoneplusdsbtlbidsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRpteTdotELoneplusdsbtlbidsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoRpteTdotELoneplusdsbtlbidsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=0 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoRpteTf.inv+dsb-isb.tex <==
\newlength{\CoRpteTfdotinvplusdsbisbH}
\setlength{\CoRpteTfdotinvplusdsbisbH}{0cm}
\newsavebox{\CoRpteTfdotinvplusdsbisbI}
\begin{lrbox}{\CoRpteTfdotinvplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTfdotinvplusdsbisbJ}
\settowidth{\CoRpteTfdotinvplusdsbisbJ}{\usebox{\CoRpteTfdotinvplusdsbisbI}}
\addtolength{\CoRpteTfdotinvplusdsbisbH}{\CoRpteTfdotinvplusdsbisbJ}
\newsavebox{\CoRpteTfdotinvplusdsbisbK}
\begin{lrbox}{\CoRpteTfdotinvplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTfdotinvplusdsbisbL}
\settowidth{\CoRpteTfdotinvplusdsbisbL}{\usebox{\CoRpteTfdotinvplusdsbisbK}}
\addtolength{\CoRpteTfdotinvplusdsbisbH}{\CoRpteTfdotinvplusdsbisbL}
\newsavebox{\CoRpteTfdotinvplusdsbisbM}
\begin{lrbox}{\CoRpteTfdotinvplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTfdotinvplusdsbisbN}
\settowidth{\CoRpteTfdotinvplusdsbisbN}{\usebox{\CoRpteTfdotinvplusdsbisbM}}
\addtolength{\CoRpteTfdotinvplusdsbisbH}{\CoRpteTfdotinvplusdsbisbN}
\newsavebox{\CoRpteTfdotinvplusdsbisbO}
\begin{lrbox}{\CoRpteTfdotinvplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    option default_tables = true;
    physical pa1;
    intermediate ipa1;

    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    identity 0x1000 with code;

    *pa1 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTfdotinvplusdsbisbP}
\settowidth{\CoRpteTfdotinvplusdsbisbP}{\usebox{\CoRpteTfdotinvplusdsbisbO}}
\newsavebox{\CoRpteTfdotinvplusdsbisbA}
\begin{lrbox}{\CoRpteTfdotinvplusdsbisbA}
\begin{minipage}{\CoRpteTfdotinvplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRpteTf.inv+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRpteTfdotinvplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRpteTfdotinvplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRpteTfdotinvplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRpteTfdotinvplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRpteTfdotinvplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoRpteTfdotinvplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=desc3(y,page_table_base) & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoRpteTf.inv+dsb.tex <==
\newlength{\CoRpteTfdotinvplusdsbH}
\setlength{\CoRpteTfdotinvplusdsbH}{0cm}
\newsavebox{\CoRpteTfdotinvplusdsbI}
\begin{lrbox}{\CoRpteTfdotinvplusdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTfdotinvplusdsbJ}
\settowidth{\CoRpteTfdotinvplusdsbJ}{\usebox{\CoRpteTfdotinvplusdsbI}}
\addtolength{\CoRpteTfdotinvplusdsbH}{\CoRpteTfdotinvplusdsbJ}
\newsavebox{\CoRpteTfdotinvplusdsbK}
\begin{lrbox}{\CoRpteTfdotinvplusdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTfdotinvplusdsbL}
\settowidth{\CoRpteTfdotinvplusdsbL}{\usebox{\CoRpteTfdotinvplusdsbK}}
\addtolength{\CoRpteTfdotinvplusdsbH}{\CoRpteTfdotinvplusdsbL}
\newsavebox{\CoRpteTfdotinvplusdsbM}
\begin{lrbox}{\CoRpteTfdotinvplusdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTfdotinvplusdsbN}
\settowidth{\CoRpteTfdotinvplusdsbN}{\usebox{\CoRpteTfdotinvplusdsbM}}
\addtolength{\CoRpteTfdotinvplusdsbH}{\CoRpteTfdotinvplusdsbN}
\newsavebox{\CoRpteTfdotinvplusdsbO}
\begin{lrbox}{\CoRpteTfdotinvplusdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    identity 0x1000 with code;

    *pa1 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTfdotinvplusdsbP}
\settowidth{\CoRpteTfdotinvplusdsbP}{\usebox{\CoRpteTfdotinvplusdsbO}}
\newsavebox{\CoRpteTfdotinvplusdsbA}
\begin{lrbox}{\CoRpteTfdotinvplusdsbA}
\begin{minipage}{\CoRpteTfdotinvplusdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRpteTf.inv+dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRpteTfdotinvplusdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRpteTfdotinvplusdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRpteTfdotinvplusdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRpteTfdotinvplusdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRpteTfdotinvplusdsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoRpteTfdotinvplusdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=desc3(y,page_table_base) & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoTRpte.inv+dsb-isb.tex <==
\newlength{\CoTRptedotinvplusdsbisbH}
\setlength{\CoTRptedotinvplusdsbisbH}{0cm}
\newsavebox{\CoTRptedotinvplusdsbisbI}
\begin{lrbox}{\CoTRptedotinvplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvplusdsbisbJ}
\settowidth{\CoTRptedotinvplusdsbisbJ}{\usebox{\CoTRptedotinvplusdsbisbI}}
\addtolength{\CoTRptedotinvplusdsbisbH}{\CoTRptedotinvplusdsbisbJ}
\newsavebox{\CoTRptedotinvplusdsbisbK}
\begin{lrbox}{\CoTRptedotinvplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvplusdsbisbL}
\settowidth{\CoTRptedotinvplusdsbisbL}{\usebox{\CoTRptedotinvplusdsbisbK}}
\addtolength{\CoTRptedotinvplusdsbisbH}{\CoTRptedotinvplusdsbisbL}
\newsavebox{\CoTRptedotinvplusdsbisbM}
\begin{lrbox}{\CoTRptedotinvplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvplusdsbisbN}
\settowidth{\CoTRptedotinvplusdsbisbN}{\usebox{\CoTRptedotinvplusdsbisbM}}
\addtolength{\CoTRptedotinvplusdsbisbH}{\CoTRptedotinvplusdsbisbN}
\newsavebox{\CoTRptedotinvplusdsbisbO}
\begin{lrbox}{\CoTRptedotinvplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvplusdsbisbP}
\settowidth{\CoTRptedotinvplusdsbisbP}{\usebox{\CoTRptedotinvplusdsbisbO}}
\newsavebox{\CoTRptedotinvplusdsbisbA}
\begin{lrbox}{\CoTRptedotinvplusdsbisbA}
\begin{minipage}{\CoTRptedotinvplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTRpte.inv+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTRptedotinvplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTRptedotinvplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTRptedotinvplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoTRpte.inv+dsb.tex <==
\newlength{\CoTRptedotinvplusdsbH}
\setlength{\CoTRptedotinvplusdsbH}{0cm}
\newsavebox{\CoTRptedotinvplusdsbI}
\begin{lrbox}{\CoTRptedotinvplusdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvplusdsbJ}
\settowidth{\CoTRptedotinvplusdsbJ}{\usebox{\CoTRptedotinvplusdsbI}}
\addtolength{\CoTRptedotinvplusdsbH}{\CoTRptedotinvplusdsbJ}
\newsavebox{\CoTRptedotinvplusdsbK}
\begin{lrbox}{\CoTRptedotinvplusdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvplusdsbL}
\settowidth{\CoTRptedotinvplusdsbL}{\usebox{\CoTRptedotinvplusdsbK}}
\addtolength{\CoTRptedotinvplusdsbH}{\CoTRptedotinvplusdsbL}
\newsavebox{\CoTRptedotinvplusdsbM}
\begin{lrbox}{\CoTRptedotinvplusdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvplusdsbN}
\settowidth{\CoTRptedotinvplusdsbN}{\usebox{\CoTRptedotinvplusdsbM}}
\addtolength{\CoTRptedotinvplusdsbH}{\CoTRptedotinvplusdsbN}
\newsavebox{\CoTRptedotinvplusdsbO}
\begin{lrbox}{\CoTRptedotinvplusdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *y = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvplusdsbP}
\settowidth{\CoTRptedotinvplusdsbP}{\usebox{\CoTRptedotinvplusdsbO}}
\newsavebox{\CoTRptedotinvplusdsbA}
\begin{lrbox}{\CoTRptedotinvplusdsbA}
\begin{minipage}{\CoTRptedotinvplusdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTRpte.inv+dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTRptedotinvplusdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTRptedotinvplusdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTRptedotinvplusdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvplusdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvplusdsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvplusdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoTRpte.inv+po.tex <==
\newlength{\CoTRptedotinvpluspoH}
\setlength{\CoTRptedotinvpluspoH}{0cm}
\newsavebox{\CoTRptedotinvpluspoI}
\begin{lrbox}{\CoTRptedotinvpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvpluspoJ}
\settowidth{\CoTRptedotinvpluspoJ}{\usebox{\CoTRptedotinvpluspoI}}
\addtolength{\CoTRptedotinvpluspoH}{\CoTRptedotinvpluspoJ}
\newsavebox{\CoTRptedotinvpluspoK}
\begin{lrbox}{\CoTRptedotinvpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvpluspoL}
\settowidth{\CoTRptedotinvpluspoL}{\usebox{\CoTRptedotinvpluspoK}}
\addtolength{\CoTRptedotinvpluspoH}{\CoTRptedotinvpluspoL}
\newsavebox{\CoTRptedotinvpluspoM}
\begin{lrbox}{\CoTRptedotinvpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvpluspoN}
\settowidth{\CoTRptedotinvpluspoN}{\usebox{\CoTRptedotinvpluspoM}}
\addtolength{\CoTRptedotinvpluspoH}{\CoTRptedotinvpluspoN}
\newsavebox{\CoTRptedotinvpluspoO}
\begin{lrbox}{\CoTRptedotinvpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *y = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvpluspoP}
\settowidth{\CoTRptedotinvpluspoP}{\usebox{\CoTRptedotinvpluspoO}}
\newsavebox{\CoTRptedotinvpluspoA}
\begin{lrbox}{\CoTRptedotinvpluspoA}
\begin{minipage}{\CoTRptedotinvpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTRpte.inv+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTRptedotinvpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTRptedotinvpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTRptedotinvpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoTT.ro+dmb.tex <==
\newlength{\CoTTdotroplusdmbH}
\setlength{\CoTTdotroplusdmbH}{0cm}
\newsavebox{\CoTTdotroplusdmbI}
\begin{lrbox}{\CoTTdotroplusdmbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotroplusdmbJ}
\settowidth{\CoTTdotroplusdmbJ}{\usebox{\CoTTdotroplusdmbI}}
\addtolength{\CoTTdotroplusdmbH}{\CoTTdotroplusdmbJ}
\newsavebox{\CoTTdotroplusdmbK}
\begin{lrbox}{\CoTTdotroplusdmbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotroplusdmbL}
\settowidth{\CoTTdotroplusdmbL}{\usebox{\CoTTdotroplusdmbK}}
\addtolength{\CoTTdotroplusdmbH}{\CoTTdotroplusdmbL}
\newsavebox{\CoTTdotroplusdmbM}
\begin{lrbox}{\CoTTdotroplusdmbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1 with [AP = 0b11] and default;
    x ?-> pa2 with [AP = 0b11] and default;
    y |-> pa2 with [AP = 0b11] and default;

    *pa2 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotroplusdmbN}
\settowidth{\CoTTdotroplusdmbN}{\usebox{\CoTTdotroplusdmbM}}
\newsavebox{\CoTTdotroplusdmbO}
\begin{lrbox}{\CoTTdotroplusdmbO}
\begin{minipage}{\CoTTdotroplusdmbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTT.ro+dmb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTTdotroplusdmbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTTdotroplusdmbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTTdotroplusdmbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTTdotroplusdmbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTTdotroplusdmbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoTT.ro+dsb-isb.tex <==
\newlength{\CoTTdotroplusdsbisbH}
\setlength{\CoTTdotroplusdsbisbH}{0cm}
\newsavebox{\CoTTdotroplusdsbisbI}
\begin{lrbox}{\CoTTdotroplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotroplusdsbisbJ}
\settowidth{\CoTTdotroplusdsbisbJ}{\usebox{\CoTTdotroplusdsbisbI}}
\addtolength{\CoTTdotroplusdsbisbH}{\CoTTdotroplusdsbisbJ}
\newsavebox{\CoTTdotroplusdsbisbK}
\begin{lrbox}{\CoTTdotroplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotroplusdsbisbL}
\settowidth{\CoTTdotroplusdsbisbL}{\usebox{\CoTTdotroplusdsbisbK}}
\addtolength{\CoTTdotroplusdsbisbH}{\CoTTdotroplusdsbisbL}
\newsavebox{\CoTTdotroplusdsbisbM}
\begin{lrbox}{\CoTTdotroplusdsbisbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1 with [AP = 0b11] and default;
    x ?-> pa2 with [AP = 0b11] and default;
    y |-> pa2 with [AP = 0b11] and default;

    *pa2 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotroplusdsbisbN}
\settowidth{\CoTTdotroplusdsbisbN}{\usebox{\CoTTdotroplusdsbisbM}}
\newsavebox{\CoTTdotroplusdsbisbO}
\begin{lrbox}{\CoTTdotroplusdsbisbO}
\begin{minipage}{\CoTTdotroplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTT.ro+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTTdotroplusdsbisbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTTdotroplusdsbisbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTTdotroplusdsbisbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTTdotroplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTTdotroplusdsbisbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoTT.ro+po.tex <==
\newlength{\CoTTdotropluspoH}
\setlength{\CoTTdotropluspoH}{0cm}
\newsavebox{\CoTTdotropluspoI}
\begin{lrbox}{\CoTTdotropluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotropluspoJ}
\settowidth{\CoTTdotropluspoJ}{\usebox{\CoTTdotropluspoI}}
\addtolength{\CoTTdotropluspoH}{\CoTTdotropluspoJ}
\newsavebox{\CoTTdotropluspoK}
\begin{lrbox}{\CoTTdotropluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotropluspoL}
\settowidth{\CoTTdotropluspoL}{\usebox{\CoTTdotropluspoK}}
\addtolength{\CoTTdotropluspoH}{\CoTTdotropluspoL}
\newsavebox{\CoTTdotropluspoM}
\begin{lrbox}{\CoTTdotropluspoM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1 with [AP = 0b11] and default;
    x ?-> pa2 with [AP = 0b11] and default;
    y |-> pa2 with [AP = 0b11] and default;

    *pa2 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotropluspoN}
\settowidth{\CoTTdotropluspoN}{\usebox{\CoTTdotropluspoM}}
\newsavebox{\CoTTdotropluspoO}
\begin{lrbox}{\CoTTdotropluspoO}
\begin{minipage}{\CoTTdotropluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTT.ro+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTTdotropluspoN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTTdotropluspoM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTTdotropluspoO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTTdotropluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTTdotropluspoK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoTTf.inv+dsb-isb.tex <==
\newlength{\CoTTfdotinvplusdsbisbH}
\setlength{\CoTTfdotinvplusdsbisbH}{0cm}
\newsavebox{\CoTTfdotinvplusdsbisbI}
\begin{lrbox}{\CoTTfdotinvplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTfdotinvplusdsbisbJ}
\settowidth{\CoTTfdotinvplusdsbisbJ}{\usebox{\CoTTfdotinvplusdsbisbI}}
\addtolength{\CoTTfdotinvplusdsbisbH}{\CoTTfdotinvplusdsbisbJ}
\newsavebox{\CoTTfdotinvplusdsbisbK}
\begin{lrbox}{\CoTTfdotinvplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTfdotinvplusdsbisbL}
\settowidth{\CoTTfdotinvplusdsbisbL}{\usebox{\CoTTfdotinvplusdsbisbK}}
\addtolength{\CoTTfdotinvplusdsbisbH}{\CoTTfdotinvplusdsbisbL}
\newsavebox{\CoTTfdotinvplusdsbisbM}
\begin{lrbox}{\CoTTfdotinvplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTfdotinvplusdsbisbN}
\settowidth{\CoTTfdotinvplusdsbisbN}{\usebox{\CoTTfdotinvplusdsbisbM}}
\addtolength{\CoTTfdotinvplusdsbisbH}{\CoTTfdotinvplusdsbisbN}
\newsavebox{\CoTTfdotinvplusdsbisbO}
\begin{lrbox}{\CoTTfdotinvplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTfdotinvplusdsbisbP}
\settowidth{\CoTTfdotinvplusdsbisbP}{\usebox{\CoTTfdotinvplusdsbisbO}}
\newsavebox{\CoTTfdotinvplusdsbisbA}
\begin{lrbox}{\CoTTfdotinvplusdsbisbA}
\begin{minipage}{\CoTTfdotinvplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTTf.inv+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTTfdotinvplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTTfdotinvplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTTfdotinvplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTTfdotinvplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTTfdotinvplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTTfdotinvplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoTTf.inv+po.tex <==
\newlength{\CoTTfdotinvpluspoH}
\setlength{\CoTTfdotinvpluspoH}{0cm}
\newsavebox{\CoTTfdotinvpluspoI}
\begin{lrbox}{\CoTTfdotinvpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTfdotinvpluspoJ}
\settowidth{\CoTTfdotinvpluspoJ}{\usebox{\CoTTfdotinvpluspoI}}
\addtolength{\CoTTfdotinvpluspoH}{\CoTTfdotinvpluspoJ}
\newsavebox{\CoTTfdotinvpluspoK}
\begin{lrbox}{\CoTTfdotinvpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTfdotinvpluspoL}
\settowidth{\CoTTfdotinvpluspoL}{\usebox{\CoTTfdotinvpluspoK}}
\addtolength{\CoTTfdotinvpluspoH}{\CoTTfdotinvpluspoL}
\newsavebox{\CoTTfdotinvpluspoM}
\begin{lrbox}{\CoTTfdotinvpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTfdotinvpluspoN}
\settowidth{\CoTTfdotinvpluspoN}{\usebox{\CoTTfdotinvpluspoM}}
\addtolength{\CoTTfdotinvpluspoH}{\CoTTfdotinvpluspoN}
\newsavebox{\CoTTfdotinvpluspoO}
\begin{lrbox}{\CoTTfdotinvpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTfdotinvpluspoP}
\settowidth{\CoTTfdotinvpluspoP}{\usebox{\CoTTfdotinvpluspoO}}
\newsavebox{\CoTTfdotinvpluspoA}
\begin{lrbox}{\CoTTfdotinvpluspoA}
\begin{minipage}{\CoTTfdotinvpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTTf.inv+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTTfdotinvpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTTfdotinvpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTTfdotinvpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTTfdotinvpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTTfdotinvpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTTfdotinvpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoTW1.inv.tex <==
\newlength{\CoTWonedotinvH}
\setlength{\CoTWonedotinvH}{0cm}
\newsavebox{\CoTWonedotinvI}
\begin{lrbox}{\CoTWonedotinvI}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTWonedotinvJ}
\settowidth{\CoTWonedotinvJ}{\usebox{\CoTWonedotinvI}}
\addtolength{\CoTWonedotinvH}{\CoTWonedotinvJ}
\newsavebox{\CoTWonedotinvK}
\begin{lrbox}{\CoTWonedotinvK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTWonedotinvL}
\settowidth{\CoTWonedotinvL}{\usebox{\CoTWonedotinvK}}
\addtolength{\CoTWonedotinvH}{\CoTWonedotinvL}
\newsavebox{\CoTWonedotinvM}
\begin{lrbox}{\CoTWonedotinvM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTWonedotinvN}
\settowidth{\CoTWonedotinvN}{\usebox{\CoTWonedotinvM}}
\newsavebox{\CoTWonedotinvO}
\begin{lrbox}{\CoTWonedotinvO}
\begin{minipage}{\CoTWonedotinvH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=x|\\
\lstinline[language=IslaLitmusExp]|R2=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTW1.inv|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTWonedotinvN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTWonedotinvM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTWonedotinvO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTWonedotinvI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTWonedotinvK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoTWinv.tex <==
\newlength{\CoTWinvH}
\setlength{\CoTWinvH}{0cm}
\newsavebox{\CoTWinvI}
\begin{lrbox}{\CoTWinvI}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTWinvJ}
\settowidth{\CoTWinvJ}{\usebox{\CoTWinvI}}
\addtolength{\CoTWinvH}{\CoTWinvJ}
\newsavebox{\CoTWinvK}
\begin{lrbox}{\CoTWinvK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTWinvL}
\settowidth{\CoTWinvL}{\usebox{\CoTWinvK}}
\addtolength{\CoTWinvH}{\CoTWinvL}
\newsavebox{\CoTWinvM}
\begin{lrbox}{\CoTWinvM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTWinvN}
\settowidth{\CoTWinvN}{\usebox{\CoTWinvM}}
\newsavebox{\CoTWinvO}
\begin{lrbox}{\CoTWinvO}
\begin{minipage}{\CoTWinvH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=x|\\
\lstinline[language=IslaLitmusExp]|R2=0b0|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTWinv|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTWinvN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTWinvM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTWinvO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTWinvI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTWinvK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoTfRpte+dsb-isb.tex <==
\newlength{\CoTfRpteplusdsbisbH}
\setlength{\CoTfRpteplusdsbisbH}{0cm}
\newsavebox{\CoTfRpteplusdsbisbI}
\begin{lrbox}{\CoTfRpteplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRpteplusdsbisbJ}
\settowidth{\CoTfRpteplusdsbisbJ}{\usebox{\CoTfRpteplusdsbisbI}}
\addtolength{\CoTfRpteplusdsbisbH}{\CoTfRpteplusdsbisbJ}
\newsavebox{\CoTfRpteplusdsbisbK}
\begin{lrbox}{\CoTfRpteplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRpteplusdsbisbL}
\settowidth{\CoTfRpteplusdsbisbL}{\usebox{\CoTfRpteplusdsbisbK}}
\addtolength{\CoTfRpteplusdsbisbH}{\CoTfRpteplusdsbisbL}
\newsavebox{\CoTfRpteplusdsbisbM}
\begin{lrbox}{\CoTfRpteplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRpteplusdsbisbN}
\settowidth{\CoTfRpteplusdsbisbN}{\usebox{\CoTfRpteplusdsbisbM}}
\addtolength{\CoTfRpteplusdsbisbH}{\CoTfRpteplusdsbisbN}
\newsavebox{\CoTfRpteplusdsbisbO}
\begin{lrbox}{\CoTfRpteplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;
    y |-> pa1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRpteplusdsbisbP}
\settowidth{\CoTfRpteplusdsbisbP}{\usebox{\CoTfRpteplusdsbisbO}}
\newsavebox{\CoTfRpteplusdsbisbA}
\begin{lrbox}{\CoTfRpteplusdsbisbA}
\begin{minipage}{\CoTfRpteplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfRpte+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfRpteplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfRpteplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfRpteplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfRpteplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTfRpteplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfRpteplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=desc3(y,page_table_base)|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoTfRpte+dsb.tex <==
\newlength{\CoTfRpteplusdsbH}
\setlength{\CoTfRpteplusdsbH}{0cm}
\newsavebox{\CoTfRpteplusdsbI}
\begin{lrbox}{\CoTfRpteplusdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRpteplusdsbJ}
\settowidth{\CoTfRpteplusdsbJ}{\usebox{\CoTfRpteplusdsbI}}
\addtolength{\CoTfRpteplusdsbH}{\CoTfRpteplusdsbJ}
\newsavebox{\CoTfRpteplusdsbK}
\begin{lrbox}{\CoTfRpteplusdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRpteplusdsbL}
\settowidth{\CoTfRpteplusdsbL}{\usebox{\CoTfRpteplusdsbK}}
\addtolength{\CoTfRpteplusdsbH}{\CoTfRpteplusdsbL}
\newsavebox{\CoTfRpteplusdsbM}
\begin{lrbox}{\CoTfRpteplusdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRpteplusdsbN}
\settowidth{\CoTfRpteplusdsbN}{\usebox{\CoTfRpteplusdsbM}}
\addtolength{\CoTfRpteplusdsbH}{\CoTfRpteplusdsbN}
\newsavebox{\CoTfRpteplusdsbO}
\begin{lrbox}{\CoTfRpteplusdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;
    y |-> pa1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRpteplusdsbP}
\settowidth{\CoTfRpteplusdsbP}{\usebox{\CoTfRpteplusdsbO}}
\newsavebox{\CoTfRpteplusdsbA}
\begin{lrbox}{\CoTfRpteplusdsbA}
\begin{minipage}{\CoTfRpteplusdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfRpte+dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfRpteplusdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfRpteplusdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfRpteplusdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfRpteplusdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTfRpteplusdsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfRpteplusdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=desc3(y,page_table_base)|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoTfRpte+eret.tex <==
\newlength{\CoTfRptepluseretH}
\setlength{\CoTfRptepluseretH}{0cm}
\newsavebox{\CoTfRptepluseretI}
\begin{lrbox}{\CoTfRptepluseretI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRptepluseretJ}
\settowidth{\CoTfRptepluseretJ}{\usebox{\CoTfRptepluseretI}}
\addtolength{\CoTfRptepluseretH}{\CoTfRptepluseretJ}
\newsavebox{\CoTfRptepluseretK}
\begin{lrbox}{\CoTfRptepluseretK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRptepluseretL}
\settowidth{\CoTfRptepluseretL}{\usebox{\CoTfRptepluseretK}}
\addtolength{\CoTfRptepluseretH}{\CoTfRptepluseretL}
\newsavebox{\CoTfRptepluseretM}
\begin{lrbox}{\CoTfRptepluseretM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRptepluseretN}
\settowidth{\CoTfRptepluseretN}{\usebox{\CoTfRptepluseretM}}
\addtolength{\CoTfRptepluseretH}{\CoTfRptepluseretN}
\newsavebox{\CoTfRptepluseretO}
\begin{lrbox}{\CoTfRptepluseretO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;
    y |-> pa1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRptepluseretP}
\settowidth{\CoTfRptepluseretP}{\usebox{\CoTfRptepluseretO}}
\newsavebox{\CoTfRptepluseretA}
\begin{lrbox}{\CoTfRptepluseretA}
\begin{minipage}{\CoTfRptepluseretH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfRpte+eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfRptepluseretP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfRptepluseretO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfRptepluseretA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfRptepluseretI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTfRptepluseretK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfRptepluseretM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=desc3(y,page_table_base)|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoTfRpte+po.tex <==
\newlength{\CoTfRptepluspoH}
\setlength{\CoTfRptepluspoH}{0cm}
\newsavebox{\CoTfRptepluspoI}
\begin{lrbox}{\CoTfRptepluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRptepluspoJ}
\settowidth{\CoTfRptepluspoJ}{\usebox{\CoTfRptepluspoI}}
\addtolength{\CoTfRptepluspoH}{\CoTfRptepluspoJ}
\newsavebox{\CoTfRptepluspoK}
\begin{lrbox}{\CoTfRptepluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRptepluspoL}
\settowidth{\CoTfRptepluspoL}{\usebox{\CoTfRptepluspoK}}
\addtolength{\CoTfRptepluspoH}{\CoTfRptepluspoL}
\newsavebox{\CoTfRptepluspoM}
\begin{lrbox}{\CoTfRptepluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRptepluspoN}
\settowidth{\CoTfRptepluspoN}{\usebox{\CoTfRptepluspoM}}
\addtolength{\CoTfRptepluspoH}{\CoTfRptepluspoN}
\newsavebox{\CoTfRptepluspoO}
\begin{lrbox}{\CoTfRptepluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;
    y |-> pa1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRptepluspoP}
\settowidth{\CoTfRptepluspoP}{\usebox{\CoTfRptepluspoO}}
\newsavebox{\CoTfRptepluspoA}
\begin{lrbox}{\CoTfRptepluspoA}
\begin{minipage}{\CoTfRptepluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfRpte+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfRptepluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfRptepluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfRptepluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfRptepluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTfRptepluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfRptepluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=desc3(y,page_table_base)|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoTfT+dsb-isb.tex <==
\newlength{\CoTfTplusdsbisbH}
\setlength{\CoTfTplusdsbisbH}{0cm}
\newsavebox{\CoTfTplusdsbisbI}
\begin{lrbox}{\CoTfTplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfTplusdsbisbJ}
\settowidth{\CoTfTplusdsbisbJ}{\usebox{\CoTfTplusdsbisbI}}
\addtolength{\CoTfTplusdsbisbH}{\CoTfTplusdsbisbJ}
\newsavebox{\CoTfTplusdsbisbK}
\begin{lrbox}{\CoTfTplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfTplusdsbisbL}
\settowidth{\CoTfTplusdsbisbL}{\usebox{\CoTfTplusdsbisbK}}
\addtolength{\CoTfTplusdsbisbH}{\CoTfTplusdsbisbL}
\newsavebox{\CoTfTplusdsbisbM}
\begin{lrbox}{\CoTfTplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfTplusdsbisbN}
\settowidth{\CoTfTplusdsbisbN}{\usebox{\CoTfTplusdsbisbM}}
\addtolength{\CoTfTplusdsbisbH}{\CoTfTplusdsbisbN}
\newsavebox{\CoTfTplusdsbisbO}
\begin{lrbox}{\CoTfTplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;
    y |-> pa1;
    *pa1 = 0;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfTplusdsbisbP}
\settowidth{\CoTfTplusdsbisbP}{\usebox{\CoTfTplusdsbisbO}}
\newsavebox{\CoTfTplusdsbisbA}
\begin{lrbox}{\CoTfTplusdsbisbA}
\begin{minipage}{\CoTfTplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfT+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfTplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfTplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfTplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfTplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTfTplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfTplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoTfT+po.tex <==
\newlength{\CoTfTpluspoH}
\setlength{\CoTfTpluspoH}{0cm}
\newsavebox{\CoTfTpluspoI}
\begin{lrbox}{\CoTfTpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfTpluspoJ}
\settowidth{\CoTfTpluspoJ}{\usebox{\CoTfTpluspoI}}
\addtolength{\CoTfTpluspoH}{\CoTfTpluspoJ}
\newsavebox{\CoTfTpluspoK}
\begin{lrbox}{\CoTfTpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfTpluspoL}
\settowidth{\CoTfTpluspoL}{\usebox{\CoTfTpluspoK}}
\addtolength{\CoTfTpluspoH}{\CoTfTpluspoL}
\newsavebox{\CoTfTpluspoM}
\begin{lrbox}{\CoTfTpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfTpluspoN}
\settowidth{\CoTfTpluspoN}{\usebox{\CoTfTpluspoM}}
\addtolength{\CoTfTpluspoH}{\CoTfTpluspoN}
\newsavebox{\CoTfTpluspoO}
\begin{lrbox}{\CoTfTpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;
    y |-> pa1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfTpluspoP}
\settowidth{\CoTfTpluspoP}{\usebox{\CoTfTpluspoO}}
\newsavebox{\CoTfTpluspoA}
\begin{lrbox}{\CoTfTpluspoA}
\begin{minipage}{\CoTfTpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfT+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfTpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfTpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfTpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfTpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTfTpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfTpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoTfW.inv+dsb-isb.tex <==
\newlength{\CoTfWdotinvplusdsbisbH}
\setlength{\CoTfWdotinvplusdsbisbH}{0cm}
\newsavebox{\CoTfWdotinvplusdsbisbI}
\begin{lrbox}{\CoTfWdotinvplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvplusdsbisbJ}
\settowidth{\CoTfWdotinvplusdsbisbJ}{\usebox{\CoTfWdotinvplusdsbisbI}}
\addtolength{\CoTfWdotinvplusdsbisbH}{\CoTfWdotinvplusdsbisbJ}
\newsavebox{\CoTfWdotinvplusdsbisbK}
\begin{lrbox}{\CoTfWdotinvplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvplusdsbisbL}
\settowidth{\CoTfWdotinvplusdsbisbL}{\usebox{\CoTfWdotinvplusdsbisbK}}
\addtolength{\CoTfWdotinvplusdsbisbH}{\CoTfWdotinvplusdsbisbL}
\newsavebox{\CoTfWdotinvplusdsbisbM}
\begin{lrbox}{\CoTfWdotinvplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvplusdsbisbN}
\settowidth{\CoTfWdotinvplusdsbisbN}{\usebox{\CoTfWdotinvplusdsbisbM}}
\addtolength{\CoTfWdotinvplusdsbisbH}{\CoTfWdotinvplusdsbisbN}
\newsavebox{\CoTfWdotinvplusdsbisbO}
\begin{lrbox}{\CoTfWdotinvplusdsbisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvplusdsbisbP}
\settowidth{\CoTfWdotinvplusdsbisbP}{\usebox{\CoTfWdotinvplusdsbisbO}}
\addtolength{\CoTfWdotinvplusdsbisbH}{\CoTfWdotinvplusdsbisbP}
\newsavebox{\CoTfWdotinvplusdsbisbA}
\begin{lrbox}{\CoTfWdotinvplusdsbisbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    x ?-> raw(2);
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvplusdsbisbB}
\settowidth{\CoTfWdotinvplusdsbisbB}{\usebox{\CoTfWdotinvplusdsbisbA}}
\newsavebox{\CoTfWdotinvplusdsbisbC}
\begin{lrbox}{\CoTfWdotinvplusdsbisbC}
\begin{minipage}{\CoTfWdotinvplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b10|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:R1=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfW.inv+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfWdotinvplusdsbisbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfWdotinvplusdsbisbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfWdotinvplusdsbisbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfWdotinvplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTfWdotinvplusdsbisbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\CoTfWdotinvplusdsbisbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfWdotinvplusdsbisbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=2 & 2:R2=mkdesc3(oa=pa1)|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoTfW.inv+po.tex <==
\newlength{\CoTfWdotinvpluspoH}
\setlength{\CoTfWdotinvpluspoH}{0cm}
\newsavebox{\CoTfWdotinvpluspoI}
\begin{lrbox}{\CoTfWdotinvpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvpluspoJ}
\settowidth{\CoTfWdotinvpluspoJ}{\usebox{\CoTfWdotinvpluspoI}}
\addtolength{\CoTfWdotinvpluspoH}{\CoTfWdotinvpluspoJ}
\newsavebox{\CoTfWdotinvpluspoK}
\begin{lrbox}{\CoTfWdotinvpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvpluspoL}
\settowidth{\CoTfWdotinvpluspoL}{\usebox{\CoTfWdotinvpluspoK}}
\addtolength{\CoTfWdotinvpluspoH}{\CoTfWdotinvpluspoL}
\newsavebox{\CoTfWdotinvpluspoM}
\begin{lrbox}{\CoTfWdotinvpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvpluspoN}
\settowidth{\CoTfWdotinvpluspoN}{\usebox{\CoTfWdotinvpluspoM}}
\addtolength{\CoTfWdotinvpluspoH}{\CoTfWdotinvpluspoN}
\newsavebox{\CoTfWdotinvpluspoO}
\begin{lrbox}{\CoTfWdotinvpluspoO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvpluspoP}
\settowidth{\CoTfWdotinvpluspoP}{\usebox{\CoTfWdotinvpluspoO}}
\addtolength{\CoTfWdotinvpluspoH}{\CoTfWdotinvpluspoP}
\newsavebox{\CoTfWdotinvpluspoA}
\begin{lrbox}{\CoTfWdotinvpluspoA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    x ?-> raw(2);
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvpluspoB}
\settowidth{\CoTfWdotinvpluspoB}{\usebox{\CoTfWdotinvpluspoA}}
\newsavebox{\CoTfWdotinvpluspoC}
\begin{lrbox}{\CoTfWdotinvpluspoC}
\begin{minipage}{\CoTfWdotinvpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b10|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:R1=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfW.inv+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfWdotinvpluspoB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfWdotinvpluspoA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfWdotinvpluspoC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfWdotinvpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTfWdotinvpluspoK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\CoTfWdotinvpluspoM}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfWdotinvpluspoO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=2 & 2:R2=mkdesc3(oa=pa1)|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoTfW1.inv+si.tex <==
\newlength{\CoTfWonedotinvplussiH}
\setlength{\CoTfWonedotinvplussiH}{0cm}
\newsavebox{\CoTfWonedotinvplussiI}
\begin{lrbox}{\CoTfWonedotinvplussiI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWonedotinvplussiJ}
\settowidth{\CoTfWonedotinvplussiJ}{\usebox{\CoTfWonedotinvplussiI}}
\addtolength{\CoTfWonedotinvplussiH}{\CoTfWonedotinvplussiJ}
\newsavebox{\CoTfWonedotinvplussiK}
\begin{lrbox}{\CoTfWonedotinvplussiK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWonedotinvplussiL}
\settowidth{\CoTfWonedotinvplussiL}{\usebox{\CoTfWonedotinvplussiK}}
\addtolength{\CoTfWonedotinvplussiH}{\CoTfWonedotinvplussiL}
\newsavebox{\CoTfWonedotinvplussiM}
\begin{lrbox}{\CoTfWonedotinvplussiM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWonedotinvplussiN}
\settowidth{\CoTfWonedotinvplussiN}{\usebox{\CoTfWonedotinvplussiM}}
\newsavebox{\CoTfWonedotinvplussiO}
\begin{lrbox}{\CoTfWonedotinvplussiO}
\begin{minipage}{\CoTfWonedotinvplussiH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=0b10|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(0x1000,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfW1.inv+si|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfWonedotinvplussiN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfWonedotinvplussiM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfWonedotinvplussiO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfWonedotinvplussiI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfWonedotinvplussiK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R0=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoWR.alias.tex <==
\newlength{\CoWRdotaliasH}
\setlength{\CoWRdotaliasH}{0cm}
\newsavebox{\CoWRdotaliasI}
\begin{lrbox}{\CoWRdotaliasI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWRdotaliasJ}
\settowidth{\CoWRdotaliasJ}{\usebox{\CoWRdotaliasI}}
\addtolength{\CoWRdotaliasH}{\CoWRdotaliasJ}
\newsavebox{\CoWRdotaliasK}
\begin{lrbox}{\CoWRdotaliasK}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    y |-> pa1;
    *pa1 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWRdotaliasL}
\settowidth{\CoWRdotaliasL}{\usebox{\CoWRdotaliasK}}
\newsavebox{\CoWRdotaliasM}
\begin{lrbox}{\CoWRdotaliasM}
\begin{minipage}{\CoWRdotaliasH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|R0=0x1|\\
\lstinline[language=IslaLitmusExp]|R1=x|\\
\lstinline[language=IslaLitmusExp]|R3=y|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWR.alias|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWRdotaliasL}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWRdotaliasK}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWRdotaliasM}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWRdotaliasI}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoWR.inv.tex <==
\newlength{\CoWRdotinvH}
\setlength{\CoWRdotinvH}{0cm}
\newsavebox{\CoWRdotinvI}
\begin{lrbox}{\CoWRdotinvI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWRdotinvJ}
\settowidth{\CoWRdotinvJ}{\usebox{\CoWRdotinvI}}
\addtolength{\CoWRdotinvH}{\CoWRdotinvJ}
\newsavebox{\CoWRdotinvK}
\begin{lrbox}{\CoWRdotinvK}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWRdotinvL}
\settowidth{\CoWRdotinvL}{\usebox{\CoWRdotinvK}}
\newsavebox{\CoWRdotinvM}
\begin{lrbox}{\CoWRdotinvM}
\begin{minipage}{\CoWRdotinvH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWR.inv|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWRdotinvL}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWRdotinvK}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWRdotinvM}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWRdotinvI}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoWTa1.1.inv+dsb-tlbiasidis-dsb-eret.tex <==
\newlength{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetH}
\setlength{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetH}{0cm}
\newsavebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetI}
\begin{lrbox}{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI ASIDE1IS,X4
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetJ}
\settowidth{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetJ}{\usebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetI}}
\addtolength{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetH}{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetJ}
\newsavebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetK}
\begin{lrbox}{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetL}
\settowidth{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetL}{\usebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetK}}
\addtolength{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetH}{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetL}
\newsavebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetM}
\begin{lrbox}{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;

    y |-> pa1;

    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetN}
\settowidth{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetN}{\usebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetM}}
\newsavebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetO}
\begin{lrbox}{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetO}
\begin{minipage}{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL1=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=asid(0x1)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL1=0b00000|\\
\lstinline[language=IslaLitmusExp]|TTBR0_EL1=ttbr(asid=0x0001,base=page_table_base)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTa1.1.inv+dsb-tlbiasidis-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoWTa2.1.inv+dsb-tlbiasidis-dsb-eret.tex <==
\newlength{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetH}
\setlength{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetH}{0cm}
\newsavebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetI}
\begin{lrbox}{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI ASIDE1IS,X4
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetJ}
\settowidth{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetJ}{\usebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetI}}
\addtolength{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetH}{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetJ}
\newsavebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetK}
\begin{lrbox}{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetL}
\settowidth{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetL}{\usebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetK}}
\addtolength{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetH}{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetL}
\newsavebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetM}
\begin{lrbox}{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;

    y |-> pa1;

    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetN}
\settowidth{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetN}{\usebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetM}}
\newsavebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetO}
\begin{lrbox}{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetO}
\begin{minipage}{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL1=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=asid(0x2)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL1=0b00000|\\
\lstinline[language=IslaLitmusExp]|TTBR0_EL1=ttbr(asid=0x0001,base=page_table_base)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTa2.1.inv+dsb-tlbiasidis-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoWTf.inv+_dmb_-dmb-addr.tex <==
\newlength{\CoWTfdotinvplus[dmb]dmbaddrH}
\setlength{\CoWTfdotinvplus[dmb]dmbaddrH}{0cm}
\newsavebox{\CoWTfdotinvplus[dmb]dmbaddrI}
\begin{lrbox}{\CoWTfdotinvplus[dmb]dmbaddrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X2,[X1]
DSB ST
LDR X3,[X4]
EOR X5,X3,X3
LDR X6,[X7,X5]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplus[dmb]dmbaddrJ}
\settowidth{\CoWTfdotinvplus[dmb]dmbaddrJ}{\usebox{\CoWTfdotinvplus[dmb]dmbaddrI}}
\addtolength{\CoWTfdotinvplus[dmb]dmbaddrH}{\CoWTfdotinvplus[dmb]dmbaddrJ}
\newsavebox{\CoWTfdotinvplus[dmb]dmbaddrK}
\begin{lrbox}{\CoWTfdotinvplus[dmb]dmbaddrK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplus[dmb]dmbaddrL}
\settowidth{\CoWTfdotinvplus[dmb]dmbaddrL}{\usebox{\CoWTfdotinvplus[dmb]dmbaddrK}}
\addtolength{\CoWTfdotinvplus[dmb]dmbaddrH}{\CoWTfdotinvplus[dmb]dmbaddrL}
\newsavebox{\CoWTfdotinvplus[dmb]dmbaddrM}
\begin{lrbox}{\CoWTfdotinvplus[dmb]dmbaddrM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X6,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplus[dmb]dmbaddrN}
\settowidth{\CoWTfdotinvplus[dmb]dmbaddrN}{\usebox{\CoWTfdotinvplus[dmb]dmbaddrM}}
\addtolength{\CoWTfdotinvplus[dmb]dmbaddrH}{\CoWTfdotinvplus[dmb]dmbaddrN}
\newsavebox{\CoWTfdotinvplus[dmb]dmbaddrO}
\begin{lrbox}{\CoWTfdotinvplus[dmb]dmbaddrO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplus[dmb]dmbaddrP}
\settowidth{\CoWTfdotinvplus[dmb]dmbaddrP}{\usebox{\CoWTfdotinvplus[dmb]dmbaddrO}}
\newsavebox{\CoWTfdotinvplus[dmb]dmbaddrA}
\begin{lrbox}{\CoWTfdotinvplus[dmb]dmbaddrA}
\begin{minipage}{\CoWTfdotinvplus[dmb]dmbaddrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R4=y|\\
\lstinline[language=IslaLitmusExp]|0:R7=x|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+[dmb]-dmb-addr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvplus[dmb]dmbaddrP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvplus[dmb]dmbaddrO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvplus[dmb]dmbaddrA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplus[dmb]dmbaddrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplus[dmb]dmbaddrK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplus[dmb]dmbaddrM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R3=2 & 0:R6=0 & 1:R0=desc3(z,page_table_base)|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoWTf.inv+dsb-isb.tex <==
\newlength{\CoWTfdotinvplusdsbisbH}
\setlength{\CoWTfdotinvplusdsbisbH}{0cm}
\newsavebox{\CoWTfdotinvplusdsbisbI}
\begin{lrbox}{\CoWTfdotinvplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusdsbisbJ}
\settowidth{\CoWTfdotinvplusdsbisbJ}{\usebox{\CoWTfdotinvplusdsbisbI}}
\addtolength{\CoWTfdotinvplusdsbisbH}{\CoWTfdotinvplusdsbisbJ}
\newsavebox{\CoWTfdotinvplusdsbisbK}
\begin{lrbox}{\CoWTfdotinvplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusdsbisbL}
\settowidth{\CoWTfdotinvplusdsbisbL}{\usebox{\CoWTfdotinvplusdsbisbK}}
\addtolength{\CoWTfdotinvplusdsbisbH}{\CoWTfdotinvplusdsbisbL}
\newsavebox{\CoWTfdotinvplusdsbisbM}
\begin{lrbox}{\CoWTfdotinvplusdsbisbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusdsbisbN}
\settowidth{\CoWTfdotinvplusdsbisbN}{\usebox{\CoWTfdotinvplusdsbisbM}}
\newsavebox{\CoWTfdotinvplusdsbisbO}
\begin{lrbox}{\CoWTfdotinvplusdsbisbO}
\begin{minipage}{\CoWTfdotinvplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvplusdsbisbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvplusdsbisbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvplusdsbisbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplusdsbisbI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplusdsbisbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoWTf.inv+po-ctrl+po.tex <==
\newlength{\CoWTfdotinvpluspoctrlpluspoH}
\setlength{\CoWTfdotinvpluspoctrlpluspoH}{0cm}
\newsavebox{\CoWTfdotinvpluspoctrlpluspoI}
\begin{lrbox}{\CoWTfdotinvpluspoctrlpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
CBNZ X2,L0
L0:
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlpluspoJ}
\settowidth{\CoWTfdotinvpluspoctrlpluspoJ}{\usebox{\CoWTfdotinvpluspoctrlpluspoI}}
\addtolength{\CoWTfdotinvpluspoctrlpluspoH}{\CoWTfdotinvpluspoctrlpluspoJ}
\newsavebox{\CoWTfdotinvpluspoctrlpluspoK}
\begin{lrbox}{\CoWTfdotinvpluspoctrlpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlpluspoL}
\settowidth{\CoWTfdotinvpluspoctrlpluspoL}{\usebox{\CoWTfdotinvpluspoctrlpluspoK}}
\addtolength{\CoWTfdotinvpluspoctrlpluspoH}{\CoWTfdotinvpluspoctrlpluspoL}
\newsavebox{\CoWTfdotinvpluspoctrlpluspoM}
\begin{lrbox}{\CoWTfdotinvpluspoctrlpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlpluspoN}
\settowidth{\CoWTfdotinvpluspoctrlpluspoN}{\usebox{\CoWTfdotinvpluspoctrlpluspoM}}
\addtolength{\CoWTfdotinvpluspoctrlpluspoH}{\CoWTfdotinvpluspoctrlpluspoN}
\newsavebox{\CoWTfdotinvpluspoctrlpluspoO}
\begin{lrbox}{\CoWTfdotinvpluspoctrlpluspoO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlpluspoP}
\settowidth{\CoWTfdotinvpluspoctrlpluspoP}{\usebox{\CoWTfdotinvpluspoctrlpluspoO}}
\addtolength{\CoWTfdotinvpluspoctrlpluspoH}{\CoWTfdotinvpluspoctrlpluspoP}
\newsavebox{\CoWTfdotinvpluspoctrlpluspoA}
\begin{lrbox}{\CoWTfdotinvpluspoctrlpluspoA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    *pa2 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlpluspoB}
\settowidth{\CoWTfdotinvpluspoctrlpluspoB}{\usebox{\CoWTfdotinvpluspoctrlpluspoA}}
\newsavebox{\CoWTfdotinvpluspoctrlpluspoC}
\begin{lrbox}{\CoWTfdotinvpluspoctrlpluspoC}
\begin{minipage}{\CoWTfdotinvpluspoctrlpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R5=x|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+po-ctrl+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvpluspoctrlpluspoB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvpluspoctrlpluspoA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvpluspoctrlpluspoC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoctrlpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoctrlpluspoK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoctrlpluspoM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoctrlpluspoO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=1 & 0:R4=0 & 1:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoWTf.inv+po-ctrl-isb+po.tex <==
\newlength{\CoWTfdotinvpluspoctrlisbpluspoH}
\setlength{\CoWTfdotinvpluspoctrlisbpluspoH}{0cm}
\newsavebox{\CoWTfdotinvpluspoctrlisbpluspoI}
\begin{lrbox}{\CoWTfdotinvpluspoctrlisbpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
CBNZ X2,L0
L0:
ISB
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlisbpluspoJ}
\settowidth{\CoWTfdotinvpluspoctrlisbpluspoJ}{\usebox{\CoWTfdotinvpluspoctrlisbpluspoI}}
\addtolength{\CoWTfdotinvpluspoctrlisbpluspoH}{\CoWTfdotinvpluspoctrlisbpluspoJ}
\newsavebox{\CoWTfdotinvpluspoctrlisbpluspoK}
\begin{lrbox}{\CoWTfdotinvpluspoctrlisbpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlisbpluspoL}
\settowidth{\CoWTfdotinvpluspoctrlisbpluspoL}{\usebox{\CoWTfdotinvpluspoctrlisbpluspoK}}
\addtolength{\CoWTfdotinvpluspoctrlisbpluspoH}{\CoWTfdotinvpluspoctrlisbpluspoL}
\newsavebox{\CoWTfdotinvpluspoctrlisbpluspoM}
\begin{lrbox}{\CoWTfdotinvpluspoctrlisbpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlisbpluspoN}
\settowidth{\CoWTfdotinvpluspoctrlisbpluspoN}{\usebox{\CoWTfdotinvpluspoctrlisbpluspoM}}
\addtolength{\CoWTfdotinvpluspoctrlisbpluspoH}{\CoWTfdotinvpluspoctrlisbpluspoN}
\newsavebox{\CoWTfdotinvpluspoctrlisbpluspoO}
\begin{lrbox}{\CoWTfdotinvpluspoctrlisbpluspoO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlisbpluspoP}
\settowidth{\CoWTfdotinvpluspoctrlisbpluspoP}{\usebox{\CoWTfdotinvpluspoctrlisbpluspoO}}
\addtolength{\CoWTfdotinvpluspoctrlisbpluspoH}{\CoWTfdotinvpluspoctrlisbpluspoP}
\newsavebox{\CoWTfdotinvpluspoctrlisbpluspoA}
\begin{lrbox}{\CoWTfdotinvpluspoctrlisbpluspoA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    *pa2 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlisbpluspoB}
\settowidth{\CoWTfdotinvpluspoctrlisbpluspoB}{\usebox{\CoWTfdotinvpluspoctrlisbpluspoA}}
\newsavebox{\CoWTfdotinvpluspoctrlisbpluspoC}
\begin{lrbox}{\CoWTfdotinvpluspoctrlisbpluspoC}
\begin{minipage}{\CoWTfdotinvpluspoctrlisbpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R5=x|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+po-ctrl-isb+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvpluspoctrlisbpluspoB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvpluspoctrlisbpluspoA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvpluspoctrlisbpluspoC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoctrlisbpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoctrlisbpluspoK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoctrlisbpluspoM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoctrlisbpluspoO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=1 & 0:R4=0 & 1:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoWTf.inv+po.tex <==
\newlength{\CoWTfdotinvpluspoH}
\setlength{\CoWTfdotinvpluspoH}{0cm}
\newsavebox{\CoWTfdotinvpluspoI}
\begin{lrbox}{\CoWTfdotinvpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoJ}
\settowidth{\CoWTfdotinvpluspoJ}{\usebox{\CoWTfdotinvpluspoI}}
\addtolength{\CoWTfdotinvpluspoH}{\CoWTfdotinvpluspoJ}
\newsavebox{\CoWTfdotinvpluspoK}
\begin{lrbox}{\CoWTfdotinvpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoL}
\settowidth{\CoWTfdotinvpluspoL}{\usebox{\CoWTfdotinvpluspoK}}
\addtolength{\CoWTfdotinvpluspoH}{\CoWTfdotinvpluspoL}
\newsavebox{\CoWTfdotinvpluspoM}
\begin{lrbox}{\CoWTfdotinvpluspoM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoN}
\settowidth{\CoWTfdotinvpluspoN}{\usebox{\CoWTfdotinvpluspoM}}
\newsavebox{\CoWTfdotinvpluspoO}
\begin{lrbox}{\CoWTfdotinvpluspoO}
\begin{minipage}{\CoWTfdotinvpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvpluspoN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvpluspoM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvpluspoO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoWTf.inv+poloc-ctrl-isb.tex <==
\newlength{\CoWTfdotinvpluspolocctrlisbH}
\setlength{\CoWTfdotinvpluspolocctrlisbH}{0cm}
\newsavebox{\CoWTfdotinvpluspolocctrlisbI}
\begin{lrbox}{\CoWTfdotinvpluspolocctrlisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X4,[X1]
CBNZ X4,L0
L0:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspolocctrlisbJ}
\settowidth{\CoWTfdotinvpluspolocctrlisbJ}{\usebox{\CoWTfdotinvpluspolocctrlisbI}}
\addtolength{\CoWTfdotinvpluspolocctrlisbH}{\CoWTfdotinvpluspolocctrlisbJ}
\newsavebox{\CoWTfdotinvpluspolocctrlisbK}
\begin{lrbox}{\CoWTfdotinvpluspolocctrlisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspolocctrlisbL}
\settowidth{\CoWTfdotinvpluspolocctrlisbL}{\usebox{\CoWTfdotinvpluspolocctrlisbK}}
\addtolength{\CoWTfdotinvpluspolocctrlisbH}{\CoWTfdotinvpluspolocctrlisbL}
\newsavebox{\CoWTfdotinvpluspolocctrlisbM}
\begin{lrbox}{\CoWTfdotinvpluspolocctrlisbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *y = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspolocctrlisbN}
\settowidth{\CoWTfdotinvpluspolocctrlisbN}{\usebox{\CoWTfdotinvpluspolocctrlisbM}}
\newsavebox{\CoWTfdotinvpluspolocctrlisbO}
\begin{lrbox}{\CoWTfdotinvpluspolocctrlisbO}
\begin{minipage}{\CoWTfdotinvpluspolocctrlisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+poloc-ctrl-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvpluspolocctrlisbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvpluspolocctrlisbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvpluspolocctrlisbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspolocctrlisbI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspolocctrlisbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoWTf.inv+rfi-addr.tex <==
\newlength{\CoWTfdotinvplusrfiaddrH}
\setlength{\CoWTfdotinvplusrfiaddrH}{0cm}
\newsavebox{\CoWTfdotinvplusrfiaddrI}
\begin{lrbox}{\CoWTfdotinvplusrfiaddrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusrfiaddrJ}
\settowidth{\CoWTfdotinvplusrfiaddrJ}{\usebox{\CoWTfdotinvplusrfiaddrI}}
\addtolength{\CoWTfdotinvplusrfiaddrH}{\CoWTfdotinvplusrfiaddrJ}
\newsavebox{\CoWTfdotinvplusrfiaddrK}
\begin{lrbox}{\CoWTfdotinvplusrfiaddrK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#0
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusrfiaddrL}
\settowidth{\CoWTfdotinvplusrfiaddrL}{\usebox{\CoWTfdotinvplusrfiaddrK}}
\addtolength{\CoWTfdotinvplusrfiaddrH}{\CoWTfdotinvplusrfiaddrL}
\newsavebox{\CoWTfdotinvplusrfiaddrM}
\begin{lrbox}{\CoWTfdotinvplusrfiaddrM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusrfiaddrN}
\settowidth{\CoWTfdotinvplusrfiaddrN}{\usebox{\CoWTfdotinvplusrfiaddrM}}
\newsavebox{\CoWTfdotinvplusrfiaddrO}
\begin{lrbox}{\CoWTfdotinvplusrfiaddrO}
\begin{minipage}{\CoWTfdotinvplusrfiaddrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R5=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+rfi-addr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvplusrfiaddrN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvplusrfiaddrM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvplusrfiaddrO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplusrfiaddrI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplusrfiaddrK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=desc3(y,page_table_base) & 0:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoWTf.inv+rfi-ctrl-isb.tex <==
\newlength{\CoWTfdotinvplusrfictrlisbH}
\setlength{\CoWTfdotinvplusrfictrlisbH}{0cm}
\newsavebox{\CoWTfdotinvplusrfictrlisbI}
\begin{lrbox}{\CoWTfdotinvplusrfictrlisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
CBNZ X2,L0
L0:
ISB
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusrfictrlisbJ}
\settowidth{\CoWTfdotinvplusrfictrlisbJ}{\usebox{\CoWTfdotinvplusrfictrlisbI}}
\addtolength{\CoWTfdotinvplusrfictrlisbH}{\CoWTfdotinvplusrfictrlisbJ}
\newsavebox{\CoWTfdotinvplusrfictrlisbK}
\begin{lrbox}{\CoWTfdotinvplusrfictrlisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusrfictrlisbL}
\settowidth{\CoWTfdotinvplusrfictrlisbL}{\usebox{\CoWTfdotinvplusrfictrlisbK}}
\addtolength{\CoWTfdotinvplusrfictrlisbH}{\CoWTfdotinvplusrfictrlisbL}
\newsavebox{\CoWTfdotinvplusrfictrlisbM}
\begin{lrbox}{\CoWTfdotinvplusrfictrlisbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    *pa2 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusrfictrlisbN}
\settowidth{\CoWTfdotinvplusrfictrlisbN}{\usebox{\CoWTfdotinvplusrfictrlisbM}}
\newsavebox{\CoWTfdotinvplusrfictrlisbO}
\begin{lrbox}{\CoWTfdotinvplusrfictrlisbO}
\begin{minipage}{\CoWTfdotinvplusrfictrlisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R5=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+rfi-ctrl-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvplusrfictrlisbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvplusrfictrlisbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvplusrfictrlisbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplusrfictrlisbI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplusrfictrlisbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=desc3(u,page_table_base) & 0:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoWTf.inv+svc.tex <==
\newlength{\CoWTfdotinvplussvcH}
\setlength{\CoWTfdotinvplussvcH}{0cm}
\newsavebox{\CoWTfdotinvplussvcI}
\begin{lrbox}{\CoWTfdotinvplussvcI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
SVC #0x0
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplussvcJ}
\settowidth{\CoWTfdotinvplussvcJ}{\usebox{\CoWTfdotinvplussvcI}}
\addtolength{\CoWTfdotinvplussvcH}{\CoWTfdotinvplussvcJ}
\newsavebox{\CoWTfdotinvplussvcK}
\begin{lrbox}{\CoWTfdotinvplussvcK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1200:
MOV X2,#0
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplussvcL}
\settowidth{\CoWTfdotinvplussvcL}{\usebox{\CoWTfdotinvplussvcK}}
\addtolength{\CoWTfdotinvplussvcH}{\CoWTfdotinvplussvcL}
\newsavebox{\CoWTfdotinvplussvcM}
\begin{lrbox}{\CoWTfdotinvplussvcM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS X10,ELR_EL1
LDR X2,[X3]
MSR ELR_EL1,X10
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplussvcN}
\settowidth{\CoWTfdotinvplussvcN}{\usebox{\CoWTfdotinvplussvcM}}
\addtolength{\CoWTfdotinvplussvcH}{\CoWTfdotinvplussvcN}
\newsavebox{\CoWTfdotinvplussvcO}
\begin{lrbox}{\CoWTfdotinvplussvcO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *y = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplussvcP}
\settowidth{\CoWTfdotinvplussvcP}{\usebox{\CoWTfdotinvplussvcO}}
\newsavebox{\CoWTfdotinvplussvcA}
\begin{lrbox}{\CoWTfdotinvplussvcA}
\begin{minipage}{\CoWTfdotinvplussvcH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+svc|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvplussvcP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvplussvcO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvplussvcA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplussvcI}\\
  \cline{2-2}
  & thread0 el1 handler same exc\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplussvcK}\\
  \cline{2-2}
  & thread0 el1 handler lower exc\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplussvcM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoWTf.inv.EL1+dsb-eret.tex <==
\newlength{\CoWTfdotinvdotELoneplusdsberetH}
\setlength{\CoWTfdotinvdotELoneplusdsberetH}{0cm}
\newsavebox{\CoWTfdotinvdotELoneplusdsberetI}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELoneplusdsberetJ}
\settowidth{\CoWTfdotinvdotELoneplusdsberetJ}{\usebox{\CoWTfdotinvdotELoneplusdsberetI}}
\addtolength{\CoWTfdotinvdotELoneplusdsberetH}{\CoWTfdotinvdotELoneplusdsberetJ}
\newsavebox{\CoWTfdotinvdotELoneplusdsberetK}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELoneplusdsberetL}
\settowidth{\CoWTfdotinvdotELoneplusdsberetL}{\usebox{\CoWTfdotinvdotELoneplusdsberetK}}
\addtolength{\CoWTfdotinvdotELoneplusdsberetH}{\CoWTfdotinvdotELoneplusdsberetL}
\newsavebox{\CoWTfdotinvdotELoneplusdsberetM}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *y = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELoneplusdsberetN}
\settowidth{\CoWTfdotinvdotELoneplusdsberetN}{\usebox{\CoWTfdotinvdotELoneplusdsberetM}}
\newsavebox{\CoWTfdotinvdotELoneplusdsberetO}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsberetO}
\begin{minipage}{\CoWTfdotinvdotELoneplusdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL1=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL1=0b00000|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv.EL1+dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvdotELoneplusdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvdotELoneplusdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvdotELoneplusdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELoneplusdsberetI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELoneplusdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoWTf.inv.EL1+dsb-svc.tex <==
\newlength{\CoWTfdotinvdotELoneplusdsbsvcH}
\setlength{\CoWTfdotinvdotELoneplusdsbsvcH}{0cm}
\newsavebox{\CoWTfdotinvdotELoneplusdsbsvcI}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsbsvcI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
SVC #0x0
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELoneplusdsbsvcJ}
\settowidth{\CoWTfdotinvdotELoneplusdsbsvcJ}{\usebox{\CoWTfdotinvdotELoneplusdsbsvcI}}
\addtolength{\CoWTfdotinvdotELoneplusdsbsvcH}{\CoWTfdotinvdotELoneplusdsbsvcJ}
\newsavebox{\CoWTfdotinvdotELoneplusdsbsvcK}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsbsvcK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1200:
MOV X2,#0
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELoneplusdsbsvcL}
\settowidth{\CoWTfdotinvdotELoneplusdsbsvcL}{\usebox{\CoWTfdotinvdotELoneplusdsbsvcK}}
\addtolength{\CoWTfdotinvdotELoneplusdsbsvcH}{\CoWTfdotinvdotELoneplusdsbsvcL}
\newsavebox{\CoWTfdotinvdotELoneplusdsbsvcM}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsbsvcM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS X10,ELR_EL1
LDR X2,[X3]
MSR ELR_EL1,X10
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELoneplusdsbsvcN}
\settowidth{\CoWTfdotinvdotELoneplusdsbsvcN}{\usebox{\CoWTfdotinvdotELoneplusdsbsvcM}}
\addtolength{\CoWTfdotinvdotELoneplusdsbsvcH}{\CoWTfdotinvdotELoneplusdsbsvcN}
\newsavebox{\CoWTfdotinvdotELoneplusdsbsvcO}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsbsvcO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *y = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELoneplusdsbsvcP}
\settowidth{\CoWTfdotinvdotELoneplusdsbsvcP}{\usebox{\CoWTfdotinvdotELoneplusdsbsvcO}}
\newsavebox{\CoWTfdotinvdotELoneplusdsbsvcA}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsbsvcA}
\begin{minipage}{\CoWTfdotinvdotELoneplusdsbsvcH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv.EL1+dsb-svc|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvdotELoneplusdsbsvcP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvdotELoneplusdsbsvcO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvdotELoneplusdsbsvcA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELoneplusdsbsvcI}\\
  \cline{2-2}
  & thread0 el1 handler same exc\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELoneplusdsbsvcK}\\
  \cline{2-2}
  & thread0 el1 handler lower exc\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELoneplusdsbsvcM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoWTf.inv.EL1+eret.tex <==
\newlength{\CoWTfdotinvdotELonepluseretH}
\setlength{\CoWTfdotinvdotELonepluseretH}{0cm}
\newsavebox{\CoWTfdotinvdotELonepluseretI}
\begin{lrbox}{\CoWTfdotinvdotELonepluseretI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELonepluseretJ}
\settowidth{\CoWTfdotinvdotELonepluseretJ}{\usebox{\CoWTfdotinvdotELonepluseretI}}
\addtolength{\CoWTfdotinvdotELonepluseretH}{\CoWTfdotinvdotELonepluseretJ}
\newsavebox{\CoWTfdotinvdotELonepluseretK}
\begin{lrbox}{\CoWTfdotinvdotELonepluseretK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELonepluseretL}
\settowidth{\CoWTfdotinvdotELonepluseretL}{\usebox{\CoWTfdotinvdotELonepluseretK}}
\addtolength{\CoWTfdotinvdotELonepluseretH}{\CoWTfdotinvdotELonepluseretL}
\newsavebox{\CoWTfdotinvdotELonepluseretM}
\begin{lrbox}{\CoWTfdotinvdotELonepluseretM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *y = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELonepluseretN}
\settowidth{\CoWTfdotinvdotELonepluseretN}{\usebox{\CoWTfdotinvdotELonepluseretM}}
\newsavebox{\CoWTfdotinvdotELonepluseretO}
\begin{lrbox}{\CoWTfdotinvdotELonepluseretO}
\begin{minipage}{\CoWTfdotinvdotELonepluseretH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL1=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL1=0b00000|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv.EL1+eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvdotELonepluseretN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvdotELonepluseretM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvdotELonepluseretO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELonepluseretI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELonepluseretK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoWTf.inv.EL2+dsb-tlbiipa-dsb-tlbiis-dsb-eret.tex <==
\newlength{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetH}
\setlength{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetH}{0cm}
\newsavebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetI}
\begin{lrbox}{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1,X4
DSB SY
TLBI VMALLE1IS
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetJ}
\settowidth{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetJ}{\usebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetI}}
\addtolength{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetH}{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetJ}
\newsavebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetK}
\begin{lrbox}{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X20,ELR_EL2
ADD X20,X20,#4
MSR ELR_EL2,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetL}
\settowidth{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetL}{\usebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetK}}
\addtolength{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetH}{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetL}
\newsavebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetM}
\begin{lrbox}{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;

    ipa1 |-> invalid;
    ipa1 ?-> pa1;

    *pa1 = 1;

    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetN}
\settowidth{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetN}{\usebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetM}}
\newsavebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetO}
\begin{lrbox}{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetO}
\begin{minipage}{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00100|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv.EL2+dsb-tlbiipa-dsb-tlbiis-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetI}\\
  \cline{2-2}
  & thread0 el2 handler lower exc\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoWTf.inv.EL2+po.tex <==
\newlength{\CoWTfdotinvdotELtwopluspoH}
\setlength{\CoWTfdotinvdotELtwopluspoH}{0cm}
\newsavebox{\CoWTfdotinvdotELtwopluspoI}
\begin{lrbox}{\CoWTfdotinvdotELtwopluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELtwopluspoJ}
\settowidth{\CoWTfdotinvdotELtwopluspoJ}{\usebox{\CoWTfdotinvdotELtwopluspoI}}
\addtolength{\CoWTfdotinvdotELtwopluspoH}{\CoWTfdotinvdotELtwopluspoJ}
\newsavebox{\CoWTfdotinvdotELtwopluspoK}
\begin{lrbox}{\CoWTfdotinvdotELtwopluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X20,ELR_EL2
ADD X20,X20,#4
MSR ELR_EL2,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELtwopluspoL}
\settowidth{\CoWTfdotinvdotELtwopluspoL}{\usebox{\CoWTfdotinvdotELtwopluspoK}}
\addtolength{\CoWTfdotinvdotELtwopluspoH}{\CoWTfdotinvdotELtwopluspoL}
\newsavebox{\CoWTfdotinvdotELtwopluspoM}
\begin{lrbox}{\CoWTfdotinvdotELtwopluspoM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;

    ipa1 |-> invalid;
    ipa1 ?-> pa1;

    *pa1 = 1;

    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELtwopluspoN}
\settowidth{\CoWTfdotinvdotELtwopluspoN}{\usebox{\CoWTfdotinvdotELtwopluspoM}}
\newsavebox{\CoWTfdotinvdotELtwopluspoO}
\begin{lrbox}{\CoWTfdotinvdotELtwopluspoO}
\begin{minipage}{\CoWTfdotinvdotELtwopluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00100|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv.EL2+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvdotELtwopluspoN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvdotELtwopluspoM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvdotELtwopluspoO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELtwopluspoI}\\
  \cline{2-2}
  & thread0 el2 handler lower exc\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELtwopluspoK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoWTv2.2.inv+dsb-tlbivmidis-dsb-eret.tex <==
\newlength{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetH}
\setlength{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetH}{0cm}
\newsavebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetI}
\begin{lrbox}{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VMALLS12E1IS
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetJ}
\settowidth{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetJ}{\usebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetI}}
\addtolength{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetH}{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetJ}
\newsavebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetK}
\begin{lrbox}{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetL}
\settowidth{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetL}{\usebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetK}}
\addtolength{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetH}{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetL}
\newsavebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetM}
\begin{lrbox}{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;
    ipa1 |-> invalid;
    ipa1 ?-> pa1;

    *pa1 = 1;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetN}
\settowidth{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetN}{\usebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetM}}
\newsavebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetO}
\begin{lrbox}{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetO}
\begin{minipage}{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00101|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTv2.2.inv+dsb-tlbivmidis-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetI}\\
  \cline{2-2}
  & thread0 el2 handler\\
  \cline{2-2}
  & \usebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoWW.alias.tex <==
\newlength{\CoWWdotaliasH}
\setlength{\CoWWdotaliasH}{0cm}
\newsavebox{\CoWWdotaliasI}
\begin{lrbox}{\CoWWdotaliasI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWWdotaliasJ}
\settowidth{\CoWWdotaliasJ}{\usebox{\CoWWdotaliasI}}
\addtolength{\CoWWdotaliasH}{\CoWWdotaliasJ}
\newsavebox{\CoWWdotaliasK}
\begin{lrbox}{\CoWWdotaliasK}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    y |-> pa1;
    *pa1 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWWdotaliasL}
\settowidth{\CoWWdotaliasL}{\usebox{\CoWWdotaliasK}}
\newsavebox{\CoWWdotaliasM}
\begin{lrbox}{\CoWWdotaliasM}
\begin{minipage}{\CoWWdotaliasH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=0b01|\\
\lstinline[language=IslaLitmusExp]|R1=x|\\
\lstinline[language=IslaLitmusExp]|R2=0b10|\\
\lstinline[language=IslaLitmusExp]|R3=y|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWW.alias|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWWdotaliasL}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWWdotaliasK}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWWdotaliasM}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWWdotaliasI}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|x=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoWinvRpte+po.tex <==
\newlength{\CoWinvRptepluspoH}
\setlength{\CoWinvRptepluspoH}{0cm}
\newsavebox{\CoWinvRptepluspoI}
\begin{lrbox}{\CoWinvRptepluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvRptepluspoJ}
\settowidth{\CoWinvRptepluspoJ}{\usebox{\CoWinvRptepluspoI}}
\addtolength{\CoWinvRptepluspoH}{\CoWinvRptepluspoJ}
\newsavebox{\CoWinvRptepluspoK}
\begin{lrbox}{\CoWinvRptepluspoK}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;

    *pa1 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvRptepluspoL}
\settowidth{\CoWinvRptepluspoL}{\usebox{\CoWinvRptepluspoK}}
\newsavebox{\CoWinvRptepluspoM}
\begin{lrbox}{\CoWinvRptepluspoM}
\begin{minipage}{\CoWinvRptepluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=0x0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvRpte+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvRptepluspoL}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvRptepluspoK}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvRptepluspoM}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvRptepluspoI}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|~0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoWinvT+dsb-isb.tex <==
\newlength{\CoWinvTplusdsbisbH}
\setlength{\CoWinvTplusdsbisbH}{0cm}
\newsavebox{\CoWinvTplusdsbisbI}
\begin{lrbox}{\CoWinvTplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTplusdsbisbJ}
\settowidth{\CoWinvTplusdsbisbJ}{\usebox{\CoWinvTplusdsbisbI}}
\addtolength{\CoWinvTplusdsbisbH}{\CoWinvTplusdsbisbJ}
\newsavebox{\CoWinvTplusdsbisbK}
\begin{lrbox}{\CoWinvTplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTplusdsbisbL}
\settowidth{\CoWinvTplusdsbisbL}{\usebox{\CoWinvTplusdsbisbK}}
\addtolength{\CoWinvTplusdsbisbH}{\CoWinvTplusdsbisbL}
\newsavebox{\CoWinvTplusdsbisbM}
\begin{lrbox}{\CoWinvTplusdsbisbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTplusdsbisbN}
\settowidth{\CoWinvTplusdsbisbN}{\usebox{\CoWinvTplusdsbisbM}}
\newsavebox{\CoWinvTplusdsbisbO}
\begin{lrbox}{\CoWinvTplusdsbisbO}
\begin{minipage}{\CoWinvTplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvT+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTplusdsbisbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTplusdsbisbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTplusdsbisbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTplusdsbisbI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTplusdsbisbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoWinvT+po.tex <==
\newlength{\CoWinvTpluspoH}
\setlength{\CoWinvTpluspoH}{0cm}
\newsavebox{\CoWinvTpluspoI}
\begin{lrbox}{\CoWinvTpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTpluspoJ}
\settowidth{\CoWinvTpluspoJ}{\usebox{\CoWinvTpluspoI}}
\addtolength{\CoWinvTpluspoH}{\CoWinvTpluspoJ}
\newsavebox{\CoWinvTpluspoK}
\begin{lrbox}{\CoWinvTpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTpluspoL}
\settowidth{\CoWinvTpluspoL}{\usebox{\CoWinvTpluspoK}}
\addtolength{\CoWinvTpluspoH}{\CoWinvTpluspoL}
\newsavebox{\CoWinvTpluspoM}
\begin{lrbox}{\CoWinvTpluspoM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTpluspoN}
\settowidth{\CoWinvTpluspoN}{\usebox{\CoWinvTpluspoM}}
\newsavebox{\CoWinvTpluspoO}
\begin{lrbox}{\CoWinvTpluspoO}
\begin{minipage}{\CoWinvTpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvT+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTpluspoN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTpluspoM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTpluspoO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTpluspoI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTpluspoK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoWinvT.EL1+dsb-tlbi-dsb-isb.tex <==
\newlength{\CoWinvTdotELoneplusdsbtlbidsbisbH}
\setlength{\CoWinvTdotELoneplusdsbtlbidsbisbH}{0cm}
\newsavebox{\CoWinvTdotELoneplusdsbtlbidsbisbI}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbidsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1,X5
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbidsbisbJ}
\settowidth{\CoWinvTdotELoneplusdsbtlbidsbisbJ}{\usebox{\CoWinvTdotELoneplusdsbtlbidsbisbI}}
\addtolength{\CoWinvTdotELoneplusdsbtlbidsbisbH}{\CoWinvTdotELoneplusdsbtlbidsbisbJ}
\newsavebox{\CoWinvTdotELoneplusdsbtlbidsbisbK}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbidsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1000:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbidsbisbL}
\settowidth{\CoWinvTdotELoneplusdsbtlbidsbisbL}{\usebox{\CoWinvTdotELoneplusdsbtlbidsbisbK}}
\addtolength{\CoWinvTdotELoneplusdsbtlbidsbisbH}{\CoWinvTdotELoneplusdsbtlbidsbisbL}
\newsavebox{\CoWinvTdotELoneplusdsbtlbidsbisbM}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbidsbisbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbidsbisbN}
\settowidth{\CoWinvTdotELoneplusdsbtlbidsbisbN}{\usebox{\CoWinvTdotELoneplusdsbtlbidsbisbM}}
\newsavebox{\CoWinvTdotELoneplusdsbtlbidsbisbO}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbidsbisbO}
\begin{minipage}{\CoWinvTdotELoneplusdsbtlbidsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R5=page(x)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvT.EL1+dsb-tlbi-dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTdotELoneplusdsbtlbidsbisbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTdotELoneplusdsbtlbidsbisbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTdotELoneplusdsbtlbidsbisbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTdotELoneplusdsbtlbidsbisbI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTdotELoneplusdsbtlbidsbisbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoWinvT.EL1+dsb-tlbi-dsb.tex <==
\newlength{\CoWinvTdotELoneplusdsbtlbidsbH}
\setlength{\CoWinvTdotELoneplusdsbtlbidsbH}{0cm}
\newsavebox{\CoWinvTdotELoneplusdsbtlbidsbI}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbidsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1,X5
DSB SY
MOV X2,#0
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbidsbJ}
\settowidth{\CoWinvTdotELoneplusdsbtlbidsbJ}{\usebox{\CoWinvTdotELoneplusdsbtlbidsbI}}
\addtolength{\CoWinvTdotELoneplusdsbtlbidsbH}{\CoWinvTdotELoneplusdsbtlbidsbJ}
\newsavebox{\CoWinvTdotELoneplusdsbtlbidsbK}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbidsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1000:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbidsbL}
\settowidth{\CoWinvTdotELoneplusdsbtlbidsbL}{\usebox{\CoWinvTdotELoneplusdsbtlbidsbK}}
\addtolength{\CoWinvTdotELoneplusdsbtlbidsbH}{\CoWinvTdotELoneplusdsbtlbidsbL}
\newsavebox{\CoWinvTdotELoneplusdsbtlbidsbM}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbidsbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbidsbN}
\settowidth{\CoWinvTdotELoneplusdsbtlbidsbN}{\usebox{\CoWinvTdotELoneplusdsbtlbidsbM}}
\newsavebox{\CoWinvTdotELoneplusdsbtlbidsbO}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbidsbO}
\begin{minipage}{\CoWinvTdotELoneplusdsbtlbidsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R5=page(x)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvT.EL1+dsb-tlbi-dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTdotELoneplusdsbtlbidsbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTdotELoneplusdsbtlbidsbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTdotELoneplusdsbtlbidsbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTdotELoneplusdsbtlbidsbI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTdotELoneplusdsbtlbidsbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoWinvT.EL1+dsb-tlbiis-dsb-isb.tex <==
\newlength{\CoWinvTdotELoneplusdsbtlbiisdsbisbH}
\setlength{\CoWinvTdotELoneplusdsbtlbiisdsbisbH}{0cm}
\newsavebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbI}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbiisdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X5
DSB SY
ISB
MOV X2,#0
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbiisdsbisbJ}
\settowidth{\CoWinvTdotELoneplusdsbtlbiisdsbisbJ}{\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbI}}
\addtolength{\CoWinvTdotELoneplusdsbtlbiisdsbisbH}{\CoWinvTdotELoneplusdsbtlbiisdsbisbJ}
\newsavebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbK}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbiisdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1000:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbiisdsbisbL}
\settowidth{\CoWinvTdotELoneplusdsbtlbiisdsbisbL}{\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbK}}
\addtolength{\CoWinvTdotELoneplusdsbtlbiisdsbisbH}{\CoWinvTdotELoneplusdsbtlbiisdsbisbL}
\newsavebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbM}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbiisdsbisbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbiisdsbisbN}
\settowidth{\CoWinvTdotELoneplusdsbtlbiisdsbisbN}{\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbM}}
\newsavebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbO}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbiisdsbisbO}
\begin{minipage}{\CoWinvTdotELoneplusdsbtlbiisdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R5=page(x)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvT.EL1+dsb-tlbiis-dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTdotELoneplusdsbtlbiisdsbisbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoWinvT.EL1+dsb-tlbiis-dsb.tex <==
\newlength{\CoWinvTdotELoneplusdsbtlbiisdsbH}
\setlength{\CoWinvTdotELoneplusdsbtlbiisdsbH}{0cm}
\newsavebox{\CoWinvTdotELoneplusdsbtlbiisdsbI}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbiisdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X5
DSB SY
MOV X2,#0
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbiisdsbJ}
\settowidth{\CoWinvTdotELoneplusdsbtlbiisdsbJ}{\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbI}}
\addtolength{\CoWinvTdotELoneplusdsbtlbiisdsbH}{\CoWinvTdotELoneplusdsbtlbiisdsbJ}
\newsavebox{\CoWinvTdotELoneplusdsbtlbiisdsbK}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbiisdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1000:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbiisdsbL}
\settowidth{\CoWinvTdotELoneplusdsbtlbiisdsbL}{\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbK}}
\addtolength{\CoWinvTdotELoneplusdsbtlbiisdsbH}{\CoWinvTdotELoneplusdsbtlbiisdsbL}
\newsavebox{\CoWinvTdotELoneplusdsbtlbiisdsbM}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbiisdsbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbiisdsbN}
\settowidth{\CoWinvTdotELoneplusdsbtlbiisdsbN}{\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbM}}
\newsavebox{\CoWinvTdotELoneplusdsbtlbiisdsbO}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbiisdsbO}
\begin{minipage}{\CoWinvTdotELoneplusdsbtlbiisdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R5=page(x)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvT.EL1+dsb-tlbiis-dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTdotELoneplusdsbtlbiisdsbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTdotELoneplusdsbtlbiisdsbI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTdotELoneplusdsbtlbiisdsbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoWinvT2+dsb-tlbiipa-dsb-eret.tex <==
\newlength{\CoWinvTtwoplusdsbtlbiipadsberetH}
\setlength{\CoWinvTtwoplusdsbtlbiipadsberetH}{0cm}
\newsavebox{\CoWinvTtwoplusdsbtlbiipadsberetI}
\begin{lrbox}{\CoWinvTtwoplusdsbtlbiipadsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1,X4
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTtwoplusdsbtlbiipadsberetJ}
\settowidth{\CoWinvTtwoplusdsbtlbiipadsberetJ}{\usebox{\CoWinvTtwoplusdsbtlbiipadsberetI}}
\addtolength{\CoWinvTtwoplusdsbtlbiipadsberetH}{\CoWinvTtwoplusdsbtlbiipadsberetJ}
\newsavebox{\CoWinvTtwoplusdsbtlbiipadsberetK}
\begin{lrbox}{\CoWinvTtwoplusdsbtlbiipadsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X20,ELR_EL2
ADD X20,X20,#4
MSR ELR_EL2,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTtwoplusdsbtlbiipadsberetL}
\settowidth{\CoWinvTtwoplusdsbtlbiipadsberetL}{\usebox{\CoWinvTtwoplusdsbtlbiipadsberetK}}
\addtolength{\CoWinvTtwoplusdsbtlbiipadsberetH}{\CoWinvTtwoplusdsbtlbiipadsberetL}
\newsavebox{\CoWinvTtwoplusdsbtlbiipadsberetM}
\begin{lrbox}{\CoWinvTtwoplusdsbtlbiipadsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;

    ipa1 |-> invalid;
    ipa1 ?-> pa1;

    *pa1 = 1;

    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTtwoplusdsbtlbiipadsberetN}
\settowidth{\CoWinvTtwoplusdsbtlbiipadsberetN}{\usebox{\CoWinvTtwoplusdsbtlbiipadsberetM}}
\newsavebox{\CoWinvTtwoplusdsbtlbiipadsberetO}
\begin{lrbox}{\CoWinvTtwoplusdsbtlbiipadsberetO}
\begin{minipage}{\CoWinvTtwoplusdsbtlbiipadsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=page(ipa1)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00100|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvT2+dsb-tlbiipa-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTtwoplusdsbtlbiipadsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTtwoplusdsbtlbiipadsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTtwoplusdsbtlbiipadsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTtwoplusdsbtlbiipadsberetI}\\
  \cline{2-2}
  & thread0 el2 handler lower exc\\
  \cline{2-2}
  & \usebox{\CoWinvTtwoplusdsbtlbiipadsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoWinvT2+dsb-tlbiipa-dsb-tlbivmall-dsb-eret.tex <==
\newlength{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetH}
\setlength{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetH}{0cm}
\newsavebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetI}
\begin{lrbox}{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1,X4
DSB SY
TLBI VMALLE1
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetJ}
\settowidth{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetJ}{\usebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetI}}
\addtolength{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetH}{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetJ}
\newsavebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetK}
\begin{lrbox}{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#1
MRS X20,ELR_EL2
ADD X20,X20,#4
MSR ELR_EL2,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetL}
\settowidth{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetL}{\usebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetK}}
\addtolength{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetH}{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetL}
\newsavebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetM}
\begin{lrbox}{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;

    ipa1 |-> pa1;
    ipa1 ?-> invalid;

    *pa1 = 0;

    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetN}
\settowidth{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetN}{\usebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetM}}
\newsavebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetO}
\begin{lrbox}{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetO}
\begin{minipage}{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=page(ipa1)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00100|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvT2+dsb-tlbiipa-dsb-tlbivmall-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetI}\\
  \cline{2-2}
  & thread0 el2 handler lower exc\\
  \cline{2-2}
  & \usebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoWinvTa1.1+dsb-tlbiasidis-dsb-eret.tex <==
\newlength{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetH}
\setlength{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetH}{0cm}
\newsavebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetI}
\begin{lrbox}{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI ASIDE1IS,X4
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetJ}
\settowidth{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetJ}{\usebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetI}}
\addtolength{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetH}{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetJ}
\newsavebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetK}
\begin{lrbox}{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetL}
\settowidth{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetL}{\usebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetK}}
\addtolength{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetH}{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetL}
\newsavebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetM}
\begin{lrbox}{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetN}
\settowidth{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetN}{\usebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetM}}
\newsavebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetO}
\begin{lrbox}{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetO}
\begin{minipage}{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL1=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=asid(0x1)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL1=0b00000|\\
\lstinline[language=IslaLitmusExp]|TTBR0_EL1=ttbr(asid=0x0001,base=page_table_base)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvTa1.1+dsb-tlbiasidis-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoWinvTa2.1+dsb-tlbiasidis-dsb-eret.tex <==
\newlength{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetH}
\setlength{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetH}{0cm}
\newsavebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetI}
\begin{lrbox}{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI ASIDE1IS,X4
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetJ}
\settowidth{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetJ}{\usebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetI}}
\addtolength{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetH}{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetJ}
\newsavebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetK}
\begin{lrbox}{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetL}
\settowidth{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetL}{\usebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetK}}
\addtolength{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetH}{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetL}
\newsavebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetM}
\begin{lrbox}{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetN}
\settowidth{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetN}{\usebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetM}}
\newsavebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetO}
\begin{lrbox}{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetO}
\begin{minipage}{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL1=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=asid(0x2)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL1=0b00000|\\
\lstinline[language=IslaLitmusExp]|TTBR0_EL1=ttbr(base=page_table_base,asid=0x0001)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvTa2.1+dsb-tlbiasidis-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoWinvTv1.2+dsb-tlbivmidis-dsb-eret.tex <==
\newlength{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetH}
\setlength{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetH}{0cm}
\newsavebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetI}
\begin{lrbox}{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VMALLS12E1IS
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetJ}
\settowidth{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetJ}{\usebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetI}}
\addtolength{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetH}{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetJ}
\newsavebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetK}
\begin{lrbox}{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#1
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetL}
\settowidth{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetL}{\usebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetK}}
\addtolength{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetH}{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetL}
\newsavebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetM}
\begin{lrbox}{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;
    ipa1 |-> pa1;
    ipa1 ?-> invalid;

    *pa1 = 0;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetN}
\settowidth{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetN}{\usebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetM}}
\newsavebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetO}
\begin{lrbox}{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetO}
\begin{minipage}{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00101|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvTv1.2+dsb-tlbivmidis-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetI}\\
  \cline{2-2}
  & thread0 el2 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/CoWinvTv2.2+dsb-tlbivmidis-msrvttbr-dsb-eret.tex <==
\newlength{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetH}
\setlength{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetH}{0cm}
\newsavebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetI}
\begin{lrbox}{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VMALLS12E1IS
DSB SY
MSR VTTBR_EL2,X4
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetJ}
\settowidth{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetJ}{\usebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetI}}
\addtolength{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetH}{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetJ}
\newsavebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetK}
\begin{lrbox}{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#1
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetL}
\settowidth{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetL}{\usebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetK}}
\addtolength{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetH}{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetL}
\newsavebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetM}
\begin{lrbox}{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;
    ipa1 |-> pa1;
    ipa1 ?-> invalid;

    *pa1 = 0;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetN}
\settowidth{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetN}{\usebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetM}}
\newsavebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetO}
\begin{lrbox}{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetO}
\begin{minipage}{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=ttbr(base=s2_page_table_base,vmid=0x0001)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00101|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvTv2.2+dsb-tlbivmidis-msrvttbr-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetI}\\
  \cline{2-2}
  & thread0 el2 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/ETS.tex <==
\newlength{\ETSH}
\setlength{\ETSH}{0cm}
\newsavebox{\ETSI}
\begin{lrbox}{\ETSI}
\begin{lstlisting}[language=AArch64,showlines=true]
MOV X0,#1
STR X0,[X3]
DMB SY
STR X0,[X2]
\end{lstlisting}
\end{lrbox}
\newlength{\ETSJ}
\settowidth{\ETSJ}{\usebox{\ETSI}}
\addtolength{\ETSH}{\ETSJ}
\newsavebox{\ETSK}
\begin{lrbox}{\ETSK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X2]
STR X0,[X1]
MOV X4,#2
STR X4,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\ETSL}
\settowidth{\ETSL}{\usebox{\ETSK}}
\addtolength{\ETSH}{\ETSL}
\newsavebox{\ETSM}
\begin{lrbox}{\ETSM}
\begin{lstlisting}[language=AArch64,showlines=true]
MOV X0,#0
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\ETSN}
\settowidth{\ETSN}{\usebox{\ETSM}}
\addtolength{\ETSH}{\ETSN}
\newsavebox{\ETSO}
\begin{lrbox}{\ETSO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
LDR X7,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\ETSP}
\settowidth{\ETSP}{\usebox{\ETSO}}
\addtolength{\ETSH}{\ETSP}
\newsavebox{\ETSA}
\begin{lrbox}{\ETSA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> pa1;
    x ?-> invalid;
    y |-> pa2;
    z |-> pa3;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\ETSB}
\settowidth{\ETSB}{\usebox{\ETSA}}
\newsavebox{\ETSC}
\begin{lrbox}{\ETSC}
\begin{minipage}{\ETSH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R2=y|\\
\lstinline[language=IslaLitmusExp]|0:R3=z|\\
\lstinline[language=IslaLitmusExp]|1:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=z|\\
\lstinline[language=IslaLitmusExp]|1:R6=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R7=0b1|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:R1=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|ETS|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\ETSB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\ETSA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\ETSC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\ETSI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\ETSK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\ETSM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\ETSO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & x=1 & 1:R7=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/IRIW.TTf.TTf.inv+addrs.tex <==
\newlength{\IRIWdotTTfdotTTfdotinvplusaddrsH}
\setlength{\IRIWdotTTfdotTTfdotinvplusaddrsH}{0cm}
\newsavebox{\IRIWdotTTfdotTTfdotinvplusaddrsI}
\begin{lrbox}{\IRIWdotTTfdotTTfdotinvplusaddrsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\IRIWdotTTfdotTTfdotinvplusaddrsJ}
\settowidth{\IRIWdotTTfdotTTfdotinvplusaddrsJ}{\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsI}}
\addtolength{\IRIWdotTTfdotTTfdotinvplusaddrsH}{\IRIWdotTTfdotTTfdotinvplusaddrsJ}
\newsavebox{\IRIWdotTTfdotTTfdotinvplusaddrsK}
\begin{lrbox}{\IRIWdotTTfdotTTfdotinvplusaddrsK}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\IRIWdotTTfdotTTfdotinvplusaddrsL}
\settowidth{\IRIWdotTTfdotTTfdotinvplusaddrsL}{\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsK}}
\addtolength{\IRIWdotTTfdotTTfdotinvplusaddrsH}{\IRIWdotTTfdotTTfdotinvplusaddrsL}
\newsavebox{\IRIWdotTTfdotTTfdotinvplusaddrsM}
\begin{lrbox}{\IRIWdotTTfdotTTfdotinvplusaddrsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\IRIWdotTTfdotTTfdotinvplusaddrsN}
\settowidth{\IRIWdotTTfdotTTfdotinvplusaddrsN}{\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsM}}
\addtolength{\IRIWdotTTfdotTTfdotinvplusaddrsH}{\IRIWdotTTfdotTTfdotinvplusaddrsN}
\newsavebox{\IRIWdotTTfdotTTfdotinvplusaddrsO}
\begin{lrbox}{\IRIWdotTTfdotTTfdotinvplusaddrsO}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\IRIWdotTTfdotTTfdotinvplusaddrsP}
\settowidth{\IRIWdotTTfdotTTfdotinvplusaddrsP}{\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsO}}
\addtolength{\IRIWdotTTfdotTTfdotinvplusaddrsH}{\IRIWdotTTfdotTTfdotinvplusaddrsP}
\newsavebox{\IRIWdotTTfdotTTfdotinvplusaddrsA}
\begin{lrbox}{\IRIWdotTTfdotTTfdotinvplusaddrsA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\IRIWdotTTfdotTTfdotinvplusaddrsB}
\settowidth{\IRIWdotTTfdotTTfdotinvplusaddrsB}{\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsA}}
\addtolength{\IRIWdotTTfdotTTfdotinvplusaddrsH}{\IRIWdotTTfdotTTfdotinvplusaddrsB}
\newsavebox{\IRIWdotTTfdotTTfdotinvplusaddrsC}
\begin{lrbox}{\IRIWdotTTfdotTTfdotinvplusaddrsC}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\IRIWdotTTfdotTTfdotinvplusaddrsD}
\settowidth{\IRIWdotTTfdotTTfdotinvplusaddrsD}{\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsC}}
\addtolength{\IRIWdotTTfdotTTfdotinvplusaddrsH}{\IRIWdotTTfdotTTfdotinvplusaddrsD}
\newsavebox{\IRIWdotTTfdotTTfdotinvplusaddrsE}
\begin{lrbox}{\IRIWdotTTfdotTTfdotinvplusaddrsE}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> invalid;
    y ?-> pa2;
    v |-> pa2;
    *pa2 = 1;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\IRIWdotTTfdotTTfdotinvplusaddrsF}
\settowidth{\IRIWdotTTfdotTTfdotinvplusaddrsF}{\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsE}}
\newsavebox{\IRIWdotTTfdotTTfdotinvplusaddrsHG}
\begin{lrbox}{\IRIWdotTTfdotTTfdotinvplusaddrsHG}
\begin{minipage}{\IRIWdotTTfdotTTfdotinvplusaddrsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R0=desc3(v,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=x|\\
\lstinline[language=IslaLitmusExp]|2:R3=y|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|3:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|3:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|3:R1=y|\\
\lstinline[language=IslaLitmusExp]|3:R3=x|\\
\lstinline[language=IslaLitmusExp]|3:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|IRIW.TTf.TTf.inv+addrs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\IRIWdotTTfdotTTfdotinvplusaddrsF}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsE}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsHG}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\IRIWdotTTfdotTTfdotinvplusaddrsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\IRIWdotTTfdotTTfdotinvplusaddrsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\IRIWdotTTfdotTTfdotinvplusaddrsM}\\
  \cline{2-2}
  & Thread 3\\
  \cline{2-2}
  & \usebox{\IRIWdotTTfdotTTfdotinvplusaddrsO}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\IRIWdotTTfdotTTfdotinvplusaddrsA}\\
  \cline{2-2}
  & thread3 el1 handler\\
  \cline{2-2}
  & \usebox{\IRIWdotTTfdotTTfdotinvplusaddrsC}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|2:R0=1 & 2:R2=0 & 3:R0=1 & 3:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/ISA2.RRTf.inv+dsb+addr+addr.tex <==
\newlength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrH}
\setlength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrH}{0cm}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrI}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrJ}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrJ}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrI}}
\addtolength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrH}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrJ}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrK}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
STR X3,[X4,X2]
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrL}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrL}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrK}}
\addtolength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrH}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrL}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrM}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
LDR X3,[X4,X2]
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrN}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrN}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrM}}
\addtolength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrH}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrN}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrO}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X3,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrP}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrP}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrO}}
\addtolength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrH}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrP}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrA}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    *pa2 = 0;

    z |-> pa3;
    *pa3 = 0;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrB}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrB}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrA}}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrC}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrC}
\begin{minipage}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R4=z|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=z|\\
\lstinline[language=IslaLitmusExp]|2:R4=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|ISA2.RRTf.inv+dsb+addr+addr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrM}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R3=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/ISA2.RRTf.inv+dsb+data+addr.tex <==
\newlength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrH}
\setlength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrH}{0cm}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrI}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrJ}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrJ}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrI}}
\addtolength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrH}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrJ}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrK}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
ORR X3,X3,X2
STR X3,[X4]
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrL}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrL}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrK}}
\addtolength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrH}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrL}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrM}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
LDR X3,[X4,X2]
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrN}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrN}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrM}}
\addtolength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrH}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrN}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrO}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X3,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrP}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrP}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrO}}
\addtolength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrH}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrP}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrA}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    *pa2 = 0;

    z |-> pa3;
    *pa3 = 0;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrB}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrB}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrA}}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrC}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrC}
\begin{minipage}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R4=z|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=z|\\
\lstinline[language=IslaLitmusExp]|2:R4=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|ISA2.RRTf.inv+dsb+data+addr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrM}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R3=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/LB+addr-trfis.tex <==
\newlength{\LBplusaddrtrfisH}
\setlength{\LBplusaddrtrfisH}{0cm}
\newsavebox{\LBplusaddrtrfisI}
\begin{lrbox}{\LBplusaddrtrfisI}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
STR X3,[X4,X2]
STR X5,[X6]
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusaddrtrfisJ}
\settowidth{\LBplusaddrtrfisJ}{\usebox{\LBplusaddrtrfisI}}
\addtolength{\LBplusaddrtrfisH}{\LBplusaddrtrfisJ}
\newsavebox{\LBplusaddrtrfisK}
\begin{lrbox}{\LBplusaddrtrfisK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
STR X3,[X4,X2]
STR X5,[X6]
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusaddrtrfisL}
\settowidth{\LBplusaddrtrfisL}{\usebox{\LBplusaddrtrfisK}}
\addtolength{\LBplusaddrtrfisH}{\LBplusaddrtrfisL}
\newsavebox{\LBplusaddrtrfisM}
\begin{lrbox}{\LBplusaddrtrfisM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X7,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusaddrtrfisN}
\settowidth{\LBplusaddrtrfisN}{\usebox{\LBplusaddrtrfisM}}
\addtolength{\LBplusaddrtrfisH}{\LBplusaddrtrfisN}
\newsavebox{\LBplusaddrtrfisO}
\begin{lrbox}{\LBplusaddrtrfisO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X7,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusaddrtrfisP}
\settowidth{\LBplusaddrtrfisP}{\usebox{\LBplusaddrtrfisO}}
\addtolength{\LBplusaddrtrfisH}{\LBplusaddrtrfisP}
\newsavebox{\LBplusaddrtrfisA}
\begin{lrbox}{\LBplusaddrtrfisA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3 pa4;
    x |-> pa1;
    y |-> pa2;
    u |-> invalid;
    u ?-> pa2;
    v |-> invalid;
    v ?-> pa1;
    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusaddrtrfisB}
\settowidth{\LBplusaddrtrfisB}{\usebox{\LBplusaddrtrfisA}}
\newsavebox{\LBplusaddrtrfisC}
\begin{lrbox}{\LBplusaddrtrfisC}
\begin{minipage}{\LBplusaddrtrfisH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R3=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R4=pte3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R5=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R6=u|\\
\lstinline[language=IslaLitmusExp]|0:R7=0b1|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|0:__isla_monomorphize_writes=true|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=desc3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R4=pte3(v,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R5=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R6=v|\\
\lstinline[language=IslaLitmusExp]|1:R7=0b1|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\lstinline[language=IslaLitmusExp]|1:__isla_monomorphize_writes=true|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|LB+addr-trfis|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\LBplusaddrtrfisB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\LBplusaddrtrfisA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\LBplusaddrtrfisC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\LBplusaddrtrfisI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\LBplusaddrtrfisK}\\
  \cline{2-2}
  & thread1 el0 handler\\
  \cline{2-2}
  & \usebox{\LBplusaddrtrfisM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\LBplusaddrtrfisO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R0=1 & 0:R7=1 & 1:R0=1 & 1:R7=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/LB+data-trfis.tex <==
\newlength{\LBplusdatatrfisH}
\setlength{\LBplusdatatrfisH}{0cm}
\newsavebox{\LBplusdatatrfisI}
\begin{lrbox}{\LBplusdatatrfisI}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
ORR X3,X3,X2
STR X3,[X4]
STR X5,[X6]
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusdatatrfisJ}
\settowidth{\LBplusdatatrfisJ}{\usebox{\LBplusdatatrfisI}}
\addtolength{\LBplusdatatrfisH}{\LBplusdatatrfisJ}
\newsavebox{\LBplusdatatrfisK}
\begin{lrbox}{\LBplusdatatrfisK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
ORR X3,X3,X2
STR X3,[X4]
STR X5,[X6]
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusdatatrfisL}
\settowidth{\LBplusdatatrfisL}{\usebox{\LBplusdatatrfisK}}
\addtolength{\LBplusdatatrfisH}{\LBplusdatatrfisL}
\newsavebox{\LBplusdatatrfisM}
\begin{lrbox}{\LBplusdatatrfisM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X7,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusdatatrfisN}
\settowidth{\LBplusdatatrfisN}{\usebox{\LBplusdatatrfisM}}
\addtolength{\LBplusdatatrfisH}{\LBplusdatatrfisN}
\newsavebox{\LBplusdatatrfisO}
\begin{lrbox}{\LBplusdatatrfisO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X7,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusdatatrfisP}
\settowidth{\LBplusdatatrfisP}{\usebox{\LBplusdatatrfisO}}
\addtolength{\LBplusdatatrfisH}{\LBplusdatatrfisP}
\newsavebox{\LBplusdatatrfisA}
\begin{lrbox}{\LBplusdatatrfisA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3 pa4;
    x |-> pa1;
    y |-> pa2;
    u |-> invalid;
    u ?-> pa2;
    v |-> invalid;
    v ?-> pa1;
    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusdatatrfisB}
\settowidth{\LBplusdatatrfisB}{\usebox{\LBplusdatatrfisA}}
\newsavebox{\LBplusdatatrfisC}
\begin{lrbox}{\LBplusdatatrfisC}
\begin{minipage}{\LBplusdatatrfisH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R3=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R4=pte3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R5=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R6=u|\\
\lstinline[language=IslaLitmusExp]|0:R7=0b1|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=desc3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R4=pte3(v,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R5=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R6=v|\\
\lstinline[language=IslaLitmusExp]|1:R7=0b1|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|LB+data-trfis|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\LBplusdatatrfisB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\LBplusdatatrfisA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\LBplusdatatrfisC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\LBplusdatatrfisI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\LBplusdatatrfisK}\\
  \cline{2-2}
  & thread1 el0 handler\\
  \cline{2-2}
  & \usebox{\LBplusdatatrfisM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\LBplusdatatrfisO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R0=1 & 0:R7=1 & 1:R0=1 & 1:R7=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/LB.TT.inv+pos.tex <==
\newlength{\LBdotTTdotinvplusposH}
\setlength{\LBdotTTdotinvplusposH}{0cm}
\newsavebox{\LBdotTTdotinvplusposI}
\begin{lrbox}{\LBdotTTdotinvplusposI}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\LBdotTTdotinvplusposJ}
\settowidth{\LBdotTTdotinvplusposJ}{\usebox{\LBdotTTdotinvplusposI}}
\addtolength{\LBdotTTdotinvplusposH}{\LBdotTTdotinvplusposJ}
\newsavebox{\LBdotTTdotinvplusposK}
\begin{lrbox}{\LBdotTTdotinvplusposK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\LBdotTTdotinvplusposL}
\settowidth{\LBdotTTdotinvplusposL}{\usebox{\LBdotTTdotinvplusposK}}
\addtolength{\LBdotTTdotinvplusposH}{\LBdotTTdotinvplusposL}
\newsavebox{\LBdotTTdotinvplusposM}
\begin{lrbox}{\LBdotTTdotinvplusposM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\LBdotTTdotinvplusposN}
\settowidth{\LBdotTTdotinvplusposN}{\usebox{\LBdotTTdotinvplusposM}}
\addtolength{\LBdotTTdotinvplusposH}{\LBdotTTdotinvplusposN}
\newsavebox{\LBdotTTdotinvplusposO}
\begin{lrbox}{\LBdotTTdotinvplusposO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\LBdotTTdotinvplusposP}
\settowidth{\LBdotTTdotinvplusposP}{\usebox{\LBdotTTdotinvplusposO}}
\addtolength{\LBdotTTdotinvplusposH}{\LBdotTTdotinvplusposP}
\newsavebox{\LBdotTTdotinvplusposA}
\begin{lrbox}{\LBdotTTdotinvplusposA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    y |-> invalid;

    x ?-> pa1;
    y ?-> pa1;

    *pa1 = 1;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\LBdotTTdotinvplusposB}
\settowidth{\LBdotTTdotinvplusposB}{\usebox{\LBdotTTdotinvplusposA}}
\newsavebox{\LBdotTTdotinvplusposC}
\begin{lrbox}{\LBdotTTdotinvplusposC}
\begin{minipage}{\LBdotTTdotinvplusposH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|LB.TT.inv+pos|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\LBdotTTdotinvplusposB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\LBdotTTdotinvplusposA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\LBdotTTdotinvplusposC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\LBdotTTdotinvplusposI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\LBdotTTdotinvplusposK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\LBdotTTdotinvplusposM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\LBdotTTdotinvplusposO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R0=1 & 1:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.BBM1+dsb-tlbiis-dsb-dsb+ctrl-isb.tex <==
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbH}
\setlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbH}{0cm}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbI}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X6
DSB SY
STR X2,[X1]
DSB SY
STR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbJ}
\settowidth{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbJ}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbI}}
\addtolength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbH}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbJ}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbK}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBNZ X0,L0
L0:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbL}
\settowidth{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbL}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbK}}
\addtolength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbH}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbL}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbM}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbN}
\settowidth{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbN}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbM}}
\addtolength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbH}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbN}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbO}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> pa1;
    x ?-> invalid;
    x ?-> pa2;

    y |-> pa3;
    identity 0x1000 with code;

    *pa2 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbP}
\settowidth{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbP}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbO}}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbA}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbA}
\begin{minipage}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R4=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R5=y|\\
\lstinline[language=IslaLitmusExp]|0:R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.BBM1+dsb-tlbiis-dsb-dsb+ctrl-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.BBM1+dsb-tlbiis-dsb-dsb+dsb-isb.tex <==
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbH}
\setlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbI}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X6
DSB SY
STR X2,[X1]
DSB SY
STR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbJ}
\settowidth{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbJ}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbI}}
\addtolength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbH}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbJ}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbK}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbL}
\settowidth{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbL}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbK}}
\addtolength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbH}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbL}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbM}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbN}
\settowidth{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbN}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbM}}
\addtolength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbH}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbN}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbO}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> pa1;
    x ?-> invalid;
    x ?-> pa2;

    y |-> pa3;
    identity 0x1000 with code;

    *pa2 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbP}
\settowidth{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbP}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbO}}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbA}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbA}
\begin{minipage}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R4=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R5=y|\\
\lstinline[language=IslaLitmusExp]|0:R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.BBM1+dsb-tlbiis-dsb-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.RT.EL1+dsb+dsb-tlbi-dsb+dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbH}
\setlength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbJ}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbJ}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbI}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
TLBI VAE1,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbL}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbL}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbK}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbL}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbN}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbN}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbM}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbN}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbP}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbP}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbO}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbP}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbB}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbB}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbA}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbB}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbC}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> pa1;
    x ?-> invalid;

    y |-> pa2;

    a |-> pa3;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbD}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbD}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbC}}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbE}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbE}
\begin{minipage}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R3=a|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:R1=a|\\
\lstinline[language=IslaLitmusExp]|1:R2=0x2|\\
\lstinline[language=IslaLitmusExp]|1:R3=a|\\
\lstinline[language=IslaLitmusExp]|1:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|2:R1=a|\\
\lstinline[language=IslaLitmusExp]|2:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|2:R3=y|\\
\lstinline[language=IslaLitmusExp]|3:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|3:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|3:R1=y|\\
\lstinline[language=IslaLitmusExp]|3:R3=x|\\
\lstinline[language=IslaLitmusExp]|3:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL1+dsb+dsb-tlbi-dsb+dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbM}\\
  \cline{2-2}
  & Thread 3\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbO}\\
  \cline{2-2}
  & thread3 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=2 & 3:R0=1 & 3:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.RT.EL1+dsb+dsb-tlbiis-dsb+dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbH}
\setlength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbJ}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbJ}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbI}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbL}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbL}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbK}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbL}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbN}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbN}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbM}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbN}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbP}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbP}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbO}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbP}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbB}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbB}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbA}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbB}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbC}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> pa1;
    x ?-> invalid;

    y |-> pa2;

    a |-> pa3;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbD}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbD}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbC}}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbE}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbE}
\begin{minipage}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R3=a|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:R1=a|\\
\lstinline[language=IslaLitmusExp]|1:R2=0x2|\\
\lstinline[language=IslaLitmusExp]|1:R3=a|\\
\lstinline[language=IslaLitmusExp]|1:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|2:R1=a|\\
\lstinline[language=IslaLitmusExp]|2:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|2:R3=y|\\
\lstinline[language=IslaLitmusExp]|3:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|3:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|3:R1=y|\\
\lstinline[language=IslaLitmusExp]|3:R3=x|\\
\lstinline[language=IslaLitmusExp]|3:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL1+dsb+dsb-tlbiis-dsb+dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbM}\\
  \cline{2-2}
  & Thread 3\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbO}\\
  \cline{2-2}
  & thread3 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=2 & 3:R0=1 & 3:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.RT.EL1+dsb-shootdown-dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbH}
\setlength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X4,[X5]
LDR X6,[X5]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbJ}
\settowidth{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbJ}{\usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbI}}
\addtolength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbH}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X4,[X5]
SVC #0
STR X7,[X5]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbL}
\settowidth{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbL}{\usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbK}}
\addtolength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbH}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbL}
\newsavebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS X9,ESR_EL1
LSR X9,X9,#26
SUB X9,X9,#0b010101
CBNZ X9,1f
0:
DSB SY
TLBI VAE1,X6
DSB SY
ISB
ERET
1:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbN}
\settowidth{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbN}{\usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbM}}
\addtolength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbH}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbN}
\newsavebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> pa1;
    x ?-> invalid;

    y |-> pa2;
    *pa2 = 0;

    f |-> pa3;
    *pa3 = 0;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbP}
\settowidth{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbP}{\usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbO}}
\newsavebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbA}
\begin{minipage}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R5=f|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=f|\\
\lstinline[language=IslaLitmusExp]|1:R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:R7=0b10|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL1+dsb-shootdown-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R4=1 & 0:R6=2 & 1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.RT.EL1+dsb-tlbi-dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbH}
\setlength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbJ}
\settowidth{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbJ}{\usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbI}}
\addtolength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbH}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbL}
\settowidth{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbL}{\usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbK}}
\addtolength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbH}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbL}
\newsavebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbN}
\settowidth{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbN}{\usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbM}}
\addtolength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbH}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbN}
\newsavebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbP}
\settowidth{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbP}{\usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbO}}
\newsavebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbA}
\begin{minipage}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL1+dsb-tlbi-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.RT.EL1+dsb-tlbiis-dsb+dmb.tex <==
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbH}
\setlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbH}{0cm}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbI}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbJ}
\settowidth{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbJ}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbI}}
\addtolength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbJ}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbK}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbL}
\settowidth{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbL}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbK}}
\addtolength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbL}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbM}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbN}
\settowidth{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbN}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbM}}
\addtolength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbN}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbO}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbP}
\settowidth{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbP}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbO}}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbA}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbA}
\begin{minipage}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL1+dsb-tlbiis-dsb+dmb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.RT.EL1+dsb-tlbiis-dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbH}
\setlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbJ}
\settowidth{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbJ}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbI}}
\addtolength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbL}
\settowidth{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbL}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbK}}
\addtolength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbL}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbN}
\settowidth{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbN}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbM}}
\addtolength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbN}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbP}
\settowidth{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbP}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbO}}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbA}
\begin{minipage}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL1+dsb-tlbiis-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.RT.EL2+dsb-tlbiipa-dsb-tlbiis-dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbH}
\setlength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1,X4
DSB SY
TLBI VMALLE1IS
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbJ}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbJ}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbI}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbL}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbL}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbK}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbL}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#1
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbN}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbN}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbM}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbN}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
physical pa1 pa2;
intermediate ipa1 ipa2;

x |-> ipa1;
ipa1 |-> pa1;
ipa1 ?-> invalid;

y |-> ipa2;
ipa2 |-> pa2;

identity 0x2000 with code;

*pa1 = 0;
*pa2 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbP}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbP}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbO}}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbA}
\begin{minipage}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=bvlshr(ipa1,0xC)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL2+dsb-tlbiipa-dsb-tlbiis-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.RT.EL2+dsb-tlbiipais-dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbH}
\setlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbJ}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbJ}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbI}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbL}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbL}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbK}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbL}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#1
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbN}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbN}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbM}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbN}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
physical pa1 pa2;
intermediate ipa1 ipa2;

x |-> ipa1;
ipa1 |-> pa1;
ipa1 ?-> invalid;

y |-> ipa2;
ipa2 |-> pa2;

identity 0x2000 with code;

*pa1 = 1;
*pa2 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbP}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbP}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbO}}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbA}
\begin{minipage}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(ipa1)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL2+dsb-tlbiipais-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|true|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.RT.EL2+dsb-tlbiipais-dsb-tlbiis-dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbH}
\setlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1IS,X4
DSB SY
TLBI VMALLE1IS
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbJ}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbJ}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbI}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
isb
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbL}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbL}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbK}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbL}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#1
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbN}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbN}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbM}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbN}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
physical pa1 pa2;
intermediate ipa1 ipa2;

x |-> ipa1;
ipa1 |-> pa1;
ipa1 ?-> invalid;

y |-> ipa2;
ipa2 |-> pa2;

identity 0x2000 with code;

*pa1 = 0;
*pa2 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbP}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbP}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbO}}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbA}
\begin{minipage}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(ipa1)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL2+dsb-tlbiipais-dsb-tlbiis-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.RT.EL2+dsb-tlbiis-dsb-tlbiipais-dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbH}
\setlength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VMALLE1IS
DSB SY
TLBI IPAS2E1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbJ}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbJ}{\usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbI}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
isb
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbL}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbL}{\usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbK}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbL}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#1
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbN}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbN}{\usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbM}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbN}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
physical pa1 pa2;
intermediate ipa1 ipa2;

x |-> ipa1;
ipa1 |-> pa1;
ipa1 ?-> invalid;

y |-> ipa2;
ipa2 |-> pa2;

identity 0x2000 with code;

*pa1 = 0;
*pa2 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbP}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbP}{\usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbO}}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbA}
\begin{minipage}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(ipa1)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL2+dsb-tlbiis-dsb-tlbiipais-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.RT.inv+dmb+addr-po-isb.tex <==
\newlength{\MPdotRTdotinvplusdmbplusaddrpoisbH}
\setlength{\MPdotRTdotinvplusdmbplusaddrpoisbH}{0cm}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpoisbI}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpoisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpoisbJ}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpoisbJ}{\usebox{\MPdotRTdotinvplusdmbplusaddrpoisbI}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpoisbH}{\MPdotRTdotinvplusdmbplusaddrpoisbJ}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpoisbK}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpoisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
EOR X6,X2,X2
LDR X7,[X8,X6]
ISB
LDR X4,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpoisbL}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpoisbL}{\usebox{\MPdotRTdotinvplusdmbplusaddrpoisbK}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpoisbH}{\MPdotRTdotinvplusdmbplusaddrpoisbL}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpoisbM}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpoisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpoisbN}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpoisbN}{\usebox{\MPdotRTdotinvplusdmbplusaddrpoisbM}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpoisbH}{\MPdotRTdotinvplusdmbplusaddrpoisbN}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpoisbO}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpoisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X4,#0
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpoisbP}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpoisbP}{\usebox{\MPdotRTdotinvplusdmbplusaddrpoisbO}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpoisbH}{\MPdotRTdotinvplusdmbplusaddrpoisbP}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpoisbA}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpoisbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;

    x |-> invalid;
    x ?-> pa1;

    y |-> pa2;

    z |-> pa3;

    *pa1 = 1;
    *pa2 = 0;
    *pa3 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpoisbB}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpoisbB}{\usebox{\MPdotRTdotinvplusdmbplusaddrpoisbA}}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpoisbC}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpoisbC}
\begin{minipage}{\MPdotRTdotinvplusdmbplusaddrpoisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R8=z|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.inv+dmb+addr-po-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotinvplusdmbplusaddrpoisbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotinvplusdmbplusaddrpoisbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotinvplusdmbplusaddrpoisbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpoisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpoisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpoisbM}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpoisbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R2=1 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.RT.inv+dmb+addr-po-msr-isb.tex <==
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrisbH}
\setlength{\MPdotRTdotinvplusdmbplusaddrpomsrisbH}{0cm}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbI}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrisbJ}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrisbJ}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbI}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpomsrisbH}{\MPdotRTdotinvplusdmbplusaddrpomsrisbJ}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbK}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
EOR X6,X2,X2
LDR X7,[X8,X6]
MSR ELR_EL1,X5
ISB
LDR X4,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrisbL}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrisbL}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbK}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpomsrisbH}{\MPdotRTdotinvplusdmbplusaddrpomsrisbL}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbM}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrisbN}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrisbN}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbM}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpomsrisbH}{\MPdotRTdotinvplusdmbplusaddrpomsrisbN}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbO}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X4,#0
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrisbP}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrisbP}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbO}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpomsrisbH}{\MPdotRTdotinvplusdmbplusaddrpomsrisbP}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbA}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrisbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;

    x |-> invalid;
    x ?-> pa1;

    y |-> pa2;

    z |-> pa3;

    *pa1 = 1;
    *pa2 = 0;
    *pa3 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrisbB}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrisbB}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbA}}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbC}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrisbC}
\begin{minipage}{\MPdotRTdotinvplusdmbplusaddrpomsrisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:R8=z|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.inv+dmb+addr-po-msr-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotinvplusdmbplusaddrpomsrisbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbM}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R2=1 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.RT.inv+dmb+addr-po-msr.tex <==
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrH}
\setlength{\MPdotRTdotinvplusdmbplusaddrpomsrH}{0cm}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrI}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrJ}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrJ}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrI}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpomsrH}{\MPdotRTdotinvplusdmbplusaddrpomsrJ}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrK}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
EOR X6,X2,X2
LDR X7,[X8,X6]
MSR ELR_EL1,X5
LDR X4,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrL}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrL}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrK}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpomsrH}{\MPdotRTdotinvplusdmbplusaddrpomsrL}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrM}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrN}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrN}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrM}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpomsrH}{\MPdotRTdotinvplusdmbplusaddrpomsrN}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrO}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X4,#0
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrP}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrP}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrO}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpomsrH}{\MPdotRTdotinvplusdmbplusaddrpomsrP}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrA}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;

    x |-> invalid;
    x ?-> pa1;

    y |-> pa2;

    z |-> pa3;

    *pa1 = 1;
    *pa2 = 0;
    *pa3 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrB}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrB}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrA}}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrC}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrC}
\begin{minipage}{\MPdotRTdotinvplusdmbplusaddrpomsrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:R8=z|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.inv+dmb+addr-po-msr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotinvplusdmbplusaddrpomsrB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpomsrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpomsrK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpomsrM}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpomsrO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R2=1 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.RT.inv+dmb+ctrl-trfi.tex <==
\newlength{\MPdotRTdotinvplusdmbplusctrltrfiH}
\setlength{\MPdotRTdotinvplusdmbplusctrltrfiH}{0cm}
\newsavebox{\MPdotRTdotinvplusdmbplusctrltrfiI}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusctrltrfiI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusctrltrfiJ}
\settowidth{\MPdotRTdotinvplusdmbplusctrltrfiJ}{\usebox{\MPdotRTdotinvplusdmbplusctrltrfiI}}
\addtolength{\MPdotRTdotinvplusdmbplusctrltrfiH}{\MPdotRTdotinvplusdmbplusctrltrfiJ}
\newsavebox{\MPdotRTdotinvplusdmbplusctrltrfiK}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusctrltrfiK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBZ X0,LC00
LC00:
STR X2,[X3]
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusctrltrfiL}
\settowidth{\MPdotRTdotinvplusdmbplusctrltrfiL}{\usebox{\MPdotRTdotinvplusdmbplusctrltrfiK}}
\addtolength{\MPdotRTdotinvplusdmbplusctrltrfiH}{\MPdotRTdotinvplusdmbplusctrltrfiL}
\newsavebox{\MPdotRTdotinvplusdmbplusctrltrfiM}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusctrltrfiM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#2
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusctrltrfiN}
\settowidth{\MPdotRTdotinvplusdmbplusctrltrfiN}{\usebox{\MPdotRTdotinvplusdmbplusctrltrfiM}}
\addtolength{\MPdotRTdotinvplusdmbplusctrltrfiH}{\MPdotRTdotinvplusdmbplusctrltrfiN}
\newsavebox{\MPdotRTdotinvplusdmbplusctrltrfiO}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusctrltrfiO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    w |-> invalid;
    w ?-> pa1;
    x |-> pa1;
    *pa1 = 0;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusctrltrfiP}
\settowidth{\MPdotRTdotinvplusdmbplusctrltrfiP}{\usebox{\MPdotRTdotinvplusdmbplusctrltrfiO}}
\newsavebox{\MPdotRTdotinvplusdmbplusctrltrfiA}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusctrltrfiA}
\begin{minipage}{\MPdotRTdotinvplusdmbplusctrltrfiH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(w,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R5=w|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.inv+dmb+ctrl-trfi|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotinvplusdmbplusctrltrfiP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotinvplusdmbplusctrltrfiO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotinvplusdmbplusctrltrfiA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusctrltrfiI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusctrltrfiK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusctrltrfiM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.RT.inv+trfi-data+addr.toml.tex <==
\newlength{\MPdotRTdotinvplustrfidataplusaddrdottomlH}
\setlength{\MPdotRTdotinvplustrfidataplusaddrdottomlH}{0cm}
\newsavebox{\MPdotRTdotinvplustrfidataplusaddrdottomlI}
\begin{lrbox}{\MPdotRTdotinvplustrfidataplusaddrdottomlI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
STR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplustrfidataplusaddrdottomlJ}
\settowidth{\MPdotRTdotinvplustrfidataplusaddrdottomlJ}{\usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlI}}
\addtolength{\MPdotRTdotinvplustrfidataplusaddrdottomlH}{\MPdotRTdotinvplustrfidataplusaddrdottomlJ}
\newsavebox{\MPdotRTdotinvplustrfidataplusaddrdottomlK}
\begin{lrbox}{\MPdotRTdotinvplustrfidataplusaddrdottomlK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
LDR X3,[X4,X2]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplustrfidataplusaddrdottomlL}
\settowidth{\MPdotRTdotinvplustrfidataplusaddrdottomlL}{\usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlK}}
\addtolength{\MPdotRTdotinvplustrfidataplusaddrdottomlH}{\MPdotRTdotinvplustrfidataplusaddrdottomlL}
\newsavebox{\MPdotRTdotinvplustrfidataplusaddrdottomlM}
\begin{lrbox}{\MPdotRTdotinvplustrfidataplusaddrdottomlM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplustrfidataplusaddrdottomlN}
\settowidth{\MPdotRTdotinvplustrfidataplusaddrdottomlN}{\usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlM}}
\addtolength{\MPdotRTdotinvplustrfidataplusaddrdottomlH}{\MPdotRTdotinvplustrfidataplusaddrdottomlN}
\newsavebox{\MPdotRTdotinvplustrfidataplusaddrdottomlO}
\begin{lrbox}{\MPdotRTdotinvplustrfidataplusaddrdottomlO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X3,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplustrfidataplusaddrdottomlP}
\settowidth{\MPdotRTdotinvplustrfidataplusaddrdottomlP}{\usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlO}}
\addtolength{\MPdotRTdotinvplustrfidataplusaddrdottomlH}{\MPdotRTdotinvplustrfidataplusaddrdottomlP}
\newsavebox{\MPdotRTdotinvplustrfidataplusaddrdottomlA}
\begin{lrbox}{\MPdotRTdotinvplustrfidataplusaddrdottomlA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    w |-> invalid;
    w ?-> pa1;
    x |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplustrfidataplusaddrdottomlB}
\settowidth{\MPdotRTdotinvplustrfidataplusaddrdottomlB}{\usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlA}}
\newsavebox{\MPdotRTdotinvplustrfidataplusaddrdottomlC}
\begin{lrbox}{\MPdotRTdotinvplustrfidataplusaddrdottomlC}
\begin{minipage}{\MPdotRTdotinvplustrfidataplusaddrdottomlH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(w,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R3=w|\\
\lstinline[language=IslaLitmusExp]|0:R4=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R5=y|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(w,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R4=w|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.inv+trfi-data+addr.toml|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotinvplustrfidataplusaddrdottomlB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=1 & 1:R0=1 & 1:R3=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.RTT.EL1+dsb-tlbiis-tlbiis-dsb+dsb-isb.tex <==
\newlength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbH}
\setlength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
STR X2,[X3]
DSB SY
TLBI VAE1IS,X4
TLBI VAE1IS,X5
DSB SY
STR X6,[X7]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbJ}
\settowidth{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbJ}{\usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbI}}
\addtolength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbH}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbJ}
\newsavebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X4,[X3]
MOV X2,X4
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbL}
\settowidth{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbL}{\usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbK}}
\addtolength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbH}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbL}
\newsavebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbN}
\settowidth{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbN}{\usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbM}}
\addtolength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbH}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbN}
\newsavebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> pa1;
    x ?-> invalid;

    y |-> pa2;

    z |-> pa3;
    z ?-> invalid;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbP}
\settowidth{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbP}{\usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbO}}
\newsavebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbA}
\begin{minipage}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|0:R5=page(z)|\\
\lstinline[language=IslaLitmusExp]|0:R6=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R7=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=z|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTT.EL1+dsb-tlbiis-tlbiis-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.RTf.inv+dmb+addr.tex <==
\newlength{\MPdotRTfdotinvplusdmbplusaddrH}
\setlength{\MPdotRTfdotinvplusdmbplusaddrH}{0cm}
\newsavebox{\MPdotRTfdotinvplusdmbplusaddrI}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusaddrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB ST
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusaddrJ}
\settowidth{\MPdotRTfdotinvplusdmbplusaddrJ}{\usebox{\MPdotRTfdotinvplusdmbplusaddrI}}
\addtolength{\MPdotRTfdotinvplusdmbplusaddrH}{\MPdotRTfdotinvplusdmbplusaddrJ}
\newsavebox{\MPdotRTfdotinvplusdmbplusaddrK}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusaddrK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusaddrL}
\settowidth{\MPdotRTfdotinvplusdmbplusaddrL}{\usebox{\MPdotRTfdotinvplusdmbplusaddrK}}
\addtolength{\MPdotRTfdotinvplusdmbplusaddrH}{\MPdotRTfdotinvplusdmbplusaddrL}
\newsavebox{\MPdotRTfdotinvplusdmbplusaddrM}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusaddrM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusaddrN}
\settowidth{\MPdotRTfdotinvplusdmbplusaddrN}{\usebox{\MPdotRTfdotinvplusdmbplusaddrM}}
\addtolength{\MPdotRTfdotinvplusdmbplusaddrH}{\MPdotRTfdotinvplusdmbplusaddrN}
\newsavebox{\MPdotRTfdotinvplusdmbplusaddrO}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusaddrO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusaddrP}
\settowidth{\MPdotRTfdotinvplusdmbplusaddrP}{\usebox{\MPdotRTfdotinvplusdmbplusaddrO}}
\newsavebox{\MPdotRTfdotinvplusdmbplusaddrA}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusaddrA}
\begin{minipage}{\MPdotRTfdotinvplusdmbplusaddrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv+dmb+addr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvplusdmbplusaddrP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvplusdmbplusaddrO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvplusdmbplusaddrA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusaddrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusaddrK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusaddrM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.RTf.inv+dmb+ctrl-isb.tex <==
\newlength{\MPdotRTfdotinvplusdmbplusctrlisbH}
\setlength{\MPdotRTfdotinvplusdmbplusctrlisbH}{0cm}
\newsavebox{\MPdotRTfdotinvplusdmbplusctrlisbI}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusctrlisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusctrlisbJ}
\settowidth{\MPdotRTfdotinvplusdmbplusctrlisbJ}{\usebox{\MPdotRTfdotinvplusdmbplusctrlisbI}}
\addtolength{\MPdotRTfdotinvplusdmbplusctrlisbH}{\MPdotRTfdotinvplusdmbplusctrlisbJ}
\newsavebox{\MPdotRTfdotinvplusdmbplusctrlisbK}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusctrlisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBNZ X0,L0
L0:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusctrlisbL}
\settowidth{\MPdotRTfdotinvplusdmbplusctrlisbL}{\usebox{\MPdotRTfdotinvplusdmbplusctrlisbK}}
\addtolength{\MPdotRTfdotinvplusdmbplusctrlisbH}{\MPdotRTfdotinvplusdmbplusctrlisbL}
\newsavebox{\MPdotRTfdotinvplusdmbplusctrlisbM}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusctrlisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusctrlisbN}
\settowidth{\MPdotRTfdotinvplusdmbplusctrlisbN}{\usebox{\MPdotRTfdotinvplusdmbplusctrlisbM}}
\addtolength{\MPdotRTfdotinvplusdmbplusctrlisbH}{\MPdotRTfdotinvplusdmbplusctrlisbN}
\newsavebox{\MPdotRTfdotinvplusdmbplusctrlisbO}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusctrlisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusctrlisbP}
\settowidth{\MPdotRTfdotinvplusdmbplusctrlisbP}{\usebox{\MPdotRTfdotinvplusdmbplusctrlisbO}}
\newsavebox{\MPdotRTfdotinvplusdmbplusctrlisbA}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusctrlisbA}
\begin{minipage}{\MPdotRTfdotinvplusdmbplusctrlisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv+dmb+ctrl-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvplusdmbplusctrlisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvplusdmbplusctrlisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvplusdmbplusctrlisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusctrlisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusctrlisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusctrlisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.RTf.inv+dmb+data.tex <==
\newlength{\MPdotRTfdotinvplusdmbplusdataH}
\setlength{\MPdotRTfdotinvplusdmbplusdataH}{0cm}
\newsavebox{\MPdotRTfdotinvplusdmbplusdataI}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdataI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB ST
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusdataJ}
\settowidth{\MPdotRTfdotinvplusdmbplusdataJ}{\usebox{\MPdotRTfdotinvplusdmbplusdataI}}
\addtolength{\MPdotRTfdotinvplusdmbplusdataH}{\MPdotRTfdotinvplusdmbplusdataJ}
\newsavebox{\MPdotRTfdotinvplusdmbplusdataK}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdataK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
ORR X6,X4,X5
STR X6,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusdataL}
\settowidth{\MPdotRTfdotinvplusdmbplusdataL}{\usebox{\MPdotRTfdotinvplusdmbplusdataK}}
\addtolength{\MPdotRTfdotinvplusdmbplusdataH}{\MPdotRTfdotinvplusdmbplusdataL}
\newsavebox{\MPdotRTfdotinvplusdmbplusdataM}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdataM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusdataN}
\settowidth{\MPdotRTfdotinvplusdmbplusdataN}{\usebox{\MPdotRTfdotinvplusdmbplusdataM}}
\addtolength{\MPdotRTfdotinvplusdmbplusdataH}{\MPdotRTfdotinvplusdmbplusdataN}
\newsavebox{\MPdotRTfdotinvplusdmbplusdataO}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdataO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusdataP}
\settowidth{\MPdotRTfdotinvplusdmbplusdataP}{\usebox{\MPdotRTfdotinvplusdmbplusdataO}}
\newsavebox{\MPdotRTfdotinvplusdmbplusdataA}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdataA}
\begin{minipage}{\MPdotRTfdotinvplusdmbplusdataH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=0b1|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv+dmb+data|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvplusdmbplusdataP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvplusdmbplusdataO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvplusdmbplusdataA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusdataI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusdataK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusdataM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.RTf.inv+dmb+dsb-isb.tex <==
\newlength{\MPdotRTfdotinvplusdmbplusdsbisbH}
\setlength{\MPdotRTfdotinvplusdmbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTfdotinvplusdmbplusdsbisbI}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusdsbisbJ}
\settowidth{\MPdotRTfdotinvplusdmbplusdsbisbJ}{\usebox{\MPdotRTfdotinvplusdmbplusdsbisbI}}
\addtolength{\MPdotRTfdotinvplusdmbplusdsbisbH}{\MPdotRTfdotinvplusdmbplusdsbisbJ}
\newsavebox{\MPdotRTfdotinvplusdmbplusdsbisbK}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusdsbisbL}
\settowidth{\MPdotRTfdotinvplusdmbplusdsbisbL}{\usebox{\MPdotRTfdotinvplusdmbplusdsbisbK}}
\addtolength{\MPdotRTfdotinvplusdmbplusdsbisbH}{\MPdotRTfdotinvplusdmbplusdsbisbL}
\newsavebox{\MPdotRTfdotinvplusdmbplusdsbisbM}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusdsbisbN}
\settowidth{\MPdotRTfdotinvplusdmbplusdsbisbN}{\usebox{\MPdotRTfdotinvplusdmbplusdsbisbM}}
\addtolength{\MPdotRTfdotinvplusdmbplusdsbisbH}{\MPdotRTfdotinvplusdmbplusdsbisbN}
\newsavebox{\MPdotRTfdotinvplusdmbplusdsbisbO}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusdsbisbP}
\settowidth{\MPdotRTfdotinvplusdmbplusdsbisbP}{\usebox{\MPdotRTfdotinvplusdmbplusdsbisbO}}
\newsavebox{\MPdotRTfdotinvplusdmbplusdsbisbA}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdsbisbA}
\begin{minipage}{\MPdotRTfdotinvplusdmbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv+dmb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvplusdmbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvplusdmbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvplusdmbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.RTf.inv+dmb+po.tex <==
\newlength{\MPdotRTfdotinvplusdmbpluspoH}
\setlength{\MPdotRTfdotinvplusdmbpluspoH}{0cm}
\newsavebox{\MPdotRTfdotinvplusdmbpluspoI}
\begin{lrbox}{\MPdotRTfdotinvplusdmbpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB ST
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbpluspoJ}
\settowidth{\MPdotRTfdotinvplusdmbpluspoJ}{\usebox{\MPdotRTfdotinvplusdmbpluspoI}}
\addtolength{\MPdotRTfdotinvplusdmbpluspoH}{\MPdotRTfdotinvplusdmbpluspoJ}
\newsavebox{\MPdotRTfdotinvplusdmbpluspoK}
\begin{lrbox}{\MPdotRTfdotinvplusdmbpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbpluspoL}
\settowidth{\MPdotRTfdotinvplusdmbpluspoL}{\usebox{\MPdotRTfdotinvplusdmbpluspoK}}
\addtolength{\MPdotRTfdotinvplusdmbpluspoH}{\MPdotRTfdotinvplusdmbpluspoL}
\newsavebox{\MPdotRTfdotinvplusdmbpluspoM}
\begin{lrbox}{\MPdotRTfdotinvplusdmbpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbpluspoN}
\settowidth{\MPdotRTfdotinvplusdmbpluspoN}{\usebox{\MPdotRTfdotinvplusdmbpluspoM}}
\addtolength{\MPdotRTfdotinvplusdmbpluspoH}{\MPdotRTfdotinvplusdmbpluspoN}
\newsavebox{\MPdotRTfdotinvplusdmbpluspoO}
\begin{lrbox}{\MPdotRTfdotinvplusdmbpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbpluspoP}
\settowidth{\MPdotRTfdotinvplusdmbpluspoP}{\usebox{\MPdotRTfdotinvplusdmbpluspoO}}
\newsavebox{\MPdotRTfdotinvplusdmbpluspoA}
\begin{lrbox}{\MPdotRTfdotinvplusdmbpluspoA}
\begin{minipage}{\MPdotRTfdotinvplusdmbpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv+dmb+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvplusdmbpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvplusdmbpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvplusdmbpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.RTf.inv+dmbs.tex <==
\newlength{\MPdotRTfdotinvplusdmbsH}
\setlength{\MPdotRTfdotinvplusdmbsH}{0cm}
\newsavebox{\MPdotRTfdotinvplusdmbsI}
\begin{lrbox}{\MPdotRTfdotinvplusdmbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB ST
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbsJ}
\settowidth{\MPdotRTfdotinvplusdmbsJ}{\usebox{\MPdotRTfdotinvplusdmbsI}}
\addtolength{\MPdotRTfdotinvplusdmbsH}{\MPdotRTfdotinvplusdmbsJ}
\newsavebox{\MPdotRTfdotinvplusdmbsK}
\begin{lrbox}{\MPdotRTfdotinvplusdmbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbsL}
\settowidth{\MPdotRTfdotinvplusdmbsL}{\usebox{\MPdotRTfdotinvplusdmbsK}}
\addtolength{\MPdotRTfdotinvplusdmbsH}{\MPdotRTfdotinvplusdmbsL}
\newsavebox{\MPdotRTfdotinvplusdmbsM}
\begin{lrbox}{\MPdotRTfdotinvplusdmbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbsN}
\settowidth{\MPdotRTfdotinvplusdmbsN}{\usebox{\MPdotRTfdotinvplusdmbsM}}
\addtolength{\MPdotRTfdotinvplusdmbsH}{\MPdotRTfdotinvplusdmbsN}
\newsavebox{\MPdotRTfdotinvplusdmbsO}
\begin{lrbox}{\MPdotRTfdotinvplusdmbsO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbsP}
\settowidth{\MPdotRTfdotinvplusdmbsP}{\usebox{\MPdotRTfdotinvplusdmbsO}}
\newsavebox{\MPdotRTfdotinvplusdmbsA}
\begin{lrbox}{\MPdotRTfdotinvplusdmbsA}
\begin{minipage}{\MPdotRTfdotinvplusdmbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv+dmbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvplusdmbsP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvplusdmbsO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvplusdmbsA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbsK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbsM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.RTf.inv.EL1+dsb-tlbiis-dsb+addr.tex <==
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrH}
\setlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrH}{0cm}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrI}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrJ}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrJ}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrI}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrJ}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrK}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrL}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrL}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrK}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrL}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrM}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrN}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrN}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrM}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrN}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrO}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrP}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrP}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrO}}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrA}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrA}
\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv.EL1+dsb-tlbiis-dsb+addr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.RTf.inv.EL1+dsb-tlbiis-dsb+ctrl-isb.tex <==
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbH}
\setlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbH}{0cm}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbI}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbJ}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbJ}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbI}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbJ}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbK}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBNZ X0,L0
L0:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbL}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbL}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbK}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbL}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbM}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbN}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbN}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbM}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbN}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbO}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbP}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbP}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbO}}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbA}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbA}
\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv.EL1+dsb-tlbiis-dsb+ctrl-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.RTf.inv.EL1+dsb-tlbiis-dsb+ctrl.tex <==
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}
\setlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}{0cm}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlI}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlJ}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlJ}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlI}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlJ}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlK}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBNZ X0,L0
L0:
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlL}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlL}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlK}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlL}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlM}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlN}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlN}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlM}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlN}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlO}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlP}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlP}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlO}}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlA}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlA}
\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv.EL1+dsb-tlbiis-dsb+ctrl|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.RTf.inv.EL1+dsb-tlbiis-dsb+data.tex <==
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}
\setlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}{0cm}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataI}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataJ}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataJ}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataI}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataJ}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataK}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
STR X4,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataL}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataL}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataK}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataL}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataM}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataN}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataN}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataM}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataN}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataO}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataP}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataP}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataO}}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataA}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataA}
\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv.EL1+dsb-tlbiis-dsb+data|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.RTf.inv.EL1+dsb-tlbiis-dsb+dmb.tex <==
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}
\setlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{0cm}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}
\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv.EL1+dsb-tlbiis-dsb+dmb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.RTf.inv.EL1+dsb-tlbiis-dsb+dsb-isb.tex <==
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}
\setlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbJ}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbJ}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbI}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbJ}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbL}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbL}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbK}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbL}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbN}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbN}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbM}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbN}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbP}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbP}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbO}}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbA}
\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv.EL1+dsb-tlbiis-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.RTf.inv.EL1+dsb-tlbiis-dsb+po.tex <==
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}
\setlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}{0cm}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoI}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoJ}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoJ}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoI}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoJ}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoK}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoL}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoL}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoK}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoL}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoM}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoN}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoN}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoM}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoN}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoO}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoP}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoP}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoO}}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoA}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoA}
\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv.EL1+dsb-tlbiis-dsb+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.RTf.inv.EL1+dsb-tlbiis-dsb+poap.tex <==
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}
\setlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}{0cm}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapI}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapJ}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapJ}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapI}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapJ}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapK}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDAR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapL}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapL}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapK}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapL}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapM}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapN}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapN}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapM}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapN}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapO}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapP}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapP}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapO}}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapA}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapA}
\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv.EL1+dsb-tlbiis-dsb+poap|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.TR.inv+dmb+isb.tex <==
\newlength{\MPdotTRdotinvplusdmbplusisbH}
\setlength{\MPdotTRdotinvplusdmbplusisbH}{0cm}
\newsavebox{\MPdotTRdotinvplusdmbplusisbI}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusisbJ}
\settowidth{\MPdotTRdotinvplusdmbplusisbJ}{\usebox{\MPdotTRdotinvplusdmbplusisbI}}
\addtolength{\MPdotTRdotinvplusdmbplusisbH}{\MPdotTRdotinvplusdmbplusisbJ}
\newsavebox{\MPdotTRdotinvplusdmbplusisbK}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
ISB
LDR X4,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusisbL}
\settowidth{\MPdotTRdotinvplusdmbplusisbL}{\usebox{\MPdotTRdotinvplusdmbplusisbK}}
\addtolength{\MPdotTRdotinvplusdmbplusisbH}{\MPdotTRdotinvplusdmbplusisbL}
\newsavebox{\MPdotTRdotinvplusdmbplusisbM}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusisbN}
\settowidth{\MPdotTRdotinvplusdmbplusisbN}{\usebox{\MPdotTRdotinvplusdmbplusisbM}}
\addtolength{\MPdotTRdotinvplusdmbplusisbH}{\MPdotTRdotinvplusdmbplusisbN}
\newsavebox{\MPdotTRdotinvplusdmbplusisbO}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusisbP}
\settowidth{\MPdotTRdotinvplusdmbplusisbP}{\usebox{\MPdotTRdotinvplusdmbplusisbO}}
\addtolength{\MPdotTRdotinvplusdmbplusisbH}{\MPdotTRdotinvplusdmbplusisbP}
\newsavebox{\MPdotTRdotinvplusdmbplusisbA}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusisbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 0;
    *pa2 = 1;
    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusisbB}
\settowidth{\MPdotTRdotinvplusdmbplusisbB}{\usebox{\MPdotTRdotinvplusdmbplusisbA}}
\newsavebox{\MPdotTRdotinvplusdmbplusisbC}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusisbC}
\begin{minipage}{\MPdotTRdotinvplusdmbplusisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TR.inv+dmb+isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTRdotinvplusdmbplusisbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTRdotinvplusdmbplusisbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTRdotinvplusdmbplusisbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusisbM}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusisbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R2=1 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.TR.inv+dmb+msr-isb.tex <==
\newlength{\MPdotTRdotinvplusdmbplusmsrisbH}
\setlength{\MPdotTRdotinvplusdmbplusmsrisbH}{0cm}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrisbI}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrisbJ}
\settowidth{\MPdotTRdotinvplusdmbplusmsrisbJ}{\usebox{\MPdotTRdotinvplusdmbplusmsrisbI}}
\addtolength{\MPdotTRdotinvplusdmbplusmsrisbH}{\MPdotTRdotinvplusdmbplusmsrisbJ}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrisbK}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MSR ELR_EL1,X5
ISB
LDR X4,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrisbL}
\settowidth{\MPdotTRdotinvplusdmbplusmsrisbL}{\usebox{\MPdotTRdotinvplusdmbplusmsrisbK}}
\addtolength{\MPdotTRdotinvplusdmbplusmsrisbH}{\MPdotTRdotinvplusdmbplusmsrisbL}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrisbM}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrisbN}
\settowidth{\MPdotTRdotinvplusdmbplusmsrisbN}{\usebox{\MPdotTRdotinvplusdmbplusmsrisbM}}
\addtolength{\MPdotTRdotinvplusdmbplusmsrisbH}{\MPdotTRdotinvplusdmbplusmsrisbN}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrisbO}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrisbP}
\settowidth{\MPdotTRdotinvplusdmbplusmsrisbP}{\usebox{\MPdotTRdotinvplusdmbplusmsrisbO}}
\addtolength{\MPdotTRdotinvplusdmbplusmsrisbH}{\MPdotTRdotinvplusdmbplusmsrisbP}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrisbA}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrisbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 0;
    *pa2 = 1;
    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrisbB}
\settowidth{\MPdotTRdotinvplusdmbplusmsrisbB}{\usebox{\MPdotTRdotinvplusdmbplusmsrisbA}}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrisbC}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrisbC}
\begin{minipage}{\MPdotTRdotinvplusdmbplusmsrisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TR.inv+dmb+msr-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTRdotinvplusdmbplusmsrisbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTRdotinvplusdmbplusmsrisbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTRdotinvplusdmbplusmsrisbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusmsrisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusmsrisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusmsrisbM}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusmsrisbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R2=1 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.TR.inv+dmb+msr.tex <==
\newlength{\MPdotTRdotinvplusdmbplusmsrH}
\setlength{\MPdotTRdotinvplusdmbplusmsrH}{0cm}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrI}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrJ}
\settowidth{\MPdotTRdotinvplusdmbplusmsrJ}{\usebox{\MPdotTRdotinvplusdmbplusmsrI}}
\addtolength{\MPdotTRdotinvplusdmbplusmsrH}{\MPdotTRdotinvplusdmbplusmsrJ}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrK}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MSR ELR_EL1,X5
LDR X4,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrL}
\settowidth{\MPdotTRdotinvplusdmbplusmsrL}{\usebox{\MPdotTRdotinvplusdmbplusmsrK}}
\addtolength{\MPdotTRdotinvplusdmbplusmsrH}{\MPdotTRdotinvplusdmbplusmsrL}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrM}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrN}
\settowidth{\MPdotTRdotinvplusdmbplusmsrN}{\usebox{\MPdotTRdotinvplusdmbplusmsrM}}
\addtolength{\MPdotTRdotinvplusdmbplusmsrH}{\MPdotTRdotinvplusdmbplusmsrN}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrO}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrP}
\settowidth{\MPdotTRdotinvplusdmbplusmsrP}{\usebox{\MPdotTRdotinvplusdmbplusmsrO}}
\addtolength{\MPdotTRdotinvplusdmbplusmsrH}{\MPdotTRdotinvplusdmbplusmsrP}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrA}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 0;
    *pa2 = 1;
    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrB}
\settowidth{\MPdotTRdotinvplusdmbplusmsrB}{\usebox{\MPdotTRdotinvplusdmbplusmsrA}}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrC}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrC}
\begin{minipage}{\MPdotTRdotinvplusdmbplusmsrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TR.inv+dmb+msr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTRdotinvplusdmbplusmsrB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTRdotinvplusdmbplusmsrA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTRdotinvplusdmbplusmsrC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusmsrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusmsrK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusmsrM}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusmsrO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R2=1 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.TTf.inv+dmb+addr.tex <==
\newlength{\MPdotTTfdotinvplusdmbplusaddrH}
\setlength{\MPdotTTfdotinvplusdmbplusaddrH}{0cm}
\newsavebox{\MPdotTTfdotinvplusdmbplusaddrI}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusaddrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbplusaddrJ}
\settowidth{\MPdotTTfdotinvplusdmbplusaddrJ}{\usebox{\MPdotTTfdotinvplusdmbplusaddrI}}
\addtolength{\MPdotTTfdotinvplusdmbplusaddrH}{\MPdotTTfdotinvplusdmbplusaddrJ}
\newsavebox{\MPdotTTfdotinvplusdmbplusaddrK}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusaddrK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
EOR X4,X0,X0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbplusaddrL}
\settowidth{\MPdotTTfdotinvplusdmbplusaddrL}{\usebox{\MPdotTTfdotinvplusdmbplusaddrK}}
\addtolength{\MPdotTTfdotinvplusdmbplusaddrH}{\MPdotTTfdotinvplusdmbplusaddrL}
\newsavebox{\MPdotTTfdotinvplusdmbplusaddrM}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusaddrM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbplusaddrN}
\settowidth{\MPdotTTfdotinvplusdmbplusaddrN}{\usebox{\MPdotTTfdotinvplusdmbplusaddrM}}
\addtolength{\MPdotTTfdotinvplusdmbplusaddrH}{\MPdotTTfdotinvplusdmbplusaddrN}
\newsavebox{\MPdotTTfdotinvplusdmbplusaddrO}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusaddrO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbplusaddrP}
\settowidth{\MPdotTTfdotinvplusdmbplusaddrP}{\usebox{\MPdotTTfdotinvplusdmbplusaddrO}}
\newsavebox{\MPdotTTfdotinvplusdmbplusaddrA}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusaddrA}
\begin{minipage}{\MPdotTTfdotinvplusdmbplusaddrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv+dmb+addr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvplusdmbplusaddrP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvplusdmbplusaddrO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvplusdmbplusaddrA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbplusaddrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbplusaddrK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbplusaddrM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.TTf.inv+dmb+dsb-isb.tex <==
\newlength{\MPdotTTfdotinvplusdmbplusdsbisbH}
\setlength{\MPdotTTfdotinvplusdmbplusdsbisbH}{0cm}
\newsavebox{\MPdotTTfdotinvplusdmbplusdsbisbI}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbplusdsbisbJ}
\settowidth{\MPdotTTfdotinvplusdmbplusdsbisbJ}{\usebox{\MPdotTTfdotinvplusdmbplusdsbisbI}}
\addtolength{\MPdotTTfdotinvplusdmbplusdsbisbH}{\MPdotTTfdotinvplusdmbplusdsbisbJ}
\newsavebox{\MPdotTTfdotinvplusdmbplusdsbisbK}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbplusdsbisbL}
\settowidth{\MPdotTTfdotinvplusdmbplusdsbisbL}{\usebox{\MPdotTTfdotinvplusdmbplusdsbisbK}}
\addtolength{\MPdotTTfdotinvplusdmbplusdsbisbH}{\MPdotTTfdotinvplusdmbplusdsbisbL}
\newsavebox{\MPdotTTfdotinvplusdmbplusdsbisbM}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbplusdsbisbN}
\settowidth{\MPdotTTfdotinvplusdmbplusdsbisbN}{\usebox{\MPdotTTfdotinvplusdmbplusdsbisbM}}
\addtolength{\MPdotTTfdotinvplusdmbplusdsbisbH}{\MPdotTTfdotinvplusdmbplusdsbisbN}
\newsavebox{\MPdotTTfdotinvplusdmbplusdsbisbO}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbplusdsbisbP}
\settowidth{\MPdotTTfdotinvplusdmbplusdsbisbP}{\usebox{\MPdotTTfdotinvplusdmbplusdsbisbO}}
\newsavebox{\MPdotTTfdotinvplusdmbplusdsbisbA}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusdsbisbA}
\begin{minipage}{\MPdotTTfdotinvplusdmbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv+dmb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvplusdmbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvplusdmbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvplusdmbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.TTf.inv+dmb+po.tex <==
\newlength{\MPdotTTfdotinvplusdmbpluspoH}
\setlength{\MPdotTTfdotinvplusdmbpluspoH}{0cm}
\newsavebox{\MPdotTTfdotinvplusdmbpluspoI}
\begin{lrbox}{\MPdotTTfdotinvplusdmbpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbpluspoJ}
\settowidth{\MPdotTTfdotinvplusdmbpluspoJ}{\usebox{\MPdotTTfdotinvplusdmbpluspoI}}
\addtolength{\MPdotTTfdotinvplusdmbpluspoH}{\MPdotTTfdotinvplusdmbpluspoJ}
\newsavebox{\MPdotTTfdotinvplusdmbpluspoK}
\begin{lrbox}{\MPdotTTfdotinvplusdmbpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbpluspoL}
\settowidth{\MPdotTTfdotinvplusdmbpluspoL}{\usebox{\MPdotTTfdotinvplusdmbpluspoK}}
\addtolength{\MPdotTTfdotinvplusdmbpluspoH}{\MPdotTTfdotinvplusdmbpluspoL}
\newsavebox{\MPdotTTfdotinvplusdmbpluspoM}
\begin{lrbox}{\MPdotTTfdotinvplusdmbpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbpluspoN}
\settowidth{\MPdotTTfdotinvplusdmbpluspoN}{\usebox{\MPdotTTfdotinvplusdmbpluspoM}}
\addtolength{\MPdotTTfdotinvplusdmbpluspoH}{\MPdotTTfdotinvplusdmbpluspoN}
\newsavebox{\MPdotTTfdotinvplusdmbpluspoO}
\begin{lrbox}{\MPdotTTfdotinvplusdmbpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbpluspoP}
\settowidth{\MPdotTTfdotinvplusdmbpluspoP}{\usebox{\MPdotTTfdotinvplusdmbpluspoO}}
\newsavebox{\MPdotTTfdotinvplusdmbpluspoA}
\begin{lrbox}{\MPdotTTfdotinvplusdmbpluspoA}
\begin{minipage}{\MPdotTTfdotinvplusdmbpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv+dmb+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvplusdmbpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvplusdmbpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvplusdmbpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.TTf.inv+dsb+ctrl-isb.tex <==
\newlength{\MPdotTTfdotinvplusdsbplusctrlisbH}
\setlength{\MPdotTTfdotinvplusdsbplusctrlisbH}{0cm}
\newsavebox{\MPdotTTfdotinvplusdsbplusctrlisbI}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusctrlisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbplusctrlisbJ}
\settowidth{\MPdotTTfdotinvplusdsbplusctrlisbJ}{\usebox{\MPdotTTfdotinvplusdsbplusctrlisbI}}
\addtolength{\MPdotTTfdotinvplusdsbplusctrlisbH}{\MPdotTTfdotinvplusdsbplusctrlisbJ}
\newsavebox{\MPdotTTfdotinvplusdsbplusctrlisbK}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusctrlisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
CBNZ X0,L0
L0:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbplusctrlisbL}
\settowidth{\MPdotTTfdotinvplusdsbplusctrlisbL}{\usebox{\MPdotTTfdotinvplusdsbplusctrlisbK}}
\addtolength{\MPdotTTfdotinvplusdsbplusctrlisbH}{\MPdotTTfdotinvplusdsbplusctrlisbL}
\newsavebox{\MPdotTTfdotinvplusdsbplusctrlisbM}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusctrlisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbplusctrlisbN}
\settowidth{\MPdotTTfdotinvplusdsbplusctrlisbN}{\usebox{\MPdotTTfdotinvplusdsbplusctrlisbM}}
\addtolength{\MPdotTTfdotinvplusdsbplusctrlisbH}{\MPdotTTfdotinvplusdsbplusctrlisbN}
\newsavebox{\MPdotTTfdotinvplusdsbplusctrlisbO}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusctrlisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbplusctrlisbP}
\settowidth{\MPdotTTfdotinvplusdsbplusctrlisbP}{\usebox{\MPdotTTfdotinvplusdsbplusctrlisbO}}
\newsavebox{\MPdotTTfdotinvplusdsbplusctrlisbA}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusctrlisbA}
\begin{minipage}{\MPdotTTfdotinvplusdsbplusctrlisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv+dsb+ctrl-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvplusdsbplusctrlisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvplusdsbplusctrlisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvplusdsbplusctrlisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbplusctrlisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbplusctrlisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbplusctrlisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.TTf.inv+dsb+dsb-isb.tex <==
\newlength{\MPdotTTfdotinvplusdsbplusdsbisbH}
\setlength{\MPdotTTfdotinvplusdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotTTfdotinvplusdsbplusdsbisbI}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbplusdsbisbJ}
\settowidth{\MPdotTTfdotinvplusdsbplusdsbisbJ}{\usebox{\MPdotTTfdotinvplusdsbplusdsbisbI}}
\addtolength{\MPdotTTfdotinvplusdsbplusdsbisbH}{\MPdotTTfdotinvplusdsbplusdsbisbJ}
\newsavebox{\MPdotTTfdotinvplusdsbplusdsbisbK}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbplusdsbisbL}
\settowidth{\MPdotTTfdotinvplusdsbplusdsbisbL}{\usebox{\MPdotTTfdotinvplusdsbplusdsbisbK}}
\addtolength{\MPdotTTfdotinvplusdsbplusdsbisbH}{\MPdotTTfdotinvplusdsbplusdsbisbL}
\newsavebox{\MPdotTTfdotinvplusdsbplusdsbisbM}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbplusdsbisbN}
\settowidth{\MPdotTTfdotinvplusdsbplusdsbisbN}{\usebox{\MPdotTTfdotinvplusdsbplusdsbisbM}}
\addtolength{\MPdotTTfdotinvplusdsbplusdsbisbH}{\MPdotTTfdotinvplusdsbplusdsbisbN}
\newsavebox{\MPdotTTfdotinvplusdsbplusdsbisbO}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbplusdsbisbP}
\settowidth{\MPdotTTfdotinvplusdsbplusdsbisbP}{\usebox{\MPdotTTfdotinvplusdsbplusdsbisbO}}
\newsavebox{\MPdotTTfdotinvplusdsbplusdsbisbA}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusdsbisbA}
\begin{minipage}{\MPdotTTfdotinvplusdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv+dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvplusdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvplusdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvplusdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.TTf.inv+dsb+po.tex <==
\newlength{\MPdotTTfdotinvplusdsbpluspoH}
\setlength{\MPdotTTfdotinvplusdsbpluspoH}{0cm}
\newsavebox{\MPdotTTfdotinvplusdsbpluspoI}
\begin{lrbox}{\MPdotTTfdotinvplusdsbpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbpluspoJ}
\settowidth{\MPdotTTfdotinvplusdsbpluspoJ}{\usebox{\MPdotTTfdotinvplusdsbpluspoI}}
\addtolength{\MPdotTTfdotinvplusdsbpluspoH}{\MPdotTTfdotinvplusdsbpluspoJ}
\newsavebox{\MPdotTTfdotinvplusdsbpluspoK}
\begin{lrbox}{\MPdotTTfdotinvplusdsbpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbpluspoL}
\settowidth{\MPdotTTfdotinvplusdsbpluspoL}{\usebox{\MPdotTTfdotinvplusdsbpluspoK}}
\addtolength{\MPdotTTfdotinvplusdsbpluspoH}{\MPdotTTfdotinvplusdsbpluspoL}
\newsavebox{\MPdotTTfdotinvplusdsbpluspoM}
\begin{lrbox}{\MPdotTTfdotinvplusdsbpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbpluspoN}
\settowidth{\MPdotTTfdotinvplusdsbpluspoN}{\usebox{\MPdotTTfdotinvplusdsbpluspoM}}
\addtolength{\MPdotTTfdotinvplusdsbpluspoH}{\MPdotTTfdotinvplusdsbpluspoN}
\newsavebox{\MPdotTTfdotinvplusdsbpluspoO}
\begin{lrbox}{\MPdotTTfdotinvplusdsbpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbpluspoP}
\settowidth{\MPdotTTfdotinvplusdsbpluspoP}{\usebox{\MPdotTTfdotinvplusdsbpluspoO}}
\newsavebox{\MPdotTTfdotinvplusdsbpluspoA}
\begin{lrbox}{\MPdotTTfdotinvplusdsbpluspoA}
\begin{minipage}{\MPdotTTfdotinvplusdsbpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv+dsb+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvplusdsbpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvplusdsbpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvplusdsbpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.TTf.inv+dsbs.tex <==
\newlength{\MPdotTTfdotinvplusdsbsH}
\setlength{\MPdotTTfdotinvplusdsbsH}{0cm}
\newsavebox{\MPdotTTfdotinvplusdsbsI}
\begin{lrbox}{\MPdotTTfdotinvplusdsbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbsJ}
\settowidth{\MPdotTTfdotinvplusdsbsJ}{\usebox{\MPdotTTfdotinvplusdsbsI}}
\addtolength{\MPdotTTfdotinvplusdsbsH}{\MPdotTTfdotinvplusdsbsJ}
\newsavebox{\MPdotTTfdotinvplusdsbsK}
\begin{lrbox}{\MPdotTTfdotinvplusdsbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbsL}
\settowidth{\MPdotTTfdotinvplusdsbsL}{\usebox{\MPdotTTfdotinvplusdsbsK}}
\addtolength{\MPdotTTfdotinvplusdsbsH}{\MPdotTTfdotinvplusdsbsL}
\newsavebox{\MPdotTTfdotinvplusdsbsM}
\begin{lrbox}{\MPdotTTfdotinvplusdsbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbsN}
\settowidth{\MPdotTTfdotinvplusdsbsN}{\usebox{\MPdotTTfdotinvplusdsbsM}}
\addtolength{\MPdotTTfdotinvplusdsbsH}{\MPdotTTfdotinvplusdsbsN}
\newsavebox{\MPdotTTfdotinvplusdsbsO}
\begin{lrbox}{\MPdotTTfdotinvplusdsbsO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbsP}
\settowidth{\MPdotTTfdotinvplusdsbsP}{\usebox{\MPdotTTfdotinvplusdsbsO}}
\newsavebox{\MPdotTTfdotinvplusdsbsA}
\begin{lrbox}{\MPdotTTfdotinvplusdsbsA}
\begin{minipage}{\MPdotTTfdotinvplusdsbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv+dsbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvplusdsbsP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvplusdsbsO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvplusdsbsA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbsK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbsM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.TTf.inv.EL1+dsb-tlbiis-dsb+dmb.tex <==
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}
\setlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{0cm}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}
\begin{minipage}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv.EL1+dsb-tlbiis-dsb+dmb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.TTf.inv.EL1+dsb-tlbiis-dsb+dsb-isb.tex <==
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}
\setlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbI}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbJ}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbJ}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbI}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbJ}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbK}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbL}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbL}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbK}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbL}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbM}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbN}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbN}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbM}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbN}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbO}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbP}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbP}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbO}}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbA}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbA}
\begin{minipage}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv.EL1+dsb-tlbiis-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.TTf.inv.EL1+dsb-tlbiis-dsb+po.tex <==
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}
\setlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}{0cm}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoI}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoJ}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoJ}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoI}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoJ}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoK}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoL}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoL}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoK}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoL}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoM}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoN}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoN}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoM}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoN}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoO}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoP}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoP}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoO}}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoA}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoA}
\begin{minipage}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv.EL1+dsb-tlbiis-dsb+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.TfR+dmb+eret.tex <==
\newlength{\MPdotTfRplusdmbpluseretH}
\setlength{\MPdotTfRplusdmbpluseretH}{0cm}
\newsavebox{\MPdotTfRplusdmbpluseretI}
\begin{lrbox}{\MPdotTfRplusdmbpluseretI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTfRplusdmbpluseretJ}
\settowidth{\MPdotTfRplusdmbpluseretJ}{\usebox{\MPdotTfRplusdmbpluseretI}}
\addtolength{\MPdotTfRplusdmbpluseretH}{\MPdotTfRplusdmbpluseretJ}
\newsavebox{\MPdotTfRplusdmbpluseretK}
\begin{lrbox}{\MPdotTfRplusdmbpluseretK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
LDR X4,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTfRplusdmbpluseretL}
\settowidth{\MPdotTfRplusdmbpluseretL}{\usebox{\MPdotTfRplusdmbpluseretK}}
\addtolength{\MPdotTfRplusdmbpluseretH}{\MPdotTfRplusdmbpluseretL}
\newsavebox{\MPdotTfRplusdmbpluseretM}
\begin{lrbox}{\MPdotTfRplusdmbpluseretM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTfRplusdmbpluseretN}
\settowidth{\MPdotTfRplusdmbpluseretN}{\usebox{\MPdotTfRplusdmbpluseretM}}
\addtolength{\MPdotTfRplusdmbpluseretH}{\MPdotTfRplusdmbpluseretN}
\newsavebox{\MPdotTfRplusdmbpluseretO}
\begin{lrbox}{\MPdotTfRplusdmbpluseretO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;

    y |-> pa2;
    y ?-> invalid;

    *pa1 = 0;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTfRplusdmbpluseretP}
\settowidth{\MPdotTfRplusdmbpluseretP}{\usebox{\MPdotTfRplusdmbpluseretO}}
\newsavebox{\MPdotTfRplusdmbpluseretA}
\begin{lrbox}{\MPdotTfRplusdmbpluseretA}
\begin{minipage}{\MPdotTfRplusdmbpluseretH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TfR+dmb+eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTfRplusdmbpluseretP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTfRplusdmbpluseretO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTfRplusdmbpluseretA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTfRplusdmbpluseretI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTfRplusdmbpluseretK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTfRplusdmbpluseretM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R2=0 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/MP.alias3+rfi-data+dmb.tex <==
\newlength{\MPdotaliasthreeplusrfidataplusdmbH}
\setlength{\MPdotaliasthreeplusrfidataplusdmbH}{0cm}
\newsavebox{\MPdotaliasthreeplusrfidataplusdmbI}
\begin{lrbox}{\MPdotaliasthreeplusrfidataplusdmbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
STR X2,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotaliasthreeplusrfidataplusdmbJ}
\settowidth{\MPdotaliasthreeplusrfidataplusdmbJ}{\usebox{\MPdotaliasthreeplusrfidataplusdmbI}}
\addtolength{\MPdotaliasthreeplusrfidataplusdmbH}{\MPdotaliasthreeplusrfidataplusdmbJ}
\newsavebox{\MPdotaliasthreeplusrfidataplusdmbK}
\begin{lrbox}{\MPdotaliasthreeplusrfidataplusdmbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotaliasthreeplusrfidataplusdmbL}
\settowidth{\MPdotaliasthreeplusrfidataplusdmbL}{\usebox{\MPdotaliasthreeplusrfidataplusdmbK}}
\addtolength{\MPdotaliasthreeplusrfidataplusdmbH}{\MPdotaliasthreeplusrfidataplusdmbL}
\newsavebox{\MPdotaliasthreeplusrfidataplusdmbM}
\begin{lrbox}{\MPdotaliasthreeplusrfidataplusdmbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    y |-> pa2;
    z |-> pa1;
    *pa1 = 0;
    *pa2 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotaliasthreeplusrfidataplusdmbN}
\settowidth{\MPdotaliasthreeplusrfidataplusdmbN}{\usebox{\MPdotaliasthreeplusrfidataplusdmbM}}
\newsavebox{\MPdotaliasthreeplusrfidataplusdmbO}
\begin{lrbox}{\MPdotaliasthreeplusrfidataplusdmbO}
\begin{minipage}{\MPdotaliasthreeplusrfidataplusdmbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R3=z|\\
\lstinline[language=IslaLitmusExp]|0:R5=y|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.alias3+rfi-data+dmb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotaliasthreeplusrfidataplusdmbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotaliasthreeplusrfidataplusdmbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotaliasthreeplusrfidataplusdmbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotaliasthreeplusrfidataplusdmbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotaliasthreeplusrfidataplusdmbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/PPOAA.alias.tex <==
\newlength{\PPOAAdotaliasH}
\setlength{\PPOAAdotaliasH}{0cm}
\newsavebox{\PPOAAdotaliasI}
\begin{lrbox}{\PPOAAdotaliasI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\PPOAAdotaliasJ}
\settowidth{\PPOAAdotaliasJ}{\usebox{\PPOAAdotaliasI}}
\addtolength{\PPOAAdotaliasH}{\PPOAAdotaliasJ}
\newsavebox{\PPOAAdotaliasK}
\begin{lrbox}{\PPOAAdotaliasK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X9,X0,X0
STR X2,[X3,X9]
LDR X4,[X5]
EOR X8,X4,X4
LDR X6,[X7,X8]
\end{lstlisting}
\end{lrbox}
\newlength{\PPOAAdotaliasL}
\settowidth{\PPOAAdotaliasL}{\usebox{\PPOAAdotaliasK}}
\addtolength{\PPOAAdotaliasH}{\PPOAAdotaliasL}
\newsavebox{\PPOAAdotaliasM}
\begin{lrbox}{\PPOAAdotaliasM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    w |-> pa1;
    x |-> pa1;
    y |-> pa2;
    z |-> pa3;
\end{lstlisting}
\end{lrbox}
\newlength{\PPOAAdotaliasN}
\settowidth{\PPOAAdotaliasN}{\usebox{\PPOAAdotaliasM}}
\newsavebox{\PPOAAdotaliasO}
\begin{lrbox}{\PPOAAdotaliasO}
\begin{minipage}{\PPOAAdotaliasH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R1=z|\\
\lstinline[language=IslaLitmusExp]|0:R2=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0x1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=w|\\
\lstinline[language=IslaLitmusExp]|1:R7=z|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|PPOAA.alias|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\PPOAAdotaliasN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\PPOAAdotaliasM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\PPOAAdotaliasO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\PPOAAdotaliasI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\PPOAAdotaliasK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R4=1 & 1:R6=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/PPOCA.alias.tex <==
\newlength{\PPOCAdotaliasH}
\setlength{\PPOCAdotaliasH}{0cm}
\newsavebox{\PPOCAdotaliasI}
\begin{lrbox}{\PPOCAdotaliasI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\PPOCAdotaliasJ}
\settowidth{\PPOCAdotaliasJ}{\usebox{\PPOCAdotaliasI}}
\addtolength{\PPOCAdotaliasH}{\PPOCAdotaliasJ}
\newsavebox{\PPOCAdotaliasK}
\begin{lrbox}{\PPOCAdotaliasK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBNZ X0,L0
L0:
STR X2,[X3]
LDR X4,[X5]
EOR X8,X4,X4
LDR X6,[X7,X8]
\end{lstlisting}
\end{lrbox}
\newlength{\PPOCAdotaliasL}
\settowidth{\PPOCAdotaliasL}{\usebox{\PPOCAdotaliasK}}
\addtolength{\PPOCAdotaliasH}{\PPOCAdotaliasL}
\newsavebox{\PPOCAdotaliasM}
\begin{lrbox}{\PPOCAdotaliasM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    w |-> pa1;
    x |-> pa1;
    y |-> pa2;
    z |-> pa3;
    *pa1 = 0;
    *pa2 = 0;
    *pa3 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\PPOCAdotaliasN}
\settowidth{\PPOCAdotaliasN}{\usebox{\PPOCAdotaliasM}}
\newsavebox{\PPOCAdotaliasO}
\begin{lrbox}{\PPOCAdotaliasO}
\begin{minipage}{\PPOCAdotaliasH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R1=z|\\
\lstinline[language=IslaLitmusExp]|0:R2=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0x1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=w|\\
\lstinline[language=IslaLitmusExp]|1:R7=z|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|PPOCA.alias|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\PPOCAdotaliasN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\PPOCAdotaliasM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\PPOCAdotaliasO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\PPOCAdotaliasI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\PPOCAdotaliasK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R4=1 & 1:R6=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/PPODA.RT.inv.tex <==
\newlength{\PPODAdotRTdotinvH}
\setlength{\PPODAdotRTdotinvH}{0cm}
\newsavebox{\PPODAdotRTdotinvI}
\begin{lrbox}{\PPODAdotRTdotinvI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\PPODAdotRTdotinvJ}
\settowidth{\PPODAdotRTdotinvJ}{\usebox{\PPODAdotRTdotinvI}}
\addtolength{\PPODAdotRTdotinvH}{\PPODAdotRTdotinvJ}
\newsavebox{\PPODAdotRTdotinvK}
\begin{lrbox}{\PPODAdotRTdotinvK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
ORR X2,X2,X3
STR X2,[X4]
LDR X6,[X5]
EOR X8,X6,X6
LDR X9,[X7,X8]
\end{lstlisting}
\end{lrbox}
\newlength{\PPODAdotRTdotinvL}
\settowidth{\PPODAdotRTdotinvL}{\usebox{\PPODAdotRTdotinvK}}
\addtolength{\PPODAdotRTdotinvH}{\PPODAdotRTdotinvL}
\newsavebox{\PPODAdotRTdotinvM}
\begin{lrbox}{\PPODAdotRTdotinvM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X6,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\PPODAdotRTdotinvN}
\settowidth{\PPODAdotRTdotinvN}{\usebox{\PPODAdotRTdotinvM}}
\addtolength{\PPODAdotRTdotinvH}{\PPODAdotRTdotinvN}
\newsavebox{\PPODAdotRTdotinvO}
\begin{lrbox}{\PPODAdotRTdotinvO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    w |-> pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa2;
    z |-> pa3;
    *pa1 = 1;
    *pa2 = 0;
    *pa3 = 0;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\PPODAdotRTdotinvP}
\settowidth{\PPODAdotRTdotinvP}{\usebox{\PPODAdotRTdotinvO}}
\newsavebox{\PPODAdotRTdotinvA}
\begin{lrbox}{\PPODAdotRTdotinvA}
\begin{minipage}{\PPODAdotRTdotinvH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R1=z|\\
\lstinline[language=IslaLitmusExp]|0:R2=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=desc3(w,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R4=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R5=x|\\
\lstinline[language=IslaLitmusExp]|1:R7=z|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|PPODA.RT.inv|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\PPODAdotRTdotinvP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\PPODAdotRTdotinvO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\PPODAdotRTdotinvA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\PPODAdotRTdotinvI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\PPODAdotRTdotinvK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\PPODAdotRTdotinvM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R6=1 & 1:R9=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/R.RTf.inv.EL1+dsb-tlbiis-dsb+popl.tex <==
\newlength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}
\setlength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}{0cm}
\newsavebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplI}
\begin{lrbox}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplJ}
\settowidth{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplJ}{\usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplI}}
\addtolength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplJ}
\newsavebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplK}
\begin{lrbox}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplK}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
STLR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplL}
\settowidth{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplL}{\usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplK}}
\addtolength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplL}
\newsavebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplM}
\begin{lrbox}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplN}
\settowidth{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplN}{\usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplM}}
\addtolength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplN}
\newsavebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplO}
\begin{lrbox}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplP}
\settowidth{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplP}{\usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplO}}
\newsavebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplA}
\begin{lrbox}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplA}
\begin{minipage}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R0=0x2|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|R.RTf.inv.EL1+dsb-tlbiis-dsb+popl|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|y=2 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/R.inv.tex <==
\newlength{\RdotinvH}
\setlength{\RdotinvH}{0cm}
\newsavebox{\RdotinvI}
\begin{lrbox}{\RdotinvI}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\RdotinvJ}
\settowidth{\RdotinvJ}{\usebox{\RdotinvI}}
\addtolength{\RdotinvH}{\RdotinvJ}
\newsavebox{\RdotinvK}
\begin{lrbox}{\RdotinvK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\RdotinvL}
\settowidth{\RdotinvL}{\usebox{\RdotinvK}}
\addtolength{\RdotinvH}{\RdotinvL}
\newsavebox{\RdotinvM}
\begin{lrbox}{\RdotinvM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    identity 0x1000 with code;
    *pa1 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\RdotinvN}
\settowidth{\RdotinvN}{\usebox{\RdotinvM}}
\newsavebox{\RdotinvO}
\begin{lrbox}{\RdotinvO}
\begin{minipage}{\RdotinvH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|R.inv|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\RdotinvN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\RdotinvM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\RdotinvO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\RdotinvI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\RdotinvK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R0=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/RBS+dsb-tlbiis-dsb.tex <==
\newlength{\RBSplusdsbtlbiisdsbH}
\setlength{\RBSplusdsbtlbiisdsbH}{0cm}
\newsavebox{\RBSplusdsbtlbiisdsbI}
\begin{lrbox}{\RBSplusdsbtlbiisdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X5
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\RBSplusdsbtlbiisdsbJ}
\settowidth{\RBSplusdsbtlbiisdsbJ}{\usebox{\RBSplusdsbtlbiisdsbI}}
\addtolength{\RBSplusdsbtlbiisdsbH}{\RBSplusdsbtlbiisdsbJ}
\newsavebox{\RBSplusdsbtlbiisdsbK}
\begin{lrbox}{\RBSplusdsbtlbiisdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\RBSplusdsbtlbiisdsbL}
\settowidth{\RBSplusdsbtlbiisdsbL}{\usebox{\RBSplusdsbtlbiisdsbK}}
\addtolength{\RBSplusdsbtlbiisdsbH}{\RBSplusdsbtlbiisdsbL}
\newsavebox{\RBSplusdsbtlbiisdsbM}
\begin{lrbox}{\RBSplusdsbtlbiisdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\RBSplusdsbtlbiisdsbN}
\settowidth{\RBSplusdsbtlbiisdsbN}{\usebox{\RBSplusdsbtlbiisdsbM}}
\addtolength{\RBSplusdsbtlbiisdsbH}{\RBSplusdsbtlbiisdsbN}
\newsavebox{\RBSplusdsbtlbiisdsbO}
\begin{lrbox}{\RBSplusdsbtlbiisdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;
    y |-> pa1;
    *pa1 = 0;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\RBSplusdsbtlbiisdsbP}
\settowidth{\RBSplusdsbtlbiisdsbP}{\usebox{\RBSplusdsbtlbiisdsbO}}
\newsavebox{\RBSplusdsbtlbiisdsbA}
\begin{lrbox}{\RBSplusdsbtlbiisdsbA}
\begin{minipage}{\RBSplusdsbtlbiisdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0x2|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R5=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|RBS+dsb-tlbiis-dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\RBSplusdsbtlbiisdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\RBSplusdsbtlbiisdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\RBSplusdsbtlbiisdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\RBSplusdsbtlbiisdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\RBSplusdsbtlbiisdsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\RBSplusdsbtlbiisdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=2|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/RDW.alias.tex <==
\newlength{\RDWdotaliasH}
\setlength{\RDWdotaliasH}{0cm}
\newsavebox{\RDWdotaliasI}
\begin{lrbox}{\RDWdotaliasI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\RDWdotaliasJ}
\settowidth{\RDWdotaliasJ}{\usebox{\RDWdotaliasI}}
\addtolength{\RDWdotaliasH}{\RDWdotaliasJ}
\newsavebox{\RDWdotaliasK}
\begin{lrbox}{\RDWdotaliasK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
LDR X3,[X4,X2]
LDR X5,[X6]
EOR X7,X5,X5
LDR X8,[X9,X7]
\end{lstlisting}
\end{lrbox}
\newlength{\RDWdotaliasL}
\settowidth{\RDWdotaliasL}{\usebox{\RDWdotaliasK}}
\addtolength{\RDWdotaliasH}{\RDWdotaliasL}
\newsavebox{\RDWdotaliasM}
\begin{lrbox}{\RDWdotaliasM}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\RDWdotaliasN}
\settowidth{\RDWdotaliasN}{\usebox{\RDWdotaliasM}}
\addtolength{\RDWdotaliasH}{\RDWdotaliasN}
\newsavebox{\RDWdotaliasO}
\begin{lrbox}{\RDWdotaliasO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    w |-> pa1;
    x |-> pa1;
    y |-> pa2;
    z |-> pa3;
    *pa1 = 0;
    *pa2 = 0;
    *pa3 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\RDWdotaliasP}
\settowidth{\RDWdotaliasP}{\usebox{\RDWdotaliasO}}
\newsavebox{\RDWdotaliasA}
\begin{lrbox}{\RDWdotaliasA}
\begin{minipage}{\RDWdotaliasH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=z|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R4=w|\\
\lstinline[language=IslaLitmusExp]|1:R6=x|\\
\lstinline[language=IslaLitmusExp]|1:R9=z|\\
\lstinline[language=IslaLitmusExp]|2:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|2:R1=x|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|RDW.alias|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\RDWdotaliasP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\RDWdotaliasO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\RDWdotaliasA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\RDWdotaliasI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\RDWdotaliasK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\RDWdotaliasM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R3=0 & 1:R5=1 & 1:R8=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/ROT.inv+dmbst.tex <==
\newlength{\ROTdotinvplusdmbstH}
\setlength{\ROTdotinvplusdmbstH}{0cm}
\newsavebox{\ROTdotinvplusdmbstI}
\begin{lrbox}{\ROTdotinvplusdmbstI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB ST
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvplusdmbstJ}
\settowidth{\ROTdotinvplusdmbstJ}{\usebox{\ROTdotinvplusdmbstI}}
\addtolength{\ROTdotinvplusdmbstH}{\ROTdotinvplusdmbstJ}
\newsavebox{\ROTdotinvplusdmbstK}
\begin{lrbox}{\ROTdotinvplusdmbstK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvplusdmbstL}
\settowidth{\ROTdotinvplusdmbstL}{\usebox{\ROTdotinvplusdmbstK}}
\addtolength{\ROTdotinvplusdmbstH}{\ROTdotinvplusdmbstL}
\newsavebox{\ROTdotinvplusdmbstM}
\begin{lrbox}{\ROTdotinvplusdmbstM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS x14,esr_el1
AND X14,X14,#0b111
CMP x14,#0b111
MOV X17,#1
MOV X18,#2
// if ESR_EL1.ISS.DFSC == Translation Level 3 then x2 = 1 else x2 = 2
CSEL x0,x17,x18,eq
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvplusdmbstN}
\settowidth{\ROTdotinvplusdmbstN}{\usebox{\ROTdotinvplusdmbstM}}
\addtolength{\ROTdotinvplusdmbstH}{\ROTdotinvplusdmbstN}
\newsavebox{\ROTdotinvplusdmbstO}
\begin{lrbox}{\ROTdotinvplusdmbstO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
physical pa1;
intermediate ipa1;

assert pa1 == ipa1;
ipa1 |-> pa1;

s1table new_table 0x280000 {
  x |-> invalid;
  x ?-> ipa1;
};

identity 0x283000 with default;

x |-> invalid at level 2;
x ?-> table(0x283000) at level 2;

identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvplusdmbstP}
\settowidth{\ROTdotinvplusdmbstP}{\usebox{\ROTdotinvplusdmbstO}}
\newsavebox{\ROTdotinvplusdmbstA}
\begin{lrbox}{\ROTdotinvplusdmbstA}
\begin{minipage}{\ROTdotinvplusdmbstH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=ipa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,new_table)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc2(table=0x283000)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte2(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|ROT.inv+dmbst|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\ROTdotinvplusdmbstP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\ROTdotinvplusdmbstO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\ROTdotinvplusdmbstA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\ROTdotinvplusdmbstI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\ROTdotinvplusdmbstK}\\
  \cline{2-2}
  & thread 1 el1 handler\\
  \cline{2-2}
  & \usebox{\ROTdotinvplusdmbstM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/ROT.inv+dsb.tex <==
\newlength{\ROTdotinvplusdsbH}
\setlength{\ROTdotinvplusdsbH}{0cm}
\newsavebox{\ROTdotinvplusdsbI}
\begin{lrbox}{\ROTdotinvplusdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvplusdsbJ}
\settowidth{\ROTdotinvplusdsbJ}{\usebox{\ROTdotinvplusdsbI}}
\addtolength{\ROTdotinvplusdsbH}{\ROTdotinvplusdsbJ}
\newsavebox{\ROTdotinvplusdsbK}
\begin{lrbox}{\ROTdotinvplusdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvplusdsbL}
\settowidth{\ROTdotinvplusdsbL}{\usebox{\ROTdotinvplusdsbK}}
\addtolength{\ROTdotinvplusdsbH}{\ROTdotinvplusdsbL}
\newsavebox{\ROTdotinvplusdsbM}
\begin{lrbox}{\ROTdotinvplusdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS X14,ESR_EL1
AND X14,X14,#0b111
CMP X14,#0b111
MOV X17,#1
MOV X18,#2
// if ESR_EL1.ISS.DFSC == Translation Level 3 then x2 = 1 else x2 = 2
CSEL X0,X17,X18,eq
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvplusdsbN}
\settowidth{\ROTdotinvplusdsbN}{\usebox{\ROTdotinvplusdsbM}}
\addtolength{\ROTdotinvplusdsbH}{\ROTdotinvplusdsbN}
\newsavebox{\ROTdotinvplusdsbO}
\begin{lrbox}{\ROTdotinvplusdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
physical pa1;
intermediate ipa1;

assert pa1 == ipa1;
ipa1 |-> pa1;

s1table new_table 0x280000 {
  x |-> invalid;
  x ?-> ipa1;
};

identity 0x283000 with default;

x |-> invalid at level 2;
x ?-> table(0x283000) at level 2;

identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvplusdsbP}
\settowidth{\ROTdotinvplusdsbP}{\usebox{\ROTdotinvplusdsbO}}
\newsavebox{\ROTdotinvplusdsbA}
\begin{lrbox}{\ROTdotinvplusdsbA}
\begin{minipage}{\ROTdotinvplusdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=ipa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,new_table)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc2(table=0x283000)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte2(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|ROT.inv+dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\ROTdotinvplusdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\ROTdotinvplusdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\ROTdotinvplusdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\ROTdotinvplusdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\ROTdotinvplusdsbK}\\
  \cline{2-2}
  & thread 1 el1 handler\\
  \cline{2-2}
  & \usebox{\ROTdotinvplusdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/ROT.inv+po.tex <==
\newlength{\ROTdotinvpluspoH}
\setlength{\ROTdotinvpluspoH}{0cm}
\newsavebox{\ROTdotinvpluspoI}
\begin{lrbox}{\ROTdotinvpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvpluspoJ}
\settowidth{\ROTdotinvpluspoJ}{\usebox{\ROTdotinvpluspoI}}
\addtolength{\ROTdotinvpluspoH}{\ROTdotinvpluspoJ}
\newsavebox{\ROTdotinvpluspoK}
\begin{lrbox}{\ROTdotinvpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvpluspoL}
\settowidth{\ROTdotinvpluspoL}{\usebox{\ROTdotinvpluspoK}}
\addtolength{\ROTdotinvpluspoH}{\ROTdotinvpluspoL}
\newsavebox{\ROTdotinvpluspoM}
\begin{lrbox}{\ROTdotinvpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS X14,ESR_EL1
AND X14,X14,#0b111
CMP X14,#0b111
MOV X17,#1
MOV X18,#2
// if ESR_EL1.ISS.DFSC == Translation Level 3 then x2 = 1 else x2 = 2
CSEL X0,X17,X18,eq
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvpluspoN}
\settowidth{\ROTdotinvpluspoN}{\usebox{\ROTdotinvpluspoM}}
\addtolength{\ROTdotinvpluspoH}{\ROTdotinvpluspoN}
\newsavebox{\ROTdotinvpluspoO}
\begin{lrbox}{\ROTdotinvpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
physical pa1;
intermediate ipa1;

assert pa1 == ipa1;
ipa1 |-> pa1;

s1table new_table 0x280000 {
  x |-> invalid;
  x ?-> ipa1;
};

identity 0x283000 with default;

x |-> invalid at level 2;
x ?-> table(0x283000) at level 2;

identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvpluspoP}
\settowidth{\ROTdotinvpluspoP}{\usebox{\ROTdotinvpluspoO}}
\newsavebox{\ROTdotinvpluspoA}
\begin{lrbox}{\ROTdotinvpluspoA}
\begin{minipage}{\ROTdotinvpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=ipa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,new_table)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc2(table=0x283000)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte2(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|ROT.inv+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\ROTdotinvpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\ROTdotinvpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\ROTdotinvpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\ROTdotinvpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\ROTdotinvpluspoK}\\
  \cline{2-2}
  & thread 1 el1 handler\\
  \cline{2-2}
  & \usebox{\ROTdotinvpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/RSW.alias.tex <==
\newlength{\RSWdotaliasH}
\setlength{\RSWdotaliasH}{0cm}
\newsavebox{\RSWdotaliasI}
\begin{lrbox}{\RSWdotaliasI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\RSWdotaliasJ}
\settowidth{\RSWdotaliasJ}{\usebox{\RSWdotaliasI}}
\addtolength{\RSWdotaliasH}{\RSWdotaliasJ}
\newsavebox{\RSWdotaliasK}
\begin{lrbox}{\RSWdotaliasK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
LDR X3,[X4,X2]
LDR X5,[X6]
EOR X7,X5,X5
LDR X8,[X9,X7]
\end{lstlisting}
\end{lrbox}
\newlength{\RSWdotaliasL}
\settowidth{\RSWdotaliasL}{\usebox{\RSWdotaliasK}}
\addtolength{\RSWdotaliasH}{\RSWdotaliasL}
\newsavebox{\RSWdotaliasM}
\begin{lrbox}{\RSWdotaliasM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    w |-> pa1;
    x |-> pa1;
    y |-> pa2;
    z |-> pa3;
    *pa1 = 0;
    *pa2 = 0;
    *pa3 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\RSWdotaliasN}
\settowidth{\RSWdotaliasN}{\usebox{\RSWdotaliasM}}
\newsavebox{\RSWdotaliasO}
\begin{lrbox}{\RSWdotaliasO}
\begin{minipage}{\RSWdotaliasH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=z|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R4=w|\\
\lstinline[language=IslaLitmusExp]|1:R6=x|\\
\lstinline[language=IslaLitmusExp]|1:R9=z|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|RSW.alias|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\RSWdotaliasN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\RSWdotaliasM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\RSWdotaliasO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\RSWdotaliasI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\RSWdotaliasK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R8=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/RWC.RTR.EL1+dsb-isb+dsb-tlbi-dsb.tex <==
\newlength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbH}
\setlength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbH}{0cm}
\newsavebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbI}
\begin{lrbox}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbJ}
\settowidth{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbJ}{\usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbI}}
\addtolength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbH}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbJ}
\newsavebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbK}
\begin{lrbox}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X3,[X4,X2]
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbL}
\settowidth{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbL}{\usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbK}}
\addtolength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbH}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbL}
\newsavebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbM}
\begin{lrbox}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X2
DSB SY
LDR X3,[X4]
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbN}
\settowidth{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbN}{\usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbM}}
\addtolength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbH}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbN}
\newsavebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbO}
\begin{lrbox}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X3,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbP}
\settowidth{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbP}{\usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbO}}
\addtolength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbH}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbP}
\newsavebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbA}
\begin{lrbox}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;

    y |-> pa2;
    y ?-> invalid;
    z |-> pa2;
    *pa1 = 1;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbB}
\settowidth{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbB}{\usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbA}}
\newsavebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbC}
\begin{lrbox}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbC}
\begin{minipage}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R4=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|2:R1=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R2=page(x)|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|RWC.RTR.EL1+dsb-isb+dsb-tlbi-dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R1=1 & 1:R3=0 & 2:R3=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/RWC.RTfR.inv+addr+dmb.tex <==
\newlength{\RWCdotRTfRdotinvplusaddrplusdmbH}
\setlength{\RWCdotRTfRdotinvplusaddrplusdmbH}{0cm}
\newsavebox{\RWCdotRTfRdotinvplusaddrplusdmbI}
\begin{lrbox}{\RWCdotRTfRdotinvplusaddrplusdmbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTfRdotinvplusaddrplusdmbJ}
\settowidth{\RWCdotRTfRdotinvplusaddrplusdmbJ}{\usebox{\RWCdotRTfRdotinvplusaddrplusdmbI}}
\addtolength{\RWCdotRTfRdotinvplusaddrplusdmbH}{\RWCdotRTfRdotinvplusaddrplusdmbJ}
\newsavebox{\RWCdotRTfRdotinvplusaddrplusdmbK}
\begin{lrbox}{\RWCdotRTfRdotinvplusaddrplusdmbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
LDR X3,[X4,X2]
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTfRdotinvplusaddrplusdmbL}
\settowidth{\RWCdotRTfRdotinvplusaddrplusdmbL}{\usebox{\RWCdotRTfRdotinvplusaddrplusdmbK}}
\addtolength{\RWCdotRTfRdotinvplusaddrplusdmbH}{\RWCdotRTfRdotinvplusaddrplusdmbL}
\newsavebox{\RWCdotRTfRdotinvplusaddrplusdmbM}
\begin{lrbox}{\RWCdotRTfRdotinvplusaddrplusdmbM}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTfRdotinvplusaddrplusdmbN}
\settowidth{\RWCdotRTfRdotinvplusaddrplusdmbN}{\usebox{\RWCdotRTfRdotinvplusaddrplusdmbM}}
\addtolength{\RWCdotRTfRdotinvplusaddrplusdmbH}{\RWCdotRTfRdotinvplusaddrplusdmbN}
\newsavebox{\RWCdotRTfRdotinvplusaddrplusdmbO}
\begin{lrbox}{\RWCdotRTfRdotinvplusaddrplusdmbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X3,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTfRdotinvplusaddrplusdmbP}
\settowidth{\RWCdotRTfRdotinvplusaddrplusdmbP}{\usebox{\RWCdotRTfRdotinvplusaddrplusdmbO}}
\addtolength{\RWCdotRTfRdotinvplusaddrplusdmbH}{\RWCdotRTfRdotinvplusaddrplusdmbP}
\newsavebox{\RWCdotRTfRdotinvplusaddrplusdmbA}
\begin{lrbox}{\RWCdotRTfRdotinvplusaddrplusdmbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;

    y |-> invalid;
    y ?-> pa2;
    z |-> pa2;
    *pa1 = 1;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTfRdotinvplusaddrplusdmbB}
\settowidth{\RWCdotRTfRdotinvplusaddrplusdmbB}{\usebox{\RWCdotRTfRdotinvplusaddrplusdmbA}}
\newsavebox{\RWCdotRTfRdotinvplusaddrplusdmbC}
\begin{lrbox}{\RWCdotRTfRdotinvplusaddrplusdmbC}
\begin{minipage}{\RWCdotRTfRdotinvplusaddrplusdmbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R4=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|2:R1=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|RWC.RTfR.inv+addr+dmb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\RWCdotRTfRdotinvplusaddrplusdmbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\RWCdotRTfRdotinvplusaddrplusdmbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\RWCdotRTfRdotinvplusaddrplusdmbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\RWCdotRTfRdotinvplusaddrplusdmbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\RWCdotRTfRdotinvplusaddrplusdmbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\RWCdotRTfRdotinvplusaddrplusdmbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\RWCdotRTfRdotinvplusaddrplusdmbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R1=1 & 1:R3=0 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/S.RT.ro+dsb-tlbiis-dsb+dsb-isb.tex <==
\newlength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbH}
\setlength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbH}{0cm}
\newsavebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbI}
\begin{lrbox}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbJ}
\settowidth{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbJ}{\usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbI}}
\addtolength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbH}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbJ}
\newsavebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbK}
\begin{lrbox}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbL}
\settowidth{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbL}{\usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbK}}
\addtolength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbH}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbL}
\newsavebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbM}
\begin{lrbox}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbN}
\settowidth{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbN}{\usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbM}}
\addtolength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbH}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbN}
\newsavebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbO}
\begin{lrbox}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1 with [AP = 0b11] and default;
    x ?-> pa1;
    z |-> pa1;
    y |-> pa2;

    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbP}
\settowidth{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbP}{\usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbO}}
\newsavebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbA}
\begin{lrbox}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbA}
\begin{minipage}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|S.RT.ro+dsb-tlbiis-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/S.RTf.inv.EL1+dsb-tlbiis-dsb+ctrl.tex <==
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}
\setlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}{0cm}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlI}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlJ}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlJ}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlI}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlJ}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlK}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBNZ X0,L0
L0:
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlL}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlL}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlK}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlL}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlM}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlN}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlN}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlM}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlN}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlO}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlP}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlP}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlO}}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlA}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlA}
\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|S.RTf.inv.EL1+dsb-tlbiis-dsb+ctrl|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/S.RTf.inv.EL1+dsb-tlbiis-dsb+data.tex <==
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}
\setlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}{0cm}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataI}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataJ}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataJ}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataI}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataJ}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataK}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
ORR X2,X2,X4
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataL}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataL}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataK}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataL}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataM}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataN}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataN}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataM}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataN}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataO}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataP}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataP}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataO}}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataA}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataA}
\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|S.RTf.inv.EL1+dsb-tlbiis-dsb+data|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/S.RTf.inv.EL1+dsb-tlbiis-dsb+dmb.tex <==
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}
\setlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{0cm}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}
\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|S.RTf.inv.EL1+dsb-tlbiis-dsb+dmb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/S.RTf.inv.EL1+dsb-tlbiis-dsb+poap.tex <==
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}
\setlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}{0cm}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapI}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapJ}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapJ}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapI}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapJ}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapK}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDAR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapL}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapL}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapK}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapL}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapM}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapN}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapN}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapM}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapN}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapO}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapP}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapP}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapO}}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapA}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapA}
\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|S.RTf.inv.EL1+dsb-tlbiis-dsb+poap|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/S.RTf.inv.EL1+dsb-tlbiis-dsb+popl.tex <==
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}
\setlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}{0cm}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplI}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplJ}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplJ}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplI}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplJ}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplK}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STLR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplL}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplL}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplK}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplL}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplM}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplN}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplN}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplM}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplN}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplO}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplP}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplP}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplO}}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplA}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplA}
\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|S.RTf.inv.EL1+dsb-tlbiis-dsb+popl|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/S.T+dmb+po.tex <==
\newlength{\SdotTplusdmbpluspoH}
\setlength{\SdotTplusdmbpluspoH}{0cm}
\newsavebox{\SdotTplusdmbpluspoI}
\begin{lrbox}{\SdotTplusdmbpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotTplusdmbpluspoJ}
\settowidth{\SdotTplusdmbpluspoJ}{\usebox{\SdotTplusdmbpluspoI}}
\addtolength{\SdotTplusdmbpluspoH}{\SdotTplusdmbpluspoJ}
\newsavebox{\SdotTplusdmbpluspoK}
\begin{lrbox}{\SdotTplusdmbpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotTplusdmbpluspoL}
\settowidth{\SdotTplusdmbpluspoL}{\usebox{\SdotTplusdmbpluspoK}}
\addtolength{\SdotTplusdmbpluspoH}{\SdotTplusdmbpluspoL}
\newsavebox{\SdotTplusdmbpluspoM}
\begin{lrbox}{\SdotTplusdmbpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SdotTplusdmbpluspoN}
\settowidth{\SdotTplusdmbpluspoN}{\usebox{\SdotTplusdmbpluspoM}}
\addtolength{\SdotTplusdmbpluspoH}{\SdotTplusdmbpluspoN}
\newsavebox{\SdotTplusdmbpluspoO}
\begin{lrbox}{\SdotTplusdmbpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 0;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SdotTplusdmbpluspoP}
\settowidth{\SdotTplusdmbpluspoP}{\usebox{\SdotTplusdmbpluspoO}}
\newsavebox{\SdotTplusdmbpluspoA}
\begin{lrbox}{\SdotTplusdmbpluspoA}
\begin{minipage}{\SdotTplusdmbpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0x2|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|S.T+dmb+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SdotTplusdmbpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SdotTplusdmbpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SdotTplusdmbpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SdotTplusdmbpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SdotTplusdmbpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SdotTplusdmbpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & x=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/SB.TfTf.inv+dmb-ctrl-isbs.tex <==
\newlength{\SBdotTfTfdotinvplusdmbctrlisbsH}
\setlength{\SBdotTfTfdotinvplusdmbctrlisbsH}{0cm}
\newsavebox{\SBdotTfTfdotinvplusdmbctrlisbsI}
\begin{lrbox}{\SBdotTfTfdotinvplusdmbctrlisbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
LDR X7,[X8]
CBNZ X7,L0
L0:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdmbctrlisbsJ}
\settowidth{\SBdotTfTfdotinvplusdmbctrlisbsJ}{\usebox{\SBdotTfTfdotinvplusdmbctrlisbsI}}
\addtolength{\SBdotTfTfdotinvplusdmbctrlisbsH}{\SBdotTfTfdotinvplusdmbctrlisbsJ}
\newsavebox{\SBdotTfTfdotinvplusdmbctrlisbsK}
\begin{lrbox}{\SBdotTfTfdotinvplusdmbctrlisbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
LDR X7,[X8]
CBNZ X7,L1
L1:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdmbctrlisbsL}
\settowidth{\SBdotTfTfdotinvplusdmbctrlisbsL}{\usebox{\SBdotTfTfdotinvplusdmbctrlisbsK}}
\addtolength{\SBdotTfTfdotinvplusdmbctrlisbsH}{\SBdotTfTfdotinvplusdmbctrlisbsL}
\newsavebox{\SBdotTfTfdotinvplusdmbctrlisbsM}
\begin{lrbox}{\SBdotTfTfdotinvplusdmbctrlisbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdmbctrlisbsN}
\settowidth{\SBdotTfTfdotinvplusdmbctrlisbsN}{\usebox{\SBdotTfTfdotinvplusdmbctrlisbsM}}
\addtolength{\SBdotTfTfdotinvplusdmbctrlisbsH}{\SBdotTfTfdotinvplusdmbctrlisbsN}
\newsavebox{\SBdotTfTfdotinvplusdmbctrlisbsO}
\begin{lrbox}{\SBdotTfTfdotinvplusdmbctrlisbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdmbctrlisbsP}
\settowidth{\SBdotTfTfdotinvplusdmbctrlisbsP}{\usebox{\SBdotTfTfdotinvplusdmbctrlisbsO}}
\addtolength{\SBdotTfTfdotinvplusdmbctrlisbsH}{\SBdotTfTfdotinvplusdmbctrlisbsP}
\newsavebox{\SBdotTfTfdotinvplusdmbctrlisbsA}
\begin{lrbox}{\SBdotTfTfdotinvplusdmbctrlisbsA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> invalid;
    y ?-> pa2;
    v |-> pa2;
    *pa2 = 1;

    z |-> pa3;
    *pa3 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdmbctrlisbsB}
\settowidth{\SBdotTfTfdotinvplusdmbctrlisbsB}{\usebox{\SBdotTfTfdotinvplusdmbctrlisbsA}}
\newsavebox{\SBdotTfTfdotinvplusdmbctrlisbsC}
\begin{lrbox}{\SBdotTfTfdotinvplusdmbctrlisbsC}
\begin{minipage}{\SBdotTfTfdotinvplusdmbctrlisbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R8=z|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R0=desc3(v,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R8=z|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|SB.TfTf.inv+dmb-ctrl-isbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SBdotTfTfdotinvplusdmbctrlisbsB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SBdotTfTfdotinvplusdmbctrlisbsA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SBdotTfTfdotinvplusdmbctrlisbsC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvplusdmbctrlisbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvplusdmbctrlisbsK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvplusdmbctrlisbsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvplusdmbctrlisbsO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/SB.TfTf.inv+dsb-isbs.tex <==
\newlength{\SBdotTfTfdotinvplusdsbisbsH}
\setlength{\SBdotTfTfdotinvplusdsbisbsH}{0cm}
\newsavebox{\SBdotTfTfdotinvplusdsbisbsI}
\begin{lrbox}{\SBdotTfTfdotinvplusdsbisbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdsbisbsJ}
\settowidth{\SBdotTfTfdotinvplusdsbisbsJ}{\usebox{\SBdotTfTfdotinvplusdsbisbsI}}
\addtolength{\SBdotTfTfdotinvplusdsbisbsH}{\SBdotTfTfdotinvplusdsbisbsJ}
\newsavebox{\SBdotTfTfdotinvplusdsbisbsK}
\begin{lrbox}{\SBdotTfTfdotinvplusdsbisbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdsbisbsL}
\settowidth{\SBdotTfTfdotinvplusdsbisbsL}{\usebox{\SBdotTfTfdotinvplusdsbisbsK}}
\addtolength{\SBdotTfTfdotinvplusdsbisbsH}{\SBdotTfTfdotinvplusdsbisbsL}
\newsavebox{\SBdotTfTfdotinvplusdsbisbsM}
\begin{lrbox}{\SBdotTfTfdotinvplusdsbisbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdsbisbsN}
\settowidth{\SBdotTfTfdotinvplusdsbisbsN}{\usebox{\SBdotTfTfdotinvplusdsbisbsM}}
\addtolength{\SBdotTfTfdotinvplusdsbisbsH}{\SBdotTfTfdotinvplusdsbisbsN}
\newsavebox{\SBdotTfTfdotinvplusdsbisbsO}
\begin{lrbox}{\SBdotTfTfdotinvplusdsbisbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdsbisbsP}
\settowidth{\SBdotTfTfdotinvplusdsbisbsP}{\usebox{\SBdotTfTfdotinvplusdsbisbsO}}
\addtolength{\SBdotTfTfdotinvplusdsbisbsH}{\SBdotTfTfdotinvplusdsbisbsP}
\newsavebox{\SBdotTfTfdotinvplusdsbisbsA}
\begin{lrbox}{\SBdotTfTfdotinvplusdsbisbsA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> invalid;
    y ?-> pa2;
    v |-> pa2;
    *pa2 = 1;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdsbisbsB}
\settowidth{\SBdotTfTfdotinvplusdsbisbsB}{\usebox{\SBdotTfTfdotinvplusdsbisbsA}}
\newsavebox{\SBdotTfTfdotinvplusdsbisbsC}
\begin{lrbox}{\SBdotTfTfdotinvplusdsbisbsC}
\begin{minipage}{\SBdotTfTfdotinvplusdsbisbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R0=desc3(v,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|SB.TfTf.inv+dsb-isbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SBdotTfTfdotinvplusdsbisbsB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SBdotTfTfdotinvplusdsbisbsA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SBdotTfTfdotinvplusdsbisbsC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvplusdsbisbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvplusdsbisbsK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvplusdsbisbsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvplusdsbisbsO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/SB.TfTf.invv+rfi-ctrl-isbs.tex <==
\newlength{\SBdotTfTfdotinvvplusrfictrlisbsH}
\setlength{\SBdotTfTfdotinvvplusrfictrlisbsH}{0cm}
\newsavebox{\SBdotTfTfdotinvvplusrfictrlisbsI}
\begin{lrbox}{\SBdotTfTfdotinvvplusrfictrlisbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X7,[X1]
CBNZ X7,L0
L0:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvvplusrfictrlisbsJ}
\settowidth{\SBdotTfTfdotinvvplusrfictrlisbsJ}{\usebox{\SBdotTfTfdotinvvplusrfictrlisbsI}}
\addtolength{\SBdotTfTfdotinvvplusrfictrlisbsH}{\SBdotTfTfdotinvvplusrfictrlisbsJ}
\newsavebox{\SBdotTfTfdotinvvplusrfictrlisbsK}
\begin{lrbox}{\SBdotTfTfdotinvvplusrfictrlisbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X7,[X1]
CBNZ X7,L1
L1:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvvplusrfictrlisbsL}
\settowidth{\SBdotTfTfdotinvvplusrfictrlisbsL}{\usebox{\SBdotTfTfdotinvvplusrfictrlisbsK}}
\addtolength{\SBdotTfTfdotinvvplusrfictrlisbsH}{\SBdotTfTfdotinvvplusrfictrlisbsL}
\newsavebox{\SBdotTfTfdotinvvplusrfictrlisbsM}
\begin{lrbox}{\SBdotTfTfdotinvvplusrfictrlisbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvvplusrfictrlisbsN}
\settowidth{\SBdotTfTfdotinvvplusrfictrlisbsN}{\usebox{\SBdotTfTfdotinvvplusrfictrlisbsM}}
\addtolength{\SBdotTfTfdotinvvplusrfictrlisbsH}{\SBdotTfTfdotinvvplusrfictrlisbsN}
\newsavebox{\SBdotTfTfdotinvvplusrfictrlisbsO}
\begin{lrbox}{\SBdotTfTfdotinvvplusrfictrlisbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvvplusrfictrlisbsP}
\settowidth{\SBdotTfTfdotinvvplusrfictrlisbsP}{\usebox{\SBdotTfTfdotinvvplusrfictrlisbsO}}
\addtolength{\SBdotTfTfdotinvvplusrfictrlisbsH}{\SBdotTfTfdotinvvplusrfictrlisbsP}
\newsavebox{\SBdotTfTfdotinvvplusrfictrlisbsA}
\begin{lrbox}{\SBdotTfTfdotinvvplusrfictrlisbsA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> invalid;
    y ?-> pa2;
    v |-> pa2;
    *pa2 = 1;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvvplusrfictrlisbsB}
\settowidth{\SBdotTfTfdotinvvplusrfictrlisbsB}{\usebox{\SBdotTfTfdotinvvplusrfictrlisbsA}}
\newsavebox{\SBdotTfTfdotinvvplusrfictrlisbsC}
\begin{lrbox}{\SBdotTfTfdotinvvplusrfictrlisbsC}
\begin{minipage}{\SBdotTfTfdotinvvplusrfictrlisbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R0=desc3(v,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|SB.TfTf.invv+rfi-ctrl-isbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SBdotTfTfdotinvvplusrfictrlisbsB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SBdotTfTfdotinvvplusrfictrlisbsA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SBdotTfTfdotinvvplusrfictrlisbsC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvvplusrfictrlisbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvvplusrfictrlisbsK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvvplusrfictrlisbsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvvplusrfictrlisbsO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0 & 0:R7=desc3(u,page_table_base) & 1:R2=0 & 1:R7=desc3(v,page_table_base)|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/SwitchTable.EL2+msrttbr-eret.tex <==
\newlength{\SwitchTabledotELtwoplusmsrttbreretH}
\setlength{\SwitchTabledotELtwoplusmsrttbreretH}{0cm}
\newsavebox{\SwitchTabledotELtwoplusmsrttbreretI}
\begin{lrbox}{\SwitchTabledotELtwoplusmsrttbreretI}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
HVC #0
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SwitchTabledotELtwoplusmsrttbreretJ}
\settowidth{\SwitchTabledotELtwoplusmsrttbreretJ}{\usebox{\SwitchTabledotELtwoplusmsrttbreretI}}
\addtolength{\SwitchTabledotELtwoplusmsrttbreretH}{\SwitchTabledotELtwoplusmsrttbreretJ}
\newsavebox{\SwitchTabledotELtwoplusmsrttbreretK}
\begin{lrbox}{\SwitchTabledotELtwoplusmsrttbreretK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MSR TTBR0_EL1,X4
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SwitchTabledotELtwoplusmsrttbreretL}
\settowidth{\SwitchTabledotELtwoplusmsrttbreretL}{\usebox{\SwitchTabledotELtwoplusmsrttbreretK}}
\addtolength{\SwitchTabledotELtwoplusmsrttbreretH}{\SwitchTabledotELtwoplusmsrttbreretL}
\newsavebox{\SwitchTabledotELtwoplusmsrttbreretM}
\begin{lrbox}{\SwitchTabledotELtwoplusmsrttbreretM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
option default_tables = false;
physical pa1 pa2;

s1table initial_table 0x200000 {
    x |-> pa1 at level 3;
}

s1table new_table 0x280000  {
    x |-> pa2 at level 3;
}

s1table el2_table 0x300000 {
    identity 0x2000 with code;
}

*pa1 = 0;
*pa2 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\SwitchTabledotELtwoplusmsrttbreretN}
\settowidth{\SwitchTabledotELtwoplusmsrttbreretN}{\usebox{\SwitchTabledotELtwoplusmsrttbreretM}}
\newsavebox{\SwitchTabledotELtwoplusmsrttbreretO}
\begin{lrbox}{\SwitchTabledotELtwoplusmsrttbreretO}
\begin{minipage}{\SwitchTabledotELtwoplusmsrttbreretH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|R1=x|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=ttbr(asid=0x0000,base=new_table)|\\
\lstinline[language=IslaLitmusExp]|TTBR0_EL1=ttbr(base=initial_table,asid=0x0000)|\\
\lstinline[language=IslaLitmusExp]|TTBR0_EL2=ttbr(base=el2_table,asid=0x0000)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|SwitchTable.EL2+msrttbr-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SwitchTabledotELtwoplusmsrttbreretN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SwitchTabledotELtwoplusmsrttbreretM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SwitchTabledotELtwoplusmsrttbreretO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SwitchTabledotELtwoplusmsrttbreretI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\SwitchTabledotELtwoplusmsrttbreretK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/SwitchTable.same-asid+eret.toml.tex <==
\newlength{\SwitchTabledotsameasidpluseretdottomlH}
\setlength{\SwitchTabledotsameasidpluseretdottomlH}{0cm}
\newsavebox{\SwitchTabledotsameasidpluseretdottomlI}
\begin{lrbox}{\SwitchTabledotsameasidpluseretdottomlI}
\begin{lstlisting}[language=AArch64,showlines=true]
MSR TTBR0_EL1,X0
ERET
L0:
LDR X1,[X2]
\end{lstlisting}
\end{lrbox}
\newlength{\SwitchTabledotsameasidpluseretdottomlJ}
\settowidth{\SwitchTabledotsameasidpluseretdottomlJ}{\usebox{\SwitchTabledotsameasidpluseretdottomlI}}
\addtolength{\SwitchTabledotsameasidpluseretdottomlH}{\SwitchTabledotsameasidpluseretdottomlJ}
\newsavebox{\SwitchTabledotsameasidpluseretdottomlK}
\begin{lrbox}{\SwitchTabledotsameasidpluseretdottomlK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X1,#1
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SwitchTabledotsameasidpluseretdottomlL}
\settowidth{\SwitchTabledotsameasidpluseretdottomlL}{\usebox{\SwitchTabledotsameasidpluseretdottomlK}}
\addtolength{\SwitchTabledotsameasidpluseretdottomlH}{\SwitchTabledotsameasidpluseretdottomlL}
\newsavebox{\SwitchTabledotsameasidpluseretdottomlM}
\begin{lrbox}{\SwitchTabledotsameasidpluseretdottomlM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    intermediate ipa1;
    physical pa1;

    *pa1 = 0;

    s1table table0 0x2C0000 {
        identity 0x1000 with code;
        x |-> pa1;
    };
    s1table table1 0x300000 {
        identity 0x1000 with code;
        x |-> invalid;
    };

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SwitchTabledotsameasidpluseretdottomlN}
\settowidth{\SwitchTabledotsameasidpluseretdottomlN}{\usebox{\SwitchTabledotsameasidpluseretdottomlM}}
\newsavebox{\SwitchTabledotsameasidpluseretdottomlO}
\begin{lrbox}{\SwitchTabledotsameasidpluseretdottomlO}
\begin{minipage}{\SwitchTabledotsameasidpluseretdottomlH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL1=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b1|\\
\lstinline[language=IslaLitmusExp]|R0=ttbr(asid=0x01,base=table1)|\\
\lstinline[language=IslaLitmusExp]|R2=x|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL1=0b00000|\\
\lstinline[language=IslaLitmusExp]|TTBR0_EL1=ttbr(base=table0,asid=0x00)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|SwitchTable.same-asid+eret.toml|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SwitchTabledotsameasidpluseretdottomlN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SwitchTabledotsameasidpluseretdottomlM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SwitchTabledotsameasidpluseretdottomlO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SwitchTabledotsameasidpluseretdottomlI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\SwitchTabledotsameasidpluseretdottomlK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R1=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/W+T.tex <==
\newlength{\WplusTH}
\setlength{\WplusTH}{0cm}
\newsavebox{\WplusTI}
\begin{lrbox}{\WplusTI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WplusTJ}
\settowidth{\WplusTJ}{\usebox{\WplusTI}}
\addtolength{\WplusTH}{\WplusTJ}
\newsavebox{\WplusTK}
\begin{lrbox}{\WplusTK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WplusTL}
\settowidth{\WplusTL}{\usebox{\WplusTK}}
\addtolength{\WplusTH}{\WplusTL}
\newsavebox{\WplusTM}
\begin{lrbox}{\WplusTM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1000:
MOV X0,#0
\end{lstlisting}
\end{lrbox}
\newlength{\WplusTN}
\settowidth{\WplusTN}{\usebox{\WplusTM}}
\addtolength{\WplusTH}{\WplusTN}
\newsavebox{\WplusTO}
\begin{lrbox}{\WplusTO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid at level 2;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WplusTP}
\settowidth{\WplusTP}{\usebox{\WplusTO}}
\newsavebox{\WplusTA}
\begin{lrbox}{\WplusTA}
\begin{minipage}{\WplusTH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte2(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|W+T|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WplusTP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WplusTO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WplusTA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WplusTI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WplusTK}\\
  \cline{2-2}
  & handler\\
  \cline{2-2}
  & \usebox{\WplusTM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|true|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/W.tex <==
\newlength{\WH}
\setlength{\WH}{0cm}
\newsavebox{\WI}
\begin{lrbox}{\WI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WJ}
\settowidth{\WJ}{\usebox{\WI}}
\addtolength{\WH}{\WJ}
\newsavebox{\WK}
\begin{lrbox}{\WK}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
\end{lstlisting}
\end{lrbox}
\newlength{\WL}
\settowidth{\WL}{\usebox{\WK}}
\newsavebox{\WM}
\begin{lrbox}{\WM}
\begin{minipage}{\WH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=x|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|W|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WL}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WK}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WM}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WI}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|true|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/WBM+dsb-tlbiis-dsb.tex <==
\newlength{\WBMplusdsbtlbiisdsbH}
\setlength{\WBMplusdsbtlbiisdsbH}{0cm}
\newsavebox{\WBMplusdsbtlbiisdsbI}
\begin{lrbox}{\WBMplusdsbtlbiisdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X5
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WBMplusdsbtlbiisdsbJ}
\settowidth{\WBMplusdsbtlbiisdsbJ}{\usebox{\WBMplusdsbtlbiisdsbI}}
\addtolength{\WBMplusdsbtlbiisdsbH}{\WBMplusdsbtlbiisdsbJ}
\newsavebox{\WBMplusdsbtlbiisdsbK}
\begin{lrbox}{\WBMplusdsbtlbiisdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WBMplusdsbtlbiisdsbL}
\settowidth{\WBMplusdsbtlbiisdsbL}{\usebox{\WBMplusdsbtlbiisdsbK}}
\addtolength{\WBMplusdsbtlbiisdsbH}{\WBMplusdsbtlbiisdsbL}
\newsavebox{\WBMplusdsbtlbiisdsbM}
\begin{lrbox}{\WBMplusdsbtlbiisdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WBMplusdsbtlbiisdsbN}
\settowidth{\WBMplusdsbtlbiisdsbN}{\usebox{\WBMplusdsbtlbiisdsbM}}
\addtolength{\WBMplusdsbtlbiisdsbH}{\WBMplusdsbtlbiisdsbN}
\newsavebox{\WBMplusdsbtlbiisdsbO}
\begin{lrbox}{\WBMplusdsbtlbiisdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    y |-> pa1;
    *pa1 = 0;
    x ?-> invalid;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WBMplusdsbtlbiisdsbP}
\settowidth{\WBMplusdsbtlbiisdsbP}{\usebox{\WBMplusdsbtlbiisdsbO}}
\newsavebox{\WBMplusdsbtlbiisdsbA}
\begin{lrbox}{\WBMplusdsbtlbiisdsbA}
\begin{minipage}{\WBMplusdsbtlbiisdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0x2|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R5=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:R0=0x1|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WBM+dsb-tlbiis-dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WBMplusdsbtlbiisdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WBMplusdsbtlbiisdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WBMplusdsbtlbiisdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WBMplusdsbtlbiisdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WBMplusdsbtlbiisdsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WBMplusdsbtlbiisdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|x=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/WDS+dsb-tlbiipa-dsb-eret-po.tex <==
\newlength{\WDSplusdsbtlbiipadsberetpoH}
\setlength{\WDSplusdsbtlbiipadsberetpoH}{0cm}
\newsavebox{\WDSplusdsbtlbiipadsberetpoI}
\begin{lrbox}{\WDSplusdsbtlbiipadsberetpoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1,X6
DSB SY
ERET
L0:
STR X2,[X3]
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\WDSplusdsbtlbiipadsberetpoJ}
\settowidth{\WDSplusdsbtlbiipadsberetpoJ}{\usebox{\WDSplusdsbtlbiipadsberetpoI}}
\addtolength{\WDSplusdsbtlbiipadsberetpoH}{\WDSplusdsbtlbiipadsberetpoJ}
\newsavebox{\WDSplusdsbtlbiipadsberetpoK}
\begin{lrbox}{\WDSplusdsbtlbiipadsberetpoK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1200:
MOV X4,#1
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WDSplusdsbtlbiipadsberetpoL}
\settowidth{\WDSplusdsbtlbiipadsberetpoL}{\usebox{\WDSplusdsbtlbiipadsberetpoK}}
\addtolength{\WDSplusdsbtlbiipadsberetpoH}{\WDSplusdsbtlbiipadsberetpoL}
\newsavebox{\WDSplusdsbtlbiipadsberetpoM}
\begin{lrbox}{\WDSplusdsbtlbiipadsberetpoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X4,#2
MRS X20,ELR_EL2
ADD X20,X20,#4
MSR ELR_EL2,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WDSplusdsbtlbiipadsberetpoN}
\settowidth{\WDSplusdsbtlbiipadsberetpoN}{\usebox{\WDSplusdsbtlbiipadsberetpoM}}
\addtolength{\WDSplusdsbtlbiipadsberetpoH}{\WDSplusdsbtlbiipadsberetpoN}
\newsavebox{\WDSplusdsbtlbiipadsberetpoO}
\begin{lrbox}{\WDSplusdsbtlbiipadsberetpoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;
    x ?-> invalid;

    ipa1 |-> pa1;
    ipa1 ?-> invalid;

    *pa1 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WDSplusdsbtlbiipadsberetpoP}
\settowidth{\WDSplusdsbtlbiipadsberetpoP}{\usebox{\WDSplusdsbtlbiipadsberetpoO}}
\newsavebox{\WDSplusdsbtlbiipadsberetpoA}
\begin{lrbox}{\WDSplusdsbtlbiipadsberetpoA}
\begin{minipage}{\WDSplusdsbtlbiipadsberetpoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R2=0b0|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R5=x|\\
\lstinline[language=IslaLitmusExp]|R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00100|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WDS+dsb-tlbiipa-dsb-eret-po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WDSplusdsbtlbiipadsberetpoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WDSplusdsbtlbiipadsberetpoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WDSplusdsbtlbiipadsberetpoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WDSplusdsbtlbiipadsberetpoI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\WDSplusdsbtlbiipadsberetpoK}\\
  \cline{2-2}
  & thread0 el2 handler lower exc\\
  \cline{2-2}
  & \usebox{\WDSplusdsbtlbiipadsberetpoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/WDS+po-dsb-tlbiipa-dsb-eret.tex <==
\newlength{\WDSpluspodsbtlbiipadsberetH}
\setlength{\WDSpluspodsbtlbiipadsberetH}{0cm}
\newsavebox{\WDSpluspodsbtlbiipadsberetI}
\begin{lrbox}{\WDSpluspodsbtlbiipadsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
STR X2,[X3]
DSB SY
TLBI IPAS2E1,X6
DSB SY
ERET
L0:
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsberetJ}
\settowidth{\WDSpluspodsbtlbiipadsberetJ}{\usebox{\WDSpluspodsbtlbiipadsberetI}}
\addtolength{\WDSpluspodsbtlbiipadsberetH}{\WDSpluspodsbtlbiipadsberetJ}
\newsavebox{\WDSpluspodsbtlbiipadsberetK}
\begin{lrbox}{\WDSpluspodsbtlbiipadsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1200:
MOV X4,#1
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsberetL}
\settowidth{\WDSpluspodsbtlbiipadsberetL}{\usebox{\WDSpluspodsbtlbiipadsberetK}}
\addtolength{\WDSpluspodsbtlbiipadsberetH}{\WDSpluspodsbtlbiipadsberetL}
\newsavebox{\WDSpluspodsbtlbiipadsberetM}
\begin{lrbox}{\WDSpluspodsbtlbiipadsberetM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X4,#2
MRS X20,ELR_EL2
ADD X20,X20,#4
MSR ELR_EL2,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsberetN}
\settowidth{\WDSpluspodsbtlbiipadsberetN}{\usebox{\WDSpluspodsbtlbiipadsberetM}}
\addtolength{\WDSpluspodsbtlbiipadsberetH}{\WDSpluspodsbtlbiipadsberetN}
\newsavebox{\WDSpluspodsbtlbiipadsberetO}
\begin{lrbox}{\WDSpluspodsbtlbiipadsberetO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;
    x ?-> invalid;

    ipa1 |-> pa1;
    ipa1 ?-> invalid;

    *pa1 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsberetP}
\settowidth{\WDSpluspodsbtlbiipadsberetP}{\usebox{\WDSpluspodsbtlbiipadsberetO}}
\newsavebox{\WDSpluspodsbtlbiipadsberetA}
\begin{lrbox}{\WDSpluspodsbtlbiipadsberetA}
\begin{minipage}{\WDSpluspodsbtlbiipadsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R2=0b0|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R5=x|\\
\lstinline[language=IslaLitmusExp]|R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00100|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WDS+po-dsb-tlbiipa-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WDSpluspodsbtlbiipadsberetP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WDSpluspodsbtlbiipadsberetO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WDSpluspodsbtlbiipadsberetA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsberetI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsberetK}\\
  \cline{2-2}
  & thread0 el2 handler lower exc\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsberetM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/WDS+po-dsb-tlbiipa-dsb-po-eret.tex <==
\newlength{\WDSpluspodsbtlbiipadsbpoeretH}
\setlength{\WDSpluspodsbtlbiipadsbpoeretH}{0cm}
\newsavebox{\WDSpluspodsbtlbiipadsbpoeretI}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbpoeretI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1,X6
DSB SY
STR X2,[X3]
ERET
L0:
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsbpoeretJ}
\settowidth{\WDSpluspodsbtlbiipadsbpoeretJ}{\usebox{\WDSpluspodsbtlbiipadsbpoeretI}}
\addtolength{\WDSpluspodsbtlbiipadsbpoeretH}{\WDSpluspodsbtlbiipadsbpoeretJ}
\newsavebox{\WDSpluspodsbtlbiipadsbpoeretK}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbpoeretK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1200:
MOV X4,#1
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsbpoeretL}
\settowidth{\WDSpluspodsbtlbiipadsbpoeretL}{\usebox{\WDSpluspodsbtlbiipadsbpoeretK}}
\addtolength{\WDSpluspodsbtlbiipadsbpoeretH}{\WDSpluspodsbtlbiipadsbpoeretL}
\newsavebox{\WDSpluspodsbtlbiipadsbpoeretM}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbpoeretM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X4,#2
MRS X20,ELR_EL2
ADD X20,X20,#4
MSR ELR_EL2,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsbpoeretN}
\settowidth{\WDSpluspodsbtlbiipadsbpoeretN}{\usebox{\WDSpluspodsbtlbiipadsbpoeretM}}
\addtolength{\WDSpluspodsbtlbiipadsbpoeretH}{\WDSpluspodsbtlbiipadsbpoeretN}
\newsavebox{\WDSpluspodsbtlbiipadsbpoeretO}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbpoeretO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;
    x ?-> invalid;

    ipa1 |-> pa1;
    ipa1 ?-> invalid;

    *pa1 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsbpoeretP}
\settowidth{\WDSpluspodsbtlbiipadsbpoeretP}{\usebox{\WDSpluspodsbtlbiipadsbpoeretO}}
\newsavebox{\WDSpluspodsbtlbiipadsbpoeretA}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbpoeretA}
\begin{minipage}{\WDSpluspodsbtlbiipadsbpoeretH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R2=0b0|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R5=x|\\
\lstinline[language=IslaLitmusExp]|R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00100|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WDS+po-dsb-tlbiipa-dsb-po-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WDSpluspodsbtlbiipadsbpoeretP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WDSpluspodsbtlbiipadsbpoeretO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WDSpluspodsbtlbiipadsbpoeretA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsbpoeretI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsbpoeretK}\\
  \cline{2-2}
  & thread0 el2 handler lower exc\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsbpoeretM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/WDS+po-dsb-tlbiipa-dsb-tlbiis-dsb-eret.tex <==
\newlength{\WDSpluspodsbtlbiipadsbtlbiisdsberetH}
\setlength{\WDSpluspodsbtlbiipadsbtlbiisdsberetH}{0cm}
\newsavebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetI}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbtlbiisdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
STR X2,[X3]
DSB SY
TLBI IPAS2E1,X6
DSB SY
TLBI VMALLE1IS
DSB SY
ERET
L0:
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsbtlbiisdsberetJ}
\settowidth{\WDSpluspodsbtlbiipadsbtlbiisdsberetJ}{\usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetI}}
\addtolength{\WDSpluspodsbtlbiipadsbtlbiisdsberetH}{\WDSpluspodsbtlbiipadsbtlbiisdsberetJ}
\newsavebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetK}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbtlbiisdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1200:
MOV X4,#1
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsbtlbiisdsberetL}
\settowidth{\WDSpluspodsbtlbiipadsbtlbiisdsberetL}{\usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetK}}
\addtolength{\WDSpluspodsbtlbiipadsbtlbiisdsberetH}{\WDSpluspodsbtlbiipadsbtlbiisdsberetL}
\newsavebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetM}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbtlbiisdsberetM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X4,#2
MRS X20,ELR_EL2
ADD X20,X20,#4
MSR ELR_EL2,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsbtlbiisdsberetN}
\settowidth{\WDSpluspodsbtlbiipadsbtlbiisdsberetN}{\usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetM}}
\addtolength{\WDSpluspodsbtlbiipadsbtlbiisdsberetH}{\WDSpluspodsbtlbiipadsbtlbiisdsberetN}
\newsavebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetO}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbtlbiisdsberetO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;
    x ?-> invalid;

    ipa1 |-> pa1;
    ipa1 ?-> invalid;

    *pa1 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsbtlbiisdsberetP}
\settowidth{\WDSpluspodsbtlbiipadsbtlbiisdsberetP}{\usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetO}}
\newsavebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetA}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbtlbiisdsberetA}
\begin{minipage}{\WDSpluspodsbtlbiipadsbtlbiisdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R2=0b0|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R5=x|\\
\lstinline[language=IslaLitmusExp]|R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00100|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WDS+po-dsb-tlbiipa-dsb-tlbiis-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WDSpluspodsbtlbiipadsbtlbiisdsberetP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetK}\\
  \cline{2-2}
  & thread0 el2 handler lower exc\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/WRC.RRTf.inv+addrs.tex <==
\newlength{\WRCdotRRTfdotinvplusaddrsH}
\setlength{\WRCdotRRTfdotinvplusaddrsH}{0cm}
\newsavebox{\WRCdotRRTfdotinvplusaddrsI}
\begin{lrbox}{\WRCdotRRTfdotinvplusaddrsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusaddrsJ}
\settowidth{\WRCdotRRTfdotinvplusaddrsJ}{\usebox{\WRCdotRRTfdotinvplusaddrsI}}
\addtolength{\WRCdotRRTfdotinvplusaddrsH}{\WRCdotRRTfdotinvplusaddrsJ}
\newsavebox{\WRCdotRRTfdotinvplusaddrsK}
\begin{lrbox}{\WRCdotRRTfdotinvplusaddrsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
STR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusaddrsL}
\settowidth{\WRCdotRRTfdotinvplusaddrsL}{\usebox{\WRCdotRRTfdotinvplusaddrsK}}
\addtolength{\WRCdotRRTfdotinvplusaddrsH}{\WRCdotRRTfdotinvplusaddrsL}
\newsavebox{\WRCdotRRTfdotinvplusaddrsM}
\begin{lrbox}{\WRCdotRRTfdotinvplusaddrsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusaddrsN}
\settowidth{\WRCdotRRTfdotinvplusaddrsN}{\usebox{\WRCdotRRTfdotinvplusaddrsM}}
\addtolength{\WRCdotRRTfdotinvplusaddrsH}{\WRCdotRRTfdotinvplusaddrsN}
\newsavebox{\WRCdotRRTfdotinvplusaddrsO}
\begin{lrbox}{\WRCdotRRTfdotinvplusaddrsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusaddrsP}
\settowidth{\WRCdotRRTfdotinvplusaddrsP}{\usebox{\WRCdotRRTfdotinvplusaddrsO}}
\addtolength{\WRCdotRRTfdotinvplusaddrsH}{\WRCdotRRTfdotinvplusaddrsP}
\newsavebox{\WRCdotRRTfdotinvplusaddrsA}
\begin{lrbox}{\WRCdotRRTfdotinvplusaddrsA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusaddrsB}
\settowidth{\WRCdotRRTfdotinvplusaddrsB}{\usebox{\WRCdotRRTfdotinvplusaddrsA}}
\newsavebox{\WRCdotRRTfdotinvplusaddrsC}
\begin{lrbox}{\WRCdotRRTfdotinvplusaddrsC}
\begin{minipage}{\WRCdotRRTfdotinvplusaddrsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.RRTf.inv+addrs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotRRTfdotinvplusaddrsB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotRRTfdotinvplusaddrsA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotRRTfdotinvplusaddrsC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusaddrsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusaddrsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusaddrsM}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusaddrsO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=desc3(z,page_table_base) & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/WRC.RRTf.inv+dmbs.tex <==
\newlength{\WRCdotRRTfdotinvplusdmbsH}
\setlength{\WRCdotRRTfdotinvplusdmbsH}{0cm}
\newsavebox{\WRCdotRRTfdotinvplusdmbsI}
\begin{lrbox}{\WRCdotRRTfdotinvplusdmbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdmbsJ}
\settowidth{\WRCdotRRTfdotinvplusdmbsJ}{\usebox{\WRCdotRRTfdotinvplusdmbsI}}
\addtolength{\WRCdotRRTfdotinvplusdmbsH}{\WRCdotRRTfdotinvplusdmbsJ}
\newsavebox{\WRCdotRRTfdotinvplusdmbsK}
\begin{lrbox}{\WRCdotRRTfdotinvplusdmbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdmbsL}
\settowidth{\WRCdotRRTfdotinvplusdmbsL}{\usebox{\WRCdotRRTfdotinvplusdmbsK}}
\addtolength{\WRCdotRRTfdotinvplusdmbsH}{\WRCdotRRTfdotinvplusdmbsL}
\newsavebox{\WRCdotRRTfdotinvplusdmbsM}
\begin{lrbox}{\WRCdotRRTfdotinvplusdmbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdmbsN}
\settowidth{\WRCdotRRTfdotinvplusdmbsN}{\usebox{\WRCdotRRTfdotinvplusdmbsM}}
\addtolength{\WRCdotRRTfdotinvplusdmbsH}{\WRCdotRRTfdotinvplusdmbsN}
\newsavebox{\WRCdotRRTfdotinvplusdmbsO}
\begin{lrbox}{\WRCdotRRTfdotinvplusdmbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdmbsP}
\settowidth{\WRCdotRRTfdotinvplusdmbsP}{\usebox{\WRCdotRRTfdotinvplusdmbsO}}
\addtolength{\WRCdotRRTfdotinvplusdmbsH}{\WRCdotRRTfdotinvplusdmbsP}
\newsavebox{\WRCdotRRTfdotinvplusdmbsA}
\begin{lrbox}{\WRCdotRRTfdotinvplusdmbsA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdmbsB}
\settowidth{\WRCdotRRTfdotinvplusdmbsB}{\usebox{\WRCdotRRTfdotinvplusdmbsA}}
\newsavebox{\WRCdotRRTfdotinvplusdmbsC}
\begin{lrbox}{\WRCdotRRTfdotinvplusdmbsC}
\begin{minipage}{\WRCdotRRTfdotinvplusdmbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.RRTf.inv+dmbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotRRTfdotinvplusdmbsB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotRRTfdotinvplusdmbsA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotRRTfdotinvplusdmbsC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdmbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdmbsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdmbsM}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdmbsO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=desc3(z,page_table_base) & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/WRC.RRTf.inv+dsb+ctrl-isb.tex <==
\newlength{\WRCdotRRTfdotinvplusdsbplusctrlisbH}
\setlength{\WRCdotRRTfdotinvplusdsbplusctrlisbH}{0cm}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusctrlisbI}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusctrlisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusctrlisbJ}
\settowidth{\WRCdotRRTfdotinvplusdsbplusctrlisbJ}{\usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbI}}
\addtolength{\WRCdotRRTfdotinvplusdsbplusctrlisbH}{\WRCdotRRTfdotinvplusdsbplusctrlisbJ}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusctrlisbK}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusctrlisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusctrlisbL}
\settowidth{\WRCdotRRTfdotinvplusdsbplusctrlisbL}{\usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbK}}
\addtolength{\WRCdotRRTfdotinvplusdsbplusctrlisbH}{\WRCdotRRTfdotinvplusdsbplusctrlisbL}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusctrlisbM}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusctrlisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBNZ X0,L0
L0:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusctrlisbN}
\settowidth{\WRCdotRRTfdotinvplusdsbplusctrlisbN}{\usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbM}}
\addtolength{\WRCdotRRTfdotinvplusdsbplusctrlisbH}{\WRCdotRRTfdotinvplusdsbplusctrlisbN}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusctrlisbO}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusctrlisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusctrlisbP}
\settowidth{\WRCdotRRTfdotinvplusdsbplusctrlisbP}{\usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbO}}
\addtolength{\WRCdotRRTfdotinvplusdsbplusctrlisbH}{\WRCdotRRTfdotinvplusdsbplusctrlisbP}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusctrlisbA}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusctrlisbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusctrlisbB}
\settowidth{\WRCdotRRTfdotinvplusdsbplusctrlisbB}{\usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbA}}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusctrlisbC}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusctrlisbC}
\begin{minipage}{\WRCdotRRTfdotinvplusdsbplusctrlisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.RRTf.inv+dsb+ctrl-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotRRTfdotinvplusdsbplusctrlisbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbM}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=desc3(z,page_table_base) & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/WRC.RRTf.inv+dsb+dsb-isb.tex <==
\newlength{\WRCdotRRTfdotinvplusdsbplusdsbisbH}
\setlength{\WRCdotRRTfdotinvplusdsbplusdsbisbH}{0cm}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusdsbisbI}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusdsbisbJ}
\settowidth{\WRCdotRRTfdotinvplusdsbplusdsbisbJ}{\usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbI}}
\addtolength{\WRCdotRRTfdotinvplusdsbplusdsbisbH}{\WRCdotRRTfdotinvplusdsbplusdsbisbJ}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusdsbisbK}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusdsbisbL}
\settowidth{\WRCdotRRTfdotinvplusdsbplusdsbisbL}{\usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbK}}
\addtolength{\WRCdotRRTfdotinvplusdsbplusdsbisbH}{\WRCdotRRTfdotinvplusdsbplusdsbisbL}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusdsbisbM}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusdsbisbN}
\settowidth{\WRCdotRRTfdotinvplusdsbplusdsbisbN}{\usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbM}}
\addtolength{\WRCdotRRTfdotinvplusdsbplusdsbisbH}{\WRCdotRRTfdotinvplusdsbplusdsbisbN}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusdsbisbO}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusdsbisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusdsbisbP}
\settowidth{\WRCdotRRTfdotinvplusdsbplusdsbisbP}{\usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbO}}
\addtolength{\WRCdotRRTfdotinvplusdsbplusdsbisbH}{\WRCdotRRTfdotinvplusdsbplusdsbisbP}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusdsbisbA}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusdsbisbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusdsbisbB}
\settowidth{\WRCdotRRTfdotinvplusdsbplusdsbisbB}{\usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbA}}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusdsbisbC}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusdsbisbC}
\begin{minipage}{\WRCdotRRTfdotinvplusdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.RRTf.inv+dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotRRTfdotinvplusdsbplusdsbisbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbM}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=desc3(z,page_table_base) & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/WRC.RRTf.inv+dsbs.tex <==
\newlength{\WRCdotRRTfdotinvplusdsbsH}
\setlength{\WRCdotRRTfdotinvplusdsbsH}{0cm}
\newsavebox{\WRCdotRRTfdotinvplusdsbsI}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbsJ}
\settowidth{\WRCdotRRTfdotinvplusdsbsJ}{\usebox{\WRCdotRRTfdotinvplusdsbsI}}
\addtolength{\WRCdotRRTfdotinvplusdsbsH}{\WRCdotRRTfdotinvplusdsbsJ}
\newsavebox{\WRCdotRRTfdotinvplusdsbsK}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbsL}
\settowidth{\WRCdotRRTfdotinvplusdsbsL}{\usebox{\WRCdotRRTfdotinvplusdsbsK}}
\addtolength{\WRCdotRRTfdotinvplusdsbsH}{\WRCdotRRTfdotinvplusdsbsL}
\newsavebox{\WRCdotRRTfdotinvplusdsbsM}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbsN}
\settowidth{\WRCdotRRTfdotinvplusdsbsN}{\usebox{\WRCdotRRTfdotinvplusdsbsM}}
\addtolength{\WRCdotRRTfdotinvplusdsbsH}{\WRCdotRRTfdotinvplusdsbsN}
\newsavebox{\WRCdotRRTfdotinvplusdsbsO}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbsP}
\settowidth{\WRCdotRRTfdotinvplusdsbsP}{\usebox{\WRCdotRRTfdotinvplusdsbsO}}
\addtolength{\WRCdotRRTfdotinvplusdsbsH}{\WRCdotRRTfdotinvplusdsbsP}
\newsavebox{\WRCdotRRTfdotinvplusdsbsA}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbsA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbsB}
\settowidth{\WRCdotRRTfdotinvplusdsbsB}{\usebox{\WRCdotRRTfdotinvplusdsbsA}}
\newsavebox{\WRCdotRRTfdotinvplusdsbsC}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbsC}
\begin{minipage}{\WRCdotRRTfdotinvplusdsbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.RRTf.inv+dsbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotRRTfdotinvplusdsbsB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotRRTfdotinvplusdsbsA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotRRTfdotinvplusdsbsC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbsM}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbsO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=desc3(z,page_table_base) & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/WRC.RRTf.inv+pos.tex <==
\newlength{\WRCdotRRTfdotinvplusposH}
\setlength{\WRCdotRRTfdotinvplusposH}{0cm}
\newsavebox{\WRCdotRRTfdotinvplusposI}
\begin{lrbox}{\WRCdotRRTfdotinvplusposI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusposJ}
\settowidth{\WRCdotRRTfdotinvplusposJ}{\usebox{\WRCdotRRTfdotinvplusposI}}
\addtolength{\WRCdotRRTfdotinvplusposH}{\WRCdotRRTfdotinvplusposJ}
\newsavebox{\WRCdotRRTfdotinvplusposK}
\begin{lrbox}{\WRCdotRRTfdotinvplusposK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusposL}
\settowidth{\WRCdotRRTfdotinvplusposL}{\usebox{\WRCdotRRTfdotinvplusposK}}
\addtolength{\WRCdotRRTfdotinvplusposH}{\WRCdotRRTfdotinvplusposL}
\newsavebox{\WRCdotRRTfdotinvplusposM}
\begin{lrbox}{\WRCdotRRTfdotinvplusposM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusposN}
\settowidth{\WRCdotRRTfdotinvplusposN}{\usebox{\WRCdotRRTfdotinvplusposM}}
\addtolength{\WRCdotRRTfdotinvplusposH}{\WRCdotRRTfdotinvplusposN}
\newsavebox{\WRCdotRRTfdotinvplusposO}
\begin{lrbox}{\WRCdotRRTfdotinvplusposO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusposP}
\settowidth{\WRCdotRRTfdotinvplusposP}{\usebox{\WRCdotRRTfdotinvplusposO}}
\addtolength{\WRCdotRRTfdotinvplusposH}{\WRCdotRRTfdotinvplusposP}
\newsavebox{\WRCdotRRTfdotinvplusposA}
\begin{lrbox}{\WRCdotRRTfdotinvplusposA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusposB}
\settowidth{\WRCdotRRTfdotinvplusposB}{\usebox{\WRCdotRRTfdotinvplusposA}}
\newsavebox{\WRCdotRRTfdotinvplusposC}
\begin{lrbox}{\WRCdotRRTfdotinvplusposC}
\begin{minipage}{\WRCdotRRTfdotinvplusposH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.RRTf.inv+pos|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotRRTfdotinvplusposB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotRRTfdotinvplusposA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotRRTfdotinvplusposC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusposI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusposK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusposM}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusposO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=desc3(z,page_table_base) & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/WRC.TRTf.inv+addrs.tex <==
\newlength{\WRCdotTRTfdotinvplusaddrsH}
\setlength{\WRCdotTRTfdotinvplusaddrsH}{0cm}
\newsavebox{\WRCdotTRTfdotinvplusaddrsI}
\begin{lrbox}{\WRCdotTRTfdotinvplusaddrsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusaddrsJ}
\settowidth{\WRCdotTRTfdotinvplusaddrsJ}{\usebox{\WRCdotTRTfdotinvplusaddrsI}}
\addtolength{\WRCdotTRTfdotinvplusaddrsH}{\WRCdotTRTfdotinvplusaddrsJ}
\newsavebox{\WRCdotTRTfdotinvplusaddrsK}
\begin{lrbox}{\WRCdotTRTfdotinvplusaddrsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
STR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusaddrsL}
\settowidth{\WRCdotTRTfdotinvplusaddrsL}{\usebox{\WRCdotTRTfdotinvplusaddrsK}}
\addtolength{\WRCdotTRTfdotinvplusaddrsH}{\WRCdotTRTfdotinvplusaddrsL}
\newsavebox{\WRCdotTRTfdotinvplusaddrsM}
\begin{lrbox}{\WRCdotTRTfdotinvplusaddrsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusaddrsN}
\settowidth{\WRCdotTRTfdotinvplusaddrsN}{\usebox{\WRCdotTRTfdotinvplusaddrsM}}
\addtolength{\WRCdotTRTfdotinvplusaddrsH}{\WRCdotTRTfdotinvplusaddrsN}
\newsavebox{\WRCdotTRTfdotinvplusaddrsO}
\begin{lrbox}{\WRCdotTRTfdotinvplusaddrsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusaddrsP}
\settowidth{\WRCdotTRTfdotinvplusaddrsP}{\usebox{\WRCdotTRTfdotinvplusaddrsO}}
\addtolength{\WRCdotTRTfdotinvplusaddrsH}{\WRCdotTRTfdotinvplusaddrsP}
\newsavebox{\WRCdotTRTfdotinvplusaddrsA}
\begin{lrbox}{\WRCdotTRTfdotinvplusaddrsA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusaddrsB}
\settowidth{\WRCdotTRTfdotinvplusaddrsB}{\usebox{\WRCdotTRTfdotinvplusaddrsA}}
\addtolength{\WRCdotTRTfdotinvplusaddrsH}{\WRCdotTRTfdotinvplusaddrsB}
\newsavebox{\WRCdotTRTfdotinvplusaddrsC}
\begin{lrbox}{\WRCdotTRTfdotinvplusaddrsC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusaddrsD}
\settowidth{\WRCdotTRTfdotinvplusaddrsD}{\usebox{\WRCdotTRTfdotinvplusaddrsC}}
\newsavebox{\WRCdotTRTfdotinvplusaddrsE}
\begin{lrbox}{\WRCdotTRTfdotinvplusaddrsE}
\begin{minipage}{\WRCdotTRTfdotinvplusaddrsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TRTf.inv+addrs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTRTfdotinvplusaddrsD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTRTfdotinvplusaddrsC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTRTfdotinvplusaddrsE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusaddrsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusaddrsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusaddrsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusaddrsO}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusaddrsA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/WRC.TRTf.inv+dmbs.tex <==
\newlength{\WRCdotTRTfdotinvplusdmbsH}
\setlength{\WRCdotTRTfdotinvplusdmbsH}{0cm}
\newsavebox{\WRCdotTRTfdotinvplusdmbsI}
\begin{lrbox}{\WRCdotTRTfdotinvplusdmbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdmbsJ}
\settowidth{\WRCdotTRTfdotinvplusdmbsJ}{\usebox{\WRCdotTRTfdotinvplusdmbsI}}
\addtolength{\WRCdotTRTfdotinvplusdmbsH}{\WRCdotTRTfdotinvplusdmbsJ}
\newsavebox{\WRCdotTRTfdotinvplusdmbsK}
\begin{lrbox}{\WRCdotTRTfdotinvplusdmbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdmbsL}
\settowidth{\WRCdotTRTfdotinvplusdmbsL}{\usebox{\WRCdotTRTfdotinvplusdmbsK}}
\addtolength{\WRCdotTRTfdotinvplusdmbsH}{\WRCdotTRTfdotinvplusdmbsL}
\newsavebox{\WRCdotTRTfdotinvplusdmbsM}
\begin{lrbox}{\WRCdotTRTfdotinvplusdmbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdmbsN}
\settowidth{\WRCdotTRTfdotinvplusdmbsN}{\usebox{\WRCdotTRTfdotinvplusdmbsM}}
\addtolength{\WRCdotTRTfdotinvplusdmbsH}{\WRCdotTRTfdotinvplusdmbsN}
\newsavebox{\WRCdotTRTfdotinvplusdmbsO}
\begin{lrbox}{\WRCdotTRTfdotinvplusdmbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdmbsP}
\settowidth{\WRCdotTRTfdotinvplusdmbsP}{\usebox{\WRCdotTRTfdotinvplusdmbsO}}
\addtolength{\WRCdotTRTfdotinvplusdmbsH}{\WRCdotTRTfdotinvplusdmbsP}
\newsavebox{\WRCdotTRTfdotinvplusdmbsA}
\begin{lrbox}{\WRCdotTRTfdotinvplusdmbsA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdmbsB}
\settowidth{\WRCdotTRTfdotinvplusdmbsB}{\usebox{\WRCdotTRTfdotinvplusdmbsA}}
\addtolength{\WRCdotTRTfdotinvplusdmbsH}{\WRCdotTRTfdotinvplusdmbsB}
\newsavebox{\WRCdotTRTfdotinvplusdmbsC}
\begin{lrbox}{\WRCdotTRTfdotinvplusdmbsC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdmbsD}
\settowidth{\WRCdotTRTfdotinvplusdmbsD}{\usebox{\WRCdotTRTfdotinvplusdmbsC}}
\newsavebox{\WRCdotTRTfdotinvplusdmbsE}
\begin{lrbox}{\WRCdotTRTfdotinvplusdmbsE}
\begin{minipage}{\WRCdotTRTfdotinvplusdmbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TRTf.inv+dmbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTRTfdotinvplusdmbsD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTRTfdotinvplusdmbsC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTRTfdotinvplusdmbsE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdmbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdmbsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdmbsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdmbsO}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdmbsA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/WRC.TRTf.inv+dsb+dsb-isb.tex <==
\newlength{\WRCdotTRTfdotinvplusdsbplusdsbisbH}
\setlength{\WRCdotTRTfdotinvplusdsbplusdsbisbH}{0cm}
\newsavebox{\WRCdotTRTfdotinvplusdsbplusdsbisbI}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbplusdsbisbJ}
\settowidth{\WRCdotTRTfdotinvplusdsbplusdsbisbJ}{\usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbI}}
\addtolength{\WRCdotTRTfdotinvplusdsbplusdsbisbH}{\WRCdotTRTfdotinvplusdsbplusdsbisbJ}
\newsavebox{\WRCdotTRTfdotinvplusdsbplusdsbisbK}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbplusdsbisbL}
\settowidth{\WRCdotTRTfdotinvplusdsbplusdsbisbL}{\usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbK}}
\addtolength{\WRCdotTRTfdotinvplusdsbplusdsbisbH}{\WRCdotTRTfdotinvplusdsbplusdsbisbL}
\newsavebox{\WRCdotTRTfdotinvplusdsbplusdsbisbM}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbplusdsbisbN}
\settowidth{\WRCdotTRTfdotinvplusdsbplusdsbisbN}{\usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbM}}
\addtolength{\WRCdotTRTfdotinvplusdsbplusdsbisbH}{\WRCdotTRTfdotinvplusdsbplusdsbisbN}
\newsavebox{\WRCdotTRTfdotinvplusdsbplusdsbisbO}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbplusdsbisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbplusdsbisbP}
\settowidth{\WRCdotTRTfdotinvplusdsbplusdsbisbP}{\usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbO}}
\addtolength{\WRCdotTRTfdotinvplusdsbplusdsbisbH}{\WRCdotTRTfdotinvplusdsbplusdsbisbP}
\newsavebox{\WRCdotTRTfdotinvplusdsbplusdsbisbA}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbplusdsbisbA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbplusdsbisbB}
\settowidth{\WRCdotTRTfdotinvplusdsbplusdsbisbB}{\usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbA}}
\addtolength{\WRCdotTRTfdotinvplusdsbplusdsbisbH}{\WRCdotTRTfdotinvplusdsbplusdsbisbB}
\newsavebox{\WRCdotTRTfdotinvplusdsbplusdsbisbC}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbplusdsbisbC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbplusdsbisbD}
\settowidth{\WRCdotTRTfdotinvplusdsbplusdsbisbD}{\usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbC}}
\newsavebox{\WRCdotTRTfdotinvplusdsbplusdsbisbE}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbplusdsbisbE}
\begin{minipage}{\WRCdotTRTfdotinvplusdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TRTf.inv+dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTRTfdotinvplusdsbplusdsbisbD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbO}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/WRC.TRTf.inv+dsbs.tex <==
\newlength{\WRCdotTRTfdotinvplusdsbsH}
\setlength{\WRCdotTRTfdotinvplusdsbsH}{0cm}
\newsavebox{\WRCdotTRTfdotinvplusdsbsI}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbsJ}
\settowidth{\WRCdotTRTfdotinvplusdsbsJ}{\usebox{\WRCdotTRTfdotinvplusdsbsI}}
\addtolength{\WRCdotTRTfdotinvplusdsbsH}{\WRCdotTRTfdotinvplusdsbsJ}
\newsavebox{\WRCdotTRTfdotinvplusdsbsK}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbsL}
\settowidth{\WRCdotTRTfdotinvplusdsbsL}{\usebox{\WRCdotTRTfdotinvplusdsbsK}}
\addtolength{\WRCdotTRTfdotinvplusdsbsH}{\WRCdotTRTfdotinvplusdsbsL}
\newsavebox{\WRCdotTRTfdotinvplusdsbsM}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbsN}
\settowidth{\WRCdotTRTfdotinvplusdsbsN}{\usebox{\WRCdotTRTfdotinvplusdsbsM}}
\addtolength{\WRCdotTRTfdotinvplusdsbsH}{\WRCdotTRTfdotinvplusdsbsN}
\newsavebox{\WRCdotTRTfdotinvplusdsbsO}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbsP}
\settowidth{\WRCdotTRTfdotinvplusdsbsP}{\usebox{\WRCdotTRTfdotinvplusdsbsO}}
\addtolength{\WRCdotTRTfdotinvplusdsbsH}{\WRCdotTRTfdotinvplusdsbsP}
\newsavebox{\WRCdotTRTfdotinvplusdsbsA}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbsA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbsB}
\settowidth{\WRCdotTRTfdotinvplusdsbsB}{\usebox{\WRCdotTRTfdotinvplusdsbsA}}
\addtolength{\WRCdotTRTfdotinvplusdsbsH}{\WRCdotTRTfdotinvplusdsbsB}
\newsavebox{\WRCdotTRTfdotinvplusdsbsC}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbsC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbsD}
\settowidth{\WRCdotTRTfdotinvplusdsbsD}{\usebox{\WRCdotTRTfdotinvplusdsbsC}}
\newsavebox{\WRCdotTRTfdotinvplusdsbsE}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbsE}
\begin{minipage}{\WRCdotTRTfdotinvplusdsbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TRTf.inv+dsbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTRTfdotinvplusdsbsD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTRTfdotinvplusdsbsC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTRTfdotinvplusdsbsE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbsO}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbsA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/WRC.TRTf.inv+pos.tex <==
\newlength{\WRCdotTRTfdotinvplusposH}
\setlength{\WRCdotTRTfdotinvplusposH}{0cm}
\newsavebox{\WRCdotTRTfdotinvplusposI}
\begin{lrbox}{\WRCdotTRTfdotinvplusposI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusposJ}
\settowidth{\WRCdotTRTfdotinvplusposJ}{\usebox{\WRCdotTRTfdotinvplusposI}}
\addtolength{\WRCdotTRTfdotinvplusposH}{\WRCdotTRTfdotinvplusposJ}
\newsavebox{\WRCdotTRTfdotinvplusposK}
\begin{lrbox}{\WRCdotTRTfdotinvplusposK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusposL}
\settowidth{\WRCdotTRTfdotinvplusposL}{\usebox{\WRCdotTRTfdotinvplusposK}}
\addtolength{\WRCdotTRTfdotinvplusposH}{\WRCdotTRTfdotinvplusposL}
\newsavebox{\WRCdotTRTfdotinvplusposM}
\begin{lrbox}{\WRCdotTRTfdotinvplusposM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusposN}
\settowidth{\WRCdotTRTfdotinvplusposN}{\usebox{\WRCdotTRTfdotinvplusposM}}
\addtolength{\WRCdotTRTfdotinvplusposH}{\WRCdotTRTfdotinvplusposN}
\newsavebox{\WRCdotTRTfdotinvplusposO}
\begin{lrbox}{\WRCdotTRTfdotinvplusposO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusposP}
\settowidth{\WRCdotTRTfdotinvplusposP}{\usebox{\WRCdotTRTfdotinvplusposO}}
\addtolength{\WRCdotTRTfdotinvplusposH}{\WRCdotTRTfdotinvplusposP}
\newsavebox{\WRCdotTRTfdotinvplusposA}
\begin{lrbox}{\WRCdotTRTfdotinvplusposA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusposB}
\settowidth{\WRCdotTRTfdotinvplusposB}{\usebox{\WRCdotTRTfdotinvplusposA}}
\addtolength{\WRCdotTRTfdotinvplusposH}{\WRCdotTRTfdotinvplusposB}
\newsavebox{\WRCdotTRTfdotinvplusposC}
\begin{lrbox}{\WRCdotTRTfdotinvplusposC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusposD}
\settowidth{\WRCdotTRTfdotinvplusposD}{\usebox{\WRCdotTRTfdotinvplusposC}}
\newsavebox{\WRCdotTRTfdotinvplusposE}
\begin{lrbox}{\WRCdotTRTfdotinvplusposE}
\begin{minipage}{\WRCdotTRTfdotinvplusposH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TRTf.inv+pos|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTRTfdotinvplusposD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTRTfdotinvplusposC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTRTfdotinvplusposE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusposI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusposK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusposM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusposO}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusposA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/WRC.TTTf.inv+addrs.tex <==
\newlength{\WRCdotTTTfdotinvplusaddrsH}
\setlength{\WRCdotTTTfdotinvplusaddrsH}{0cm}
\newsavebox{\WRCdotTTTfdotinvplusaddrsI}
\begin{lrbox}{\WRCdotTTTfdotinvplusaddrsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusaddrsJ}
\settowidth{\WRCdotTTTfdotinvplusaddrsJ}{\usebox{\WRCdotTTTfdotinvplusaddrsI}}
\addtolength{\WRCdotTTTfdotinvplusaddrsH}{\WRCdotTTTfdotinvplusaddrsJ}
\newsavebox{\WRCdotTTTfdotinvplusaddrsK}
\begin{lrbox}{\WRCdotTTTfdotinvplusaddrsK}
\begin{lstlisting}[language=AArch64,showlines=true]
MOV X0,#0
LDR X0,[X1]
EOR X4,X0,X0
STR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusaddrsL}
\settowidth{\WRCdotTTTfdotinvplusaddrsL}{\usebox{\WRCdotTTTfdotinvplusaddrsK}}
\addtolength{\WRCdotTTTfdotinvplusaddrsH}{\WRCdotTTTfdotinvplusaddrsL}
\newsavebox{\WRCdotTTTfdotinvplusaddrsM}
\begin{lrbox}{\WRCdotTTTfdotinvplusaddrsM}
\begin{lstlisting}[language=AArch64,showlines=true]
MOV X0,#0
LDR X0,[X1]
EOR X4,X0,X0
MOV X2,#0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusaddrsN}
\settowidth{\WRCdotTTTfdotinvplusaddrsN}{\usebox{\WRCdotTTTfdotinvplusaddrsM}}
\addtolength{\WRCdotTTTfdotinvplusaddrsH}{\WRCdotTTTfdotinvplusaddrsN}
\newsavebox{\WRCdotTTTfdotinvplusaddrsO}
\begin{lrbox}{\WRCdotTTTfdotinvplusaddrsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusaddrsP}
\settowidth{\WRCdotTTTfdotinvplusaddrsP}{\usebox{\WRCdotTTTfdotinvplusaddrsO}}
\addtolength{\WRCdotTTTfdotinvplusaddrsH}{\WRCdotTTTfdotinvplusaddrsP}
\newsavebox{\WRCdotTTTfdotinvplusaddrsA}
\begin{lrbox}{\WRCdotTTTfdotinvplusaddrsA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusaddrsB}
\settowidth{\WRCdotTTTfdotinvplusaddrsB}{\usebox{\WRCdotTTTfdotinvplusaddrsA}}
\addtolength{\WRCdotTTTfdotinvplusaddrsH}{\WRCdotTTTfdotinvplusaddrsB}
\newsavebox{\WRCdotTTTfdotinvplusaddrsC}
\begin{lrbox}{\WRCdotTTTfdotinvplusaddrsC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusaddrsD}
\settowidth{\WRCdotTTTfdotinvplusaddrsD}{\usebox{\WRCdotTTTfdotinvplusaddrsC}}
\newsavebox{\WRCdotTTTfdotinvplusaddrsE}
\begin{lrbox}{\WRCdotTTTfdotinvplusaddrsE}
\begin{minipage}{\WRCdotTTTfdotinvplusaddrsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:__isla_monomorphize_writes=true|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TTTf.inv+addrs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTTTfdotinvplusaddrsD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTTTfdotinvplusaddrsC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTTTfdotinvplusaddrsE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusaddrsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusaddrsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusaddrsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusaddrsO}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusaddrsA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/WRC.TTTf.inv+data+addr.tex <==
\newlength{\WRCdotTTTfdotinvplusdataplusaddrH}
\setlength{\WRCdotTTTfdotinvplusdataplusaddrH}{0cm}
\newsavebox{\WRCdotTTTfdotinvplusdataplusaddrI}
\begin{lrbox}{\WRCdotTTTfdotinvplusdataplusaddrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusdataplusaddrJ}
\settowidth{\WRCdotTTTfdotinvplusdataplusaddrJ}{\usebox{\WRCdotTTTfdotinvplusdataplusaddrI}}
\addtolength{\WRCdotTTTfdotinvplusdataplusaddrH}{\WRCdotTTTfdotinvplusdataplusaddrJ}
\newsavebox{\WRCdotTTTfdotinvplusdataplusaddrK}
\begin{lrbox}{\WRCdotTTTfdotinvplusdataplusaddrK}
\begin{lstlisting}[language=AArch64,showlines=true]
MOV X0,#0
LDR X0,[X1]
EOR X4,X0,X0
ORR X2,X2,X4
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusdataplusaddrL}
\settowidth{\WRCdotTTTfdotinvplusdataplusaddrL}{\usebox{\WRCdotTTTfdotinvplusdataplusaddrK}}
\addtolength{\WRCdotTTTfdotinvplusdataplusaddrH}{\WRCdotTTTfdotinvplusdataplusaddrL}
\newsavebox{\WRCdotTTTfdotinvplusdataplusaddrM}
\begin{lrbox}{\WRCdotTTTfdotinvplusdataplusaddrM}
\begin{lstlisting}[language=AArch64,showlines=true]
MOV X0,#0
LDR X0,[X1]
EOR X4,X0,X0
MOV X2,#0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusdataplusaddrN}
\settowidth{\WRCdotTTTfdotinvplusdataplusaddrN}{\usebox{\WRCdotTTTfdotinvplusdataplusaddrM}}
\addtolength{\WRCdotTTTfdotinvplusdataplusaddrH}{\WRCdotTTTfdotinvplusdataplusaddrN}
\newsavebox{\WRCdotTTTfdotinvplusdataplusaddrO}
\begin{lrbox}{\WRCdotTTTfdotinvplusdataplusaddrO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusdataplusaddrP}
\settowidth{\WRCdotTTTfdotinvplusdataplusaddrP}{\usebox{\WRCdotTTTfdotinvplusdataplusaddrO}}
\addtolength{\WRCdotTTTfdotinvplusdataplusaddrH}{\WRCdotTTTfdotinvplusdataplusaddrP}
\newsavebox{\WRCdotTTTfdotinvplusdataplusaddrA}
\begin{lrbox}{\WRCdotTTTfdotinvplusdataplusaddrA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusdataplusaddrB}
\settowidth{\WRCdotTTTfdotinvplusdataplusaddrB}{\usebox{\WRCdotTTTfdotinvplusdataplusaddrA}}
\addtolength{\WRCdotTTTfdotinvplusdataplusaddrH}{\WRCdotTTTfdotinvplusdataplusaddrB}
\newsavebox{\WRCdotTTTfdotinvplusdataplusaddrC}
\begin{lrbox}{\WRCdotTTTfdotinvplusdataplusaddrC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusdataplusaddrD}
\settowidth{\WRCdotTTTfdotinvplusdataplusaddrD}{\usebox{\WRCdotTTTfdotinvplusdataplusaddrC}}
\newsavebox{\WRCdotTTTfdotinvplusdataplusaddrE}
\begin{lrbox}{\WRCdotTTTfdotinvplusdataplusaddrE}
\begin{minipage}{\WRCdotTTTfdotinvplusdataplusaddrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:__isla_monomorphize_writes=true|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TTTf.inv+data+addr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTTTfdotinvplusdataplusaddrD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTTTfdotinvplusdataplusaddrC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTTTfdotinvplusdataplusaddrE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusdataplusaddrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusdataplusaddrK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusdataplusaddrM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusdataplusaddrO}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusdataplusaddrA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/WRC.TfRR+ctrl-isb+dsb.tex <==
\newlength{\WRCdotTfRRplusctrlisbplusdsbH}
\setlength{\WRCdotTfRRplusctrlisbplusdsbH}{0cm}
\newsavebox{\WRCdotTfRRplusctrlisbplusdsbI}
\begin{lrbox}{\WRCdotTfRRplusctrlisbplusdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusctrlisbplusdsbJ}
\settowidth{\WRCdotTfRRplusctrlisbplusdsbJ}{\usebox{\WRCdotTfRRplusctrlisbplusdsbI}}
\addtolength{\WRCdotTfRRplusctrlisbplusdsbH}{\WRCdotTfRRplusctrlisbplusdsbJ}
\newsavebox{\WRCdotTfRRplusctrlisbplusdsbK}
\begin{lrbox}{\WRCdotTfRRplusctrlisbplusdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBNZ X0,L0
L0:
ISB
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusctrlisbplusdsbL}
\settowidth{\WRCdotTfRRplusctrlisbplusdsbL}{\usebox{\WRCdotTfRRplusctrlisbplusdsbK}}
\addtolength{\WRCdotTfRRplusctrlisbplusdsbH}{\WRCdotTfRRplusctrlisbplusdsbL}
\newsavebox{\WRCdotTfRRplusctrlisbplusdsbM}
\begin{lrbox}{\WRCdotTfRRplusctrlisbplusdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusctrlisbplusdsbN}
\settowidth{\WRCdotTfRRplusctrlisbplusdsbN}{\usebox{\WRCdotTfRRplusctrlisbplusdsbM}}
\addtolength{\WRCdotTfRRplusctrlisbplusdsbH}{\WRCdotTfRRplusctrlisbplusdsbN}
\newsavebox{\WRCdotTfRRplusctrlisbplusdsbO}
\begin{lrbox}{\WRCdotTfRRplusctrlisbplusdsbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusctrlisbplusdsbP}
\settowidth{\WRCdotTfRRplusctrlisbplusdsbP}{\usebox{\WRCdotTfRRplusctrlisbplusdsbO}}
\addtolength{\WRCdotTfRRplusctrlisbplusdsbH}{\WRCdotTfRRplusctrlisbplusdsbP}
\newsavebox{\WRCdotTfRRplusctrlisbplusdsbA}
\begin{lrbox}{\WRCdotTfRRplusctrlisbplusdsbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    *pa1 = 0;

    y |-> pa2;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusctrlisbplusdsbB}
\settowidth{\WRCdotTfRRplusctrlisbplusdsbB}{\usebox{\WRCdotTfRRplusctrlisbplusdsbA}}
\newsavebox{\WRCdotTfRRplusctrlisbplusdsbC}
\begin{lrbox}{\WRCdotTfRRplusctrlisbplusdsbC}
\begin{minipage}{\WRCdotTfRRplusctrlisbplusdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TfRR+ctrl-isb+dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTfRRplusctrlisbplusdsbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTfRRplusctrlisbplusdsbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTfRRplusctrlisbplusdsbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusctrlisbplusdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusctrlisbplusdsbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusctrlisbplusdsbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusctrlisbplusdsbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & ~2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/WRC.TfRR+dmbs.tex <==
\newlength{\WRCdotTfRRplusdmbsH}
\setlength{\WRCdotTfRRplusdmbsH}{0cm}
\newsavebox{\WRCdotTfRRplusdmbsI}
\begin{lrbox}{\WRCdotTfRRplusdmbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdmbsJ}
\settowidth{\WRCdotTfRRplusdmbsJ}{\usebox{\WRCdotTfRRplusdmbsI}}
\addtolength{\WRCdotTfRRplusdmbsH}{\WRCdotTfRRplusdmbsJ}
\newsavebox{\WRCdotTfRRplusdmbsK}
\begin{lrbox}{\WRCdotTfRRplusdmbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdmbsL}
\settowidth{\WRCdotTfRRplusdmbsL}{\usebox{\WRCdotTfRRplusdmbsK}}
\addtolength{\WRCdotTfRRplusdmbsH}{\WRCdotTfRRplusdmbsL}
\newsavebox{\WRCdotTfRRplusdmbsM}
\begin{lrbox}{\WRCdotTfRRplusdmbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdmbsN}
\settowidth{\WRCdotTfRRplusdmbsN}{\usebox{\WRCdotTfRRplusdmbsM}}
\addtolength{\WRCdotTfRRplusdmbsH}{\WRCdotTfRRplusdmbsN}
\newsavebox{\WRCdotTfRRplusdmbsO}
\begin{lrbox}{\WRCdotTfRRplusdmbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdmbsP}
\settowidth{\WRCdotTfRRplusdmbsP}{\usebox{\WRCdotTfRRplusdmbsO}}
\addtolength{\WRCdotTfRRplusdmbsH}{\WRCdotTfRRplusdmbsP}
\newsavebox{\WRCdotTfRRplusdmbsA}
\begin{lrbox}{\WRCdotTfRRplusdmbsA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    *pa1 = 0;

    y |-> pa2;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdmbsB}
\settowidth{\WRCdotTfRRplusdmbsB}{\usebox{\WRCdotTfRRplusdmbsA}}
\newsavebox{\WRCdotTfRRplusdmbsC}
\begin{lrbox}{\WRCdotTfRRplusdmbsC}
\begin{minipage}{\WRCdotTfRRplusdmbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TfRR+dmbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTfRRplusdmbsB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTfRRplusdmbsA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTfRRplusdmbsC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdmbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdmbsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdmbsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdmbsO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & ~2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/WRC.TfRR+dsb-isb+dsb.tex <==
\newlength{\WRCdotTfRRplusdsbisbplusdsbH}
\setlength{\WRCdotTfRRplusdsbisbplusdsbH}{0cm}
\newsavebox{\WRCdotTfRRplusdsbisbplusdsbI}
\begin{lrbox}{\WRCdotTfRRplusdsbisbplusdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbisbplusdsbJ}
\settowidth{\WRCdotTfRRplusdsbisbplusdsbJ}{\usebox{\WRCdotTfRRplusdsbisbplusdsbI}}
\addtolength{\WRCdotTfRRplusdsbisbplusdsbH}{\WRCdotTfRRplusdsbisbplusdsbJ}
\newsavebox{\WRCdotTfRRplusdsbisbplusdsbK}
\begin{lrbox}{\WRCdotTfRRplusdsbisbplusdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbisbplusdsbL}
\settowidth{\WRCdotTfRRplusdsbisbplusdsbL}{\usebox{\WRCdotTfRRplusdsbisbplusdsbK}}
\addtolength{\WRCdotTfRRplusdsbisbplusdsbH}{\WRCdotTfRRplusdsbisbplusdsbL}
\newsavebox{\WRCdotTfRRplusdsbisbplusdsbM}
\begin{lrbox}{\WRCdotTfRRplusdsbisbplusdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbisbplusdsbN}
\settowidth{\WRCdotTfRRplusdsbisbplusdsbN}{\usebox{\WRCdotTfRRplusdsbisbplusdsbM}}
\addtolength{\WRCdotTfRRplusdsbisbplusdsbH}{\WRCdotTfRRplusdsbisbplusdsbN}
\newsavebox{\WRCdotTfRRplusdsbisbplusdsbO}
\begin{lrbox}{\WRCdotTfRRplusdsbisbplusdsbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbisbplusdsbP}
\settowidth{\WRCdotTfRRplusdsbisbplusdsbP}{\usebox{\WRCdotTfRRplusdsbisbplusdsbO}}
\addtolength{\WRCdotTfRRplusdsbisbplusdsbH}{\WRCdotTfRRplusdsbisbplusdsbP}
\newsavebox{\WRCdotTfRRplusdsbisbplusdsbA}
\begin{lrbox}{\WRCdotTfRRplusdsbisbplusdsbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    *pa1 = 0;

    y |-> pa2;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbisbplusdsbB}
\settowidth{\WRCdotTfRRplusdsbisbplusdsbB}{\usebox{\WRCdotTfRRplusdsbisbplusdsbA}}
\newsavebox{\WRCdotTfRRplusdsbisbplusdsbC}
\begin{lrbox}{\WRCdotTfRRplusdsbisbplusdsbC}
\begin{minipage}{\WRCdotTfRRplusdsbisbplusdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TfRR+dsb-isb+dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTfRRplusdsbisbplusdsbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTfRRplusdsbisbplusdsbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTfRRplusdsbisbplusdsbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdsbisbplusdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdsbisbplusdsbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdsbisbplusdsbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdsbisbplusdsbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & ~2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/WRC.TfRR+dsbs.tex <==
\newlength{\WRCdotTfRRplusdsbsH}
\setlength{\WRCdotTfRRplusdsbsH}{0cm}
\newsavebox{\WRCdotTfRRplusdsbsI}
\begin{lrbox}{\WRCdotTfRRplusdsbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbsJ}
\settowidth{\WRCdotTfRRplusdsbsJ}{\usebox{\WRCdotTfRRplusdsbsI}}
\addtolength{\WRCdotTfRRplusdsbsH}{\WRCdotTfRRplusdsbsJ}
\newsavebox{\WRCdotTfRRplusdsbsK}
\begin{lrbox}{\WRCdotTfRRplusdsbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbsL}
\settowidth{\WRCdotTfRRplusdsbsL}{\usebox{\WRCdotTfRRplusdsbsK}}
\addtolength{\WRCdotTfRRplusdsbsH}{\WRCdotTfRRplusdsbsL}
\newsavebox{\WRCdotTfRRplusdsbsM}
\begin{lrbox}{\WRCdotTfRRplusdsbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbsN}
\settowidth{\WRCdotTfRRplusdsbsN}{\usebox{\WRCdotTfRRplusdsbsM}}
\addtolength{\WRCdotTfRRplusdsbsH}{\WRCdotTfRRplusdsbsN}
\newsavebox{\WRCdotTfRRplusdsbsO}
\begin{lrbox}{\WRCdotTfRRplusdsbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbsP}
\settowidth{\WRCdotTfRRplusdsbsP}{\usebox{\WRCdotTfRRplusdsbsO}}
\addtolength{\WRCdotTfRRplusdsbsH}{\WRCdotTfRRplusdsbsP}
\newsavebox{\WRCdotTfRRplusdsbsA}
\begin{lrbox}{\WRCdotTfRRplusdsbsA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    *pa1 = 0;

    y |-> pa2;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbsB}
\settowidth{\WRCdotTfRRplusdsbsB}{\usebox{\WRCdotTfRRplusdsbsA}}
\newsavebox{\WRCdotTfRRplusdsbsC}
\begin{lrbox}{\WRCdotTfRRplusdsbsC}
\begin{minipage}{\WRCdotTfRRplusdsbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TfRR+dsbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTfRRplusdsbsB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTfRRplusdsbsA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTfRRplusdsbsC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdsbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdsbsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdsbsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdsbsO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & ~2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/WRC.TfRR+po+dsb.tex <==
\newlength{\WRCdotTfRRpluspoplusdsbH}
\setlength{\WRCdotTfRRpluspoplusdsbH}{0cm}
\newsavebox{\WRCdotTfRRpluspoplusdsbI}
\begin{lrbox}{\WRCdotTfRRpluspoplusdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRpluspoplusdsbJ}
\settowidth{\WRCdotTfRRpluspoplusdsbJ}{\usebox{\WRCdotTfRRpluspoplusdsbI}}
\addtolength{\WRCdotTfRRpluspoplusdsbH}{\WRCdotTfRRpluspoplusdsbJ}
\newsavebox{\WRCdotTfRRpluspoplusdsbK}
\begin{lrbox}{\WRCdotTfRRpluspoplusdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRpluspoplusdsbL}
\settowidth{\WRCdotTfRRpluspoplusdsbL}{\usebox{\WRCdotTfRRpluspoplusdsbK}}
\addtolength{\WRCdotTfRRpluspoplusdsbH}{\WRCdotTfRRpluspoplusdsbL}
\newsavebox{\WRCdotTfRRpluspoplusdsbM}
\begin{lrbox}{\WRCdotTfRRpluspoplusdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRpluspoplusdsbN}
\settowidth{\WRCdotTfRRpluspoplusdsbN}{\usebox{\WRCdotTfRRpluspoplusdsbM}}
\addtolength{\WRCdotTfRRpluspoplusdsbH}{\WRCdotTfRRpluspoplusdsbN}
\newsavebox{\WRCdotTfRRpluspoplusdsbO}
\begin{lrbox}{\WRCdotTfRRpluspoplusdsbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRpluspoplusdsbP}
\settowidth{\WRCdotTfRRpluspoplusdsbP}{\usebox{\WRCdotTfRRpluspoplusdsbO}}
\addtolength{\WRCdotTfRRpluspoplusdsbH}{\WRCdotTfRRpluspoplusdsbP}
\newsavebox{\WRCdotTfRRpluspoplusdsbA}
\begin{lrbox}{\WRCdotTfRRpluspoplusdsbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    *pa1 = 0;

    y |-> pa2;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRpluspoplusdsbB}
\settowidth{\WRCdotTfRRpluspoplusdsbB}{\usebox{\WRCdotTfRRpluspoplusdsbA}}
\newsavebox{\WRCdotTfRRpluspoplusdsbC}
\begin{lrbox}{\WRCdotTfRRpluspoplusdsbC}
\begin{minipage}{\WRCdotTfRRpluspoplusdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TfRR+po+dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTfRRpluspoplusdsbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTfRRpluspoplusdsbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTfRRpluspoplusdsbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRpluspoplusdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRpluspoplusdsbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRpluspoplusdsbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRpluspoplusdsbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & ~2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/WRC.TfRR+pos.tex <==
\newlength{\WRCdotTfRRplusposH}
\setlength{\WRCdotTfRRplusposH}{0cm}
\newsavebox{\WRCdotTfRRplusposI}
\begin{lrbox}{\WRCdotTfRRplusposI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusposJ}
\settowidth{\WRCdotTfRRplusposJ}{\usebox{\WRCdotTfRRplusposI}}
\addtolength{\WRCdotTfRRplusposH}{\WRCdotTfRRplusposJ}
\newsavebox{\WRCdotTfRRplusposK}
\begin{lrbox}{\WRCdotTfRRplusposK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusposL}
\settowidth{\WRCdotTfRRplusposL}{\usebox{\WRCdotTfRRplusposK}}
\addtolength{\WRCdotTfRRplusposH}{\WRCdotTfRRplusposL}
\newsavebox{\WRCdotTfRRplusposM}
\begin{lrbox}{\WRCdotTfRRplusposM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusposN}
\settowidth{\WRCdotTfRRplusposN}{\usebox{\WRCdotTfRRplusposM}}
\addtolength{\WRCdotTfRRplusposH}{\WRCdotTfRRplusposN}
\newsavebox{\WRCdotTfRRplusposO}
\begin{lrbox}{\WRCdotTfRRplusposO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusposP}
\settowidth{\WRCdotTfRRplusposP}{\usebox{\WRCdotTfRRplusposO}}
\addtolength{\WRCdotTfRRplusposH}{\WRCdotTfRRplusposP}
\newsavebox{\WRCdotTfRRplusposA}
\begin{lrbox}{\WRCdotTfRRplusposA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    *pa1 = 0;

    y |-> pa2;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusposB}
\settowidth{\WRCdotTfRRplusposB}{\usebox{\WRCdotTfRRplusposA}}
\newsavebox{\WRCdotTfRRplusposC}
\begin{lrbox}{\WRCdotTfRRplusposC}
\begin{minipage}{\WRCdotTfRRplusposH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TfRR+pos|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTfRRplusposB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTfRRplusposA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTfRRplusposC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusposI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusposK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusposM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusposO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & ~2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/WRC.TfRT+dsb-tlbiis-dsb+dsb-isb.tex <==
\newlength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbH}
\setlength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbH}{0cm}
\newsavebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbI}
\begin{lrbox}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbJ}
\settowidth{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbJ}{\usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbI}}
\addtolength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbH}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbJ}
\newsavebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbK}
\begin{lrbox}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
// the TLBI is in the handler
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbL}
\settowidth{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbL}{\usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbK}}
\addtolength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbH}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbL}
\newsavebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbM}
\begin{lrbox}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbN}
\settowidth{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbN}{\usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbM}}
\addtolength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbH}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbN}
\newsavebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbO}
\begin{lrbox}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
DSB SY
TLBI VAE1IS,X4
DSB SY
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbP}
\settowidth{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbP}{\usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbO}}
\addtolength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbH}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbP}
\newsavebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbA}
\begin{lrbox}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbB}
\settowidth{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbB}{\usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbA}}
\addtolength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbH}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbB}
\newsavebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbC}
\begin{lrbox}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;

    x |-> pa1;
    x ?-> invalid;
    *pa1 = 1;

    y |-> pa2;
    *pa2 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbD}
\settowidth{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbD}{\usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbC}}
\newsavebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbE}
\begin{lrbox}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbE}
\begin{minipage}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TfRT+dsb-tlbiis-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbO}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=0 & 2:R0=1 & 2:R2=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/legion-refs/2022-01-13/latex/WRC.TfRT+po+dsb-isb.tex <==
\newlength{\WRCdotTfRTpluspoplusdsbisbH}
\setlength{\WRCdotTfRTpluspoplusdsbisbH}{0cm}
\newsavebox{\WRCdotTfRTpluspoplusdsbisbI}
\begin{lrbox}{\WRCdotTfRTpluspoplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTpluspoplusdsbisbJ}
\settowidth{\WRCdotTfRTpluspoplusdsbisbJ}{\usebox{\WRCdotTfRTpluspoplusdsbisbI}}
\addtolength{\WRCdotTfRTpluspoplusdsbisbH}{\WRCdotTfRTpluspoplusdsbisbJ}
\newsavebox{\WRCdotTfRTpluspoplusdsbisbK}
\begin{lrbox}{\WRCdotTfRTpluspoplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTpluspoplusdsbisbL}
\settowidth{\WRCdotTfRTpluspoplusdsbisbL}{\usebox{\WRCdotTfRTpluspoplusdsbisbK}}
\addtolength{\WRCdotTfRTpluspoplusdsbisbH}{\WRCdotTfRTpluspoplusdsbisbL}
\newsavebox{\WRCdotTfRTpluspoplusdsbisbM}
\begin{lrbox}{\WRCdotTfRTpluspoplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTpluspoplusdsbisbN}
\settowidth{\WRCdotTfRTpluspoplusdsbisbN}{\usebox{\WRCdotTfRTpluspoplusdsbisbM}}
\addtolength{\WRCdotTfRTpluspoplusdsbisbH}{\WRCdotTfRTpluspoplusdsbisbN}
\newsavebox{\WRCdotTfRTpluspoplusdsbisbO}
\begin{lrbox}{\WRCdotTfRTpluspoplusdsbisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTpluspoplusdsbisbP}
\settowidth{\WRCdotTfRTpluspoplusdsbisbP}{\usebox{\WRCdotTfRTpluspoplusdsbisbO}}
\addtolength{\WRCdotTfRTpluspoplusdsbisbH}{\WRCdotTfRTpluspoplusdsbisbP}
\newsavebox{\WRCdotTfRTpluspoplusdsbisbA}
\begin{lrbox}{\WRCdotTfRTpluspoplusdsbisbA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTpluspoplusdsbisbB}
\settowidth{\WRCdotTfRTpluspoplusdsbisbB}{\usebox{\WRCdotTfRTpluspoplusdsbisbA}}
\addtolength{\WRCdotTfRTpluspoplusdsbisbH}{\WRCdotTfRTpluspoplusdsbisbB}
\newsavebox{\WRCdotTfRTpluspoplusdsbisbC}
\begin{lrbox}{\WRCdotTfRTpluspoplusdsbisbC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;

    x |-> pa1;
    x ?-> invalid;
    *pa1 = 1;

    y |-> pa2;
    *pa2 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTpluspoplusdsbisbD}
\settowidth{\WRCdotTfRTpluspoplusdsbisbD}{\usebox{\WRCdotTfRTpluspoplusdsbisbC}}
\newsavebox{\WRCdotTfRTpluspoplusdsbisbE}
\begin{lrbox}{\WRCdotTfRTpluspoplusdsbisbE}
\begin{minipage}{\WRCdotTfRTpluspoplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TfRT+po+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTfRTpluspoplusdsbisbD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTfRTpluspoplusdsbisbC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTfRTpluspoplusdsbisbE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTpluspoplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTpluspoplusdsbisbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTpluspoplusdsbisbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTpluspoplusdsbisbO}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTpluspoplusdsbisbA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=0 & 2:R0=1 & 2:R2=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/model_results/pgtable_table.tex <==
&  \multicolumn{2}{c}{Strong model } & \multicolumn{2}{c}{Ets model } \\
Test Name & allow? & \hfill time \hfill & allow? & \hfill time \\
\TEST{BBM+dsb-tlbiis-dsb}\dotfill  & \hfill $\checkmark$ & \hfill 12702ms \hfill & $\checkmark$ & \hfill 19328ms \\
\TEST{BBM.Tf+dsb-tlbiis-dsb}\dotfill  & \hfill $\checkmark$ & \hfill 9196ms \hfill & $\checkmark$ & \hfill 13659ms \\
\TEST{Break2.news1}\dotfill  & \hfill $\times$ & \hfill 43306ms \hfill & $\times$ & \hfill 22677ms \\
\TEST{CoRR0.alias+po}\dotfill  & \hfill $\times$ & \hfill 2512ms \hfill & $\times$ & \hfill 1420ms \\
\TEST{CoRR2.alias+po}\dotfill  & \hfill $\times$ & \hfill 1934ms \hfill & $\times$ & \hfill 2260ms \\
\TEST{CoRT.inv+addr-trfi}\dotfill  & \hfill \textbf{\textcolor{red}{!}} & \hfill 1098ms \hfill & \textbf{\textcolor{red}{!}} & \hfill 4778ms \\
\TEST{CoRpteT+dsb}\dotfill  & \hfill $\checkmark$ & \hfill 5978ms \hfill & $\checkmark$ & \hfill 6586ms \\
\TEST{CoRpteT+dsb-isb}\dotfill  & \hfill $\checkmark$ & \hfill 7347ms \hfill & $\checkmark$ & \hfill 7604ms \\
\TEST{CoRpteT.EL1+dsb-tlbi-dsb}\dotfill  & \hfill $\checkmark$ & \hfill 10293ms \hfill & $\checkmark$ & \hfill 11815ms \\
\TEST{CoRpteT.EL1+dsb-tlbi-dsb-isb}\dotfill  & \hfill $\times$ & \hfill 53579ms \hfill & $\times$ & \hfill 28345ms \\
\TEST{CoRpteTf.inv+dsb}\dotfill  & \hfill $\checkmark$ & \hfill 5413ms \hfill & $\times$ & \hfill 2582ms \\
\TEST{CoRpteTf.inv+dsb-isb}\dotfill  & \hfill $\times$ & \hfill 3347ms \hfill & $\times$ & \hfill 3472ms \\
\TEST{CoTRpte.inv+dsb}\dotfill  & \hfill $\times$ & \hfill 5781ms \hfill & $\times$ & \hfill 5372ms \\
\TEST{CoTRpte.inv+dsb-isb}\dotfill  & \hfill $\times$ & \hfill 4436ms \hfill & $\times$ & \hfill 5367ms \\
\TEST{CoTRpte.inv+po}\dotfill  & \hfill $\checkmark$ & \hfill 7044ms \hfill & $\checkmark$ & \hfill 6839ms \\
\TEST{CoTT.ro+dmb}\dotfill  & \hfill $\checkmark$ & \hfill 36785ms \hfill & $\checkmark$ & \hfill 52018ms \\
\TEST{CoTT.ro+dsb-isb}\dotfill  & \hfill $\checkmark$ & \hfill 88419ms \hfill & $\checkmark$ & \hfill 103258ms \\
\TEST{CoTT.ro+po}\dotfill  & \hfill $\checkmark$ & \hfill 38533ms \hfill & $\checkmark$ & \hfill 38279ms \\
\TEST{CoTTf.inv+dsb-isb}\dotfill  & \hfill $\times$ & \hfill 21525ms \hfill & $\times$ & \hfill 26198ms \\
\TEST{CoTTf.inv+po}\dotfill  & \hfill $\checkmark$ & \hfill 51495ms \hfill & $\times$ & \hfill 29031ms \\
\TEST{CoTW1.inv}\dotfill  & \hfill $\times$ & \hfill 2597ms \hfill & $\times$ & \hfill 2714ms \\
\TEST{CoTWinv}\dotfill  & \hfill $\times$ & \hfill 2846ms \hfill & $\times$ & \hfill 3277ms \\
\TEST{CoTfRpte+dsb}\dotfill  & \hfill $\times$ & \hfill 4134ms \hfill & $\times$ & \hfill 4433ms \\
\TEST{CoTfRpte+dsb-isb}\dotfill  & \hfill $\times$ & \hfill 5543ms \hfill & $\times$ & \hfill 5852ms \\
\TEST{CoTfRpte+eret}\dotfill  & \hfill $\times$ & \hfill 2995ms \hfill & $\times$ & \hfill 4168ms \\
\TEST{CoTfRpte+po}\dotfill  & \hfill $\times$ & \hfill 3872ms \hfill & $\times$ & \hfill 3740ms \\
\TEST{CoTfT+dsb-isb}\dotfill  & \hfill $\checkmark$ & \hfill 78905ms \hfill & $\checkmark$ & \hfill 95644ms \\
\TEST{CoTfT+po}\dotfill  & \hfill $\checkmark$ & \hfill 71605ms \hfill & $\checkmark$ & \hfill 72598ms \\
\TEST{CoTfW.inv+dsb-isb}\dotfill  & \hfill $\times$ & \hfill 5572ms \hfill & $\times$ & \hfill 8392ms \\
\TEST{CoTfW.inv+po}\dotfill  & \hfill $\times$ & \hfill 6038ms \hfill & $\times$ & \hfill 7738ms \\
\TEST{CoTfW1.inv+si}\dotfill  & \hfill \textbf{\textcolor{red}{!}} & \hfill 220ms \hfill & \textbf{\textcolor{red}{!}} & \hfill 227ms \\
\TEST{CoWR.alias}\dotfill  & \hfill $\times$ & \hfill 977ms \hfill & $\times$ & \hfill 967ms \\
\TEST{CoWR.inv}\dotfill  & \hfill $\times$ & \hfill 825ms \hfill & $\times$ & \hfill 1104ms \\
\TEST{CoWTa1.1.inv+dsb-tlbiasidis-dsb-eret}\dotfill  & \hfill $\times$ & \hfill 4653ms \hfill & $\times$ & \hfill 3693ms \\
\TEST{CoWTa2.1.inv+dsb-tlbiasidis-dsb-eret}\dotfill  & \hfill $\times$ & \hfill 2833ms \hfill & $\times$ & \hfill 3180ms \\
\TEST{CoWTf.inv+[dmb]-dmb-addr}\dotfill  & \hfill $\times$ & \hfill 3845ms \hfill & $\times$ & \hfill 5057ms \\
\TEST{CoWTf.inv+dsb-isb}\dotfill  & \hfill $\times$ & \hfill 3024ms \hfill & $\times$ & \hfill 2475ms \\
\TEST{CoWTf.inv+po}\dotfill  & \hfill $\checkmark$ & \hfill 4112ms \hfill & $\checkmark$ & \hfill 4160ms \\
\TEST{CoWTf.inv+po-ctrl+po}\dotfill  & \hfill $\checkmark$ & \hfill 25871ms \hfill & $\checkmark$ & \hfill 24818ms \\
\TEST{CoWTf.inv+po-ctrl-isb+po}\dotfill  & \hfill $\checkmark$ & \hfill 64271ms \hfill & $\checkmark$ & \hfill 70941ms \\
\TEST{CoWTf.inv+poloc-ctrl-isb}\dotfill  & \hfill $\checkmark$ & \hfill 7161ms \hfill & $\checkmark$ & \hfill 8420ms \\
\TEST{CoWTf.inv+rfi-addr}\dotfill  & \hfill $\checkmark$ & \hfill 6419ms \hfill & $\checkmark$ & \hfill 6075ms \\
\TEST{CoWTf.inv+rfi-ctrl-isb}\dotfill  & \hfill $\checkmark$ & \hfill 8242ms \hfill & $\checkmark$ & \hfill 8255ms \\
\TEST{CoWTf.inv+svc}\dotfill  & \hfill $\checkmark$ & \hfill 6843ms \hfill & $\checkmark$ & \hfill 7037ms \\
\TEST{CoWTf.inv.EL1+dsb-eret}\dotfill  & \hfill $\times$ & \hfill 2425ms \hfill & $\times$ & \hfill 2073ms \\
\TEST{CoWTf.inv.EL1+dsb-svc}\dotfill  & \hfill $\times$ & \hfill 4906ms \hfill & $\times$ & \hfill 4442ms \\
\TEST{CoWTf.inv.EL1+eret}\dotfill  & \hfill $\checkmark$ & \hfill 4684ms \hfill & $\checkmark$ & \hfill 5627ms \\
\TEST{CoWTf.inv.EL2+dsb-tlbiipa-dsb-tlbiis-dsb-eret}\dotfill  & \hfill $\times$ & \hfill 221283ms \hfill & $\times$ & \hfill 5688ms \\
\TEST{CoWTf.inv.EL2+po}\dotfill  & \hfill $\checkmark$ & \hfill 7031ms \hfill & $\checkmark$ & \hfill 8213ms \\
\TEST{CoWTv2.2.inv+dsb-tlbivmidis-dsb-eret}\dotfill  & \hfill $\times$ & \hfill 5223ms \hfill & $\times$ & \hfill 4592ms \\
\TEST{CoWW.alias}\dotfill  & \hfill $\times$ & \hfill 822ms \hfill & $\times$ & \hfill 849ms \\
\TEST{CoWinvRpte+po}\dotfill  & \hfill $\times$ & \hfill 1024ms \hfill & $\times$ & \hfill 938ms \\
\TEST{CoWinvT+dsb-isb}\dotfill  & \hfill $\checkmark$ & \hfill 5292ms \hfill & $\checkmark$ & \hfill 5212ms \\
\TEST{CoWinvT+po}\dotfill  & \hfill $\checkmark$ & \hfill 5406ms \hfill & $\checkmark$ & \hfill 5832ms \\
\TEST{CoWinvT.EL1+dsb-tlbi-dsb}\dotfill  & \hfill $\checkmark$ & \hfill 10117ms \hfill & $\checkmark$ & \hfill 12882ms \\
\TEST{CoWinvT.EL1+dsb-tlbi-dsb-isb}\dotfill  & \hfill $\times$ & \hfill 18380ms \hfill & $\times$ & \hfill 25267ms \\
\TEST{CoWinvT.EL1+dsb-tlbiis-dsb}\dotfill  & \hfill $\checkmark$ & \hfill 11490ms \hfill & $\checkmark$ & \hfill 12759ms \\
\TEST{CoWinvT.EL1+dsb-tlbiis-dsb-isb}\dotfill  & \hfill $\times$ & \hfill 7548ms \hfill & $\times$ & \hfill 12986ms \\
\TEST{CoWinvT2+dsb-tlbiipa-dsb-eret}\dotfill  & \hfill $\times$ & \hfill 12608ms \hfill & $\times$ & \hfill 4645ms \\
\TEST{CoWinvT2+dsb-tlbiipa-dsb-tlbivmall-dsb-eret}\dotfill  & \hfill $\times$ & \hfill 114842ms \hfill & $\times$ & \hfill 196759ms \\
\TEST{CoWinvTa1.1+dsb-tlbiasidis-dsb-eret}\dotfill  & \hfill $\times$ & \hfill 7638ms \hfill & $\times$ & \hfill 99884ms \\
\TEST{CoWinvTa2.1+dsb-tlbiasidis-dsb-eret}\dotfill  & \hfill $\checkmark$ & \hfill 55920ms \hfill & $\checkmark$ & \hfill 9894ms \\
\TEST{CoWinvTv1.2+dsb-tlbivmidis-dsb-eret}\dotfill  & \hfill $\times$ & \hfill 13931ms \hfill & $\times$ & \hfill 8229ms \\
\TEST{CoWinvTv2.2+dsb-tlbivmidis-msrvttbr-dsb-eret}\dotfill  & \hfill $\checkmark$ & \hfill 10489ms \hfill & $\checkmark$ & \hfill 20604ms \\
\TEST{ETS}\dotfill  & \hfill $\times$ & \hfill 9590ms \hfill & $\times$ & \hfill 9297ms \\
\TEST{IRIW.TTf.TTf.inv+addrs}\dotfill  & \hfill $\times$ & \hfill 132223ms \hfill & $\times$ & \hfill 147911ms \\
\TEST{ISA2.RRTf.inv+dsb+addr+addr}\dotfill  & \hfill $\times$ & \hfill 4464ms \hfill & $\times$ & \hfill 4866ms \\
\TEST{ISA2.RRTf.inv+dsb+data+addr}\dotfill  & \hfill $\times$ & \hfill 5082ms \hfill & $\times$ & \hfill 5085ms \\
\TEST{LB+addr-trfis}\dotfill  & \hfill $\times$ & \hfill 7042ms \hfill & $\times$ & \hfill 7977ms \\
\TEST{LB+data-trfis}\dotfill  & \hfill $\times$ & \hfill 26579ms \hfill & $\times$ & \hfill 18056ms \\
\TEST{LB.TT.inv+pos}\dotfill  & \hfill $\times$ & \hfill 15481ms \hfill & $\times$ & \hfill 16545ms \\
\TEST{Load.inv}\dotfill  & \hfill --- & \hfill --- \hfill & $\times$ & \hfill 3345ms \\
\TEST{MP.BBM1+dsb-tlbiis-dsb-dsb+ctrl-isb}\dotfill  & \hfill $\times$ & \hfill 1068905ms \hfill & $\times$ & \hfill 571232ms \\
\TEST{MP.BBM1+dsb-tlbiis-dsb-dsb+dsb-isb}\dotfill  & \hfill $\times$ & \hfill 116116ms \hfill & \textbf{\textcolor{red}{!}} & \hfill 182456ms \\
\TEST{MP.RT.EL1+dsb+dsb-tlbi-dsb+dsb+dsb-isb}\dotfill  & \hfill $\checkmark$ & \hfill 146008ms \hfill & $\checkmark$ & \hfill 208363ms \\
\TEST{MP.RT.EL1+dsb+dsb-tlbiis-dsb+dsb+dsb-isb}\dotfill  & \hfill $\times$ & \hfill 307568ms \hfill & $\times$ & \hfill 760981ms \\
\TEST{MP.RT.EL1+dsb-shootdown-dsb+dsb-isb}\dotfill  & \hfill $\times$ & \hfill 765865ms \hfill & $\times$ & \hfill 49466ms \\
\TEST{MP.RT.EL1+dsb-tlbi-dsb+dsb-isb}\dotfill  & \hfill $\checkmark$ & \hfill 10678ms \hfill & $\checkmark$ & \hfill 87237ms \\
\TEST{MP.RT.EL1+dsb-tlbiis-dsb+dmb}\dotfill  & \hfill $\times$ & \hfill 57372ms \hfill & $\times$ & \hfill 5360ms \\
\TEST{MP.RT.EL1+dsb-tlbiis-dsb+dsb-isb}\dotfill  & \hfill $\times$ & \hfill 348942ms \hfill & $\times$ & \hfill 16656ms \\
\TEST{MP.RT.EL2+dsb-tlbiipa-dsb-tlbiis-dsb+dsb-isb}\dotfill  & \hfill $\checkmark$ & \hfill 108556ms \hfill & $\checkmark$ & \hfill 87273ms \\
\TEST{MP.RT.EL2+dsb-tlbiipais-dsb+dsb-isb}\dotfill  & \hfill $\checkmark$ & \hfill 112919ms \hfill & $\checkmark$ & \hfill 120764ms \\
\TEST{MP.RT.EL2+dsb-tlbiipais-dsb-tlbiis-dsb+dsb-isb}\dotfill  & \hfill $\checkmark$ & \hfill 145150ms \hfill & $\times$ & \hfill 435166ms \\
\TEST{MP.RT.EL2+dsb-tlbiis-dsb-tlbiipais-dsb+dsb-isb}\dotfill  & \hfill $\checkmark$ & \hfill 146011ms \hfill & $\checkmark$ & \hfill 97074ms \\
\TEST{MP.RT.inv+dmb+addr-po-isb}\dotfill  & \hfill $\times$ & \hfill 3366ms \hfill & $\times$ & \hfill 3223ms \\
\TEST{MP.RT.inv+dmb+addr-po-msr}\dotfill  & \hfill $\times$ & \hfill 3230ms \hfill & $\times$ & \hfill 3146ms \\
\TEST{MP.RT.inv+dmb+addr-po-msr-isb}\dotfill  & \hfill $\times$ & \hfill 4687ms \hfill & $\times$ & \hfill 3356ms \\
\TEST{MP.RT.inv+dmb+addr-trfi}\dotfill  & \hfill --- & \hfill --- \hfill & $\times$ & \hfill 7235ms \\
\TEST{MP.RT.inv+dmb+ctrl-trfi}\dotfill  & \hfill $\times$ & \hfill 6011ms \hfill & $\times$ & \hfill 6144ms \\
\TEST{MP.RT.inv+trfi-data+addr.toml}\dotfill  & \hfill $\checkmark$ & \hfill 40551ms \hfill & $\checkmark$ & \hfill 32442ms \\
\TEST{MP.RTT.EL1+dsb-tlbiis-tlbiis-dsb+dsb-isb}\dotfill  & \hfill $\times$ & \hfill 520042ms \hfill & $\times$ & \hfill 305092ms \\
\TEST{MP.RTf.inv+dmb+addr}\dotfill  & \hfill $\times$ & \hfill 3574ms \hfill & $\times$ & \hfill 4327ms \\
\TEST{MP.RTf.inv+dmb+ctrl-isb}\dotfill  & \hfill $\times$ & \hfill 5734ms \hfill & $\times$ & \hfill 5059ms \\
\TEST{MP.RTf.inv+dmb+data}\dotfill  & \hfill $\times$ & \hfill 3232ms \hfill & $\times$ & \hfill 3843ms \\
\TEST{MP.RTf.inv+dmb+dsb-isb}\dotfill  & \hfill $\times$ & \hfill 5345ms \hfill & $\times$ & \hfill 3982ms \\
\TEST{MP.RTf.inv+dmb+po}\dotfill  & \hfill $\checkmark$ & \hfill 5316ms \hfill & $\times$ & \hfill 2598ms \\
\TEST{MP.RTf.inv+dmbs}\dotfill  & \hfill $\checkmark$ & \hfill 5896ms \hfill & $\times$ & \hfill 3681ms \\
\TEST{MP.RTf.inv.EL1+dsb-tlbiis-dsb+addr}\dotfill  & \hfill $\times$ & \hfill 3994ms \hfill & $\times$ & \hfill 3882ms \\
\TEST{MP.RTf.inv.EL1+dsb-tlbiis-dsb+ctrl}\dotfill  & \hfill $\times$ & \hfill 15261ms \hfill & $\times$ & \hfill 6025ms \\
\TEST{MP.RTf.inv.EL1+dsb-tlbiis-dsb+ctrl-isb}\dotfill  & \hfill $\times$ & \hfill 31160ms \hfill & $\times$ & \hfill 8117ms \\
\TEST{MP.RTf.inv.EL1+dsb-tlbiis-dsb+data}\dotfill  & \hfill $\times$ & \hfill 3744ms \hfill & $\times$ & \hfill 5394ms \\
\TEST{MP.RTf.inv.EL1+dsb-tlbiis-dsb+dmb}\dotfill  & \hfill $\times$ & \hfill 10762ms \hfill & $\times$ & \hfill 5294ms \\
\TEST{MP.RTf.inv.EL1+dsb-tlbiis-dsb+dsb-isb}\dotfill  & \hfill $\times$ & \hfill 52965ms \hfill & $\times$ & \hfill 6204ms \\
\TEST{MP.RTf.inv.EL1+dsb-tlbiis-dsb+po}\dotfill  & \hfill $\times$ & \hfill 20910ms \hfill & $\times$ & \hfill 3710ms \\
\TEST{MP.RTf.inv.EL1+dsb-tlbiis-dsb+poap}\dotfill  & \hfill $\times$ & \hfill 75710ms \hfill & $\times$ & \hfill 3279ms \\
\TEST{MP.TR.inv+dmb+isb}\dotfill  & \hfill $\times$ & \hfill 2406ms \hfill & $\times$ & \hfill 3016ms \\
\TEST{MP.TR.inv+dmb+msr}\dotfill  & \hfill $\checkmark$ & \hfill 6174ms \hfill & $\checkmark$ & \hfill 6987ms \\
\TEST{MP.TR.inv+dmb+msr-isb}\dotfill  & \hfill $\times$ & \hfill 4042ms \hfill & $\times$ & \hfill 4240ms \\
\TEST{MP.TTf.inv+dmb+addr}\dotfill  & \hfill $\times$ & \hfill 12067ms \hfill & $\times$ & \hfill 16288ms \\
\TEST{MP.TTf.inv+dmb+dsb-isb}\dotfill  & \hfill $\times$ & \hfill 27192ms \hfill & $\times$ & \hfill 47972ms \\
\TEST{MP.TTf.inv+dmb+po}\dotfill  & \hfill $\checkmark$ & \hfill 52201ms \hfill & $\times$ & \hfill 9113ms \\
\TEST{MP.TTf.inv+dsb+ctrl-isb}\dotfill  & \hfill $\times$ & \hfill 30317ms \hfill & $\times$ & \hfill 37812ms \\
\TEST{MP.TTf.inv+dsb+dsb-isb}\dotfill  & \hfill $\times$ & \hfill 29708ms \hfill & $\times$ & \hfill 22505ms \\
\TEST{MP.TTf.inv+dsb+po}\dotfill  & \hfill $\checkmark$ & \hfill 42061ms \hfill & $\times$ & \hfill 23415ms \\
\TEST{MP.TTf.inv+dsbs}\dotfill  & \hfill $\checkmark$ & \hfill 64484ms \hfill & $\times$ & \hfill 28800ms \\
\TEST{MP.TTf.inv.EL1+dsb-tlbiis-dsb+dmb}\dotfill  & \hfill $\times$ & \hfill 235651ms \hfill & $\times$ & \hfill 81641ms \\
\TEST{MP.TTf.inv.EL1+dsb-tlbiis-dsb+dsb-isb}\dotfill  & \hfill $\times$ & \hfill 16436ms \hfill & $\times$ & \hfill 29491ms \\
\TEST{MP.TTf.inv.EL1+dsb-tlbiis-dsb+po}\dotfill  & \hfill $\times$ & \hfill 162552ms \hfill & $\times$ & \hfill 200958ms \\
\TEST{MP.TfR+dmb+eret}\dotfill  & \hfill $\times$ & \hfill 3508ms \hfill & $\times$ & \hfill 4473ms \\
\TEST{MP.alias3+rfi-data+dmb}\dotfill  & \hfill $\checkmark$ & \hfill 1431ms \hfill & $\checkmark$ & \hfill 1483ms \\
\TEST{PPOAA.alias}\dotfill  & \hfill $\times$ & \hfill 2645ms \hfill & $\times$ & \hfill 3113ms \\
\TEST{PPOCA.alias}\dotfill  & \hfill $\checkmark$ & \hfill 4744ms \hfill & $\checkmark$ & \hfill 4932ms \\
\TEST{PPODA.RT.inv}\dotfill  & \hfill $\times$ & \hfill 5779ms \hfill & $\times$ & \hfill 6596ms \\
\TEST{R.RTf.inv.EL1+dsb-tlbiis-dsb+popl}\dotfill  & \hfill $\times$ & \hfill 13739ms \hfill & $\times$ & \hfill 4164ms \\
\TEST{R.TR.inv+dmb+trfi}\dotfill  & \hfill $\checkmark$ & \hfill 8652ms \hfill & $\checkmark$ & \hfill 9603ms \\
\TEST{R.inv}\dotfill  & \hfill $\times$ & \hfill 1976ms \hfill & $\times$ & \hfill 2050ms \\
\TEST{RBS+dsb-tlbiis-dsb}\dotfill  & \hfill $\times$ & \hfill 4158ms \hfill & $\times$ & \hfill 12912ms \\
\TEST{RDW.alias}\dotfill  & \hfill $\times$ & \hfill 2972ms \hfill & $\times$ & \hfill 3317ms \\
\TEST{ROT.inv+dmbst}\dotfill  & \hfill $\times$ & \hfill 3998ms \hfill & $\times$ & \hfill 3919ms \\
\TEST{ROT.inv+dsb}\dotfill  & \hfill $\times$ & \hfill 2805ms \hfill & $\times$ & \hfill 3202ms \\
\TEST{ROT.inv+po}\dotfill  & \hfill $\checkmark$ & \hfill 4749ms \hfill & $\checkmark$ & \hfill 4899ms \\
\TEST{RSW.alias}\dotfill  & \hfill $\checkmark$ & \hfill 2765ms \hfill & $\checkmark$ & \hfill 2609ms \\
\TEST{RWC.RTfR.inv+addr+dmb}\dotfill  & \hfill $\times$ & \hfill 3022ms \hfill & $\times$ & \hfill 3609ms \\
\TEST{S+tlbiall+po}\dotfill  & \hfill $\checkmark$ & \hfill 3838ms \hfill & $\checkmark$ & \hfill 3787ms \\
\TEST{S.RT.ro+dsb-tlbiis-dsb+dsb-isb}\dotfill  & \hfill $\times$ & \hfill 36657ms \hfill & $\times$ & \hfill 80116ms \\
\TEST{S.RTW+tlbiall+addr-po}\dotfill  & \hfill --- & \hfill --- \hfill & $\checkmark$ & \hfill 4452ms \\
\TEST{S.RTf.inv.EL1+dsb-tlbiis-dsb+ctrl}\dotfill  & \hfill $\times$ & \hfill 12958ms \hfill & $\times$ & \hfill 4463ms \\
\TEST{S.RTf.inv.EL1+dsb-tlbiis-dsb+data}\dotfill  & \hfill $\times$ & \hfill 4120ms \hfill & $\times$ & \hfill 4535ms \\
\TEST{S.RTf.inv.EL1+dsb-tlbiis-dsb+dmb}\dotfill  & \hfill $\times$ & \hfill 11481ms \hfill & $\times$ & \hfill 4349ms \\
\TEST{S.RTf.inv.EL1+dsb-tlbiis-dsb+poap}\dotfill  & \hfill $\times$ & \hfill 45733ms \hfill & $\times$ & \hfill 3117ms \\
\TEST{S.RTf.inv.EL1+dsb-tlbiis-dsb+popl}\dotfill  & \hfill $\times$ & \hfill 28716ms \hfill & $\times$ & \hfill 4266ms \\
\TEST{S.T+dmb+po}\dotfill  & \hfill $\times$ & \hfill 6152ms \hfill & $\times$ & \hfill 4485ms \\
\TEST{S.T.alias+tlbiall+po}\dotfill  & \hfill --- & \hfill --- \hfill & $\times$ & \hfill 17937ms \\
\TEST{SB.TfTf.inv+dmb-ctrl-isbs}\dotfill  & \hfill $\times$ & \hfill 19569ms \hfill & $\times$ & \hfill 16904ms \\
\TEST{SB.TfTf.inv+dsb-isbs}\dotfill  & \hfill $\times$ & \hfill 9504ms \hfill & $\times$ & \hfill 8368ms \\
\TEST{SB.TfTf.invv+rfi-ctrl-isbs}\dotfill  & \hfill $\checkmark$ & \hfill 34795ms \hfill & $\times$ & \hfill 15059ms \\
\TEST{SwitchTable.same-asid+eret.toml}\dotfill  & \hfill $\times$ & \hfill 1245ms \hfill & $\times$ & \hfill 1294ms \\
\TEST{W}\dotfill  & \hfill $\checkmark$ & \hfill 663ms \hfill & $\checkmark$ & \hfill 694ms \\
\TEST{W+T}\dotfill  & \hfill $\checkmark$ & \hfill 3748ms \hfill & $\checkmark$ & \hfill 10144ms \\
\TEST{WBM+dsb-tlbiis-dsb}\dotfill  & \hfill $\times$ & \hfill 5104ms \hfill & $\times$ & \hfill 4658ms \\
\TEST{WDS+dsb-tlbiipa-dsb-eret-po}\dotfill  & \hfill $\checkmark$ & \hfill 59690ms \hfill & $\checkmark$ & \hfill 216640ms \\
\TEST{WDS+dsb-tlbiipa-dsb-po-eret}\dotfill  & \hfill $\times$ & \hfill 61832ms \hfill & $\times$ & \hfill 9009ms \\
\TEST{WDS+po-dsb-tlbiipa-dsb-eret}\dotfill  & \hfill $\checkmark$ & \hfill 267478ms \hfill & $\checkmark$ & \hfill 25136ms \\
\TEST{WDS+po-dsb-tlbiipa-dsb-po-eret}\dotfill  & \hfill $\checkmark$ & \hfill 146279ms \hfill & $\checkmark$ & \hfill 30736ms \\
\TEST{WDS+po-dsb-tlbiipa-dsb-tlbiis-dsb-eret}\dotfill  & \hfill $\times$ & \hfill 186945ms \hfill & $\times$ & \hfill 576750ms \\
\TEST{WRC.RRTf.inv+addrs}\dotfill  & \hfill $\times$ & \hfill 4100ms \hfill & $\times$ & \hfill 4411ms \\
\TEST{WRC.RRTf.inv+dmbs}\dotfill  & \hfill $\checkmark$ & \hfill 6441ms \hfill & $\times$ & \hfill 3589ms \\
\TEST{WRC.RRTf.inv+dsb+ctrl-isb}\dotfill  & \hfill $\times$ & \hfill 5218ms \hfill & $\times$ & \hfill 5459ms \\
\TEST{WRC.RRTf.inv+dsb+dsb-isb}\dotfill  & \hfill $\times$ & \hfill 5393ms \hfill & $\times$ & \hfill 5591ms \\
\TEST{WRC.RRTf.inv+dsbs}\dotfill  & \hfill $\checkmark$ & \hfill 8964ms \hfill & $\times$ & \hfill 4568ms \\
\TEST{WRC.RRTf.inv+pos}\dotfill  & \hfill $\checkmark$ & \hfill 5334ms \hfill & $\checkmark$ & \hfill 5239ms \\
\TEST{WRC.TRTf.inv+addrs}\dotfill  & \hfill $\times$ & \hfill 10005ms \hfill & $\times$ & \hfill 11073ms \\
\TEST{WRC.TRTf.inv+dmbs}\dotfill  & \hfill $\checkmark$ & \hfill 35492ms \hfill & $\times$ & \hfill 8559ms \\
\TEST{WRC.TRTf.inv+dsb+dsb-isb}\dotfill  & \hfill $\times$ & \hfill 9146ms \hfill & $\times$ & \hfill 16960ms \\
\TEST{WRC.TRTf.inv+dsbs}\dotfill  & \hfill $\checkmark$ & \hfill 48023ms \hfill & $\times$ & \hfill 8487ms \\
\TEST{WRC.TRTf.inv+pos}\dotfill  & \hfill $\checkmark$ & \hfill 26642ms \hfill & $\times$ & \hfill 9414ms \\
\TEST{WRC.TTTf.inv+addrs}\dotfill  & \hfill $\times$ & \hfill 31851ms \hfill & $\times$ & \hfill 23959ms \\
\TEST{WRC.TTTf.inv+data+addr}\dotfill  & \hfill $\times$ & \hfill 49883ms \hfill & $\times$ & \hfill 40834ms \\
\TEST{WRC.TfRR+ctrl-isb+dsb}\dotfill  & \hfill $\times$ & \hfill 5699ms \hfill & $\times$ & \hfill 6787ms \\
\TEST{WRC.TfRR+dmbs}\dotfill  & \hfill $\times$ & \hfill 4533ms \hfill & $\times$ & \hfill 4800ms \\
\TEST{WRC.TfRR+dsb-isb+dsb}\dotfill  & \hfill $\times$ & \hfill 5353ms \hfill & $\times$ & \hfill 5963ms \\
\TEST{WRC.TfRR+dsbs}\dotfill  & \hfill $\times$ & \hfill 3850ms \hfill & $\times$ & \hfill 5423ms \\
\TEST{WRC.TfRR+po+dsb}\dotfill  & \hfill $\times$ & \hfill 3508ms \hfill & $\times$ & \hfill 3727ms \\
\TEST{WRC.TfRR+pos}\dotfill  & \hfill $\checkmark$ & \hfill 5616ms \hfill & $\checkmark$ & \hfill 7637ms \\
\TEST{WRC.TfRT+dsb-tlbiis-dsb+dsb-isb}\dotfill  & \hfill $\times$ & \hfill 549315ms \hfill & $\times$ & \hfill 1582501ms \\
\TEST{WRC.TfRT+po+dsb-isb}\dotfill  & \hfill $\checkmark$ & \hfill 39075ms \hfill & $\checkmark$ & \hfill 57628ms \\


==> vmsa-test-index/tests/tex/BBM+dsb-tlbiis-dsb.tex <==
\newlength{\BBMplusdsbtlbiisdsbH}
\setlength{\BBMplusdsbtlbiisdsbH}{0cm}
\newsavebox{\BBMplusdsbtlbiisdsbI}
\begin{lrbox}{\BBMplusdsbtlbiisdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X6
DSB SY
STR X2,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\BBMplusdsbtlbiisdsbJ}
\settowidth{\BBMplusdsbtlbiisdsbJ}{\usebox{\BBMplusdsbtlbiisdsbI}}
\addtolength{\BBMplusdsbtlbiisdsbH}{\BBMplusdsbtlbiisdsbJ}
\newsavebox{\BBMplusdsbtlbiisdsbK}
\begin{lrbox}{\BBMplusdsbtlbiisdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\BBMplusdsbtlbiisdsbL}
\settowidth{\BBMplusdsbtlbiisdsbL}{\usebox{\BBMplusdsbtlbiisdsbK}}
\addtolength{\BBMplusdsbtlbiisdsbH}{\BBMplusdsbtlbiisdsbL}
\newsavebox{\BBMplusdsbtlbiisdsbM}
\begin{lrbox}{\BBMplusdsbtlbiisdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\BBMplusdsbtlbiisdsbN}
\settowidth{\BBMplusdsbtlbiisdsbN}{\usebox{\BBMplusdsbtlbiisdsbM}}
\addtolength{\BBMplusdsbtlbiisdsbH}{\BBMplusdsbtlbiisdsbN}
\newsavebox{\BBMplusdsbtlbiisdsbO}
\begin{lrbox}{\BBMplusdsbtlbiisdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;
    x ?-> pa2;

    identity 0x1000 with code;

    *pa2 = 2;
\end{lstlisting}
\end{lrbox}
\newlength{\BBMplusdsbtlbiisdsbP}
\settowidth{\BBMplusdsbtlbiisdsbP}{\usebox{\BBMplusdsbtlbiisdsbO}}
\newsavebox{\BBMplusdsbtlbiisdsbA}
\begin{lrbox}{\BBMplusdsbtlbiisdsbA}
\begin{minipage}{\BBMplusdsbtlbiisdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R4=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|BBM+dsb-tlbiis-dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\BBMplusdsbtlbiisdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\BBMplusdsbtlbiisdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\BBMplusdsbtlbiisdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\BBMplusdsbtlbiisdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\BBMplusdsbtlbiisdsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\BBMplusdsbtlbiisdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/BBM.Tf+dsb-tlbiis-dsb.tex <==
\newlength{\BBMdotTfplusdsbtlbiisdsbH}
\setlength{\BBMdotTfplusdsbtlbiisdsbH}{0cm}
\newsavebox{\BBMdotTfplusdsbtlbiisdsbI}
\begin{lrbox}{\BBMdotTfplusdsbtlbiisdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X6
DSB SY
STR X2,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\BBMdotTfplusdsbtlbiisdsbJ}
\settowidth{\BBMdotTfplusdsbtlbiisdsbJ}{\usebox{\BBMdotTfplusdsbtlbiisdsbI}}
\addtolength{\BBMdotTfplusdsbtlbiisdsbH}{\BBMdotTfplusdsbtlbiisdsbJ}
\newsavebox{\BBMdotTfplusdsbtlbiisdsbK}
\begin{lrbox}{\BBMdotTfplusdsbtlbiisdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\BBMdotTfplusdsbtlbiisdsbL}
\settowidth{\BBMdotTfplusdsbtlbiisdsbL}{\usebox{\BBMdotTfplusdsbtlbiisdsbK}}
\addtolength{\BBMdotTfplusdsbtlbiisdsbH}{\BBMdotTfplusdsbtlbiisdsbL}
\newsavebox{\BBMdotTfplusdsbtlbiisdsbM}
\begin{lrbox}{\BBMdotTfplusdsbtlbiisdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
\end{lstlisting}
\end{lrbox}
\newlength{\BBMdotTfplusdsbtlbiisdsbN}
\settowidth{\BBMdotTfplusdsbtlbiisdsbN}{\usebox{\BBMdotTfplusdsbtlbiisdsbM}}
\addtolength{\BBMdotTfplusdsbtlbiisdsbH}{\BBMdotTfplusdsbtlbiisdsbN}
\newsavebox{\BBMdotTfplusdsbtlbiisdsbO}
\begin{lrbox}{\BBMdotTfplusdsbtlbiisdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;
    x ?-> pa2;

    identity 0x1000 with code;

    *pa2 = 2;
\end{lstlisting}
\end{lrbox}
\newlength{\BBMdotTfplusdsbtlbiisdsbP}
\settowidth{\BBMdotTfplusdsbtlbiisdsbP}{\usebox{\BBMdotTfplusdsbtlbiisdsbO}}
\newsavebox{\BBMdotTfplusdsbtlbiisdsbA}
\begin{lrbox}{\BBMdotTfplusdsbtlbiisdsbA}
\begin{minipage}{\BBMdotTfplusdsbtlbiisdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R4=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|BBM.Tf+dsb-tlbiis-dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\BBMdotTfplusdsbtlbiisdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\BBMdotTfplusdsbtlbiisdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\BBMdotTfplusdsbtlbiisdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\BBMdotTfplusdsbtlbiisdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\BBMdotTfplusdsbtlbiisdsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\BBMdotTfplusdsbtlbiisdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/Break2.news1.tex <==
\newlength{\BreaktwodotnewsoneH}
\setlength{\BreaktwodotnewsoneH}{0cm}
\newsavebox{\BreaktwodotnewsoneI}
\begin{lrbox}{\BreaktwodotnewsoneI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1IS,X4
DSB SY
TLBI VMALLE1IS
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\BreaktwodotnewsoneJ}
\settowidth{\BreaktwodotnewsoneJ}{\usebox{\BreaktwodotnewsoneI}}
\addtolength{\BreaktwodotnewsoneH}{\BreaktwodotnewsoneJ}
\newsavebox{\BreaktwodotnewsoneK}
\begin{lrbox}{\BreaktwodotnewsoneK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\BreaktwodotnewsoneL}
\settowidth{\BreaktwodotnewsoneL}{\usebox{\BreaktwodotnewsoneK}}
\addtolength{\BreaktwodotnewsoneH}{\BreaktwodotnewsoneL}
\newsavebox{\BreaktwodotnewsoneM}
\begin{lrbox}{\BreaktwodotnewsoneM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#2
\end{lstlisting}
\end{lrbox}
\newlength{\BreaktwodotnewsoneN}
\settowidth{\BreaktwodotnewsoneN}{\usebox{\BreaktwodotnewsoneM}}
\addtolength{\BreaktwodotnewsoneH}{\BreaktwodotnewsoneN}
\newsavebox{\BreaktwodotnewsoneO}
\begin{lrbox}{\BreaktwodotnewsoneO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X0,#3
\end{lstlisting}
\end{lrbox}
\newlength{\BreaktwodotnewsoneP}
\settowidth{\BreaktwodotnewsoneP}{\usebox{\BreaktwodotnewsoneO}}
\addtolength{\BreaktwodotnewsoneH}{\BreaktwodotnewsoneP}
\newsavebox{\BreaktwodotnewsoneA}
\begin{lrbox}{\BreaktwodotnewsoneA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
option default_tables = false;
physical pa1;
intermediate ipa1;

s2table vm_stage2 0x240000  {
    ipa1 |-> pa1 at level 3;
    ipa1 ?-> invalid at level 3;
    identity pa_to_ipa(0x1000) with code;


    s1table vm_stage1 0x280000  {
        x |-> invalid at level 3;
        x ?-> ipa1 at level 3;

        identity pa_to_va(0x1000) with code;
    }
}

s1table hyp_map 0x200000 {
    identity 0x2000 with code;
    s2table vm_stage2;
    s1table vm_stage1;
}

*pa1 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\BreaktwodotnewsoneB}
\settowidth{\BreaktwodotnewsoneB}{\usebox{\BreaktwodotnewsoneA}}
\newsavebox{\BreaktwodotnewsoneC}
\begin{lrbox}{\BreaktwodotnewsoneC}
\begin{minipage}{\BreaktwodotnewsoneH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(ipa1,vm_stage2)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=ipa1)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(x,vm_stage1)|\\
\lstinline[language=IslaLitmusExp]|0:R4=bvlshr(ipa1,0xC)|\\
\lstinline[language=IslaLitmusExp]|0:TTBR0_EL2=ttbr(asid=0x0000,base=hyp_map)|\\
\lstinline[language=IslaLitmusExp]|0:VTTBR_EL2=ttbr(base=vm_stage2,vmid=0x0000)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:TTBR0_EL1=ttbr(base=vm_stage1,asid=0x0000)|\\
\lstinline[language=IslaLitmusExp]|1:TTBR0_EL2=ttbr(base=hyp_map,asid=0x0000)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\lstinline[language=IslaLitmusExp]|1:VTTBR_EL2=ttbr(vmid=0x0000,base=vm_stage2)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|Break2.news1|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\BreaktwodotnewsoneB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\BreaktwodotnewsoneA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\BreaktwodotnewsoneC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\BreaktwodotnewsoneI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\BreaktwodotnewsoneK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\BreaktwodotnewsoneM}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\BreaktwodotnewsoneO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoRR0.alias+po.tex <==
\newlength{\CoRRzerodotaliaspluspoH}
\setlength{\CoRRzerodotaliaspluspoH}{0cm}
\newsavebox{\CoRRzerodotaliaspluspoI}
\begin{lrbox}{\CoRRzerodotaliaspluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRRzerodotaliaspluspoJ}
\settowidth{\CoRRzerodotaliaspluspoJ}{\usebox{\CoRRzerodotaliaspluspoI}}
\addtolength{\CoRRzerodotaliaspluspoH}{\CoRRzerodotaliaspluspoJ}
\newsavebox{\CoRRzerodotaliaspluspoK}
\begin{lrbox}{\CoRRzerodotaliaspluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRRzerodotaliaspluspoL}
\settowidth{\CoRRzerodotaliaspluspoL}{\usebox{\CoRRzerodotaliaspluspoK}}
\addtolength{\CoRRzerodotaliaspluspoH}{\CoRRzerodotaliaspluspoL}
\newsavebox{\CoRRzerodotaliaspluspoM}
\begin{lrbox}{\CoRRzerodotaliaspluspoM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    y |-> pa1;
    *pa1 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRRzerodotaliaspluspoN}
\settowidth{\CoRRzerodotaliaspluspoN}{\usebox{\CoRRzerodotaliaspluspoM}}
\newsavebox{\CoRRzerodotaliaspluspoO}
\begin{lrbox}{\CoRRzerodotaliaspluspoO}
\begin{minipage}{\CoRRzerodotaliaspluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRR0.alias+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRRzerodotaliaspluspoN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRRzerodotaliaspluspoM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRRzerodotaliaspluspoO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRRzerodotaliaspluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRRzerodotaliaspluspoK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoRR2.alias+po.tex <==
\newlength{\CoRRtwodotaliaspluspoH}
\setlength{\CoRRtwodotaliaspluspoH}{0cm}
\newsavebox{\CoRRtwodotaliaspluspoI}
\begin{lrbox}{\CoRRtwodotaliaspluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRRtwodotaliaspluspoJ}
\settowidth{\CoRRtwodotaliaspluspoJ}{\usebox{\CoRRtwodotaliaspluspoI}}
\addtolength{\CoRRtwodotaliaspluspoH}{\CoRRtwodotaliaspluspoJ}
\newsavebox{\CoRRtwodotaliaspluspoK}
\begin{lrbox}{\CoRRtwodotaliaspluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRRtwodotaliaspluspoL}
\settowidth{\CoRRtwodotaliaspluspoL}{\usebox{\CoRRtwodotaliaspluspoK}}
\addtolength{\CoRRtwodotaliaspluspoH}{\CoRRtwodotaliaspluspoL}
\newsavebox{\CoRRtwodotaliaspluspoM}
\begin{lrbox}{\CoRRtwodotaliaspluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRRtwodotaliaspluspoN}
\settowidth{\CoRRtwodotaliaspluspoN}{\usebox{\CoRRtwodotaliaspluspoM}}
\addtolength{\CoRRtwodotaliaspluspoH}{\CoRRtwodotaliaspluspoN}
\newsavebox{\CoRRtwodotaliaspluspoO}
\begin{lrbox}{\CoRRtwodotaliaspluspoO}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRRtwodotaliaspluspoP}
\settowidth{\CoRRtwodotaliaspluspoP}{\usebox{\CoRRtwodotaliaspluspoO}}
\addtolength{\CoRRtwodotaliaspluspoH}{\CoRRtwodotaliaspluspoP}
\newsavebox{\CoRRtwodotaliaspluspoA}
\begin{lrbox}{\CoRRtwodotaliaspluspoA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    u |-> pa1;
    v |-> pa1;
    w |-> pa1;
    x |-> pa1;
    y |-> pa1;
    z |-> pa1;
    *pa1 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRRtwodotaliaspluspoB}
\settowidth{\CoRRtwodotaliaspluspoB}{\usebox{\CoRRtwodotaliaspluspoA}}
\newsavebox{\CoRRtwodotaliaspluspoC}
\begin{lrbox}{\CoRRtwodotaliaspluspoC}
\begin{minipage}{\CoRRtwodotaliaspluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R1=u|\\
\lstinline[language=IslaLitmusExp]|1:R0=0b10|\\
\lstinline[language=IslaLitmusExp]|1:R1=v|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=w|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|3:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|3:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|3:R1=y|\\
\lstinline[language=IslaLitmusExp]|3:R3=z|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRR2.alias+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRRtwodotaliaspluspoB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRRtwodotaliaspluspoA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRRtwodotaliaspluspoC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRRtwodotaliaspluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRRtwodotaliaspluspoK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\CoRRtwodotaliaspluspoM}\\
  \cline{2-2}
  & Thread 3\\
  \cline{2-2}
  & \usebox{\CoRRtwodotaliaspluspoO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|2:R0=1 & 2:R2=2 & 3:R0=2 & 3:R2=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoRT.inv+addr-trfi.tex <==
\newlength{\CoRTdotinvplusaddrtrfiH}
\setlength{\CoRTdotinvplusaddrtrfiH}{0cm}
\newsavebox{\CoRTdotinvplusaddrtrfiI}
\begin{lrbox}{\CoRTdotinvplusaddrtrfiI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRTdotinvplusaddrtrfiJ}
\settowidth{\CoRTdotinvplusaddrtrfiJ}{\usebox{\CoRTdotinvplusaddrtrfiI}}
\addtolength{\CoRTdotinvplusaddrtrfiH}{\CoRTdotinvplusaddrtrfiJ}
\newsavebox{\CoRTdotinvplusaddrtrfiK}
\begin{lrbox}{\CoRTdotinvplusaddrtrfiK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
STR X3,[X4,X2]
LDR X5,[X6]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRTdotinvplusaddrtrfiL}
\settowidth{\CoRTdotinvplusaddrtrfiL}{\usebox{\CoRTdotinvplusaddrtrfiK}}
\addtolength{\CoRTdotinvplusaddrtrfiH}{\CoRTdotinvplusaddrtrfiL}
\newsavebox{\CoRTdotinvplusaddrtrfiM}
\begin{lrbox}{\CoRTdotinvplusaddrtrfiM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X5,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoRTdotinvplusaddrtrfiN}
\settowidth{\CoRTdotinvplusaddrtrfiN}{\usebox{\CoRTdotinvplusaddrtrfiM}}
\addtolength{\CoRTdotinvplusaddrtrfiH}{\CoRTdotinvplusaddrtrfiN}
\newsavebox{\CoRTdotinvplusaddrtrfiO}
\begin{lrbox}{\CoRTdotinvplusaddrtrfiO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    y |-> invalid;
    y ?-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRTdotinvplusaddrtrfiP}
\settowidth{\CoRTdotinvplusaddrtrfiP}{\usebox{\CoRTdotinvplusaddrtrfiO}}
\newsavebox{\CoRTdotinvplusaddrtrfiA}
\begin{lrbox}{\CoRTdotinvplusaddrtrfiA}
\begin{minipage}{\CoRTdotinvplusaddrtrfiH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|1:R4=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R6=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRT.inv+addr-trfi|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRTdotinvplusaddrtrfiP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRTdotinvplusaddrtrfiO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRTdotinvplusaddrtrfiA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRTdotinvplusaddrtrfiI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRTdotinvplusaddrtrfiK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoRTdotinvplusaddrtrfiM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|true|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoRpteT+dsb-isb.tex <==
\newlength{\CoRpteTplusdsbisbH}
\setlength{\CoRpteTplusdsbisbH}{0cm}
\newsavebox{\CoRpteTplusdsbisbI}
\begin{lrbox}{\CoRpteTplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTplusdsbisbJ}
\settowidth{\CoRpteTplusdsbisbJ}{\usebox{\CoRpteTplusdsbisbI}}
\addtolength{\CoRpteTplusdsbisbH}{\CoRpteTplusdsbisbJ}
\newsavebox{\CoRpteTplusdsbisbK}
\begin{lrbox}{\CoRpteTplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTplusdsbisbL}
\settowidth{\CoRpteTplusdsbisbL}{\usebox{\CoRpteTplusdsbisbK}}
\addtolength{\CoRpteTplusdsbisbH}{\CoRpteTplusdsbisbL}
\newsavebox{\CoRpteTplusdsbisbM}
\begin{lrbox}{\CoRpteTplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTplusdsbisbN}
\settowidth{\CoRpteTplusdsbisbN}{\usebox{\CoRpteTplusdsbisbM}}
\addtolength{\CoRpteTplusdsbisbH}{\CoRpteTplusdsbisbN}
\newsavebox{\CoRpteTplusdsbisbO}
\begin{lrbox}{\CoRpteTplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;

    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;

    *pa1 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTplusdsbisbP}
\settowidth{\CoRpteTplusdsbisbP}{\usebox{\CoRpteTplusdsbisbO}}
\newsavebox{\CoRpteTplusdsbisbA}
\begin{lrbox}{\CoRpteTplusdsbisbA}
\begin{minipage}{\CoRpteTplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRpteT+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRpteTplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRpteTplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRpteTplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRpteTplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRpteTplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoRpteTplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=0 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoRpteT+dsb.tex <==
\newlength{\CoRpteTplusdsbH}
\setlength{\CoRpteTplusdsbH}{0cm}
\newsavebox{\CoRpteTplusdsbI}
\begin{lrbox}{\CoRpteTplusdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTplusdsbJ}
\settowidth{\CoRpteTplusdsbJ}{\usebox{\CoRpteTplusdsbI}}
\addtolength{\CoRpteTplusdsbH}{\CoRpteTplusdsbJ}
\newsavebox{\CoRpteTplusdsbK}
\begin{lrbox}{\CoRpteTplusdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTplusdsbL}
\settowidth{\CoRpteTplusdsbL}{\usebox{\CoRpteTplusdsbK}}
\addtolength{\CoRpteTplusdsbH}{\CoRpteTplusdsbL}
\newsavebox{\CoRpteTplusdsbM}
\begin{lrbox}{\CoRpteTplusdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTplusdsbN}
\settowidth{\CoRpteTplusdsbN}{\usebox{\CoRpteTplusdsbM}}
\addtolength{\CoRpteTplusdsbH}{\CoRpteTplusdsbN}
\newsavebox{\CoRpteTplusdsbO}
\begin{lrbox}{\CoRpteTplusdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;

    *x = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTplusdsbP}
\settowidth{\CoRpteTplusdsbP}{\usebox{\CoRpteTplusdsbO}}
\newsavebox{\CoRpteTplusdsbA}
\begin{lrbox}{\CoRpteTplusdsbA}
\begin{minipage}{\CoRpteTplusdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRpteT+dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRpteTplusdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRpteTplusdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRpteTplusdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRpteTplusdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRpteTplusdsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoRpteTplusdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=0 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoRpteT.EL1+dsb-tlbi-dsb-isb.tex <==
\newlength{\CoRpteTdotELoneplusdsbtlbidsbisbH}
\setlength{\CoRpteTdotELoneplusdsbtlbidsbisbH}{0cm}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbisbI}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTdotELoneplusdsbtlbidsbisbJ}
\settowidth{\CoRpteTdotELoneplusdsbtlbidsbisbJ}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbisbI}}
\addtolength{\CoRpteTdotELoneplusdsbtlbidsbisbH}{\CoRpteTdotELoneplusdsbtlbidsbisbJ}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbisbK}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
TLBI VAE1,X4
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTdotELoneplusdsbtlbidsbisbL}
\settowidth{\CoRpteTdotELoneplusdsbtlbidsbisbL}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbisbK}}
\addtolength{\CoRpteTdotELoneplusdsbtlbidsbisbH}{\CoRpteTdotELoneplusdsbtlbidsbisbL}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbisbM}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTdotELoneplusdsbtlbidsbisbN}
\settowidth{\CoRpteTdotELoneplusdsbtlbidsbisbN}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbisbM}}
\addtolength{\CoRpteTdotELoneplusdsbtlbidsbisbH}{\CoRpteTdotELoneplusdsbtlbidsbisbN}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbisbO}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;

    *pa1 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTdotELoneplusdsbtlbidsbisbP}
\settowidth{\CoRpteTdotELoneplusdsbtlbidsbisbP}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbisbO}}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbisbA}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbisbA}
\begin{minipage}{\CoRpteTdotELoneplusdsbtlbidsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRpteT.EL1+dsb-tlbi-dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRpteTdotELoneplusdsbtlbidsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRpteTdotELoneplusdsbtlbidsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRpteTdotELoneplusdsbtlbidsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRpteTdotELoneplusdsbtlbidsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoRpteTdotELoneplusdsbtlbidsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=0 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoRpteT.EL1+dsb-tlbi-dsb.tex <==
\newlength{\CoRpteTdotELoneplusdsbtlbidsbH}
\setlength{\CoRpteTdotELoneplusdsbtlbidsbH}{0cm}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbI}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTdotELoneplusdsbtlbidsbJ}
\settowidth{\CoRpteTdotELoneplusdsbtlbidsbJ}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbI}}
\addtolength{\CoRpteTdotELoneplusdsbtlbidsbH}{\CoRpteTdotELoneplusdsbtlbidsbJ}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbK}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
TLBI VAE1,X4
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTdotELoneplusdsbtlbidsbL}
\settowidth{\CoRpteTdotELoneplusdsbtlbidsbL}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbK}}
\addtolength{\CoRpteTdotELoneplusdsbtlbidsbH}{\CoRpteTdotELoneplusdsbtlbidsbL}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbM}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTdotELoneplusdsbtlbidsbN}
\settowidth{\CoRpteTdotELoneplusdsbtlbidsbN}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbM}}
\addtolength{\CoRpteTdotELoneplusdsbtlbidsbH}{\CoRpteTdotELoneplusdsbtlbidsbN}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbO}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;

    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;

    *pa1 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTdotELoneplusdsbtlbidsbP}
\settowidth{\CoRpteTdotELoneplusdsbtlbidsbP}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbO}}
\newsavebox{\CoRpteTdotELoneplusdsbtlbidsbA}
\begin{lrbox}{\CoRpteTdotELoneplusdsbtlbidsbA}
\begin{minipage}{\CoRpteTdotELoneplusdsbtlbidsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRpteT.EL1+dsb-tlbi-dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRpteTdotELoneplusdsbtlbidsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRpteTdotELoneplusdsbtlbidsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRpteTdotELoneplusdsbtlbidsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRpteTdotELoneplusdsbtlbidsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRpteTdotELoneplusdsbtlbidsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoRpteTdotELoneplusdsbtlbidsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=0 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoRpteTf.inv+dsb-isb.tex <==
\newlength{\CoRpteTfdotinvplusdsbisbH}
\setlength{\CoRpteTfdotinvplusdsbisbH}{0cm}
\newsavebox{\CoRpteTfdotinvplusdsbisbI}
\begin{lrbox}{\CoRpteTfdotinvplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTfdotinvplusdsbisbJ}
\settowidth{\CoRpteTfdotinvplusdsbisbJ}{\usebox{\CoRpteTfdotinvplusdsbisbI}}
\addtolength{\CoRpteTfdotinvplusdsbisbH}{\CoRpteTfdotinvplusdsbisbJ}
\newsavebox{\CoRpteTfdotinvplusdsbisbK}
\begin{lrbox}{\CoRpteTfdotinvplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTfdotinvplusdsbisbL}
\settowidth{\CoRpteTfdotinvplusdsbisbL}{\usebox{\CoRpteTfdotinvplusdsbisbK}}
\addtolength{\CoRpteTfdotinvplusdsbisbH}{\CoRpteTfdotinvplusdsbisbL}
\newsavebox{\CoRpteTfdotinvplusdsbisbM}
\begin{lrbox}{\CoRpteTfdotinvplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTfdotinvplusdsbisbN}
\settowidth{\CoRpteTfdotinvplusdsbisbN}{\usebox{\CoRpteTfdotinvplusdsbisbM}}
\addtolength{\CoRpteTfdotinvplusdsbisbH}{\CoRpteTfdotinvplusdsbisbN}
\newsavebox{\CoRpteTfdotinvplusdsbisbO}
\begin{lrbox}{\CoRpteTfdotinvplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    option default_tables = true;
    physical pa1;
    intermediate ipa1;

    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    identity 0x1000 with code;

    *pa1 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTfdotinvplusdsbisbP}
\settowidth{\CoRpteTfdotinvplusdsbisbP}{\usebox{\CoRpteTfdotinvplusdsbisbO}}
\newsavebox{\CoRpteTfdotinvplusdsbisbA}
\begin{lrbox}{\CoRpteTfdotinvplusdsbisbA}
\begin{minipage}{\CoRpteTfdotinvplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRpteTf.inv+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRpteTfdotinvplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRpteTfdotinvplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRpteTfdotinvplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRpteTfdotinvplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRpteTfdotinvplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoRpteTfdotinvplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=desc3(y,page_table_base) & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoRpteTf.inv+dsb.tex <==
\newlength{\CoRpteTfdotinvplusdsbH}
\setlength{\CoRpteTfdotinvplusdsbH}{0cm}
\newsavebox{\CoRpteTfdotinvplusdsbI}
\begin{lrbox}{\CoRpteTfdotinvplusdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTfdotinvplusdsbJ}
\settowidth{\CoRpteTfdotinvplusdsbJ}{\usebox{\CoRpteTfdotinvplusdsbI}}
\addtolength{\CoRpteTfdotinvplusdsbH}{\CoRpteTfdotinvplusdsbJ}
\newsavebox{\CoRpteTfdotinvplusdsbK}
\begin{lrbox}{\CoRpteTfdotinvplusdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTfdotinvplusdsbL}
\settowidth{\CoRpteTfdotinvplusdsbL}{\usebox{\CoRpteTfdotinvplusdsbK}}
\addtolength{\CoRpteTfdotinvplusdsbH}{\CoRpteTfdotinvplusdsbL}
\newsavebox{\CoRpteTfdotinvplusdsbM}
\begin{lrbox}{\CoRpteTfdotinvplusdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTfdotinvplusdsbN}
\settowidth{\CoRpteTfdotinvplusdsbN}{\usebox{\CoRpteTfdotinvplusdsbM}}
\addtolength{\CoRpteTfdotinvplusdsbH}{\CoRpteTfdotinvplusdsbN}
\newsavebox{\CoRpteTfdotinvplusdsbO}
\begin{lrbox}{\CoRpteTfdotinvplusdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    identity 0x1000 with code;

    *pa1 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\CoRpteTfdotinvplusdsbP}
\settowidth{\CoRpteTfdotinvplusdsbP}{\usebox{\CoRpteTfdotinvplusdsbO}}
\newsavebox{\CoRpteTfdotinvplusdsbA}
\begin{lrbox}{\CoRpteTfdotinvplusdsbA}
\begin{minipage}{\CoRpteTfdotinvplusdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoRpteTf.inv+dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoRpteTfdotinvplusdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoRpteTfdotinvplusdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoRpteTfdotinvplusdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoRpteTfdotinvplusdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoRpteTfdotinvplusdsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoRpteTfdotinvplusdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=desc3(y,page_table_base) & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoTRpte.inv+dsb-isb.tex <==
\newlength{\CoTRptedotinvplusdsbisbH}
\setlength{\CoTRptedotinvplusdsbisbH}{0cm}
\newsavebox{\CoTRptedotinvplusdsbisbI}
\begin{lrbox}{\CoTRptedotinvplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvplusdsbisbJ}
\settowidth{\CoTRptedotinvplusdsbisbJ}{\usebox{\CoTRptedotinvplusdsbisbI}}
\addtolength{\CoTRptedotinvplusdsbisbH}{\CoTRptedotinvplusdsbisbJ}
\newsavebox{\CoTRptedotinvplusdsbisbK}
\begin{lrbox}{\CoTRptedotinvplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvplusdsbisbL}
\settowidth{\CoTRptedotinvplusdsbisbL}{\usebox{\CoTRptedotinvplusdsbisbK}}
\addtolength{\CoTRptedotinvplusdsbisbH}{\CoTRptedotinvplusdsbisbL}
\newsavebox{\CoTRptedotinvplusdsbisbM}
\begin{lrbox}{\CoTRptedotinvplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvplusdsbisbN}
\settowidth{\CoTRptedotinvplusdsbisbN}{\usebox{\CoTRptedotinvplusdsbisbM}}
\addtolength{\CoTRptedotinvplusdsbisbH}{\CoTRptedotinvplusdsbisbN}
\newsavebox{\CoTRptedotinvplusdsbisbO}
\begin{lrbox}{\CoTRptedotinvplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvplusdsbisbP}
\settowidth{\CoTRptedotinvplusdsbisbP}{\usebox{\CoTRptedotinvplusdsbisbO}}
\newsavebox{\CoTRptedotinvplusdsbisbA}
\begin{lrbox}{\CoTRptedotinvplusdsbisbA}
\begin{minipage}{\CoTRptedotinvplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTRpte.inv+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTRptedotinvplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTRptedotinvplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTRptedotinvplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoTRpte.inv+dsb.tex <==
\newlength{\CoTRptedotinvplusdsbH}
\setlength{\CoTRptedotinvplusdsbH}{0cm}
\newsavebox{\CoTRptedotinvplusdsbI}
\begin{lrbox}{\CoTRptedotinvplusdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvplusdsbJ}
\settowidth{\CoTRptedotinvplusdsbJ}{\usebox{\CoTRptedotinvplusdsbI}}
\addtolength{\CoTRptedotinvplusdsbH}{\CoTRptedotinvplusdsbJ}
\newsavebox{\CoTRptedotinvplusdsbK}
\begin{lrbox}{\CoTRptedotinvplusdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvplusdsbL}
\settowidth{\CoTRptedotinvplusdsbL}{\usebox{\CoTRptedotinvplusdsbK}}
\addtolength{\CoTRptedotinvplusdsbH}{\CoTRptedotinvplusdsbL}
\newsavebox{\CoTRptedotinvplusdsbM}
\begin{lrbox}{\CoTRptedotinvplusdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvplusdsbN}
\settowidth{\CoTRptedotinvplusdsbN}{\usebox{\CoTRptedotinvplusdsbM}}
\addtolength{\CoTRptedotinvplusdsbH}{\CoTRptedotinvplusdsbN}
\newsavebox{\CoTRptedotinvplusdsbO}
\begin{lrbox}{\CoTRptedotinvplusdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *y = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvplusdsbP}
\settowidth{\CoTRptedotinvplusdsbP}{\usebox{\CoTRptedotinvplusdsbO}}
\newsavebox{\CoTRptedotinvplusdsbA}
\begin{lrbox}{\CoTRptedotinvplusdsbA}
\begin{minipage}{\CoTRptedotinvplusdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTRpte.inv+dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTRptedotinvplusdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTRptedotinvplusdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTRptedotinvplusdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvplusdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvplusdsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvplusdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoTRpte.inv+po.tex <==
\newlength{\CoTRptedotinvpluspoH}
\setlength{\CoTRptedotinvpluspoH}{0cm}
\newsavebox{\CoTRptedotinvpluspoI}
\begin{lrbox}{\CoTRptedotinvpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvpluspoJ}
\settowidth{\CoTRptedotinvpluspoJ}{\usebox{\CoTRptedotinvpluspoI}}
\addtolength{\CoTRptedotinvpluspoH}{\CoTRptedotinvpluspoJ}
\newsavebox{\CoTRptedotinvpluspoK}
\begin{lrbox}{\CoTRptedotinvpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvpluspoL}
\settowidth{\CoTRptedotinvpluspoL}{\usebox{\CoTRptedotinvpluspoK}}
\addtolength{\CoTRptedotinvpluspoH}{\CoTRptedotinvpluspoL}
\newsavebox{\CoTRptedotinvpluspoM}
\begin{lrbox}{\CoTRptedotinvpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvpluspoN}
\settowidth{\CoTRptedotinvpluspoN}{\usebox{\CoTRptedotinvpluspoM}}
\addtolength{\CoTRptedotinvpluspoH}{\CoTRptedotinvpluspoN}
\newsavebox{\CoTRptedotinvpluspoO}
\begin{lrbox}{\CoTRptedotinvpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *y = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTRptedotinvpluspoP}
\settowidth{\CoTRptedotinvpluspoP}{\usebox{\CoTRptedotinvpluspoO}}
\newsavebox{\CoTRptedotinvpluspoA}
\begin{lrbox}{\CoTRptedotinvpluspoA}
\begin{minipage}{\CoTRptedotinvpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTRpte.inv+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTRptedotinvpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTRptedotinvpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTRptedotinvpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTRptedotinvpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoTT.ro+dmb.tex <==
\newlength{\CoTTdotroplusdmbH}
\setlength{\CoTTdotroplusdmbH}{0cm}
\newsavebox{\CoTTdotroplusdmbI}
\begin{lrbox}{\CoTTdotroplusdmbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotroplusdmbJ}
\settowidth{\CoTTdotroplusdmbJ}{\usebox{\CoTTdotroplusdmbI}}
\addtolength{\CoTTdotroplusdmbH}{\CoTTdotroplusdmbJ}
\newsavebox{\CoTTdotroplusdmbK}
\begin{lrbox}{\CoTTdotroplusdmbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotroplusdmbL}
\settowidth{\CoTTdotroplusdmbL}{\usebox{\CoTTdotroplusdmbK}}
\addtolength{\CoTTdotroplusdmbH}{\CoTTdotroplusdmbL}
\newsavebox{\CoTTdotroplusdmbM}
\begin{lrbox}{\CoTTdotroplusdmbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1 with [AP = 0b11] and default;
    x ?-> pa2 with [AP = 0b11] and default;
    y |-> pa2 with [AP = 0b11] and default;

    *pa2 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotroplusdmbN}
\settowidth{\CoTTdotroplusdmbN}{\usebox{\CoTTdotroplusdmbM}}
\newsavebox{\CoTTdotroplusdmbO}
\begin{lrbox}{\CoTTdotroplusdmbO}
\begin{minipage}{\CoTTdotroplusdmbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTT.ro+dmb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTTdotroplusdmbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTTdotroplusdmbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTTdotroplusdmbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTTdotroplusdmbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTTdotroplusdmbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoTT.ro+dsb-isb.tex <==
\newlength{\CoTTdotroplusdsbisbH}
\setlength{\CoTTdotroplusdsbisbH}{0cm}
\newsavebox{\CoTTdotroplusdsbisbI}
\begin{lrbox}{\CoTTdotroplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotroplusdsbisbJ}
\settowidth{\CoTTdotroplusdsbisbJ}{\usebox{\CoTTdotroplusdsbisbI}}
\addtolength{\CoTTdotroplusdsbisbH}{\CoTTdotroplusdsbisbJ}
\newsavebox{\CoTTdotroplusdsbisbK}
\begin{lrbox}{\CoTTdotroplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotroplusdsbisbL}
\settowidth{\CoTTdotroplusdsbisbL}{\usebox{\CoTTdotroplusdsbisbK}}
\addtolength{\CoTTdotroplusdsbisbH}{\CoTTdotroplusdsbisbL}
\newsavebox{\CoTTdotroplusdsbisbM}
\begin{lrbox}{\CoTTdotroplusdsbisbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1 with [AP = 0b11] and default;
    x ?-> pa2 with [AP = 0b11] and default;
    y |-> pa2 with [AP = 0b11] and default;

    *pa2 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotroplusdsbisbN}
\settowidth{\CoTTdotroplusdsbisbN}{\usebox{\CoTTdotroplusdsbisbM}}
\newsavebox{\CoTTdotroplusdsbisbO}
\begin{lrbox}{\CoTTdotroplusdsbisbO}
\begin{minipage}{\CoTTdotroplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTT.ro+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTTdotroplusdsbisbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTTdotroplusdsbisbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTTdotroplusdsbisbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTTdotroplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTTdotroplusdsbisbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoTT.ro+po.tex <==
\newlength{\CoTTdotropluspoH}
\setlength{\CoTTdotropluspoH}{0cm}
\newsavebox{\CoTTdotropluspoI}
\begin{lrbox}{\CoTTdotropluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotropluspoJ}
\settowidth{\CoTTdotropluspoJ}{\usebox{\CoTTdotropluspoI}}
\addtolength{\CoTTdotropluspoH}{\CoTTdotropluspoJ}
\newsavebox{\CoTTdotropluspoK}
\begin{lrbox}{\CoTTdotropluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotropluspoL}
\settowidth{\CoTTdotropluspoL}{\usebox{\CoTTdotropluspoK}}
\addtolength{\CoTTdotropluspoH}{\CoTTdotropluspoL}
\newsavebox{\CoTTdotropluspoM}
\begin{lrbox}{\CoTTdotropluspoM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1 with [AP = 0b11] and default;
    x ?-> pa2 with [AP = 0b11] and default;
    y |-> pa2 with [AP = 0b11] and default;

    *pa2 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTdotropluspoN}
\settowidth{\CoTTdotropluspoN}{\usebox{\CoTTdotropluspoM}}
\newsavebox{\CoTTdotropluspoO}
\begin{lrbox}{\CoTTdotropluspoO}
\begin{minipage}{\CoTTdotropluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTT.ro+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTTdotropluspoN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTTdotropluspoM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTTdotropluspoO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTTdotropluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTTdotropluspoK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoTTf.inv+dsb-isb.tex <==
\newlength{\CoTTfdotinvplusdsbisbH}
\setlength{\CoTTfdotinvplusdsbisbH}{0cm}
\newsavebox{\CoTTfdotinvplusdsbisbI}
\begin{lrbox}{\CoTTfdotinvplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTfdotinvplusdsbisbJ}
\settowidth{\CoTTfdotinvplusdsbisbJ}{\usebox{\CoTTfdotinvplusdsbisbI}}
\addtolength{\CoTTfdotinvplusdsbisbH}{\CoTTfdotinvplusdsbisbJ}
\newsavebox{\CoTTfdotinvplusdsbisbK}
\begin{lrbox}{\CoTTfdotinvplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTfdotinvplusdsbisbL}
\settowidth{\CoTTfdotinvplusdsbisbL}{\usebox{\CoTTfdotinvplusdsbisbK}}
\addtolength{\CoTTfdotinvplusdsbisbH}{\CoTTfdotinvplusdsbisbL}
\newsavebox{\CoTTfdotinvplusdsbisbM}
\begin{lrbox}{\CoTTfdotinvplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTfdotinvplusdsbisbN}
\settowidth{\CoTTfdotinvplusdsbisbN}{\usebox{\CoTTfdotinvplusdsbisbM}}
\addtolength{\CoTTfdotinvplusdsbisbH}{\CoTTfdotinvplusdsbisbN}
\newsavebox{\CoTTfdotinvplusdsbisbO}
\begin{lrbox}{\CoTTfdotinvplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTfdotinvplusdsbisbP}
\settowidth{\CoTTfdotinvplusdsbisbP}{\usebox{\CoTTfdotinvplusdsbisbO}}
\newsavebox{\CoTTfdotinvplusdsbisbA}
\begin{lrbox}{\CoTTfdotinvplusdsbisbA}
\begin{minipage}{\CoTTfdotinvplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTTf.inv+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTTfdotinvplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTTfdotinvplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTTfdotinvplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTTfdotinvplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTTfdotinvplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTTfdotinvplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoTTf.inv+po.tex <==
\newlength{\CoTTfdotinvpluspoH}
\setlength{\CoTTfdotinvpluspoH}{0cm}
\newsavebox{\CoTTfdotinvpluspoI}
\begin{lrbox}{\CoTTfdotinvpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTfdotinvpluspoJ}
\settowidth{\CoTTfdotinvpluspoJ}{\usebox{\CoTTfdotinvpluspoI}}
\addtolength{\CoTTfdotinvpluspoH}{\CoTTfdotinvpluspoJ}
\newsavebox{\CoTTfdotinvpluspoK}
\begin{lrbox}{\CoTTfdotinvpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTfdotinvpluspoL}
\settowidth{\CoTTfdotinvpluspoL}{\usebox{\CoTTfdotinvpluspoK}}
\addtolength{\CoTTfdotinvpluspoH}{\CoTTfdotinvpluspoL}
\newsavebox{\CoTTfdotinvpluspoM}
\begin{lrbox}{\CoTTfdotinvpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTfdotinvpluspoN}
\settowidth{\CoTTfdotinvpluspoN}{\usebox{\CoTTfdotinvpluspoM}}
\addtolength{\CoTTfdotinvpluspoH}{\CoTTfdotinvpluspoN}
\newsavebox{\CoTTfdotinvpluspoO}
\begin{lrbox}{\CoTTfdotinvpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTTfdotinvpluspoP}
\settowidth{\CoTTfdotinvpluspoP}{\usebox{\CoTTfdotinvpluspoO}}
\newsavebox{\CoTTfdotinvpluspoA}
\begin{lrbox}{\CoTTfdotinvpluspoA}
\begin{minipage}{\CoTTfdotinvpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTTf.inv+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTTfdotinvpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTTfdotinvpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTTfdotinvpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTTfdotinvpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTTfdotinvpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTTfdotinvpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoTWinv.tex <==
\newlength{\CoTWinvH}
\setlength{\CoTWinvH}{0cm}
\newsavebox{\CoTWinvI}
\begin{lrbox}{\CoTWinvI}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTWinvJ}
\settowidth{\CoTWinvJ}{\usebox{\CoTWinvI}}
\addtolength{\CoTWinvH}{\CoTWinvJ}
\newsavebox{\CoTWinvK}
\begin{lrbox}{\CoTWinvK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTWinvL}
\settowidth{\CoTWinvL}{\usebox{\CoTWinvK}}
\addtolength{\CoTWinvH}{\CoTWinvL}
\newsavebox{\CoTWinvM}
\begin{lrbox}{\CoTWinvM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTWinvN}
\settowidth{\CoTWinvN}{\usebox{\CoTWinvM}}
\newsavebox{\CoTWinvO}
\begin{lrbox}{\CoTWinvO}
\begin{minipage}{\CoTWinvH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=x|\\
\lstinline[language=IslaLitmusExp]|R2=0b0|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTWinv|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTWinvN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTWinvM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTWinvO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTWinvI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTWinvK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoTfRpte+dsb-isb.tex <==
\newlength{\CoTfRpteplusdsbisbH}
\setlength{\CoTfRpteplusdsbisbH}{0cm}
\newsavebox{\CoTfRpteplusdsbisbI}
\begin{lrbox}{\CoTfRpteplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRpteplusdsbisbJ}
\settowidth{\CoTfRpteplusdsbisbJ}{\usebox{\CoTfRpteplusdsbisbI}}
\addtolength{\CoTfRpteplusdsbisbH}{\CoTfRpteplusdsbisbJ}
\newsavebox{\CoTfRpteplusdsbisbK}
\begin{lrbox}{\CoTfRpteplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRpteplusdsbisbL}
\settowidth{\CoTfRpteplusdsbisbL}{\usebox{\CoTfRpteplusdsbisbK}}
\addtolength{\CoTfRpteplusdsbisbH}{\CoTfRpteplusdsbisbL}
\newsavebox{\CoTfRpteplusdsbisbM}
\begin{lrbox}{\CoTfRpteplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRpteplusdsbisbN}
\settowidth{\CoTfRpteplusdsbisbN}{\usebox{\CoTfRpteplusdsbisbM}}
\addtolength{\CoTfRpteplusdsbisbH}{\CoTfRpteplusdsbisbN}
\newsavebox{\CoTfRpteplusdsbisbO}
\begin{lrbox}{\CoTfRpteplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;
    y |-> pa1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRpteplusdsbisbP}
\settowidth{\CoTfRpteplusdsbisbP}{\usebox{\CoTfRpteplusdsbisbO}}
\newsavebox{\CoTfRpteplusdsbisbA}
\begin{lrbox}{\CoTfRpteplusdsbisbA}
\begin{minipage}{\CoTfRpteplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfRpte+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfRpteplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfRpteplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfRpteplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfRpteplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTfRpteplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfRpteplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=desc3(y,page_table_base)|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoTfRpte+dsb.tex <==
\newlength{\CoTfRpteplusdsbH}
\setlength{\CoTfRpteplusdsbH}{0cm}
\newsavebox{\CoTfRpteplusdsbI}
\begin{lrbox}{\CoTfRpteplusdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRpteplusdsbJ}
\settowidth{\CoTfRpteplusdsbJ}{\usebox{\CoTfRpteplusdsbI}}
\addtolength{\CoTfRpteplusdsbH}{\CoTfRpteplusdsbJ}
\newsavebox{\CoTfRpteplusdsbK}
\begin{lrbox}{\CoTfRpteplusdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRpteplusdsbL}
\settowidth{\CoTfRpteplusdsbL}{\usebox{\CoTfRpteplusdsbK}}
\addtolength{\CoTfRpteplusdsbH}{\CoTfRpteplusdsbL}
\newsavebox{\CoTfRpteplusdsbM}
\begin{lrbox}{\CoTfRpteplusdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRpteplusdsbN}
\settowidth{\CoTfRpteplusdsbN}{\usebox{\CoTfRpteplusdsbM}}
\addtolength{\CoTfRpteplusdsbH}{\CoTfRpteplusdsbN}
\newsavebox{\CoTfRpteplusdsbO}
\begin{lrbox}{\CoTfRpteplusdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;
    y |-> pa1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRpteplusdsbP}
\settowidth{\CoTfRpteplusdsbP}{\usebox{\CoTfRpteplusdsbO}}
\newsavebox{\CoTfRpteplusdsbA}
\begin{lrbox}{\CoTfRpteplusdsbA}
\begin{minipage}{\CoTfRpteplusdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfRpte+dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfRpteplusdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfRpteplusdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfRpteplusdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfRpteplusdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTfRpteplusdsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfRpteplusdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=desc3(y,page_table_base)|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoTfRpte+eret.tex <==
\newlength{\CoTfRptepluseretH}
\setlength{\CoTfRptepluseretH}{0cm}
\newsavebox{\CoTfRptepluseretI}
\begin{lrbox}{\CoTfRptepluseretI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRptepluseretJ}
\settowidth{\CoTfRptepluseretJ}{\usebox{\CoTfRptepluseretI}}
\addtolength{\CoTfRptepluseretH}{\CoTfRptepluseretJ}
\newsavebox{\CoTfRptepluseretK}
\begin{lrbox}{\CoTfRptepluseretK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRptepluseretL}
\settowidth{\CoTfRptepluseretL}{\usebox{\CoTfRptepluseretK}}
\addtolength{\CoTfRptepluseretH}{\CoTfRptepluseretL}
\newsavebox{\CoTfRptepluseretM}
\begin{lrbox}{\CoTfRptepluseretM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRptepluseretN}
\settowidth{\CoTfRptepluseretN}{\usebox{\CoTfRptepluseretM}}
\addtolength{\CoTfRptepluseretH}{\CoTfRptepluseretN}
\newsavebox{\CoTfRptepluseretO}
\begin{lrbox}{\CoTfRptepluseretO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;
    y |-> pa1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRptepluseretP}
\settowidth{\CoTfRptepluseretP}{\usebox{\CoTfRptepluseretO}}
\newsavebox{\CoTfRptepluseretA}
\begin{lrbox}{\CoTfRptepluseretA}
\begin{minipage}{\CoTfRptepluseretH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfRpte+eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfRptepluseretP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfRptepluseretO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfRptepluseretA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfRptepluseretI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTfRptepluseretK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfRptepluseretM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=desc3(y,page_table_base)|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoTfRpte+po.tex <==
\newlength{\CoTfRptepluspoH}
\setlength{\CoTfRptepluspoH}{0cm}
\newsavebox{\CoTfRptepluspoI}
\begin{lrbox}{\CoTfRptepluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRptepluspoJ}
\settowidth{\CoTfRptepluspoJ}{\usebox{\CoTfRptepluspoI}}
\addtolength{\CoTfRptepluspoH}{\CoTfRptepluspoJ}
\newsavebox{\CoTfRptepluspoK}
\begin{lrbox}{\CoTfRptepluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRptepluspoL}
\settowidth{\CoTfRptepluspoL}{\usebox{\CoTfRptepluspoK}}
\addtolength{\CoTfRptepluspoH}{\CoTfRptepluspoL}
\newsavebox{\CoTfRptepluspoM}
\begin{lrbox}{\CoTfRptepluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRptepluspoN}
\settowidth{\CoTfRptepluspoN}{\usebox{\CoTfRptepluspoM}}
\addtolength{\CoTfRptepluspoH}{\CoTfRptepluspoN}
\newsavebox{\CoTfRptepluspoO}
\begin{lrbox}{\CoTfRptepluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;
    y |-> pa1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfRptepluspoP}
\settowidth{\CoTfRptepluspoP}{\usebox{\CoTfRptepluspoO}}
\newsavebox{\CoTfRptepluspoA}
\begin{lrbox}{\CoTfRptepluspoA}
\begin{minipage}{\CoTfRptepluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfRpte+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfRptepluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfRptepluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfRptepluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfRptepluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTfRptepluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfRptepluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=desc3(y,page_table_base)|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoTfT+dsb-isb.tex <==
\newlength{\CoTfTplusdsbisbH}
\setlength{\CoTfTplusdsbisbH}{0cm}
\newsavebox{\CoTfTplusdsbisbI}
\begin{lrbox}{\CoTfTplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfTplusdsbisbJ}
\settowidth{\CoTfTplusdsbisbJ}{\usebox{\CoTfTplusdsbisbI}}
\addtolength{\CoTfTplusdsbisbH}{\CoTfTplusdsbisbJ}
\newsavebox{\CoTfTplusdsbisbK}
\begin{lrbox}{\CoTfTplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfTplusdsbisbL}
\settowidth{\CoTfTplusdsbisbL}{\usebox{\CoTfTplusdsbisbK}}
\addtolength{\CoTfTplusdsbisbH}{\CoTfTplusdsbisbL}
\newsavebox{\CoTfTplusdsbisbM}
\begin{lrbox}{\CoTfTplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfTplusdsbisbN}
\settowidth{\CoTfTplusdsbisbN}{\usebox{\CoTfTplusdsbisbM}}
\addtolength{\CoTfTplusdsbisbH}{\CoTfTplusdsbisbN}
\newsavebox{\CoTfTplusdsbisbO}
\begin{lrbox}{\CoTfTplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;
    y |-> pa1;
    *pa1 = 0;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfTplusdsbisbP}
\settowidth{\CoTfTplusdsbisbP}{\usebox{\CoTfTplusdsbisbO}}
\newsavebox{\CoTfTplusdsbisbA}
\begin{lrbox}{\CoTfTplusdsbisbA}
\begin{minipage}{\CoTfTplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfT+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfTplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfTplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfTplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfTplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTfTplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfTplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoTfT+po.tex <==
\newlength{\CoTfTpluspoH}
\setlength{\CoTfTpluspoH}{0cm}
\newsavebox{\CoTfTpluspoI}
\begin{lrbox}{\CoTfTpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfTpluspoJ}
\settowidth{\CoTfTpluspoJ}{\usebox{\CoTfTpluspoI}}
\addtolength{\CoTfTpluspoH}{\CoTfTpluspoJ}
\newsavebox{\CoTfTpluspoK}
\begin{lrbox}{\CoTfTpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfTpluspoL}
\settowidth{\CoTfTpluspoL}{\usebox{\CoTfTpluspoK}}
\addtolength{\CoTfTpluspoH}{\CoTfTpluspoL}
\newsavebox{\CoTfTpluspoM}
\begin{lrbox}{\CoTfTpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfTpluspoN}
\settowidth{\CoTfTpluspoN}{\usebox{\CoTfTpluspoM}}
\addtolength{\CoTfTpluspoH}{\CoTfTpluspoN}
\newsavebox{\CoTfTpluspoO}
\begin{lrbox}{\CoTfTpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;
    y |-> pa1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfTpluspoP}
\settowidth{\CoTfTpluspoP}{\usebox{\CoTfTpluspoO}}
\newsavebox{\CoTfTpluspoA}
\begin{lrbox}{\CoTfTpluspoA}
\begin{minipage}{\CoTfTpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfT+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfTpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfTpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfTpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfTpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTfTpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfTpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoTfW.inv+dsb-isb.tex <==
\newlength{\CoTfWdotinvplusdsbisbH}
\setlength{\CoTfWdotinvplusdsbisbH}{0cm}
\newsavebox{\CoTfWdotinvplusdsbisbI}
\begin{lrbox}{\CoTfWdotinvplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvplusdsbisbJ}
\settowidth{\CoTfWdotinvplusdsbisbJ}{\usebox{\CoTfWdotinvplusdsbisbI}}
\addtolength{\CoTfWdotinvplusdsbisbH}{\CoTfWdotinvplusdsbisbJ}
\newsavebox{\CoTfWdotinvplusdsbisbK}
\begin{lrbox}{\CoTfWdotinvplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvplusdsbisbL}
\settowidth{\CoTfWdotinvplusdsbisbL}{\usebox{\CoTfWdotinvplusdsbisbK}}
\addtolength{\CoTfWdotinvplusdsbisbH}{\CoTfWdotinvplusdsbisbL}
\newsavebox{\CoTfWdotinvplusdsbisbM}
\begin{lrbox}{\CoTfWdotinvplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvplusdsbisbN}
\settowidth{\CoTfWdotinvplusdsbisbN}{\usebox{\CoTfWdotinvplusdsbisbM}}
\addtolength{\CoTfWdotinvplusdsbisbH}{\CoTfWdotinvplusdsbisbN}
\newsavebox{\CoTfWdotinvplusdsbisbO}
\begin{lrbox}{\CoTfWdotinvplusdsbisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvplusdsbisbP}
\settowidth{\CoTfWdotinvplusdsbisbP}{\usebox{\CoTfWdotinvplusdsbisbO}}
\addtolength{\CoTfWdotinvplusdsbisbH}{\CoTfWdotinvplusdsbisbP}
\newsavebox{\CoTfWdotinvplusdsbisbA}
\begin{lrbox}{\CoTfWdotinvplusdsbisbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    x ?-> raw(2);
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvplusdsbisbB}
\settowidth{\CoTfWdotinvplusdsbisbB}{\usebox{\CoTfWdotinvplusdsbisbA}}
\newsavebox{\CoTfWdotinvplusdsbisbC}
\begin{lrbox}{\CoTfWdotinvplusdsbisbC}
\begin{minipage}{\CoTfWdotinvplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b10|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:R1=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfW.inv+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfWdotinvplusdsbisbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfWdotinvplusdsbisbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfWdotinvplusdsbisbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfWdotinvplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTfWdotinvplusdsbisbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\CoTfWdotinvplusdsbisbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfWdotinvplusdsbisbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=2 & 2:R2=mkdesc3(oa=pa1)|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoTfW.inv+po.tex <==
\newlength{\CoTfWdotinvpluspoH}
\setlength{\CoTfWdotinvpluspoH}{0cm}
\newsavebox{\CoTfWdotinvpluspoI}
\begin{lrbox}{\CoTfWdotinvpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvpluspoJ}
\settowidth{\CoTfWdotinvpluspoJ}{\usebox{\CoTfWdotinvpluspoI}}
\addtolength{\CoTfWdotinvpluspoH}{\CoTfWdotinvpluspoJ}
\newsavebox{\CoTfWdotinvpluspoK}
\begin{lrbox}{\CoTfWdotinvpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvpluspoL}
\settowidth{\CoTfWdotinvpluspoL}{\usebox{\CoTfWdotinvpluspoK}}
\addtolength{\CoTfWdotinvpluspoH}{\CoTfWdotinvpluspoL}
\newsavebox{\CoTfWdotinvpluspoM}
\begin{lrbox}{\CoTfWdotinvpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvpluspoN}
\settowidth{\CoTfWdotinvpluspoN}{\usebox{\CoTfWdotinvpluspoM}}
\addtolength{\CoTfWdotinvpluspoH}{\CoTfWdotinvpluspoN}
\newsavebox{\CoTfWdotinvpluspoO}
\begin{lrbox}{\CoTfWdotinvpluspoO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvpluspoP}
\settowidth{\CoTfWdotinvpluspoP}{\usebox{\CoTfWdotinvpluspoO}}
\addtolength{\CoTfWdotinvpluspoH}{\CoTfWdotinvpluspoP}
\newsavebox{\CoTfWdotinvpluspoA}
\begin{lrbox}{\CoTfWdotinvpluspoA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    x ?-> raw(2);
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWdotinvpluspoB}
\settowidth{\CoTfWdotinvpluspoB}{\usebox{\CoTfWdotinvpluspoA}}
\newsavebox{\CoTfWdotinvpluspoC}
\begin{lrbox}{\CoTfWdotinvpluspoC}
\begin{minipage}{\CoTfWdotinvpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b10|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:R1=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfW.inv+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfWdotinvpluspoB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfWdotinvpluspoA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfWdotinvpluspoC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfWdotinvpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoTfWdotinvpluspoK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\CoTfWdotinvpluspoM}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfWdotinvpluspoO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=2 & 2:R2=mkdesc3(oa=pa1)|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoTfW1.inv+si.tex <==
\newlength{\CoTfWonedotinvplussiH}
\setlength{\CoTfWonedotinvplussiH}{0cm}
\newsavebox{\CoTfWonedotinvplussiI}
\begin{lrbox}{\CoTfWonedotinvplussiI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWonedotinvplussiJ}
\settowidth{\CoTfWonedotinvplussiJ}{\usebox{\CoTfWonedotinvplussiI}}
\addtolength{\CoTfWonedotinvplussiH}{\CoTfWonedotinvplussiJ}
\newsavebox{\CoTfWonedotinvplussiK}
\begin{lrbox}{\CoTfWonedotinvplussiK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWonedotinvplussiL}
\settowidth{\CoTfWonedotinvplussiL}{\usebox{\CoTfWonedotinvplussiK}}
\addtolength{\CoTfWonedotinvplussiH}{\CoTfWonedotinvplussiL}
\newsavebox{\CoTfWonedotinvplussiM}
\begin{lrbox}{\CoTfWonedotinvplussiM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoTfWonedotinvplussiN}
\settowidth{\CoTfWonedotinvplussiN}{\usebox{\CoTfWonedotinvplussiM}}
\newsavebox{\CoTfWonedotinvplussiO}
\begin{lrbox}{\CoTfWonedotinvplussiO}
\begin{minipage}{\CoTfWonedotinvplussiH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=0b10|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(0x1000,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoTfW1.inv+si|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoTfWonedotinvplussiN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoTfWonedotinvplussiM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoTfWonedotinvplussiO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoTfWonedotinvplussiI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoTfWonedotinvplussiK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R0=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoWR.alias.tex <==
\newlength{\CoWRdotaliasH}
\setlength{\CoWRdotaliasH}{0cm}
\newsavebox{\CoWRdotaliasI}
\begin{lrbox}{\CoWRdotaliasI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWRdotaliasJ}
\settowidth{\CoWRdotaliasJ}{\usebox{\CoWRdotaliasI}}
\addtolength{\CoWRdotaliasH}{\CoWRdotaliasJ}
\newsavebox{\CoWRdotaliasK}
\begin{lrbox}{\CoWRdotaliasK}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    y |-> pa1;
    *pa1 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWRdotaliasL}
\settowidth{\CoWRdotaliasL}{\usebox{\CoWRdotaliasK}}
\newsavebox{\CoWRdotaliasM}
\begin{lrbox}{\CoWRdotaliasM}
\begin{minipage}{\CoWRdotaliasH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|R0=0x1|\\
\lstinline[language=IslaLitmusExp]|R1=x|\\
\lstinline[language=IslaLitmusExp]|R3=y|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWR.alias|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWRdotaliasL}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWRdotaliasK}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWRdotaliasM}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWRdotaliasI}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoWR.inv.tex <==
\newlength{\CoWRdotinvH}
\setlength{\CoWRdotinvH}{0cm}
\newsavebox{\CoWRdotinvI}
\begin{lrbox}{\CoWRdotinvI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWRdotinvJ}
\settowidth{\CoWRdotinvJ}{\usebox{\CoWRdotinvI}}
\addtolength{\CoWRdotinvH}{\CoWRdotinvJ}
\newsavebox{\CoWRdotinvK}
\begin{lrbox}{\CoWRdotinvK}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWRdotinvL}
\settowidth{\CoWRdotinvL}{\usebox{\CoWRdotinvK}}
\newsavebox{\CoWRdotinvM}
\begin{lrbox}{\CoWRdotinvM}
\begin{minipage}{\CoWRdotinvH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWR.inv|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWRdotinvL}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWRdotinvK}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWRdotinvM}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWRdotinvI}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoWTa1.1.inv+dsb-tlbiasidis-dsb-eret.tex <==
\newlength{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetH}
\setlength{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetH}{0cm}
\newsavebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetI}
\begin{lrbox}{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI ASIDE1IS,X4
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetJ}
\settowidth{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetJ}{\usebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetI}}
\addtolength{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetH}{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetJ}
\newsavebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetK}
\begin{lrbox}{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetL}
\settowidth{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetL}{\usebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetK}}
\addtolength{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetH}{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetL}
\newsavebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetM}
\begin{lrbox}{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;

    y |-> pa1;

    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetN}
\settowidth{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetN}{\usebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetM}}
\newsavebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetO}
\begin{lrbox}{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetO}
\begin{minipage}{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL1=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=asid(0x1)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL1=0b00000|\\
\lstinline[language=IslaLitmusExp]|TTBR0_EL1=ttbr(asid=0x0001,base=page_table_base)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTa1.1.inv+dsb-tlbiasidis-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTaonedotonedotinvplusdsbtlbiasidisdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoWTa2.1.inv+dsb-tlbiasidis-dsb-eret.tex <==
\newlength{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetH}
\setlength{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetH}{0cm}
\newsavebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetI}
\begin{lrbox}{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI ASIDE1IS,X4
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetJ}
\settowidth{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetJ}{\usebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetI}}
\addtolength{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetH}{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetJ}
\newsavebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetK}
\begin{lrbox}{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetL}
\settowidth{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetL}{\usebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetK}}
\addtolength{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetH}{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetL}
\newsavebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetM}
\begin{lrbox}{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;

    y |-> pa1;

    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetN}
\settowidth{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetN}{\usebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetM}}
\newsavebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetO}
\begin{lrbox}{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetO}
\begin{minipage}{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL1=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=asid(0x2)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL1=0b00000|\\
\lstinline[language=IslaLitmusExp]|TTBR0_EL1=ttbr(asid=0x0001,base=page_table_base)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTa2.1.inv+dsb-tlbiasidis-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTatwodotonedotinvplusdsbtlbiasidisdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoWTf.inv+_dmb_-dmb-addr.tex <==
\newlength{\CoWTfdotinvplus[dmb]dmbaddrH}
\setlength{\CoWTfdotinvplus[dmb]dmbaddrH}{0cm}
\newsavebox{\CoWTfdotinvplus[dmb]dmbaddrI}
\begin{lrbox}{\CoWTfdotinvplus[dmb]dmbaddrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X2,[X1]
DSB ST
LDR X3,[X4]
EOR X5,X3,X3
LDR X6,[X7,X5]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplus[dmb]dmbaddrJ}
\settowidth{\CoWTfdotinvplus[dmb]dmbaddrJ}{\usebox{\CoWTfdotinvplus[dmb]dmbaddrI}}
\addtolength{\CoWTfdotinvplus[dmb]dmbaddrH}{\CoWTfdotinvplus[dmb]dmbaddrJ}
\newsavebox{\CoWTfdotinvplus[dmb]dmbaddrK}
\begin{lrbox}{\CoWTfdotinvplus[dmb]dmbaddrK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplus[dmb]dmbaddrL}
\settowidth{\CoWTfdotinvplus[dmb]dmbaddrL}{\usebox{\CoWTfdotinvplus[dmb]dmbaddrK}}
\addtolength{\CoWTfdotinvplus[dmb]dmbaddrH}{\CoWTfdotinvplus[dmb]dmbaddrL}
\newsavebox{\CoWTfdotinvplus[dmb]dmbaddrM}
\begin{lrbox}{\CoWTfdotinvplus[dmb]dmbaddrM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X6,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplus[dmb]dmbaddrN}
\settowidth{\CoWTfdotinvplus[dmb]dmbaddrN}{\usebox{\CoWTfdotinvplus[dmb]dmbaddrM}}
\addtolength{\CoWTfdotinvplus[dmb]dmbaddrH}{\CoWTfdotinvplus[dmb]dmbaddrN}
\newsavebox{\CoWTfdotinvplus[dmb]dmbaddrO}
\begin{lrbox}{\CoWTfdotinvplus[dmb]dmbaddrO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplus[dmb]dmbaddrP}
\settowidth{\CoWTfdotinvplus[dmb]dmbaddrP}{\usebox{\CoWTfdotinvplus[dmb]dmbaddrO}}
\newsavebox{\CoWTfdotinvplus[dmb]dmbaddrA}
\begin{lrbox}{\CoWTfdotinvplus[dmb]dmbaddrA}
\begin{minipage}{\CoWTfdotinvplus[dmb]dmbaddrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R4=y|\\
\lstinline[language=IslaLitmusExp]|0:R7=x|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+[dmb]-dmb-addr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvplus[dmb]dmbaddrP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvplus[dmb]dmbaddrO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvplus[dmb]dmbaddrA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplus[dmb]dmbaddrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplus[dmb]dmbaddrK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplus[dmb]dmbaddrM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R3=2 & 0:R6=0 & 1:R0=desc3(z,page_table_base)|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoWTf.inv+dsb-isb.tex <==
\newlength{\CoWTfdotinvplusdsbisbH}
\setlength{\CoWTfdotinvplusdsbisbH}{0cm}
\newsavebox{\CoWTfdotinvplusdsbisbI}
\begin{lrbox}{\CoWTfdotinvplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusdsbisbJ}
\settowidth{\CoWTfdotinvplusdsbisbJ}{\usebox{\CoWTfdotinvplusdsbisbI}}
\addtolength{\CoWTfdotinvplusdsbisbH}{\CoWTfdotinvplusdsbisbJ}
\newsavebox{\CoWTfdotinvplusdsbisbK}
\begin{lrbox}{\CoWTfdotinvplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusdsbisbL}
\settowidth{\CoWTfdotinvplusdsbisbL}{\usebox{\CoWTfdotinvplusdsbisbK}}
\addtolength{\CoWTfdotinvplusdsbisbH}{\CoWTfdotinvplusdsbisbL}
\newsavebox{\CoWTfdotinvplusdsbisbM}
\begin{lrbox}{\CoWTfdotinvplusdsbisbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusdsbisbN}
\settowidth{\CoWTfdotinvplusdsbisbN}{\usebox{\CoWTfdotinvplusdsbisbM}}
\newsavebox{\CoWTfdotinvplusdsbisbO}
\begin{lrbox}{\CoWTfdotinvplusdsbisbO}
\begin{minipage}{\CoWTfdotinvplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvplusdsbisbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvplusdsbisbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvplusdsbisbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplusdsbisbI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplusdsbisbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoWTf.inv+po-ctrl+po.tex <==
\newlength{\CoWTfdotinvpluspoctrlpluspoH}
\setlength{\CoWTfdotinvpluspoctrlpluspoH}{0cm}
\newsavebox{\CoWTfdotinvpluspoctrlpluspoI}
\begin{lrbox}{\CoWTfdotinvpluspoctrlpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
CBNZ X2,L0
L0:
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlpluspoJ}
\settowidth{\CoWTfdotinvpluspoctrlpluspoJ}{\usebox{\CoWTfdotinvpluspoctrlpluspoI}}
\addtolength{\CoWTfdotinvpluspoctrlpluspoH}{\CoWTfdotinvpluspoctrlpluspoJ}
\newsavebox{\CoWTfdotinvpluspoctrlpluspoK}
\begin{lrbox}{\CoWTfdotinvpluspoctrlpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlpluspoL}
\settowidth{\CoWTfdotinvpluspoctrlpluspoL}{\usebox{\CoWTfdotinvpluspoctrlpluspoK}}
\addtolength{\CoWTfdotinvpluspoctrlpluspoH}{\CoWTfdotinvpluspoctrlpluspoL}
\newsavebox{\CoWTfdotinvpluspoctrlpluspoM}
\begin{lrbox}{\CoWTfdotinvpluspoctrlpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlpluspoN}
\settowidth{\CoWTfdotinvpluspoctrlpluspoN}{\usebox{\CoWTfdotinvpluspoctrlpluspoM}}
\addtolength{\CoWTfdotinvpluspoctrlpluspoH}{\CoWTfdotinvpluspoctrlpluspoN}
\newsavebox{\CoWTfdotinvpluspoctrlpluspoO}
\begin{lrbox}{\CoWTfdotinvpluspoctrlpluspoO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlpluspoP}
\settowidth{\CoWTfdotinvpluspoctrlpluspoP}{\usebox{\CoWTfdotinvpluspoctrlpluspoO}}
\addtolength{\CoWTfdotinvpluspoctrlpluspoH}{\CoWTfdotinvpluspoctrlpluspoP}
\newsavebox{\CoWTfdotinvpluspoctrlpluspoA}
\begin{lrbox}{\CoWTfdotinvpluspoctrlpluspoA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    *pa2 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlpluspoB}
\settowidth{\CoWTfdotinvpluspoctrlpluspoB}{\usebox{\CoWTfdotinvpluspoctrlpluspoA}}
\newsavebox{\CoWTfdotinvpluspoctrlpluspoC}
\begin{lrbox}{\CoWTfdotinvpluspoctrlpluspoC}
\begin{minipage}{\CoWTfdotinvpluspoctrlpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R5=x|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+po-ctrl+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvpluspoctrlpluspoB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvpluspoctrlpluspoA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvpluspoctrlpluspoC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoctrlpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoctrlpluspoK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoctrlpluspoM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoctrlpluspoO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=1 & 0:R4=0 & 1:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoWTf.inv+po-ctrl-isb+po.tex <==
\newlength{\CoWTfdotinvpluspoctrlisbpluspoH}
\setlength{\CoWTfdotinvpluspoctrlisbpluspoH}{0cm}
\newsavebox{\CoWTfdotinvpluspoctrlisbpluspoI}
\begin{lrbox}{\CoWTfdotinvpluspoctrlisbpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
CBNZ X2,L0
L0:
ISB
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlisbpluspoJ}
\settowidth{\CoWTfdotinvpluspoctrlisbpluspoJ}{\usebox{\CoWTfdotinvpluspoctrlisbpluspoI}}
\addtolength{\CoWTfdotinvpluspoctrlisbpluspoH}{\CoWTfdotinvpluspoctrlisbpluspoJ}
\newsavebox{\CoWTfdotinvpluspoctrlisbpluspoK}
\begin{lrbox}{\CoWTfdotinvpluspoctrlisbpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlisbpluspoL}
\settowidth{\CoWTfdotinvpluspoctrlisbpluspoL}{\usebox{\CoWTfdotinvpluspoctrlisbpluspoK}}
\addtolength{\CoWTfdotinvpluspoctrlisbpluspoH}{\CoWTfdotinvpluspoctrlisbpluspoL}
\newsavebox{\CoWTfdotinvpluspoctrlisbpluspoM}
\begin{lrbox}{\CoWTfdotinvpluspoctrlisbpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlisbpluspoN}
\settowidth{\CoWTfdotinvpluspoctrlisbpluspoN}{\usebox{\CoWTfdotinvpluspoctrlisbpluspoM}}
\addtolength{\CoWTfdotinvpluspoctrlisbpluspoH}{\CoWTfdotinvpluspoctrlisbpluspoN}
\newsavebox{\CoWTfdotinvpluspoctrlisbpluspoO}
\begin{lrbox}{\CoWTfdotinvpluspoctrlisbpluspoO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlisbpluspoP}
\settowidth{\CoWTfdotinvpluspoctrlisbpluspoP}{\usebox{\CoWTfdotinvpluspoctrlisbpluspoO}}
\addtolength{\CoWTfdotinvpluspoctrlisbpluspoH}{\CoWTfdotinvpluspoctrlisbpluspoP}
\newsavebox{\CoWTfdotinvpluspoctrlisbpluspoA}
\begin{lrbox}{\CoWTfdotinvpluspoctrlisbpluspoA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    *pa2 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoctrlisbpluspoB}
\settowidth{\CoWTfdotinvpluspoctrlisbpluspoB}{\usebox{\CoWTfdotinvpluspoctrlisbpluspoA}}
\newsavebox{\CoWTfdotinvpluspoctrlisbpluspoC}
\begin{lrbox}{\CoWTfdotinvpluspoctrlisbpluspoC}
\begin{minipage}{\CoWTfdotinvpluspoctrlisbpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R5=x|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+po-ctrl-isb+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvpluspoctrlisbpluspoB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvpluspoctrlisbpluspoA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvpluspoctrlisbpluspoC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoctrlisbpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoctrlisbpluspoK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoctrlisbpluspoM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoctrlisbpluspoO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=1 & 0:R4=0 & 1:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoWTf.inv+po.tex <==
\newlength{\CoWTfdotinvpluspoH}
\setlength{\CoWTfdotinvpluspoH}{0cm}
\newsavebox{\CoWTfdotinvpluspoI}
\begin{lrbox}{\CoWTfdotinvpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoJ}
\settowidth{\CoWTfdotinvpluspoJ}{\usebox{\CoWTfdotinvpluspoI}}
\addtolength{\CoWTfdotinvpluspoH}{\CoWTfdotinvpluspoJ}
\newsavebox{\CoWTfdotinvpluspoK}
\begin{lrbox}{\CoWTfdotinvpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoL}
\settowidth{\CoWTfdotinvpluspoL}{\usebox{\CoWTfdotinvpluspoK}}
\addtolength{\CoWTfdotinvpluspoH}{\CoWTfdotinvpluspoL}
\newsavebox{\CoWTfdotinvpluspoM}
\begin{lrbox}{\CoWTfdotinvpluspoM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspoN}
\settowidth{\CoWTfdotinvpluspoN}{\usebox{\CoWTfdotinvpluspoM}}
\newsavebox{\CoWTfdotinvpluspoO}
\begin{lrbox}{\CoWTfdotinvpluspoO}
\begin{minipage}{\CoWTfdotinvpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvpluspoN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvpluspoM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvpluspoO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspoK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoWTf.inv+poloc-ctrl-isb.tex <==
\newlength{\CoWTfdotinvpluspolocctrlisbH}
\setlength{\CoWTfdotinvpluspolocctrlisbH}{0cm}
\newsavebox{\CoWTfdotinvpluspolocctrlisbI}
\begin{lrbox}{\CoWTfdotinvpluspolocctrlisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X4,[X1]
CBNZ X4,L0
L0:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspolocctrlisbJ}
\settowidth{\CoWTfdotinvpluspolocctrlisbJ}{\usebox{\CoWTfdotinvpluspolocctrlisbI}}
\addtolength{\CoWTfdotinvpluspolocctrlisbH}{\CoWTfdotinvpluspolocctrlisbJ}
\newsavebox{\CoWTfdotinvpluspolocctrlisbK}
\begin{lrbox}{\CoWTfdotinvpluspolocctrlisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspolocctrlisbL}
\settowidth{\CoWTfdotinvpluspolocctrlisbL}{\usebox{\CoWTfdotinvpluspolocctrlisbK}}
\addtolength{\CoWTfdotinvpluspolocctrlisbH}{\CoWTfdotinvpluspolocctrlisbL}
\newsavebox{\CoWTfdotinvpluspolocctrlisbM}
\begin{lrbox}{\CoWTfdotinvpluspolocctrlisbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *y = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvpluspolocctrlisbN}
\settowidth{\CoWTfdotinvpluspolocctrlisbN}{\usebox{\CoWTfdotinvpluspolocctrlisbM}}
\newsavebox{\CoWTfdotinvpluspolocctrlisbO}
\begin{lrbox}{\CoWTfdotinvpluspolocctrlisbO}
\begin{minipage}{\CoWTfdotinvpluspolocctrlisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+poloc-ctrl-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvpluspolocctrlisbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvpluspolocctrlisbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvpluspolocctrlisbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspolocctrlisbI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvpluspolocctrlisbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoWTf.inv+rfi-addr.tex <==
\newlength{\CoWTfdotinvplusrfiaddrH}
\setlength{\CoWTfdotinvplusrfiaddrH}{0cm}
\newsavebox{\CoWTfdotinvplusrfiaddrI}
\begin{lrbox}{\CoWTfdotinvplusrfiaddrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusrfiaddrJ}
\settowidth{\CoWTfdotinvplusrfiaddrJ}{\usebox{\CoWTfdotinvplusrfiaddrI}}
\addtolength{\CoWTfdotinvplusrfiaddrH}{\CoWTfdotinvplusrfiaddrJ}
\newsavebox{\CoWTfdotinvplusrfiaddrK}
\begin{lrbox}{\CoWTfdotinvplusrfiaddrK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#0
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusrfiaddrL}
\settowidth{\CoWTfdotinvplusrfiaddrL}{\usebox{\CoWTfdotinvplusrfiaddrK}}
\addtolength{\CoWTfdotinvplusrfiaddrH}{\CoWTfdotinvplusrfiaddrL}
\newsavebox{\CoWTfdotinvplusrfiaddrM}
\begin{lrbox}{\CoWTfdotinvplusrfiaddrM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusrfiaddrN}
\settowidth{\CoWTfdotinvplusrfiaddrN}{\usebox{\CoWTfdotinvplusrfiaddrM}}
\newsavebox{\CoWTfdotinvplusrfiaddrO}
\begin{lrbox}{\CoWTfdotinvplusrfiaddrO}
\begin{minipage}{\CoWTfdotinvplusrfiaddrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R5=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+rfi-addr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvplusrfiaddrN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvplusrfiaddrM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvplusrfiaddrO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplusrfiaddrI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplusrfiaddrK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=desc3(y,page_table_base) & 0:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoWTf.inv+rfi-ctrl-isb.tex <==
\newlength{\CoWTfdotinvplusrfictrlisbH}
\setlength{\CoWTfdotinvplusrfictrlisbH}{0cm}
\newsavebox{\CoWTfdotinvplusrfictrlisbI}
\begin{lrbox}{\CoWTfdotinvplusrfictrlisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
CBNZ X2,L0
L0:
ISB
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusrfictrlisbJ}
\settowidth{\CoWTfdotinvplusrfictrlisbJ}{\usebox{\CoWTfdotinvplusrfictrlisbI}}
\addtolength{\CoWTfdotinvplusrfictrlisbH}{\CoWTfdotinvplusrfictrlisbJ}
\newsavebox{\CoWTfdotinvplusrfictrlisbK}
\begin{lrbox}{\CoWTfdotinvplusrfictrlisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusrfictrlisbL}
\settowidth{\CoWTfdotinvplusrfictrlisbL}{\usebox{\CoWTfdotinvplusrfictrlisbK}}
\addtolength{\CoWTfdotinvplusrfictrlisbH}{\CoWTfdotinvplusrfictrlisbL}
\newsavebox{\CoWTfdotinvplusrfictrlisbM}
\begin{lrbox}{\CoWTfdotinvplusrfictrlisbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    *pa2 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplusrfictrlisbN}
\settowidth{\CoWTfdotinvplusrfictrlisbN}{\usebox{\CoWTfdotinvplusrfictrlisbM}}
\newsavebox{\CoWTfdotinvplusrfictrlisbO}
\begin{lrbox}{\CoWTfdotinvplusrfictrlisbO}
\begin{minipage}{\CoWTfdotinvplusrfictrlisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R5=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+rfi-ctrl-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvplusrfictrlisbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvplusrfictrlisbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvplusrfictrlisbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplusrfictrlisbI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplusrfictrlisbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=desc3(u,page_table_base) & 0:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoWTf.inv+svc.tex <==
\newlength{\CoWTfdotinvplussvcH}
\setlength{\CoWTfdotinvplussvcH}{0cm}
\newsavebox{\CoWTfdotinvplussvcI}
\begin{lrbox}{\CoWTfdotinvplussvcI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
SVC #0x0
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplussvcJ}
\settowidth{\CoWTfdotinvplussvcJ}{\usebox{\CoWTfdotinvplussvcI}}
\addtolength{\CoWTfdotinvplussvcH}{\CoWTfdotinvplussvcJ}
\newsavebox{\CoWTfdotinvplussvcK}
\begin{lrbox}{\CoWTfdotinvplussvcK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1200:
MOV X2,#0
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplussvcL}
\settowidth{\CoWTfdotinvplussvcL}{\usebox{\CoWTfdotinvplussvcK}}
\addtolength{\CoWTfdotinvplussvcH}{\CoWTfdotinvplussvcL}
\newsavebox{\CoWTfdotinvplussvcM}
\begin{lrbox}{\CoWTfdotinvplussvcM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS X10,ELR_EL1
LDR X2,[X3]
MSR ELR_EL1,X10
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplussvcN}
\settowidth{\CoWTfdotinvplussvcN}{\usebox{\CoWTfdotinvplussvcM}}
\addtolength{\CoWTfdotinvplussvcH}{\CoWTfdotinvplussvcN}
\newsavebox{\CoWTfdotinvplussvcO}
\begin{lrbox}{\CoWTfdotinvplussvcO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *y = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvplussvcP}
\settowidth{\CoWTfdotinvplussvcP}{\usebox{\CoWTfdotinvplussvcO}}
\newsavebox{\CoWTfdotinvplussvcA}
\begin{lrbox}{\CoWTfdotinvplussvcA}
\begin{minipage}{\CoWTfdotinvplussvcH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv+svc|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvplussvcP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvplussvcO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvplussvcA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplussvcI}\\
  \cline{2-2}
  & thread0 el1 handler same exc\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplussvcK}\\
  \cline{2-2}
  & thread0 el1 handler lower exc\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvplussvcM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoWTf.inv.EL1+dsb-eret.tex <==
\newlength{\CoWTfdotinvdotELoneplusdsberetH}
\setlength{\CoWTfdotinvdotELoneplusdsberetH}{0cm}
\newsavebox{\CoWTfdotinvdotELoneplusdsberetI}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELoneplusdsberetJ}
\settowidth{\CoWTfdotinvdotELoneplusdsberetJ}{\usebox{\CoWTfdotinvdotELoneplusdsberetI}}
\addtolength{\CoWTfdotinvdotELoneplusdsberetH}{\CoWTfdotinvdotELoneplusdsberetJ}
\newsavebox{\CoWTfdotinvdotELoneplusdsberetK}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELoneplusdsberetL}
\settowidth{\CoWTfdotinvdotELoneplusdsberetL}{\usebox{\CoWTfdotinvdotELoneplusdsberetK}}
\addtolength{\CoWTfdotinvdotELoneplusdsberetH}{\CoWTfdotinvdotELoneplusdsberetL}
\newsavebox{\CoWTfdotinvdotELoneplusdsberetM}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *y = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELoneplusdsberetN}
\settowidth{\CoWTfdotinvdotELoneplusdsberetN}{\usebox{\CoWTfdotinvdotELoneplusdsberetM}}
\newsavebox{\CoWTfdotinvdotELoneplusdsberetO}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsberetO}
\begin{minipage}{\CoWTfdotinvdotELoneplusdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL1=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL1=0b00000|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv.EL1+dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvdotELoneplusdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvdotELoneplusdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvdotELoneplusdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELoneplusdsberetI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELoneplusdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoWTf.inv.EL1+dsb-svc.tex <==
\newlength{\CoWTfdotinvdotELoneplusdsbsvcH}
\setlength{\CoWTfdotinvdotELoneplusdsbsvcH}{0cm}
\newsavebox{\CoWTfdotinvdotELoneplusdsbsvcI}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsbsvcI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
SVC #0x0
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELoneplusdsbsvcJ}
\settowidth{\CoWTfdotinvdotELoneplusdsbsvcJ}{\usebox{\CoWTfdotinvdotELoneplusdsbsvcI}}
\addtolength{\CoWTfdotinvdotELoneplusdsbsvcH}{\CoWTfdotinvdotELoneplusdsbsvcJ}
\newsavebox{\CoWTfdotinvdotELoneplusdsbsvcK}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsbsvcK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1200:
MOV X2,#0
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELoneplusdsbsvcL}
\settowidth{\CoWTfdotinvdotELoneplusdsbsvcL}{\usebox{\CoWTfdotinvdotELoneplusdsbsvcK}}
\addtolength{\CoWTfdotinvdotELoneplusdsbsvcH}{\CoWTfdotinvdotELoneplusdsbsvcL}
\newsavebox{\CoWTfdotinvdotELoneplusdsbsvcM}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsbsvcM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS X10,ELR_EL1
LDR X2,[X3]
MSR ELR_EL1,X10
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELoneplusdsbsvcN}
\settowidth{\CoWTfdotinvdotELoneplusdsbsvcN}{\usebox{\CoWTfdotinvdotELoneplusdsbsvcM}}
\addtolength{\CoWTfdotinvdotELoneplusdsbsvcH}{\CoWTfdotinvdotELoneplusdsbsvcN}
\newsavebox{\CoWTfdotinvdotELoneplusdsbsvcO}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsbsvcO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *y = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELoneplusdsbsvcP}
\settowidth{\CoWTfdotinvdotELoneplusdsbsvcP}{\usebox{\CoWTfdotinvdotELoneplusdsbsvcO}}
\newsavebox{\CoWTfdotinvdotELoneplusdsbsvcA}
\begin{lrbox}{\CoWTfdotinvdotELoneplusdsbsvcA}
\begin{minipage}{\CoWTfdotinvdotELoneplusdsbsvcH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv.EL1+dsb-svc|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvdotELoneplusdsbsvcP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvdotELoneplusdsbsvcO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvdotELoneplusdsbsvcA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELoneplusdsbsvcI}\\
  \cline{2-2}
  & thread0 el1 handler same exc\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELoneplusdsbsvcK}\\
  \cline{2-2}
  & thread0 el1 handler lower exc\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELoneplusdsbsvcM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoWTf.inv.EL1+eret.tex <==
\newlength{\CoWTfdotinvdotELonepluseretH}
\setlength{\CoWTfdotinvdotELonepluseretH}{0cm}
\newsavebox{\CoWTfdotinvdotELonepluseretI}
\begin{lrbox}{\CoWTfdotinvdotELonepluseretI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELonepluseretJ}
\settowidth{\CoWTfdotinvdotELonepluseretJ}{\usebox{\CoWTfdotinvdotELonepluseretI}}
\addtolength{\CoWTfdotinvdotELonepluseretH}{\CoWTfdotinvdotELonepluseretJ}
\newsavebox{\CoWTfdotinvdotELonepluseretK}
\begin{lrbox}{\CoWTfdotinvdotELonepluseretK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELonepluseretL}
\settowidth{\CoWTfdotinvdotELonepluseretL}{\usebox{\CoWTfdotinvdotELonepluseretK}}
\addtolength{\CoWTfdotinvdotELonepluseretH}{\CoWTfdotinvdotELonepluseretL}
\newsavebox{\CoWTfdotinvdotELonepluseretM}
\begin{lrbox}{\CoWTfdotinvdotELonepluseretM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa1;
    *y = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELonepluseretN}
\settowidth{\CoWTfdotinvdotELonepluseretN}{\usebox{\CoWTfdotinvdotELonepluseretM}}
\newsavebox{\CoWTfdotinvdotELonepluseretO}
\begin{lrbox}{\CoWTfdotinvdotELonepluseretO}
\begin{minipage}{\CoWTfdotinvdotELonepluseretH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL1=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL1=0b00000|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv.EL1+eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvdotELonepluseretN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvdotELonepluseretM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvdotELonepluseretO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELonepluseretI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELonepluseretK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoWTf.inv.EL2+dsb-tlbiipa-dsb-tlbiis-dsb-eret.tex <==
\newlength{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetH}
\setlength{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetH}{0cm}
\newsavebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetI}
\begin{lrbox}{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1,X4
DSB SY
TLBI VMALLE1IS
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetJ}
\settowidth{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetJ}{\usebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetI}}
\addtolength{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetH}{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetJ}
\newsavebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetK}
\begin{lrbox}{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X20,ELR_EL2
ADD X20,X20,#4
MSR ELR_EL2,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetL}
\settowidth{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetL}{\usebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetK}}
\addtolength{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetH}{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetL}
\newsavebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetM}
\begin{lrbox}{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;

    ipa1 |-> invalid;
    ipa1 ?-> pa1;

    *pa1 = 1;

    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetN}
\settowidth{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetN}{\usebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetM}}
\newsavebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetO}
\begin{lrbox}{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetO}
\begin{minipage}{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00100|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv.EL2+dsb-tlbiipa-dsb-tlbiis-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetI}\\
  \cline{2-2}
  & thread0 el2 handler lower exc\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELtwoplusdsbtlbiipadsbtlbiisdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoWTf.inv.EL2+po.tex <==
\newlength{\CoWTfdotinvdotELtwopluspoH}
\setlength{\CoWTfdotinvdotELtwopluspoH}{0cm}
\newsavebox{\CoWTfdotinvdotELtwopluspoI}
\begin{lrbox}{\CoWTfdotinvdotELtwopluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELtwopluspoJ}
\settowidth{\CoWTfdotinvdotELtwopluspoJ}{\usebox{\CoWTfdotinvdotELtwopluspoI}}
\addtolength{\CoWTfdotinvdotELtwopluspoH}{\CoWTfdotinvdotELtwopluspoJ}
\newsavebox{\CoWTfdotinvdotELtwopluspoK}
\begin{lrbox}{\CoWTfdotinvdotELtwopluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X20,ELR_EL2
ADD X20,X20,#4
MSR ELR_EL2,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELtwopluspoL}
\settowidth{\CoWTfdotinvdotELtwopluspoL}{\usebox{\CoWTfdotinvdotELtwopluspoK}}
\addtolength{\CoWTfdotinvdotELtwopluspoH}{\CoWTfdotinvdotELtwopluspoL}
\newsavebox{\CoWTfdotinvdotELtwopluspoM}
\begin{lrbox}{\CoWTfdotinvdotELtwopluspoM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;

    ipa1 |-> invalid;
    ipa1 ?-> pa1;

    *pa1 = 1;

    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTfdotinvdotELtwopluspoN}
\settowidth{\CoWTfdotinvdotELtwopluspoN}{\usebox{\CoWTfdotinvdotELtwopluspoM}}
\newsavebox{\CoWTfdotinvdotELtwopluspoO}
\begin{lrbox}{\CoWTfdotinvdotELtwopluspoO}
\begin{minipage}{\CoWTfdotinvdotELtwopluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00100|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTf.inv.EL2+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTfdotinvdotELtwopluspoN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTfdotinvdotELtwopluspoM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTfdotinvdotELtwopluspoO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELtwopluspoI}\\
  \cline{2-2}
  & thread0 el2 handler lower exc\\
  \cline{2-2}
  & \usebox{\CoWTfdotinvdotELtwopluspoK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoWTv2.2.inv+dsb-tlbivmidis-dsb-eret.tex <==
\newlength{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetH}
\setlength{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetH}{0cm}
\newsavebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetI}
\begin{lrbox}{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VMALLS12E1IS
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetJ}
\settowidth{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetJ}{\usebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetI}}
\addtolength{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetH}{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetJ}
\newsavebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetK}
\begin{lrbox}{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetL}
\settowidth{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetL}{\usebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetK}}
\addtolength{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetH}{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetL}
\newsavebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetM}
\begin{lrbox}{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;
    ipa1 |-> invalid;
    ipa1 ?-> pa1;

    *pa1 = 1;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetN}
\settowidth{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetN}{\usebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetM}}
\newsavebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetO}
\begin{lrbox}{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetO}
\begin{minipage}{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00101|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWTv2.2.inv+dsb-tlbivmidis-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetI}\\
  \cline{2-2}
  & thread0 el2 handler\\
  \cline{2-2}
  & \usebox{\CoWTvtwodottwodotinvplusdsbtlbivmidisdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoWW.alias.tex <==
\newlength{\CoWWdotaliasH}
\setlength{\CoWWdotaliasH}{0cm}
\newsavebox{\CoWWdotaliasI}
\begin{lrbox}{\CoWWdotaliasI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWWdotaliasJ}
\settowidth{\CoWWdotaliasJ}{\usebox{\CoWWdotaliasI}}
\addtolength{\CoWWdotaliasH}{\CoWWdotaliasJ}
\newsavebox{\CoWWdotaliasK}
\begin{lrbox}{\CoWWdotaliasK}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    y |-> pa1;
    *pa1 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWWdotaliasL}
\settowidth{\CoWWdotaliasL}{\usebox{\CoWWdotaliasK}}
\newsavebox{\CoWWdotaliasM}
\begin{lrbox}{\CoWWdotaliasM}
\begin{minipage}{\CoWWdotaliasH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=0b01|\\
\lstinline[language=IslaLitmusExp]|R1=x|\\
\lstinline[language=IslaLitmusExp]|R2=0b10|\\
\lstinline[language=IslaLitmusExp]|R3=y|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWW.alias|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWWdotaliasL}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWWdotaliasK}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWWdotaliasM}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWWdotaliasI}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|x=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoWinvRpte+po.tex <==
\newlength{\CoWinvRptepluspoH}
\setlength{\CoWinvRptepluspoH}{0cm}
\newsavebox{\CoWinvRptepluspoI}
\begin{lrbox}{\CoWinvRptepluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvRptepluspoJ}
\settowidth{\CoWinvRptepluspoJ}{\usebox{\CoWinvRptepluspoI}}
\addtolength{\CoWinvRptepluspoH}{\CoWinvRptepluspoJ}
\newsavebox{\CoWinvRptepluspoK}
\begin{lrbox}{\CoWinvRptepluspoK}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;

    *pa1 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvRptepluspoL}
\settowidth{\CoWinvRptepluspoL}{\usebox{\CoWinvRptepluspoK}}
\newsavebox{\CoWinvRptepluspoM}
\begin{lrbox}{\CoWinvRptepluspoM}
\begin{minipage}{\CoWinvRptepluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=0x0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvRpte+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvRptepluspoL}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvRptepluspoK}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvRptepluspoM}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvRptepluspoI}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|~0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoWinvT+dsb-isb.tex <==
\newlength{\CoWinvTplusdsbisbH}
\setlength{\CoWinvTplusdsbisbH}{0cm}
\newsavebox{\CoWinvTplusdsbisbI}
\begin{lrbox}{\CoWinvTplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTplusdsbisbJ}
\settowidth{\CoWinvTplusdsbisbJ}{\usebox{\CoWinvTplusdsbisbI}}
\addtolength{\CoWinvTplusdsbisbH}{\CoWinvTplusdsbisbJ}
\newsavebox{\CoWinvTplusdsbisbK}
\begin{lrbox}{\CoWinvTplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTplusdsbisbL}
\settowidth{\CoWinvTplusdsbisbL}{\usebox{\CoWinvTplusdsbisbK}}
\addtolength{\CoWinvTplusdsbisbH}{\CoWinvTplusdsbisbL}
\newsavebox{\CoWinvTplusdsbisbM}
\begin{lrbox}{\CoWinvTplusdsbisbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTplusdsbisbN}
\settowidth{\CoWinvTplusdsbisbN}{\usebox{\CoWinvTplusdsbisbM}}
\newsavebox{\CoWinvTplusdsbisbO}
\begin{lrbox}{\CoWinvTplusdsbisbO}
\begin{minipage}{\CoWinvTplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvT+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTplusdsbisbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTplusdsbisbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTplusdsbisbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTplusdsbisbI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTplusdsbisbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoWinvT+po.tex <==
\newlength{\CoWinvTpluspoH}
\setlength{\CoWinvTpluspoH}{0cm}
\newsavebox{\CoWinvTpluspoI}
\begin{lrbox}{\CoWinvTpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTpluspoJ}
\settowidth{\CoWinvTpluspoJ}{\usebox{\CoWinvTpluspoI}}
\addtolength{\CoWinvTpluspoH}{\CoWinvTpluspoJ}
\newsavebox{\CoWinvTpluspoK}
\begin{lrbox}{\CoWinvTpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTpluspoL}
\settowidth{\CoWinvTpluspoL}{\usebox{\CoWinvTpluspoK}}
\addtolength{\CoWinvTpluspoH}{\CoWinvTpluspoL}
\newsavebox{\CoWinvTpluspoM}
\begin{lrbox}{\CoWinvTpluspoM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTpluspoN}
\settowidth{\CoWinvTpluspoN}{\usebox{\CoWinvTpluspoM}}
\newsavebox{\CoWinvTpluspoO}
\begin{lrbox}{\CoWinvTpluspoO}
\begin{minipage}{\CoWinvTpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvT+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTpluspoN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTpluspoM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTpluspoO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTpluspoI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTpluspoK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoWinvT.EL1+dsb-tlbi-dsb-isb.tex <==
\newlength{\CoWinvTdotELoneplusdsbtlbidsbisbH}
\setlength{\CoWinvTdotELoneplusdsbtlbidsbisbH}{0cm}
\newsavebox{\CoWinvTdotELoneplusdsbtlbidsbisbI}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbidsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1,X5
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbidsbisbJ}
\settowidth{\CoWinvTdotELoneplusdsbtlbidsbisbJ}{\usebox{\CoWinvTdotELoneplusdsbtlbidsbisbI}}
\addtolength{\CoWinvTdotELoneplusdsbtlbidsbisbH}{\CoWinvTdotELoneplusdsbtlbidsbisbJ}
\newsavebox{\CoWinvTdotELoneplusdsbtlbidsbisbK}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbidsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1000:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbidsbisbL}
\settowidth{\CoWinvTdotELoneplusdsbtlbidsbisbL}{\usebox{\CoWinvTdotELoneplusdsbtlbidsbisbK}}
\addtolength{\CoWinvTdotELoneplusdsbtlbidsbisbH}{\CoWinvTdotELoneplusdsbtlbidsbisbL}
\newsavebox{\CoWinvTdotELoneplusdsbtlbidsbisbM}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbidsbisbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbidsbisbN}
\settowidth{\CoWinvTdotELoneplusdsbtlbidsbisbN}{\usebox{\CoWinvTdotELoneplusdsbtlbidsbisbM}}
\newsavebox{\CoWinvTdotELoneplusdsbtlbidsbisbO}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbidsbisbO}
\begin{minipage}{\CoWinvTdotELoneplusdsbtlbidsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R5=page(x)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvT.EL1+dsb-tlbi-dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTdotELoneplusdsbtlbidsbisbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTdotELoneplusdsbtlbidsbisbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTdotELoneplusdsbtlbidsbisbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTdotELoneplusdsbtlbidsbisbI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTdotELoneplusdsbtlbidsbisbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoWinvT.EL1+dsb-tlbi-dsb.tex <==
\newlength{\CoWinvTdotELoneplusdsbtlbidsbH}
\setlength{\CoWinvTdotELoneplusdsbtlbidsbH}{0cm}
\newsavebox{\CoWinvTdotELoneplusdsbtlbidsbI}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbidsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1,X5
DSB SY
MOV X2,#0
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbidsbJ}
\settowidth{\CoWinvTdotELoneplusdsbtlbidsbJ}{\usebox{\CoWinvTdotELoneplusdsbtlbidsbI}}
\addtolength{\CoWinvTdotELoneplusdsbtlbidsbH}{\CoWinvTdotELoneplusdsbtlbidsbJ}
\newsavebox{\CoWinvTdotELoneplusdsbtlbidsbK}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbidsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1000:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbidsbL}
\settowidth{\CoWinvTdotELoneplusdsbtlbidsbL}{\usebox{\CoWinvTdotELoneplusdsbtlbidsbK}}
\addtolength{\CoWinvTdotELoneplusdsbtlbidsbH}{\CoWinvTdotELoneplusdsbtlbidsbL}
\newsavebox{\CoWinvTdotELoneplusdsbtlbidsbM}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbidsbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbidsbN}
\settowidth{\CoWinvTdotELoneplusdsbtlbidsbN}{\usebox{\CoWinvTdotELoneplusdsbtlbidsbM}}
\newsavebox{\CoWinvTdotELoneplusdsbtlbidsbO}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbidsbO}
\begin{minipage}{\CoWinvTdotELoneplusdsbtlbidsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R5=page(x)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvT.EL1+dsb-tlbi-dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTdotELoneplusdsbtlbidsbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTdotELoneplusdsbtlbidsbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTdotELoneplusdsbtlbidsbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTdotELoneplusdsbtlbidsbI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTdotELoneplusdsbtlbidsbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoWinvT.EL1+dsb-tlbiis-dsb-isb.tex <==
\newlength{\CoWinvTdotELoneplusdsbtlbiisdsbisbH}
\setlength{\CoWinvTdotELoneplusdsbtlbiisdsbisbH}{0cm}
\newsavebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbI}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbiisdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X5
DSB SY
ISB
MOV X2,#0
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbiisdsbisbJ}
\settowidth{\CoWinvTdotELoneplusdsbtlbiisdsbisbJ}{\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbI}}
\addtolength{\CoWinvTdotELoneplusdsbtlbiisdsbisbH}{\CoWinvTdotELoneplusdsbtlbiisdsbisbJ}
\newsavebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbK}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbiisdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1000:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbiisdsbisbL}
\settowidth{\CoWinvTdotELoneplusdsbtlbiisdsbisbL}{\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbK}}
\addtolength{\CoWinvTdotELoneplusdsbtlbiisdsbisbH}{\CoWinvTdotELoneplusdsbtlbiisdsbisbL}
\newsavebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbM}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbiisdsbisbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbiisdsbisbN}
\settowidth{\CoWinvTdotELoneplusdsbtlbiisdsbisbN}{\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbM}}
\newsavebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbO}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbiisdsbisbO}
\begin{minipage}{\CoWinvTdotELoneplusdsbtlbiisdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R5=page(x)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvT.EL1+dsb-tlbiis-dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTdotELoneplusdsbtlbiisdsbisbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTdotELoneplusdsbtlbiisdsbisbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoWinvT.EL1+dsb-tlbiis-dsb.tex <==
\newlength{\CoWinvTdotELoneplusdsbtlbiisdsbH}
\setlength{\CoWinvTdotELoneplusdsbtlbiisdsbH}{0cm}
\newsavebox{\CoWinvTdotELoneplusdsbtlbiisdsbI}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbiisdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X5
DSB SY
MOV X2,#0
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbiisdsbJ}
\settowidth{\CoWinvTdotELoneplusdsbtlbiisdsbJ}{\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbI}}
\addtolength{\CoWinvTdotELoneplusdsbtlbiisdsbH}{\CoWinvTdotELoneplusdsbtlbiisdsbJ}
\newsavebox{\CoWinvTdotELoneplusdsbtlbiisdsbK}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbiisdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1000:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbiisdsbL}
\settowidth{\CoWinvTdotELoneplusdsbtlbiisdsbL}{\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbK}}
\addtolength{\CoWinvTdotELoneplusdsbtlbiisdsbH}{\CoWinvTdotELoneplusdsbtlbiisdsbL}
\newsavebox{\CoWinvTdotELoneplusdsbtlbiisdsbM}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbiisdsbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTdotELoneplusdsbtlbiisdsbN}
\settowidth{\CoWinvTdotELoneplusdsbtlbiisdsbN}{\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbM}}
\newsavebox{\CoWinvTdotELoneplusdsbtlbiisdsbO}
\begin{lrbox}{\CoWinvTdotELoneplusdsbtlbiisdsbO}
\begin{minipage}{\CoWinvTdotELoneplusdsbtlbiisdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R5=page(x)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvT.EL1+dsb-tlbiis-dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTdotELoneplusdsbtlbiisdsbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTdotELoneplusdsbtlbiisdsbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTdotELoneplusdsbtlbiisdsbI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTdotELoneplusdsbtlbiisdsbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoWinvT2+dsb-tlbiipa-dsb-eret.tex <==
\newlength{\CoWinvTtwoplusdsbtlbiipadsberetH}
\setlength{\CoWinvTtwoplusdsbtlbiipadsberetH}{0cm}
\newsavebox{\CoWinvTtwoplusdsbtlbiipadsberetI}
\begin{lrbox}{\CoWinvTtwoplusdsbtlbiipadsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1,X4
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTtwoplusdsbtlbiipadsberetJ}
\settowidth{\CoWinvTtwoplusdsbtlbiipadsberetJ}{\usebox{\CoWinvTtwoplusdsbtlbiipadsberetI}}
\addtolength{\CoWinvTtwoplusdsbtlbiipadsberetH}{\CoWinvTtwoplusdsbtlbiipadsberetJ}
\newsavebox{\CoWinvTtwoplusdsbtlbiipadsberetK}
\begin{lrbox}{\CoWinvTtwoplusdsbtlbiipadsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X20,ELR_EL2
ADD X20,X20,#4
MSR ELR_EL2,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTtwoplusdsbtlbiipadsberetL}
\settowidth{\CoWinvTtwoplusdsbtlbiipadsberetL}{\usebox{\CoWinvTtwoplusdsbtlbiipadsberetK}}
\addtolength{\CoWinvTtwoplusdsbtlbiipadsberetH}{\CoWinvTtwoplusdsbtlbiipadsberetL}
\newsavebox{\CoWinvTtwoplusdsbtlbiipadsberetM}
\begin{lrbox}{\CoWinvTtwoplusdsbtlbiipadsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;

    ipa1 |-> invalid;
    ipa1 ?-> pa1;

    *pa1 = 1;

    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTtwoplusdsbtlbiipadsberetN}
\settowidth{\CoWinvTtwoplusdsbtlbiipadsberetN}{\usebox{\CoWinvTtwoplusdsbtlbiipadsberetM}}
\newsavebox{\CoWinvTtwoplusdsbtlbiipadsberetO}
\begin{lrbox}{\CoWinvTtwoplusdsbtlbiipadsberetO}
\begin{minipage}{\CoWinvTtwoplusdsbtlbiipadsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=page(ipa1)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00100|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvT2+dsb-tlbiipa-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTtwoplusdsbtlbiipadsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTtwoplusdsbtlbiipadsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTtwoplusdsbtlbiipadsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTtwoplusdsbtlbiipadsberetI}\\
  \cline{2-2}
  & thread0 el2 handler lower exc\\
  \cline{2-2}
  & \usebox{\CoWinvTtwoplusdsbtlbiipadsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoWinvT2+dsb-tlbiipa-dsb-tlbivmall-dsb-eret.tex <==
\newlength{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetH}
\setlength{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetH}{0cm}
\newsavebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetI}
\begin{lrbox}{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1,X4
DSB SY
TLBI VMALLE1
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetJ}
\settowidth{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetJ}{\usebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetI}}
\addtolength{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetH}{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetJ}
\newsavebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetK}
\begin{lrbox}{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#1
MRS X20,ELR_EL2
ADD X20,X20,#4
MSR ELR_EL2,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetL}
\settowidth{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetL}{\usebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetK}}
\addtolength{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetH}{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetL}
\newsavebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetM}
\begin{lrbox}{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;

    ipa1 |-> pa1;
    ipa1 ?-> invalid;

    *pa1 = 0;

    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetN}
\settowidth{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetN}{\usebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetM}}
\newsavebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetO}
\begin{lrbox}{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetO}
\begin{minipage}{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=page(ipa1)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00100|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvT2+dsb-tlbiipa-dsb-tlbivmall-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetI}\\
  \cline{2-2}
  & thread0 el2 handler lower exc\\
  \cline{2-2}
  & \usebox{\CoWinvTtwoplusdsbtlbiipadsbtlbivmalldsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoWinvTa1.1+dsb-tlbiasidis-dsb-eret.tex <==
\newlength{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetH}
\setlength{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetH}{0cm}
\newsavebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetI}
\begin{lrbox}{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI ASIDE1IS,X4
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetJ}
\settowidth{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetJ}{\usebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetI}}
\addtolength{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetH}{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetJ}
\newsavebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetK}
\begin{lrbox}{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetL}
\settowidth{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetL}{\usebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetK}}
\addtolength{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetH}{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetL}
\newsavebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetM}
\begin{lrbox}{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetN}
\settowidth{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetN}{\usebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetM}}
\newsavebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetO}
\begin{lrbox}{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetO}
\begin{minipage}{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL1=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=asid(0x1)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL1=0b00000|\\
\lstinline[language=IslaLitmusExp]|TTBR0_EL1=ttbr(asid=0x0001,base=page_table_base)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvTa1.1+dsb-tlbiasidis-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTaonedotoneplusdsbtlbiasidisdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoWinvTa2.1+dsb-tlbiasidis-dsb-eret.tex <==
\newlength{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetH}
\setlength{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetH}{0cm}
\newsavebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetI}
\begin{lrbox}{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI ASIDE1IS,X4
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetJ}
\settowidth{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetJ}{\usebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetI}}
\addtolength{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetH}{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetJ}
\newsavebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetK}
\begin{lrbox}{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetL}
\settowidth{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetL}{\usebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetK}}
\addtolength{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetH}{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetL}
\newsavebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetM}
\begin{lrbox}{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetN}
\settowidth{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetN}{\usebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetM}}
\newsavebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetO}
\begin{lrbox}{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetO}
\begin{minipage}{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL1=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=asid(0x2)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL1=0b00000|\\
\lstinline[language=IslaLitmusExp]|TTBR0_EL1=ttbr(base=page_table_base,asid=0x0001)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvTa2.1+dsb-tlbiasidis-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTatwodotoneplusdsbtlbiasidisdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoWinvTv1.2+dsb-tlbivmidis-dsb-eret.tex <==
\newlength{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetH}
\setlength{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetH}{0cm}
\newsavebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetI}
\begin{lrbox}{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VMALLS12E1IS
DSB SY
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetJ}
\settowidth{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetJ}{\usebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetI}}
\addtolength{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetH}{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetJ}
\newsavebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetK}
\begin{lrbox}{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#1
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetL}
\settowidth{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetL}{\usebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetK}}
\addtolength{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetH}{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetL}
\newsavebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetM}
\begin{lrbox}{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;
    ipa1 |-> pa1;
    ipa1 ?-> invalid;

    *pa1 = 0;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetN}
\settowidth{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetN}{\usebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetM}}
\newsavebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetO}
\begin{lrbox}{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetO}
\begin{minipage}{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00101|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvTv1.2+dsb-tlbivmidis-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetI}\\
  \cline{2-2}
  & thread0 el2 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTvonedottwoplusdsbtlbivmidisdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/CoWinvTv2.2+dsb-tlbivmidis-msrvttbr-dsb-eret.tex <==
\newlength{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetH}
\setlength{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetH}{0cm}
\newsavebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetI}
\begin{lrbox}{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VMALLS12E1IS
DSB SY
MSR VTTBR_EL2,X4
ERET
L0:
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetJ}
\settowidth{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetJ}{\usebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetI}}
\addtolength{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetH}{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetJ}
\newsavebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetK}
\begin{lrbox}{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#1
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetL}
\settowidth{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetL}{\usebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetK}}
\addtolength{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetH}{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetL}
\newsavebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetM}
\begin{lrbox}{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;
    ipa1 |-> pa1;
    ipa1 ?-> invalid;

    *pa1 = 0;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetN}
\settowidth{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetN}{\usebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetM}}
\newsavebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetO}
\begin{lrbox}{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetO}
\begin{minipage}{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=ttbr(base=s2_page_table_base,vmid=0x0001)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00101|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|CoWinvTv2.2+dsb-tlbivmidis-msrvttbr-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetI}\\
  \cline{2-2}
  & thread0 el2 handler\\
  \cline{2-2}
  & \usebox{\CoWinvTvtwodottwoplusdsbtlbivmidismsrvttbrdsberetK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/ETS.tex <==
\newlength{\ETSH}
\setlength{\ETSH}{0cm}
\newsavebox{\ETSI}
\begin{lrbox}{\ETSI}
\begin{lstlisting}[language=AArch64,showlines=true]
MOV X0,#1
STR X0,[X3]
DMB SY
STR X0,[X2]
\end{lstlisting}
\end{lrbox}
\newlength{\ETSJ}
\settowidth{\ETSJ}{\usebox{\ETSI}}
\addtolength{\ETSH}{\ETSJ}
\newsavebox{\ETSK}
\begin{lrbox}{\ETSK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X2]
STR X0,[X1]
MOV X4,#2
STR X4,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\ETSL}
\settowidth{\ETSL}{\usebox{\ETSK}}
\addtolength{\ETSH}{\ETSL}
\newsavebox{\ETSM}
\begin{lrbox}{\ETSM}
\begin{lstlisting}[language=AArch64,showlines=true]
MOV X0,#0
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\ETSN}
\settowidth{\ETSN}{\usebox{\ETSM}}
\addtolength{\ETSH}{\ETSN}
\newsavebox{\ETSO}
\begin{lrbox}{\ETSO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
LDR X7,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\ETSP}
\settowidth{\ETSP}{\usebox{\ETSO}}
\addtolength{\ETSH}{\ETSP}
\newsavebox{\ETSA}
\begin{lrbox}{\ETSA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> pa1;
    x ?-> invalid;
    y |-> pa2;
    z |-> pa3;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\ETSB}
\settowidth{\ETSB}{\usebox{\ETSA}}
\newsavebox{\ETSC}
\begin{lrbox}{\ETSC}
\begin{minipage}{\ETSH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R2=y|\\
\lstinline[language=IslaLitmusExp]|0:R3=z|\\
\lstinline[language=IslaLitmusExp]|1:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=z|\\
\lstinline[language=IslaLitmusExp]|1:R6=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R7=0b1|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:R1=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|ETS|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\ETSB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\ETSA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\ETSC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\ETSI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\ETSK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\ETSM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\ETSO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & x=1 & 1:R7=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/IRIW.TTf.TTf.inv+addrs.tex <==
\newlength{\IRIWdotTTfdotTTfdotinvplusaddrsH}
\setlength{\IRIWdotTTfdotTTfdotinvplusaddrsH}{0cm}
\newsavebox{\IRIWdotTTfdotTTfdotinvplusaddrsI}
\begin{lrbox}{\IRIWdotTTfdotTTfdotinvplusaddrsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\IRIWdotTTfdotTTfdotinvplusaddrsJ}
\settowidth{\IRIWdotTTfdotTTfdotinvplusaddrsJ}{\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsI}}
\addtolength{\IRIWdotTTfdotTTfdotinvplusaddrsH}{\IRIWdotTTfdotTTfdotinvplusaddrsJ}
\newsavebox{\IRIWdotTTfdotTTfdotinvplusaddrsK}
\begin{lrbox}{\IRIWdotTTfdotTTfdotinvplusaddrsK}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\IRIWdotTTfdotTTfdotinvplusaddrsL}
\settowidth{\IRIWdotTTfdotTTfdotinvplusaddrsL}{\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsK}}
\addtolength{\IRIWdotTTfdotTTfdotinvplusaddrsH}{\IRIWdotTTfdotTTfdotinvplusaddrsL}
\newsavebox{\IRIWdotTTfdotTTfdotinvplusaddrsM}
\begin{lrbox}{\IRIWdotTTfdotTTfdotinvplusaddrsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\IRIWdotTTfdotTTfdotinvplusaddrsN}
\settowidth{\IRIWdotTTfdotTTfdotinvplusaddrsN}{\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsM}}
\addtolength{\IRIWdotTTfdotTTfdotinvplusaddrsH}{\IRIWdotTTfdotTTfdotinvplusaddrsN}
\newsavebox{\IRIWdotTTfdotTTfdotinvplusaddrsO}
\begin{lrbox}{\IRIWdotTTfdotTTfdotinvplusaddrsO}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\IRIWdotTTfdotTTfdotinvplusaddrsP}
\settowidth{\IRIWdotTTfdotTTfdotinvplusaddrsP}{\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsO}}
\addtolength{\IRIWdotTTfdotTTfdotinvplusaddrsH}{\IRIWdotTTfdotTTfdotinvplusaddrsP}
\newsavebox{\IRIWdotTTfdotTTfdotinvplusaddrsA}
\begin{lrbox}{\IRIWdotTTfdotTTfdotinvplusaddrsA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\IRIWdotTTfdotTTfdotinvplusaddrsB}
\settowidth{\IRIWdotTTfdotTTfdotinvplusaddrsB}{\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsA}}
\addtolength{\IRIWdotTTfdotTTfdotinvplusaddrsH}{\IRIWdotTTfdotTTfdotinvplusaddrsB}
\newsavebox{\IRIWdotTTfdotTTfdotinvplusaddrsC}
\begin{lrbox}{\IRIWdotTTfdotTTfdotinvplusaddrsC}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\IRIWdotTTfdotTTfdotinvplusaddrsD}
\settowidth{\IRIWdotTTfdotTTfdotinvplusaddrsD}{\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsC}}
\addtolength{\IRIWdotTTfdotTTfdotinvplusaddrsH}{\IRIWdotTTfdotTTfdotinvplusaddrsD}
\newsavebox{\IRIWdotTTfdotTTfdotinvplusaddrsE}
\begin{lrbox}{\IRIWdotTTfdotTTfdotinvplusaddrsE}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> invalid;
    y ?-> pa2;
    v |-> pa2;
    *pa2 = 1;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\IRIWdotTTfdotTTfdotinvplusaddrsF}
\settowidth{\IRIWdotTTfdotTTfdotinvplusaddrsF}{\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsE}}
\newsavebox{\IRIWdotTTfdotTTfdotinvplusaddrsHG}
\begin{lrbox}{\IRIWdotTTfdotTTfdotinvplusaddrsHG}
\begin{minipage}{\IRIWdotTTfdotTTfdotinvplusaddrsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R0=desc3(v,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=x|\\
\lstinline[language=IslaLitmusExp]|2:R3=y|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|3:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|3:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|3:R1=y|\\
\lstinline[language=IslaLitmusExp]|3:R3=x|\\
\lstinline[language=IslaLitmusExp]|3:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|IRIW.TTf.TTf.inv+addrs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\IRIWdotTTfdotTTfdotinvplusaddrsF}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsE}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\IRIWdotTTfdotTTfdotinvplusaddrsHG}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\IRIWdotTTfdotTTfdotinvplusaddrsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\IRIWdotTTfdotTTfdotinvplusaddrsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\IRIWdotTTfdotTTfdotinvplusaddrsM}\\
  \cline{2-2}
  & Thread 3\\
  \cline{2-2}
  & \usebox{\IRIWdotTTfdotTTfdotinvplusaddrsO}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\IRIWdotTTfdotTTfdotinvplusaddrsA}\\
  \cline{2-2}
  & thread3 el1 handler\\
  \cline{2-2}
  & \usebox{\IRIWdotTTfdotTTfdotinvplusaddrsC}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|2:R0=1 & 2:R2=0 & 3:R0=1 & 3:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/ISA2.RRTf.inv+dsb+addr+addr.tex <==
\newlength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrH}
\setlength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrH}{0cm}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrI}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrJ}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrJ}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrI}}
\addtolength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrH}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrJ}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrK}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
STR X3,[X4,X2]
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrL}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrL}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrK}}
\addtolength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrH}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrL}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrM}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
LDR X3,[X4,X2]
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrN}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrN}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrM}}
\addtolength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrH}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrN}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrO}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X3,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrP}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrP}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrO}}
\addtolength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrH}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrP}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrA}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    *pa2 = 0;

    z |-> pa3;
    *pa3 = 0;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrB}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrB}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrA}}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrC}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrC}
\begin{minipage}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R4=z|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=z|\\
\lstinline[language=IslaLitmusExp]|2:R4=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|ISA2.RRTf.inv+dsb+addr+addr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrM}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\ISAtwodotRRTfdotinvplusdsbplusaddrplusaddrO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R3=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/ISA2.RRTf.inv+dsb+data+addr.tex <==
\newlength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrH}
\setlength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrH}{0cm}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrI}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrJ}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrJ}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrI}}
\addtolength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrH}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrJ}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrK}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
ORR X3,X3,X2
STR X3,[X4]
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrL}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrL}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrK}}
\addtolength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrH}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrL}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrM}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
LDR X3,[X4,X2]
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrN}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrN}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrM}}
\addtolength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrH}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrN}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrO}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X3,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrP}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrP}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrO}}
\addtolength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrH}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrP}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrA}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    *pa2 = 0;

    z |-> pa3;
    *pa3 = 0;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrB}
\settowidth{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrB}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrA}}
\newsavebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrC}
\begin{lrbox}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrC}
\begin{minipage}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R4=z|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=z|\\
\lstinline[language=IslaLitmusExp]|2:R4=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|ISA2.RRTf.inv+dsb+data+addr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrM}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\ISAtwodotRRTfdotinvplusdsbplusdataplusaddrO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R3=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/LB+addr-trfis.tex <==
\newlength{\LBplusaddrtrfisH}
\setlength{\LBplusaddrtrfisH}{0cm}
\newsavebox{\LBplusaddrtrfisI}
\begin{lrbox}{\LBplusaddrtrfisI}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
STR X3,[X4,X2]
STR X5,[X6]
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusaddrtrfisJ}
\settowidth{\LBplusaddrtrfisJ}{\usebox{\LBplusaddrtrfisI}}
\addtolength{\LBplusaddrtrfisH}{\LBplusaddrtrfisJ}
\newsavebox{\LBplusaddrtrfisK}
\begin{lrbox}{\LBplusaddrtrfisK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
STR X3,[X4,X2]
STR X5,[X6]
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusaddrtrfisL}
\settowidth{\LBplusaddrtrfisL}{\usebox{\LBplusaddrtrfisK}}
\addtolength{\LBplusaddrtrfisH}{\LBplusaddrtrfisL}
\newsavebox{\LBplusaddrtrfisM}
\begin{lrbox}{\LBplusaddrtrfisM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X7,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusaddrtrfisN}
\settowidth{\LBplusaddrtrfisN}{\usebox{\LBplusaddrtrfisM}}
\addtolength{\LBplusaddrtrfisH}{\LBplusaddrtrfisN}
\newsavebox{\LBplusaddrtrfisO}
\begin{lrbox}{\LBplusaddrtrfisO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X7,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusaddrtrfisP}
\settowidth{\LBplusaddrtrfisP}{\usebox{\LBplusaddrtrfisO}}
\addtolength{\LBplusaddrtrfisH}{\LBplusaddrtrfisP}
\newsavebox{\LBplusaddrtrfisA}
\begin{lrbox}{\LBplusaddrtrfisA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3 pa4;
    x |-> pa1;
    y |-> pa2;
    u |-> invalid;
    u ?-> pa2;
    v |-> invalid;
    v ?-> pa1;
    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusaddrtrfisB}
\settowidth{\LBplusaddrtrfisB}{\usebox{\LBplusaddrtrfisA}}
\newsavebox{\LBplusaddrtrfisC}
\begin{lrbox}{\LBplusaddrtrfisC}
\begin{minipage}{\LBplusaddrtrfisH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R3=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R4=pte3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R5=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R6=u|\\
\lstinline[language=IslaLitmusExp]|0:R7=0b1|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|0:__isla_monomorphize_writes=true|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=desc3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R4=pte3(v,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R5=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R6=v|\\
\lstinline[language=IslaLitmusExp]|1:R7=0b1|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\lstinline[language=IslaLitmusExp]|1:__isla_monomorphize_writes=true|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|LB+addr-trfis|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\LBplusaddrtrfisB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\LBplusaddrtrfisA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\LBplusaddrtrfisC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\LBplusaddrtrfisI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\LBplusaddrtrfisK}\\
  \cline{2-2}
  & thread1 el0 handler\\
  \cline{2-2}
  & \usebox{\LBplusaddrtrfisM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\LBplusaddrtrfisO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R0=1 & 0:R7=1 & 1:R0=1 & 1:R7=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/LB+data-trfis.tex <==
\newlength{\LBplusdatatrfisH}
\setlength{\LBplusdatatrfisH}{0cm}
\newsavebox{\LBplusdatatrfisI}
\begin{lrbox}{\LBplusdatatrfisI}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
ORR X3,X3,X2
STR X3,[X4]
STR X5,[X6]
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusdatatrfisJ}
\settowidth{\LBplusdatatrfisJ}{\usebox{\LBplusdatatrfisI}}
\addtolength{\LBplusdatatrfisH}{\LBplusdatatrfisJ}
\newsavebox{\LBplusdatatrfisK}
\begin{lrbox}{\LBplusdatatrfisK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
ORR X3,X3,X2
STR X3,[X4]
STR X5,[X6]
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusdatatrfisL}
\settowidth{\LBplusdatatrfisL}{\usebox{\LBplusdatatrfisK}}
\addtolength{\LBplusdatatrfisH}{\LBplusdatatrfisL}
\newsavebox{\LBplusdatatrfisM}
\begin{lrbox}{\LBplusdatatrfisM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X7,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusdatatrfisN}
\settowidth{\LBplusdatatrfisN}{\usebox{\LBplusdatatrfisM}}
\addtolength{\LBplusdatatrfisH}{\LBplusdatatrfisN}
\newsavebox{\LBplusdatatrfisO}
\begin{lrbox}{\LBplusdatatrfisO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X7,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusdatatrfisP}
\settowidth{\LBplusdatatrfisP}{\usebox{\LBplusdatatrfisO}}
\addtolength{\LBplusdatatrfisH}{\LBplusdatatrfisP}
\newsavebox{\LBplusdatatrfisA}
\begin{lrbox}{\LBplusdatatrfisA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3 pa4;
    x |-> pa1;
    y |-> pa2;
    u |-> invalid;
    u ?-> pa2;
    v |-> invalid;
    v ?-> pa1;
    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusdatatrfisB}
\settowidth{\LBplusdatatrfisB}{\usebox{\LBplusdatatrfisA}}
\newsavebox{\LBplusdatatrfisC}
\begin{lrbox}{\LBplusdatatrfisC}
\begin{minipage}{\LBplusdatatrfisH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R3=desc3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R4=pte3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R5=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R6=u|\\
\lstinline[language=IslaLitmusExp]|0:R7=0b1|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=desc3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R4=pte3(v,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R5=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R6=v|\\
\lstinline[language=IslaLitmusExp]|1:R7=0b1|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|LB+data-trfis|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\LBplusdatatrfisB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\LBplusdatatrfisA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\LBplusdatatrfisC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\LBplusdatatrfisI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\LBplusdatatrfisK}\\
  \cline{2-2}
  & thread1 el0 handler\\
  \cline{2-2}
  & \usebox{\LBplusdatatrfisM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\LBplusdatatrfisO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R0=1 & 0:R7=1 & 1:R0=1 & 1:R7=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/LB+dmb.ld+ctrl.tex <==
\newlength{\LBplusdmbdotldplusctrlH}
\setlength{\LBplusdmbdotldplusctrlH}{0cm}
\newsavebox{\LBplusdmbdotldplusctrlI}
\begin{lrbox}{\LBplusdmbdotldplusctrlI}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR W0,[X1]
DMB LD
MOV W2,#1
STR W2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusdmbdotldplusctrlJ}
\settowidth{\LBplusdmbdotldplusctrlJ}{\usebox{\LBplusdmbdotldplusctrlI}}
\addtolength{\LBplusdmbdotldplusctrlH}{\LBplusdmbdotldplusctrlJ}
\newsavebox{\LBplusdmbdotldplusctrlK}
\begin{lrbox}{\LBplusdmbdotldplusctrlK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR W0,[X1]
CBNZ W0,L0
L0:
MOV W2,#1
STR W2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusdmbdotldplusctrlL}
\settowidth{\LBplusdmbdotldplusctrlL}{\usebox{\LBplusdmbdotldplusctrlK}}
\addtolength{\LBplusdmbdotldplusctrlH}{\LBplusdmbdotldplusctrlL}
\newsavebox{\LBplusdmbdotldplusctrlM}
\begin{lrbox}{\LBplusdmbdotldplusctrlM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusdmbdotldplusctrlN}
\settowidth{\LBplusdmbdotldplusctrlN}{\usebox{\LBplusdmbdotldplusctrlM}}
\newsavebox{\LBplusdmbdotldplusctrlO}
\begin{lrbox}{\LBplusdmbdotldplusctrlO}
\begin{minipage}{\LBplusdmbdotldplusctrlH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R1=0x600000|,
\lstinline[language=IslaLitmusExp]|0:R3=0x601000|,
\lstinline[language=IslaLitmusExp]|1:R1=0x601000|,
\lstinline[language=IslaLitmusExp]|1:R3=0x600000|,
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|LB+dmb.ld+ctrl|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\LBplusdmbdotldplusctrlN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\LBplusdmbdotldplusctrlM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\LBplusdmbdotldplusctrlO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\LBplusdmbdotldplusctrlI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\LBplusdmbdotldplusctrlK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R0=1 & 1:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/LB+pos.tex <==
\newlength{\LBplusposH}
\setlength{\LBplusposH}{0cm}
\newsavebox{\LBplusposI}
\begin{lrbox}{\LBplusposI}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR W0,[X1]
MOV W2,#1
STR W2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusposJ}
\settowidth{\LBplusposJ}{\usebox{\LBplusposI}}
\addtolength{\LBplusposH}{\LBplusposJ}
\newsavebox{\LBplusposK}
\begin{lrbox}{\LBplusposK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR W0,[X1]
MOV W2,#1
STR W2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusposL}
\settowidth{\LBplusposL}{\usebox{\LBplusposK}}
\addtolength{\LBplusposH}{\LBplusposL}
\newsavebox{\LBplusposM}
\begin{lrbox}{\LBplusposM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    y |-> pa2;
\end{lstlisting}
\end{lrbox}
\newlength{\LBplusposN}
\settowidth{\LBplusposN}{\usebox{\LBplusposM}}
\newsavebox{\LBplusposO}
\begin{lrbox}{\LBplusposO}
\begin{minipage}{\LBplusposH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R1=0x600000|,
\lstinline[language=IslaLitmusExp]|0:R3=0x601000|,
\lstinline[language=IslaLitmusExp]|1:R1=0x601000|,
\lstinline[language=IslaLitmusExp]|1:R3=0x600000|,
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|LB+pos|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\LBplusposN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\LBplusposM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\LBplusposO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\LBplusposI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\LBplusposK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R0=1 & 1:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/LB.TT.inv+pos.tex <==
\newlength{\LBdotTTdotinvplusposH}
\setlength{\LBdotTTdotinvplusposH}{0cm}
\newsavebox{\LBdotTTdotinvplusposI}
\begin{lrbox}{\LBdotTTdotinvplusposI}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\LBdotTTdotinvplusposJ}
\settowidth{\LBdotTTdotinvplusposJ}{\usebox{\LBdotTTdotinvplusposI}}
\addtolength{\LBdotTTdotinvplusposH}{\LBdotTTdotinvplusposJ}
\newsavebox{\LBdotTTdotinvplusposK}
\begin{lrbox}{\LBdotTTdotinvplusposK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\LBdotTTdotinvplusposL}
\settowidth{\LBdotTTdotinvplusposL}{\usebox{\LBdotTTdotinvplusposK}}
\addtolength{\LBdotTTdotinvplusposH}{\LBdotTTdotinvplusposL}
\newsavebox{\LBdotTTdotinvplusposM}
\begin{lrbox}{\LBdotTTdotinvplusposM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\LBdotTTdotinvplusposN}
\settowidth{\LBdotTTdotinvplusposN}{\usebox{\LBdotTTdotinvplusposM}}
\addtolength{\LBdotTTdotinvplusposH}{\LBdotTTdotinvplusposN}
\newsavebox{\LBdotTTdotinvplusposO}
\begin{lrbox}{\LBdotTTdotinvplusposO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\LBdotTTdotinvplusposP}
\settowidth{\LBdotTTdotinvplusposP}{\usebox{\LBdotTTdotinvplusposO}}
\addtolength{\LBdotTTdotinvplusposH}{\LBdotTTdotinvplusposP}
\newsavebox{\LBdotTTdotinvplusposA}
\begin{lrbox}{\LBdotTTdotinvplusposA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    y |-> invalid;

    x ?-> pa1;
    y ?-> pa1;

    *pa1 = 1;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\LBdotTTdotinvplusposB}
\settowidth{\LBdotTTdotinvplusposB}{\usebox{\LBdotTTdotinvplusposA}}
\newsavebox{\LBdotTTdotinvplusposC}
\begin{lrbox}{\LBdotTTdotinvplusposC}
\begin{minipage}{\LBdotTTdotinvplusposH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|LB.TT.inv+pos|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\LBdotTTdotinvplusposB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\LBdotTTdotinvplusposA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\LBdotTTdotinvplusposC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\LBdotTTdotinvplusposI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\LBdotTTdotinvplusposK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\LBdotTTdotinvplusposM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\LBdotTTdotinvplusposO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R0=1 & 1:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP+dmb.ld+ctrlisb.tex <==
\newlength{\MPplusdmbdotldplusctrlisbH}
\setlength{\MPplusdmbdotldplusctrlisbH}{0cm}
\newsavebox{\MPplusdmbdotldplusctrlisbI}
\begin{lrbox}{\MPplusdmbdotldplusctrlisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
MOV W0,#1
STR W0,[X1]
DMB LD
MOV W2,#1
STR W2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPplusdmbdotldplusctrlisbJ}
\settowidth{\MPplusdmbdotldplusctrlisbJ}{\usebox{\MPplusdmbdotldplusctrlisbI}}
\addtolength{\MPplusdmbdotldplusctrlisbH}{\MPplusdmbdotldplusctrlisbJ}
\newsavebox{\MPplusdmbdotldplusctrlisbK}
\begin{lrbox}{\MPplusdmbdotldplusctrlisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR W0,[X1]
CBNZ W0,LC00
LC00:
ISB
LDR W2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPplusdmbdotldplusctrlisbL}
\settowidth{\MPplusdmbdotldplusctrlisbL}{\usebox{\MPplusdmbdotldplusctrlisbK}}
\addtolength{\MPplusdmbdotldplusctrlisbH}{\MPplusdmbdotldplusctrlisbL}
\newsavebox{\MPplusdmbdotldplusctrlisbM}
\begin{lrbox}{\MPplusdmbdotldplusctrlisbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
	physical pa2;
    x |-> pa1;
    y |-> pa2;
\end{lstlisting}
\end{lrbox}
\newlength{\MPplusdmbdotldplusctrlisbN}
\settowidth{\MPplusdmbdotldplusctrlisbN}{\usebox{\MPplusdmbdotldplusctrlisbM}}
\newsavebox{\MPplusdmbdotldplusctrlisbO}
\begin{lrbox}{\MPplusdmbdotldplusctrlisbO}
\begin{minipage}{\MPplusdmbdotldplusctrlisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R1=0x600000|,
\lstinline[language=IslaLitmusExp]|0:R3=0x601000|,
\lstinline[language=IslaLitmusExp]|1:R1=0x601000|,
\lstinline[language=IslaLitmusExp]|1:R3=0x600000|,
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP+dmb.ld+ctrlisb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPplusdmbdotldplusctrlisbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPplusdmbdotldplusctrlisbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPplusdmbdotldplusctrlisbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPplusdmbdotldplusctrlisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPplusdmbdotldplusctrlisbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|x=1 & y=1 & 1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP+dmb.sy+ctrl.tex <==
\newlength{\MPplusdmbdotsyplusctrlH}
\setlength{\MPplusdmbdotsyplusctrlH}{0cm}
\newsavebox{\MPplusdmbdotsyplusctrlI}
\begin{lrbox}{\MPplusdmbdotsyplusctrlI}
\begin{lstlisting}[language=AArch64,showlines=true]
MOV W0,#1
STR W0,[X1]
DMB SY
MOV W2,#1
STR W2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPplusdmbdotsyplusctrlJ}
\settowidth{\MPplusdmbdotsyplusctrlJ}{\usebox{\MPplusdmbdotsyplusctrlI}}
\addtolength{\MPplusdmbdotsyplusctrlH}{\MPplusdmbdotsyplusctrlJ}
\newsavebox{\MPplusdmbdotsyplusctrlK}
\begin{lrbox}{\MPplusdmbdotsyplusctrlK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR W0,[X1]
CBNZ W0,LC00
LC00:
LDR W2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPplusdmbdotsyplusctrlL}
\settowidth{\MPplusdmbdotsyplusctrlL}{\usebox{\MPplusdmbdotsyplusctrlK}}
\addtolength{\MPplusdmbdotsyplusctrlH}{\MPplusdmbdotsyplusctrlL}
\newsavebox{\MPplusdmbdotsyplusctrlM}
\begin{lrbox}{\MPplusdmbdotsyplusctrlM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    y |-> pa2;
\end{lstlisting}
\end{lrbox}
\newlength{\MPplusdmbdotsyplusctrlN}
\settowidth{\MPplusdmbdotsyplusctrlN}{\usebox{\MPplusdmbdotsyplusctrlM}}
\newsavebox{\MPplusdmbdotsyplusctrlO}
\begin{lrbox}{\MPplusdmbdotsyplusctrlO}
\begin{minipage}{\MPplusdmbdotsyplusctrlH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R1=0x600000|,
\lstinline[language=IslaLitmusExp]|0:R3=0x601000|,
\lstinline[language=IslaLitmusExp]|1:R1=0x601000|,
\lstinline[language=IslaLitmusExp]|1:R3=0x600000|,
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP+dmb.sy+ctrl|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPplusdmbdotsyplusctrlN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPplusdmbdotsyplusctrlM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPplusdmbdotsyplusctrlO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPplusdmbdotsyplusctrlI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPplusdmbdotsyplusctrlK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|x=1 & y=1 & 1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP+pos.tex <==
\newlength{\MPplusposH}
\setlength{\MPplusposH}{0cm}
\newsavebox{\MPplusposI}
\begin{lrbox}{\MPplusposI}
\begin{lstlisting}[language=AArch64,showlines=true]
MOV W0,#1
STR W0,[X1]
MOV W2,#1
STR W2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPplusposJ}
\settowidth{\MPplusposJ}{\usebox{\MPplusposI}}
\addtolength{\MPplusposH}{\MPplusposJ}
\newsavebox{\MPplusposK}
\begin{lrbox}{\MPplusposK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR W0,[X1]
LDR W2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPplusposL}
\settowidth{\MPplusposL}{\usebox{\MPplusposK}}
\addtolength{\MPplusposH}{\MPplusposL}
\newsavebox{\MPplusposM}
\begin{lrbox}{\MPplusposM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    y |-> pa2;
\end{lstlisting}
\end{lrbox}
\newlength{\MPplusposN}
\settowidth{\MPplusposN}{\usebox{\MPplusposM}}
\newsavebox{\MPplusposO}
\begin{lrbox}{\MPplusposO}
\begin{minipage}{\MPplusposH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R1=0x600000|,
\lstinline[language=IslaLitmusExp]|0:R3=0x601000|,
\lstinline[language=IslaLitmusExp]|1:R1=0x601000|,
\lstinline[language=IslaLitmusExp]|1:R3=0x600000|,
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP+pos|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPplusposN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPplusposM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPplusposO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPplusposI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPplusposK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.BBM1+dsb-tlbiis-dsb-dsb+ctrl-isb.tex <==
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbH}
\setlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbH}{0cm}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbI}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X6
DSB SY
STR X2,[X1]
DSB SY
STR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbJ}
\settowidth{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbJ}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbI}}
\addtolength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbH}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbJ}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbK}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBNZ X0,L0
L0:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbL}
\settowidth{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbL}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbK}}
\addtolength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbH}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbL}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbM}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbN}
\settowidth{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbN}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbM}}
\addtolength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbH}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbN}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbO}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> pa1;
    x ?-> invalid;
    x ?-> pa2;

    y |-> pa3;
    identity 0x1000 with code;

    *pa2 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbP}
\settowidth{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbP}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbO}}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbA}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbA}
\begin{minipage}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R4=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R5=y|\\
\lstinline[language=IslaLitmusExp]|0:R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.BBM1+dsb-tlbiis-dsb-dsb+ctrl-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusctrlisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.BBM1+dsb-tlbiis-dsb-dsb+dsb-isb.tex <==
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbH}
\setlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbI}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X6
DSB SY
STR X2,[X1]
DSB SY
STR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbJ}
\settowidth{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbJ}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbI}}
\addtolength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbH}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbJ}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbK}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbL}
\settowidth{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbL}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbK}}
\addtolength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbH}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbL}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbM}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbN}
\settowidth{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbN}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbM}}
\addtolength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbH}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbN}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbO}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> pa1;
    x ?-> invalid;
    x ?-> pa2;

    y |-> pa3;
    identity 0x1000 with code;

    *pa2 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbP}
\settowidth{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbP}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbO}}
\newsavebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbA}
\begin{lrbox}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbA}
\begin{minipage}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R4=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R5=y|\\
\lstinline[language=IslaLitmusExp]|0:R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.BBM1+dsb-tlbiis-dsb-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotBBMoneplusdsbtlbiisdsbdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.RT.EL1+dsb+dsb-tlbi-dsb+dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbH}
\setlength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbJ}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbJ}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbI}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
TLBI VAE1,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbL}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbL}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbK}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbL}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbN}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbN}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbM}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbN}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbP}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbP}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbO}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbP}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbB}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbB}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbA}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbB}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbC}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> pa1;
    x ?-> invalid;

    y |-> pa2;

    a |-> pa3;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbD}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbD}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbC}}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbE}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbE}
\begin{minipage}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R3=a|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:R1=a|\\
\lstinline[language=IslaLitmusExp]|1:R2=0x2|\\
\lstinline[language=IslaLitmusExp]|1:R3=a|\\
\lstinline[language=IslaLitmusExp]|1:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|2:R1=a|\\
\lstinline[language=IslaLitmusExp]|2:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|2:R3=y|\\
\lstinline[language=IslaLitmusExp]|3:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|3:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|3:R1=y|\\
\lstinline[language=IslaLitmusExp]|3:R3=x|\\
\lstinline[language=IslaLitmusExp]|3:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL1+dsb+dsb-tlbi-dsb+dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbM}\\
  \cline{2-2}
  & Thread 3\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbO}\\
  \cline{2-2}
  & thread3 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbidsbplusdsbplusdsbisbA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=2 & 3:R0=1 & 3:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.RT.EL1+dsb+dsb-tlbiis-dsb+dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbH}
\setlength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbJ}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbJ}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbI}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbL}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbL}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbK}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbL}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbN}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbN}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbM}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbN}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbP}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbP}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbO}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbP}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbB}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbB}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbA}}
\addtolength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbB}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbC}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> pa1;
    x ?-> invalid;

    y |-> pa2;

    a |-> pa3;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbD}
\settowidth{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbD}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbC}}
\newsavebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbE}
\begin{lrbox}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbE}
\begin{minipage}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R3=a|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:R1=a|\\
\lstinline[language=IslaLitmusExp]|1:R2=0x2|\\
\lstinline[language=IslaLitmusExp]|1:R3=a|\\
\lstinline[language=IslaLitmusExp]|1:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|2:R1=a|\\
\lstinline[language=IslaLitmusExp]|2:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|2:R3=y|\\
\lstinline[language=IslaLitmusExp]|3:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|3:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|3:R1=y|\\
\lstinline[language=IslaLitmusExp]|3:R3=x|\\
\lstinline[language=IslaLitmusExp]|3:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL1+dsb+dsb-tlbiis-dsb+dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbM}\\
  \cline{2-2}
  & Thread 3\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbO}\\
  \cline{2-2}
  & thread3 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbplusdsbtlbiisdsbplusdsbplusdsbisbA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=2 & 3:R0=1 & 3:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.RT.EL1+dsb-shootdown-dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbH}
\setlength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X4,[X5]
LDR X6,[X5]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbJ}
\settowidth{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbJ}{\usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbI}}
\addtolength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbH}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X4,[X5]
SVC #0
STR X7,[X5]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbL}
\settowidth{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbL}{\usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbK}}
\addtolength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbH}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbL}
\newsavebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS X9,ESR_EL1
LSR X9,X9,#26
SUB X9,X9,#0b010101
CBNZ X9,1f
0:
DSB SY
TLBI VAE1,X6
DSB SY
ISB
ERET
1:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbN}
\settowidth{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbN}{\usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbM}}
\addtolength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbH}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbN}
\newsavebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> pa1;
    x ?-> invalid;

    y |-> pa2;
    *pa2 = 0;

    f |-> pa3;
    *pa3 = 0;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbP}
\settowidth{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbP}{\usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbO}}
\newsavebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbA}
\begin{minipage}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R5=f|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=f|\\
\lstinline[language=IslaLitmusExp]|1:R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:R7=0b10|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL1+dsb-shootdown-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbshootdowndsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R4=1 & 0:R6=2 & 1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.RT.EL1+dsb-tlbi-dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbH}
\setlength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbJ}
\settowidth{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbJ}{\usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbI}}
\addtolength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbH}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbL}
\settowidth{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbL}{\usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbK}}
\addtolength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbH}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbL}
\newsavebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbN}
\settowidth{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbN}{\usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbM}}
\addtolength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbH}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbN}
\newsavebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbP}
\settowidth{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbP}{\usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbO}}
\newsavebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbA}
\begin{minipage}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL1+dsb-tlbi-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbidsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.RT.EL1+dsb-tlbiis-dsb+dmb.tex <==
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbH}
\setlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbH}{0cm}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbI}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbJ}
\settowidth{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbJ}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbI}}
\addtolength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbJ}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbK}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbL}
\settowidth{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbL}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbK}}
\addtolength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbL}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbM}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbN}
\settowidth{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbN}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbM}}
\addtolength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbN}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbO}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbP}
\settowidth{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbP}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbO}}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbA}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbA}
\begin{minipage}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL1+dsb-tlbiis-dsb+dmb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdmbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.RT.EL1+dsb-tlbiis-dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbH}
\setlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbJ}
\settowidth{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbJ}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbI}}
\addtolength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbL}
\settowidth{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbL}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbK}}
\addtolength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbL}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbN}
\settowidth{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbN}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbM}}
\addtolength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbN}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbP}
\settowidth{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbP}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbO}}
\newsavebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbA}
\begin{minipage}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL1+dsb-tlbiis-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELoneplusdsbtlbiisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.RT.EL2+dsb-tlbiipa-dsb-tlbiis-dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbH}
\setlength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1,X4
DSB SY
TLBI VMALLE1IS
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbJ}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbJ}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbI}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbL}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbL}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbK}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbL}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#1
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbN}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbN}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbM}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbN}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
physical pa1 pa2;
intermediate ipa1 ipa2;

x |-> ipa1;
ipa1 |-> pa1;
ipa1 ?-> invalid;

y |-> ipa2;
ipa2 |-> pa2;

identity 0x2000 with code;

*pa1 = 0;
*pa2 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbP}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbP}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbO}}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbA}
\begin{minipage}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=bvlshr(ipa1,0xC)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL2+dsb-tlbiipa-dsb-tlbiis-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipadsbtlbiisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.RT.EL2+dsb-tlbiipais-dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbH}
\setlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbJ}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbJ}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbI}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbL}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbL}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbK}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbL}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#1
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbN}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbN}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbM}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbN}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
physical pa1 pa2;
intermediate ipa1 ipa2;

x |-> ipa1;
ipa1 |-> pa1;
ipa1 ?-> invalid;

y |-> ipa2;
ipa2 |-> pa2;

identity 0x2000 with code;

*pa1 = 1;
*pa2 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbP}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbP}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbO}}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbA}
\begin{minipage}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(ipa1)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL2+dsb-tlbiipais-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|true|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.RT.EL2+dsb-tlbiipais-dsb-tlbiis-dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbH}
\setlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1IS,X4
DSB SY
TLBI VMALLE1IS
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbJ}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbJ}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbI}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
isb
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbL}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbL}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbK}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbL}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#1
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbN}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbN}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbM}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbN}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
physical pa1 pa2;
intermediate ipa1 ipa2;

x |-> ipa1;
ipa1 |-> pa1;
ipa1 ?-> invalid;

y |-> ipa2;
ipa2 |-> pa2;

identity 0x2000 with code;

*pa1 = 0;
*pa2 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbP}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbP}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbO}}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbA}
\begin{minipage}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(ipa1)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL2+dsb-tlbiipais-dsb-tlbiis-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiipaisdsbtlbiisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.RT.EL2+dsb-tlbiis-dsb-tlbiipais-dsb+dsb-isb.tex <==
\newlength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbH}
\setlength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VMALLE1IS
DSB SY
TLBI IPAS2E1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbJ}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbJ}{\usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbI}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbJ}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
isb
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbL}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbL}{\usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbK}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbL}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#1
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbN}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbN}{\usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbM}}
\addtolength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbH}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbN}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
physical pa1 pa2;
intermediate ipa1 ipa2;

x |-> ipa1;
ipa1 |-> pa1;
ipa1 ?-> invalid;

y |-> ipa2;
ipa2 |-> pa2;

identity 0x2000 with code;

*pa1 = 0;
*pa2 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbP}
\settowidth{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbP}{\usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbO}}
\newsavebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbA}
\begin{minipage}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(ipa1)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.EL2+dsb-tlbiis-dsb-tlbiipais-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotELtwoplusdsbtlbiisdsbtlbiipaisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.RT.inv+dmb+addr-po-isb.tex <==
\newlength{\MPdotRTdotinvplusdmbplusaddrpoisbH}
\setlength{\MPdotRTdotinvplusdmbplusaddrpoisbH}{0cm}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpoisbI}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpoisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpoisbJ}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpoisbJ}{\usebox{\MPdotRTdotinvplusdmbplusaddrpoisbI}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpoisbH}{\MPdotRTdotinvplusdmbplusaddrpoisbJ}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpoisbK}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpoisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
EOR X6,X2,X2
LDR X7,[X8,X6]
ISB
LDR X4,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpoisbL}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpoisbL}{\usebox{\MPdotRTdotinvplusdmbplusaddrpoisbK}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpoisbH}{\MPdotRTdotinvplusdmbplusaddrpoisbL}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpoisbM}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpoisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpoisbN}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpoisbN}{\usebox{\MPdotRTdotinvplusdmbplusaddrpoisbM}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpoisbH}{\MPdotRTdotinvplusdmbplusaddrpoisbN}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpoisbO}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpoisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X4,#0
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpoisbP}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpoisbP}{\usebox{\MPdotRTdotinvplusdmbplusaddrpoisbO}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpoisbH}{\MPdotRTdotinvplusdmbplusaddrpoisbP}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpoisbA}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpoisbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;

    x |-> invalid;
    x ?-> pa1;

    y |-> pa2;

    z |-> pa3;

    *pa1 = 1;
    *pa2 = 0;
    *pa3 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpoisbB}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpoisbB}{\usebox{\MPdotRTdotinvplusdmbplusaddrpoisbA}}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpoisbC}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpoisbC}
\begin{minipage}{\MPdotRTdotinvplusdmbplusaddrpoisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R8=z|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.inv+dmb+addr-po-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotinvplusdmbplusaddrpoisbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotinvplusdmbplusaddrpoisbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotinvplusdmbplusaddrpoisbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpoisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpoisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpoisbM}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpoisbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R2=1 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.RT.inv+dmb+addr-po-msr-isb.tex <==
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrisbH}
\setlength{\MPdotRTdotinvplusdmbplusaddrpomsrisbH}{0cm}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbI}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrisbJ}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrisbJ}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbI}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpomsrisbH}{\MPdotRTdotinvplusdmbplusaddrpomsrisbJ}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbK}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
EOR X6,X2,X2
LDR X7,[X8,X6]
MSR ELR_EL1,X5
ISB
LDR X4,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrisbL}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrisbL}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbK}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpomsrisbH}{\MPdotRTdotinvplusdmbplusaddrpomsrisbL}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbM}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrisbN}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrisbN}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbM}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpomsrisbH}{\MPdotRTdotinvplusdmbplusaddrpomsrisbN}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbO}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X4,#0
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrisbP}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrisbP}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbO}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpomsrisbH}{\MPdotRTdotinvplusdmbplusaddrpomsrisbP}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbA}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrisbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;

    x |-> invalid;
    x ?-> pa1;

    y |-> pa2;

    z |-> pa3;

    *pa1 = 1;
    *pa2 = 0;
    *pa3 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrisbB}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrisbB}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbA}}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbC}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrisbC}
\begin{minipage}{\MPdotRTdotinvplusdmbplusaddrpomsrisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:R8=z|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.inv+dmb+addr-po-msr-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotinvplusdmbplusaddrpomsrisbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbM}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpomsrisbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R2=1 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.RT.inv+dmb+addr-po-msr.tex <==
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrH}
\setlength{\MPdotRTdotinvplusdmbplusaddrpomsrH}{0cm}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrI}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrJ}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrJ}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrI}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpomsrH}{\MPdotRTdotinvplusdmbplusaddrpomsrJ}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrK}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
EOR X6,X2,X2
LDR X7,[X8,X6]
MSR ELR_EL1,X5
LDR X4,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrL}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrL}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrK}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpomsrH}{\MPdotRTdotinvplusdmbplusaddrpomsrL}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrM}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrN}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrN}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrM}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpomsrH}{\MPdotRTdotinvplusdmbplusaddrpomsrN}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrO}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X4,#0
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrP}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrP}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrO}}
\addtolength{\MPdotRTdotinvplusdmbplusaddrpomsrH}{\MPdotRTdotinvplusdmbplusaddrpomsrP}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrA}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;

    x |-> invalid;
    x ?-> pa1;

    y |-> pa2;

    z |-> pa3;

    *pa1 = 1;
    *pa2 = 0;
    *pa3 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusaddrpomsrB}
\settowidth{\MPdotRTdotinvplusdmbplusaddrpomsrB}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrA}}
\newsavebox{\MPdotRTdotinvplusdmbplusaddrpomsrC}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusaddrpomsrC}
\begin{minipage}{\MPdotRTdotinvplusdmbplusaddrpomsrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:R8=z|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.inv+dmb+addr-po-msr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotinvplusdmbplusaddrpomsrB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotinvplusdmbplusaddrpomsrC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpomsrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpomsrK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpomsrM}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusaddrpomsrO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R2=1 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.RT.inv+dmb+ctrl-trfi.tex <==
\newlength{\MPdotRTdotinvplusdmbplusctrltrfiH}
\setlength{\MPdotRTdotinvplusdmbplusctrltrfiH}{0cm}
\newsavebox{\MPdotRTdotinvplusdmbplusctrltrfiI}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusctrltrfiI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusctrltrfiJ}
\settowidth{\MPdotRTdotinvplusdmbplusctrltrfiJ}{\usebox{\MPdotRTdotinvplusdmbplusctrltrfiI}}
\addtolength{\MPdotRTdotinvplusdmbplusctrltrfiH}{\MPdotRTdotinvplusdmbplusctrltrfiJ}
\newsavebox{\MPdotRTdotinvplusdmbplusctrltrfiK}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusctrltrfiK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBZ X0,LC00
LC00:
STR X2,[X3]
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusctrltrfiL}
\settowidth{\MPdotRTdotinvplusdmbplusctrltrfiL}{\usebox{\MPdotRTdotinvplusdmbplusctrltrfiK}}
\addtolength{\MPdotRTdotinvplusdmbplusctrltrfiH}{\MPdotRTdotinvplusdmbplusctrltrfiL}
\newsavebox{\MPdotRTdotinvplusdmbplusctrltrfiM}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusctrltrfiM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#2
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusctrltrfiN}
\settowidth{\MPdotRTdotinvplusdmbplusctrltrfiN}{\usebox{\MPdotRTdotinvplusdmbplusctrltrfiM}}
\addtolength{\MPdotRTdotinvplusdmbplusctrltrfiH}{\MPdotRTdotinvplusdmbplusctrltrfiN}
\newsavebox{\MPdotRTdotinvplusdmbplusctrltrfiO}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusctrltrfiO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    w |-> invalid;
    w ?-> pa1;
    x |-> pa1;
    *pa1 = 0;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplusdmbplusctrltrfiP}
\settowidth{\MPdotRTdotinvplusdmbplusctrltrfiP}{\usebox{\MPdotRTdotinvplusdmbplusctrltrfiO}}
\newsavebox{\MPdotRTdotinvplusdmbplusctrltrfiA}
\begin{lrbox}{\MPdotRTdotinvplusdmbplusctrltrfiA}
\begin{minipage}{\MPdotRTdotinvplusdmbplusctrltrfiH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(w,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R5=w|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.inv+dmb+ctrl-trfi|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotinvplusdmbplusctrltrfiP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotinvplusdmbplusctrltrfiO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotinvplusdmbplusctrltrfiA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusctrltrfiI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusctrltrfiK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplusdmbplusctrltrfiM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.RT.inv+trfi-data+addr.toml.tex <==
\newlength{\MPdotRTdotinvplustrfidataplusaddrdottomlH}
\setlength{\MPdotRTdotinvplustrfidataplusaddrdottomlH}{0cm}
\newsavebox{\MPdotRTdotinvplustrfidataplusaddrdottomlI}
\begin{lrbox}{\MPdotRTdotinvplustrfidataplusaddrdottomlI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
STR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplustrfidataplusaddrdottomlJ}
\settowidth{\MPdotRTdotinvplustrfidataplusaddrdottomlJ}{\usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlI}}
\addtolength{\MPdotRTdotinvplustrfidataplusaddrdottomlH}{\MPdotRTdotinvplustrfidataplusaddrdottomlJ}
\newsavebox{\MPdotRTdotinvplustrfidataplusaddrdottomlK}
\begin{lrbox}{\MPdotRTdotinvplustrfidataplusaddrdottomlK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
LDR X3,[X4,X2]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplustrfidataplusaddrdottomlL}
\settowidth{\MPdotRTdotinvplustrfidataplusaddrdottomlL}{\usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlK}}
\addtolength{\MPdotRTdotinvplustrfidataplusaddrdottomlH}{\MPdotRTdotinvplustrfidataplusaddrdottomlL}
\newsavebox{\MPdotRTdotinvplustrfidataplusaddrdottomlM}
\begin{lrbox}{\MPdotRTdotinvplustrfidataplusaddrdottomlM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplustrfidataplusaddrdottomlN}
\settowidth{\MPdotRTdotinvplustrfidataplusaddrdottomlN}{\usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlM}}
\addtolength{\MPdotRTdotinvplustrfidataplusaddrdottomlH}{\MPdotRTdotinvplustrfidataplusaddrdottomlN}
\newsavebox{\MPdotRTdotinvplustrfidataplusaddrdottomlO}
\begin{lrbox}{\MPdotRTdotinvplustrfidataplusaddrdottomlO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X3,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplustrfidataplusaddrdottomlP}
\settowidth{\MPdotRTdotinvplustrfidataplusaddrdottomlP}{\usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlO}}
\addtolength{\MPdotRTdotinvplustrfidataplusaddrdottomlH}{\MPdotRTdotinvplustrfidataplusaddrdottomlP}
\newsavebox{\MPdotRTdotinvplustrfidataplusaddrdottomlA}
\begin{lrbox}{\MPdotRTdotinvplustrfidataplusaddrdottomlA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    w |-> invalid;
    w ?-> pa1;
    x |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTdotinvplustrfidataplusaddrdottomlB}
\settowidth{\MPdotRTdotinvplustrfidataplusaddrdottomlB}{\usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlA}}
\newsavebox{\MPdotRTdotinvplustrfidataplusaddrdottomlC}
\begin{lrbox}{\MPdotRTdotinvplustrfidataplusaddrdottomlC}
\begin{minipage}{\MPdotRTdotinvplustrfidataplusaddrdottomlH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(w,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R3=w|\\
\lstinline[language=IslaLitmusExp]|0:R4=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R5=y|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(w,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R4=w|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RT.inv+trfi-data+addr.toml|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTdotinvplustrfidataplusaddrdottomlB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTdotinvplustrfidataplusaddrdottomlO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=1 & 1:R0=1 & 1:R3=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.RTT.EL1+dsb-tlbiis-tlbiis-dsb+dsb-isb.tex <==
\newlength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbH}
\setlength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
STR X2,[X3]
DSB SY
TLBI VAE1IS,X4
TLBI VAE1IS,X5
DSB SY
STR X6,[X7]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbJ}
\settowidth{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbJ}{\usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbI}}
\addtolength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbH}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbJ}
\newsavebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X4,[X3]
MOV X2,X4
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbL}
\settowidth{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbL}{\usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbK}}
\addtolength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbH}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbL}
\newsavebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X4,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbN}
\settowidth{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbN}{\usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbM}}
\addtolength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbH}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbN}
\newsavebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> pa1;
    x ?-> invalid;

    y |-> pa2;

    z |-> pa3;
    z ?-> invalid;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbP}
\settowidth{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbP}{\usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbO}}
\newsavebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbA}
\begin{minipage}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|0:R5=page(z)|\\
\lstinline[language=IslaLitmusExp]|0:R6=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R7=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=z|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTT.EL1+dsb-tlbiis-tlbiis-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTTdotELoneplusdsbtlbiistlbiisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.RTf.inv+dmb+addr.tex <==
\newlength{\MPdotRTfdotinvplusdmbplusaddrH}
\setlength{\MPdotRTfdotinvplusdmbplusaddrH}{0cm}
\newsavebox{\MPdotRTfdotinvplusdmbplusaddrI}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusaddrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB ST
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusaddrJ}
\settowidth{\MPdotRTfdotinvplusdmbplusaddrJ}{\usebox{\MPdotRTfdotinvplusdmbplusaddrI}}
\addtolength{\MPdotRTfdotinvplusdmbplusaddrH}{\MPdotRTfdotinvplusdmbplusaddrJ}
\newsavebox{\MPdotRTfdotinvplusdmbplusaddrK}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusaddrK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusaddrL}
\settowidth{\MPdotRTfdotinvplusdmbplusaddrL}{\usebox{\MPdotRTfdotinvplusdmbplusaddrK}}
\addtolength{\MPdotRTfdotinvplusdmbplusaddrH}{\MPdotRTfdotinvplusdmbplusaddrL}
\newsavebox{\MPdotRTfdotinvplusdmbplusaddrM}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusaddrM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusaddrN}
\settowidth{\MPdotRTfdotinvplusdmbplusaddrN}{\usebox{\MPdotRTfdotinvplusdmbplusaddrM}}
\addtolength{\MPdotRTfdotinvplusdmbplusaddrH}{\MPdotRTfdotinvplusdmbplusaddrN}
\newsavebox{\MPdotRTfdotinvplusdmbplusaddrO}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusaddrO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusaddrP}
\settowidth{\MPdotRTfdotinvplusdmbplusaddrP}{\usebox{\MPdotRTfdotinvplusdmbplusaddrO}}
\newsavebox{\MPdotRTfdotinvplusdmbplusaddrA}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusaddrA}
\begin{minipage}{\MPdotRTfdotinvplusdmbplusaddrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv+dmb+addr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvplusdmbplusaddrP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvplusdmbplusaddrO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvplusdmbplusaddrA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusaddrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusaddrK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusaddrM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.RTf.inv+dmb+ctrl-isb.tex <==
\newlength{\MPdotRTfdotinvplusdmbplusctrlisbH}
\setlength{\MPdotRTfdotinvplusdmbplusctrlisbH}{0cm}
\newsavebox{\MPdotRTfdotinvplusdmbplusctrlisbI}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusctrlisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusctrlisbJ}
\settowidth{\MPdotRTfdotinvplusdmbplusctrlisbJ}{\usebox{\MPdotRTfdotinvplusdmbplusctrlisbI}}
\addtolength{\MPdotRTfdotinvplusdmbplusctrlisbH}{\MPdotRTfdotinvplusdmbplusctrlisbJ}
\newsavebox{\MPdotRTfdotinvplusdmbplusctrlisbK}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusctrlisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBNZ X0,L0
L0:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusctrlisbL}
\settowidth{\MPdotRTfdotinvplusdmbplusctrlisbL}{\usebox{\MPdotRTfdotinvplusdmbplusctrlisbK}}
\addtolength{\MPdotRTfdotinvplusdmbplusctrlisbH}{\MPdotRTfdotinvplusdmbplusctrlisbL}
\newsavebox{\MPdotRTfdotinvplusdmbplusctrlisbM}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusctrlisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusctrlisbN}
\settowidth{\MPdotRTfdotinvplusdmbplusctrlisbN}{\usebox{\MPdotRTfdotinvplusdmbplusctrlisbM}}
\addtolength{\MPdotRTfdotinvplusdmbplusctrlisbH}{\MPdotRTfdotinvplusdmbplusctrlisbN}
\newsavebox{\MPdotRTfdotinvplusdmbplusctrlisbO}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusctrlisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusctrlisbP}
\settowidth{\MPdotRTfdotinvplusdmbplusctrlisbP}{\usebox{\MPdotRTfdotinvplusdmbplusctrlisbO}}
\newsavebox{\MPdotRTfdotinvplusdmbplusctrlisbA}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusctrlisbA}
\begin{minipage}{\MPdotRTfdotinvplusdmbplusctrlisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv+dmb+ctrl-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvplusdmbplusctrlisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvplusdmbplusctrlisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvplusdmbplusctrlisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusctrlisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusctrlisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusctrlisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.RTf.inv+dmb+data.tex <==
\newlength{\MPdotRTfdotinvplusdmbplusdataH}
\setlength{\MPdotRTfdotinvplusdmbplusdataH}{0cm}
\newsavebox{\MPdotRTfdotinvplusdmbplusdataI}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdataI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB ST
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusdataJ}
\settowidth{\MPdotRTfdotinvplusdmbplusdataJ}{\usebox{\MPdotRTfdotinvplusdmbplusdataI}}
\addtolength{\MPdotRTfdotinvplusdmbplusdataH}{\MPdotRTfdotinvplusdmbplusdataJ}
\newsavebox{\MPdotRTfdotinvplusdmbplusdataK}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdataK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
ORR X6,X4,X5
STR X6,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusdataL}
\settowidth{\MPdotRTfdotinvplusdmbplusdataL}{\usebox{\MPdotRTfdotinvplusdmbplusdataK}}
\addtolength{\MPdotRTfdotinvplusdmbplusdataH}{\MPdotRTfdotinvplusdmbplusdataL}
\newsavebox{\MPdotRTfdotinvplusdmbplusdataM}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdataM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusdataN}
\settowidth{\MPdotRTfdotinvplusdmbplusdataN}{\usebox{\MPdotRTfdotinvplusdmbplusdataM}}
\addtolength{\MPdotRTfdotinvplusdmbplusdataH}{\MPdotRTfdotinvplusdmbplusdataN}
\newsavebox{\MPdotRTfdotinvplusdmbplusdataO}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdataO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusdataP}
\settowidth{\MPdotRTfdotinvplusdmbplusdataP}{\usebox{\MPdotRTfdotinvplusdmbplusdataO}}
\newsavebox{\MPdotRTfdotinvplusdmbplusdataA}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdataA}
\begin{minipage}{\MPdotRTfdotinvplusdmbplusdataH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=0b1|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv+dmb+data|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvplusdmbplusdataP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvplusdmbplusdataO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvplusdmbplusdataA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusdataI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusdataK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusdataM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.RTf.inv+dmb+dsb-isb.tex <==
\newlength{\MPdotRTfdotinvplusdmbplusdsbisbH}
\setlength{\MPdotRTfdotinvplusdmbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTfdotinvplusdmbplusdsbisbI}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusdsbisbJ}
\settowidth{\MPdotRTfdotinvplusdmbplusdsbisbJ}{\usebox{\MPdotRTfdotinvplusdmbplusdsbisbI}}
\addtolength{\MPdotRTfdotinvplusdmbplusdsbisbH}{\MPdotRTfdotinvplusdmbplusdsbisbJ}
\newsavebox{\MPdotRTfdotinvplusdmbplusdsbisbK}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusdsbisbL}
\settowidth{\MPdotRTfdotinvplusdmbplusdsbisbL}{\usebox{\MPdotRTfdotinvplusdmbplusdsbisbK}}
\addtolength{\MPdotRTfdotinvplusdmbplusdsbisbH}{\MPdotRTfdotinvplusdmbplusdsbisbL}
\newsavebox{\MPdotRTfdotinvplusdmbplusdsbisbM}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusdsbisbN}
\settowidth{\MPdotRTfdotinvplusdmbplusdsbisbN}{\usebox{\MPdotRTfdotinvplusdmbplusdsbisbM}}
\addtolength{\MPdotRTfdotinvplusdmbplusdsbisbH}{\MPdotRTfdotinvplusdmbplusdsbisbN}
\newsavebox{\MPdotRTfdotinvplusdmbplusdsbisbO}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbplusdsbisbP}
\settowidth{\MPdotRTfdotinvplusdmbplusdsbisbP}{\usebox{\MPdotRTfdotinvplusdmbplusdsbisbO}}
\newsavebox{\MPdotRTfdotinvplusdmbplusdsbisbA}
\begin{lrbox}{\MPdotRTfdotinvplusdmbplusdsbisbA}
\begin{minipage}{\MPdotRTfdotinvplusdmbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv+dmb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvplusdmbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvplusdmbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvplusdmbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.RTf.inv+dmb+po.tex <==
\newlength{\MPdotRTfdotinvplusdmbpluspoH}
\setlength{\MPdotRTfdotinvplusdmbpluspoH}{0cm}
\newsavebox{\MPdotRTfdotinvplusdmbpluspoI}
\begin{lrbox}{\MPdotRTfdotinvplusdmbpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB ST
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbpluspoJ}
\settowidth{\MPdotRTfdotinvplusdmbpluspoJ}{\usebox{\MPdotRTfdotinvplusdmbpluspoI}}
\addtolength{\MPdotRTfdotinvplusdmbpluspoH}{\MPdotRTfdotinvplusdmbpluspoJ}
\newsavebox{\MPdotRTfdotinvplusdmbpluspoK}
\begin{lrbox}{\MPdotRTfdotinvplusdmbpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbpluspoL}
\settowidth{\MPdotRTfdotinvplusdmbpluspoL}{\usebox{\MPdotRTfdotinvplusdmbpluspoK}}
\addtolength{\MPdotRTfdotinvplusdmbpluspoH}{\MPdotRTfdotinvplusdmbpluspoL}
\newsavebox{\MPdotRTfdotinvplusdmbpluspoM}
\begin{lrbox}{\MPdotRTfdotinvplusdmbpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbpluspoN}
\settowidth{\MPdotRTfdotinvplusdmbpluspoN}{\usebox{\MPdotRTfdotinvplusdmbpluspoM}}
\addtolength{\MPdotRTfdotinvplusdmbpluspoH}{\MPdotRTfdotinvplusdmbpluspoN}
\newsavebox{\MPdotRTfdotinvplusdmbpluspoO}
\begin{lrbox}{\MPdotRTfdotinvplusdmbpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbpluspoP}
\settowidth{\MPdotRTfdotinvplusdmbpluspoP}{\usebox{\MPdotRTfdotinvplusdmbpluspoO}}
\newsavebox{\MPdotRTfdotinvplusdmbpluspoA}
\begin{lrbox}{\MPdotRTfdotinvplusdmbpluspoA}
\begin{minipage}{\MPdotRTfdotinvplusdmbpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv+dmb+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvplusdmbpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvplusdmbpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvplusdmbpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.RTf.inv+dmbs.tex <==
\newlength{\MPdotRTfdotinvplusdmbsH}
\setlength{\MPdotRTfdotinvplusdmbsH}{0cm}
\newsavebox{\MPdotRTfdotinvplusdmbsI}
\begin{lrbox}{\MPdotRTfdotinvplusdmbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB ST
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbsJ}
\settowidth{\MPdotRTfdotinvplusdmbsJ}{\usebox{\MPdotRTfdotinvplusdmbsI}}
\addtolength{\MPdotRTfdotinvplusdmbsH}{\MPdotRTfdotinvplusdmbsJ}
\newsavebox{\MPdotRTfdotinvplusdmbsK}
\begin{lrbox}{\MPdotRTfdotinvplusdmbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbsL}
\settowidth{\MPdotRTfdotinvplusdmbsL}{\usebox{\MPdotRTfdotinvplusdmbsK}}
\addtolength{\MPdotRTfdotinvplusdmbsH}{\MPdotRTfdotinvplusdmbsL}
\newsavebox{\MPdotRTfdotinvplusdmbsM}
\begin{lrbox}{\MPdotRTfdotinvplusdmbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbsN}
\settowidth{\MPdotRTfdotinvplusdmbsN}{\usebox{\MPdotRTfdotinvplusdmbsM}}
\addtolength{\MPdotRTfdotinvplusdmbsH}{\MPdotRTfdotinvplusdmbsN}
\newsavebox{\MPdotRTfdotinvplusdmbsO}
\begin{lrbox}{\MPdotRTfdotinvplusdmbsO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvplusdmbsP}
\settowidth{\MPdotRTfdotinvplusdmbsP}{\usebox{\MPdotRTfdotinvplusdmbsO}}
\newsavebox{\MPdotRTfdotinvplusdmbsA}
\begin{lrbox}{\MPdotRTfdotinvplusdmbsA}
\begin{minipage}{\MPdotRTfdotinvplusdmbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv+dmbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvplusdmbsP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvplusdmbsO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvplusdmbsA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbsK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvplusdmbsM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.RTf.inv.EL1+dsb-tlbiis-dsb+addr.tex <==
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrH}
\setlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrH}{0cm}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrI}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrJ}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrJ}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrI}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrJ}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrK}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrL}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrL}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrK}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrL}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrM}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrN}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrN}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrM}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrN}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrO}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrP}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrP}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrO}}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrA}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrA}
\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv.EL1+dsb-tlbiis-dsb+addr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusaddrM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.RTf.inv.EL1+dsb-tlbiis-dsb+ctrl-isb.tex <==
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbH}
\setlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbH}{0cm}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbI}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbJ}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbJ}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbI}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbJ}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbK}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBNZ X0,L0
L0:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbL}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbL}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbK}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbL}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbM}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbN}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbN}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbM}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbN}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbO}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbP}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbP}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbO}}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbA}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbA}
\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv.EL1+dsb-tlbiis-dsb+ctrl-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.RTf.inv.EL1+dsb-tlbiis-dsb+ctrl.tex <==
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}
\setlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}{0cm}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlI}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlJ}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlJ}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlI}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlJ}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlK}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBNZ X0,L0
L0:
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlL}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlL}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlK}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlL}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlM}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlN}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlN}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlM}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlN}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlO}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlP}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlP}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlO}}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlA}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlA}
\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv.EL1+dsb-tlbiis-dsb+ctrl|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.RTf.inv.EL1+dsb-tlbiis-dsb+data.tex <==
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}
\setlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}{0cm}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataI}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataJ}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataJ}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataI}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataJ}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataK}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
STR X4,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataL}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataL}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataK}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataL}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataM}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataN}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataN}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataM}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataN}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataO}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataP}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataP}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataO}}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataA}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataA}
\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv.EL1+dsb-tlbiis-dsb+data|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.RTf.inv.EL1+dsb-tlbiis-dsb+dmb.tex <==
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}
\setlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{0cm}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}
\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv.EL1+dsb-tlbiis-dsb+dmb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.RTf.inv.EL1+dsb-tlbiis-dsb+dsb-isb.tex <==
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}
\setlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbI}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbJ}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbJ}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbI}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbJ}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbK}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbL}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbL}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbK}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbL}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbM}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbN}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbN}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbM}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbN}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbO}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbP}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbP}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbO}}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbA}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbA}
\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv.EL1+dsb-tlbiis-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.RTf.inv.EL1+dsb-tlbiis-dsb+po.tex <==
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}
\setlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}{0cm}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoI}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoJ}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoJ}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoI}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoJ}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoK}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoL}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoL}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoK}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoL}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoM}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoN}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoN}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoM}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoN}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoO}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoP}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoP}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoO}}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoA}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoA}
\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv.EL1+dsb-tlbiis-dsb+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.RTf.inv.EL1+dsb-tlbiis-dsb+poap.tex <==
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}
\setlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}{0cm}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapI}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapJ}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapJ}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapI}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapJ}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapK}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDAR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapL}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapL}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapK}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapL}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapM}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapN}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapN}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapM}}
\addtolength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapN}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapO}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapP}
\settowidth{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapP}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapO}}
\newsavebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapA}
\begin{lrbox}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapA}
\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.RTf.inv.EL1+dsb-tlbiis-dsb+poap|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.TR.inv+dmb+isb.tex <==
\newlength{\MPdotTRdotinvplusdmbplusisbH}
\setlength{\MPdotTRdotinvplusdmbplusisbH}{0cm}
\newsavebox{\MPdotTRdotinvplusdmbplusisbI}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusisbJ}
\settowidth{\MPdotTRdotinvplusdmbplusisbJ}{\usebox{\MPdotTRdotinvplusdmbplusisbI}}
\addtolength{\MPdotTRdotinvplusdmbplusisbH}{\MPdotTRdotinvplusdmbplusisbJ}
\newsavebox{\MPdotTRdotinvplusdmbplusisbK}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
ISB
LDR X4,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusisbL}
\settowidth{\MPdotTRdotinvplusdmbplusisbL}{\usebox{\MPdotTRdotinvplusdmbplusisbK}}
\addtolength{\MPdotTRdotinvplusdmbplusisbH}{\MPdotTRdotinvplusdmbplusisbL}
\newsavebox{\MPdotTRdotinvplusdmbplusisbM}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusisbN}
\settowidth{\MPdotTRdotinvplusdmbplusisbN}{\usebox{\MPdotTRdotinvplusdmbplusisbM}}
\addtolength{\MPdotTRdotinvplusdmbplusisbH}{\MPdotTRdotinvplusdmbplusisbN}
\newsavebox{\MPdotTRdotinvplusdmbplusisbO}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusisbP}
\settowidth{\MPdotTRdotinvplusdmbplusisbP}{\usebox{\MPdotTRdotinvplusdmbplusisbO}}
\addtolength{\MPdotTRdotinvplusdmbplusisbH}{\MPdotTRdotinvplusdmbplusisbP}
\newsavebox{\MPdotTRdotinvplusdmbplusisbA}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusisbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 0;
    *pa2 = 1;
    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusisbB}
\settowidth{\MPdotTRdotinvplusdmbplusisbB}{\usebox{\MPdotTRdotinvplusdmbplusisbA}}
\newsavebox{\MPdotTRdotinvplusdmbplusisbC}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusisbC}
\begin{minipage}{\MPdotTRdotinvplusdmbplusisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TR.inv+dmb+isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTRdotinvplusdmbplusisbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTRdotinvplusdmbplusisbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTRdotinvplusdmbplusisbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusisbM}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusisbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R2=1 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.TR.inv+dmb+msr-isb.tex <==
\newlength{\MPdotTRdotinvplusdmbplusmsrisbH}
\setlength{\MPdotTRdotinvplusdmbplusmsrisbH}{0cm}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrisbI}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrisbJ}
\settowidth{\MPdotTRdotinvplusdmbplusmsrisbJ}{\usebox{\MPdotTRdotinvplusdmbplusmsrisbI}}
\addtolength{\MPdotTRdotinvplusdmbplusmsrisbH}{\MPdotTRdotinvplusdmbplusmsrisbJ}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrisbK}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MSR ELR_EL1,X5
ISB
LDR X4,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrisbL}
\settowidth{\MPdotTRdotinvplusdmbplusmsrisbL}{\usebox{\MPdotTRdotinvplusdmbplusmsrisbK}}
\addtolength{\MPdotTRdotinvplusdmbplusmsrisbH}{\MPdotTRdotinvplusdmbplusmsrisbL}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrisbM}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrisbN}
\settowidth{\MPdotTRdotinvplusdmbplusmsrisbN}{\usebox{\MPdotTRdotinvplusdmbplusmsrisbM}}
\addtolength{\MPdotTRdotinvplusdmbplusmsrisbH}{\MPdotTRdotinvplusdmbplusmsrisbN}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrisbO}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrisbP}
\settowidth{\MPdotTRdotinvplusdmbplusmsrisbP}{\usebox{\MPdotTRdotinvplusdmbplusmsrisbO}}
\addtolength{\MPdotTRdotinvplusdmbplusmsrisbH}{\MPdotTRdotinvplusdmbplusmsrisbP}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrisbA}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrisbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 0;
    *pa2 = 1;
    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrisbB}
\settowidth{\MPdotTRdotinvplusdmbplusmsrisbB}{\usebox{\MPdotTRdotinvplusdmbplusmsrisbA}}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrisbC}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrisbC}
\begin{minipage}{\MPdotTRdotinvplusdmbplusmsrisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TR.inv+dmb+msr-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTRdotinvplusdmbplusmsrisbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTRdotinvplusdmbplusmsrisbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTRdotinvplusdmbplusmsrisbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusmsrisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusmsrisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusmsrisbM}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusmsrisbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R2=1 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.TR.inv+dmb+msr.tex <==
\newlength{\MPdotTRdotinvplusdmbplusmsrH}
\setlength{\MPdotTRdotinvplusdmbplusmsrH}{0cm}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrI}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrJ}
\settowidth{\MPdotTRdotinvplusdmbplusmsrJ}{\usebox{\MPdotTRdotinvplusdmbplusmsrI}}
\addtolength{\MPdotTRdotinvplusdmbplusmsrH}{\MPdotTRdotinvplusdmbplusmsrJ}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrK}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MSR ELR_EL1,X5
LDR X4,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrL}
\settowidth{\MPdotTRdotinvplusdmbplusmsrL}{\usebox{\MPdotTRdotinvplusdmbplusmsrK}}
\addtolength{\MPdotTRdotinvplusdmbplusmsrH}{\MPdotTRdotinvplusdmbplusmsrL}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrM}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrN}
\settowidth{\MPdotTRdotinvplusdmbplusmsrN}{\usebox{\MPdotTRdotinvplusdmbplusmsrM}}
\addtolength{\MPdotTRdotinvplusdmbplusmsrH}{\MPdotTRdotinvplusdmbplusmsrN}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrO}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL2
ADD X13,X13,#4
MSR ELR_EL2,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrP}
\settowidth{\MPdotTRdotinvplusdmbplusmsrP}{\usebox{\MPdotTRdotinvplusdmbplusmsrO}}
\addtolength{\MPdotTRdotinvplusdmbplusmsrH}{\MPdotTRdotinvplusdmbplusmsrP}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrA}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 0;
    *pa2 = 1;
    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTRdotinvplusdmbplusmsrB}
\settowidth{\MPdotTRdotinvplusdmbplusmsrB}{\usebox{\MPdotTRdotinvplusdmbplusmsrA}}
\newsavebox{\MPdotTRdotinvplusdmbplusmsrC}
\begin{lrbox}{\MPdotTRdotinvplusdmbplusmsrC}
\begin{minipage}{\MPdotTRdotinvplusdmbplusmsrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TR.inv+dmb+msr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTRdotinvplusdmbplusmsrB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTRdotinvplusdmbplusmsrA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTRdotinvplusdmbplusmsrC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusmsrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusmsrK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusmsrM}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\MPdotTRdotinvplusdmbplusmsrO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R2=1 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.TTf.inv+dmb+addr.tex <==
\newlength{\MPdotTTfdotinvplusdmbplusaddrH}
\setlength{\MPdotTTfdotinvplusdmbplusaddrH}{0cm}
\newsavebox{\MPdotTTfdotinvplusdmbplusaddrI}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusaddrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbplusaddrJ}
\settowidth{\MPdotTTfdotinvplusdmbplusaddrJ}{\usebox{\MPdotTTfdotinvplusdmbplusaddrI}}
\addtolength{\MPdotTTfdotinvplusdmbplusaddrH}{\MPdotTTfdotinvplusdmbplusaddrJ}
\newsavebox{\MPdotTTfdotinvplusdmbplusaddrK}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusaddrK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
EOR X4,X0,X0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbplusaddrL}
\settowidth{\MPdotTTfdotinvplusdmbplusaddrL}{\usebox{\MPdotTTfdotinvplusdmbplusaddrK}}
\addtolength{\MPdotTTfdotinvplusdmbplusaddrH}{\MPdotTTfdotinvplusdmbplusaddrL}
\newsavebox{\MPdotTTfdotinvplusdmbplusaddrM}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusaddrM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbplusaddrN}
\settowidth{\MPdotTTfdotinvplusdmbplusaddrN}{\usebox{\MPdotTTfdotinvplusdmbplusaddrM}}
\addtolength{\MPdotTTfdotinvplusdmbplusaddrH}{\MPdotTTfdotinvplusdmbplusaddrN}
\newsavebox{\MPdotTTfdotinvplusdmbplusaddrO}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusaddrO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbplusaddrP}
\settowidth{\MPdotTTfdotinvplusdmbplusaddrP}{\usebox{\MPdotTTfdotinvplusdmbplusaddrO}}
\newsavebox{\MPdotTTfdotinvplusdmbplusaddrA}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusaddrA}
\begin{minipage}{\MPdotTTfdotinvplusdmbplusaddrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv+dmb+addr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvplusdmbplusaddrP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvplusdmbplusaddrO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvplusdmbplusaddrA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbplusaddrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbplusaddrK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbplusaddrM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.TTf.inv+dmb+dsb-isb.tex <==
\newlength{\MPdotTTfdotinvplusdmbplusdsbisbH}
\setlength{\MPdotTTfdotinvplusdmbplusdsbisbH}{0cm}
\newsavebox{\MPdotTTfdotinvplusdmbplusdsbisbI}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbplusdsbisbJ}
\settowidth{\MPdotTTfdotinvplusdmbplusdsbisbJ}{\usebox{\MPdotTTfdotinvplusdmbplusdsbisbI}}
\addtolength{\MPdotTTfdotinvplusdmbplusdsbisbH}{\MPdotTTfdotinvplusdmbplusdsbisbJ}
\newsavebox{\MPdotTTfdotinvplusdmbplusdsbisbK}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbplusdsbisbL}
\settowidth{\MPdotTTfdotinvplusdmbplusdsbisbL}{\usebox{\MPdotTTfdotinvplusdmbplusdsbisbK}}
\addtolength{\MPdotTTfdotinvplusdmbplusdsbisbH}{\MPdotTTfdotinvplusdmbplusdsbisbL}
\newsavebox{\MPdotTTfdotinvplusdmbplusdsbisbM}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbplusdsbisbN}
\settowidth{\MPdotTTfdotinvplusdmbplusdsbisbN}{\usebox{\MPdotTTfdotinvplusdmbplusdsbisbM}}
\addtolength{\MPdotTTfdotinvplusdmbplusdsbisbH}{\MPdotTTfdotinvplusdmbplusdsbisbN}
\newsavebox{\MPdotTTfdotinvplusdmbplusdsbisbO}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbplusdsbisbP}
\settowidth{\MPdotTTfdotinvplusdmbplusdsbisbP}{\usebox{\MPdotTTfdotinvplusdmbplusdsbisbO}}
\newsavebox{\MPdotTTfdotinvplusdmbplusdsbisbA}
\begin{lrbox}{\MPdotTTfdotinvplusdmbplusdsbisbA}
\begin{minipage}{\MPdotTTfdotinvplusdmbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv+dmb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvplusdmbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvplusdmbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvplusdmbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.TTf.inv+dmb+po.tex <==
\newlength{\MPdotTTfdotinvplusdmbpluspoH}
\setlength{\MPdotTTfdotinvplusdmbpluspoH}{0cm}
\newsavebox{\MPdotTTfdotinvplusdmbpluspoI}
\begin{lrbox}{\MPdotTTfdotinvplusdmbpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbpluspoJ}
\settowidth{\MPdotTTfdotinvplusdmbpluspoJ}{\usebox{\MPdotTTfdotinvplusdmbpluspoI}}
\addtolength{\MPdotTTfdotinvplusdmbpluspoH}{\MPdotTTfdotinvplusdmbpluspoJ}
\newsavebox{\MPdotTTfdotinvplusdmbpluspoK}
\begin{lrbox}{\MPdotTTfdotinvplusdmbpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbpluspoL}
\settowidth{\MPdotTTfdotinvplusdmbpluspoL}{\usebox{\MPdotTTfdotinvplusdmbpluspoK}}
\addtolength{\MPdotTTfdotinvplusdmbpluspoH}{\MPdotTTfdotinvplusdmbpluspoL}
\newsavebox{\MPdotTTfdotinvplusdmbpluspoM}
\begin{lrbox}{\MPdotTTfdotinvplusdmbpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbpluspoN}
\settowidth{\MPdotTTfdotinvplusdmbpluspoN}{\usebox{\MPdotTTfdotinvplusdmbpluspoM}}
\addtolength{\MPdotTTfdotinvplusdmbpluspoH}{\MPdotTTfdotinvplusdmbpluspoN}
\newsavebox{\MPdotTTfdotinvplusdmbpluspoO}
\begin{lrbox}{\MPdotTTfdotinvplusdmbpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdmbpluspoP}
\settowidth{\MPdotTTfdotinvplusdmbpluspoP}{\usebox{\MPdotTTfdotinvplusdmbpluspoO}}
\newsavebox{\MPdotTTfdotinvplusdmbpluspoA}
\begin{lrbox}{\MPdotTTfdotinvplusdmbpluspoA}
\begin{minipage}{\MPdotTTfdotinvplusdmbpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv+dmb+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvplusdmbpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvplusdmbpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvplusdmbpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdmbpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.TTf.inv+dsb+ctrl-isb.tex <==
\newlength{\MPdotTTfdotinvplusdsbplusctrlisbH}
\setlength{\MPdotTTfdotinvplusdsbplusctrlisbH}{0cm}
\newsavebox{\MPdotTTfdotinvplusdsbplusctrlisbI}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusctrlisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbplusctrlisbJ}
\settowidth{\MPdotTTfdotinvplusdsbplusctrlisbJ}{\usebox{\MPdotTTfdotinvplusdsbplusctrlisbI}}
\addtolength{\MPdotTTfdotinvplusdsbplusctrlisbH}{\MPdotTTfdotinvplusdsbplusctrlisbJ}
\newsavebox{\MPdotTTfdotinvplusdsbplusctrlisbK}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusctrlisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
CBNZ X0,L0
L0:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbplusctrlisbL}
\settowidth{\MPdotTTfdotinvplusdsbplusctrlisbL}{\usebox{\MPdotTTfdotinvplusdsbplusctrlisbK}}
\addtolength{\MPdotTTfdotinvplusdsbplusctrlisbH}{\MPdotTTfdotinvplusdsbplusctrlisbL}
\newsavebox{\MPdotTTfdotinvplusdsbplusctrlisbM}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusctrlisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbplusctrlisbN}
\settowidth{\MPdotTTfdotinvplusdsbplusctrlisbN}{\usebox{\MPdotTTfdotinvplusdsbplusctrlisbM}}
\addtolength{\MPdotTTfdotinvplusdsbplusctrlisbH}{\MPdotTTfdotinvplusdsbplusctrlisbN}
\newsavebox{\MPdotTTfdotinvplusdsbplusctrlisbO}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusctrlisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbplusctrlisbP}
\settowidth{\MPdotTTfdotinvplusdsbplusctrlisbP}{\usebox{\MPdotTTfdotinvplusdsbplusctrlisbO}}
\newsavebox{\MPdotTTfdotinvplusdsbplusctrlisbA}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusctrlisbA}
\begin{minipage}{\MPdotTTfdotinvplusdsbplusctrlisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv+dsb+ctrl-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvplusdsbplusctrlisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvplusdsbplusctrlisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvplusdsbplusctrlisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbplusctrlisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbplusctrlisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbplusctrlisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.TTf.inv+dsb+dsb-isb.tex <==
\newlength{\MPdotTTfdotinvplusdsbplusdsbisbH}
\setlength{\MPdotTTfdotinvplusdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotTTfdotinvplusdsbplusdsbisbI}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbplusdsbisbJ}
\settowidth{\MPdotTTfdotinvplusdsbplusdsbisbJ}{\usebox{\MPdotTTfdotinvplusdsbplusdsbisbI}}
\addtolength{\MPdotTTfdotinvplusdsbplusdsbisbH}{\MPdotTTfdotinvplusdsbplusdsbisbJ}
\newsavebox{\MPdotTTfdotinvplusdsbplusdsbisbK}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbplusdsbisbL}
\settowidth{\MPdotTTfdotinvplusdsbplusdsbisbL}{\usebox{\MPdotTTfdotinvplusdsbplusdsbisbK}}
\addtolength{\MPdotTTfdotinvplusdsbplusdsbisbH}{\MPdotTTfdotinvplusdsbplusdsbisbL}
\newsavebox{\MPdotTTfdotinvplusdsbplusdsbisbM}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbplusdsbisbN}
\settowidth{\MPdotTTfdotinvplusdsbplusdsbisbN}{\usebox{\MPdotTTfdotinvplusdsbplusdsbisbM}}
\addtolength{\MPdotTTfdotinvplusdsbplusdsbisbH}{\MPdotTTfdotinvplusdsbplusdsbisbN}
\newsavebox{\MPdotTTfdotinvplusdsbplusdsbisbO}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbplusdsbisbP}
\settowidth{\MPdotTTfdotinvplusdsbplusdsbisbP}{\usebox{\MPdotTTfdotinvplusdsbplusdsbisbO}}
\newsavebox{\MPdotTTfdotinvplusdsbplusdsbisbA}
\begin{lrbox}{\MPdotTTfdotinvplusdsbplusdsbisbA}
\begin{minipage}{\MPdotTTfdotinvplusdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv+dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvplusdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvplusdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvplusdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.TTf.inv+dsb+po.tex <==
\newlength{\MPdotTTfdotinvplusdsbpluspoH}
\setlength{\MPdotTTfdotinvplusdsbpluspoH}{0cm}
\newsavebox{\MPdotTTfdotinvplusdsbpluspoI}
\begin{lrbox}{\MPdotTTfdotinvplusdsbpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbpluspoJ}
\settowidth{\MPdotTTfdotinvplusdsbpluspoJ}{\usebox{\MPdotTTfdotinvplusdsbpluspoI}}
\addtolength{\MPdotTTfdotinvplusdsbpluspoH}{\MPdotTTfdotinvplusdsbpluspoJ}
\newsavebox{\MPdotTTfdotinvplusdsbpluspoK}
\begin{lrbox}{\MPdotTTfdotinvplusdsbpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbpluspoL}
\settowidth{\MPdotTTfdotinvplusdsbpluspoL}{\usebox{\MPdotTTfdotinvplusdsbpluspoK}}
\addtolength{\MPdotTTfdotinvplusdsbpluspoH}{\MPdotTTfdotinvplusdsbpluspoL}
\newsavebox{\MPdotTTfdotinvplusdsbpluspoM}
\begin{lrbox}{\MPdotTTfdotinvplusdsbpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbpluspoN}
\settowidth{\MPdotTTfdotinvplusdsbpluspoN}{\usebox{\MPdotTTfdotinvplusdsbpluspoM}}
\addtolength{\MPdotTTfdotinvplusdsbpluspoH}{\MPdotTTfdotinvplusdsbpluspoN}
\newsavebox{\MPdotTTfdotinvplusdsbpluspoO}
\begin{lrbox}{\MPdotTTfdotinvplusdsbpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbpluspoP}
\settowidth{\MPdotTTfdotinvplusdsbpluspoP}{\usebox{\MPdotTTfdotinvplusdsbpluspoO}}
\newsavebox{\MPdotTTfdotinvplusdsbpluspoA}
\begin{lrbox}{\MPdotTTfdotinvplusdsbpluspoA}
\begin{minipage}{\MPdotTTfdotinvplusdsbpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv+dsb+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvplusdsbpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvplusdsbpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvplusdsbpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.TTf.inv+dsbs.tex <==
\newlength{\MPdotTTfdotinvplusdsbsH}
\setlength{\MPdotTTfdotinvplusdsbsH}{0cm}
\newsavebox{\MPdotTTfdotinvplusdsbsI}
\begin{lrbox}{\MPdotTTfdotinvplusdsbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbsJ}
\settowidth{\MPdotTTfdotinvplusdsbsJ}{\usebox{\MPdotTTfdotinvplusdsbsI}}
\addtolength{\MPdotTTfdotinvplusdsbsH}{\MPdotTTfdotinvplusdsbsJ}
\newsavebox{\MPdotTTfdotinvplusdsbsK}
\begin{lrbox}{\MPdotTTfdotinvplusdsbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbsL}
\settowidth{\MPdotTTfdotinvplusdsbsL}{\usebox{\MPdotTTfdotinvplusdsbsK}}
\addtolength{\MPdotTTfdotinvplusdsbsH}{\MPdotTTfdotinvplusdsbsL}
\newsavebox{\MPdotTTfdotinvplusdsbsM}
\begin{lrbox}{\MPdotTTfdotinvplusdsbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbsN}
\settowidth{\MPdotTTfdotinvplusdsbsN}{\usebox{\MPdotTTfdotinvplusdsbsM}}
\addtolength{\MPdotTTfdotinvplusdsbsH}{\MPdotTTfdotinvplusdsbsN}
\newsavebox{\MPdotTTfdotinvplusdsbsO}
\begin{lrbox}{\MPdotTTfdotinvplusdsbsO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvplusdsbsP}
\settowidth{\MPdotTTfdotinvplusdsbsP}{\usebox{\MPdotTTfdotinvplusdsbsO}}
\newsavebox{\MPdotTTfdotinvplusdsbsA}
\begin{lrbox}{\MPdotTTfdotinvplusdsbsA}
\begin{minipage}{\MPdotTTfdotinvplusdsbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv+dsbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvplusdsbsP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvplusdsbsO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvplusdsbsA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbsK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvplusdsbsM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.TTf.inv.EL1+dsb-tlbiis-dsb+dmb.tex <==
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}
\setlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{0cm}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}
\begin{minipage}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv.EL1+dsb-tlbiis-dsb+dmb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.TTf.inv.EL1+dsb-tlbiis-dsb+dsb-isb.tex <==
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}
\setlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}{0cm}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbI}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbJ}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbJ}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbI}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbJ}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbK}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbL}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbL}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbK}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbL}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbM}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbN}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbN}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbM}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbN}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbO}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbP}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbP}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbO}}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbA}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbA}
\begin{minipage}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv.EL1+dsb-tlbiis-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.TTf.inv.EL1+dsb-tlbiis-dsb+po.tex <==
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}
\setlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}{0cm}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoI}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoJ}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoJ}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoI}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoJ}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoK}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
MOV X0,X2
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoL}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoL}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoK}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoL}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoM}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoN}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoN}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoM}}
\addtolength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoN}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoO}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoP}
\settowidth{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoP}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoO}}
\newsavebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoA}
\begin{lrbox}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoA}
\begin{minipage}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TTf.inv.EL1+dsb-tlbiis-dsb+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTTfdotinvdotELoneplusdsbtlbiisdsbpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.TfR+dmb+eret.tex <==
\newlength{\MPdotTfRplusdmbpluseretH}
\setlength{\MPdotTfRplusdmbpluseretH}{0cm}
\newsavebox{\MPdotTfRplusdmbpluseretI}
\begin{lrbox}{\MPdotTfRplusdmbpluseretI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTfRplusdmbpluseretJ}
\settowidth{\MPdotTfRplusdmbpluseretJ}{\usebox{\MPdotTfRplusdmbpluseretI}}
\addtolength{\MPdotTfRplusdmbpluseretH}{\MPdotTfRplusdmbpluseretJ}
\newsavebox{\MPdotTfRplusdmbpluseretK}
\begin{lrbox}{\MPdotTfRplusdmbpluseretK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X2,[X1]
LDR X4,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTfRplusdmbpluseretL}
\settowidth{\MPdotTfRplusdmbpluseretL}{\usebox{\MPdotTfRplusdmbpluseretK}}
\addtolength{\MPdotTfRplusdmbpluseretH}{\MPdotTfRplusdmbpluseretL}
\newsavebox{\MPdotTfRplusdmbpluseretM}
\begin{lrbox}{\MPdotTfRplusdmbpluseretM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTfRplusdmbpluseretN}
\settowidth{\MPdotTfRplusdmbpluseretN}{\usebox{\MPdotTfRplusdmbpluseretM}}
\addtolength{\MPdotTfRplusdmbpluseretH}{\MPdotTfRplusdmbpluseretN}
\newsavebox{\MPdotTfRplusdmbpluseretO}
\begin{lrbox}{\MPdotTfRplusdmbpluseretO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;

    y |-> pa2;
    y ?-> invalid;

    *pa1 = 0;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotTfRplusdmbpluseretP}
\settowidth{\MPdotTfRplusdmbpluseretP}{\usebox{\MPdotTfRplusdmbpluseretO}}
\newsavebox{\MPdotTfRplusdmbpluseretA}
\begin{lrbox}{\MPdotTfRplusdmbpluseretA}
\begin{minipage}{\MPdotTfRplusdmbpluseretH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.TfR+dmb+eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotTfRplusdmbpluseretP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotTfRplusdmbpluseretO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotTfRplusdmbpluseretA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotTfRplusdmbpluseretI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotTfRplusdmbpluseretK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\MPdotTfRplusdmbpluseretM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R2=0 & 1:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/MP.alias3+rfi-data+dmb.tex <==
\newlength{\MPdotaliasthreeplusrfidataplusdmbH}
\setlength{\MPdotaliasthreeplusrfidataplusdmbH}{0cm}
\newsavebox{\MPdotaliasthreeplusrfidataplusdmbI}
\begin{lrbox}{\MPdotaliasthreeplusrfidataplusdmbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X2,[X3]
STR X2,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotaliasthreeplusrfidataplusdmbJ}
\settowidth{\MPdotaliasthreeplusrfidataplusdmbJ}{\usebox{\MPdotaliasthreeplusrfidataplusdmbI}}
\addtolength{\MPdotaliasthreeplusrfidataplusdmbH}{\MPdotaliasthreeplusrfidataplusdmbJ}
\newsavebox{\MPdotaliasthreeplusrfidataplusdmbK}
\begin{lrbox}{\MPdotaliasthreeplusrfidataplusdmbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotaliasthreeplusrfidataplusdmbL}
\settowidth{\MPdotaliasthreeplusrfidataplusdmbL}{\usebox{\MPdotaliasthreeplusrfidataplusdmbK}}
\addtolength{\MPdotaliasthreeplusrfidataplusdmbH}{\MPdotaliasthreeplusrfidataplusdmbL}
\newsavebox{\MPdotaliasthreeplusrfidataplusdmbM}
\begin{lrbox}{\MPdotaliasthreeplusrfidataplusdmbM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    y |-> pa2;
    z |-> pa1;
    *pa1 = 0;
    *pa2 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\MPdotaliasthreeplusrfidataplusdmbN}
\settowidth{\MPdotaliasthreeplusrfidataplusdmbN}{\usebox{\MPdotaliasthreeplusrfidataplusdmbM}}
\newsavebox{\MPdotaliasthreeplusrfidataplusdmbO}
\begin{lrbox}{\MPdotaliasthreeplusrfidataplusdmbO}
\begin{minipage}{\MPdotaliasthreeplusrfidataplusdmbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R3=z|\\
\lstinline[language=IslaLitmusExp]|0:R5=y|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|MP.alias3+rfi-data+dmb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\MPdotaliasthreeplusrfidataplusdmbN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\MPdotaliasthreeplusrfidataplusdmbM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\MPdotaliasthreeplusrfidataplusdmbO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\MPdotaliasthreeplusrfidataplusdmbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\MPdotaliasthreeplusrfidataplusdmbK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/PPOAA.alias.tex <==
\newlength{\PPOAAdotaliasH}
\setlength{\PPOAAdotaliasH}{0cm}
\newsavebox{\PPOAAdotaliasI}
\begin{lrbox}{\PPOAAdotaliasI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\PPOAAdotaliasJ}
\settowidth{\PPOAAdotaliasJ}{\usebox{\PPOAAdotaliasI}}
\addtolength{\PPOAAdotaliasH}{\PPOAAdotaliasJ}
\newsavebox{\PPOAAdotaliasK}
\begin{lrbox}{\PPOAAdotaliasK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X9,X0,X0
STR X2,[X3,X9]
LDR X4,[X5]
EOR X8,X4,X4
LDR X6,[X7,X8]
\end{lstlisting}
\end{lrbox}
\newlength{\PPOAAdotaliasL}
\settowidth{\PPOAAdotaliasL}{\usebox{\PPOAAdotaliasK}}
\addtolength{\PPOAAdotaliasH}{\PPOAAdotaliasL}
\newsavebox{\PPOAAdotaliasM}
\begin{lrbox}{\PPOAAdotaliasM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    w |-> pa1;
    x |-> pa1;
    y |-> pa2;
    z |-> pa3;
\end{lstlisting}
\end{lrbox}
\newlength{\PPOAAdotaliasN}
\settowidth{\PPOAAdotaliasN}{\usebox{\PPOAAdotaliasM}}
\newsavebox{\PPOAAdotaliasO}
\begin{lrbox}{\PPOAAdotaliasO}
\begin{minipage}{\PPOAAdotaliasH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R1=z|\\
\lstinline[language=IslaLitmusExp]|0:R2=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0x1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=w|\\
\lstinline[language=IslaLitmusExp]|1:R7=z|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|PPOAA.alias|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\PPOAAdotaliasN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\PPOAAdotaliasM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\PPOAAdotaliasO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\PPOAAdotaliasI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\PPOAAdotaliasK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R4=1 & 1:R6=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/PPOCA.alias.tex <==
\newlength{\PPOCAdotaliasH}
\setlength{\PPOCAdotaliasH}{0cm}
\newsavebox{\PPOCAdotaliasI}
\begin{lrbox}{\PPOCAdotaliasI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\PPOCAdotaliasJ}
\settowidth{\PPOCAdotaliasJ}{\usebox{\PPOCAdotaliasI}}
\addtolength{\PPOCAdotaliasH}{\PPOCAdotaliasJ}
\newsavebox{\PPOCAdotaliasK}
\begin{lrbox}{\PPOCAdotaliasK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBNZ X0,L0
L0:
STR X2,[X3]
LDR X4,[X5]
EOR X8,X4,X4
LDR X6,[X7,X8]
\end{lstlisting}
\end{lrbox}
\newlength{\PPOCAdotaliasL}
\settowidth{\PPOCAdotaliasL}{\usebox{\PPOCAdotaliasK}}
\addtolength{\PPOCAdotaliasH}{\PPOCAdotaliasL}
\newsavebox{\PPOCAdotaliasM}
\begin{lrbox}{\PPOCAdotaliasM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    w |-> pa1;
    x |-> pa1;
    y |-> pa2;
    z |-> pa3;
    *pa1 = 0;
    *pa2 = 0;
    *pa3 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\PPOCAdotaliasN}
\settowidth{\PPOCAdotaliasN}{\usebox{\PPOCAdotaliasM}}
\newsavebox{\PPOCAdotaliasO}
\begin{lrbox}{\PPOCAdotaliasO}
\begin{minipage}{\PPOCAdotaliasH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R1=z|\\
\lstinline[language=IslaLitmusExp]|0:R2=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0x1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R5=w|\\
\lstinline[language=IslaLitmusExp]|1:R7=z|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|PPOCA.alias|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\PPOCAdotaliasN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\PPOCAdotaliasM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\PPOCAdotaliasO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\PPOCAdotaliasI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\PPOCAdotaliasK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R4=1 & 1:R6=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/PPODA.RT.inv.tex <==
\newlength{\PPODAdotRTdotinvH}
\setlength{\PPODAdotRTdotinvH}{0cm}
\newsavebox{\PPODAdotRTdotinvI}
\begin{lrbox}{\PPODAdotRTdotinvI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\PPODAdotRTdotinvJ}
\settowidth{\PPODAdotRTdotinvJ}{\usebox{\PPODAdotRTdotinvI}}
\addtolength{\PPODAdotRTdotinvH}{\PPODAdotRTdotinvJ}
\newsavebox{\PPODAdotRTdotinvK}
\begin{lrbox}{\PPODAdotRTdotinvK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
ORR X2,X2,X3
STR X2,[X4]
LDR X6,[X5]
EOR X8,X6,X6
LDR X9,[X7,X8]
\end{lstlisting}
\end{lrbox}
\newlength{\PPODAdotRTdotinvL}
\settowidth{\PPODAdotRTdotinvL}{\usebox{\PPODAdotRTdotinvK}}
\addtolength{\PPODAdotRTdotinvH}{\PPODAdotRTdotinvL}
\newsavebox{\PPODAdotRTdotinvM}
\begin{lrbox}{\PPODAdotRTdotinvM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X6,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\PPODAdotRTdotinvN}
\settowidth{\PPODAdotRTdotinvN}{\usebox{\PPODAdotRTdotinvM}}
\addtolength{\PPODAdotRTdotinvH}{\PPODAdotRTdotinvN}
\newsavebox{\PPODAdotRTdotinvO}
\begin{lrbox}{\PPODAdotRTdotinvO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    w |-> pa1;
    x |-> invalid;
    x ?-> pa1;
    y |-> pa2;
    z |-> pa3;
    *pa1 = 1;
    *pa2 = 0;
    *pa3 = 0;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\PPODAdotRTdotinvP}
\settowidth{\PPODAdotRTdotinvP}{\usebox{\PPODAdotRTdotinvO}}
\newsavebox{\PPODAdotRTdotinvA}
\begin{lrbox}{\PPODAdotRTdotinvA}
\begin{minipage}{\PPODAdotRTdotinvH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R1=z|\\
\lstinline[language=IslaLitmusExp]|0:R2=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=desc3(w,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R4=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R5=x|\\
\lstinline[language=IslaLitmusExp]|1:R7=z|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|PPODA.RT.inv|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\PPODAdotRTdotinvP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\PPODAdotRTdotinvO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\PPODAdotRTdotinvA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\PPODAdotRTdotinvI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\PPODAdotRTdotinvK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\PPODAdotRTdotinvM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R6=1 & 1:R9=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/R.RTf.inv.EL1+dsb-tlbiis-dsb+popl.tex <==
\newlength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}
\setlength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}{0cm}
\newsavebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplI}
\begin{lrbox}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplJ}
\settowidth{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplJ}{\usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplI}}
\addtolength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplJ}
\newsavebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplK}
\begin{lrbox}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplK}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
STLR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplL}
\settowidth{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplL}{\usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplK}}
\addtolength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplL}
\newsavebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplM}
\begin{lrbox}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplN}
\settowidth{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplN}{\usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplM}}
\addtolength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplN}
\newsavebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplO}
\begin{lrbox}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplP}
\settowidth{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplP}{\usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplO}}
\newsavebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplA}
\begin{lrbox}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplA}
\begin{minipage}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R0=0x2|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|R.RTf.inv.EL1+dsb-tlbiis-dsb+popl|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\RdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|y=2 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/R.inv.tex <==
\newlength{\RdotinvH}
\setlength{\RdotinvH}{0cm}
\newsavebox{\RdotinvI}
\begin{lrbox}{\RdotinvI}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\RdotinvJ}
\settowidth{\RdotinvJ}{\usebox{\RdotinvI}}
\addtolength{\RdotinvH}{\RdotinvJ}
\newsavebox{\RdotinvK}
\begin{lrbox}{\RdotinvK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\RdotinvL}
\settowidth{\RdotinvL}{\usebox{\RdotinvK}}
\addtolength{\RdotinvH}{\RdotinvL}
\newsavebox{\RdotinvM}
\begin{lrbox}{\RdotinvM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> invalid;
    x ?-> pa1;
    identity 0x1000 with code;
    *pa1 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\RdotinvN}
\settowidth{\RdotinvN}{\usebox{\RdotinvM}}
\newsavebox{\RdotinvO}
\begin{lrbox}{\RdotinvO}
\begin{minipage}{\RdotinvH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=x|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|R.inv|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\RdotinvN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\RdotinvM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\RdotinvO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\RdotinvI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\RdotinvK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R0=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/RBS+dsb-tlbiis-dsb.tex <==
\newlength{\RBSplusdsbtlbiisdsbH}
\setlength{\RBSplusdsbtlbiisdsbH}{0cm}
\newsavebox{\RBSplusdsbtlbiisdsbI}
\begin{lrbox}{\RBSplusdsbtlbiisdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X5
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\RBSplusdsbtlbiisdsbJ}
\settowidth{\RBSplusdsbtlbiisdsbJ}{\usebox{\RBSplusdsbtlbiisdsbI}}
\addtolength{\RBSplusdsbtlbiisdsbH}{\RBSplusdsbtlbiisdsbJ}
\newsavebox{\RBSplusdsbtlbiisdsbK}
\begin{lrbox}{\RBSplusdsbtlbiisdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\RBSplusdsbtlbiisdsbL}
\settowidth{\RBSplusdsbtlbiisdsbL}{\usebox{\RBSplusdsbtlbiisdsbK}}
\addtolength{\RBSplusdsbtlbiisdsbH}{\RBSplusdsbtlbiisdsbL}
\newsavebox{\RBSplusdsbtlbiisdsbM}
\begin{lrbox}{\RBSplusdsbtlbiisdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\RBSplusdsbtlbiisdsbN}
\settowidth{\RBSplusdsbtlbiisdsbN}{\usebox{\RBSplusdsbtlbiisdsbM}}
\addtolength{\RBSplusdsbtlbiisdsbH}{\RBSplusdsbtlbiisdsbN}
\newsavebox{\RBSplusdsbtlbiisdsbO}
\begin{lrbox}{\RBSplusdsbtlbiisdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid;
    y |-> pa1;
    *pa1 = 0;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\RBSplusdsbtlbiisdsbP}
\settowidth{\RBSplusdsbtlbiisdsbP}{\usebox{\RBSplusdsbtlbiisdsbO}}
\newsavebox{\RBSplusdsbtlbiisdsbA}
\begin{lrbox}{\RBSplusdsbtlbiisdsbA}
\begin{minipage}{\RBSplusdsbtlbiisdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0x2|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R5=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|RBS+dsb-tlbiis-dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\RBSplusdsbtlbiisdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\RBSplusdsbtlbiisdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\RBSplusdsbtlbiisdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\RBSplusdsbtlbiisdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\RBSplusdsbtlbiisdsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\RBSplusdsbtlbiisdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=2|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/RDW.alias.tex <==
\newlength{\RDWdotaliasH}
\setlength{\RDWdotaliasH}{0cm}
\newsavebox{\RDWdotaliasI}
\begin{lrbox}{\RDWdotaliasI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\RDWdotaliasJ}
\settowidth{\RDWdotaliasJ}{\usebox{\RDWdotaliasI}}
\addtolength{\RDWdotaliasH}{\RDWdotaliasJ}
\newsavebox{\RDWdotaliasK}
\begin{lrbox}{\RDWdotaliasK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
LDR X3,[X4,X2]
LDR X5,[X6]
EOR X7,X5,X5
LDR X8,[X9,X7]
\end{lstlisting}
\end{lrbox}
\newlength{\RDWdotaliasL}
\settowidth{\RDWdotaliasL}{\usebox{\RDWdotaliasK}}
\addtolength{\RDWdotaliasH}{\RDWdotaliasL}
\newsavebox{\RDWdotaliasM}
\begin{lrbox}{\RDWdotaliasM}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\RDWdotaliasN}
\settowidth{\RDWdotaliasN}{\usebox{\RDWdotaliasM}}
\addtolength{\RDWdotaliasH}{\RDWdotaliasN}
\newsavebox{\RDWdotaliasO}
\begin{lrbox}{\RDWdotaliasO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    w |-> pa1;
    x |-> pa1;
    y |-> pa2;
    z |-> pa3;
    *pa1 = 0;
    *pa2 = 0;
    *pa3 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\RDWdotaliasP}
\settowidth{\RDWdotaliasP}{\usebox{\RDWdotaliasO}}
\newsavebox{\RDWdotaliasA}
\begin{lrbox}{\RDWdotaliasA}
\begin{minipage}{\RDWdotaliasH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=z|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R4=w|\\
\lstinline[language=IslaLitmusExp]|1:R6=x|\\
\lstinline[language=IslaLitmusExp]|1:R9=z|\\
\lstinline[language=IslaLitmusExp]|2:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|2:R1=x|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|RDW.alias|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\RDWdotaliasP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\RDWdotaliasO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\RDWdotaliasA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\RDWdotaliasI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\RDWdotaliasK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\RDWdotaliasM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R3=0 & 1:R5=1 & 1:R8=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/ROT.inv+dmbst.tex <==
\newlength{\ROTdotinvplusdmbstH}
\setlength{\ROTdotinvplusdmbstH}{0cm}
\newsavebox{\ROTdotinvplusdmbstI}
\begin{lrbox}{\ROTdotinvplusdmbstI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB ST
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvplusdmbstJ}
\settowidth{\ROTdotinvplusdmbstJ}{\usebox{\ROTdotinvplusdmbstI}}
\addtolength{\ROTdotinvplusdmbstH}{\ROTdotinvplusdmbstJ}
\newsavebox{\ROTdotinvplusdmbstK}
\begin{lrbox}{\ROTdotinvplusdmbstK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvplusdmbstL}
\settowidth{\ROTdotinvplusdmbstL}{\usebox{\ROTdotinvplusdmbstK}}
\addtolength{\ROTdotinvplusdmbstH}{\ROTdotinvplusdmbstL}
\newsavebox{\ROTdotinvplusdmbstM}
\begin{lrbox}{\ROTdotinvplusdmbstM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS x14,esr_el1
AND X14,X14,#0b111
CMP x14,#0b111
MOV X17,#1
MOV X18,#2
// if ESR_EL1.ISS.DFSC == Translation Level 3 then x2 = 1 else x2 = 2
CSEL x0,x17,x18,eq
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvplusdmbstN}
\settowidth{\ROTdotinvplusdmbstN}{\usebox{\ROTdotinvplusdmbstM}}
\addtolength{\ROTdotinvplusdmbstH}{\ROTdotinvplusdmbstN}
\newsavebox{\ROTdotinvplusdmbstO}
\begin{lrbox}{\ROTdotinvplusdmbstO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
physical pa1;
intermediate ipa1;

assert pa1 == ipa1;
ipa1 |-> pa1;

s1table new_table 0x280000 {
  x |-> invalid;
  x ?-> ipa1;
};

identity 0x283000 with default;

x |-> invalid at level 2;
x ?-> table(0x283000) at level 2;

identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvplusdmbstP}
\settowidth{\ROTdotinvplusdmbstP}{\usebox{\ROTdotinvplusdmbstO}}
\newsavebox{\ROTdotinvplusdmbstA}
\begin{lrbox}{\ROTdotinvplusdmbstA}
\begin{minipage}{\ROTdotinvplusdmbstH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=ipa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,new_table)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc2(table=0x283000)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte2(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|ROT.inv+dmbst|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\ROTdotinvplusdmbstP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\ROTdotinvplusdmbstO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\ROTdotinvplusdmbstA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\ROTdotinvplusdmbstI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\ROTdotinvplusdmbstK}\\
  \cline{2-2}
  & thread 1 el1 handler\\
  \cline{2-2}
  & \usebox{\ROTdotinvplusdmbstM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/ROT.inv+dsb.tex <==
\newlength{\ROTdotinvplusdsbH}
\setlength{\ROTdotinvplusdsbH}{0cm}
\newsavebox{\ROTdotinvplusdsbI}
\begin{lrbox}{\ROTdotinvplusdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvplusdsbJ}
\settowidth{\ROTdotinvplusdsbJ}{\usebox{\ROTdotinvplusdsbI}}
\addtolength{\ROTdotinvplusdsbH}{\ROTdotinvplusdsbJ}
\newsavebox{\ROTdotinvplusdsbK}
\begin{lrbox}{\ROTdotinvplusdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvplusdsbL}
\settowidth{\ROTdotinvplusdsbL}{\usebox{\ROTdotinvplusdsbK}}
\addtolength{\ROTdotinvplusdsbH}{\ROTdotinvplusdsbL}
\newsavebox{\ROTdotinvplusdsbM}
\begin{lrbox}{\ROTdotinvplusdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS X14,ESR_EL1
AND X14,X14,#0b111
CMP X14,#0b111
MOV X17,#1
MOV X18,#2
// if ESR_EL1.ISS.DFSC == Translation Level 3 then x2 = 1 else x2 = 2
CSEL X0,X17,X18,eq
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvplusdsbN}
\settowidth{\ROTdotinvplusdsbN}{\usebox{\ROTdotinvplusdsbM}}
\addtolength{\ROTdotinvplusdsbH}{\ROTdotinvplusdsbN}
\newsavebox{\ROTdotinvplusdsbO}
\begin{lrbox}{\ROTdotinvplusdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
physical pa1;
intermediate ipa1;

assert pa1 == ipa1;
ipa1 |-> pa1;

s1table new_table 0x280000 {
  x |-> invalid;
  x ?-> ipa1;
};

identity 0x283000 with default;

x |-> invalid at level 2;
x ?-> table(0x283000) at level 2;

identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvplusdsbP}
\settowidth{\ROTdotinvplusdsbP}{\usebox{\ROTdotinvplusdsbO}}
\newsavebox{\ROTdotinvplusdsbA}
\begin{lrbox}{\ROTdotinvplusdsbA}
\begin{minipage}{\ROTdotinvplusdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=ipa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,new_table)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc2(table=0x283000)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte2(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|ROT.inv+dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\ROTdotinvplusdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\ROTdotinvplusdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\ROTdotinvplusdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\ROTdotinvplusdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\ROTdotinvplusdsbK}\\
  \cline{2-2}
  & thread 1 el1 handler\\
  \cline{2-2}
  & \usebox{\ROTdotinvplusdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/ROT.inv+po.tex <==
\newlength{\ROTdotinvpluspoH}
\setlength{\ROTdotinvpluspoH}{0cm}
\newsavebox{\ROTdotinvpluspoI}
\begin{lrbox}{\ROTdotinvpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvpluspoJ}
\settowidth{\ROTdotinvpluspoJ}{\usebox{\ROTdotinvpluspoI}}
\addtolength{\ROTdotinvpluspoH}{\ROTdotinvpluspoJ}
\newsavebox{\ROTdotinvpluspoK}
\begin{lrbox}{\ROTdotinvpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvpluspoL}
\settowidth{\ROTdotinvpluspoL}{\usebox{\ROTdotinvpluspoK}}
\addtolength{\ROTdotinvpluspoH}{\ROTdotinvpluspoL}
\newsavebox{\ROTdotinvpluspoM}
\begin{lrbox}{\ROTdotinvpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS X14,ESR_EL1
AND X14,X14,#0b111
CMP X14,#0b111
MOV X17,#1
MOV X18,#2
// if ESR_EL1.ISS.DFSC == Translation Level 3 then x2 = 1 else x2 = 2
CSEL X0,X17,X18,eq
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvpluspoN}
\settowidth{\ROTdotinvpluspoN}{\usebox{\ROTdotinvpluspoM}}
\addtolength{\ROTdotinvpluspoH}{\ROTdotinvpluspoN}
\newsavebox{\ROTdotinvpluspoO}
\begin{lrbox}{\ROTdotinvpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
physical pa1;
intermediate ipa1;

assert pa1 == ipa1;
ipa1 |-> pa1;

s1table new_table 0x280000 {
  x |-> invalid;
  x ?-> ipa1;
};

identity 0x283000 with default;

x |-> invalid at level 2;
x ?-> table(0x283000) at level 2;

identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\ROTdotinvpluspoP}
\settowidth{\ROTdotinvpluspoP}{\usebox{\ROTdotinvpluspoO}}
\newsavebox{\ROTdotinvpluspoA}
\begin{lrbox}{\ROTdotinvpluspoA}
\begin{minipage}{\ROTdotinvpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=ipa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,new_table)|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc2(table=0x283000)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte2(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|ROT.inv+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\ROTdotinvpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\ROTdotinvpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\ROTdotinvpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\ROTdotinvpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\ROTdotinvpluspoK}\\
  \cline{2-2}
  & thread 1 el1 handler\\
  \cline{2-2}
  & \usebox{\ROTdotinvpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/RSW.alias.tex <==
\newlength{\RSWdotaliasH}
\setlength{\RSWdotaliasH}{0cm}
\newsavebox{\RSWdotaliasI}
\begin{lrbox}{\RSWdotaliasI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\RSWdotaliasJ}
\settowidth{\RSWdotaliasJ}{\usebox{\RSWdotaliasI}}
\addtolength{\RSWdotaliasH}{\RSWdotaliasJ}
\newsavebox{\RSWdotaliasK}
\begin{lrbox}{\RSWdotaliasK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
LDR X3,[X4,X2]
LDR X5,[X6]
EOR X7,X5,X5
LDR X8,[X9,X7]
\end{lstlisting}
\end{lrbox}
\newlength{\RSWdotaliasL}
\settowidth{\RSWdotaliasL}{\usebox{\RSWdotaliasK}}
\addtolength{\RSWdotaliasH}{\RSWdotaliasL}
\newsavebox{\RSWdotaliasM}
\begin{lrbox}{\RSWdotaliasM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    w |-> pa1;
    x |-> pa1;
    y |-> pa2;
    z |-> pa3;
    *pa1 = 0;
    *pa2 = 0;
    *pa3 = 0;
\end{lstlisting}
\end{lrbox}
\newlength{\RSWdotaliasN}
\settowidth{\RSWdotaliasN}{\usebox{\RSWdotaliasM}}
\newsavebox{\RSWdotaliasO}
\begin{lrbox}{\RSWdotaliasO}
\begin{minipage}{\RSWdotaliasH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=z|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R4=w|\\
\lstinline[language=IslaLitmusExp]|1:R6=x|\\
\lstinline[language=IslaLitmusExp]|1:R9=z|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|RSW.alias|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\RSWdotaliasN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\RSWdotaliasM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\RSWdotaliasO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\RSWdotaliasI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\RSWdotaliasK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R8=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/RWC.RTR.EL1+dsb-isb+dsb-tlbi-dsb.tex <==
\newlength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbH}
\setlength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbH}{0cm}
\newsavebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbI}
\begin{lrbox}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbJ}
\settowidth{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbJ}{\usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbI}}
\addtolength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbH}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbJ}
\newsavebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbK}
\begin{lrbox}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X3,[X4,X2]
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbL}
\settowidth{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbL}{\usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbK}}
\addtolength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbH}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbL}
\newsavebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbM}
\begin{lrbox}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X2
DSB SY
LDR X3,[X4]
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbN}
\settowidth{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbN}{\usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbM}}
\addtolength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbH}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbN}
\newsavebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbO}
\begin{lrbox}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X3,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbP}
\settowidth{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbP}{\usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbO}}
\addtolength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbH}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbP}
\newsavebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbA}
\begin{lrbox}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;

    y |-> pa2;
    y ?-> invalid;
    z |-> pa2;
    *pa1 = 1;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbB}
\settowidth{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbB}{\usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbA}}
\newsavebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbC}
\begin{lrbox}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbC}
\begin{minipage}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R4=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|2:R1=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R2=page(x)|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|RWC.RTR.EL1+dsb-isb+dsb-tlbi-dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\RWCdotRTRdotELoneplusdsbisbplusdsbtlbidsbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R1=1 & 1:R3=0 & 2:R3=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/RWC.RTfR.inv+addr+dmb.tex <==
\newlength{\RWCdotRTfRdotinvplusaddrplusdmbH}
\setlength{\RWCdotRTfRdotinvplusaddrplusdmbH}{0cm}
\newsavebox{\RWCdotRTfRdotinvplusaddrplusdmbI}
\begin{lrbox}{\RWCdotRTfRdotinvplusaddrplusdmbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTfRdotinvplusaddrplusdmbJ}
\settowidth{\RWCdotRTfRdotinvplusaddrplusdmbJ}{\usebox{\RWCdotRTfRdotinvplusaddrplusdmbI}}
\addtolength{\RWCdotRTfRdotinvplusaddrplusdmbH}{\RWCdotRTfRdotinvplusaddrplusdmbJ}
\newsavebox{\RWCdotRTfRdotinvplusaddrplusdmbK}
\begin{lrbox}{\RWCdotRTfRdotinvplusaddrplusdmbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X2,X0,X0
LDR X3,[X4,X2]
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTfRdotinvplusaddrplusdmbL}
\settowidth{\RWCdotRTfRdotinvplusaddrplusdmbL}{\usebox{\RWCdotRTfRdotinvplusaddrplusdmbK}}
\addtolength{\RWCdotRTfRdotinvplusaddrplusdmbH}{\RWCdotRTfRdotinvplusaddrplusdmbL}
\newsavebox{\RWCdotRTfRdotinvplusaddrplusdmbM}
\begin{lrbox}{\RWCdotRTfRdotinvplusaddrplusdmbM}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTfRdotinvplusaddrplusdmbN}
\settowidth{\RWCdotRTfRdotinvplusaddrplusdmbN}{\usebox{\RWCdotRTfRdotinvplusaddrplusdmbM}}
\addtolength{\RWCdotRTfRdotinvplusaddrplusdmbH}{\RWCdotRTfRdotinvplusaddrplusdmbN}
\newsavebox{\RWCdotRTfRdotinvplusaddrplusdmbO}
\begin{lrbox}{\RWCdotRTfRdotinvplusaddrplusdmbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X3,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTfRdotinvplusaddrplusdmbP}
\settowidth{\RWCdotRTfRdotinvplusaddrplusdmbP}{\usebox{\RWCdotRTfRdotinvplusaddrplusdmbO}}
\addtolength{\RWCdotRTfRdotinvplusaddrplusdmbH}{\RWCdotRTfRdotinvplusaddrplusdmbP}
\newsavebox{\RWCdotRTfRdotinvplusaddrplusdmbA}
\begin{lrbox}{\RWCdotRTfRdotinvplusaddrplusdmbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;

    y |-> invalid;
    y ?-> pa2;
    z |-> pa2;
    *pa1 = 1;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\RWCdotRTfRdotinvplusaddrplusdmbB}
\settowidth{\RWCdotRTfRdotinvplusaddrplusdmbB}{\usebox{\RWCdotRTfRdotinvplusaddrplusdmbA}}
\newsavebox{\RWCdotRTfRdotinvplusaddrplusdmbC}
\begin{lrbox}{\RWCdotRTfRdotinvplusaddrplusdmbC}
\begin{minipage}{\RWCdotRTfRdotinvplusaddrplusdmbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R3=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R4=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|2:R1=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|RWC.RTfR.inv+addr+dmb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\RWCdotRTfRdotinvplusaddrplusdmbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\RWCdotRTfRdotinvplusaddrplusdmbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\RWCdotRTfRdotinvplusaddrplusdmbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\RWCdotRTfRdotinvplusaddrplusdmbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\RWCdotRTfRdotinvplusaddrplusdmbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\RWCdotRTfRdotinvplusaddrplusdmbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\RWCdotRTfRdotinvplusaddrplusdmbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R1=1 & 1:R3=0 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/S.RT.ro+dsb-tlbiis-dsb+dsb-isb.tex <==
\newlength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbH}
\setlength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbH}{0cm}
\newsavebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbI}
\begin{lrbox}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbJ}
\settowidth{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbJ}{\usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbI}}
\addtolength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbH}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbJ}
\newsavebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbK}
\begin{lrbox}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbL}
\settowidth{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbL}{\usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbK}}
\addtolength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbH}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbL}
\newsavebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbM}
\begin{lrbox}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbN}
\settowidth{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbN}{\usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbM}}
\addtolength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbH}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbN}
\newsavebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbO}
\begin{lrbox}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1 with [AP = 0b11] and default;
    x ?-> pa1;
    z |-> pa1;
    y |-> pa2;

    *pa1 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbP}
\settowidth{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbP}{\usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbO}}
\newsavebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbA}
\begin{lrbox}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbA}
\begin{minipage}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|S.RT.ro+dsb-tlbiis-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SdotRTdotroplusdsbtlbiisdsbplusdsbisbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/S.RTf.inv.EL1+dsb-tlbiis-dsb+ctrl.tex <==
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}
\setlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}{0cm}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlI}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlJ}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlJ}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlI}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlJ}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlK}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBNZ X0,L0
L0:
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlL}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlL}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlK}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlL}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlM}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlN}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlN}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlM}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlN}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlO}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlP}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlP}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlO}}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlA}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlA}
\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|S.RTf.inv.EL1+dsb-tlbiis-dsb+ctrl|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusctrlM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/S.RTf.inv.EL1+dsb-tlbiis-dsb+data.tex <==
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}
\setlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}{0cm}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataI}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataJ}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataJ}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataI}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataJ}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataK}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
ORR X2,X2,X4
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataL}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataL}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataK}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataL}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataM}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataN}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataN}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataM}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataN}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataO}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataP}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataP}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataO}}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataA}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataA}
\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|S.RTf.inv.EL1+dsb-tlbiis-dsb+data|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdataM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/S.RTf.inv.EL1+dsb-tlbiis-dsb+dmb.tex <==
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}
\setlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{0cm}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbJ}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbL}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbN}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}
\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|S.RTf.inv.EL1+dsb-tlbiis-dsb+dmb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbplusdmbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/S.RTf.inv.EL1+dsb-tlbiis-dsb+poap.tex <==
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}
\setlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}{0cm}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapI}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapJ}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapJ}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapI}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapJ}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapK}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDAR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapL}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapL}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapK}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapL}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapM}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapN}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapN}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapM}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapN}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapO}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapP}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapP}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapO}}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapA}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapA}
\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|S.RTf.inv.EL1+dsb-tlbiis-dsb+poap|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoapM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/S.RTf.inv.EL1+dsb-tlbiis-dsb+popl.tex <==
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}
\setlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}{0cm}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplI}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X4
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplJ}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplJ}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplI}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplJ}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplK}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STLR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplL}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplL}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplK}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplL}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplM}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplN}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplN}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplM}}
\addtolength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplN}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplO}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplP}
\settowidth{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplP}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplO}}
\newsavebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplA}
\begin{lrbox}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplA}
\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|S.RTf.inv.EL1+dsb-tlbiis-dsb+popl|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SdotRTfdotinvdotELoneplusdsbtlbiisdsbpluspoplM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/S.T+dmb+po.tex <==
\newlength{\SdotTplusdmbpluspoH}
\setlength{\SdotTplusdmbpluspoH}{0cm}
\newsavebox{\SdotTplusdmbpluspoI}
\begin{lrbox}{\SdotTplusdmbpluspoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotTplusdmbpluspoJ}
\settowidth{\SdotTplusdmbpluspoJ}{\usebox{\SdotTplusdmbpluspoI}}
\addtolength{\SdotTplusdmbpluspoH}{\SdotTplusdmbpluspoJ}
\newsavebox{\SdotTplusdmbpluspoK}
\begin{lrbox}{\SdotTplusdmbpluspoK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SdotTplusdmbpluspoL}
\settowidth{\SdotTplusdmbpluspoL}{\usebox{\SdotTplusdmbpluspoK}}
\addtolength{\SdotTplusdmbpluspoH}{\SdotTplusdmbpluspoL}
\newsavebox{\SdotTplusdmbpluspoM}
\begin{lrbox}{\SdotTplusdmbpluspoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SdotTplusdmbpluspoN}
\settowidth{\SdotTplusdmbpluspoN}{\usebox{\SdotTplusdmbpluspoM}}
\addtolength{\SdotTplusdmbpluspoH}{\SdotTplusdmbpluspoN}
\newsavebox{\SdotTplusdmbpluspoO}
\begin{lrbox}{\SdotTplusdmbpluspoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 0;
    *pa2 = 1;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SdotTplusdmbpluspoP}
\settowidth{\SdotTplusdmbpluspoP}{\usebox{\SdotTplusdmbpluspoO}}
\newsavebox{\SdotTplusdmbpluspoA}
\begin{lrbox}{\SdotTplusdmbpluspoA}
\begin{minipage}{\SdotTplusdmbpluspoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:R0=0x1|\\
\lstinline[language=IslaLitmusExp]|0:R1=x|\\
\lstinline[language=IslaLitmusExp]|0:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|0:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=y|\\
\lstinline[language=IslaLitmusExp]|1:R2=0x2|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|S.T+dmb+po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SdotTplusdmbpluspoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SdotTplusdmbpluspoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SdotTplusdmbpluspoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SdotTplusdmbpluspoI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SdotTplusdmbpluspoK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SdotTplusdmbpluspoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & x=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/SB.TfTf.inv+dmb-ctrl-isbs.tex <==
\newlength{\SBdotTfTfdotinvplusdmbctrlisbsH}
\setlength{\SBdotTfTfdotinvplusdmbctrlisbsH}{0cm}
\newsavebox{\SBdotTfTfdotinvplusdmbctrlisbsI}
\begin{lrbox}{\SBdotTfTfdotinvplusdmbctrlisbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
LDR X7,[X8]
CBNZ X7,L0
L0:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdmbctrlisbsJ}
\settowidth{\SBdotTfTfdotinvplusdmbctrlisbsJ}{\usebox{\SBdotTfTfdotinvplusdmbctrlisbsI}}
\addtolength{\SBdotTfTfdotinvplusdmbctrlisbsH}{\SBdotTfTfdotinvplusdmbctrlisbsJ}
\newsavebox{\SBdotTfTfdotinvplusdmbctrlisbsK}
\begin{lrbox}{\SBdotTfTfdotinvplusdmbctrlisbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DMB SY
LDR X7,[X8]
CBNZ X7,L1
L1:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdmbctrlisbsL}
\settowidth{\SBdotTfTfdotinvplusdmbctrlisbsL}{\usebox{\SBdotTfTfdotinvplusdmbctrlisbsK}}
\addtolength{\SBdotTfTfdotinvplusdmbctrlisbsH}{\SBdotTfTfdotinvplusdmbctrlisbsL}
\newsavebox{\SBdotTfTfdotinvplusdmbctrlisbsM}
\begin{lrbox}{\SBdotTfTfdotinvplusdmbctrlisbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdmbctrlisbsN}
\settowidth{\SBdotTfTfdotinvplusdmbctrlisbsN}{\usebox{\SBdotTfTfdotinvplusdmbctrlisbsM}}
\addtolength{\SBdotTfTfdotinvplusdmbctrlisbsH}{\SBdotTfTfdotinvplusdmbctrlisbsN}
\newsavebox{\SBdotTfTfdotinvplusdmbctrlisbsO}
\begin{lrbox}{\SBdotTfTfdotinvplusdmbctrlisbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdmbctrlisbsP}
\settowidth{\SBdotTfTfdotinvplusdmbctrlisbsP}{\usebox{\SBdotTfTfdotinvplusdmbctrlisbsO}}
\addtolength{\SBdotTfTfdotinvplusdmbctrlisbsH}{\SBdotTfTfdotinvplusdmbctrlisbsP}
\newsavebox{\SBdotTfTfdotinvplusdmbctrlisbsA}
\begin{lrbox}{\SBdotTfTfdotinvplusdmbctrlisbsA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> invalid;
    y ?-> pa2;
    v |-> pa2;
    *pa2 = 1;

    z |-> pa3;
    *pa3 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdmbctrlisbsB}
\settowidth{\SBdotTfTfdotinvplusdmbctrlisbsB}{\usebox{\SBdotTfTfdotinvplusdmbctrlisbsA}}
\newsavebox{\SBdotTfTfdotinvplusdmbctrlisbsC}
\begin{lrbox}{\SBdotTfTfdotinvplusdmbctrlisbsC}
\begin{minipage}{\SBdotTfTfdotinvplusdmbctrlisbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R8=z|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R0=desc3(v,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:R8=z|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|SB.TfTf.inv+dmb-ctrl-isbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SBdotTfTfdotinvplusdmbctrlisbsB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SBdotTfTfdotinvplusdmbctrlisbsA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SBdotTfTfdotinvplusdmbctrlisbsC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvplusdmbctrlisbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvplusdmbctrlisbsK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvplusdmbctrlisbsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvplusdmbctrlisbsO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/SB.TfTf.inv+dsb-isbs.tex <==
\newlength{\SBdotTfTfdotinvplusdsbisbsH}
\setlength{\SBdotTfTfdotinvplusdsbisbsH}{0cm}
\newsavebox{\SBdotTfTfdotinvplusdsbisbsI}
\begin{lrbox}{\SBdotTfTfdotinvplusdsbisbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdsbisbsJ}
\settowidth{\SBdotTfTfdotinvplusdsbisbsJ}{\usebox{\SBdotTfTfdotinvplusdsbisbsI}}
\addtolength{\SBdotTfTfdotinvplusdsbisbsH}{\SBdotTfTfdotinvplusdsbisbsJ}
\newsavebox{\SBdotTfTfdotinvplusdsbisbsK}
\begin{lrbox}{\SBdotTfTfdotinvplusdsbisbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdsbisbsL}
\settowidth{\SBdotTfTfdotinvplusdsbisbsL}{\usebox{\SBdotTfTfdotinvplusdsbisbsK}}
\addtolength{\SBdotTfTfdotinvplusdsbisbsH}{\SBdotTfTfdotinvplusdsbisbsL}
\newsavebox{\SBdotTfTfdotinvplusdsbisbsM}
\begin{lrbox}{\SBdotTfTfdotinvplusdsbisbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdsbisbsN}
\settowidth{\SBdotTfTfdotinvplusdsbisbsN}{\usebox{\SBdotTfTfdotinvplusdsbisbsM}}
\addtolength{\SBdotTfTfdotinvplusdsbisbsH}{\SBdotTfTfdotinvplusdsbisbsN}
\newsavebox{\SBdotTfTfdotinvplusdsbisbsO}
\begin{lrbox}{\SBdotTfTfdotinvplusdsbisbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdsbisbsP}
\settowidth{\SBdotTfTfdotinvplusdsbisbsP}{\usebox{\SBdotTfTfdotinvplusdsbisbsO}}
\addtolength{\SBdotTfTfdotinvplusdsbisbsH}{\SBdotTfTfdotinvplusdsbisbsP}
\newsavebox{\SBdotTfTfdotinvplusdsbisbsA}
\begin{lrbox}{\SBdotTfTfdotinvplusdsbisbsA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> invalid;
    y ?-> pa2;
    v |-> pa2;
    *pa2 = 1;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvplusdsbisbsB}
\settowidth{\SBdotTfTfdotinvplusdsbisbsB}{\usebox{\SBdotTfTfdotinvplusdsbisbsA}}
\newsavebox{\SBdotTfTfdotinvplusdsbisbsC}
\begin{lrbox}{\SBdotTfTfdotinvplusdsbisbsC}
\begin{minipage}{\SBdotTfTfdotinvplusdsbisbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R0=desc3(v,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|SB.TfTf.inv+dsb-isbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SBdotTfTfdotinvplusdsbisbsB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SBdotTfTfdotinvplusdsbisbsA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SBdotTfTfdotinvplusdsbisbsC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvplusdsbisbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvplusdsbisbsK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvplusdsbisbsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvplusdsbisbsO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/SB.TfTf.inv.dsb-isbs.tex <==
\newlength{\SBdotTfTfdotinvdotdsbisbsH}
\setlength{\SBdotTfTfdotinvdotdsbisbsH}{0cm}
\newsavebox{\SBdotTfTfdotinvdotdsbisbsI}
\begin{lrbox}{\SBdotTfTfdotinvdotdsbisbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvdotdsbisbsJ}
\settowidth{\SBdotTfTfdotinvdotdsbisbsJ}{\usebox{\SBdotTfTfdotinvdotdsbisbsI}}
\addtolength{\SBdotTfTfdotinvdotdsbisbsH}{\SBdotTfTfdotinvdotdsbisbsJ}
\newsavebox{\SBdotTfTfdotinvdotdsbisbsK}
\begin{lrbox}{\SBdotTfTfdotinvdotdsbisbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvdotdsbisbsL}
\settowidth{\SBdotTfTfdotinvdotdsbisbsL}{\usebox{\SBdotTfTfdotinvdotdsbisbsK}}
\addtolength{\SBdotTfTfdotinvdotdsbisbsH}{\SBdotTfTfdotinvdotdsbisbsL}
\newsavebox{\SBdotTfTfdotinvdotdsbisbsM}
\begin{lrbox}{\SBdotTfTfdotinvdotdsbisbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvdotdsbisbsN}
\settowidth{\SBdotTfTfdotinvdotdsbisbsN}{\usebox{\SBdotTfTfdotinvdotdsbisbsM}}
\addtolength{\SBdotTfTfdotinvdotdsbisbsH}{\SBdotTfTfdotinvdotdsbisbsN}
\newsavebox{\SBdotTfTfdotinvdotdsbisbsO}
\begin{lrbox}{\SBdotTfTfdotinvdotdsbisbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvdotdsbisbsP}
\settowidth{\SBdotTfTfdotinvdotdsbisbsP}{\usebox{\SBdotTfTfdotinvdotdsbisbsO}}
\addtolength{\SBdotTfTfdotinvdotdsbisbsH}{\SBdotTfTfdotinvdotdsbisbsP}
\newsavebox{\SBdotTfTfdotinvdotdsbisbsA}
\begin{lrbox}{\SBdotTfTfdotinvdotdsbisbsA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> invalid;
    y ?-> pa2;
    v |-> pa2;
    *pa2 = 1;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvdotdsbisbsB}
\settowidth{\SBdotTfTfdotinvdotdsbisbsB}{\usebox{\SBdotTfTfdotinvdotdsbisbsA}}
\newsavebox{\SBdotTfTfdotinvdotdsbisbsC}
\begin{lrbox}{\SBdotTfTfdotinvdotdsbisbsC}
\begin{minipage}{\SBdotTfTfdotinvdotdsbisbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R0=desc3(v,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|SB.TfTf.inv.dsb-isbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SBdotTfTfdotinvdotdsbisbsB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SBdotTfTfdotinvdotdsbisbsA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SBdotTfTfdotinvdotdsbisbsC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvdotdsbisbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvdotdsbisbsK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvdotdsbisbsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvdotdsbisbsO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0 & 1:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/SB.TfTf.invv+rfi-ctrl-isbs.tex <==
\newlength{\SBdotTfTfdotinvvplusrfictrlisbsH}
\setlength{\SBdotTfTfdotinvvplusrfictrlisbsH}{0cm}
\newsavebox{\SBdotTfTfdotinvvplusrfictrlisbsI}
\begin{lrbox}{\SBdotTfTfdotinvvplusrfictrlisbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X7,[X1]
CBNZ X7,L0
L0:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvvplusrfictrlisbsJ}
\settowidth{\SBdotTfTfdotinvvplusrfictrlisbsJ}{\usebox{\SBdotTfTfdotinvvplusrfictrlisbsI}}
\addtolength{\SBdotTfTfdotinvvplusrfictrlisbsH}{\SBdotTfTfdotinvvplusrfictrlisbsJ}
\newsavebox{\SBdotTfTfdotinvvplusrfictrlisbsK}
\begin{lrbox}{\SBdotTfTfdotinvvplusrfictrlisbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
LDR X7,[X1]
CBNZ X7,L1
L1:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvvplusrfictrlisbsL}
\settowidth{\SBdotTfTfdotinvvplusrfictrlisbsL}{\usebox{\SBdotTfTfdotinvvplusrfictrlisbsK}}
\addtolength{\SBdotTfTfdotinvvplusrfictrlisbsH}{\SBdotTfTfdotinvvplusrfictrlisbsL}
\newsavebox{\SBdotTfTfdotinvvplusrfictrlisbsM}
\begin{lrbox}{\SBdotTfTfdotinvvplusrfictrlisbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvvplusrfictrlisbsN}
\settowidth{\SBdotTfTfdotinvvplusrfictrlisbsN}{\usebox{\SBdotTfTfdotinvvplusrfictrlisbsM}}
\addtolength{\SBdotTfTfdotinvvplusrfictrlisbsH}{\SBdotTfTfdotinvvplusrfictrlisbsN}
\newsavebox{\SBdotTfTfdotinvvplusrfictrlisbsO}
\begin{lrbox}{\SBdotTfTfdotinvvplusrfictrlisbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvvplusrfictrlisbsP}
\settowidth{\SBdotTfTfdotinvvplusrfictrlisbsP}{\usebox{\SBdotTfTfdotinvvplusrfictrlisbsO}}
\addtolength{\SBdotTfTfdotinvvplusrfictrlisbsH}{\SBdotTfTfdotinvvplusrfictrlisbsP}
\newsavebox{\SBdotTfTfdotinvvplusrfictrlisbsA}
\begin{lrbox}{\SBdotTfTfdotinvvplusrfictrlisbsA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2 pa3;
    x |-> invalid;
    x ?-> pa1;
    u |-> pa1;
    *pa1 = 1;

    y |-> invalid;
    y ?-> pa2;
    v |-> pa2;
    *pa2 = 1;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SBdotTfTfdotinvvplusrfictrlisbsB}
\settowidth{\SBdotTfTfdotinvvplusrfictrlisbsB}{\usebox{\SBdotTfTfdotinvvplusrfictrlisbsA}}
\newsavebox{\SBdotTfTfdotinvvplusrfictrlisbsC}
\begin{lrbox}{\SBdotTfTfdotinvvplusrfictrlisbsC}
\begin{minipage}{\SBdotTfTfdotinvvplusrfictrlisbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(u,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R0=desc3(v,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R3=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|SB.TfTf.invv+rfi-ctrl-isbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SBdotTfTfdotinvvplusrfictrlisbsB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SBdotTfTfdotinvvplusrfictrlisbsA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SBdotTfTfdotinvvplusrfictrlisbsC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvvplusrfictrlisbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvvplusrfictrlisbsK}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvvplusrfictrlisbsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\SBdotTfTfdotinvvplusrfictrlisbsO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0 & 0:R7=desc3(u,page_table_base) & 1:R2=0 & 1:R7=desc3(v,page_table_base)|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/SwitchTable.EL2+msrttbr-eret.tex <==
\newlength{\SwitchTabledotELtwoplusmsrttbreretH}
\setlength{\SwitchTabledotELtwoplusmsrttbreretH}{0cm}
\newsavebox{\SwitchTabledotELtwoplusmsrttbreretI}
\begin{lrbox}{\SwitchTabledotELtwoplusmsrttbreretI}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
HVC #0
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\SwitchTabledotELtwoplusmsrttbreretJ}
\settowidth{\SwitchTabledotELtwoplusmsrttbreretJ}{\usebox{\SwitchTabledotELtwoplusmsrttbreretI}}
\addtolength{\SwitchTabledotELtwoplusmsrttbreretH}{\SwitchTabledotELtwoplusmsrttbreretJ}
\newsavebox{\SwitchTabledotELtwoplusmsrttbreretK}
\begin{lrbox}{\SwitchTabledotELtwoplusmsrttbreretK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MSR TTBR0_EL1,X4
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SwitchTabledotELtwoplusmsrttbreretL}
\settowidth{\SwitchTabledotELtwoplusmsrttbreretL}{\usebox{\SwitchTabledotELtwoplusmsrttbreretK}}
\addtolength{\SwitchTabledotELtwoplusmsrttbreretH}{\SwitchTabledotELtwoplusmsrttbreretL}
\newsavebox{\SwitchTabledotELtwoplusmsrttbreretM}
\begin{lrbox}{\SwitchTabledotELtwoplusmsrttbreretM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
option default_tables = false;
physical pa1 pa2;

s1table initial_table 0x200000 {
    x |-> pa1 at level 3;
}

s1table new_table 0x280000  {
    x |-> pa2 at level 3;
}

s1table el2_table 0x300000 {
    identity 0x2000 with code;
}

*pa1 = 0;
*pa2 = 1;
\end{lstlisting}
\end{lrbox}
\newlength{\SwitchTabledotELtwoplusmsrttbreretN}
\settowidth{\SwitchTabledotELtwoplusmsrttbreretN}{\usebox{\SwitchTabledotELtwoplusmsrttbreretM}}
\newsavebox{\SwitchTabledotELtwoplusmsrttbreretO}
\begin{lrbox}{\SwitchTabledotELtwoplusmsrttbreretO}
\begin{minipage}{\SwitchTabledotELtwoplusmsrttbreretH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|R1=x|\\
\lstinline[language=IslaLitmusExp]|R3=x|\\
\lstinline[language=IslaLitmusExp]|R4=ttbr(asid=0x0000,base=new_table)|\\
\lstinline[language=IslaLitmusExp]|TTBR0_EL1=ttbr(base=initial_table,asid=0x0000)|\\
\lstinline[language=IslaLitmusExp]|TTBR0_EL2=ttbr(base=el2_table,asid=0x0000)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|SwitchTable.EL2+msrttbr-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SwitchTabledotELtwoplusmsrttbreretN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SwitchTabledotELtwoplusmsrttbreretM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SwitchTabledotELtwoplusmsrttbreretO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SwitchTabledotELtwoplusmsrttbreretI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\SwitchTabledotELtwoplusmsrttbreretK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/SwitchTable.same-asid+eret.toml.tex <==
\newlength{\SwitchTabledotsameasidpluseretdottomlH}
\setlength{\SwitchTabledotsameasidpluseretdottomlH}{0cm}
\newsavebox{\SwitchTabledotsameasidpluseretdottomlI}
\begin{lrbox}{\SwitchTabledotsameasidpluseretdottomlI}
\begin{lstlisting}[language=AArch64,showlines=true]
MSR TTBR0_EL1,X0
ERET
L0:
LDR X1,[X2]
\end{lstlisting}
\end{lrbox}
\newlength{\SwitchTabledotsameasidpluseretdottomlJ}
\settowidth{\SwitchTabledotsameasidpluseretdottomlJ}{\usebox{\SwitchTabledotsameasidpluseretdottomlI}}
\addtolength{\SwitchTabledotsameasidpluseretdottomlH}{\SwitchTabledotsameasidpluseretdottomlJ}
\newsavebox{\SwitchTabledotsameasidpluseretdottomlK}
\begin{lrbox}{\SwitchTabledotsameasidpluseretdottomlK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X1,#1
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\SwitchTabledotsameasidpluseretdottomlL}
\settowidth{\SwitchTabledotsameasidpluseretdottomlL}{\usebox{\SwitchTabledotsameasidpluseretdottomlK}}
\addtolength{\SwitchTabledotsameasidpluseretdottomlH}{\SwitchTabledotsameasidpluseretdottomlL}
\newsavebox{\SwitchTabledotsameasidpluseretdottomlM}
\begin{lrbox}{\SwitchTabledotsameasidpluseretdottomlM}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    intermediate ipa1;
    physical pa1;

    *pa1 = 0;

    s1table table0 0x2C0000 {
        identity 0x1000 with code;
        x |-> pa1;
    };
    s1table table1 0x300000 {
        identity 0x1000 with code;
        x |-> invalid;
    };

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\SwitchTabledotsameasidpluseretdottomlN}
\settowidth{\SwitchTabledotsameasidpluseretdottomlN}{\usebox{\SwitchTabledotsameasidpluseretdottomlM}}
\newsavebox{\SwitchTabledotsameasidpluseretdottomlO}
\begin{lrbox}{\SwitchTabledotsameasidpluseretdottomlO}
\begin{minipage}{\SwitchTabledotsameasidpluseretdottomlH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL1=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b1|\\
\lstinline[language=IslaLitmusExp]|R0=ttbr(asid=0x01,base=table1)|\\
\lstinline[language=IslaLitmusExp]|R2=x|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL1=0b00000|\\
\lstinline[language=IslaLitmusExp]|TTBR0_EL1=ttbr(base=table0,asid=0x00)|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|SwitchTable.same-asid+eret.toml|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\SwitchTabledotsameasidpluseretdottomlN}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\SwitchTabledotsameasidpluseretdottomlM}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\SwitchTabledotsameasidpluseretdottomlO}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\SwitchTabledotsameasidpluseretdottomlI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\SwitchTabledotsameasidpluseretdottomlK}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R1=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/W+T.tex <==
\newlength{\WplusTH}
\setlength{\WplusTH}{0cm}
\newsavebox{\WplusTI}
\begin{lrbox}{\WplusTI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WplusTJ}
\settowidth{\WplusTJ}{\usebox{\WplusTI}}
\addtolength{\WplusTH}{\WplusTJ}
\newsavebox{\WplusTK}
\begin{lrbox}{\WplusTK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WplusTL}
\settowidth{\WplusTL}{\usebox{\WplusTK}}
\addtolength{\WplusTH}{\WplusTL}
\newsavebox{\WplusTM}
\begin{lrbox}{\WplusTM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1000:
MOV X0,#0
\end{lstlisting}
\end{lrbox}
\newlength{\WplusTN}
\settowidth{\WplusTN}{\usebox{\WplusTM}}
\addtolength{\WplusTH}{\WplusTN}
\newsavebox{\WplusTO}
\begin{lrbox}{\WplusTO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    x ?-> invalid at level 2;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WplusTP}
\settowidth{\WplusTP}{\usebox{\WplusTO}}
\newsavebox{\WplusTA}
\begin{lrbox}{\WplusTA}
\begin{minipage}{\WplusTH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte2(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|W+T|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WplusTP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WplusTO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WplusTA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WplusTI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WplusTK}\\
  \cline{2-2}
  & handler\\
  \cline{2-2}
  & \usebox{\WplusTM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|true|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/W.tex <==
\newlength{\WH}
\setlength{\WH}{0cm}
\newsavebox{\WI}
\begin{lrbox}{\WI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WJ}
\settowidth{\WJ}{\usebox{\WI}}
\addtolength{\WH}{\WJ}
\newsavebox{\WK}
\begin{lrbox}{\WK}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
\end{lstlisting}
\end{lrbox}
\newlength{\WL}
\settowidth{\WL}{\usebox{\WK}}
\newsavebox{\WM}
\begin{lrbox}{\WM}
\begin{minipage}{\WH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=x|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|W|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WL}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WK}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WM}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WI}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|true|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/WBM+dsb-tlbiis-dsb.tex <==
\newlength{\WBMplusdsbtlbiisdsbH}
\setlength{\WBMplusdsbtlbiisdsbH}{0cm}
\newsavebox{\WBMplusdsbtlbiisdsbI}
\begin{lrbox}{\WBMplusdsbtlbiisdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI VAE1IS,X5
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WBMplusdsbtlbiisdsbJ}
\settowidth{\WBMplusdsbtlbiisdsbJ}{\usebox{\WBMplusdsbtlbiisdsbI}}
\addtolength{\WBMplusdsbtlbiisdsbH}{\WBMplusdsbtlbiisdsbJ}
\newsavebox{\WBMplusdsbtlbiisdsbK}
\begin{lrbox}{\WBMplusdsbtlbiisdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WBMplusdsbtlbiisdsbL}
\settowidth{\WBMplusdsbtlbiisdsbL}{\usebox{\WBMplusdsbtlbiisdsbK}}
\addtolength{\WBMplusdsbtlbiisdsbH}{\WBMplusdsbtlbiisdsbL}
\newsavebox{\WBMplusdsbtlbiisdsbM}
\begin{lrbox}{\WBMplusdsbtlbiisdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WBMplusdsbtlbiisdsbN}
\settowidth{\WBMplusdsbtlbiisdsbN}{\usebox{\WBMplusdsbtlbiisdsbM}}
\addtolength{\WBMplusdsbtlbiisdsbH}{\WBMplusdsbtlbiisdsbN}
\newsavebox{\WBMplusdsbtlbiisdsbO}
\begin{lrbox}{\WBMplusdsbtlbiisdsbO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    x |-> pa1;
    y |-> pa1;
    *pa1 = 0;
    x ?-> invalid;
    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WBMplusdsbtlbiisdsbP}
\settowidth{\WBMplusdsbtlbiisdsbP}{\usebox{\WBMplusdsbtlbiisdsbO}}
\newsavebox{\WBMplusdsbtlbiisdsbA}
\begin{lrbox}{\WBMplusdsbtlbiisdsbA}
\begin{minipage}{\WBMplusdsbtlbiisdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b01|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R2=0x2|\\
\lstinline[language=IslaLitmusExp]|0:R3=y|\\
\lstinline[language=IslaLitmusExp]|0:R5=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:R0=0x1|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WBM+dsb-tlbiis-dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WBMplusdsbtlbiisdsbP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WBMplusdsbtlbiisdsbO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WBMplusdsbtlbiisdsbA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WBMplusdsbtlbiisdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WBMplusdsbtlbiisdsbK}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WBMplusdsbtlbiisdsbM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|x=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/WDS+dsb-tlbiipa-dsb-eret-po.tex <==
\newlength{\WDSplusdsbtlbiipadsberetpoH}
\setlength{\WDSplusdsbtlbiipadsberetpoH}{0cm}
\newsavebox{\WDSplusdsbtlbiipadsberetpoI}
\begin{lrbox}{\WDSplusdsbtlbiipadsberetpoI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1,X6
DSB SY
ERET
L0:
STR X2,[X3]
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\WDSplusdsbtlbiipadsberetpoJ}
\settowidth{\WDSplusdsbtlbiipadsberetpoJ}{\usebox{\WDSplusdsbtlbiipadsberetpoI}}
\addtolength{\WDSplusdsbtlbiipadsberetpoH}{\WDSplusdsbtlbiipadsberetpoJ}
\newsavebox{\WDSplusdsbtlbiipadsberetpoK}
\begin{lrbox}{\WDSplusdsbtlbiipadsberetpoK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1200:
MOV X4,#1
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WDSplusdsbtlbiipadsberetpoL}
\settowidth{\WDSplusdsbtlbiipadsberetpoL}{\usebox{\WDSplusdsbtlbiipadsberetpoK}}
\addtolength{\WDSplusdsbtlbiipadsberetpoH}{\WDSplusdsbtlbiipadsberetpoL}
\newsavebox{\WDSplusdsbtlbiipadsberetpoM}
\begin{lrbox}{\WDSplusdsbtlbiipadsberetpoM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X4,#2
MRS X20,ELR_EL2
ADD X20,X20,#4
MSR ELR_EL2,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WDSplusdsbtlbiipadsberetpoN}
\settowidth{\WDSplusdsbtlbiipadsberetpoN}{\usebox{\WDSplusdsbtlbiipadsberetpoM}}
\addtolength{\WDSplusdsbtlbiipadsberetpoH}{\WDSplusdsbtlbiipadsberetpoN}
\newsavebox{\WDSplusdsbtlbiipadsberetpoO}
\begin{lrbox}{\WDSplusdsbtlbiipadsberetpoO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;
    x ?-> invalid;

    ipa1 |-> pa1;
    ipa1 ?-> invalid;

    *pa1 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WDSplusdsbtlbiipadsberetpoP}
\settowidth{\WDSplusdsbtlbiipadsberetpoP}{\usebox{\WDSplusdsbtlbiipadsberetpoO}}
\newsavebox{\WDSplusdsbtlbiipadsberetpoA}
\begin{lrbox}{\WDSplusdsbtlbiipadsberetpoA}
\begin{minipage}{\WDSplusdsbtlbiipadsberetpoH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R2=0b0|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R5=x|\\
\lstinline[language=IslaLitmusExp]|R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00100|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WDS+dsb-tlbiipa-dsb-eret-po|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WDSplusdsbtlbiipadsberetpoP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WDSplusdsbtlbiipadsberetpoO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WDSplusdsbtlbiipadsberetpoA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WDSplusdsbtlbiipadsberetpoI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\WDSplusdsbtlbiipadsberetpoK}\\
  \cline{2-2}
  & thread0 el2 handler lower exc\\
  \cline{2-2}
  & \usebox{\WDSplusdsbtlbiipadsberetpoM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/WDS+dsb-tlbiipa-dsb-po-eret.tex <==
\newlength{\WDSplusdsbtlbiipadsbpoeretH}
\setlength{\WDSplusdsbtlbiipadsbpoeretH}{0cm}
\newsavebox{\WDSplusdsbtlbiipadsbpoeretI}
\begin{lrbox}{\WDSplusdsbtlbiipadsbpoeretI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1,X6
DSB SY
STR X2,[X3]
ERET
L0:
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\WDSplusdsbtlbiipadsbpoeretJ}
\settowidth{\WDSplusdsbtlbiipadsbpoeretJ}{\usebox{\WDSplusdsbtlbiipadsbpoeretI}}
\addtolength{\WDSplusdsbtlbiipadsbpoeretH}{\WDSplusdsbtlbiipadsbpoeretJ}
\newsavebox{\WDSplusdsbtlbiipadsbpoeretK}
\begin{lrbox}{\WDSplusdsbtlbiipadsbpoeretK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1200:
MOV X4,#1
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WDSplusdsbtlbiipadsbpoeretL}
\settowidth{\WDSplusdsbtlbiipadsbpoeretL}{\usebox{\WDSplusdsbtlbiipadsbpoeretK}}
\addtolength{\WDSplusdsbtlbiipadsbpoeretH}{\WDSplusdsbtlbiipadsbpoeretL}
\newsavebox{\WDSplusdsbtlbiipadsbpoeretM}
\begin{lrbox}{\WDSplusdsbtlbiipadsbpoeretM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X4,#2
MRS X20,ELR_EL2
ADD X20,X20,#4
MSR ELR_EL2,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WDSplusdsbtlbiipadsbpoeretN}
\settowidth{\WDSplusdsbtlbiipadsbpoeretN}{\usebox{\WDSplusdsbtlbiipadsbpoeretM}}
\addtolength{\WDSplusdsbtlbiipadsbpoeretH}{\WDSplusdsbtlbiipadsbpoeretN}
\newsavebox{\WDSplusdsbtlbiipadsbpoeretO}
\begin{lrbox}{\WDSplusdsbtlbiipadsbpoeretO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> invalid;
    x ?-> ipa1;

    ipa1 |-> invalid;
    ipa1 ?-> pa1;

    *pa1 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WDSplusdsbtlbiipadsbpoeretP}
\settowidth{\WDSplusdsbtlbiipadsbpoeretP}{\usebox{\WDSplusdsbtlbiipadsbpoeretO}}
\newsavebox{\WDSplusdsbtlbiipadsbpoeretA}
\begin{lrbox}{\WDSplusdsbtlbiipadsbpoeretA}
\begin{minipage}{\WDSplusdsbtlbiipadsbpoeretH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R2=mkdesc3(oa=ipa1)|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R5=x|\\
\lstinline[language=IslaLitmusExp]|R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00100|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WDS+dsb-tlbiipa-dsb-po-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WDSplusdsbtlbiipadsbpoeretP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WDSplusdsbtlbiipadsbpoeretO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WDSplusdsbtlbiipadsbpoeretA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WDSplusdsbtlbiipadsbpoeretI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\WDSplusdsbtlbiipadsbpoeretK}\\
  \cline{2-2}
  & thread0 el2 handler lower exc\\
  \cline{2-2}
  & \usebox{\WDSplusdsbtlbiipadsbpoeretM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R4=2|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/WDS+po-dsb-tlbiipa-dsb-eret.tex <==
\newlength{\WDSpluspodsbtlbiipadsberetH}
\setlength{\WDSpluspodsbtlbiipadsberetH}{0cm}
\newsavebox{\WDSpluspodsbtlbiipadsberetI}
\begin{lrbox}{\WDSpluspodsbtlbiipadsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
STR X2,[X3]
DSB SY
TLBI IPAS2E1,X6
DSB SY
ERET
L0:
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsberetJ}
\settowidth{\WDSpluspodsbtlbiipadsberetJ}{\usebox{\WDSpluspodsbtlbiipadsberetI}}
\addtolength{\WDSpluspodsbtlbiipadsberetH}{\WDSpluspodsbtlbiipadsberetJ}
\newsavebox{\WDSpluspodsbtlbiipadsberetK}
\begin{lrbox}{\WDSpluspodsbtlbiipadsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1200:
MOV X4,#1
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsberetL}
\settowidth{\WDSpluspodsbtlbiipadsberetL}{\usebox{\WDSpluspodsbtlbiipadsberetK}}
\addtolength{\WDSpluspodsbtlbiipadsberetH}{\WDSpluspodsbtlbiipadsberetL}
\newsavebox{\WDSpluspodsbtlbiipadsberetM}
\begin{lrbox}{\WDSpluspodsbtlbiipadsberetM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X4,#2
MRS X20,ELR_EL2
ADD X20,X20,#4
MSR ELR_EL2,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsberetN}
\settowidth{\WDSpluspodsbtlbiipadsberetN}{\usebox{\WDSpluspodsbtlbiipadsberetM}}
\addtolength{\WDSpluspodsbtlbiipadsberetH}{\WDSpluspodsbtlbiipadsberetN}
\newsavebox{\WDSpluspodsbtlbiipadsberetO}
\begin{lrbox}{\WDSpluspodsbtlbiipadsberetO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;
    x ?-> invalid;

    ipa1 |-> pa1;
    ipa1 ?-> invalid;

    *pa1 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsberetP}
\settowidth{\WDSpluspodsbtlbiipadsberetP}{\usebox{\WDSpluspodsbtlbiipadsberetO}}
\newsavebox{\WDSpluspodsbtlbiipadsberetA}
\begin{lrbox}{\WDSpluspodsbtlbiipadsberetA}
\begin{minipage}{\WDSpluspodsbtlbiipadsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R2=0b0|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R5=x|\\
\lstinline[language=IslaLitmusExp]|R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00100|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WDS+po-dsb-tlbiipa-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WDSpluspodsbtlbiipadsberetP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WDSpluspodsbtlbiipadsberetO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WDSpluspodsbtlbiipadsberetA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsberetI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsberetK}\\
  \cline{2-2}
  & thread0 el2 handler lower exc\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsberetM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/WDS+po-dsb-tlbiipa-dsb-po-eret.tex <==
\newlength{\WDSpluspodsbtlbiipadsbpoeretH}
\setlength{\WDSpluspodsbtlbiipadsbpoeretH}{0cm}
\newsavebox{\WDSpluspodsbtlbiipadsbpoeretI}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbpoeretI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
DSB SY
TLBI IPAS2E1,X6
DSB SY
STR X2,[X3]
ERET
L0:
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsbpoeretJ}
\settowidth{\WDSpluspodsbtlbiipadsbpoeretJ}{\usebox{\WDSpluspodsbtlbiipadsbpoeretI}}
\addtolength{\WDSpluspodsbtlbiipadsbpoeretH}{\WDSpluspodsbtlbiipadsbpoeretJ}
\newsavebox{\WDSpluspodsbtlbiipadsbpoeretK}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbpoeretK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1200:
MOV X4,#1
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsbpoeretL}
\settowidth{\WDSpluspodsbtlbiipadsbpoeretL}{\usebox{\WDSpluspodsbtlbiipadsbpoeretK}}
\addtolength{\WDSpluspodsbtlbiipadsbpoeretH}{\WDSpluspodsbtlbiipadsbpoeretL}
\newsavebox{\WDSpluspodsbtlbiipadsbpoeretM}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbpoeretM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X4,#2
MRS X20,ELR_EL2
ADD X20,X20,#4
MSR ELR_EL2,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsbpoeretN}
\settowidth{\WDSpluspodsbtlbiipadsbpoeretN}{\usebox{\WDSpluspodsbtlbiipadsbpoeretM}}
\addtolength{\WDSpluspodsbtlbiipadsbpoeretH}{\WDSpluspodsbtlbiipadsbpoeretN}
\newsavebox{\WDSpluspodsbtlbiipadsbpoeretO}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbpoeretO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;
    x ?-> invalid;

    ipa1 |-> pa1;
    ipa1 ?-> invalid;

    *pa1 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsbpoeretP}
\settowidth{\WDSpluspodsbtlbiipadsbpoeretP}{\usebox{\WDSpluspodsbtlbiipadsbpoeretO}}
\newsavebox{\WDSpluspodsbtlbiipadsbpoeretA}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbpoeretA}
\begin{minipage}{\WDSpluspodsbtlbiipadsbpoeretH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R2=0b0|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R5=x|\\
\lstinline[language=IslaLitmusExp]|R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00100|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WDS+po-dsb-tlbiipa-dsb-po-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WDSpluspodsbtlbiipadsbpoeretP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WDSpluspodsbtlbiipadsbpoeretO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WDSpluspodsbtlbiipadsbpoeretA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsbpoeretI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsbpoeretK}\\
  \cline{2-2}
  & thread0 el2 handler lower exc\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsbpoeretM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/WDS+po-dsb-tlbiipa-dsb-tlbiis-dsb-eret.tex <==
\newlength{\WDSpluspodsbtlbiipadsbtlbiisdsberetH}
\setlength{\WDSpluspodsbtlbiipadsbtlbiisdsberetH}{0cm}
\newsavebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetI}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbtlbiisdsberetI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
STR X2,[X3]
DSB SY
TLBI IPAS2E1,X6
DSB SY
TLBI VMALLE1IS
DSB SY
ERET
L0:
LDR X4,[X5]
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsbtlbiisdsberetJ}
\settowidth{\WDSpluspodsbtlbiipadsbtlbiisdsberetJ}{\usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetI}}
\addtolength{\WDSpluspodsbtlbiipadsbtlbiisdsberetH}{\WDSpluspodsbtlbiipadsbtlbiisdsberetJ}
\newsavebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetK}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbtlbiisdsberetK}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1200:
MOV X4,#1
MRS X20,ELR_EL1
ADD X20,X20,#4
MSR ELR_EL1,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsbtlbiisdsberetL}
\settowidth{\WDSpluspodsbtlbiipadsbtlbiisdsberetL}{\usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetK}}
\addtolength{\WDSpluspodsbtlbiipadsbtlbiisdsberetH}{\WDSpluspodsbtlbiipadsbtlbiisdsberetL}
\newsavebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetM}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbtlbiisdsberetM}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X4,#2
MRS X20,ELR_EL2
ADD X20,X20,#4
MSR ELR_EL2,X20
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsbtlbiisdsberetN}
\settowidth{\WDSpluspodsbtlbiipadsbtlbiisdsberetN}{\usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetM}}
\addtolength{\WDSpluspodsbtlbiipadsbtlbiisdsberetH}{\WDSpluspodsbtlbiipadsbtlbiisdsberetN}
\newsavebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetO}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbtlbiisdsberetO}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1;
    intermediate ipa1;

    x |-> ipa1;
    x ?-> invalid;

    ipa1 |-> pa1;
    ipa1 ?-> invalid;

    *pa1 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WDSpluspodsbtlbiipadsbtlbiisdsberetP}
\settowidth{\WDSpluspodsbtlbiipadsbtlbiisdsberetP}{\usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetO}}
\newsavebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetA}
\begin{lrbox}{\WDSpluspodsbtlbiipadsbtlbiisdsberetA}
\begin{minipage}{\WDSpluspodsbtlbiipadsbtlbiisdsberetH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|ELR_EL2=L0:|\\
\lstinline[language=IslaLitmusExp]|PSTATE.EL=0b10|\\
\lstinline[language=IslaLitmusExp]|R0=0b0|\\
\lstinline[language=IslaLitmusExp]|R1=pte3(ipa1,s2_page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R2=0b0|\\
\lstinline[language=IslaLitmusExp]|R3=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|R5=x|\\
\lstinline[language=IslaLitmusExp]|R6=page(x)|\\
\lstinline[language=IslaLitmusExp]|SPSR_EL2=0b00100|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|VBAR_EL2=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WDS+po-dsb-tlbiipa-dsb-tlbiis-dsb-eret|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WDSpluspodsbtlbiipadsbtlbiisdsberetP}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetO}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetA}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetI}\\
  \cline{2-2}
  & thread0 el1 handler\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetK}\\
  \cline{2-2}
  & thread0 el2 handler lower exc\\
  \cline{2-2}
  & \usebox{\WDSpluspodsbtlbiipadsbtlbiisdsberetM}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|0:R4=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/WRC.RRTf.inv+addrs.tex <==
\newlength{\WRCdotRRTfdotinvplusaddrsH}
\setlength{\WRCdotRRTfdotinvplusaddrsH}{0cm}
\newsavebox{\WRCdotRRTfdotinvplusaddrsI}
\begin{lrbox}{\WRCdotRRTfdotinvplusaddrsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusaddrsJ}
\settowidth{\WRCdotRRTfdotinvplusaddrsJ}{\usebox{\WRCdotRRTfdotinvplusaddrsI}}
\addtolength{\WRCdotRRTfdotinvplusaddrsH}{\WRCdotRRTfdotinvplusaddrsJ}
\newsavebox{\WRCdotRRTfdotinvplusaddrsK}
\begin{lrbox}{\WRCdotRRTfdotinvplusaddrsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
STR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusaddrsL}
\settowidth{\WRCdotRRTfdotinvplusaddrsL}{\usebox{\WRCdotRRTfdotinvplusaddrsK}}
\addtolength{\WRCdotRRTfdotinvplusaddrsH}{\WRCdotRRTfdotinvplusaddrsL}
\newsavebox{\WRCdotRRTfdotinvplusaddrsM}
\begin{lrbox}{\WRCdotRRTfdotinvplusaddrsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusaddrsN}
\settowidth{\WRCdotRRTfdotinvplusaddrsN}{\usebox{\WRCdotRRTfdotinvplusaddrsM}}
\addtolength{\WRCdotRRTfdotinvplusaddrsH}{\WRCdotRRTfdotinvplusaddrsN}
\newsavebox{\WRCdotRRTfdotinvplusaddrsO}
\begin{lrbox}{\WRCdotRRTfdotinvplusaddrsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusaddrsP}
\settowidth{\WRCdotRRTfdotinvplusaddrsP}{\usebox{\WRCdotRRTfdotinvplusaddrsO}}
\addtolength{\WRCdotRRTfdotinvplusaddrsH}{\WRCdotRRTfdotinvplusaddrsP}
\newsavebox{\WRCdotRRTfdotinvplusaddrsA}
\begin{lrbox}{\WRCdotRRTfdotinvplusaddrsA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusaddrsB}
\settowidth{\WRCdotRRTfdotinvplusaddrsB}{\usebox{\WRCdotRRTfdotinvplusaddrsA}}
\newsavebox{\WRCdotRRTfdotinvplusaddrsC}
\begin{lrbox}{\WRCdotRRTfdotinvplusaddrsC}
\begin{minipage}{\WRCdotRRTfdotinvplusaddrsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.RRTf.inv+addrs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotRRTfdotinvplusaddrsB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotRRTfdotinvplusaddrsA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotRRTfdotinvplusaddrsC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusaddrsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusaddrsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusaddrsM}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusaddrsO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=desc3(z,page_table_base) & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/WRC.RRTf.inv+dmbs.tex <==
\newlength{\WRCdotRRTfdotinvplusdmbsH}
\setlength{\WRCdotRRTfdotinvplusdmbsH}{0cm}
\newsavebox{\WRCdotRRTfdotinvplusdmbsI}
\begin{lrbox}{\WRCdotRRTfdotinvplusdmbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdmbsJ}
\settowidth{\WRCdotRRTfdotinvplusdmbsJ}{\usebox{\WRCdotRRTfdotinvplusdmbsI}}
\addtolength{\WRCdotRRTfdotinvplusdmbsH}{\WRCdotRRTfdotinvplusdmbsJ}
\newsavebox{\WRCdotRRTfdotinvplusdmbsK}
\begin{lrbox}{\WRCdotRRTfdotinvplusdmbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdmbsL}
\settowidth{\WRCdotRRTfdotinvplusdmbsL}{\usebox{\WRCdotRRTfdotinvplusdmbsK}}
\addtolength{\WRCdotRRTfdotinvplusdmbsH}{\WRCdotRRTfdotinvplusdmbsL}
\newsavebox{\WRCdotRRTfdotinvplusdmbsM}
\begin{lrbox}{\WRCdotRRTfdotinvplusdmbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdmbsN}
\settowidth{\WRCdotRRTfdotinvplusdmbsN}{\usebox{\WRCdotRRTfdotinvplusdmbsM}}
\addtolength{\WRCdotRRTfdotinvplusdmbsH}{\WRCdotRRTfdotinvplusdmbsN}
\newsavebox{\WRCdotRRTfdotinvplusdmbsO}
\begin{lrbox}{\WRCdotRRTfdotinvplusdmbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdmbsP}
\settowidth{\WRCdotRRTfdotinvplusdmbsP}{\usebox{\WRCdotRRTfdotinvplusdmbsO}}
\addtolength{\WRCdotRRTfdotinvplusdmbsH}{\WRCdotRRTfdotinvplusdmbsP}
\newsavebox{\WRCdotRRTfdotinvplusdmbsA}
\begin{lrbox}{\WRCdotRRTfdotinvplusdmbsA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdmbsB}
\settowidth{\WRCdotRRTfdotinvplusdmbsB}{\usebox{\WRCdotRRTfdotinvplusdmbsA}}
\newsavebox{\WRCdotRRTfdotinvplusdmbsC}
\begin{lrbox}{\WRCdotRRTfdotinvplusdmbsC}
\begin{minipage}{\WRCdotRRTfdotinvplusdmbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.RRTf.inv+dmbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotRRTfdotinvplusdmbsB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotRRTfdotinvplusdmbsA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotRRTfdotinvplusdmbsC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdmbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdmbsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdmbsM}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdmbsO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=desc3(z,page_table_base) & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/WRC.RRTf.inv+dsb+ctrl-isb.tex <==
\newlength{\WRCdotRRTfdotinvplusdsbplusctrlisbH}
\setlength{\WRCdotRRTfdotinvplusdsbplusctrlisbH}{0cm}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusctrlisbI}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusctrlisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusctrlisbJ}
\settowidth{\WRCdotRRTfdotinvplusdsbplusctrlisbJ}{\usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbI}}
\addtolength{\WRCdotRRTfdotinvplusdsbplusctrlisbH}{\WRCdotRRTfdotinvplusdsbplusctrlisbJ}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusctrlisbK}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusctrlisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusctrlisbL}
\settowidth{\WRCdotRRTfdotinvplusdsbplusctrlisbL}{\usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbK}}
\addtolength{\WRCdotRRTfdotinvplusdsbplusctrlisbH}{\WRCdotRRTfdotinvplusdsbplusctrlisbL}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusctrlisbM}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusctrlisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBNZ X0,L0
L0:
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusctrlisbN}
\settowidth{\WRCdotRRTfdotinvplusdsbplusctrlisbN}{\usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbM}}
\addtolength{\WRCdotRRTfdotinvplusdsbplusctrlisbH}{\WRCdotRRTfdotinvplusdsbplusctrlisbN}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusctrlisbO}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusctrlisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusctrlisbP}
\settowidth{\WRCdotRRTfdotinvplusdsbplusctrlisbP}{\usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbO}}
\addtolength{\WRCdotRRTfdotinvplusdsbplusctrlisbH}{\WRCdotRRTfdotinvplusdsbplusctrlisbP}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusctrlisbA}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusctrlisbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusctrlisbB}
\settowidth{\WRCdotRRTfdotinvplusdsbplusctrlisbB}{\usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbA}}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusctrlisbC}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusctrlisbC}
\begin{minipage}{\WRCdotRRTfdotinvplusdsbplusctrlisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.RRTf.inv+dsb+ctrl-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotRRTfdotinvplusdsbplusctrlisbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbM}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbplusctrlisbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=desc3(z,page_table_base) & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/WRC.RRTf.inv+dsb+dsb-isb.tex <==
\newlength{\WRCdotRRTfdotinvplusdsbplusdsbisbH}
\setlength{\WRCdotRRTfdotinvplusdsbplusdsbisbH}{0cm}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusdsbisbI}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusdsbisbJ}
\settowidth{\WRCdotRRTfdotinvplusdsbplusdsbisbJ}{\usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbI}}
\addtolength{\WRCdotRRTfdotinvplusdsbplusdsbisbH}{\WRCdotRRTfdotinvplusdsbplusdsbisbJ}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusdsbisbK}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusdsbisbL}
\settowidth{\WRCdotRRTfdotinvplusdsbplusdsbisbL}{\usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbK}}
\addtolength{\WRCdotRRTfdotinvplusdsbplusdsbisbH}{\WRCdotRRTfdotinvplusdsbplusdsbisbL}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusdsbisbM}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusdsbisbN}
\settowidth{\WRCdotRRTfdotinvplusdsbplusdsbisbN}{\usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbM}}
\addtolength{\WRCdotRRTfdotinvplusdsbplusdsbisbH}{\WRCdotRRTfdotinvplusdsbplusdsbisbN}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusdsbisbO}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusdsbisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusdsbisbP}
\settowidth{\WRCdotRRTfdotinvplusdsbplusdsbisbP}{\usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbO}}
\addtolength{\WRCdotRRTfdotinvplusdsbplusdsbisbH}{\WRCdotRRTfdotinvplusdsbplusdsbisbP}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusdsbisbA}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusdsbisbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbplusdsbisbB}
\settowidth{\WRCdotRRTfdotinvplusdsbplusdsbisbB}{\usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbA}}
\newsavebox{\WRCdotRRTfdotinvplusdsbplusdsbisbC}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbplusdsbisbC}
\begin{minipage}{\WRCdotRRTfdotinvplusdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.RRTf.inv+dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotRRTfdotinvplusdsbplusdsbisbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbM}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbplusdsbisbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=desc3(z,page_table_base) & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/WRC.RRTf.inv+dsbs.tex <==
\newlength{\WRCdotRRTfdotinvplusdsbsH}
\setlength{\WRCdotRRTfdotinvplusdsbsH}{0cm}
\newsavebox{\WRCdotRRTfdotinvplusdsbsI}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbsJ}
\settowidth{\WRCdotRRTfdotinvplusdsbsJ}{\usebox{\WRCdotRRTfdotinvplusdsbsI}}
\addtolength{\WRCdotRRTfdotinvplusdsbsH}{\WRCdotRRTfdotinvplusdsbsJ}
\newsavebox{\WRCdotRRTfdotinvplusdsbsK}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbsL}
\settowidth{\WRCdotRRTfdotinvplusdsbsL}{\usebox{\WRCdotRRTfdotinvplusdsbsK}}
\addtolength{\WRCdotRRTfdotinvplusdsbsH}{\WRCdotRRTfdotinvplusdsbsL}
\newsavebox{\WRCdotRRTfdotinvplusdsbsM}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbsN}
\settowidth{\WRCdotRRTfdotinvplusdsbsN}{\usebox{\WRCdotRRTfdotinvplusdsbsM}}
\addtolength{\WRCdotRRTfdotinvplusdsbsH}{\WRCdotRRTfdotinvplusdsbsN}
\newsavebox{\WRCdotRRTfdotinvplusdsbsO}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbsP}
\settowidth{\WRCdotRRTfdotinvplusdsbsP}{\usebox{\WRCdotRRTfdotinvplusdsbsO}}
\addtolength{\WRCdotRRTfdotinvplusdsbsH}{\WRCdotRRTfdotinvplusdsbsP}
\newsavebox{\WRCdotRRTfdotinvplusdsbsA}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbsA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusdsbsB}
\settowidth{\WRCdotRRTfdotinvplusdsbsB}{\usebox{\WRCdotRRTfdotinvplusdsbsA}}
\newsavebox{\WRCdotRRTfdotinvplusdsbsC}
\begin{lrbox}{\WRCdotRRTfdotinvplusdsbsC}
\begin{minipage}{\WRCdotRRTfdotinvplusdsbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.RRTf.inv+dsbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotRRTfdotinvplusdsbsB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotRRTfdotinvplusdsbsA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotRRTfdotinvplusdsbsC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbsM}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusdsbsO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=desc3(z,page_table_base) & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/WRC.RRTf.inv+pos.tex <==
\newlength{\WRCdotRRTfdotinvplusposH}
\setlength{\WRCdotRRTfdotinvplusposH}{0cm}
\newsavebox{\WRCdotRRTfdotinvplusposI}
\begin{lrbox}{\WRCdotRRTfdotinvplusposI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusposJ}
\settowidth{\WRCdotRRTfdotinvplusposJ}{\usebox{\WRCdotRRTfdotinvplusposI}}
\addtolength{\WRCdotRRTfdotinvplusposH}{\WRCdotRRTfdotinvplusposJ}
\newsavebox{\WRCdotRRTfdotinvplusposK}
\begin{lrbox}{\WRCdotRRTfdotinvplusposK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusposL}
\settowidth{\WRCdotRRTfdotinvplusposL}{\usebox{\WRCdotRRTfdotinvplusposK}}
\addtolength{\WRCdotRRTfdotinvplusposH}{\WRCdotRRTfdotinvplusposL}
\newsavebox{\WRCdotRRTfdotinvplusposM}
\begin{lrbox}{\WRCdotRRTfdotinvplusposM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusposN}
\settowidth{\WRCdotRRTfdotinvplusposN}{\usebox{\WRCdotRRTfdotinvplusposM}}
\addtolength{\WRCdotRRTfdotinvplusposH}{\WRCdotRRTfdotinvplusposN}
\newsavebox{\WRCdotRRTfdotinvplusposO}
\begin{lrbox}{\WRCdotRRTfdotinvplusposO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusposP}
\settowidth{\WRCdotRRTfdotinvplusposP}{\usebox{\WRCdotRRTfdotinvplusposO}}
\addtolength{\WRCdotRRTfdotinvplusposH}{\WRCdotRRTfdotinvplusposP}
\newsavebox{\WRCdotRRTfdotinvplusposA}
\begin{lrbox}{\WRCdotRRTfdotinvplusposA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotRRTfdotinvplusposB}
\settowidth{\WRCdotRRTfdotinvplusposB}{\usebox{\WRCdotRRTfdotinvplusposA}}
\newsavebox{\WRCdotRRTfdotinvplusposC}
\begin{lrbox}{\WRCdotRRTfdotinvplusposC}
\begin{minipage}{\WRCdotRRTfdotinvplusposH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.RRTf.inv+pos|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotRRTfdotinvplusposB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotRRTfdotinvplusposA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotRRTfdotinvplusposC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusposI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusposK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusposM}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotRRTfdotinvplusposO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=desc3(z,page_table_base) & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/WRC.TRTf.inv+addrs.tex <==
\newlength{\WRCdotTRTfdotinvplusaddrsH}
\setlength{\WRCdotTRTfdotinvplusaddrsH}{0cm}
\newsavebox{\WRCdotTRTfdotinvplusaddrsI}
\begin{lrbox}{\WRCdotTRTfdotinvplusaddrsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusaddrsJ}
\settowidth{\WRCdotTRTfdotinvplusaddrsJ}{\usebox{\WRCdotTRTfdotinvplusaddrsI}}
\addtolength{\WRCdotTRTfdotinvplusaddrsH}{\WRCdotTRTfdotinvplusaddrsJ}
\newsavebox{\WRCdotTRTfdotinvplusaddrsK}
\begin{lrbox}{\WRCdotTRTfdotinvplusaddrsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
STR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusaddrsL}
\settowidth{\WRCdotTRTfdotinvplusaddrsL}{\usebox{\WRCdotTRTfdotinvplusaddrsK}}
\addtolength{\WRCdotTRTfdotinvplusaddrsH}{\WRCdotTRTfdotinvplusaddrsL}
\newsavebox{\WRCdotTRTfdotinvplusaddrsM}
\begin{lrbox}{\WRCdotTRTfdotinvplusaddrsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
EOR X4,X0,X0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusaddrsN}
\settowidth{\WRCdotTRTfdotinvplusaddrsN}{\usebox{\WRCdotTRTfdotinvplusaddrsM}}
\addtolength{\WRCdotTRTfdotinvplusaddrsH}{\WRCdotTRTfdotinvplusaddrsN}
\newsavebox{\WRCdotTRTfdotinvplusaddrsO}
\begin{lrbox}{\WRCdotTRTfdotinvplusaddrsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusaddrsP}
\settowidth{\WRCdotTRTfdotinvplusaddrsP}{\usebox{\WRCdotTRTfdotinvplusaddrsO}}
\addtolength{\WRCdotTRTfdotinvplusaddrsH}{\WRCdotTRTfdotinvplusaddrsP}
\newsavebox{\WRCdotTRTfdotinvplusaddrsA}
\begin{lrbox}{\WRCdotTRTfdotinvplusaddrsA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusaddrsB}
\settowidth{\WRCdotTRTfdotinvplusaddrsB}{\usebox{\WRCdotTRTfdotinvplusaddrsA}}
\addtolength{\WRCdotTRTfdotinvplusaddrsH}{\WRCdotTRTfdotinvplusaddrsB}
\newsavebox{\WRCdotTRTfdotinvplusaddrsC}
\begin{lrbox}{\WRCdotTRTfdotinvplusaddrsC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusaddrsD}
\settowidth{\WRCdotTRTfdotinvplusaddrsD}{\usebox{\WRCdotTRTfdotinvplusaddrsC}}
\newsavebox{\WRCdotTRTfdotinvplusaddrsE}
\begin{lrbox}{\WRCdotTRTfdotinvplusaddrsE}
\begin{minipage}{\WRCdotTRTfdotinvplusaddrsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TRTf.inv+addrs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTRTfdotinvplusaddrsD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTRTfdotinvplusaddrsC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTRTfdotinvplusaddrsE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusaddrsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusaddrsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusaddrsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusaddrsO}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusaddrsA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/WRC.TRTf.inv+dmbs.tex <==
\newlength{\WRCdotTRTfdotinvplusdmbsH}
\setlength{\WRCdotTRTfdotinvplusdmbsH}{0cm}
\newsavebox{\WRCdotTRTfdotinvplusdmbsI}
\begin{lrbox}{\WRCdotTRTfdotinvplusdmbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdmbsJ}
\settowidth{\WRCdotTRTfdotinvplusdmbsJ}{\usebox{\WRCdotTRTfdotinvplusdmbsI}}
\addtolength{\WRCdotTRTfdotinvplusdmbsH}{\WRCdotTRTfdotinvplusdmbsJ}
\newsavebox{\WRCdotTRTfdotinvplusdmbsK}
\begin{lrbox}{\WRCdotTRTfdotinvplusdmbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdmbsL}
\settowidth{\WRCdotTRTfdotinvplusdmbsL}{\usebox{\WRCdotTRTfdotinvplusdmbsK}}
\addtolength{\WRCdotTRTfdotinvplusdmbsH}{\WRCdotTRTfdotinvplusdmbsL}
\newsavebox{\WRCdotTRTfdotinvplusdmbsM}
\begin{lrbox}{\WRCdotTRTfdotinvplusdmbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdmbsN}
\settowidth{\WRCdotTRTfdotinvplusdmbsN}{\usebox{\WRCdotTRTfdotinvplusdmbsM}}
\addtolength{\WRCdotTRTfdotinvplusdmbsH}{\WRCdotTRTfdotinvplusdmbsN}
\newsavebox{\WRCdotTRTfdotinvplusdmbsO}
\begin{lrbox}{\WRCdotTRTfdotinvplusdmbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdmbsP}
\settowidth{\WRCdotTRTfdotinvplusdmbsP}{\usebox{\WRCdotTRTfdotinvplusdmbsO}}
\addtolength{\WRCdotTRTfdotinvplusdmbsH}{\WRCdotTRTfdotinvplusdmbsP}
\newsavebox{\WRCdotTRTfdotinvplusdmbsA}
\begin{lrbox}{\WRCdotTRTfdotinvplusdmbsA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdmbsB}
\settowidth{\WRCdotTRTfdotinvplusdmbsB}{\usebox{\WRCdotTRTfdotinvplusdmbsA}}
\addtolength{\WRCdotTRTfdotinvplusdmbsH}{\WRCdotTRTfdotinvplusdmbsB}
\newsavebox{\WRCdotTRTfdotinvplusdmbsC}
\begin{lrbox}{\WRCdotTRTfdotinvplusdmbsC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdmbsD}
\settowidth{\WRCdotTRTfdotinvplusdmbsD}{\usebox{\WRCdotTRTfdotinvplusdmbsC}}
\newsavebox{\WRCdotTRTfdotinvplusdmbsE}
\begin{lrbox}{\WRCdotTRTfdotinvplusdmbsE}
\begin{minipage}{\WRCdotTRTfdotinvplusdmbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TRTf.inv+dmbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTRTfdotinvplusdmbsD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTRTfdotinvplusdmbsC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTRTfdotinvplusdmbsE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdmbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdmbsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdmbsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdmbsO}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdmbsA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/WRC.TRTf.inv+dsb+dsb-isb.tex <==
\newlength{\WRCdotTRTfdotinvplusdsbplusdsbisbH}
\setlength{\WRCdotTRTfdotinvplusdsbplusdsbisbH}{0cm}
\newsavebox{\WRCdotTRTfdotinvplusdsbplusdsbisbI}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbplusdsbisbJ}
\settowidth{\WRCdotTRTfdotinvplusdsbplusdsbisbJ}{\usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbI}}
\addtolength{\WRCdotTRTfdotinvplusdsbplusdsbisbH}{\WRCdotTRTfdotinvplusdsbplusdsbisbJ}
\newsavebox{\WRCdotTRTfdotinvplusdsbplusdsbisbK}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbplusdsbisbL}
\settowidth{\WRCdotTRTfdotinvplusdsbplusdsbisbL}{\usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbK}}
\addtolength{\WRCdotTRTfdotinvplusdsbplusdsbisbH}{\WRCdotTRTfdotinvplusdsbplusdsbisbL}
\newsavebox{\WRCdotTRTfdotinvplusdsbplusdsbisbM}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbplusdsbisbN}
\settowidth{\WRCdotTRTfdotinvplusdsbplusdsbisbN}{\usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbM}}
\addtolength{\WRCdotTRTfdotinvplusdsbplusdsbisbH}{\WRCdotTRTfdotinvplusdsbplusdsbisbN}
\newsavebox{\WRCdotTRTfdotinvplusdsbplusdsbisbO}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbplusdsbisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbplusdsbisbP}
\settowidth{\WRCdotTRTfdotinvplusdsbplusdsbisbP}{\usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbO}}
\addtolength{\WRCdotTRTfdotinvplusdsbplusdsbisbH}{\WRCdotTRTfdotinvplusdsbplusdsbisbP}
\newsavebox{\WRCdotTRTfdotinvplusdsbplusdsbisbA}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbplusdsbisbA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbplusdsbisbB}
\settowidth{\WRCdotTRTfdotinvplusdsbplusdsbisbB}{\usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbA}}
\addtolength{\WRCdotTRTfdotinvplusdsbplusdsbisbH}{\WRCdotTRTfdotinvplusdsbplusdsbisbB}
\newsavebox{\WRCdotTRTfdotinvplusdsbplusdsbisbC}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbplusdsbisbC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbplusdsbisbD}
\settowidth{\WRCdotTRTfdotinvplusdsbplusdsbisbD}{\usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbC}}
\newsavebox{\WRCdotTRTfdotinvplusdsbplusdsbisbE}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbplusdsbisbE}
\begin{minipage}{\WRCdotTRTfdotinvplusdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TRTf.inv+dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTRTfdotinvplusdsbplusdsbisbD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbO}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbplusdsbisbA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/WRC.TRTf.inv+dsbs.tex <==
\newlength{\WRCdotTRTfdotinvplusdsbsH}
\setlength{\WRCdotTRTfdotinvplusdsbsH}{0cm}
\newsavebox{\WRCdotTRTfdotinvplusdsbsI}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbsJ}
\settowidth{\WRCdotTRTfdotinvplusdsbsJ}{\usebox{\WRCdotTRTfdotinvplusdsbsI}}
\addtolength{\WRCdotTRTfdotinvplusdsbsH}{\WRCdotTRTfdotinvplusdsbsJ}
\newsavebox{\WRCdotTRTfdotinvplusdsbsK}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbsL}
\settowidth{\WRCdotTRTfdotinvplusdsbsL}{\usebox{\WRCdotTRTfdotinvplusdsbsK}}
\addtolength{\WRCdotTRTfdotinvplusdsbsH}{\WRCdotTRTfdotinvplusdsbsL}
\newsavebox{\WRCdotTRTfdotinvplusdsbsM}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbsN}
\settowidth{\WRCdotTRTfdotinvplusdsbsN}{\usebox{\WRCdotTRTfdotinvplusdsbsM}}
\addtolength{\WRCdotTRTfdotinvplusdsbsH}{\WRCdotTRTfdotinvplusdsbsN}
\newsavebox{\WRCdotTRTfdotinvplusdsbsO}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbsP}
\settowidth{\WRCdotTRTfdotinvplusdsbsP}{\usebox{\WRCdotTRTfdotinvplusdsbsO}}
\addtolength{\WRCdotTRTfdotinvplusdsbsH}{\WRCdotTRTfdotinvplusdsbsP}
\newsavebox{\WRCdotTRTfdotinvplusdsbsA}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbsA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbsB}
\settowidth{\WRCdotTRTfdotinvplusdsbsB}{\usebox{\WRCdotTRTfdotinvplusdsbsA}}
\addtolength{\WRCdotTRTfdotinvplusdsbsH}{\WRCdotTRTfdotinvplusdsbsB}
\newsavebox{\WRCdotTRTfdotinvplusdsbsC}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbsC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusdsbsD}
\settowidth{\WRCdotTRTfdotinvplusdsbsD}{\usebox{\WRCdotTRTfdotinvplusdsbsC}}
\newsavebox{\WRCdotTRTfdotinvplusdsbsE}
\begin{lrbox}{\WRCdotTRTfdotinvplusdsbsE}
\begin{minipage}{\WRCdotTRTfdotinvplusdsbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TRTf.inv+dsbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTRTfdotinvplusdsbsD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTRTfdotinvplusdsbsC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTRTfdotinvplusdsbsE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbsO}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusdsbsA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/WRC.TRTf.inv+pos.tex <==
\newlength{\WRCdotTRTfdotinvplusposH}
\setlength{\WRCdotTRTfdotinvplusposH}{0cm}
\newsavebox{\WRCdotTRTfdotinvplusposI}
\begin{lrbox}{\WRCdotTRTfdotinvplusposI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusposJ}
\settowidth{\WRCdotTRTfdotinvplusposJ}{\usebox{\WRCdotTRTfdotinvplusposI}}
\addtolength{\WRCdotTRTfdotinvplusposH}{\WRCdotTRTfdotinvplusposJ}
\newsavebox{\WRCdotTRTfdotinvplusposK}
\begin{lrbox}{\WRCdotTRTfdotinvplusposK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusposL}
\settowidth{\WRCdotTRTfdotinvplusposL}{\usebox{\WRCdotTRTfdotinvplusposK}}
\addtolength{\WRCdotTRTfdotinvplusposH}{\WRCdotTRTfdotinvplusposL}
\newsavebox{\WRCdotTRTfdotinvplusposM}
\begin{lrbox}{\WRCdotTRTfdotinvplusposM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusposN}
\settowidth{\WRCdotTRTfdotinvplusposN}{\usebox{\WRCdotTRTfdotinvplusposM}}
\addtolength{\WRCdotTRTfdotinvplusposH}{\WRCdotTRTfdotinvplusposN}
\newsavebox{\WRCdotTRTfdotinvplusposO}
\begin{lrbox}{\WRCdotTRTfdotinvplusposO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusposP}
\settowidth{\WRCdotTRTfdotinvplusposP}{\usebox{\WRCdotTRTfdotinvplusposO}}
\addtolength{\WRCdotTRTfdotinvplusposH}{\WRCdotTRTfdotinvplusposP}
\newsavebox{\WRCdotTRTfdotinvplusposA}
\begin{lrbox}{\WRCdotTRTfdotinvplusposA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X2,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusposB}
\settowidth{\WRCdotTRTfdotinvplusposB}{\usebox{\WRCdotTRTfdotinvplusposA}}
\addtolength{\WRCdotTRTfdotinvplusposH}{\WRCdotTRTfdotinvplusposB}
\newsavebox{\WRCdotTRTfdotinvplusposC}
\begin{lrbox}{\WRCdotTRTfdotinvplusposC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;

    x ?-> pa1;
    z |-> pa1;
    *pa1 = 1;

    y |-> pa2;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTRTfdotinvplusposD}
\settowidth{\WRCdotTRTfdotinvplusposD}{\usebox{\WRCdotTRTfdotinvplusposC}}
\newsavebox{\WRCdotTRTfdotinvplusposE}
\begin{lrbox}{\WRCdotTRTfdotinvplusposE}
\begin{minipage}{\WRCdotTRTfdotinvplusposH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TRTf.inv+pos|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTRTfdotinvplusposD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTRTfdotinvplusposC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTRTfdotinvplusposE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusposI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusposK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusposM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusposO}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTRTfdotinvplusposA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/WRC.TTTf.inv+addrs.tex <==
\newlength{\WRCdotTTTfdotinvplusaddrsH}
\setlength{\WRCdotTTTfdotinvplusaddrsH}{0cm}
\newsavebox{\WRCdotTTTfdotinvplusaddrsI}
\begin{lrbox}{\WRCdotTTTfdotinvplusaddrsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusaddrsJ}
\settowidth{\WRCdotTTTfdotinvplusaddrsJ}{\usebox{\WRCdotTTTfdotinvplusaddrsI}}
\addtolength{\WRCdotTTTfdotinvplusaddrsH}{\WRCdotTTTfdotinvplusaddrsJ}
\newsavebox{\WRCdotTTTfdotinvplusaddrsK}
\begin{lrbox}{\WRCdotTTTfdotinvplusaddrsK}
\begin{lstlisting}[language=AArch64,showlines=true]
MOV X0,#0
LDR X0,[X1]
EOR X4,X0,X0
STR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusaddrsL}
\settowidth{\WRCdotTTTfdotinvplusaddrsL}{\usebox{\WRCdotTTTfdotinvplusaddrsK}}
\addtolength{\WRCdotTTTfdotinvplusaddrsH}{\WRCdotTTTfdotinvplusaddrsL}
\newsavebox{\WRCdotTTTfdotinvplusaddrsM}
\begin{lrbox}{\WRCdotTTTfdotinvplusaddrsM}
\begin{lstlisting}[language=AArch64,showlines=true]
MOV X0,#0
LDR X0,[X1]
EOR X4,X0,X0
MOV X2,#0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusaddrsN}
\settowidth{\WRCdotTTTfdotinvplusaddrsN}{\usebox{\WRCdotTTTfdotinvplusaddrsM}}
\addtolength{\WRCdotTTTfdotinvplusaddrsH}{\WRCdotTTTfdotinvplusaddrsN}
\newsavebox{\WRCdotTTTfdotinvplusaddrsO}
\begin{lrbox}{\WRCdotTTTfdotinvplusaddrsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusaddrsP}
\settowidth{\WRCdotTTTfdotinvplusaddrsP}{\usebox{\WRCdotTTTfdotinvplusaddrsO}}
\addtolength{\WRCdotTTTfdotinvplusaddrsH}{\WRCdotTTTfdotinvplusaddrsP}
\newsavebox{\WRCdotTTTfdotinvplusaddrsA}
\begin{lrbox}{\WRCdotTTTfdotinvplusaddrsA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusaddrsB}
\settowidth{\WRCdotTTTfdotinvplusaddrsB}{\usebox{\WRCdotTTTfdotinvplusaddrsA}}
\addtolength{\WRCdotTTTfdotinvplusaddrsH}{\WRCdotTTTfdotinvplusaddrsB}
\newsavebox{\WRCdotTTTfdotinvplusaddrsC}
\begin{lrbox}{\WRCdotTTTfdotinvplusaddrsC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusaddrsD}
\settowidth{\WRCdotTTTfdotinvplusaddrsD}{\usebox{\WRCdotTTTfdotinvplusaddrsC}}
\newsavebox{\WRCdotTTTfdotinvplusaddrsE}
\begin{lrbox}{\WRCdotTTTfdotinvplusaddrsE}
\begin{minipage}{\WRCdotTTTfdotinvplusaddrsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:__isla_monomorphize_writes=true|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TTTf.inv+addrs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTTTfdotinvplusaddrsD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTTTfdotinvplusaddrsC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTTTfdotinvplusaddrsE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusaddrsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusaddrsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusaddrsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusaddrsO}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusaddrsA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/WRC.TTTf.inv+data+addr.tex <==
\newlength{\WRCdotTTTfdotinvplusdataplusaddrH}
\setlength{\WRCdotTTTfdotinvplusdataplusaddrH}{0cm}
\newsavebox{\WRCdotTTTfdotinvplusdataplusaddrI}
\begin{lrbox}{\WRCdotTTTfdotinvplusdataplusaddrI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusdataplusaddrJ}
\settowidth{\WRCdotTTTfdotinvplusdataplusaddrJ}{\usebox{\WRCdotTTTfdotinvplusdataplusaddrI}}
\addtolength{\WRCdotTTTfdotinvplusdataplusaddrH}{\WRCdotTTTfdotinvplusdataplusaddrJ}
\newsavebox{\WRCdotTTTfdotinvplusdataplusaddrK}
\begin{lrbox}{\WRCdotTTTfdotinvplusdataplusaddrK}
\begin{lstlisting}[language=AArch64,showlines=true]
MOV X0,#0
LDR X0,[X1]
EOR X4,X0,X0
ORR X2,X2,X4
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusdataplusaddrL}
\settowidth{\WRCdotTTTfdotinvplusdataplusaddrL}{\usebox{\WRCdotTTTfdotinvplusdataplusaddrK}}
\addtolength{\WRCdotTTTfdotinvplusdataplusaddrH}{\WRCdotTTTfdotinvplusdataplusaddrL}
\newsavebox{\WRCdotTTTfdotinvplusdataplusaddrM}
\begin{lrbox}{\WRCdotTTTfdotinvplusdataplusaddrM}
\begin{lstlisting}[language=AArch64,showlines=true]
MOV X0,#0
LDR X0,[X1]
EOR X4,X0,X0
MOV X2,#0
LDR X2,[X3,X4]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusdataplusaddrN}
\settowidth{\WRCdotTTTfdotinvplusdataplusaddrN}{\usebox{\WRCdotTTTfdotinvplusdataplusaddrM}}
\addtolength{\WRCdotTTTfdotinvplusdataplusaddrH}{\WRCdotTTTfdotinvplusdataplusaddrN}
\newsavebox{\WRCdotTTTfdotinvplusdataplusaddrO}
\begin{lrbox}{\WRCdotTTTfdotinvplusdataplusaddrO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusdataplusaddrP}
\settowidth{\WRCdotTTTfdotinvplusdataplusaddrP}{\usebox{\WRCdotTTTfdotinvplusdataplusaddrO}}
\addtolength{\WRCdotTTTfdotinvplusdataplusaddrH}{\WRCdotTTTfdotinvplusdataplusaddrP}
\newsavebox{\WRCdotTTTfdotinvplusdataplusaddrA}
\begin{lrbox}{\WRCdotTTTfdotinvplusdataplusaddrA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusdataplusaddrB}
\settowidth{\WRCdotTTTfdotinvplusdataplusaddrB}{\usebox{\WRCdotTTTfdotinvplusdataplusaddrA}}
\addtolength{\WRCdotTTTfdotinvplusdataplusaddrH}{\WRCdotTTTfdotinvplusdataplusaddrB}
\newsavebox{\WRCdotTTTfdotinvplusdataplusaddrC}
\begin{lrbox}{\WRCdotTTTfdotinvplusdataplusaddrC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> invalid;
    x ?-> pa1;

    y |-> invalid;
    y ?-> pa2;

    *pa1 = 1;
    *pa2 = 1;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTTTfdotinvplusdataplusaddrD}
\settowidth{\WRCdotTTTfdotinvplusdataplusaddrD}{\usebox{\WRCdotTTTfdotinvplusdataplusaddrC}}
\newsavebox{\WRCdotTTTfdotinvplusdataplusaddrE}
\begin{lrbox}{\WRCdotTTTfdotinvplusdataplusaddrE}
\begin{minipage}{\WRCdotTTTfdotinvplusdataplusaddrH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=mkdesc3(oa=pa1)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=mkdesc3(oa=pa2)|\\
\lstinline[language=IslaLitmusExp]|1:R3=pte3(y,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|1:__isla_monomorphize_writes=true|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TTTf.inv+data+addr|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTTTfdotinvplusdataplusaddrD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTTTfdotinvplusdataplusaddrC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTTTfdotinvplusdataplusaddrE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusdataplusaddrI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusdataplusaddrK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusdataplusaddrM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusdataplusaddrO}\\
  \cline{2-2}
  & thread2 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTTTfdotinvplusdataplusaddrA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & 2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/WRC.TfRR+ctrl-isb+dsb.tex <==
\newlength{\WRCdotTfRRplusctrlisbplusdsbH}
\setlength{\WRCdotTfRRplusctrlisbplusdsbH}{0cm}
\newsavebox{\WRCdotTfRRplusctrlisbplusdsbI}
\begin{lrbox}{\WRCdotTfRRplusctrlisbplusdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusctrlisbplusdsbJ}
\settowidth{\WRCdotTfRRplusctrlisbplusdsbJ}{\usebox{\WRCdotTfRRplusctrlisbplusdsbI}}
\addtolength{\WRCdotTfRRplusctrlisbplusdsbH}{\WRCdotTfRRplusctrlisbplusdsbJ}
\newsavebox{\WRCdotTfRRplusctrlisbplusdsbK}
\begin{lrbox}{\WRCdotTfRRplusctrlisbplusdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
CBNZ X0,L0
L0:
ISB
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusctrlisbplusdsbL}
\settowidth{\WRCdotTfRRplusctrlisbplusdsbL}{\usebox{\WRCdotTfRRplusctrlisbplusdsbK}}
\addtolength{\WRCdotTfRRplusctrlisbplusdsbH}{\WRCdotTfRRplusctrlisbplusdsbL}
\newsavebox{\WRCdotTfRRplusctrlisbplusdsbM}
\begin{lrbox}{\WRCdotTfRRplusctrlisbplusdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusctrlisbplusdsbN}
\settowidth{\WRCdotTfRRplusctrlisbplusdsbN}{\usebox{\WRCdotTfRRplusctrlisbplusdsbM}}
\addtolength{\WRCdotTfRRplusctrlisbplusdsbH}{\WRCdotTfRRplusctrlisbplusdsbN}
\newsavebox{\WRCdotTfRRplusctrlisbplusdsbO}
\begin{lrbox}{\WRCdotTfRRplusctrlisbplusdsbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusctrlisbplusdsbP}
\settowidth{\WRCdotTfRRplusctrlisbplusdsbP}{\usebox{\WRCdotTfRRplusctrlisbplusdsbO}}
\addtolength{\WRCdotTfRRplusctrlisbplusdsbH}{\WRCdotTfRRplusctrlisbplusdsbP}
\newsavebox{\WRCdotTfRRplusctrlisbplusdsbA}
\begin{lrbox}{\WRCdotTfRRplusctrlisbplusdsbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    *pa1 = 0;

    y |-> pa2;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusctrlisbplusdsbB}
\settowidth{\WRCdotTfRRplusctrlisbplusdsbB}{\usebox{\WRCdotTfRRplusctrlisbplusdsbA}}
\newsavebox{\WRCdotTfRRplusctrlisbplusdsbC}
\begin{lrbox}{\WRCdotTfRRplusctrlisbplusdsbC}
\begin{minipage}{\WRCdotTfRRplusctrlisbplusdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TfRR+ctrl-isb+dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTfRRplusctrlisbplusdsbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTfRRplusctrlisbplusdsbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTfRRplusctrlisbplusdsbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusctrlisbplusdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusctrlisbplusdsbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusctrlisbplusdsbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusctrlisbplusdsbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & ~2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/WRC.TfRR+dmbs.tex <==
\newlength{\WRCdotTfRRplusdmbsH}
\setlength{\WRCdotTfRRplusdmbsH}{0cm}
\newsavebox{\WRCdotTfRRplusdmbsI}
\begin{lrbox}{\WRCdotTfRRplusdmbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdmbsJ}
\settowidth{\WRCdotTfRRplusdmbsJ}{\usebox{\WRCdotTfRRplusdmbsI}}
\addtolength{\WRCdotTfRRplusdmbsH}{\WRCdotTfRRplusdmbsJ}
\newsavebox{\WRCdotTfRRplusdmbsK}
\begin{lrbox}{\WRCdotTfRRplusdmbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdmbsL}
\settowidth{\WRCdotTfRRplusdmbsL}{\usebox{\WRCdotTfRRplusdmbsK}}
\addtolength{\WRCdotTfRRplusdmbsH}{\WRCdotTfRRplusdmbsL}
\newsavebox{\WRCdotTfRRplusdmbsM}
\begin{lrbox}{\WRCdotTfRRplusdmbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DMB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdmbsN}
\settowidth{\WRCdotTfRRplusdmbsN}{\usebox{\WRCdotTfRRplusdmbsM}}
\addtolength{\WRCdotTfRRplusdmbsH}{\WRCdotTfRRplusdmbsN}
\newsavebox{\WRCdotTfRRplusdmbsO}
\begin{lrbox}{\WRCdotTfRRplusdmbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdmbsP}
\settowidth{\WRCdotTfRRplusdmbsP}{\usebox{\WRCdotTfRRplusdmbsO}}
\addtolength{\WRCdotTfRRplusdmbsH}{\WRCdotTfRRplusdmbsP}
\newsavebox{\WRCdotTfRRplusdmbsA}
\begin{lrbox}{\WRCdotTfRRplusdmbsA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    *pa1 = 0;

    y |-> pa2;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdmbsB}
\settowidth{\WRCdotTfRRplusdmbsB}{\usebox{\WRCdotTfRRplusdmbsA}}
\newsavebox{\WRCdotTfRRplusdmbsC}
\begin{lrbox}{\WRCdotTfRRplusdmbsC}
\begin{minipage}{\WRCdotTfRRplusdmbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TfRR+dmbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTfRRplusdmbsB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTfRRplusdmbsA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTfRRplusdmbsC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdmbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdmbsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdmbsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdmbsO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & ~2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/WRC.TfRR+dsb-isb+dsb.tex <==
\newlength{\WRCdotTfRRplusdsbisbplusdsbH}
\setlength{\WRCdotTfRRplusdsbisbplusdsbH}{0cm}
\newsavebox{\WRCdotTfRRplusdsbisbplusdsbI}
\begin{lrbox}{\WRCdotTfRRplusdsbisbplusdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbisbplusdsbJ}
\settowidth{\WRCdotTfRRplusdsbisbplusdsbJ}{\usebox{\WRCdotTfRRplusdsbisbplusdsbI}}
\addtolength{\WRCdotTfRRplusdsbisbplusdsbH}{\WRCdotTfRRplusdsbisbplusdsbJ}
\newsavebox{\WRCdotTfRRplusdsbisbplusdsbK}
\begin{lrbox}{\WRCdotTfRRplusdsbisbplusdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbisbplusdsbL}
\settowidth{\WRCdotTfRRplusdsbisbplusdsbL}{\usebox{\WRCdotTfRRplusdsbisbplusdsbK}}
\addtolength{\WRCdotTfRRplusdsbisbplusdsbH}{\WRCdotTfRRplusdsbisbplusdsbL}
\newsavebox{\WRCdotTfRRplusdsbisbplusdsbM}
\begin{lrbox}{\WRCdotTfRRplusdsbisbplusdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbisbplusdsbN}
\settowidth{\WRCdotTfRRplusdsbisbplusdsbN}{\usebox{\WRCdotTfRRplusdsbisbplusdsbM}}
\addtolength{\WRCdotTfRRplusdsbisbplusdsbH}{\WRCdotTfRRplusdsbisbplusdsbN}
\newsavebox{\WRCdotTfRRplusdsbisbplusdsbO}
\begin{lrbox}{\WRCdotTfRRplusdsbisbplusdsbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbisbplusdsbP}
\settowidth{\WRCdotTfRRplusdsbisbplusdsbP}{\usebox{\WRCdotTfRRplusdsbisbplusdsbO}}
\addtolength{\WRCdotTfRRplusdsbisbplusdsbH}{\WRCdotTfRRplusdsbisbplusdsbP}
\newsavebox{\WRCdotTfRRplusdsbisbplusdsbA}
\begin{lrbox}{\WRCdotTfRRplusdsbisbplusdsbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    *pa1 = 0;

    y |-> pa2;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbisbplusdsbB}
\settowidth{\WRCdotTfRRplusdsbisbplusdsbB}{\usebox{\WRCdotTfRRplusdsbisbplusdsbA}}
\newsavebox{\WRCdotTfRRplusdsbisbplusdsbC}
\begin{lrbox}{\WRCdotTfRRplusdsbisbplusdsbC}
\begin{minipage}{\WRCdotTfRRplusdsbisbplusdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TfRR+dsb-isb+dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTfRRplusdsbisbplusdsbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTfRRplusdsbisbplusdsbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTfRRplusdsbisbplusdsbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdsbisbplusdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdsbisbplusdsbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdsbisbplusdsbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdsbisbplusdsbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & ~2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/WRC.TfRR+dsbs.tex <==
\newlength{\WRCdotTfRRplusdsbsH}
\setlength{\WRCdotTfRRplusdsbsH}{0cm}
\newsavebox{\WRCdotTfRRplusdsbsI}
\begin{lrbox}{\WRCdotTfRRplusdsbsI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbsJ}
\settowidth{\WRCdotTfRRplusdsbsJ}{\usebox{\WRCdotTfRRplusdsbsI}}
\addtolength{\WRCdotTfRRplusdsbsH}{\WRCdotTfRRplusdsbsJ}
\newsavebox{\WRCdotTfRRplusdsbsK}
\begin{lrbox}{\WRCdotTfRRplusdsbsK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbsL}
\settowidth{\WRCdotTfRRplusdsbsL}{\usebox{\WRCdotTfRRplusdsbsK}}
\addtolength{\WRCdotTfRRplusdsbsH}{\WRCdotTfRRplusdsbsL}
\newsavebox{\WRCdotTfRRplusdsbsM}
\begin{lrbox}{\WRCdotTfRRplusdsbsM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbsN}
\settowidth{\WRCdotTfRRplusdsbsN}{\usebox{\WRCdotTfRRplusdsbsM}}
\addtolength{\WRCdotTfRRplusdsbsH}{\WRCdotTfRRplusdsbsN}
\newsavebox{\WRCdotTfRRplusdsbsO}
\begin{lrbox}{\WRCdotTfRRplusdsbsO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbsP}
\settowidth{\WRCdotTfRRplusdsbsP}{\usebox{\WRCdotTfRRplusdsbsO}}
\addtolength{\WRCdotTfRRplusdsbsH}{\WRCdotTfRRplusdsbsP}
\newsavebox{\WRCdotTfRRplusdsbsA}
\begin{lrbox}{\WRCdotTfRRplusdsbsA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    *pa1 = 0;

    y |-> pa2;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusdsbsB}
\settowidth{\WRCdotTfRRplusdsbsB}{\usebox{\WRCdotTfRRplusdsbsA}}
\newsavebox{\WRCdotTfRRplusdsbsC}
\begin{lrbox}{\WRCdotTfRRplusdsbsC}
\begin{minipage}{\WRCdotTfRRplusdsbsH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TfRR+dsbs|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTfRRplusdsbsB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTfRRplusdsbsA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTfRRplusdsbsC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdsbsI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdsbsK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdsbsM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusdsbsO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & ~2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/WRC.TfRR+po+dsb.tex <==
\newlength{\WRCdotTfRRpluspoplusdsbH}
\setlength{\WRCdotTfRRpluspoplusdsbH}{0cm}
\newsavebox{\WRCdotTfRRpluspoplusdsbI}
\begin{lrbox}{\WRCdotTfRRpluspoplusdsbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRpluspoplusdsbJ}
\settowidth{\WRCdotTfRRpluspoplusdsbJ}{\usebox{\WRCdotTfRRpluspoplusdsbI}}
\addtolength{\WRCdotTfRRpluspoplusdsbH}{\WRCdotTfRRpluspoplusdsbJ}
\newsavebox{\WRCdotTfRRpluspoplusdsbK}
\begin{lrbox}{\WRCdotTfRRpluspoplusdsbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRpluspoplusdsbL}
\settowidth{\WRCdotTfRRpluspoplusdsbL}{\usebox{\WRCdotTfRRpluspoplusdsbK}}
\addtolength{\WRCdotTfRRpluspoplusdsbH}{\WRCdotTfRRpluspoplusdsbL}
\newsavebox{\WRCdotTfRRpluspoplusdsbM}
\begin{lrbox}{\WRCdotTfRRpluspoplusdsbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRpluspoplusdsbN}
\settowidth{\WRCdotTfRRpluspoplusdsbN}{\usebox{\WRCdotTfRRpluspoplusdsbM}}
\addtolength{\WRCdotTfRRpluspoplusdsbH}{\WRCdotTfRRpluspoplusdsbN}
\newsavebox{\WRCdotTfRRpluspoplusdsbO}
\begin{lrbox}{\WRCdotTfRRpluspoplusdsbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRpluspoplusdsbP}
\settowidth{\WRCdotTfRRpluspoplusdsbP}{\usebox{\WRCdotTfRRpluspoplusdsbO}}
\addtolength{\WRCdotTfRRpluspoplusdsbH}{\WRCdotTfRRpluspoplusdsbP}
\newsavebox{\WRCdotTfRRpluspoplusdsbA}
\begin{lrbox}{\WRCdotTfRRpluspoplusdsbA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    *pa1 = 0;

    y |-> pa2;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRpluspoplusdsbB}
\settowidth{\WRCdotTfRRpluspoplusdsbB}{\usebox{\WRCdotTfRRpluspoplusdsbA}}
\newsavebox{\WRCdotTfRRpluspoplusdsbC}
\begin{lrbox}{\WRCdotTfRRpluspoplusdsbC}
\begin{minipage}{\WRCdotTfRRpluspoplusdsbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TfRR+po+dsb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTfRRpluspoplusdsbB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTfRRpluspoplusdsbA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTfRRpluspoplusdsbC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRpluspoplusdsbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRpluspoplusdsbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRpluspoplusdsbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRpluspoplusdsbO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & ~2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/WRC.TfRR+pos.tex <==
\newlength{\WRCdotTfRRplusposH}
\setlength{\WRCdotTfRRplusposH}{0cm}
\newsavebox{\WRCdotTfRRplusposI}
\begin{lrbox}{\WRCdotTfRRplusposI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusposJ}
\settowidth{\WRCdotTfRRplusposJ}{\usebox{\WRCdotTfRRplusposI}}
\addtolength{\WRCdotTfRRplusposH}{\WRCdotTfRRplusposJ}
\newsavebox{\WRCdotTfRRplusposK}
\begin{lrbox}{\WRCdotTfRRplusposK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusposL}
\settowidth{\WRCdotTfRRplusposL}{\usebox{\WRCdotTfRRplusposK}}
\addtolength{\WRCdotTfRRplusposH}{\WRCdotTfRRplusposL}
\newsavebox{\WRCdotTfRRplusposM}
\begin{lrbox}{\WRCdotTfRRplusposM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusposN}
\settowidth{\WRCdotTfRRplusposN}{\usebox{\WRCdotTfRRplusposM}}
\addtolength{\WRCdotTfRRplusposH}{\WRCdotTfRRplusposN}
\newsavebox{\WRCdotTfRRplusposO}
\begin{lrbox}{\WRCdotTfRRplusposO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#1
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusposP}
\settowidth{\WRCdotTfRRplusposP}{\usebox{\WRCdotTfRRplusposO}}
\addtolength{\WRCdotTfRRplusposH}{\WRCdotTfRRplusposP}
\newsavebox{\WRCdotTfRRplusposA}
\begin{lrbox}{\WRCdotTfRRplusposA}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;
    x |-> pa1;
    x ?-> invalid;

    *pa1 = 0;

    y |-> pa2;

    identity 0x1000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRRplusposB}
\settowidth{\WRCdotTfRRplusposB}{\usebox{\WRCdotTfRRplusposA}}
\newsavebox{\WRCdotTfRRplusposC}
\begin{lrbox}{\WRCdotTfRRplusposC}
\begin{minipage}{\WRCdotTfRRplusposH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=desc3(z,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=pte3(x,page_table_base)|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TfRR+pos|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTfRRplusposB}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTfRRplusposA}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTfRRplusposC}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusposI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusposK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusposM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRRplusposO}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=1 & 2:R0=1 & ~2:R2=0|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/WRC.TfRT+dsb-tlbiis-dsb+dsb-isb.tex <==
\newlength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbH}
\setlength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbH}{0cm}
\newsavebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbI}
\begin{lrbox}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbJ}
\settowidth{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbJ}{\usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbI}}
\addtolength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbH}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbJ}
\newsavebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbK}
\begin{lrbox}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
// the TLBI is in the handler
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbL}
\settowidth{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbL}{\usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbK}}
\addtolength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbH}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbL}
\newsavebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbM}
\begin{lrbox}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbN}
\settowidth{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbN}{\usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbM}}
\addtolength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbH}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbN}
\newsavebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbO}
\begin{lrbox}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
DSB SY
TLBI VAE1IS,X4
DSB SY
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbP}
\settowidth{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbP}{\usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbO}}
\addtolength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbH}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbP}
\newsavebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbA}
\begin{lrbox}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbB}
\settowidth{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbB}{\usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbA}}
\addtolength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbH}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbB}
\newsavebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbC}
\begin{lrbox}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;

    x |-> pa1;
    x ?-> invalid;
    *pa1 = 1;

    y |-> pa2;
    *pa2 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbD}
\settowidth{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbD}{\usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbC}}
\newsavebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbE}
\begin{lrbox}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbE}
\begin{minipage}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:R4=page(x)|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TfRT+dsb-tlbiis-dsb+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbO}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTplusdsbtlbiisdsbplusdsbisbA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=0 & 2:R0=1 & 2:R2=1|\\
  \hline
\end{tabular}


==> vmsa-test-index/tests/tex/WRC.TfRT+po+dsb-isb.tex <==
\newlength{\WRCdotTfRTpluspoplusdsbisbH}
\setlength{\WRCdotTfRTpluspoplusdsbisbH}{0cm}
\newsavebox{\WRCdotTfRTpluspoplusdsbisbI}
\begin{lrbox}{\WRCdotTfRTpluspoplusdsbisbI}
\begin{lstlisting}[language=AArch64,showlines=true]
STR X0,[X1]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTpluspoplusdsbisbJ}
\settowidth{\WRCdotTfRTpluspoplusdsbisbJ}{\usebox{\WRCdotTfRTpluspoplusdsbisbI}}
\addtolength{\WRCdotTfRTpluspoplusdsbisbH}{\WRCdotTfRTpluspoplusdsbisbJ}
\newsavebox{\WRCdotTfRTpluspoplusdsbisbK}
\begin{lrbox}{\WRCdotTfRTpluspoplusdsbisbK}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
STR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTpluspoplusdsbisbL}
\settowidth{\WRCdotTfRTpluspoplusdsbisbL}{\usebox{\WRCdotTfRTpluspoplusdsbisbK}}
\addtolength{\WRCdotTfRTpluspoplusdsbisbH}{\WRCdotTfRTpluspoplusdsbisbL}
\newsavebox{\WRCdotTfRTpluspoplusdsbisbM}
\begin{lrbox}{\WRCdotTfRTpluspoplusdsbisbM}
\begin{lstlisting}[language=AArch64,showlines=true]
LDR X0,[X1]
DSB SY
ISB
LDR X2,[X3]
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTpluspoplusdsbisbN}
\settowidth{\WRCdotTfRTpluspoplusdsbisbN}{\usebox{\WRCdotTfRTpluspoplusdsbisbM}}
\addtolength{\WRCdotTfRTpluspoplusdsbisbH}{\WRCdotTfRTpluspoplusdsbisbN}
\newsavebox{\WRCdotTfRTpluspoplusdsbisbO}
\begin{lrbox}{\WRCdotTfRTpluspoplusdsbisbO}
\begin{lstlisting}[language=AArch64,showlines=true]
0x1400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTpluspoplusdsbisbP}
\settowidth{\WRCdotTfRTpluspoplusdsbisbP}{\usebox{\WRCdotTfRTpluspoplusdsbisbO}}
\addtolength{\WRCdotTfRTpluspoplusdsbisbH}{\WRCdotTfRTpluspoplusdsbisbP}
\newsavebox{\WRCdotTfRTpluspoplusdsbisbA}
\begin{lrbox}{\WRCdotTfRTpluspoplusdsbisbA}
\begin{lstlisting}[language=AArch64,showlines=true]
0x2400:
MOV X0,#0
MRS X13,ELR_EL1
ADD X13,X13,#4
MSR ELR_EL1,X13
ERET
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTpluspoplusdsbisbB}
\settowidth{\WRCdotTfRTpluspoplusdsbisbB}{\usebox{\WRCdotTfRTpluspoplusdsbisbA}}
\addtolength{\WRCdotTfRTpluspoplusdsbisbH}{\WRCdotTfRTpluspoplusdsbisbB}
\newsavebox{\WRCdotTfRTpluspoplusdsbisbC}
\begin{lrbox}{\WRCdotTfRTpluspoplusdsbisbC}
\begin{lstlisting}[language=IslaPageTableSetup,showlines=true]
    physical pa1 pa2;

    x |-> pa1;
    x ?-> invalid;
    *pa1 = 1;

    y |-> pa2;
    *pa2 = 0;

    identity 0x1000 with code;
    identity 0x2000 with code;
\end{lstlisting}
\end{lrbox}
\newlength{\WRCdotTfRTpluspoplusdsbisbD}
\settowidth{\WRCdotTfRTpluspoplusdsbisbD}{\usebox{\WRCdotTfRTpluspoplusdsbisbC}}
\newsavebox{\WRCdotTfRTpluspoplusdsbisbE}
\begin{lrbox}{\WRCdotTfRTpluspoplusdsbisbE}
\begin{minipage}{\WRCdotTfRTpluspoplusdsbisbH}
\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Initial state:\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|0:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R0=0b0|\\
\lstinline[language=IslaLitmusExp]|0:R1=pte3(x,page_table_base)|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|1:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|1:R1=x|\\
\lstinline[language=IslaLitmusExp]|1:R2=0b1|\\
\lstinline[language=IslaLitmusExp]|1:R3=y|\\
\lstinline[language=IslaLitmusExp]|1:VBAR_EL1=0x1000|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.EL=0b00|\\
\lstinline[language=IslaLitmusExp]|2:PSTATE.SP=0b0|\\
\lstinline[language=IslaLitmusExp]|2:R1=y|\\
\lstinline[language=IslaLitmusExp]|2:R3=x|\\
\lstinline[language=IslaLitmusExp]|2:VBAR_EL1=0x2000|\\
\end{minipage}
\end{lrbox}
\begin{tabular}{|l|l|}
  \multicolumn{2}{l}{\textbf{AArch64} \lstinline[language=IslaLitmusName]|WRC.TfRT+po+dsb-isb|}\\
  \hline
  \multirow{6}{*}{\begin{minipage}{\WRCdotTfRTpluspoplusdsbisbD}\vphantom{$\vcenter{\hbox{\rule{0pt}{1.8em}}}$}Page table setup:\\\usebox{\WRCdotTfRTpluspoplusdsbisbC}\end{minipage}} & \cellcolor{IslaInitialState}{\usebox{\WRCdotTfRTpluspoplusdsbisbE}}\\
  \cline{2-2}
  & Thread 0\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTpluspoplusdsbisbI}\\
  \cline{2-2}
  & Thread 1\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTpluspoplusdsbisbK}\\
  \cline{2-2}
  & Thread 2\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTpluspoplusdsbisbM}\\
  \cline{2-2}
  & thread1 el1 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTpluspoplusdsbisbO}\\
  \cline{2-2}
  & thread1 el2 handler\\
  \cline{2-2}
  & \usebox{\WRCdotTfRTpluspoplusdsbisbA}\\
  \cline{2-2}
  & Final state: \lstinline[language=IslaLitmusExp]|1:R0=0 & 2:R0=1 & 2:R2=1|\\
  \hline
\end{tabular}

